Programs as Diagrams: From Categorical Computability to Computable Categories

This is a draft of the textbook/monograph that presents computability theory using string diagrams. The introductory chapters have been taught as graduate and undergraduate courses and evolved through 8 years of lecture notes. The later chapters contain new ideas and results about categorical computability and some first steps into computable category theory. The underlying categorical view of computation is based on monoidal categories with program evaluators, called *monoidal computers*. This categorical structure can be viewed as a single-instruction diagrammatic programming language called Run, whose only instruction is called RUN. This version: improved text, moved the final chapter to the next volume. (The final version will continue lots of exercises and workouts, but already this version has severely degraded graphics to meet the size bounds.)

==> 21-COMPUT/28-comput-work.tex <==
% !TEX root = ../000-monc.tex

\subsection[How many programs?]{How many programs?}\label{Sec:how-many}
Is there a computer with 3 programs? No. There are either infinitely many, or there is just one and $\true = \flse$. We first discharge this trivial case, and then as soon as $\true\neq \flse$, there must be infinitely many different programs for each computation. 

\begin{enumerate}[a.]
\item Consider a monoidal computer $\CCC$ where $\true = \flse$. In other words, suppose that the programs for $\true$ and $\flse$ chosen in \eqref{eq:truth} turn out to be equal. Prove the following claims. 
\begin{enumerate}[i)]
\item\label{work:phi-gamma} Any pair of \funnn s $\varphi, \gamma : \DP\to \DP$ in $\CCC$ satisfy $\varphi = \gamma$.


\item\label{work:fg}  Any pair of \funnn s $f,g: A\to B$ in $\CCC$ satisfy $f=g$.

\item\label{work:CD} For any pair of types $C,D $ in $\CCC$ there is an isomorphism $C\cong D$ (i.e. a pair of \funnn s $\begin{tikzar}{}
C \ar[bend right=20]{r}[swap]{d} \& D \ar[bend right=20]{l}[swap]{c}
\end{tikzar}$ such that $c\circ d = \id_C$ and $d\circ c = \id_D$).

\item Conclude that any monoidal computer $\CCC$ with $\true =\flse$ is equivalent with the trivial category consisting of a single object and a single morphism.
\end{enumerate}

\item\label{Prop:infi-prog} Consider a monoidal computer $\CCC$ where $\true \neq \flse$. Prove that the following claims are valid for any number $n$. 
\begin{enumerate}[i)]
\item The programming language $\DP$ in $\CCC$ contains at least $2^{n}$ different programs.

\item For any \funnn\ $f:A\to B$ there are at least $2^{n}$ different programs $F:\DP$ such that $f = \uev F$.
\end{enumerate}

Conclude that any monoidal computer $\CCC$ where $\true \neq \flse$ contains infinitely many programs, and that any computable  \funnn\ $f:A\to B$ can be encoded by infinitely many different programs $F:\DP$ that evaluate to $f=\uev F$.

\item Explain that in a monoidal computer $\CCC$, 
\begin{itemize}
\item either every indexed \funnn\  $g\in \CCC(X\times A, B)$ has infinitely many programs $G\in\tot\CCC(X,\DP)$ with $g = \uev G$, 
\item or $\CCC\simeq 1$.
\end{itemize}
\end{enumerate}

\subsection{Counting by evaluating: Church numerals} \label{Sec:churchnum}
The simplest form of computation is counting. The simplest programs that can be derived from program evaluators are the numbers, counting how many times a program is evaluated over its inputs. The idea is to redefine the numbers internally in a computer as  the programs $\overline 0, \overline 1, \overline 2\ldots$ such that
\bea\label{eq:churchnum}
\uev{\overline 0}(F,a) & = &  \uev F ^{0} a\ \ =\ \ a \notag \\
\uev{\overline 1}(F,a) & = & \uev F ^{1} a\ \ =\ \ \uev F a\notag\\
\uev{\overline 2}(F,a) & = & \uev F ^{2} a\ \ =\ \ \uev F\circ \uev F a \notag\\
\uev{\overline 3}(F,a) & = & \uev F ^{3} a\ \ =\ \ \uev F\circ \uev F\circ \uev F a \notag\\
&\cdots\notag\\
\uev{\overline n}(F,a) & = & \uev F ^{n} a\ \ =\ \ \underbrace{\uev F\circ\cdots \circ \uev F\circ \uev F}_{n\  \mbox{\scriptsize times}} a %\notag\\
%n+1 & = & \{0,1,2,\ldots, n-1,n\}
\eea 
The overlined $\overline n$ is thus a number-as-program, internal in a computer, whereas $n$ is the usual, "external" number. When the distinction is irrelevant, we identify them. The string-diagrammatic view of the internal numbers is in Fig.~\ref{Fig:Church-num}.
\begin{figure}[!ht]
\newcommand{\zzero}{\scriptstyle \overline 0}
\newcommand{\oone}{\scriptstyle \overline 1}
\newcommand{\ttwo}{\scriptstyle \overline 2}
\newcommand{\tthree}{\scriptstyle \overline 3}
\def\JPicScale{.4}
\begin{center}
\input{PIC/numbers-0.tex}
\caption{Church's numerals (without the $\lambda$-abstractions)}
\label{Fig:Church-num}
\end{center}
\end{figure}

\para{Remark.} The task of redefining numbers as programs is a first step into \emph{reverse programming}, explained in Sec.~\ref{Sec:CTT}. The programs in Fig.~\ref{Fig:Church-num} follow Church's idea from \cite{ChurchA:calculi}. % Applying the $\lambda$-abstractions Church's numbers were fixed $\lambda$-terms, here we choose and fix a program for each number.

\para{Exercises.} Specify programs to implement the following arithmetic operations on Church's numerals:
\begin{enumerate}[a.]
\item $\suce(\overline n) = \overline{n+1}$
\item $\addd(\overline m, \overline n) = \overline{m+n}$
\item $\mult(\overline m, \overline n) = \overline{m\times n}$
%\item $\eee(\overline m, \overline n) = \overline{n^{m}}$
% For simple exponentiation, we need a different definition of the numerals: 0 is the 3rd projectin and n is the number of partial evaluations of the first argument on the second one. Diagrams start from p. 69 of slides for 4. Software and metaprogramming from ICS 222 for 2017. 
\end{enumerate}


\subsection{Monoid computer?}\label{Sec:uniform}\sindex{evaluator!uniform} 
In Sec.~\ref{Sec:retracts}, we saw that any type $A$ of a monoidal computer comes with a retraction $\begin{tikzar}{}
A \ar[tail,bend right=15]{r}[swap]{\incl} \& \DP \ar[two heads,bend right=15]{l}[swap]{\retr}
\end{tikzar}$ and can be identified with the induced  idempotent $\rho=\incl\circ\retr$ on $\DP$. The question arises: 
\begin{quote}
\emph{\textbf{Can all structure of a monoidal computer $\CCC$ be reduced to its programming language $\DP$?}}
\end{quote}
In this workout, we pursue this question in parts, asking how to reduce the underlying category, its monoidal structure, and the program evaluators of a monoidal computer to the monoid of computable \funnn s on its programming language. Some of the answers require categorical background (see Appendix~\ref{Appendix:cat}) and probably too much work for the first round but they have interesting repercussions, so please come back. The first ones are easy.

\subsubsection{Universal program evaluator $\universal\colon\DP\times\DP\longrightarrow \DP$}
\label{work:uni-eval}\sindex{evaluator!universal}
Prove the following claims:
\begin{enumerate}[a.]
\item\label{work:uniform-op} 
Any program evaluator $\universal_\DP^\DP$ induces the program evaluators $\universal_A^B$ as the following composites
\beq\label{uniform-op}
\begin{split}
\newcommand{\program}{$\upsilon_A^B$}
\newcommand{\Progtype}{\scriptstyle \DP}
\newcommand{\Progk}{\scriptstyle B}
\newcommand{\Progn}{\scriptstyle A}
\renewcommand{\universal}{\Big\{\Big\}^\DP_\DP}
\newcommand{\decok}{\retr}
\newcommand{\encon}{\incl}
\def\JPicScale{.6}
\input{PIC/uniform-op.tex}
\end{split}
\eeq
for all types $A,B$. Prove that the composite \eqref{uniform-op} satisfies condition (\ref{eq:uev}--\ref{eq:uev-formal}).

\item  \label{work:uni-idem} Any program evaluator $\universal_{A}^{B}$ can be reduced to $\universal_{\DP}^{\DP}$ using a program transformer $\upsilon_A^B$ and the type projections and embeddings, in the following form
\beq\label{uni-idem}
\begin{split}
\newcommand{\program}{$\upsilon_A^B$}
\newcommand{\Progtype}{\scriptstyle \DP}
\newcommand{\Progk}{\scriptstyle B}
\newcommand{\Progn}{\scriptstyle A}
%\newcommand{\lasrevinu}{\big\{\big\}^B_A}
\renewcommand{\universal}{\Big\{\Big\}^\DP_\DP}
\newcommand{\decok}{\retr}
\newcommand{\encon}{\incl}
\newcommand{\eqlsb}{\Large =}
\def\JPicScale{.6}
\input{PIC/uni-idem.tex}
\end{split}
\eeq
\end{enumerate}

\subsubsection{$\CCC$ is the idempotent completion of its submonoid on $\DP$}
\label{work:monoid-completion}\label{work:abs-com}
Let $\PPP\times \PPP\tto \circ \PPP\oot{\id_\DP} 1$ be a monoid, viewed as a category with a single object, call it $\DP$. Its \emph{idempotent completion}\/ is defined to be the following category
\sindex{category!of idempotents}
\bea
\lvert\, \Kar\PPP\,\rvert & = & \left\{\varrho \in \PPP\ |\ \varrho\circ \varrho = \varrho
\right\}\notag\\
\Kar\PPP(\varrho, \varsigma) & = & \left\{\varphi\in \PPP\ |\ \varsigma\circ \varphi = \varphi = \varphi\circ \varrho\right\}\label{eq:abscom}
\eea
See Appendix~\ref{Appendix:idemp} for more about this construction. It comes with the embedding 
\beq\label{eq:flat}
\flat \colon \PPP \mono \Kar\PPP
\eeq 
which maps $\DP$, the sole object of $\PPP$, to the unit $\id$ as an idempotent, and any element $\varphi$ of $\PPP$ to itself, as an endomorphism on the idempotent $\id$.

Prove the following claims.

\begin{enumerate}[a.]
\item Let $\CCC$ be a category where all idempotents split (as in Appendix~\ref{Appendix:idemp}). Then any functor $F:\PPP\to \CCC$ has a unique extension $F^\sharp :\Kar \PPP\to \CCC$, making the following diagram commute
\beq
\begin{split}
\begin{tikzar}{}
\PPP \ar[tail,bend left=15]{rr}{\flat} \ar{dr}[description]{F} \&\& \Kar\PPP\ar{dl}[description]{F^\sharp}\\
\& \CCC
\end{tikzar}
\end{split}
\eeq
%The embedding $\flat :\PPP \mono \Kar\PPP$ thus induces a one-to-one correspondence between the functor categories $\CCC^\PPP \simeq \CCC^{\Kar\PPP}$ for any category where the idempotents split. $\Kar\PPP$ is thus the completion of $\PPP$


\item\label{work:rho} Given an object $\DP$ of $\CCC$, consider the monoid $\PPP = \CCC(\DP,\DP)$ as a full subcategory of $\CCC$. Show that the embedding $\flat \colon \PPP \mono \Kar\PPP$ from \eqref{eq:flat} extends along the subcategory inclusion $\PPP\inclusion \CCC$ to a functor $\rho\colon \CCC\to \Kar\PPP$, making the following diagram commute
\beq
\begin{split}
\begin{tikzar}{}
\PPP \ar[hook',bend left=15]{rr} \ar[tail]{dr}[description]{\flat} \&\& \CCC\ar{dl}[description]{\rho}\\
\& \Kar\PPP
\end{tikzar}
\end{split}
\eeq
if and only if every object $A\in \lvert\CCC\rvert$ is a retract of $\DP$. Verify moreover that $\rho$ is full and faithful (i.e., that it establishes a bijection $\CCC(A,B)\cong\Kar(\rho_A,\rho_B)$ for all pairs $A, B$) and that it is determined by $\PPP\inclusion \CCC$ up to isomorphism.


\item\label{work:compltn} Let $\CCC$ be a category where every object $A$ is a retract of $\DP$ and all idempotents split. Then the functor $\rho$ is an equivalence of categories \sindex{equivalence of categories} with a mate $\widehat{(-)}$
\beq\label{eq:equiv-rho}
\begin{tikzar}[column sep = 5em]
\CCC \ar[bend right=15]{r}[swap]{\rho} \ar[phantom]{r}[description]{\simeq}\& \Kar\PPP \ar[bend right=15]{l}[swap]{\widehat{(-)}}
\end{tikzar}
\eeq
and there are isomorphisms $\widehat{\rho_A} \cong A$ in $\CCC$ and $\rho_{\widehat\varrho} \cong \varrho$ in $\Kar \PPP$, natural in $A$ and $\varrho$. 

\item The equivalence $\rho\colon\CCC\to \Kar\PPP$  induces a bijection $\CCC(\DP,\DP)\cong \Kar\PPP(\rho_\DP,\rho_\DP)$. Show that this implies that $\rho_\DP$ must be invertible, and furthermore that the components of the splitting $\rho_\DP=\big(\DP\eepi{\retr}\widehat{\rho_\DP}\mmono{\incl}\DP\big)$ must also be invertible. 
\end{enumerate}


\para{Summary.} The functor $\rho$ selects for every type $A\in\lvert\CCC\rvert$ an idempotent 
\bea\label{eq:rho}
\rho_A & = & \left(\DP\eepi{\retr}A\mmono\incl \DP\right)
\eea 
The mate $\widehat{(-)}$ selects for every idempotent $\varrho\in \CCC(\DP,\DP)$ a splitting  
\bea\label{eq:varrho}
\left(\DP\eepi{\retr}\widehat \varrho \mmono\incl \DP\right) & = & \varrho
\eea
The equivalence functors thus assign to every $A\in \CCC$ a particular program encoding \eqref{eq:rho}, and to every idempotent $\varrho\in \Kar\PPP$ a particular splitting \eqref{eq:varrho}.



\subsubsection{Relating the products in $\CCC$ and the pairing on $\DP$} \label{work:monoidal}
Any equivalence of categories $\XXX\simeq \YYY$ allows transferring a given monoidal structure from $\XXX$ to $\YYY$. Continuing with the category $\CCC$ and its submonoid $\PPP$ from \ref{work:abs-com}, it may be instructive to first work out this general structure transfer for the special case of the monoidal structure $(\CCC,\times,I)$ and transfer it along the equivalence $\CCC \simeq \Kar\PPP$. But going further, in this special case at hand, the monoidal structure of $\CCC$ is also reflected on its submonoid $\PPP$ in terms of the retractions
\beq\label{eq:retraction-prod}
 \rho_{\DP\times \DP} = \left(\DP\begin{tikzar}[column sep=4em]\hspace{-.3em}\arrow[two heads]{r}{\left<\fstt -, \sndd -\right>}\&\hspace{-.2em}\end{tikzar}\DP\times \DP \begin{tikzar}[column sep=3.5em]\hspace{-.3em}\arrow[tail]{r}{\pairr - -}\&\hspace{-.2em}\end{tikzar} \DP\right) \qquad\qquad\qquad\qquad  \rho_I = \left(\DP\eepi{\scun} I \mmono{\nultuple} \DP\right) \eeq
It is interesting, and can be subtle, to express the monoidal structure of $\Kar\PPP$ in terms of these retractions.

\begin{enumerate}[a.]
\item Mapping any pair $\varrho, \varsigma \in \lvert \Kar\PPP\rvert$ along the equivalence in  to $\widehat \varrho, \widehat \varsigma \in \lvert \CCC\rvert$, and then their product $\widehat\varrho \times \widehat \varsigma$ back to $\Kar\PPP$ gives 
\bea\label{eq:otimes}
\varrho \otimes \varsigma & = & \rho_{\widehat \varrho \times \widehat \varsigma} 
\eea
Verify that this defines a functor $\otimes \colon \Kar \PPP\times \Kar \PPP \to \Kar \PPP$ and that $(\Kar\PPP,\otimes\, ,\rho_I)$ is a monoidal category.

\item Work out the data services in $\Kar\PPP$ induced by the data services in $\CCC$.

\begin{figure}[!ht]
\newcommand{\pairrrr}{\pairr - -}
\newcommand{\projjj}{\scriptstyle\left<\fstt -, \sndd - \right>}
\newcommand{\varrhoo}{\varphi}
\newcommand{\varsigmaa}{\psi}
\def\JPicScale{.5}
\begin{center}
\input{PIC/convolution.tex}
\caption{The convolution $\left(\varphi\star\psi\right)x \ =\ \pairr{\varphi\fstt x}{\psi\sndd x}$}
\label{Fig:convolution}
\end{center}
\end{figure}

\item\label{item:nondeg} The pairing in \eqref{eq:retraction-prod} determines a \emph{convolution}\/ operation $(\star)\colon \PPP \times \PPP\to \PPP$ displayed in Fig.~\ref{Fig:convolution}. Prove the following claims.

\begin{enumerate}[i)]
\item $\varphi\star\psi$ is idempotent whenever $\varphi$ and $\psi$ are idempotent.
\item $\varrho\star\varsigma\  \cong\  \varrho \otimes \varsigma$ holds for all idempotents $\varrho, \varsigma$ on $\DP$.
\item There are monoidal equivalences $(\Kar\PPP,\, (\star)\, ,  \rho_I) \  \simeq \  (\Kar\PPP,\, \otimes\, , \rho_I)\  \simeq \  (\CCC\, ,\times\, , I)$
\end{enumerate}


\item\label{item:yesdeg} Suppose that the operation $(\star)\colon \PPP \times \PPP\to \PPP$ is associative and has a unit $\nultuple$, which yields a monoidal structure $(\PPP, \star,\rho_I)$ making the monoid $(\PPP,\circ,\id_\DP)$ into a monoidal category. Note that this means that $\star$ and $\circ$ satisfy the middle-two-interchange law from Sec.~\ref{Sec:godement}\sindex{middle-two-interchange}. Show that the two monoidal structures must coincide, with $\varphi\star \psi = \varphi\circ \psi$ and  $\rho_I = \id_\DP$ and leading to $I\cong \DP$ and reducing the category $\CCC$ to a commutative monoid. 

\item In summary, for any monoidal category $\CCC$ where all objects are retracts of a single object $\DP$ and for the submonoid $\PPP = \CCC(\DP,\DP)$, we so far proved that 
\begin{itemize}
\item[(\ref{item:nondeg}.)] the operation $(\star)$ is  associative and unitary on $\Kar\PPP$, but 
\item[(\ref{item:yesdeg}.)] if the operation $(\star)$  is associative and unitary on $\PPP$, then $\DP\cong I$. 
\end{itemize}
Does it follow that every monoidal category where all objects are retracts of a single object must collapse to a commutative monoid? Explain!
\end{enumerate}

\para{Lookahead.} In Sec.~\ref{Work:assoc-pair}, we will work out a pairing operation $\pairr - -\colon \DP\times \DP \mono \DP$ (with projections) which is associative up to isomorphism in $\PPP$, and has a one-sided unit. %It can be constructed in any monoidal computer with well-ordered programs. 

\subsubsection{Reducing program evaluators $\universal_A^B$ to $\universal_\DP^\DP$}
\label{work:uniform}
Sec.~\ref{work:abs-com} reduced the underlying category of a monoidal computer $\CCC$ to its submonoid $\PPP$ on $\DP$. Sec.~\ref{work:monoidal} reduced $\CCC$'s monoidal structure and data services to the pairing operation on $\DP$. Up to equivalence, the monoidal category $\CCC$ underlying a monoidal computer can be recovered from its submonoid $\PPP$ on $\DP$. Can the program evaluators be reduced in a similar way? 

Sec.~\ref{work:uni-eval} made some first steps towards an answer. Claim~\ref{work:uni-idem} was that general program evaluators $\universal_A^B$ in $\Kar\PPP$ can be derived from $\universal_\DP^\DP$ using the type retractions and program transformers $\upsilon^B_A$. Claim~\ref{work:uniform-op} was that a special family of program evaluators $\universal_A^B$ in $\Kar\PPP$ can be derived from $\universal_\DP^\DP$  even without the program transformers, i.e. assuming that $\upsilon^B_A=\id$. We work out the special properties of this special family  of program evaluators.


\begin{enumerate}[a.]
\item Let $(\PPP,\circ,\DP)$ be a monoid such that its idemputent completion $(\Kar\PPP,\, (\star)\, ,  I)$ is a monoidal category  with data services. For 
\begin{enumerate}[i)]
\item a morphism $\universal \in \Kar\PPP(\DP\star \DP, \DP)$ and 
\item a family $\{\upsilon_\varrho^\varsigma\}_{\varrho, \varsigma \in \Kar\PPP}$, 
\end{enumerate}
spell out the suitable versions of condition \eqref{eq:uev-formal} which makes
\bear
\uev{-}_\varrho^\varsigma  & = &  \varsigma\circ \uev{\upsilon_\varrho^\varsigma(-)}\circ\varrho
\eear
displayed in \eqref{uni-idem}, into a $\varrho\varsigma$-indexed family of program evaluators,  and $\Kar \PPP$ into a monoidal computer.


\item\label{work:def-uniform} \sindex{uniform monoidal computer}\sindex{monoidal!computer!uniform} We call a monoidal computer $\CCC\simeq \Kar\PPP$ \emph{uniform}\/ if in (ii) above, all $\upsilon_\varrho^\varsigma$ are identities and the $\varrho\varsigma$-program evaluators are in the form
\bear
\universal_\varrho^\varsigma  & = &  \varsigma\circ \universal\circ\varrho
\eear
as displayed in \eqref{uniform-op}. In this part we work out the special properties of uniform monoidal computers.

\begin{enumerate}[i)]
\item If $\CCC$ a uniform monoidal computer, then the idempotents $\rho_A$ and their splittings  $\big(\DP\eepi\retr A\mmono\incl\DP\big)$, both selected by the equivalence $\CCC\simeq \Kar\PPP$, interact with the partial evaluations. Prove that the encodings satisfy the following equations
\begin{align*}
\incl_{A\times B} & = \incl_{\DP\times \DP}\circ \big(\incl_{A}\times \incl_{B}\big)
&\incl_{\DP} &= \id_{\DP}\\
\incl_{\DP\times \DP\times \DP} &= \incl_{\DP\times \DP}\circ \big(\incl_{\DP\times \DP}\times \id_{\DP}\big) &
\incl_{\DP\times \DP}\circ\big(\incl_{I}\times \id_{\DP}\big) & = \id_{\DP}
\end{align*}
\item Conclude that $\retr^\DP = \id_\DP$ and that definig $\retr^A = \universal_I^A$, like we did in  Sec.~\ref{Sec:retracts}, implies $\universal_A^\DP = \prtial_A$. We well see in Sec.~\ref{Sec:divergence} that this is impossible, unless the computer is degenerate, because there are $F,a$ for which $\uev F_A^\DP a$ cannot be assigned a value whereas $\pev F_A$ is required to be total. 



%
%\item Show that instantiating  \eqref{eq:uni-idem} to $A= B=\DP$ defines a universal evaluator if and only if the retraction $\begin{tikzar}{}
%\DP \ar[tail,bend right=20]{r}[swap]{\incl} \& \DP \ar[two heads,bend right]{l}[swap]{\retr}
%\end{tikzar}$ is invertible. Since $\incl = \enco{-}$ and $\retr = \universal$, this means that in addition to $\uev{\enco{p}} = p$, the equation $\enco{\uev{p}} = p$ must also hold, and that there is thus a single program for every  computation.
\end{enumerate}

\end{enumerate}
%
%
%\para{Monoid computer.} A monoidal computer $\CCC$ is a \emph{monoid computer}\/ if all of its program evaluators $\universal_{A}^{B}$ are derived from $\universal_{\DP}^{\DP}$ as in \eqref{uniform-op} and thus satisfy
%\bea\label{eq:uni-idem-AB}
%\universal_{A}^{B} & = & \left(\DP\times A \mmono{\DP\times \incl_{A}}\DP\times \DP\tto{\hspace{.5em}\universal_{\DP}^{\DP}\hspace{.5em}} \DP\stackrel{\retr^B}\twoheadrightarrow B
%\right)
%\eea
%The program evaluators of the monoid computer $\CCC$ are uniformly determined by its submonoid $\PPP$ and transferred along the equivalence $\Kar\PPP\simeq \CCC$. We call the program evaluators \emph{uniform}\/ \sindex{evaluator!uniform} when they satisfy \eqref{eq:uni-idem-AB}. The uniform evaluators in a monoid computer thus evaluate all programs as computations of type $\DP\to\DP$ and project them to the type $A\to B$ by restricting the inputs to the type $A$ and projecting the outputs to the type $B$. Such computers turn out to be of a very special kind, assigning canonical programs to some computations.
%
%
%
%
%\subsubsection{Monoidal uniformity}\label{work:prods}
%\sindex{uniform monoidal computer}
%\para{Computational monoids.} Let $\MMM$ be a monoidal category with data services. A monoid of endomorphisms $\MMM(P,P)$ of a fixed type $P$ is called \emph{computational} if $P$ comes with the following structure:
%\begin{enumerate}[(1)]
%\item pairing monoid $P\times P\tto{\pairr - -} P \oot{\nultuple} I$ which induces the tupling operations
%\[\pairr{\pairr x y} {z} = \pairrr{x,y,z} = \pairr {x} {\pairr{y}{z}} \qquad \qquad\qquad\qquad \pairr{x}{\nultuple} = x = \pairr{\nultuple}{x}
%\]
%\item projections $\fstt -, \sndd -\colon P\to P$ satisfying
%\[\fstt{\pairr x y} =  x\qquad\qquad\qquad\qquad \sndd{\pairr x y} = y\]
%from which all projections $\nnth{\pairrr{x_{0},\ldots,x_{n}}}{k} = x_{k}$ are derived;
%\item universal evaluator $\universal\colon P\times P\to P$ such that for every $f\colon P\to P$ there is $F\colon I\stricto P$ such that
%\bear
%f & = & \uev F
%\eear
%\item partial evaluator $\prtial\colon P\times P \stricto P$ such that
%\bear
%\uev{F}{\pairr x y} & = & \uev{\pev{F} x} y
%\eear
%\end{enumerate}
%
%\para{Partial combinatory algebras.} A partial combinatory algebra is a type $P$ with
%\begin{itemize}
%\item a partial binary operation $(\cdot )\colon P\times P\to P$, usually elided so that $x\cdot y$ is written $xy$, and grouped to the left so that $xyz$ means $(xy)z$; and moreover
%\item distinguished elements $K,S\in P$ satisfying
%\[Kxy = x\qquad\qquad\qquad Sxy\!\downarrow \qquad\qquad\qquad Sxyz = xz(yz)\]
%where the equalities are strong, in the sense that each side has a value if and only if the other side does.
%\end{itemize}
%
%\para{Prove the following claims:}
%
%\begin{enumerate}[a.]
%\item Every computational monoid in the category of sets and partial functions is a partial combinatory algebra with $xy = \uev x y$.
%
%\item Every partial combinatory algebra in a monoidal computer is a computational monoid with $f\circ g = \lambda x.\ f(g(x))$.
%
%\item Every uniform monoidal computer contains a computational monoid. In particular, in any uniform monoidal computer, for any pair of types $A,B$, the encodings $\incl$ satisfy the following equations:
%\begin{align*}
%\incl_{A\times B} & = \incl_{\DP\times \DP}\circ \big(\incl_{A}\times \incl_{B}\big)
%&\incl_{\DP} &= \id_{\DP}\\
%\incl_{\DP\times \DP\times \DP} &= \incl_{\DP\times \DP}\circ \big(\incl_{\DP\times \DP}\times \id_{\DP}\big) &
%\incl_{\DP\times \DP}\circ\big(\incl_{I}\times \id_{\DP}\big) & = \id_{\DP}
%\end{align*}
%%\begin{enumerate}[i)]
%%\item $\incl_{A\times B} = \incl_{\DP\times \DP}\circ \big(\incl_{A}\times \incl_{B}\big)$
%%\item $\incl_{\DP} = \id_{\DP}$
%%\item $\incl_{\DP\times \DP\times \DP} = \incl_{\DP\times \DP}\circ \big(\incl_{\DP\times \DP}\times \id_{\DP}\big)$
%%\item $\incl_{\DP\times \DP}\circ\big(\incl_{I}\times \id_{\DP}\big) = \id_{\DP}$
%%\end{enumerate}
%Derive that conditions (1--4) from the definition of computational monoids are satisfied by
%\begin{align*}
%\pairr {-}{-}  &= \incl_{\DP\times \DP}& \fstt - &= \retr^{\DP\times \DP}\circ(\id_{\DP}\, \times\,  \cun\,)  \\
%\nultuple &= \incl_{I} & \sndd - &= \retr^{\DP\times \DP}\circ(\cun\, \times\,  \id_{\DP})
%\end{align*}
%
%\item Every computational monoid $P$ in a category $\MMM$ gives rise to a uniform monoidal computer $\UUu$ defined as follows:
%\bea
%\lvert\UUu\rvert& = & \{\rho \in \MMM(P,P)\ |\ \rho\circ\rho = \rho\}\\
%\UUu(\rho,\varsigma) & = & \{f\in \MMM(P,P) \ |\ \varsigma\circ f \circ \rho = f\}\notag
%\eea
%Claims:
%\begin{enumerate}[i)]
%\item The computational monoid structure (1--2) induces the retraction $P\times P\hspace{-1ex}\begin{tikzar}[row sep=1.5cm]
%\hspace{1ex} \ar[tail,bend right=15]{r}[swap]{\incl_{P\times P}} \& \hspace{1ex} \ar[two heads,bend right=15]{l}[swap]{\retr^{P\times P}}
%\end{tikzar}\hspace{-1ex}  P$ by
%\[\incl_{P\times P} =\left(P\times P\tto{\pairr - - } P\right)\qquad \qquad \retr^{P\times P} = \left(P\ttoams{\Big<\fstt -, \sndd -\Big>} P\times P\right)\]
%\item The operations $\UUu\times \UUu\tto\otimes \UUu\oot I 1$ defined
%\beq\label{eq:convol}
%\left(\rho \otimes \varsigma\right) (z)\  =\  \pairr{\rho\left(\fstt z\right)}{\varsigma\left(\sndd z\right)}\qquad\qquad\qquad \qquad I\  =\  \nultuple\circ \cun
%\eeq
%make $\UUu$ into a monoidal category with data services. In the notation of a., the former can be written more succinctly as $\rho \otimes \varsigma \ = \ \incl_{P\times P}\circ(\rho \times \varsigma)\circ \retr^{P\times P}$.
%
%\item The objects $\rho$ of $\UUu$ come with retractions $\rho\hspace{-1ex}\begin{tikzar}[row sep=1.5cm]
%\hspace{1ex} \ar[tail,bend right=15]{r}[swap]{\incl_{\rho}} \& \hspace{1ex} \ar[two heads,bend right=15]{l}[swap]{\retr^{\rho}}
%\end{tikzar}\hspace{-1ex}  \id_{P}$ which are coherent with respect to the monoidal structure in the sense that
%\[
%\incl_{\rho\otimes \varsigma} = \pairr{\incl_{\rho}}{\incl_{\varsigma}}\qquad \qquad\qquad \qquad \incl_{I} = \nultuple
%\]
%
%\item The computational monoid structure (3--4) makes $\UUu$ into a monoidal computer with the program evaluations defined by
%\bea
%\universal_{\rho}^{\varsigma} & = & \left(P\otimes\rho \mmono{P\otimes \incl_{\rho}}P\otimes P\tto{\hspace{.5em}\universal\hspace{.5em}} P\stackrel{\retr^\varsigma}\twoheadrightarrow \varsigma
%\right)
%\eea
%\end{enumerate}
%
%\item%{Uniform monoidal computers are degenerate.} 
%Show that in all computations of type $\DP$ in a uniform monoidal computer must be total, since the program evaluators boil down to partial evaluators: $\uev F x = \pev F x$. The only partial \funnn s are the type decodings.
%\end{enumerate}
%
%
%


==> 21-COMPUT/29-story.tex <==
% !TEX root = ../000-monc.tex

\subsection{Who invented the computer?}\label{Sec:Hilbert} 
The \emph{invention}\/ of the computer as a universal state machine led to the \emph{discovery}\/ of computation as a universal process in nature. The advent of computer engineering had a tremendous impact on the economic expansion in the second half of the XX century. But the advent of computer science opened a new era of science, of our interaction with nature and with ourselves. Nothing will ever be the same.
\begin{figure}
\begin{center}
\begin{minipage}[b]{0.23\linewidth}
\centering
\includegraphics[height=4cm%,viewport = 0 500 500 0,clip
]{PIC/hilbert-1.eps}
{David Hilbert}
\label{Fig:Hilbert}
\end{minipage}
%\hspace{.6cm}
\begin{minipage}[b]{0.23\linewidth}
\centering
\includegraphics[height=4cm%,viewport = 0 500 500 0,clip
]{PIC/goedel-young.eps}
{Kurt G\"odel}
\label{Fig:Goedel}
\end{minipage}
%\hspace{.6cm}
\begin{minipage}[b]{0.23\linewidth}
\centering
\def\JPicScale{.25}
\includegraphics[height=4cm%,viewport = 0 500 500 0,clip
]{PIC/turing.eps}
{Alan Turing}
\label{Fig:Turing}
\end{minipage}
%\hspace{.6cm}
\begin{minipage}[b]{0.23\linewidth}
\centering
\includegraphics[height=4cm%,viewport = 0 500 500 0,clip
]{PIC/Neumann.eps}
{John von Neumann}
\end{minipage}
\caption{The relays from Entscheidungsproblem to  computer}
\label{Fig:Entscheidung}
\end{center}
\end{figure}

The successes of the XIX century science gave rise to the optimism expressed by David Hilbert in his famous slogan:
\begin{quote}
There is no ignorabimus in science. We must know, and we shall know!
\end{quote}
He closed with this exclamation his K\"onigsberg address in September 1930, at the conference held in his honor, on the occasion of his retirement. For mathematicians, Hilbert had previously distilled this quest for an \sindex{Decision Problem} omnipotent science in the \emph{Decision Problem} (\emph{Entscheidungsproblem}), which can be paraphrased as the challenge to 
\begin{quote}
Find a method to decide by finitary means the truth value of any formal statement. \sindex{Decision Problem} \sindex{Entscheidungsproblem| see {Decision Problem}}
\end{quote}
This was the centerpiece of the famous Hilbert's Program\sindex{Hilbert's Program}. A positive solution was hoped to provide a logical foundation for science. However, at the same K\"onigsberg conference, in one of the late sessions, the 24-year-old Kurt G\"odel shyly announced that he had constructed a provably undecidable statement in the elementary theory of arithmetic. The construction was based on a completely new method, invented by G\"odel for this purpose. At the K\"onigsberg conference, G\"odel's announcement went largely unnoticed, certainly by Hilbert\footnote{Von Neumann allegedly whispered to Bernays as soon as G\"odel finished his talk: "[Hilbert's Program] is finished". In the coming weeks, he derived an important consequence of G\"odel's result, and briefly corresponded with G\"odel about it. He never announced it, because G\"odel had already proved the result himself, and included it the paper that he was writing. The result came to be known as the Second Incompleteness Theorem. But John von Neumann seemed to be the only person who immediately understood G\"odel's result.}. A year later, when G\"odel published the details of his result \cite{GoedelK:ueber}, it shattered the foundational movement straddling the communities of mathematicians and logicians. It left Hilbert confused, and allegedly in denial. G\"odel's method provided the first stepping stone into the science of computation. Using the recursion schema  (discussed in Sec.~\ref{Sec:Rec}), G\"odel encoded the formulas of arithmetic as numbers and the proofs of theorems as special arithmetic operations. The insight of G\"odel's proof was that the logical theories, and in particular the theory of arithmetic, can be encoded as word processing, and that word processing can be encoded in arithmetic. In this way, the elementary arithmetic can encode its own proofs \emph{and}\/ check their derivability from axioms. G\"odel's basically invented  \emph{programming}, albeit without a computer. The computer had to wait for Turing. G\"odel used arithmetic as a universal  computer, or more precisely as a universal logical theory, expressive enough to encode logical theories in general, and to derive their proofs. He constructed his undecidable statement by encoding the elementary arithmetic in itself and instantiating the code of the statement "This number is the code of a false statement" to the number that encodes that same statement. The resulting statement is undecidable because its truth would imply its falsity, and vice versa. This is a \emph{diagonal}\/ argument, going back to Cantor, and previously used by Russell to construct his paradox which shook up Frege's hopes like G\"odel shook up Hilbert's. Yet another avatar of the diagonal argument is the Fundamental Theorem of Computation, which we will encounter in Sec.~\ref{Sec:kleene}. 

The computer as a machine was first described in the 1936 paper by the 24-year-old Alan Turing. Turing propagated G\"odel's idea of programming from logical formulas to state machines. Just like the arithmetic formulas can be encoded as numbers and processed in arithmetic, Turing machines can be encoded and processed by Turing machines. While G\"odel noticed that the logical theory of arithmetic was capable of encoding and processing itself, Turing performed the remarkable feat of specifying from scratch a family of machines where the same was possible. In the very same paper where he introduced his machines, Turing constructed a Universal Machine, that inputs a description of an arbitrary Turing machine, and then acts as that machine, i.e. performs its computations on its inputs, and produces its outputs. Turing's Universal Machine was the first computer. While G\"odel's insight was logical, Turing's concretized it into a foundation of a science. He seems to have initially thought of it as of a science of mind, but it got further concretized into the science of computation. The central idea of Turing's computer science, that programs can be processed as data, was promoted by von Neumann into the architectural principle of computer engineering. In Sec.~\ref{Sec:dataprog}, we saw the first of the unexpected repercussions: that processing programs as data leads to encoding data as programs. As WWII engaged both Turing and von Neumann, the practical consequences of their ideas that emerged from the ashes of Hilbert's ideals, got concretized further. John von Neumann played an important role in transferring the concept of a  Universal Machine into a computer architecture that came to carry his name. Some of the first von Neumann computers were used for work on the first nuclear bombs. Alan Turing worked during the war on a different kind of bomb. He developed up a ``cryptological bomb". It was conceived by Polish cryptographers\footnote{The original name, ``bomba kryptologiczna", was allegedly meant to refer to an ``ice-cream bombe". The war was still a year ahead.}, but Turing used his computing machinery and actually broke German cryptosystems. The achievement is said to have saved many lives and played a critical role in the allied victory. After the war, Turing returned to his work on computation and published his seminal ideas relating computation, life, and what later came to be called artificial intelligence. His ideas about morphogenesis are sometimes said to have been as much of a paradigm shift in biology as his ideas about computers were in logic. His concept of testing and indistinguishability remains in the foundations of the areas of computer science as different as semantics and cryptography. In 1952, Alan Turing was prosecuted for homosexuality, which was at the time a criminal offense in the UK, and sentenced to undergo hormonal treatment to suppress his libido. He died two years later, at the age of 41. The cause of death was poisoning with cyanide, that was found in the apple from which he had taken a bite. Although his favorite tale was known to be \emph{"The Snow White"}, it remains uncertain whether his death was intentional.

\subsection{How many truth values?} 
The XX century logic expanded the horizons of truth far beyond $\Bool = \{\true,\flse\}$. The theory of computation allowed refining the Brouwer-Heyting-Kolmogorov view of mathematical constructions, mentioned in Sec.~\ref{Sec:cat-logic}, into a  theory of \emph{realizability}\/ of logical statements \cite{HylandJME:efft,KleeneS:realiz,TroelstraA:metamath}. The practice of computation allowed realizing the semantics of \emph{propositions-as-types}\/ \cite{HowardW:curry,LawvereFW:dialectica}, also discussed in Sec.~\ref{Sec:cat-logic}, as a programming tool \cite{WadlerP:curry-howard}. We shall see in Ch.~\ref{Chap:Numrec} that the truth values $\true$ and $\flse$ suffice for drawing lots of programs. On the other hand, already in Ch.~\ref{Chap:Prog}, we shall see that even the simplest computations may be unable to decide whether to return $\true$ or $\flse$. The basic undecidability \sindex{undecidability} constructions are spelled out  in Ch.~\ref{Chap:Undec}.% as a logical limitation and in Ch.~\ref{Chap:Effop} as computational tool. 

==> 31-PROG/38-work-prog.tex <==
% !TEX root = ../000-monc.tex


\subsection{Divergence and lazy branching}\label{Sec:better-branch}\sindex{lazy!branching} \sindex{branching!lazy} \sindex{branching|lazy $\iif$}
The divergence is that any computation composed with a divergent component gets swallowed by the divergence. This is not always justified. E.g., the branching instruction $\iif(\bpredc,\true,\fixp)$ is normally expected to output $\true$ if $\bpredc=\true$ and to diverge if $\bpredc=\flse$. However, the implementation $\iif(\bpredc,f,g) = \uev \bpredc (f,g)$ in Sec.~\ref{Sec:branch} requires that $\bpredc$, $f$, and $g$ are evaluated before their outputs are passed to $\iif$. With that implementation, $\iif(\true,\true,\fixp)$ will always diverge.  To avoid this undesired behavior, most languages make use of programmability of the branches $f$ and $g$, and implement a branching operation $\IIFL(\bpredc,f,g)$ which evaluates the condition $\bpredc$ and outputs a program $F$ for $f = \uev F$ when $\bpredc=\true$ or  a program $G$ for $g=\uev G$ when $\bpredc=\flse$. In this way, only one of the branches is evaluated, and only after the branching. A more practical \emph{lazy}\/ branching should therefore satisfy  
\bea\label{eq:lazy-iif}
\iifl\Big(\bpredc,F,G\Big) & = & \uev{\uev \bpredc (F,G)}
\eea
\begin{enumerate}[a.]
\item Program a diagram for the lazy branching in \eqref{eq:lazy-iif}.
\item Specify the program transformers $\IIF, \IIFL:\DP^3\stricto\DP$ such that $\uev{\IIF(\bpredc,F,G)} = \iif\Big(\bpredc, \uev F, \uev G \Big)$ and $\uev{\IIFL(\bpredc,F,G)} = \iifl\Big(\bpredc, F, G \Big)$. While both evaluate $\bpredc$, input $F$ and $G$ and output a program that runs $F$ if $\bpredc$ is true and $G$ if it false, they behave differently. Provide examples of different and of indifferent behaviors. 
\item Given an idempotent $\rho_{A}\colon \DP\to \DP$ such that $x = \rho_{A}(x)$ holds just for the (programs that encode) elements of $A$ as in Sec.~\ref{Sec:retracts}, construct an idempotent $\check\rho_{A}\colon \DP\to \DP$ that still fixes the elements of $A$ and is moreover a subfunction of the identity on $\DP$. In other words, for all programs $y$ that do not encode elements of $A$, $\check\rho_{A}(y)$ should diverge.
\end{enumerate}



%\subsection{Decidable equality precludes uniform evaluators}\sindex{evaluator!uniform}\label{Work:nouni}
%The constructions from Sec.~\ref{Sec:divergence} imply that the uniform evaluators from workout~\ref{Sec:uniform} make the program equality undecidable.
%
%
%
%\begin{enumerate}[a.]
%\item  Show that Church's numerals, defined in Workout~\ref{Sec:churchnum}, faithfully represent all finite natural numbers, in the sense that $\overline n = \overline m$ implies $n=m$. One way to show this is to prove that for any pair of natural numbers $n,k$, $\overline{n+k} = \overline n$ implies $k=0$ or $n\gt \ell$ for all finite numbers $\ell$. 
%
%\item\label{work:uniform-collapse}
%Prove that the decidable equality $(\iseq):\DP\times \DP\stricto\Bool$ in monoidal computers precludes the uniform evaluators from Workout~\ref{Sec:uniform}.
%
%\end{enumerate}

\subsection{Stateful fixpoints}\sindex{fixpoint!stateful}\label{Work:statefix}
The Fundamental Theorem remains valid for stateful (indexed) \funnn s and programs. Here we work out two kinds of stateful Kleene fixpoints.

\begin{enumerate}[a.]
\item Show that any $X$-indexed computation $g:\DP\times X \times A \to B$ has an $X$-indexed Kleene fixpoint $\Gamma:X\stricto \DP$ such that for all $a\colon A$ 
\bea
g\left(\Gamma x, x, a\right) & = & \uev{\Gamma x} a \eea


\item Show that any $X$-indexed program transformer $\theta:\DP\times X \stricto \DP$ has an $X$-indexed fixpoint $\Theta:X\stricto \DP$ such that
\bear
\uev{\theta(\Theta x, x)} & = & \uev{\Theta x} \eear
\end{enumerate}

\subsection{Qing, kuine, narcissist, virus generator}\label{Work:kuine}
\begin{enumerate}[a.]
\item A\sindex{narcissist} \emph{narcissist}\/ is a program $T$ which inputs programs and outputs its own images along the \funnn s that the programs encode:
\bear
\uev T x & = & \uev x T
\eear
Find a narcissist!

\item A \emph{virus generator}\/\sindex{virus!generator} is a program transformer $\gamma:\DP\stricto \DP$ which transforms programs into viruses. Its function is:
\bear
\uev{\gamma F}x  & = & \Big< \gamma F,\ \gamma F,\  \uev{F} x\Big>
\eear
Program a virus generator!

\item Show that there are programs $Q$ing and $K$uine \sindex{quine!qing and kuine}which on any input output each other's text:
\[\uev K x = Q \qquad \qquad \qquad \qquad \uev Q x = K\]

\end{enumerate}

\subsection{A loopy software system}\sindex{software}
The \emph{Loopy Credit Union (LCU)}\/ account system consists of
\begin{itemize}
\item a database $B = \seq{ x_{u} }_{u\in U}$ where
\begin{itemize}
\item $U$ is the list of customers,
\item $x_{u}$ is the account balance of the customer $u\in U$
\item $\ell\in U$ is the account into which the LCU collects the fees for their services;
\end{itemize}
\item three types of transactions:
\begin{itemize}
\item deposit $d(u,x) = B + x_{u}$ for each $u\in U$,
\item withdrawal $w(u,x) = B - x_{u}$ for each $u\in U$, and
\item transfer $t(u,v,x) = \Big(w(u,x)\ \, ;\ d(v,x)\ \, ;\ t(v,\ell,rx)\Big)$ for every pair $u,v\in U$.
\end{itemize}
\end{itemize}
While the deposits and the withdrawals are free of charge, the recipient of each transfer of $x$ coins is charged a fee of $rx$ coins, transferred to the fee account $\ell$. A transfer from a customer $u$ to a customer $v$ is implemented as a sequential composition of a withdrawal of $x$ from $u$'s account, followed by a deposit of $x$ into $v$'s account, followed by a transfer of $rx$ into $\ell$s account.

Develop the LSU-software system as a fixpoint.







==> 31-PROG/39-story-fixp.tex <==
% !TEX root = ../000-monc.tex

The Fundamental Theorem of Computation says that every computational process has a Kleene fixpoint.\sindex{fundamental theorem!of computation}\sindex{Kleene's Second Recursion Theorem} This realization evolved through several fundamental ideas. First there was Cantor's diagonal argument \cite{CantorG:1891uber}. Then there was Russel's application of that argument to derive his paradox from Frege's unrestricted set-comprehension \cite{RussellB:paradox}. Then there was G\"odel's application of that construction in logic, to derive incompleteness of Russell-Whitehead's \emph{Principia}\/ and all other systems containing the arithmetic \cite{GoedelK:ueber}. Then Stephen Kleene proved the Fundamental Theorem of Computation as a remark in the short paper \cite{KleeneS:ordinal-fund}. He continued to treat it as an offshoot of his extensional \emph{Recursion Theorem} \cite[\S 66]{KleeneS:metamathematics}. 
Some years later, the program transformer version was formulated \cite{RogersH:book} and Kleene's  remark got promoted into the \emph{"Second Recursion Theorem"}. Many years and many fundamental applications later, the name got extended to \emph{"Kleene's Amazing Second Recursion Theorem"} \cite{MoschovakisY:Kleene}. 
\begin{figure}[ht]
\begin{minipage}[b]{0.5\linewidth}
\centering
\includegraphics[height=5cm%,viewport = 0 500 500 0,clip
]{PIC/kleene.eps}
\caption{Stephen C. Kleene}% the enemy}
\label{Fig:kleene-photo}
\end{minipage}
\begin{minipage}[b]{0.5\linewidth}
\centering
\includegraphics[height=5cm%,viewport = 0 500 500 0,clip
]{PIC/smullyan.eps}
\caption{Raymond Smullyan}% the enemy}
\label{Fig:smullyan}
\end{minipage}
\end{figure}
Raymond Smullyan proved the double-fixpoint version from Sec.~\ref{Sec:joint} and studied the general approach in his book about \emph{"Diagonalization and Self-Reference"} \cite{SmullyanR:diagonalization}. He also wrote many popular books about the logic of self-reference \cite{SmullyanR:what-name,SmullyanR:mock}. The topic lent itself to other popular treatments \cite{HofstadterD:GEB,PoundstoneW:recursive}. In the years before his death, John von Neumann had noticed that computational self-reference implies structural self-reproduction, which is the characteristic of life. On his deathbed, he was preparing a series of lectures about life as computation \cite{NeumannJ:self-reproducing}. The idea was that a universal computer with sensors and actuators could gather materials, process them, and produce a copy of itself. Or several copies, slightly modified, letting nature select the fittest. The computational aspects of life also preoccupied Alan Turing towards the end of his short life \cite{TuringA:morphogenesis-book}.








==> 41-NUMREC/48-work-num.tex <==
% !TEX root = ../000-monc.tex
\subsection{Early induction}\label{Work:fibonacci}
A rabbit population grows according to the following rules:
\begin{enumerate}[1)]
\item in the beginning there is a single pair of \emph{baby}\/ rabbits; 
\item each baby rabbit becomes an \emph{adult} rabbit within a month;
\item each pair of adult rabbits produces a pair of baby rabbits within a month,
\item rabbits never die.
\end{enumerate}
Draw a string program for computing the total number of pairs of rabbits after $n$ months.

\para{Background.} This early example of induction is due to Leonardo Pisano Bigollo ($\sim$1175--1250),  the "Traveller from Pisa", who actually grew up and studied in North Africa, where his father \emph{Bonacci}\/ held a Pisan trade outpost. Bonacci's son \emph{Fibonacci}\/ travelled back to Pisa and brought with him not only the rabbit-counting function, but also the positional numeral system in use today. In Europe at the time,  even arithmetic was still done in Latin. Fibonacci noted even in the title of some of his writings that his methods originated from India.

\subsection{Recursion work}\label{Work:recursion}
\begin{enumerate}[a.]
\item Draw string  programs for the following functions:
\begin{enumerate}[i)]
	\item $m + n$
	\item $m\times n$
	\item $ {m} \dotdiv {n} = \begin{cases} m-n &  m \gt n \\ 0 & \otherwise \end{cases}$
	\item $\Sigma({n}) =  {0}+  {1} +  {2} + \cdots +  {n}$
\end{enumerate}


\item The recursion schema from Sec.~\ref{Sec:prog-recursion} requires that both $g$ and $h$ are evaluated each time when $\cata{g,h}$ is evaluated. This is wasteful, since $g$ only needs to be evaluated in the base-case $n=0$, $h$ only in the step-cases  $n=m+1$.  A similar issue arose with respect to the  gives rise to the same issue like the the $\iif$-branching from Sec.~\ref{Sec:branch}. Given some programs $G$ and $H$ for the computations $g$ and $h$, implement a lazy recursion schema, where $g$ and $h$ are only evaluated when needed. \sindex{lazy!recursion} \sindex{recursion!lazy|see{lazy, recursion}}
\end{enumerate}



\subsection{Search work}\label{Work:search}
\begin{enumerate}[a.]
\item Draw a string program for discrete cubic root search $\sqrt[3]{n} = \begin{cases} m & n = m^{3} \\ \uparrow & \otherwise  \end{cases} $

%\item Georg Cantor, the inventor of set theory, defined his pairing function $\cantorJ: \NNn\times \NNn \to \NNn$ as follows 
%\bear
%\cantorJ(m,n) & = & m + \sum_{k=1}^{m+n} k
%\eear
%The claim is that this function provides a recursive bijection between $\NNn\times \NNn$ and $\NNn$. 
%
%\begin{enumerate}[i)]
%\item Show that $\cantorJ$ is primitive recursive and injective.
%\item Towards the surjectiveness, spell out the inverse $\proj = <\proj_0, \proj_1>: \NNn\to \NNn\times \NNn$ of $\cantorJ: \NNn\times \NNn \to \NNn$, i.e. the functions $\proj_0, \proj_1:\NNn\to \NNn$ such that
%\begin{gather*}
%\proj_0\left(\cantorJ(m,n)\right) = m \qquad \proj_1\left(\cantorJ(m,n)\right) = n\\
%\cantorJ\left(\proj_0(\ell), \proj_1(\ell)\right) = \ell
%\end{gather*}
%\item Try to show that $\proj_0$ and $\proj_1$ are primitive recursive. Explain why this seems hard.
%\end{enumerate}
%
%

%\item Explain the input-output behavior of the following functions: 
%\begin{enumerate}[i)]
%\item $t_1(n) = \mu x.\  n+x+1 = 0$
%	\item $t_2(n) = \mu x.\  n+x = 0$
%	\item $t_3(n) = \mu x.\  x\gt n$
%	\item $t_4(n) = \mu x.\  x\lt n$
%	\item $t_5(n) = \mu x.\  x+n = n$
%	\item $t_6(n) = \mu x.\  x+n = x$
%\end{enumerate}

\item Implement in monoidal computer  the following program schemas: \begin{enumerate}[i)]
\item bounded search: \[\prooftree
k \in\NNn\qquad \qquad g: \NNn \ttimes A \to \NNn \justifies
f = \MU(k, g): A \to \NNn
\endprooftree\]
where $f = \MU(k, g)$ means that $f(x) = \mu n\leq k.\ \iszero g(n,x)$ is the smallest number $n\leq k$ where $g(n,x)=0$, i.e.
\bear
f(x) = n &  \iff &  \iszero g(n, x)\  \wedge\ g\leq k\ \wedge\ \forall m\leq k.\ \iszero g(m,x) \Rightarrow \iszero(n\dotdiv m)
\eear
Prove that bounded search always terminates. 

\item \emph{FOR}\/-loop:
\[\prooftree
k \in \NNn \qquad\qquad h: A \times B \to A \justifies
f = FOR(k,h): A \times B \to A
\endprooftree\]
where $f_{k} = FOR(k,h)$ is defined on $x:A$ and $y:B$ inductively, as the sequence
\[f_0 = x\qquad \mbox{ and } \qquad \vec f_{i+1} = h(f_i, y) \]
\end{enumerate}
\end{enumerate}


==> 41-NUMREC/49-story-CTT.tex <==
% !TEX root = ../000-monc.tex

\subsection{Church's reverse programming} \label{Sec:Church-reverse}
In this chapter, we built programs by composing copies of the program evaluator, i.e. by applying the \runn-instruction. The arithmetic operations and the program constructors have been reverse-programmed (in the sense of Sec.~\ref{Sec:Reverse}) in the single-instruction language Run. The seminal example of reverse programming was Alonzo Church's reconstruction of the arithmetic and the logical operations in his $\lambda$-calculus \sindex{lambda-calculus@$\lambda$-calculus} \cite[Ch.~III]{ChurchA:calculi}. In the present context, the $\lambda$-calculus can be viewed as a two-instruction programming language. The first instruction is a version of the \runn-instruction, the \emph{function application}\/ operation,\sindex{function!application} which applies a function to its inputs. It is usually abbreviated to concatenation, writing $\apply(f)(x) = fx$. The second instruction is the \emph{function abstraction}\/ \sindex{function!abstraction} operation, written $\abss(x)(f) = \lambda x.f$.\footnote{The letter $\lambda$ was, according to the oral lore, chosen by the typesetters of Alonzo Church's early publications. They  apparently had trouble typesetting $\hat x$, used in Russell-Whitehead's \emph{Principia}\/ \cite{Russell-Whitehead:principia}, so they first modified it to \, $\hat{}x$, and then proposed $\lambda x$, which was accepted.} The function abstraction is different from the program abstraction in that for every computable function $f$ there are many programs $F$ such that $\uev F a = f(a)$, whereas the abstraction picks $\lambda  x. f$ such that $(\lambda x. f)a = f(a)$.  But the function abstraction is similar to the program\sindex{instruction!application}\sindex{instruction!abstraction} abstraction\sindex{abstraction} in that it is an inverse to the \apply-instruction, as displayed in Fig.~\ref{Fig:CTT}, just like the program abstraction is an inverse to the \runn-instruction, as displayed in Figures~\ref{Fig:prog-run} and \ref{Fig:head-tail}. A more precise categorical correspondence is in Fig.~\ref{Fig:PCC} and detailed accounts can be found in  \cite{BarendregtH:book,Lambek-Scott:book}. 
\begin{figure}[!ht]
\begin{center}
\begin{tikzpicture}[shorten >=1pt,node distance=3cm]
  \node[state,minimum size=35pt,draw=black,very thick]   
  (nocarry)                {\begin{minipage}[c]{1.75cm}\begin{center} Functions \end{center}\end{minipage}};
   \node[state,minimum size=0pt,draw=black,very thick] (carry)    [right=of nocarry]              
   {\begin{minipage}[c]{1.75cm}\begin{center} Functions \end{center}\end{minipage}};
  \path[->] 
  (nocarry) 
  edge [bend right,thick] node [below] {\abss} node [above] {$\scriptstyle f\ {\displaystyle \mapsto}\  \lambda x. f$} 
  (carry)
  (carry) 
  edge [bend right,thick] node [above] {\apply} node [below] {$\scriptstyle fx \  \mapsfrom\  f$}  
  (nocarry);
   \end{tikzpicture}
   \caption{%The $\lambda$-conversation:
   The operations of function abstraction and application} 
\label{Fig:CTT}
\end{center}
\end{figure}
While a programmer tries to abstract from a given function $f$ a program $F$ such that $\runn\big(F\big) = f$, the $\lambda$-abstraction operation abstracts from $f$ the function abstraction $\abss(f)$ such that $\apply\big(\abss(f)\big) = f$. This requirement that \abss\ is a right inverse to \apply, written in the abbreviated form $(\lambda x. f) a = fa$, is called the \sindex{beta-conversion@$\beta$-conversion} \emph{$\beta$-conversion}\/ rule in the $\lambda$-calculus. The requirement that \abss\ is also a left inverse to \apply, i.e. $\abss\big(\apply(f)\big) = f$, written in the abbreviated form $\lambda x. (fx) = f$, is called the \sindex{eta-conversion@$\eta$-conversion} \emph{$\eta$-conversion}\/ rule. While the $\beta$-conversion requirement is always imposed, the  $\lambda$-calculus satisfying the $\eta$-conversion requirement is called \emph{extensional}.\sindex{extensionality!rule} In the\sindex{extensional!lambda-calculus@$\lambda$-calculus} \sindex{lambda-calculus@$\lambda$-calculus!extensional} extensional $\lambda$-calculi, the operations \abss\ and \apply\ form a bijection between the functions and their abstractions.  %A function abstraction thus corresponds to set of program abstractions of a function, i.e. to an equivalence class of programs modulo the extensionality relation from Sec.~\ref{Sec:Ext}. 

The $\lambda$-calculus was the outcome of Church's effort to provide an abstract account of G\"odel's encodings \cite{GoedelK:ueber} of \funnn s as numbers \cite[Ch.~IV]{ChurchA:calculi}. While G\"odel's encodings can be viewed as an example of abstracting programs from functions, Church leveled the field by making functions into first-class citizens (indeed, the \emph{only}\/ citizens) of his theory, and used the function abstraction operation (now distinguished from the program abstraction, which is not an operation but a process) to provide an algebraic account of the process of computation. He provided a roadmap for reverse programming and demonstrated that the basic instructions \abss\ and \apply\ suffice to compute everything that can be computed. The point of the present chapter is\sindex{instruction!application}\sindex{instruction!run@{\runn}} that the lone cousin of the \apply-instruction, the \runn-instruction, suffices on its own. The role of Church's function abstraction operation is played by the assumption in \eqref{eq:uev-formal} that a computable \funnn\  always has a program abstraction, which boils down to assuming that the \runn-operation is surjective. The upshot is that the \runn-operation alone also suffices for defining the notions of computability and "effective procedure", which was the original purpose of it all.

\subsection{Story of curly brackets}\label{Sec:curly} \sindex{run-instruction@\runn-instruction} The relationship between the function abstraction and the program abstraction is subtle and convoluted\sindex{abstraction!function vs program}. Both emerged from attempts to capture the idea behind  G\"odel's encoding arithmetic in itself; to formalize his abstractions of the arithmetic functions, formulas, and statements into numbers, available as for processing by arithmetic functions, formulas, and statements. The function abstraction provided an abstract view, the operation mapping a function $f$ to its abstraction $\lambda x. f$. The program abstraction provided a concrete view, where a programmer specifies a program $F$ for $f$. The function is recovered as $f(a) = (\lambda x. f) a$, by applying its abstraction, or as $f(a) = \uev F a$, by evaluating its program. In  \cite{KleeneS:lambda}, Kleene wrote the function application in the form $f(a) = \uev{\lambda x. f} a$. In \cite{TuringA:Entscheidung}, Turing adopted the same notation to describe the evaluation $\uev M a = f(a)$ of a machine $M$ constructed for any $\lambda$-definable $f$. Kleene then adopted the same notation for the actual program evaluators of the primordial programming language of G\"odel encodings of recursive functions \cite[\S 66]{KleeneS:metamathematics}. The curly brackets as general program evaluators remain with us as a reminder of the common origin of running and the application, and of programming and the abstraction.



\subsection{The Church-Turing Thesis} 
Theory of computation was born of Hilbert's Program to develop  mathematical logic as a metamathematical foundation. The original goal of this effort was to find the \emph{"effective procedures"}\/ to decide whether scientific theories are true or false. The first task was to formally define the notion of an effective procedure. The concept of computability emerged from that task. The most significant first step was made in G\"odel's proof of his Incompleteness Theorem \cite{GoedelK:ueber}. It  finished off Hilbert's Program to develop effective procedures for deciding everything, but provided a stepping stone towards defining what is an effective procedure. At the heart of G\"odel's proof was the the recursion schema.\sindex{schema!recursion}\sindex{recursion|see {schema}} Informal recurrences had been in use for a long time, and Dedekind had formalized the recursion  schema decades earlier \cite{DedekindR:zahlen}. G\"odel used it as a programming tool in his proof, and uncovered its capability to encode itself, which was the crucial step towards the concept of programming. One could argue that programs existed since the early XIX century as the patterns fed to Jacquard's looms, and even more compellingly as Ada Lovelace's formalization of Bernoulli's algorithm, which was recursive. Most histories of computation provide a full account. G\"odel's insight \cite{GoedelK:ueber}  that recursively defined arithmetic functions can be encoded as numbers and processed by recursively defined arithmetic functions, encoding some arithmetic proofs, brought the idea of programming to another level. Or to infinitely many levels of such self-applications  \cite{HofstadterD:GEB}. While the recursion schema was clearly an effective procedure sufficient for the purposes of G\"odel's paper, he stated clearly, explicitly, and repeatedly that the recursion schema alone did not provide a complete characterization of all effective procedures. Simple examples of arithmetic functions that are effective but not recursive can be found in Sec.~\ref{Sec:iteration}. 

Alonzo Church converged towards his thesis iteratively, through his quest for characterization of computable ("effectively calculable") functions \cite{ChurchA:unsolvable}. He developed his calculus of $\lambda$-abstraction upon Bertrand Russell's type theory \cite{RussellB:types}, avoiding the non-constructive (and thus uncomputable) aspects of the set-theoretic foundations. The operation of $\lambda$-abstraction extracts a description from a function, and can be construed as an abstract form of G\"odel's encoding of arithmetic functions as numbers \cite{GoedelK:ueber}. This encoding is the central part of G\"odel's groundbreaking incompleteness theorems, and the origin of the \emph{programs-are-data}\/ paradigm. But G\"odel rejected Church's proposals to define computability in terms of the function abstraction operation outright \cite[Ch.~17]{SoareR:CTA}. Church updated his proposal to include G\"odel's extension of the recursion schema along the lines proposed by Herbrand, and eventually arrived at the postulate that not only his type-theoretic model, and G\"odel's recursion-theoretic model, but also all other models of computation proposed at the time or in the future must  compute the same family of functions \cite[Sec.~17.2]{SoareR:CTA}. This was Church's Thesis. G\"odel remained  unswayed, continuing to object that the G\"odel-Herbrand schemas were indeed effective, but that there were no grounds for claiming that all procedures that may come to be considered effective will be reducible to this or that combination of schemas. Then Turing's model appeared, and provided the grounds. G\"odel not only accepted that "the correct definition of mechanical computability was established beyond any doubt by Turing", but added that Turing has "for the first time succeeded in giving an absolute definition of an  interesting epistemological notion,  i.e., one not depending on the formalism chosen" \cite{GoedelK:bicentennial}. Although G\"odel was the undisputed arbiter of the matter, Turing was at the time a graduate student, Church was his advisor, and the community did not rush to recognize Turing's breakthrough. The other models were proved to provide correct definitions of computability by demonstrating their equivalence with Turing's. It was first proved that the G\"odel-Herbrand recursive functions\sindex{function!recursive}\sindex{recursive function|see {function}} coincide with the \emph{total}\/ functions computable by the Turing machines\sindex{function!total}\sindex{total function|see {function}}. Then Stephen Kleene, another student of Church's, realized that adding the minimization schema from Sec.~\ref{Sec:search} to the recursion schema from Sec.~\ref{Sec:prog-recursion} allows deriving the same family of computable functions like Turing's machines \cite{KleeneS:general-bulletin,KleeneS:general}. As the time went by, Emil Post's canonical word-processing systems, Jim Lambek's abacus, Zuse's cellular automata (with Conway's Game of Life as a special case), and an entire bestiarium of other machines, rewrite systems, and circuit ensembles (uniformly generated by Turing machines!) were all proved to make the same \funnn s computable, lending cridibility to Church's Thesis. The multitude of different ways to compute the same class of \funnn s was hailed as evidence of its robustness \cite[\S 62]{KleeneS:metamathematics}. 

Although Kleene's combination of recursion and minimization does not look different from other equivalent models, it came to dominate the theory of computation, to the point that Turing's concept of \sindex{function!computable}\emph{computable}\/ function got overridden by the  \sindex{function!partial recursive}\sindex{partial recursive function|see {function}} term \emph{partial recursive}\/ function, and the theory of computation itself came to be called the \emph{theory of recursion}  \sindex{recursion!theory} \cite[Sec.~17.2]{SoareR:CTA}. To fit the bill, the recursion schema used by G\"odel  in his epochal \cite{GoedelK:ueber} got renamed to \emph{``primitive"} recursion, leaving the name \emph{``recursive functions"}\/ for the functions defined in Kleene's system that happen to be total \cite{KleeneS:general}. It took time to remember that the partial recursive functions were just the computable functions renamed by a particular implementation \cite{SoareR:RE,SoareR:CTA}. For his part, G\"odel seems to have rejected the conundrum \cite[Sec.~17.7.1]{SoareR:CTA} and in any case continued to use the term recursion for the schema in \eqref{eq:banana-recursion}, as introduced into logic by him in \cite{GoedelK:ueber} and developed by Rozsa Peter in \cite{Rozsa}, whom he referenced in this context. We revert to G\"odel's terminology. Although Peter's work initially met wide recognition (a presentation at the International Congress of Mathematicians in 1932, an invitation to the founding editorial board of the Journal of Symbolic Logic, all at time when women were still largely barred from holding academic positions), the upsurge of antisemitism and the ensuing iron curtain put an end to her research, leaving it with the \emph{"primitive"}\/ moniker.\sindex{recursion!primitive} 

\begin{figure}[ht]
\begin{minipage}[b]{0.5\linewidth}
\centering
\includegraphics[height=5cm]{PIC/alonzo-church-young.eps}
\caption{Alonzo Church}
\label{Fig:church}
\end{minipage}
\begin{minipage}[b]{0.5\linewidth}
\centering
\includegraphics[height=5cm]{PIC/Rozsa-Peter-young.eps}
\caption{Peter Rozsa}
\label{Fig:rozsa}
\end{minipage}
\end{figure}

It should be noted that Turing did not propose a thesis or postulate, but proved that his model satisfied the requirements of a definition of "effective procedure" arising from G\"odel's proofs  \cite{GandyR:confluence}. There is no evidence that the idea of balancing his answer against his thesis advisor's Thesis ever crossed Turing's mind. That balancing act was a part of Kleene's project of reducing theory of computation to theory of recursion   \cite[\S 60, Thesis I]{KleeneS:metamathematics}, which he justified by reinterpreting Church's proposal to G\"odel [ibidem, \S 62]. At the time when Kleene's was working on his monumental \emph{Summa}, Turing was zeroing on computation as life \cite{TuringA:morphogenesis-book} and approaching the end of his life. He broached the boundaries of epistemology by providing a mathematical model of how we compute. His theory of computation can be interpreted as a solution of the mind-body problem. The driving forces behind his work may have included an early death of a friend and a world war. But he never spoke up, leaving it to the murmurations of computers to spell out his message.  

\subsection{Turing completeness} \sindex{Turing-completeness|see {programming language, Turing complete}} \sindex{programming!language!Turing complete}
The multitude of models used in theory of computation is echoed by the multitude of the programming languages used in practice. Some are more convenient for some application domains, some for other, and some are not domain-specific but general-purpose and programmers' choices are often based of taste and habit. The diversity of programming languages is a product of the same divergent evolution as the diversity of natural languages. However, while the common foundations of natural languages are the ongoing studies in epistemology and paleolinguistics \cite{ChomskyN:mind}, the common foundations of the programming practices are the mathematical proofs, sometimes offered as the empiric evidence for the Church-Turing Thesis, \sindex{Church-Turing!Thesis} that any given pair of proposed models of computation describe the same computable \funnn s, and that any pair of standard programming languages are as expressive as each other, i.e. that they also describe the same family of computable \funnn s. The crucial requirement for this is obviously \eqref{eq:uev}, i.e. that they allow programming their own program evaluators. \emph{The programming languages that allow programming all computable \funnn s, including their own program evaluators, are called \textbf{Turing-complete}.} A majority of the programming languages encountered in practice are Turing-complete.\footnote{The only exceptions are some special-purpose languages, like early SQL, or the Berkeley Packet Filter, which restrict their programs regular expressions. In other words, they are as expressive as finite-state machines, rather than the Turing machines. The markup languages like XML and HTML are sometimes also mentioned as exceptions, although they are not programming languages so it is not clear what the notion of Turing-completeness would mean for them.}


==> 51-UNDEC/58-work-undec.tex <==
% !TEX root = ../000-monc.tex


%\subsection{The Rice routine}
Rice's Theorem says that a computable predicate cannot at the same time be extensional, decidable, and nontrivial. This theorem is thus usually applied by showing that a computable predicate satisfies two of the properties, and deriving that it does not satisfy the third one.

Determine whether the following predicates are decidable:
\begin{multicols}{2}
\begin{enumerate}[a.]
\item $P_1(x) \iff \{x\}4 = 7$
\item $P_{2}(x) \iff \{4\}x = 7$
\item $P_3(x) \iff \{x\}25 \lt 1000$
\item $P_4(x) \iff \{x\}2 \leq \{x\}3$
\item $P_5(x) \iff \pev{x}2  = 2  $
\item $P_6(x) \iff \{x\}13\! \uparrow$
\item $P_7(x) \iff \{13\}x\! \uparrow$
\item $P_{8}(x) \iff \pev{\pev{x}}x\! \uparrow$
\item $P_9(x) \iff \Big(\{x\}7\halts\  \Longrightarrow \{x\}8\halts\Big)$
\item $P_{10}(x) \iff \forall n.\ \{x\}n \leq \{x\}(n+1)$
\item $P_{11}(x) \iff \exists n. \ \{x\}n \halts$
\item $P_{12}(x) \iff \{x\}x\halts$
\end{enumerate}
\end{multicols}
Prove your claims!



==> 51-UNDEC/59-story-CTA.tex <==
% !TEX root = ../000-monc.tex

\subsection{I cannot decide whether I lie}%, but I can say it by a program}
This chapter asked what can be decided about the computation of a program without running it. The simple \emph{general}\/ answer is: \emph{nothing}. There are, of course, \emph{particular}\/ programs where it is easy to tell what they do. The claim is that there is no \emph{general}\/ way to tell for all programs. More precisely, any predicate computable over all programs but extensional, and thus predicated over the corresponding functions, must leave some programs undecided, unless it blindly assigns the same truth value to all programs. That is what Rice's Theorem says. Its proof says that this is a consequence of the fact that any computable predicate over programs is also predicated over its own programs, and over the programs of its negation. A predicate over its negation negation outputs the truth value of the statement ``I lie''. That statement is false if it is true, and true if it is false. It is an instance of the Liar Paradox \sindex{paradox!liar}.  The theorems of G\"odel, Tarski, Turing, and Rice are all proved as instances of the Liar Paradox. Each of the four original proofs encodes the paradox in a different setting. G\"odel encoded the formal arithmetic in itself and discovered that definitions of arithmetic functions can be encoded as numbers \cite{GoedelK:ueber}. Tarski encoded the semantical assignment of a logical theory in itself \cite{TarskiA:truth}. Turing encoded his machines and evaluated them in a universal machine \cite{TuringA:Entscheidung}. He constructed the universal computer for the purpose of this encoding. Rice encoded the diagonal argument in the general framework of recursive enumerations \cite{RiceHG:rice-thm}. G\"odel's encodings of functions as numbers were the first programs in a universal programming language. Turing's universal machine was the first universal computer. Each of the four theorems used a different programming language and a different computer, but they all used the same gadget to connect the two: a program evaluator. And they all used it to construct an instance of the fixpoint from Sec.~\ref{Sec:divergence}. The four no-go theorems opened a maze of paths into the logic of self-reference \sindex{self-reference}  \cite{HofstadterD:GEB,LevinL:forbidden,SmorynskiC:self-reference,SmullyanR:diagonalization,SmullyanR:what-name,YanofskyN:outer}, and an alley into computation. 



\subsection{The Church-Turing Antithesis}\label{Sec:CTA}
The Church-Turing Thesis,\sindex{Church-Turing!Thesis} discussed in Sec.~\ref{Sec:CTT}, presents computability theory as a quilt of diverse models of computation, stitched together by computable encodings and reductions. Church's $\lambda$-calculus, Turing's machines, and Kleene's partial recursive functions are just parts of the quilt, together with Post's production systems, von Neumann's cellular automata, and many other equivalent models. But some models came to be viewed as more equivalent than others. Kleene's model became so popular among logicians that theory of computation was called theory of recursion as a part of mathematical logic  \cite{KleeneS:metamathematics,RogersH:book}.  Turing's and Church's models spanned the two coordinate axes of theoretical computer science, called ``track A: algorithmics" and ``track B: semantics" in some leading publishing venues, conferences, and handbooks  \cite{LeeuwenJ:handbook-A,LeeuwenJ:handbook-B}. On ``track A", Turing machines are used to measure computational complexity. On ``track B", Church's $\lambda$-calculi and type systems are used to assign formal meanings to programs. At times, the two ``tracks" were distinguished even by the geographic locations of the respective research communities \cite{GurevichY:east-west}%%,VardiM:CTA
\footnote{Ironically, the geographic origins got switched and Church's legacy of high-level calculi got at first pursued mostly in Europe, Turing's legacy of low-level machines mostly in the US.}.

%The Church-Turing Thesis can be interpreted as the statement that there is no Tower of Babel, no universal language, not for conversations and not for programming. 



But the Church-Turing \emph{Anti}\/thesis \sindex{Church-Turing!Antithesis} is not just a gap between research communities. After the initial confluence of ideas in 1936, \cite{GandyR:confluence}, the models of computation bifurcated into the \emph{extensional}\/ and the \emph{intensional}, as soon as they were used for solving Hilbert's \emph{Entscheidungsproblem}.  \begin{figure}[!ht]
\begin{center}
\begin{tikzpicture}[shorten >=1pt,node distance=3cm]
  \node[state,minimum size=35pt,draw=black,very thick]   
  (nocarry)                {\begin{minipage}[c]{1.75cm}\begin{center} Extensional\\
  (functions) \end{center}\end{minipage}};
   \node[state,minimum size=0pt,draw=black,very thick] (carry)    [right=of nocarry]              
   {\begin{minipage}[c]{1.75cm}\begin{center} Intensional\\
   (machines) \end{center}\end{minipage}};
  \path[->] 
  (nocarry) 
  edge [bend right,dotted,thin] node [below] {programming} 
  (carry);
   \path[->>] 
  (carry) 
  edge [bend right,thick] node [above] {\Large$\universal$}  
  (nocarry);
   \end{tikzpicture}
   \caption{Programming is not an operation} 
\label{Fig:CTA}
\end{center}
\end{figure} 
Alonzo Church's solution  \cite{ChurchA:unsolvable}  was based on the operations of function abstraction and application, whereas Alan Turing's solution \cite{TuringA:Entscheidung} was based on programming a universal machine to simulate computational processes. Church's idea was to provide a high-level characterization of computable functions in terms of function abstraction. Turing provided a low-level characterization in terms of computing machines. While the operation function abstraction establishes the one-to-one correspondence in Fig.~\ref{Fig:CTT} between the functions and their abstractions, program abstraction is not a routinely operation but programmers' effort to construct programs, as displayed in Fig.~\ref{Fig:CTA}. The fact (worked out in Sec.~\ref{Sec:how-many}) that each computation can be programmed in infinitely many ways is not a technicality but a fact of life. Programs do not arise by magic of abstraction as an operation, but through abstraction as creation\footnote{Creativity is a property of evolutionary processes. Machines may evolve and create. The original computers that Turing thought of when he defined his machines were the persons that perform computations. Future programmers may be the machines that design algorithms.}. The Church-Turing Antithesis is the antithesis of the extensional and the intensional views of computations: as functions and as programs. As programs are evaluated into functions, the induced extensionality relation \eqref{eq:ext-def} aligns the two views. The concept of extensionality  goes back to Hermann Grassman's \emph{linear extension theory} \cite[Ch.~I]{GrassmannH:new}, an algebra of geometry whose offspring was the linear algebra that we nowadays use  \cite{GrassmannH:extension}. In set theory, the \textbf{\emph{Extensionality Axiom}}\/ says that sets are the objects that are equal if and only if they have the same elements. It follows that the functions between sets are equal if and only if they map the same elements to the same elements. In computation, many different programs are evaluated to each function. That fact, worked out in Sec.~\ref{Sec:how-many}, should perhaps be called the \textbf{\emph{Intensionality Theorem}}. The concept of intensionality goes back to Grassman again, but the usage evolved. %Unlike set theory, computer science studies objects that may be extensionally indistinguishable but intensionally different. E.g., the same function can be implemented by different algorithms, which can be expressed by even more different programs. Computer science is concerned with the performance or structure of the different programs, set theory only with the same functions, taking the same inputs to the same outputs. 
% The extensional equivalence identifies different programs if they compute the same function. 
The results presented in this chapter display the gap between the extensional and the intensional views: there are no nontrivial extensional predicates (i.e. over functions) that are decidable intensionally (i.e. over programs).

\para{Non-extensional function abstraction?} The correspondence imposed by the $\lambda$-abstraction in Fig.~\ref{Fig:CTT} does not have to be one-to-one. The original $\lambda$-calculus introduced by Alonzo Church in \cite{ChurchA:unsolvable} was not extensional, since the\sindex{extensionality!rule} \emph{extensionality rule}\/ of $\eta$-conversion, discussed in Sec.~\ref{Sec:CTT}, was imposed only later. Intuitively, the rule asserts that $\varphi a = \psi a$ implies $\varphi = \psi$ and hence that $\varphi a = f(a)$ implies $\varphi = \lambda x. f$. Without that rule, there may be $\varphi \neq \lambda x. f$ with $\varphi a = f(a)$ for all $a$, and $\lambda x. f$ is not the sole implementation of $f$. \sindex{lambda-calculus@$\lambda$-calculus!non-extensional} Don't such non-extensional $\lambda$-calculi capture the intensional aspects of computation?

\para{The non-extensional function abstraction is essentially extensional.} A  sequence of results in the 1980s \cite{HayashiS:semifunctors,Koymans,ScottD:relating} demonstrated that every non-extensional $\lambda$-model contains an extensional model as a computable retract. In other words, a non-extensional model can be made extensional by identifying the $\lambda$-terms along a computable extensional equivalence relation, with a $\lambda$-abstraction contained in each equivalence class. The mere presence of function abstraction as an operation makes program abstraction into an operation. 

\para{Bridging the gap?} The extensional models factor out the intensional properties. The intensional models, by Rice's theorem, factor out all nontrivial decidable extensional properties. Neither of the two views subsumes the other. 

Beyond the bifurcation, both paths have in the meantime widened significantly. Church's high-level view of function abstraction and typing provided a mathematical foundation for the programming language design  \cite{ScottD:outline,WinskelG:book}. Turing's low-level approach gave rise to deep mathematical analyses of the computational processes \cite{Vitanyi-Li:book,PapaC:CX}. The traffic across the median moves in both directions, yet reaching an agreement about a solution of equation \eqref{eq:X} still requires scaling the language barriers. 




==> 61-METAPROG/68-work-meta.tex <==
% !TEX root = ../000-monc.tex

\subsection{Is there a fourth Futamura projection?}\label{Work:noFuta}
The three Futamura projections are based on  the same evaluation pattern. In Fig.~\ref{Fig:FirstFuta}, the first one partially evaluates the interpreter $H$ on the $\HHh$-programs. In Fig.~\ref{Fig:SecondFuta}, the second one partially evaluates the specializer $S$ on the interpreter $H$, previously specialized to $\HHh$-programs. In Fig.~\ref{Fig:ThirdFuta}, the third one partially evaluates the specializer $S$ on the instance of itself, previously specialized to the interpreter $H$. Continuing in the same way, a fourth projection would partially evaluate the specializer $S$ on the instance of itself, previously specialized to another instance of itself. Does this projection improve compilation in the same way as the preceding ones?


\subsection{Is iteration all that hyper?} \label{work:hyper}
Looking at Fig.~\ref{Fig:Ackermann}, one might wonder whether we really need mataprogramming here. The function $e:\NNn\to \DP$ is clearly primitive recursive, with $e = \cata{\Xi, \pev W}$. Its diagrammatic definition in Fig.~\ref{Fig:Ackermann} is a special case of the schema in Fig.~\ref{Figure:PR}. The metaprogram for $e$ builds the programs for Ackermann's hyperfunction recursively. The following exercises explore whether this primitive recursive metaprogram can be transformed into a primitive recursive program. Do we really need metaprogramming here?


\begin{enumerate}[a.]
\item Fig.~\ref{Fig:Ackermann} shows that the computation of $m\uparrow^k n$ boils down to the primitive recursion of $e(k)$, and just an $\uev{}$-evaluation of its output $e(k)$ on $n$ and $m$, to get $\uev{e(k)}(n,m) = m\uparrow^k n$.

Answer the following questions.

\begin{enumerate}[i)]
%\item  If we move the final $\uev{}$-evaluation inside the primitive recursive definition of $e$, and evaluate the $\Xi$-branch and the $\pev W$-branch on $n$ and $m$ inside that definition, then the whole definition of Ackermann's hyperfunction would be in the format of primitive recursion. Or not? If not, why not?
%
\item Given the functions $f:\NNn\times A \to \PPp$,  $g:A\to \PPp$, and $h:\NNn\times \PPp \times A\to \PPp$, define
\bear
\varphi(k,x,y) & = & \uev{f(k,x)}y\\
\gamma(x,y) & = & \uev{g(x)} y\\
\chi(k,u,x,y) & = & \uev{h(k,u,x)}y
\eear
Is it true that 
\bea\label{eq:ackerimplic}
f = \cata{g,h} & \stackrel ? \implies & \varphi = \cata{\gamma, \chi}
\eea
Draw the programs and explain the answer.
\end{enumerate}

\item Consider the following function $A:\NNn^2\to \NNn$ (defined and studied by Rozsa P\'eter \cite{Rozsa}) 
\bear
A(0,n) & = & n+1\\
A(k+1,0) & = & A(k,1)\\
A(k+1,n+1) & = & A(k, A(k+1,n)) 
\eear
Prove the following claims:
\begin{enumerate}[i)]
\item $A(k,n) = 2 \uparrow^{k-2} (n+3) -3$
\item Let $\AAA = \{f:\NNn^\ell \to \NNn \ |\  \exists k \forall \vec x \in \NNn.\ f(\vec x)\lt A(k, \hat x)\}$, where $\hat x = \max\{x_1, x_2, \ldots, x_\ell\}$ for $\vec x = (x_1 x_2\ldots x_\ell)$. Then the class $\AAA$ contains the  data services and the successor function, and it is closed under composition and recursion.
\item The function $A$ is not primitive recursive.
\item Ackermann's hyperfunction $\uparrow : \NNn^3 \to \NNn$ is not primitive recursive.
\end{enumerate}
\end{enumerate}



==> 61-METAPROG/69-story-meta.tex <==
% !TEX root = ../000-monc.tex


\subsection[Programming languages]{Programming languages}\sindex{programming!language}
Programming is the art of making computers do what you want.\footnote{If the programming task, a function $f$, is viewed as a problem, then a program $F$ that computes it as $f = \uev F$ is a solution. Programmers thus infuse computers with their problem-solving capacity: the \emph{intelligence}. If computers acquire a problem-solving capacity, and return the favor, then the process of programming will be inverted, and the intelligence will flow in the opposite direction. Artificial intelligence can in that sense become dual to programming. If programming is the process of people telling computers what to do, then artificial intelligence may be the process of computers telling people what to do. The two processes may interleave into a conversation between people and computers.} In the first instance, making a computer do what you want is not all that different from building and running any other machine: you try to anticipate what the components will do, things get complicated, a lot of trial and error. Writing a program directly in a machine language (e.g. as a list of 5-tuples describing a Turing machine to a universal Turing machine) can be immensely frustrating. Some parts are hard to get right, while other parts are repetitive and deadly boring. 

That was the state of affairs in the early days of computer programming. Programming early computers was similar to programming the clockwork-based calculators, built for particular calculations since  XVIII century. But computers are different from calculators. Computers can be programmed to do \emph{anything}. So it didn't take long before people came up with the idea that \emph{computers}\/ could be used to simplify computer programming. E.g., certain fixed lists of machine instructions are repeated in many programs. When executed, they perform some frequently reoccurring operations, such as copying data from one memory location to another, adding binary numbers, etc. Each such list  of machine instructions is grouped into a single \emph{program instruction}; and then a machine program is written, instructing the computer to replace each program instruction with the corresponding list of machine instructions. These program instructions form a \emph{programming language}. 
A programming language whose program instructions are directly translated into machine instructions is called an \emph{assembly}\/ language. A metaprogram that instructs the computer how to replace the assembly language instructions with lists of machine instructions is called an \emph{assembler}. The idea is displayed in Fig.~\ref{Fig:interpret-compile}. 
\begin{figure}[ht]
\begin{center}
\newcommand{\Progtype}{\MMm}
\newcommand{\Lprogtype}{\LLl}
\newcommand{\Hprogtype}{\HHh}
\newcommand{\programnote}{\footnotesize \begin{minipage}{1.05cm}machine\\ program\end{minipage} $\leadsto$}
\newcommand{\mtag}{P_m}
\newcommand{\metaprogramnote}{\footnotesize \begin{minipage}[c]{1.5cm}\centering assembler\end{minipage} $\leadsto$}
\newcommand{\itag}{A}
\newcommand{\compilernote}{\footnotesize compiler $\leadsto$}
\newcommand{\ctag}{C}
\newcommand{\lprogramnote}{\footnotesize \begin{minipage}[c]{1.2cm}low-level\\ program\end{minipage} $\leadsto$}
\newcommand{\ltag}{P_\ell}
\newcommand{\hprogramnote}{\footnotesize \begin{minipage}[c]{1.2cm}high-level\\program\end{minipage} $\leadsto$}
\newcommand{\htag}{P_h}
\newcommand{\Highprogtype}{\HHh}
\newcommand{\Lowprogtype}{\LLl}
%%\newcommand{\EQLS}{\large =}
\def\JPicScale{.42}
\input{PIC/prog-compilation-2.tex}
\caption{Computing machine programs from low-level programs from high-level programs}
\label{Fig:interpret-compile}
\end{center}
\end{figure}
The strings $\MMm$, $\LLl$ and $\HHh$ correspond to three types of programs, in three types of programming languages: the $\MMm$achine languages, the $\LLl$ow-level languages, and the $\HHh$igh-level languages. The program evaluator evaluates programs written in the machine language. One such program is $P_m$. Another such program is an assembler $A$. At least initially, an assembler must also be written in the machine language, because there are no metaprograms, before an assembler is written, that would translate the assembler into the machine code. However, once an assembler is available, then another assembler can be written in the assembly language, and assembled into the machine language by the first assembler. 

It quickly becomes clear that the idea of translating human-written programs into machine-executable programs can be iterated. E.g., it often happens that certain fixed lists of assembly instructions are often repeated in programs of a certain kind, usually within the same application domain. It is then useful to group each such list of \emph{low-level}\/ program instructions into a single \emph{high-level} program instruction, and another metaprogram is written to translate such high-level program instructions into lists of low-level program instructions. A stack of programming languages is created, and the metaprograms are written to translate high-level code to low-level code. Already in the 1950s, for the most important application domains, programmers started developing high-level programming languages. The early ones were the \emph{Algo}\/rythmic \emph{l}\/anguage \emph{Algol}, then also FORTRAN, for FORmula TRANslations and calculations in science and engineering, and a COmmon Business-Oriented Language, standardized in the late 1950s as COBOL. \emph{Algol} was said to be "so far ahead of its time that it was not only an improvement on its predecessors but also on nearly all its successors" \cite{Hoare:hints}. It was probably one of the most studied but least used programming languages in the history of computation. FORTRAN and COBOL are still in use, though for different reasons. COBOL was largely designed by Grace Murray Hopper, one of the first programmers, see Fig.~\ref{Fig:grace-hopper}. She did not name her language,
\begin{figure}[ht]
\begin{minipage}[b]{0.5\linewidth}
\centering
\includegraphics[height=5cm%,viewport = 0 500 500 0,clip
]{PIC/grace-hopper.eps}
\caption{Grace Murray Hopper}% the enemy}
\label{Fig:grace-hopper}
\end{minipage}
\begin{minipage}[b]{0.5\linewidth}
\centering
\includegraphics[height=5cm%,viewport = 0 500 500 0,clip
]{PIC/grace-hopper-bug.eps}
\caption{The original software bug}% the enemy}
\label{Fig:bug}
\end{minipage}
\end{figure}
but she did name a basic concept of computation: the \emph{bug}. The primordial software bug first appeared in Grace Murray Hopper's lab note, see Fig.~\ref{Fig:bug}. She had long suspected that software failures were caused by bugs, and when she finally caught one, stuck in the computer hardware, she duly taped it in the notebook.

Ever since those early days, programming was facilitated by a steady stream of diverse high-level languages, often very domain-specific, habit-specific, and even taste-specific. In 1977 the US Department of Defense (DoD) counted 450 different programming languages in their codebase, and initiated a large project to design a new programming language Ada, to supersede all of them. In 1991, the Ada project was declared a victory, and the DoD mandated that all software procured for them be written in Ada, except in the exceptional, explicitly approved cases. In 1997, after many exceptions, the mandate was removed. Nowadays, the variety of programming languages is greater than ever, but software engineers seem to have adopted the linguistic diversity as a feature of their world, and not a bug.

Programming languages seem to evolve just like natural languages: they undergo a sort of natural (or social, or market) selection. Some of them accumulate random mutations.\footnote{Through the 1980s and 1990s, programming language research  was based on mathematical semantics of computation, and geared towards semantically based language design. The hope was that judicious, mathematically based language design could not only increase programmers' productivity, but also preclude some programming errors. Many of my friends from that research community still do not accept the idea that programming languages evolve like natural languages. Some of them believe in evolution of natural languages, and in intelligent design of programming languages.% Some language designers actually take offense at the statement that programming languages accummulate random mutations.
}  They are still used by people to tell computers what to do; but they are used by many people to tell many computers to do many things, all at the same time. So modern programming is not just a flow of instructions from people to computers, but it involves a great deal of coordination between the programmers, and coordination between computers, and cross-coordinations of all kinds. Most importantly, as nearly all economic and social processes involve software in one way or another, the coordination involved in programming is not always cooperative, but is often competitive, and even adversarial. As social processes are becoming increasingly computational, computation is acquiring social dimensions. For better or for worse, security has grown into one of the central problems of computation.  The basic concepts of software and of complexity are the main milestones on this path.

\subsection[Software systems and networks]{Software systems and networks}
\subsubsection[System programming]{System programming}\sindex{software}
As software applications grew in size, they also grew in complexity. Their computational complexity got formalized and became one of the central concerns in  algorithmics, and the foundation of security in computing and networking. Their architectural complexity became one of the main problems of software engineering. Through years, a whole gamut of methods was devised for partitioning software into components, and for connecting software components into software systems. In order to develop, run, and maintain application software, the programmers need to develop, run, and maintain system software. Some of it gets bundled into \emph{operating systems}, all of it grows in size and complexity. The realm of \emph{system programming}\/ is thus gradually distinguished from the realm of \emph{application programming}. Such partitions of engineering disciplines tend to be often breached, and sometimes confused. The boundary between system programming and application programming is particularly vague, as system programmers often adopt certain applications into their systems, while application programmers sometimes embed system functions into their applications. On the other hand, the interactions of the goals and the needs of application programming and of system programming have left many traces and scars on the landscape of software engineering. We mention some of them.

Early system programs were written in assembly languages. But assembly programming does not scale up, and the high-level programming languages were invented and deployed as soon as large-scale programming projects had to be tackled. Probably the most prominent such language is C, which came after B, which came after BCPL. The UNIX operating system was written in it, and used for the early, friendly versions of Apple's OSX. On the other hand, although designed for system programming, C turned out to be very convenient for application programming, where it was succeeded by C++, which was succeeded by Java, etc. Like people, languages often have more children than parents. Java has aged a little (like some of us) but still occupies a particularly interesting place, where things got a little complicated.

\subsubsection[Portable executables]{Portable executables}
Compiled programming languages dominated the scene as long as programs were designed by programmers, and run by computers. This meant that the \emph{\textbf{software lifetime}}\/ was clearly separated into three phases:
\begin{itemize}
\item \emph{design-time}, when programmers transform ideas into programs, and 
\item \emph{run-time}, when computers transform programs into computations, and in-between them there is
\item \emph{compile-time}, where compilers translate programmers' high-level programs into computers' low-level programs. 
\end{itemize}
All languages mentioned so far are compiled. 

These tidy times ended with the advent of the web. Java was released a couple of years into the web explosion. The web brought network interactions to a new level. Long before the web, software systems were connected into networks, and exchanged messages. But the messages were static: only data. The web significantly expanded the scope of network interactions, initially just by passing around not just data but also \emph{metadata}, that allow web servers to send text formatting and network links to be reconstructed on the client side. Very soon, these enhanced network functions inspired \emph{dynamic}\/ interactions, where web servers distributed not only data and metadata but also some program code, to be executed on the client side.  Such executables distributed on the web are called \emph{applets}. 

The challenge of serving applets on the web was that they had to be \emph{portable executables}, that could be compiled on the server side, and executed on the client side. Since servers and clients run on different machines, all with different machine languages, applets had to be compiled on the server side from a high-level language into an intermediary language, high enough to allow assembly into all clients' machine languages, but low enough to allow efficient interpretation by every client. Java was designed to compile into such an intermediary language,  the \emph{Java bytecode}, which is then interpreted by different interpreters at different machines. 

\para{Historic remark.} The idea of portable executables emerged in 1969, in the early days of ARPANET research. A machine-independent language DEL was specified, and an interpreter was prototyped at SRI in Menlo Park. The project was discussed and definition of the language was announced in the Network Working Group RFC 5. %\cite{rfc5}. 

\subsubsection[Interpreters and scripting]{Interpreters and scripting} \sindex{scripting|see {programming language, scripting}}\sindex{interpreter}\sindex{programming! language!scripting}
In a basic computer, programs are directly evaluated. If programs are coded in a high-level language, then the evaluator must be programmed in a machine language, at least initially. So there must be an interpreter for the high-level language. If we partially evaluate that interpreter, we get a compiler. That was the first Futamura projection, Fig.~\ref{Fig:FirstFuta}. Since compilation provides an opportunity for optimizations, the high-level languages of the first generation of were always compiled. But when software systems got connected into networks, the compilation phase of high-level code into a machine executable had to be split into a compilation on the server side into a portable executable, and an interpretation on the client side into a machine executable. This software evaluation scenario was realized in Java, and many variations have been realized in other languages.

Another boost for interpreters came from a different direction at the same time. Since the early days of system programming, a divide of the development tasks into \emph{programming-in-the-small}\/ and \emph{programming-in-the-large}\/ was felt and discussed. %\cite{prog-small-large} 
With the growth of software systems in size and scope, the large became larger, the divide increased, and new  languages for programming-in-the-small started emerging: the \emph{scripting}\/ languages. %\cite{ousterhout}. 
Nowadays, we use JavaScript, PHP, Perl for web programming. They are all purely interpreted languages. Scripting for the web is metaprogramming of computations with metadata.  For different reasons, Matlab, Mathematica, or any language underlying a spreadsheet is also interpreted.

\para{What do Java and JavaScript have in common?} Both are mentioned in the story about interpreters. Both emerged with the web. Both have "Java" in their name. Other than that, they could hardly be more different. One has objects and classes, the other throws everything on the heap. Java was designed at Sun Inc in 1991, as a language for programming appliances, like set-top boxes and washing machines. The portability requirement meant that the compiled code should be suitable for different appliances. The design was deemed "too advanced", as the thought of streaming TV was still some years away, and the web was only just conceived. So the project was shelved. But a couple of years later, in May 1995, the designers of Netscape web browser came to Sun Inc to ask for a language that could be compiled to portable executables, and got Java. They also needed an interpreter for web scripts, and when they settled on Java, they wanted to make the syntax of their scripting language maximally similar to Java. One of them, Brian Eich, specified a Java-like syntax for a scripting language over a weekend, prototyped the needed interpreter in 10 days, and it shipped in Netscape Navigator 2.0 in September 1995. The name JavaScript settled a couple of months later.

\subsection{Software}\sindex{software}
Software makes computation into a large-scale process. The basic concepts of computation become tools of computation \cite{JonesN:book-computability}
\begin{itemize}
	\item the \textbf{program evaluators} become the \textit{interpreters}, whereas
	\item the \textbf{partial evaluators}  become the \textit{specializers}.
\end{itemize}
Partially evaluating programs for  those basic components generates compilers, compiler generators, and other varieties of familiar or less familiar program transformers. 

Programming program transformers is an instance of metaprogramming. Metaprogramming can be construed as the main feature of programmable computation: that programs themselves can also be computed, and the computations that compute programs can themselves be programmed. And so on.

If programs describe computations, then software is the narrative comprised of descriptions. If programs are generated by applying some program constructor schemas (induction, recursion, parallel and sequential composition, bounded and unbounded search, etc.) on some basic operations (logical and arithmetic), then software is generated by applying software patterns and architectures to build systems from programs. If the basic operations are letters, then programs are words, software components are sentences, software systems are stories.

But some stories cannot be told in a linear narrative: "this happened, and then that happened, and then something else". You have to pop up a level, make some abstractions, and tell a story about the story. Similarly, when a computational task does not yield to applying standard program constructions, like in the case of the Ackermann function in Sec.~\ref{Sec:iteration}, then you pop up a level up, make new abstractions, and metaprogram. Instead of composing operations to process data, you compose abstractions the process algorithms. The Ackermann function and the transfinite counting cannot be programmed using the recursion schema, so they get metaprogrammed. The infinities, by definition, cannot be reached by simple counting, but they are reached by iterating, i.e. by counting the counting processes. This took in  the preceding chapter us to the constructions of transfinite ordinals as primordial metaprograms, and back to Cantor as the originator, along the lines mentioned in Sec.~\ref{Sec:work-wire}, of the finite descriptions of infinite processes that we now call programs. A particular "program" due to Cantor will play a central role at the end of the next chapter as well.




%
%
%
%Remarkably, we encounter Georg Cantor here at the beginning of the story, and we will encounter him again at the very end. At the beginning, well before the notion of computability was defined, Cantor enters scene as the misunderstood originator of the "canvas" of the \emph{foundations of mathematics}. This is "Cantor's Paradise" from which, Hilbert asserted, mathematicians should never be expelled. At the end, Cantor's construction plays the central place in proving the uniqueness of computability. In the meantime, the edifices of the universes of mathematics and comutation were painted upon Cantor's foundational canvas, built upon misunderstandings.
%
%
%Why categories?
%
%Why types and not sets? --- Groups for invariant preservation, not matter.
%
%Cantor: types. Russell: types.




==> 71-STATE/78-work.tex <==
% !TEX root = ../000-monc.tex

\subsection{Lossless simulations}\label{Work:lossless}\sindex{simulation!lossless}
\para{Idea.} A simulation is called lossless if it records the states that it simulates. The idea is that the  execution trace should be something like: 
\beq\label{eq:lossless-sim}
\begin{split}
\prooftree
\prooftree
\hspace{3.5em}a_1\ ,\hspace{5em} a_2\  ,\hspace{5em}a_3\ ,\hspace{3em}  \ldots
\justifies
\hspace{1.4em} x_0 \hspace{1.4em} \xmapsto{a_1/b_1}\hspace{1.4em} x_1\hspace{1.4em} \xmapsto{a_2/b_2} \hspace{1.4em} x_2 \hspace{1.4em}\xmapsto{a_3/b_3} \hspace{1.4em} x_3 \hspace{1.4em}  \cdots
\endprooftree
\justifies
\pairr{x_0}{Qx_0} \xmapsto{a_1/b_1} \pairr{x_1}{Qx_1}\xmapsto{a_2/b_2} \pairr{x_2}{Qx_2} \xmapsto{a_3/b_3} \pairr{x_3}{Qx_3}  \cdots
\endprooftree
\end{split}
\eeq
Lossless programs can be refined to record all of the previous states and acummulate the execution traces as they go. They are processed in \sindex{program!execution!lossless} \emph{lossless}\/ executions. A lossless program is obviously faithful, but it may not be full.

\para{Construction.}  Any program $Q:X\stricto \DP$ for a \procs\ $q\colon X\times A\to X\times B$ is expanded into a lossless one using $\widetilde{Q}: X\times X \stricto \DP$ with  
\beq\label{eq:padded-idea}
\widetilde{Q} (x,x')  \  = \    \pairr x {Qx'}\qquad\qquad\mbox{and}\qquad\qquad \overline Q x = \widetilde{Q}(x,x)
\eeq 
Given a program execution \procs\ $\puniversal:\DP\times A\to \DP\times B$ for general programs $Q$, the lossless versions   $\overline Q$ should be executed using the lossless simulator $\PadRunn:\DP\times A\to \DP\times B$ satisfying
\beq
\sta{\PadRun{\overline Qx}}a \  = \ \big\lceil{x}\, , \sta{\puev{Qx}}a\big\rceil \qquad\qquad\qquad\qquad \out{\PadRun{\overline Qx}}a \  = \ \out{\puev{Qx}}a
\eeq
Draw the programs as diagrams and prove that they work as required.

\subsection{Program execution as a polymorphic operation}\label{Work:exee}
In Sec.~\ref{Sec:surj}, the \runn-instruction was presented as an $X$-natural family of surjections 
$$\CCC(X\times A\, ,\,  B) \begin{tikzar}[row sep=-.25em,column sep=1em]
\hspace{0.01em}  \&\&\& \hspace{0.01em} \arrow[twoheadrightarrow,bend right=16]{lll}[swap,pos=0.45]{\runn^{AB}_X}
\end{tikzar}\tot \CCC(X, \DP)$$  
indexed over all pairs of types $A,B$. For each pair, the family was induced  by the program evaluator in Fig.~\ref{Fig:gamma}, naturally with respect to \strict\ \funnn s in Fig.~\ref{Fig:gamma-nat}. The \strict\ \funnn s form the category $\tot \CCC$.   

\begin{figure}[!ht]
\begin{center}
\begin{tikzar}[row sep=1em,column sep=1em]
\CCC(\DP \times A, \DP\times B) \arrow[two heads]{dddddd}[description]{(\pi_X\times B)\circ(-)\circ(\Theta\times A)}  
\&\&\&\&\&\&
\CCC(\DP \times A, \DP\times B)   \arrow[two heads]{llllll}{(-)\circ(\pi_1\times A)}
\&\&\&\&\&\&
\tot \CCC(\DP,\DP) \arrow[two heads]{dddddd}[description]{(-)\circ\Theta}  \arrow[two heads]{llllll}{\runn^{A(\DP B)}_\DP} \arrow[two heads,bend right=13]{llllllllllll}[swap]{\exee^{AB}_\DP} 
\\[2.25ex]
\&\Runn \arrow[mapsto]{dddd} \&\&\&\&\& \universal \arrow[mapsto]{lllll}  \&\&\&\&\& \id_\DP \arrow[mapsto]{dddd} \arrow[mapsto]{lllll} \\
\\
\\
\\
\& (\pi_X\times B)\circ \Run \Theta \&\&\&\&\&\&\&\&\&\&  \Theta \arrow[mapsto]{llllllllll} 
\\[2.25ex] 
  \CCC(X\times A, X\times B) 
 \&\&\&\&\&\&   \CCC(X\times A, \DP \times B) \arrow[two heads]
 {llllll}[swap]{(\pi_X\times B)\circ(-)\circ(\pi_1\times A)}
 \&\&\&\&\&\&
  \CCC^\ast(X,\DP)  \arrow[two heads]
 {llllll}[swap]{\runn^{A(\DP B)}_X}\arrow[two heads,bend left=13]
 {llllllllllll}{\exee^{AB}_X}
\end{tikzar}
\caption{Program execution as a polymorphic surjection of imperative programs}
\label{Fig:exee}
\end{center}
\end{figure}

In a similar way, the program executions induce a family of surjections 
\beq\label{eq:surj-exe}
\CCC(X\times A\, ,\,  X\times B) \begin{tikzar}[row sep=-.25em,column sep=1em]
\hspace{0.01em}  \&\&\& \hspace{0.01em} \arrow[twoheadrightarrow,bend right=16]{lll}[swap,pos=0.45]{\exee^{AB}_X}
\end{tikzar}\CCC^\ast (X, \DP)
\eeq 
Where $\CCC^\ast (X, \DP)$ denotes the set of imperative programs over the state space $X$. Their construction of the execution operations $\exee^{AB}$ for all pairs of types $A, B$ is displayed in Fig.~\ref{Fig:exee}. Each of them is \emph{polymorphic}, in the sense that the outer rectangle commutes for all types $X$ and all imperative programs $\Theta\colon X\stricto \DP$. It follows that for every pair $A,B$, the instruction $\exee^{AB}$ is  induced by the universal program execution \procs\ $\exee^{AB}_{\DP}\left(\id_{\DP}\right) = \Runn$.  In contrast with the \runn-instruction, the \exee-instruction is, however, not natural with respect to a class of \funnn\ extending the imperative programs.  Explain how the \exee-instruction is induced polymorphically by the padded program executions from Workout~\ref{Work:lossless}. %why does this polymorphism not extend to naturality with respect to a nontrivial family of computable \funnn s.

%
%
%This time, the naturality is with respect to the $\retr$-split \funnn s in the category $\CCC_\retr$ defined 
%\bea
%\lvert \CCC_\retr \rvert & = & \lvert \CCC \rvert\\ 
%\CCC_\retr(X,Y) & = & \left\{ u\in \CCC(X,Y)\ |\ \retr^{YX}\circ u = \id_X \notag
%\right\}
%\eea
%where $\retr^{YX}\in \CCC(Y,X)$, if it exists, retracts $Y$ to $X$ consistently with the retractions 
%$$\retr^X =\left(\DP\eepi\universal X\right)\qquad\mbox{ and }\qquad \retr^Y =\left(\DP\eepi\universal Y\right)$$ from Sec.~\ref{Sec:retracts}. In summary, the $\CCC_\retr$-morphisms make the following diagrams commute for all $A,B$.
%\[\begin{tikzar}[row sep = large,column sep=large]
%X\ar[equals,thin]{d} \& \DP \ar[two heads,thin]{l}[description]{\retr^X}\ar[two heads,thin]{d}[description]{\retr^Y}\\
%X \ar[tail,thick]{r}[description]{u} \& Y\ar[two heads,thin]{ul}[description]{\retr^{YX}}
%\end{tikzar}
%\]
%The functors in \eqref{eq:surj-exe} are contravariant (a reader familiar with categories with recognize them as \emph{presheaves}\/ \cite[Sec.~IV.10]{MacLaneS:CWM}) over $\CCC_\ast$. They are defined
%%\begin{align*}
%%\CCC_{(\ast)}(-\times A\, ,\,  -\times B)\  \colon\ \  \CCC_\ast^{o} & \tto{\hspace{3em}} \Set &  \CCC^\ast_{(\ast)}(-, \DP)\ \colon\ \  \CCC_\ast^{o} & \tto{\hspace{2em}} \Set\\
%%X & \longmapsto \CCC(X\times A, X\times B) & X & \longmapsto \CCC^\ast(X, \DP)
%%\end{align*}
%\begin{align*}
%\CCC_{\ast}(-\times A\, ,\,  -\times B)\  \colon\ \  \CCC_\retr^{o} & \tto{\hspace{3em}} \Set &  \CCC^\ast(-, \DP)\ \colon\ \  \CCC_\retr^{o} & \tto{\hspace{2em}} \Set\\
%\left(\ \ \begin{tikzar}[cramped,sep = 5ex]
%\scriptstyle X\ar[tail]{d}[description]{u}\\
%\scriptstyle Y\end{tikzar}\ \  \right) & \longmapsto\  \left(\ \ \ \begin{tikzar}[cramped,sep = 5ex]
%\scriptstyle \CCC(X\times A, X\times B)\\
%\scriptstyle \CCC(Y\times A, Y\times B) \ar[two heads]{u}[description,pos=0.4]{u^\#}\end{tikzar}\ \ \ \right)  
%&
%\left(\ \ \begin{tikzar}[cramped,sep = 5ex]
%\scriptstyle X\ar[tail]{d}[description]{u}\\
%\scriptstyle Y\end{tikzar}\ \  \right) & \longmapsto\  \left(\ \ \ \begin{tikzar}[cramped,sep = 5ex]
%\scriptstyle \CCC^\ast(X, \DP)\\
%\scriptstyle \CCC^\ast(Y, \DP) \ar[two heads]{u}[description,pos=0.4]{^o u}\end{tikzar}\ \ \ \right)  
%\end{align*}
%where the object parts are, respectively, the sets of \procs es $\CCC(X\times A,X\times B)$ and the sets of imperative programs\sindex{program!imperative} 
%\bear
%\CCC^\ast(X,\DP) & = & \left\{Q\in \tot\CCC(X,\DP)\ |\ \pi_X\circ Q = \id\ \wedge (Q\circ\pi_X\times B)\circ\Run Q = \Run Q \right\}
%\eear
%and the arrow parts are
%\bear
%u^\#\left(Y\times A\tto r Y\times B\right) & = & \left(X\times A\tto{u\times \id} Y\times A\tto r Y\times B \tto{\retr\times \id}X\times B \right)\\
%^o u\left(Y\strictto R \DP\right) & = & \left(X\strictto{u} Y\strictto R \DP \right)
%\eear
%To verify the soundness of the arrow part of $\CCC^\ast(-,\DP)$, take $R\in \CCC^\ast(Y,\DP)$. 
%
%
% follows from the fact that $\retr^{YX}\circ\retr^Y=\retr^X$ implies $\retr^{YX}\circ \pi_Y = \pi_X$ follows from \eqref{eq:pis}
%
%





==> 71-STATE/79-story.tex <==
% !TEX root = ../000-monc.tex


\para{Universality from abstract to concrete.}\sindex{universality}
In this chapter we closed the loop of universality. We started the tour of computers as universal machines in Ch.~\ref{Chap:Comput} with universal programmability of all \funnn s computable in a monoidal computer. From chapter to chapter, we derived more concrete programs. In the present one, we showed that abstract programmability of computable \funnn s implies concrete programmability of computational \procs es. This descent from abstract program evaluations to concrete program executions can be interpreted as a climb from the Church-Turing Thesis to the corresponding Antithesis \sindex{Church-Turing!Thesis} sketched in Sec.~\ref{Sec:CTA}\footnote{This climb from the Church-Turing Thesis to the Church-Turing Antithesis is a logical development, not historic. Church's and Turing's models emerged at the same time. It is a historic fact that they developed independently (although Church was Turing's thesis advisor). It is a logical fact that Church's view evolved into the extensional view of computation, as it manifests itself, e.g., in domain theory, whereas Turing's view evolved into the intensional view, as ,e.g., in complexity theory.}.\sindex{Church-Turing!Antithesis} Church viewed computation as a discharge of \funnn\ applications charged by  \funnn\ abstractions. Turing viewed computation as a \procs, and specified his machine model by looking at human computers. Stateful computers are the interfaces between the internal states of mind and the external states of the world. E.g., to multiply integers, I store the multiplication tables and the carryovers internally, write the intermediary results externally, and read this trail of breadcrumbs to add them up, again using the internally stored tables and carryovers, this time for the addition, and writing the final result externally. Turing mechanized such stateful \procs es using the states of an abstract machine as the internal memory and its virtual tapes as the external memory. The \procs\ of jointly updating the internal and the external states of a state machine was specified as a list of instructions --- a program. Turing noticed that programs could also be executed by a state machine as inputs, just like the numbers can be processed into sums or products. The machine executing the programs was thus universal in the sense that it could execute all \procs es that state other machines could execute. Yet it was not universal enough to decide its own Halting Problem, as we saw in Sec.~\ref{Sec:halting}. This negative result was the main point of \cite{TuringA:Entscheidung}. Its positive result was that, a couple of years and a world war later, Turing's abstract machines crystallized into electronic computers, and the human computers evolved into programmers. 

\para{Process calculi.} \sindex{process!calculus} A couple of decades of programming later, Turing's Halting Problem and the other no-go theorems from Ch.~\ref{Chap:Undec}, saying that no nontrivial properties of computations generally can be read off from their programs, grew into the practical problem that programmers often weren't sure what exactly their programs meant, i.e. what they did. Computational behaviors turned out to be not just undecidable in principle, but hard to comprehend in practice. The efforts to solve this problem led to the idea of mathematical semantics of computation \sindex{semantics of computation}  \cite{Engeler:semantics,Scott-Strachey:semantics,ScottD:outline}. Abstract machines re-emerged, this time not as low-level models of computers but as high-level models of computations. Stateful computations. State machines were previously used by Mealy to synthesize circuits \cite{MealyG} and by Moore to distinguish externally observable computational behaviors from their internal implementations \cite{Moore:Gedanken}. Robin Milner reinterpreted them as computational \procs es \cite{MilnerR:processes}. In Milner's work, Moore's idea of \emph{Gedanken}-experiments, as a semantical link between observable behaviors and their implementations, became a stepping stone into the vast area of \sindex{process!calculus}  \emph{process calculi}\/ as metalanguages of computation \cite{HoareCAR:CSP,MilnerR:CCS,MilnerR:space}. The diagrams on the blackboard behind Milner in Fig.~\ref{Fig:milner} represent processes in his calculus of bigraphs, to which he arrived after some 30 years of work. The idea of \sindex{simulation} simulations between processes, sketched in Sec.~\ref{Sec:simul}, appeared at the beginning of that journey, in \cite{MilnerR:CCS80}. It arose from the insight that observable computational behaviors do not boil down to computable  \funnn s but always include side-effects and often involve state updates.  \sindex{side-effect} In monoidal computers, the side-effects are what makes computable \funnn s monoidal: some of them diverge, some raise exceptions, other produce many different outputs on the same inputs, due to possible, probable, parametrized, non-deterministic aspects of computers and of their environments. Already Turing proved in \cite{TuringA:Entscheidung} that there are always some computations that must diverge. Milner added in \cite{MilnerR:processes} that the interactions of internal and external states imply there are always other side-effects as well. % Computation is a stateful process where the states of the world and the states of mind update each other. 

\para{Idea of simulation.} A pair of processes implementing the same input-output mapping but causing different side-effects is displayed in Fig.~\ref{Fig:icecream}.\sindex{side-effect} A similar example was the starting point of \cite{MilnerR:CCS80}. Jack wakes up and proceeds towards the fridge to get an ice cream or a glass of juice. The only inputs that Jack enters in the \procs\ as it progresses  towards his goal is to keep going, instances of a \emph{``Go!"}-instruction, so we take the input type to be $A \cong 1$ and ignore it. We take the desired outputs and the two state spaces for two implementations of Jack's quest to be:
\[B \ =\  \{\mbox{fridge}, \mbox{ice cream}, \mbox{juice} \}\qquad\qquad
X \ =\   \{x_0, x_{\rm fi}, x_{\rm fj}, x_{\rm i}, x_{\rm j} \}\qquad\qquad
Y \ =\  \{y_0, y_{\rm f}, y_{\rm i}, y_{\rm j} \}
\]
Consider the \procs es $q\colon X\to X\times B$ and $r\colon Y\to Y\times B$, displayed in Fig.~\ref{Fig:icecream}. 
\begin{figure}[!ht]
\begin{center}
\newcommand{\fridge}{fridge}
\newcommand{\icecream}{ice cream}
\newcommand{\juice}{juice}
\newcommand{\xooo}{x_0}
\newcommand{\xice}{x_{\rm i}}
\newcommand{\xjuice}{x_{\rm j}}
\newcommand{\xfice}{x_{\textrm{fi}}}
\newcommand{\xfjuice}{x_{\textrm{fj}}}
\newcommand{\yooo}{y_0}
\newcommand{\yice}{y_{\rm i}}
\newcommand{\yjuice}{y_{\rm j}}
\newcommand{\yfridge}{y_{\rm f}}
\def\JPicScale{.45}
\input{PIC/icecr.tex}
\caption{Two \procs es of getting a juice or an ice cream from a fridge}
\label{Fig:icecream}
\end{center}
\end{figure}
In the \procs\ $r$, Jack goes to the fridge and gets the ice cream or the juice, whichever he lays his hand on. In the \procs\ $q$, Jack decides in advance whether he wants juice of ice cream, and the process branches at the beginning. If the decision is to get an ice cream but there is only juice in the fridge, then the \procs\ $q$ will deadlock after Jack reaches the fridge. Ditto the other way around. The two \procs es have the same input-output behavior, since two \emph{``Go!"}\/-inputs lead to the same possible outputs
\[\Big\{(\mbox{fridge};\mbox{ice cream}), (\mbox{fridge};\mbox{juice})\Big\}\]
The difference beetween the two \procs\ is that $r$ always terminates if there is either juice or ice cream in the fridge, whereas $q$ deadlocks if Jack's initial choice is not available in the fridge. Formally, this difference is captured by the fact that $r$ can simulate $q$ but $q$ cannot simulate $r$. The simulation $s\colon q\to r$ is realized by the \strict\ \funnn
\bear
s\colon X & \stricto & Y\\
x_{\rm z\ast} & \mapsto & y_{\rm z}
\eear
where z is f, i, or j, and $\ast$ is empty or not. Whenever $q$ makes a step $x\xmapsto{\ \rm z\ } x'$, $r$ makes a step $sx\xmapsto{\ \rm z\ } sx'$. To see that there is no simulation in the opposite direction, note that $r$ starts with $y_0\xmapsto{\mbox{\tiny fridge}} y_{\rm f}$ and 
$q$ with either $x_0\xmapsto{\mbox{\tiny fridge}} x_{\textrm{fi}}$ or  $x_0\xmapsto{\mbox{\tiny fridge}} x_{\textrm{fj}}$. A simulation of $r$ by $q$ should map $y_{\rm f}$ to either $x_{\textrm{fi}}$ or $x_{\textrm{fj}}$. In the first case, $q$ will be stuck whenever there is no ice cream, whereas $r$ will proceed to $y_{\rm f}\xmapsto{\mbox{\tiny fridge}} y_{\rm j}$. Since $q$ is unable to follow $r$'s step, there is no simulation. Similarly in the second case, if $y_f$ is simulated by $x_{\textrm{fj}}$.

\para{Coalgebra.} In categories, \procs\  are presented as coalgebras \sindex{coalgebra, coinduction} and simulations are captured as coalgebra homomorphisms \cite{AdamekJ:coalg,Barwise-Moss:vicious,JacobsB:book-coalg}. The underlying method of \emph{coinduction}\/ provides a common ground for impredicative reasoning about computational processes in computer science and natural processes in mathematical analysis \cite{RuttenJ:stream,PavlovicD:retracing,PavlovicD:MSCS17,PavlovicD:LICS98,RuttenJ:universal}. %Different observables captured by different functors lead to different coalgebras, different simulations, and different \procs\ semantics. With the coinductive aspects often implicit, the categorical approach has been an indispensable tool of semantics of computation from the outset, refining the extensional theory of computability into denotational semantics of type systems and operational semantics of programming languages.

\begin{figure}[!ht]
\centering
\begin{minipage}[b]{0.35\linewidth}
\centering
\includegraphics[height=5cm%,viewport = 0 500 500 0,clip
]{PIC/Descartes.eps}
\caption{Ren\'e Descartes}
\label{Fig:descartes}
\end{minipage}
\hspace{0.1\linewidth}
\begin{minipage}[b]{0.45\linewidth}
\centering
\includegraphics[height=5cm%,viewport = 0 500 500 0,clip
]{PIC/milner-speaks.eps}
\caption{Robin Milner}
\label{Fig:milner}
\end{minipage}
\end{figure}

\para{Metaphysical troubles with simulations: Cartesian doubt.}
Simulation is a concept with deep repercussions. Its consequences resonate through the foundations of modern science from their origin in the work of Ren\'e Descartes, looking on from Fig.~\ref{Fig:descartes}. Descartes did not use a mathematical formalization of simulation like the one in Sec.~\ref{Sec:simul} (mainly because the notion of formalization was yet to be formalized), but he drew its fundamental logical consequences (and on the way invented some of the main formats of mathematical formalizations). If different \procs es can simulate each other and no observations can distinguish them, then how can I know which one I am observing? If mechanical toys simulate animals, and all animal functions can be simulated by causal mechanisms, then how can I be certain that I am not surrounded by mechanical simulations? This type of reasoning led to the \emph{cartesian\footnote{\emph{Cartesius}\/ was Descartes' name in Latin. The system of coordinates that he used (though never explicitly defined) in his geometry is therefore known as the \emph{cartesian} coordinates. His philosophy is the \emph{cartesian}\/ philosophy, and his doubt is the \emph{cartesian doubt}.} doubt},\sindex{cartesian doubt} the driving force behind Descartes' investigations and an update of the starting point of Aristotle's metaphysics\footnote{``Why is there something, rather than nothing?''} into a starting point of modern science. Proceeding along his path, scientific methodologies have been striving to address the doubts about the reality of our observations and the soundness of our conclusions. Ever since Descartes, each generation raised the doubt that we might be living in a simulation again and again, in their own styles and languages, aware or unaware of Descartes' meditations about it. The doubts whether the reality is real or simulated nowadays fill the space from combinatorial physics through popular philosophy to action movies. Descartes' own  resolution of the cartesian doubt was to authenticate reality by observing the reality of the doubt itself: \emph{``Cogito, ergo sum"} --- ``I am thinking, therefore I exist". Even if all animals around me are \sindex{cogito} simulations, all simulations are interpreted in my mind, so at least my mind cannot be a simulation. Or can it? \emph{``Can human mind be simulated?"}\/ --- Turing asked.\sindex{Turing Test}

\para{Descartes, Turing, and Milner} are not discussed together very often, probably for a good reason. But their different pursuits of the problems of simulation and indistinguishability got entangled in computers. Milner formalized \procs\ semantics and studied what is observable, how \procs es simulate each other, and how to tell them apart. Turing modeled human computers as abstract computers, and when his abstract computers came into being as  electronic computers, he had to wonder  whether computers could simulate humans, and how to tell them apart. Descartes modeled natural \procs es as mechanical \procs es, noticed that one could simulate the other, and wondered how to tell them apart. We transition into the next one with a bird's eye view of the common thread of their stories.\footnote{A bird's eye, of course, misses many details and many other stories through which the same thread is woven.}

\para{Observations are simulations.} The notion of simulation $s\colon q\to r$ starts out from a simulating \procs\ $r$ and a simulated \procs\ $q$. Since $r$ makes the same steps as $q$, it observes $q$ as its own subprocess. If two \procs\ $q'$ and $q''$ induce the same sub\procs\ $r_q\inclusion r$, then $r$ cannot tell them apart, as shown in Fig.~\ref{Fig:rq}. 
\begin{figure}[!ht]
\begin{center}
\begin{tikzar}[row sep=2em,column sep=2em]
\&\&\& Y \times B
\\   
X'\times B \ar[two heads,bend right=10]{rr} \&\& Y_{q} \times B \ar[hook]{ur} \&\& Y\times A  \ar{ul}[description]{r} 
 \\ 
 \& X'\times A \ar{ul}[description]{q'} \ar[two heads,bend right=10]{rr} 
 \&\& Y_{q} \times A  \ar[hook]{ur} \ar{ul}[description]{r_{q}} 
 \\
\&\& X''\times B \ar[crossing over,two heads,bend left=17]{uu}
\\
 \&\&\& X''\times A \ar{ul}[description]{q''} \ar[two heads,bend left=15]{uu}
 \end{tikzar}
\caption{Processes $q'$ and $q''$ are indistinguishable for the observer $r$
}
\label{Fig:rq}
\end{center}
\end{figure}
The \procs\ $q'$ and $q''$ are  \emph{observationally indistinguishable}\/ for $r$. Simulations convey to the simulator what is observable and filter out the irrelevant implementation details as unobservable. \emph{\textbf{To observe is to simulate internally.}} 

\para{A universal simulator is a universal observer.}\sindex{universal!simulator}\sindex{universal!observer} When a \procs\ $q\colon X\times A\to X\times B$, implemented by a program $Q\colon X\stricto \DP$ in the sense of Fig.~\ref{Fig:exec-eval}, consumes inputs $a_{1}, a_{2}, a_{3},\ldots$ and produces a computation
\[x_0 \hspace{0.35em} \xmapsto{a_1/b_1}\hspace{0.35em} x_1\hspace{0.35em} \xmapsto{a_2/b_2} \hspace{0.35em} x_2 \hspace{0.35em}\xmapsto{a_3/b_3} \hspace{0.35em} x_3 \hspace{0.35em} \xmapsto{\hspace{1.3em}} \cdots
\]
where $x_{i+1} = \sta q_{x_{i}}(a_{i})$ and $b_{i+1} = \out q_{x_{i}}(a_{i})$, then this computation is observed by a universal simulator $\puniversal\colon \DP\times A\to \DP\times B$ as the execution of $Q$
\[Qx_0 \xmapsto{a_1/b_1} Qx_1\xmapsto{a_2/b_2} Qx_2 \xmapsto{a_3/b_3} Qx_3 \xmapsto{\hspace{1.3em}} \cdots
\]
where $Qx_{i+1}=\sta{\puev{Qx_{i}}}a_{i}$ and $b_{i+1}=\out{\puev{Qx_{i}}}a_{i}$. 
If two \procs es are indistinguishable for the universal simulator, then they are indistinguishable for every simulator; if there is an observable distinction, the universal simulator will observe it. By specifying what is observable, a universal simulator as universal observer determines a \procs\ semantics.\sindex{universality}

\para{Universal simulations.} When a universal \procs\ $\puniversal_{0}\colon \DP_{0}\times A\to \DP_{0}\times B$ simulates another universal \procs\ $\puniversal_{1}\colon \DP_{1}\times A\to \DP_{1}\times B$, all \procs es that $\puniversal_{0}$ observes are simulations $\DP_{1}\stricto \DP_{0}$. Observer $\puniversal_{0}$'s world is simulated by the simulator $\puniversal_{1}$. Descartes' \emph{cogito}\/ says that there is still at least one \procs\ that  $\puniversal_{0}$ can observe directly: $\puniversal_{0}$ itself. The universal \procs\ $\puniversal_{0}$ observes itself through the identity simulation $\DP_{0}\strictto{\id} \DP_{0}$. However, the universality of $\puniversal_{1}$, as discovered by Turing and discussed in Ch.~\ref{Chap:Comput}, implies that $\DP_{0}$ is a retract of $\DP_{1}$ along
\bear
\id_{\DP_{0}} & = & \left(\DP_{0}\begin{tikzar}[column sep=3.6em]
\hspace{-.3em}
\arrow[tail]{r}{\incl_A=\enc}[description,pos=.95]{\!\!\!\mbox{\large$\bullet$}\!}\&%
\hspace{-.3em}\end{tikzar} \DP_{1} \begin{tikzar}[column sep=3.4em]\hspace{-.3em}\arrow[two heads]{r}{\retr^A=\{\}}\&\hspace{-.2em}\end{tikzar}  \DP_{0}\right)
\eear
Even $\puniversal_{0}$'s identity may be simulated by $\puniversal_{1}$. In the world of computers, \textbf{\emph{``Cogito, ergo sum''}\/ may be false.} The thoughts that I am observing may be simulated.

In the next chapter we show that \emph{it does not matter}. Universal simulators may simulate each other, but they cannot deceive each other more than each of them can deceive itself on its own.

==> 81-PCC/88-work.tex <==
% !TEX root = ../000-monc.tex

\subsection{Exercises}
\begin{enumerate}[a.]

\item \label{Exercise:inf-sup-prog} Draw programs as diagrams for the infima in   \eqref{eq:pwedge} and for the suprema with respect to the same order.

\item Draw a diagram for program  \eqref{eq:prd}.

\item\label{Work:order} Verify the claim that every decidable type must be well-ordered as soon as $\DP$ is well-ordered

\item Recall from Sec.~\ref{Sec:retracts} that any computable type $A$ corresponds to a computable  idempotent $\rho_A:\DP\to \DP$ \sindex{type!as idempotent} such that $x=\rho_A(x)$ just for $x:A$. Prove that $\rho_A$ is \strict\ if and only if the \sindex{predicate!characteristic} characteristic predicate $\chi_A:\DP\to\Bool$ is decidable, where $\chi_A(x) = \left(x\iseq \rho_A(x)\right)$.

\item Given a monotone unbounded \strict\ \funnn\ $f\colon A\stricto B$ and $f^{*}\colon B\stricto A$ defined by \eqref{eq:f-ast}, verify that  
\begin{enumerate}[i)]
\item $f^\ast \circ f(x) \pleq x$ and $y \pleq f\circ f^\ast(y)$ hold for all $x\colon A$ and $y\colon B$;
\item $\overleftarrow f = \left(A\strictto f B\strictto{f^\ast} A\right)$  and $\overrightarrow f = \left(B\strictto{f^\ast}A\strictto{f} B \right)$ 
are idempotent;
\item the splittings $A_{f}$ of $\overleftarrow f$ and $B_{f}$ of $\overrightarrow f$ are isomorphic;
\item there is $x\colon A$ such that $f(x)=y$ if and only if $f\circ f^\ast(y) = y$, i.e. $y\colon B_f$.
\end{enumerate}

\item Verify that the isomorphism constructed in Sec.~\ref{Sec:hartley} preserves the program executions, i.e. that both of its componenets are simulations.

% \end{enumerate}
% 
%\subsection{Surjective pairing}
\item \label{Work:surjective-pairing}
\sindex{pairing!surjective}
Given a programming language $\DP$ with program execution machines $\Runn\colon\DP\times A\to \DP\times B$, show that $\DP^{2}= \DP\times \DP$ is also a programming language, with the program execution machines  $\Runn^{2}\colon\DP^{2}\times A\to \DP^{2}\times B$ defined 
\bea
\Run{F_{0},F_{1}}^{2} & = & \Run{F_{1}}
\eea
Use the Isomorphism Theorem to conclude that every program-closed category supports an isomorphism
\beq\label{eq:surjective-pairing} 
\DP\times \DP \begin{tikzar}[column sep = 6em]
\hspace{-.2em} \arrow[nothing-cart,bend right=20,shorten=.75mm]{r}[swap]{\pairr - -} \ar[phantom]{r}[description]{\cong} \& \hspace{-.2em} \ar[nothing-cart,bend right=20,shorten=.75mm]{l}[swap]{\left<\fstt - , \sndd -  \right>}
\end{tikzar} \DP
\eeq 
satisfying 
\beq\label{eq:surjective-pairing-conditions} \fstt{\pairr x y} = x \qquad\qquad \sndd{\pairr x y} = y \qquad\qquad \pairr{\fstt z} {\sndd z} = z\eeq
While the operations defined in Sec.~\ref{Sec:pairing} for all monoidal computers satisfied the first two equations, making the pairing injective, they did not satisfy the third one, making it surjective. Program-closed categories support all three.
\end{enumerate}

\subsection{Application: Associative pairing monoid oracle}\label{Work:assoc-pair}\sindex{pairing!associative}
Given a surjective pairing \eqref{eq:surjective-pairing} satisfying \eqref{eq:surjective-pairing-conditions}, it would be nice to refine it to also satisfy the monoid equations
\beq\label{eq:monoid}
\pairr{\pairr p q} {r} = \pairr {p} {\pairr q r} \qquad \qquad\qquad\qquad \pairr \curlywedge {p}  = p = \pairr p \curlywedge
\eeq
say on another programming language $\DDP\cong \DP$. Then we could define the tupling operations $\pairrr - ^{n} \colon \DDP^{n}\stricto\DDP$  for all finite arities $n$ by
\bea 
\pairrr{p_{1},p_{2},\ldots,p_{n}} & = & \begin{cases}\hspace{4em}\curlywedge & \mbox{ if } n=0\\[2ex]
 \lceil p_{1} \lceil p_{2} \lceil \cdots \lceil p_{n},\curlywedge  \overbrace{\rceil\rceil\cdots \rceil\rceil}^{n\ \mbox{\scriptsize layers}} & \mbox{ if } n\gt 0
\end{cases}
\eea
and they would satisfy
\[\pairr{\pairrr{p_{1},\ldots,p_{m}}^{m}}{\pairrr{p_{m+1},\ldots,p_{m+n}}^{n}} \ = \ \pairrr{p_{1},\ldots, p_{m+n}}^{m+n}\qquad\quad \pairrr{\ldots,\curlywedge,\ldots}^{n+1}\ =\ \pairrr{\ldots,\ldots}^{n}
\]
The empty tuple would be represented by the minimal program $\curlywedge$, discussed in Sec.~\ref{Sec:order}. Equations \eqref{eq:monoid} mean that the following diagrams commute
%\beq\label{eq:mon-cond}
%\begin{tikzar}[row sep=4em,column sep=5em]
%\DDP\times \DDP\times\DDP \ar{r}{\pairr - -    \times \id}   \ar{d}[swap]{\id\times \pairr - -   }\& \DDP\times\DDP\ar{d}{\pairr - -   }
%\&
%\DDP \ar{r}{\curlywedge \times \id}   \ar{d}[swap]{\id\times \curlywedge} \ar[equals]{dr}\& \DDP\times\DDP\ar{d}{\pairr - -   }
%\\
%\DDP\times \DDP \ar{r}[swap]{\pairr - -   } \& \DDP
%\&
%\DDP\times \DDP \ar{r}[swap]{\pairr - -   } \& \DDP
%\end{tikzar}
%\eeq
\beq\label{eq:mon-cond}
\begin{tikzar}[row sep=3em,column sep=3em]
\DDP\times \DDP\times\DDP \ar{rr}[description]{\pairr - -    \times \id}   \ar{dd}[description]{\id\times \pairr - -   }\&\& \DDP\times\DDP\ar{dl}[description]{\pairr - -   }
\\
\& \DDP \ar[equals]{dr}
\\
\DDP\times \DDP \ar{ur}[description]{\pairr - -   } 
\&\& 
\DDP \ar{uu}[description]{\curlywedge \times \id}
\ar{ll}[description]{\id\times \curlywedge}
\end{tikzar}
\eeq
%\beq\label{eq:mon-cond}
%\begin{tikzar}[row sep=3em,column sep=3em]
%\DDP\times \DDP\times\DDP \ar[nothing-cart]{rr}[description]{\pairr - -    \times \id}   \ar[nothing-cart]{dd}[description]{\id\times \pairr - -   }\&\& \DDP\times\DDP\ar[nothing-cart]{dl}[description]{\pairr - -   }
%\\
%\& \DDP \ar[equals]{dr}
%\\
%\DDP\times \DDP \ar[nothing-cart]{ur}[description]{\pairr - -   } 
%\&\& 
%\DDP \ar[nothing-cart]{uu}[description]{\curlywedge \times \id}
%\ar[nothing-cart]{ll}[description]{\id\times \curlywedge}
%\end{tikzar}
%\eeq
making $(\DDP,\pairr - -, \curlywedge)$ into a monoid. One idea is to take $\DDP$ to comprise of (the programs of) the \emph{pairing}\/-\funnn s $\overline p \colon \DP\to\DP$, defined by the pairing $\overline p(x) = \pairr p x$ for some $p\colon \DP$, and to define $\pairr{\overline p}{\overline q} =  \overline p \circ \overline q$.  Realizing this idea in a program-closed category will lead us to an example of an interesting phenomenon: the \emph{oracles}.\sindex{oracle}

\begin{enumerate}[a.]
\item Use the monotone increasing unbounded \strict\ \funnn s $\pairr p -, \pairr - p \colon \DP\stricto \DP$ induced by the surjective pairing, and the well-order of $\DP$, to show that the minimal program $\curlywedge$ satisfies $\pairr \curlywedge y = y = \pairr y \curlywedge$ for every $y\colon \DP$.

\item\label{item:alpha} Construct an invertible \funnn\ $\alpha\colon\DP\to \DP$ such that
\bea
\alpha\left(\pairr{\pairr x y} z\right) & = & \pairr x {\pairr y z}
\eea

\item Define the set of pairing \funnn s together with the witnesses of their pairing property as follows:
\bea
\PPPP & = & \left\{f,\alpha\colon \DP\stricto \DP\ |\ f\pairr p q  =\alpha\pairr {f(p)} {q}\right\}
\eea
Prove the following statements.
\begin{enumerate}[i)]
\item $\PPPP$ is a submonoid of the monoid $(\PPP,\circ,\id_{\DP})$ from Sec.~\ref{work:monoid-completion};
\item There is a retraction
\beq
\tot \CCC(I,\DP)\begin{tikzar}[column sep = 3em]
\hspace{.2em} \ar[tail,bend left=20,shorten=.75mm]{r}{\overline{(-)}} \& \hspace{.2em} \ar[two heads,bend left=20]{l}{\underline{(-)}}
\end{tikzar}\PPPP
\eeq 
such that $\underline{<f,\alpha>} = \underline{<g,\beta>}$ if and only if there is an invertible \funnn\ $\gamma\colon \DP\stricto\DP$ such that $f=\gamma\circ g$.
\item Show that \funnn\ $\pairr - -\colon\PPPP\times \PPPP\to \PPPP$ defined by $\pairr {\overline p}{\overline q} = \overline p \circ \overline q$, with $\overline p \circ \overline q \cong \overline{ \pairr p q}$, satisfies \eqref{eq:monoid} and is therefore a tupling monoid.
\end{enumerate}
\end{enumerate}

%\subsection{Lookahead: Monoid oracle}
%\begin{enumerate}[a.]
%
%\item Let $\overline P\colon \DP\to\Bool$ be the characteristic predicate for the programs of pairing \funnn s:
%\bea\label{eq:P}
%P(x) & \iff & \Big<\uev{\fstt x}, \uev{\sndd x}\Big> \in \PPPP
%\\ 
%&\iff & \forall pq\colon \DP.\ \uev{\fstt x}\pairr p q \ = \ \uev{\sndd x}\pairr{\uev{\fstt x}p} {q}\notag
%\eea
%Show that $P$ is undecidable but that $\neg P$ is computable. What can we tell about the computability of $P$?
%
%\item Let $\CCC[\varpi]$ be the monoidal computer extended by the \emph{oracle}\/ $\varpi\colon\DP\to\DP$ as follows
%\bea
%\lvert\poly \CCC \varpi \rvert & = & \lvert\CCC\rvert\\
%\poly \CCC \varpi (A,B) & = & \left\{f_{x}\in \CCC(A,B)\ |\ \exists F\colon\DP\stricto \DP.\ \uev{F_{\varpi(x)}} = f_x\right\} \notag\eea
%Let $\varpi$ be the oracle recognizing the predicate $P$ from \eqref{eq:P}
%\bea
%\varpi(x) & =& \begin{cases} x & \mbox{ if } P(x)\\
%\divg & \mbox{ otherwise}
%\end{cases}
%\eea
%Let $\DDP$ be the type obtained in $\CCC[\varpi]$ by splitting the idempotent $\varpi$. Then $\DDP$ is a programming language with the program execution
%\bea
%\overline{\Run{F}} & = & \Run{\uev{\fstt F}\curlywedge}
%\eea
%also supporting  the tupling monoid worked out above.
%\end{enumerate}
%
%
%\end{enumerate}



%
%
%
%
%In Sec.~\ref{Sec:pairing}, a pairing $\pairr - - \colon \DP\times \DP\stricto \DP$ and the projections $\fstt -, \sndd -\colon \DP\to \DP$ \funnn s were defined  for any monoidal computer and they satisfied
%\[
%\fstt{\pairr {x_{0}} {x_{1}}} = x_{0}\qquad \qquad \qquad  \qquad \sndd{\pairr {x_{0}} {x_{1}}} = x_{1}\]
%for all \strict\ $x_{0}, x_{1}\colon X \stricto \DP$. A similar construction provides tupling operations $\pairrr{\cdots} \colon\DP^{n}\stricto \DP$ and accompanying  the projections $\nnth - 0, \nnth -1,\ldots,\nnth - n:\DP\to \DP$ for all $n$, satisfying
%\[\nnth{\pairrr{x_{0},\ldots,x_{n}}}{k} = x_{k}\]
%for all $k\lt n$. The claim is now that in any program-closed category, the tupling operations can be made \emph{extensionally coherent}, so that all $m$-tuples and $n$-tuples satisfy
%\bear
%\pairr{\pairrr{x_{0},\ldots,x_{m}}}{\pairrr{x_{m+1},\ldots,x_{m+n}}} & \eeext & \pairrr{x_{0},\ldots,x_{m},x_{m+1}, x_{m+n}}
%\eear
%%where $f\cong g$ means that there is a pair of \funnn s $\kappa,\chi\colon \DP \to \DP$ such that $\kappa\circ \chi = \id =\chi\circ\kappa$ and $f=\kappa\circ g$ which implies $\chi\circ f = g$.
%This can be achieved by finding an \emph{extensional pairing semigroup}\/ with unit
%\[
%\DP\times \DP\strictto{\pairr - -} \DP \strictoot{\nultuple} I
%\]
%where the associativity and the unitarity mean
%\[\pairr{\pairr x y} {z} \eeext \pairr {x} {\pairr{y}{z}} \qquad \qquad\qquad\qquad \pairr{x}{\nultuple} \eeext x 
%\]
%for all $x,y,z \colon \DP$. For the rest of this workout we fix a pairing $\pairr - - \colon \DP\times \DP\stricto \DP$, as constructed in \eqref{eq:tupling}, and derive from it a pairing semigroup.
%
%\para{Prove the following claims.} 
%\begin{enumerate}[a.]
%\item There is a program $\nultuple$ such that all $x\colon\DP$ satisfy
%\bear \pairr x \nultuple & \eeext & x\eear
%
%
%\item A \strict\ \funnn\ $f\colon \DP\stricto \DP$ is said to be \emph{$\pairrr{-}$-strong}\/ if it satisfies
%\bear
%f\Big(\pairr x y\Big) & \eeext & \Big\lceil f(x), y\Big\rceil% \pairr{f(x)} y
%\eear
%Let $\strong \subseteq \tot \CCC(\DP,\DP)$ be the set of $\pairrr{-}$-strong \funnn s. Show that $\left(\strong,\circ,\id \right)$ is a monoid.
%
%
%
% Construct a bijection
%\[\tot\CCC(I,\DP)\hspace{-1ex}\begin{tikzar}[column sep=1.5cm]
%\hspace{1ex} \ar[bend right=20]{r}\ar[phantom]{r}[description]{\cong}\& \hspace{1ex} \ar[bend right=20]{l}
%\end{tikzar}\hspace{-1ex}  \strong
%\]
%
%
%pairing monoid $P\times P\tto{\pairr - -} P \oot{\nultuple} I$ which induces the tupling operations
%\[\pairr{\pairr x y} {z} = \pairrr{x,y,z} = \pairr {x} {\pairr{y}{z}} \qquad \qquad\qquad\qquad \pairr{x}{\nultuple} = x = \pairr{\nultuple}{x}
%\]
%\item projections $\fstt -, \sndd -\colon P\to P$ satisfying
%\[\fstt{\pairr x y} =  x\qquad\qquad\qquad\qquad \sndd{\pairr x y} = y\]
%from which all projections $\nnth{\pairrr{x_{0},\ldots,x_{n}}}{k} = x_{k}$ are derived;
%
%\end{enumerate}
% 
% 
% 
 




==> 81-PCC/89-story.tex <==
% !TEX root = ../000-monc.tex

\subsection{Prehistory of well-order} \label{Sec:story-order}
Our story of well-order, like the story of types in Sec.~\ref{Sec:story-type}, begins from Cantor's \emph{order types}\sindex{type!order types}. As equivalence classes of ordered sets up to isomorphism, order types anticipated one of the tenets of the categorical approach but Cantor's contemporaries brushed it aside. The assumption that sets can be well-ordered anticipated one of the tenets of programming but Cantor himself tried to avoid it wherever possible. Why was that?

Mathematics begins with counting. Counting the elements of a set imposes a well-order on it. Cantor developed the theory of counting past infinity. The well-order played a central role. But the idea of counting and well-ordering past infinity takes getting used to. The well-order obtained by counting the reals clashes against the intuition of their continuous order on the real line. Cantor's notable contemporaries thought that the idea of well-ordering the reals was preposterous. For Kronecker and  Poincar\'e, such ideas were a youth-corrupting mathematical malady \cite{CantorG:dauben}. Cantor tried to compromise with the powerful critics by concealing and marginalizing some of his central ideas in his publications.

The task of extracting a bijection out of two injections arises from the claim that all numbers, finite and transfinite, are linearly ordered. If a set $P_0$ is not larger than $P_1$ and $P_1$ is not larger than $P_0$, then they should have the same number of elements. We say that $P_0$ is not larger than $P_1$ when there is an injection $\theta_{01}\colon P_0\mono P_1$; that $P_1$ is not larger than $P_0$ means that there is an injection  $\theta_{10}\colon P_1\mono P_0$; and that $P_0$ and $P_1$ have the same number of elements when there is a bijection $\kappa:P_0\cong P_1:\chi$. If $P_0$ and $P_1$ are well-ordered and the injections $\theta_0$ and $\theta_1$ are monotone, then there is a bijection constructed like in Sec.~\ref{Sec:hartley}.  It is as effective as the injections and the well-orders. Cantor's correspondence with Dedekind suggests that he was aware of some such construction \sindex{orbits of programs!alternating orbits} \cite{Cantor-Dedekind:Briefwechsel}. Yet he followed Dedekind's advice to work towards removing the well-order assumption, developed nonconstructive\footnote{In elementary toposes, the Cantor-Bernstein Theorem is equivalent to the Law of Excluded Middle \cite{PavlovicD:Cantor-categories}.} error-prone arguments, and never published a proof \cite{HinkisA:cantor-bernstein}. Dedekind adopted a proof in his famous monograph about numbers \cite{DedekindR:zahlen}. In the manuscript he attributed it to Cantor, but removed the reference in the first edition. The tangled history of the non-constructive unordered versions of the Cantor-Bernstein Theorem\footnote{For more than a century, and still all over the web, this theorem went under the name ``the Schr\"oder-Bernstein Theorem", in recognition of E.~Schr\"oder's deeply flawed argument, published as a proof of ``Cantor's Conjecture", sufficiently complicated to survive the test of time.}   \cite{HinkisA:cantor-bernstein} obscured the effective well-ordered construction that Cantor seems to had conceived. It is probably fair to say that he used well-order to construct functions before the notion of constructing functions was understood. Once it was understood, constructive versions of the Cantor-Bernstein theorem were published in a quick succession, as John Myhill's \cite{MyhillJ:creative} and Hartley Rogers'  \cite{Hartley:isomorphism} isomorphism theorems for computably enumerated sets\footnote{See \cite[III.7]{Odifreddi:one} for a succinct explanation of the meaning and the impact of these theorems.}. The Isomorphism Theorem for program-closed categories is more elementary than either of them, probably a minor variation of Cantor's construction. 

\subsection{Towards categorical computers}
Computable functions are defined as whatever can be implemented in any of the many equivalent models of computation, or in any of the usual (Turing-complete) programming languages. The models and the languages vary vastly and some of the implementation details are always irrelevant. Categories, on the other hand, are a mathematical tool for displaying the structures of interest while hiding the irrelevant implementation details.\footnote{The tookits of such methods in linguistics and anthropology have gone under the name \emph{structuralism}. In programming, the tasks of abstracting away the irrelevant implementation details is what led to the high-level programming languages, to modular and object-oriented programming, and so on. Category theory could be thought of as a ``structuralist programming language of mathematics''.} The case for a  categorical approach to computing is strong. What is computability without the irrelevant implementation details?

Early efforts in this direction go back to Yuri Ershov, Fig.~\ref{Fig:ershov}. A fast-advancing student of the great Maltcev in Novosibirsk, Ershov picked up Myhill's work on creative sets and recursive isomorphisms, and announced a program towards extracting isomorphism-invariant structures, abstracting away the irrelevant implementation details by describing all constructions in terms of program enumerations of computable functions  \cite{ErshovY:enum67,ErshovY:enum68}. By 1971, working towards higher-order recursion, he defined a cartesian-closed category of enumerations \sindex{category!cartesian-closed} \cite{ErshovY:enum-ccc} --- apparently unaware of the name, the logical background, or any previous work on cartesian-closed categories. A full account of the structure of this category was worked out by 1977 and presented in a book \cite{ErshovY:enum-book}. But when Ershov visited the US on a Fulbright Stipend in the 1980, his talks were picketed by protestors accusing him of complicity, derived from his administrative, in the antisemitic suppression rampant in the Soviet academia \cite[pp 363--365]{Fefferman:Tarski}. The incidents around his visit overshadowed the presentations of his work, and assured that Soviet mathematicians' restricted view of the logical content of cartesian-closed categories was  counterbalanced by western mathematicians' restricted view of the computational content of the same structure. Information trickled nevertheless, and Ershov's categorical treatment of enumerations was the stepping stone into realizability toposes, the extensional universes of sets with computably realized functions \cite{HylandJME:efft,MulryP:efft,MulryP:adjointness-recursion}.
\begin{figure}[!ht]
\centering
\begin{minipage}[b]{0.3\linewidth}
\centering
\includegraphics[height=5cm%,viewport = 0 500 500 0,clip
]{PIC/Myhill.eps}
\caption{John Myhill}
\label{Fig:myhill}
\end{minipage}
\begin{minipage}[b]{0.3\linewidth}
\centering
\includegraphics[height=5cm%,viewport = 0 500 500 0,clip
]{PIC/Ershov-Yuri.eps}
\caption{Yuri L. Ershov}
\label{Fig:ershov}
\end{minipage}
\begin{minipage}[b]{0.3\linewidth}
\centering
\includegraphics[height=5cm%,viewport = 0 500 500 0,clip
]{PIC/hofstra.eps}
\caption{Pieter Hofstra}
\label{Fig:hofstra}
\end{minipage}
\end{figure}
A bridge between Ershof's theory and the broader context of cartesian-closed category was built in the work Giuseppe Longo and Eugenio Moggi, published in 1984 \cite{Longo-Moggi:enumerations,Longo-Moggi:hereditary}. At the time, Mogi had not yet started working on his PhD, which would take him to the greener pastures of denotational semantics (and equip denotational semantics with the powerful toolkit of computational monads \cite{MoggiE:monad}). Still in the 80s, DiPaola and Heller proposed \emph{dominions}, an algebraic structure that allows capturing partiality of computable functions in cartesian categories \cite{DiPaola-Heller:dominical}. Then in the 90s, as denotational and topos-theoretic approaches to computation peaked  \cite{Abramsky-Gabbay:handbook-semantics-3,OostenJ:book}, the categorical accounts of the intensional aspects of computation, as sporadic as they were, faded in the background. 

The closest relatives of the monoidal computer emerged in the 2000s in the thesis work of Lars Birkedal \cite{BirkedalL:thesis} and \emph{Turing categories}\/ project of Robin Cockett and Pieter Hofstra \cite{Cockett-Hofstra:turing,CockettR:timed}. Our program evaluators correspond to  Birkedal's \emph{universal objects}\/ and Cocket-Hofstra's \emph{Turing objects}. All three are obvious categorical variations on the theme of \emph{acceptable program enumerations}. The difference between the three is that a monoidal computer is based on monoidal categories, Birkedal works with \emph{WCPC-categories} (acronym of ``Weakly Closed Partial Cartesian''), whereas Cockett and Hofstra work with cartesian categories extended by a simplified version of DiPaola-Heller's dominion operations. While monoidal computers are slightly more general, since they accommodate other computational effects besides partiality\footnote{The dominion of a function can is definable by copying the inputs and deleting the outputs of a monoidal function. This operation is not idempotent in quantum computation, and can be used to characterize classical computation, be it deterministic, possibilistic, or probabilistic.}  ---  the difference with respect to the main goal of modeling intensional computations seems cosmetic\footnote{Truth be told, this is not Birkedal's main goal, but a step on the path from partial combinatory algebras to realizability toposes, and he only spells out that aspect.}. In all cases, all morphisms are computable in the sense that they can be decomposed through evaluators on universal Turing objects and the total single-valued maps representing programs. Whether the data live in a monoidal category with a cartesian subcategory of total single-valued morphisms determined by the data services or in a cartesian category extended by the dominion operations, or in WCPC-categories, seems marginal. Surprisingly, there is a substantial difference between the three structures. 

Both the WCPC-categories and the Turing categories arose from work on \emph{partial combinatory algebras (pcas)} \sindex{partial combinatory algebra} \cite{LongleyJ:thesis,OostenJ:book}, an essentially algebraic applicative structure from which realizability toposes are usually built. Both structures are in a suitable sense equivalent to pcas, as their typed completions. This was proved by Birkedal in \cite[Prop.~3.1.18]{BirkedalL:thesis} and by Cocket-Hofstra in \cite[Thm.~4.9]{Cockett-Hofstra:turing}. But it is well-known that pcas support an abstraction operation \cite[Ch.~1]{OostenJ:book}. Although partiality of the application operation prevents expanding this operation to a full $\lambda$-calculus\footnote{This was attempted in Henk Barendregt's 1971 thesis, and he proved that it is impossible in the reissue \cite{BarendregtH:proefschrift-20}.}, it still nevertheless inductively assigns a canonical program to any function specified in the signature of partial combinatory algebra. Although the program enumerations\footnote{E.g., Kleene's program indices are one of the first examples of pcas.} do induce partial combinatory algebras, with program evaluation as the application operation, the algebraic signature does not allow specifying all programs, but only those that are inductively defined, and yield to the inductively definable program abstraction. A pca can be defined over the set of program expression of, say, the Python programming language, and we have seen that all computable functions can be specified in terms of its program evaluators. But if we reduce them to  the pca structure, then the programs specified in its signature allow the inductively defined program abstraction. Programs that include coinductive operations, such as the while loops, cannot be specified in an essentially algebraic signature. Categories of functions that arise by evaluating such programs correspond to an inductive family of \emph{uniform}\/ monoidal computers, worked out in Sec.~\ref{Sec:uniform}. \sindex{uniform monoidal computer} A slew of results in the 1980s indicated that the presence of an abstraction operation, even without the extensionality axiom, make the models essentially extensional, in the sense that it contains a computable extensional retract \cite{HayashiS:semifunctors,Hoofman-Moerdijk,Koymans,ScottD:relating}. The results were proved for the non-extensional $\lambda$-abstraction, but similar methods seem to be applicable to the abstraction operation assigning canonical programs to pca-specified functions. This would suggest that the mere presence of an abstraction operation in a categorical computer factors out the intensional content of programs and algorithms. Verifying this is beyond the scope of the present work. 




%\subsection{WHAT COULD GO WRONG?}
%The central operation in categories is the function composition. The central operation in computers is the program evaluation. What could go wrong? When programs are evalated on each other, the program evaluation yields the binary operation of application.\sindex{instruction!application} (See Sec.~\ref{} for more.) While composition is associative, application is not. Church's central idea was to capture computable functions in terms of applications. Function applications are naturally studied with function abstractions. Together, the two make the function composition as a derived operation, associative and unitary. The three operations live together in cartesian-closed categories. 

The problem with capturing program evaluation in terms of function application is that the operation of function abstraction, application's natural companion, makes abstracting programs from functions as easy as applying them to data. Both are operations. This is not how it works in reality. Programs are applied by computers and abstracted by programmers. One is a push-button operation, the other requires work. That is why the function abstraction is not the same thing as the  program abstraction, as every semanticist will tell you. One is an abstract operation, the other is a concrete process. We should not confuse them.\sindex{abstraction!function vs program} Fair enough.

Through the 90s and beyond, the categorical theory of computation has been developed over the applicative structures \emph{without}\/ the abstraction operation, usually the \emph{partial combinatory algebras}. The realizability-based universes of sets are nearly invariably based on them. --- But they do support an abstraction operation, extracting canonical programs for the functions defined in the pca-signature. Turing categories and WCPC-categories have been proved to consist of morphisms specified in the pca-signature. They are weakly closed, in the sense that they allow weak abstraction. Weak abstraction, like non-extensional abstraction, still assigns a canonical program to each computation.

Program abstraction is presented as an operation just like the program application.

Programming is as easy as running a program. Both are push-button operations.

Programmers' work is as easy as computers' work.

This is a very special part of the world of computation.


%
%
%
%
%
%
%
%
%
%\subsubsection{LOOSE ENDS}
%\para{What do all computers have in common?} The Church-Turing thesis, discussed in Sec.~\ref{Sec:CTT}, suggests that computability is realized by many different structures: Church's $\lambda$-calculus implements it in one way, Turing's machines in another way, Lambek's abacus in yet another way, G\"odel's and Dedekind's recursive functions still differently. While there are translations that make any two realizations equivalent, in the sense that they implement the same computable functions, it has been postulated that there is no intrinsic \emph{property}\/ of functions on their own, that could be recognized without a recourse to one of the extrinsic \emph{structures}\/ of the models of computers that compute the computable functions \cite{AbramskyS:definability}. Each of the models of computers is a structure by the very definition of computation as an intensional process, implemented by many different programs as different structures. The interpretations between such models are not canonical, in the sense that each can be interpreted in any other in many different ways. Each of them can actually interpret its own computations in infinitely many semantically sound, extensionally equivalent, but intensionally different ways.
%
%Remarkably, being program-closed turns out to be a property of a monoidal category. This means that the categorical structure that enables computation in a monoidal category is unique up to isomorphism. The upshot is that computability, as a property of computable functions, can be recognized intrinsically, on the \funnn s themselves, provided that they are viewed within a monoidal category as a type universe and described as black boxes, in terms of their relationships, \emph{not}\/ in terms of the elements used to implement their computations. Categories abstract away the implementation details of the models of computation just like they abstract away the elements permuted by groups or contained by sets. Computations are presented in terms of relationships between the boxes enclosing abstract computations, just like groups are presented in terms of the group homomorphisms between the boxes enclosing the abstract transformations that they perform. The string diagram are a natural visualization of such approaches.
%
%Each of the abstract Church-Turing models, as well as any of the concrete programming languages, are subsumed, in the sense that each generates a category that is easily seen to carry the structure of a monoidal computer. This contradicts the  intuitions about the Tower of Babel of languages. We must tread carefully to understand what is going on. There are many forms of life, but just one property of being alive.



==> PIC/ACK-m.tex <==
%%Created by jPicEdt 1.4.1_03: mixed JPIC-XML/LaTeX format
%%Wed Feb 24 12:59:40 GMT-10:00 2021
%%Begin JPIC-XML
%<?xml version="1.0" standalone="yes"?>
%<jpic x-min="0" x-max="265" y-min="-5" y-max="275" auto-bounding="true">
%<multicurve fill-style= "none"
%	 points= "(145,185);(145,185);(180,185);(180,185)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(200,165);(200,165);(180,185);(180,185)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(190,200);(190,200);(190,175);(190,175)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(95,200);(95,200);(95,165);(95,165)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(165,155);(165,155);(200,155);(200,155)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(200,135);(200,135);(200,155);(200,155)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(190,165);(190,165);(190,155);(190,155)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(185,135);(185,135);(200,135);(200,135)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(175,145);(175,145);(35,75);(35,75)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(165,155);(165,155);(185,135);(185,135)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(110,65);(110,65);(190,105);(190,105)"
%	 stroke-width= "0.6"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(187.5,145)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\utag$
%</text>
%<multicurve fill-style= "none"
%	 points= "(35,165);(35,165);(35,105);(35,105)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(15,185);(15,185);(55,185);(55,185)"
%	 stroke-width= "0.6"
%	 />
%<multicurve fill-style= "none"
%	 points= "(55,165);(55,165);(55,185);(55,185)"
%	 stroke-width= "0.6"
%	 />
%<multicurve fill-style= "none"
%	 points= "(15,165);(15,165);(55,165);(55,165)"
%	 stroke-width= "0.6"
%	 />
%<multicurve fill-style= "none"
%	 points= "(15,185);(15,185);(15,165);(15,165)"
%	 stroke-width= "0.6"
%	 />
%<multicurve fill-style= "none"
%	 points= "(35,195);(35,195);(35,185);(35,185)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(110,65);(110,65);(110,-5);(110,-5)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 stroke-overstrike-width= "2"
%	 points= "(35,105);(35,105);(110,65);(110,65)"
%	 stroke-overstrike= "true"
%	 stroke-width= "0.6"
%	 />
%<multicurve fill-style= "none"
%	 points= "(35,210);(35,210);(35,185);(35,185)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(25,220);(25,220);(205,220);(205,220)"
%	 stroke-width= "0.6"
%	 />
%<multicurve fill-style= "none"
%	 points= "(205,200);(205,200);(205,220);(205,220)"
%	 stroke-width= "0.6"
%	 />
%<multicurve fill-style= "none"
%	 points= "(45,200);(45,200);(205,200);(205,200)"
%	 stroke-width= "0.6"
%	 />
%<multicurve fill-style= "none"
%	 points= "(25,220);(25,220);(45,200);(45,200)"
%	 stroke-width= "0.6"
%	 />
%<multicurve fill-style= "none"
%	 points= "(140,245);(140,245);(140,220);(140,220)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(205,110);(205,110);(205,125);(205,125)"
%	 stroke-width= "0.6"
%	 />
%<multicurve fill-style= "none"
%	 points= "(175,110);(175,110);(205,110);(205,110)"
%	 stroke-width= "0.6"
%	 />
%<multicurve fill-style= "none"
%	 points= "(175,125);(175,125);(175,110);(175,110)"
%	 stroke-width= "0.6"
%	 />
%<multicurve fill-style= "none"
%	 points= "(190,135);(190,135);(190,125);(190,125)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(190,110);(190,110);(190,105);(190,105)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(35,75);(35,75);(35,35);(35,35)"
%	 stroke-width= "0.75"
%	 />
%<ellipse p3= "(111.28,63.71)"
%	 fill-style= "solid"
%	 p2= "(111.28,66.29)"
%	 fill-color= "#330033"
%	 p1= "(108.72,66.29)"
%	 closure= "open"
%	 angle-end= "0"
%	 stroke-width= "2.5"
%	 angle-start= "0"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(35,175)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\zerotag$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(117.5,210)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\iiftag$
%</text>
%<multicurve fill-style= "none"
%	 stroke-overstrike-width= "2"
%	 points= "(155,175);(155,175);(145,165);(145,165)"
%	 stroke-overstrike= "true"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(165,165);(165,165);(200,165);(200,165)"
%	 stroke-width= "0.75"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(190,117.5)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\predtag$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(32.5,65)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\pee$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(107.5,0)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\een$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(227.5,0)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\eex$
%</text>
%<multicurve fill-style= "none"
%	 points= "(175,125);(175,125);(205,125);(205,125)"
%	 stroke-width= "0.6"
%	 />
%<multicurve fill-style= "none"
%	 points= "(230,235);(230,235);(230,-5);(230,-5)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(130,255);(130,255);(255,255);(255,255)"
%	 stroke-width= "0.6"
%	 />
%<multicurve fill-style= "none"
%	 points= "(255,235);(255,235);(255,255);(255,255)"
%	 stroke-width= "0.6"
%	 />
%<multicurve fill-style= "none"
%	 points= "(150,235);(150,235);(255,235);(255,235)"
%	 stroke-width= "0.6"
%	 />
%<multicurve fill-style= "none"
%	 points= "(130,255);(130,255);(150,235);(150,235)"
%	 stroke-width= "0.6"
%	 />
%<multicurve fill-style= "none"
%	 points= "(235,275);(235,275);(235,255);(235,255)"
%	 stroke-width= "0.75"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(195,245)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\utag$
%</text>
%<multicurve fill-style= "none"
%	 points= "(80,150);(80,150);(80,180);(80,180)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(80,150);(80,150);(110,150);(110,150)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(80,180);(80,180);(110,150);(110,150)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(145,185);(145,185);(165,165);(165,165)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(130,150);(130,150);(130,180);(130,180)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(130,150);(130,150);(160,150);(160,150)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(130,180);(130,180);(160,150);(160,150)"
%	 stroke-width= "0.75"
%	 />
%<parallelogram p3= "(210,55)"
%	 fill-style= "none"
%	 p2= "(210,225)"
%	 p1= "(10,225)"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(200,65)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\atilde$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(30,30)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\gtag$
%</text>
%<multicurve fill-style= "none"
%	 points= "(20,20);(20,20);(20,50);(20,50)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(20,20);(20,20);(50,20);(50,20)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(20,50);(20,50);(50,20);(50,20)"
%	 stroke-width= "0.75"
%	 />
%<parallelogram p3= "(215,15)"
%	 fill-style= "none"
%	 p2= "(215,230)"
%	 p1= "(5,230)"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(205,25)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\aflat$
%</text>
%<parallelogram p3= "(265,10)"
%	 fill-style= "none"
%	 p2= "(265,260)"
%	 p1= "(0,260)"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(255,147.5)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\ackermann$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(90,160)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\htag$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(140,160)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\ktag$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(172.5,175)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\specializer$
%</text>
%<multicurve fill-style= "none"
%	 points= "(245,235);(245,235);(245,-5);(245,-5)"
%	 stroke-width= "0.75"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "solid"
%	 anchor-point= "(242.5,0)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\eem$
%</text>
%</jpic>
%%End JPIC-XML
%LaTeX-picture environment using emulated lines and arcs
%You can rescale the whole picture (to 80% for instance) by using the command \def\JPicScale{0.8}
\ifx\JPicScale\undefined\def\JPicScale{1}\fi
\unitlength \JPicScale mm
\begin{picture}(265,275)(0,0)
\linethickness{0.75mm}
\put(145,185){\line(1,0){35}}
\linethickness{0.75mm}
\multiput(180,185)(0.12,-0.12){167}{\line(1,0){0.12}}
\linethickness{0.75mm}
\put(190,175){\line(0,1){25}}
\linethickness{0.75mm}
\put(95,165){\line(0,1){35}}
\linethickness{0.75mm}
\put(165,155){\line(1,0){35}}
\linethickness{0.75mm}
\put(200,135){\line(0,1){20}}
\linethickness{0.75mm}
\put(190,155){\line(0,1){10}}
\linethickness{0.75mm}
\put(185,135){\line(1,0){15}}
\linethickness{0.75mm}
\multiput(35,75)(0.24,0.12){583}{\line(1,0){0.24}}
\linethickness{0.75mm}
\multiput(165,155)(0.12,-0.12){167}{\line(1,0){0.12}}
\linethickness{0.6mm}
\multiput(110,65)(0.24,0.12){333}{\line(1,0){0.24}}
\put(187.5,145){\makebox(0,0)[cc]{$\utag$}}

\linethickness{0.75mm}
\put(35,105){\line(0,1){60}}
\linethickness{0.6mm}
\put(15,185){\line(1,0){40}}
\linethickness{0.6mm}
\put(55,165){\line(0,1){20}}
\linethickness{0.6mm}
\put(15,165){\line(1,0){40}}
\linethickness{0.6mm}
\put(15,165){\line(0,1){20}}
\linethickness{0.75mm}
\put(35,185){\line(0,1){10}}
\linethickness{0.75mm}
\put(110,-5){\line(0,1){70}}
\linethickness{0.6mm}
\multiput(35,105)(0.23,-0.12){333}{\line(1,0){0.23}}
\linethickness{0.75mm}
\put(35,185){\line(0,1){25}}
\linethickness{0.6mm}
\put(25,220){\line(1,0){180}}
\linethickness{0.6mm}
\put(205,200){\line(0,1){20}}
\linethickness{0.6mm}
\put(45,200){\line(1,0){160}}
\linethickness{0.6mm}
\multiput(25,220)(0.12,-0.12){167}{\line(1,0){0.12}}
\linethickness{0.75mm}
\put(140,220){\line(0,1){25}}
\linethickness{0.6mm}
\put(205,110){\line(0,1){15}}
\linethickness{0.6mm}
\put(175,110){\line(1,0){30}}
\linethickness{0.6mm}
\put(175,110){\line(0,1){15}}
\linethickness{0.75mm}
\put(190,125){\line(0,1){10}}
\linethickness{0.75mm}
\put(190,105){\line(0,1){5}}
\linethickness{0.75mm}
\put(35,35){\line(0,1){40}}
\linethickness{2.5mm}
\put(111.26,64.75){\line(0,1){0.5}}
\multiput(111.07,64.28)(0.1,0.23){2}{\line(0,1){0.23}}
\multiput(110.71,63.93)(0.12,0.12){3}{\line(0,1){0.12}}
\multiput(110.25,63.73)(0.23,0.1){2}{\line(1,0){0.23}}
\put(109.75,63.73){\line(1,0){0.5}}
\multiput(109.29,63.93)(0.23,-0.1){2}{\line(1,0){0.23}}
\multiput(108.93,64.28)(0.12,-0.12){3}{\line(0,-1){0.12}}
\multiput(108.74,64.75)(0.1,-0.23){2}{\line(0,-1){0.23}}
\put(108.74,64.75){\line(0,1){0.5}}
\multiput(108.74,65.25)(0.1,0.23){2}{\line(0,1){0.23}}
\multiput(108.93,65.72)(0.12,0.12){3}{\line(0,1){0.12}}
\multiput(109.29,66.07)(0.23,0.1){2}{\line(1,0){0.23}}
\put(109.75,66.27){\line(1,0){0.5}}
\multiput(110.25,66.27)(0.23,-0.1){2}{\line(1,0){0.23}}
\multiput(110.71,66.07)(0.12,-0.12){3}{\line(0,-1){0.12}}
\multiput(111.07,65.72)(0.1,-0.23){2}{\line(0,-1){0.23}}

\put(35,175){\makebox(0,0)[cc]{$\zerotag$}}

\put(117.5,210){\makebox(0,0)[cc]{$\iiftag$}}

\linethickness{0.75mm}
\multiput(145,165)(0.12,0.12){83}{\line(1,0){0.12}}
\linethickness{0.75mm}
\put(165,165){\line(1,0){35}}
\put(190,117.5){\makebox(0,0)[cc]{$\predtag$}}

\put(32.5,65){\makebox(0,0)[cr]{$\pee$}}

\put(107.5,0){\makebox(0,0)[cr]{$\een$}}

\put(227.5,0){\makebox(0,0)[cr]{$\eex$}}

\linethickness{0.6mm}
\put(175,125){\line(1,0){30}}
\linethickness{0.75mm}
\put(230,-5){\line(0,1){240}}
\linethickness{0.6mm}
\put(130,255){\line(1,0){125}}
\linethickness{0.6mm}
\put(255,235){\line(0,1){20}}
\linethickness{0.6mm}
\put(150,235){\line(1,0){105}}
\linethickness{0.6mm}
\multiput(130,255)(0.12,-0.12){167}{\line(1,0){0.12}}
\linethickness{0.75mm}
\put(235,255){\line(0,1){20}}
\put(195,245){\makebox(0,0)[cc]{$\utag$}}

\linethickness{0.75mm}
\put(80,150){\line(0,1){30}}
\linethickness{0.75mm}
\put(80,150){\line(1,0){30}}
\linethickness{0.75mm}
\multiput(80,180)(0.12,-0.12){250}{\line(1,0){0.12}}
\linethickness{0.75mm}
\multiput(145,185)(0.12,-0.12){167}{\line(1,0){0.12}}
\linethickness{0.75mm}
\put(130,150){\line(0,1){30}}
\linethickness{0.75mm}
\put(130,150){\line(1,0){30}}
\linethickness{0.75mm}
\multiput(130,180)(0.12,-0.12){250}{\line(1,0){0.12}}
\linethickness{0.3mm}
\put(10,225){\line(1,0){200}}
\put(10,55){\line(0,1){170}}
\put(210,55){\line(0,1){170}}
\put(10,55){\line(1,0){200}}
\put(200,65){\makebox(0,0)[cc]{$\atilde$}}

\put(30,30){\makebox(0,0)[cc]{$\gtag$}}

\linethickness{0.75mm}
\put(20,20){\line(0,1){30}}
\linethickness{0.75mm}
\put(20,20){\line(1,0){30}}
\linethickness{0.75mm}
\multiput(20,50)(0.12,-0.12){250}{\line(1,0){0.12}}
\linethickness{0.3mm}
\put(5,230){\line(1,0){210}}
\put(5,15){\line(0,1){215}}
\put(215,15){\line(0,1){215}}
\put(5,15){\line(1,0){210}}
\put(205,25){\makebox(0,0)[cc]{$\aflat$}}

\linethickness{0.3mm}
\put(0,260){\line(1,0){265}}
\put(0,10){\line(0,1){250}}
\put(265,10){\line(0,1){250}}
\put(0,10){\line(1,0){265}}
\put(255,147.5){\makebox(0,0)[cc]{$\ackermann$}}

\put(90,160){\makebox(0,0)[cc]{$\htag$}}

\put(140,160){\makebox(0,0)[cc]{$\ktag$}}

\put(172.5,175){\makebox(0,0)[cc]{$\specializer$}}

\linethickness{0.75mm}
\put(245,-5){\line(0,1){240}}
\put(242.5,0){\makebox(0,0)[cr]{$\eem$}}

\end{picture}


==> PIC/ACK-mm.tex <==
%%Created by jPicEdt 1.4.1_03: mixed JPIC-XML/LaTeX format
%%Wed Feb 24 13:06:02 GMT-10:00 2021
%%Begin JPIC-XML
%<?xml version="1.0" standalone="yes"?>
%<jpic x-min="0" x-max="265" y-min="-5" y-max="275" auto-bounding="true">
%<multicurve fill-style= "none"
%	 points= "(145,185);(145,185);(180,185);(180,185)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(200,165);(200,165);(180,185);(180,185)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(190,200);(190,200);(190,175);(190,175)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(95,200);(95,200);(95,165);(95,165)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(165,155);(165,155);(200,155);(200,155)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(200,135);(200,135);(200,155);(200,155)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(190,165);(190,165);(190,155);(190,155)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(185,135);(185,135);(200,135);(200,135)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(175,145);(175,145);(35,75);(35,75)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(165,155);(165,155);(185,135);(185,135)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(110,65);(110,65);(190,105);(190,105)"
%	 stroke-width= "0.6"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(187.5,145)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\utag$
%</text>
%<multicurve fill-style= "none"
%	 points= "(35,165);(35,165);(35,105);(35,105)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(15,185);(15,185);(55,185);(55,185)"
%	 stroke-width= "0.6"
%	 />
%<multicurve fill-style= "none"
%	 points= "(55,165);(55,165);(55,185);(55,185)"
%	 stroke-width= "0.6"
%	 />
%<multicurve fill-style= "none"
%	 points= "(15,165);(15,165);(55,165);(55,165)"
%	 stroke-width= "0.6"
%	 />
%<multicurve fill-style= "none"
%	 points= "(15,185);(15,185);(15,165);(15,165)"
%	 stroke-width= "0.6"
%	 />
%<multicurve fill-style= "none"
%	 points= "(35,195);(35,195);(35,185);(35,185)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(110,65);(110,65);(110,-5);(110,-5)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 stroke-overstrike-width= "2"
%	 points= "(35,105);(35,105);(110,65);(110,65)"
%	 stroke-overstrike= "true"
%	 stroke-width= "0.6"
%	 />
%<multicurve fill-style= "none"
%	 points= "(35,210);(35,210);(35,185);(35,185)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(25,220);(25,220);(205,220);(205,220)"
%	 stroke-width= "0.6"
%	 />
%<multicurve fill-style= "none"
%	 points= "(205,200);(205,200);(205,220);(205,220)"
%	 stroke-width= "0.6"
%	 />
%<multicurve fill-style= "none"
%	 points= "(45,200);(45,200);(205,200);(205,200)"
%	 stroke-width= "0.6"
%	 />
%<multicurve fill-style= "none"
%	 points= "(25,220);(25,220);(45,200);(45,200)"
%	 stroke-width= "0.6"
%	 />
%<multicurve fill-style= "none"
%	 points= "(140,245);(140,245);(140,220);(140,220)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(205,110);(205,110);(205,125);(205,125)"
%	 stroke-width= "0.6"
%	 />
%<multicurve fill-style= "none"
%	 points= "(175,110);(175,110);(205,110);(205,110)"
%	 stroke-width= "0.6"
%	 />
%<multicurve fill-style= "none"
%	 points= "(175,125);(175,125);(175,110);(175,110)"
%	 stroke-width= "0.6"
%	 />
%<multicurve fill-style= "none"
%	 points= "(190,135);(190,135);(190,125);(190,125)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(190,110);(190,110);(190,105);(190,105)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(35,75);(35,75);(35,35);(35,35)"
%	 stroke-width= "0.75"
%	 />
%<ellipse p3= "(112.57,62.42)"
%	 fill-style= "solid"
%	 p2= "(112.57,67.58)"
%	 fill-color= "#330033"
%	 p1= "(107.43,67.58)"
%	 closure= "open"
%	 angle-end= "0"
%	 angle-start= "0"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(35,175)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\zerotag$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(117.5,210)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\iiftag$
%</text>
%<multicurve fill-style= "none"
%	 stroke-overstrike-width= "2"
%	 points= "(155,175);(155,175);(145,165);(145,165)"
%	 stroke-overstrike= "true"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(165,165);(165,165);(200,165);(200,165)"
%	 stroke-width= "0.75"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(190,117.5)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\predtag$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(32.5,65)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\pee$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(107.5,0)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\een$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(227.5,0)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\eex$
%</text>
%<multicurve fill-style= "none"
%	 points= "(175,125);(175,125);(205,125);(205,125)"
%	 stroke-width= "0.6"
%	 />
%<multicurve fill-style= "none"
%	 points= "(230,235);(230,235);(230,-5);(230,-5)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(130,255);(130,255);(255,255);(255,255)"
%	 stroke-width= "0.6"
%	 />
%<multicurve fill-style= "none"
%	 points= "(255,235);(255,235);(255,255);(255,255)"
%	 stroke-width= "0.6"
%	 />
%<multicurve fill-style= "none"
%	 points= "(150,235);(150,235);(255,235);(255,235)"
%	 stroke-width= "0.6"
%	 />
%<multicurve fill-style= "none"
%	 points= "(130,255);(130,255);(150,235);(150,235)"
%	 stroke-width= "0.6"
%	 />
%<multicurve fill-style= "none"
%	 points= "(235,275);(235,275);(235,255);(235,255)"
%	 stroke-width= "0.75"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(195,245)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\utag$
%</text>
%<multicurve fill-style= "none"
%	 points= "(80,150);(80,150);(80,180);(80,180)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(80,150);(80,150);(110,150);(110,150)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(80,180);(80,180);(110,150);(110,150)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(145,185);(145,185);(165,165);(165,165)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(130,150);(130,150);(130,180);(130,180)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(130,150);(130,150);(160,150);(160,150)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(130,180);(130,180);(160,150);(160,150)"
%	 stroke-width= "0.75"
%	 />
%<parallelogram p3= "(210,55)"
%	 fill-style= "none"
%	 p2= "(210,225)"
%	 p1= "(10,225)"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(200,65)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\atilde$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(30,30)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\gtag$
%</text>
%<multicurve fill-style= "none"
%	 points= "(20,20);(20,20);(20,50);(20,50)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(20,20);(20,20);(50,20);(50,20)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(20,50);(20,50);(50,20);(50,20)"
%	 stroke-width= "0.75"
%	 />
%<parallelogram p3= "(215,15)"
%	 fill-style= "none"
%	 p2= "(215,230)"
%	 p1= "(5,230)"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(205,25)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\aflat$
%</text>
%<parallelogram p3= "(265,10)"
%	 fill-style= "none"
%	 p2= "(265,260)"
%	 p1= "(0,260)"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(255,20)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\ackermann$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(90,160)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\htag$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(140,160)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\ktag$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(172.5,175)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\specializer$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(242.5,0)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\eex$
%</text>
%<multicurve fill-style= "none"
%	 points= "(245,235);(245,235);(245,-5);(245,-5)"
%	 stroke-width= "0.75"
%	 />
%</jpic>
%%End JPIC-XML
%LaTeX-picture environment using emulated lines and arcs
%You can rescale the whole picture (to 80% for instance) by using the command \def\JPicScale{0.8}
\ifx\JPicScale\undefined\def\JPicScale{1}\fi
\unitlength \JPicScale mm
\begin{picture}(265,275)(0,0)
\linethickness{0.75mm}
\put(145,185){\line(1,0){35}}
\linethickness{0.75mm}
\multiput(180,185)(0.12,-0.12){167}{\line(1,0){0.12}}
\linethickness{0.75mm}
\put(190,175){\line(0,1){25}}
\linethickness{0.75mm}
\put(95,165){\line(0,1){35}}
\linethickness{0.75mm}
\put(165,155){\line(1,0){35}}
\linethickness{0.75mm}
\put(200,135){\line(0,1){20}}
\linethickness{0.75mm}
\put(190,155){\line(0,1){10}}
\linethickness{0.75mm}
\put(185,135){\line(1,0){15}}
\linethickness{0.75mm}
\multiput(35,75)(0.24,0.12){583}{\line(1,0){0.24}}
\linethickness{0.75mm}
\multiput(165,155)(0.12,-0.12){167}{\line(1,0){0.12}}
\linethickness{0.6mm}
\multiput(110,65)(0.24,0.12){333}{\line(1,0){0.24}}
\put(187.5,145){\makebox(0,0)[cc]{$\utag$}}

\linethickness{0.75mm}
\put(35,105){\line(0,1){60}}
\linethickness{0.6mm}
\put(15,185){\line(1,0){40}}
\linethickness{0.6mm}
\put(55,165){\line(0,1){20}}
\linethickness{0.6mm}
\put(15,165){\line(1,0){40}}
\linethickness{0.6mm}
\put(15,165){\line(0,1){20}}
\linethickness{0.75mm}
\put(35,185){\line(0,1){10}}
\linethickness{0.75mm}
\put(110,-5){\line(0,1){70}}
\linethickness{0.6mm}
\multiput(35,105)(0.23,-0.12){333}{\line(1,0){0.23}}
\linethickness{0.75mm}
\put(35,185){\line(0,1){25}}
\linethickness{0.6mm}
\put(25,220){\line(1,0){180}}
\linethickness{0.6mm}
\put(205,200){\line(0,1){20}}
\linethickness{0.6mm}
\put(45,200){\line(1,0){160}}
\linethickness{0.6mm}
\multiput(25,220)(0.12,-0.12){167}{\line(1,0){0.12}}
\linethickness{0.75mm}
\put(140,220){\line(0,1){25}}
\linethickness{0.6mm}
\put(205,110){\line(0,1){15}}
\linethickness{0.6mm}
\put(175,110){\line(1,0){30}}
\linethickness{0.6mm}
\put(175,110){\line(0,1){15}}
\linethickness{0.75mm}
\put(190,125){\line(0,1){10}}
\linethickness{0.75mm}
\put(190,105){\line(0,1){5}}
\linethickness{0.75mm}
\put(35,35){\line(0,1){40}}
\linethickness{0.3mm}
\put(112.56,64.75){\line(0,1){0.51}}
\multiput(112.46,64.25)(0.1,0.5){1}{\line(0,1){0.5}}
\multiput(112.27,63.78)(0.1,0.23){2}{\line(0,1){0.23}}
\multiput(111.99,63.36)(0.14,0.21){2}{\line(0,1){0.21}}
\multiput(111.63,63.01)(0.12,0.12){3}{\line(0,1){0.12}}
\multiput(111.21,62.72)(0.21,0.14){2}{\line(1,0){0.21}}
\multiput(110.75,62.53)(0.23,0.1){2}{\line(1,0){0.23}}
\multiput(110.25,62.43)(0.49,0.1){1}{\line(1,0){0.49}}
\put(109.75,62.43){\line(1,0){0.5}}
\multiput(109.25,62.53)(0.49,-0.1){1}{\line(1,0){0.49}}
\multiput(108.79,62.72)(0.23,-0.1){2}{\line(1,0){0.23}}
\multiput(108.37,63.01)(0.21,-0.14){2}{\line(1,0){0.21}}
\multiput(108.01,63.36)(0.12,-0.12){3}{\line(0,-1){0.12}}
\multiput(107.73,63.78)(0.14,-0.21){2}{\line(0,-1){0.21}}
\multiput(107.54,64.25)(0.1,-0.23){2}{\line(0,-1){0.23}}
\multiput(107.44,64.75)(0.1,-0.5){1}{\line(0,-1){0.5}}
\put(107.44,64.75){\line(0,1){0.51}}
\multiput(107.44,65.25)(0.1,0.5){1}{\line(0,1){0.5}}
\multiput(107.54,65.75)(0.1,0.23){2}{\line(0,1){0.23}}
\multiput(107.73,66.22)(0.14,0.21){2}{\line(0,1){0.21}}
\multiput(108.01,66.64)(0.12,0.12){3}{\line(0,1){0.12}}
\multiput(108.37,66.99)(0.21,0.14){2}{\line(1,0){0.21}}
\multiput(108.79,67.28)(0.23,0.1){2}{\line(1,0){0.23}}
\multiput(109.25,67.47)(0.49,0.1){1}{\line(1,0){0.49}}
\put(109.75,67.57){\line(1,0){0.5}}
\multiput(110.25,67.57)(0.49,-0.1){1}{\line(1,0){0.49}}
\multiput(110.75,67.47)(0.23,-0.1){2}{\line(1,0){0.23}}
\multiput(111.21,67.28)(0.21,-0.14){2}{\line(1,0){0.21}}
\multiput(111.63,66.99)(0.12,-0.12){3}{\line(0,-1){0.12}}
\multiput(111.99,66.64)(0.14,-0.21){2}{\line(0,-1){0.21}}
\multiput(112.27,66.22)(0.1,-0.23){2}{\line(0,-1){0.23}}
\multiput(112.46,65.75)(0.1,-0.5){1}{\line(0,-1){0.5}}

\put(35,175){\makebox(0,0)[cc]{$\zerotag$}}

\put(117.5,210){\makebox(0,0)[cc]{$\iiftag$}}

\linethickness{0.75mm}
\multiput(145,165)(0.12,0.12){83}{\line(1,0){0.12}}
\linethickness{0.75mm}
\put(165,165){\line(1,0){35}}
\put(190,117.5){\makebox(0,0)[cc]{$\predtag$}}

\put(32.5,65){\makebox(0,0)[cr]{$\pee$}}

\put(107.5,0){\makebox(0,0)[cr]{$\een$}}

\put(227.5,0){\makebox(0,0)[cr]{$\eex$}}

\linethickness{0.6mm}
\put(175,125){\line(1,0){30}}
\linethickness{0.75mm}
\put(230,-5){\line(0,1){240}}
\linethickness{0.6mm}
\put(130,255){\line(1,0){125}}
\linethickness{0.6mm}
\put(255,235){\line(0,1){20}}
\linethickness{0.6mm}
\put(150,235){\line(1,0){105}}
\linethickness{0.6mm}
\multiput(130,255)(0.12,-0.12){167}{\line(1,0){0.12}}
\linethickness{0.75mm}
\put(235,255){\line(0,1){20}}
\put(195,245){\makebox(0,0)[cc]{$\utag$}}

\linethickness{0.75mm}
\put(80,150){\line(0,1){30}}
\linethickness{0.75mm}
\put(80,150){\line(1,0){30}}
\linethickness{0.75mm}
\multiput(80,180)(0.12,-0.12){250}{\line(1,0){0.12}}
\linethickness{0.75mm}
\multiput(145,185)(0.12,-0.12){167}{\line(1,0){0.12}}
\linethickness{0.75mm}
\put(130,150){\line(0,1){30}}
\linethickness{0.75mm}
\put(130,150){\line(1,0){30}}
\linethickness{0.75mm}
\multiput(130,180)(0.12,-0.12){250}{\line(1,0){0.12}}
\linethickness{0.3mm}
\put(10,225){\line(1,0){200}}
\put(10,55){\line(0,1){170}}
\put(210,55){\line(0,1){170}}
\put(10,55){\line(1,0){200}}
\put(200,65){\makebox(0,0)[cc]{$\atilde$}}

\put(30,30){\makebox(0,0)[cc]{$\gtag$}}

\linethickness{0.75mm}
\put(20,20){\line(0,1){30}}
\linethickness{0.75mm}
\put(20,20){\line(1,0){30}}
\linethickness{0.75mm}
\multiput(20,50)(0.12,-0.12){250}{\line(1,0){0.12}}
\linethickness{0.3mm}
\put(5,230){\line(1,0){210}}
\put(5,15){\line(0,1){215}}
\put(215,15){\line(0,1){215}}
\put(5,15){\line(1,0){210}}
\put(205,25){\makebox(0,0)[cc]{$\aflat$}}

\linethickness{0.3mm}
\put(0,260){\line(1,0){265}}
\put(0,10){\line(0,1){250}}
\put(265,10){\line(0,1){250}}
\put(0,10){\line(1,0){265}}
\put(255,20){\makebox(0,0)[cc]{$\ackermann$}}

\put(90,160){\makebox(0,0)[cc]{$\htag$}}

\put(140,160){\makebox(0,0)[cc]{$\ktag$}}

\put(172.5,175){\makebox(0,0)[cc]{$\specializer$}}

\put(242.5,0){\makebox(0,0)[cr]{$\eex$}}

\linethickness{0.75mm}
\put(245,-5){\line(0,1){240}}
\end{picture}


==> PIC/FOR.tex <==
%%Created by jPicEdt 1.4.1_03: mixed JPIC-XML/LaTeX format
%%Thu Dec 07 22:54:55 HST 2017
%%Begin JPIC-XML
%<?xml version="1.0" standalone="yes"?>
%<jpic x-min="0" x-max="250" y-min="0" y-max="205" auto-bounding="true">
%<multicurve stroke-width= "0.75"
%	 points= "(145,150);(145,150);(250,150);(250,150)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.75"
%	 points= "(250,130);(250,130);(250,150);(250,150)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.75"
%	 points= "(165,130);(165,130);(250,130);(250,130)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.6"
%	 points= "(140,40);(140,40);(200,80);(200,80)"
%	 fill-style= "none"
%	 />
%<text text-vert-align= "center-v"
%	 anchor-point= "(205,140)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\utag$
%</text>
%<multicurve stroke-width= "0.75"
%	 points= "(40,130);(40,130);(40,40);(40,40)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.6"
%	 points= "(20,150);(20,150);(60,150);(60,150)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.6"
%	 points= "(60,130);(60,130);(60,150);(60,150)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.6"
%	 points= "(20,130);(20,130);(60,130);(60,130)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.6"
%	 points= "(20,150);(20,150);(20,130);(20,130)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.75"
%	 points= "(100,165);(100,165);(100,65.62);(100,65.62)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.6"
%	 points= "(40,40);(40,40);(70,20);(70,20)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.75"
%	 points= "(40,175);(40,175);(40,150);(40,150)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.6"
%	 points= "(30,185);(30,185);(250,185);(250,185)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.6"
%	 points= "(250,165);(250,165);(250,185);(250,185)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.6"
%	 points= "(30,185);(30,185);(50,165);(50,165)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.75"
%	 points= "(152.5,205);(152.5,205);(152.5,185);(152.5,185)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.75"
%	 points= "(240,130);(240,130);(240,100);(240,100)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.6"
%	 points= "(180,100);(180,100);(180,120);(180,120)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.6"
%	 points= "(160,100);(160,100);(180,100);(180,100)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.6"
%	 points= "(160,120);(160,120);(160,100);(160,100)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.75"
%	 points= "(170,130);(170,130);(170,120);(170,120)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.75"
%	 points= "(170,100);(170,100);(170,86.25);(170,86.25)"
%	 fill-style= "none"
%	 />
%<ellipse p3= "(142.57,37.42)"
%	 p2= "(142.57,42.58)"
%	 p1= "(137.43,42.58)"
%	 closure= "open"
%	 angle-end= "0"
%	 fill-style= "solid"
%	 angle-start= "0"
%	 fill-color= "#330033"
%	 />
%<text text-vert-align= "center-v"
%	 anchor-point= "(40,140)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\zerotag$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(152.5,175)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\iiftag$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(170,110)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\predtag$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(67.5,5)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\een$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(137.5,5)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\eex$
%</text>
%<multicurve stroke-width= "0.6"
%	 points= "(160,120);(160,120);(180,120);(180,120)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.6"
%	 points= "(220,100);(220,100);(220,120);(220,120)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.6"
%	 points= "(190,100);(190,100);(220,100);(220,100)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.6"
%	 points= "(190,120);(190,120);(190,100);(190,100)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.75"
%	 points= "(205,130);(205,130);(205,120);(205,120)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.75"
%	 points= "(205,165);(205,165);(205,150);(205,150)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.6"
%	 points= "(190,120);(190,120);(220,120);(220,120)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.6"
%	 points= "(0,30);(0,30);(30,0);(30,0)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.6"
%	 points= "(30,0);(30,0);(0,0);(0,0)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.6"
%	 points= "(0,0);(0,0);(0,30);(0,30)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.75"
%	 points= "(15,50);(15,50);(15,15);(15,15)"
%	 fill-style= "none"
%	 />
%<text text-vert-align= "center-v"
%	 anchor-point= "(10,10)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\function$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(205,110)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\sucetag$
%</text>
%<multicurve stroke-width= "0.6"
%	 points= "(50,165);(50,165);(250,165);(250,165)"
%	 fill-style= "none"
%	 />
%<ellipse p3= "(72.57,17.42)"
%	 p2= "(72.57,22.58)"
%	 p1= "(67.43,22.58)"
%	 closure= "open"
%	 angle-end= "0"
%	 fill-style= "solid"
%	 angle-start= "0"
%	 fill-color= "#330033"
%	 />
%<multicurve stroke-width= "0.6"
%	 points= "(210,0);(210,0);(210,100);(210,100)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-overstrike-width= "1.5"
%	 stroke-overstrike= "true"
%	 stroke-width= "0.75"
%	 points= "(155,140);(155,140);(15,50);(15,50)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.75"
%	 points= "(145,150);(145,150);(165,130);(165,130)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.6"
%	 points= "(200,80);(200,80);(200,100);(200,100)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.6"
%	 points= "(70,0);(70,0);(70,20);(70,20)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.6"
%	 points= "(70,20);(70,20);(170,86.25);(170,86.25)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.6"
%	 points= "(210,80);(210,80);(240,100);(240,100)"
%	 fill-style= "none"
%	 />
%<ellipse p3= "(212.57,77.42)"
%	 p2= "(212.57,82.58)"
%	 p1= "(207.43,82.58)"
%	 closure= "open"
%	 angle-end= "0"
%	 fill-style= "solid"
%	 angle-start= "0"
%	 fill-color= "#330033"
%	 />
%<multicurve stroke-width= "0.6"
%	 points= "(100,66.25);(100,66.25);(140,40);(140,40)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.75"
%	 points= "(140,40);(140,40);(140,0);(140,0)"
%	 fill-style= "none"
%	 />
%<text text-vert-align= "center-v"
%	 anchor-point= "(207.5,5)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\eey$
%</text>
%</jpic>
%%End JPIC-XML
%PSTricks content-type (pstricks.sty package needed)
%Add \usepackage{pstricks} in the preamble of your LaTeX file
%You can rescale the whole picture (to 80% for instance) by using the command \def\JPicScale{0.8}
\ifx\JPicScale\undefined\def\JPicScale{1}\fi
\psset{unit=\JPicScale mm}
\psset{linewidth=0.3,dotsep=1,hatchwidth=0.3,hatchsep=1.5,shadowsize=1,dimen=middle}
\psset{dotsize=0.7 2.5,dotscale=1 1,fillcolor=black}
\psset{arrowsize=1 2,arrowlength=1,arrowinset=0.25,tbarsize=0.7 5,bracketlength=0.15,rbracketlength=0.15}
\begin{pspicture}(0,0)(250,205)
\psline[linewidth=0.75](145,150)(250,150)
\psline[linewidth=0.75](250,130)(250,150)
\psline[linewidth=0.75](165,130)(250,130)
\psline[linewidth=0.6](140,40)(200,80)
\rput(205,140){$\utag$}
\psline[linewidth=0.75](40,130)(40,40)
\psline[linewidth=0.6](20,150)(60,150)
\psline[linewidth=0.6](60,130)(60,150)
\psline[linewidth=0.6](20,130)(60,130)
\psline[linewidth=0.6](20,150)(20,130)
\psline[linewidth=0.75](100,165)(100,65.62)
\psline[linewidth=0.6](40,40)(70,20)
\psline[linewidth=0.75](40,175)(40,150)
\psline[linewidth=0.6](30,185)(250,185)
\psline[linewidth=0.6](250,165)(250,185)
\psline[linewidth=0.6](30,185)(50,165)
\psline[linewidth=0.75](152.5,205)(152.5,185)
\psline[linewidth=0.75](240,130)(240,100)
\psline[linewidth=0.6](180,100)(180,120)
\psline[linewidth=0.6](160,100)(180,100)
\psline[linewidth=0.6](160,120)(160,100)
\psline[linewidth=0.75](170,130)(170,120)
\psline[linewidth=0.75](170,100)(170,86.25)
\newrgbcolor{userFillColour}{0.2 0 0.2}
\rput{90}(140,40){\psellipse[fillcolor=userFillColour,fillstyle=solid](0,0)(2.58,-2.57)}
\rput(40,140){$\zerotag$}
\rput(152.5,175){$\iiftag$}
\rput(170,110){$\predtag$}
\rput[r](67.5,5){$\een$}
\rput[r](137.5,5){$\eex$}
\psline[linewidth=0.6](160,120)(180,120)
\psline[linewidth=0.6](220,100)(220,120)
\psline[linewidth=0.6](190,100)(220,100)
\psline[linewidth=0.6](190,120)(190,100)
\psline[linewidth=0.75](205,130)(205,120)
\psline[linewidth=0.75](205,165)(205,150)
\psline[linewidth=0.6](190,120)(220,120)
\psline[linewidth=0.6](0,30)(30,0)
\psline[linewidth=0.6](30,0)(0,0)
\psline[linewidth=0.6](0,0)(0,30)
\psline[linewidth=0.75](15,50)(15,15)
\rput(10,10){$\function$}
\rput(205,110){$\sucetag$}
\psline[linewidth=0.6](50,165)(250,165)
\newrgbcolor{userFillColour}{0.2 0 0.2}
\rput{90}(70,20){\psellipse[fillcolor=userFillColour,fillstyle=solid](0,0)(2.58,-2.57)}
\psline[linewidth=0.6](210,0)(210,100)
\psline[linewidth=0.75,border=1.5](155,140)(15,50)
\psline[linewidth=0.75](145,150)(165,130)
\psline[linewidth=0.6](200,80)(200,100)
\psline[linewidth=0.6](70,0)(70,20)
\psline[linewidth=0.6](70,20)(170,86.25)
\psline[linewidth=0.6](210,80)(240,100)
\newrgbcolor{userFillColour}{0.2 0 0.2}
\rput{90}(210,80){\psellipse[fillcolor=userFillColour,fillstyle=solid](0,0)(2.58,-2.57)}
\psline[linewidth=0.6](100,66.25)(140,40)
\psline[linewidth=0.75](140,40)(140,0)
\rput[r](207.5,5){$\eey$}
\end{pspicture}


==> PIC/MU-root.tex <==
%%Created by jPicEdt 1.4.1_03: mixed JPIC-XML/LaTeX format
%%Sat Nov 10 07:52:51 GMT-10:00 2018
%%Begin JPIC-XML
%<?xml version="1.0" standalone="yes"?>
%<jpic x-min="0" x-max="210" y-min="0" y-max="190" auto-bounding="true">
%<multicurve fill-style= "none"
%	 stroke-width= "0.6"
%	 points= "(10,110);(10,110);(50,110);(50,110)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.6"
%	 points= "(50,90);(50,90);(50,110);(50,110)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.6"
%	 points= "(10,110);(10,110);(10,90);(10,90)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(150,135);(150,135);(210,135);(210,135)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(210,115);(210,115);(210,135);(210,135)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(190,150);(190,150);(190,135);(190,135)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(170,115);(170,115);(210,115);(210,115)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(160,125);(160,125);(10,50);(10,50)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(150,135);(150,135);(170,115);(170,115)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(120,40);(120,40);(120,0);(120,0)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.6"
%	 points= "(100,40);(100,40);(180,80);(180,80)"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(185,125)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\utag$
%</text>
%<multicurve fill-style= "none"
%	 stroke-width= "0.6"
%	 points= "(20,135);(20,135);(40,135);(40,135)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.6"
%	 points= "(40,120);(40,120);(40,135);(40,135)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.6"
%	 points= "(20,120);(20,120);(40,120);(40,120)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.6"
%	 points= "(20,135);(20,135);(20,120);(20,120)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(100,40);(100,40);(100,0);(100,0)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.6"
%	 stroke-overstrike= "true"
%	 points= "(20,80);(20,80);(100,40);(100,40)"
%	 stroke-overstrike-width= "2"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(30,160);(30,160);(30,135);(30,135)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.6"
%	 points= "(20,170);(20,170);(210,170);(210,170)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.6"
%	 points= "(210,150);(210,150);(210,170);(210,170)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.6"
%	 points= "(20,170);(20,170);(40,150);(40,150)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(120,190);(120,190);(120,170);(120,170)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.6"
%	 points= "(120,40);(120,40);(200,80);(200,80)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.6"
%	 points= "(190,90);(190,90);(190,105);(190,105)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.6"
%	 points= "(170,90);(170,90);(190,90);(190,90)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.6"
%	 points= "(170,105);(170,105);(170,90);(170,90)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(180,90);(180,90);(180,80);(180,80)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(10,50);(10,50);(10,20);(10,20)"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(30,100)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\gtag$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(30,127.5)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\zerotag$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(120,160)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\iiftag$
%</text>
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 stroke-overstrike= "true"
%	 points= "(40,90);(40,90);(40,80);(40,80)"
%	 stroke-overstrike-width= "2"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.6"
%	 points= "(10,90);(10,90);(50,90);(50,90)"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(180,97.5)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\predtag$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(5,15)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\pee$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(97.5,2.5)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\een$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(117.5,2.5)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\eex$
%</text>
%<multicurve fill-style= "none"
%	 stroke-width= "0.6"
%	 points= "(170,105);(170,105);(190,105);(190,105)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(20,90);(20,90);(20,80);(20,80)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(30,120);(30,120);(30,110);(30,110)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(180,115);(180,115);(180,105);(180,105)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(200,80);(200,80);(200,115);(200,115)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 stroke-overstrike= "true"
%	 points= "(100,150);(100,150);(100,40);(100,40)"
%	 stroke-overstrike-width= "1.3"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.6"
%	 stroke-overstrike= "true"
%	 points= "(120,40);(120,40);(40,80);(40,80)"
%	 stroke-overstrike-width= "2"
%	 />
%<ellipse fill-color= "#330033"
%	 p3= "(102.57,37.42)"
%	 p2= "(102.57,42.58)"
%	 fill-style= "solid"
%	 p1= "(97.43,42.58)"
%	 closure= "open"
%	 angle-end= "0"
%	 angle-start= "0"
%	 />
%<ellipse fill-color= "#330033"
%	 p3= "(122.57,37.42)"
%	 p2= "(122.57,42.58)"
%	 fill-style= "solid"
%	 p1= "(117.43,42.58)"
%	 closure= "open"
%	 angle-end= "0"
%	 angle-start= "0"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.6"
%	 points= "(40,150);(40,150);(210,150);(210,150)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.6"
%	 points= "(0,30);(0,30);(20,10);(20,10)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.6"
%	 points= "(20,10);(20,10);(0,10);(0,10)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.6"
%	 points= "(0,10);(0,10);(0,30);(0,30)"
%	 />
%</jpic>
%%End JPIC-XML
%PSTricks content-type (pstricks.sty package needed)
%Add \usepackage{pstricks} in the preamble of your LaTeX file
%You can rescale the whole picture (to 80% for instance) by using the command \def\JPicScale{0.8}
\ifx\JPicScale\undefined\def\JPicScale{1}\fi
\psset{unit=\JPicScale mm}
\psset{linewidth=0.3,dotsep=1,hatchwidth=0.3,hatchsep=1.5,shadowsize=1,dimen=middle}
\psset{dotsize=0.7 2.5,dotscale=1 1,fillcolor=black}
\psset{arrowsize=1 2,arrowlength=1,arrowinset=0.25,tbarsize=0.7 5,bracketlength=0.15,rbracketlength=0.15}
\begin{pspicture}(0,0)(210,190)
\psline[linewidth=0.6](10,110)(50,110)
\psline[linewidth=0.6](50,90)(50,110)
\psline[linewidth=0.6](10,110)(10,90)
\psline[linewidth=0.75](150,135)(210,135)
\psline[linewidth=0.75](210,115)(210,135)
\psline[linewidth=0.75](190,150)(190,135)
\psline[linewidth=0.75](170,115)(210,115)
\psline[linewidth=0.75](160,125)(10,50)
\psline[linewidth=0.75](150,135)(170,115)
\psline[linewidth=0.75](120,40)(120,0)
\psline[linewidth=0.6](100,40)(180,80)
\rput(185,125){$\utag$}
\psline[linewidth=0.6](20,135)(40,135)
\psline[linewidth=0.6](40,120)(40,135)
\psline[linewidth=0.6](20,120)(40,120)
\psline[linewidth=0.6](20,135)(20,120)
\psline[linewidth=0.75](100,40)(100,0)
\psline[linewidth=0.6,border=2](20,80)(100,40)
\psline[linewidth=0.75](30,160)(30,135)
\psline[linewidth=0.6](20,170)(210,170)
\psline[linewidth=0.6](210,150)(210,170)
\psline[linewidth=0.6](20,170)(40,150)
\psline[linewidth=0.75](120,190)(120,170)
\psline[linewidth=0.6](120,40)(200,80)
\psline[linewidth=0.6](190,90)(190,105)
\psline[linewidth=0.6](170,90)(190,90)
\psline[linewidth=0.6](170,105)(170,90)
\psline[linewidth=0.75](180,90)(180,80)
\psline[linewidth=0.75](10,50)(10,20)
\rput(30,100){$\gtag$}
\rput(30,127.5){$\zerotag$}
\rput(120,160){$\iiftag$}
\psline[linewidth=0.75,border=2](40,90)(40,80)
\psline[linewidth=0.6](10,90)(50,90)
\rput(180,97.5){$\predtag$}
\rput(5,15){$\pee$}
\rput[r](97.5,2.5){$\een$}
\rput[r](117.5,2.5){$\eex$}
\psline[linewidth=0.6](170,105)(190,105)
\psline[linewidth=0.75](20,90)(20,80)
\psline[linewidth=0.75](30,120)(30,110)
\psline[linewidth=0.75](180,115)(180,105)
\psline[linewidth=0.75](200,80)(200,115)
\psline[linewidth=0.75,border=1.3](100,150)(100,40)
\psline[linewidth=0.6,border=2](120,40)(40,80)
\newrgbcolor{userFillColour}{0.2 0 0.2}
\rput{90}(100,40){\psellipse[fillcolor=userFillColour,fillstyle=solid](0,0)(2.58,-2.57)}
\newrgbcolor{userFillColour}{0.2 0 0.2}
\rput{90}(120,40){\psellipse[fillcolor=userFillColour,fillstyle=solid](0,0)(2.58,-2.57)}
\psline[linewidth=0.6](40,150)(210,150)
\psline[linewidth=0.6](0,30)(20,10)
\psline[linewidth=0.6](20,10)(0,10)
\psline[linewidth=0.6](0,10)(0,30)
\end{pspicture}


==> PIC/Omega-1.tex <==
%%Created by jPicEdt 1.4.1_03: mixed JPIC-XML/LaTeX format
%%Sun Feb 21 22:41:20 GMT-10:00 2021
%%Begin JPIC-XML
%<?xml version="1.0" standalone="yes"?>
%<jpic x-min="17.5" x-max="47.5" y-min="0" y-max="90" auto-bounding="true">
%<multicurve fill-style= "none"
%	 points= "(40,20);(40,20);(40,0);(40,0)"
%	 />
%<ellipse p3= "(41.25,18.75)"
%	 fill-style= "solid"
%	 p2= "(41.25,21.25)"
%	 p1= "(38.75,21.25)"
%	 closure= "open"
%	 angle-end= "360"
%	 angle-start= "0"
%	 />
%<multicurve fill-style= "none"
%	 points= "(45,25);(45,25);(40,20);(40,20)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(40,20);(40,20);(35,25);(35,25)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(35,25);(35,25);(35,36.25);(35,36.25)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(45,25);(45,25);(45,70);(45,70)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(30,55);(30,55);(40,55);(40,55)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(20,65);(20,65);(30,65);(30,65)"
%	 />
%<ellipse p3= "(38.52,36.48)"
%	 fill-style= "none"
%	 p2= "(38.52,43.52)"
%	 p1= "(31.48,43.52)"
%	 closure= "open"
%	 angle-end= "360"
%	 angle-start= "0"
%	 />
%<multicurve fill-style= "none"
%	 points= "(35,43.75);(35,43.75);(35,55);(35,55)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(30,65);(30,65);(40,55);(40,55)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(20,65);(20,65);(30,55);(30,55)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(20,57.5);(20,57.5);(30,47.5);(30,47.5)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(35,60);(35,60);(35,70);(35,70)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(25,52.5);(25,52.5);(25,60);(25,60)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(20,47.5);(20,47.5);(30,47.5);(30,47.5)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(20,57.5);(20,57.5);(20,47.5);(20,47.5)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(32.5,70);(32.5,70);(47.5,70);(47.5,70)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(32.5,85);(32.5,85);(32.5,70);(32.5,70)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(32.5,85);(32.5,85);(47.5,70);(47.5,70)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(40,90);(40,90);(40,77.5);(40,77.5)"
%	 />
%<multicurve fill-style= "solid"
%	 points= "(17.5,67.5);(17.5,67.5);(32.5,67.5);(32.5,67.5)"
%	 stroke-width= "0.15"
%	 />
%<multicurve fill-style= "solid"
%	 points= "(17.5,45);(17.5,45);(17.5,67.5);(17.5,67.5)"
%	 stroke-width= "0.15"
%	 />
%<multicurve fill-style= "solid"
%	 points= "(42.5,45);(42.5,45);(17.5,45);(17.5,45)"
%	 stroke-width= "0.15"
%	 />
%<multicurve fill-style= "solid"
%	 points= "(42.5,57.5);(42.5,57.5);(42.5,45);(42.5,45)"
%	 stroke-width= "0.15"
%	 />
%<multicurve fill-style= "solid"
%	 points= "(32.5,67.5);(32.5,67.5);(42.5,57.5);(42.5,57.5)"
%	 stroke-width= "0.15"
%	 />
%</jpic>
%%End JPIC-XML
%PSTricks content-type (pstricks.sty package needed)
%Add \usepackage{pstricks} in the preamble of your LaTeX file
%You can rescale the whole picture (to 80% for instance) by using the command \def\JPicScale{0.8}
\ifx\JPicScale\undefined\def\JPicScale{1}\fi
\psset{unit=\JPicScale mm}
\psset{linewidth=0.3,dotsep=1,hatchwidth=0.3,hatchsep=1.5,shadowsize=1,dimen=middle}
\psset{dotsize=0.7 2.5,dotscale=1 1,fillcolor=black}
\psset{arrowsize=1 2,arrowlength=1,arrowinset=0.25,tbarsize=0.7 5,bracketlength=0.15,rbracketlength=0.15}
\begin{pspicture}(0,0)(47.5,90)
\psline(40,20)(40,0)
\rput{0}(40,20){\psellipse[fillstyle=solid](0,0)(1.25,-1.25)}
\psline(45,25)(40,20)
\psline(40,20)(35,25)
\psline(35,25)(35,36.25)
\psline(45,25)(45,70)
\psline(30,55)(40,55)
\psline(20,65)(30,65)
\rput{0}(35,40){\psellipse[](0,0)(3.52,-3.52)}
\psline(35,43.75)(35,55)
\psline(30,65)(40,55)
\psline(20,65)(30,55)
\psline(20,57.5)(30,47.5)
\psline(35,60)(35,70)
\psline(25,52.5)(25,60)
\psline(20,47.5)(30,47.5)
\psline(20,57.5)(20,47.5)
\psline(32.5,70)(47.5,70)
\psline(32.5,85)(32.5,70)
\psline(32.5,85)(47.5,70)
\psline(40,90)(40,77.5)
\psline[linewidth=0.15,fillstyle=solid](17.5,67.5)(32.5,67.5)
\psline[linewidth=0.15,fillstyle=solid](17.5,45)(17.5,67.5)
\psline[linewidth=0.15,fillstyle=solid](42.5,45)(17.5,45)
\psline[linewidth=0.15,fillstyle=solid](42.5,57.5)(42.5,45)
\psline[linewidth=0.15,fillstyle=solid](32.5,67.5)(42.5,57.5)
\end{pspicture}


==> PIC/Omega-2.tex <==
%%Created by jPicEdt 1.4.1_03: mixed JPIC-XML/LaTeX format
%%Mon Feb 22 16:51:55 GMT-10:00 2021
%%Begin JPIC-XML
%<?xml version="1.0" standalone="yes"?>
%<jpic x-min="0" x-max="77.5" y-min="0" y-max="75" auto-bounding="true">
%<multicurve fill-style= "none"
%	 points= "(20,10);(20,10);(20,0);(20,0)"
%	 stroke-width= "0.5"
%	 />
%<ellipse p3= "(21.25,8.75)"
%	 fill-style= "solid"
%	 p2= "(21.25,11.25)"
%	 p1= "(18.75,11.25)"
%	 closure= "open"
%	 angle-end= "0"
%	 stroke-width= "0.5"
%	 angle-start= "0"
%	 />
%<multicurve fill-style= "none"
%	 points= "(25,15);(25,15);(20,10);(20,10)"
%	 stroke-width= "0.5"
%	 />
%<multicurve fill-style= "none"
%	 points= "(20,10);(20,10);(15,15);(15,15)"
%	 stroke-width= "0.5"
%	 />
%<multicurve fill-style= "none"
%	 points= "(15,15);(15,15);(15,21.25);(15,21.25)"
%	 stroke-width= "0.5"
%	 />
%<multicurve fill-style= "none"
%	 points= "(25,15);(25,15);(25,55);(25,55)"
%	 stroke-width= "0.5"
%	 />
%<multicurve fill-style= "none"
%	 points= "(10,40);(10,40);(20,40);(20,40)"
%	 stroke-width= "0.5"
%	 />
%<multicurve fill-style= "none"
%	 points= "(0,50);(0,50);(10,50);(10,50)"
%	 stroke-width= "0.5"
%	 />
%<ellipse p3= "(18.52,21.48)"
%	 fill-style= "none"
%	 p2= "(18.52,28.52)"
%	 p1= "(11.48,28.52)"
%	 closure= "open"
%	 angle-end= "0"
%	 stroke-width= "0.5"
%	 angle-start= "0"
%	 />
%<multicurve fill-style= "none"
%	 points= "(15,28.75);(15,28.75);(15,40);(15,40)"
%	 stroke-width= "0.5"
%	 />
%<multicurve fill-style= "none"
%	 points= "(10,50);(10,50);(20,40);(20,40)"
%	 stroke-width= "0.5"
%	 />
%<multicurve fill-style= "none"
%	 points= "(0,50);(0,50);(10,40);(10,40)"
%	 stroke-width= "0.5"
%	 />
%<multicurve fill-style= "none"
%	 points= "(0,42.5);(0,42.5);(10,32.5);(10,32.5)"
%	 stroke-width= "0.5"
%	 />
%<multicurve fill-style= "none"
%	 points= "(15,45);(15,45);(15,55);(15,55)"
%	 stroke-width= "0.5"
%	 />
%<multicurve fill-style= "none"
%	 points= "(5,37.5);(5,37.5);(5,45);(5,45)"
%	 stroke-width= "0.5"
%	 />
%<multicurve fill-style= "none"
%	 points= "(0,32.5);(0,32.5);(10,32.5);(10,32.5)"
%	 stroke-width= "0.5"
%	 />
%<multicurve fill-style= "none"
%	 points= "(0,42.5);(0,42.5);(0,32.5);(0,32.5)"
%	 stroke-width= "0.5"
%	 />
%<multicurve fill-style= "none"
%	 points= "(12.5,55);(12.5,55);(27.5,55);(27.5,55)"
%	 stroke-width= "0.5"
%	 />
%<multicurve fill-style= "none"
%	 points= "(12.5,70);(12.5,70);(12.5,55);(12.5,55)"
%	 stroke-width= "0.5"
%	 />
%<multicurve fill-style= "none"
%	 points= "(12.5,70);(12.5,70);(27.5,55);(27.5,55)"
%	 stroke-width= "0.5"
%	 />
%<multicurve fill-style= "none"
%	 points= "(20,75);(20,75);(20,62.5);(20,62.5)"
%	 stroke-width= "0.5"
%	 />
%<multicurve fill-style= "none"
%	 points= "(65,40);(65,40);(75,40);(75,40)"
%	 stroke-width= "0.5"
%	 />
%<multicurve fill-style= "none"
%	 points= "(55,50);(55,50);(75,50);(75,50)"
%	 stroke-width= "0.5"
%	 />
%<multicurve fill-style= "none"
%	 points= "(70,0);(70,0);(70,40);(70,40)"
%	 stroke-width= "0.5"
%	 />
%<multicurve fill-style= "none"
%	 points= "(55,50);(55,50);(65,40);(65,40)"
%	 stroke-width= "0.5"
%	 />
%<multicurve fill-style= "none"
%	 points= "(55,42.5);(55,42.5);(65,32.5);(65,32.5)"
%	 stroke-width= "0.5"
%	 />
%<multicurve fill-style= "none"
%	 points= "(60,37.5);(60,37.5);(60,45);(60,45)"
%	 stroke-width= "0.5"
%	 />
%<multicurve fill-style= "none"
%	 points= "(55,32.5);(55,32.5);(65,32.5);(65,32.5)"
%	 stroke-width= "0.5"
%	 />
%<multicurve fill-style= "none"
%	 points= "(55,42.5);(55,42.5);(55,32.5);(55,32.5)"
%	 stroke-width= "0.5"
%	 />
%<multicurve fill-style= "none"
%	 points= "(75,50);(75,50);(75,40);(75,40)"
%	 stroke-width= "0.5"
%	 />
%<multicurve fill-style= "none"
%	 points= "(70,75);(70,75);(70,50);(70,50)"
%	 stroke-width= "0.5"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "solid"
%	 anchor-point= "(40,45)"
%	 text-frame= "noframe"
%	 stroke-width= "0.5"
%	 text-hor-align= "center-h"
%	 >
%\EQLS
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "solid"
%	 anchor-point= "(2.5,35)"
%	 text-frame= "noframe"
%	 stroke-width= "0.5"
%	 text-hor-align= "center-h"
%	 >
%$\Nee$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "solid"
%	 anchor-point= "(57.5,35)"
%	 text-frame= "noframe"
%	 stroke-width= "0.5"
%	 text-hor-align= "center-h"
%	 >
%$\Nee$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "solid"
%	 anchor-point= "(15,25)"
%	 text-frame= "noframe"
%	 stroke-width= "0.5"
%	 text-hor-align= "center-h"
%	 >
%$\addd$
%</text>
%<multicurve fill-style= "solid"
%	 points= "(52.5,52.5);(52.5,52.5);(77.5,52.5);(77.5,52.5)"
%	 stroke-width= "0.15"
%	 />
%<multicurve fill-style= "solid"
%	 points= "(52.5,30);(52.5,30);(52.5,52.5);(52.5,52.5)"
%	 stroke-width= "0.15"
%	 />
%<multicurve fill-style= "solid"
%	 points= "(77.5,30);(77.5,30);(52.5,30);(52.5,30)"
%	 stroke-width= "0.15"
%	 />
%<multicurve fill-style= "solid"
%	 points= "(77.5,52.5);(77.5,52.5);(77.5,30);(77.5,30)"
%	 stroke-width= "0.15"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "solid"
%	 anchor-point= "(75,32.5)"
%	 text-frame= "noframe"
%	 stroke-width= "0.5"
%	 text-hor-align= "center-h"
%	 >
%$\Homega$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "solid"
%	 anchor-point= "(69.38,45)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\unl$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "solid"
%	 anchor-point= "(10,45)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\pnl$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "solid"
%	 anchor-point= "(17.5,58.75)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\png$
%</text>
%</jpic>
%%End JPIC-XML
%PSTricks content-type (pstricks.sty package needed)
%Add \usepackage{pstricks} in the preamble of your LaTeX file
%You can rescale the whole picture (to 80% for instance) by using the command \def\JPicScale{0.8}
\ifx\JPicScale\undefined\def\JPicScale{1}\fi
\psset{unit=\JPicScale mm}
\psset{linewidth=0.3,dotsep=1,hatchwidth=0.3,hatchsep=1.5,shadowsize=1,dimen=middle}
\psset{dotsize=0.7 2.5,dotscale=1 1,fillcolor=black}
\psset{arrowsize=1 2,arrowlength=1,arrowinset=0.25,tbarsize=0.7 5,bracketlength=0.15,rbracketlength=0.15}
\begin{pspicture}(0,0)(77.5,75)
\psline[linewidth=0.5](20,10)(20,0)
\rput{0}(20,10){\psellipse[linewidth=0.5,fillstyle=solid](0,0)(1.25,-1.25)}
\psline[linewidth=0.5](25,15)(20,10)
\psline[linewidth=0.5](20,10)(15,15)
\psline[linewidth=0.5](15,15)(15,21.25)
\psline[linewidth=0.5](25,15)(25,55)
\psline[linewidth=0.5](10,40)(20,40)
\psline[linewidth=0.5](0,50)(10,50)
\rput{0}(15,25){\psellipse[linewidth=0.5](0,0)(3.52,-3.52)}
\psline[linewidth=0.5](15,28.75)(15,40)
\psline[linewidth=0.5](10,50)(20,40)
\psline[linewidth=0.5](0,50)(10,40)
\psline[linewidth=0.5](0,42.5)(10,32.5)
\psline[linewidth=0.5](15,45)(15,55)
\psline[linewidth=0.5](5,37.5)(5,45)
\psline[linewidth=0.5](0,32.5)(10,32.5)
\psline[linewidth=0.5](0,42.5)(0,32.5)
\psline[linewidth=0.5](12.5,55)(27.5,55)
\psline[linewidth=0.5](12.5,70)(12.5,55)
\psline[linewidth=0.5](12.5,70)(27.5,55)
\psline[linewidth=0.5](20,75)(20,62.5)
\psline[linewidth=0.5](65,40)(75,40)
\psline[linewidth=0.5](55,50)(75,50)
\psline[linewidth=0.5](70,0)(70,40)
\psline[linewidth=0.5](55,50)(65,40)
\psline[linewidth=0.5](55,42.5)(65,32.5)
\psline[linewidth=0.5](60,37.5)(60,45)
\psline[linewidth=0.5](55,32.5)(65,32.5)
\psline[linewidth=0.5](55,42.5)(55,32.5)
\psline[linewidth=0.5](75,50)(75,40)
\psline[linewidth=0.5](70,75)(70,50)
\rput(40,45){\EQLS}
\rput(2.5,35){$\Nee$}
\rput(57.5,35){$\Nee$}
\rput(15,25){$\addd$}
\psline[linewidth=0.15,fillstyle=solid](52.5,52.5)(77.5,52.5)
\psline[linewidth=0.15,fillstyle=solid](52.5,30)(52.5,52.5)
\psline[linewidth=0.15,fillstyle=solid](77.5,30)(52.5,30)
\psline[linewidth=0.15,fillstyle=solid](77.5,52.5)(77.5,30)
\rput(75,32.5){$\Homega$}
\rput(69.38,45){$\unl$}
\rput(10,45){$\pnl$}
\rput(17.5,58.75){$\png$}
\end{pspicture}


==> PIC/Omega-4.tex <==
%%Created by jPicEdt 1.4.1_03: mixed JPIC-XML/LaTeX format
%%Mon Feb 22 16:25:06 GMT-10:00 2021
%%Begin JPIC-XML
%<?xml version="1.0" standalone="yes"?>
%<jpic x-min="0" x-max="80" y-min="0" y-max="53.75" auto-bounding="true">
%<multicurve fill-style= "none"
%	 points= "(20,7.5);(20,7.5);(20,0);(20,0)"
%	 stroke-width= "0.5"
%	 />
%<ellipse p3= "(21.25,6.25)"
%	 fill-style= "solid"
%	 p2= "(21.25,8.75)"
%	 p1= "(18.75,8.75)"
%	 closure= "open"
%	 angle-end= "0"
%	 stroke-width= "0.5"
%	 angle-start= "0"
%	 />
%<multicurve fill-style= "none"
%	 points= "(25,12.5);(25,12.5);(20,7.5);(20,7.5)"
%	 stroke-width= "0.5"
%	 />
%<multicurve fill-style= "none"
%	 points= "(20,7.5);(20,7.5);(15,12.5);(15,12.5)"
%	 stroke-width= "0.5"
%	 />
%<multicurve fill-style= "none"
%	 points= "(15,12.5);(15,12.5);(15,20);(15,20)"
%	 stroke-width= "0.5"
%	 />
%<multicurve fill-style= "none"
%	 points= "(25,12.5);(25,12.5);(25,52.5);(25,52.5)"
%	 stroke-width= "0.5"
%	 />
%<multicurve fill-style= "none"
%	 points= "(10,37.5);(10,37.5);(20,37.5);(20,37.5)"
%	 stroke-width= "0.5"
%	 />
%<multicurve fill-style= "none"
%	 points= "(0,47.5);(0,47.5);(10,47.5);(10,47.5)"
%	 stroke-width= "0.5"
%	 />
%<multicurve fill-style= "none"
%	 points= "(15,26.25);(15,26.25);(15,37.5);(15,37.5)"
%	 stroke-width= "0.5"
%	 />
%<multicurve fill-style= "none"
%	 points= "(10,47.5);(10,47.5);(20,37.5);(20,37.5)"
%	 stroke-width= "0.5"
%	 />
%<multicurve fill-style= "none"
%	 points= "(0,47.5);(0,47.5);(10,37.5);(10,37.5)"
%	 stroke-width= "0.5"
%	 />
%<multicurve fill-style= "none"
%	 points= "(0,40);(0,40);(10,30);(10,30)"
%	 stroke-width= "0.5"
%	 />
%<multicurve fill-style= "none"
%	 points= "(15,42.5);(15,42.5);(15,52.5);(15,52.5)"
%	 stroke-width= "0.5"
%	 />
%<multicurve fill-style= "none"
%	 points= "(5,35);(5,35);(5,42.5);(5,42.5)"
%	 stroke-width= "0.5"
%	 />
%<multicurve fill-style= "none"
%	 points= "(0,30);(0,30);(10,30);(10,30)"
%	 stroke-width= "0.5"
%	 />
%<multicurve fill-style= "none"
%	 points= "(0,40);(0,40);(0,30);(0,30)"
%	 stroke-width= "0.5"
%	 />
%<multicurve fill-style= "none"
%	 points= "(65,37.5);(65,37.5);(76.25,37.5);(76.25,37.5)"
%	 stroke-width= "0.5"
%	 />
%<multicurve fill-style= "none"
%	 points= "(55,47.5);(55,47.5);(76.25,47.5);(76.25,47.5)"
%	 stroke-width= "0.5"
%	 />
%<multicurve fill-style= "none"
%	 points= "(70,0);(70,0);(70,37.5);(70,37.5)"
%	 stroke-width= "0.5"
%	 />
%<multicurve fill-style= "none"
%	 points= "(55,47.5);(55,47.5);(65,37.5);(65,37.5)"
%	 stroke-width= "0.5"
%	 />
%<multicurve fill-style= "none"
%	 points= "(55,40);(55,40);(65,30);(65,30)"
%	 stroke-width= "0.5"
%	 />
%<multicurve fill-style= "none"
%	 points= "(60,35);(60,35);(60,42.5);(60,42.5)"
%	 stroke-width= "0.5"
%	 />
%<multicurve fill-style= "none"
%	 points= "(55,30);(55,30);(65,30);(65,30)"
%	 stroke-width= "0.5"
%	 />
%<multicurve fill-style= "none"
%	 points= "(55,40);(55,40);(55,30);(55,30)"
%	 stroke-width= "0.5"
%	 />
%<multicurve fill-style= "none"
%	 points= "(76.25,47.5);(76.25,47.5);(76.25,37.5);(76.25,37.5)"
%	 stroke-width= "0.5"
%	 />
%<multicurve fill-style= "none"
%	 points= "(65,53.75);(65,53.75);(65,47.5);(65,47.5)"
%	 stroke-width= "0.5"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "solid"
%	 anchor-point= "(40,42.5)"
%	 text-frame= "noframe"
%	 stroke-width= "0.5"
%	 text-hor-align= "center-h"
%	 >
%\EQLS
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "solid"
%	 anchor-point= "(2.5,32.5)"
%	 text-frame= "noframe"
%	 stroke-width= "0.5"
%	 text-hor-align= "center-h"
%	 >
%$\Nee$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "solid"
%	 anchor-point= "(57.5,32.5)"
%	 text-frame= "noframe"
%	 stroke-width= "0.5"
%	 text-hor-align= "center-h"
%	 >
%$\Nee$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "solid"
%	 anchor-point= "(15,23.75)"
%	 text-frame= "noframe"
%	 stroke-width= "0.5"
%	 text-hor-align= "center-h"
%	 >
%$\addd$
%</text>
%<multicurve fill-style= "solid"
%	 points= "(52.5,50);(52.5,50);(80,50);(80,50)"
%	 stroke-width= "0.15"
%	 />
%<multicurve fill-style= "solid"
%	 points= "(52.5,27.5);(52.5,27.5);(52.5,50);(52.5,50)"
%	 stroke-width= "0.15"
%	 />
%<multicurve fill-style= "solid"
%	 points= "(80,27.5);(80,27.5);(52.5,27.5);(52.5,27.5)"
%	 stroke-width= "0.15"
%	 />
%<multicurve fill-style= "solid"
%	 points= "(80,50);(80,50);(80,27.5);(80,27.5)"
%	 stroke-width= "0.15"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "solid"
%	 anchor-point= "(75,30)"
%	 text-frame= "noframe"
%	 stroke-width= "0.5"
%	 text-hor-align= "center-h"
%	 >
%$\Homega$
%</text>
%<multicurve fill-style= "none"
%	 points= "(20,20);(20,20);(20,26.25);(20,26.25)"
%	 stroke-width= "0.5"
%	 />
%<multicurve fill-style= "none"
%	 points= "(10,20);(10,20);(10,26.25);(10,26.25)"
%	 stroke-width= "0.5"
%	 />
%<multicurve fill-style= "none"
%	 points= "(10,20);(10,20);(20,20);(20,20)"
%	 stroke-width= "0.5"
%	 />
%<multicurve fill-style= "none"
%	 points= "(10,26.25);(10,26.25);(20,26.25);(20,26.25)"
%	 stroke-width= "0.5"
%	 />
%<multicurve fill-style= "none"
%	 points= "(73.75,53.75);(73.75,53.75);(73.75,47.5);(73.75,47.5)"
%	 stroke-width= "0.5"
%	 />
%</jpic>
%%End JPIC-XML
%PSTricks content-type (pstricks.sty package needed)
%Add \usepackage{pstricks} in the preamble of your LaTeX file
%You can rescale the whole picture (to 80% for instance) by using the command \def\JPicScale{0.8}
\ifx\JPicScale\undefined\def\JPicScale{1}\fi
\psset{unit=\JPicScale mm}
\psset{linewidth=0.3,dotsep=1,hatchwidth=0.3,hatchsep=1.5,shadowsize=1,dimen=middle}
\psset{dotsize=0.7 2.5,dotscale=1 1,fillcolor=black}
\psset{arrowsize=1 2,arrowlength=1,arrowinset=0.25,tbarsize=0.7 5,bracketlength=0.15,rbracketlength=0.15}
\begin{pspicture}(0,0)(80,53.75)
\psline[linewidth=0.5](20,7.5)(20,0)
\rput{0}(20,7.5){\psellipse[linewidth=0.5,fillstyle=solid](0,0)(1.25,-1.25)}
\psline[linewidth=0.5](25,12.5)(20,7.5)
\psline[linewidth=0.5](20,7.5)(15,12.5)
\psline[linewidth=0.5](15,12.5)(15,20)
\psline[linewidth=0.5](25,12.5)(25,52.5)
\psline[linewidth=0.5](10,37.5)(20,37.5)
\psline[linewidth=0.5](0,47.5)(10,47.5)
\psline[linewidth=0.5](15,26.25)(15,37.5)
\psline[linewidth=0.5](10,47.5)(20,37.5)
\psline[linewidth=0.5](0,47.5)(10,37.5)
\psline[linewidth=0.5](0,40)(10,30)
\psline[linewidth=0.5](15,42.5)(15,52.5)
\psline[linewidth=0.5](5,35)(5,42.5)
\psline[linewidth=0.5](0,30)(10,30)
\psline[linewidth=0.5](0,40)(0,30)
\psline[linewidth=0.5](65,37.5)(76.25,37.5)
\psline[linewidth=0.5](55,47.5)(76.25,47.5)
\psline[linewidth=0.5](70,0)(70,37.5)
\psline[linewidth=0.5](55,47.5)(65,37.5)
\psline[linewidth=0.5](55,40)(65,30)
\psline[linewidth=0.5](60,35)(60,42.5)
\psline[linewidth=0.5](55,30)(65,30)
\psline[linewidth=0.5](55,40)(55,30)
\psline[linewidth=0.5](76.25,47.5)(76.25,37.5)
\psline[linewidth=0.5](65,53.75)(65,47.5)
\rput(40,42.5){\EQLS}
\rput(2.5,32.5){$\Nee$}
\rput(57.5,32.5){$\Nee$}
\rput(15,23.75){$\addd$}
\psline[linewidth=0.15,fillstyle=solid](52.5,50)(80,50)
\psline[linewidth=0.15,fillstyle=solid](52.5,27.5)(52.5,50)
\psline[linewidth=0.15,fillstyle=solid](80,27.5)(52.5,27.5)
\psline[linewidth=0.15,fillstyle=solid](80,50)(80,27.5)
\rput(75,30){$\Homega$}
\psline[linewidth=0.5](20,20)(20,26.25)
\psline[linewidth=0.5](10,20)(10,26.25)
\psline[linewidth=0.5](10,20)(20,20)
\psline[linewidth=0.5](10,26.25)(20,26.25)
\psline[linewidth=0.5](73.75,53.75)(73.75,47.5)
\end{pspicture}


==> PIC/Omega-5.tex <==
%%Created by jPicEdt 1.4.1_03: mixed JPIC-XML/LaTeX format
%%Mon Feb 22 20:35:09 GMT-10:00 2021
%%Begin JPIC-XML
%<?xml version="1.0" standalone="yes"?>
%<jpic x-min="-2.5" x-max="85" y-min="0" y-max="85" auto-bounding="true">
%<multicurve fill-style= "none"
%	 points= "(77.5,5);(77.5,5);(77.5,0);(77.5,0)"
%	 stroke-width= "0.5"
%	 />
%<ellipse p3= "(78.75,3.75)"
%	 fill-style= "solid"
%	 p2= "(78.75,6.25)"
%	 p1= "(76.25,6.25)"
%	 closure= "open"
%	 angle-end= "0"
%	 stroke-width= "0.5"
%	 angle-start= "0"
%	 />
%<multicurve fill-style= "none"
%	 points= "(82.5,10);(82.5,10);(77.5,5);(77.5,5)"
%	 stroke-width= "0.5"
%	 />
%<multicurve fill-style= "none"
%	 points= "(77.5,5);(77.5,5);(72.5,10);(72.5,10)"
%	 stroke-width= "0.5"
%	 />
%<multicurve fill-style= "none"
%	 points= "(72.5,10);(72.5,10);(72.5,16.25);(72.5,16.25)"
%	 stroke-width= "0.5"
%	 />
%<multicurve fill-style= "none"
%	 points= "(82.5,10);(82.5,10);(82.5,50);(82.5,50)"
%	 stroke-width= "0.5"
%	 />
%<multicurve fill-style= "none"
%	 points= "(67.5,35);(67.5,35);(77.5,35);(77.5,35)"
%	 stroke-width= "0.5"
%	 />
%<multicurve fill-style= "none"
%	 points= "(57.5,45);(57.5,45);(77.5,45);(77.5,45)"
%	 stroke-width= "0.5"
%	 />
%<ellipse p3= "(76.02,16.48)"
%	 fill-style= "none"
%	 p2= "(76.02,23.52)"
%	 p1= "(68.98,23.52)"
%	 closure= "open"
%	 angle-end= "0"
%	 stroke-width= "0.5"
%	 angle-start= "0"
%	 />
%<multicurve fill-style= "none"
%	 points= "(72.5,23.75);(72.5,23.75);(72.5,35);(72.5,35)"
%	 stroke-width= "0.5"
%	 />
%<multicurve fill-style= "none"
%	 points= "(77.5,45);(77.5,45);(77.5,35);(77.5,35)"
%	 stroke-width= "0.5"
%	 />
%<multicurve fill-style= "none"
%	 points= "(57.5,45);(57.5,45);(67.5,35);(67.5,35)"
%	 stroke-width= "0.5"
%	 />
%<multicurve fill-style= "none"
%	 points= "(57.5,37.5);(57.5,37.5);(67.5,27.5);(67.5,27.5)"
%	 stroke-width= "0.5"
%	 />
%<multicurve fill-style= "none"
%	 points= "(72.5,45);(72.5,45);(72.5,50);(72.5,50)"
%	 stroke-width= "0.5"
%	 />
%<multicurve fill-style= "none"
%	 points= "(62.5,32.5);(62.5,32.5);(62.5,40);(62.5,40)"
%	 stroke-width= "0.5"
%	 />
%<multicurve fill-style= "none"
%	 points= "(57.5,27.5);(57.5,27.5);(67.5,27.5);(67.5,27.5)"
%	 stroke-width= "0.5"
%	 />
%<multicurve fill-style= "none"
%	 points= "(57.5,37.5);(57.5,37.5);(57.5,27.5);(57.5,27.5)"
%	 stroke-width= "0.5"
%	 />
%<multicurve fill-style= "none"
%	 points= "(70,50);(70,50);(85,50);(85,50)"
%	 stroke-width= "0.5"
%	 />
%<multicurve fill-style= "none"
%	 points= "(70,65);(70,65);(70,50);(70,50)"
%	 stroke-width= "0.5"
%	 />
%<multicurve fill-style= "none"
%	 points= "(70,65);(70,65);(85,50);(85,50)"
%	 stroke-width= "0.5"
%	 />
%<multicurve fill-style= "none"
%	 points= "(77.5,67.5);(77.5,67.5);(77.5,57.5);(77.5,57.5)"
%	 stroke-width= "0.5"
%	 />
%<multicurve fill-style= "none"
%	 points= "(10,35);(10,35);(20,35);(20,35)"
%	 stroke-width= "0.5"
%	 />
%<multicurve fill-style= "none"
%	 points= "(0,45);(0,45);(20,45);(20,45)"
%	 stroke-width= "0.5"
%	 />
%<multicurve fill-style= "none"
%	 points= "(15,0);(15,0);(15,35);(15,35)"
%	 stroke-width= "0.5"
%	 />
%<multicurve fill-style= "none"
%	 points= "(0,45);(0,45);(10,35);(10,35)"
%	 stroke-width= "0.5"
%	 />
%<multicurve fill-style= "none"
%	 points= "(0,37.5);(0,37.5);(10,27.5);(10,27.5)"
%	 stroke-width= "0.5"
%	 />
%<multicurve fill-style= "none"
%	 points= "(5,32.5);(5,32.5);(5,40);(5,40)"
%	 stroke-width= "0.5"
%	 />
%<multicurve fill-style= "none"
%	 points= "(0,27.5);(0,27.5);(10,27.5);(10,27.5)"
%	 stroke-width= "0.5"
%	 />
%<multicurve fill-style= "none"
%	 points= "(0,37.5);(0,37.5);(0,27.5);(0,27.5)"
%	 stroke-width= "0.5"
%	 />
%<multicurve fill-style= "none"
%	 points= "(20,45);(20,45);(20,35);(20,35)"
%	 stroke-width= "0.5"
%	 />
%<multicurve fill-style= "none"
%	 points= "(15,67.5);(15,67.5);(15,45);(15,45)"
%	 stroke-width= "0.5"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "solid"
%	 anchor-point= "(40,40)"
%	 text-frame= "noframe"
%	 stroke-width= "0.5"
%	 text-hor-align= "center-h"
%	 >
%\EQLS
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "solid"
%	 anchor-point= "(60,30)"
%	 text-frame= "noframe"
%	 stroke-width= "0.5"
%	 text-hor-align= "center-h"
%	 >
%$\Nee$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "solid"
%	 anchor-point= "(2.5,30)"
%	 text-frame= "noframe"
%	 stroke-width= "0.5"
%	 text-hor-align= "center-h"
%	 >
%$\Nee$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "solid"
%	 anchor-point= "(72.5,20)"
%	 text-frame= "noframe"
%	 stroke-width= "0.5"
%	 text-hor-align= "center-h"
%	 >
%$\addd$
%</text>
%<multicurve fill-style= "solid"
%	 points= "(-2.5,47.5);(-2.5,47.5);(22.5,47.5);(22.5,47.5)"
%	 stroke-width= "0.15"
%	 />
%<multicurve fill-style= "solid"
%	 points= "(-2.5,25);(-2.5,25);(-2.5,47.5);(-2.5,47.5)"
%	 stroke-width= "0.15"
%	 />
%<multicurve fill-style= "solid"
%	 points= "(22.5,25);(22.5,25);(-2.5,25);(-2.5,25)"
%	 stroke-width= "0.15"
%	 />
%<multicurve fill-style= "solid"
%	 points= "(22.5,47.5);(22.5,47.5);(22.5,25);(22.5,25)"
%	 stroke-width= "0.15"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "solid"
%	 anchor-point= "(20,27.5)"
%	 text-frame= "noframe"
%	 stroke-width= "0.5"
%	 text-hor-align= "center-h"
%	 >
%$\Homega$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "solid"
%	 anchor-point= "(14.38,40)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\unl$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "solid"
%	 anchor-point= "(75,53.75)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\png$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "solid"
%	 anchor-point= "(25,85)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%\LHS
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "solid"
%	 anchor-point= "(40,85)"
%	 text-frame= "noframe"
%	 stroke-width= "0.5"
%	 text-hor-align= "center-h"
%	 >
%\EQLS
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "solid"
%	 anchor-point= "(55,85)"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%\RHS
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "solid"
%	 anchor-point= "(72.5,40)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\unl$
%</text>
%</jpic>
%%End JPIC-XML
%PSTricks content-type (pstricks.sty package needed)
%Add \usepackage{pstricks} in the preamble of your LaTeX file
%You can rescale the whole picture (to 80% for instance) by using the command \def\JPicScale{0.8}
\ifx\JPicScale\undefined\def\JPicScale{1}\fi
\psset{unit=\JPicScale mm}
\psset{linewidth=0.3,dotsep=1,hatchwidth=0.3,hatchsep=1.5,shadowsize=1,dimen=middle}
\psset{dotsize=0.7 2.5,dotscale=1 1,fillcolor=black}
\psset{arrowsize=1 2,arrowlength=1,arrowinset=0.25,tbarsize=0.7 5,bracketlength=0.15,rbracketlength=0.15}
\begin{pspicture}(0,0)(85,85)
\psline[linewidth=0.5](77.5,5)(77.5,0)
\rput{0}(77.5,5){\psellipse[linewidth=0.5,fillstyle=solid](0,0)(1.25,-1.25)}
\psline[linewidth=0.5](82.5,10)(77.5,5)
\psline[linewidth=0.5](77.5,5)(72.5,10)
\psline[linewidth=0.5](72.5,10)(72.5,16.25)
\psline[linewidth=0.5](82.5,10)(82.5,50)
\psline[linewidth=0.5](67.5,35)(77.5,35)
\psline[linewidth=0.5](57.5,45)(77.5,45)
\rput{0}(72.5,20){\psellipse[linewidth=0.5](0,0)(3.52,-3.52)}
\psline[linewidth=0.5](72.5,23.75)(72.5,35)
\psline[linewidth=0.5](77.5,45)(77.5,35)
\psline[linewidth=0.5](57.5,45)(67.5,35)
\psline[linewidth=0.5](57.5,37.5)(67.5,27.5)
\psline[linewidth=0.5](72.5,45)(72.5,50)
\psline[linewidth=0.5](62.5,32.5)(62.5,40)
\psline[linewidth=0.5](57.5,27.5)(67.5,27.5)
\psline[linewidth=0.5](57.5,37.5)(57.5,27.5)
\psline[linewidth=0.5](70,50)(85,50)
\psline[linewidth=0.5](70,65)(70,50)
\psline[linewidth=0.5](70,65)(85,50)
\psline[linewidth=0.5](77.5,67.5)(77.5,57.5)
\psline[linewidth=0.5](10,35)(20,35)
\psline[linewidth=0.5](0,45)(20,45)
\psline[linewidth=0.5](15,0)(15,35)
\psline[linewidth=0.5](0,45)(10,35)
\psline[linewidth=0.5](0,37.5)(10,27.5)
\psline[linewidth=0.5](5,32.5)(5,40)
\psline[linewidth=0.5](0,27.5)(10,27.5)
\psline[linewidth=0.5](0,37.5)(0,27.5)
\psline[linewidth=0.5](20,45)(20,35)
\psline[linewidth=0.5](15,67.5)(15,45)
\rput(40,40){\EQLS}
\rput(60,30){$\Nee$}
\rput(2.5,30){$\Nee$}
\rput(72.5,20){$\addd$}
\psline[linewidth=0.15,fillstyle=solid](-2.5,47.5)(22.5,47.5)
\psline[linewidth=0.15,fillstyle=solid](-2.5,25)(-2.5,47.5)
\psline[linewidth=0.15,fillstyle=solid](22.5,25)(-2.5,25)
\psline[linewidth=0.15,fillstyle=solid](22.5,47.5)(22.5,25)
\rput(20,27.5){$\Homega$}
\rput(14.38,40){$\unl$}
\rput(75,53.75){$\png$}
\rput[r](25,85){\LHS}
\rput(40,85){\EQLS}
\rput[l](55,85){\RHS}
\rput(72.5,40){$\unl$}
\end{pspicture}


==> PIC/Omega-55.tex <==
%%Created by jPicEdt 1.4.1_03: mixed JPIC-XML/LaTeX format
%%Fri Mar 05 15:09:38 GMT-10:00 2021
%%Begin JPIC-XML
%<?xml version="1.0" standalone="yes"?>
%<jpic x-min="-2.5" x-max="85" y-min="0" y-max="67.5" auto-bounding="true">
%<multicurve fill-style= "none"
%	 points= "(77.5,5);(77.5,5);(77.5,0);(77.5,0)"
%	 stroke-width= "0.5"
%	 />
%<ellipse fill-style= "solid"
%	 p3= "(78.75,3.75)"
%	 p2= "(78.75,6.25)"
%	 p1= "(76.25,6.25)"
%	 closure= "open"
%	 angle-end= "0"
%	 stroke-width= "0.5"
%	 angle-start= "0"
%	 />
%<multicurve fill-style= "none"
%	 points= "(82.5,10);(82.5,10);(77.5,5);(77.5,5)"
%	 stroke-width= "0.5"
%	 />
%<multicurve fill-style= "none"
%	 points= "(77.5,5);(77.5,5);(72.5,10);(72.5,10)"
%	 stroke-width= "0.5"
%	 />
%<multicurve fill-style= "none"
%	 points= "(72.5,10);(72.5,10);(72.5,15);(72.5,15)"
%	 stroke-width= "0.5"
%	 />
%<multicurve fill-style= "none"
%	 points= "(82.5,10);(82.5,10);(82.5,50);(82.5,50)"
%	 stroke-width= "0.5"
%	 />
%<multicurve fill-style= "none"
%	 points= "(67.5,35);(67.5,35);(77.5,35);(77.5,35)"
%	 stroke-width= "0.5"
%	 />
%<multicurve fill-style= "none"
%	 points= "(57.5,45);(57.5,45);(77.5,45);(77.5,45)"
%	 stroke-width= "0.5"
%	 />
%<ellipse fill-style= "none"
%	 p3= "(76.02,15.23)"
%	 p2= "(76.02,22.27)"
%	 p1= "(68.98,22.27)"
%	 closure= "open"
%	 angle-end= "0"
%	 stroke-width= "0.5"
%	 angle-start= "0"
%	 />
%<multicurve fill-style= "none"
%	 points= "(72.5,22.5);(72.5,22.5);(72.5,35);(72.5,35)"
%	 stroke-width= "0.5"
%	 />
%<multicurve fill-style= "none"
%	 points= "(77.5,45);(77.5,45);(77.5,35);(77.5,35)"
%	 stroke-width= "0.5"
%	 />
%<multicurve fill-style= "none"
%	 points= "(57.5,45);(57.5,45);(67.5,35);(67.5,35)"
%	 stroke-width= "0.5"
%	 />
%<multicurve fill-style= "none"
%	 points= "(57.5,37.5);(57.5,37.5);(67.5,27.5);(67.5,27.5)"
%	 stroke-width= "0.5"
%	 />
%<multicurve fill-style= "none"
%	 points= "(72.5,45);(72.5,45);(72.5,50);(72.5,50)"
%	 stroke-width= "0.5"
%	 />
%<multicurve fill-style= "none"
%	 points= "(62.5,32.5);(62.5,32.5);(62.5,40);(62.5,40)"
%	 stroke-width= "0.5"
%	 />
%<multicurve fill-style= "none"
%	 points= "(57.5,27.5);(57.5,27.5);(67.5,27.5);(67.5,27.5)"
%	 stroke-width= "0.5"
%	 />
%<multicurve fill-style= "none"
%	 points= "(57.5,37.5);(57.5,37.5);(57.5,27.5);(57.5,27.5)"
%	 stroke-width= "0.5"
%	 />
%<multicurve fill-style= "none"
%	 points= "(70,50);(70,50);(85,50);(85,50)"
%	 stroke-width= "0.5"
%	 />
%<multicurve fill-style= "none"
%	 points= "(70,65);(70,65);(70,50);(70,50)"
%	 stroke-width= "0.5"
%	 />
%<multicurve fill-style= "none"
%	 points= "(70,65);(70,65);(85,50);(85,50)"
%	 stroke-width= "0.5"
%	 />
%<multicurve fill-style= "none"
%	 points= "(77.5,67.5);(77.5,67.5);(77.5,57.5);(77.5,57.5)"
%	 stroke-width= "0.5"
%	 />
%<multicurve fill-style= "none"
%	 points= "(10,35);(10,35);(20,35);(20,35)"
%	 stroke-width= "0.5"
%	 />
%<multicurve fill-style= "none"
%	 points= "(0,45);(0,45);(20,45);(20,45)"
%	 stroke-width= "0.5"
%	 />
%<multicurve fill-style= "none"
%	 points= "(15,0);(15,0);(15,35);(15,35)"
%	 stroke-width= "0.5"
%	 />
%<multicurve fill-style= "none"
%	 points= "(0,45);(0,45);(10,35);(10,35)"
%	 stroke-width= "0.5"
%	 />
%<multicurve fill-style= "none"
%	 points= "(0,37.5);(0,37.5);(10,27.5);(10,27.5)"
%	 stroke-width= "0.5"
%	 />
%<multicurve fill-style= "none"
%	 points= "(5,32.5);(5,32.5);(5,40);(5,40)"
%	 stroke-width= "0.5"
%	 />
%<multicurve fill-style= "none"
%	 points= "(0,27.5);(0,27.5);(10,27.5);(10,27.5)"
%	 stroke-width= "0.5"
%	 />
%<multicurve fill-style= "none"
%	 points= "(0,37.5);(0,37.5);(0,27.5);(0,27.5)"
%	 stroke-width= "0.5"
%	 />
%<multicurve fill-style= "none"
%	 points= "(20,45);(20,45);(20,35);(20,35)"
%	 stroke-width= "0.5"
%	 />
%<multicurve fill-style= "none"
%	 points= "(15,67.5);(15,67.5);(15,45);(15,45)"
%	 stroke-width= "0.5"
%	 />
%<text fill-style= "solid"
%	 text-vert-align= "center-v"
%	 anchor-point= "(40,40)"
%	 stroke-width= "0.5"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\EQLS
%</text>
%<text fill-style= "solid"
%	 text-vert-align= "center-v"
%	 anchor-point= "(60,30)"
%	 stroke-width= "0.5"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\Nee$
%</text>
%<text fill-style= "solid"
%	 text-vert-align= "center-v"
%	 anchor-point= "(2.5,30)"
%	 stroke-width= "0.5"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\Nee$
%</text>
%<text fill-style= "solid"
%	 text-vert-align= "center-v"
%	 anchor-point= "(72.5,18.75)"
%	 stroke-width= "0.5"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\addd$
%</text>
%<multicurve fill-style= "solid"
%	 points= "(-2.5,47.5);(-2.5,47.5);(22.5,47.5);(22.5,47.5)"
%	 stroke-width= "0.15"
%	 />
%<multicurve fill-style= "solid"
%	 points= "(-2.5,25);(-2.5,25);(-2.5,47.5);(-2.5,47.5)"
%	 stroke-width= "0.15"
%	 />
%<multicurve fill-style= "solid"
%	 points= "(22.5,25);(22.5,25);(-2.5,25);(-2.5,25)"
%	 stroke-width= "0.15"
%	 />
%<multicurve fill-style= "solid"
%	 points= "(22.5,47.5);(22.5,47.5);(22.5,25);(22.5,25)"
%	 stroke-width= "0.15"
%	 />
%<text fill-style= "solid"
%	 text-vert-align= "center-v"
%	 anchor-point= "(19.38,27.5)"
%	 stroke-width= "0.5"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\Homega$
%</text>
%<text fill-style= "solid"
%	 text-vert-align= "center-v"
%	 anchor-point= "(14.38,40)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\unl$
%</text>
%<text fill-style= "solid"
%	 text-vert-align= "center-v"
%	 anchor-point= "(75,53.75)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\png$
%</text>
%<text fill-style= "solid"
%	 text-vert-align= "center-v"
%	 anchor-point= "(72.5,40)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\unl$
%</text>
%<multicurve fill-style= "solid"
%	 points= "(55,47.5);(55,47.5);(80,47.5);(80,47.5)"
%	 stroke-width= "0.15"
%	 />
%<multicurve fill-style= "solid"
%	 points= "(55,25);(55,25);(55,47.5);(55,47.5)"
%	 stroke-width= "0.15"
%	 />
%<multicurve fill-style= "solid"
%	 points= "(80,25);(80,25);(55,25);(55,25)"
%	 stroke-width= "0.15"
%	 />
%<multicurve fill-style= "solid"
%	 points= "(80,47.5);(80,47.5);(80,25);(80,25)"
%	 stroke-width= "0.15"
%	 />
%<text fill-style= "solid"
%	 text-vert-align= "center-v"
%	 anchor-point= "(76.25,27.5)"
%	 stroke-width= "0.5"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\Homega$
%</text>
%</jpic>
%%End JPIC-XML
%PSTricks content-type (pstricks.sty package needed)
%Add \usepackage{pstricks} in the preamble of your LaTeX file
%You can rescale the whole picture (to 80% for instance) by using the command \def\JPicScale{0.8}
\ifx\JPicScale\undefined\def\JPicScale{1}\fi
\psset{unit=\JPicScale mm}
\psset{linewidth=0.3,dotsep=1,hatchwidth=0.3,hatchsep=1.5,shadowsize=1,dimen=middle}
\psset{dotsize=0.7 2.5,dotscale=1 1,fillcolor=black}
\psset{arrowsize=1 2,arrowlength=1,arrowinset=0.25,tbarsize=0.7 5,bracketlength=0.15,rbracketlength=0.15}
\begin{pspicture}(0,0)(85,67.5)
\psline[linewidth=0.5](77.5,5)(77.5,0)
\rput{0}(77.5,5){\psellipse[linewidth=0.5,fillstyle=solid](0,0)(1.25,-1.25)}
\psline[linewidth=0.5](82.5,10)(77.5,5)
\psline[linewidth=0.5](77.5,5)(72.5,10)
\psline[linewidth=0.5](72.5,10)(72.5,15)
\psline[linewidth=0.5](82.5,10)(82.5,50)
\psline[linewidth=0.5](67.5,35)(77.5,35)
\psline[linewidth=0.5](57.5,45)(77.5,45)
\rput{90}(72.5,18.75){\psellipse[linewidth=0.5](0,0)(3.52,-3.52)}
\psline[linewidth=0.5](72.5,22.5)(72.5,35)
\psline[linewidth=0.5](77.5,45)(77.5,35)
\psline[linewidth=0.5](57.5,45)(67.5,35)
\psline[linewidth=0.5](57.5,37.5)(67.5,27.5)
\psline[linewidth=0.5](72.5,45)(72.5,50)
\psline[linewidth=0.5](62.5,32.5)(62.5,40)
\psline[linewidth=0.5](57.5,27.5)(67.5,27.5)
\psline[linewidth=0.5](57.5,37.5)(57.5,27.5)
\psline[linewidth=0.5](70,50)(85,50)
\psline[linewidth=0.5](70,65)(70,50)
\psline[linewidth=0.5](70,65)(85,50)
\psline[linewidth=0.5](77.5,67.5)(77.5,57.5)
\psline[linewidth=0.5](10,35)(20,35)
\psline[linewidth=0.5](0,45)(20,45)
\psline[linewidth=0.5](15,0)(15,35)
\psline[linewidth=0.5](0,45)(10,35)
\psline[linewidth=0.5](0,37.5)(10,27.5)
\psline[linewidth=0.5](5,32.5)(5,40)
\psline[linewidth=0.5](0,27.5)(10,27.5)
\psline[linewidth=0.5](0,37.5)(0,27.5)
\psline[linewidth=0.5](20,45)(20,35)
\psline[linewidth=0.5](15,67.5)(15,45)
\rput(40,40){\EQLS}
\rput(60,30){$\Nee$}
\rput(2.5,30){$\Nee$}
\rput(72.5,18.75){$\addd$}
\psline[linewidth=0.15,fillstyle=solid](-2.5,47.5)(22.5,47.5)
\psline[linewidth=0.15,fillstyle=solid](-2.5,25)(-2.5,47.5)
\psline[linewidth=0.15,fillstyle=solid](22.5,25)(-2.5,25)
\psline[linewidth=0.15,fillstyle=solid](22.5,47.5)(22.5,25)
\rput(19.38,27.5){$\Homega$}
\rput(14.38,40){$\unl$}
\rput(75,53.75){$\png$}
\rput(72.5,40){$\unl$}
\psline[linewidth=0.15,fillstyle=solid](55,47.5)(80,47.5)
\psline[linewidth=0.15,fillstyle=solid](55,25)(55,47.5)
\psline[linewidth=0.15,fillstyle=solid](80,25)(55,25)
\psline[linewidth=0.15,fillstyle=solid](80,47.5)(80,25)
\rput(76.25,27.5){$\Homega$}
\end{pspicture}


==> PIC/Omega-56.tex <==
%%Created by jPicEdt 1.4.1_03: mixed JPIC-XML/LaTeX format
%%Fri Mar 05 14:35:23 GMT-10:00 2021
%%Begin JPIC-XML
%<?xml version="1.0" standalone="yes"?>
%<jpic x-min="0" x-max="223.75" y-min="0" y-max="75" auto-bounding="true">
%<multicurve fill-style= "none"
%	 points= "(147.5,10);(147.5,10);(147.5,0);(147.5,0)"
%	 stroke-width= "0.5"
%	 />
%<ellipse fill-style= "solid"
%	 p3= "(148.75,8.75)"
%	 p2= "(148.75,11.25)"
%	 p1= "(146.25,11.25)"
%	 closure= "open"
%	 angle-end= "0"
%	 stroke-width= "0.5"
%	 angle-start= "0"
%	 />
%<multicurve fill-style= "none"
%	 points= "(152.5,15);(152.5,15);(147.5,10);(147.5,10)"
%	 stroke-width= "0.5"
%	 />
%<multicurve fill-style= "none"
%	 points= "(147.5,10);(147.5,10);(142.5,15);(142.5,15)"
%	 stroke-width= "0.5"
%	 />
%<multicurve fill-style= "none"
%	 points= "(152.5,15);(152.5,15);(152.5,55);(152.5,55)"
%	 stroke-width= "0.5"
%	 />
%<multicurve fill-style= "none"
%	 points= "(117.5,40);(117.5,40);(147.5,40);(147.5,40)"
%	 stroke-width= "0.5"
%	 />
%<multicurve fill-style= "none"
%	 points= "(107.5,50);(107.5,50);(147.5,50);(147.5,50)"
%	 stroke-width= "0.5"
%	 />
%<multicurve fill-style= "none"
%	 points= "(147.5,50);(147.5,50);(147.5,40);(147.5,40)"
%	 stroke-width= "0.5"
%	 />
%<multicurve fill-style= "none"
%	 points= "(107.5,50);(107.5,50);(117.5,40);(117.5,40)"
%	 stroke-width= "0.5"
%	 />
%<multicurve fill-style= "none"
%	 points= "(142.5,50);(142.5,50);(142.5,55);(142.5,55)"
%	 stroke-width= "0.5"
%	 />
%<multicurve fill-style= "none"
%	 points= "(122.5,15);(122.5,15);(122.5,40);(122.5,40)"
%	 stroke-width= "0.5"
%	 />
%<multicurve fill-style= "none"
%	 points= "(140,55);(140,55);(155,55);(155,55)"
%	 stroke-width= "0.5"
%	 />
%<multicurve fill-style= "none"
%	 points= "(140,70);(140,70);(140,55);(140,55)"
%	 stroke-width= "0.5"
%	 />
%<multicurve fill-style= "none"
%	 points= "(140,70);(140,70);(155,55);(155,55)"
%	 stroke-width= "0.5"
%	 />
%<multicurve fill-style= "none"
%	 points= "(147.5,75);(147.5,75);(147.5,62.5);(147.5,62.5)"
%	 stroke-width= "0.5"
%	 />
%<text fill-style= "solid"
%	 text-vert-align= "center-v"
%	 anchor-point= "(145,58.75)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\png$
%</text>
%<text fill-style= "solid"
%	 text-vert-align= "center-v"
%	 anchor-point= "(135,45)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\unl$
%</text>
%<multicurve fill-style= "none"
%	 points= "(137.5,20);(137.5,20);(147.5,20);(147.5,20)"
%	 stroke-width= "0.5"
%	 />
%<multicurve fill-style= "none"
%	 points= "(127.5,30);(127.5,30);(147.5,30);(147.5,30)"
%	 stroke-width= "0.5"
%	 />
%<multicurve fill-style= "none"
%	 points= "(142.5,15);(142.5,15);(142.5,20);(142.5,20)"
%	 stroke-width= "0.5"
%	 />
%<multicurve fill-style= "none"
%	 points= "(147.5,30);(147.5,30);(147.5,20);(147.5,20)"
%	 stroke-width= "0.5"
%	 />
%<multicurve fill-style= "none"
%	 points= "(127.5,30);(127.5,30);(137.5,20);(137.5,20)"
%	 stroke-width= "0.5"
%	 />
%<multicurve fill-style= "none"
%	 points= "(107.5,10);(107.5,10);(117.5,0);(117.5,0)"
%	 stroke-width= "0.5"
%	 />
%<multicurve fill-style= "none"
%	 points= "(142.5,30);(142.5,30);(142.5,40);(142.5,40)"
%	 stroke-width= "0.5"
%	 />
%<multicurve fill-style= "none"
%	 points= "(132.5,15);(132.5,15);(132.5,25);(132.5,25)"
%	 stroke-width= "0.5"
%	 />
%<multicurve fill-style= "none"
%	 points= "(107.5,0);(107.5,0);(117.5,0);(117.5,0)"
%	 stroke-width= "0.5"
%	 />
%<multicurve fill-style= "none"
%	 points= "(107.5,10);(107.5,10);(107.5,0);(107.5,0)"
%	 stroke-width= "0.5"
%	 />
%<text fill-style= "solid"
%	 text-vert-align= "center-v"
%	 anchor-point= "(111.25,2.5)"
%	 stroke-width= "0.5"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\Nee$
%</text>
%<text fill-style= "solid"
%	 text-vert-align= "center-v"
%	 anchor-point= "(141.25,25)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\unl$
%</text>
%<multicurve fill-style= "none"
%	 points= "(127.5,10);(127.5,10);(127.5,0);(127.5,0)"
%	 stroke-width= "0.5"
%	 />
%<ellipse fill-style= "solid"
%	 p3= "(128.75,8.75)"
%	 p2= "(128.75,11.25)"
%	 p1= "(126.25,11.25)"
%	 closure= "open"
%	 angle-end= "0"
%	 stroke-width= "0.5"
%	 angle-start= "0"
%	 />
%<multicurve fill-style= "none"
%	 points= "(132.5,15);(132.5,15);(127.5,10);(127.5,10)"
%	 stroke-width= "0.5"
%	 />
%<multicurve fill-style= "none"
%	 points= "(127.5,10);(127.5,10);(122.5,15);(122.5,15)"
%	 stroke-width= "0.5"
%	 />
%<multicurve fill-style= "none"
%	 points= "(112.5,5);(112.5,5);(112.5,45);(112.5,45)"
%	 stroke-width= "0.5"
%	 />
%<multicurve fill-style= "solid"
%	 points= "(0,43.75);(0,43.75);(12.5,43.75);(12.5,43.75)"
%	 stroke-width= "0.15"
%	 />
%<text fill-style= "solid"
%	 text-vert-align= "center-v"
%	 anchor-point= "(163.75,45)"
%	 stroke-width= "0.5"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\EQLS
%</text>
%<multicurve fill-style= "none"
%	 points= "(216.25,10);(216.25,10);(216.25,0);(216.25,0)"
%	 stroke-width= "0.5"
%	 />
%<ellipse fill-style= "solid"
%	 p3= "(217.5,8.75)"
%	 p2= "(217.5,11.25)"
%	 p1= "(215,11.25)"
%	 closure= "open"
%	 angle-end= "0"
%	 stroke-width= "0.5"
%	 angle-start= "0"
%	 />
%<multicurve fill-style= "none"
%	 points= "(221.25,15);(221.25,15);(216.25,10);(216.25,10)"
%	 stroke-width= "0.5"
%	 />
%<multicurve fill-style= "none"
%	 points= "(216.25,10);(216.25,10);(211.25,15);(211.25,15)"
%	 stroke-width= "0.5"
%	 />
%<multicurve fill-style= "none"
%	 points= "(221.25,15);(221.25,15);(221.25,55);(221.25,55)"
%	 stroke-width= "0.5"
%	 />
%<multicurve fill-style= "none"
%	 points= "(193.75,40);(193.75,40);(216.25,40);(216.25,40)"
%	 stroke-width= "0.5"
%	 />
%<multicurve fill-style= "none"
%	 points= "(183.75,50);(183.75,50);(216.25,50);(216.25,50)"
%	 stroke-width= "0.5"
%	 />
%<multicurve fill-style= "none"
%	 points= "(216.25,50);(216.25,50);(216.25,40);(216.25,40)"
%	 stroke-width= "0.5"
%	 />
%<multicurve fill-style= "none"
%	 points= "(183.75,50);(183.75,50);(193.75,40);(193.75,40)"
%	 stroke-width= "0.5"
%	 />
%<multicurve fill-style= "none"
%	 points= "(211.25,50);(211.25,50);(211.25,55);(211.25,55)"
%	 stroke-width= "0.5"
%	 />
%<multicurve fill-style= "none"
%	 points= "(208.75,55);(208.75,55);(223.75,55);(223.75,55)"
%	 stroke-width= "0.5"
%	 />
%<multicurve fill-style= "none"
%	 points= "(208.75,70);(208.75,70);(208.75,55);(208.75,55)"
%	 stroke-width= "0.5"
%	 />
%<multicurve fill-style= "none"
%	 points= "(208.75,70);(208.75,70);(223.75,55);(223.75,55)"
%	 stroke-width= "0.5"
%	 />
%<multicurve fill-style= "none"
%	 points= "(216.25,75);(216.25,75);(216.25,62.5);(216.25,62.5)"
%	 stroke-width= "0.5"
%	 />
%<text fill-style= "solid"
%	 text-vert-align= "center-v"
%	 anchor-point= "(213.75,58.75)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\png$
%</text>
%<text fill-style= "solid"
%	 text-vert-align= "center-v"
%	 anchor-point= "(203.75,45)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\unl$
%</text>
%<multicurve fill-style= "none"
%	 points= "(206.25,20);(206.25,20);(216.25,20);(216.25,20)"
%	 stroke-width= "0.5"
%	 />
%<multicurve fill-style= "none"
%	 points= "(196.25,30);(196.25,30);(216.25,30);(216.25,30)"
%	 stroke-width= "0.5"
%	 />
%<multicurve fill-style= "none"
%	 points= "(211.25,15);(211.25,15);(211.25,20);(211.25,20)"
%	 stroke-width= "0.5"
%	 />
%<multicurve fill-style= "none"
%	 points= "(216.25,30);(216.25,30);(216.25,20);(216.25,20)"
%	 stroke-width= "0.5"
%	 />
%<multicurve fill-style= "none"
%	 points= "(196.25,30);(196.25,30);(206.25,20);(206.25,20)"
%	 stroke-width= "0.5"
%	 />
%<multicurve fill-style= "none"
%	 points= "(211.25,30);(211.25,30);(211.25,40);(211.25,40)"
%	 stroke-width= "0.5"
%	 />
%<multicurve fill-style= "none"
%	 points= "(201.25,15);(201.25,15);(201.25,25);(201.25,25)"
%	 stroke-width= "0.5"
%	 />
%<text fill-style= "solid"
%	 text-vert-align= "center-v"
%	 anchor-point= "(210,25)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\unl$
%</text>
%<multicurve fill-style= "none"
%	 points= "(195,10);(195,10);(195,0);(195,0)"
%	 stroke-width= "0.5"
%	 />
%<ellipse fill-style= "solid"
%	 p3= "(196.25,8.75)"
%	 p2= "(196.25,11.25)"
%	 p1= "(193.75,11.25)"
%	 closure= "open"
%	 angle-end= "0"
%	 stroke-width= "0.5"
%	 angle-start= "0"
%	 />
%<multicurve fill-style= "none"
%	 points= "(201.25,15);(201.25,15);(195,10);(195,10)"
%	 stroke-width= "0.5"
%	 />
%<multicurve fill-style= "none"
%	 points= "(195,10);(195,10);(188.75,15);(188.75,15)"
%	 stroke-width= "0.5"
%	 />
%<multicurve fill-style= "none"
%	 points= "(82.5,0);(82.5,0);(82.5,40);(82.5,40)"
%	 stroke-width= "0.5"
%	 />
%<multicurve fill-style= "none"
%	 points= "(61.25,40);(61.25,40);(88.75,40);(88.75,40)"
%	 stroke-width= "0.5"
%	 />
%<multicurve fill-style= "none"
%	 points= "(51.25,50);(51.25,50);(88.75,50);(88.75,50)"
%	 stroke-width= "0.5"
%	 />
%<multicurve fill-style= "none"
%	 points= "(88.75,50);(88.75,50);(88.75,40);(88.75,40)"
%	 stroke-width= "0.5"
%	 />
%<multicurve fill-style= "none"
%	 points= "(51.25,50);(51.25,50);(61.25,40);(61.25,40)"
%	 stroke-width= "0.5"
%	 />
%<multicurve fill-style= "none"
%	 points= "(82.5,50);(82.5,50);(82.5,75);(82.5,75)"
%	 stroke-width= "0.5"
%	 />
%<multicurve fill-style= "none"
%	 points= "(68.75,0);(68.75,0);(68.75,40);(68.75,40)"
%	 stroke-width= "0.5"
%	 />
%<text fill-style= "solid"
%	 text-vert-align= "center-v"
%	 anchor-point= "(76.25,45)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\unl$
%</text>
%<multicurve fill-style= "none"
%	 points= "(51.25,10);(51.25,10);(61.25,0);(61.25,0)"
%	 stroke-width= "0.5"
%	 />
%<multicurve fill-style= "none"
%	 points= "(51.25,0);(51.25,0);(61.25,0);(61.25,0)"
%	 stroke-width= "0.5"
%	 />
%<multicurve fill-style= "none"
%	 points= "(51.25,10);(51.25,10);(51.25,0);(51.25,0)"
%	 stroke-width= "0.5"
%	 />
%<text fill-style= "solid"
%	 text-vert-align= "center-v"
%	 anchor-point= "(55,2.5)"
%	 stroke-width= "0.5"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\Nee$
%</text>
%<multicurve fill-style= "none"
%	 points= "(56.25,5);(56.25,5);(56.25,45);(56.25,45)"
%	 stroke-width= "0.5"
%	 />
%<multicurve fill-style= "solid"
%	 points= "(0,26.25);(0,26.25);(22.5,26.25);(22.5,26.25)"
%	 stroke-width= "0.15"
%	 />
%<text fill-style= "solid"
%	 text-vert-align= "center-v"
%	 anchor-point= "(98.75,45)"
%	 stroke-width= "0.5"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\EQLS
%</text>
%<multicurve fill-style= "none"
%	 points= "(28.75,0);(28.75,0);(28.75,40);(28.75,40)"
%	 stroke-width= "0.5"
%	 />
%<multicurve fill-style= "none"
%	 points= "(21.25,40);(21.25,40);(36.25,40);(36.25,40)"
%	 stroke-width= "0.5"
%	 />
%<multicurve fill-style= "none"
%	 points= "(11.25,50);(11.25,50);(36.25,50);(36.25,50)"
%	 stroke-width= "0.5"
%	 />
%<multicurve fill-style= "none"
%	 points= "(36.25,50);(36.25,50);(36.25,40);(36.25,40)"
%	 stroke-width= "0.5"
%	 />
%<multicurve fill-style= "none"
%	 points= "(1.25,42.5);(1.25,42.5);(11.25,42.5);(11.25,42.5)"
%	 stroke-width= "0.5"
%	 />
%<multicurve fill-style= "none"
%	 points= "(28.75,50);(28.75,50);(28.75,75);(28.75,75)"
%	 stroke-width= "0.5"
%	 />
%<multicurve fill-style= "none"
%	 points= "(16.25,0);(16.25,0);(16.25,32.5);(16.25,32.5)"
%	 stroke-width= "0.5"
%	 />
%<text fill-style= "solid"
%	 text-vert-align= "center-v"
%	 anchor-point= "(28.75,45)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\unl$
%</text>
%<multicurve fill-style= "none"
%	 points= "(1.25,37.5);(1.25,37.5);(11.25,27.5);(11.25,27.5)"
%	 stroke-width= "0.5"
%	 />
%<multicurve fill-style= "none"
%	 points= "(1.25,27.5);(1.25,27.5);(11.25,27.5);(11.25,27.5)"
%	 stroke-width= "0.5"
%	 />
%<multicurve fill-style= "none"
%	 points= "(1.25,37.5);(1.25,37.5);(1.25,27.5);(1.25,27.5)"
%	 stroke-width= "0.5"
%	 />
%<text fill-style= "solid"
%	 text-vert-align= "center-v"
%	 anchor-point= "(5,30)"
%	 stroke-width= "0.5"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\Nee$
%</text>
%<multicurve fill-style= "none"
%	 points= "(6.25,32.5);(6.25,32.5);(6.25,37.5);(6.25,37.5)"
%	 stroke-width= "0.5"
%	 />
%<text fill-style= "solid"
%	 text-vert-align= "center-v"
%	 anchor-point= "(45,45)"
%	 stroke-width= "0.5"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\EQLS
%</text>
%<multicurve fill-style= "none"
%	 points= "(11.25,50);(11.25,50);(21.25,40);(21.25,40)"
%	 stroke-width= "0.5"
%	 />
%<multicurve fill-style= "none"
%	 points= "(11.25,32.5);(11.25,32.5);(21.25,32.5);(21.25,32.5)"
%	 stroke-width= "0.5"
%	 />
%<multicurve fill-style= "none"
%	 points= "(11.25,42.5);(11.25,42.5);(21.25,32.5);(21.25,32.5)"
%	 stroke-width= "0.5"
%	 />
%<multicurve fill-style= "none"
%	 points= "(1.25,42.5);(1.25,42.5);(11.25,32.5);(11.25,32.5)"
%	 stroke-width= "0.5"
%	 />
%<multicurve fill-style= "none"
%	 points= "(16.25,37.5);(16.25,37.5);(16.25,45);(16.25,45)"
%	 stroke-width= "0.5"
%	 />
%<multicurve fill-style= "solid"
%	 points= "(22.5,26.25);(22.5,26.25);(22.5,33.75);(22.5,33.75)"
%	 stroke-width= "0.15"
%	 />
%<multicurve fill-style= "solid"
%	 points= "(12.5,43.75);(12.5,43.75);(22.5,33.75);(22.5,33.75)"
%	 stroke-width= "0.15"
%	 />
%<multicurve fill-style= "solid"
%	 points= "(0,43.75);(0,43.75);(0,26.25);(0,26.25)"
%	 stroke-width= "0.15"
%	 />
%<multicurve fill-style= "solid"
%	 points= "(172.5,43.75);(172.5,43.75);(185,43.75);(185,43.75)"
%	 stroke-width= "0.15"
%	 />
%<multicurve fill-style= "solid"
%	 points= "(172.5,26.25);(172.5,26.25);(195,26.25);(195,26.25)"
%	 stroke-width= "0.15"
%	 />
%<multicurve fill-style= "none"
%	 points= "(173.75,42.5);(173.75,42.5);(183.75,42.5);(183.75,42.5)"
%	 stroke-width= "0.5"
%	 />
%<multicurve fill-style= "none"
%	 points= "(188.75,15);(188.75,15);(188.75,32.5);(188.75,32.5)"
%	 stroke-width= "0.5"
%	 />
%<multicurve fill-style= "none"
%	 points= "(173.75,37.5);(173.75,37.5);(183.75,27.5);(183.75,27.5)"
%	 stroke-width= "0.5"
%	 />
%<multicurve fill-style= "none"
%	 points= "(173.75,27.5);(173.75,27.5);(183.75,27.5);(183.75,27.5)"
%	 stroke-width= "0.5"
%	 />
%<multicurve fill-style= "none"
%	 points= "(173.75,37.5);(173.75,37.5);(173.75,27.5);(173.75,27.5)"
%	 stroke-width= "0.5"
%	 />
%<text fill-style= "solid"
%	 text-vert-align= "center-v"
%	 anchor-point= "(177.5,30)"
%	 stroke-width= "0.5"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\Nee$
%</text>
%<multicurve fill-style= "none"
%	 points= "(178.75,32.5);(178.75,32.5);(178.75,37.5);(178.75,37.5)"
%	 stroke-width= "0.5"
%	 />
%<multicurve fill-style= "none"
%	 points= "(183.75,32.5);(183.75,32.5);(193.75,32.5);(193.75,32.5)"
%	 stroke-width= "0.5"
%	 />
%<multicurve fill-style= "none"
%	 points= "(183.75,42.5);(183.75,42.5);(193.75,32.5);(193.75,32.5)"
%	 stroke-width= "0.5"
%	 />
%<multicurve fill-style= "none"
%	 points= "(173.75,42.5);(173.75,42.5);(183.75,32.5);(183.75,32.5)"
%	 stroke-width= "0.5"
%	 />
%<multicurve fill-style= "none"
%	 points= "(188.75,37.5);(188.75,37.5);(188.75,45);(188.75,45)"
%	 stroke-width= "0.5"
%	 />
%<multicurve fill-style= "solid"
%	 points= "(195,26.25);(195,26.25);(195,33.75);(195,33.75)"
%	 stroke-width= "0.15"
%	 />
%<multicurve fill-style= "solid"
%	 points= "(185,43.75);(185,43.75);(195,33.75);(195,33.75)"
%	 stroke-width= "0.15"
%	 />
%<multicurve fill-style= "solid"
%	 points= "(172.5,43.75);(172.5,43.75);(172.5,26.25);(172.5,26.25)"
%	 stroke-width= "0.15"
%	 />
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(11.25,37.5)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\pnl$
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(183.75,37.5)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\pnl$
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(20,28.75)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\dubb$
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(192.5,28.75)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\dubb$
%</text>
%</jpic>
%%End JPIC-XML
%PSTricks content-type (pstricks.sty package needed)
%Add \usepackage{pstricks} in the preamble of your LaTeX file
%You can rescale the whole picture (to 80% for instance) by using the command \def\JPicScale{0.8}
\ifx\JPicScale\undefined\def\JPicScale{1}\fi
\psset{unit=\JPicScale mm}
\psset{linewidth=0.3,dotsep=1,hatchwidth=0.3,hatchsep=1.5,shadowsize=1,dimen=middle}
\psset{dotsize=0.7 2.5,dotscale=1 1,fillcolor=black}
\psset{arrowsize=1 2,arrowlength=1,arrowinset=0.25,tbarsize=0.7 5,bracketlength=0.15,rbracketlength=0.15}
\begin{pspicture}(0,0)(223.75,75)
\psline[linewidth=0.5](147.5,10)(147.5,0)
\rput{0}(147.5,10){\psellipse[linewidth=0.5,fillstyle=solid](0,0)(1.25,-1.25)}
\psline[linewidth=0.5](152.5,15)(147.5,10)
\psline[linewidth=0.5](147.5,10)(142.5,15)
\psline[linewidth=0.5](152.5,15)(152.5,55)
\psline[linewidth=0.5](117.5,40)(147.5,40)
\psline[linewidth=0.5](107.5,50)(147.5,50)
\psline[linewidth=0.5](147.5,50)(147.5,40)
\psline[linewidth=0.5](107.5,50)(117.5,40)
\psline[linewidth=0.5](142.5,50)(142.5,55)
\psline[linewidth=0.5](122.5,15)(122.5,40)
\psline[linewidth=0.5](140,55)(155,55)
\psline[linewidth=0.5](140,70)(140,55)
\psline[linewidth=0.5](140,70)(155,55)
\psline[linewidth=0.5](147.5,75)(147.5,62.5)
\rput(145,58.75){$\png$}
\rput(135,45){$\unl$}
\psline[linewidth=0.5](137.5,20)(147.5,20)
\psline[linewidth=0.5](127.5,30)(147.5,30)
\psline[linewidth=0.5](142.5,15)(142.5,20)
\psline[linewidth=0.5](147.5,30)(147.5,20)
\psline[linewidth=0.5](127.5,30)(137.5,20)
\psline[linewidth=0.5](107.5,10)(117.5,0)
\psline[linewidth=0.5](142.5,30)(142.5,40)
\psline[linewidth=0.5](132.5,15)(132.5,25)
\psline[linewidth=0.5](107.5,0)(117.5,0)
\psline[linewidth=0.5](107.5,10)(107.5,0)
\rput(111.25,2.5){$\Nee$}
\rput(141.25,25){$\unl$}
\psline[linewidth=0.5](127.5,10)(127.5,0)
\rput{0}(127.5,10){\psellipse[linewidth=0.5,fillstyle=solid](0,0)(1.25,-1.25)}
\psline[linewidth=0.5](132.5,15)(127.5,10)
\psline[linewidth=0.5](127.5,10)(122.5,15)
\psline[linewidth=0.5](112.5,5)(112.5,45)
\psline[linewidth=0.15,fillstyle=solid](0,43.75)(12.5,43.75)
\rput(163.75,45){\EQLS}
\psline[linewidth=0.5](216.25,10)(216.25,0)
\rput{0}(216.25,10){\psellipse[linewidth=0.5,fillstyle=solid](0,0)(1.25,-1.25)}
\psline[linewidth=0.5](221.25,15)(216.25,10)
\psline[linewidth=0.5](216.25,10)(211.25,15)
\psline[linewidth=0.5](221.25,15)(221.25,55)
\psline[linewidth=0.5](193.75,40)(216.25,40)
\psline[linewidth=0.5](183.75,50)(216.25,50)
\psline[linewidth=0.5](216.25,50)(216.25,40)
\psline[linewidth=0.5](183.75,50)(193.75,40)
\psline[linewidth=0.5](211.25,50)(211.25,55)
\psline[linewidth=0.5](208.75,55)(223.75,55)
\psline[linewidth=0.5](208.75,70)(208.75,55)
\psline[linewidth=0.5](208.75,70)(223.75,55)
\psline[linewidth=0.5](216.25,75)(216.25,62.5)
\rput(213.75,58.75){$\png$}
\rput(203.75,45){$\unl$}
\psline[linewidth=0.5](206.25,20)(216.25,20)
\psline[linewidth=0.5](196.25,30)(216.25,30)
\psline[linewidth=0.5](211.25,15)(211.25,20)
\psline[linewidth=0.5](216.25,30)(216.25,20)
\psline[linewidth=0.5](196.25,30)(206.25,20)
\psline[linewidth=0.5](211.25,30)(211.25,40)
\psline[linewidth=0.5](201.25,15)(201.25,25)
\rput(210,25){$\unl$}
\psline[linewidth=0.5](195,10)(195,0)
\rput{0}(195,10){\psellipse[linewidth=0.5,fillstyle=solid](0,0)(1.25,-1.25)}
\psline[linewidth=0.5](201.25,15)(195,10)
\psline[linewidth=0.5](195,10)(188.75,15)
\psline[linewidth=0.5](82.5,0)(82.5,40)
\psline[linewidth=0.5](61.25,40)(88.75,40)
\psline[linewidth=0.5](51.25,50)(88.75,50)
\psline[linewidth=0.5](88.75,50)(88.75,40)
\psline[linewidth=0.5](51.25,50)(61.25,40)
\psline[linewidth=0.5](82.5,50)(82.5,75)
\psline[linewidth=0.5](68.75,0)(68.75,40)
\rput(76.25,45){$\unl$}
\psline[linewidth=0.5](51.25,10)(61.25,0)
\psline[linewidth=0.5](51.25,0)(61.25,0)
\psline[linewidth=0.5](51.25,10)(51.25,0)
\rput(55,2.5){$\Nee$}
\psline[linewidth=0.5](56.25,5)(56.25,45)
\psline[linewidth=0.15,fillstyle=solid](0,26.25)(22.5,26.25)
\rput(98.75,45){\EQLS}
\psline[linewidth=0.5](28.75,0)(28.75,40)
\psline[linewidth=0.5](21.25,40)(36.25,40)
\psline[linewidth=0.5](11.25,50)(36.25,50)
\psline[linewidth=0.5](36.25,50)(36.25,40)
\psline[linewidth=0.5](1.25,42.5)(11.25,42.5)
\psline[linewidth=0.5](28.75,50)(28.75,75)
\psline[linewidth=0.5](16.25,0)(16.25,32.5)
\rput(28.75,45){$\unl$}
\psline[linewidth=0.5](1.25,37.5)(11.25,27.5)
\psline[linewidth=0.5](1.25,27.5)(11.25,27.5)
\psline[linewidth=0.5](1.25,37.5)(1.25,27.5)
\rput(5,30){$\Nee$}
\psline[linewidth=0.5](6.25,32.5)(6.25,37.5)
\rput(45,45){\EQLS}
\psline[linewidth=0.5](11.25,50)(21.25,40)
\psline[linewidth=0.5](11.25,32.5)(21.25,32.5)
\psline[linewidth=0.5](11.25,42.5)(21.25,32.5)
\psline[linewidth=0.5](1.25,42.5)(11.25,32.5)
\psline[linewidth=0.5](16.25,37.5)(16.25,45)
\psline[linewidth=0.15,fillstyle=solid](22.5,26.25)(22.5,33.75)
\psline[linewidth=0.15,fillstyle=solid](12.5,43.75)(22.5,33.75)
\psline[linewidth=0.15,fillstyle=solid](0,43.75)(0,26.25)
\psline[linewidth=0.15,fillstyle=solid](172.5,43.75)(185,43.75)
\psline[linewidth=0.15,fillstyle=solid](172.5,26.25)(195,26.25)
\psline[linewidth=0.5](173.75,42.5)(183.75,42.5)
\psline[linewidth=0.5](188.75,15)(188.75,32.5)
\psline[linewidth=0.5](173.75,37.5)(183.75,27.5)
\psline[linewidth=0.5](173.75,27.5)(183.75,27.5)
\psline[linewidth=0.5](173.75,37.5)(173.75,27.5)
\rput(177.5,30){$\Nee$}
\psline[linewidth=0.5](178.75,32.5)(178.75,37.5)
\psline[linewidth=0.5](183.75,32.5)(193.75,32.5)
\psline[linewidth=0.5](183.75,42.5)(193.75,32.5)
\psline[linewidth=0.5](173.75,42.5)(183.75,32.5)
\psline[linewidth=0.5](188.75,37.5)(188.75,45)
\psline[linewidth=0.15,fillstyle=solid](195,26.25)(195,33.75)
\psline[linewidth=0.15,fillstyle=solid](185,43.75)(195,33.75)
\psline[linewidth=0.15,fillstyle=solid](172.5,43.75)(172.5,26.25)
\rput(11.25,37.5){$\pnl$}
\rput(183.75,37.5){$\pnl$}
\rput(20,28.75){$\dubb$}
\rput(192.5,28.75){$\dubb$}
\end{pspicture}


==> PIC/Omega-57.tex <==
%%Created by jPicEdt 1.4.1_03: mixed JPIC-XML/LaTeX format
%%Fri Mar 05 17:37:18 GMT-10:00 2021
%%Begin JPIC-XML
%<?xml version="1.0" standalone="yes"?>
%<jpic x-min="1.25" x-max="157.5" y-min="0" y-max="75" auto-bounding="true">
%<multicurve fill-style= "solid"
%	 points= "(121.25,21.25);(121.25,21.25);(133.75,21.25);(133.75,21.25)"
%	 stroke-width= "0.15"
%	 />
%<multicurve fill-style= "none"
%	 points= "(93.75,0);(93.75,0);(93.75,40);(93.75,40)"
%	 stroke-width= "0.4"
%	 />
%<multicurve fill-style= "none"
%	 points= "(72.5,40);(72.5,40);(100,40);(100,40)"
%	 stroke-width= "0.4"
%	 />
%<multicurve fill-style= "none"
%	 points= "(62.5,50);(62.5,50);(100,50);(100,50)"
%	 stroke-width= "0.4"
%	 />
%<multicurve fill-style= "none"
%	 points= "(100,50);(100,50);(100,40);(100,40)"
%	 stroke-width= "0.4"
%	 />
%<multicurve fill-style= "none"
%	 points= "(62.5,50);(62.5,50);(72.5,40);(72.5,40)"
%	 stroke-width= "0.4"
%	 />
%<multicurve fill-style= "none"
%	 points= "(93.75,50);(93.75,50);(93.75,75);(93.75,75)"
%	 stroke-width= "0.4"
%	 />
%<multicurve fill-style= "none"
%	 points= "(80,0);(80,0);(80,40);(80,40)"
%	 stroke-width= "0.4"
%	 />
%<text fill-style= "solid"
%	 text-vert-align= "center-v"
%	 anchor-point= "(87.5,45)"
%	 stroke-width= "0.4"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\unl$
%</text>
%<multicurve fill-style= "none"
%	 points= "(62.5,15);(62.5,15);(72.5,5);(72.5,5)"
%	 stroke-width= "0.4"
%	 />
%<multicurve fill-style= "none"
%	 points= "(62.5,5);(62.5,5);(72.5,5);(72.5,5)"
%	 stroke-width= "0.4"
%	 />
%<multicurve fill-style= "none"
%	 points= "(62.5,15);(62.5,15);(62.5,5);(62.5,5)"
%	 stroke-width= "0.4"
%	 />
%<text fill-style= "solid"
%	 text-vert-align= "center-v"
%	 anchor-point= "(66.25,7.5)"
%	 stroke-width= "0.4"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\Nee$
%</text>
%<multicurve fill-style= "none"
%	 points= "(67.5,10);(67.5,10);(67.5,45);(67.5,45)"
%	 stroke-width= "0.4"
%	 />
%<multicurve fill-style= "solid"
%	 points= "(121.25,3.75);(121.25,3.75);(146.25,3.75);(146.25,3.75)"
%	 stroke-width= "0.15"
%	 />
%<text fill-style= "solid"
%	 text-vert-align= "center-v"
%	 anchor-point= "(50,45)"
%	 stroke-width= "0.4"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\EQLS
%</text>
%<multicurve fill-style= "none"
%	 points= "(150,0);(150,0);(150,40);(150,40)"
%	 stroke-width= "0.4"
%	 />
%<multicurve fill-style= "none"
%	 points= "(142.5,40);(142.5,40);(157.5,40);(157.5,40)"
%	 stroke-width= "0.4"
%	 />
%<multicurve fill-style= "none"
%	 points= "(132.5,50);(132.5,50);(157.5,50);(157.5,50)"
%	 stroke-width= "0.4"
%	 />
%<multicurve fill-style= "none"
%	 points= "(157.5,50);(157.5,50);(157.5,40);(157.5,40)"
%	 stroke-width= "0.4"
%	 />
%<multicurve fill-style= "none"
%	 points= "(122.5,20);(122.5,20);(132.5,20);(132.5,20)"
%	 stroke-width= "0.4"
%	 />
%<multicurve fill-style= "none"
%	 points= "(150,50);(150,50);(150,75);(150,75)"
%	 stroke-width= "0.4"
%	 />
%<multicurve fill-style= "none"
%	 points= "(137.5,0);(137.5,0);(137.5,10);(137.5,10)"
%	 stroke-width= "0.4"
%	 />
%<text fill-style= "solid"
%	 text-vert-align= "center-v"
%	 anchor-point= "(150,45)"
%	 stroke-width= "0.4"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\unl$
%</text>
%<multicurve fill-style= "none"
%	 points= "(122.5,15);(122.5,15);(132.5,5);(132.5,5)"
%	 stroke-width= "0.4"
%	 />
%<multicurve fill-style= "none"
%	 points= "(122.5,5);(122.5,5);(132.5,5);(132.5,5)"
%	 stroke-width= "0.4"
%	 />
%<multicurve fill-style= "none"
%	 points= "(122.5,15);(122.5,15);(122.5,5);(122.5,5)"
%	 stroke-width= "0.4"
%	 />
%<text fill-style= "solid"
%	 text-vert-align= "center-v"
%	 anchor-point= "(126.25,7.5)"
%	 stroke-width= "0.4"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\Nee$
%</text>
%<multicurve fill-style= "none"
%	 points= "(127.5,10);(127.5,10);(127.5,15);(127.5,15)"
%	 stroke-width= "0.4"
%	 />
%<text fill-style= "solid"
%	 text-vert-align= "center-v"
%	 anchor-point= "(112.5,45)"
%	 stroke-width= "0.4"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\EQLS
%</text>
%<multicurve fill-style= "none"
%	 points= "(132.5,50);(132.5,50);(142.5,40);(142.5,40)"
%	 stroke-width= "0.4"
%	 />
%<multicurve fill-style= "none"
%	 points= "(132.5,10);(132.5,10);(142.5,10);(142.5,10)"
%	 stroke-width= "0.4"
%	 />
%<multicurve fill-style= "none"
%	 points= "(132.5,20);(132.5,20);(142.5,10);(142.5,10)"
%	 stroke-width= "0.4"
%	 />
%<multicurve fill-style= "none"
%	 points= "(122.5,20);(122.5,20);(132.5,10);(132.5,10)"
%	 stroke-width= "0.4"
%	 />
%<multicurve fill-style= "none"
%	 points= "(137.5,15);(137.5,15);(137.5,45);(137.5,45)"
%	 stroke-width= "0.4"
%	 />
%<multicurve fill-style= "solid"
%	 points= "(146.25,3.75);(146.25,3.75);(146.25,8.75);(146.25,8.75)"
%	 stroke-width= "0.15"
%	 />
%<multicurve fill-style= "solid"
%	 points= "(133.75,21.25);(133.75,21.25);(146.25,8.75);(146.25,8.75)"
%	 stroke-width= "0.15"
%	 />
%<multicurve fill-style= "solid"
%	 points= "(121.25,21.25);(121.25,21.25);(121.25,3.75);(121.25,3.75)"
%	 stroke-width= "0.15"
%	 />
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(132.5,15)"
%	 stroke-width= "0.4"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\pnl$
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(142.5,6.25)"
%	 stroke-width= "0.4"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\dubb$
%</text>
%<multicurve fill-style= "solid"
%	 points= "(1.25,21.25);(1.25,21.25);(13.75,21.25);(13.75,21.25)"
%	 stroke-width= "0.15"
%	 />
%<multicurve fill-style= "solid"
%	 points= "(1.25,3.75);(1.25,3.75);(26.25,3.75);(26.25,3.75)"
%	 stroke-width= "0.15"
%	 />
%<multicurve fill-style= "none"
%	 points= "(30,0);(30,0);(30,40);(30,40)"
%	 stroke-width= "0.4"
%	 />
%<multicurve fill-style= "none"
%	 points= "(22.5,40);(22.5,40);(37.5,40);(37.5,40)"
%	 stroke-width= "0.4"
%	 />
%<multicurve fill-style= "none"
%	 points= "(12.5,50);(12.5,50);(37.5,50);(37.5,50)"
%	 stroke-width= "0.4"
%	 />
%<multicurve fill-style= "none"
%	 points= "(37.5,50);(37.5,50);(37.5,40);(37.5,40)"
%	 stroke-width= "0.4"
%	 />
%<multicurve fill-style= "none"
%	 points= "(2.5,20);(2.5,20);(12.5,20);(12.5,20)"
%	 stroke-width= "0.4"
%	 />
%<multicurve fill-style= "none"
%	 points= "(30,50);(30,50);(30,75);(30,75)"
%	 stroke-width= "0.4"
%	 />
%<multicurve fill-style= "none"
%	 points= "(17.5,0);(17.5,0);(17.5,10);(17.5,10)"
%	 stroke-width= "0.4"
%	 />
%<text fill-style= "solid"
%	 text-vert-align= "center-v"
%	 anchor-point= "(30,45)"
%	 stroke-width= "0.4"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\unl$
%</text>
%<multicurve fill-style= "none"
%	 points= "(2.5,15);(2.5,15);(12.5,5);(12.5,5)"
%	 stroke-width= "0.4"
%	 />
%<multicurve fill-style= "none"
%	 points= "(2.5,5);(2.5,5);(12.5,5);(12.5,5)"
%	 stroke-width= "0.4"
%	 />
%<multicurve fill-style= "none"
%	 points= "(2.5,15);(2.5,15);(2.5,5);(2.5,5)"
%	 stroke-width= "0.4"
%	 />
%<text fill-style= "solid"
%	 text-vert-align= "center-v"
%	 anchor-point= "(6.25,7.5)"
%	 stroke-width= "0.4"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\Nee$
%</text>
%<multicurve fill-style= "none"
%	 points= "(7.5,10);(7.5,10);(7.5,15);(7.5,15)"
%	 stroke-width= "0.4"
%	 />
%<multicurve fill-style= "none"
%	 points= "(12.5,50);(12.5,50);(22.5,40);(22.5,40)"
%	 stroke-width= "0.4"
%	 />
%<multicurve fill-style= "none"
%	 points= "(12.5,10);(12.5,10);(22.5,10);(22.5,10)"
%	 stroke-width= "0.4"
%	 />
%<multicurve fill-style= "none"
%	 points= "(12.5,20);(12.5,20);(22.5,10);(22.5,10)"
%	 stroke-width= "0.4"
%	 />
%<multicurve fill-style= "none"
%	 points= "(2.5,20);(2.5,20);(12.5,10);(12.5,10)"
%	 stroke-width= "0.4"
%	 />
%<multicurve fill-style= "none"
%	 points= "(17.5,15);(17.5,15);(17.5,25);(17.5,25)"
%	 stroke-width= "0.4"
%	 />
%<multicurve fill-style= "solid"
%	 points= "(26.25,3.75);(26.25,3.75);(26.25,8.75);(26.25,8.75)"
%	 stroke-width= "0.15"
%	 />
%<multicurve fill-style= "solid"
%	 points= "(13.75,21.25);(13.75,21.25);(26.25,8.75);(26.25,8.75)"
%	 stroke-width= "0.15"
%	 />
%<multicurve fill-style= "solid"
%	 points= "(1.25,21.25);(1.25,21.25);(1.25,3.75);(1.25,3.75)"
%	 stroke-width= "0.15"
%	 />
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(12.5,15)"
%	 stroke-width= "0.4"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\pnl$
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(22.5,6.25)"
%	 stroke-width= "0.4"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\dubb$
%</text>
%<multicurve fill-style= "solid"
%	 points= "(12.5,30);(12.5,30);(22.5,20);(22.5,20)"
%	 stroke-width= "0.4"
%	 />
%<multicurve fill-style= "solid"
%	 points= "(22.5,20);(22.5,20);(22.5,30);(22.5,30)"
%	 stroke-width= "0.4"
%	 />
%<multicurve fill-style= "solid"
%	 points= "(12.5,40);(12.5,40);(22.5,30);(22.5,30)"
%	 stroke-width= "0.4"
%	 />
%<multicurve fill-style= "solid"
%	 points= "(12.5,40);(12.5,40);(12.5,30);(12.5,30)"
%	 stroke-width= "0.4"
%	 />
%<multicurve fill-style= "none"
%	 points= "(17.5,35);(17.5,35);(17.5,45);(17.5,45)"
%	 stroke-width= "0.4"
%	 />
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(17.5,30)"
%	 stroke-width= "0.4"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\woo$
%</text>
%</jpic>
%%End JPIC-XML
%PSTricks content-type (pstricks.sty package needed)
%Add \usepackage{pstricks} in the preamble of your LaTeX file
%You can rescale the whole picture (to 80% for instance) by using the command \def\JPicScale{0.8}
\ifx\JPicScale\undefined\def\JPicScale{1}\fi
\psset{unit=\JPicScale mm}
\psset{linewidth=0.3,dotsep=1,hatchwidth=0.3,hatchsep=1.5,shadowsize=1,dimen=middle}
\psset{dotsize=0.7 2.5,dotscale=1 1,fillcolor=black}
\psset{arrowsize=1 2,arrowlength=1,arrowinset=0.25,tbarsize=0.7 5,bracketlength=0.15,rbracketlength=0.15}
\begin{pspicture}(0,0)(157.5,75)
\psline[linewidth=0.15,fillstyle=solid](121.25,21.25)(133.75,21.25)
\psline[linewidth=0.4](93.75,0)(93.75,40)
\psline[linewidth=0.4](72.5,40)(100,40)
\psline[linewidth=0.4](62.5,50)(100,50)
\psline[linewidth=0.4](100,50)(100,40)
\psline[linewidth=0.4](62.5,50)(72.5,40)
\psline[linewidth=0.4](93.75,50)(93.75,75)
\psline[linewidth=0.4](80,0)(80,40)
\rput(87.5,45){$\unl$}
\psline[linewidth=0.4](62.5,15)(72.5,5)
\psline[linewidth=0.4](62.5,5)(72.5,5)
\psline[linewidth=0.4](62.5,15)(62.5,5)
\rput(66.25,7.5){$\Nee$}
\psline[linewidth=0.4](67.5,10)(67.5,45)
\psline[linewidth=0.15,fillstyle=solid](121.25,3.75)(146.25,3.75)
\rput(50,45){\EQLS}
\psline[linewidth=0.4](150,0)(150,40)
\psline[linewidth=0.4](142.5,40)(157.5,40)
\psline[linewidth=0.4](132.5,50)(157.5,50)
\psline[linewidth=0.4](157.5,50)(157.5,40)
\psline[linewidth=0.4](122.5,20)(132.5,20)
\psline[linewidth=0.4](150,50)(150,75)
\psline[linewidth=0.4](137.5,0)(137.5,10)
\rput(150,45){$\unl$}
\psline[linewidth=0.4](122.5,15)(132.5,5)
\psline[linewidth=0.4](122.5,5)(132.5,5)
\psline[linewidth=0.4](122.5,15)(122.5,5)
\rput(126.25,7.5){$\Nee$}
\psline[linewidth=0.4](127.5,10)(127.5,15)
\rput(112.5,45){\EQLS}
\psline[linewidth=0.4](132.5,50)(142.5,40)
\psline[linewidth=0.4](132.5,10)(142.5,10)
\psline[linewidth=0.4](132.5,20)(142.5,10)
\psline[linewidth=0.4](122.5,20)(132.5,10)
\psline[linewidth=0.4](137.5,15)(137.5,45)
\psline[linewidth=0.15,fillstyle=solid](146.25,3.75)(146.25,8.75)
\psline[linewidth=0.15,fillstyle=solid](133.75,21.25)(146.25,8.75)
\psline[linewidth=0.15,fillstyle=solid](121.25,21.25)(121.25,3.75)
\rput(132.5,15){$\pnl$}
\rput(142.5,6.25){$\dubb$}
\psline[linewidth=0.15,fillstyle=solid](1.25,21.25)(13.75,21.25)
\psline[linewidth=0.15,fillstyle=solid](1.25,3.75)(26.25,3.75)
\psline[linewidth=0.4](30,0)(30,40)
\psline[linewidth=0.4](22.5,40)(37.5,40)
\psline[linewidth=0.4](12.5,50)(37.5,50)
\psline[linewidth=0.4](37.5,50)(37.5,40)
\psline[linewidth=0.4](2.5,20)(12.5,20)
\psline[linewidth=0.4](30,50)(30,75)
\psline[linewidth=0.4](17.5,0)(17.5,10)
\rput(30,45){$\unl$}
\psline[linewidth=0.4](2.5,15)(12.5,5)
\psline[linewidth=0.4](2.5,5)(12.5,5)
\psline[linewidth=0.4](2.5,15)(2.5,5)
\rput(6.25,7.5){$\Nee$}
\psline[linewidth=0.4](7.5,10)(7.5,15)
\psline[linewidth=0.4](12.5,50)(22.5,40)
\psline[linewidth=0.4](12.5,10)(22.5,10)
\psline[linewidth=0.4](12.5,20)(22.5,10)
\psline[linewidth=0.4](2.5,20)(12.5,10)
\psline[linewidth=0.4](17.5,15)(17.5,25)
\psline[linewidth=0.15,fillstyle=solid](26.25,3.75)(26.25,8.75)
\psline[linewidth=0.15,fillstyle=solid](13.75,21.25)(26.25,8.75)
\psline[linewidth=0.15,fillstyle=solid](1.25,21.25)(1.25,3.75)
\rput(12.5,15){$\pnl$}
\rput(22.5,6.25){$\dubb$}
\psline[linewidth=0.4,fillstyle=solid](12.5,30)(22.5,20)
\psline[linewidth=0.4,fillstyle=solid](22.5,20)(22.5,30)
\psline[linewidth=0.4,fillstyle=solid](12.5,40)(22.5,30)
\psline[linewidth=0.4,fillstyle=solid](12.5,40)(12.5,30)
\psline[linewidth=0.4](17.5,35)(17.5,45)
\rput(17.5,30){$\woo$}
\end{pspicture}


==> PIC/Omega-6.tex <==
%%Created by jPicEdt 1.4.1_03: mixed JPIC-XML/LaTeX format
%%Mon Feb 22 17:18:55 GMT-10:00 2021
%%Begin JPIC-XML
%<?xml version="1.0" standalone="yes"?>
%<jpic x-min="-2.5" x-max="85" y-min="0" y-max="90" auto-bounding="true">
%<multicurve fill-style= "none"
%	 points= "(77.5,10);(77.5,10);(77.5,0);(77.5,0)"
%	 stroke-width= "0.5"
%	 />
%<ellipse p3= "(78.75,8.75)"
%	 fill-style= "solid"
%	 p2= "(78.75,11.25)"
%	 p1= "(76.25,11.25)"
%	 closure= "open"
%	 angle-end= "0"
%	 stroke-width= "0.5"
%	 angle-start= "0"
%	 />
%<multicurve fill-style= "none"
%	 points= "(82.5,15);(82.5,15);(77.5,10);(77.5,10)"
%	 stroke-width= "0.5"
%	 />
%<multicurve fill-style= "none"
%	 points= "(77.5,10);(77.5,10);(72.5,15);(72.5,15)"
%	 stroke-width= "0.5"
%	 />
%<multicurve fill-style= "none"
%	 points= "(72.5,15);(72.5,15);(72.5,21.25);(72.5,21.25)"
%	 stroke-width= "0.5"
%	 />
%<multicurve fill-style= "none"
%	 points= "(82.5,15);(82.5,15);(82.5,55);(82.5,55)"
%	 stroke-width= "0.5"
%	 />
%<multicurve fill-style= "none"
%	 points= "(67.5,40);(67.5,40);(77.5,40);(77.5,40)"
%	 stroke-width= "0.5"
%	 />
%<multicurve fill-style= "none"
%	 points= "(57.5,50);(57.5,50);(67.5,50);(67.5,50)"
%	 stroke-width= "0.5"
%	 />
%<ellipse p3= "(76.02,21.48)"
%	 fill-style= "none"
%	 p2= "(76.02,28.52)"
%	 p1= "(68.98,28.52)"
%	 closure= "open"
%	 angle-end= "0"
%	 stroke-width= "0.5"
%	 angle-start= "0"
%	 />
%<multicurve fill-style= "none"
%	 points= "(72.5,28.75);(72.5,28.75);(72.5,40);(72.5,40)"
%	 stroke-width= "0.5"
%	 />
%<multicurve fill-style= "none"
%	 points= "(67.5,50);(67.5,50);(77.5,40);(77.5,40)"
%	 stroke-width= "0.5"
%	 />
%<multicurve fill-style= "none"
%	 points= "(57.5,50);(57.5,50);(67.5,40);(67.5,40)"
%	 stroke-width= "0.5"
%	 />
%<multicurve fill-style= "none"
%	 points= "(57.5,42.5);(57.5,42.5);(67.5,32.5);(67.5,32.5)"
%	 stroke-width= "0.5"
%	 />
%<multicurve fill-style= "none"
%	 points= "(72.5,45);(72.5,45);(72.5,55);(72.5,55)"
%	 stroke-width= "0.5"
%	 />
%<multicurve fill-style= "none"
%	 points= "(62.5,37.5);(62.5,37.5);(62.5,45);(62.5,45)"
%	 stroke-width= "0.5"
%	 />
%<multicurve fill-style= "none"
%	 points= "(57.5,32.5);(57.5,32.5);(67.5,32.5);(67.5,32.5)"
%	 stroke-width= "0.5"
%	 />
%<multicurve fill-style= "none"
%	 points= "(57.5,42.5);(57.5,42.5);(57.5,32.5);(57.5,32.5)"
%	 stroke-width= "0.5"
%	 />
%<multicurve fill-style= "none"
%	 points= "(70,55);(70,55);(85,55);(85,55)"
%	 stroke-width= "0.5"
%	 />
%<multicurve fill-style= "none"
%	 points= "(70,70);(70,70);(70,55);(70,55)"
%	 stroke-width= "0.5"
%	 />
%<multicurve fill-style= "none"
%	 points= "(70,70);(70,70);(85,55);(85,55)"
%	 stroke-width= "0.5"
%	 />
%<multicurve fill-style= "none"
%	 points= "(77.5,75);(77.5,75);(77.5,62.5);(77.5,62.5)"
%	 stroke-width= "0.5"
%	 />
%<multicurve fill-style= "none"
%	 points= "(10,40);(10,40);(20,40);(20,40)"
%	 stroke-width= "0.5"
%	 />
%<multicurve fill-style= "none"
%	 points= "(0,50);(0,50);(20,50);(20,50)"
%	 stroke-width= "0.5"
%	 />
%<multicurve fill-style= "none"
%	 points= "(15,0);(15,0);(15,40);(15,40)"
%	 stroke-width= "0.5"
%	 />
%<multicurve fill-style= "none"
%	 points= "(0,50);(0,50);(10,40);(10,40)"
%	 stroke-width= "0.5"
%	 />
%<multicurve fill-style= "none"
%	 points= "(0,42.5);(0,42.5);(10,32.5);(10,32.5)"
%	 stroke-width= "0.5"
%	 />
%<multicurve fill-style= "none"
%	 points= "(5,37.5);(5,37.5);(5,45);(5,45)"
%	 stroke-width= "0.5"
%	 />
%<multicurve fill-style= "none"
%	 points= "(0,32.5);(0,32.5);(10,32.5);(10,32.5)"
%	 stroke-width= "0.5"
%	 />
%<multicurve fill-style= "none"
%	 points= "(0,42.5);(0,42.5);(0,32.5);(0,32.5)"
%	 stroke-width= "0.5"
%	 />
%<multicurve fill-style= "none"
%	 points= "(20,50);(20,50);(20,40);(20,40)"
%	 stroke-width= "0.5"
%	 />
%<multicurve fill-style= "none"
%	 points= "(15,75);(15,75);(15,50);(15,50)"
%	 stroke-width= "0.5"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "solid"
%	 anchor-point= "(40,45)"
%	 text-frame= "noframe"
%	 stroke-width= "0.5"
%	 text-hor-align= "center-h"
%	 >
%\EQLS
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "solid"
%	 anchor-point= "(60,35)"
%	 text-frame= "noframe"
%	 stroke-width= "0.5"
%	 text-hor-align= "center-h"
%	 >
%$\Nee$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "solid"
%	 anchor-point= "(2.5,35)"
%	 text-frame= "noframe"
%	 stroke-width= "0.5"
%	 text-hor-align= "center-h"
%	 >
%$\Nee$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "solid"
%	 anchor-point= "(72.5,25)"
%	 text-frame= "noframe"
%	 stroke-width= "0.5"
%	 text-hor-align= "center-h"
%	 >
%$\addd$
%</text>
%<multicurve fill-style= "solid"
%	 points= "(-2.5,52.5);(-2.5,52.5);(22.5,52.5);(22.5,52.5)"
%	 stroke-width= "0.15"
%	 />
%<multicurve fill-style= "solid"
%	 points= "(-2.5,30);(-2.5,30);(-2.5,52.5);(-2.5,52.5)"
%	 stroke-width= "0.15"
%	 />
%<multicurve fill-style= "solid"
%	 points= "(22.5,30);(22.5,30);(-2.5,30);(-2.5,30)"
%	 stroke-width= "0.15"
%	 />
%<multicurve fill-style= "solid"
%	 points= "(22.5,52.5);(22.5,52.5);(22.5,30);(22.5,30)"
%	 stroke-width= "0.15"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "solid"
%	 anchor-point= "(20,32.5)"
%	 text-frame= "noframe"
%	 stroke-width= "0.5"
%	 text-hor-align= "center-h"
%	 >
%$\Homega$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "solid"
%	 anchor-point= "(14.38,45)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\unl$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "solid"
%	 anchor-point= "(67.5,45)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\pnl$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "solid"
%	 anchor-point= "(75,58.75)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\png$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "solid"
%	 anchor-point= "(25,90)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%\LHS
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "solid"
%	 anchor-point= "(40,90)"
%	 text-frame= "noframe"
%	 stroke-width= "0.5"
%	 text-hor-align= "center-h"
%	 >
%\EQLS
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "solid"
%	 anchor-point= "(55,90)"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%\RHS
%</text>
%</jpic>
%%End JPIC-XML
%PSTricks content-type (pstricks.sty package needed)
%Add \usepackage{pstricks} in the preamble of your LaTeX file
%You can rescale the whole picture (to 80% for instance) by using the command \def\JPicScale{0.8}
\ifx\JPicScale\undefined\def\JPicScale{1}\fi
\psset{unit=\JPicScale mm}
\psset{linewidth=0.3,dotsep=1,hatchwidth=0.3,hatchsep=1.5,shadowsize=1,dimen=middle}
\psset{dotsize=0.7 2.5,dotscale=1 1,fillcolor=black}
\psset{arrowsize=1 2,arrowlength=1,arrowinset=0.25,tbarsize=0.7 5,bracketlength=0.15,rbracketlength=0.15}
\begin{pspicture}(0,0)(85,90)
\psline[linewidth=0.5](77.5,10)(77.5,0)
\rput{0}(77.5,10){\psellipse[linewidth=0.5,fillstyle=solid](0,0)(1.25,-1.25)}
\psline[linewidth=0.5](82.5,15)(77.5,10)
\psline[linewidth=0.5](77.5,10)(72.5,15)
\psline[linewidth=0.5](72.5,15)(72.5,21.25)
\psline[linewidth=0.5](82.5,15)(82.5,55)
\psline[linewidth=0.5](67.5,40)(77.5,40)
\psline[linewidth=0.5](57.5,50)(67.5,50)
\rput{0}(72.5,25){\psellipse[linewidth=0.5](0,0)(3.52,-3.52)}
\psline[linewidth=0.5](72.5,28.75)(72.5,40)
\psline[linewidth=0.5](67.5,50)(77.5,40)
\psline[linewidth=0.5](57.5,50)(67.5,40)
\psline[linewidth=0.5](57.5,42.5)(67.5,32.5)
\psline[linewidth=0.5](72.5,45)(72.5,55)
\psline[linewidth=0.5](62.5,37.5)(62.5,45)
\psline[linewidth=0.5](57.5,32.5)(67.5,32.5)
\psline[linewidth=0.5](57.5,42.5)(57.5,32.5)
\psline[linewidth=0.5](70,55)(85,55)
\psline[linewidth=0.5](70,70)(70,55)
\psline[linewidth=0.5](70,70)(85,55)
\psline[linewidth=0.5](77.5,75)(77.5,62.5)
\psline[linewidth=0.5](10,40)(20,40)
\psline[linewidth=0.5](0,50)(20,50)
\psline[linewidth=0.5](15,0)(15,40)
\psline[linewidth=0.5](0,50)(10,40)
\psline[linewidth=0.5](0,42.5)(10,32.5)
\psline[linewidth=0.5](5,37.5)(5,45)
\psline[linewidth=0.5](0,32.5)(10,32.5)
\psline[linewidth=0.5](0,42.5)(0,32.5)
\psline[linewidth=0.5](20,50)(20,40)
\psline[linewidth=0.5](15,75)(15,50)
\rput(40,45){\EQLS}
\rput(60,35){$\Nee$}
\rput(2.5,35){$\Nee$}
\rput(72.5,25){$\addd$}
\psline[linewidth=0.15,fillstyle=solid](-2.5,52.5)(22.5,52.5)
\psline[linewidth=0.15,fillstyle=solid](-2.5,30)(-2.5,52.5)
\psline[linewidth=0.15,fillstyle=solid](22.5,30)(-2.5,30)
\psline[linewidth=0.15,fillstyle=solid](22.5,52.5)(22.5,30)
\rput(20,32.5){$\Homega$}
\rput(14.38,45){$\unl$}
\rput(67.5,45){$\pnl$}
\rput(75,58.75){$\png$}
\rput[r](25,90){\LHS}
\rput(40,90){\EQLS}
\rput[l](55,90){\RHS}
\end{pspicture}


==> PIC/Omega-7.tex <==
%%Created by jPicEdt 1.4.1_03: mixed JPIC-XML/LaTeX format
%%Wed Feb 24 10:18:28 GMT-10:00 2021
%%Begin JPIC-XML
%<?xml version="1.0" standalone="yes"?>
%<jpic x-min="2.5" x-max="197.5" y-min="0" y-max="85" auto-bounding="true">
%<multicurve fill-style= "none"
%	 points= "(75,5);(75,5);(75,0);(75,0)"
%	 stroke-width= "0.5"
%	 />
%<ellipse p3= "(76.25,3.75)"
%	 fill-style= "solid"
%	 p2= "(76.25,6.25)"
%	 p1= "(73.75,6.25)"
%	 closure= "open"
%	 angle-end= "0"
%	 stroke-width= "0.5"
%	 angle-start= "0"
%	 />
%<multicurve fill-style= "none"
%	 points= "(80,10);(80,10);(75,5);(75,5)"
%	 stroke-width= "0.5"
%	 />
%<multicurve fill-style= "none"
%	 points= "(75,5);(75,5);(70,10);(70,10)"
%	 stroke-width= "0.5"
%	 />
%<multicurve fill-style= "none"
%	 points= "(70,10);(70,10);(70,13.75);(70,13.75)"
%	 stroke-width= "0.5"
%	 />
%<multicurve fill-style= "none"
%	 points= "(80,10);(80,10);(80,55);(80,55)"
%	 stroke-width= "0.5"
%	 />
%<multicurve fill-style= "none"
%	 points= "(65,40);(65,40);(75,40);(75,40)"
%	 stroke-width= "0.5"
%	 />
%<multicurve fill-style= "none"
%	 points= "(55,50);(55,50);(75,50);(75,50)"
%	 stroke-width= "0.5"
%	 />
%<ellipse p3= "(73.52,13.98)"
%	 fill-style= "none"
%	 p2= "(73.52,21.02)"
%	 p1= "(66.48,21.02)"
%	 closure= "open"
%	 angle-end= "0"
%	 stroke-width= "0.5"
%	 angle-start= "0"
%	 />
%<multicurve fill-style= "none"
%	 points= "(70,21.25);(70,21.25);(70,40);(70,40)"
%	 stroke-width= "0.5"
%	 />
%<multicurve fill-style= "none"
%	 points= "(75,50);(75,50);(75,40);(75,40)"
%	 stroke-width= "0.5"
%	 />
%<multicurve fill-style= "none"
%	 points= "(55,50);(55,50);(65,40);(65,40)"
%	 stroke-width= "0.5"
%	 />
%<multicurve fill-style= "none"
%	 points= "(55,42.5);(55,42.5);(65,32.5);(65,32.5)"
%	 stroke-width= "0.5"
%	 />
%<multicurve fill-style= "none"
%	 points= "(70,50);(70,50);(70,55);(70,55)"
%	 stroke-width= "0.5"
%	 />
%<multicurve fill-style= "none"
%	 points= "(60,37.5);(60,37.5);(60,45);(60,45)"
%	 stroke-width= "0.5"
%	 />
%<multicurve fill-style= "none"
%	 points= "(55,32.5);(55,32.5);(65,32.5);(65,32.5)"
%	 stroke-width= "0.5"
%	 />
%<multicurve fill-style= "none"
%	 points= "(55,42.5);(55,42.5);(55,32.5);(55,32.5)"
%	 stroke-width= "0.5"
%	 />
%<multicurve fill-style= "none"
%	 points= "(67.5,55);(67.5,55);(82.5,55);(82.5,55)"
%	 stroke-width= "0.5"
%	 />
%<multicurve fill-style= "none"
%	 points= "(67.5,70);(67.5,70);(67.5,55);(67.5,55)"
%	 stroke-width= "0.5"
%	 />
%<multicurve fill-style= "none"
%	 points= "(67.5,70);(67.5,70);(82.5,55);(82.5,55)"
%	 stroke-width= "0.5"
%	 />
%<multicurve fill-style= "none"
%	 points= "(75,67.5);(75,67.5);(75,62.5);(75,62.5)"
%	 stroke-width= "0.5"
%	 />
%<multicurve fill-style= "none"
%	 points= "(15,40);(15,40);(25,40);(25,40)"
%	 stroke-width= "0.5"
%	 />
%<multicurve fill-style= "none"
%	 points= "(5,50);(5,50);(25,50);(25,50)"
%	 stroke-width= "0.5"
%	 />
%<multicurve fill-style= "none"
%	 points= "(20,0);(20,0);(20,40);(20,40)"
%	 stroke-width= "0.5"
%	 />
%<multicurve fill-style= "none"
%	 points= "(5,50);(5,50);(15,40);(15,40)"
%	 stroke-width= "0.5"
%	 />
%<multicurve fill-style= "none"
%	 points= "(5,42.5);(5,42.5);(15,32.5);(15,32.5)"
%	 stroke-width= "0.5"
%	 />
%<multicurve fill-style= "none"
%	 points= "(10,37.5);(10,37.5);(10,45);(10,45)"
%	 stroke-width= "0.5"
%	 />
%<multicurve fill-style= "none"
%	 points= "(5,32.5);(5,32.5);(15,32.5);(15,32.5)"
%	 stroke-width= "0.5"
%	 />
%<multicurve fill-style= "none"
%	 points= "(5,42.5);(5,42.5);(5,32.5);(5,32.5)"
%	 stroke-width= "0.5"
%	 />
%<multicurve fill-style= "none"
%	 points= "(25,50);(25,50);(25,40);(25,40)"
%	 stroke-width= "0.5"
%	 />
%<multicurve fill-style= "none"
%	 points= "(20,67.5);(20,67.5);(20,50);(20,50)"
%	 stroke-width= "0.5"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "solid"
%	 anchor-point= "(40,45)"
%	 text-frame= "noframe"
%	 stroke-width= "0.5"
%	 text-hor-align= "center-h"
%	 >
%\EQLS
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "solid"
%	 anchor-point= "(57.5,35)"
%	 text-frame= "noframe"
%	 stroke-width= "0.5"
%	 text-hor-align= "center-h"
%	 >
%$\Nee$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "solid"
%	 anchor-point= "(7.5,35)"
%	 text-frame= "noframe"
%	 stroke-width= "0.5"
%	 text-hor-align= "center-h"
%	 >
%$\Nee$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "solid"
%	 anchor-point= "(70,17.5)"
%	 text-frame= "noframe"
%	 stroke-width= "0.5"
%	 text-hor-align= "center-h"
%	 >
%$\addd$
%</text>
%<multicurve fill-style= "solid"
%	 points= "(2.5,52.5);(2.5,52.5);(27.5,52.5);(27.5,52.5)"
%	 stroke-width= "0.15"
%	 />
%<multicurve fill-style= "solid"
%	 points= "(2.5,30);(2.5,30);(2.5,52.5);(2.5,52.5)"
%	 stroke-width= "0.15"
%	 />
%<multicurve fill-style= "solid"
%	 points= "(27.5,30);(27.5,30);(2.5,30);(2.5,30)"
%	 stroke-width= "0.15"
%	 />
%<multicurve fill-style= "solid"
%	 points= "(27.5,52.5);(27.5,52.5);(27.5,30);(27.5,30)"
%	 stroke-width= "0.15"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "solid"
%	 anchor-point= "(24.38,32.5)"
%	 text-frame= "noframe"
%	 stroke-width= "0.5"
%	 text-hor-align= "center-h"
%	 >
%$\Homega$
%</text>
%<multicurve fill-style= "none"
%	 points= "(67.5,75);(67.5,75);(82.5,75);(82.5,75)"
%	 stroke-width= "0.5"
%	 />
%<multicurve fill-style= "none"
%	 points= "(82.5,75);(82.5,75);(82.5,60);(82.5,60)"
%	 stroke-width= "0.5"
%	 />
%<multicurve fill-style= "none"
%	 points= "(67.5,75);(67.5,75);(82.5,60);(82.5,60)"
%	 stroke-width= "0.5"
%	 />
%<multicurve fill-style= "none"
%	 points= "(70,85);(70,85);(70,75);(70,75)"
%	 stroke-width= "0.5"
%	 />
%<multicurve fill-style= "none"
%	 points= "(80,80);(80,80);(80,75);(80,75)"
%	 stroke-width= "0.5"
%	 />
%<ellipse p3= "(81.25,78.75)"
%	 fill-style= "solid"
%	 p2= "(81.25,81.25)"
%	 p1= "(78.75,81.25)"
%	 closure= "open"
%	 angle-end= "0"
%	 stroke-width= "0.5"
%	 angle-start= "0"
%	 />
%<multicurve fill-style= "none"
%	 points= "(12.5,75);(12.5,75);(27.5,75);(27.5,75)"
%	 stroke-width= "0.5"
%	 />
%<multicurve fill-style= "none"
%	 points= "(27.5,75);(27.5,75);(27.5,60);(27.5,60)"
%	 stroke-width= "0.5"
%	 />
%<multicurve fill-style= "none"
%	 points= "(12.5,75);(12.5,75);(27.5,60);(27.5,60)"
%	 stroke-width= "0.5"
%	 />
%<multicurve fill-style= "none"
%	 points= "(25,80);(25,80);(25,75);(25,75)"
%	 stroke-width= "0.5"
%	 />
%<ellipse p3= "(26.25,78.75)"
%	 fill-style= "solid"
%	 p2= "(26.25,81.25)"
%	 p1= "(23.75,81.25)"
%	 closure= "open"
%	 angle-end= "0"
%	 stroke-width= "0.5"
%	 angle-start= "0"
%	 />
%<multicurve fill-style= "none"
%	 points= "(135,5);(135,5);(135,0);(135,0)"
%	 stroke-width= "0.5"
%	 />
%<ellipse p3= "(136.25,3.75)"
%	 fill-style= "solid"
%	 p2= "(136.25,6.25)"
%	 p1= "(133.75,6.25)"
%	 closure= "open"
%	 angle-end= "0"
%	 stroke-width= "0.5"
%	 angle-start= "0"
%	 />
%<multicurve fill-style= "none"
%	 points= "(140,10);(140,10);(135,5);(135,5)"
%	 stroke-width= "0.5"
%	 />
%<multicurve fill-style= "none"
%	 points= "(135,5);(135,5);(130,10);(130,10)"
%	 stroke-width= "0.5"
%	 />
%<multicurve fill-style= "none"
%	 points= "(130,10);(130,10);(130,13.75);(130,13.75)"
%	 stroke-width= "0.5"
%	 />
%<multicurve fill-style= "none"
%	 points= "(140,10);(140,10);(140,80);(140,80)"
%	 stroke-width= "0.5"
%	 />
%<multicurve fill-style= "none"
%	 points= "(125,40);(125,40);(135,40);(135,40)"
%	 stroke-width= "0.5"
%	 />
%<multicurve fill-style= "none"
%	 points= "(115,50);(115,50);(135,50);(135,50)"
%	 stroke-width= "0.5"
%	 />
%<ellipse p3= "(133.52,13.98)"
%	 fill-style= "none"
%	 p2= "(133.52,21.02)"
%	 p1= "(126.48,21.02)"
%	 closure= "open"
%	 angle-end= "0"
%	 stroke-width= "0.5"
%	 angle-start= "0"
%	 />
%<multicurve fill-style= "none"
%	 points= "(130,21.25);(130,21.25);(130,40);(130,40)"
%	 stroke-width= "0.5"
%	 />
%<multicurve fill-style= "none"
%	 points= "(115,50);(115,50);(125,40);(125,40)"
%	 stroke-width= "0.5"
%	 />
%<multicurve fill-style= "none"
%	 points= "(115,42.5);(115,42.5);(125,32.5);(125,32.5)"
%	 stroke-width= "0.5"
%	 />
%<multicurve fill-style= "none"
%	 points= "(120,37.5);(120,37.5);(120,45);(120,45)"
%	 stroke-width= "0.5"
%	 />
%<multicurve fill-style= "none"
%	 points= "(115,32.5);(115,32.5);(125,32.5);(125,32.5)"
%	 stroke-width= "0.5"
%	 />
%<multicurve fill-style= "none"
%	 points= "(115,42.5);(115,42.5);(115,32.5);(115,32.5)"
%	 stroke-width= "0.5"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "solid"
%	 anchor-point= "(100,45)"
%	 text-frame= "noframe"
%	 stroke-width= "0.5"
%	 text-hor-align= "center-h"
%	 >
%\EQLS
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "solid"
%	 anchor-point= "(117.5,35)"
%	 text-frame= "noframe"
%	 stroke-width= "0.5"
%	 text-hor-align= "center-h"
%	 >
%$\Nee$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "solid"
%	 anchor-point= "(130,17.5)"
%	 text-frame= "noframe"
%	 stroke-width= "0.5"
%	 text-hor-align= "center-h"
%	 >
%$\addd$
%</text>
%<ellipse p3= "(141.25,78.75)"
%	 fill-style= "solid"
%	 p2= "(141.25,81.25)"
%	 p1= "(138.75,81.25)"
%	 closure= "open"
%	 angle-end= "0"
%	 stroke-width= "0.5"
%	 angle-start= "0"
%	 />
%<multicurve fill-style= "none"
%	 points= "(135,50);(135,50);(135,40);(135,40)"
%	 stroke-width= "0.5"
%	 />
%<multicurve fill-style= "none"
%	 points= "(130,85);(130,85);(130,50);(130,50)"
%	 stroke-width= "0.5"
%	 />
%<multicurve fill-style= "none"
%	 points= "(190,0);(190,0);(190,13.75);(190,13.75)"
%	 stroke-width= "0.5"
%	 />
%<multicurve fill-style= "none"
%	 points= "(185,40);(185,40);(195,40);(195,40)"
%	 stroke-width= "0.5"
%	 />
%<multicurve fill-style= "none"
%	 points= "(175,50);(175,50);(195,50);(195,50)"
%	 stroke-width= "0.5"
%	 />
%<ellipse p3= "(193.52,13.98)"
%	 fill-style= "none"
%	 p2= "(193.52,21.02)"
%	 p1= "(186.48,21.02)"
%	 closure= "open"
%	 angle-end= "0"
%	 stroke-width= "0.5"
%	 angle-start= "0"
%	 />
%<multicurve fill-style= "none"
%	 points= "(190,21.25);(190,21.25);(190,40);(190,40)"
%	 stroke-width= "0.5"
%	 />
%<multicurve fill-style= "none"
%	 points= "(175,50);(175,50);(185,40);(185,40)"
%	 stroke-width= "0.5"
%	 />
%<multicurve fill-style= "none"
%	 points= "(175,42.5);(175,42.5);(185,32.5);(185,32.5)"
%	 stroke-width= "0.5"
%	 />
%<multicurve fill-style= "none"
%	 points= "(180,37.5);(180,37.5);(180,45);(180,45)"
%	 stroke-width= "0.5"
%	 />
%<multicurve fill-style= "none"
%	 points= "(175,32.5);(175,32.5);(185,32.5);(185,32.5)"
%	 stroke-width= "0.5"
%	 />
%<multicurve fill-style= "none"
%	 points= "(175,42.5);(175,42.5);(175,32.5);(175,32.5)"
%	 stroke-width= "0.5"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "solid"
%	 anchor-point= "(160,45)"
%	 text-frame= "noframe"
%	 stroke-width= "0.5"
%	 text-hor-align= "center-h"
%	 >
%\EQLS
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "solid"
%	 anchor-point= "(177.5,35)"
%	 text-frame= "noframe"
%	 stroke-width= "0.5"
%	 text-hor-align= "center-h"
%	 >
%$\Nee$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "solid"
%	 anchor-point= "(190,17.5)"
%	 text-frame= "noframe"
%	 stroke-width= "0.5"
%	 text-hor-align= "center-h"
%	 >
%$\addd$
%</text>
%<multicurve fill-style= "none"
%	 points= "(195,50);(195,50);(195,40);(195,40)"
%	 stroke-width= "0.5"
%	 />
%<multicurve fill-style= "none"
%	 points= "(190,85);(190,85);(190,50);(190,50)"
%	 stroke-width= "0.5"
%	 />
%<multicurve fill-style= "solid"
%	 points= "(172.5,52.5);(172.5,52.5);(197.5,52.5);(197.5,52.5)"
%	 stroke-width= "0.15"
%	 />
%<multicurve fill-style= "solid"
%	 points= "(172.5,30);(172.5,30);(172.5,52.5);(172.5,52.5)"
%	 stroke-width= "0.15"
%	 />
%<multicurve fill-style= "solid"
%	 points= "(197.5,30);(197.5,30);(172.5,30);(172.5,30)"
%	 stroke-width= "0.15"
%	 />
%<multicurve fill-style= "solid"
%	 points= "(197.5,52.5);(197.5,52.5);(197.5,30);(197.5,30)"
%	 stroke-width= "0.15"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "solid"
%	 anchor-point= "(194.38,32.5)"
%	 text-frame= "noframe"
%	 stroke-width= "0.5"
%	 text-hor-align= "center-h"
%	 >
%$\Homega$
%</text>
%<multicurve fill-style= "none"
%	 points= "(20,85);(20,85);(20,75);(20,75)"
%	 stroke-width= "0.5"
%	 />
%<multicurve fill-style= "solid"
%	 points= "(52.5,52.5);(52.5,52.5);(77.5,52.5);(77.5,52.5)"
%	 stroke-width= "0.15"
%	 />
%<multicurve fill-style= "solid"
%	 points= "(52.5,30);(52.5,30);(52.5,52.5);(52.5,52.5)"
%	 stroke-width= "0.15"
%	 />
%<multicurve fill-style= "solid"
%	 points= "(77.5,30);(77.5,30);(52.5,30);(52.5,30)"
%	 stroke-width= "0.15"
%	 />
%<multicurve fill-style= "solid"
%	 points= "(77.5,52.5);(77.5,52.5);(77.5,30);(77.5,30)"
%	 stroke-width= "0.15"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "solid"
%	 anchor-point= "(74.38,32.5)"
%	 text-frame= "noframe"
%	 stroke-width= "0.5"
%	 text-hor-align= "center-h"
%	 >
%$\Homega$
%</text>
%<multicurve fill-style= "solid"
%	 points= "(112.5,52.5);(112.5,52.5);(137.5,52.5);(137.5,52.5)"
%	 stroke-width= "0.15"
%	 />
%<multicurve fill-style= "solid"
%	 points= "(112.5,30);(112.5,30);(112.5,52.5);(112.5,52.5)"
%	 stroke-width= "0.15"
%	 />
%<multicurve fill-style= "solid"
%	 points= "(137.5,30);(137.5,30);(112.5,30);(112.5,30)"
%	 stroke-width= "0.15"
%	 />
%<multicurve fill-style= "solid"
%	 points= "(137.5,52.5);(137.5,52.5);(137.5,30);(137.5,30)"
%	 stroke-width= "0.15"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "solid"
%	 anchor-point= "(134.38,32.5)"
%	 text-frame= "noframe"
%	 stroke-width= "0.5"
%	 text-hor-align= "center-h"
%	 >
%$\Homega$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "solid"
%	 anchor-point= "(20,45)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\unl$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "solid"
%	 anchor-point= "(72.5,58.75)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\png$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "solid"
%	 anchor-point= "(70,45)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\unl$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "solid"
%	 anchor-point= "(130,45)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\unl$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "solid"
%	 anchor-point= "(190,45)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\unl$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "solid"
%	 anchor-point= "(78.12,70)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\prj$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "solid"
%	 anchor-point= "(23.12,70)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\prj$
%</text>
%</jpic>
%%End JPIC-XML
%PSTricks content-type (pstricks.sty package needed)
%Add \usepackage{pstricks} in the preamble of your LaTeX file
%You can rescale the whole picture (to 80% for instance) by using the command \def\JPicScale{0.8}
\ifx\JPicScale\undefined\def\JPicScale{1}\fi
\psset{unit=\JPicScale mm}
\psset{linewidth=0.3,dotsep=1,hatchwidth=0.3,hatchsep=1.5,shadowsize=1,dimen=middle}
\psset{dotsize=0.7 2.5,dotscale=1 1,fillcolor=black}
\psset{arrowsize=1 2,arrowlength=1,arrowinset=0.25,tbarsize=0.7 5,bracketlength=0.15,rbracketlength=0.15}
\begin{pspicture}(0,0)(197.5,85)
\psline[linewidth=0.5](75,5)(75,0)
\rput{0}(75,5){\psellipse[linewidth=0.5,fillstyle=solid](0,0)(1.25,-1.25)}
\psline[linewidth=0.5](80,10)(75,5)
\psline[linewidth=0.5](75,5)(70,10)
\psline[linewidth=0.5](70,10)(70,13.75)
\psline[linewidth=0.5](80,10)(80,55)
\psline[linewidth=0.5](65,40)(75,40)
\psline[linewidth=0.5](55,50)(75,50)
\rput{0}(70,17.5){\psellipse[linewidth=0.5](0,0)(3.52,-3.52)}
\psline[linewidth=0.5](70,21.25)(70,40)
\psline[linewidth=0.5](75,50)(75,40)
\psline[linewidth=0.5](55,50)(65,40)
\psline[linewidth=0.5](55,42.5)(65,32.5)
\psline[linewidth=0.5](70,50)(70,55)
\psline[linewidth=0.5](60,37.5)(60,45)
\psline[linewidth=0.5](55,32.5)(65,32.5)
\psline[linewidth=0.5](55,42.5)(55,32.5)
\psline[linewidth=0.5](67.5,55)(82.5,55)
\psline[linewidth=0.5](67.5,70)(67.5,55)
\psline[linewidth=0.5](67.5,70)(82.5,55)
\psline[linewidth=0.5](75,67.5)(75,62.5)
\psline[linewidth=0.5](15,40)(25,40)
\psline[linewidth=0.5](5,50)(25,50)
\psline[linewidth=0.5](20,0)(20,40)
\psline[linewidth=0.5](5,50)(15,40)
\psline[linewidth=0.5](5,42.5)(15,32.5)
\psline[linewidth=0.5](10,37.5)(10,45)
\psline[linewidth=0.5](5,32.5)(15,32.5)
\psline[linewidth=0.5](5,42.5)(5,32.5)
\psline[linewidth=0.5](25,50)(25,40)
\psline[linewidth=0.5](20,67.5)(20,50)
\rput(40,45){\EQLS}
\rput(57.5,35){$\Nee$}
\rput(7.5,35){$\Nee$}
\rput(70,17.5){$\addd$}
\psline[linewidth=0.15,fillstyle=solid](2.5,52.5)(27.5,52.5)
\psline[linewidth=0.15,fillstyle=solid](2.5,30)(2.5,52.5)
\psline[linewidth=0.15,fillstyle=solid](27.5,30)(2.5,30)
\psline[linewidth=0.15,fillstyle=solid](27.5,52.5)(27.5,30)
\rput(24.38,32.5){$\Homega$}
\psline[linewidth=0.5](67.5,75)(82.5,75)
\psline[linewidth=0.5](82.5,75)(82.5,60)
\psline[linewidth=0.5](67.5,75)(82.5,60)
\psline[linewidth=0.5](70,85)(70,75)
\psline[linewidth=0.5](80,80)(80,75)
\rput{0}(80,80){\psellipse[linewidth=0.5,fillstyle=solid](0,0)(1.25,-1.25)}
\psline[linewidth=0.5](12.5,75)(27.5,75)
\psline[linewidth=0.5](27.5,75)(27.5,60)
\psline[linewidth=0.5](12.5,75)(27.5,60)
\psline[linewidth=0.5](25,80)(25,75)
\rput{0}(25,80){\psellipse[linewidth=0.5,fillstyle=solid](0,0)(1.25,-1.25)}
\psline[linewidth=0.5](135,5)(135,0)
\rput{0}(135,5){\psellipse[linewidth=0.5,fillstyle=solid](0,0)(1.25,-1.25)}
\psline[linewidth=0.5](140,10)(135,5)
\psline[linewidth=0.5](135,5)(130,10)
\psline[linewidth=0.5](130,10)(130,13.75)
\psline[linewidth=0.5](140,10)(140,80)
\psline[linewidth=0.5](125,40)(135,40)
\psline[linewidth=0.5](115,50)(135,50)
\rput{0}(130,17.5){\psellipse[linewidth=0.5](0,0)(3.52,-3.52)}
\psline[linewidth=0.5](130,21.25)(130,40)
\psline[linewidth=0.5](115,50)(125,40)
\psline[linewidth=0.5](115,42.5)(125,32.5)
\psline[linewidth=0.5](120,37.5)(120,45)
\psline[linewidth=0.5](115,32.5)(125,32.5)
\psline[linewidth=0.5](115,42.5)(115,32.5)
\rput(100,45){\EQLS}
\rput(117.5,35){$\Nee$}
\rput(130,17.5){$\addd$}
\rput{0}(140,80){\psellipse[linewidth=0.5,fillstyle=solid](0,0)(1.25,-1.25)}
\psline[linewidth=0.5](135,50)(135,40)
\psline[linewidth=0.5](130,85)(130,50)
\psline[linewidth=0.5](190,0)(190,13.75)
\psline[linewidth=0.5](185,40)(195,40)
\psline[linewidth=0.5](175,50)(195,50)
\rput{0}(190,17.5){\psellipse[linewidth=0.5](0,0)(3.52,-3.52)}
\psline[linewidth=0.5](190,21.25)(190,40)
\psline[linewidth=0.5](175,50)(185,40)
\psline[linewidth=0.5](175,42.5)(185,32.5)
\psline[linewidth=0.5](180,37.5)(180,45)
\psline[linewidth=0.5](175,32.5)(185,32.5)
\psline[linewidth=0.5](175,42.5)(175,32.5)
\rput(160,45){\EQLS}
\rput(177.5,35){$\Nee$}
\rput(190,17.5){$\addd$}
\psline[linewidth=0.5](195,50)(195,40)
\psline[linewidth=0.5](190,85)(190,50)
\psline[linewidth=0.15,fillstyle=solid](172.5,52.5)(197.5,52.5)
\psline[linewidth=0.15,fillstyle=solid](172.5,30)(172.5,52.5)
\psline[linewidth=0.15,fillstyle=solid](197.5,30)(172.5,30)
\psline[linewidth=0.15,fillstyle=solid](197.5,52.5)(197.5,30)
\rput(194.38,32.5){$\Homega$}
\psline[linewidth=0.5](20,85)(20,75)
\psline[linewidth=0.15,fillstyle=solid](52.5,52.5)(77.5,52.5)
\psline[linewidth=0.15,fillstyle=solid](52.5,30)(52.5,52.5)
\psline[linewidth=0.15,fillstyle=solid](77.5,30)(52.5,30)
\psline[linewidth=0.15,fillstyle=solid](77.5,52.5)(77.5,30)
\rput(74.38,32.5){$\Homega$}
\psline[linewidth=0.15,fillstyle=solid](112.5,52.5)(137.5,52.5)
\psline[linewidth=0.15,fillstyle=solid](112.5,30)(112.5,52.5)
\psline[linewidth=0.15,fillstyle=solid](137.5,30)(112.5,30)
\psline[linewidth=0.15,fillstyle=solid](137.5,52.5)(137.5,30)
\rput(134.38,32.5){$\Homega$}
\rput(20,45){$\unl$}
\rput(72.5,58.75){$\png$}
\rput(70,45){$\unl$}
\rput(130,45){$\unl$}
\rput(190,45){$\unl$}
\rput(78.12,70){$\prj$}
\rput(23.12,70){$\prj$}
\end{pspicture}


==> PIC/Omega-plus.tex <==
%%Created by jPicEdt 1.4.1_03: mixed JPIC-XML/LaTeX format
%%Thu Feb 25 21:30:25 GMT-10:00 2021
%%Begin JPIC-XML
%<?xml version="1.0" standalone="yes"?>
%<jpic x-min="0" x-max="193.75" y-min="1.25" y-max="162.5" auto-bounding="true">
%<multicurve fill-style= "none"
%	 points= "(65,47.5);(65,47.5);(65,42.5);(65,42.5)"
%	 stroke-width= "0.5"
%	 />
%<ellipse p3= "(71.25,23.75)"
%	 fill-style= "solid"
%	 p2= "(71.25,26.25)"
%	 p1= "(68.75,26.25)"
%	 closure= "open"
%	 angle-end= "0"
%	 stroke-width= "0.5"
%	 angle-start= "0"
%	 />
%<multicurve fill-style= "none"
%	 points= "(75,30);(75,30);(70,25);(70,25)"
%	 stroke-width= "0.5"
%	 />
%<multicurve fill-style= "none"
%	 points= "(70,25);(70,25);(65,30);(65,30)"
%	 stroke-width= "0.5"
%	 />
%<multicurve fill-style= "none"
%	 points= "(65,30);(65,30);(65,35);(65,35)"
%	 stroke-width= "0.5"
%	 />
%<multicurve fill-style= "none"
%	 points= "(75,30);(75,30);(75,61.25);(75,61.25)"
%	 stroke-width= "0.5"
%	 />
%<multicurve fill-style= "none"
%	 points= "(60,47.5);(60,47.5);(70,47.5);(70,47.5)"
%	 stroke-width= "0.5"
%	 />
%<multicurve fill-style= "none"
%	 points= "(70,56.25);(70,56.25);(70,47.5);(70,47.5)"
%	 stroke-width= "0.5"
%	 />
%<multicurve fill-style= "none"
%	 points= "(65,56.25);(65,56.25);(65,61.25);(65,61.25)"
%	 stroke-width= "0.5"
%	 />
%<multicurve fill-style= "none"
%	 points= "(62.5,61.25);(62.5,61.25);(77.5,61.25);(77.5,61.25)"
%	 stroke-width= "0.5"
%	 />
%<multicurve fill-style= "none"
%	 points= "(62.5,76.25);(62.5,76.25);(62.5,61.25);(62.5,61.25)"
%	 stroke-width= "0.5"
%	 />
%<multicurve fill-style= "none"
%	 points= "(62.5,76.25);(62.5,76.25);(77.5,61.25);(77.5,61.25)"
%	 stroke-width= "0.5"
%	 />
%<multicurve fill-style= "none"
%	 points= "(70,80);(70,80);(70,68.75);(70,68.75)"
%	 stroke-width= "0.5"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "solid"
%	 anchor-point= "(50,30)"
%	 text-frame= "noframe"
%	 stroke-width= "0.5"
%	 text-hor-align= "center-h"
%	 >
%\EQLS
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "solid"
%	 anchor-point= "(65,38.75)"
%	 text-frame= "noframe"
%	 stroke-width= "0.5"
%	 text-hor-align= "center-h"
%	 >
%$\addd$
%</text>
%<multicurve fill-style= "none"
%	 points= "(65,6.25);(65,6.25);(70,1.25);(70,1.25)"
%	 stroke-width= "0.5"
%	 />
%<multicurve fill-style= "none"
%	 points= "(65,6.25);(65,6.25);(75,6.25);(75,6.25)"
%	 stroke-width= "0.5"
%	 />
%<multicurve fill-style= "none"
%	 points= "(75,6.25);(75,6.25);(70,1.25);(70,1.25)"
%	 stroke-width= "0.5"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "solid"
%	 anchor-point= "(65,51.25)"
%	 text-frame= "noframe"
%	 stroke-width= "0.5"
%	 text-hor-align= "center-h"
%	 >
%$\Homega$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "solid"
%	 anchor-point= "(67.5,65)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\png$
%</text>
%<ellipse p3= "(68.75,42.5)"
%	 fill-style= "none"
%	 p2= "(68.75,35)"
%	 p1= "(61.25,35)"
%	 closure= "open"
%	 angle-end= "360"
%	 stroke-width= "0.5"
%	 angle-start= "0"
%	 />
%<multicurve fill-style= "none"
%	 points= "(60,56.25);(60,56.25);(60,47.5);(60,47.5)"
%	 stroke-width= "0.5"
%	 />
%<multicurve fill-style= "none"
%	 points= "(60,56.25);(60,56.25);(70,56.25);(70,56.25)"
%	 stroke-width= "0.5"
%	 />
%<multicurve fill-style= "none"
%	 points= "(70,11.25);(70,11.25);(70,6.25);(70,6.25)"
%	 stroke-width= "0.5"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(70,3.75)"
%	 text-frame= "noframe"
%	 stroke-width= "1"
%	 text-hor-align= "center-h"
%	 >
%$\beeh$
%</text>
%<multicurve fill-style= "none"
%	 points= "(30,12.5);(30,12.5);(30,6.25);(30,6.25)"
%	 stroke-width= "0.5"
%	 />
%<multicurve fill-style= "none"
%	 points= "(25,26.25);(25,26.25);(35,26.25);(35,26.25)"
%	 stroke-width= "0.5"
%	 />
%<multicurve fill-style= "none"
%	 points= "(35,35);(35,35);(35,26.25);(35,26.25)"
%	 stroke-width= "0.5"
%	 />
%<multicurve fill-style= "none"
%	 points= "(30,35);(30,35);(30,40);(30,40)"
%	 stroke-width= "0.5"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "solid"
%	 anchor-point= "(30,30)"
%	 text-frame= "noframe"
%	 stroke-width= "0.5"
%	 text-hor-align= "center-h"
%	 >
%$\Homega$
%</text>
%<multicurve fill-style= "none"
%	 points= "(25,35);(25,35);(25,26.25);(25,26.25)"
%	 stroke-width= "0.5"
%	 />
%<multicurve fill-style= "none"
%	 points= "(25,35);(25,35);(35,35);(35,35)"
%	 stroke-width= "0.5"
%	 />
%<multicurve fill-style= "none"
%	 points= "(25,6.25);(25,6.25);(35,6.25);(35,6.25)"
%	 stroke-width= "0.5"
%	 />
%<multicurve fill-style= "none"
%	 points= "(35,6.25);(35,6.25);(30,1.25);(30,1.25)"
%	 stroke-width= "0.5"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(30,3.75)"
%	 text-frame= "noframe"
%	 stroke-width= "1"
%	 text-hor-align= "center-h"
%	 >
%$\beeh$
%</text>
%<multicurve fill-style= "none"
%	 points= "(25,6.25);(25,6.25);(30,1.25);(30,1.25)"
%	 stroke-width= "0.5"
%	 />
%<multicurve fill-style= "none"
%	 points= "(105,70);(105,70);(105,65);(105,65)"
%	 stroke-width= "0.5"
%	 />
%<ellipse p3= "(111.25,46.25)"
%	 fill-style= "solid"
%	 p2= "(111.25,48.75)"
%	 p1= "(108.75,48.75)"
%	 closure= "open"
%	 angle-end= "0"
%	 stroke-width= "0.5"
%	 angle-start= "0"
%	 />
%<multicurve fill-style= "none"
%	 points= "(115,52.5);(115,52.5);(110,47.5);(110,47.5)"
%	 stroke-width= "0.5"
%	 />
%<multicurve fill-style= "none"
%	 points= "(110,47.5);(110,47.5);(105,52.5);(105,52.5)"
%	 stroke-width= "0.5"
%	 />
%<multicurve fill-style= "none"
%	 points= "(105,52.5);(105,52.5);(105,57.5);(105,57.5)"
%	 stroke-width= "0.5"
%	 />
%<multicurve fill-style= "none"
%	 points= "(115,52.5);(115,52.5);(115,83.75);(115,83.75)"
%	 stroke-width= "0.5"
%	 />
%<multicurve fill-style= "none"
%	 points= "(100,70);(100,70);(110,70);(110,70)"
%	 stroke-width= "0.5"
%	 />
%<multicurve fill-style= "none"
%	 points= "(110,78.75);(110,78.75);(110,70);(110,70)"
%	 stroke-width= "0.5"
%	 />
%<multicurve fill-style= "none"
%	 points= "(105,78.75);(105,78.75);(105,83.75);(105,83.75)"
%	 stroke-width= "0.5"
%	 />
%<multicurve fill-style= "none"
%	 points= "(102.5,83.75);(102.5,83.75);(117.5,83.75);(117.5,83.75)"
%	 stroke-width= "0.5"
%	 />
%<multicurve fill-style= "none"
%	 points= "(102.5,98.75);(102.5,98.75);(102.5,83.75);(102.5,83.75)"
%	 stroke-width= "0.5"
%	 />
%<multicurve fill-style= "none"
%	 points= "(102.5,98.75);(102.5,98.75);(117.5,83.75);(117.5,83.75)"
%	 stroke-width= "0.5"
%	 />
%<multicurve fill-style= "none"
%	 points= "(110,102.5);(110,102.5);(110,91.25);(110,91.25)"
%	 stroke-width= "0.5"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "solid"
%	 anchor-point= "(105,61.25)"
%	 text-frame= "noframe"
%	 stroke-width= "0.5"
%	 text-hor-align= "center-h"
%	 >
%$\addd$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "solid"
%	 anchor-point= "(105,73.75)"
%	 text-frame= "noframe"
%	 stroke-width= "0.5"
%	 text-hor-align= "center-h"
%	 >
%$\Homega$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "solid"
%	 anchor-point= "(107.5,87.5)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\png$
%</text>
%<ellipse p3= "(108.75,65)"
%	 fill-style= "none"
%	 p2= "(108.75,57.5)"
%	 p1= "(101.25,57.5)"
%	 closure= "open"
%	 angle-end= "360"
%	 stroke-width= "0.5"
%	 angle-start= "0"
%	 />
%<multicurve fill-style= "none"
%	 points= "(100,78.75);(100,78.75);(100,70);(100,70)"
%	 stroke-width= "0.5"
%	 />
%<multicurve fill-style= "none"
%	 points= "(100,78.75);(100,78.75);(110,78.75);(110,78.75)"
%	 stroke-width= "0.5"
%	 />
%<multicurve fill-style= "none"
%	 points= "(110,47.5);(110,47.5);(110,42.5);(110,42.5)"
%	 stroke-width= "0.5"
%	 />
%<ellipse p3= "(116.25,23.75)"
%	 fill-style= "solid"
%	 p2= "(116.25,26.25)"
%	 p1= "(113.75,26.25)"
%	 closure= "open"
%	 angle-end= "0"
%	 stroke-width= "0.5"
%	 angle-start= "0"
%	 />
%<multicurve fill-style= "none"
%	 points= "(120,30);(120,30);(115,25);(115,25)"
%	 stroke-width= "0.5"
%	 />
%<multicurve fill-style= "none"
%	 points= "(115,25);(115,25);(110,30);(110,30)"
%	 stroke-width= "0.5"
%	 />
%<multicurve fill-style= "none"
%	 points= "(110,30);(110,30);(110,35);(110,35)"
%	 stroke-width= "0.5"
%	 />
%<multicurve fill-style= "none"
%	 points= "(120,30);(120,30);(120,102.5);(120,102.5)"
%	 stroke-width= "0.5"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "solid"
%	 anchor-point= "(110,38.75)"
%	 text-frame= "noframe"
%	 stroke-width= "0.5"
%	 text-hor-align= "center-h"
%	 >
%$\addd$
%</text>
%<ellipse p3= "(113.75,42.5)"
%	 fill-style= "none"
%	 p2= "(113.75,35)"
%	 p1= "(106.25,35)"
%	 closure= "open"
%	 angle-end= "360"
%	 stroke-width= "0.5"
%	 angle-start= "0"
%	 />
%<multicurve fill-style= "none"
%	 points= "(115,11.25);(115,11.25);(115,6.25);(115,6.25)"
%	 stroke-width= "0.5"
%	 />
%<multicurve fill-style= "none"
%	 points= "(110,6.25);(110,6.25);(120,6.25);(120,6.25)"
%	 stroke-width= "0.5"
%	 />
%<multicurve fill-style= "none"
%	 points= "(120,6.25);(120,6.25);(115,1.25);(115,1.25)"
%	 stroke-width= "0.5"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(115,3.75)"
%	 text-frame= "noframe"
%	 stroke-width= "1"
%	 text-hor-align= "center-h"
%	 >
%$\beeh$
%</text>
%<multicurve fill-style= "none"
%	 points= "(110,6.25);(110,6.25);(115,1.25);(115,1.25)"
%	 stroke-width= "0.5"
%	 />
%<multicurve fill-style= "none"
%	 points= "(107.5,102.5);(107.5,102.5);(122.5,102.5);(122.5,102.5)"
%	 stroke-width= "0.5"
%	 />
%<multicurve fill-style= "none"
%	 points= "(107.5,117.5);(107.5,117.5);(122.5,102.5);(122.5,102.5)"
%	 stroke-width= "0.5"
%	 />
%<multicurve fill-style= "none"
%	 points= "(115,121.25);(115,121.25);(115,110);(115,110)"
%	 stroke-width= "0.5"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "solid"
%	 anchor-point= "(112.5,106.25)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\png$
%</text>
%<multicurve fill-style= "none"
%	 points= "(107.5,117.5);(107.5,117.5);(107.5,102.5);(107.5,102.5)"
%	 stroke-width= "0.5"
%	 />
%<multicurve fill-style= "none"
%	 points= "(150,92.5);(150,92.5);(150,87.5);(150,87.5)"
%	 stroke-width= "0.5"
%	 />
%<ellipse p3= "(156.25,68.75)"
%	 fill-style= "solid"
%	 p2= "(156.25,71.25)"
%	 p1= "(153.75,71.25)"
%	 closure= "open"
%	 angle-end= "0"
%	 stroke-width= "0.5"
%	 angle-start= "0"
%	 />
%<multicurve fill-style= "none"
%	 points= "(160,75);(160,75);(155,70);(155,70)"
%	 stroke-width= "0.5"
%	 />
%<multicurve fill-style= "none"
%	 points= "(155,70);(155,70);(150,75);(150,75)"
%	 stroke-width= "0.5"
%	 />
%<multicurve fill-style= "none"
%	 points= "(150,75);(150,75);(150,80);(150,80)"
%	 stroke-width= "0.5"
%	 />
%<multicurve fill-style= "none"
%	 points= "(160,75);(160,75);(160,106.25);(160,106.25)"
%	 stroke-width= "0.5"
%	 />
%<multicurve fill-style= "none"
%	 points= "(145,92.5);(145,92.5);(155,92.5);(155,92.5)"
%	 stroke-width= "0.5"
%	 />
%<multicurve fill-style= "none"
%	 points= "(155,101.25);(155,101.25);(155,92.5);(155,92.5)"
%	 stroke-width= "0.5"
%	 />
%<multicurve fill-style= "none"
%	 points= "(150,101.25);(150,101.25);(150,106.25);(150,106.25)"
%	 stroke-width= "0.5"
%	 />
%<multicurve fill-style= "none"
%	 points= "(147.5,106.25);(147.5,106.25);(162.5,106.25);(162.5,106.25)"
%	 stroke-width= "0.5"
%	 />
%<multicurve fill-style= "none"
%	 points= "(147.5,121.25);(147.5,121.25);(147.5,106.25);(147.5,106.25)"
%	 stroke-width= "0.5"
%	 />
%<multicurve fill-style= "none"
%	 points= "(147.5,121.25);(147.5,121.25);(162.5,106.25);(162.5,106.25)"
%	 stroke-width= "0.5"
%	 />
%<multicurve fill-style= "none"
%	 points= "(155,125);(155,125);(155,113.75);(155,113.75)"
%	 stroke-width= "0.5"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "solid"
%	 anchor-point= "(150,83.75)"
%	 text-frame= "noframe"
%	 stroke-width= "0.5"
%	 text-hor-align= "center-h"
%	 >
%$\addd$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "solid"
%	 anchor-point= "(150,96.25)"
%	 text-frame= "noframe"
%	 stroke-width= "0.5"
%	 text-hor-align= "center-h"
%	 >
%$\Homega$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "solid"
%	 anchor-point= "(152.5,110)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\png$
%</text>
%<ellipse p3= "(153.75,87.5)"
%	 fill-style= "none"
%	 p2= "(153.75,80)"
%	 p1= "(146.25,80)"
%	 closure= "open"
%	 angle-end= "360"
%	 stroke-width= "0.5"
%	 angle-start= "0"
%	 />
%<multicurve fill-style= "none"
%	 points= "(145,101.25);(145,101.25);(145,92.5);(145,92.5)"
%	 stroke-width= "0.5"
%	 />
%<multicurve fill-style= "none"
%	 points= "(145,101.25);(145,101.25);(155,101.25);(155,101.25)"
%	 stroke-width= "0.5"
%	 />
%<multicurve fill-style= "none"
%	 points= "(155,70);(155,70);(155,65);(155,65)"
%	 stroke-width= "0.5"
%	 />
%<ellipse p3= "(161.25,46.25)"
%	 fill-style= "solid"
%	 p2= "(161.25,48.75)"
%	 p1= "(158.75,48.75)"
%	 closure= "open"
%	 angle-end= "0"
%	 stroke-width= "0.5"
%	 angle-start= "0"
%	 />
%<multicurve fill-style= "none"
%	 points= "(165,52.5);(165,52.5);(160,47.5);(160,47.5)"
%	 stroke-width= "0.5"
%	 />
%<multicurve fill-style= "none"
%	 points= "(160,47.5);(160,47.5);(155,52.5);(155,52.5)"
%	 stroke-width= "0.5"
%	 />
%<multicurve fill-style= "none"
%	 points= "(155,52.5);(155,52.5);(155,57.5);(155,57.5)"
%	 stroke-width= "0.5"
%	 />
%<multicurve fill-style= "none"
%	 points= "(165,52.5);(165,52.5);(165,125);(165,125)"
%	 stroke-width= "0.5"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "solid"
%	 anchor-point= "(155,61.25)"
%	 text-frame= "noframe"
%	 stroke-width= "0.5"
%	 text-hor-align= "center-h"
%	 >
%$\addd$
%</text>
%<ellipse p3= "(158.75,65)"
%	 fill-style= "none"
%	 p2= "(158.75,57.5)"
%	 p1= "(151.25,57.5)"
%	 closure= "open"
%	 angle-end= "360"
%	 stroke-width= "0.5"
%	 angle-start= "0"
%	 />
%<multicurve fill-style= "none"
%	 points= "(152.5,125);(152.5,125);(167.5,125);(167.5,125)"
%	 stroke-width= "0.5"
%	 />
%<multicurve fill-style= "none"
%	 points= "(152.5,140);(152.5,140);(167.5,125);(167.5,125)"
%	 stroke-width= "0.5"
%	 />
%<multicurve fill-style= "none"
%	 points= "(160,143.75);(160,143.75);(160,132.5);(160,132.5)"
%	 stroke-width= "0.5"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "solid"
%	 anchor-point= "(157.5,128.75)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\png$
%</text>
%<multicurve fill-style= "none"
%	 points= "(152.5,140);(152.5,140);(152.5,125);(152.5,125)"
%	 stroke-width= "0.5"
%	 />
%<multicurve fill-style= "none"
%	 points= "(160,47.5);(160,47.5);(160,42.5);(160,42.5)"
%	 stroke-width= "0.5"
%	 />
%<ellipse p3= "(166.25,23.75)"
%	 fill-style= "solid"
%	 p2= "(166.25,26.25)"
%	 p1= "(163.75,26.25)"
%	 closure= "open"
%	 angle-end= "0"
%	 stroke-width= "0.5"
%	 angle-start= "0"
%	 />
%<multicurve fill-style= "none"
%	 points= "(170,30);(170,30);(165,25);(165,25)"
%	 stroke-width= "0.5"
%	 />
%<multicurve fill-style= "none"
%	 points= "(165,25);(165,25);(160,30);(160,30)"
%	 stroke-width= "0.5"
%	 />
%<multicurve fill-style= "none"
%	 points= "(160,30);(160,30);(160,35);(160,35)"
%	 stroke-width= "0.5"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "solid"
%	 anchor-point= "(160,38.75)"
%	 text-frame= "noframe"
%	 stroke-width= "0.5"
%	 text-hor-align= "center-h"
%	 >
%$\addd$
%</text>
%<ellipse p3= "(163.75,42.5)"
%	 fill-style= "none"
%	 p2= "(163.75,35)"
%	 p1= "(156.25,35)"
%	 closure= "open"
%	 angle-end= "360"
%	 stroke-width= "0.5"
%	 angle-start= "0"
%	 />
%<multicurve fill-style= "none"
%	 points= "(165,11.25);(165,11.25);(165,6.25);(165,6.25)"
%	 stroke-width= "0.5"
%	 />
%<multicurve fill-style= "none"
%	 points= "(160,6.25);(160,6.25);(170,6.25);(170,6.25)"
%	 stroke-width= "0.5"
%	 />
%<multicurve fill-style= "none"
%	 points= "(170,6.25);(170,6.25);(165,1.25);(165,1.25)"
%	 stroke-width= "0.5"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(165,3.75)"
%	 text-frame= "noframe"
%	 stroke-width= "1"
%	 text-hor-align= "center-h"
%	 >
%$\beeh$
%</text>
%<multicurve fill-style= "none"
%	 points= "(160,6.25);(160,6.25);(165,1.25);(165,1.25)"
%	 stroke-width= "0.5"
%	 />
%<multicurve fill-style= "none"
%	 points= "(170,30);(170,30);(170,143.75);(170,143.75)"
%	 stroke-width= "0.5"
%	 />
%<multicurve fill-style= "none"
%	 points= "(157.5,143.75);(157.5,143.75);(172.5,143.75);(172.5,143.75)"
%	 stroke-width= "0.5"
%	 />
%<multicurve fill-style= "none"
%	 points= "(157.5,158.75);(157.5,158.75);(172.5,143.75);(172.5,143.75)"
%	 stroke-width= "0.5"
%	 />
%<multicurve fill-style= "none"
%	 points= "(165,162.5);(165,162.5);(165,151.25);(165,151.25)"
%	 stroke-width= "0.5"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "solid"
%	 anchor-point= "(162.5,147.5)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\png$
%</text>
%<multicurve fill-style= "none"
%	 points= "(157.5,158.75);(157.5,158.75);(157.5,143.75);(157.5,143.75)"
%	 stroke-width= "0.5"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "solid"
%	 anchor-point= "(90,30)"
%	 text-frame= "noframe"
%	 stroke-width= "0.5"
%	 text-hor-align= "center-h"
%	 >
%\EQLS
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "solid"
%	 anchor-point= "(135,30)"
%	 text-frame= "noframe"
%	 stroke-width= "0.5"
%	 text-hor-align= "center-h"
%	 >
%\EQLS
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "solid"
%	 anchor-point= "(185,30)"
%	 text-frame= "noframe"
%	 stroke-width= "0.5"
%	 text-hor-align= "center-h"
%	 >
%\EQLS
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(193.75,30)"
%	 text-frame= "noframe"
%	 stroke-width= "1"
%	 text-hor-align= "center-h"
%	 >
%$\cdots$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(0,30)"
%	 text-frame= "noframe"
%	 stroke-width= "1"
%	 text-hor-align= "center-h"
%	 >
%$\ordin$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "solid"
%	 anchor-point= "(13.75,30)"
%	 text-frame= "noframe"
%	 stroke-width= "0.5"
%	 text-hor-align= "center-h"
%	 >
%\EQLS
%</text>
%<multicurve fill-style= "none"
%	 points= "(25,12.5);(25,12.5);(35,12.5);(35,12.5)"
%	 stroke-width= "0.5"
%	 />
%<multicurve fill-style= "none"
%	 points= "(35,21.25);(35,21.25);(35,12.5);(35,12.5)"
%	 stroke-width= "0.5"
%	 />
%<multicurve fill-style= "none"
%	 points= "(30,21.25);(30,21.25);(30,26.25);(30,26.25)"
%	 stroke-width= "0.5"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "solid"
%	 anchor-point= "(30,16.25)"
%	 text-frame= "noframe"
%	 stroke-width= "0.5"
%	 text-hor-align= "center-h"
%	 >
%$\Homega$
%</text>
%<multicurve fill-style= "none"
%	 points= "(25,21.25);(25,21.25);(25,12.5);(25,12.5)"
%	 stroke-width= "0.5"
%	 />
%<multicurve fill-style= "none"
%	 points= "(25,21.25);(25,21.25);(35,21.25);(35,21.25)"
%	 stroke-width= "0.5"
%	 />
%<multicurve fill-style= "none"
%	 points= "(65,11.25);(65,11.25);(75,11.25);(75,11.25)"
%	 stroke-width= "0.5"
%	 />
%<multicurve fill-style= "none"
%	 points= "(75,20);(75,20);(75,11.25);(75,11.25)"
%	 stroke-width= "0.5"
%	 />
%<multicurve fill-style= "none"
%	 points= "(70,20);(70,20);(70,25);(70,25)"
%	 stroke-width= "0.5"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "solid"
%	 anchor-point= "(70,15)"
%	 text-frame= "noframe"
%	 stroke-width= "0.5"
%	 text-hor-align= "center-h"
%	 >
%$\Homega$
%</text>
%<multicurve fill-style= "none"
%	 points= "(65,20);(65,20);(65,11.25);(65,11.25)"
%	 stroke-width= "0.5"
%	 />
%<multicurve fill-style= "none"
%	 points= "(65,20);(65,20);(75,20);(75,20)"
%	 stroke-width= "0.5"
%	 />
%<multicurve fill-style= "none"
%	 points= "(110,11.25);(110,11.25);(120,11.25);(120,11.25)"
%	 stroke-width= "0.5"
%	 />
%<multicurve fill-style= "none"
%	 points= "(120,20);(120,20);(120,11.25);(120,11.25)"
%	 stroke-width= "0.5"
%	 />
%<multicurve fill-style= "none"
%	 points= "(115,20);(115,20);(115,25);(115,25)"
%	 stroke-width= "0.5"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "solid"
%	 anchor-point= "(115,15)"
%	 text-frame= "noframe"
%	 stroke-width= "0.5"
%	 text-hor-align= "center-h"
%	 >
%$\Homega$
%</text>
%<multicurve fill-style= "none"
%	 points= "(110,20);(110,20);(110,11.25);(110,11.25)"
%	 stroke-width= "0.5"
%	 />
%<multicurve fill-style= "none"
%	 points= "(110,20);(110,20);(120,20);(120,20)"
%	 stroke-width= "0.5"
%	 />
%<multicurve fill-style= "none"
%	 points= "(160,11.25);(160,11.25);(170,11.25);(170,11.25)"
%	 stroke-width= "0.5"
%	 />
%<multicurve fill-style= "none"
%	 points= "(170,20);(170,20);(170,11.25);(170,11.25)"
%	 stroke-width= "0.5"
%	 />
%<multicurve fill-style= "none"
%	 points= "(165,20);(165,20);(165,25);(165,25)"
%	 stroke-width= "0.5"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "solid"
%	 anchor-point= "(165,15)"
%	 text-frame= "noframe"
%	 stroke-width= "0.5"
%	 text-hor-align= "center-h"
%	 >
%$\Homega$
%</text>
%<multicurve fill-style= "none"
%	 points= "(160,20);(160,20);(160,11.25);(160,11.25)"
%	 stroke-width= "0.5"
%	 />
%<multicurve fill-style= "none"
%	 points= "(160,20);(160,20);(170,20);(170,20)"
%	 stroke-width= "0.5"
%	 />
%</jpic>
%%End JPIC-XML
%PSTricks content-type (pstricks.sty package needed)
%Add \usepackage{pstricks} in the preamble of your LaTeX file
%You can rescale the whole picture (to 80% for instance) by using the command \def\JPicScale{0.8}
\ifx\JPicScale\undefined\def\JPicScale{1}\fi
\psset{unit=\JPicScale mm}
\psset{linewidth=0.3,dotsep=1,hatchwidth=0.3,hatchsep=1.5,shadowsize=1,dimen=middle}
\psset{dotsize=0.7 2.5,dotscale=1 1,fillcolor=black}
\psset{arrowsize=1 2,arrowlength=1,arrowinset=0.25,tbarsize=0.7 5,bracketlength=0.15,rbracketlength=0.15}
\begin{pspicture}(0,0)(193.75,162.5)
\psline[linewidth=0.5](65,47.5)(65,42.5)
\rput{0}(70,25){\psellipse[linewidth=0.5,fillstyle=solid](0,0)(1.25,-1.25)}
\psline[linewidth=0.5](75,30)(70,25)
\psline[linewidth=0.5](70,25)(65,30)
\psline[linewidth=0.5](65,30)(65,35)
\psline[linewidth=0.5](75,30)(75,61.25)
\psline[linewidth=0.5](60,47.5)(70,47.5)
\psline[linewidth=0.5](70,56.25)(70,47.5)
\psline[linewidth=0.5](65,56.25)(65,61.25)
\psline[linewidth=0.5](62.5,61.25)(77.5,61.25)
\psline[linewidth=0.5](62.5,76.25)(62.5,61.25)
\psline[linewidth=0.5](62.5,76.25)(77.5,61.25)
\psline[linewidth=0.5](70,80)(70,68.75)
\rput(50,30){\EQLS}
\rput(65,38.75){$\addd$}
\psline[linewidth=0.5](65,6.25)(70,1.25)
\psline[linewidth=0.5](65,6.25)(75,6.25)
\psline[linewidth=0.5](75,6.25)(70,1.25)
\rput(65,51.25){$\Homega$}
\rput(67.5,65){$\png$}
\rput{0}(65,38.75){\psellipse[linewidth=0.5](0,0)(3.75,3.75)}
\psline[linewidth=0.5](60,56.25)(60,47.5)
\psline[linewidth=0.5](60,56.25)(70,56.25)
\psline[linewidth=0.5](70,11.25)(70,6.25)
\rput(70,3.75){$\beeh$}
\psline[linewidth=0.5](30,12.5)(30,6.25)
\psline[linewidth=0.5](25,26.25)(35,26.25)
\psline[linewidth=0.5](35,35)(35,26.25)
\psline[linewidth=0.5](30,35)(30,40)
\rput(30,30){$\Homega$}
\psline[linewidth=0.5](25,35)(25,26.25)
\psline[linewidth=0.5](25,35)(35,35)
\psline[linewidth=0.5](25,6.25)(35,6.25)
\psline[linewidth=0.5](35,6.25)(30,1.25)
\rput(30,3.75){$\beeh$}
\psline[linewidth=0.5](25,6.25)(30,1.25)
\psline[linewidth=0.5](105,70)(105,65)
\rput{0}(110,47.5){\psellipse[linewidth=0.5,fillstyle=solid](0,0)(1.25,-1.25)}
\psline[linewidth=0.5](115,52.5)(110,47.5)
\psline[linewidth=0.5](110,47.5)(105,52.5)
\psline[linewidth=0.5](105,52.5)(105,57.5)
\psline[linewidth=0.5](115,52.5)(115,83.75)
\psline[linewidth=0.5](100,70)(110,70)
\psline[linewidth=0.5](110,78.75)(110,70)
\psline[linewidth=0.5](105,78.75)(105,83.75)
\psline[linewidth=0.5](102.5,83.75)(117.5,83.75)
\psline[linewidth=0.5](102.5,98.75)(102.5,83.75)
\psline[linewidth=0.5](102.5,98.75)(117.5,83.75)
\psline[linewidth=0.5](110,102.5)(110,91.25)
\rput(105,61.25){$\addd$}
\rput(105,73.75){$\Homega$}
\rput(107.5,87.5){$\png$}
\rput{0}(105,61.25){\psellipse[linewidth=0.5](0,0)(3.75,3.75)}
\psline[linewidth=0.5](100,78.75)(100,70)
\psline[linewidth=0.5](100,78.75)(110,78.75)
\psline[linewidth=0.5](110,47.5)(110,42.5)
\rput{0}(115,25){\psellipse[linewidth=0.5,fillstyle=solid](0,0)(1.25,-1.25)}
\psline[linewidth=0.5](120,30)(115,25)
\psline[linewidth=0.5](115,25)(110,30)
\psline[linewidth=0.5](110,30)(110,35)
\psline[linewidth=0.5](120,30)(120,102.5)
\rput(110,38.75){$\addd$}
\rput{0}(110,38.75){\psellipse[linewidth=0.5](0,0)(3.75,3.75)}
\psline[linewidth=0.5](115,11.25)(115,6.25)
\psline[linewidth=0.5](110,6.25)(120,6.25)
\psline[linewidth=0.5](120,6.25)(115,1.25)
\rput(115,3.75){$\beeh$}
\psline[linewidth=0.5](110,6.25)(115,1.25)
\psline[linewidth=0.5](107.5,102.5)(122.5,102.5)
\psline[linewidth=0.5](107.5,117.5)(122.5,102.5)
\psline[linewidth=0.5](115,121.25)(115,110)
\rput(112.5,106.25){$\png$}
\psline[linewidth=0.5](107.5,117.5)(107.5,102.5)
\psline[linewidth=0.5](150,92.5)(150,87.5)
\rput{0}(155,70){\psellipse[linewidth=0.5,fillstyle=solid](0,0)(1.25,-1.25)}
\psline[linewidth=0.5](160,75)(155,70)
\psline[linewidth=0.5](155,70)(150,75)
\psline[linewidth=0.5](150,75)(150,80)
\psline[linewidth=0.5](160,75)(160,106.25)
\psline[linewidth=0.5](145,92.5)(155,92.5)
\psline[linewidth=0.5](155,101.25)(155,92.5)
\psline[linewidth=0.5](150,101.25)(150,106.25)
\psline[linewidth=0.5](147.5,106.25)(162.5,106.25)
\psline[linewidth=0.5](147.5,121.25)(147.5,106.25)
\psline[linewidth=0.5](147.5,121.25)(162.5,106.25)
\psline[linewidth=0.5](155,125)(155,113.75)
\rput(150,83.75){$\addd$}
\rput(150,96.25){$\Homega$}
\rput(152.5,110){$\png$}
\rput{0}(150,83.75){\psellipse[linewidth=0.5](0,0)(3.75,3.75)}
\psline[linewidth=0.5](145,101.25)(145,92.5)
\psline[linewidth=0.5](145,101.25)(155,101.25)
\psline[linewidth=0.5](155,70)(155,65)
\rput{0}(160,47.5){\psellipse[linewidth=0.5,fillstyle=solid](0,0)(1.25,-1.25)}
\psline[linewidth=0.5](165,52.5)(160,47.5)
\psline[linewidth=0.5](160,47.5)(155,52.5)
\psline[linewidth=0.5](155,52.5)(155,57.5)
\psline[linewidth=0.5](165,52.5)(165,125)
\rput(155,61.25){$\addd$}
\rput{0}(155,61.25){\psellipse[linewidth=0.5](0,0)(3.75,3.75)}
\psline[linewidth=0.5](152.5,125)(167.5,125)
\psline[linewidth=0.5](152.5,140)(167.5,125)
\psline[linewidth=0.5](160,143.75)(160,132.5)
\rput(157.5,128.75){$\png$}
\psline[linewidth=0.5](152.5,140)(152.5,125)
\psline[linewidth=0.5](160,47.5)(160,42.5)
\rput{0}(165,25){\psellipse[linewidth=0.5,fillstyle=solid](0,0)(1.25,-1.25)}
\psline[linewidth=0.5](170,30)(165,25)
\psline[linewidth=0.5](165,25)(160,30)
\psline[linewidth=0.5](160,30)(160,35)
\rput(160,38.75){$\addd$}
\rput{0}(160,38.75){\psellipse[linewidth=0.5](0,0)(3.75,3.75)}
\psline[linewidth=0.5](165,11.25)(165,6.25)
\psline[linewidth=0.5](160,6.25)(170,6.25)
\psline[linewidth=0.5](170,6.25)(165,1.25)
\rput(165,3.75){$\beeh$}
\psline[linewidth=0.5](160,6.25)(165,1.25)
\psline[linewidth=0.5](170,30)(170,143.75)
\psline[linewidth=0.5](157.5,143.75)(172.5,143.75)
\psline[linewidth=0.5](157.5,158.75)(172.5,143.75)
\psline[linewidth=0.5](165,162.5)(165,151.25)
\rput(162.5,147.5){$\png$}
\psline[linewidth=0.5](157.5,158.75)(157.5,143.75)
\rput(90,30){\EQLS}
\rput(135,30){\EQLS}
\rput(185,30){\EQLS}
\rput(193.75,30){$\cdots$}
\rput(0,30){$\ordin$}
\rput(13.75,30){\EQLS}
\psline[linewidth=0.5](25,12.5)(35,12.5)
\psline[linewidth=0.5](35,21.25)(35,12.5)
\psline[linewidth=0.5](30,21.25)(30,26.25)
\rput(30,16.25){$\Homega$}
\psline[linewidth=0.5](25,21.25)(25,12.5)
\psline[linewidth=0.5](25,21.25)(35,21.25)
\psline[linewidth=0.5](65,11.25)(75,11.25)
\psline[linewidth=0.5](75,20)(75,11.25)
\psline[linewidth=0.5](70,20)(70,25)
\rput(70,15){$\Homega$}
\psline[linewidth=0.5](65,20)(65,11.25)
\psline[linewidth=0.5](65,20)(75,20)
\psline[linewidth=0.5](110,11.25)(120,11.25)
\psline[linewidth=0.5](120,20)(120,11.25)
\psline[linewidth=0.5](115,20)(115,25)
\rput(115,15){$\Homega$}
\psline[linewidth=0.5](110,20)(110,11.25)
\psline[linewidth=0.5](110,20)(120,20)
\psline[linewidth=0.5](160,11.25)(170,11.25)
\psline[linewidth=0.5](170,20)(170,11.25)
\psline[linewidth=0.5](165,20)(165,25)
\rput(165,15){$\Homega$}
\psline[linewidth=0.5](160,20)(160,11.25)
\psline[linewidth=0.5](160,20)(170,20)
\end{pspicture}


==> PIC/Omega-times.tex <==
%%Created by jPicEdt 1.4.1_03: mixed JPIC-XML/LaTeX format
%%Thu Feb 25 21:56:06 GMT-10:00 2021
%%Begin JPIC-XML
%<?xml version="1.0" standalone="yes"?>
%<jpic x-min="0" x-max="193.75" y-min="1.25" y-max="148.75" auto-bounding="true">
%<multicurve fill-style= "none"
%	 points= "(65,33.75);(65,33.75);(65,30);(65,30)"
%	 stroke-width= "0.5"
%	 />
%<ellipse p3= "(71.25,10)"
%	 fill-style= "solid"
%	 p2= "(71.25,12.5)"
%	 p1= "(68.75,12.5)"
%	 closure= "open"
%	 angle-end= "0"
%	 stroke-width= "0.5"
%	 angle-start= "0"
%	 />
%<multicurve fill-style= "none"
%	 points= "(75,16.25);(75,16.25);(70,11.25);(70,11.25)"
%	 stroke-width= "0.5"
%	 />
%<multicurve fill-style= "none"
%	 points= "(70,11.25);(70,11.25);(65,16.25);(65,16.25)"
%	 stroke-width= "0.5"
%	 />
%<multicurve fill-style= "none"
%	 points= "(65,16.25);(65,16.25);(65,21.25);(65,21.25)"
%	 stroke-width= "0.5"
%	 />
%<multicurve fill-style= "none"
%	 points= "(75,16.25);(75,16.25);(75,47.5);(75,47.5)"
%	 stroke-width= "0.5"
%	 />
%<multicurve fill-style= "none"
%	 points= "(60,33.75);(60,33.75);(70,33.75);(70,33.75)"
%	 stroke-width= "0.5"
%	 />
%<multicurve fill-style= "none"
%	 points= "(70,42.5);(70,42.5);(70,33.75);(70,33.75)"
%	 stroke-width= "0.5"
%	 />
%<multicurve fill-style= "none"
%	 points= "(65,42.5);(65,42.5);(65,47.5);(65,47.5)"
%	 stroke-width= "0.5"
%	 />
%<multicurve fill-style= "none"
%	 points= "(62.5,47.5);(62.5,47.5);(77.5,47.5);(77.5,47.5)"
%	 stroke-width= "0.5"
%	 />
%<multicurve fill-style= "none"
%	 points= "(62.5,62.5);(62.5,62.5);(62.5,47.5);(62.5,47.5)"
%	 stroke-width= "0.5"
%	 />
%<multicurve fill-style= "none"
%	 points= "(62.5,62.5);(62.5,62.5);(77.5,47.5);(77.5,47.5)"
%	 stroke-width= "0.5"
%	 />
%<multicurve fill-style= "none"
%	 points= "(70,66.25);(70,66.25);(70,55);(70,55)"
%	 stroke-width= "0.5"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "solid"
%	 anchor-point= "(50,16.25)"
%	 text-frame= "noframe"
%	 stroke-width= "0.5"
%	 text-hor-align= "center-h"
%	 >
%\EQLS
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "solid"
%	 anchor-point= "(65,25.62)"
%	 text-frame= "noframe"
%	 stroke-width= "0.5"
%	 text-hor-align= "center-h"
%	 >
%$\addd$
%</text>
%<multicurve fill-style= "none"
%	 points= "(65,6.25);(65,6.25);(70,1.25);(70,1.25)"
%	 stroke-width= "0.5"
%	 />
%<multicurve fill-style= "none"
%	 points= "(65,6.25);(65,6.25);(75,6.25);(75,6.25)"
%	 stroke-width= "0.5"
%	 />
%<multicurve fill-style= "none"
%	 points= "(75,6.25);(75,6.25);(70,1.25);(70,1.25)"
%	 stroke-width= "0.5"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "solid"
%	 anchor-point= "(65,37.5)"
%	 text-frame= "noframe"
%	 stroke-width= "0.5"
%	 text-hor-align= "center-h"
%	 >
%$\Homega$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "solid"
%	 anchor-point= "(67.5,51.25)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\png$
%</text>
%<multicurve fill-style= "none"
%	 points= "(60,42.5);(60,42.5);(60,33.75);(60,33.75)"
%	 stroke-width= "0.5"
%	 />
%<multicurve fill-style= "none"
%	 points= "(60,42.5);(60,42.5);(70,42.5);(70,42.5)"
%	 stroke-width= "0.5"
%	 />
%<multicurve fill-style= "none"
%	 points= "(70,11.25);(70,11.25);(70,6.25);(70,6.25)"
%	 stroke-width= "0.5"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(70,3.75)"
%	 text-frame= "noframe"
%	 stroke-width= "1"
%	 text-hor-align= "center-h"
%	 >
%$\beeh$
%</text>
%<multicurve fill-style= "none"
%	 points= "(30,11.25);(30,11.25);(30,6.25);(30,6.25)"
%	 stroke-width= "0.5"
%	 />
%<multicurve fill-style= "none"
%	 points= "(60,21.25);(60,21.25);(70,21.25);(70,21.25)"
%	 stroke-width= "0.5"
%	 />
%<multicurve fill-style= "none"
%	 points= "(70,30);(70,30);(70,21.25);(70,21.25)"
%	 stroke-width= "0.5"
%	 />
%<multicurve fill-style= "none"
%	 points= "(60,30);(60,30);(60,21.25);(60,21.25)"
%	 stroke-width= "0.5"
%	 />
%<multicurve fill-style= "none"
%	 points= "(60,30);(60,30);(70,30);(70,30)"
%	 stroke-width= "0.5"
%	 />
%<multicurve fill-style= "none"
%	 points= "(25,6.25);(25,6.25);(35,6.25);(35,6.25)"
%	 stroke-width= "0.5"
%	 />
%<multicurve fill-style= "none"
%	 points= "(35,6.25);(35,6.25);(30,1.25);(30,1.25)"
%	 stroke-width= "0.5"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(30,3.75)"
%	 text-frame= "noframe"
%	 stroke-width= "1"
%	 text-hor-align= "center-h"
%	 >
%$\beeh$
%</text>
%<multicurve fill-style= "none"
%	 points= "(25,6.25);(25,6.25);(30,1.25);(30,1.25)"
%	 stroke-width= "0.5"
%	 />
%<multicurve fill-style= "none"
%	 points= "(105,56.25);(105,56.25);(105,52.5);(105,52.5)"
%	 stroke-width= "0.5"
%	 />
%<ellipse p3= "(111.25,32.5)"
%	 fill-style= "solid"
%	 p2= "(111.25,35)"
%	 p1= "(108.75,35)"
%	 closure= "open"
%	 angle-end= "0"
%	 stroke-width= "0.5"
%	 angle-start= "0"
%	 />
%<multicurve fill-style= "none"
%	 points= "(115,38.75);(115,38.75);(110,33.75);(110,33.75)"
%	 stroke-width= "0.5"
%	 />
%<multicurve fill-style= "none"
%	 points= "(110,33.75);(110,33.75);(105,38.75);(105,38.75)"
%	 stroke-width= "0.5"
%	 />
%<multicurve fill-style= "none"
%	 points= "(105,38.75);(105,38.75);(105,43.75);(105,43.75)"
%	 stroke-width= "0.5"
%	 />
%<multicurve fill-style= "none"
%	 points= "(115,38.75);(115,38.75);(115,70);(115,70)"
%	 stroke-width= "0.5"
%	 />
%<multicurve fill-style= "none"
%	 points= "(100,56.25);(100,56.25);(110,56.25);(110,56.25)"
%	 stroke-width= "0.5"
%	 />
%<multicurve fill-style= "none"
%	 points= "(110,65);(110,65);(110,56.25);(110,56.25)"
%	 stroke-width= "0.5"
%	 />
%<multicurve fill-style= "none"
%	 points= "(105,65);(105,65);(105,70);(105,70)"
%	 stroke-width= "0.5"
%	 />
%<multicurve fill-style= "none"
%	 points= "(102.5,70);(102.5,70);(117.5,70);(117.5,70)"
%	 stroke-width= "0.5"
%	 />
%<multicurve fill-style= "none"
%	 points= "(102.5,85);(102.5,85);(102.5,70);(102.5,70)"
%	 stroke-width= "0.5"
%	 />
%<multicurve fill-style= "none"
%	 points= "(102.5,85);(102.5,85);(117.5,70);(117.5,70)"
%	 stroke-width= "0.5"
%	 />
%<multicurve fill-style= "none"
%	 points= "(110,88.75);(110,88.75);(110,77.5);(110,77.5)"
%	 stroke-width= "0.5"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "solid"
%	 anchor-point= "(105,48.12)"
%	 text-frame= "noframe"
%	 stroke-width= "0.5"
%	 text-hor-align= "center-h"
%	 >
%$\addd$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "solid"
%	 anchor-point= "(105,60)"
%	 text-frame= "noframe"
%	 stroke-width= "0.5"
%	 text-hor-align= "center-h"
%	 >
%$\Homega$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "solid"
%	 anchor-point= "(107.5,73.75)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\png$
%</text>
%<multicurve fill-style= "none"
%	 points= "(100,65);(100,65);(100,56.25);(100,56.25)"
%	 stroke-width= "0.5"
%	 />
%<multicurve fill-style= "none"
%	 points= "(100,65);(100,65);(110,65);(110,65)"
%	 stroke-width= "0.5"
%	 />
%<multicurve fill-style= "none"
%	 points= "(110,33.75);(110,33.75);(110,30);(110,30)"
%	 stroke-width= "0.5"
%	 />
%<ellipse p3= "(116.25,10)"
%	 fill-style= "solid"
%	 p2= "(116.25,12.5)"
%	 p1= "(113.75,12.5)"
%	 closure= "open"
%	 angle-end= "0"
%	 stroke-width= "0.5"
%	 angle-start= "0"
%	 />
%<multicurve fill-style= "none"
%	 points= "(120,16.25);(120,16.25);(115,11.25);(115,11.25)"
%	 stroke-width= "0.5"
%	 />
%<multicurve fill-style= "none"
%	 points= "(115,11.25);(115,11.25);(110,16.25);(110,16.25)"
%	 stroke-width= "0.5"
%	 />
%<multicurve fill-style= "none"
%	 points= "(110,16.25);(110,16.25);(110,21.25);(110,21.25)"
%	 stroke-width= "0.5"
%	 />
%<multicurve fill-style= "none"
%	 points= "(120,16.25);(120,16.25);(120,88.75);(120,88.75)"
%	 stroke-width= "0.5"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "solid"
%	 anchor-point= "(110,25.62)"
%	 text-frame= "noframe"
%	 stroke-width= "0.5"
%	 text-hor-align= "center-h"
%	 >
%$\addd$
%</text>
%<multicurve fill-style= "none"
%	 points= "(115,11.25);(115,11.25);(115,6.25);(115,6.25)"
%	 stroke-width= "0.5"
%	 />
%<multicurve fill-style= "none"
%	 points= "(110,6.25);(110,6.25);(120,6.25);(120,6.25)"
%	 stroke-width= "0.5"
%	 />
%<multicurve fill-style= "none"
%	 points= "(120,6.25);(120,6.25);(115,1.25);(115,1.25)"
%	 stroke-width= "0.5"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(115,3.75)"
%	 text-frame= "noframe"
%	 stroke-width= "1"
%	 text-hor-align= "center-h"
%	 >
%$\beeh$
%</text>
%<multicurve fill-style= "none"
%	 points= "(110,6.25);(110,6.25);(115,1.25);(115,1.25)"
%	 stroke-width= "0.5"
%	 />
%<multicurve fill-style= "none"
%	 points= "(107.5,88.75);(107.5,88.75);(122.5,88.75);(122.5,88.75)"
%	 stroke-width= "0.5"
%	 />
%<multicurve fill-style= "none"
%	 points= "(107.5,103.75);(107.5,103.75);(122.5,88.75);(122.5,88.75)"
%	 stroke-width= "0.5"
%	 />
%<multicurve fill-style= "none"
%	 points= "(115,107.5);(115,107.5);(115,96.25);(115,96.25)"
%	 stroke-width= "0.5"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "solid"
%	 anchor-point= "(112.5,92.5)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\png$
%</text>
%<multicurve fill-style= "none"
%	 points= "(107.5,103.75);(107.5,103.75);(107.5,88.75);(107.5,88.75)"
%	 stroke-width= "0.5"
%	 />
%<multicurve fill-style= "none"
%	 points= "(150,78.75);(150,78.75);(150,75);(150,75)"
%	 stroke-width= "0.5"
%	 />
%<ellipse p3= "(156.25,55)"
%	 fill-style= "solid"
%	 p2= "(156.25,57.5)"
%	 p1= "(153.75,57.5)"
%	 closure= "open"
%	 angle-end= "0"
%	 stroke-width= "0.5"
%	 angle-start= "0"
%	 />
%<multicurve fill-style= "none"
%	 points= "(160,61.25);(160,61.25);(155,56.25);(155,56.25)"
%	 stroke-width= "0.5"
%	 />
%<multicurve fill-style= "none"
%	 points= "(155,56.25);(155,56.25);(150,61.25);(150,61.25)"
%	 stroke-width= "0.5"
%	 />
%<multicurve fill-style= "none"
%	 points= "(150,61.25);(150,61.25);(150,66.25);(150,66.25)"
%	 stroke-width= "0.5"
%	 />
%<multicurve fill-style= "none"
%	 points= "(160,61.25);(160,61.25);(160,92.5);(160,92.5)"
%	 stroke-width= "0.5"
%	 />
%<multicurve fill-style= "none"
%	 points= "(145,78.75);(145,78.75);(155,78.75);(155,78.75)"
%	 stroke-width= "0.5"
%	 />
%<multicurve fill-style= "none"
%	 points= "(155,87.5);(155,87.5);(155,78.75);(155,78.75)"
%	 stroke-width= "0.5"
%	 />
%<multicurve fill-style= "none"
%	 points= "(150,87.5);(150,87.5);(150,92.5);(150,92.5)"
%	 stroke-width= "0.5"
%	 />
%<multicurve fill-style= "none"
%	 points= "(147.5,92.5);(147.5,92.5);(162.5,92.5);(162.5,92.5)"
%	 stroke-width= "0.5"
%	 />
%<multicurve fill-style= "none"
%	 points= "(147.5,107.5);(147.5,107.5);(147.5,92.5);(147.5,92.5)"
%	 stroke-width= "0.5"
%	 />
%<multicurve fill-style= "none"
%	 points= "(147.5,107.5);(147.5,107.5);(162.5,92.5);(162.5,92.5)"
%	 stroke-width= "0.5"
%	 />
%<multicurve fill-style= "none"
%	 points= "(155,111.25);(155,111.25);(155,100);(155,100)"
%	 stroke-width= "0.5"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "solid"
%	 anchor-point= "(150,70.62)"
%	 text-frame= "noframe"
%	 stroke-width= "0.5"
%	 text-hor-align= "center-h"
%	 >
%$\addd$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "solid"
%	 anchor-point= "(150,82.5)"
%	 text-frame= "noframe"
%	 stroke-width= "0.5"
%	 text-hor-align= "center-h"
%	 >
%$\Homega$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "solid"
%	 anchor-point= "(152.5,96.25)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\png$
%</text>
%<multicurve fill-style= "none"
%	 points= "(145,87.5);(145,87.5);(145,78.75);(145,78.75)"
%	 stroke-width= "0.5"
%	 />
%<multicurve fill-style= "none"
%	 points= "(145,87.5);(145,87.5);(155,87.5);(155,87.5)"
%	 stroke-width= "0.5"
%	 />
%<multicurve fill-style= "none"
%	 points= "(155,56.25);(155,56.25);(155,52.5);(155,52.5)"
%	 stroke-width= "0.5"
%	 />
%<ellipse p3= "(161.25,32.5)"
%	 fill-style= "solid"
%	 p2= "(161.25,35)"
%	 p1= "(158.75,35)"
%	 closure= "open"
%	 angle-end= "0"
%	 stroke-width= "0.5"
%	 angle-start= "0"
%	 />
%<multicurve fill-style= "none"
%	 points= "(165,38.75);(165,38.75);(160,33.75);(160,33.75)"
%	 stroke-width= "0.5"
%	 />
%<multicurve fill-style= "none"
%	 points= "(160,33.75);(160,33.75);(155,38.75);(155,38.75)"
%	 stroke-width= "0.5"
%	 />
%<multicurve fill-style= "none"
%	 points= "(155,38.75);(155,38.75);(155,43.75);(155,43.75)"
%	 stroke-width= "0.5"
%	 />
%<multicurve fill-style= "none"
%	 points= "(165,38.75);(165,38.75);(165,111.25);(165,111.25)"
%	 stroke-width= "0.5"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "solid"
%	 anchor-point= "(155,48.12)"
%	 text-frame= "noframe"
%	 stroke-width= "0.5"
%	 text-hor-align= "center-h"
%	 >
%$\addd$
%</text>
%<multicurve fill-style= "none"
%	 points= "(152.5,111.25);(152.5,111.25);(167.5,111.25);(167.5,111.25)"
%	 stroke-width= "0.5"
%	 />
%<multicurve fill-style= "none"
%	 points= "(152.5,126.25);(152.5,126.25);(167.5,111.25);(167.5,111.25)"
%	 stroke-width= "0.5"
%	 />
%<multicurve fill-style= "none"
%	 points= "(160,130);(160,130);(160,118.75);(160,118.75)"
%	 stroke-width= "0.5"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "solid"
%	 anchor-point= "(157.5,115)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\png$
%</text>
%<multicurve fill-style= "none"
%	 points= "(152.5,126.25);(152.5,126.25);(152.5,111.25);(152.5,111.25)"
%	 stroke-width= "0.5"
%	 />
%<multicurve fill-style= "none"
%	 points= "(160,33.75);(160,33.75);(160,30);(160,30)"
%	 stroke-width= "0.5"
%	 />
%<ellipse p3= "(166.25,10)"
%	 fill-style= "solid"
%	 p2= "(166.25,12.5)"
%	 p1= "(163.75,12.5)"
%	 closure= "open"
%	 angle-end= "0"
%	 stroke-width= "0.5"
%	 angle-start= "0"
%	 />
%<multicurve fill-style= "none"
%	 points= "(170,16.25);(170,16.25);(165,11.25);(165,11.25)"
%	 stroke-width= "0.5"
%	 />
%<multicurve fill-style= "none"
%	 points= "(165,11.25);(165,11.25);(160,16.25);(160,16.25)"
%	 stroke-width= "0.5"
%	 />
%<multicurve fill-style= "none"
%	 points= "(160,16.25);(160,16.25);(160,21.25);(160,21.25)"
%	 stroke-width= "0.5"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "solid"
%	 anchor-point= "(160,25.62)"
%	 text-frame= "noframe"
%	 stroke-width= "0.5"
%	 text-hor-align= "center-h"
%	 >
%$\addd$
%</text>
%<multicurve fill-style= "none"
%	 points= "(165,11.25);(165,11.25);(165,6.25);(165,6.25)"
%	 stroke-width= "0.5"
%	 />
%<multicurve fill-style= "none"
%	 points= "(160,6.25);(160,6.25);(170,6.25);(170,6.25)"
%	 stroke-width= "0.5"
%	 />
%<multicurve fill-style= "none"
%	 points= "(170,6.25);(170,6.25);(165,1.25);(165,1.25)"
%	 stroke-width= "0.5"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(165,3.75)"
%	 text-frame= "noframe"
%	 stroke-width= "1"
%	 text-hor-align= "center-h"
%	 >
%$\beeh$
%</text>
%<multicurve fill-style= "none"
%	 points= "(160,6.25);(160,6.25);(165,1.25);(165,1.25)"
%	 stroke-width= "0.5"
%	 />
%<multicurve fill-style= "none"
%	 points= "(170,16.25);(170,16.25);(170,130);(170,130)"
%	 stroke-width= "0.5"
%	 />
%<multicurve fill-style= "none"
%	 points= "(157.5,130);(157.5,130);(172.5,130);(172.5,130)"
%	 stroke-width= "0.5"
%	 />
%<multicurve fill-style= "none"
%	 points= "(157.5,145);(157.5,145);(172.5,130);(172.5,130)"
%	 stroke-width= "0.5"
%	 />
%<multicurve fill-style= "none"
%	 points= "(165,148.75);(165,148.75);(165,137.5);(165,137.5)"
%	 stroke-width= "0.5"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "solid"
%	 anchor-point= "(162.5,133.75)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\png$
%</text>
%<multicurve fill-style= "none"
%	 points= "(157.5,145);(157.5,145);(157.5,130);(157.5,130)"
%	 stroke-width= "0.5"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "solid"
%	 anchor-point= "(90,16.25)"
%	 text-frame= "noframe"
%	 stroke-width= "0.5"
%	 text-hor-align= "center-h"
%	 >
%\EQLS
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "solid"
%	 anchor-point= "(135,16.25)"
%	 text-frame= "noframe"
%	 stroke-width= "0.5"
%	 text-hor-align= "center-h"
%	 >
%\EQLS
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "solid"
%	 anchor-point= "(185,16.25)"
%	 text-frame= "noframe"
%	 stroke-width= "0.5"
%	 text-hor-align= "center-h"
%	 >
%\EQLS
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(193.75,16.25)"
%	 text-frame= "noframe"
%	 stroke-width= "1"
%	 text-hor-align= "center-h"
%	 >
%$\cdots$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(0,16.25)"
%	 text-frame= "noframe"
%	 stroke-width= "1"
%	 text-hor-align= "center-h"
%	 >
%$\ordin$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "solid"
%	 anchor-point= "(13.75,16.25)"
%	 text-frame= "noframe"
%	 stroke-width= "0.5"
%	 text-hor-align= "center-h"
%	 >
%\EQLS
%</text>
%<multicurve fill-style= "none"
%	 points= "(25,11.25);(25,11.25);(35,11.25);(35,11.25)"
%	 stroke-width= "0.5"
%	 />
%<multicurve fill-style= "none"
%	 points= "(35,20);(35,20);(35,11.25);(35,11.25)"
%	 stroke-width= "0.5"
%	 />
%<multicurve fill-style= "none"
%	 points= "(30,20);(30,20);(30,25);(30,25)"
%	 stroke-width= "0.5"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "solid"
%	 anchor-point= "(30,15)"
%	 text-frame= "noframe"
%	 stroke-width= "0.5"
%	 text-hor-align= "center-h"
%	 >
%$\Homega$
%</text>
%<multicurve fill-style= "none"
%	 points= "(25,20);(25,20);(25,11.25);(25,11.25)"
%	 stroke-width= "0.5"
%	 />
%<multicurve fill-style= "none"
%	 points= "(25,20);(25,20);(35,20);(35,20)"
%	 stroke-width= "0.5"
%	 />
%<multicurve fill-style= "none"
%	 points= "(100,43.75);(100,43.75);(110,43.75);(110,43.75)"
%	 stroke-width= "0.5"
%	 />
%<multicurve fill-style= "none"
%	 points= "(110,52.5);(110,52.5);(110,43.75);(110,43.75)"
%	 stroke-width= "0.5"
%	 />
%<multicurve fill-style= "none"
%	 points= "(100,52.5);(100,52.5);(100,43.75);(100,43.75)"
%	 stroke-width= "0.5"
%	 />
%<multicurve fill-style= "none"
%	 points= "(100,52.5);(100,52.5);(110,52.5);(110,52.5)"
%	 stroke-width= "0.5"
%	 />
%<multicurve fill-style= "none"
%	 points= "(150,43.75);(150,43.75);(160,43.75);(160,43.75)"
%	 stroke-width= "0.5"
%	 />
%<multicurve fill-style= "none"
%	 points= "(160,52.5);(160,52.5);(160,43.75);(160,43.75)"
%	 stroke-width= "0.5"
%	 />
%<multicurve fill-style= "none"
%	 points= "(150,52.5);(150,52.5);(150,43.75);(150,43.75)"
%	 stroke-width= "0.5"
%	 />
%<multicurve fill-style= "none"
%	 points= "(150,52.5);(150,52.5);(160,52.5);(160,52.5)"
%	 stroke-width= "0.5"
%	 />
%<multicurve fill-style= "none"
%	 points= "(105,21.25);(105,21.25);(115,21.25);(115,21.25)"
%	 stroke-width= "0.5"
%	 />
%<multicurve fill-style= "none"
%	 points= "(115,30);(115,30);(115,21.25);(115,21.25)"
%	 stroke-width= "0.5"
%	 />
%<multicurve fill-style= "none"
%	 points= "(105,30);(105,30);(105,21.25);(105,21.25)"
%	 stroke-width= "0.5"
%	 />
%<multicurve fill-style= "none"
%	 points= "(105,30);(105,30);(115,30);(115,30)"
%	 stroke-width= "0.5"
%	 />
%<multicurve fill-style= "none"
%	 points= "(155,21.25);(155,21.25);(165,21.25);(165,21.25)"
%	 stroke-width= "0.5"
%	 />
%<multicurve fill-style= "none"
%	 points= "(165,30);(165,30);(165,21.25);(165,21.25)"
%	 stroke-width= "0.5"
%	 />
%<multicurve fill-style= "none"
%	 points= "(155,30);(155,30);(155,21.25);(155,21.25)"
%	 stroke-width= "0.5"
%	 />
%<multicurve fill-style= "none"
%	 points= "(155,30);(155,30);(165,30);(165,30)"
%	 stroke-width= "0.5"
%	 />
%<multicurve fill-style= "none"
%	 points= "(145,66.25);(145,66.25);(155,66.25);(155,66.25)"
%	 stroke-width= "0.5"
%	 />
%<multicurve fill-style= "none"
%	 points= "(155,75);(155,75);(155,66.25);(155,66.25)"
%	 stroke-width= "0.5"
%	 />
%<multicurve fill-style= "none"
%	 points= "(145,75);(145,75);(145,66.25);(145,66.25)"
%	 stroke-width= "0.5"
%	 />
%<multicurve fill-style= "none"
%	 points= "(145,75);(145,75);(155,75);(155,75)"
%	 stroke-width= "0.5"
%	 />
%</jpic>
%%End JPIC-XML
%PSTricks content-type (pstricks.sty package needed)
%Add \usepackage{pstricks} in the preamble of your LaTeX file
%You can rescale the whole picture (to 80% for instance) by using the command \def\JPicScale{0.8}
\ifx\JPicScale\undefined\def\JPicScale{1}\fi
\psset{unit=\JPicScale mm}
\psset{linewidth=0.3,dotsep=1,hatchwidth=0.3,hatchsep=1.5,shadowsize=1,dimen=middle}
\psset{dotsize=0.7 2.5,dotscale=1 1,fillcolor=black}
\psset{arrowsize=1 2,arrowlength=1,arrowinset=0.25,tbarsize=0.7 5,bracketlength=0.15,rbracketlength=0.15}
\begin{pspicture}(0,0)(193.75,148.75)
\psline[linewidth=0.5](65,33.75)(65,30)
\rput{0}(70,11.25){\psellipse[linewidth=0.5,fillstyle=solid](0,0)(1.25,-1.25)}
\psline[linewidth=0.5](75,16.25)(70,11.25)
\psline[linewidth=0.5](70,11.25)(65,16.25)
\psline[linewidth=0.5](65,16.25)(65,21.25)
\psline[linewidth=0.5](75,16.25)(75,47.5)
\psline[linewidth=0.5](60,33.75)(70,33.75)
\psline[linewidth=0.5](70,42.5)(70,33.75)
\psline[linewidth=0.5](65,42.5)(65,47.5)
\psline[linewidth=0.5](62.5,47.5)(77.5,47.5)
\psline[linewidth=0.5](62.5,62.5)(62.5,47.5)
\psline[linewidth=0.5](62.5,62.5)(77.5,47.5)
\psline[linewidth=0.5](70,66.25)(70,55)
\rput(50,16.25){\EQLS}
\rput(65,25.62){$\addd$}
\psline[linewidth=0.5](65,6.25)(70,1.25)
\psline[linewidth=0.5](65,6.25)(75,6.25)
\psline[linewidth=0.5](75,6.25)(70,1.25)
\rput(65,37.5){$\Homega$}
\rput(67.5,51.25){$\png$}
\psline[linewidth=0.5](60,42.5)(60,33.75)
\psline[linewidth=0.5](60,42.5)(70,42.5)
\psline[linewidth=0.5](70,11.25)(70,6.25)
\rput(70,3.75){$\beeh$}
\psline[linewidth=0.5](30,11.25)(30,6.25)
\psline[linewidth=0.5](60,21.25)(70,21.25)
\psline[linewidth=0.5](70,30)(70,21.25)
\psline[linewidth=0.5](60,30)(60,21.25)
\psline[linewidth=0.5](60,30)(70,30)
\psline[linewidth=0.5](25,6.25)(35,6.25)
\psline[linewidth=0.5](35,6.25)(30,1.25)
\rput(30,3.75){$\beeh$}
\psline[linewidth=0.5](25,6.25)(30,1.25)
\psline[linewidth=0.5](105,56.25)(105,52.5)
\rput{0}(110,33.75){\psellipse[linewidth=0.5,fillstyle=solid](0,0)(1.25,-1.25)}
\psline[linewidth=0.5](115,38.75)(110,33.75)
\psline[linewidth=0.5](110,33.75)(105,38.75)
\psline[linewidth=0.5](105,38.75)(105,43.75)
\psline[linewidth=0.5](115,38.75)(115,70)
\psline[linewidth=0.5](100,56.25)(110,56.25)
\psline[linewidth=0.5](110,65)(110,56.25)
\psline[linewidth=0.5](105,65)(105,70)
\psline[linewidth=0.5](102.5,70)(117.5,70)
\psline[linewidth=0.5](102.5,85)(102.5,70)
\psline[linewidth=0.5](102.5,85)(117.5,70)
\psline[linewidth=0.5](110,88.75)(110,77.5)
\rput(105,48.12){$\addd$}
\rput(105,60){$\Homega$}
\rput(107.5,73.75){$\png$}
\psline[linewidth=0.5](100,65)(100,56.25)
\psline[linewidth=0.5](100,65)(110,65)
\psline[linewidth=0.5](110,33.75)(110,30)
\rput{0}(115,11.25){\psellipse[linewidth=0.5,fillstyle=solid](0,0)(1.25,-1.25)}
\psline[linewidth=0.5](120,16.25)(115,11.25)
\psline[linewidth=0.5](115,11.25)(110,16.25)
\psline[linewidth=0.5](110,16.25)(110,21.25)
\psline[linewidth=0.5](120,16.25)(120,88.75)
\rput(110,25.62){$\addd$}
\psline[linewidth=0.5](115,11.25)(115,6.25)
\psline[linewidth=0.5](110,6.25)(120,6.25)
\psline[linewidth=0.5](120,6.25)(115,1.25)
\rput(115,3.75){$\beeh$}
\psline[linewidth=0.5](110,6.25)(115,1.25)
\psline[linewidth=0.5](107.5,88.75)(122.5,88.75)
\psline[linewidth=0.5](107.5,103.75)(122.5,88.75)
\psline[linewidth=0.5](115,107.5)(115,96.25)
\rput(112.5,92.5){$\png$}
\psline[linewidth=0.5](107.5,103.75)(107.5,88.75)
\psline[linewidth=0.5](150,78.75)(150,75)
\rput{0}(155,56.25){\psellipse[linewidth=0.5,fillstyle=solid](0,0)(1.25,-1.25)}
\psline[linewidth=0.5](160,61.25)(155,56.25)
\psline[linewidth=0.5](155,56.25)(150,61.25)
\psline[linewidth=0.5](150,61.25)(150,66.25)
\psline[linewidth=0.5](160,61.25)(160,92.5)
\psline[linewidth=0.5](145,78.75)(155,78.75)
\psline[linewidth=0.5](155,87.5)(155,78.75)
\psline[linewidth=0.5](150,87.5)(150,92.5)
\psline[linewidth=0.5](147.5,92.5)(162.5,92.5)
\psline[linewidth=0.5](147.5,107.5)(147.5,92.5)
\psline[linewidth=0.5](147.5,107.5)(162.5,92.5)
\psline[linewidth=0.5](155,111.25)(155,100)
\rput(150,70.62){$\addd$}
\rput(150,82.5){$\Homega$}
\rput(152.5,96.25){$\png$}
\psline[linewidth=0.5](145,87.5)(145,78.75)
\psline[linewidth=0.5](145,87.5)(155,87.5)
\psline[linewidth=0.5](155,56.25)(155,52.5)
\rput{0}(160,33.75){\psellipse[linewidth=0.5,fillstyle=solid](0,0)(1.25,-1.25)}
\psline[linewidth=0.5](165,38.75)(160,33.75)
\psline[linewidth=0.5](160,33.75)(155,38.75)
\psline[linewidth=0.5](155,38.75)(155,43.75)
\psline[linewidth=0.5](165,38.75)(165,111.25)
\rput(155,48.12){$\addd$}
\psline[linewidth=0.5](152.5,111.25)(167.5,111.25)
\psline[linewidth=0.5](152.5,126.25)(167.5,111.25)
\psline[linewidth=0.5](160,130)(160,118.75)
\rput(157.5,115){$\png$}
\psline[linewidth=0.5](152.5,126.25)(152.5,111.25)
\psline[linewidth=0.5](160,33.75)(160,30)
\rput{0}(165,11.25){\psellipse[linewidth=0.5,fillstyle=solid](0,0)(1.25,-1.25)}
\psline[linewidth=0.5](170,16.25)(165,11.25)
\psline[linewidth=0.5](165,11.25)(160,16.25)
\psline[linewidth=0.5](160,16.25)(160,21.25)
\rput(160,25.62){$\addd$}
\psline[linewidth=0.5](165,11.25)(165,6.25)
\psline[linewidth=0.5](160,6.25)(170,6.25)
\psline[linewidth=0.5](170,6.25)(165,1.25)
\rput(165,3.75){$\beeh$}
\psline[linewidth=0.5](160,6.25)(165,1.25)
\psline[linewidth=0.5](170,16.25)(170,130)
\psline[linewidth=0.5](157.5,130)(172.5,130)
\psline[linewidth=0.5](157.5,145)(172.5,130)
\psline[linewidth=0.5](165,148.75)(165,137.5)
\rput(162.5,133.75){$\png$}
\psline[linewidth=0.5](157.5,145)(157.5,130)
\rput(90,16.25){\EQLS}
\rput(135,16.25){\EQLS}
\rput(185,16.25){\EQLS}
\rput(193.75,16.25){$\cdots$}
\rput(0,16.25){$\ordin$}
\rput(13.75,16.25){\EQLS}
\psline[linewidth=0.5](25,11.25)(35,11.25)
\psline[linewidth=0.5](35,20)(35,11.25)
\psline[linewidth=0.5](30,20)(30,25)
\rput(30,15){$\Homega$}
\psline[linewidth=0.5](25,20)(25,11.25)
\psline[linewidth=0.5](25,20)(35,20)
\psline[linewidth=0.5](100,43.75)(110,43.75)
\psline[linewidth=0.5](110,52.5)(110,43.75)
\psline[linewidth=0.5](100,52.5)(100,43.75)
\psline[linewidth=0.5](100,52.5)(110,52.5)
\psline[linewidth=0.5](150,43.75)(160,43.75)
\psline[linewidth=0.5](160,52.5)(160,43.75)
\psline[linewidth=0.5](150,52.5)(150,43.75)
\psline[linewidth=0.5](150,52.5)(160,52.5)
\psline[linewidth=0.5](105,21.25)(115,21.25)
\psline[linewidth=0.5](115,30)(115,21.25)
\psline[linewidth=0.5](105,30)(105,21.25)
\psline[linewidth=0.5](105,30)(115,30)
\psline[linewidth=0.5](155,21.25)(165,21.25)
\psline[linewidth=0.5](165,30)(165,21.25)
\psline[linewidth=0.5](155,30)(155,21.25)
\psline[linewidth=0.5](155,30)(165,30)
\psline[linewidth=0.5](145,66.25)(155,66.25)
\psline[linewidth=0.5](155,75)(155,66.25)
\psline[linewidth=0.5](145,75)(145,66.25)
\psline[linewidth=0.5](145,75)(155,75)
\end{pspicture}


==> PIC/Omega-unfold.tex <==
%%Created by jPicEdt 1.4.1_03: mixed JPIC-XML/LaTeX format
%%Thu Feb 25 21:23:59 GMT-10:00 2021
%%Begin JPIC-XML
%<?xml version="1.0" standalone="yes"?>
%<jpic x-min="0" x-max="193.75" y-min="0" y-max="147.5" auto-bounding="true">
%<multicurve fill-style= "none"
%	 points= "(65,32.5);(65,32.5);(65,27.5);(65,27.5)"
%	 stroke-width= "0.5"
%	 />
%<ellipse p3= "(71.25,8.75)"
%	 fill-style= "solid"
%	 p2= "(71.25,11.25)"
%	 p1= "(68.75,11.25)"
%	 closure= "open"
%	 angle-end= "0"
%	 stroke-width= "0.5"
%	 angle-start= "0"
%	 />
%<multicurve fill-style= "none"
%	 points= "(75,15);(75,15);(70,10);(70,10)"
%	 stroke-width= "0.5"
%	 />
%<multicurve fill-style= "none"
%	 points= "(70,10);(70,10);(65,15);(65,15)"
%	 stroke-width= "0.5"
%	 />
%<multicurve fill-style= "none"
%	 points= "(65,15);(65,15);(65,20);(65,20)"
%	 stroke-width= "0.5"
%	 />
%<multicurve fill-style= "none"
%	 points= "(75,15);(75,15);(75,46.25);(75,46.25)"
%	 stroke-width= "0.5"
%	 />
%<multicurve fill-style= "none"
%	 points= "(60,32.5);(60,32.5);(70,32.5);(70,32.5)"
%	 stroke-width= "0.5"
%	 />
%<multicurve fill-style= "none"
%	 points= "(70,41.25);(70,41.25);(70,32.5);(70,32.5)"
%	 stroke-width= "0.5"
%	 />
%<multicurve fill-style= "none"
%	 points= "(65,41.25);(65,41.25);(65,46.25);(65,46.25)"
%	 stroke-width= "0.5"
%	 />
%<multicurve fill-style= "none"
%	 points= "(62.5,46.25);(62.5,46.25);(77.5,46.25);(77.5,46.25)"
%	 stroke-width= "0.5"
%	 />
%<multicurve fill-style= "none"
%	 points= "(62.5,61.25);(62.5,61.25);(62.5,46.25);(62.5,46.25)"
%	 stroke-width= "0.5"
%	 />
%<multicurve fill-style= "none"
%	 points= "(62.5,61.25);(62.5,61.25);(77.5,46.25);(77.5,46.25)"
%	 stroke-width= "0.5"
%	 />
%<multicurve fill-style= "none"
%	 points= "(70,65);(70,65);(70,53.75);(70,53.75)"
%	 stroke-width= "0.5"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "solid"
%	 anchor-point= "(50,15)"
%	 text-frame= "noframe"
%	 stroke-width= "0.5"
%	 text-hor-align= "center-h"
%	 >
%\EQLS
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "solid"
%	 anchor-point= "(65,23.75)"
%	 text-frame= "noframe"
%	 stroke-width= "0.5"
%	 text-hor-align= "center-h"
%	 >
%$\addd$
%</text>
%<multicurve fill-style= "none"
%	 points= "(65,5);(65,5);(70,0);(70,0)"
%	 stroke-width= "0.5"
%	 />
%<multicurve fill-style= "none"
%	 points= "(65,5);(65,5);(75,5);(75,5)"
%	 stroke-width= "0.5"
%	 />
%<multicurve fill-style= "none"
%	 points= "(75,5);(75,5);(70,0);(70,0)"
%	 stroke-width= "0.5"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "solid"
%	 anchor-point= "(65,36.25)"
%	 text-frame= "noframe"
%	 stroke-width= "0.5"
%	 text-hor-align= "center-h"
%	 >
%$\Homega$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "solid"
%	 anchor-point= "(67.5,50)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\png$
%</text>
%<ellipse p3= "(68.75,27.5)"
%	 fill-style= "none"
%	 p2= "(68.75,20)"
%	 p1= "(61.25,20)"
%	 closure= "open"
%	 angle-end= "360"
%	 stroke-width= "0.5"
%	 angle-start= "0"
%	 />
%<multicurve fill-style= "none"
%	 points= "(60,41.25);(60,41.25);(60,32.5);(60,32.5)"
%	 stroke-width= "0.5"
%	 />
%<multicurve fill-style= "none"
%	 points= "(60,41.25);(60,41.25);(70,41.25);(70,41.25)"
%	 stroke-width= "0.5"
%	 />
%<multicurve fill-style= "none"
%	 points= "(70,10);(70,10);(70,5);(70,5)"
%	 stroke-width= "0.5"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(70,2.5)"
%	 text-frame= "noframe"
%	 stroke-width= "1"
%	 text-hor-align= "center-h"
%	 >
%$\beeh$
%</text>
%<multicurve fill-style= "none"
%	 points= "(30,11.25);(30,11.25);(30,5);(30,5)"
%	 stroke-width= "0.5"
%	 />
%<multicurve fill-style= "none"
%	 points= "(25,11.25);(25,11.25);(35,11.25);(35,11.25)"
%	 stroke-width= "0.5"
%	 />
%<multicurve fill-style= "none"
%	 points= "(35,20);(35,20);(35,11.25);(35,11.25)"
%	 stroke-width= "0.5"
%	 />
%<multicurve fill-style= "none"
%	 points= "(30,20);(30,20);(30,25);(30,25)"
%	 stroke-width= "0.5"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "solid"
%	 anchor-point= "(30,15)"
%	 text-frame= "noframe"
%	 stroke-width= "0.5"
%	 text-hor-align= "center-h"
%	 >
%$\Homega$
%</text>
%<multicurve fill-style= "none"
%	 points= "(25,20);(25,20);(25,11.25);(25,11.25)"
%	 stroke-width= "0.5"
%	 />
%<multicurve fill-style= "none"
%	 points= "(25,20);(25,20);(35,20);(35,20)"
%	 stroke-width= "0.5"
%	 />
%<multicurve fill-style= "none"
%	 points= "(25,5);(25,5);(35,5);(35,5)"
%	 stroke-width= "0.5"
%	 />
%<multicurve fill-style= "none"
%	 points= "(35,5);(35,5);(30,0);(30,0)"
%	 stroke-width= "0.5"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(30,2.5)"
%	 text-frame= "noframe"
%	 stroke-width= "1"
%	 text-hor-align= "center-h"
%	 >
%$\beeh$
%</text>
%<multicurve fill-style= "none"
%	 points= "(25,5);(25,5);(30,0);(30,0)"
%	 stroke-width= "0.5"
%	 />
%<multicurve fill-style= "none"
%	 points= "(105,55);(105,55);(105,50);(105,50)"
%	 stroke-width= "0.5"
%	 />
%<ellipse p3= "(111.25,31.25)"
%	 fill-style= "solid"
%	 p2= "(111.25,33.75)"
%	 p1= "(108.75,33.75)"
%	 closure= "open"
%	 angle-end= "0"
%	 stroke-width= "0.5"
%	 angle-start= "0"
%	 />
%<multicurve fill-style= "none"
%	 points= "(115,37.5);(115,37.5);(110,32.5);(110,32.5)"
%	 stroke-width= "0.5"
%	 />
%<multicurve fill-style= "none"
%	 points= "(110,32.5);(110,32.5);(105,37.5);(105,37.5)"
%	 stroke-width= "0.5"
%	 />
%<multicurve fill-style= "none"
%	 points= "(105,37.5);(105,37.5);(105,42.5);(105,42.5)"
%	 stroke-width= "0.5"
%	 />
%<multicurve fill-style= "none"
%	 points= "(115,37.5);(115,37.5);(115,68.75);(115,68.75)"
%	 stroke-width= "0.5"
%	 />
%<multicurve fill-style= "none"
%	 points= "(100,55);(100,55);(110,55);(110,55)"
%	 stroke-width= "0.5"
%	 />
%<multicurve fill-style= "none"
%	 points= "(110,63.75);(110,63.75);(110,55);(110,55)"
%	 stroke-width= "0.5"
%	 />
%<multicurve fill-style= "none"
%	 points= "(105,63.75);(105,63.75);(105,68.75);(105,68.75)"
%	 stroke-width= "0.5"
%	 />
%<multicurve fill-style= "none"
%	 points= "(102.5,68.75);(102.5,68.75);(117.5,68.75);(117.5,68.75)"
%	 stroke-width= "0.5"
%	 />
%<multicurve fill-style= "none"
%	 points= "(102.5,83.75);(102.5,83.75);(102.5,68.75);(102.5,68.75)"
%	 stroke-width= "0.5"
%	 />
%<multicurve fill-style= "none"
%	 points= "(102.5,83.75);(102.5,83.75);(117.5,68.75);(117.5,68.75)"
%	 stroke-width= "0.5"
%	 />
%<multicurve fill-style= "none"
%	 points= "(110,87.5);(110,87.5);(110,76.25);(110,76.25)"
%	 stroke-width= "0.5"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "solid"
%	 anchor-point= "(105,46.25)"
%	 text-frame= "noframe"
%	 stroke-width= "0.5"
%	 text-hor-align= "center-h"
%	 >
%$\addd$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "solid"
%	 anchor-point= "(105,58.75)"
%	 text-frame= "noframe"
%	 stroke-width= "0.5"
%	 text-hor-align= "center-h"
%	 >
%$\Homega$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "solid"
%	 anchor-point= "(107.5,72.5)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\png$
%</text>
%<ellipse p3= "(108.75,50)"
%	 fill-style= "none"
%	 p2= "(108.75,42.5)"
%	 p1= "(101.25,42.5)"
%	 closure= "open"
%	 angle-end= "360"
%	 stroke-width= "0.5"
%	 angle-start= "0"
%	 />
%<multicurve fill-style= "none"
%	 points= "(100,63.75);(100,63.75);(100,55);(100,55)"
%	 stroke-width= "0.5"
%	 />
%<multicurve fill-style= "none"
%	 points= "(100,63.75);(100,63.75);(110,63.75);(110,63.75)"
%	 stroke-width= "0.5"
%	 />
%<multicurve fill-style= "none"
%	 points= "(110,32.5);(110,32.5);(110,27.5);(110,27.5)"
%	 stroke-width= "0.5"
%	 />
%<ellipse p3= "(116.25,8.75)"
%	 fill-style= "solid"
%	 p2= "(116.25,11.25)"
%	 p1= "(113.75,11.25)"
%	 closure= "open"
%	 angle-end= "0"
%	 stroke-width= "0.5"
%	 angle-start= "0"
%	 />
%<multicurve fill-style= "none"
%	 points= "(120,15);(120,15);(115,10);(115,10)"
%	 stroke-width= "0.5"
%	 />
%<multicurve fill-style= "none"
%	 points= "(115,10);(115,10);(110,15);(110,15)"
%	 stroke-width= "0.5"
%	 />
%<multicurve fill-style= "none"
%	 points= "(110,15);(110,15);(110,20);(110,20)"
%	 stroke-width= "0.5"
%	 />
%<multicurve fill-style= "none"
%	 points= "(120,15);(120,15);(120,87.5);(120,87.5)"
%	 stroke-width= "0.5"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "solid"
%	 anchor-point= "(110,23.75)"
%	 text-frame= "noframe"
%	 stroke-width= "0.5"
%	 text-hor-align= "center-h"
%	 >
%$\addd$
%</text>
%<ellipse p3= "(113.75,27.5)"
%	 fill-style= "none"
%	 p2= "(113.75,20)"
%	 p1= "(106.25,20)"
%	 closure= "open"
%	 angle-end= "360"
%	 stroke-width= "0.5"
%	 angle-start= "0"
%	 />
%<multicurve fill-style= "none"
%	 points= "(115,10);(115,10);(115,5);(115,5)"
%	 stroke-width= "0.5"
%	 />
%<multicurve fill-style= "none"
%	 points= "(110,5);(110,5);(120,5);(120,5)"
%	 stroke-width= "0.5"
%	 />
%<multicurve fill-style= "none"
%	 points= "(120,5);(120,5);(115,0);(115,0)"
%	 stroke-width= "0.5"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(115,2.5)"
%	 text-frame= "noframe"
%	 stroke-width= "1"
%	 text-hor-align= "center-h"
%	 >
%$\beeh$
%</text>
%<multicurve fill-style= "none"
%	 points= "(110,5);(110,5);(115,0);(115,0)"
%	 stroke-width= "0.5"
%	 />
%<multicurve fill-style= "none"
%	 points= "(107.5,87.5);(107.5,87.5);(122.5,87.5);(122.5,87.5)"
%	 stroke-width= "0.5"
%	 />
%<multicurve fill-style= "none"
%	 points= "(107.5,102.5);(107.5,102.5);(122.5,87.5);(122.5,87.5)"
%	 stroke-width= "0.5"
%	 />
%<multicurve fill-style= "none"
%	 points= "(115,106.25);(115,106.25);(115,95);(115,95)"
%	 stroke-width= "0.5"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "solid"
%	 anchor-point= "(112.5,91.25)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\png$
%</text>
%<multicurve fill-style= "none"
%	 points= "(107.5,102.5);(107.5,102.5);(107.5,87.5);(107.5,87.5)"
%	 stroke-width= "0.5"
%	 />
%<multicurve fill-style= "none"
%	 points= "(150,77.5);(150,77.5);(150,72.5);(150,72.5)"
%	 stroke-width= "0.5"
%	 />
%<ellipse p3= "(156.25,53.75)"
%	 fill-style= "solid"
%	 p2= "(156.25,56.25)"
%	 p1= "(153.75,56.25)"
%	 closure= "open"
%	 angle-end= "0"
%	 stroke-width= "0.5"
%	 angle-start= "0"
%	 />
%<multicurve fill-style= "none"
%	 points= "(160,60);(160,60);(155,55);(155,55)"
%	 stroke-width= "0.5"
%	 />
%<multicurve fill-style= "none"
%	 points= "(155,55);(155,55);(150,60);(150,60)"
%	 stroke-width= "0.5"
%	 />
%<multicurve fill-style= "none"
%	 points= "(150,60);(150,60);(150,65);(150,65)"
%	 stroke-width= "0.5"
%	 />
%<multicurve fill-style= "none"
%	 points= "(160,60);(160,60);(160,91.25);(160,91.25)"
%	 stroke-width= "0.5"
%	 />
%<multicurve fill-style= "none"
%	 points= "(145,77.5);(145,77.5);(155,77.5);(155,77.5)"
%	 stroke-width= "0.5"
%	 />
%<multicurve fill-style= "none"
%	 points= "(155,86.25);(155,86.25);(155,77.5);(155,77.5)"
%	 stroke-width= "0.5"
%	 />
%<multicurve fill-style= "none"
%	 points= "(150,86.25);(150,86.25);(150,91.25);(150,91.25)"
%	 stroke-width= "0.5"
%	 />
%<multicurve fill-style= "none"
%	 points= "(147.5,91.25);(147.5,91.25);(162.5,91.25);(162.5,91.25)"
%	 stroke-width= "0.5"
%	 />
%<multicurve fill-style= "none"
%	 points= "(147.5,106.25);(147.5,106.25);(147.5,91.25);(147.5,91.25)"
%	 stroke-width= "0.5"
%	 />
%<multicurve fill-style= "none"
%	 points= "(147.5,106.25);(147.5,106.25);(162.5,91.25);(162.5,91.25)"
%	 stroke-width= "0.5"
%	 />
%<multicurve fill-style= "none"
%	 points= "(155,110);(155,110);(155,98.75);(155,98.75)"
%	 stroke-width= "0.5"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "solid"
%	 anchor-point= "(150,68.75)"
%	 text-frame= "noframe"
%	 stroke-width= "0.5"
%	 text-hor-align= "center-h"
%	 >
%$\addd$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "solid"
%	 anchor-point= "(150,81.25)"
%	 text-frame= "noframe"
%	 stroke-width= "0.5"
%	 text-hor-align= "center-h"
%	 >
%$\Homega$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "solid"
%	 anchor-point= "(152.5,95)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\png$
%</text>
%<ellipse p3= "(153.75,72.5)"
%	 fill-style= "none"
%	 p2= "(153.75,65)"
%	 p1= "(146.25,65)"
%	 closure= "open"
%	 angle-end= "360"
%	 stroke-width= "0.5"
%	 angle-start= "0"
%	 />
%<multicurve fill-style= "none"
%	 points= "(145,86.25);(145,86.25);(145,77.5);(145,77.5)"
%	 stroke-width= "0.5"
%	 />
%<multicurve fill-style= "none"
%	 points= "(145,86.25);(145,86.25);(155,86.25);(155,86.25)"
%	 stroke-width= "0.5"
%	 />
%<multicurve fill-style= "none"
%	 points= "(155,55);(155,55);(155,50);(155,50)"
%	 stroke-width= "0.5"
%	 />
%<ellipse p3= "(161.25,31.25)"
%	 fill-style= "solid"
%	 p2= "(161.25,33.75)"
%	 p1= "(158.75,33.75)"
%	 closure= "open"
%	 angle-end= "0"
%	 stroke-width= "0.5"
%	 angle-start= "0"
%	 />
%<multicurve fill-style= "none"
%	 points= "(165,37.5);(165,37.5);(160,32.5);(160,32.5)"
%	 stroke-width= "0.5"
%	 />
%<multicurve fill-style= "none"
%	 points= "(160,32.5);(160,32.5);(155,37.5);(155,37.5)"
%	 stroke-width= "0.5"
%	 />
%<multicurve fill-style= "none"
%	 points= "(155,37.5);(155,37.5);(155,42.5);(155,42.5)"
%	 stroke-width= "0.5"
%	 />
%<multicurve fill-style= "none"
%	 points= "(165,37.5);(165,37.5);(165,110);(165,110)"
%	 stroke-width= "0.5"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "solid"
%	 anchor-point= "(155,46.25)"
%	 text-frame= "noframe"
%	 stroke-width= "0.5"
%	 text-hor-align= "center-h"
%	 >
%$\addd$
%</text>
%<ellipse p3= "(158.75,50)"
%	 fill-style= "none"
%	 p2= "(158.75,42.5)"
%	 p1= "(151.25,42.5)"
%	 closure= "open"
%	 angle-end= "360"
%	 stroke-width= "0.5"
%	 angle-start= "0"
%	 />
%<multicurve fill-style= "none"
%	 points= "(152.5,110);(152.5,110);(167.5,110);(167.5,110)"
%	 stroke-width= "0.5"
%	 />
%<multicurve fill-style= "none"
%	 points= "(152.5,125);(152.5,125);(167.5,110);(167.5,110)"
%	 stroke-width= "0.5"
%	 />
%<multicurve fill-style= "none"
%	 points= "(160,128.75);(160,128.75);(160,117.5);(160,117.5)"
%	 stroke-width= "0.5"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "solid"
%	 anchor-point= "(157.5,113.75)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\png$
%</text>
%<multicurve fill-style= "none"
%	 points= "(152.5,125);(152.5,125);(152.5,110);(152.5,110)"
%	 stroke-width= "0.5"
%	 />
%<multicurve fill-style= "none"
%	 points= "(160,32.5);(160,32.5);(160,27.5);(160,27.5)"
%	 stroke-width= "0.5"
%	 />
%<ellipse p3= "(166.25,8.75)"
%	 fill-style= "solid"
%	 p2= "(166.25,11.25)"
%	 p1= "(163.75,11.25)"
%	 closure= "open"
%	 angle-end= "0"
%	 stroke-width= "0.5"
%	 angle-start= "0"
%	 />
%<multicurve fill-style= "none"
%	 points= "(170,15);(170,15);(165,10);(165,10)"
%	 stroke-width= "0.5"
%	 />
%<multicurve fill-style= "none"
%	 points= "(165,10);(165,10);(160,15);(160,15)"
%	 stroke-width= "0.5"
%	 />
%<multicurve fill-style= "none"
%	 points= "(160,15);(160,15);(160,20);(160,20)"
%	 stroke-width= "0.5"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "solid"
%	 anchor-point= "(160,23.75)"
%	 text-frame= "noframe"
%	 stroke-width= "0.5"
%	 text-hor-align= "center-h"
%	 >
%$\addd$
%</text>
%<ellipse p3= "(163.75,27.5)"
%	 fill-style= "none"
%	 p2= "(163.75,20)"
%	 p1= "(156.25,20)"
%	 closure= "open"
%	 angle-end= "360"
%	 stroke-width= "0.5"
%	 angle-start= "0"
%	 />
%<multicurve fill-style= "none"
%	 points= "(165,10);(165,10);(165,5);(165,5)"
%	 stroke-width= "0.5"
%	 />
%<multicurve fill-style= "none"
%	 points= "(160,5);(160,5);(170,5);(170,5)"
%	 stroke-width= "0.5"
%	 />
%<multicurve fill-style= "none"
%	 points= "(170,5);(170,5);(165,0);(165,0)"
%	 stroke-width= "0.5"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(165,2.5)"
%	 text-frame= "noframe"
%	 stroke-width= "1"
%	 text-hor-align= "center-h"
%	 >
%$\beeh$
%</text>
%<multicurve fill-style= "none"
%	 points= "(160,5);(160,5);(165,0);(165,0)"
%	 stroke-width= "0.5"
%	 />
%<multicurve fill-style= "none"
%	 points= "(170,15);(170,15);(170,128.75);(170,128.75)"
%	 stroke-width= "0.5"
%	 />
%<multicurve fill-style= "none"
%	 points= "(157.5,128.75);(157.5,128.75);(172.5,128.75);(172.5,128.75)"
%	 stroke-width= "0.5"
%	 />
%<multicurve fill-style= "none"
%	 points= "(157.5,143.75);(157.5,143.75);(172.5,128.75);(172.5,128.75)"
%	 stroke-width= "0.5"
%	 />
%<multicurve fill-style= "none"
%	 points= "(165,147.5);(165,147.5);(165,136.25);(165,136.25)"
%	 stroke-width= "0.5"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "solid"
%	 anchor-point= "(162.5,132.5)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\png$
%</text>
%<multicurve fill-style= "none"
%	 points= "(157.5,143.75);(157.5,143.75);(157.5,128.75);(157.5,128.75)"
%	 stroke-width= "0.5"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "solid"
%	 anchor-point= "(90,15)"
%	 text-frame= "noframe"
%	 stroke-width= "0.5"
%	 text-hor-align= "center-h"
%	 >
%\EQLS
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "solid"
%	 anchor-point= "(135,15)"
%	 text-frame= "noframe"
%	 stroke-width= "0.5"
%	 text-hor-align= "center-h"
%	 >
%\EQLS
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "solid"
%	 anchor-point= "(185,15)"
%	 text-frame= "noframe"
%	 stroke-width= "0.5"
%	 text-hor-align= "center-h"
%	 >
%\EQLS
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(193.75,15)"
%	 text-frame= "noframe"
%	 stroke-width= "1"
%	 text-hor-align= "center-h"
%	 >
%$\cdots$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(0,15)"
%	 text-frame= "noframe"
%	 stroke-width= "1"
%	 text-hor-align= "center-h"
%	 >
%$\ordin$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "solid"
%	 anchor-point= "(13.75,15)"
%	 text-frame= "noframe"
%	 stroke-width= "0.5"
%	 text-hor-align= "center-h"
%	 >
%\EQLS
%</text>
%</jpic>
%%End JPIC-XML
%PSTricks content-type (pstricks.sty package needed)
%Add \usepackage{pstricks} in the preamble of your LaTeX file
%You can rescale the whole picture (to 80% for instance) by using the command \def\JPicScale{0.8}
\ifx\JPicScale\undefined\def\JPicScale{1}\fi
\psset{unit=\JPicScale mm}
\psset{linewidth=0.3,dotsep=1,hatchwidth=0.3,hatchsep=1.5,shadowsize=1,dimen=middle}
\psset{dotsize=0.7 2.5,dotscale=1 1,fillcolor=black}
\psset{arrowsize=1 2,arrowlength=1,arrowinset=0.25,tbarsize=0.7 5,bracketlength=0.15,rbracketlength=0.15}
\begin{pspicture}(0,0)(193.75,147.5)
\psline[linewidth=0.5](65,32.5)(65,27.5)
\rput{0}(70,10){\psellipse[linewidth=0.5,fillstyle=solid](0,0)(1.25,-1.25)}
\psline[linewidth=0.5](75,15)(70,10)
\psline[linewidth=0.5](70,10)(65,15)
\psline[linewidth=0.5](65,15)(65,20)
\psline[linewidth=0.5](75,15)(75,46.25)
\psline[linewidth=0.5](60,32.5)(70,32.5)
\psline[linewidth=0.5](70,41.25)(70,32.5)
\psline[linewidth=0.5](65,41.25)(65,46.25)
\psline[linewidth=0.5](62.5,46.25)(77.5,46.25)
\psline[linewidth=0.5](62.5,61.25)(62.5,46.25)
\psline[linewidth=0.5](62.5,61.25)(77.5,46.25)
\psline[linewidth=0.5](70,65)(70,53.75)
\rput(50,15){\EQLS}
\rput(65,23.75){$\addd$}
\psline[linewidth=0.5](65,5)(70,0)
\psline[linewidth=0.5](65,5)(75,5)
\psline[linewidth=0.5](75,5)(70,0)
\rput(65,36.25){$\Homega$}
\rput(67.5,50){$\png$}
\rput{0}(65,23.75){\psellipse[linewidth=0.5](0,0)(3.75,3.75)}
\psline[linewidth=0.5](60,41.25)(60,32.5)
\psline[linewidth=0.5](60,41.25)(70,41.25)
\psline[linewidth=0.5](70,10)(70,5)
\rput(70,2.5){$\beeh$}
\psline[linewidth=0.5](30,11.25)(30,5)
\psline[linewidth=0.5](25,11.25)(35,11.25)
\psline[linewidth=0.5](35,20)(35,11.25)
\psline[linewidth=0.5](30,20)(30,25)
\rput(30,15){$\Homega$}
\psline[linewidth=0.5](25,20)(25,11.25)
\psline[linewidth=0.5](25,20)(35,20)
\psline[linewidth=0.5](25,5)(35,5)
\psline[linewidth=0.5](35,5)(30,0)
\rput(30,2.5){$\beeh$}
\psline[linewidth=0.5](25,5)(30,0)
\psline[linewidth=0.5](105,55)(105,50)
\rput{0}(110,32.5){\psellipse[linewidth=0.5,fillstyle=solid](0,0)(1.25,-1.25)}
\psline[linewidth=0.5](115,37.5)(110,32.5)
\psline[linewidth=0.5](110,32.5)(105,37.5)
\psline[linewidth=0.5](105,37.5)(105,42.5)
\psline[linewidth=0.5](115,37.5)(115,68.75)
\psline[linewidth=0.5](100,55)(110,55)
\psline[linewidth=0.5](110,63.75)(110,55)
\psline[linewidth=0.5](105,63.75)(105,68.75)
\psline[linewidth=0.5](102.5,68.75)(117.5,68.75)
\psline[linewidth=0.5](102.5,83.75)(102.5,68.75)
\psline[linewidth=0.5](102.5,83.75)(117.5,68.75)
\psline[linewidth=0.5](110,87.5)(110,76.25)
\rput(105,46.25){$\addd$}
\rput(105,58.75){$\Homega$}
\rput(107.5,72.5){$\png$}
\rput{0}(105,46.25){\psellipse[linewidth=0.5](0,0)(3.75,3.75)}
\psline[linewidth=0.5](100,63.75)(100,55)
\psline[linewidth=0.5](100,63.75)(110,63.75)
\psline[linewidth=0.5](110,32.5)(110,27.5)
\rput{0}(115,10){\psellipse[linewidth=0.5,fillstyle=solid](0,0)(1.25,-1.25)}
\psline[linewidth=0.5](120,15)(115,10)
\psline[linewidth=0.5](115,10)(110,15)
\psline[linewidth=0.5](110,15)(110,20)
\psline[linewidth=0.5](120,15)(120,87.5)
\rput(110,23.75){$\addd$}
\rput{0}(110,23.75){\psellipse[linewidth=0.5](0,0)(3.75,3.75)}
\psline[linewidth=0.5](115,10)(115,5)
\psline[linewidth=0.5](110,5)(120,5)
\psline[linewidth=0.5](120,5)(115,0)
\rput(115,2.5){$\beeh$}
\psline[linewidth=0.5](110,5)(115,0)
\psline[linewidth=0.5](107.5,87.5)(122.5,87.5)
\psline[linewidth=0.5](107.5,102.5)(122.5,87.5)
\psline[linewidth=0.5](115,106.25)(115,95)
\rput(112.5,91.25){$\png$}
\psline[linewidth=0.5](107.5,102.5)(107.5,87.5)
\psline[linewidth=0.5](150,77.5)(150,72.5)
\rput{0}(155,55){\psellipse[linewidth=0.5,fillstyle=solid](0,0)(1.25,-1.25)}
\psline[linewidth=0.5](160,60)(155,55)
\psline[linewidth=0.5](155,55)(150,60)
\psline[linewidth=0.5](150,60)(150,65)
\psline[linewidth=0.5](160,60)(160,91.25)
\psline[linewidth=0.5](145,77.5)(155,77.5)
\psline[linewidth=0.5](155,86.25)(155,77.5)
\psline[linewidth=0.5](150,86.25)(150,91.25)
\psline[linewidth=0.5](147.5,91.25)(162.5,91.25)
\psline[linewidth=0.5](147.5,106.25)(147.5,91.25)
\psline[linewidth=0.5](147.5,106.25)(162.5,91.25)
\psline[linewidth=0.5](155,110)(155,98.75)
\rput(150,68.75){$\addd$}
\rput(150,81.25){$\Homega$}
\rput(152.5,95){$\png$}
\rput{0}(150,68.75){\psellipse[linewidth=0.5](0,0)(3.75,3.75)}
\psline[linewidth=0.5](145,86.25)(145,77.5)
\psline[linewidth=0.5](145,86.25)(155,86.25)
\psline[linewidth=0.5](155,55)(155,50)
\rput{0}(160,32.5){\psellipse[linewidth=0.5,fillstyle=solid](0,0)(1.25,-1.25)}
\psline[linewidth=0.5](165,37.5)(160,32.5)
\psline[linewidth=0.5](160,32.5)(155,37.5)
\psline[linewidth=0.5](155,37.5)(155,42.5)
\psline[linewidth=0.5](165,37.5)(165,110)
\rput(155,46.25){$\addd$}
\rput{0}(155,46.25){\psellipse[linewidth=0.5](0,0)(3.75,3.75)}
\psline[linewidth=0.5](152.5,110)(167.5,110)
\psline[linewidth=0.5](152.5,125)(167.5,110)
\psline[linewidth=0.5](160,128.75)(160,117.5)
\rput(157.5,113.75){$\png$}
\psline[linewidth=0.5](152.5,125)(152.5,110)
\psline[linewidth=0.5](160,32.5)(160,27.5)
\rput{0}(165,10){\psellipse[linewidth=0.5,fillstyle=solid](0,0)(1.25,-1.25)}
\psline[linewidth=0.5](170,15)(165,10)
\psline[linewidth=0.5](165,10)(160,15)
\psline[linewidth=0.5](160,15)(160,20)
\rput(160,23.75){$\addd$}
\rput{0}(160,23.75){\psellipse[linewidth=0.5](0,0)(3.75,3.75)}
\psline[linewidth=0.5](165,10)(165,5)
\psline[linewidth=0.5](160,5)(170,5)
\psline[linewidth=0.5](170,5)(165,0)
\rput(165,2.5){$\beeh$}
\psline[linewidth=0.5](160,5)(165,0)
\psline[linewidth=0.5](170,15)(170,128.75)
\psline[linewidth=0.5](157.5,128.75)(172.5,128.75)
\psline[linewidth=0.5](157.5,143.75)(172.5,128.75)
\psline[linewidth=0.5](165,147.5)(165,136.25)
\rput(162.5,132.5){$\png$}
\psline[linewidth=0.5](157.5,143.75)(157.5,128.75)
\rput(90,15){\EQLS}
\rput(135,15){\EQLS}
\rput(185,15){\EQLS}
\rput(193.75,15){$\cdots$}
\rput(0,15){$\ordin$}
\rput(13.75,15){\EQLS}
\end{pspicture}


==> PIC/Omega.tex <==
%%Created by jPicEdt 1.4.1_03: mixed JPIC-XML/LaTeX format
%%Sun Feb 21 23:06:59 GMT-10:00 2021
%%Begin JPIC-XML
%<?xml version="1.0" standalone="yes"?>
%<jpic x-min="-2.5" x-max="107.5" y-min="0" y-max="75" auto-bounding="true">
%<multicurve fill-style= "none"
%	 points= "(20,10);(20,10);(20,0);(20,0)"
%	 stroke-width= "0.5"
%	 />
%<ellipse p3= "(21.25,8.75)"
%	 fill-style= "solid"
%	 p2= "(21.25,11.25)"
%	 p1= "(18.75,11.25)"
%	 closure= "open"
%	 angle-end= "360"
%	 stroke-width= "0.5"
%	 angle-start= "0"
%	 />
%<multicurve fill-style= "none"
%	 points= "(25,15);(25,15);(20,10);(20,10)"
%	 stroke-width= "0.5"
%	 />
%<multicurve fill-style= "none"
%	 points= "(20,10);(20,10);(15,15);(15,15)"
%	 stroke-width= "0.5"
%	 />
%<multicurve fill-style= "none"
%	 points= "(15,15);(15,15);(15,21.25);(15,21.25)"
%	 stroke-width= "0.5"
%	 />
%<multicurve fill-style= "none"
%	 points= "(25,15);(25,15);(25,55);(25,55)"
%	 stroke-width= "0.5"
%	 />
%<multicurve fill-style= "none"
%	 points= "(10,40);(10,40);(20,40);(20,40)"
%	 stroke-width= "0.5"
%	 />
%<multicurve fill-style= "none"
%	 points= "(0,50);(0,50);(10,50);(10,50)"
%	 stroke-width= "0.5"
%	 />
%<ellipse p3= "(18.52,21.48)"
%	 fill-style= "none"
%	 p2= "(18.52,28.52)"
%	 p1= "(11.48,28.52)"
%	 closure= "open"
%	 angle-end= "360"
%	 stroke-width= "0.5"
%	 angle-start= "0"
%	 />
%<multicurve fill-style= "none"
%	 points= "(15,28.75);(15,28.75);(15,40);(15,40)"
%	 stroke-width= "0.5"
%	 />
%<multicurve fill-style= "none"
%	 points= "(10,50);(10,50);(20,40);(20,40)"
%	 stroke-width= "0.5"
%	 />
%<multicurve fill-style= "none"
%	 points= "(0,50);(0,50);(10,40);(10,40)"
%	 stroke-width= "0.5"
%	 />
%<multicurve fill-style= "none"
%	 points= "(0,42.5);(0,42.5);(10,32.5);(10,32.5)"
%	 stroke-width= "0.5"
%	 />
%<multicurve fill-style= "none"
%	 points= "(15,45);(15,45);(15,55);(15,55)"
%	 stroke-width= "0.5"
%	 />
%<multicurve fill-style= "none"
%	 points= "(5,37.5);(5,37.5);(5,45);(5,45)"
%	 stroke-width= "0.5"
%	 />
%<multicurve fill-style= "none"
%	 points= "(0,32.5);(0,32.5);(10,32.5);(10,32.5)"
%	 stroke-width= "0.5"
%	 />
%<multicurve fill-style= "none"
%	 points= "(0,42.5);(0,42.5);(0,32.5);(0,32.5)"
%	 stroke-width= "0.5"
%	 />
%<multicurve fill-style= "none"
%	 points= "(12.5,55);(12.5,55);(27.5,55);(27.5,55)"
%	 stroke-width= "0.5"
%	 />
%<multicurve fill-style= "none"
%	 points= "(12.5,70);(12.5,70);(12.5,55);(12.5,55)"
%	 stroke-width= "0.5"
%	 />
%<multicurve fill-style= "none"
%	 points= "(12.5,70);(12.5,70);(27.5,55);(27.5,55)"
%	 stroke-width= "0.5"
%	 />
%<multicurve fill-style= "none"
%	 points= "(20,75);(20,75);(20,62.5);(20,62.5)"
%	 stroke-width= "0.5"
%	 />
%<multicurve fill-style= "none"
%	 points= "(95,40);(95,40);(105,40);(105,40)"
%	 stroke-width= "0.5"
%	 />
%<multicurve fill-style= "none"
%	 points= "(85,50);(85,50);(95,50);(95,50)"
%	 stroke-width= "0.5"
%	 />
%<multicurve fill-style= "none"
%	 points= "(100,0);(100,0);(100,40);(100,40)"
%	 stroke-width= "0.5"
%	 />
%<multicurve fill-style= "none"
%	 points= "(95,50);(95,50);(105,40);(105,40)"
%	 stroke-width= "0.5"
%	 />
%<multicurve fill-style= "none"
%	 points= "(85,50);(85,50);(95,40);(95,40)"
%	 stroke-width= "0.5"
%	 />
%<multicurve fill-style= "none"
%	 points= "(85,42.5);(85,42.5);(95,32.5);(95,32.5)"
%	 stroke-width= "0.5"
%	 />
%<multicurve fill-style= "none"
%	 points= "(100,45);(100,45);(100,55);(100,55)"
%	 stroke-width= "0.5"
%	 />
%<multicurve fill-style= "none"
%	 points= "(90,37.5);(90,37.5);(90,45);(90,45)"
%	 stroke-width= "0.5"
%	 />
%<multicurve fill-style= "none"
%	 points= "(85,32.5);(85,32.5);(95,32.5);(95,32.5)"
%	 stroke-width= "0.5"
%	 />
%<multicurve fill-style= "none"
%	 points= "(85,42.5);(85,42.5);(85,32.5);(85,32.5)"
%	 stroke-width= "0.5"
%	 />
%<multicurve fill-style= "none"
%	 points= "(105,60);(105,60);(105,50);(105,50)"
%	 stroke-width= "0.5"
%	 />
%<multicurve fill-style= "none"
%	 points= "(100,75);(100,75);(100,60);(100,60)"
%	 stroke-width= "0.5"
%	 />
%<multicurve fill-style= "none"
%	 points= "(95,60);(95,60);(105,50);(105,50)"
%	 stroke-width= "0.5"
%	 />
%<multicurve fill-style= "none"
%	 points= "(105,60);(105,60);(95,60);(95,60)"
%	 stroke-width= "0.5"
%	 />
%<multicurve fill-style= "none"
%	 points= "(55,40);(55,40);(65,40);(65,40)"
%	 stroke-width= "0.5"
%	 />
%<multicurve fill-style= "none"
%	 points= "(45,50);(45,50);(65,50);(65,50)"
%	 stroke-width= "0.5"
%	 />
%<multicurve fill-style= "none"
%	 points= "(60,0);(60,0);(60,40);(60,40)"
%	 stroke-width= "0.5"
%	 />
%<multicurve fill-style= "none"
%	 points= "(45,50);(45,50);(55,40);(55,40)"
%	 stroke-width= "0.5"
%	 />
%<multicurve fill-style= "none"
%	 points= "(45,42.5);(45,42.5);(55,32.5);(55,32.5)"
%	 stroke-width= "0.5"
%	 />
%<multicurve fill-style= "none"
%	 points= "(50,37.5);(50,37.5);(50,45);(50,45)"
%	 stroke-width= "0.5"
%	 />
%<multicurve fill-style= "none"
%	 points= "(45,32.5);(45,32.5);(55,32.5);(55,32.5)"
%	 stroke-width= "0.5"
%	 />
%<multicurve fill-style= "none"
%	 points= "(45,42.5);(45,42.5);(45,32.5);(45,32.5)"
%	 stroke-width= "0.5"
%	 />
%<multicurve fill-style= "none"
%	 points= "(65,50);(65,50);(65,40);(65,40)"
%	 stroke-width= "0.5"
%	 />
%<multicurve fill-style= "none"
%	 points= "(60,75);(60,75);(60,50);(60,50)"
%	 stroke-width= "0.5"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "solid"
%	 anchor-point= "(35,45)"
%	 text-frame= "noframe"
%	 stroke-width= "0.5"
%	 text-hor-align= "center-h"
%	 >
%\EQLS
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "solid"
%	 anchor-point= "(75,45)"
%	 text-frame= "noframe"
%	 stroke-width= "0.5"
%	 text-hor-align= "center-h"
%	 >
%\EQLS
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "solid"
%	 anchor-point= "(2.5,35)"
%	 text-frame= "noframe"
%	 stroke-width= "0.5"
%	 text-hor-align= "center-h"
%	 >
%$\Nee$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "solid"
%	 anchor-point= "(47.5,35)"
%	 text-frame= "noframe"
%	 stroke-width= "0.5"
%	 text-hor-align= "center-h"
%	 >
%$\Nee$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "solid"
%	 anchor-point= "(15,25)"
%	 text-frame= "noframe"
%	 stroke-width= "0.5"
%	 text-hor-align= "center-h"
%	 >
%$\addd$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "solid"
%	 anchor-point= "(87.5,35)"
%	 text-frame= "noframe"
%	 stroke-width= "0.5"
%	 text-hor-align= "center-h"
%	 >
%$\Nee$
%</text>
%<multicurve fill-style= "solid"
%	 points= "(-2.5,52.5);(-2.5,52.5);(12.5,52.5);(12.5,52.5)"
%	 stroke-width= "0.15"
%	 />
%<multicurve fill-style= "solid"
%	 points= "(-2.5,30);(-2.5,30);(-2.5,52.5);(-2.5,52.5)"
%	 stroke-width= "0.15"
%	 />
%<multicurve fill-style= "solid"
%	 points= "(22.5,30);(22.5,30);(-2.5,30);(-2.5,30)"
%	 stroke-width= "0.15"
%	 />
%<multicurve fill-style= "solid"
%	 points= "(22.5,42.5);(22.5,42.5);(22.5,30);(22.5,30)"
%	 stroke-width= "0.15"
%	 />
%<multicurve fill-style= "solid"
%	 points= "(12.5,52.5);(12.5,52.5);(22.5,42.5);(22.5,42.5)"
%	 stroke-width= "0.15"
%	 />
%<multicurve fill-style= "solid"
%	 points= "(82.5,52.5);(82.5,52.5);(97.5,52.5);(97.5,52.5)"
%	 stroke-width= "0.15"
%	 />
%<multicurve fill-style= "solid"
%	 points= "(82.5,30);(82.5,30);(82.5,52.5);(82.5,52.5)"
%	 stroke-width= "0.15"
%	 />
%<multicurve fill-style= "solid"
%	 points= "(107.5,30);(107.5,30);(82.5,30);(82.5,30)"
%	 stroke-width= "0.15"
%	 />
%<multicurve fill-style= "solid"
%	 points= "(107.5,42.5);(107.5,42.5);(107.5,30);(107.5,30)"
%	 stroke-width= "0.15"
%	 />
%<multicurve fill-style= "solid"
%	 points= "(97.5,52.5);(97.5,52.5);(107.5,42.5);(107.5,42.5)"
%	 stroke-width= "0.15"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "solid"
%	 anchor-point= "(105,32.5)"
%	 text-frame= "noframe"
%	 stroke-width= "0.5"
%	 text-hor-align= "center-h"
%	 >
%$\Homega$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "solid"
%	 anchor-point= "(20,32.5)"
%	 text-frame= "noframe"
%	 stroke-width= "0.5"
%	 text-hor-align= "center-h"
%	 >
%$\Homega$
%</text>
%</jpic>
%%End JPIC-XML
%PSTricks content-type (pstricks.sty package needed)
%Add \usepackage{pstricks} in the preamble of your LaTeX file
%You can rescale the whole picture (to 80% for instance) by using the command \def\JPicScale{0.8}
\ifx\JPicScale\undefined\def\JPicScale{1}\fi
\psset{unit=\JPicScale mm}
\psset{linewidth=0.3,dotsep=1,hatchwidth=0.3,hatchsep=1.5,shadowsize=1,dimen=middle}
\psset{dotsize=0.7 2.5,dotscale=1 1,fillcolor=black}
\psset{arrowsize=1 2,arrowlength=1,arrowinset=0.25,tbarsize=0.7 5,bracketlength=0.15,rbracketlength=0.15}
\begin{pspicture}(0,0)(107.5,75)
\psline[linewidth=0.5](20,10)(20,0)
\rput{0}(20,10){\psellipse[linewidth=0.5,fillstyle=solid](0,0)(1.25,-1.25)}
\psline[linewidth=0.5](25,15)(20,10)
\psline[linewidth=0.5](20,10)(15,15)
\psline[linewidth=0.5](15,15)(15,21.25)
\psline[linewidth=0.5](25,15)(25,55)
\psline[linewidth=0.5](10,40)(20,40)
\psline[linewidth=0.5](0,50)(10,50)
\rput{0}(15,25){\psellipse[linewidth=0.5](0,0)(3.52,-3.52)}
\psline[linewidth=0.5](15,28.75)(15,40)
\psline[linewidth=0.5](10,50)(20,40)
\psline[linewidth=0.5](0,50)(10,40)
\psline[linewidth=0.5](0,42.5)(10,32.5)
\psline[linewidth=0.5](15,45)(15,55)
\psline[linewidth=0.5](5,37.5)(5,45)
\psline[linewidth=0.5](0,32.5)(10,32.5)
\psline[linewidth=0.5](0,42.5)(0,32.5)
\psline[linewidth=0.5](12.5,55)(27.5,55)
\psline[linewidth=0.5](12.5,70)(12.5,55)
\psline[linewidth=0.5](12.5,70)(27.5,55)
\psline[linewidth=0.5](20,75)(20,62.5)
\psline[linewidth=0.5](95,40)(105,40)
\psline[linewidth=0.5](85,50)(95,50)
\psline[linewidth=0.5](100,0)(100,40)
\psline[linewidth=0.5](95,50)(105,40)
\psline[linewidth=0.5](85,50)(95,40)
\psline[linewidth=0.5](85,42.5)(95,32.5)
\psline[linewidth=0.5](100,45)(100,55)
\psline[linewidth=0.5](90,37.5)(90,45)
\psline[linewidth=0.5](85,32.5)(95,32.5)
\psline[linewidth=0.5](85,42.5)(85,32.5)
\psline[linewidth=0.5](105,60)(105,50)
\psline[linewidth=0.5](100,75)(100,60)
\psline[linewidth=0.5](95,60)(105,50)
\psline[linewidth=0.5](105,60)(95,60)
\psline[linewidth=0.5](55,40)(65,40)
\psline[linewidth=0.5](45,50)(65,50)
\psline[linewidth=0.5](60,0)(60,40)
\psline[linewidth=0.5](45,50)(55,40)
\psline[linewidth=0.5](45,42.5)(55,32.5)
\psline[linewidth=0.5](50,37.5)(50,45)
\psline[linewidth=0.5](45,32.5)(55,32.5)
\psline[linewidth=0.5](45,42.5)(45,32.5)
\psline[linewidth=0.5](65,50)(65,40)
\psline[linewidth=0.5](60,75)(60,50)
\rput(35,45){\EQLS}
\rput(75,45){\EQLS}
\rput(2.5,35){$\Nee$}
\rput(47.5,35){$\Nee$}
\rput(15,25){$\addd$}
\rput(87.5,35){$\Nee$}
\psline[linewidth=0.15,fillstyle=solid](-2.5,52.5)(12.5,52.5)
\psline[linewidth=0.15,fillstyle=solid](-2.5,30)(-2.5,52.5)
\psline[linewidth=0.15,fillstyle=solid](22.5,30)(-2.5,30)
\psline[linewidth=0.15,fillstyle=solid](22.5,42.5)(22.5,30)
\psline[linewidth=0.15,fillstyle=solid](12.5,52.5)(22.5,42.5)
\psline[linewidth=0.15,fillstyle=solid](82.5,52.5)(97.5,52.5)
\psline[linewidth=0.15,fillstyle=solid](82.5,30)(82.5,52.5)
\psline[linewidth=0.15,fillstyle=solid](107.5,30)(82.5,30)
\psline[linewidth=0.15,fillstyle=solid](107.5,42.5)(107.5,30)
\psline[linewidth=0.15,fillstyle=solid](97.5,52.5)(107.5,42.5)
\rput(105,32.5){$\Homega$}
\rput(20,32.5){$\Homega$}
\end{pspicture}


==> PIC/PR-dotdiv.tex <==
%%Created by jPicEdt 1.4.1_03: mixed JPIC-XML/LaTeX format
%%Tue Nov 28 12:44:15 HST 2017
%%Begin JPIC-XML
%<?xml version="1.0" standalone="yes"?>
%<jpic x-min="-5" x-max="235" y-min="0" y-max="215" auto-bounding="true">
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(180,130);(180,130);(235,130);(235,130)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(235,110);(235,110);(235,130);(235,130)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(200,110);(200,110);(235,110);(235,110)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(190,120);(190,120);(10,30);(10,30)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(180,130);(180,130);(200,110);(200,110)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(170,20);(170,20);(170,0);(170,0)"
%	 />
%<multicurve stroke-width= "0.6"
%	 fill-style= "none"
%	 points= "(100,20);(100,20);(205,70);(205,70)"
%	 />
%<text text-vert-align= "center-v"
%	 anchor-point= "(215,120)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\utag$
%</text>
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(30,140);(30,140);(30,55);(30,55)"
%	 />
%<multicurve stroke-width= "0.6"
%	 fill-style= "none"
%	 points= "(10,160);(10,160);(50,160);(50,160)"
%	 />
%<multicurve stroke-width= "0.6"
%	 fill-style= "none"
%	 points= "(50,140);(50,140);(50,160);(50,160)"
%	 />
%<multicurve stroke-width= "0.6"
%	 fill-style= "none"
%	 points= "(10,140);(10,140);(50,140);(50,140)"
%	 />
%<multicurve stroke-width= "0.6"
%	 fill-style= "none"
%	 points= "(10,160);(10,160);(10,140);(10,140)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(30,170);(30,170);(30,160);(30,160)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(100,20);(100,20);(100,0);(100,0)"
%	 />
%<multicurve stroke-overstrike= "true"
%	 stroke-width= "0.6"
%	 stroke-overstrike-width= "2"
%	 fill-style= "none"
%	 points= "(30,55);(30,55);(100,20);(100,20)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(30,185);(30,185);(30,160);(30,160)"
%	 />
%<multicurve stroke-width= "0.6"
%	 fill-style= "none"
%	 points= "(20,195);(20,195);(235,195);(235,195)"
%	 />
%<multicurve stroke-width= "0.6"
%	 fill-style= "none"
%	 points= "(235,175);(235,175);(235,195);(235,195)"
%	 />
%<multicurve stroke-width= "0.6"
%	 fill-style= "none"
%	 points= "(40,175);(40,175);(235,175);(235,175)"
%	 />
%<multicurve stroke-width= "0.6"
%	 fill-style= "none"
%	 points= "(20,195);(20,195);(40,175);(40,175)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(135,215);(135,215);(135,195);(135,195)"
%	 />
%<multicurve stroke-width= "0.6"
%	 fill-style= "none"
%	 points= "(170,20);(170,20);(230,50);(230,50)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(230,110);(230,110);(230,50);(230,50)"
%	 />
%<multicurve stroke-width= "0.6"
%	 fill-style= "none"
%	 points= "(220,80);(220,80);(220,100);(220,100)"
%	 />
%<multicurve stroke-width= "0.6"
%	 fill-style= "none"
%	 points= "(190,80);(190,80);(220,80);(220,80)"
%	 />
%<multicurve stroke-width= "0.6"
%	 fill-style= "none"
%	 points= "(190,100);(190,100);(190,80);(190,80)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(205,110);(205,110);(205,100);(205,100)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(205,80);(205,80);(205,70);(205,70)"
%	 />
%<ellipse p3= "(102.57,17.42)"
%	 p2= "(102.57,22.58)"
%	 p1= "(97.43,22.58)"
%	 closure= "open"
%	 fill-style= "solid"
%	 angle-end= "0"
%	 fill-color= "#330033"
%	 angle-start= "0"
%	 />
%<text text-vert-align= "center-v"
%	 anchor-point= "(30,150)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\zerotag$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(135,185)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\iiftag$
%</text>
%<multicurve stroke-overstrike= "true"
%	 stroke-width= "0.75"
%	 stroke-overstrike-width= "2"
%	 fill-style= "none"
%	 points= "(100,175);(100,175);(100,55);(100,55)"
%	 />
%<multicurve stroke-overstrike= "true"
%	 stroke-width= "0.6"
%	 stroke-overstrike-width= "2"
%	 fill-style= "none"
%	 points= "(170,20);(170,20);(100,55);(100,55)"
%	 />
%<ellipse p3= "(172.57,17.42)"
%	 p2= "(172.57,22.58)"
%	 p1= "(167.43,22.58)"
%	 closure= "open"
%	 fill-style= "solid"
%	 angle-end= "0"
%	 fill-color= "#330033"
%	 angle-start= "0"
%	 />
%<text text-vert-align= "center-v"
%	 anchor-point= "(205,90)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\predtag$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(98.12,5.62)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\een$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(168.75,5.62)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\eex$
%</text>
%<multicurve stroke-width= "0.6"
%	 fill-style= "none"
%	 points= "(190,100);(190,100);(220,100);(220,100)"
%	 />
%<multicurve stroke-width= "0.6"
%	 fill-style= "none"
%	 points= "(230,140);(230,140);(230,160);(230,160)"
%	 />
%<multicurve stroke-width= "0.6"
%	 fill-style= "none"
%	 points= "(200,140);(200,140);(230,140);(230,140)"
%	 />
%<multicurve stroke-width= "0.6"
%	 fill-style= "none"
%	 points= "(200,160);(200,160);(200,140);(200,140)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(215,175);(215,175);(215,160);(215,160)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(215,140);(215,140);(215,130);(215,130)"
%	 />
%<text text-vert-align= "center-v"
%	 anchor-point= "(215,150)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\predtag$
%</text>
%<multicurve stroke-width= "0.6"
%	 fill-style= "none"
%	 points= "(200,160);(200,160);(230,160);(230,160)"
%	 />
%<multicurve stroke-width= "0.6"
%	 fill-style= "none"
%	 points= "(-5,30);(-5,30);(25,0);(25,0)"
%	 />
%<multicurve stroke-width= "0.6"
%	 fill-style= "none"
%	 points= "(25,0);(25,0);(-5,0);(-5,0)"
%	 />
%<multicurve stroke-width= "0.6"
%	 fill-style= "none"
%	 points= "(-5,0);(-5,0);(-5,30);(-5,30)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(10,30);(10,30);(10,15);(10,15)"
%	 />
%<text text-vert-align= "center-v"
%	 anchor-point= "(5,10)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\function$
%</text>
%</jpic>
%%End JPIC-XML
%PSTricks content-type (pstricks.sty package needed)
%Add \usepackage{pstricks} in the preamble of your LaTeX file
%You can rescale the whole picture (to 80% for instance) by using the command \def\JPicScale{0.8}
\ifx\JPicScale\undefined\def\JPicScale{1}\fi
\psset{unit=\JPicScale mm}
\psset{linewidth=0.3,dotsep=1,hatchwidth=0.3,hatchsep=1.5,shadowsize=1,dimen=middle}
\psset{dotsize=0.7 2.5,dotscale=1 1,fillcolor=black}
\psset{arrowsize=1 2,arrowlength=1,arrowinset=0.25,tbarsize=0.7 5,bracketlength=0.15,rbracketlength=0.15}
\begin{pspicture}(0,0)(235,215)
\psline[linewidth=0.75](180,130)(235,130)
\psline[linewidth=0.75](235,110)(235,130)
\psline[linewidth=0.75](200,110)(235,110)
\psline[linewidth=0.75](190,120)(10,30)
\psline[linewidth=0.75](180,130)(200,110)
\psline[linewidth=0.75](170,20)(170,0)
\psline[linewidth=0.6](100,20)(205,70)
\rput(215,120){$\utag$}
\psline[linewidth=0.75](30,140)(30,55)
\psline[linewidth=0.6](10,160)(50,160)
\psline[linewidth=0.6](50,140)(50,160)
\psline[linewidth=0.6](10,140)(50,140)
\psline[linewidth=0.6](10,160)(10,140)
\psline[linewidth=0.75](30,170)(30,160)
\psline[linewidth=0.75](100,20)(100,0)
\psline[linewidth=0.6,border=2](30,55)(100,20)
\psline[linewidth=0.75](30,185)(30,160)
\psline[linewidth=0.6](20,195)(235,195)
\psline[linewidth=0.6](235,175)(235,195)
\psline[linewidth=0.6](40,175)(235,175)
\psline[linewidth=0.6](20,195)(40,175)
\psline[linewidth=0.75](135,215)(135,195)
\psline[linewidth=0.6](170,20)(230,50)
\psline[linewidth=0.75](230,110)(230,50)
\psline[linewidth=0.6](220,80)(220,100)
\psline[linewidth=0.6](190,80)(220,80)
\psline[linewidth=0.6](190,100)(190,80)
\psline[linewidth=0.75](205,110)(205,100)
\psline[linewidth=0.75](205,80)(205,70)
\newrgbcolor{userFillColour}{0.2 0 0.2}
\rput{90}(100,20){\psellipse[fillcolor=userFillColour,fillstyle=solid](0,0)(2.58,-2.57)}
\rput(30,150){$\zerotag$}
\rput(135,185){$\iiftag$}
\psline[linewidth=0.75,border=2](100,175)(100,55)
\psline[linewidth=0.6,border=2](170,20)(100,55)
\newrgbcolor{userFillColour}{0.2 0 0.2}
\rput{90}(170,20){\psellipse[fillcolor=userFillColour,fillstyle=solid](0,0)(2.58,-2.57)}
\rput(205,90){$\predtag$}
\rput[r](98.12,5.62){$\een$}
\rput[r](168.75,5.62){$\eex$}
\psline[linewidth=0.6](190,100)(220,100)
\psline[linewidth=0.6](230,140)(230,160)
\psline[linewidth=0.6](200,140)(230,140)
\psline[linewidth=0.6](200,160)(200,140)
\psline[linewidth=0.75](215,175)(215,160)
\psline[linewidth=0.75](215,140)(215,130)
\rput(215,150){$\predtag$}
\psline[linewidth=0.6](200,160)(230,160)
\psline[linewidth=0.6](-5,30)(25,0)
\psline[linewidth=0.6](25,0)(-5,0)
\psline[linewidth=0.6](-5,0)(-5,30)
\psline[linewidth=0.75](10,30)(10,15)
\rput(5,10){$\function$}
\end{pspicture}


==> PIC/PR-round.tex <==
%%Created by jPicEdt 1.4.1_03: mixed JPIC-XML/LaTeX format
%%Sun Jan 03 10:33:21 GMT-10:00 2021
%%Begin JPIC-XML
%<?xml version="1.0" standalone="yes"?>
%<jpic x-min="0" x-max="340" y-min="0" y-max="260" auto-bounding="true">
%<multicurve fill-style= "none"
%	 points= "(200,205);(200,205);(290,205);(290,205)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(290,185);(290,185);(290,205);(290,205)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(245,220);(245,220);(245,205);(245,205)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(280,185);(280,185);(280,100);(280,100)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(200,205);(200,205);(200,185);(200,185)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(120,205);(120,205);(160,205);(160,205)"
%	 stroke-width= "0.6"
%	 />
%<multicurve fill-style= "none"
%	 points= "(160,185);(160,185);(160,205);(160,205)"
%	 stroke-width= "0.6"
%	 />
%<multicurve fill-style= "none"
%	 points= "(120,205);(120,205);(120,185);(120,185)"
%	 stroke-width= "0.6"
%	 />
%<multicurve fill-style= "none"
%	 points= "(140,220);(140,220);(140,205);(140,205)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(220,175);(220,175);(262.5,175);(262.5,175)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(262.5,155);(262.5,155);(262.5,175);(262.5,175)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(245,185);(245,185);(245,175);(245,175)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(240,155);(240,155);(262.5,155);(262.5,155)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(230,165);(230,165);(70,85);(70,85)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(220,175);(220,175);(240,155);(240,155)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(210,65);(210,65);(210,0);(210,0)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(140,65);(140,65);(210,100);(210,100)"
%	 stroke-width= "0.6"
%	 />
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(247.5,165)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\utag$
%</text>
%<multicurve fill-style= "none"
%	 points= "(70,185);(70,185);(70,100);(70,100)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(50,205);(50,205);(90,205);(90,205)"
%	 stroke-width= "0.6"
%	 />
%<multicurve fill-style= "none"
%	 points= "(90,185);(90,185);(90,205);(90,205)"
%	 stroke-width= "0.6"
%	 />
%<multicurve fill-style= "none"
%	 points= "(50,185);(50,185);(90,185);(90,185)"
%	 stroke-width= "0.6"
%	 />
%<multicurve fill-style= "none"
%	 points= "(50,205);(50,205);(50,185);(50,185)"
%	 stroke-width= "0.6"
%	 />
%<multicurve fill-style= "none"
%	 points= "(70,215);(70,215);(70,205);(70,205)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(140,65);(140,65);(140,0);(140,0)"
%	 stroke-width= "0.75"
%	 />
%<multicurve stroke-overstrike= "true"
%	 fill-style= "none"
%	 points= "(70,100);(70,100);(140,65);(140,65)"
%	 stroke-width= "0.6"
%	 stroke-overstrike-width= "2"
%	 />
%<multicurve fill-style= "none"
%	 points= "(70,230);(70,230);(70,205);(70,205)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(60,240);(60,240);(270,240);(270,240)"
%	 stroke-width= "0.6"
%	 />
%<multicurve fill-style= "none"
%	 points= "(270,220);(270,220);(270,240);(270,240)"
%	 stroke-width= "0.6"
%	 />
%<multicurve fill-style= "none"
%	 points= "(80,220);(80,220);(270,220);(270,220)"
%	 stroke-width= "0.6"
%	 />
%<multicurve fill-style= "none"
%	 points= "(60,240);(60,240);(80,220);(80,220)"
%	 stroke-width= "0.6"
%	 />
%<multicurve fill-style= "none"
%	 points= "(175,260);(175,260);(175,240);(175,240)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(210,65);(210,65);(280,100);(280,100)"
%	 stroke-width= "0.6"
%	 />
%<multicurve fill-style= "none"
%	 points= "(255,155);(255,155);(255,145);(255,145)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(225,105);(225,105);(225,120);(225,120)"
%	 stroke-width= "0.6"
%	 />
%<multicurve fill-style= "none"
%	 points= "(195,105);(195,105);(225,105);(225,105)"
%	 stroke-width= "0.6"
%	 />
%<multicurve fill-style= "none"
%	 points= "(195,120);(195,120);(195,105);(195,105)"
%	 stroke-width= "0.6"
%	 />
%<multicurve fill-style= "none"
%	 points= "(245,155);(245,155);(245,145);(245,145)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(210,105);(210,105);(210,100);(210,100)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(70,85);(70,85);(70,35);(70,35)"
%	 stroke-width= "0.75"
%	 />
%<ellipse fill-style= "solid"
%	 p3= "(142.57,62.42)"
%	 fill-color= "#330033"
%	 p2= "(142.57,67.58)"
%	 p1= "(137.43,67.58)"
%	 closure= "open"
%	 angle-end= "0"
%	 angle-start= "0"
%	 />
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(140,195)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\gtag$
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(70,195)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\zerotag$
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(175,230)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\iiftag$
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(245,195)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\htag$
%</text>
%<multicurve stroke-overstrike= "true"
%	 fill-style= "none"
%	 points= "(210,185);(210,185);(210,120);(210,120)"
%	 stroke-width= "0.75"
%	 stroke-overstrike-width= "2"
%	 />
%<ellipse fill-style= "solid"
%	 p3= "(212.57,124.92)"
%	 fill-color= "#330033"
%	 p2= "(212.57,130.08)"
%	 p1= "(207.43,130.08)"
%	 closure= "open"
%	 angle-end= "0"
%	 angle-start= "0"
%	 />
%<multicurve fill-style= "none"
%	 points= "(200,185);(200,185);(290,185);(290,185)"
%	 stroke-width= "0.75"
%	 />
%<multicurve stroke-overstrike= "true"
%	 fill-style= "none"
%	 points= "(140,185);(140,185);(140,100);(140,100)"
%	 stroke-width= "0.75"
%	 stroke-overstrike-width= "2"
%	 />
%<multicurve fill-style= "none"
%	 points= "(120,185);(120,185);(160,185);(160,185)"
%	 stroke-width= "0.6"
%	 />
%<multicurve stroke-overstrike= "true"
%	 fill-style= "none"
%	 points= "(210,65);(210,65);(140,100);(140,100)"
%	 stroke-width= "0.6"
%	 stroke-overstrike-width= "2"
%	 />
%<ellipse fill-style= "solid"
%	 p3= "(212.57,62.42)"
%	 fill-color= "#330033"
%	 p2= "(212.57,67.58)"
%	 p1= "(207.43,67.58)"
%	 closure= "open"
%	 angle-end= "0"
%	 angle-start= "0"
%	 />
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(210,112.5)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\predtag$
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(68.12,75)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\pee$
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(138.75,2.5)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\een$
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(207.5,2.5)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\eex$
%</text>
%<multicurve fill-style= "none"
%	 points= "(210,127.5);(210,127.5);(245,145);(245,145)"
%	 stroke-width= "0.6"
%	 />
%<multicurve fill-style= "none"
%	 points= "(195,120);(195,120);(225,120);(225,120)"
%	 stroke-width= "0.6"
%	 />
%<ellipse fill-style= "solid"
%	 p3= "(282.57,129.92)"
%	 fill-color= "#330033"
%	 p2= "(282.57,135.08)"
%	 p1= "(277.43,135.08)"
%	 closure= "open"
%	 angle-end= "0"
%	 angle-start= "0"
%	 />
%<multicurve fill-style= "none"
%	 points= "(255,145);(255,145);(280,132.5);(280,132.5)"
%	 stroke-width= "0.6"
%	 />
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(177.5,256.88)"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\Beh$
%</text>
%<parallelogram fill-style= "none"
%	 p3= "(45,55)"
%	 p2= "(45,245)"
%	 p1= "(295,245)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(60,45);(60,45);(80,25);(80,25)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(60,45);(60,45);(60,25);(60,25)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(60,25);(60,25);(80,25);(80,25)"
%	 stroke-width= "0.75"
%	 />
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(65.62,31.25)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\Ftilde$
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(260,35)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\function$
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(270,70)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\ftilde$
%</text>
%<ellipse fill-style= "none"
%	 p3= "(340,15)"
%	 p2= "(340,250)"
%	 p1= "(260,250)"
%	 closure= "open"
%	 angle-end= "90"
%	 angle-start= "-90"
%	 />
%<multicurve fill-style= "none"
%	 points= "(40,15);(40,15);(300,15);(300,15)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(40,250);(40,250);(300,250);(300,250)"
%	 />
%<ellipse fill-style= "none"
%	 p3= "(80,15)"
%	 p2= "(80,250)"
%	 p1= "(0,250)"
%	 closure= "open"
%	 angle-end= "271.89"
%	 angle-start= "88.15"
%	 />
%<ellipse fill-style= "none"
%	 p3= "(105,15)"
%	 p2= "(105,250)"
%	 p1= "(25,250)"
%	 closure= "open"
%	 angle-end= "271.89"
%	 angle-start= "88.15"
%	 />
%</jpic>
%%End JPIC-XML
%PSTricks content-type (pstricks.sty package needed)
%Add \usepackage{pstricks} in the preamble of your LaTeX file
%You can rescale the whole picture (to 80% for instance) by using the command \def\JPicScale{0.8}
\ifx\JPicScale\undefined\def\JPicScale{1}\fi
\psset{unit=\JPicScale mm}
\psset{linewidth=0.3,dotsep=1,hatchwidth=0.3,hatchsep=1.5,shadowsize=1,dimen=middle}
\psset{dotsize=0.7 2.5,dotscale=1 1,fillcolor=black}
\psset{arrowsize=1 2,arrowlength=1,arrowinset=0.25,tbarsize=0.7 5,bracketlength=0.15,rbracketlength=0.15}
\begin{pspicture}(0,0)(340,260)
\psline[linewidth=0.75](200,205)(290,205)
\psline[linewidth=0.75](290,185)(290,205)
\psline[linewidth=0.75](245,220)(245,205)
\psline[linewidth=0.75](280,185)(280,100)
\psline[linewidth=0.75](200,205)(200,185)
\psline[linewidth=0.6](120,205)(160,205)
\psline[linewidth=0.6](160,185)(160,205)
\psline[linewidth=0.6](120,205)(120,185)
\psline[linewidth=0.75](140,220)(140,205)
\psline[linewidth=0.75](220,175)(262.5,175)
\psline[linewidth=0.75](262.5,155)(262.5,175)
\psline[linewidth=0.75](245,185)(245,175)
\psline[linewidth=0.75](240,155)(262.5,155)
\psline[linewidth=0.75](230,165)(70,85)
\psline[linewidth=0.75](220,175)(240,155)
\psline[linewidth=0.75](210,65)(210,0)
\psline[linewidth=0.6](140,65)(210,100)
\rput(247.5,165){$\utag$}
\psline[linewidth=0.75](70,185)(70,100)
\psline[linewidth=0.6](50,205)(90,205)
\psline[linewidth=0.6](90,185)(90,205)
\psline[linewidth=0.6](50,185)(90,185)
\psline[linewidth=0.6](50,205)(50,185)
\psline[linewidth=0.75](70,215)(70,205)
\psline[linewidth=0.75](140,65)(140,0)
\psline[linewidth=0.6,border=2](70,100)(140,65)
\psline[linewidth=0.75](70,230)(70,205)
\psline[linewidth=0.6](60,240)(270,240)
\psline[linewidth=0.6](270,220)(270,240)
\psline[linewidth=0.6](80,220)(270,220)
\psline[linewidth=0.6](60,240)(80,220)
\psline[linewidth=0.75](175,260)(175,240)
\psline[linewidth=0.6](210,65)(280,100)
\psline[linewidth=0.75](255,155)(255,145)
\psline[linewidth=0.6](225,105)(225,120)
\psline[linewidth=0.6](195,105)(225,105)
\psline[linewidth=0.6](195,120)(195,105)
\psline[linewidth=0.75](245,155)(245,145)
\psline[linewidth=0.75](210,105)(210,100)
\psline[linewidth=0.75](70,85)(70,35)
\newrgbcolor{userFillColour}{0.2 0 0.2}
\rput{90}(140,65){\psellipse[fillcolor=userFillColour,fillstyle=solid](0,0)(2.58,-2.57)}
\rput(140,195){$\gtag$}
\rput(70,195){$\zerotag$}
\rput(175,230){$\iiftag$}
\rput(245,195){$\htag$}
\psline[linewidth=0.75,border=2](210,185)(210,120)
\newrgbcolor{userFillColour}{0.2 0 0.2}
\rput{90}(210,127.5){\psellipse[fillcolor=userFillColour,fillstyle=solid](0,0)(2.58,-2.57)}
\psline[linewidth=0.75](200,185)(290,185)
\psline[linewidth=0.75,border=2](140,185)(140,100)
\psline[linewidth=0.6](120,185)(160,185)
\psline[linewidth=0.6,border=2](210,65)(140,100)
\newrgbcolor{userFillColour}{0.2 0 0.2}
\rput{90}(210,65){\psellipse[fillcolor=userFillColour,fillstyle=solid](0,0)(2.58,-2.57)}
\rput(210,112.5){$\predtag$}
\rput[r](68.12,75){$\pee$}
\rput[r](138.75,2.5){$\een$}
\rput[r](207.5,2.5){$\eex$}
\psline[linewidth=0.6](210,127.5)(245,145)
\psline[linewidth=0.6](195,120)(225,120)
\newrgbcolor{userFillColour}{0.2 0 0.2}
\rput{90}(280,132.5){\psellipse[fillcolor=userFillColour,fillstyle=solid](0,0)(2.58,-2.57)}
\psline[linewidth=0.6](255,145)(280,132.5)
\rput[l](177.5,256.88){$\Beh$}
\pspolygon[](295,245)(45,245)(45,55)(295,55)
\psline[linewidth=0.75](60,45)(80,25)
\psline[linewidth=0.75](60,45)(60,25)
\psline[linewidth=0.75](60,25)(80,25)
\rput(65.62,31.25){$\Ftilde$}
\rput(260,35){$\function$}
\rput(270,70){$\ftilde$}
\rput{90}(300,132.5){\psellipticarc[](0,0)(117.5,-40){-0}{180}}
\psline(40,15)(300,15)
\psline(40,250)(300,250)
\rput{90}(40,132.5){\psellipticarc[](0,0)(117.5,-40){180}{0}}
\end{pspicture}


==> PIC/PR-run.tex <==
%%Created by jPicEdt 1.4.1_03: mixed JPIC-XML/LaTeX format
%%Wed Dec 11 16:32:10 GMT-10:00 2019
%%Begin JPIC-XML
%<?xml version="1.0" standalone="yes"?>
%<jpic x-min="5" x-max="540" y-min="0" y-max="245" auto-bounding="true">
%<multicurve fill-style= "none"
%	 points= "(160,190);(160,190);(250,190);(250,190)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(250,170);(250,170);(250,190);(250,190)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(205,205);(205,205);(205,190);(205,190)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(240,170);(240,170);(240,75);(240,75)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(160,190);(160,190);(160,170);(160,170)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(80,190);(80,190);(120,190);(120,190)"
%	 stroke-width= "0.6"
%	 />
%<multicurve fill-style= "none"
%	 points= "(120,170);(120,170);(120,190);(120,190)"
%	 stroke-width= "0.6"
%	 />
%<multicurve fill-style= "none"
%	 points= "(80,190);(80,190);(80,170);(80,170)"
%	 stroke-width= "0.6"
%	 />
%<multicurve fill-style= "none"
%	 points= "(100,205);(100,205);(100,190);(100,190)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(180,160);(180,160);(220,160);(220,160)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(220,140);(220,140);(220,160);(220,160)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(205,170);(205,170);(205,160);(205,160)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(200,140);(200,140);(220,140);(220,140)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(190,150);(190,150);(190,140);(190,140)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(180,160);(180,160);(200,140);(200,140)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(170,40);(170,40);(170,0);(170,0)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(100,40);(100,40);(170,75);(170,75)"
%	 stroke-width= "0.6"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(207.5,150)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\utag$
%</text>
%<multicurve fill-style= "none"
%	 points= "(30,170);(30,170);(30,75);(30,75)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(10,190);(10,190);(50,190);(50,190)"
%	 stroke-width= "0.6"
%	 />
%<multicurve fill-style= "none"
%	 points= "(50,170);(50,170);(50,190);(50,190)"
%	 stroke-width= "0.6"
%	 />
%<multicurve fill-style= "none"
%	 points= "(10,170);(10,170);(50,170);(50,170)"
%	 stroke-width= "0.6"
%	 />
%<multicurve fill-style= "none"
%	 points= "(10,190);(10,190);(10,170);(10,170)"
%	 stroke-width= "0.6"
%	 />
%<multicurve fill-style= "none"
%	 points= "(30,200);(30,200);(30,190);(30,190)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(100,40);(100,40);(100,0);(100,0)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 stroke-overstrike-width= "2"
%	 points= "(30,75);(30,75);(100,40);(100,40)"
%	 stroke-overstrike= "true"
%	 stroke-width= "0.6"
%	 />
%<multicurve fill-style= "none"
%	 points= "(30,215);(30,215);(30,190);(30,190)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(20,225);(20,225);(230,225);(230,225)"
%	 stroke-width= "0.6"
%	 />
%<multicurve fill-style= "none"
%	 points= "(230,205);(230,205);(230,225);(230,225)"
%	 stroke-width= "0.6"
%	 />
%<multicurve fill-style= "none"
%	 points= "(40,205);(40,205);(230,205);(230,205)"
%	 stroke-width= "0.6"
%	 />
%<multicurve fill-style= "none"
%	 points= "(20,225);(20,225);(40,205);(40,205)"
%	 stroke-width= "0.6"
%	 />
%<multicurve fill-style= "none"
%	 points= "(135,245);(135,245);(135,225);(135,225)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(170,40);(170,40);(240,75);(240,75)"
%	 stroke-width= "0.6"
%	 />
%<multicurve fill-style= "none"
%	 points= "(215,140);(215,140);(215,120);(215,120)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(185,80);(185,80);(185,95);(185,95)"
%	 stroke-width= "0.6"
%	 />
%<multicurve fill-style= "none"
%	 points= "(155,80);(155,80);(185,80);(185,80)"
%	 stroke-width= "0.6"
%	 />
%<multicurve fill-style= "none"
%	 points= "(155,95);(155,95);(155,80);(155,80)"
%	 stroke-width= "0.6"
%	 />
%<multicurve fill-style= "none"
%	 points= "(205,140);(205,140);(205,120);(205,120)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(170,80);(170,80);(170,75);(170,75)"
%	 stroke-width= "0.75"
%	 />
%<ellipse p3= "(102.57,37.42)"
%	 fill-style= "solid"
%	 p2= "(102.57,42.58)"
%	 fill-color= "#330033"
%	 p1= "(97.43,42.58)"
%	 closure= "open"
%	 angle-end= "0"
%	 angle-start= "0"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(100,180)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\gtag$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(30,180)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\zerotag$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(135,215)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\iiftag$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(205,180)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\htag$
%</text>
%<multicurve fill-style= "none"
%	 stroke-overstrike-width= "2"
%	 points= "(170,170);(170,170);(170,95);(170,95)"
%	 stroke-overstrike= "true"
%	 stroke-width= "0.75"
%	 />
%<ellipse p3= "(172.57,99.92)"
%	 fill-style= "solid"
%	 p2= "(172.57,105.08)"
%	 fill-color= "#330033"
%	 p1= "(167.43,105.08)"
%	 closure= "open"
%	 angle-end= "0"
%	 angle-start= "0"
%	 />
%<multicurve fill-style= "none"
%	 points= "(160,170);(160,170);(250,170);(250,170)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 stroke-overstrike-width= "2"
%	 points= "(100,170);(100,170);(100,75);(100,75)"
%	 stroke-overstrike= "true"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(80,170);(80,170);(120,170);(120,170)"
%	 stroke-width= "0.6"
%	 />
%<multicurve fill-style= "none"
%	 stroke-overstrike-width= "2"
%	 points= "(170,40);(170,40);(100,75);(100,75)"
%	 stroke-overstrike= "true"
%	 stroke-width= "0.6"
%	 />
%<ellipse p3= "(172.57,37.42)"
%	 fill-style= "solid"
%	 p2= "(172.57,42.58)"
%	 fill-color= "#330033"
%	 p1= "(167.43,42.58)"
%	 closure= "open"
%	 angle-end= "0"
%	 angle-start= "0"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(170,87.5)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\predtag$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(97.5,1.25)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\een$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(167.5,1.25)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\eex$
%</text>
%<multicurve fill-style= "none"
%	 points= "(170,102.5);(170,102.5);(205,120);(205,120)"
%	 stroke-width= "0.6"
%	 />
%<multicurve fill-style= "none"
%	 points= "(155,95);(155,95);(185,95);(185,95)"
%	 stroke-width= "0.6"
%	 />
%<ellipse p3= "(242.57,104.92)"
%	 fill-style= "solid"
%	 p2= "(242.57,110.08)"
%	 fill-color= "#330033"
%	 p1= "(237.43,110.08)"
%	 closure= "open"
%	 angle-end= "0"
%	 angle-start= "0"
%	 />
%<multicurve fill-style= "none"
%	 points= "(215,120);(215,120);(240,107.5);(240,107.5)"
%	 stroke-width= "0.6"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(137.5,241.88)"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\Beh$
%</text>
%<parallelogram p3= "(5,30)"
%	 fill-style= "none"
%	 p2= "(5,230)"
%	 p1= "(255,230)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(180,150);(180,150);(200,130);(200,130)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(180,150);(180,150);(180,130);(180,130)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(180,130);(180,130);(200,130);(200,130)"
%	 stroke-width= "0.75"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(185.62,136.25)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\Ftilde$
%</text>
%<parallelogram p3= "(175,125)"
%	 fill-style= "none"
%	 p2= "(175,165)"
%	 p1= "(225,165)"
%	 stroke-color= "#ff0066"
%	 />
%<multicurve fill-style= "none"
%	 points= "(360,205);(360,205);(520,205);(520,205)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(520,125);(520,125);(520,205);(520,205)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(450,245);(450,245);(450,205);(450,205)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(440,125);(440,125);(520,125);(520,125)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(400,165);(400,165);(400,125);(400,125)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(510,125);(510,125);(510,0);(510,0)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(450,125);(450,125);(450,0);(450,0)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(360,165);(360,165);(440,85);(440,85)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(360,165);(360,165);(360,85);(360,85)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(360,85);(360,85);(440,85);(440,85)"
%	 stroke-width= "0.75"
%	 />
%<parallelogram p3= "(340,65)"
%	 fill-style= "none"
%	 p2= "(340,225)"
%	 p1= "(540,225)"
%	 stroke-color= "#ff0066"
%	 />
%<multicurve fill-style= "none"
%	 points= "(360,205);(360,205);(440,125);(440,125)"
%	 stroke-width= "0.75"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(295,135)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\EQLS
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(480,85)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\ftilde$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(447.5,2.5)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\een$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(507.5,2.5)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\eex$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(452.5,242.5)"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\Beh$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(385,110)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\bigFtilde
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(470,165)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\bigutag
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(225,45)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\function$
%</text>
%</jpic>
%%End JPIC-XML
%PSTricks content-type (pstricks.sty package needed)
%Add \usepackage{pstricks} in the preamble of your LaTeX file
%You can rescale the whole picture (to 80% for instance) by using the command \def\JPicScale{0.8}
\ifx\JPicScale\undefined\def\JPicScale{1}\fi
\psset{unit=\JPicScale mm}
\psset{linewidth=0.3,dotsep=1,hatchwidth=0.3,hatchsep=1.5,shadowsize=1,dimen=middle}
\psset{dotsize=0.7 2.5,dotscale=1 1,fillcolor=black}
\psset{arrowsize=1 2,arrowlength=1,arrowinset=0.25,tbarsize=0.7 5,bracketlength=0.15,rbracketlength=0.15}
\begin{pspicture}(0,0)(540,245)
\psline[linewidth=0.75](160,190)(250,190)
\psline[linewidth=0.75](250,170)(250,190)
\psline[linewidth=0.75](205,205)(205,190)
\psline[linewidth=0.75](240,170)(240,75)
\psline[linewidth=0.75](160,190)(160,170)
\psline[linewidth=0.6](80,190)(120,190)
\psline[linewidth=0.6](120,170)(120,190)
\psline[linewidth=0.6](80,190)(80,170)
\psline[linewidth=0.75](100,205)(100,190)
\psline[linewidth=0.75](180,160)(220,160)
\psline[linewidth=0.75](220,140)(220,160)
\psline[linewidth=0.75](205,170)(205,160)
\psline[linewidth=0.75](200,140)(220,140)
\psline[linewidth=0.75](190,150)(190,140)
\psline[linewidth=0.75](180,160)(200,140)
\psline[linewidth=0.75](170,40)(170,0)
\psline[linewidth=0.6](100,40)(170,75)
\rput(207.5,150){$\utag$}
\psline[linewidth=0.75](30,170)(30,75)
\psline[linewidth=0.6](10,190)(50,190)
\psline[linewidth=0.6](50,170)(50,190)
\psline[linewidth=0.6](10,170)(50,170)
\psline[linewidth=0.6](10,190)(10,170)
\psline[linewidth=0.75](30,200)(30,190)
\psline[linewidth=0.75](100,40)(100,0)
\psline[linewidth=0.6,border=2](30,75)(100,40)
\psline[linewidth=0.75](30,215)(30,190)
\psline[linewidth=0.6](20,225)(230,225)
\psline[linewidth=0.6](230,205)(230,225)
\psline[linewidth=0.6](40,205)(230,205)
\psline[linewidth=0.6](20,225)(40,205)
\psline[linewidth=0.75](135,245)(135,225)
\psline[linewidth=0.6](170,40)(240,75)
\psline[linewidth=0.75](215,140)(215,120)
\psline[linewidth=0.6](185,80)(185,95)
\psline[linewidth=0.6](155,80)(185,80)
\psline[linewidth=0.6](155,95)(155,80)
\psline[linewidth=0.75](205,140)(205,120)
\psline[linewidth=0.75](170,80)(170,75)
\newrgbcolor{userFillColour}{0.2 0 0.2}
\rput{90}(100,40){\psellipse[fillcolor=userFillColour,fillstyle=solid](0,0)(2.58,-2.57)}
\rput(100,180){$\gtag$}
\rput(30,180){$\zerotag$}
\rput(135,215){$\iiftag$}
\rput(205,180){$\htag$}
\psline[linewidth=0.75,border=2](170,170)(170,95)
\newrgbcolor{userFillColour}{0.2 0 0.2}
\rput{90}(170,102.5){\psellipse[fillcolor=userFillColour,fillstyle=solid](0,0)(2.58,-2.57)}
\psline[linewidth=0.75](160,170)(250,170)
\psline[linewidth=0.75,border=2](100,170)(100,75)
\psline[linewidth=0.6](80,170)(120,170)
\psline[linewidth=0.6,border=2](170,40)(100,75)
\newrgbcolor{userFillColour}{0.2 0 0.2}
\rput{90}(170,40){\psellipse[fillcolor=userFillColour,fillstyle=solid](0,0)(2.58,-2.57)}
\rput(170,87.5){$\predtag$}
\rput[r](97.5,1.25){$\een$}
\rput[r](167.5,1.25){$\eex$}
\psline[linewidth=0.6](170,102.5)(205,120)
\psline[linewidth=0.6](155,95)(185,95)
\newrgbcolor{userFillColour}{0.2 0 0.2}
\rput{90}(240,107.5){\psellipse[fillcolor=userFillColour,fillstyle=solid](0,0)(2.58,-2.57)}
\psline[linewidth=0.6](215,120)(240,107.5)
\rput[l](137.5,241.88){$\Beh$}
\pspolygon[](255,230)(5,230)(5,30)(255,30)
\psline[linewidth=0.75](180,150)(200,130)
\psline[linewidth=0.75](180,150)(180,130)
\psline[linewidth=0.75](180,130)(200,130)
\rput(185.62,136.25){$\Ftilde$}
\newrgbcolor{userLineColour}{1 0 0.4}
\pspolygon[linecolor=userLineColour](225,165)(175,165)(175,125)(225,125)
\psline[linewidth=0.75](360,205)(520,205)
\psline[linewidth=0.75](520,125)(520,205)
\psline[linewidth=0.75](450,245)(450,205)
\psline[linewidth=0.75](440,125)(520,125)
\psline[linewidth=0.75](400,165)(400,125)
\psline[linewidth=0.75](510,125)(510,0)
\psline[linewidth=0.75](450,125)(450,0)
\psline[linewidth=0.75](360,165)(440,85)
\psline[linewidth=0.75](360,165)(360,85)
\psline[linewidth=0.75](360,85)(440,85)
\newrgbcolor{userLineColour}{1 0 0.4}
\pspolygon[linecolor=userLineColour](540,225)(340,225)(340,65)(540,65)
\psline[linewidth=0.75](360,205)(440,125)
\rput(295,135){\EQLS}
\rput(480,85){$\ftilde$}
\rput[r](447.5,2.5){$\een$}
\rput[r](507.5,2.5){$\eex$}
\rput[l](452.5,242.5){$\Beh$}
\rput(385,110){\bigFtilde}
\rput(470,165){\bigutag}
\rput(225,45){$\function$}
\end{pspicture}


==> PIC/PR-sum.tex <==
%%Created by jPicEdt 1.4.1_03: mixed JPIC-XML/LaTeX format
%%Wed Dec 13 21:53:48 HST 2017
%%Begin JPIC-XML
%<?xml version="1.0" standalone="yes"?>
%<jpic x-min="-5" x-max="235" y-min="0" y-max="215" auto-bounding="true">
%<multicurve stroke-width= "0.75"
%	 points= "(175,130);(175,130);(210,130);(210,130)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.75"
%	 points= "(210,110);(210,110);(210,130);(210,130)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.75"
%	 points= "(195,110);(195,110);(210,110);(210,110)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.75"
%	 points= "(187.5,117.5);(187.5,117.5);(10,30);(10,30)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.75"
%	 points= "(175,130);(175,130);(195,110);(195,110)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.6"
%	 points= "(100,20);(100,20);(225,87.5);(225,87.5)"
%	 fill-style= "none"
%	 />
%<text text-vert-align= "center-v"
%	 anchor-point= "(200,120)"
%	 text-frame= "noframe"
%	 fill-style= "none"
%	 text-hor-align= "center-h"
%	 >
%$\utag$
%</text>
%<multicurve stroke-width= "0.75"
%	 points= "(30,140);(30,140);(30,55);(30,55)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.6"
%	 points= "(10,160);(10,160);(50,160);(50,160)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.6"
%	 points= "(50,140);(50,140);(50,160);(50,160)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.6"
%	 points= "(10,140);(10,140);(50,140);(50,140)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.6"
%	 points= "(10,160);(10,160);(10,140);(10,140)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.75"
%	 points= "(30,170);(30,170);(30,160);(30,160)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.75"
%	 points= "(100,20);(100,20);(100,0);(100,0)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-overstrike-width= "2"
%	 stroke-overstrike= "true"
%	 stroke-width= "0.6"
%	 points= "(30,55);(30,55);(100,20);(100,20)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.75"
%	 points= "(30,185);(30,185);(30,160);(30,160)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.6"
%	 points= "(20,195);(20,195);(235,195);(235,195)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.6"
%	 points= "(235,175);(235,175);(235,195);(235,195)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.6"
%	 points= "(20,195);(20,195);(40,175);(40,175)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.75"
%	 points= "(155,215);(155,215);(155,195);(155,195)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.6"
%	 points= "(210,85);(210,85);(210,105);(210,105)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.6"
%	 points= "(190,85);(190,85);(210,85);(210,85)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.6"
%	 points= "(190,105);(190,105);(190,85);(190,85)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.75"
%	 points= "(200,110);(200,110);(200,105);(200,105)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.75"
%	 points= "(200,85);(200,85);(200,73.75);(200,73.75)"
%	 fill-style= "none"
%	 />
%<text text-vert-align= "center-v"
%	 anchor-point= "(30,150)"
%	 text-frame= "noframe"
%	 fill-style= "none"
%	 text-hor-align= "center-h"
%	 >
%$\zerotag$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(155,185)"
%	 text-frame= "noframe"
%	 fill-style= "none"
%	 text-hor-align= "center-h"
%	 >
%$\iiftag$
%</text>
%<multicurve stroke-overstrike-width= "2"
%	 stroke-overstrike= "true"
%	 stroke-width= "0.75"
%	 points= "(100,175);(100,175);(100,20);(100,20)"
%	 fill-style= "none"
%	 />
%<text text-vert-align= "center-v"
%	 anchor-point= "(200,95)"
%	 text-frame= "noframe"
%	 fill-style= "none"
%	 text-hor-align= "center-h"
%	 >
%$\predtag$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(98.12,5.62)"
%	 text-frame= "noframe"
%	 fill-style= "none"
%	 text-hor-align= "right"
%	 >
%$\een$
%</text>
%<multicurve stroke-width= "0.6"
%	 points= "(190,105);(190,105);(210,105);(210,105)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.6"
%	 points= "(235,140);(235,140);(235,160);(235,160)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.6"
%	 points= "(190,140);(190,140);(235,140);(235,140)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.6"
%	 points= "(190,160);(190,160);(190,140);(190,140)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.75"
%	 points= "(212.5,175);(212.5,175);(212.5,160);(212.5,160)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.75"
%	 points= "(200,140);(200,140);(200,130);(200,130)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.6"
%	 points= "(190,160);(190,160);(235,160);(235,160)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.6"
%	 points= "(-5,30);(-5,30);(25,0);(25,0)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.6"
%	 points= "(25,0);(25,0);(-5,0);(-5,0)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.6"
%	 points= "(-5,0);(-5,0);(-5,30);(-5,30)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.75"
%	 points= "(10,30);(10,30);(10,15);(10,15)"
%	 fill-style= "none"
%	 />
%<text text-vert-align= "center-v"
%	 anchor-point= "(5,10)"
%	 text-frame= "noframe"
%	 fill-style= "none"
%	 text-hor-align= "center-h"
%	 >
%$\function$
%</text>
%<multicurve stroke-width= "0.6"
%	 points= "(40,175);(40,175);(235,175);(235,175)"
%	 fill-style= "none"
%	 />
%<ellipse p3= "(102.57,17.42)"
%	 p2= "(102.57,22.58)"
%	 p1= "(97.43,22.58)"
%	 closure= "open"
%	 fill-color= "#330033"
%	 angle-end= "0"
%	 fill-style= "solid"
%	 angle-start= "0"
%	 />
%<multicurve stroke-width= "0.75"
%	 points= "(225,140);(225,140);(225,87.5);(225,87.5)"
%	 fill-style= "none"
%	 />
%<ellipse p3= "(202.57,71.8)"
%	 p2= "(202.57,76.96)"
%	 p1= "(197.43,76.96)"
%	 closure= "open"
%	 fill-color= "#330033"
%	 angle-end= "0"
%	 fill-style= "solid"
%	 angle-start= "0"
%	 />
%<text text-vert-align= "center-v"
%	 anchor-point= "(215,150)"
%	 text-frame= "noframe"
%	 fill-style= "none"
%	 text-hor-align= "center-h"
%	 >
%$\addition$
%</text>
%</jpic>
%%End JPIC-XML
%PSTricks content-type (pstricks.sty package needed)
%Add \usepackage{pstricks} in the preamble of your LaTeX file
%You can rescale the whole picture (to 80% for instance) by using the command \def\JPicScale{0.8}
\ifx\JPicScale\undefined\def\JPicScale{1}\fi
\psset{unit=\JPicScale mm}
\psset{linewidth=0.3,dotsep=1,hatchwidth=0.3,hatchsep=1.5,shadowsize=1,dimen=middle}
\psset{dotsize=0.7 2.5,dotscale=1 1,fillcolor=black}
\psset{arrowsize=1 2,arrowlength=1,arrowinset=0.25,tbarsize=0.7 5,bracketlength=0.15,rbracketlength=0.15}
\begin{pspicture}(0,0)(235,215)
\psline[linewidth=0.75](175,130)(210,130)
\psline[linewidth=0.75](210,110)(210,130)
\psline[linewidth=0.75](195,110)(210,110)
\psline[linewidth=0.75](187.5,117.5)(10,30)
\psline[linewidth=0.75](175,130)(195,110)
\psline[linewidth=0.6](100,20)(225,87.5)
\rput(200,120){$\utag$}
\psline[linewidth=0.75](30,140)(30,55)
\psline[linewidth=0.6](10,160)(50,160)
\psline[linewidth=0.6](50,140)(50,160)
\psline[linewidth=0.6](10,140)(50,140)
\psline[linewidth=0.6](10,160)(10,140)
\psline[linewidth=0.75](30,170)(30,160)
\psline[linewidth=0.75](100,20)(100,0)
\psline[linewidth=0.6,border=2](30,55)(100,20)
\psline[linewidth=0.75](30,185)(30,160)
\psline[linewidth=0.6](20,195)(235,195)
\psline[linewidth=0.6](235,175)(235,195)
\psline[linewidth=0.6](20,195)(40,175)
\psline[linewidth=0.75](155,215)(155,195)
\psline[linewidth=0.6](210,85)(210,105)
\psline[linewidth=0.6](190,85)(210,85)
\psline[linewidth=0.6](190,105)(190,85)
\psline[linewidth=0.75](200,110)(200,105)
\psline[linewidth=0.75](200,85)(200,73.75)
\rput(30,150){$\zerotag$}
\rput(155,185){$\iiftag$}
\psline[linewidth=0.75,border=2](100,175)(100,20)
\rput(200,95){$\predtag$}
\rput[r](98.12,5.62){$\een$}
\psline[linewidth=0.6](190,105)(210,105)
\psline[linewidth=0.6](235,140)(235,160)
\psline[linewidth=0.6](190,140)(235,140)
\psline[linewidth=0.6](190,160)(190,140)
\psline[linewidth=0.75](212.5,175)(212.5,160)
\psline[linewidth=0.75](200,140)(200,130)
\psline[linewidth=0.6](190,160)(235,160)
\psline[linewidth=0.6](-5,30)(25,0)
\psline[linewidth=0.6](25,0)(-5,0)
\psline[linewidth=0.6](-5,0)(-5,30)
\psline[linewidth=0.75](10,30)(10,15)
\rput(5,10){$\function$}
\psline[linewidth=0.6](40,175)(235,175)
\newrgbcolor{userFillColour}{0.2 0 0.2}
\rput{90}(100,20){\psellipse[fillcolor=userFillColour,fillstyle=solid](0,0)(2.58,-2.57)}
\psline[linewidth=0.75](225,140)(225,87.5)
\newrgbcolor{userFillColour}{0.2 0 0.2}
\rput{90}(200,74.38){\psellipse[fillcolor=userFillColour,fillstyle=solid](0,0)(2.58,-2.57)}
\rput(215,150){$\addition$}
\end{pspicture}


==> PIC/PR.tex <==
%%Created by jPicEdt 1.4.1_03: mixed JPIC-XML/LaTeX format
%%Wed Dec 11 16:31:42 GMT-10:00 2019
%%Begin JPIC-XML
%<?xml version="1.0" standalone="yes"?>
%<jpic x-min="0" x-max="260" y-min="0" y-max="260" auto-bounding="true">
%<multicurve fill-style= "none"
%	 points= "(160,205);(160,205);(250,205);(250,205)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(250,185);(250,185);(250,205);(250,205)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(205,220);(205,220);(205,205);(205,205)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(240,185);(240,185);(240,100);(240,100)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(160,205);(160,205);(160,185);(160,185)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(80,205);(80,205);(120,205);(120,205)"
%	 stroke-width= "0.6"
%	 />
%<multicurve fill-style= "none"
%	 points= "(120,185);(120,185);(120,205);(120,205)"
%	 stroke-width= "0.6"
%	 />
%<multicurve fill-style= "none"
%	 points= "(80,205);(80,205);(80,185);(80,185)"
%	 stroke-width= "0.6"
%	 />
%<multicurve fill-style= "none"
%	 points= "(100,220);(100,220);(100,205);(100,205)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(180,175);(180,175);(222.5,175);(222.5,175)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(222.5,155);(222.5,155);(222.5,175);(222.5,175)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(205,185);(205,185);(205,175);(205,175)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(200,155);(200,155);(222.5,155);(222.5,155)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(190,165);(190,165);(30,85);(30,85)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(180,175);(180,175);(200,155);(200,155)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(170,65);(170,65);(170,0);(170,0)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(100,65);(100,65);(170,100);(170,100)"
%	 stroke-width= "0.6"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(207.5,165)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\utag$
%</text>
%<multicurve fill-style= "none"
%	 points= "(30,185);(30,185);(30,100);(30,100)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(10,205);(10,205);(50,205);(50,205)"
%	 stroke-width= "0.6"
%	 />
%<multicurve fill-style= "none"
%	 points= "(50,185);(50,185);(50,205);(50,205)"
%	 stroke-width= "0.6"
%	 />
%<multicurve fill-style= "none"
%	 points= "(10,185);(10,185);(50,185);(50,185)"
%	 stroke-width= "0.6"
%	 />
%<multicurve fill-style= "none"
%	 points= "(10,205);(10,205);(10,185);(10,185)"
%	 stroke-width= "0.6"
%	 />
%<multicurve fill-style= "none"
%	 points= "(30,215);(30,215);(30,205);(30,205)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(100,65);(100,65);(100,0);(100,0)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 stroke-overstrike-width= "2"
%	 points= "(30,100);(30,100);(100,65);(100,65)"
%	 stroke-overstrike= "true"
%	 stroke-width= "0.6"
%	 />
%<multicurve fill-style= "none"
%	 points= "(30,230);(30,230);(30,205);(30,205)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(20,240);(20,240);(230,240);(230,240)"
%	 stroke-width= "0.6"
%	 />
%<multicurve fill-style= "none"
%	 points= "(230,220);(230,220);(230,240);(230,240)"
%	 stroke-width= "0.6"
%	 />
%<multicurve fill-style= "none"
%	 points= "(40,220);(40,220);(230,220);(230,220)"
%	 stroke-width= "0.6"
%	 />
%<multicurve fill-style= "none"
%	 points= "(20,240);(20,240);(40,220);(40,220)"
%	 stroke-width= "0.6"
%	 />
%<multicurve fill-style= "none"
%	 points= "(135,260);(135,260);(135,240);(135,240)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(170,65);(170,65);(240,100);(240,100)"
%	 stroke-width= "0.6"
%	 />
%<multicurve fill-style= "none"
%	 points= "(215,155);(215,155);(215,145);(215,145)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(185,105);(185,105);(185,120);(185,120)"
%	 stroke-width= "0.6"
%	 />
%<multicurve fill-style= "none"
%	 points= "(155,105);(155,105);(185,105);(185,105)"
%	 stroke-width= "0.6"
%	 />
%<multicurve fill-style= "none"
%	 points= "(155,120);(155,120);(155,105);(155,105)"
%	 stroke-width= "0.6"
%	 />
%<multicurve fill-style= "none"
%	 points= "(205,155);(205,155);(205,145);(205,145)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(170,105);(170,105);(170,100);(170,100)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(30,85);(30,85);(30,35);(30,35)"
%	 stroke-width= "0.75"
%	 />
%<ellipse p3= "(102.57,62.42)"
%	 fill-style= "solid"
%	 p2= "(102.57,67.58)"
%	 fill-color= "#330033"
%	 p1= "(97.43,67.58)"
%	 closure= "open"
%	 angle-end= "0"
%	 angle-start= "0"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(100,195)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\gtag$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(30,195)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\zerotag$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(135,230)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\iiftag$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(205,195)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\htag$
%</text>
%<multicurve fill-style= "none"
%	 stroke-overstrike-width= "2"
%	 points= "(170,185);(170,185);(170,120);(170,120)"
%	 stroke-overstrike= "true"
%	 stroke-width= "0.75"
%	 />
%<ellipse p3= "(172.57,124.92)"
%	 fill-style= "solid"
%	 p2= "(172.57,130.08)"
%	 fill-color= "#330033"
%	 p1= "(167.43,130.08)"
%	 closure= "open"
%	 angle-end= "0"
%	 angle-start= "0"
%	 />
%<multicurve fill-style= "none"
%	 points= "(160,185);(160,185);(250,185);(250,185)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 stroke-overstrike-width= "2"
%	 points= "(100,185);(100,185);(100,100);(100,100)"
%	 stroke-overstrike= "true"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(80,185);(80,185);(120,185);(120,185)"
%	 stroke-width= "0.6"
%	 />
%<multicurve fill-style= "none"
%	 stroke-overstrike-width= "2"
%	 points= "(170,65);(170,65);(100,100);(100,100)"
%	 stroke-overstrike= "true"
%	 stroke-width= "0.6"
%	 />
%<ellipse p3= "(172.57,62.42)"
%	 fill-style= "solid"
%	 p2= "(172.57,67.58)"
%	 fill-color= "#330033"
%	 p1= "(167.43,67.58)"
%	 closure= "open"
%	 angle-end= "0"
%	 angle-start= "0"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(170,112.5)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\predtag$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(28.12,75)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\pee$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(98.75,2.5)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\een$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(167.5,2.5)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\eex$
%</text>
%<multicurve fill-style= "none"
%	 points= "(170,127.5);(170,127.5);(205,145);(205,145)"
%	 stroke-width= "0.6"
%	 />
%<multicurve fill-style= "none"
%	 points= "(155,120);(155,120);(185,120);(185,120)"
%	 stroke-width= "0.6"
%	 />
%<ellipse p3= "(242.57,129.92)"
%	 fill-style= "solid"
%	 p2= "(242.57,135.08)"
%	 fill-color= "#330033"
%	 p1= "(237.43,135.08)"
%	 closure= "open"
%	 angle-end= "0"
%	 angle-start= "0"
%	 />
%<multicurve fill-style= "none"
%	 points= "(215,145);(215,145);(240,132.5);(240,132.5)"
%	 stroke-width= "0.6"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(137.5,256.88)"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\Beh$
%</text>
%<parallelogram p3= "(5,55)"
%	 fill-style= "none"
%	 p2= "(5,245)"
%	 p1= "(255,245)"
%	 />
%<parallelogram p3= "(260,15)"
%	 fill-style= "none"
%	 p2= "(260,250)"
%	 p1= "(0,250)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(20,45);(20,45);(40,25);(40,25)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(20,45);(20,45);(20,25);(20,25)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(20,25);(20,25);(40,25);(40,25)"
%	 stroke-width= "0.75"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(25.62,31.25)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\Ftilde$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(220,35)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\function$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(230,70)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\ftilde$
%</text>
%</jpic>
%%End JPIC-XML
%PSTricks content-type (pstricks.sty package needed)
%Add \usepackage{pstricks} in the preamble of your LaTeX file
%You can rescale the whole picture (to 80% for instance) by using the command \def\JPicScale{0.8}
\ifx\JPicScale\undefined\def\JPicScale{1}\fi
\psset{unit=\JPicScale mm}
\psset{linewidth=0.3,dotsep=1,hatchwidth=0.3,hatchsep=1.5,shadowsize=1,dimen=middle}
\psset{dotsize=0.7 2.5,dotscale=1 1,fillcolor=black}
\psset{arrowsize=1 2,arrowlength=1,arrowinset=0.25,tbarsize=0.7 5,bracketlength=0.15,rbracketlength=0.15}
\begin{pspicture}(0,0)(260,260)
\psline[linewidth=0.75](160,205)(250,205)
\psline[linewidth=0.75](250,185)(250,205)
\psline[linewidth=0.75](205,220)(205,205)
\psline[linewidth=0.75](240,185)(240,100)
\psline[linewidth=0.75](160,205)(160,185)
\psline[linewidth=0.6](80,205)(120,205)
\psline[linewidth=0.6](120,185)(120,205)
\psline[linewidth=0.6](80,205)(80,185)
\psline[linewidth=0.75](100,220)(100,205)
\psline[linewidth=0.75](180,175)(222.5,175)
\psline[linewidth=0.75](222.5,155)(222.5,175)
\psline[linewidth=0.75](205,185)(205,175)
\psline[linewidth=0.75](200,155)(222.5,155)
\psline[linewidth=0.75](190,165)(30,85)
\psline[linewidth=0.75](180,175)(200,155)
\psline[linewidth=0.75](170,65)(170,0)
\psline[linewidth=0.6](100,65)(170,100)
\rput(207.5,165){$\utag$}
\psline[linewidth=0.75](30,185)(30,100)
\psline[linewidth=0.6](10,205)(50,205)
\psline[linewidth=0.6](50,185)(50,205)
\psline[linewidth=0.6](10,185)(50,185)
\psline[linewidth=0.6](10,205)(10,185)
\psline[linewidth=0.75](30,215)(30,205)
\psline[linewidth=0.75](100,65)(100,0)
\psline[linewidth=0.6,border=2](30,100)(100,65)
\psline[linewidth=0.75](30,230)(30,205)
\psline[linewidth=0.6](20,240)(230,240)
\psline[linewidth=0.6](230,220)(230,240)
\psline[linewidth=0.6](40,220)(230,220)
\psline[linewidth=0.6](20,240)(40,220)
\psline[linewidth=0.75](135,260)(135,240)
\psline[linewidth=0.6](170,65)(240,100)
\psline[linewidth=0.75](215,155)(215,145)
\psline[linewidth=0.6](185,105)(185,120)
\psline[linewidth=0.6](155,105)(185,105)
\psline[linewidth=0.6](155,120)(155,105)
\psline[linewidth=0.75](205,155)(205,145)
\psline[linewidth=0.75](170,105)(170,100)
\psline[linewidth=0.75](30,85)(30,35)
\newrgbcolor{userFillColour}{0.2 0 0.2}
\rput{90}(100,65){\psellipse[fillcolor=userFillColour,fillstyle=solid](0,0)(2.58,-2.57)}
\rput(100,195){$\gtag$}
\rput(30,195){$\zerotag$}
\rput(135,230){$\iiftag$}
\rput(205,195){$\htag$}
\psline[linewidth=0.75,border=2](170,185)(170,120)
\newrgbcolor{userFillColour}{0.2 0 0.2}
\rput{90}(170,127.5){\psellipse[fillcolor=userFillColour,fillstyle=solid](0,0)(2.58,-2.57)}
\psline[linewidth=0.75](160,185)(250,185)
\psline[linewidth=0.75,border=2](100,185)(100,100)
\psline[linewidth=0.6](80,185)(120,185)
\psline[linewidth=0.6,border=2](170,65)(100,100)
\newrgbcolor{userFillColour}{0.2 0 0.2}
\rput{90}(170,65){\psellipse[fillcolor=userFillColour,fillstyle=solid](0,0)(2.58,-2.57)}
\rput(170,112.5){$\predtag$}
\rput[r](28.12,75){$\pee$}
\rput[r](98.75,2.5){$\een$}
\rput[r](167.5,2.5){$\eex$}
\psline[linewidth=0.6](170,127.5)(205,145)
\psline[linewidth=0.6](155,120)(185,120)
\newrgbcolor{userFillColour}{0.2 0 0.2}
\rput{90}(240,132.5){\psellipse[fillcolor=userFillColour,fillstyle=solid](0,0)(2.58,-2.57)}
\psline[linewidth=0.6](215,145)(240,132.5)
\rput[l](137.5,256.88){$\Beh$}
\pspolygon[](255,245)(5,245)(5,55)(255,55)
\pspolygon[](0,250)(260,250)(260,15)(0,15)
\psline[linewidth=0.75](20,45)(40,25)
\psline[linewidth=0.75](20,45)(20,25)
\psline[linewidth=0.75](20,25)(40,25)
\rput(25.62,31.25){$\Ftilde$}
\rput(220,35){$\function$}
\rput(230,70){$\ftilde$}
\end{pspicture}


==> PIC/WHILE.tex <==
%%Created by jPicEdt 1.4.1_03: mixed JPIC-XML/LaTeX format
%%Fri Oct 28 19:07:32 EDT 2016
%%Begin JPIC-XML
%<?xml version="1.0" standalone="yes"?>
%<jpic x-min="-1.25" x-max="150" y-min="0" y-max="145" auto-bounding="true">
%<multicurve stroke-width= "0.6"
%	 fill-style= "none"
%	 points= "(0,90);(0,90);(40,90);(40,90)"
%	 />
%<multicurve stroke-width= "0.6"
%	 fill-style= "none"
%	 points= "(40,70);(40,70);(40,90);(40,90)"
%	 />
%<multicurve stroke-width= "0.6"
%	 fill-style= "none"
%	 points= "(0,90);(0,90);(0,70);(0,70)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(60,90);(60,90);(120,90);(120,90)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(120,70);(120,70);(120,90);(120,90)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(100,110);(100,110);(100,90);(100,90)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(70,80);(70,80);(0,45);(0,45)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(60,90);(60,90);(80,70);(80,70)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(110,20);(110,20);(110,0);(110,0)"
%	 />
%<multicurve stroke-width= "0.6"
%	 fill-style= "none"
%	 points= "(90,20);(90,20);(140,45);(140,45)"
%	 />
%<text text-vert-align= "center-v"
%	 anchor-point= "(95,80)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\utag$
%</text>
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(90,20);(90,20);(90,0);(90,0)"
%	 />
%<multicurve stroke-overstrike= "true"
%	 stroke-width= "0.6"
%	 stroke-overstrike-width= "2"
%	 fill-style= "none"
%	 points= "(10,60);(10,60);(90,20);(90,20)"
%	 />
%<multicurve stroke-width= "0.6"
%	 fill-style= "none"
%	 points= "(10,130);(10,130);(150,130);(150,130)"
%	 />
%<multicurve stroke-width= "0.6"
%	 fill-style= "none"
%	 points= "(150,110);(150,110);(150,130);(150,130)"
%	 />
%<multicurve stroke-width= "0.6"
%	 fill-style= "none"
%	 points= "(10,130);(10,130);(30,110);(30,110)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(0,45);(0,45);(0,0);(0,0)"
%	 />
%<text text-vert-align= "center-v"
%	 anchor-point= "(20,80)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\gtag$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(100,120)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\iiftag$
%</text>
%<multicurve stroke-overstrike= "true"
%	 stroke-width= "0.75"
%	 stroke-overstrike-width= "2"
%	 fill-style= "none"
%	 points= "(30,70);(30,70);(30,60);(30,60)"
%	 />
%<multicurve stroke-width= "0.6"
%	 fill-style= "none"
%	 points= "(0,70);(0,70);(40,70);(40,70)"
%	 />
%<text text-vert-align= "center-v"
%	 anchor-point= "(-1.25,5.62)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\pee$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(88.12,5.62)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\een$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(108.75,5.62)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\eex$
%</text>
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(10,70);(10,70);(10,60);(10,60)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(20,120);(20,120);(20,90);(20,90)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(140,45);(140,45);(140,110);(140,110)"
%	 />
%<multicurve stroke-overstrike= "true"
%	 stroke-width= "0.75"
%	 stroke-overstrike-width= "1.3"
%	 fill-style= "none"
%	 points= "(90,70);(90,70);(90,20);(90,20)"
%	 />
%<multicurve stroke-overstrike= "true"
%	 stroke-width= "0.6"
%	 stroke-overstrike-width= "2"
%	 fill-style= "none"
%	 points= "(110,20);(110,20);(30,60);(30,60)"
%	 />
%<ellipse p3= "(92.57,17.42)"
%	 p2= "(92.57,22.58)"
%	 p1= "(87.43,22.58)"
%	 closure= "open"
%	 fill-style= "solid"
%	 angle-end= "0"
%	 fill-color= "#330033"
%	 angle-start= "0"
%	 />
%<multicurve stroke-width= "0.6"
%	 fill-style= "none"
%	 points= "(30,110);(30,110);(150,110);(150,110)"
%	 />
%<multicurve stroke-overstrike= "true"
%	 stroke-width= "0.75"
%	 stroke-overstrike-width= "1.3"
%	 fill-style= "none"
%	 points= "(110,70);(110,70);(110,20);(110,20)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(80,70);(80,70);(120,70);(120,70)"
%	 />
%<ellipse p3= "(112.57,17.42)"
%	 p2= "(112.57,22.58)"
%	 p1= "(107.43,22.58)"
%	 closure= "open"
%	 fill-style= "solid"
%	 angle-end= "0"
%	 fill-color= "#330033"
%	 angle-start= "0"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(100,145);(100,145);(100,130);(100,130)"
%	 />
%</jpic>
%%End JPIC-XML
%PSTricks content-type (pstricks.sty package needed)
%Add \usepackage{pstricks} in the preamble of your LaTeX file
%You can rescale the whole picture (to 80% for instance) by using the command \def\JPicScale{0.8}
\ifx\JPicScale\undefined\def\JPicScale{1}\fi
\psset{unit=\JPicScale mm}
\psset{linewidth=0.3,dotsep=1,hatchwidth=0.3,hatchsep=1.5,shadowsize=1,dimen=middle}
\psset{dotsize=0.7 2.5,dotscale=1 1,fillcolor=black}
\psset{arrowsize=1 2,arrowlength=1,arrowinset=0.25,tbarsize=0.7 5,bracketlength=0.15,rbracketlength=0.15}
\begin{pspicture}(0,0)(150,145)
\psline[linewidth=0.6](0,90)(40,90)
\psline[linewidth=0.6](40,70)(40,90)
\psline[linewidth=0.6](0,90)(0,70)
\psline[linewidth=0.75](60,90)(120,90)
\psline[linewidth=0.75](120,70)(120,90)
\psline[linewidth=0.75](100,110)(100,90)
\psline[linewidth=0.75](70,80)(0,45)
\psline[linewidth=0.75](60,90)(80,70)
\psline[linewidth=0.75](110,20)(110,0)
\psline[linewidth=0.6](90,20)(140,45)
\rput(95,80){$\utag$}
\psline[linewidth=0.75](90,20)(90,0)
\psline[linewidth=0.6,border=2](10,60)(90,20)
\psline[linewidth=0.6](10,130)(150,130)
\psline[linewidth=0.6](150,110)(150,130)
\psline[linewidth=0.6](10,130)(30,110)
\psline[linewidth=0.75](0,45)(0,0)
\rput(20,80){$\gtag$}
\rput(100,120){$\iiftag$}
\psline[linewidth=0.75,border=2](30,70)(30,60)
\psline[linewidth=0.6](0,70)(40,70)
\rput[r](-1.25,5.62){$\pee$}
\rput[r](88.12,5.62){$\een$}
\rput[r](108.75,5.62){$\eex$}
\psline[linewidth=0.75](10,70)(10,60)
\psline[linewidth=0.75](20,120)(20,90)
\psline[linewidth=0.75](140,45)(140,110)
\psline[linewidth=0.75,border=1.3](90,70)(90,20)
\psline[linewidth=0.6,border=2](110,20)(30,60)
\newrgbcolor{userFillColour}{0.2 0 0.2}
\rput{90}(90,20){\psellipse[fillcolor=userFillColour,fillstyle=solid](0,0)(2.58,-2.57)}
\psline[linewidth=0.6](30,110)(150,110)
\psline[linewidth=0.75,border=1.3](110,70)(110,20)
\psline[linewidth=0.75](80,70)(120,70)
\newrgbcolor{userFillColour}{0.2 0 0.2}
\rput{90}(110,20){\psellipse[fillcolor=userFillColour,fillstyle=solid](0,0)(2.58,-2.57)}
\psline[linewidth=0.75](100,145)(100,130)
\end{pspicture}


==> PIC/aut-lang.tex <==
%%Created by jPicEdt 1.4.1_03: mixed JPIC-XML/LaTeX format
%%Sun Sep 04 11:55:05 HST 2016
%%Begin JPIC-XML
%<?xml version="1.0" standalone="yes"?>
%<jpic x-min="20" x-max="70" y-min="-5" y-max="35" auto-bounding="true">
%<text text-vert-align= "center-v"
%	 anchor-point= "(20,1.25)"
%	 text-frame= "noframe"
%	 fill-style= "none"
%	 text-hor-align= "center-h"
%	 >
%\Machines
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(20,35)"
%	 text-frame= "noframe"
%	 fill-style= "none"
%	 text-hor-align= "center-h"
%	 >
%\Languages
%</text>
%<multicurve stroke-width= "0.65"
%	 arrow-head-inset-scale= "0.4"
%	 arrow-head-length-scale= "1.6"
%	 left-arrow= "head"
%	 arrow-head-width-minimum= "2.05"
%	 points= "(20,31.25);(20,31.25);(20,5);(20,5)"
%	 fill-style= "none"
%	 />
%<multicurve points= "(50,5);(50,5);(70,5);(70,5)"
%	 fill-style= "none"
%	 />
%<multicurve points= "(50,5);(50,5);(60,-5);(60,-5)"
%	 fill-style= "none"
%	 />
%<multicurve points= "(60,-5);(60,-5);(70,5);(70,5)"
%	 fill-style= "none"
%	 />
%<multicurve points= "(60,29.38);(60,29.38);(60,5);(60,5)"
%	 fill-style= "none"
%	 />
%<text text-vert-align= "center-v"
%	 anchor-point= "(60,1.25)"
%	 text-frame= "noframe"
%	 fill-style= "none"
%	 text-hor-align= "center-h"
%	 >
%$\namemach$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(60,35)"
%	 text-frame= "noframe"
%	 fill-style= "none"
%	 text-hor-align= "center-h"
%	 >
%$\nameslang$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(42.5,1.25)"
%	 text-frame= "noframe"
%	 fill-style= "none"
%	 text-hor-align= "center-h"
%	 >
%$\bigin$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(42.5,35)"
%	 text-frame= "noframe"
%	 fill-style= "none"
%	 text-hor-align= "center-h"
%	 >
%$\bigin$
%</text>
%</jpic>
%%End JPIC-XML
%PSTricks content-type (pstricks.sty package needed)
%Add \usepackage{pstricks} in the preamble of your LaTeX file
%You can rescale the whole picture (to 80% for instance) by using the command \def\JPicScale{0.8}
\ifx\JPicScale\undefined\def\JPicScale{1}\fi
\psset{unit=\JPicScale mm}
\psset{linewidth=0.3,dotsep=1,hatchwidth=0.3,hatchsep=1.5,shadowsize=1,dimen=middle}
\psset{dotsize=0.7 2.5,dotscale=1 1,fillcolor=black}
\psset{arrowsize=1 2,arrowlength=1,arrowinset=0.25,tbarsize=0.7 5,bracketlength=0.15,rbracketlength=0.15}
\begin{pspicture}(0,0)(70,35)
\rput(20,1.25){\Machines}
\rput(20,35){\Languages}
\psline[linewidth=0.65,arrowsize=2.05 2,arrowlength=1.6,arrowinset=0.4]{<-}(20,31.25)(20,5)
\psline(50,5)(70,5)
\psline(50,5)(60,-5)
\psline(60,-5)(70,5)
\psline(60,29.38)(60,5)
\rput(60,1.25){$\namemach$}
\rput(60,35){$\nameslang$}
\rput(42.5,1.25){$\bigin$}
\rput(42.5,35){$\bigin$}
\end{pspicture}


==> PIC/aut-mealy-0.tex <==
%%Created by jPicEdt 1.4.1_03: mixed JPIC-XML/LaTeX format
%%Sun Sep 04 12:13:00 HST 2016
%%Begin JPIC-XML
%<?xml version="1.0" standalone="yes"?>
%<jpic x-min="20" x-max="70" y-min="1.25" y-max="60" auto-bounding="true">
%<text text-vert-align= "center-v"
%	 anchor-point= "(20,30)"
%	 text-frame= "noframe"
%	 fill-style= "none"
%	 text-hor-align= "center-h"
%	 >
%\Machines
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(20,60)"
%	 text-frame= "noframe"
%	 fill-style= "none"
%	 text-hor-align= "center-h"
%	 >
%\Languages
%</text>
%<multicurve stroke-width= "0.65"
%	 arrow-head-inset-scale= "0.4"
%	 arrow-head-length-scale= "1.6"
%	 left-arrow= "head"
%	 arrow-head-width-minimum= "2.05"
%	 points= "(20,56.25);(20,56.25);(20,34.38);(20,34.38)"
%	 fill-style= "none"
%	 />
%<multicurve points= "(50,35);(50,35);(70,35);(70,35)"
%	 fill-style= "none"
%	 />
%<multicurve points= "(50,35);(50,35);(60,25);(60,25)"
%	 fill-style= "none"
%	 />
%<multicurve points= "(60,25);(60,25);(70,35);(70,35)"
%	 fill-style= "none"
%	 />
%<multicurve points= "(60,54.38);(60,54.38);(60,35);(60,35)"
%	 fill-style= "none"
%	 />
%<text text-vert-align= "center-v"
%	 anchor-point= "(60,30)"
%	 text-frame= "noframe"
%	 fill-style= "none"
%	 text-hor-align= "center-h"
%	 >
%$\namemach$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(60,60)"
%	 text-frame= "noframe"
%	 fill-style= "none"
%	 text-hor-align= "center-h"
%	 >
%$\nameslang$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(42.5,30)"
%	 text-frame= "noframe"
%	 fill-style= "none"
%	 text-hor-align= "center-h"
%	 >
%$\bigin$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(42.5,60)"
%	 text-frame= "noframe"
%	 fill-style= "none"
%	 text-hor-align= "center-h"
%	 >
%$\bigin$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(20,1.25)"
%	 text-frame= "noframe"
%	 fill-style= "none"
%	 text-hor-align= "center-h"
%	 >
%$\InLanguages$
%</text>
%</jpic>
%%End JPIC-XML
%PSTricks content-type (pstricks.sty package needed)
%Add \usepackage{pstricks} in the preamble of your LaTeX file
%You can rescale the whole picture (to 80% for instance) by using the command \def\JPicScale{0.8}
\ifx\JPicScale\undefined\def\JPicScale{1}\fi
\psset{unit=\JPicScale mm}
\psset{linewidth=0.3,dotsep=1,hatchwidth=0.3,hatchsep=1.5,shadowsize=1,dimen=middle}
\psset{dotsize=0.7 2.5,dotscale=1 1,fillcolor=black}
\psset{arrowsize=1 2,arrowlength=1,arrowinset=0.25,tbarsize=0.7 5,bracketlength=0.15,rbracketlength=0.15}
\begin{pspicture}(0,0)(70,60)
\rput(20,30){\Machines}
\rput(20,60){\Languages}
\psline[linewidth=0.65,arrowsize=2.05 2,arrowlength=1.6,arrowinset=0.4]{<-}(20,56.25)(20,34.38)
\psline(50,35)(70,35)
\psline(50,35)(60,25)
\psline(60,25)(70,35)
\psline(60,54.38)(60,35)
\rput(60,30){$\namemach$}
\rput(60,60){$\nameslang$}
\rput(42.5,30){$\bigin$}
\rput(42.5,60){$\bigin$}
\rput(20,1.25){$\InLanguages$}
\end{pspicture}


==> PIC/aut-mealy.tex <==
%%Created by jPicEdt 1.4.1_03: mixed JPIC-XML/LaTeX format
%%Sun Sep 04 12:26:52 HST 2016
%%Begin JPIC-XML
%<?xml version="1.0" standalone="yes"?>
%<jpic x-min="20" x-max="70" y-min="1.25" y-max="60" auto-bounding="true">
%<text text-vert-align= "center-v"
%	 anchor-point= "(20,30)"
%	 text-frame= "noframe"
%	 fill-style= "none"
%	 text-hor-align= "center-h"
%	 >
%\Machines
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(20,60)"
%	 text-frame= "noframe"
%	 fill-style= "none"
%	 text-hor-align= "center-h"
%	 >
%\Languages
%</text>
%<multicurve stroke-width= "0.65"
%	 arrow-head-inset-scale= "0.4"
%	 arrow-head-length-scale= "1.6"
%	 left-arrow= "head"
%	 arrow-head-width-minimum= "2.05"
%	 points= "(20,56.25);(20,56.25);(20,34.38);(20,34.38)"
%	 fill-style= "none"
%	 />
%<multicurve points= "(50,35);(50,35);(70,35);(70,35)"
%	 fill-style= "none"
%	 />
%<multicurve points= "(50,35);(50,35);(50,25);(50,25)"
%	 fill-style= "none"
%	 />
%<multicurve points= "(70,25);(70,25);(70,35);(70,35)"
%	 fill-style= "none"
%	 />
%<multicurve points= "(60,54.38);(60,54.38);(60,35);(60,35)"
%	 fill-style= "none"
%	 />
%<text text-vert-align= "center-v"
%	 anchor-point= "(60,30)"
%	 text-frame= "noframe"
%	 fill-style= "none"
%	 text-hor-align= "center-h"
%	 >
%$\namemach$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(60,60)"
%	 text-frame= "noframe"
%	 fill-style= "none"
%	 text-hor-align= "center-h"
%	 >
%$\nameslang$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(42.5,30)"
%	 text-frame= "noframe"
%	 fill-style= "none"
%	 text-hor-align= "center-h"
%	 >
%$\bigin$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(42.5,60)"
%	 text-frame= "noframe"
%	 fill-style= "none"
%	 text-hor-align= "center-h"
%	 >
%$\bigin$
%</text>
%<multicurve stroke-width= "0.65"
%	 arrow-head-inset-scale= "0.4"
%	 arrow-head-length-scale= "1.6"
%	 left-arrow= "head"
%	 arrow-head-width-minimum= "2.05"
%	 points= "(20,26.25);(20,26.25);(20,4.38);(20,4.38)"
%	 fill-style= "none"
%	 />
%<text text-vert-align= "center-v"
%	 anchor-point= "(60,1.25)"
%	 text-frame= "noframe"
%	 fill-style= "none"
%	 text-hor-align= "center-h"
%	 >
%$\inputt$
%</text>
%<multicurve points= "(50,25);(50,25);(70,25);(70,25)"
%	 fill-style= "none"
%	 />
%<multicurve points= "(60,25);(60,25);(60,4.38);(60,4.38)"
%	 fill-style= "none"
%	 />
%<text text-vert-align= "center-v"
%	 anchor-point= "(43.12,1.25)"
%	 text-frame= "noframe"
%	 fill-style= "none"
%	 text-hor-align= "center-h"
%	 >
%$\biginn$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(20,1.25)"
%	 text-frame= "noframe"
%	 fill-style= "none"
%	 text-hor-align= "center-h"
%	 >
%\InLanguages
%</text>
%</jpic>
%%End JPIC-XML
%PSTricks content-type (pstricks.sty package needed)
%Add \usepackage{pstricks} in the preamble of your LaTeX file
%You can rescale the whole picture (to 80% for instance) by using the command \def\JPicScale{0.8}
\ifx\JPicScale\undefined\def\JPicScale{1}\fi
\psset{unit=\JPicScale mm}
\psset{linewidth=0.3,dotsep=1,hatchwidth=0.3,hatchsep=1.5,shadowsize=1,dimen=middle}
\psset{dotsize=0.7 2.5,dotscale=1 1,fillcolor=black}
\psset{arrowsize=1 2,arrowlength=1,arrowinset=0.25,tbarsize=0.7 5,bracketlength=0.15,rbracketlength=0.15}
\begin{pspicture}(0,0)(70,60)
\rput(20,30){\Machines}
\rput(20,60){\Languages}
\psline[linewidth=0.65,arrowsize=2.05 2,arrowlength=1.6,arrowinset=0.4]{<-}(20,56.25)(20,34.38)
\psline(50,35)(70,35)
\psline(50,35)(50,25)
\psline(70,25)(70,35)
\psline(60,54.38)(60,35)
\rput(60,30){$\namemach$}
\rput(60,60){$\nameslang$}
\rput(42.5,30){$\bigin$}
\rput(42.5,60){$\bigin$}
\psline[linewidth=0.65,arrowsize=2.05 2,arrowlength=1.6,arrowinset=0.4]{<-}(20,26.25)(20,4.38)
\rput(60,1.25){$\inputt$}
\psline(50,25)(70,25)
\psline(60,25)(60,4.38)
\rput(43.12,1.25){$\biginn$}
\rput(20,1.25){\InLanguages}
\end{pspicture}


==> PIC/black-fun.tex <==
%%Created by jPicEdt 1.4.1_03: mixed JPIC-XML/LaTeX format
%%Sun Jul 17 09:53:53 GMT+01:00 2022
%%Begin JPIC-XML
%<?xml version="1.0" standalone="yes"?>
%<jpic x-min="0" x-max="80" y-min="0" y-max="120" auto-bounding="true">
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 stroke-width= "0.35"
%	 anchor-point= "(45,117.5)"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\Cee$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 stroke-width= "0.35"
%	 anchor-point= "(15,2.5)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\Aee$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 stroke-width= "0.35"
%	 anchor-point= "(55,2.5)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\Bee$
%</text>
%<multicurve fill-style= "none"
%	 stroke-width= "0.35"
%	 points= "(80,80);(80,80);(80,40);(80,40)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.35"
%	 points= "(80,40);(80,40);(0,40);(0,40)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.35"
%	 points= "(0,80);(0,80);(80,80);(80,80)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.5"
%	 points= "(60,40);(60,40);(60,0);(60,0)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.5"
%	 points= "(40,120);(40,120);(40,80);(40,80)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.35"
%	 points= "(0,80);(0,80);(0,40);(0,40)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.5"
%	 points= "(20,40);(20,40);(20,0);(20,0)"
%	 />
%<parallelogram p3= "(80,40)"
%	 p2= "(80,80)"
%	 fill-style= "solid"
%	 p1= "(0,80)"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 stroke-width= "0.35"
%	 anchor-point= "(40,60)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\fee$
%</text>
%</jpic>
%%End JPIC-XML
%LaTeX-picture environment using emulated lines and arcs
%You can rescale the whole picture (to 80% for instance) by using the command \def\JPicScale{0.8}
\ifx\JPicScale\undefined\def\JPicScale{1}\fi
\unitlength \JPicScale mm
\begin{picture}(80,120)(0,0)
\put(45,117.5){\makebox(0,0)[cl]{$\Cee$}}

\put(15,2.5){\makebox(0,0)[cr]{$\Aee$}}

\put(55,2.5){\makebox(0,0)[cr]{$\Bee$}}

\linethickness{0.35mm}
\put(80,40){\line(0,1){40}}
\linethickness{0.35mm}
\put(0,40){\line(1,0){80}}
\linethickness{0.35mm}
\put(0,80){\line(1,0){80}}
\linethickness{0.5mm}
\put(60,0){\line(0,1){40}}
\linethickness{0.5mm}
\put(40,80){\line(0,1){40}}
\linethickness{0.35mm}
\put(0,40){\line(0,1){40}}
\linethickness{0.5mm}
\put(20,0){\line(0,1){40}}
\linethickness{0.3mm}
\put(0,80){\rule{80\unitlength}{40\unitlength}}
\put(40,60){\makebox(0,0)[cc]{$\fee$}}

\end{picture}


==> PIC/boolidem-1.tex <==
%%Created by jPicEdt 1.4.1_03: mixed JPIC-XML/LaTeX format
%%Wed May 19 19:39:19 GMT-10:00 2021
%%Begin JPIC-XML
%<?xml version="1.0" standalone="yes"?>
%<jpic x-min="0" x-max="167.5" y-min="0" y-max="190" auto-bounding="true">
%<multicurve fill-style= "none"
%	 points= "(0,55);(0,55);(40,15);(40,15)"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(0,175);(0,175);(0,55);(0,55)"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(5,130);(5,130);(75,130);(75,130)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(75,110);(75,110);(75,130);(75,130)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(52.5,190);(52.5,190);(52.5,130);(52.5,130)"
%	 stroke-width= "1.5"
%	 />
%<multicurve fill-style= "none"
%	 points= "(25,110);(25,110);(75,110);(75,110)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(65,110);(65,110);(65,30);(65,30)"
%	 stroke-width= "1.5"
%	 />
%<multicurve fill-style= "none"
%	 points= "(15,120);(15,120);(15,105);(15,105)"
%	 stroke-width= "1.5"
%	 />
%<multicurve fill-style= "none"
%	 points= "(5,130);(5,130);(25,110);(25,110)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(5,90);(5,90);(25,90);(25,90)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(5,90);(5,90);(5,105);(5,105)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(5,105);(5,105);(25,105);(25,105)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(40,110);(40,110);(40,55);(40,55)"
%	 stroke-width= "1.5"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(100,90)"
%	 text-frame= "noframe"
%	 stroke-width= "0.75"
%	 text-hor-align= "center-h"
%	 >
%\EQLS
%</text>
%<multicurve fill-style= "none"
%	 points= "(30,45);(30,45);(50,45);(50,45)"
%	 stroke-width= "0.5"
%	 />
%<multicurve fill-style= "none"
%	 points= "(30,45);(30,45);(30,65);(30,65)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(30,65);(30,65);(50,45);(50,45)"
%	 stroke-width= "0.75"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(35,50)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\oone$
%</text>
%<multicurve fill-style= "none"
%	 points= "(55,20);(55,20);(75,20);(75,20)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(55,20);(55,20);(55,40);(55,40)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(55,40);(55,40);(75,20);(75,20)"
%	 stroke-width= "0.75"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(52.5,130)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\DOTT
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(15,105)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\DOTT
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(40,55)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\DOTT
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(65,30)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\DOTT
%</text>
%<multicurve fill-style= "none"
%	 points= "(25,90);(25,90);(25,105);(25,105)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(10,90);(10,90);(10,0);(10,0)"
%	 stroke-width= "1.5"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(40,65)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\DOTT
%</text>
%<multicurve fill-style= "none"
%	 points= "(20,90);(20,90);(20,85);(20,85)"
%	 stroke-width= "1.5"
%	 />
%<multicurve fill-style= "none"
%	 points= "(20,85);(20,85);(40,65);(40,65)"
%	 stroke-width= "1.5"
%	 />
%<multicurve fill-style= "none"
%	 points= "(40,175);(40,175);(80,135);(80,135)"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(80,135);(80,135);(80,15);(80,15)"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(40,15);(40,15);(80,15);(80,15)"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(0,175);(0,175);(40,175);(40,175)"
%	 stroke-width= "0.35"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(20,150)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\beeeta$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(15,97.5)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\smaller$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(62.5,25)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\zzero$
%</text>
%<multicurve fill-style= "none"
%	 points= "(127.5,47.5);(127.5,47.5);(160,15);(160,15)"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(127.5,175);(127.5,175);(127.5,47.5);(127.5,47.5)"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(147.5,190);(147.5,190);(147.5,155);(147.5,155)"
%	 stroke-width= "1.5"
%	 />
%<multicurve fill-style= "none"
%	 points= "(147.5,35);(147.5,35);(147.5,0);(147.5,0)"
%	 stroke-width= "1.5"
%	 />
%<multicurve fill-style= "none"
%	 points= "(135,175);(135,175);(167.5,142.5);(167.5,142.5)"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(167.5,142.5);(167.5,142.5);(167.5,15);(167.5,15)"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(132.5,140);(132.5,140);(162.5,140);(162.5,140)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(132.5,140);(132.5,140);(132.5,170);(132.5,170)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(132.5,170);(132.5,170);(162.5,140);(162.5,140)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(132.5,50);(132.5,50);(162.5,50);(162.5,50)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(162.5,20);(162.5,20);(162.5,50);(162.5,50)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(132.5,50);(132.5,50);(162.5,20);(162.5,20)"
%	 stroke-width= "0.75"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(147.5,155)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\DOTT
%</text>
%<multicurve fill-style= "none"
%	 points= "(147.5,50);(147.5,50);(147.5,140);(147.5,140)"
%	 stroke-width= "0.2"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(150,90)"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\Ree$
%</text>
%<multicurve fill-style= "none"
%	 points= "(167.5,15);(167.5,15);(160,15);(160,15)"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(135,175);(135,175);(127.5,175);(127.5,175)"
%	 stroke-width= "0.35"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(142.5,147.5)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\encobool$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(53.75,120)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\booleval$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(151.25,41.25)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\booleval$
%</text>
%</jpic>
%%End JPIC-XML
%PSTricks content-type (pstricks.sty package needed)
%Add \usepackage{pstricks} in the preamble of your LaTeX file
%You can rescale the whole picture (to 80% for instance) by using the command \def\JPicScale{0.8}
\ifx\JPicScale\undefined\def\JPicScale{1}\fi
\psset{unit=\JPicScale mm}
\psset{linewidth=0.3,dotsep=1,hatchwidth=0.3,hatchsep=1.5,shadowsize=1,dimen=middle}
\psset{dotsize=0.7 2.5,dotscale=1 1,fillcolor=black}
\psset{arrowsize=1 2,arrowlength=1,arrowinset=0.25,tbarsize=0.7 5,bracketlength=0.15,rbracketlength=0.15}
\begin{pspicture}(0,0)(167.5,190)
\psline[linewidth=0.35](0,55)(40,15)
\psline[linewidth=0.35](0,175)(0,55)
\psline[linewidth=0.75](5,130)(75,130)
\psline[linewidth=0.75](75,110)(75,130)
\psline[linewidth=1.5](52.5,190)(52.5,130)
\psline[linewidth=0.75](25,110)(75,110)
\psline[linewidth=1.5](65,110)(65,30)
\psline[linewidth=1.5](15,120)(15,105)
\psline[linewidth=0.75](5,130)(25,110)
\psline[linewidth=0.75](5,90)(25,90)
\psline[linewidth=0.75](5,90)(5,105)
\psline[linewidth=0.75](5,105)(25,105)
\psline[linewidth=1.5](40,110)(40,55)
\rput(100,90){\EQLS}
\psline[linewidth=0.5](30,45)(50,45)
\psline[linewidth=0.75](30,45)(30,65)
\psline[linewidth=0.75](30,65)(50,45)
\rput(35,50){$\oone$}
\psline[linewidth=0.75](55,20)(75,20)
\psline[linewidth=0.75](55,20)(55,40)
\psline[linewidth=0.75](55,40)(75,20)
\rput(52.5,130){\DOTT}
\rput(15,105){\DOTT}
\rput(40,55){\DOTT}
\rput(65,30){\DOTT}
\psline[linewidth=0.75](25,90)(25,105)
\psline[linewidth=1.5](10,90)(10,0)
\rput(40,65){\DOTT}
\psline[linewidth=1.5](20,90)(20,85)
\psline[linewidth=1.5](20,85)(40,65)
\psline[linewidth=0.35](40,175)(80,135)
\psline[linewidth=0.35](80,135)(80,15)
\psline[linewidth=0.35](40,15)(80,15)
\psline[linewidth=0.35](0,175)(40,175)
\rput(20,150){$\beeeta$}
\rput(15,97.5){$\smaller$}
\rput(62.5,25){$\zzero$}
\psline[linewidth=0.35](127.5,47.5)(160,15)
\psline[linewidth=0.35](127.5,175)(127.5,47.5)
\psline[linewidth=1.5](147.5,190)(147.5,155)
\psline[linewidth=1.5](147.5,35)(147.5,0)
\psline[linewidth=0.35](135,175)(167.5,142.5)
\psline[linewidth=0.35](167.5,142.5)(167.5,15)
\psline[linewidth=0.75](132.5,140)(162.5,140)
\psline[linewidth=0.75](132.5,140)(132.5,170)
\psline[linewidth=0.75](132.5,170)(162.5,140)
\psline[linewidth=0.75](132.5,50)(162.5,50)
\psline[linewidth=0.75](162.5,20)(162.5,50)
\psline[linewidth=0.75](132.5,50)(162.5,20)
\rput(147.5,155){\DOTT}
\psline[linewidth=0.2](147.5,50)(147.5,140)
\rput[l](150,90){$\Ree$}
\psline[linewidth=0.35](167.5,15)(160,15)
\psline[linewidth=0.35](135,175)(127.5,175)
\rput(142.5,147.5){$\encobool$}
\rput(53.75,120){$\booleval$}
\rput(151.25,41.25){$\booleval$}
\end{pspicture}


==> PIC/branch-1.tex <==
%%Created by jPicEdt 1.4.1_03: mixed JPIC-XML/LaTeX format
%%Mon Sep 05 19:19:28 GMT-10:00 2022
%%Begin JPIC-XML
%<?xml version="1.0" standalone="yes"?>
%<jpic x-min="0" x-max="180" y-min="0" y-max="110" auto-bounding="true">
%<multicurve fill-style= "none"
%	 points= "(0,85);(0,85);(60,85);(60,85)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(60,65);(60,65);(60,85);(60,85)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(20,65);(20,65);(60,65);(60,65)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(0,85);(0,85);(20,65);(20,65)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(10,75);(10,75);(10,40);(10,40)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(30,65);(30,65);(30,40);(30,40)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(30,30);(30,30);(30,20);(30,20)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(50,65);(50,65);(50,40);(50,40)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(45,40);(45,40);(55,40);(55,40)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(55,40);(55,40);(55,30);(55,30)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(55,30);(55,30);(45,30);(45,30)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(45,30);(45,30);(45,40);(45,40)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(50,30);(50,30);(50,20);(50,20)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(50,20);(50,20);(40,10);(40,10)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(30,20);(30,20);(40,10);(40,10)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(40,10);(40,10);(40,0);(40,0)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(100,70);(100,70);(160,70);(160,70)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(160,50);(160,50);(160,70);(160,70)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(120,50);(120,50);(160,50);(160,50)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(100,70);(100,70);(120,50);(120,50)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(110,60);(110,60);(110,40);(110,40)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(130,50);(130,50);(130,35);(130,35)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(123.75,41.25);(123.75,41.25);(136.25,28.75);(136.25,28.75)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(136.25,28.75);(136.25,28.75);(123.75,28.75);(123.75,28.75)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(123.75,28.75);(123.75,28.75);(123.75,41.25);(123.75,41.25)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(150,50);(150,50);(150,35);(150,35)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(143.75,41.25);(143.75,41.25);(156.25,28.75);(156.25,28.75)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(156.25,28.75);(156.25,28.75);(143.75,28.75);(143.75,28.75)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(143.75,28.75);(143.75,28.75);(143.75,41.25);(143.75,41.25)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(170,40);(170,40);(140,10);(140,10)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(140,10);(140,10);(140,0);(140,0)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(170,80);(170,80);(170,40);(170,40)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(140,90);(140,90);(140,70);(140,70)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(40,110);(40,110);(40,85);(40,85)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(130,100);(130,100);(180,100);(180,100)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(180,80);(180,80);(180,100);(180,100)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(150,80);(150,80);(180,80);(180,80)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(130,100);(130,100);(150,80);(150,80)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(160,110);(160,110);(160,100);(160,100)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(25,40);(25,40);(35,40);(35,40)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(35,40);(35,40);(35,30);(35,30)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(35,30);(35,30);(25,30);(25,30)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(25,30);(25,30);(25,40);(25,40)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(5,40);(5,40);(15,40);(15,40)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(15,40);(15,40);(15,30);(15,30)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(15,30);(15,30);(5,30);(5,30)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(5,30);(5,30);(5,40);(5,40)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(105,40);(105,40);(115,40);(115,40)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(115,40);(115,40);(115,30);(115,30)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(115,30);(115,30);(105,30);(105,30)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(105,30);(105,30);(105,40);(105,40)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(110,30);(110,30);(110,0);(110,0)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(10,30);(10,30);(10,0);(10,0)"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(80,75)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\EQLS
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(10,35)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\beee$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(30,35)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\feee$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(50,35)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\geee$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(126.88,33.12)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\Feee$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(146.88,33.12)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\Geee$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(40,10)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\Dottt
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(110,35)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\beee$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(35,75)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\IIIF$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(135,60)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\evv$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(160,90)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\evv$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(150,35)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\dottt
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(130,35)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\dottt
%</text>
%</jpic>
%%End JPIC-XML
%LaTeX-picture environment using emulated lines and arcs
%You can rescale the whole picture (to 80% for instance) by using the command \def\JPicScale{0.8}
\ifx\JPicScale\undefined\def\JPicScale{1}\fi
\unitlength \JPicScale mm
\begin{picture}(180,110)(0,0)
\linethickness{0.3mm}
\put(0,85){\line(1,0){60}}
\linethickness{0.3mm}
\put(60,65){\line(0,1){20}}
\linethickness{0.3mm}
\put(20,65){\line(1,0){40}}
\linethickness{0.3mm}
\multiput(0,85)(0.12,-0.12){167}{\line(1,0){0.12}}
\linethickness{0.3mm}
\put(10,40){\line(0,1){35}}
\linethickness{0.3mm}
\put(30,40){\line(0,1){25}}
\linethickness{0.3mm}
\put(30,20){\line(0,1){10}}
\linethickness{0.3mm}
\put(50,40){\line(0,1){25}}
\linethickness{0.3mm}
\put(45,40){\line(1,0){10}}
\linethickness{0.3mm}
\put(55,30){\line(0,1){10}}
\linethickness{0.3mm}
\put(45,30){\line(1,0){10}}
\linethickness{0.3mm}
\put(45,30){\line(0,1){10}}
\linethickness{0.3mm}
\put(50,20){\line(0,1){10}}
\linethickness{0.3mm}
\multiput(40,10)(0.12,0.12){83}{\line(1,0){0.12}}
\linethickness{0.3mm}
\multiput(30,20)(0.12,-0.12){83}{\line(1,0){0.12}}
\linethickness{0.3mm}
\put(40,0){\line(0,1){10}}
\linethickness{0.3mm}
\put(100,70){\line(1,0){60}}
\linethickness{0.3mm}
\put(160,50){\line(0,1){20}}
\linethickness{0.3mm}
\put(120,50){\line(1,0){40}}
\linethickness{0.3mm}
\multiput(100,70)(0.12,-0.12){167}{\line(1,0){0.12}}
\linethickness{0.3mm}
\put(110,40){\line(0,1){20}}
\linethickness{0.3mm}
\put(130,35){\line(0,1){15}}
\linethickness{0.3mm}
\multiput(123.75,41.25)(0.12,-0.12){104}{\line(1,0){0.12}}
\linethickness{0.3mm}
\put(123.75,28.75){\line(1,0){12.5}}
\linethickness{0.3mm}
\put(123.75,28.75){\line(0,1){12.5}}
\linethickness{0.3mm}
\put(150,35){\line(0,1){15}}
\linethickness{0.3mm}
\multiput(143.75,41.25)(0.12,-0.12){104}{\line(1,0){0.12}}
\linethickness{0.3mm}
\put(143.75,28.75){\line(1,0){12.5}}
\linethickness{0.3mm}
\put(143.75,28.75){\line(0,1){12.5}}
\linethickness{0.3mm}
\multiput(140,10)(0.12,0.12){250}{\line(1,0){0.12}}
\linethickness{0.3mm}
\put(140,0){\line(0,1){10}}
\linethickness{0.3mm}
\put(170,40){\line(0,1){40}}
\linethickness{0.3mm}
\put(140,70){\line(0,1){20}}
\linethickness{0.3mm}
\put(40,85){\line(0,1){25}}
\linethickness{0.3mm}
\put(130,100){\line(1,0){50}}
\linethickness{0.3mm}
\put(180,80){\line(0,1){20}}
\linethickness{0.3mm}
\put(150,80){\line(1,0){30}}
\linethickness{0.3mm}
\multiput(130,100)(0.12,-0.12){167}{\line(1,0){0.12}}
\linethickness{0.3mm}
\put(160,100){\line(0,1){10}}
\linethickness{0.3mm}
\put(25,40){\line(1,0){10}}
\linethickness{0.3mm}
\put(35,30){\line(0,1){10}}
\linethickness{0.3mm}
\put(25,30){\line(1,0){10}}
\linethickness{0.3mm}
\put(25,30){\line(0,1){10}}
\linethickness{0.3mm}
\put(5,40){\line(1,0){10}}
\linethickness{0.3mm}
\put(15,30){\line(0,1){10}}
\linethickness{0.3mm}
\put(5,30){\line(1,0){10}}
\linethickness{0.3mm}
\put(5,30){\line(0,1){10}}
\linethickness{0.3mm}
\put(105,40){\line(1,0){10}}
\linethickness{0.3mm}
\put(115,30){\line(0,1){10}}
\linethickness{0.3mm}
\put(105,30){\line(1,0){10}}
\linethickness{0.3mm}
\put(105,30){\line(0,1){10}}
\linethickness{0.3mm}
\put(110,0){\line(0,1){30}}
\linethickness{0.3mm}
\put(10,0){\line(0,1){30}}
\put(80,75){\makebox(0,0)[cc]{\EQLS}}

\put(10,35){\makebox(0,0)[cc]{$\beee$}}

\put(30,35){\makebox(0,0)[cc]{$\feee$}}

\put(50,35){\makebox(0,0)[cc]{$\geee$}}

\put(126.88,33.12){\makebox(0,0)[cc]{$\Feee$}}

\put(146.88,33.12){\makebox(0,0)[cc]{$\Geee$}}

\put(40,10){\makebox(0,0)[cc]{\Dottt}}

\put(110,35){\makebox(0,0)[cc]{$\beee$}}

\put(35,75){\makebox(0,0)[cc]{$\IIIF$}}

\put(135,60){\makebox(0,0)[cc]{$\evv$}}

\put(160,90){\makebox(0,0)[cc]{$\evv$}}

\put(150,35){\makebox(0,0)[cc]{\dottt}}

\put(130,35){\makebox(0,0)[cc]{\dottt}}

\end{picture}


==> PIC/branch-2.tex <==
%%Created by jPicEdt 1.4.1_03: mixed JPIC-XML/LaTeX format
%%Fri Nov 04 07:19:11 GMT-10:00 2022
%%Begin JPIC-XML
%<?xml version="1.0" standalone="yes"?>
%<jpic x-min="0" x-max="160" y-min="0" y-max="110" auto-bounding="true">
%<multicurve fill-style= "none"
%	 points= "(0,85);(0,85);(60,85);(60,85)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(60,65);(60,65);(60,85);(60,85)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(20,65);(20,65);(60,65);(60,65)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(0,85);(0,85);(20,65);(20,65)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(10,75);(10,75);(10,0);(10,0)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(32.5,65);(32.5,65);(32.5,40);(32.5,40)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(25,23.75);(25,23.75);(25,20);(25,20)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(52.5,65);(52.5,65);(52.5,40);(52.5,40)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(40,40);(40,40);(55,40);(55,40)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(55,40);(55,40);(55,30);(55,30)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(55,30);(55,30);(50,30);(50,30)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(50,30);(50,30);(40,40);(40,40)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(45,23.75);(45,23.75);(45,20);(45,20)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(45,20);(45,20);(35,10);(35,10)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(25,20);(25,20);(35,10);(35,10)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(35,10);(35,10);(35,0);(35,0)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(100,70);(100,70);(160,70);(160,70)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(160,50);(160,50);(160,70);(160,70)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(120,50);(120,50);(160,50);(160,50)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(100,70);(100,70);(120,50);(120,50)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(110,60);(110,60);(110,0);(110,0)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(130,50);(130,50);(130,35);(130,35)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(125,40);(125,40);(135.62,29.38);(135.62,29.38)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(135.62,29.38);(135.62,29.38);(125,29.38);(125,29.38)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(125,29.38);(125,29.38);(125,40);(125,40)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(150,50);(150,50);(150,35);(150,35)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(145,40);(145,40);(155.62,29.38);(155.62,29.38)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(155.62,29.38);(155.62,29.38);(145,29.38);(145,29.38)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(145,29.38);(145,29.38);(145,40);(145,40)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(140,90);(140,90);(140,70);(140,70)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(40,110);(40,110);(40,85);(40,85)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(130,100);(130,100);(150,100);(150,100)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(150,80);(150,80);(150,100);(150,100)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(130,100);(130,100);(150,80);(150,80)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(140,110);(140,110);(140,100);(140,100)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(20,40);(20,40);(35,40);(35,40)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(35,40);(35,40);(35,30);(35,30)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(35,30);(35,30);(30,30);(30,30)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(30,30);(30,30);(20,40);(20,40)"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(80,75)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\EQLS
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(30,35)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\feee$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(50,35)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\geee$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(127.5,31.88)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\Feee$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(147.5,31.88)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\Geee$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(35,10)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\Dottt
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(35,75)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\IIIF$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(135,60)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\evv$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(143.75,92.5)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\evv$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(150,35)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\dottt
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(130,35)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\dottt
%</text>
%<multicurve fill-style= "none"
%	 points= "(130,29.38);(130,29.38);(130,18.75);(130,18.75)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(150,29.38);(150,29.38);(150,18.75);(150,18.75)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(150,18.75);(150,18.75);(140,8.75);(140,8.75)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(130,18.75);(130,18.75);(140,8.75);(140,8.75)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(140,8.75);(140,8.75);(140,0);(140,0)"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(140,8.75)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\Dottt
%</text>
%<multicurve fill-style= "none"
%	 points= "(45,35);(45,35);(45,28.75);(45,28.75)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(40,33.75);(40,33.75);(50,23.75);(50,23.75)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(50,23.75);(50,23.75);(40,23.75);(40,23.75)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(40,23.75);(40,23.75);(40,33.75);(40,33.75)"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(42.5,26.25)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\Feee$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(45,28.75)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\dottt
%</text>
%<multicurve fill-style= "none"
%	 points= "(25,35);(25,35);(25,28.75);(25,28.75)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(20,33.75);(20,33.75);(30,23.75);(30,23.75)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(30,23.75);(30,23.75);(20,23.75);(20,23.75)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(20,23.75);(20,23.75);(20,33.75);(20,33.75)"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(25,28.75)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\dottt
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(23.12,26.25)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\Geee$
%</text>
%</jpic>
%%End JPIC-XML
%LaTeX-picture environment using emulated lines and arcs
%You can rescale the whole picture (to 80% for instance) by using the command \def\JPicScale{0.8}
\ifx\JPicScale\undefined\def\JPicScale{1}\fi
\unitlength \JPicScale mm
\begin{picture}(160,110)(0,0)
\linethickness{0.3mm}
\put(0,85){\line(1,0){60}}
\linethickness{0.3mm}
\put(60,65){\line(0,1){20}}
\linethickness{0.3mm}
\put(20,65){\line(1,0){40}}
\linethickness{0.3mm}
\multiput(0,85)(0.12,-0.12){167}{\line(1,0){0.12}}
\linethickness{0.3mm}
\put(10,0){\line(0,1){75}}
\linethickness{0.3mm}
\put(32.5,40){\line(0,1){25}}
\linethickness{0.3mm}
\put(25,20){\line(0,1){3.75}}
\linethickness{0.3mm}
\put(52.5,40){\line(0,1){25}}
\linethickness{0.3mm}
\put(40,40){\line(1,0){15}}
\linethickness{0.3mm}
\put(55,30){\line(0,1){10}}
\linethickness{0.3mm}
\put(50,30){\line(1,0){5}}
\linethickness{0.3mm}
\multiput(40,40)(0.12,-0.12){83}{\line(1,0){0.12}}
\linethickness{0.3mm}
\put(45,20){\line(0,1){3.75}}
\linethickness{0.3mm}
\multiput(35,10)(0.12,0.12){83}{\line(1,0){0.12}}
\linethickness{0.3mm}
\multiput(25,20)(0.12,-0.12){83}{\line(1,0){0.12}}
\linethickness{0.3mm}
\put(35,0){\line(0,1){10}}
\linethickness{0.3mm}
\put(100,70){\line(1,0){60}}
\linethickness{0.3mm}
\put(160,50){\line(0,1){20}}
\linethickness{0.3mm}
\put(120,50){\line(1,0){40}}
\linethickness{0.3mm}
\multiput(100,70)(0.12,-0.12){167}{\line(1,0){0.12}}
\linethickness{0.3mm}
\put(110,0){\line(0,1){60}}
\linethickness{0.3mm}
\put(130,35){\line(0,1){15}}
\linethickness{0.3mm}
\multiput(125,40)(0.12,-0.12){89}{\line(1,0){0.12}}
\linethickness{0.3mm}
\put(125,29.38){\line(1,0){10.62}}
\linethickness{0.3mm}
\put(125,29.38){\line(0,1){10.62}}
\linethickness{0.3mm}
\put(150,35){\line(0,1){15}}
\linethickness{0.3mm}
\multiput(145,40)(0.12,-0.12){89}{\line(1,0){0.12}}
\linethickness{0.3mm}
\put(145,29.38){\line(1,0){10.62}}
\linethickness{0.3mm}
\put(145,29.38){\line(0,1){10.62}}
\linethickness{0.3mm}
\put(140,70){\line(0,1){20}}
\linethickness{0.3mm}
\put(40,85){\line(0,1){25}}
\linethickness{0.3mm}
\put(130,100){\line(1,0){20}}
\linethickness{0.3mm}
\put(150,80){\line(0,1){20}}
\linethickness{0.3mm}
\multiput(130,100)(0.12,-0.12){167}{\line(1,0){0.12}}
\linethickness{0.3mm}
\put(140,100){\line(0,1){10}}
\linethickness{0.3mm}
\put(20,40){\line(1,0){15}}
\linethickness{0.3mm}
\put(35,30){\line(0,1){10}}
\linethickness{0.3mm}
\put(30,30){\line(1,0){5}}
\linethickness{0.3mm}
\multiput(20,40)(0.12,-0.12){83}{\line(1,0){0.12}}
\put(80,75){\makebox(0,0)[cc]{\EQLS}}

\put(30,35){\makebox(0,0)[cc]{$\feee$}}

\put(50,35){\makebox(0,0)[cc]{$\geee$}}

\put(127.5,31.88){\makebox(0,0)[cc]{$\Feee$}}

\put(147.5,31.88){\makebox(0,0)[cc]{$\Geee$}}

\put(35,10){\makebox(0,0)[cc]{\Dottt}}

\put(35,75){\makebox(0,0)[cc]{$\IIIF$}}

\put(135,60){\makebox(0,0)[cc]{$\evv$}}

\put(143.75,92.5){\makebox(0,0)[cc]{$\evv$}}

\put(150,35){\makebox(0,0)[cc]{\dottt}}

\put(130,35){\makebox(0,0)[cc]{\dottt}}

\linethickness{0.3mm}
\put(130,18.75){\line(0,1){10.62}}
\linethickness{0.3mm}
\put(150,18.75){\line(0,1){10.62}}
\linethickness{0.3mm}
\multiput(140,8.75)(0.12,0.12){83}{\line(1,0){0.12}}
\linethickness{0.3mm}
\multiput(130,18.75)(0.12,-0.12){83}{\line(1,0){0.12}}
\linethickness{0.3mm}
\put(140,0){\line(0,1){8.75}}
\put(140,8.75){\makebox(0,0)[cc]{\Dottt}}

\linethickness{0.3mm}
\put(45,28.75){\line(0,1){6.25}}
\linethickness{0.3mm}
\multiput(40,33.75)(0.12,-0.12){83}{\line(1,0){0.12}}
\linethickness{0.3mm}
\put(40,23.75){\line(1,0){10}}
\linethickness{0.3mm}
\put(40,23.75){\line(0,1){10}}
\put(42.5,26.25){\makebox(0,0)[cc]{$\Feee$}}

\put(45,28.75){\makebox(0,0)[cc]{\dottt}}

\linethickness{0.3mm}
\put(25,28.75){\line(0,1){6.25}}
\linethickness{0.3mm}
\multiput(20,33.75)(0.12,-0.12){83}{\line(1,0){0.12}}
\linethickness{0.3mm}
\put(20,23.75){\line(1,0){10}}
\linethickness{0.3mm}
\put(20,23.75){\line(0,1){10}}
\put(25,28.75){\makebox(0,0)[cc]{\dottt}}

\put(23.12,26.25){\makebox(0,0)[cc]{$\Geee$}}

\end{picture}


==> PIC/branch-3.tex <==
%%Created by jPicEdt 1.4.1_03: mixed JPIC-XML/LaTeX format
%%Fri Nov 04 08:32:44 GMT-10:00 2022
%%Begin JPIC-XML
%<?xml version="1.0" standalone="yes"?>
%<jpic x-min="0" x-max="250" y-min="0" y-max="90" auto-bounding="true">
%<multicurve fill-style= "none"
%	 points= "(95,65);(95,65);(155,65);(155,65)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(155,45);(155,45);(155,65);(155,65)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(95,45);(95,45);(155,45);(155,45)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(95,65);(95,65);(95,45);(95,45)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(0,50);(0,50);(60,50);(60,50)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(60,30);(60,30);(60,50);(60,50)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(20,30);(20,30);(60,30);(60,30)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(0,50);(0,50);(20,30);(20,30)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(10,40);(10,40);(10,20);(10,20)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(30,30);(30,30);(30,15);(30,15)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(50,30);(50,30);(50,15);(50,15)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(50,70);(50,70);(50,50);(50,50)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(125,90);(125,90);(125,65);(125,65)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(40,80);(40,80);(60,80);(60,80)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(60,60);(60,60);(60,80);(60,80)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(40,80);(40,80);(60,60);(60,60)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(50,90);(50,90);(50,80);(50,80)"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(80,52.5)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\EQLS
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(35,40)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\evv$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(53.75,72.5)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\evv$
%</text>
%<multicurve fill-style= "none"
%	 points= "(105,45);(105,45);(105,20);(105,20)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(125,45);(125,45);(125,15);(125,15)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(120,20);(120,20);(131.25,8.75);(131.25,8.75)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(131.25,8.75);(131.25,8.75);(120,8.75);(120,8.75)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(120,8.75);(120,8.75);(120,20);(120,20)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(145,45);(145,45);(145,15);(145,15)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(140,20);(140,20);(151.25,8.75);(151.25,8.75)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(151.25,8.75);(151.25,8.75);(140,8.75);(140,8.75)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(140,8.75);(140,8.75);(140,20);(140,20)"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(122.5,11.88)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\Feee$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(143.12,11.88)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\Geee$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(145,15)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\dottt
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(125,15)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\dottt
%</text>
%<multicurve fill-style= "none"
%	 points= "(125,8.75);(125,8.75);(125,0);(125,0)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(145,8.75);(145,8.75);(145,0);(145,0)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(100,20);(100,20);(110,20);(110,20)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(110,20);(110,20);(110,8.75);(110,8.75)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(110,8.75);(110,8.75);(100,8.75);(100,8.75)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(100,8.75);(100,8.75);(100,20);(100,20)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(105,8.75);(105,8.75);(105,0);(105,0)"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(105,14.38)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\beee$
%</text>
%<multicurve fill-style= "none"
%	 points= "(230,80);(230,80);(250,80);(250,80)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(250,60);(250,60);(250,80);(250,80)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(190,45);(190,45);(250,45);(250,45)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(190,65);(190,65);(190,45);(190,45)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(240,90);(240,90);(240,80);(240,80)"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(175,52.5)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\EQLS
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(215,55)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\IIIF$
%</text>
%<multicurve fill-style= "none"
%	 points= "(200,45);(200,45);(200,20);(200,20)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(220,45);(220,45);(220,15);(220,15)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(240,45);(240,45);(240,15);(240,15)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(230,80);(230,80);(250,60);(250,60)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(190,65);(190,65);(230,65);(230,65)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(230,65);(230,65);(250,45);(250,45)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(240,70);(240,70);(240,55);(240,55)"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(240,55)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\dottt
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(245,72.5)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\evv$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(125,55)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\iiif$
%</text>
%<multicurve fill-style= "none"
%	 points= "(25,20);(25,20);(36.25,8.75);(36.25,8.75)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(36.25,8.75);(36.25,8.75);(25,8.75);(25,8.75)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(25,8.75);(25,8.75);(25,20);(25,20)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(45,20);(45,20);(56.25,8.75);(56.25,8.75)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(56.25,8.75);(56.25,8.75);(45,8.75);(45,8.75)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(45,8.75);(45,8.75);(45,20);(45,20)"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(27.5,11.88)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\Feee$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(48.12,11.88)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\Geee$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(50,15)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\dottt
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(30,15)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\dottt
%</text>
%<multicurve fill-style= "none"
%	 points= "(30,8.75);(30,8.75);(30,0);(30,0)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(50,8.75);(50,8.75);(50,0);(50,0)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(5,20);(5,20);(15,20);(15,20)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(15,20);(15,20);(15,8.75);(15,8.75)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(15,8.75);(15,8.75);(5,8.75);(5,8.75)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(5,8.75);(5,8.75);(5,20);(5,20)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(10,8.75);(10,8.75);(10,0);(10,0)"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(10,14.38)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\beee$
%</text>
%<multicurve fill-style= "none"
%	 points= "(215,20);(215,20);(226.25,8.75);(226.25,8.75)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(226.25,8.75);(226.25,8.75);(215,8.75);(215,8.75)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(215,8.75);(215,8.75);(215,20);(215,20)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(235,20);(235,20);(246.25,8.75);(246.25,8.75)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(246.25,8.75);(246.25,8.75);(235,8.75);(235,8.75)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(235,8.75);(235,8.75);(235,20);(235,20)"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(217.5,11.88)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\Feee$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(238.12,11.88)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\Geee$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(240,15)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\dottt
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(220,15)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\dottt
%</text>
%<multicurve fill-style= "none"
%	 points= "(220,8.75);(220,8.75);(220,0);(220,0)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(240,8.75);(240,8.75);(240,0);(240,0)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(195,20);(195,20);(205,20);(205,20)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(205,20);(205,20);(205,8.75);(205,8.75)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(205,8.75);(205,8.75);(195,8.75);(195,8.75)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(195,8.75);(195,8.75);(195,20);(195,20)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(200,8.75);(200,8.75);(200,0);(200,0)"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(200,14.38)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\beee$
%</text>
%</jpic>
%%End JPIC-XML
%LaTeX-picture environment using emulated lines and arcs
%You can rescale the whole picture (to 80% for instance) by using the command \def\JPicScale{0.8}
\ifx\JPicScale\undefined\def\JPicScale{1}\fi
\unitlength \JPicScale mm
\begin{picture}(250,90)(0,0)
\linethickness{0.3mm}
\put(95,65){\line(1,0){60}}
\linethickness{0.3mm}
\put(155,45){\line(0,1){20}}
\linethickness{0.3mm}
\put(95,45){\line(1,0){60}}
\linethickness{0.3mm}
\put(95,45){\line(0,1){20}}
\linethickness{0.3mm}
\put(0,50){\line(1,0){60}}
\linethickness{0.3mm}
\put(60,30){\line(0,1){20}}
\linethickness{0.3mm}
\put(20,30){\line(1,0){40}}
\linethickness{0.3mm}
\multiput(0,50)(0.12,-0.12){167}{\line(1,0){0.12}}
\linethickness{0.3mm}
\put(10,20){\line(0,1){20}}
\linethickness{0.3mm}
\put(30,15){\line(0,1){15}}
\linethickness{0.3mm}
\put(50,15){\line(0,1){15}}
\linethickness{0.3mm}
\put(50,50){\line(0,1){20}}
\linethickness{0.3mm}
\put(125,65){\line(0,1){25}}
\linethickness{0.3mm}
\put(40,80){\line(1,0){20}}
\linethickness{0.3mm}
\put(60,60){\line(0,1){20}}
\linethickness{0.3mm}
\multiput(40,80)(0.12,-0.12){167}{\line(1,0){0.12}}
\linethickness{0.3mm}
\put(50,80){\line(0,1){10}}
\put(80,52.5){\makebox(0,0)[cc]{\EQLS}}

\put(35,40){\makebox(0,0)[cc]{$\evv$}}

\put(53.75,72.5){\makebox(0,0)[cc]{$\evv$}}

\linethickness{0.3mm}
\put(105,20){\line(0,1){25}}
\linethickness{0.3mm}
\put(125,15){\line(0,1){30}}
\linethickness{0.3mm}
\multiput(120,20)(0.12,-0.12){94}{\line(1,0){0.12}}
\linethickness{0.3mm}
\put(120,8.75){\line(1,0){11.25}}
\linethickness{0.3mm}
\put(120,8.75){\line(0,1){11.25}}
\linethickness{0.3mm}
\put(145,15){\line(0,1){30}}
\linethickness{0.3mm}
\multiput(140,20)(0.12,-0.12){94}{\line(1,0){0.12}}
\linethickness{0.3mm}
\put(140,8.75){\line(1,0){11.25}}
\linethickness{0.3mm}
\put(140,8.75){\line(0,1){11.25}}
\put(122.5,11.88){\makebox(0,0)[cc]{$\Feee$}}

\put(143.12,11.88){\makebox(0,0)[cc]{$\Geee$}}

\put(145,15){\makebox(0,0)[cc]{\dottt}}

\put(125,15){\makebox(0,0)[cc]{\dottt}}

\linethickness{0.3mm}
\put(125,0){\line(0,1){8.75}}
\linethickness{0.3mm}
\put(145,0){\line(0,1){8.75}}
\linethickness{0.3mm}
\put(100,20){\line(1,0){10}}
\linethickness{0.3mm}
\put(110,8.75){\line(0,1){11.25}}
\linethickness{0.3mm}
\put(100,8.75){\line(1,0){10}}
\linethickness{0.3mm}
\put(100,8.75){\line(0,1){11.25}}
\linethickness{0.3mm}
\put(105,0){\line(0,1){8.75}}
\put(105,14.38){\makebox(0,0)[cc]{$\beee$}}

\linethickness{0.3mm}
\put(230,80){\line(1,0){20}}
\linethickness{0.3mm}
\put(250,60){\line(0,1){20}}
\linethickness{0.3mm}
\put(190,45){\line(1,0){60}}
\linethickness{0.3mm}
\put(190,45){\line(0,1){20}}
\linethickness{0.3mm}
\put(240,80){\line(0,1){10}}
\put(175,52.5){\makebox(0,0)[cc]{\EQLS}}

\put(215,55){\makebox(0,0)[cc]{$\IIIF$}}

\linethickness{0.3mm}
\put(200,20){\line(0,1){25}}
\linethickness{0.3mm}
\put(220,15){\line(0,1){30}}
\linethickness{0.3mm}
\put(240,15){\line(0,1){30}}
\linethickness{0.3mm}
\multiput(230,80)(0.12,-0.12){167}{\line(1,0){0.12}}
\linethickness{0.3mm}
\put(190,65){\line(1,0){40}}
\linethickness{0.3mm}
\multiput(230,65)(0.12,-0.12){167}{\line(1,0){0.12}}
\linethickness{0.3mm}
\put(240,55){\line(0,1){15}}
\put(240,55){\makebox(0,0)[cc]{\dottt}}

\put(245,72.5){\makebox(0,0)[cc]{$\evv$}}

\put(125,55){\makebox(0,0)[cc]{$\iiif$}}

\linethickness{0.3mm}
\multiput(25,20)(0.12,-0.12){94}{\line(1,0){0.12}}
\linethickness{0.3mm}
\put(25,8.75){\line(1,0){11.25}}
\linethickness{0.3mm}
\put(25,8.75){\line(0,1){11.25}}
\linethickness{0.3mm}
\multiput(45,20)(0.12,-0.12){94}{\line(1,0){0.12}}
\linethickness{0.3mm}
\put(45,8.75){\line(1,0){11.25}}
\linethickness{0.3mm}
\put(45,8.75){\line(0,1){11.25}}
\put(27.5,11.88){\makebox(0,0)[cc]{$\Feee$}}

\put(48.12,11.88){\makebox(0,0)[cc]{$\Geee$}}

\put(50,15){\makebox(0,0)[cc]{\dottt}}

\put(30,15){\makebox(0,0)[cc]{\dottt}}

\linethickness{0.3mm}
\put(30,0){\line(0,1){8.75}}
\linethickness{0.3mm}
\put(50,0){\line(0,1){8.75}}
\linethickness{0.3mm}
\put(5,20){\line(1,0){10}}
\linethickness{0.3mm}
\put(15,8.75){\line(0,1){11.25}}
\linethickness{0.3mm}
\put(5,8.75){\line(1,0){10}}
\linethickness{0.3mm}
\put(5,8.75){\line(0,1){11.25}}
\linethickness{0.3mm}
\put(10,0){\line(0,1){8.75}}
\put(10,14.38){\makebox(0,0)[cc]{$\beee$}}

\linethickness{0.3mm}
\multiput(215,20)(0.12,-0.12){94}{\line(1,0){0.12}}
\linethickness{0.3mm}
\put(215,8.75){\line(1,0){11.25}}
\linethickness{0.3mm}
\put(215,8.75){\line(0,1){11.25}}
\linethickness{0.3mm}
\multiput(235,20)(0.12,-0.12){94}{\line(1,0){0.12}}
\linethickness{0.3mm}
\put(235,8.75){\line(1,0){11.25}}
\linethickness{0.3mm}
\put(235,8.75){\line(0,1){11.25}}
\put(217.5,11.88){\makebox(0,0)[cc]{$\Feee$}}

\put(238.12,11.88){\makebox(0,0)[cc]{$\Geee$}}

\put(240,15){\makebox(0,0)[cc]{\dottt}}

\put(220,15){\makebox(0,0)[cc]{\dottt}}

\linethickness{0.3mm}
\put(220,0){\line(0,1){8.75}}
\linethickness{0.3mm}
\put(240,0){\line(0,1){8.75}}
\linethickness{0.3mm}
\put(195,20){\line(1,0){10}}
\linethickness{0.3mm}
\put(205,8.75){\line(0,1){11.25}}
\linethickness{0.3mm}
\put(195,8.75){\line(1,0){10}}
\linethickness{0.3mm}
\put(195,8.75){\line(0,1){11.25}}
\linethickness{0.3mm}
\put(200,0){\line(0,1){8.75}}
\put(200,14.38){\makebox(0,0)[cc]{$\beee$}}

\end{picture}


==> PIC/branch.tex <==
%%Created by jPicEdt 1.4.1_03: mixed JPIC-XML/LaTeX format
%%Mon Sep 05 19:15:24 GMT-10:00 2022
%%Begin JPIC-XML
%<?xml version="1.0" standalone="yes"?>
%<jpic x-min="0" x-max="180" y-min="0" y-max="110" auto-bounding="true">
%<multicurve fill-style= "none"
%	 points= "(0,85);(0,85);(60,85);(60,85)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(60,65);(60,65);(60,85);(60,85)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(20,65);(20,65);(60,65);(60,65)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(0,85);(0,85);(20,65);(20,65)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(10,75);(10,75);(10,40);(10,40)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(30,65);(30,65);(30,40);(30,40)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(30,30);(30,30);(30,20);(30,20)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(50,65);(50,65);(50,40);(50,40)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(45,40);(45,40);(55,40);(55,40)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(55,40);(55,40);(55,30);(55,30)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(55,30);(55,30);(45,30);(45,30)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(45,30);(45,30);(45,40);(45,40)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(50,30);(50,30);(50,20);(50,20)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(50,20);(50,20);(40,10);(40,10)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(30,20);(30,20);(40,10);(40,10)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(40,10);(40,10);(40,0);(40,0)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(100,70);(100,70);(160,70);(160,70)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(160,50);(160,50);(160,70);(160,70)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(120,50);(120,50);(160,50);(160,50)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(100,70);(100,70);(120,50);(120,50)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(110,60);(110,60);(110,40);(110,40)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(130,50);(130,50);(130,35);(130,35)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(125,40);(125,40);(135,30);(135,30)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(135,30);(135,30);(125,30);(125,30)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(125,30);(125,30);(125,40);(125,40)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(150,50);(150,50);(150,35);(150,35)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(145,40);(145,40);(155,30);(155,30)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(155,30);(155,30);(145,30);(145,30)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(145,30);(145,30);(145,40);(145,40)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(170,40);(170,40);(140,10);(140,10)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(140,10);(140,10);(140,0);(140,0)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(170,80);(170,80);(170,40);(170,40)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(140,90);(140,90);(140,70);(140,70)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(40,110);(40,110);(40,85);(40,85)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(130,100);(130,100);(180,100);(180,100)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(180,80);(180,80);(180,100);(180,100)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(150,80);(150,80);(180,80);(180,80)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(130,100);(130,100);(150,80);(150,80)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(160,110);(160,110);(160,100);(160,100)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(25,40);(25,40);(35,40);(35,40)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(35,40);(35,40);(35,30);(35,30)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(35,30);(35,30);(25,30);(25,30)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(25,30);(25,30);(25,40);(25,40)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(5,40);(5,40);(15,40);(15,40)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(15,40);(15,40);(15,30);(15,30)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(15,30);(15,30);(5,30);(5,30)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(5,30);(5,30);(5,40);(5,40)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(105,40);(105,40);(115,40);(115,40)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(115,40);(115,40);(115,30);(115,30)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(115,30);(115,30);(105,30);(105,30)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(105,30);(105,30);(105,40);(105,40)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(110,30);(110,30);(110,0);(110,0)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(10,30);(10,30);(10,0);(10,0)"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(80,75)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\EQLS
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(10,35)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\beee$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(30,35)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\feee$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(50,35)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\geee$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(127.5,32.5)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\Feee$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(147.5,32.5)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\Geee$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(40,10)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\Dottt
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(110,35)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\beee$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(35,75)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\IIIF$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(135,60)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\evv$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(160,90)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\evv$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(150,35)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\dottt
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(130,35)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\dottt
%</text>
%</jpic>
%%End JPIC-XML
%LaTeX-picture environment using emulated lines and arcs
%You can rescale the whole picture (to 80% for instance) by using the command \def\JPicScale{0.8}
\ifx\JPicScale\undefined\def\JPicScale{1}\fi
\unitlength \JPicScale mm
\begin{picture}(180,110)(0,0)
\linethickness{0.3mm}
\put(0,85){\line(1,0){60}}
\linethickness{0.3mm}
\put(60,65){\line(0,1){20}}
\linethickness{0.3mm}
\put(20,65){\line(1,0){40}}
\linethickness{0.3mm}
\multiput(0,85)(0.12,-0.12){167}{\line(1,0){0.12}}
\linethickness{0.3mm}
\put(10,40){\line(0,1){35}}
\linethickness{0.3mm}
\put(30,40){\line(0,1){25}}
\linethickness{0.3mm}
\put(30,20){\line(0,1){10}}
\linethickness{0.3mm}
\put(50,40){\line(0,1){25}}
\linethickness{0.3mm}
\put(45,40){\line(1,0){10}}
\linethickness{0.3mm}
\put(55,30){\line(0,1){10}}
\linethickness{0.3mm}
\put(45,30){\line(1,0){10}}
\linethickness{0.3mm}
\put(45,30){\line(0,1){10}}
\linethickness{0.3mm}
\put(50,20){\line(0,1){10}}
\linethickness{0.3mm}
\multiput(40,10)(0.12,0.12){83}{\line(1,0){0.12}}
\linethickness{0.3mm}
\multiput(30,20)(0.12,-0.12){83}{\line(1,0){0.12}}
\linethickness{0.3mm}
\put(40,0){\line(0,1){10}}
\linethickness{0.3mm}
\put(100,70){\line(1,0){60}}
\linethickness{0.3mm}
\put(160,50){\line(0,1){20}}
\linethickness{0.3mm}
\put(120,50){\line(1,0){40}}
\linethickness{0.3mm}
\multiput(100,70)(0.12,-0.12){167}{\line(1,0){0.12}}
\linethickness{0.3mm}
\put(110,40){\line(0,1){20}}
\linethickness{0.3mm}
\put(130,35){\line(0,1){15}}
\linethickness{0.3mm}
\multiput(125,40)(0.12,-0.12){83}{\line(1,0){0.12}}
\linethickness{0.3mm}
\put(125,30){\line(1,0){10}}
\linethickness{0.3mm}
\put(125,30){\line(0,1){10}}
\linethickness{0.3mm}
\put(150,35){\line(0,1){15}}
\linethickness{0.3mm}
\multiput(145,40)(0.12,-0.12){83}{\line(1,0){0.12}}
\linethickness{0.3mm}
\put(145,30){\line(1,0){10}}
\linethickness{0.3mm}
\put(145,30){\line(0,1){10}}
\linethickness{0.3mm}
\multiput(140,10)(0.12,0.12){250}{\line(1,0){0.12}}
\linethickness{0.3mm}
\put(140,0){\line(0,1){10}}
\linethickness{0.3mm}
\put(170,40){\line(0,1){40}}
\linethickness{0.3mm}
\put(140,70){\line(0,1){20}}
\linethickness{0.3mm}
\put(40,85){\line(0,1){25}}
\linethickness{0.3mm}
\put(130,100){\line(1,0){50}}
\linethickness{0.3mm}
\put(180,80){\line(0,1){20}}
\linethickness{0.3mm}
\put(150,80){\line(1,0){30}}
\linethickness{0.3mm}
\multiput(130,100)(0.12,-0.12){167}{\line(1,0){0.12}}
\linethickness{0.3mm}
\put(160,100){\line(0,1){10}}
\linethickness{0.3mm}
\put(25,40){\line(1,0){10}}
\linethickness{0.3mm}
\put(35,30){\line(0,1){10}}
\linethickness{0.3mm}
\put(25,30){\line(1,0){10}}
\linethickness{0.3mm}
\put(25,30){\line(0,1){10}}
\linethickness{0.3mm}
\put(5,40){\line(1,0){10}}
\linethickness{0.3mm}
\put(15,30){\line(0,1){10}}
\linethickness{0.3mm}
\put(5,30){\line(1,0){10}}
\linethickness{0.3mm}
\put(5,30){\line(0,1){10}}
\linethickness{0.3mm}
\put(105,40){\line(1,0){10}}
\linethickness{0.3mm}
\put(115,30){\line(0,1){10}}
\linethickness{0.3mm}
\put(105,30){\line(1,0){10}}
\linethickness{0.3mm}
\put(105,30){\line(0,1){10}}
\linethickness{0.3mm}
\put(110,0){\line(0,1){30}}
\linethickness{0.3mm}
\put(10,0){\line(0,1){30}}
\put(80,75){\makebox(0,0)[cc]{\EQLS}}

\put(10,35){\makebox(0,0)[cc]{$\beee$}}

\put(30,35){\makebox(0,0)[cc]{$\feee$}}

\put(50,35){\makebox(0,0)[cc]{$\geee$}}

\put(127.5,32.5){\makebox(0,0)[cc]{$\Feee$}}

\put(147.5,32.5){\makebox(0,0)[cc]{$\Geee$}}

\put(40,10){\makebox(0,0)[cc]{\Dottt}}

\put(110,35){\makebox(0,0)[cc]{$\beee$}}

\put(35,75){\makebox(0,0)[cc]{$\IIIF$}}

\put(135,60){\makebox(0,0)[cc]{$\evv$}}

\put(160,90){\makebox(0,0)[cc]{$\evv$}}

\put(150,35){\makebox(0,0)[cc]{\dottt}}

\put(130,35){\makebox(0,0)[cc]{\dottt}}

\end{picture}


==> PIC/cmn-four.tex <==
%%Created by jPicEdt 1.4.1_03: mixed JPIC-XML/LaTeX format
%%Sat Sep 02 17:46:24 HST 2017
%%Begin JPIC-XML
%<?xml version="1.0" standalone="yes"?>
%<jpic x-min="2.5" x-max="17.5" y-min="-7.5" y-max="10" auto-bounding="true">
%<ellipse p3= "(8.43,1.56)"
%	 p2= "(8.43,-1.56)"
%	 p1= "(11.56,-1.56)"
%	 closure= "open"
%	 angle-end= "0"
%	 fill-style= "solid"
%	 angle-start= "0"
%	 />
%<multicurve points= "(10,0);(10,0);(10,-7.5);(10,-7.5)"
%	 fill-style= "none"
%	 />
%<multicurve points= "(17.5,5);(17.5,5);(10,0);(10,0)"
%	 fill-style= "none"
%	 />
%<multicurve points= "(12.5,5);(12.5,5);(10,0);(10,0)"
%	 fill-style= "none"
%	 />
%<multicurve points= "(2.5,5);(2.5,5);(10,0);(10,0)"
%	 fill-style= "none"
%	 />
%<multicurve points= "(17.5,10);(17.5,10);(17.5,5);(17.5,5)"
%	 fill-style= "none"
%	 />
%<multicurve points= "(2.5,10);(2.5,10);(2.5,5);(2.5,5)"
%	 fill-style= "none"
%	 />
%<multicurve points= "(7.5,5);(7.5,5);(10,0);(10,0)"
%	 fill-style= "none"
%	 />
%<multicurve points= "(12.5,10);(12.5,10);(12.5,5);(12.5,5)"
%	 fill-style= "none"
%	 />
%<multicurve points= "(7.5,10);(7.5,10);(7.5,5);(7.5,5)"
%	 fill-style= "none"
%	 />
%</jpic>
%%End JPIC-XML
%PSTricks content-type (pstricks.sty package needed)
%Add \usepackage{pstricks} in the preamble of your LaTeX file
%You can rescale the whole picture (to 80% for instance) by using the command \def\JPicScale{0.8}
\ifx\JPicScale\undefined\def\JPicScale{1}\fi
\psset{unit=\JPicScale mm}
\psset{linewidth=0.3,dotsep=1,hatchwidth=0.3,hatchsep=1.5,shadowsize=1,dimen=middle}
\psset{dotsize=0.7 2.5,dotscale=1 1,fillcolor=black}
\psset{arrowsize=1 2,arrowlength=1,arrowinset=0.25,tbarsize=0.7 5,bracketlength=0.15,rbracketlength=0.15}
\begin{pspicture}(0,0)(17.5,10)
\rput{0}(10,0){\psellipse[fillstyle=solid](0,0)(1.56,-1.57)}
\psline(10,0)(10,-7.5)
\psline(17.5,5)(10,0)
\psline(12.5,5)(10,0)
\psline(2.5,5)(10,0)
\psline(17.5,10)(17.5,5)
\psline(2.5,10)(2.5,5)
\psline(7.5,5)(10,0)
\psline(12.5,10)(12.5,5)
\psline(7.5,10)(7.5,5)
\end{pspicture}


==> PIC/cmn-id.tex <==
%%Created by jPicEdt 1.4.1_03: mixed JPIC-XML/LaTeX format
%%Sat Sep 02 17:28:32 HST 2017
%%Begin JPIC-XML
%<?xml version="1.0" standalone="yes"?>
%<jpic x-min="-2.19" x-max="45" y-min="-10.62" y-max="8.12" auto-bounding="true">
%<text text-vert-align= "center-v"
%	 anchor-point= "(38.12,1.88)"
%	 text-frame= "noframe"
%	 fill-style= "none"
%	 text-hor-align= "center-h"
%	 >
%$=$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(14.38,1.25)"
%	 text-frame= "noframe"
%	 fill-style= "none"
%	 text-hor-align= "center-h"
%	 >
%$=$
%</text>
%<ellipse p3= "(29.06,2.81)"
%	 p2= "(29.06,-0.31)"
%	 p1= "(32.19,-0.31)"
%	 closure= "open"
%	 angle-end= "0"
%	 fill-style= "solid"
%	 angle-start= "0"
%	 />
%<ellipse p3= "(22.81,-3.44)"
%	 p2= "(22.81,-6.56)"
%	 p1= "(25.94,-6.56)"
%	 closure= "open"
%	 angle-end= "0"
%	 fill-style= "solid"
%	 angle-start= "0"
%	 />
%<multicurve points= "(0.62,0);(0.62,0);(5.62,-5);(5.62,-5);(5.62,-5);(4.38,-5);
%	(4.38,-5);(4.38,-5);(5,-5);(5,-5)"
%	 fill-style= "none"
%	 />
%<multicurve points= "(24.38,-6.25);(24.38,-6.25);(24.38,-10);(24.38,-10);(24.38,-10);(24.38,-10.62);
%	(24.38,-10.62);(24.38,-10.62);(24.38,-10);(24.38,-10)"
%	 fill-style= "none"
%	 />
%<multicurve points= "(19.37,8.12);(19.37,8.12);(19.38,1.87);(19.38,1.87);(19.38,1.87);(19.38,0);
%	(19.38,0);(19.38,0);(23.13,-3.75);(23.13,-3.75)"
%	 fill-style= "none"
%	 />
%<ellipse p3= "(-2.19,2.81)"
%	 p2= "(-2.19,-0.31)"
%	 p1= "(0.94,-0.31)"
%	 closure= "open"
%	 angle-end= "0"
%	 fill-style= "solid"
%	 angle-start= "0"
%	 />
%<ellipse p3= "(3.75,-3.13)"
%	 p2= "(3.75,-6.25)"
%	 p1= "(6.88,-6.25)"
%	 closure= "open"
%	 angle-end= "0"
%	 fill-style= "solid"
%	 angle-start= "0"
%	 />
%<multicurve points= "(10,8.12);(10,8.12);(10,5.62);(10,5.62);(10,5.62);(10,0);
%	(10,0);(10,0);(6.25,-3.75);(6.25,-3.75)"
%	 fill-style= "none"
%	 />
%<multicurve points= "(5,-6.25);(5,-6.25);(5,-10);(5,-10);(5,-10);(5,-10.62);
%	(5,-10.62);(5,-10.62);(5,-10);(5,-10)"
%	 fill-style= "none"
%	 />
%<multicurve points= "(29.38,0);(29.38,0);(24.38,-5);(24.38,-5);(24.38,-5);(24.38,-5);
%	(24.38,-5);(24.38,-5);(24.38,-5);(24.38,-5)"
%	 fill-style= "none"
%	 />
%<multicurve points= "(45,8.12);(45,8.12);(45,-10);(45,-10);(45,-10);(45,-10.62);
%	(45,-10.62);(45,-10.62);(45,-10);(45,-10)"
%	 fill-style= "none"
%	 />
%</jpic>
%%End JPIC-XML
%PSTricks content-type (pstricks.sty package needed)
%Add \usepackage{pstricks} in the preamble of your LaTeX file
%You can rescale the whole picture (to 80% for instance) by using the command \def\JPicScale{0.8}
\ifx\JPicScale\undefined\def\JPicScale{1}\fi
\psset{unit=\JPicScale mm}
\psset{linewidth=0.3,dotsep=1,hatchwidth=0.3,hatchsep=1.5,shadowsize=1,dimen=middle}
\psset{dotsize=0.7 2.5,dotscale=1 1,fillcolor=black}
\psset{arrowsize=1 2,arrowlength=1,arrowinset=0.25,tbarsize=0.7 5,bracketlength=0.15,rbracketlength=0.15}
\begin{pspicture}(0,0)(45,8.12)
\rput(38.12,1.88){$=$}
\rput(14.38,1.25){$=$}
\rput{0}(30.62,1.25){\psellipse[fillstyle=solid](0,0)(1.56,-1.56)}
\rput{0}(24.38,-5){\psellipse[fillstyle=solid](0,0)(1.57,-1.56)}
\psline(0.62,0)
(5.62,-5)
(4.38,-5)(5,-5)
\psline(24.38,-6.25)
(24.38,-10)
(24.38,-10.62)(24.38,-10)
\psline(19.37,8.12)
(19.38,1.87)
(19.38,0)(23.13,-3.75)
\rput{0}(-0.62,1.25){\psellipse[fillstyle=solid](0,0)(1.57,-1.56)}
\rput{0}(5.31,-4.69){\psellipse[fillstyle=solid](0,0)(1.57,-1.56)}
\psline(10,8.12)
(10,5.62)
(10,0)(6.25,-3.75)
\psline(5,-6.25)
(5,-10)
(5,-10.62)(5,-10)
\pscustom[]{\psline(29.38,0)(24.38,-5)
\psbezier(24.38,-5)(24.38,-5)(24.38,-5)
\psbezier(24.38,-5)(24.38,-5)(24.38,-5)
}
\psline(45,8.12)
(45,-10)
(45,-10.62)(45,-10)
\end{pspicture}


==> PIC/cmn-left.tex <==
%%Created by jPicEdt 1.4.1_03: mixed JPIC-XML/LaTeX format
%%Tue Nov 05 13:13:30 GMT-10:00 2019
%%Begin JPIC-XML
%<?xml version="1.0" standalone="yes"?>
%<jpic x-min="-0.63" x-max="15" y-min="-10.62" y-max="7.5" auto-bounding="true">
%<multicurve fill-style= "none"
%	 points= "(5.62,-0.62);(5.62,-0.62);(10.62,-5.62);(10.62,-5.62);(10.62,-5.62);(9.38,-5.62);
%	(9.38,-5.62);(9.38,-5.62);(10,-5.62);(10,-5.62)"
%	 />
%<ellipse fill-style= "solid"
%	 p3= "(2.81,2.19)"
%	 p2= "(2.81,-0.94)"
%	 p1= "(5.94,-0.94)"
%	 closure= "open"
%	 angle-end= "0"
%	 angle-start= "0"
%	 />
%<ellipse fill-style= "solid"
%	 p3= "(8.75,-3.75)"
%	 p2= "(8.75,-6.88)"
%	 p1= "(11.88,-6.88)"
%	 closure= "open"
%	 angle-end= "0"
%	 angle-start= "0"
%	 />
%<multicurve fill-style= "none"
%	 points= "(15,7.5);(15,7.5);(15,5);(15,5);(15,5);(15,-0.63);
%	(15,-0.63);(15,-0.63);(11.25,-4.38);(11.25,-4.38)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(9.37,7.5);(9.37,7.5);(9.37,6.87);(9.37,6.87);(9.37,6.87);(9.38,5);
%	(9.38,5);(9.38,5);(5.63,1.25);(5.63,1.25)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(-0.63,7.5);(-0.63,7.5);(-0.63,6.87);(-0.63,6.87);(-0.63,6.87);(-0.62,5);
%	(-0.62,5);(-0.62,5);(3.13,1.25);(3.13,1.25)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(10,-6.88);(10,-6.88);(10,-10);(10,-10);(10,-10);(10,-10.62);
%	(10,-10.62);(10,-10.62);(10,-10);(10,-10)"
%	 />
%</jpic>
%%End JPIC-XML
%PSTricks content-type (pstricks.sty package needed)
%Add \usepackage{pstricks} in the preamble of your LaTeX file
%You can rescale the whole picture (to 80% for instance) by using the command \def\JPicScale{0.8}
\ifx\JPicScale\undefined\def\JPicScale{1}\fi
\psset{unit=\JPicScale mm}
\psset{linewidth=0.3,dotsep=1,hatchwidth=0.3,hatchsep=1.5,shadowsize=1,dimen=middle}
\psset{dotsize=0.7 2.5,dotscale=1 1,fillcolor=black}
\psset{arrowsize=1 2,arrowlength=1,arrowinset=0.25,tbarsize=0.7 5,bracketlength=0.15,rbracketlength=0.15}
\begin{pspicture}(0,0)(15,7.5)
\psline(5.62,-0.62)
(10.62,-5.62)
(9.38,-5.62)(10,-5.62)
\rput{0}(4.38,0.62){\psellipse[fillstyle=solid](0,0)(1.56,-1.57)}
\rput{0}(10.32,-5.31){\psellipse[fillstyle=solid](0,0)(1.56,-1.57)}
\psline(15,7.5)
(15,5)
(15,-0.63)(11.25,-4.38)
\psline(9.37,7.5)
(9.37,6.87)
(9.38,5)(5.63,1.25)
\psline(-0.63,7.5)
(-0.63,6.87)
(-0.62,5)(3.13,1.25)
\psline(10,-6.88)
(10,-10)
(10,-10.62)(10,-10)
\end{pspicture}


==> PIC/cmn-multi.tex <==
%%Created by jPicEdt 1.4.1_03: mixed JPIC-XML/LaTeX format
%%Sat Sep 02 17:44:40 HST 2017
%%Begin JPIC-XML
%<?xml version="1.0" standalone="yes"?>
%<jpic x-min="5" x-max="15" y-min="-7.5" y-max="10" auto-bounding="true">
%<ellipse p3= "(8.43,1.56)"
%	 p2= "(8.43,-1.56)"
%	 p1= "(11.56,-1.56)"
%	 closure= "open"
%	 angle-end= "0"
%	 fill-style= "solid"
%	 angle-start= "0"
%	 />
%<multicurve points= "(10,0);(10,0);(10,-7.5);(10,-7.5)"
%	 fill-style= "none"
%	 />
%<multicurve points= "(15,5);(15,5);(10,0);(10,0)"
%	 fill-style= "none"
%	 />
%<multicurve points= "(10,10);(10,10);(10,0);(10,0)"
%	 fill-style= "none"
%	 />
%<multicurve points= "(5,5);(5,5);(10,0);(10,0)"
%	 fill-style= "none"
%	 />
%<multicurve points= "(15,10);(15,10);(15,5);(15,5)"
%	 fill-style= "none"
%	 />
%<multicurve points= "(5,10);(5,10);(5,5);(5,5)"
%	 fill-style= "none"
%	 />
%</jpic>
%%End JPIC-XML
%PSTricks content-type (pstricks.sty package needed)
%Add \usepackage{pstricks} in the preamble of your LaTeX file
%You can rescale the whole picture (to 80% for instance) by using the command \def\JPicScale{0.8}
\ifx\JPicScale\undefined\def\JPicScale{1}\fi
\psset{unit=\JPicScale mm}
\psset{linewidth=0.3,dotsep=1,hatchwidth=0.3,hatchsep=1.5,shadowsize=1,dimen=middle}
\psset{dotsize=0.7 2.5,dotscale=1 1,fillcolor=black}
\psset{arrowsize=1 2,arrowlength=1,arrowinset=0.25,tbarsize=0.7 5,bracketlength=0.15,rbracketlength=0.15}
\begin{pspicture}(0,0)(15,10)
\rput{0}(10,0){\psellipse[fillstyle=solid](0,0)(1.56,-1.57)}
\psline(10,0)(10,-7.5)
\psline(15,5)(10,0)
\psline(10,10)(10,0)
\psline(5,5)(10,0)
\psline(15,10)(15,5)
\psline(5,10)(5,5)
\end{pspicture}


==> PIC/cmn-right.tex <==
%%Created by jPicEdt 1.4.1_03: mixed JPIC-XML/LaTeX format
%%Tue Nov 05 13:13:30 GMT-10:00 2019
%%Begin JPIC-XML
%<?xml version="1.0" standalone="yes"?>
%<jpic x-min="-0.63" x-max="15.63" y-min="-10.62" y-max="8.12" auto-bounding="true">
%<ellipse fill-style= "solid"
%	 p3= "(9.06,2.19)"
%	 p2= "(9.06,-0.94)"
%	 p1= "(12.19,-0.94)"
%	 closure= "open"
%	 angle-end= "0"
%	 angle-start= "0"
%	 />
%<multicurve fill-style= "none"
%	 points= "(15.62,8.12);(15.62,8.12);(15.62,7.5);(15.62,7.5);(15.62,7.5);(15.63,5.62);
%	(15.63,5.62);(15.63,5.62);(11.88,1.87);(11.88,1.87)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(5.62,8.12);(5.62,8.12);(5.62,7.5);(5.62,7.5);(5.62,7.5);(5.63,5.62);
%	(5.63,5.62);(5.63,5.62);(9.38,1.87);(9.38,1.87)"
%	 />
%<ellipse fill-style= "solid"
%	 p3= "(2.81,-4.06)"
%	 p2= "(2.81,-7.19)"
%	 p1= "(5.94,-7.19)"
%	 closure= "open"
%	 angle-end= "0"
%	 angle-start= "0"
%	 />
%<multicurve fill-style= "none"
%	 points= "(-0.63,7.5);(-0.63,7.5);(-0.62,1.25);(-0.62,1.25);(-0.62,1.25);(-0.62,-0.63);
%	(-0.62,-0.63);(-0.62,-0.63);(3.13,-4.38);(3.13,-4.38)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(9.38,-0.62);(9.38,-0.62);(4.38,-5.62);(4.38,-5.62);(4.38,-5.62);(4.38,-5.62);
%	(4.38,-5.62);(4.38,-5.62);(4.38,-5.62);(4.38,-5.62)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(4.38,-6.88);(4.38,-6.88);(4.38,-10);(4.38,-10);(4.38,-10);(4.38,-10.62);
%	(4.38,-10.62);(4.38,-10.62);(4.38,-10);(4.38,-10)"
%	 />
%</jpic>
%%End JPIC-XML
%PSTricks content-type (pstricks.sty package needed)
%Add \usepackage{pstricks} in the preamble of your LaTeX file
%You can rescale the whole picture (to 80% for instance) by using the command \def\JPicScale{0.8}
\ifx\JPicScale\undefined\def\JPicScale{1}\fi
\psset{unit=\JPicScale mm}
\psset{linewidth=0.3,dotsep=1,hatchwidth=0.3,hatchsep=1.5,shadowsize=1,dimen=middle}
\psset{dotsize=0.7 2.5,dotscale=1 1,fillcolor=black}
\psset{arrowsize=1 2,arrowlength=1,arrowinset=0.25,tbarsize=0.7 5,bracketlength=0.15,rbracketlength=0.15}
\begin{pspicture}(0,0)(15.63,8.12)
\rput{0}(10.62,0.62){\psellipse[fillstyle=solid](0,0)(1.57,-1.56)}
\psline(15.62,8.12)
(15.62,7.5)
(15.63,5.62)(11.88,1.87)
\psline(5.62,8.12)
(5.62,7.5)
(5.63,5.62)(9.38,1.87)
\rput{0}(4.38,-5.62){\psellipse[fillstyle=solid](0,0)(1.57,-1.57)}
\psline(-0.63,7.5)
(-0.62,1.25)
(-0.62,-0.63)(3.13,-4.38)
\pscustom[]{\psline(9.38,-0.62)(4.38,-5.62)
\psbezier(4.38,-5.62)(4.38,-5.62)(4.38,-5.62)
\psbezier(4.38,-5.62)(4.38,-5.62)(4.38,-5.62)
}
\psline(4.38,-6.88)
(4.38,-10)
(4.38,-10.62)(4.38,-10)
\end{pspicture}


==> PIC/cmn-sym.tex <==
%%Created by jPicEdt 1.4.1_03: mixed JPIC-XML/LaTeX format
%%Sat Sep 02 18:07:01 HST 2017
%%Begin JPIC-XML
%<?xml version="1.0" standalone="yes"?>
%<jpic x-min="0" x-max="5" y-min="-7.5" y-max="10" auto-bounding="true">
%<ellipse p3= "(0.93,-0.94)"
%	 p2= "(0.93,-4.06)"
%	 p1= "(4.06,-4.06)"
%	 closure= "open"
%	 angle-end= "0"
%	 fill-style= "solid"
%	 angle-start= "0"
%	 />
%<multicurve points= "(2.5,-2.5);(2.5,-2.5);(2.5,-7.5);(2.5,-7.5)"
%	 fill-style= "none"
%	 />
%<multicurve points= "(5,0);(5,0);(2.5,-2.5);(2.5,-2.5)"
%	 fill-style= "none"
%	 />
%<multicurve points= "(0,0);(0,0);(2.5,-2.5);(2.5,-2.5)"
%	 fill-style= "none"
%	 />
%<multicurve points= "(5,2.5);(5,2.5);(5,0);(5,0)"
%	 fill-style= "none"
%	 />
%<multicurve points= "(0,2.5);(0,2.5);(0,0);(0,0)"
%	 fill-style= "none"
%	 />
%<multicurve points= "(0,7.5);(0,7.5);(5,2.5);(5,2.5)"
%	 fill-style= "none"
%	 />
%<multicurve points= "(0,2.5);(0,2.5);(5,7.5);(5,7.5)"
%	 fill-style= "none"
%	 />
%<multicurve points= "(5,10);(5,10);(5,7.5);(5,7.5)"
%	 fill-style= "none"
%	 />
%<multicurve points= "(0,10);(0,10);(0,7.5);(0,7.5)"
%	 fill-style= "none"
%	 />
%</jpic>
%%End JPIC-XML
%PSTricks content-type (pstricks.sty package needed)
%Add \usepackage{pstricks} in the preamble of your LaTeX file
%You can rescale the whole picture (to 80% for instance) by using the command \def\JPicScale{0.8}
\ifx\JPicScale\undefined\def\JPicScale{1}\fi
\psset{unit=\JPicScale mm}
\psset{linewidth=0.3,dotsep=1,hatchwidth=0.3,hatchsep=1.5,shadowsize=1,dimen=middle}
\psset{dotsize=0.7 2.5,dotscale=1 1,fillcolor=black}
\psset{arrowsize=1 2,arrowlength=1,arrowinset=0.25,tbarsize=0.7 5,bracketlength=0.15,rbracketlength=0.15}
\begin{pspicture}(0,0)(5,10)
\rput{0}(2.5,-2.5){\psellipse[fillstyle=solid](0,0)(1.56,-1.57)}
\psline(2.5,-2.5)(2.5,-7.5)
\psline(5,0)(2.5,-2.5)
\psline(0,0)(2.5,-2.5)
\psline(5,2.5)(5,0)
\psline(0,2.5)(0,0)
\psline(0,7.5)(5,2.5)
\psline(0,2.5)(5,7.5)
\psline(5,10)(5,7.5)
\psline(0,10)(0,7.5)
\end{pspicture}


==> PIC/cmn-tupling-1.tex <==
%%Created by jPicEdt 1.4.1_03: mixed JPIC-XML/LaTeX format
%%Mon Aug 31 15:54:20 GMT-10:00 2020
%%Begin JPIC-XML
%<?xml version="1.0" standalone="yes"?>
%<jpic x-min="0" x-max="63.13" y-min="0.62" y-max="21.25" auto-bounding="true">
%<ellipse p3= "(3.43,10.31)"
%	 fill-style= "solid"
%	 p2= "(3.43,7.19)"
%	 p1= "(6.56,7.19)"
%	 closure= "open"
%	 angle-end= "0"
%	 angle-start= "0"
%	 />
%<multicurve fill-style= "none"
%	 points= "(5,8.75);(5,8.75);(5,2.5);(5,2.5)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(10,13.75);(10,13.75);(5,8.75);(5,8.75)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(5,20);(5,20);(5,8.75);(5,8.75)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(0,13.75);(0,13.75);(5,8.75);(5,8.75)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(10,20);(10,20);(10,13.75);(10,13.75)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(0,20);(0,20);(0,13.75);(0,13.75)"
%	 />
%<ellipse p3= "(56.56,14.69)"
%	 fill-style= "solid"
%	 p2= "(56.56,11.56)"
%	 p1= "(59.69,11.56)"
%	 closure= "open"
%	 angle-end= "0"
%	 angle-start= "0"
%	 />
%<multicurve fill-style= "none"
%	 points= "(63.12,20.62);(63.12,20.62);(63.12,20);(63.12,20);(63.12,20);(63.13,18.12);
%	(63.13,18.12);(63.13,18.12);(59.38,14.37);(59.38,14.37)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(53.12,20.62);(53.12,20.62);(53.12,20);(53.12,20);(53.12,20);(53.13,18.12);
%	(53.13,18.12);(53.13,18.12);(56.88,14.37);(56.88,14.37)"
%	 />
%<ellipse p3= "(50.31,8.44)"
%	 fill-style= "solid"
%	 p2= "(50.31,5.31)"
%	 p1= "(53.44,5.31)"
%	 closure= "open"
%	 angle-end= "0"
%	 angle-start= "0"
%	 />
%<multicurve fill-style= "none"
%	 points= "(46.87,20);(46.87,20);(46.88,13.75);(46.88,13.75);(46.88,13.75);(46.88,11.87);
%	(46.88,11.87);(46.88,11.87);(50.63,8.12);(50.63,8.12)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(56.88,11.88);(56.88,11.88);(51.88,6.88);(51.88,6.88);(51.88,6.88);(51.88,6.88);
%	(51.88,6.88);(51.88,6.88);(51.88,6.88);(51.88,6.88)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(51.88,5.62);(51.88,5.62);(51.88,2.5);(51.88,2.5);(51.88,2.5);(51.88,1.88);
%	(51.88,1.88);(51.88,1.88);(51.88,2.5);(51.88,2.5)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(26.87,11.88);(26.87,11.88);(31.87,6.88);(31.87,6.88);(31.87,6.88);(30.63,6.88);
%	(30.63,6.88);(30.63,6.88);(31.25,6.88);(31.25,6.88)"
%	 />
%<ellipse p3= "(24.06,14.69)"
%	 fill-style= "solid"
%	 p2= "(24.06,11.56)"
%	 p1= "(27.19,11.56)"
%	 closure= "open"
%	 angle-end= "0"
%	 angle-start= "0"
%	 />
%<ellipse p3= "(30,8.75)"
%	 fill-style= "solid"
%	 p2= "(30,5.62)"
%	 p1= "(33.13,5.62)"
%	 closure= "open"
%	 angle-end= "0"
%	 angle-start= "0"
%	 />
%<multicurve fill-style= "none"
%	 points= "(36.25,20);(36.25,20);(36.25,17.5);(36.25,17.5);(36.25,17.5);(36.25,11.87);
%	(36.25,11.87);(36.25,11.87);(32.5,8.12);(32.5,8.12)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(30.62,20);(30.62,20);(30.62,19.37);(30.62,19.37);(30.62,19.37);(30.63,17.5);
%	(30.63,17.5);(30.63,17.5);(26.88,13.75);(26.88,13.75)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(20.62,20);(20.62,20);(20.62,19.37);(20.62,19.37);(20.62,19.37);(20.63,17.5);
%	(20.63,17.5);(20.63,17.5);(24.38,13.75);(24.38,13.75)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(31.25,5.62);(31.25,5.62);(31.25,2.5);(31.25,2.5);(31.25,2.5);(31.25,1.88);
%	(31.25,1.88);(31.25,1.88);(31.25,2.5);(31.25,2.5)"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(15,12.5)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\EQLS
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(41.25,12.5)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\EQLS
%</text>
%<text text-vert-align= "bottom"
%	 fill-style= "none"
%	 anchor-point= "(5,21.25)"
%	 text-frame= "noframe"
%	 stroke-width= "0.75"
%	 text-hor-align= "center-h"
%	 >
%$\eex$
%</text>
%<text text-vert-align= "bottom"
%	 fill-style= "none"
%	 anchor-point= "(10,21.25)"
%	 text-frame= "noframe"
%	 stroke-width= "0.75"
%	 text-hor-align= "center-h"
%	 >
%$\eex$
%</text>
%<text text-vert-align= "bottom"
%	 fill-style= "none"
%	 anchor-point= "(0,21.25)"
%	 text-frame= "noframe"
%	 stroke-width= "0.75"
%	 text-hor-align= "center-h"
%	 >
%$\eex$
%</text>
%<text text-vert-align= "bottom"
%	 fill-style= "none"
%	 anchor-point= "(20.62,21.25)"
%	 text-frame= "noframe"
%	 stroke-width= "0.75"
%	 text-hor-align= "center-h"
%	 >
%$\eex$
%</text>
%<text text-vert-align= "bottom"
%	 fill-style= "none"
%	 anchor-point= "(30.62,21.25)"
%	 text-frame= "noframe"
%	 stroke-width= "0.75"
%	 text-hor-align= "center-h"
%	 >
%$\eex$
%</text>
%<text text-vert-align= "bottom"
%	 fill-style= "none"
%	 anchor-point= "(36.25,21.25)"
%	 text-frame= "noframe"
%	 stroke-width= "0.75"
%	 text-hor-align= "center-h"
%	 >
%$\eex$
%</text>
%<text text-vert-align= "bottom"
%	 fill-style= "none"
%	 anchor-point= "(46.88,21.25)"
%	 text-frame= "noframe"
%	 stroke-width= "0.75"
%	 text-hor-align= "center-h"
%	 >
%$\eex$
%</text>
%<text text-vert-align= "bottom"
%	 fill-style= "none"
%	 anchor-point= "(53.12,21.25)"
%	 text-frame= "noframe"
%	 stroke-width= "0.75"
%	 text-hor-align= "center-h"
%	 >
%$\eex$
%</text>
%<text text-vert-align= "bottom"
%	 fill-style= "none"
%	 anchor-point= "(63.12,21.25)"
%	 text-frame= "noframe"
%	 stroke-width= "0.75"
%	 text-hor-align= "center-h"
%	 >
%$\eex$
%</text>
%<text text-vert-align= "top"
%	 fill-style= "none"
%	 anchor-point= "(51.88,0.62)"
%	 text-frame= "noframe"
%	 stroke-width= "0.75"
%	 text-hor-align= "center-h"
%	 >
%$\eex$
%</text>
%<text text-vert-align= "top"
%	 fill-style= "none"
%	 anchor-point= "(31.25,0.62)"
%	 text-frame= "noframe"
%	 stroke-width= "0.75"
%	 text-hor-align= "center-h"
%	 >
%$\eex$
%</text>
%<text text-vert-align= "top"
%	 fill-style= "none"
%	 anchor-point= "(5,0.62)"
%	 text-frame= "noframe"
%	 stroke-width= "0.75"
%	 text-hor-align= "center-h"
%	 >
%$\eex$
%</text>
%</jpic>
%%End JPIC-XML
%PSTricks content-type (pstricks.sty package needed)
%Add \usepackage{pstricks} in the preamble of your LaTeX file
%You can rescale the whole picture (to 80% for instance) by using the command \def\JPicScale{0.8}
\ifx\JPicScale\undefined\def\JPicScale{1}\fi
\psset{unit=\JPicScale mm}
\psset{linewidth=0.3,dotsep=1,hatchwidth=0.3,hatchsep=1.5,shadowsize=1,dimen=middle}
\psset{dotsize=0.7 2.5,dotscale=1 1,fillcolor=black}
\psset{arrowsize=1 2,arrowlength=1,arrowinset=0.25,tbarsize=0.7 5,bracketlength=0.15,rbracketlength=0.15}
\begin{pspicture}(0,0)(63.13,21.25)
\rput{0}(5,8.75){\psellipse[fillstyle=solid](0,0)(1.56,-1.56)}
\psline(5,8.75)(5,2.5)
\psline(10,13.75)(5,8.75)
\psline(5,20)(5,8.75)
\psline(0,13.75)(5,8.75)
\psline(10,20)(10,13.75)
\psline(0,20)(0,13.75)
\rput{0}(58.12,13.12){\psellipse[fillstyle=solid](0,0)(1.56,-1.56)}
\psline(63.12,20.62)
(63.12,20)
(63.13,18.12)(59.38,14.37)
\psline(53.12,20.62)
(53.12,20)
(53.13,18.12)(56.88,14.37)
\rput{90}(51.88,6.88){\psellipse[fillstyle=solid](0,0)(1.57,-1.56)}
\psline(46.87,20)
(46.88,13.75)
(46.88,11.87)(50.63,8.12)
\pscustom[]{\psline(56.88,11.88)(51.88,6.88)
\psbezier(51.88,6.88)(51.88,6.88)(51.88,6.88)
\psbezier(51.88,6.88)(51.88,6.88)(51.88,6.88)
}
\psline(51.88,5.62)
(51.88,2.5)
(51.88,1.88)(51.88,2.5)
\psline(26.87,11.88)
(31.87,6.88)
(30.63,6.88)(31.25,6.88)
\rput{0}(25.62,13.12){\psellipse[fillstyle=solid](0,0)(1.56,-1.57)}
\rput{0}(31.56,7.19){\psellipse[fillstyle=solid](0,0)(1.56,-1.57)}
\psline(36.25,20)
(36.25,17.5)
(36.25,11.87)(32.5,8.12)
\psline(30.62,20)
(30.62,19.37)
(30.63,17.5)(26.88,13.75)
\psline(20.62,20)
(20.62,19.37)
(20.63,17.5)(24.38,13.75)
\psline(31.25,5.62)
(31.25,2.5)
(31.25,1.88)(31.25,2.5)
\rput(15,12.5){\EQLS}
\rput(41.25,12.5){\EQLS}
\rput[b](5,21.25){$\eex$}
\rput[b](10,21.25){$\eex$}
\rput[b](0,21.25){$\eex$}
\rput[b](20.62,21.25){$\eex$}
\rput[b](30.62,21.25){$\eex$}
\rput[b](36.25,21.25){$\eex$}
\rput[b](46.88,21.25){$\eex$}
\rput[b](53.12,21.25){$\eex$}
\rput[b](63.12,21.25){$\eex$}
\rput[t](51.88,0.62){$\eex$}
\rput[t](31.25,0.62){$\eex$}
\rput[t](5,0.62){$\eex$}
\end{pspicture}


==> PIC/cmn-tupling-2.tex <==
%%Created by jPicEdt 1.4.1_03: mixed JPIC-XML/LaTeX format
%%Mon Aug 31 15:35:12 GMT-10:00 2020
%%Begin JPIC-XML
%<?xml version="1.0" standalone="yes"?>
%<jpic x-min="2.5" x-max="65.62" y-min="0.62" y-max="20.62" auto-bounding="true">
%<ellipse p3= "(8.43,11.56)"
%	 fill-style= "solid"
%	 p2= "(8.43,8.44)"
%	 p1= "(11.56,8.44)"
%	 closure= "open"
%	 angle-end= "0"
%	 angle-start= "0"
%	 />
%<multicurve fill-style= "none"
%	 points= "(10,10);(10,10);(10,2.5);(10,2.5)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(17.5,15);(17.5,15);(10,10);(10,10)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(7.5,15);(7.5,15);(10,10);(10,10)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(2.5,15);(2.5,15);(10,10);(10,10)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(17.5,20);(17.5,20);(17.5,15);(17.5,15)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(2.5,20);(2.5,20);(2.5,15);(2.5,15)"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(23.75,12.5)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\EQLS
%</text>
%<multicurve fill-style= "none"
%	 points= "(7.5,20);(7.5,20);(7.5,15);(7.5,15)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(12.5,20);(12.5,20);(12.5,15);(12.5,15)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(12.5,15);(12.5,15);(10,10);(10,10)"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(56.25,12.5)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\EQLS
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(65.62,12.5)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\FURTHER
%</text>
%<ellipse p3= "(40,9.38)"
%	 fill-style= "solid"
%	 p2= "(40,6.25)"
%	 p1= "(43.13,6.25)"
%	 closure= "open"
%	 angle-end= "0"
%	 angle-start= "0"
%	 />
%<multicurve fill-style= "none"
%	 points= "(41.25,6.25);(41.25,6.25);(41.25,3.12);(41.25,3.12);(41.25,3.12);(41.25,2.51);
%	(41.25,2.51);(41.25,2.51);(41.25,3.12);(41.25,3.12)"
%	 />
%<ellipse p3= "(45.94,14.69)"
%	 fill-style= "solid"
%	 p2= "(45.94,11.56)"
%	 p1= "(49.06,11.56)"
%	 closure= "open"
%	 angle-end= "0"
%	 angle-start= "0"
%	 />
%<multicurve fill-style= "none"
%	 points= "(50.62,20);(50.62,20);(50.62,18.12);(50.62,18.12);(50.62,18.12);(50.64,16.25);
%	(50.64,16.25);(50.64,16.25);(46.88,12.5);(46.88,12.5)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(44.38,20);(44.38,20);(44.38,18.12);(44.38,18.12);(44.38,18.12);(44.38,16.25);
%	(44.38,16.25);(44.38,16.25);(48.14,12.5);(48.14,12.5)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(41.88,8.12);(41.88,8.12);(47.5,13.12);(47.5,13.12)"
%	 />
%<ellipse p3= "(33.44,14.69)"
%	 fill-style= "solid"
%	 p2= "(33.44,11.56)"
%	 p1= "(36.56,11.56)"
%	 closure= "open"
%	 angle-end= "0"
%	 angle-start= "0"
%	 />
%<multicurve fill-style= "none"
%	 points= "(38.12,20);(38.12,20);(38.12,18.12);(38.12,18.12);(38.12,18.12);(38.14,16.25);
%	(38.14,16.25);(38.14,16.25);(34.38,12.5);(34.38,12.5)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(31.88,20);(31.88,20);(31.88,18.12);(31.88,18.12);(31.88,18.12);(31.88,16.25);
%	(31.88,16.25);(31.88,16.25);(35.63,12.5);(35.63,12.5)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(41.88,7.5);(41.88,7.5);(35,13.12);(35,13.12)"
%	 />
%<text text-vert-align= "top"
%	 fill-style= "none"
%	 anchor-point= "(10,0.62)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\why$
%</text>
%<text text-vert-align= "top"
%	 fill-style= "none"
%	 anchor-point= "(41.25,0.62)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\why$
%</text>
%<text text-vert-align= "bottom"
%	 fill-style= "none"
%	 anchor-point= "(50.62,20.62)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\why$
%</text>
%<text text-vert-align= "bottom"
%	 fill-style= "none"
%	 anchor-point= "(45,20.62)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\why$
%</text>
%<text text-vert-align= "bottom"
%	 fill-style= "none"
%	 anchor-point= "(38.12,20.62)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\why$
%</text>
%<text text-vert-align= "bottom"
%	 fill-style= "none"
%	 anchor-point= "(31.88,20.62)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\why$
%</text>
%<text text-vert-align= "bottom"
%	 fill-style= "none"
%	 anchor-point= "(17.5,20.62)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\why$
%</text>
%<text text-vert-align= "bottom"
%	 fill-style= "none"
%	 anchor-point= "(12.5,20.62)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\why$
%</text>
%<text text-vert-align= "bottom"
%	 fill-style= "none"
%	 anchor-point= "(7.5,20.62)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\why$
%</text>
%<text text-vert-align= "bottom"
%	 fill-style= "none"
%	 anchor-point= "(2.5,20.62)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\why$
%</text>
%</jpic>
%%End JPIC-XML
%PSTricks content-type (pstricks.sty package needed)
%Add \usepackage{pstricks} in the preamble of your LaTeX file
%You can rescale the whole picture (to 80% for instance) by using the command \def\JPicScale{0.8}
\ifx\JPicScale\undefined\def\JPicScale{1}\fi
\psset{unit=\JPicScale mm}
\psset{linewidth=0.3,dotsep=1,hatchwidth=0.3,hatchsep=1.5,shadowsize=1,dimen=middle}
\psset{dotsize=0.7 2.5,dotscale=1 1,fillcolor=black}
\psset{arrowsize=1 2,arrowlength=1,arrowinset=0.25,tbarsize=0.7 5,bracketlength=0.15,rbracketlength=0.15}
\begin{pspicture}(0,0)(65.62,20.62)
\rput{0}(10,10){\psellipse[fillstyle=solid](0,0)(1.57,-1.56)}
\psline(10,10)(10,2.5)
\psline(17.5,15)(10,10)
\psline(7.5,15)(10,10)
\psline(2.5,15)(10,10)
\psline(17.5,20)(17.5,15)
\psline(2.5,20)(2.5,15)
\rput(23.75,12.5){\EQLS}
\psline(7.5,20)(7.5,15)
\psline(12.5,20)(12.5,15)
\psline(12.5,15)(10,10)
\rput(56.25,12.5){\EQLS}
\rput(65.62,12.5){\FURTHER}
\rput{0}(41.56,7.82){\psellipse[fillstyle=solid](0,0)(1.57,-1.56)}
\psline(41.25,6.25)
(41.25,3.12)
(41.25,2.51)(41.25,3.12)
\rput{90}(47.5,13.12){\psellipse[fillstyle=solid](0,0)(1.57,-1.56)}
\psline(50.62,20)
(50.62,18.12)
(50.64,16.25)(46.88,12.5)
\psline(44.38,20)
(44.38,18.12)
(44.38,16.25)(48.14,12.5)
\psline(41.88,8.12)(47.5,13.12)
\rput{90}(35,13.12){\psellipse[fillstyle=solid](0,0)(1.57,-1.56)}
\psline(38.12,20)
(38.12,18.12)
(38.14,16.25)(34.38,12.5)
\psline(31.88,20)
(31.88,18.12)
(31.88,16.25)(35.63,12.5)
\psline(41.88,7.5)(35,13.12)
\rput[t](10,0.62){$\why$}
\rput[t](41.25,0.62){$\why$}
\rput[b](50.62,20.62){$\why$}
\rput[b](45,20.62){$\why$}
\rput[b](38.12,20.62){$\why$}
\rput[b](31.88,20.62){$\why$}
\rput[b](17.5,20.62){$\why$}
\rput[b](12.5,20.62){$\why$}
\rput[b](7.5,20.62){$\why$}
\rput[b](2.5,20.62){$\why$}
\end{pspicture}


==> PIC/cmn-tupling-3.tex <==
%%Created by jPicEdt 1.4.1_03: mixed JPIC-XML/LaTeX format
%%Sat May 15 13:00:56 GMT-10:00 2021
%%Begin JPIC-XML
%<?xml version="1.0" standalone="yes"?>
%<jpic x-min="0" x-max="155.62" y-min="0.62" y-max="21.25" auto-bounding="true">
%<ellipse p3= "(3.43,10.31)"
%	 p2= "(3.43,7.19)"
%	 fill-style= "solid"
%	 p1= "(6.56,7.19)"
%	 stroke-width= "0.55"
%	 closure= "open"
%	 angle-end= "0"
%	 angle-start= "0"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.55"
%	 points= "(5,8.75);(5,8.75);(5,2.5);(5,2.5)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.55"
%	 points= "(10,13.75);(10,13.75);(5,8.75);(5,8.75)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.55"
%	 points= "(5,20);(5,20);(5,8.75);(5,8.75)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.55"
%	 points= "(0,13.75);(0,13.75);(5,8.75);(5,8.75)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.55"
%	 points= "(10,20);(10,20);(10,13.75);(10,13.75)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.55"
%	 points= "(0,20);(0,20);(0,13.75);(0,13.75)"
%	 />
%<ellipse p3= "(56.56,14.69)"
%	 p2= "(56.56,11.56)"
%	 fill-style= "solid"
%	 p1= "(59.69,11.56)"
%	 stroke-width= "0.55"
%	 closure= "open"
%	 angle-end= "0"
%	 angle-start= "0"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.55"
%	 points= "(63.12,20.62);(63.12,20.62);(63.12,20);(63.12,20);(63.12,20);(63.13,18.12);
%	(63.13,18.12);(63.13,18.12);(59.38,14.37);(59.38,14.37)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.55"
%	 points= "(53.12,20.62);(53.12,20.62);(53.12,20);(53.12,20);(53.12,20);(53.13,18.12);
%	(53.13,18.12);(53.13,18.12);(56.88,14.37);(56.88,14.37)"
%	 />
%<ellipse p3= "(50.31,8.44)"
%	 p2= "(50.31,5.31)"
%	 fill-style= "solid"
%	 p1= "(53.44,5.31)"
%	 stroke-width= "0.55"
%	 closure= "open"
%	 angle-end= "0"
%	 angle-start= "0"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.55"
%	 points= "(46.87,20);(46.87,20);(46.88,13.75);(46.88,13.75);(46.88,13.75);(46.88,11.87);
%	(46.88,11.87);(46.88,11.87);(50.63,8.12);(50.63,8.12)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.55"
%	 points= "(56.88,11.88);(56.88,11.88);(51.88,6.88);(51.88,6.88);(51.88,6.88);(51.88,6.88);
%	(51.88,6.88);(51.88,6.88);(51.88,6.88);(51.88,6.88)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.55"
%	 points= "(51.88,5.62);(51.88,5.62);(51.88,2.5);(51.88,2.5);(51.88,2.5);(51.88,1.88);
%	(51.88,1.88);(51.88,1.88);(51.88,2.5);(51.88,2.5)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.55"
%	 points= "(26.87,11.88);(26.87,11.88);(31.87,6.88);(31.87,6.88);(31.87,6.88);(30.63,6.88);
%	(30.63,6.88);(30.63,6.88);(31.25,6.88);(31.25,6.88)"
%	 />
%<ellipse p3= "(24.06,14.69)"
%	 p2= "(24.06,11.56)"
%	 fill-style= "solid"
%	 p1= "(27.19,11.56)"
%	 stroke-width= "0.55"
%	 closure= "open"
%	 angle-end= "0"
%	 angle-start= "0"
%	 />
%<ellipse p3= "(30,8.75)"
%	 p2= "(30,5.62)"
%	 fill-style= "solid"
%	 p1= "(33.13,5.62)"
%	 stroke-width= "0.55"
%	 closure= "open"
%	 angle-end= "0"
%	 angle-start= "0"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.55"
%	 points= "(36.25,20);(36.25,20);(36.25,17.5);(36.25,17.5);(36.25,17.5);(36.25,11.87);
%	(36.25,11.87);(36.25,11.87);(32.5,8.12);(32.5,8.12)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.55"
%	 points= "(30.62,20);(30.62,20);(30.62,19.37);(30.62,19.37);(30.62,19.37);(30.63,17.5);
%	(30.63,17.5);(30.63,17.5);(26.88,13.75);(26.88,13.75)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.55"
%	 points= "(20.62,20);(20.62,20);(20.62,19.37);(20.62,19.37);(20.62,19.37);(20.63,17.5);
%	(20.63,17.5);(20.63,17.5);(24.38,13.75);(24.38,13.75)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.55"
%	 points= "(31.25,5.62);(31.25,5.62);(31.25,2.5);(31.25,2.5);(31.25,2.5);(31.25,1.88);
%	(31.25,1.88);(31.25,1.88);(31.25,2.5);(31.25,2.5)"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 stroke-width= "0.55"
%	 anchor-point= "(15,12.5)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\EQLS
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 stroke-width= "0.55"
%	 anchor-point= "(41.25,12.5)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\EQLS
%</text>
%<ellipse p3= "(98.43,11.56)"
%	 p2= "(98.43,8.44)"
%	 fill-style= "solid"
%	 p1= "(101.56,8.44)"
%	 stroke-width= "0.55"
%	 closure= "open"
%	 angle-end= "0"
%	 angle-start= "0"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.55"
%	 points= "(100,10);(100,10);(100,2.5);(100,2.5)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.55"
%	 points= "(107.5,15);(107.5,15);(100,10);(100,10)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.55"
%	 points= "(97.5,15);(97.5,15);(100,10);(100,10)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.55"
%	 points= "(92.5,15);(92.5,15);(100,10);(100,10)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.55"
%	 points= "(107.5,20);(107.5,20);(107.5,15);(107.5,15)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.55"
%	 points= "(92.5,20);(92.5,20);(92.5,15);(92.5,15)"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 stroke-width= "0.55"
%	 anchor-point= "(113.75,12.5)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\EQLS
%</text>
%<multicurve fill-style= "none"
%	 stroke-width= "0.55"
%	 points= "(97.5,20);(97.5,20);(97.5,15);(97.5,15)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.55"
%	 points= "(102.5,20);(102.5,20);(102.5,15);(102.5,15)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.55"
%	 points= "(102.5,15);(102.5,15);(100,10);(100,10)"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 stroke-width= "0.55"
%	 anchor-point= "(146.25,12.5)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\EQLS
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 stroke-width= "0.55"
%	 anchor-point= "(155.62,12.5)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\FURTHER
%</text>
%<ellipse p3= "(130,9.38)"
%	 p2= "(130,6.25)"
%	 fill-style= "solid"
%	 p1= "(133.13,6.25)"
%	 stroke-width= "0.55"
%	 closure= "open"
%	 angle-end= "0"
%	 angle-start= "0"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.55"
%	 points= "(131.25,6.25);(131.25,6.25);(131.25,3.12);(131.25,3.12);(131.25,3.12);(131.25,2.51);
%	(131.25,2.51);(131.25,2.51);(131.25,3.12);(131.25,3.12)"
%	 />
%<ellipse p3= "(135.94,14.69)"
%	 p2= "(135.94,11.56)"
%	 fill-style= "solid"
%	 p1= "(139.06,11.56)"
%	 stroke-width= "0.55"
%	 closure= "open"
%	 angle-end= "0"
%	 angle-start= "0"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.55"
%	 points= "(140.62,20);(140.62,20);(140.62,18.12);(140.62,18.12);(140.62,18.12);(140.64,16.25);
%	(140.64,16.25);(140.64,16.25);(136.88,12.5);(136.88,12.5)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.55"
%	 points= "(134.38,20);(134.38,20);(134.38,18.12);(134.38,18.12);(134.38,18.12);(134.38,16.25);
%	(134.38,16.25);(134.38,16.25);(138.14,12.5);(138.14,12.5)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.55"
%	 points= "(131.88,8.12);(131.88,8.12);(137.5,13.12);(137.5,13.12)"
%	 />
%<ellipse p3= "(123.44,14.69)"
%	 p2= "(123.44,11.56)"
%	 fill-style= "solid"
%	 p1= "(126.56,11.56)"
%	 stroke-width= "0.55"
%	 closure= "open"
%	 angle-end= "0"
%	 angle-start= "0"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.55"
%	 points= "(128.12,20);(128.12,20);(128.12,18.12);(128.12,18.12);(128.12,18.12);(128.14,16.25);
%	(128.14,16.25);(128.14,16.25);(124.38,12.5);(124.38,12.5)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.55"
%	 points= "(121.88,20);(121.88,20);(121.88,18.12);(121.88,18.12);(121.88,18.12);(121.88,16.25);
%	(121.88,16.25);(121.88,16.25);(125.63,12.5);(125.63,12.5)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.55"
%	 points= "(131.88,7.5);(131.88,7.5);(125,13.12);(125,13.12)"
%	 />
%<text text-vert-align= "bottom"
%	 fill-style= "none"
%	 stroke-width= "0.55"
%	 anchor-point= "(5,21.25)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\eex$
%</text>
%<text text-vert-align= "bottom"
%	 fill-style= "none"
%	 stroke-width= "0.55"
%	 anchor-point= "(10,21.25)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\eex$
%</text>
%<text text-vert-align= "bottom"
%	 fill-style= "none"
%	 stroke-width= "0.55"
%	 anchor-point= "(0,21.25)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\eex$
%</text>
%<text text-vert-align= "bottom"
%	 fill-style= "none"
%	 stroke-width= "0.55"
%	 anchor-point= "(20.62,21.25)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\eex$
%</text>
%<text text-vert-align= "bottom"
%	 fill-style= "none"
%	 stroke-width= "0.55"
%	 anchor-point= "(30.62,21.25)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\eex$
%</text>
%<text text-vert-align= "bottom"
%	 fill-style= "none"
%	 stroke-width= "0.55"
%	 anchor-point= "(36.25,21.25)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\eex$
%</text>
%<text text-vert-align= "bottom"
%	 fill-style= "none"
%	 stroke-width= "0.55"
%	 anchor-point= "(46.88,21.25)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\eex$
%</text>
%<text text-vert-align= "bottom"
%	 fill-style= "none"
%	 stroke-width= "0.55"
%	 anchor-point= "(53.12,21.25)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\eex$
%</text>
%<text text-vert-align= "bottom"
%	 fill-style= "none"
%	 stroke-width= "0.55"
%	 anchor-point= "(63.12,21.25)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\eex$
%</text>
%<text text-vert-align= "top"
%	 fill-style= "none"
%	 stroke-width= "0.55"
%	 anchor-point= "(51.88,0.62)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\eex$
%</text>
%<text text-vert-align= "top"
%	 fill-style= "none"
%	 stroke-width= "0.55"
%	 anchor-point= "(31.25,0.62)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\eex$
%</text>
%<text text-vert-align= "top"
%	 fill-style= "none"
%	 stroke-width= "0.55"
%	 anchor-point= "(5,0.62)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\eex$
%</text>
%<text text-vert-align= "top"
%	 fill-style= "none"
%	 stroke-width= "0.55"
%	 anchor-point= "(100,0.62)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\why$
%</text>
%<text text-vert-align= "top"
%	 fill-style= "none"
%	 stroke-width= "0.55"
%	 anchor-point= "(131.25,0.62)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\why$
%</text>
%<text text-vert-align= "bottom"
%	 fill-style= "none"
%	 stroke-width= "0.55"
%	 anchor-point= "(140.62,20.62)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\why$
%</text>
%<text text-vert-align= "bottom"
%	 fill-style= "none"
%	 stroke-width= "0.55"
%	 anchor-point= "(135,20.62)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\why$
%</text>
%<text text-vert-align= "bottom"
%	 fill-style= "none"
%	 stroke-width= "0.55"
%	 anchor-point= "(128.12,20.62)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\why$
%</text>
%<text text-vert-align= "bottom"
%	 fill-style= "none"
%	 stroke-width= "0.55"
%	 anchor-point= "(121.88,20.62)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\why$
%</text>
%<text text-vert-align= "bottom"
%	 fill-style= "none"
%	 stroke-width= "0.55"
%	 anchor-point= "(107.5,20.62)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\why$
%</text>
%<text text-vert-align= "bottom"
%	 fill-style= "none"
%	 stroke-width= "0.55"
%	 anchor-point= "(102.5,20.62)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\why$
%</text>
%<text text-vert-align= "bottom"
%	 fill-style= "none"
%	 stroke-width= "0.55"
%	 anchor-point= "(97.5,20.62)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\why$
%</text>
%<text text-vert-align= "bottom"
%	 fill-style= "none"
%	 stroke-width= "0.55"
%	 anchor-point= "(92.5,20.62)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\why$
%</text>
%</jpic>
%%End JPIC-XML
%PSTricks content-type (pstricks.sty package needed)
%Add \usepackage{pstricks} in the preamble of your LaTeX file
%You can rescale the whole picture (to 80% for instance) by using the command \def\JPicScale{0.8}
\ifx\JPicScale\undefined\def\JPicScale{1}\fi
\psset{unit=\JPicScale mm}
\psset{linewidth=0.3,dotsep=1,hatchwidth=0.3,hatchsep=1.5,shadowsize=1,dimen=middle}
\psset{dotsize=0.7 2.5,dotscale=1 1,fillcolor=black}
\psset{arrowsize=1 2,arrowlength=1,arrowinset=0.25,tbarsize=0.7 5,bracketlength=0.15,rbracketlength=0.15}
\begin{pspicture}(0,0)(155.62,21.25)
\rput{0}(5,8.75){\psellipse[linewidth=0.55,fillstyle=solid](0,0)(1.56,-1.56)}
\psline[linewidth=0.55](5,8.75)(5,2.5)
\psline[linewidth=0.55](10,13.75)(5,8.75)
\psline[linewidth=0.55](5,20)(5,8.75)
\psline[linewidth=0.55](0,13.75)(5,8.75)
\psline[linewidth=0.55](10,20)(10,13.75)
\psline[linewidth=0.55](0,20)(0,13.75)
\rput{0}(58.12,13.12){\psellipse[linewidth=0.55,fillstyle=solid](0,0)(1.56,-1.56)}
\psline[linewidth=0.55](63.12,20.62)
(63.12,20)
(63.13,18.12)(59.38,14.37)
\psline[linewidth=0.55](53.12,20.62)
(53.12,20)
(53.13,18.12)(56.88,14.37)
\rput{90}(51.88,6.88){\psellipse[linewidth=0.55,fillstyle=solid](0,0)(1.57,-1.56)}
\psline[linewidth=0.55](46.87,20)
(46.88,13.75)
(46.88,11.87)(50.63,8.12)
\pscustom[linewidth=0.55]{\psline(56.88,11.88)(51.88,6.88)
\psbezier(51.88,6.88)(51.88,6.88)(51.88,6.88)
\psbezier(51.88,6.88)(51.88,6.88)(51.88,6.88)
}
\psline[linewidth=0.55](51.88,5.62)
(51.88,2.5)
(51.88,1.88)(51.88,2.5)
\psline[linewidth=0.55](26.87,11.88)
(31.87,6.88)
(30.63,6.88)(31.25,6.88)
\rput{0}(25.62,13.12){\psellipse[linewidth=0.55,fillstyle=solid](0,0)(1.56,-1.57)}
\rput{0}(31.56,7.19){\psellipse[linewidth=0.55,fillstyle=solid](0,0)(1.56,-1.57)}
\psline[linewidth=0.55](36.25,20)
(36.25,17.5)
(36.25,11.87)(32.5,8.12)
\psline[linewidth=0.55](30.62,20)
(30.62,19.37)
(30.63,17.5)(26.88,13.75)
\psline[linewidth=0.55](20.62,20)
(20.62,19.37)
(20.63,17.5)(24.38,13.75)
\psline[linewidth=0.55](31.25,5.62)
(31.25,2.5)
(31.25,1.88)(31.25,2.5)
\rput(15,12.5){\EQLS}
\rput(41.25,12.5){\EQLS}
\rput{0}(100,10){\psellipse[linewidth=0.55,fillstyle=solid](0,0)(1.57,-1.56)}
\psline[linewidth=0.55](100,10)(100,2.5)
\psline[linewidth=0.55](107.5,15)(100,10)
\psline[linewidth=0.55](97.5,15)(100,10)
\psline[linewidth=0.55](92.5,15)(100,10)
\psline[linewidth=0.55](107.5,20)(107.5,15)
\psline[linewidth=0.55](92.5,20)(92.5,15)
\rput(113.75,12.5){\EQLS}
\psline[linewidth=0.55](97.5,20)(97.5,15)
\psline[linewidth=0.55](102.5,20)(102.5,15)
\psline[linewidth=0.55](102.5,15)(100,10)
\rput(146.25,12.5){\EQLS}
\rput(155.62,12.5){\FURTHER}
\rput{0}(131.56,7.82){\psellipse[linewidth=0.55,fillstyle=solid](0,0)(1.57,-1.56)}
\psline[linewidth=0.55](131.25,6.25)
(131.25,3.12)
(131.25,2.51)(131.25,3.12)
\rput{90}(137.5,13.12){\psellipse[linewidth=0.55,fillstyle=solid](0,0)(1.57,-1.56)}
\psline[linewidth=0.55](140.62,20)
(140.62,18.12)
(140.64,16.25)(136.88,12.5)
\psline[linewidth=0.55](134.38,20)
(134.38,18.12)
(134.38,16.25)(138.14,12.5)
\psline[linewidth=0.55](131.88,8.12)(137.5,13.12)
\rput{90}(125,13.12){\psellipse[linewidth=0.55,fillstyle=solid](0,0)(1.57,-1.56)}
\psline[linewidth=0.55](128.12,20)
(128.12,18.12)
(128.14,16.25)(124.38,12.5)
\psline[linewidth=0.55](121.88,20)
(121.88,18.12)
(121.88,16.25)(125.63,12.5)
\psline[linewidth=0.55](131.88,7.5)(125,13.12)
\rput[b](5,21.25){$\eex$}
\rput[b](10,21.25){$\eex$}
\rput[b](0,21.25){$\eex$}
\rput[b](20.62,21.25){$\eex$}
\rput[b](30.62,21.25){$\eex$}
\rput[b](36.25,21.25){$\eex$}
\rput[b](46.88,21.25){$\eex$}
\rput[b](53.12,21.25){$\eex$}
\rput[b](63.12,21.25){$\eex$}
\rput[t](51.88,0.62){$\eex$}
\rput[t](31.25,0.62){$\eex$}
\rput[t](5,0.62){$\eex$}
\rput[t](100,0.62){$\why$}
\rput[t](131.25,0.62){$\why$}
\rput[b](140.62,20.62){$\why$}
\rput[b](135,20.62){$\why$}
\rput[b](128.12,20.62){$\why$}
\rput[b](121.88,20.62){$\why$}
\rput[b](107.5,20.62){$\why$}
\rput[b](102.5,20.62){$\why$}
\rput[b](97.5,20.62){$\why$}
\rput[b](92.5,20.62){$\why$}
\end{pspicture}


==> PIC/cmn-tupling.tex <==
%%Created by jPicEdt 1.4.1_03: mixed JPIC-XML/LaTeX format
%%Wed Aug 26 15:00:31 GMT-10:00 2020
%%Begin JPIC-XML
%<?xml version="1.0" standalone="yes"?>
%<jpic x-min="0" x-max="155.62" y-min="0.62" y-max="21.25" auto-bounding="true">
%<ellipse p3= "(3.43,10.31)"
%	 fill-style= "solid"
%	 p2= "(3.43,7.19)"
%	 p1= "(6.56,7.19)"
%	 closure= "open"
%	 angle-end= "0"
%	 angle-start= "0"
%	 />
%<multicurve fill-style= "none"
%	 points= "(5,8.75);(5,8.75);(5,2.5);(5,2.5)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(10,13.75);(10,13.75);(5,8.75);(5,8.75)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(5,20);(5,20);(5,8.75);(5,8.75)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(0,13.75);(0,13.75);(5,8.75);(5,8.75)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(10,20);(10,20);(10,13.75);(10,13.75)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(0,20);(0,20);(0,13.75);(0,13.75)"
%	 />
%<ellipse p3= "(56.56,14.69)"
%	 fill-style= "solid"
%	 p2= "(56.56,11.56)"
%	 p1= "(59.69,11.56)"
%	 closure= "open"
%	 angle-end= "0"
%	 angle-start= "0"
%	 />
%<multicurve fill-style= "none"
%	 points= "(63.12,20.62);(63.12,20.62);(63.12,20);(63.12,20);(63.12,20);(63.13,18.12);
%	(63.13,18.12);(63.13,18.12);(59.38,14.37);(59.38,14.37)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(53.12,20.62);(53.12,20.62);(53.12,20);(53.12,20);(53.12,20);(53.13,18.12);
%	(53.13,18.12);(53.13,18.12);(56.88,14.37);(56.88,14.37)"
%	 />
%<ellipse p3= "(50.31,8.44)"
%	 fill-style= "solid"
%	 p2= "(50.31,5.31)"
%	 p1= "(53.44,5.31)"
%	 closure= "open"
%	 angle-end= "0"
%	 angle-start= "0"
%	 />
%<multicurve fill-style= "none"
%	 points= "(46.87,20);(46.87,20);(46.88,13.75);(46.88,13.75);(46.88,13.75);(46.88,11.87);
%	(46.88,11.87);(46.88,11.87);(50.63,8.12);(50.63,8.12)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(56.88,11.88);(56.88,11.88);(51.88,6.88);(51.88,6.88);(51.88,6.88);(51.88,6.88);
%	(51.88,6.88);(51.88,6.88);(51.88,6.88);(51.88,6.88)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(51.88,5.62);(51.88,5.62);(51.88,2.5);(51.88,2.5);(51.88,2.5);(51.88,1.88);
%	(51.88,1.88);(51.88,1.88);(51.88,2.5);(51.88,2.5)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(26.87,11.88);(26.87,11.88);(31.87,6.88);(31.87,6.88);(31.87,6.88);(30.63,6.88);
%	(30.63,6.88);(30.63,6.88);(31.25,6.88);(31.25,6.88)"
%	 />
%<ellipse p3= "(24.06,14.69)"
%	 fill-style= "solid"
%	 p2= "(24.06,11.56)"
%	 p1= "(27.19,11.56)"
%	 closure= "open"
%	 angle-end= "0"
%	 angle-start= "0"
%	 />
%<ellipse p3= "(30,8.75)"
%	 fill-style= "solid"
%	 p2= "(30,5.62)"
%	 p1= "(33.13,5.62)"
%	 closure= "open"
%	 angle-end= "0"
%	 angle-start= "0"
%	 />
%<multicurve fill-style= "none"
%	 points= "(36.25,20);(36.25,20);(36.25,17.5);(36.25,17.5);(36.25,17.5);(36.25,11.87);
%	(36.25,11.87);(36.25,11.87);(32.5,8.12);(32.5,8.12)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(30.62,20);(30.62,20);(30.62,19.37);(30.62,19.37);(30.62,19.37);(30.63,17.5);
%	(30.63,17.5);(30.63,17.5);(26.88,13.75);(26.88,13.75)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(20.62,20);(20.62,20);(20.62,19.37);(20.62,19.37);(20.62,19.37);(20.63,17.5);
%	(20.63,17.5);(20.63,17.5);(24.38,13.75);(24.38,13.75)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(31.25,5.62);(31.25,5.62);(31.25,2.5);(31.25,2.5);(31.25,2.5);(31.25,1.88);
%	(31.25,1.88);(31.25,1.88);(31.25,2.5);(31.25,2.5)"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(15,12.5)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\EQLS
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(41.25,12.5)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\EQLS
%</text>
%<ellipse p3= "(98.43,11.56)"
%	 fill-style= "solid"
%	 p2= "(98.43,8.44)"
%	 p1= "(101.56,8.44)"
%	 closure= "open"
%	 angle-end= "0"
%	 angle-start= "0"
%	 />
%<multicurve fill-style= "none"
%	 points= "(100,10);(100,10);(100,2.5);(100,2.5)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(107.5,15);(107.5,15);(100,10);(100,10)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(97.5,15);(97.5,15);(100,10);(100,10)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(92.5,15);(92.5,15);(100,10);(100,10)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(107.5,20);(107.5,20);(107.5,15);(107.5,15)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(92.5,20);(92.5,20);(92.5,15);(92.5,15)"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(113.75,12.5)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\EQLS
%</text>
%<multicurve fill-style= "none"
%	 points= "(97.5,20);(97.5,20);(97.5,15);(97.5,15)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(102.5,20);(102.5,20);(102.5,15);(102.5,15)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(102.5,15);(102.5,15);(100,10);(100,10)"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(146.25,12.5)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\EQLS
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(155.62,12.5)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\FURTHER
%</text>
%<ellipse p3= "(130,9.38)"
%	 fill-style= "solid"
%	 p2= "(130,6.25)"
%	 p1= "(133.13,6.25)"
%	 closure= "open"
%	 angle-end= "0"
%	 angle-start= "0"
%	 />
%<multicurve fill-style= "none"
%	 points= "(131.25,6.25);(131.25,6.25);(131.25,3.12);(131.25,3.12);(131.25,3.12);(131.25,2.51);
%	(131.25,2.51);(131.25,2.51);(131.25,3.12);(131.25,3.12)"
%	 />
%<ellipse p3= "(135.94,14.69)"
%	 fill-style= "solid"
%	 p2= "(135.94,11.56)"
%	 p1= "(139.06,11.56)"
%	 closure= "open"
%	 angle-end= "0"
%	 angle-start= "0"
%	 />
%<multicurve fill-style= "none"
%	 points= "(140.62,20);(140.62,20);(140.62,18.12);(140.62,18.12);(140.62,18.12);(140.64,16.25);
%	(140.64,16.25);(140.64,16.25);(136.88,12.5);(136.88,12.5)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(134.38,20);(134.38,20);(134.38,18.12);(134.38,18.12);(134.38,18.12);(134.38,16.25);
%	(134.38,16.25);(134.38,16.25);(138.14,12.5);(138.14,12.5)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(131.88,8.12);(131.88,8.12);(137.5,13.12);(137.5,13.12)"
%	 />
%<ellipse p3= "(123.44,14.69)"
%	 fill-style= "solid"
%	 p2= "(123.44,11.56)"
%	 p1= "(126.56,11.56)"
%	 closure= "open"
%	 angle-end= "0"
%	 angle-start= "0"
%	 />
%<multicurve fill-style= "none"
%	 points= "(128.12,20);(128.12,20);(128.12,18.12);(128.12,18.12);(128.12,18.12);(128.14,16.25);
%	(128.14,16.25);(128.14,16.25);(124.38,12.5);(124.38,12.5)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(121.88,20);(121.88,20);(121.88,18.12);(121.88,18.12);(121.88,18.12);(121.88,16.25);
%	(121.88,16.25);(121.88,16.25);(125.63,12.5);(125.63,12.5)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(131.88,7.5);(131.88,7.5);(125,13.12);(125,13.12)"
%	 />
%<text text-vert-align= "bottom"
%	 fill-style= "none"
%	 anchor-point= "(5,21.25)"
%	 text-frame= "noframe"
%	 stroke-width= "0.75"
%	 text-hor-align= "center-h"
%	 >
%$\eex$
%</text>
%<text text-vert-align= "bottom"
%	 fill-style= "none"
%	 anchor-point= "(10,21.25)"
%	 text-frame= "noframe"
%	 stroke-width= "0.75"
%	 text-hor-align= "center-h"
%	 >
%$\eex$
%</text>
%<text text-vert-align= "bottom"
%	 fill-style= "none"
%	 anchor-point= "(0,21.25)"
%	 text-frame= "noframe"
%	 stroke-width= "0.75"
%	 text-hor-align= "center-h"
%	 >
%$\eex$
%</text>
%<text text-vert-align= "bottom"
%	 fill-style= "none"
%	 anchor-point= "(20.62,21.25)"
%	 text-frame= "noframe"
%	 stroke-width= "0.75"
%	 text-hor-align= "center-h"
%	 >
%$\eex$
%</text>
%<text text-vert-align= "bottom"
%	 fill-style= "none"
%	 anchor-point= "(30.62,21.25)"
%	 text-frame= "noframe"
%	 stroke-width= "0.75"
%	 text-hor-align= "center-h"
%	 >
%$\eex$
%</text>
%<text text-vert-align= "bottom"
%	 fill-style= "none"
%	 anchor-point= "(36.25,21.25)"
%	 text-frame= "noframe"
%	 stroke-width= "0.75"
%	 text-hor-align= "center-h"
%	 >
%$\eex$
%</text>
%<text text-vert-align= "bottom"
%	 fill-style= "none"
%	 anchor-point= "(46.88,21.25)"
%	 text-frame= "noframe"
%	 stroke-width= "0.75"
%	 text-hor-align= "center-h"
%	 >
%$\eex$
%</text>
%<text text-vert-align= "bottom"
%	 fill-style= "none"
%	 anchor-point= "(53.12,21.25)"
%	 text-frame= "noframe"
%	 stroke-width= "0.75"
%	 text-hor-align= "center-h"
%	 >
%$\eex$
%</text>
%<text text-vert-align= "bottom"
%	 fill-style= "none"
%	 anchor-point= "(63.12,21.25)"
%	 text-frame= "noframe"
%	 stroke-width= "0.75"
%	 text-hor-align= "center-h"
%	 >
%$\eex$
%</text>
%<text text-vert-align= "top"
%	 fill-style= "none"
%	 anchor-point= "(51.88,0.62)"
%	 text-frame= "noframe"
%	 stroke-width= "0.75"
%	 text-hor-align= "center-h"
%	 >
%$\eex$
%</text>
%<text text-vert-align= "top"
%	 fill-style= "none"
%	 anchor-point= "(31.25,0.62)"
%	 text-frame= "noframe"
%	 stroke-width= "0.75"
%	 text-hor-align= "center-h"
%	 >
%$\eex$
%</text>
%<text text-vert-align= "top"
%	 fill-style= "none"
%	 anchor-point= "(5,0.62)"
%	 text-frame= "noframe"
%	 stroke-width= "0.75"
%	 text-hor-align= "center-h"
%	 >
%$\eex$
%</text>
%<text text-vert-align= "top"
%	 fill-style= "none"
%	 anchor-point= "(100,0.62)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\why$
%</text>
%<text text-vert-align= "top"
%	 fill-style= "none"
%	 anchor-point= "(131.25,0.62)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\why$
%</text>
%<text text-vert-align= "bottom"
%	 fill-style= "none"
%	 anchor-point= "(140.62,20.62)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\why$
%</text>
%<text text-vert-align= "bottom"
%	 fill-style= "none"
%	 anchor-point= "(135,20.62)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\why$
%</text>
%<text text-vert-align= "bottom"
%	 fill-style= "none"
%	 anchor-point= "(128.12,20.62)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\why$
%</text>
%<text text-vert-align= "bottom"
%	 fill-style= "none"
%	 anchor-point= "(121.88,20.62)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\why$
%</text>
%<text text-vert-align= "bottom"
%	 fill-style= "none"
%	 anchor-point= "(107.5,20.62)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\why$
%</text>
%<text text-vert-align= "bottom"
%	 fill-style= "none"
%	 anchor-point= "(102.5,20.62)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\why$
%</text>
%<text text-vert-align= "bottom"
%	 fill-style= "none"
%	 anchor-point= "(97.5,20.62)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\why$
%</text>
%<text text-vert-align= "bottom"
%	 fill-style= "none"
%	 anchor-point= "(92.5,20.62)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\why$
%</text>
%</jpic>
%%End JPIC-XML
%PSTricks content-type (pstricks.sty package needed)
%Add \usepackage{pstricks} in the preamble of your LaTeX file
%You can rescale the whole picture (to 80% for instance) by using the command \def\JPicScale{0.8}
\ifx\JPicScale\undefined\def\JPicScale{1}\fi
\psset{unit=\JPicScale mm}
\psset{linewidth=0.3,dotsep=1,hatchwidth=0.3,hatchsep=1.5,shadowsize=1,dimen=middle}
\psset{dotsize=0.7 2.5,dotscale=1 1,fillcolor=black}
\psset{arrowsize=1 2,arrowlength=1,arrowinset=0.25,tbarsize=0.7 5,bracketlength=0.15,rbracketlength=0.15}
\begin{pspicture}(0,0)(155.62,21.25)
\rput{0}(5,8.75){\psellipse[fillstyle=solid](0,0)(1.57,-1.56)}
\psline(5,8.75)(5,2.5)
\psline(10,13.75)(5,8.75)
\psline(5,20)(5,8.75)
\psline(0,13.75)(5,8.75)
\psline(10,20)(10,13.75)
\psline(0,20)(0,13.75)
\rput{0}(58.12,13.12){\psellipse[fillstyle=solid](0,0)(1.56,-1.56)}
\psline(63.12,20.62)
(63.12,20)
(63.13,18.12)(59.38,14.37)
\psline(53.12,20.62)
(53.12,20)
(53.13,18.12)(56.88,14.37)
\rput{0}(51.88,6.88){\psellipse[fillstyle=solid](0,0)(1.57,-1.56)}
\psline(46.87,20)
(46.88,13.75)
(46.88,11.87)(50.63,8.12)
\pscustom[]{\psline(56.88,11.88)(51.88,6.88)
\psbezier(51.88,6.88)(51.88,6.88)(51.88,6.88)
\psbezier(51.88,6.88)(51.88,6.88)(51.88,6.88)
}
\psline(51.88,5.62)
(51.88,2.5)
(51.88,1.88)(51.88,2.5)
\psline(26.87,11.88)
(31.87,6.88)
(30.63,6.88)(31.25,6.88)
\rput{0}(25.62,13.12){\psellipse[fillstyle=solid](0,0)(1.56,-1.57)}
\rput{0}(31.56,7.19){\psellipse[fillstyle=solid](0,0)(1.56,-1.57)}
\psline(36.25,20)
(36.25,17.5)
(36.25,11.87)(32.5,8.12)
\psline(30.62,20)
(30.62,19.37)
(30.63,17.5)(26.88,13.75)
\psline(20.62,20)
(20.62,19.37)
(20.63,17.5)(24.38,13.75)
\psline(31.25,5.62)
(31.25,2.5)
(31.25,1.88)(31.25,2.5)
\rput(15,12.5){\EQLS}
\rput(41.25,12.5){\EQLS}
\rput{0}(100,10){\psellipse[fillstyle=solid](0,0)(1.56,-1.56)}
\psline(100,10)(100,2.5)
\psline(107.5,15)(100,10)
\psline(97.5,15)(100,10)
\psline(92.5,15)(100,10)
\psline(107.5,20)(107.5,15)
\psline(92.5,20)(92.5,15)
\rput(113.75,12.5){\EQLS}
\psline(97.5,20)(97.5,15)
\psline(102.5,20)(102.5,15)
\psline(102.5,15)(100,10)
\rput(146.25,12.5){\EQLS}
\rput(155.62,12.5){\FURTHER}
\rput{90}(131.56,7.81){\psellipse[fillstyle=solid](0,0)(1.57,-1.56)}
\psline(131.25,6.25)
(131.25,3.12)
(131.25,2.51)(131.25,3.12)
\rput{90}(137.5,13.12){\psellipse[fillstyle=solid](0,0)(1.57,-1.56)}
\psline(140.62,20)
(140.62,18.12)
(140.64,16.25)(136.88,12.5)
\psline(134.38,20)
(134.38,18.12)
(134.38,16.25)(138.14,12.5)
\psline(131.88,8.12)(137.5,13.12)
\rput{90}(125,13.12){\psellipse[fillstyle=solid](0,0)(1.57,-1.56)}
\psline(128.12,20)
(128.12,18.12)
(128.14,16.25)(124.38,12.5)
\psline(121.88,20)
(121.88,18.12)
(121.88,16.25)(125.63,12.5)
\psline(131.88,7.5)(125,13.12)
\rput[b](5,21.25){$\eex$}
\rput[b](10,21.25){$\eex$}
\rput[b](0,21.25){$\eex$}
\rput[b](20.62,21.25){$\eex$}
\rput[b](30.62,21.25){$\eex$}
\rput[b](36.25,21.25){$\eex$}
\rput[b](46.88,21.25){$\eex$}
\rput[b](53.12,21.25){$\eex$}
\rput[b](63.12,21.25){$\eex$}
\rput[t](51.88,0.62){$\eex$}
\rput[t](31.25,0.62){$\eex$}
\rput[t](5,0.62){$\eex$}
\rput[t](100,0.62){$\why$}
\rput[t](131.25,0.62){$\why$}
\rput[b](140.62,20.62){$\why$}
\rput[b](135,20.62){$\why$}
\rput[b](128.12,20.62){$\why$}
\rput[b](121.88,20.62){$\why$}
\rput[b](107.5,20.62){$\why$}
\rput[b](102.5,20.62){$\why$}
\rput[b](97.5,20.62){$\why$}
\rput[b](92.5,20.62){$\why$}
\end{pspicture}


==> PIC/cmn-tuplings.tex <==
%%Created by jPicEdt 1.4.1_03: mixed JPIC-XML/LaTeX format
%%Tue Nov 05 13:15:40 GMT-10:00 2019
%%Begin JPIC-XML
%<?xml version="1.0" standalone="yes"?>
%<jpic x-min="0" x-max="157.5" y-min="-0.62" y-max="18.12" auto-bounding="true">
%<ellipse fill-style= "solid"
%	 p3= "(3.43,7.81)"
%	 p2= "(3.43,4.69)"
%	 p1= "(6.56,4.69)"
%	 closure= "open"
%	 angle-end= "0"
%	 angle-start= "0"
%	 />
%<multicurve fill-style= "none"
%	 points= "(5,6.25);(5,6.25);(5,0);(5,0)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(10,11.25);(10,11.25);(5,6.25);(5,6.25)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(5,17.5);(5,17.5);(5,6.25);(5,6.25)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(0,11.25);(0,11.25);(5,6.25);(5,6.25)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(10,17.5);(10,17.5);(10,11.25);(10,11.25)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(0,17.5);(0,17.5);(0,11.25);(0,11.25)"
%	 />
%<ellipse fill-style= "solid"
%	 p3= "(56.56,12.19)"
%	 p2= "(56.56,9.06)"
%	 p1= "(59.69,9.06)"
%	 closure= "open"
%	 angle-end= "0"
%	 angle-start= "0"
%	 />
%<multicurve fill-style= "none"
%	 points= "(63.12,18.12);(63.12,18.12);(63.12,17.5);(63.12,17.5);(63.12,17.5);(63.13,15.62);
%	(63.13,15.62);(63.13,15.62);(59.38,11.87);(59.38,11.87)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(53.12,18.12);(53.12,18.12);(53.12,17.5);(53.12,17.5);(53.12,17.5);(53.13,15.62);
%	(53.13,15.62);(53.13,15.62);(56.88,11.87);(56.88,11.87)"
%	 />
%<ellipse fill-style= "solid"
%	 p3= "(50.31,5.94)"
%	 p2= "(50.31,2.81)"
%	 p1= "(53.44,2.81)"
%	 closure= "open"
%	 angle-end= "0"
%	 angle-start= "0"
%	 />
%<multicurve fill-style= "none"
%	 points= "(46.87,17.5);(46.87,17.5);(46.88,11.25);(46.88,11.25);(46.88,11.25);(46.88,9.37);
%	(46.88,9.37);(46.88,9.37);(50.63,5.62);(50.63,5.62)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(56.88,9.38);(56.88,9.38);(51.88,4.38);(51.88,4.38);(51.88,4.38);(51.88,4.38);
%	(51.88,4.38);(51.88,4.38);(51.88,4.38);(51.88,4.38)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(51.88,3.12);(51.88,3.12);(51.88,0);(51.88,0);(51.88,0);(51.88,-0.62);
%	(51.88,-0.62);(51.88,-0.62);(51.88,0);(51.88,0)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(26.87,9.38);(26.87,9.38);(31.87,4.38);(31.87,4.38);(31.87,4.38);(30.63,4.38);
%	(30.63,4.38);(30.63,4.38);(31.25,4.38);(31.25,4.38)"
%	 />
%<ellipse fill-style= "solid"
%	 p3= "(24.06,12.19)"
%	 p2= "(24.06,9.06)"
%	 p1= "(27.19,9.06)"
%	 closure= "open"
%	 angle-end= "0"
%	 angle-start= "0"
%	 />
%<ellipse fill-style= "solid"
%	 p3= "(30,6.25)"
%	 p2= "(30,3.12)"
%	 p1= "(33.13,3.12)"
%	 closure= "open"
%	 angle-end= "0"
%	 angle-start= "0"
%	 />
%<multicurve fill-style= "none"
%	 points= "(36.25,17.5);(36.25,17.5);(36.25,15);(36.25,15);(36.25,15);(36.25,9.37);
%	(36.25,9.37);(36.25,9.37);(32.5,5.62);(32.5,5.62)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(30.62,17.5);(30.62,17.5);(30.62,16.87);(30.62,16.87);(30.62,16.87);(30.63,15);
%	(30.63,15);(30.63,15);(26.88,11.25);(26.88,11.25)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(20.62,17.5);(20.62,17.5);(20.62,16.87);(20.62,16.87);(20.62,16.87);(20.63,15);
%	(20.63,15);(20.63,15);(24.38,11.25);(24.38,11.25)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(31.25,3.12);(31.25,3.12);(31.25,0);(31.25,0);(31.25,0);(31.25,-0.62);
%	(31.25,-0.62);(31.25,-0.62);(31.25,0);(31.25,0)"
%	 />
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(15,10)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\EQLS
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(41.25,10)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\EQLS
%</text>
%<ellipse fill-style= "solid"
%	 p3= "(98.43,9.06)"
%	 p2= "(98.43,5.94)"
%	 p1= "(101.56,5.94)"
%	 closure= "open"
%	 angle-end= "0"
%	 angle-start= "0"
%	 />
%<multicurve fill-style= "none"
%	 points= "(100,7.5);(100,7.5);(100,0);(100,0)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(107.5,12.5);(107.5,12.5);(100,7.5);(100,7.5)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(97.5,12.5);(97.5,12.5);(100,7.5);(100,7.5)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(92.5,12.5);(92.5,12.5);(100,7.5);(100,7.5)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(107.5,17.5);(107.5,17.5);(107.5,12.5);(107.5,12.5)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(92.5,17.5);(92.5,17.5);(92.5,12.5);(92.5,12.5)"
%	 />
%<ellipse fill-style= "solid"
%	 p3= "(130,6.88)"
%	 p2= "(130,3.75)"
%	 p1= "(133.13,3.75)"
%	 closure= "open"
%	 angle-end= "0"
%	 angle-start= "0"
%	 />
%<multicurve fill-style= "none"
%	 points= "(131.25,3.75);(131.25,3.75);(131.25,0.62);(131.25,0.62);(131.25,0.62);(131.25,0.01);
%	(131.25,0.01);(131.25,0.01);(131.25,0.62);(131.25,0.62)"
%	 />
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(113.75,10)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\EQLS
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(146.25,10)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\EQLS
%</text>
%<multicurve fill-style= "none"
%	 points= "(97.5,17.5);(97.5,17.5);(97.5,12.5);(97.5,12.5)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(102.5,17.5);(102.5,17.5);(102.5,12.5);(102.5,12.5)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(102.5,12.5);(102.5,12.5);(100,7.5);(100,7.5)"
%	 />
%<ellipse fill-style= "solid"
%	 p3= "(123.44,12.19)"
%	 p2= "(123.44,9.06)"
%	 p1= "(126.56,9.06)"
%	 closure= "open"
%	 angle-end= "0"
%	 angle-start= "0"
%	 />
%<multicurve fill-style= "none"
%	 points= "(128.12,17.5);(128.12,17.5);(128.12,15.62);(128.12,15.62);(128.12,15.62);(128.14,13.75);
%	(128.14,13.75);(128.14,13.75);(124.38,10);(124.38,10)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(121.88,17.5);(121.88,17.5);(121.88,17.5);(121.88,17.5);(121.88,17.5);(121.88,13.75);
%	(121.88,13.75);(121.88,13.75);(125.62,10);(125.62,10)"
%	 />
%<ellipse fill-style= "solid"
%	 p3= "(135.94,12.19)"
%	 p2= "(135.94,9.06)"
%	 p1= "(139.06,9.06)"
%	 closure= "open"
%	 angle-end= "0"
%	 angle-start= "0"
%	 />
%<multicurve fill-style= "none"
%	 points= "(140.62,17.5);(140.62,17.5);(140.62,15.62);(140.62,15.62);(140.62,15.62);(140.64,13.75);
%	(140.64,13.75);(140.64,13.75);(136.88,10);(136.88,10)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(134.38,17.5);(134.38,17.5);(134.38,15.62);(134.38,15.62);(134.38,15.62);(134.38,13.75);
%	(134.38,13.75);(134.38,13.75);(138.14,10);(138.14,10)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(131.88,5.62);(131.88,5.62);(137.5,10.62);(137.5,10.62)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(125,10.62);(125,10.62);(131.88,5);(131.88,5)"
%	 />
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(157.5,10)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\FURTHER
%</text>
%</jpic>
%%End JPIC-XML
%PSTricks content-type (pstricks.sty package needed)
%Add \usepackage{pstricks} in the preamble of your LaTeX file
%You can rescale the whole picture (to 80% for instance) by using the command \def\JPicScale{0.8}
\ifx\JPicScale\undefined\def\JPicScale{1}\fi
\psset{unit=\JPicScale mm}
\psset{linewidth=0.3,dotsep=1,hatchwidth=0.3,hatchsep=1.5,shadowsize=1,dimen=middle}
\psset{dotsize=0.7 2.5,dotscale=1 1,fillcolor=black}
\psset{arrowsize=1 2,arrowlength=1,arrowinset=0.25,tbarsize=0.7 5,bracketlength=0.15,rbracketlength=0.15}
\begin{pspicture}(0,0)(157.5,18.12)
\rput{0}(5,6.25){\psellipse[fillstyle=solid](0,0)(1.57,-1.56)}
\psline(5,6.25)(5,0)
\psline(10,11.25)(5,6.25)
\psline(5,17.5)(5,6.25)
\psline(0,11.25)(5,6.25)
\psline(10,17.5)(10,11.25)
\psline(0,17.5)(0,11.25)
\rput{0}(58.12,10.63){\psellipse[fillstyle=solid](0,0)(1.57,-1.56)}
\psline(63.12,18.12)
(63.12,17.5)
(63.13,15.62)(59.38,11.87)
\psline(53.12,18.12)
(53.12,17.5)
(53.13,15.62)(56.88,11.87)
\rput{0}(51.88,4.38){\psellipse[fillstyle=solid](0,0)(1.57,-1.57)}
\psline(46.87,17.5)
(46.88,11.25)
(46.88,9.37)(50.63,5.62)
\pscustom[]{\psline(56.88,9.38)(51.88,4.38)
\psbezier(51.88,4.38)(51.88,4.38)(51.88,4.38)
\psbezier(51.88,4.38)(51.88,4.38)(51.88,4.38)
}
\psline(51.88,3.12)
(51.88,0)
(51.88,-0.62)(51.88,0)
\psline(26.87,9.38)
(31.87,4.38)
(30.63,4.38)(31.25,4.38)
\rput{0}(25.62,10.62){\psellipse[fillstyle=solid](0,0)(1.56,-1.57)}
\rput{0}(31.56,4.69){\psellipse[fillstyle=solid](0,0)(1.56,-1.57)}
\psline(36.25,17.5)
(36.25,15)
(36.25,9.37)(32.5,5.62)
\psline(30.62,17.5)
(30.62,16.87)
(30.63,15)(26.88,11.25)
\psline(20.62,17.5)
(20.62,16.87)
(20.63,15)(24.38,11.25)
\psline(31.25,3.12)
(31.25,0)
(31.25,-0.62)(31.25,0)
\rput(15,10){\EQLS}
\rput(41.25,10){\EQLS}
\rput{0}(100,7.5){\psellipse[fillstyle=solid](0,0)(1.57,-1.56)}
\psline(100,7.5)(100,0)
\psline(107.5,12.5)(100,7.5)
\psline(97.5,12.5)(100,7.5)
\psline(92.5,12.5)(100,7.5)
\psline(107.5,17.5)(107.5,12.5)
\psline(92.5,17.5)(92.5,12.5)
\rput{0}(131.56,5.31){\psellipse[fillstyle=solid](0,0)(1.56,-1.57)}
\psline(131.25,3.75)
(131.25,0.62)
(131.25,0.01)(131.25,0.62)
\rput(113.75,10){\EQLS}
\rput(146.25,10){\EQLS}
\psline(97.5,17.5)(97.5,12.5)
\psline(102.5,17.5)(102.5,12.5)
\psline(102.5,12.5)(100,7.5)
\rput{0}(125,10.62){\psellipse[fillstyle=solid](0,0)(1.56,-1.57)}
\psline(128.12,17.5)
(128.12,15.62)
(128.14,13.75)(124.38,10)
\pscustom[]{\psbezier(121.88,17.5)(121.88,17.5)(121.88,17.5)(121.88,17.5)
\psline(121.88,17.5)(121.88,13.75)
\psline(121.88,13.75)(125.62,10)
}
\rput{0}(137.5,10.62){\psellipse[fillstyle=solid](0,0)(1.56,-1.57)}
\psline(140.62,17.5)
(140.62,15.62)
(140.64,13.75)(136.88,10)
\psline(134.38,17.5)
(134.38,15.62)
(134.38,13.75)(138.14,10)
\psline(131.88,5.62)(137.5,10.62)
\psline(125,10.62)(131.88,5)
\rput(157.5,10){\FURTHER}
\end{pspicture}


==> PIC/cmn.tex <==
%%Created by jPicEdt 1.4.1_03: mixed JPIC-XML/LaTeX format
%%Sat Sep 02 18:07:55 HST 2017
%%Begin JPIC-XML
%<?xml version="1.0" standalone="yes"?>
%<jpic x-min="0" x-max="5" y-min="-7.5" y-max="10" auto-bounding="true">
%<ellipse p3= "(0.93,-0.94)"
%	 p2= "(0.93,-4.06)"
%	 p1= "(4.06,-4.06)"
%	 closure= "open"
%	 angle-end= "0"
%	 fill-style= "solid"
%	 angle-start= "0"
%	 />
%<multicurve points= "(2.5,-2.5);(2.5,-2.5);(2.5,-7.5);(2.5,-7.5)"
%	 fill-style= "none"
%	 />
%<multicurve points= "(5,0);(5,0);(2.5,-2.5);(2.5,-2.5)"
%	 fill-style= "none"
%	 />
%<multicurve points= "(0,0);(0,0);(2.5,-2.5);(2.5,-2.5)"
%	 fill-style= "none"
%	 />
%<multicurve points= "(5,10);(5,10);(5,0);(5,0)"
%	 fill-style= "none"
%	 />
%<multicurve points= "(0,10);(0,10);(0,0);(0,0)"
%	 fill-style= "none"
%	 />
%</jpic>
%%End JPIC-XML
%PSTricks content-type (pstricks.sty package needed)
%Add \usepackage{pstricks} in the preamble of your LaTeX file
%You can rescale the whole picture (to 80% for instance) by using the command \def\JPicScale{0.8}
\ifx\JPicScale\undefined\def\JPicScale{1}\fi
\psset{unit=\JPicScale mm}
\psset{linewidth=0.3,dotsep=1,hatchwidth=0.3,hatchsep=1.5,shadowsize=1,dimen=middle}
\psset{dotsize=0.7 2.5,dotscale=1 1,fillcolor=black}
\psset{arrowsize=1 2,arrowlength=1,arrowinset=0.25,tbarsize=0.7 5,bracketlength=0.15,rbracketlength=0.15}
\begin{pspicture}(0,0)(5,10)
\rput{0}(2.5,-2.5){\psellipse[fillstyle=solid](0,0)(1.57,-1.56)}
\psline(2.5,-2.5)(2.5,-7.5)
\psline(5,0)(2.5,-2.5)
\psline(0,0)(2.5,-2.5)
\psline(5,10)(5,0)
\psline(0,10)(0,0)
\end{pspicture}


==> PIC/coind-coalg.tex <==
%%Created by jPicEdt 1.4.1_03: mixed JPIC-XML/LaTeX format
%%Fri Jan 01 16:39:01 GMT-10:00 2021
%%Begin JPIC-XML
%<?xml version="1.0" standalone="yes"?>
%<jpic x-min="0.63" x-max="42.11" y-min="1.25" y-max="51.25" auto-bounding="true">
%<multicurve fill-style= "none"
%	 points= "(5.63,13.12);(5.63,13.12);(5.63,24.37);(5.63,24.37)"
%	 stroke-width= "0.2"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(5.62,29.38)"
%	 text-frame= "noframe"
%	 stroke-width= "0.2"
%	 text-hor-align= "center-h"
%	 >
%$\ahh$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(3.75,11.25)"
%	 text-frame= "noframe"
%	 stroke-width= "0.2"
%	 text-hor-align= "center-h"
%	 >
%$\aah$
%</text>
%<multicurve fill-style= "none"
%	 points= "(0.63,18.11);(0.63,18.11);(10.61,8.13);(10.61,8.13);(10.61,8.13);(0.63,8.13);
%	(0.63,8.13);(0.63,8.13);(0.63,18.11)"
%	 stroke-width= "0.2"
%	 />
%<multicurve fill-style= "none"
%	 points= "(5.62,34.38);(5.62,34.38);(5.63,48.12);(5.63,48.12)"
%	 stroke-width= "0.2"
%	 />
%<multicurve fill-style= "none"
%	 points= "(5.63,4.38);(5.63,4.38);(5.63,8.12);(5.63,8.12)"
%	 stroke-width= "0.2"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(5.63,1.25)"
%	 text-frame= "noframe"
%	 stroke-width= "0.2"
%	 text-hor-align= "center-h"
%	 >
%$\xxh$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(5,20.62)"
%	 text-frame= "noframe"
%	 stroke-width= "0.2"
%	 text-hor-align= "right"
%	 >
%$\RRsmall$
%</text>
%<multicurve fill-style= "none"
%	 points= "(10.63,19.37);(10.63,19.37);(0.63,29.38);(0.63,29.38)"
%	 stroke-width= "0.2"
%	 />
%<multicurve fill-style= "none"
%	 points= "(10.62,29.37);(10.62,29.37);(10.62,19.38);(10.62,19.38)"
%	 stroke-width= "0.2"
%	 />
%<multicurve fill-style= "none"
%	 points= "(0.63,39.38);(0.63,39.38);(0.63,29.38);(0.63,29.38)"
%	 stroke-width= "0.2"
%	 />
%<multicurve fill-style= "none"
%	 points= "(10.63,29.38);(10.63,29.38);(0.63,39.38);(0.63,39.38)"
%	 stroke-width= "0.2"
%	 />
%<multicurve fill-style= "none"
%	 points= "(31.87,25.62);(31.87,25.62);(31.87,19.38);(31.87,19.38);(31.87,19.38);(41.88,19.38);
%	(41.88,19.38);(41.88,19.38);(41.88,29.38);(41.88,29.38);(41.88,29.38);(31.87,29.38);
%	(31.87,29.38);(31.87,29.38);(31.88,29.38);(31.88,29.38);(31.88,29.38);(31.87,29.38);
%	(31.87,29.38);(31.87,29.38);(31.87,25.62);(31.87,25.62)"
%	 stroke-width= "0.2"
%	 />
%<multicurve fill-style= "none"
%	 points= "(36.87,4.38);(36.87,4.38);(36.87,19.38);(36.87,19.38)"
%	 stroke-width= "0.2"
%	 />
%<multicurve fill-style= "none"
%	 points= "(36.87,29.38);(36.87,29.38);(36.87,38.12);(36.87,38.12)"
%	 stroke-width= "0.2"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(36.87,1.25)"
%	 text-frame= "noframe"
%	 stroke-width= "0.2"
%	 text-hor-align= "center-h"
%	 >
%$\xxh$
%</text>
%<multicurve fill-style= "none"
%	 points= "(36.87,43.75);(36.87,43.75);(36.87,48.75);(36.87,48.75)"
%	 stroke-width= "0.2"
%	 />
%<multicurve fill-style= "none"
%	 points= "(32.13,48.24);(32.13,48.24);(42.11,38.25);(42.11,38.25);(42.11,38.25);(32.13,38.25);
%	(32.13,38.25);(32.13,38.25);(32.13,48.24)"
%	 stroke-width= "0.2"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(21.25,25)"
%	 text-frame= "noframe"
%	 stroke-width= "0.2"
%	 text-hor-align= "center-h"
%	 >
%\EQLS
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(36.88,24.38)"
%	 text-frame= "noframe"
%	 stroke-width= "0.2"
%	 text-hor-align= "center-h"
%	 >
%$\coalg$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(35.62,33.75)"
%	 text-frame= "noframe"
%	 stroke-width= "0.2"
%	 text-hor-align= "right"
%	 >
%$\txxh$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(36.88,51.25)"
%	 text-frame= "noframe"
%	 stroke-width= "0.2"
%	 text-hor-align= "center-h"
%	 >
%$\tRRsmall$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(5.62,50.62)"
%	 text-frame= "noframe"
%	 stroke-width= "0.2"
%	 text-hor-align= "center-h"
%	 >
%$\tRRsmall$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(35.62,40.62)"
%	 text-frame= "noframe"
%	 stroke-width= "0.2"
%	 text-hor-align= "center-h"
%	 >
%$\taah$
%</text>
%</jpic>
%%End JPIC-XML
%PSTricks content-type (pstricks.sty package needed)
%Add \usepackage{pstricks} in the preamble of your LaTeX file
%You can rescale the whole picture (to 80% for instance) by using the command \def\JPicScale{0.8}
\ifx\JPicScale\undefined\def\JPicScale{1}\fi
\psset{unit=\JPicScale mm}
\psset{linewidth=0.3,dotsep=1,hatchwidth=0.3,hatchsep=1.5,shadowsize=1,dimen=middle}
\psset{dotsize=0.7 2.5,dotscale=1 1,fillcolor=black}
\psset{arrowsize=1 2,arrowlength=1,arrowinset=0.25,tbarsize=0.7 5,bracketlength=0.15,rbracketlength=0.15}
\begin{pspicture}(0,0)(42.11,51.25)
\psline[linewidth=0.2](5.63,13.12)(5.63,24.37)
\rput(5.62,29.38){$\ahh$}
\rput(3.75,11.25){$\aah$}
\pspolygon[linewidth=0.2](0.63,18.11)
(10.61,8.13)
(0.63,8.13)(0.63,18.11)
\psline[linewidth=0.2](5.62,34.38)(5.63,48.12)
\psline[linewidth=0.2](5.63,4.38)(5.63,8.12)
\rput(5.63,1.25){$\xxh$}
\rput[r](5,20.62){$\RRsmall$}
\psline[linewidth=0.2](10.63,19.37)(0.63,29.38)
\psline[linewidth=0.2](10.62,29.37)(10.62,19.38)
\psline[linewidth=0.2](0.63,39.38)(0.63,29.38)
\psline[linewidth=0.2](10.63,29.38)(0.63,39.38)
\psline[linewidth=0.2](31.87,25.62)
(31.87,19.38)
(41.88,19.38)
(41.88,29.38)
(31.87,29.38)
(31.88,29.38)
(31.87,29.38)(31.87,25.62)
\psline[linewidth=0.2](36.87,4.38)(36.87,19.38)
\psline[linewidth=0.2](36.87,29.38)(36.87,38.12)
\rput(36.87,1.25){$\xxh$}
\psline[linewidth=0.2](36.87,43.75)(36.87,48.75)
\pspolygon[linewidth=0.2](32.13,48.24)
(42.11,38.25)
(32.13,38.25)(32.13,48.24)
\rput(21.25,25){\EQLS}
\rput(36.88,24.38){$\coalg$}
\rput[r](35.62,33.75){$\txxh$}
\rput(36.88,51.25){$\tRRsmall$}
\rput(5.62,50.62){$\tRRsmall$}
\rput(35.62,40.62){$\taah$}
\end{pspicture}


==> PIC/coind-coind.tex <==
%%Created by jPicEdt 1.4.1_03: mixed JPIC-XML/LaTeX format
%%Sat Jan 02 10:29:15 GMT-10:00 2021
%%Begin JPIC-XML
%<?xml version="1.0" standalone="yes"?>
%<jpic x-min="0" x-max="260" y-min="5" y-max="295" auto-bounding="true">
%<multicurve fill-style= "none"
%	 points= "(30,135);(30,135);(90,135);(90,135)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(10,155);(10,155);(30,135);(30,135)"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(57.5,148.75)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\universal
%</text>
%<multicurve fill-style= "none"
%	 points= "(10,165);(10,165);(90,165);(90,165)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(10,165);(10,165);(10,155);(10,155)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(70,195);(70,195);(70,165);(70,165)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(90,135);(90,135);(90,165);(90,165)"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(130,147.5)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\EQLS
%</text>
%<multicurve fill-style= "none"
%	 points= "(90,25);(90,25);(90,65);(90,65)"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(72.5,75)"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\nameslang$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(67.5,5)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\inputt$
%</text>
%<multicurve fill-style= "none"
%	 points= "(50,25);(50,25);(90,25);(90,25)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(70,25);(70,25);(70,5);(70,5)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(20,115);(20,115);(20,105);(20,105)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(10,95);(10,95);(10,115);(10,115)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(30,95);(30,95);(10,95);(10,95)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(10,115);(10,115);(30,95);(30,95)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(50,65);(50,65);(90,65);(90,65)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(50,65);(50,65);(50,25);(50,25)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(70,135);(70,135);(70,65);(70,65)"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(15,100)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\Peeg$
%</text>
%<multicurve fill-style= "none"
%	 points= "(70,255);(70,255);(70,215);(70,215)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(50,195);(50,195);(50,235);(50,235)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(90,195);(90,195);(50,195);(50,195)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(50,235);(50,235);(90,195);(90,195)"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(232.5,210)"
%	 text-frame= "noframe"
%	 stroke-width= "0.35"
%	 text-hor-align= "left"
%	 >
%$\progtype$
%</text>
%<multicurve fill-style= "none"
%	 points= "(10,142.5);(10,142.5);(30,122.5);(30,122.5)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(10,125);(10,125);(30,105);(30,105)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(10,142.5);(10,142.5);(10,125);(10,125)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(30,122.5);(30,122.5);(30,105);(30,105)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(20,145);(20,145);(20,132.5);(20,132.5)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(190,135);(190,135);(250,135);(250,135)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(170,155);(170,155);(190,135);(190,135)"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(217.5,148.75)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\universal
%</text>
%<multicurve fill-style= "none"
%	 points= "(170,165);(170,165);(250,165);(250,165)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(170,165);(170,165);(170,155);(170,155)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(230,255);(230,255);(230,165);(230,165)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(250,135);(250,135);(250,165);(250,165)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(230,135);(230,135);(230,5);(230,5)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(180,145);(180,145);(180,105);(180,105)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(170,95);(170,95);(170,115);(170,115)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(190,95);(190,95);(170,95);(170,95)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(170,115);(170,115);(190,95);(190,95)"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(177.5,127.5)"
%	 text-frame= "noframe"
%	 stroke-width= "0.35"
%	 text-hor-align= "right"
%	 >
%$\progtype$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(175,100)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\Peeg$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(227.5,5)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\inputt$
%</text>
%<multicurve fill-style= "none"
%	 points= "(90,235);(90,235);(90,275);(90,275)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(90,275);(90,275);(50,275);(50,275)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(50,275);(50,275);(90,235);(90,235)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(70,275);(70,275);(70,295);(70,295)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(250,235);(250,235);(250,275);(250,275)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(250,275);(250,275);(210,275);(210,275)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(210,275);(210,275);(250,235);(250,235)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(230,275);(230,275);(230,295);(230,295)"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 arrow-head-inset-scale= "0"
%	 anchor-point= "(20,122.5)"
%	 text-frame= "noframe"
%	 stroke-width= "0.95"
%	 text-hor-align= "center-h"
%	 right-arrow= "head"
%	 >
%$\Transf$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 arrow-head-inset-scale= "0"
%	 anchor-point= "(62.5,207.5)"
%	 text-frame= "noframe"
%	 stroke-width= "0.95"
%	 text-hor-align= "center-h"
%	 right-arrow= "head"
%	 >
%$\eencode$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 arrow-head-inset-scale= "0"
%	 anchor-point= "(77.5,262.5)"
%	 text-frame= "noframe"
%	 stroke-width= "0.95"
%	 text-hor-align= "center-h"
%	 right-arrow= "head"
%	 >
%$\deecode$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 arrow-head-inset-scale= "0"
%	 anchor-point= "(237.5,265)"
%	 text-frame= "noframe"
%	 stroke-width= "0.95"
%	 text-hor-align= "center-h"
%	 right-arrow= "head"
%	 >
%$\deecode$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 arrow-head-inset-scale= "0"
%	 anchor-point= "(72.5,185)"
%	 text-frame= "noframe"
%	 stroke-width= "0.95"
%	 text-hor-align= "left"
%	 right-arrow= "head"
%	 >
%$\Tprogtype$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 arrow-head-inset-scale= "0"
%	 anchor-point= "(72.5,295)"
%	 text-frame= "noframe"
%	 stroke-width= "0.95"
%	 text-hor-align= "left"
%	 right-arrow= "head"
%	 >
%$\Tprogtype$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 arrow-head-inset-scale= "0"
%	 anchor-point= "(232.5,295)"
%	 text-frame= "noframe"
%	 stroke-width= "0.95"
%	 text-hor-align= "left"
%	 right-arrow= "head"
%	 >
%$\Tprogtype$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 arrow-head-inset-scale= "0"
%	 anchor-point= "(70,45)"
%	 text-frame= "noframe"
%	 stroke-width= "0.95"
%	 text-hor-align= "center-h"
%	 right-arrow= "head"
%	 >
%$\rgee$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(72.5,232.5)"
%	 text-frame= "noframe"
%	 stroke-width= "0.35"
%	 text-hor-align= "left"
%	 >
%$\progtype$
%</text>
%<multicurve fill-style= "none"
%	 points= "(0,85);(0,85);(100,85);(100,85)"
%	 stroke-width= "0.2"
%	 />
%<multicurve fill-style= "none"
%	 points= "(0,175);(0,175);(100,175);(100,175)"
%	 stroke-width= "0.2"
%	 />
%<multicurve fill-style= "none"
%	 points= "(0,175);(0,175);(0,85);(0,85)"
%	 stroke-width= "0.2"
%	 />
%<multicurve fill-style= "none"
%	 points= "(100,175);(100,175);(100,85);(100,85)"
%	 stroke-width= "0.2"
%	 />
%<multicurve fill-style= "none"
%	 points= "(160,85);(160,85);(260,85);(260,85)"
%	 stroke-width= "0.2"
%	 />
%<multicurve fill-style= "none"
%	 points= "(160,175);(160,175);(260,175);(260,175)"
%	 stroke-width= "0.2"
%	 />
%<multicurve fill-style= "none"
%	 points= "(160,175);(160,175);(160,85);(160,85)"
%	 stroke-width= "0.2"
%	 />
%<multicurve fill-style= "none"
%	 points= "(260,175);(260,175);(260,85);(260,85)"
%	 stroke-width= "0.2"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 arrow-head-inset-scale= "0"
%	 anchor-point= "(50,92.5)"
%	 text-frame= "noframe"
%	 stroke-width= "0.95"
%	 text-hor-align= "center-h"
%	 right-arrow= "head"
%	 >
%$\Tanag$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 arrow-head-inset-scale= "0"
%	 anchor-point= "(210,92.5)"
%	 text-frame= "noframe"
%	 stroke-width= "0.95"
%	 text-hor-align= "center-h"
%	 right-arrow= "head"
%	 >
%$\anag$
%</text>
%</jpic>
%%End JPIC-XML
%LaTeX-picture environment using emulated lines and arcs
%You can rescale the whole picture (to 80% for instance) by using the command \def\JPicScale{0.8}
\ifx\JPicScale\undefined\def\JPicScale{1}\fi
\unitlength \JPicScale mm
\begin{picture}(260,295)(0,0)
\linethickness{0.3mm}
\put(30,135){\line(1,0){60}}
\linethickness{0.3mm}
\multiput(10,155)(0.12,-0.12){167}{\line(1,0){0.12}}
\put(57.5,148.75){\makebox(0,0)[cc]{\universal}}

\linethickness{0.3mm}
\put(10,165){\line(1,0){80}}
\linethickness{0.3mm}
\put(10,155){\line(0,1){10}}
\linethickness{0.3mm}
\put(70,165){\line(0,1){30}}
\linethickness{0.3mm}
\put(90,135){\line(0,1){30}}
\put(130,147.5){\makebox(0,0)[cc]{\EQLS}}

\linethickness{0.3mm}
\put(90,25){\line(0,1){40}}
\put(72.5,75){\makebox(0,0)[cl]{$\nameslang$}}

\put(67.5,5){\makebox(0,0)[cr]{$\inputt$}}

\linethickness{0.3mm}
\put(50,25){\line(1,0){40}}
\linethickness{0.3mm}
\put(70,5){\line(0,1){20}}
\linethickness{0.3mm}
\put(20,105){\line(0,1){10}}
\linethickness{0.3mm}
\put(10,95){\line(0,1){20}}
\linethickness{0.3mm}
\put(10,95){\line(1,0){20}}
\linethickness{0.3mm}
\multiput(10,115)(0.12,-0.12){167}{\line(1,0){0.12}}
\linethickness{0.3mm}
\put(50,65){\line(1,0){40}}
\linethickness{0.3mm}
\put(50,25){\line(0,1){40}}
\linethickness{0.3mm}
\put(70,65){\line(0,1){70}}
\put(15,100){\makebox(0,0)[cc]{$\Peeg$}}

\linethickness{0.3mm}
\put(70,215){\line(0,1){40}}
\linethickness{0.3mm}
\put(50,195){\line(0,1){40}}
\linethickness{0.3mm}
\put(50,195){\line(1,0){40}}
\linethickness{0.3mm}
\multiput(50,235)(0.12,-0.12){333}{\line(1,0){0.12}}
\put(232.5,210){\makebox(0,0)[cl]{$\progtype$}}

\linethickness{0.3mm}
\multiput(10,142.5)(0.12,-0.12){167}{\line(1,0){0.12}}
\linethickness{0.3mm}
\multiput(10,125)(0.12,-0.12){167}{\line(0,-1){0.12}}
\linethickness{0.3mm}
\put(10,125){\line(0,1){17.5}}
\linethickness{0.3mm}
\put(30,105){\line(0,1){17.5}}
\linethickness{0.3mm}
\put(20,132.5){\line(0,1){12.5}}
\linethickness{0.3mm}
\put(190,135){\line(1,0){60}}
\linethickness{0.3mm}
\multiput(170,155)(0.12,-0.12){167}{\line(1,0){0.12}}
\put(217.5,148.75){\makebox(0,0)[cc]{\universal}}

\linethickness{0.3mm}
\put(170,165){\line(1,0){80}}
\linethickness{0.3mm}
\put(170,155){\line(0,1){10}}
\linethickness{0.3mm}
\put(230,165){\line(0,1){90}}
\linethickness{0.3mm}
\put(250,135){\line(0,1){30}}
\linethickness{0.3mm}
\put(230,5){\line(0,1){130}}
\linethickness{0.3mm}
\put(180,105){\line(0,1){40}}
\linethickness{0.3mm}
\put(170,95){\line(0,1){20}}
\linethickness{0.3mm}
\put(170,95){\line(1,0){20}}
\linethickness{0.3mm}
\multiput(170,115)(0.12,-0.12){167}{\line(1,0){0.12}}
\put(177.5,127.5){\makebox(0,0)[cr]{$\progtype$}}

\put(175,100){\makebox(0,0)[cc]{$\Peeg$}}

\put(227.5,5){\makebox(0,0)[cr]{$\inputt$}}

\linethickness{0.3mm}
\put(90,235){\line(0,1){40}}
\linethickness{0.3mm}
\put(50,275){\line(1,0){40}}
\linethickness{0.3mm}
\multiput(50,275)(0.12,-0.12){333}{\line(1,0){0.12}}
\linethickness{0.3mm}
\put(70,275){\line(0,1){20}}
\linethickness{0.3mm}
\put(250,235){\line(0,1){40}}
\linethickness{0.3mm}
\put(210,275){\line(1,0){40}}
\linethickness{0.3mm}
\multiput(210,275)(0.12,-0.12){333}{\line(1,0){0.12}}
\linethickness{0.3mm}
\put(230,275){\line(0,1){20}}
\put(20,122.5){\makebox(0,0)[cc]{$\Transf$}}

\put(62.5,207.5){\makebox(0,0)[cc]{$\eencode$}}

\put(77.5,262.5){\makebox(0,0)[cc]{$\deecode$}}

\put(237.5,265){\makebox(0,0)[cc]{$\deecode$}}

\put(72.5,185){\makebox(0,0)[cl]{$\Tprogtype$}}

\put(72.5,295){\makebox(0,0)[cl]{$\Tprogtype$}}

\put(232.5,295){\makebox(0,0)[cl]{$\Tprogtype$}}

\put(70,45){\makebox(0,0)[cc]{$\rgee$}}

\put(72.5,232.5){\makebox(0,0)[cl]{$\progtype$}}

\linethickness{0.2mm}
\put(0,85){\line(1,0){100}}
\linethickness{0.2mm}
\put(0,175){\line(1,0){100}}
\linethickness{0.2mm}
\put(0,85){\line(0,1){90}}
\linethickness{0.2mm}
\put(100,85){\line(0,1){90}}
\linethickness{0.2mm}
\put(160,85){\line(1,0){100}}
\linethickness{0.2mm}
\put(160,175){\line(1,0){100}}
\linethickness{0.2mm}
\put(160,85){\line(0,1){90}}
\linethickness{0.2mm}
\put(260,85){\line(0,1){90}}
\put(50,92.5){\makebox(0,0)[cc]{$\Tanag$}}

\put(210,92.5){\makebox(0,0)[cc]{$\anag$}}

\end{picture}


==> PIC/coind-mach.tex <==
%%Created by jPicEdt 1.4.1_03: mixed JPIC-XML/LaTeX format
%%Fri Jan 01 16:14:17 GMT-10:00 2021
%%Begin JPIC-XML
%<?xml version="1.0" standalone="yes"?>
%<jpic x-min="0.63" x-max="63.75" y-min="1.25" y-max="51.88" auto-bounding="true">
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(17.5,51.25)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\dh$
%</text>
%<multicurve fill-style= "none"
%	 points= "(5.63,13.12);(5.63,13.12);(5.63,24.37);(5.63,24.37)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(17.63,29.37);(17.63,29.37);(17.5,48.12);(17.5,48.12)"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(11.87,25)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\ahh$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(3.75,11.25)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\aah$
%</text>
%<multicurve fill-style= "none"
%	 points= "(17.5,5);(17.5,5);(17.63,19.37);(17.63,19.37)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(0.63,18.11);(0.63,18.11);(10.61,8.13);(10.61,8.13);(10.61,8.13);(0.63,8.13);
%	(0.63,8.13);(0.63,8.13);(0.63,18.11)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(5.62,34.38);(5.62,34.38);(5.63,48.12);(5.63,48.12)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(5.63,4.38);(5.63,4.38);(5.63,8.12);(5.63,8.12)"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(5.63,1.25)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\xxh$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(5,20.62)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\RRsmall$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(17.5,1.25)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\bhh$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(5.63,51.25)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\RRsmall$
%</text>
%<multicurve fill-style= "none"
%	 points= "(10.63,19.37);(10.63,19.37);(0.63,29.38);(0.63,29.38)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(21.87,19.38);(21.87,19.38);(10.63,19.38);(10.63,19.38)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(21.87,29.38);(21.87,29.38);(21.87,19.38);(21.87,19.38)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(21.87,29.38);(21.87,29.38);(10.63,29.38);(10.63,29.38)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(0.63,39.38);(0.63,39.38);(0.63,29.38);(0.63,29.38)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(10.63,29.38);(10.63,29.38);(0.63,39.38);(0.63,39.38)"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(58.75,51.88)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\dh$
%</text>
%<multicurve fill-style= "none"
%	 points= "(59.37,5);(59.37,5);(59.37,19.38);(59.37,19.38)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(58.75,29.38);(58.75,29.38);(58.75,48.75);(58.75,48.75)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(41.87,25.62);(41.87,25.62);(41.87,19.38);(41.87,19.38);(41.87,19.38);(63.75,19.38);
%	(63.75,19.38);(63.75,19.38);(63.75,29.38);(63.75,29.38);(63.75,29.38);(41.87,29.38);
%	(41.87,29.38);(41.87,29.38);(60,29.36);(60,29.36);(60,29.36);(41.87,29.38);
%	(41.87,29.38);(41.87,29.38);(41.87,25.62);(41.87,25.62)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(46.87,4.38);(46.87,4.38);(46.87,19.38);(46.87,19.38)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(46.87,29.38);(46.87,29.38);(46.87,38.12);(46.87,38.12)"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(46.87,1.25)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\xxh$
%</text>
%<multicurve fill-style= "none"
%	 points= "(46.87,43.75);(46.87,43.75);(46.87,48.75);(46.87,48.75)"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(45.25,41.38)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\aah$
%</text>
%<multicurve fill-style= "none"
%	 points= "(42.13,48.24);(42.13,48.24);(52.11,38.25);(52.11,38.25);(52.11,38.25);(42.13,38.25);
%	(42.13,38.25);(42.13,38.25);(42.13,48.24)"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(45.63,33.75)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\xxh$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(59.37,1.25)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\bhh$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(46.87,51.88)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\RRsmall$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(31.25,25)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\EQLS
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(52,24)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\coalg$
%</text>
%</jpic>
%%End JPIC-XML
%PSTricks content-type (pstricks.sty package needed)
%Add \usepackage{pstricks} in the preamble of your LaTeX file
%You can rescale the whole picture (to 80% for instance) by using the command \def\JPicScale{0.8}
\ifx\JPicScale\undefined\def\JPicScale{1}\fi
\psset{unit=\JPicScale mm}
\psset{linewidth=0.3,dotsep=1,hatchwidth=0.3,hatchsep=1.5,shadowsize=1,dimen=middle}
\psset{dotsize=0.7 2.5,dotscale=1 1,fillcolor=black}
\psset{arrowsize=1 2,arrowlength=1,arrowinset=0.25,tbarsize=0.7 5,bracketlength=0.15,rbracketlength=0.15}
\begin{pspicture}(0,0)(63.75,51.88)
\rput(17.5,51.25){$\dh$}
\psline(5.63,13.12)(5.63,24.37)
\psline(17.63,29.37)(17.5,48.12)
\rput(11.87,25){$\ahh$}
\rput(3.75,11.25){$\aah$}
\psline(17.5,5)(17.63,19.37)
\pspolygon(0.63,18.11)
(10.61,8.13)
(0.63,8.13)(0.63,18.11)
\psline(5.62,34.38)(5.63,48.12)
\psline(5.63,4.38)(5.63,8.12)
\rput(5.63,1.25){$\xxh$}
\rput[r](5,20.62){$\RRsmall$}
\rput(17.5,1.25){$\bhh$}
\rput(5.63,51.25){$\RRsmall$}
\psline(10.63,19.37)(0.63,29.38)
\psline(21.87,19.38)(10.63,19.38)
\psline(21.87,29.38)(21.87,19.38)
\psline(21.87,29.38)(10.63,29.38)
\psline(0.63,39.38)(0.63,29.38)
\psline(10.63,29.38)(0.63,39.38)
\rput(58.75,51.88){$\dh$}
\psline(59.37,5)(59.37,19.38)
\psline(58.75,29.38)(58.75,48.75)
\psline(41.87,25.62)
(41.87,19.38)
(63.75,19.38)
(63.75,29.38)
(41.87,29.38)
(60,29.36)
(41.87,29.38)(41.87,25.62)
\psline(46.87,4.38)(46.87,19.38)
\psline(46.87,29.38)(46.87,38.12)
\rput(46.87,1.25){$\xxh$}
\psline(46.87,43.75)(46.87,48.75)
\rput(45.25,41.38){$\aah$}
\pspolygon(42.13,48.24)
(52.11,38.25)
(42.13,38.25)(42.13,48.24)
\rput[r](45.63,33.75){$\xxh$}
\rput(59.37,1.25){$\bhh$}
\rput(46.87,51.88){$\RRsmall$}
\rput(31.25,25){\EQLS}
\rput(52,24){$\coalg$}
\end{pspicture}


==> PIC/collapse.tex <==
%%Created by jPicEdt 1.4.1_03: mixed JPIC-XML/LaTeX format
%%Fri Dec 30 07:25:09 GMT-10:00 2022
%%Begin JPIC-XML
%<?xml version="1.0" standalone="yes"?>
%<jpic x-min="0" x-max="245" y-min="0" y-max="50" auto-bounding="true">
%<multicurve fill-style= "none"
%	 points= "(10,30);(10,30);(10,0);(10,0)"
%	 stroke-width= "1"
%	 />
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(12.5,35)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\qee$
%</text>
%<multicurve fill-style= "none"
%	 points= "(0,40);(0,40);(20,40);(20,40)"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(0,40);(0,40);(20,20);(20,20)"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(20,40);(20,40);(20,20);(20,20)"
%	 stroke-width= "0.35"
%	 />
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(27.5,30)"
%	 stroke-width= "0.35"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\EQLS
%</text>
%<multicurve fill-style= "none"
%	 points= "(10,50);(10,50);(10,40);(10,40)"
%	 stroke-width= "1"
%	 />
%<multicurve fill-style= "none"
%	 points= "(35,50);(35,50);(35,0);(35,0)"
%	 stroke-width= "1"
%	 />
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(70,30)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\THENN
%</text>
%<multicurve fill-style= "none"
%	 points= "(180,30);(180,30);(180,20);(180,20)"
%	 stroke-width= "1"
%	 />
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(182.5,35)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\qee$
%</text>
%<multicurve fill-style= "none"
%	 points= "(170,40);(170,40);(190,40);(190,40)"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(170,40);(170,40);(190,20);(190,20)"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(190,40);(190,40);(190,20);(190,20)"
%	 stroke-width= "0.35"
%	 />
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(197.5,30)"
%	 stroke-width= "0.35"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\EQLS
%</text>
%<multicurve fill-style= "none"
%	 points= "(180,50);(180,50);(180,40);(180,40)"
%	 stroke-width= "1"
%	 />
%<multicurve fill-style= "none"
%	 points= "(170,10);(170,10);(190,10);(190,10)"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(170,30);(170,30);(190,10);(190,10)"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(170,30);(170,30);(150,30);(150,30)"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(150,30);(150,30);(170,10);(170,10)"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(160,20);(160,20);(160,0);(160,0)"
%	 stroke-width= "1"
%	 />
%<multicurve fill-style= "none"
%	 points= "(180,10);(180,10);(180,0);(180,0)"
%	 stroke-width= "0.35"
%	 />
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(120,20)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\qee$
%</text>
%<multicurve fill-style= "none"
%	 points= "(95,30);(95,30);(135,30);(135,30)"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(135,30);(135,30);(135,10);(135,10)"
%	 stroke-width= "0.35"
%	 />
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(142.5,30)"
%	 stroke-width= "0.35"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\EQLS
%</text>
%<multicurve fill-style= "none"
%	 points= "(125,50);(125,50);(125,30);(125,30)"
%	 stroke-width= "1"
%	 />
%<multicurve fill-style= "none"
%	 points= "(115,10);(115,10);(135,10);(135,10)"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(95,30);(95,30);(115,10);(115,10)"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(105,20);(105,20);(105,0);(105,0)"
%	 stroke-width= "1"
%	 />
%<multicurve fill-style= "none"
%	 points= "(125,10);(125,10);(125,0);(125,0)"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(205,30);(205,30);(225,30);(225,30)"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(225,30);(225,30);(245,10);(245,10)"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(235,50);(235,50);(235,20);(235,20)"
%	 stroke-width= "1"
%	 />
%<multicurve fill-style= "none"
%	 points= "(225,10);(225,10);(245,10);(245,10)"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(205,30);(205,30);(225,10);(225,10)"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(215,20);(215,20);(215,0);(215,0)"
%	 stroke-width= "1"
%	 />
%<multicurve fill-style= "none"
%	 points= "(235,10);(235,10);(235,0);(235,0)"
%	 stroke-width= "0.35"
%	 />
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(170,20)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\see$
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(225,20)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\see$
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(180,20)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\Dottt
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(235,20)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\Dottt
%</text>
%</jpic>
%%End JPIC-XML
%LaTeX-picture environment using emulated lines and arcs
%You can rescale the whole picture (to 80% for instance) by using the command \def\JPicScale{0.8}
\ifx\JPicScale\undefined\def\JPicScale{1}\fi
\unitlength \JPicScale mm
\begin{picture}(245,50)(0,0)
\linethickness{1mm}
\put(10,0){\line(0,1){30}}
\put(12.5,35){\makebox(0,0)[cc]{$\qee$}}

\linethickness{0.35mm}
\put(0,40){\line(1,0){20}}
\linethickness{0.35mm}
\multiput(0,40)(0.12,-0.12){167}{\line(1,0){0.12}}
\linethickness{0.35mm}
\put(20,20){\line(0,1){20}}
\put(27.5,30){\makebox(0,0)[cc]{\EQLS}}

\linethickness{1mm}
\put(10,40){\line(0,1){10}}
\linethickness{1mm}
\put(35,0){\line(0,1){50}}
\put(70,30){\makebox(0,0)[cc]{\THENN}}

\linethickness{1mm}
\put(180,20){\line(0,1){10}}
\put(182.5,35){\makebox(0,0)[cc]{$\qee$}}

\linethickness{0.35mm}
\put(170,40){\line(1,0){20}}
\linethickness{0.35mm}
\multiput(170,40)(0.12,-0.12){167}{\line(1,0){0.12}}
\linethickness{0.35mm}
\put(190,20){\line(0,1){20}}
\put(197.5,30){\makebox(0,0)[cc]{\EQLS}}

\linethickness{1mm}
\put(180,40){\line(0,1){10}}
\linethickness{0.35mm}
\put(170,10){\line(1,0){20}}
\linethickness{0.35mm}
\multiput(170,30)(0.12,-0.12){167}{\line(1,0){0.12}}
\linethickness{0.35mm}
\put(150,30){\line(1,0){20}}
\linethickness{0.35mm}
\multiput(150,30)(0.12,-0.12){167}{\line(1,0){0.12}}
\linethickness{1mm}
\put(160,0){\line(0,1){20}}
\linethickness{0.35mm}
\put(180,0){\line(0,1){10}}
\put(120,20){\makebox(0,0)[cc]{$\qee$}}

\linethickness{0.35mm}
\put(95,30){\line(1,0){40}}
\linethickness{0.35mm}
\put(135,10){\line(0,1){20}}
\put(142.5,30){\makebox(0,0)[cc]{\EQLS}}

\linethickness{1mm}
\put(125,30){\line(0,1){20}}
\linethickness{0.35mm}
\put(115,10){\line(1,0){20}}
\linethickness{0.35mm}
\multiput(95,30)(0.12,-0.12){167}{\line(1,0){0.12}}
\linethickness{1mm}
\put(105,0){\line(0,1){20}}
\linethickness{0.35mm}
\put(125,0){\line(0,1){10}}
\linethickness{0.35mm}
\put(205,30){\line(1,0){20}}
\linethickness{0.35mm}
\multiput(225,30)(0.12,-0.12){167}{\line(1,0){0.12}}
\linethickness{1mm}
\put(235,20){\line(0,1){30}}
\linethickness{0.35mm}
\put(225,10){\line(1,0){20}}
\linethickness{0.35mm}
\multiput(205,30)(0.12,-0.12){167}{\line(1,0){0.12}}
\linethickness{1mm}
\put(215,0){\line(0,1){20}}
\linethickness{0.35mm}
\put(235,0){\line(0,1){10}}
\put(170,20){\makebox(0,0)[cc]{$\see$}}

\put(225,20){\makebox(0,0)[cc]{$\see$}}

\put(180,20){\makebox(0,0)[cc]{\Dottt}}

\put(235,20){\makebox(0,0)[cc]{\Dottt}}

\end{picture}


==> PIC/comp-0.tex <==
%%Created by jPicEdt 1.4.1_03: mixed JPIC-XML/LaTeX format
%%Sun Oct 23 22:17:48 HST 2016
%%Begin JPIC-XML
%<?xml version="1.0" standalone="yes"?>
%<jpic x-min="0" x-max="160" y-min="0" y-max="97.5" auto-bounding="true">
%<multicurve stroke-width= "0.75"
%	 points= "(112.5,40);(112.5,40);(160,40);(160,40)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.75"
%	 points= "(160,20);(160,20);(160,40);(160,40)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.75"
%	 points= "(155,67.5);(155,67.5);(155,40);(155,40)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.75"
%	 points= "(132.5,20);(132.5,20);(160,20);(160,20)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.75"
%	 points= "(155,20);(155,20);(155,0);(155,0)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.75"
%	 points= "(135,20.01);(135,20.01);(135,0);(135,0)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.75"
%	 points= "(112.5,40);(112.5,40);(132.5,20);(132.5,20)"
%	 fill-style= "none"
%	 />
%<ellipse p3= "(137.58,7.42)"
%	 p2= "(137.58,12.58)"
%	 p1= "(132.42,12.58)"
%	 closure= "open"
%	 fill-color= "#330033"
%	 angle-end= "0"
%	 fill-style= "solid"
%	 angle-start= "0"
%	 />
%<multicurve stroke-width= "0.75"
%	 points= "(130,62.5);(130,62.5);(106.25,38.75);(106.25,38.75)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.75"
%	 points= "(106.25,38.75);(106.25,38.75);(135,10);(135,10)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.75"
%	 points= "(105,87.5);(105,87.5);(160,87.5);(160,87.5)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.75"
%	 points= "(160,67.5);(160,67.5);(160,87.5);(160,87.5)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.75"
%	 points= "(150,97.5);(150,97.5);(150,87.5);(150,87.5)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.75"
%	 points= "(125,67.5);(125,67.5);(160,67.5);(160,67.5)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.75"
%	 points= "(130,67.5);(130,67.5);(130,62.5);(130,62.5)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.75"
%	 points= "(105,87.5);(105,87.5);(125,67.5);(125,67.5)"
%	 fill-style= "none"
%	 />
%<text text-vert-align= "center-v"
%	 stroke-width= "0.75"
%	 anchor-point= "(80,67.5)"
%	 text-frame= "noframe"
%	 fill-style= "none"
%	 text-hor-align= "center-h"
%	 >
%\EQLS
%</text>
%<multicurve stroke-width= "0.75"
%	 points= "(5,87.5);(5,87.5);(55,87.5);(55,87.5)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.75"
%	 points= "(55,67.5);(55,67.5);(55,87.5);(55,87.5)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.75"
%	 points= "(40,97.5);(40,97.5);(40,87.5);(40,87.5)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.75"
%	 points= "(25,67.5);(25,67.5);(55,67.5);(55,67.5)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.75"
%	 points= "(50,67.5);(50,67.5);(50,0);(50,0)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.75"
%	 points= "(15,77.5);(15,77.5);(10,72.5);(10,72.5)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.75"
%	 points= "(5,87.5);(5,87.5);(25,67.5);(25,67.5)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.75"
%	 points= "(30,67.5);(30,67.5);(30,0);(30,0)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.75"
%	 points= "(100,62.5);(100,62.5);(100,0);(100,0)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.75"
%	 points= "(0,62.5);(0,62.5);(0,82.5);(0,82.5)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.75"
%	 points= "(0,82.5);(0,82.5);(20,62.5);(20,62.5)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.75"
%	 points= "(0,62.5);(0,62.5);(20,42.5);(20,42.5)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.75"
%	 points= "(20,42.5);(20,42.5);(20,62.5);(20,62.5)"
%	 fill-style= "none"
%	 />
%<text text-vert-align= "center-v"
%	 anchor-point= "(10,62.5)"
%	 text-frame= "noframe"
%	 fill-style= "none"
%	 text-hor-align= "center-h"
%	 >
%$\suces$
%</text>
%<multicurve stroke-width= "0.75"
%	 points= "(5,57.5);(5,57.5);(5,0);(5,0)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.75"
%	 points= "(15,47.5);(15,47.5);(15,0);(15,0)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.75"
%	 points= "(115,77.5);(115,77.5);(100,62.5);(100,62.5)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-overstrike-width= "1"
%	 stroke-overstrike= "true"
%	 stroke-width= "0.75"
%	 points= "(122.5,30);(122.5,30);(112.5,20);(112.5,20)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.75"
%	 points= "(112.5,20);(112.5,20);(112.5,0);(112.5,0)"
%	 fill-style= "none"
%	 />
%</jpic>
%%End JPIC-XML
%PSTricks content-type (pstricks.sty package needed)
%Add \usepackage{pstricks} in the preamble of your LaTeX file
%You can rescale the whole picture (to 80% for instance) by using the command \def\JPicScale{0.8}
\ifx\JPicScale\undefined\def\JPicScale{1}\fi
\psset{unit=\JPicScale mm}
\psset{linewidth=0.3,dotsep=1,hatchwidth=0.3,hatchsep=1.5,shadowsize=1,dimen=middle}
\psset{dotsize=0.7 2.5,dotscale=1 1,fillcolor=black}
\psset{arrowsize=1 2,arrowlength=1,arrowinset=0.25,tbarsize=0.7 5,bracketlength=0.15,rbracketlength=0.15}
\begin{pspicture}(0,0)(160,97.5)
\psline[linewidth=0.75](112.5,40)(160,40)
\psline[linewidth=0.75](160,20)(160,40)
\psline[linewidth=0.75](155,67.5)(155,40)
\psline[linewidth=0.75](132.5,20)(160,20)
\psline[linewidth=0.75](155,20)(155,0)
\psline[linewidth=0.75](135,20.01)(135,0)
\psline[linewidth=0.75](112.5,40)(132.5,20)
\newrgbcolor{userFillColour}{0.2 0 0.2}
\rput{0}(135,10){\psellipse[fillcolor=userFillColour,fillstyle=solid](0,0)(2.58,-2.58)}
\psline[linewidth=0.75](130,62.5)(106.25,38.75)
\psline[linewidth=0.75](106.25,38.75)(135,10)
\psline[linewidth=0.75](105,87.5)(160,87.5)
\psline[linewidth=0.75](160,67.5)(160,87.5)
\psline[linewidth=0.75](150,97.5)(150,87.5)
\psline[linewidth=0.75](125,67.5)(160,67.5)
\psline[linewidth=0.75](130,67.5)(130,62.5)
\psline[linewidth=0.75](105,87.5)(125,67.5)
\rput(80,67.5){\EQLS}
\psline[linewidth=0.75](5,87.5)(55,87.5)
\psline[linewidth=0.75](55,67.5)(55,87.5)
\psline[linewidth=0.75](40,97.5)(40,87.5)
\psline[linewidth=0.75](25,67.5)(55,67.5)
\psline[linewidth=0.75](50,67.5)(50,0)
\psline[linewidth=0.75](15,77.5)(10,72.5)
\psline[linewidth=0.75](5,87.5)(25,67.5)
\psline[linewidth=0.75](30,67.5)(30,0)
\psline[linewidth=0.75](100,62.5)(100,0)
\psline[linewidth=0.75](0,62.5)(0,82.5)
\psline[linewidth=0.75](0,82.5)(20,62.5)
\psline[linewidth=0.75](0,62.5)(20,42.5)
\psline[linewidth=0.75](20,42.5)(20,62.5)
\rput(10,62.5){$\suces$}
\psline[linewidth=0.75](5,57.5)(5,0)
\psline[linewidth=0.75](15,47.5)(15,0)
\psline[linewidth=0.75](115,77.5)(100,62.5)
\psline[linewidth=0.75,border=1](122.5,30)(112.5,20)
\psline[linewidth=0.75](112.5,20)(112.5,0)
\end{pspicture}


==> PIC/comp-1.tex <==
%%Created by jPicEdt 1.4.1_03: mixed JPIC-XML/LaTeX format
%%Wed Sep 28 17:29:19 HST 2016
%%Begin JPIC-XML
%<?xml version="1.0" standalone="yes"?>
%<jpic x-min="0" x-max="130" y-min="1.25" y-max="100" auto-bounding="true">
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(0,47.5);(0,47.5);(40,47.5);(40,47.5)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(0,47.5);(0,47.5);(0,22.5);(0,22.5)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(40,22.5);(40,22.5);(40,47.5);(40,47.5)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(20,65);(20,65);(20,47.5);(20,47.5)"
%	 />
%<text stroke-width= "0.75"
%	 text-vert-align= "center-v"
%	 anchor-point= "(20,71.25)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\nameslang$
%</text>
%<text stroke-width= "0.75"
%	 text-vert-align= "center-v"
%	 anchor-point= "(20,1.25)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\inputt$
%</text>
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(0,22.5);(0,22.5);(40,22.5);(40,22.5)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(20,22.5);(20,22.5);(20,7.5);(20,7.5)"
%	 />
%<text stroke-width= "0.75"
%	 text-vert-align= "center-v"
%	 anchor-point= "(20,35)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\machine
%</text>
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(70,53.12);(70,53.12);(130,53.12);(130,53.12)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(70,31.25);(70,31.25);(70,6.25);(70,6.25)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(130,28.12);(130,28.12);(130,53.12);(130,53.12)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(110,65);(110,65);(110,53.12);(110,53.12)"
%	 />
%<text stroke-width= "0.75"
%	 text-vert-align= "center-v"
%	 anchor-point= "(110,71.25)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\nameslang$
%</text>
%<text stroke-width= "0.75"
%	 text-vert-align= "center-v"
%	 anchor-point= "(110,1.25)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\inputt$
%</text>
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(95,28.12);(95,28.12);(130,28.12);(130,28.12)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(110,28.12);(110,28.12);(110,7.5);(110,7.5)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(70,6.25);(70,6.25);(95,6.25);(95,6.25)"
%	 />
%<text stroke-width= "0.75"
%	 text-vert-align= "center-v"
%	 anchor-point= "(108.12,40)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\universal
%</text>
%<text stroke-width= "0.75"
%	 text-vert-align= "center-v"
%	 anchor-point= "(77.5,13.12)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\program
%</text>
%<text stroke-width= "0.75"
%	 text-vert-align= "center-v"
%	 anchor-point= "(55,35)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\EQLS
%</text>
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(70,31.25);(70,31.25);(95,6.25);(95,6.25)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(82.5,40.62);(82.5,40.62);(82.5,18.75);(82.5,18.75)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(70,53.12);(70,53.12);(95,28.12);(95,28.12)"
%	 />
%<multicurve arrow-head-width-minimum= "1.5"
%	 stroke-width= "1.2"
%	 right-arrow= "double-head"
%	 arrow-head-length-scale= "1.6"
%	 fill-style= "none"
%	 points= "(95,100);(95,100);(45,100);(45,100)"
%	 />
%<text stroke-width= "0.8"
%	 text-vert-align= "center-v"
%	 anchor-point= "(20,100)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\computations
%</text>
%<text stroke-width= "0.8"
%	 text-vert-align= "center-v"
%	 anchor-point= "(110,100)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\data
%</text>
%<text stroke-width= "0.8"
%	 text-vert-align= "center-v"
%	 anchor-point= "(81.25,33.12)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%\progtype
%</text>
%</jpic>
%%End JPIC-XML
%PSTricks content-type (pstricks.sty package needed)
%Add \usepackage{pstricks} in the preamble of your LaTeX file
%You can rescale the whole picture (to 80% for instance) by using the command \def\JPicScale{0.8}
\ifx\JPicScale\undefined\def\JPicScale{1}\fi
\psset{unit=\JPicScale mm}
\psset{linewidth=0.3,dotsep=1,hatchwidth=0.3,hatchsep=1.5,shadowsize=1,dimen=middle}
\psset{dotsize=0.7 2.5,dotscale=1 1,fillcolor=black}
\psset{arrowsize=1 2,arrowlength=1,arrowinset=0.25,tbarsize=0.7 5,bracketlength=0.15,rbracketlength=0.15}
\begin{pspicture}(0,0)(130,100)
\psline[linewidth=0.75](0,47.5)(40,47.5)
\psline[linewidth=0.75](0,47.5)(0,22.5)
\psline[linewidth=0.75](40,22.5)(40,47.5)
\psline[linewidth=0.75](20,65)(20,47.5)
\rput(20,71.25){$\nameslang$}
\rput(20,1.25){$\inputt$}
\psline[linewidth=0.75](0,22.5)(40,22.5)
\psline[linewidth=0.75](20,22.5)(20,7.5)
\rput(20,35){\machine}
\psline[linewidth=0.75](70,53.12)(130,53.12)
\psline[linewidth=0.75](70,31.25)(70,6.25)
\psline[linewidth=0.75](130,28.12)(130,53.12)
\psline[linewidth=0.75](110,65)(110,53.12)
\rput(110,71.25){$\nameslang$}
\rput(110,1.25){$\inputt$}
\psline[linewidth=0.75](95,28.12)(130,28.12)
\psline[linewidth=0.75](110,28.12)(110,7.5)
\psline[linewidth=0.75](70,6.25)(95,6.25)
\rput(108.12,40){\universal}
\rput(77.5,13.12){\program}
\rput(55,35){\EQLS}
\psline[linewidth=0.75](70,31.25)(95,6.25)
\psline[linewidth=0.75](82.5,40.62)(82.5,18.75)
\psline[linewidth=0.75](70,53.12)(95,28.12)
\psline[linewidth=1.2,arrowsize=1.5 2,arrowlength=1.6]{->>}(95,100)(45,100)
\rput(20,100){\computations}
\rput(110,100){\data}
\rput[r](81.25,33.12){\progtype}
\end{pspicture}


==> PIC/comp-10.tex <==
%%Created by jPicEdt 1.4.1_03: mixed JPIC-XML/LaTeX format
%%Thu Nov 09 14:11:52 HST 2017
%%Begin JPIC-XML
%<?xml version="1.0" standalone="yes"?>
%<jpic x-min="0" x-max="130" y-min="1.25" y-max="71.25" auto-bounding="true">
%<multicurve stroke-width= "0.75"
%	 points= "(0,47.5);(0,47.5);(40,47.5);(40,47.5)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.75"
%	 points= "(0,47.5);(0,47.5);(0,22.5);(0,22.5)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.75"
%	 points= "(40,22.5);(40,22.5);(40,47.5);(40,47.5)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.75"
%	 points= "(20,65);(20,65);(20,47.5);(20,47.5)"
%	 fill-style= "none"
%	 />
%<text text-vert-align= "center-v"
%	 stroke-width= "0.75"
%	 anchor-point= "(20,71.25)"
%	 text-frame= "noframe"
%	 fill-style= "none"
%	 text-hor-align= "center-h"
%	 >
%$\nameslang$
%</text>
%<text text-vert-align= "center-v"
%	 stroke-width= "0.75"
%	 anchor-point= "(12.5,2.5)"
%	 text-frame= "noframe"
%	 fill-style= "none"
%	 text-hor-align= "center-h"
%	 >
%$\inputt$
%</text>
%<multicurve stroke-width= "0.75"
%	 points= "(0,22.5);(0,22.5);(40,22.5);(40,22.5)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.75"
%	 points= "(12.5,22.5);(12.5,22.5);(12.5,7.5);(12.5,7.5)"
%	 fill-style= "none"
%	 />
%<text text-vert-align= "center-v"
%	 stroke-width= "0.75"
%	 anchor-point= "(20,35)"
%	 text-frame= "noframe"
%	 fill-style= "none"
%	 text-hor-align= "center-h"
%	 >
%\machine
%</text>
%<multicurve stroke-width= "0.75"
%	 points= "(70,53.12);(70,53.12);(130,53.12);(130,53.12)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.75"
%	 points= "(70,41.25);(70,41.25);(70,16.25);(70,16.25)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.75"
%	 points= "(110,65);(110,65);(110,53.12);(110,53.12)"
%	 fill-style= "none"
%	 />
%<text text-vert-align= "center-v"
%	 stroke-width= "0.75"
%	 anchor-point= "(110,71.25)"
%	 text-frame= "noframe"
%	 fill-style= "none"
%	 text-hor-align= "center-h"
%	 >
%$\nameslang$
%</text>
%<text text-vert-align= "center-v"
%	 stroke-width= "0.75"
%	 anchor-point= "(117.5,1.25)"
%	 text-frame= "noframe"
%	 fill-style= "none"
%	 text-hor-align= "center-h"
%	 >
%$\inputt$
%</text>
%<multicurve stroke-width= "0.75"
%	 points= "(95,28.12);(95,28.12);(130,28.12);(130,28.12)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.75"
%	 points= "(117.5,28.12);(117.5,28.12);(117.5,7.5);(117.5,7.5)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.75"
%	 points= "(70,16.25);(70,16.25);(95,16.25);(95,16.25)"
%	 fill-style= "none"
%	 />
%<text text-vert-align= "center-v"
%	 stroke-width= "0.75"
%	 anchor-point= "(110,40)"
%	 text-frame= "noframe"
%	 fill-style= "none"
%	 text-hor-align= "center-h"
%	 >
%\universal
%</text>
%<text text-vert-align= "center-v"
%	 stroke-width= "0.75"
%	 anchor-point= "(77.5,23.12)"
%	 text-frame= "noframe"
%	 fill-style= "none"
%	 text-hor-align= "center-h"
%	 >
%\program
%</text>
%<text text-vert-align= "center-v"
%	 stroke-width= "0.75"
%	 anchor-point= "(55,35)"
%	 text-frame= "noframe"
%	 fill-style= "none"
%	 text-hor-align= "center-h"
%	 >
%\EQLS
%</text>
%<multicurve stroke-width= "0.75"
%	 points= "(70,41.25);(70,41.25);(95,16.25);(95,16.25)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.75"
%	 points= "(83.12,40);(83.12,40);(83.12,28.12);(83.12,28.12)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.75"
%	 points= "(70,53.12);(70,53.12);(95,28.12);(95,28.12)"
%	 fill-style= "none"
%	 />
%<text text-vert-align= "center-v"
%	 stroke-width= "0.75"
%	 anchor-point= "(27.5,2.5)"
%	 text-frame= "noframe"
%	 fill-style= "none"
%	 text-hor-align= "center-h"
%	 >
%$\inputt$
%</text>
%<multicurve stroke-width= "0.75"
%	 points= "(27.5,22.5);(27.5,22.5);(27.5,7.5);(27.5,7.5)"
%	 fill-style= "none"
%	 />
%<text text-vert-align= "center-v"
%	 stroke-width= "0.75"
%	 anchor-point= "(102.5,1.25)"
%	 text-frame= "noframe"
%	 fill-style= "none"
%	 text-hor-align= "center-h"
%	 >
%$\inputt$
%</text>
%<multicurve stroke-width= "0.75"
%	 points= "(102.5,28.12);(102.5,28.12);(102.5,7.5);(102.5,7.5)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.75"
%	 points= "(130,28.12);(130,28.12);(130,53.12);(130,53.12)"
%	 fill-style= "none"
%	 />
%</jpic>
%%End JPIC-XML
%PSTricks content-type (pstricks.sty package needed)
%Add \usepackage{pstricks} in the preamble of your LaTeX file
%You can rescale the whole picture (to 80% for instance) by using the command \def\JPicScale{0.8}
\ifx\JPicScale\undefined\def\JPicScale{1}\fi
\psset{unit=\JPicScale mm}
\psset{linewidth=0.3,dotsep=1,hatchwidth=0.3,hatchsep=1.5,shadowsize=1,dimen=middle}
\psset{dotsize=0.7 2.5,dotscale=1 1,fillcolor=black}
\psset{arrowsize=1 2,arrowlength=1,arrowinset=0.25,tbarsize=0.7 5,bracketlength=0.15,rbracketlength=0.15}
\begin{pspicture}(0,0)(130,71.25)
\psline[linewidth=0.75](0,47.5)(40,47.5)
\psline[linewidth=0.75](0,47.5)(0,22.5)
\psline[linewidth=0.75](40,22.5)(40,47.5)
\psline[linewidth=0.75](20,65)(20,47.5)
\rput(20,71.25){$\nameslang$}
\rput(12.5,2.5){$\inputt$}
\psline[linewidth=0.75](0,22.5)(40,22.5)
\psline[linewidth=0.75](12.5,22.5)(12.5,7.5)
\rput(20,35){\machine}
\psline[linewidth=0.75](70,53.12)(130,53.12)
\psline[linewidth=0.75](70,41.25)(70,16.25)
\psline[linewidth=0.75](110,65)(110,53.12)
\rput(110,71.25){$\nameslang$}
\rput(117.5,1.25){$\inputt$}
\psline[linewidth=0.75](95,28.12)(130,28.12)
\psline[linewidth=0.75](117.5,28.12)(117.5,7.5)
\psline[linewidth=0.75](70,16.25)(95,16.25)
\rput(110,40){\universal}
\rput(77.5,23.12){\program}
\rput(55,35){\EQLS}
\psline[linewidth=0.75](70,41.25)(95,16.25)
\psline[linewidth=0.75](83.12,40)(83.12,28.12)
\psline[linewidth=0.75](70,53.12)(95,28.12)
\rput(27.5,2.5){$\inputt$}
\psline[linewidth=0.75](27.5,22.5)(27.5,7.5)
\rput(102.5,1.25){$\inputt$}
\psline[linewidth=0.75](102.5,28.12)(102.5,7.5)
\psline[linewidth=0.75](130,28.12)(130,53.12)
\end{pspicture}


==> PIC/comp-2.tex <==
%%Created by jPicEdt 1.4.1_03: mixed JPIC-XML/LaTeX format
%%Wed Sep 28 17:30:39 HST 2016
%%Begin JPIC-XML
%<?xml version="1.0" standalone="yes"?>
%<jpic x-min="20" x-max="110" y-min="1.25" y-max="100" auto-bounding="true">
%<text stroke-width= "0.75"
%	 text-vert-align= "center-v"
%	 anchor-point= "(20,1.25)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\inputt$
%</text>
%<text stroke-width= "0.75"
%	 text-vert-align= "center-v"
%	 anchor-point= "(110,1.25)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\inputt$
%</text>
%<multicurve arrow-head-width-minimum= "1.5"
%	 stroke-width= "1.2"
%	 right-arrow= "double-head"
%	 arrow-head-length-scale= "1.6"
%	 fill-style= "none"
%	 points= "(95,100);(95,100);(45,100);(45,100)"
%	 />
%<text stroke-width= "0.8"
%	 text-vert-align= "center-v"
%	 anchor-point= "(20,100)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\computations
%</text>
%<text stroke-width= "0.8"
%	 text-vert-align= "center-v"
%	 anchor-point= "(110,100)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\data
%</text>
%</jpic>
%%End JPIC-XML
%PSTricks content-type (pstricks.sty package needed)
%Add \usepackage{pstricks} in the preamble of your LaTeX file
%You can rescale the whole picture (to 80% for instance) by using the command \def\JPicScale{0.8}
\ifx\JPicScale\undefined\def\JPicScale{1}\fi
\psset{unit=\JPicScale mm}
\psset{linewidth=0.3,dotsep=1,hatchwidth=0.3,hatchsep=1.5,shadowsize=1,dimen=middle}
\psset{dotsize=0.7 2.5,dotscale=1 1,fillcolor=black}
\psset{arrowsize=1 2,arrowlength=1,arrowinset=0.25,tbarsize=0.7 5,bracketlength=0.15,rbracketlength=0.15}
\begin{pspicture}(0,0)(110,100)
\rput(20,1.25){$\inputt$}
\rput(110,1.25){$\inputt$}
\psline[linewidth=1.2,arrowsize=1.5 2,arrowlength=1.6]{->>}(95,100)(45,100)
\rput(20,100){\computations}
\rput(110,100){\data}
\end{pspicture}


==> PIC/comp-3.tex <==
%%Created by jPicEdt 1.4.1_03: mixed JPIC-XML/LaTeX format
%%Tue Sep 27 03:16:28 HST 2016
%%Begin JPIC-XML
%<?xml version="1.0" standalone="yes"?>
%<jpic x-min="20" x-max="110" y-min="1.25" y-max="100" auto-bounding="true">
%<text stroke-width= "0.75"
%	 text-vert-align= "center-v"
%	 anchor-point= "(20,1.25)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\inputt$
%</text>
%<text stroke-width= "0.75"
%	 text-vert-align= "center-v"
%	 anchor-point= "(110,1.25)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\inputt$
%</text>
%<multicurve arrow-head-width-minimum= "1.5"
%	 stroke-width= "1.2"
%	 right-arrow= "double-head"
%	 arrow-head-length-scale= "1.6"
%	 fill-style= "none"
%	 points= "(67.5,100);(67.5,100);(55,100);(55,100)"
%	 />
%<text stroke-width= "0.8"
%	 text-vert-align= "center-v"
%	 anchor-point= "(20,100)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\computations
%</text>
%<text stroke-width= "0.8"
%	 text-vert-align= "center-v"
%	 anchor-point= "(110,100)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\data
%</text>
%</jpic>
%%End JPIC-XML
%PSTricks content-type (pstricks.sty package needed)
%Add \usepackage{pstricks} in the preamble of your LaTeX file
%You can rescale the whole picture (to 80% for instance) by using the command \def\JPicScale{0.8}
\ifx\JPicScale\undefined\def\JPicScale{1}\fi
\psset{unit=\JPicScale mm}
\psset{linewidth=0.3,dotsep=1,hatchwidth=0.3,hatchsep=1.5,shadowsize=1,dimen=middle}
\psset{dotsize=0.7 2.5,dotscale=1 1,fillcolor=black}
\psset{arrowsize=1 2,arrowlength=1,arrowinset=0.25,tbarsize=0.7 5,bracketlength=0.15,rbracketlength=0.15}
\begin{pspicture}(0,0)(110,100)
\rput(20,1.25){$\inputt$}
\rput(110,1.25){$\inputt$}
\psline[linewidth=1.2,arrowsize=1.5 2,arrowlength=1.6]{->>}(67.5,100)(55,100)
\rput(20,100){\computations}
\rput(110,100){\data}
\end{pspicture}


==> PIC/comp-4.tex <==
%%Created by jPicEdt 1.4.1_03: mixed JPIC-XML/LaTeX format
%%Sun Oct 02 14:27:48 HST 2016
%%Begin JPIC-XML
%<?xml version="1.0" standalone="yes"?>
%<jpic x-min="0" x-max="130" y-min="1.25" y-max="71.25" auto-bounding="true">
%<multicurve stroke-width= "0.75"
%	 points= "(0,47.5);(0,47.5);(40,47.5);(40,47.5)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.75"
%	 points= "(0,47.5);(0,47.5);(0,22.5);(0,22.5)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.75"
%	 points= "(40,22.5);(40,22.5);(40,47.5);(40,47.5)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.75"
%	 points= "(20,65);(20,65);(20,47.5);(20,47.5)"
%	 fill-style= "none"
%	 />
%<text text-vert-align= "center-v"
%	 stroke-width= "0.75"
%	 anchor-point= "(20,71.25)"
%	 text-frame= "noframe"
%	 fill-style= "none"
%	 text-hor-align= "center-h"
%	 >
%$\nameslang$
%</text>
%<text text-vert-align= "center-v"
%	 stroke-width= "0.75"
%	 anchor-point= "(20,1.25)"
%	 text-frame= "noframe"
%	 fill-style= "none"
%	 text-hor-align= "center-h"
%	 >
%$\inputt$
%</text>
%<multicurve stroke-width= "0.75"
%	 points= "(0,22.5);(0,22.5);(40,22.5);(40,22.5)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.75"
%	 points= "(20,22.5);(20,22.5);(20,7.5);(20,7.5)"
%	 fill-style= "none"
%	 />
%<text text-vert-align= "center-v"
%	 stroke-width= "0.75"
%	 anchor-point= "(20,35)"
%	 text-frame= "noframe"
%	 fill-style= "none"
%	 text-hor-align= "center-h"
%	 >
%\machine
%</text>
%<multicurve stroke-width= "0.75"
%	 points= "(70,53.12);(70,53.12);(130,53.12);(130,53.12)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.75"
%	 points= "(70,31.25);(70,31.25);(70,6.25);(70,6.25)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.75"
%	 points= "(130,28.12);(130,28.12);(130,53.12);(130,53.12)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.75"
%	 points= "(110,65);(110,65);(110,53.12);(110,53.12)"
%	 fill-style= "none"
%	 />
%<text text-vert-align= "center-v"
%	 stroke-width= "0.75"
%	 anchor-point= "(110,71.25)"
%	 text-frame= "noframe"
%	 fill-style= "none"
%	 text-hor-align= "center-h"
%	 >
%$\nameslang$
%</text>
%<text text-vert-align= "center-v"
%	 stroke-width= "0.75"
%	 anchor-point= "(110,1.25)"
%	 text-frame= "noframe"
%	 fill-style= "none"
%	 text-hor-align= "center-h"
%	 >
%$\inputt$
%</text>
%<multicurve stroke-width= "0.75"
%	 points= "(95,28.12);(95,28.12);(130,28.12);(130,28.12)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.75"
%	 points= "(110,28.12);(110,28.12);(110,7.5);(110,7.5)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.75"
%	 points= "(70,6.25);(70,6.25);(95,6.25);(95,6.25)"
%	 fill-style= "none"
%	 />
%<text text-vert-align= "center-v"
%	 stroke-width= "0.75"
%	 anchor-point= "(108.12,40)"
%	 text-frame= "noframe"
%	 fill-style= "none"
%	 text-hor-align= "center-h"
%	 >
%\universal
%</text>
%<text text-vert-align= "center-v"
%	 stroke-width= "0.75"
%	 anchor-point= "(77.5,13.12)"
%	 text-frame= "noframe"
%	 fill-style= "none"
%	 text-hor-align= "center-h"
%	 >
%\program
%</text>
%<text text-vert-align= "center-v"
%	 stroke-width= "0.75"
%	 anchor-point= "(55,35)"
%	 text-frame= "noframe"
%	 fill-style= "none"
%	 text-hor-align= "center-h"
%	 >
%\EQLS
%</text>
%<multicurve stroke-width= "0.75"
%	 points= "(70,31.25);(70,31.25);(95,6.25);(95,6.25)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.75"
%	 points= "(82.5,40.62);(82.5,40.62);(82.5,18.75);(82.5,18.75)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.75"
%	 points= "(70,53.12);(70,53.12);(95,28.12);(95,28.12)"
%	 fill-style= "none"
%	 />
%<text text-vert-align= "center-v"
%	 stroke-width= "0.8"
%	 anchor-point= "(81.25,33.12)"
%	 text-frame= "noframe"
%	 fill-style= "none"
%	 text-hor-align= "right"
%	 >
%\progtype
%</text>
%</jpic>
%%End JPIC-XML
%PSTricks content-type (pstricks.sty package needed)
%Add \usepackage{pstricks} in the preamble of your LaTeX file
%You can rescale the whole picture (to 80% for instance) by using the command \def\JPicScale{0.8}
\ifx\JPicScale\undefined\def\JPicScale{1}\fi
\psset{unit=\JPicScale mm}
\psset{linewidth=0.3,dotsep=1,hatchwidth=0.3,hatchsep=1.5,shadowsize=1,dimen=middle}
\psset{dotsize=0.7 2.5,dotscale=1 1,fillcolor=black}
\psset{arrowsize=1 2,arrowlength=1,arrowinset=0.25,tbarsize=0.7 5,bracketlength=0.15,rbracketlength=0.15}
\begin{pspicture}(0,0)(130,71.25)
\psline[linewidth=0.75](0,47.5)(40,47.5)
\psline[linewidth=0.75](0,47.5)(0,22.5)
\psline[linewidth=0.75](40,22.5)(40,47.5)
\psline[linewidth=0.75](20,65)(20,47.5)
\rput(20,71.25){$\nameslang$}
\rput(20,1.25){$\inputt$}
\psline[linewidth=0.75](0,22.5)(40,22.5)
\psline[linewidth=0.75](20,22.5)(20,7.5)
\rput(20,35){\machine}
\psline[linewidth=0.75](70,53.12)(130,53.12)
\psline[linewidth=0.75](70,31.25)(70,6.25)
\psline[linewidth=0.75](130,28.12)(130,53.12)
\psline[linewidth=0.75](110,65)(110,53.12)
\rput(110,71.25){$\nameslang$}
\rput(110,1.25){$\inputt$}
\psline[linewidth=0.75](95,28.12)(130,28.12)
\psline[linewidth=0.75](110,28.12)(110,7.5)
\psline[linewidth=0.75](70,6.25)(95,6.25)
\rput(108.12,40){\universal}
\rput(77.5,13.12){\program}
\rput(55,35){\EQLS}
\psline[linewidth=0.75](70,31.25)(95,6.25)
\psline[linewidth=0.75](82.5,40.62)(82.5,18.75)
\psline[linewidth=0.75](70,53.12)(95,28.12)
\rput[r](81.25,33.12){\progtype}
\end{pspicture}


==> PIC/comp-M-tape.tex <==
%%Created by jPicEdt 1.4.1_03: mixed JPIC-XML/LaTeX format
%%Sun Nov 15 23:08:27 GMT-10:00 2020
%%Begin JPIC-XML
%<?xml version="1.0" standalone="yes"?>
%<jpic x-min="0" x-max="130" y-min="1.25" y-max="71.25" auto-bounding="true">
%<multicurve fill-style= "none"
%	 points= "(0,47.5);(0,47.5);(0,22.5);(0,22.5)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(40,22.5);(40,22.5);(40,47.5);(40,47.5)"
%	 stroke-width= "0.75"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(20,71.25)"
%	 text-frame= "noframe"
%	 stroke-width= "0.75"
%	 text-hor-align= "center-h"
%	 >
%$\nameslang$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(20,1.25)"
%	 text-frame= "noframe"
%	 stroke-width= "0.75"
%	 text-hor-align= "center-h"
%	 >
%$\inputt$
%</text>
%<multicurve fill-style= "none"
%	 points= "(0,22.5);(0,22.5);(40,22.5);(40,22.5)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(20,22.5);(20,22.5);(20,7.5);(20,7.5)"
%	 stroke-width= "0.75"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(20,35)"
%	 text-frame= "noframe"
%	 stroke-width= "0.75"
%	 text-hor-align= "center-h"
%	 >
%\machine
%</text>
%<multicurve fill-style= "none"
%	 points= "(70,41.25);(70,41.25);(70,16.25);(70,16.25)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(130,28.12);(130,28.12);(130,53.12);(130,53.12)"
%	 stroke-width= "0.75"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(110,71.25)"
%	 text-frame= "noframe"
%	 stroke-width= "0.75"
%	 text-hor-align= "center-h"
%	 >
%$\nameslang$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(110,1.25)"
%	 text-frame= "noframe"
%	 stroke-width= "0.75"
%	 text-hor-align= "center-h"
%	 >
%$\inputt$
%</text>
%<multicurve fill-style= "none"
%	 points= "(95,28.12);(95,28.12);(130,28.12);(130,28.12)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(110,28.12);(110,28.12);(110,7.5);(110,7.5)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(70,16.25);(70,16.25);(95,16.25);(95,16.25)"
%	 stroke-width= "0.75"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(108.12,40)"
%	 text-frame= "noframe"
%	 stroke-width= "0.75"
%	 text-hor-align= "center-h"
%	 >
%\universal
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(78.12,23.75)"
%	 text-frame= "noframe"
%	 stroke-width= "0.75"
%	 text-hor-align= "center-h"
%	 >
%\program
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(55,35)"
%	 text-frame= "noframe"
%	 stroke-width= "0.75"
%	 text-hor-align= "center-h"
%	 >
%\EQLS
%</text>
%<multicurve fill-style= "none"
%	 points= "(70,41.25);(70,41.25);(95,16.25);(95,16.25)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(83.12,40);(83.12,40);(83.12,28.12);(83.12,28.12)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(70,53.12);(70,53.12);(95,28.12);(95,28.12)"
%	 stroke-width= "0.75"
%	 />
%<parallelogram p3= "(17.5,65)"
%	 fill-style= "solid"
%	 p2= "(17.5,47.5)"
%	 fill-color= "#999999"
%	 p1= "(22.5,47.5)"
%	 stroke-color= "#999999"
%	 />
%<multicurve fill-style= "none"
%	 points= "(20,65);(20,65);(20,47.5);(20,47.5)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(0,47.5);(0,47.5);(40,47.5);(40,47.5)"
%	 stroke-width= "0.75"
%	 />
%<parallelogram p3= "(107.5,66.25)"
%	 fill-style= "solid"
%	 p2= "(107.5,53.75)"
%	 fill-color= "#999999"
%	 p1= "(112.5,53.75)"
%	 stroke-color= "#999999"
%	 />
%<multicurve fill-style= "none"
%	 points= "(70,53.75);(70,53.75);(130,53.75);(130,53.75)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(110,65.63);(110,65.63);(110,53.75);(110,53.75)"
%	 stroke-width= "0.75"
%	 />
%</jpic>
%%End JPIC-XML
%LaTeX-picture environment using emulated lines and arcs
%You can rescale the whole picture (to 80% for instance) by using the command \def\JPicScale{0.8}
\ifx\JPicScale\undefined\def\JPicScale{1}\fi
\unitlength \JPicScale mm
\begin{picture}(130,71.25)(0,0)
\linethickness{0.75mm}
\put(0,22.5){\line(0,1){25}}
\linethickness{0.75mm}
\put(40,22.5){\line(0,1){25}}
\put(20,71.25){\makebox(0,0)[cc]{$\nameslang$}}

\put(20,1.25){\makebox(0,0)[cc]{$\inputt$}}

\linethickness{0.75mm}
\put(0,22.5){\line(1,0){40}}
\linethickness{0.75mm}
\put(20,7.5){\line(0,1){15}}
\put(20,35){\makebox(0,0)[cc]{\machine}}

\linethickness{0.75mm}
\put(70,16.25){\line(0,1){25}}
\linethickness{0.75mm}
\put(130,28.12){\line(0,1){25}}
\put(110,71.25){\makebox(0,0)[cc]{$\nameslang$}}

\put(110,1.25){\makebox(0,0)[cc]{$\inputt$}}

\linethickness{0.75mm}
\put(95,28.12){\line(1,0){35}}
\linethickness{0.75mm}
\put(110,7.5){\line(0,1){20.62}}
\linethickness{0.75mm}
\put(70,16.25){\line(1,0){25}}
\put(108.12,40){\makebox(0,0)[cc]{\universal}}

\put(78.12,23.75){\makebox(0,0)[cc]{\program}}

\put(55,35){\makebox(0,0)[cc]{\EQLS}}

\linethickness{0.75mm}
\multiput(70,41.25)(0.12,-0.12){208}{\line(1,0){0.12}}
\linethickness{0.75mm}
\put(83.12,28.12){\line(0,1){11.88}}
\linethickness{0.75mm}
\multiput(70,53.12)(0.12,-0.12){208}{\line(1,0){0.12}}
\linethickness{0.3mm}
\put(22.5,47.5){\rule{5\unitlength}{17.5\unitlength}}
\linethickness{0.75mm}
\put(20,47.5){\line(0,1){17.5}}
\linethickness{0.75mm}
\put(0,47.5){\line(1,0){40}}
\linethickness{0.3mm}
\put(112.5,53.75){\rule{5\unitlength}{12.5\unitlength}}
\linethickness{0.75mm}
\put(70,53.75){\line(1,0){60}}
\linethickness{0.75mm}
\put(110,53.75){\line(0,1){11.88}}
\end{picture}


==> PIC/comp-M.tex <==
%%Created by jPicEdt 1.4.1_03: mixed JPIC-XML/LaTeX format
%%Sun Nov 15 23:09:58 GMT-10:00 2020
%%Begin JPIC-XML
%<?xml version="1.0" standalone="yes"?>
%<jpic x-min="0" x-max="130" y-min="1.25" y-max="71.25" auto-bounding="true">
%<multicurve fill-style= "none"
%	 points= "(0,47.5);(0,47.5);(0,22.5);(0,22.5)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(40,22.5);(40,22.5);(40,47.5);(40,47.5)"
%	 stroke-width= "0.75"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(20,71.25)"
%	 text-frame= "noframe"
%	 stroke-width= "0.75"
%	 text-hor-align= "center-h"
%	 >
%$\nameslang$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(20,1.25)"
%	 text-frame= "noframe"
%	 stroke-width= "0.75"
%	 text-hor-align= "center-h"
%	 >
%$\inputt$
%</text>
%<multicurve fill-style= "none"
%	 points= "(0,22.5);(0,22.5);(40,22.5);(40,22.5)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(20,22.5);(20,22.5);(20,7.5);(20,7.5)"
%	 stroke-width= "0.75"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(20,35)"
%	 text-frame= "noframe"
%	 stroke-width= "0.75"
%	 text-hor-align= "center-h"
%	 >
%\machine
%</text>
%<multicurve fill-style= "none"
%	 points= "(70,41.25);(70,41.25);(70,16.25);(70,16.25)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(130,28.12);(130,28.12);(130,53.75);(130,53.75)"
%	 stroke-width= "0.75"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(110,71.25)"
%	 text-frame= "noframe"
%	 stroke-width= "0.75"
%	 text-hor-align= "center-h"
%	 >
%$\nameslang$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(110,1.25)"
%	 text-frame= "noframe"
%	 stroke-width= "0.75"
%	 text-hor-align= "center-h"
%	 >
%$\inputt$
%</text>
%<multicurve fill-style= "none"
%	 points= "(95,28.12);(95,28.12);(130,28.12);(130,28.12)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(110,28.12);(110,28.12);(110,7.5);(110,7.5)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(70,16.25);(70,16.25);(95,16.25);(95,16.25)"
%	 stroke-width= "0.75"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(108.12,40)"
%	 text-frame= "noframe"
%	 stroke-width= "0.75"
%	 text-hor-align= "center-h"
%	 >
%\universal
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(78.12,23.75)"
%	 text-frame= "noframe"
%	 stroke-width= "0.75"
%	 text-hor-align= "center-h"
%	 >
%\program
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(55,35)"
%	 text-frame= "noframe"
%	 stroke-width= "0.75"
%	 text-hor-align= "center-h"
%	 >
%\EQLS
%</text>
%<multicurve fill-style= "none"
%	 points= "(70,41.25);(70,41.25);(95,16.25);(95,16.25)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(83.12,40);(83.12,40);(83.12,28.12);(83.12,28.12)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(69.38,53.75);(69.38,53.75);(95,28.12);(95,28.12)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(20,65);(20,65);(20,47.5);(20,47.5)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(0,47.5);(0,47.5);(40,47.5);(40,47.5)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(70,53.75);(70,53.75);(130,53.75);(130,53.75)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(110,65.63);(110,65.63);(110,53.75);(110,53.75)"
%	 stroke-width= "0.75"
%	 />
%</jpic>
%%End JPIC-XML
%LaTeX-picture environment using emulated lines and arcs
%You can rescale the whole picture (to 80% for instance) by using the command \def\JPicScale{0.8}
\ifx\JPicScale\undefined\def\JPicScale{1}\fi
\unitlength \JPicScale mm
\begin{picture}(130,71.25)(0,0)
\linethickness{0.75mm}
\put(0,22.5){\line(0,1){25}}
\linethickness{0.75mm}
\put(40,22.5){\line(0,1){25}}
\put(20,71.25){\makebox(0,0)[cc]{$\nameslang$}}

\put(20,1.25){\makebox(0,0)[cc]{$\inputt$}}

\linethickness{0.75mm}
\put(0,22.5){\line(1,0){40}}
\linethickness{0.75mm}
\put(20,7.5){\line(0,1){15}}
\put(20,35){\makebox(0,0)[cc]{\machine}}

\linethickness{0.75mm}
\put(70,16.25){\line(0,1){25}}
\linethickness{0.75mm}
\put(130,28.12){\line(0,1){25.63}}
\put(110,71.25){\makebox(0,0)[cc]{$\nameslang$}}

\put(110,1.25){\makebox(0,0)[cc]{$\inputt$}}

\linethickness{0.75mm}
\put(95,28.12){\line(1,0){35}}
\linethickness{0.75mm}
\put(110,7.5){\line(0,1){20.62}}
\linethickness{0.75mm}
\put(70,16.25){\line(1,0){25}}
\put(108.12,40){\makebox(0,0)[cc]{\universal}}

\put(78.12,23.75){\makebox(0,0)[cc]{\program}}

\put(55,35){\makebox(0,0)[cc]{\EQLS}}

\linethickness{0.75mm}
\multiput(70,41.25)(0.12,-0.12){208}{\line(1,0){0.12}}
\linethickness{0.75mm}
\put(83.12,28.12){\line(0,1){11.88}}
\linethickness{0.75mm}
\multiput(69.38,53.75)(0.12,-0.12){214}{\line(0,-1){0.12}}
\linethickness{0.75mm}
\put(20,47.5){\line(0,1){17.5}}
\linethickness{0.75mm}
\put(0,47.5){\line(1,0){40}}
\linethickness{0.75mm}
\put(70,53.75){\line(1,0){60}}
\linethickness{0.75mm}
\put(110,53.75){\line(0,1){11.88}}
\end{picture}


==> PIC/comp-fix.tex <==
%%Created by jPicEdt 1.4.1_03: mixed JPIC-XML/LaTeX format
%%Thu Jul 14 13:57:18 GMT+01:00 2022
%%Begin JPIC-XML
%<?xml version="1.0" standalone="yes"?>
%<jpic x-min="0" x-max="130" y-min="1.25" y-max="78.75" auto-bounding="true">
%<multicurve fill-style= "none"
%	 stroke-width= "0.35"
%	 points= "(0,55);(0,55);(40,55);(40,55)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.35"
%	 points= "(0,55);(0,55);(0,22.5);(0,22.5)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.35"
%	 points= "(40,22.5);(40,22.5);(40,55);(40,55)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.35"
%	 points= "(20,72.5);(20,72.5);(20,55);(20,55)"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 stroke-width= "0.35"
%	 anchor-point= "(20,78.75)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\nameslang$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 stroke-width= "0.35"
%	 anchor-point= "(20,1.25)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\inputt$
%</text>
%<multicurve fill-style= "none"
%	 stroke-width= "0.35"
%	 points= "(0,22.5);(0,22.5);(40,22.5);(40,22.5)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.35"
%	 points= "(20,22.5);(20,22.5);(20,7.5);(20,7.5)"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 stroke-width= "0.35"
%	 anchor-point= "(20,38.75)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\machine
%</text>
%<multicurve fill-style= "none"
%	 stroke-width= "0.35"
%	 points= "(70,60);(70,60);(130,60);(130,60)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.35"
%	 points= "(70,41.25);(70,41.25);(70,16.25);(70,16.25)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.35"
%	 points= "(130,28.12);(130,28.12);(130,60);(130,60)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.35"
%	 points= "(110,72.5);(110,72.5);(110,60);(110,60)"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 stroke-width= "0.35"
%	 anchor-point= "(110,78.75)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\nameslang$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 stroke-width= "0.35"
%	 anchor-point= "(110,1.25)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\inputt$
%</text>
%<multicurve fill-style= "none"
%	 stroke-width= "0.35"
%	 points= "(95,28.12);(95,28.12);(130,28.12);(130,28.12)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.35"
%	 points= "(110,28.12);(110,28.12);(110,7.5);(110,7.5)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.35"
%	 points= "(70,16.25);(70,16.25);(95,16.25);(95,16.25)"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 stroke-width= "0.35"
%	 anchor-point= "(107.5,43.75)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\universal
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 stroke-width= "0.35"
%	 anchor-point= "(78.12,23.75)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\program
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 stroke-width= "0.35"
%	 anchor-point= "(55,35)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\EQLS
%</text>
%<multicurve fill-style= "none"
%	 stroke-width= "0.35"
%	 points= "(70,41.25);(70,41.25);(95,16.25);(95,16.25)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.35"
%	 points= "(83.12,40);(83.12,40);(83.12,28.12);(83.12,28.12)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.35"
%	 points= "(70,53.12);(70,53.12);(95,28.12);(95,28.12)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.35"
%	 points= "(70,53.12);(70,53.12);(70,60);(70,60)"
%	 />
%</jpic>
%%End JPIC-XML
%LaTeX-picture environment using emulated lines and arcs
%You can rescale the whole picture (to 80% for instance) by using the command \def\JPicScale{0.8}
\ifx\JPicScale\undefined\def\JPicScale{1}\fi
\unitlength \JPicScale mm
\begin{picture}(130,78.75)(0,0)
\linethickness{0.35mm}
\put(0,55){\line(1,0){40}}
\linethickness{0.35mm}
\put(0,22.5){\line(0,1){32.5}}
\linethickness{0.35mm}
\put(40,22.5){\line(0,1){32.5}}
\linethickness{0.35mm}
\put(20,55){\line(0,1){17.5}}
\put(20,78.75){\makebox(0,0)[cc]{$\nameslang$}}

\put(20,1.25){\makebox(0,0)[cc]{$\inputt$}}

\linethickness{0.35mm}
\put(0,22.5){\line(1,0){40}}
\linethickness{0.35mm}
\put(20,7.5){\line(0,1){15}}
\put(20,38.75){\makebox(0,0)[cc]{\machine}}

\linethickness{0.35mm}
\put(70,60){\line(1,0){60}}
\linethickness{0.35mm}
\put(70,16.25){\line(0,1){25}}
\linethickness{0.35mm}
\put(130,28.12){\line(0,1){31.88}}
\linethickness{0.35mm}
\put(110,60){\line(0,1){12.5}}
\put(110,78.75){\makebox(0,0)[cc]{$\nameslang$}}

\put(110,1.25){\makebox(0,0)[cc]{$\inputt$}}

\linethickness{0.35mm}
\put(95,28.12){\line(1,0){35}}
\linethickness{0.35mm}
\put(110,7.5){\line(0,1){20.62}}
\linethickness{0.35mm}
\put(70,16.25){\line(1,0){25}}
\put(107.5,43.75){\makebox(0,0)[cc]{\universal}}

\put(78.12,23.75){\makebox(0,0)[cc]{\program}}

\put(55,35){\makebox(0,0)[cc]{\EQLS}}

\linethickness{0.35mm}
\multiput(70,41.25)(0.12,-0.12){208}{\line(1,0){0.12}}
\linethickness{0.35mm}
\put(83.12,28.12){\line(0,1){11.88}}
\linethickness{0.35mm}
\multiput(70,53.12)(0.12,-0.12){208}{\line(1,0){0.12}}
\linethickness{0.35mm}
\put(70,53.12){\line(0,1){6.88}}
\end{picture}


==> PIC/comp-von.tex <==
%%Created by jPicEdt 1.4.1_03: mixed JPIC-XML/LaTeX format
%%Sun Sep 25 18:48:17 CDT 2016
%%Begin JPIC-XML
%<?xml version="1.0" standalone="yes"?>
%<jpic x-min="0" x-max="130.62" y-min="1.25" y-max="71.25" auto-bounding="true">
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(0,47.5);(0,47.5);(40,47.5);(40,47.5)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(0,47.5);(0,47.5);(0,22.5);(0,22.5)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(40,22.5);(40,22.5);(40,47.5);(40,47.5)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(20,65);(20,65);(20,47.5);(20,47.5)"
%	 />
%<text stroke-width= "0.75"
%	 text-vert-align= "center-v"
%	 anchor-point= "(20,71.25)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\nameslang$
%</text>
%<text stroke-width= "0.75"
%	 text-vert-align= "center-v"
%	 anchor-point= "(20,1.25)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\inputt$
%</text>
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(0,22.5);(0,22.5);(40,22.5);(40,22.5)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(20,22.5);(20,22.5);(20,7.5);(20,7.5)"
%	 />
%<text stroke-width= "0.75"
%	 text-vert-align= "center-v"
%	 anchor-point= "(20,35)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\machine
%</text>
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(70,41.25);(70,41.25);(70,16.25);(70,16.25)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(130,28.12);(130,28.12);(130,53.12);(130,53.12)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(110,65);(110,65);(110,53.12);(110,53.12)"
%	 />
%<text stroke-width= "0.75"
%	 text-vert-align= "center-v"
%	 anchor-point= "(110,71.25)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\nameslang$
%</text>
%<text stroke-width= "0.75"
%	 text-vert-align= "center-v"
%	 anchor-point= "(110,1.25)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\inputt$
%</text>
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(110,28.12);(110,28.12);(110,7.5);(110,7.5)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(70,16.25);(70,16.25);(95,16.25);(95,16.25)"
%	 />
%<text stroke-width= "0.75"
%	 text-vert-align= "center-v"
%	 anchor-point= "(112.5,41.25)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\universal
%</text>
%<text stroke-width= "0.75"
%	 text-vert-align= "center-v"
%	 anchor-point= "(77.5,23.12)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\program
%</text>
%<text stroke-width= "0.75"
%	 text-vert-align= "center-v"
%	 anchor-point= "(55,35)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\EQLS
%</text>
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(70,41.25);(70,41.25);(95,16.25);(95,16.25)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(83.12,40);(83.12,40);(83.12,28.12);(83.12,28.12)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(70,53.12);(70,53.12);(95,28.12);(95,28.12)"
%	 />
%<multicurve stroke-width= "0.6"
%	 stroke-color= "#ff3333"
%	 stroke-dasharray= "1;1"
%	 fill-style= "none"
%	 points= "(95,28.12);(95,28.12);(95,53.12);(95,53.12)"
%	 stroke-style= "dashed"
%	 />
%<text text-vert-align= "center-v"
%	 anchor-point= "(88.12,45)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\CPU
%</text>
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(70.62,53.12);(70.62,53.12);(130.62,53.12);(130.62,53.12)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(95,28.12);(95,28.12);(130,28.12);(130,28.12)"
%	 />
%</jpic>
%%End JPIC-XML
%PSTricks content-type (pstricks.sty package needed)
%Add \usepackage{pstricks} in the preamble of your LaTeX file
%You can rescale the whole picture (to 80% for instance) by using the command \def\JPicScale{0.8}
\ifx\JPicScale\undefined\def\JPicScale{1}\fi
\psset{unit=\JPicScale mm}
\psset{linewidth=0.3,dotsep=1,hatchwidth=0.3,hatchsep=1.5,shadowsize=1,dimen=middle}
\psset{dotsize=0.7 2.5,dotscale=1 1,fillcolor=black}
\psset{arrowsize=1 2,arrowlength=1,arrowinset=0.25,tbarsize=0.7 5,bracketlength=0.15,rbracketlength=0.15}
\begin{pspicture}(0,0)(130.62,71.25)
\psline[linewidth=0.75](0,47.5)(40,47.5)
\psline[linewidth=0.75](0,47.5)(0,22.5)
\psline[linewidth=0.75](40,22.5)(40,47.5)
\psline[linewidth=0.75](20,65)(20,47.5)
\rput(20,71.25){$\nameslang$}
\rput(20,1.25){$\inputt$}
\psline[linewidth=0.75](0,22.5)(40,22.5)
\psline[linewidth=0.75](20,22.5)(20,7.5)
\rput(20,35){\machine}
\psline[linewidth=0.75](70,41.25)(70,16.25)
\psline[linewidth=0.75](130,28.12)(130,53.12)
\psline[linewidth=0.75](110,65)(110,53.12)
\rput(110,71.25){$\nameslang$}
\rput(110,1.25){$\inputt$}
\psline[linewidth=0.75](110,28.12)(110,7.5)
\psline[linewidth=0.75](70,16.25)(95,16.25)
\rput(112.5,41.25){\universal}
\rput(77.5,23.12){\program}
\rput(55,35){\EQLS}
\psline[linewidth=0.75](70,41.25)(95,16.25)
\psline[linewidth=0.75](83.12,40)(83.12,28.12)
\psline[linewidth=0.75](70,53.12)(95,28.12)
\newrgbcolor{userLineColour}{1 0.2 0.2}
\psline[linewidth=0.6,linecolor=userLineColour,linestyle=dashed,dash=1 1](95,28.12)(95,53.12)
\rput(88.12,45){\CPU}
\psline[linewidth=0.75](70.62,53.12)(130.62,53.12)
\psline[linewidth=0.75](95,28.12)(130,28.12)
\end{pspicture}


==> PIC/comp.tex <==
%%Created by jPicEdt 1.4.1_03: mixed JPIC-XML/LaTeX format
%%Thu Jul 14 14:01:28 GMT+01:00 2022
%%Begin JPIC-XML
%<?xml version="1.0" standalone="yes"?>
%<jpic x-min="0" x-max="130" y-min="1.25" y-max="78.75" auto-bounding="true">
%<multicurve fill-style= "none"
%	 stroke-width= "0.35"
%	 points= "(0,55);(0,55);(40,55);(40,55)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.35"
%	 points= "(0,55);(0,55);(0,22.5);(0,22.5)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.35"
%	 points= "(40,22.5);(40,22.5);(40,55);(40,55)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.35"
%	 points= "(20,72.5);(20,72.5);(20,55);(20,55)"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 stroke-width= "0.35"
%	 anchor-point= "(20,78.75)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\nameslang$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 stroke-width= "0.35"
%	 anchor-point= "(20,1.25)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\inputt$
%</text>
%<multicurve fill-style= "none"
%	 stroke-width= "0.35"
%	 points= "(0,22.5);(0,22.5);(40,22.5);(40,22.5)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.35"
%	 points= "(20,22.5);(20,22.5);(20,7.5);(20,7.5)"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 stroke-width= "0.35"
%	 anchor-point= "(20,38.75)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\machine
%</text>
%<multicurve fill-style= "none"
%	 stroke-width= "0.35"
%	 points= "(70,60);(70,60);(130,60);(130,60)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.35"
%	 points= "(70,41.25);(70,41.25);(70,16.25);(70,16.25)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.35"
%	 points= "(130,28.12);(130,28.12);(130,60);(130,60)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.35"
%	 points= "(110,72.5);(110,72.5);(110,60);(110,60)"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 stroke-width= "0.35"
%	 anchor-point= "(110,78.75)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\nameslang$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 stroke-width= "0.35"
%	 anchor-point= "(115,1.25)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\inputt$
%</text>
%<multicurve fill-style= "none"
%	 stroke-width= "0.35"
%	 points= "(95,28.12);(95,28.12);(130,28.12);(130,28.12)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.35"
%	 points= "(115,28.12);(115,28.12);(115,7.5);(115,7.5)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.35"
%	 points= "(70,16.25);(70,16.25);(95,16.25);(95,16.25)"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 stroke-width= "0.35"
%	 anchor-point= "(107.5,43.75)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\universal
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 stroke-width= "0.35"
%	 anchor-point= "(78.12,23.75)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\program
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 stroke-width= "0.35"
%	 anchor-point= "(55,35)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\EQLS
%</text>
%<multicurve fill-style= "none"
%	 stroke-width= "0.35"
%	 points= "(70,41.25);(70,41.25);(95,16.25);(95,16.25)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.35"
%	 points= "(81.88,41.25);(81.88,41.25);(81.88,29.37);(81.88,29.37)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.35"
%	 points= "(70,53.12);(70,53.12);(95,28.12);(95,28.12)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.35"
%	 points= "(70,53.12);(70,53.12);(70,60);(70,60)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.35"
%	 points= "(81.88,16.25);(81.88,16.25);(81.88,4.37);(81.88,4.37)"
%	 />
%</jpic>
%%End JPIC-XML
%LaTeX-picture environment using emulated lines and arcs
%You can rescale the whole picture (to 80% for instance) by using the command \def\JPicScale{0.8}
\ifx\JPicScale\undefined\def\JPicScale{1}\fi
\unitlength \JPicScale mm
\begin{picture}(130,78.75)(0,0)
\linethickness{0.35mm}
\put(0,55){\line(1,0){40}}
\linethickness{0.35mm}
\put(0,22.5){\line(0,1){32.5}}
\linethickness{0.35mm}
\put(40,22.5){\line(0,1){32.5}}
\linethickness{0.35mm}
\put(20,55){\line(0,1){17.5}}
\put(20,78.75){\makebox(0,0)[cc]{$\nameslang$}}

\put(20,1.25){\makebox(0,0)[cc]{$\inputt$}}

\linethickness{0.35mm}
\put(0,22.5){\line(1,0){40}}
\linethickness{0.35mm}
\put(20,7.5){\line(0,1){15}}
\put(20,38.75){\makebox(0,0)[cc]{\machine}}

\linethickness{0.35mm}
\put(70,60){\line(1,0){60}}
\linethickness{0.35mm}
\put(70,16.25){\line(0,1){25}}
\linethickness{0.35mm}
\put(130,28.12){\line(0,1){31.88}}
\linethickness{0.35mm}
\put(110,60){\line(0,1){12.5}}
\put(110,78.75){\makebox(0,0)[cc]{$\nameslang$}}

\put(115,1.25){\makebox(0,0)[cc]{$\inputt$}}

\linethickness{0.35mm}
\put(95,28.12){\line(1,0){35}}
\linethickness{0.35mm}
\put(115,7.5){\line(0,1){20.62}}
\linethickness{0.35mm}
\put(70,16.25){\line(1,0){25}}
\put(107.5,43.75){\makebox(0,0)[cc]{\universal}}

\put(78.12,23.75){\makebox(0,0)[cc]{\program}}

\put(55,35){\makebox(0,0)[cc]{\EQLS}}

\linethickness{0.35mm}
\multiput(70,41.25)(0.12,-0.12){208}{\line(1,0){0.12}}
\linethickness{0.35mm}
\put(81.88,29.37){\line(0,1){11.88}}
\linethickness{0.35mm}
\multiput(70,53.12)(0.12,-0.12){208}{\line(1,0){0.12}}
\linethickness{0.35mm}
\put(70,53.12){\line(0,1){6.88}}
\linethickness{0.35mm}
\put(81.88,4.37){\line(0,1){11.88}}
\end{picture}


==> PIC/composition-prog.tex <==
%%Created by jPicEdt 1.4.1_03: mixed JPIC-XML/LaTeX format
%%Mon Dec 03 17:26:20 GMT-10:00 2018
%%Begin JPIC-XML
%<?xml version="1.0" standalone="yes"?>
%<jpic x-min="0" x-max="85" y-min="1.25" y-max="100" auto-bounding="true">
%<multicurve stroke-width= "0.75"
%	 points= "(65,50);(65,50);(85,50);(85,50)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.75"
%	 points= "(85,30);(85,30);(85,50);(85,50)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.75"
%	 points= "(80,70);(80,70);(80,50);(80,50)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.75"
%	 points= "(65,30);(65,30);(85,30);(85,30)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.75"
%	 points= "(70,30);(70,30);(70,5);(70,5)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.75"
%	 points= "(65,90);(65,90);(85,90);(85,90)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.75"
%	 points= "(85,70);(85,70);(85,90);(85,90)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.75"
%	 points= "(80,100);(80,100);(80,90);(80,90)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.75"
%	 points= "(65,70);(65,70);(85,70);(85,70)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.75"
%	 points= "(65,90);(65,90);(65,70);(65,70)"
%	 fill-style= "none"
%	 />
%<text text-vert-align= "center-v"
%	 anchor-point= "(40,50)"
%	 stroke-width= "0.75"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 fill-style= "none"
%	 >
%\EQLS
%</text>
%<multicurve stroke-width= "0.75"
%	 points= "(0,60);(0,60);(20,60);(20,60)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.75"
%	 points= "(20,40);(20,40);(20,60);(20,60)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.75"
%	 points= "(10,100);(10,100);(10,60);(10,60)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.75"
%	 points= "(0,40);(0,40);(20,40);(20,40)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.75"
%	 points= "(0,60);(0,60);(0,40);(0,40)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.75"
%	 points= "(5,40);(5,40);(5,5);(5,5)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.75"
%	 points= "(60,55);(60,55);(70,65);(70,65)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-overstrike-width= "1"
%	 stroke-width= "0.75"
%	 points= "(60,55);(60,55);(60,25);(60,25)"
%	 stroke-overstrike= "true"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.75"
%	 points= "(15,40);(15,40);(15,5);(15,5)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.75"
%	 points= "(70,70);(70,70);(70,65);(70,65)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.75"
%	 points= "(70,15);(70,15);(60,25);(60,25)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.75"
%	 points= "(80,30);(80,30);(80,5);(80,5)"
%	 fill-style= "none"
%	 />
%<ellipse p3= "(72.5,12.5)"
%	 p2= "(72.5,17.5)"
%	 p1= "(67.5,17.5)"
%	 closure= "open"
%	 angle-end= "360"
%	 angle-start= "0"
%	 fill-style= "solid"
%	 />
%<text text-vert-align= "center-v"
%	 anchor-point= "(70,1.25)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 fill-style= "none"
%	 >
%$\Mee$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(5,1.25)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 fill-style= "none"
%	 >
%$\Mee$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(80,1.25)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 fill-style= "none"
%	 >
%$\Ahh$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(15,1.25)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 fill-style= "none"
%	 >
%$\Ahh$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(75,40)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 fill-style= "none"
%	 >
%$\Bee$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(75,80)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 fill-style= "none"
%	 >
%$\Cee$
%</text>
%<multicurve stroke-width= "0.75"
%	 points= "(65,50);(65,50);(65,30);(65,30)"
%	 fill-style= "none"
%	 />
%<text text-vert-align= "center-v"
%	 anchor-point= "(10,50)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 fill-style= "none"
%	 >
%$\Dee$
%</text>
%</jpic>
%%End JPIC-XML
%PSTricks content-type (pstricks.sty package needed)
%Add \usepackage{pstricks} in the preamble of your LaTeX file
%You can rescale the whole picture (to 80% for instance) by using the command \def\JPicScale{0.8}
\ifx\JPicScale\undefined\def\JPicScale{1}\fi
\psset{unit=\JPicScale mm}
\psset{linewidth=0.3,dotsep=1,hatchwidth=0.3,hatchsep=1.5,shadowsize=1,dimen=middle}
\psset{dotsize=0.7 2.5,dotscale=1 1,fillcolor=black}
\psset{arrowsize=1 2,arrowlength=1,arrowinset=0.25,tbarsize=0.7 5,bracketlength=0.15,rbracketlength=0.15}
\begin{pspicture}(0,0)(85,100)
\psline[linewidth=0.75](65,50)(85,50)
\psline[linewidth=0.75](85,30)(85,50)
\psline[linewidth=0.75](80,70)(80,50)
\psline[linewidth=0.75](65,30)(85,30)
\psline[linewidth=0.75](70,30)(70,5)
\psline[linewidth=0.75](65,90)(85,90)
\psline[linewidth=0.75](85,70)(85,90)
\psline[linewidth=0.75](80,100)(80,90)
\psline[linewidth=0.75](65,70)(85,70)
\psline[linewidth=0.75](65,90)(65,70)
\rput(40,50){\EQLS}
\psline[linewidth=0.75](0,60)(20,60)
\psline[linewidth=0.75](20,40)(20,60)
\psline[linewidth=0.75](10,100)(10,60)
\psline[linewidth=0.75](0,40)(20,40)
\psline[linewidth=0.75](0,60)(0,40)
\psline[linewidth=0.75](5,40)(5,5)
\psline[linewidth=0.75](60,55)(70,65)
\psline[linewidth=0.75,border=1](60,55)(60,25)
\psline[linewidth=0.75](15,40)(15,5)
\psline[linewidth=0.75](70,70)(70,65)
\psline[linewidth=0.75](70,15)(60,25)
\psline[linewidth=0.75](80,30)(80,5)
\rput{0}(70,15){\psellipse[fillstyle=solid](0,0)(2.5,-2.5)}
\rput(70,1.25){$\Mee$}
\rput(5,1.25){$\Mee$}
\rput(80,1.25){$\Ahh$}
\rput(15,1.25){$\Ahh$}
\rput(75,40){$\Bee$}
\rput(75,80){$\Cee$}
\psline[linewidth=0.75](65,50)(65,30)
\rput(10,50){$\Dee$}
\end{pspicture}


==> PIC/composition.tex <==
%%Created by jPicEdt 1.4.1_03: mixed JPIC-XML/LaTeX format
%%Sun Oct 23 22:25:36 HST 2016
%%Begin JPIC-XML
%<?xml version="1.0" standalone="yes"?>
%<jpic x-min="0" x-max="160" y-min="0" y-max="70" auto-bounding="true">
%<multicurve stroke-width= "0.75"
%	 points= "(112.5,30);(112.5,30);(160,30);(160,30)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.75"
%	 points= "(160,10);(160,10);(160,30);(160,30)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.75"
%	 points= "(140,40);(140,40);(140,30);(140,30)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.75"
%	 points= "(132.5,10);(132.5,10);(160,10);(160,10)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.75"
%	 points= "(140,10);(140,10);(140,0);(140,0)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.75"
%	 points= "(112.5,30);(112.5,30);(132.5,10);(132.5,10)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.75"
%	 points= "(105,60);(105,60);(160,60);(160,60)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.75"
%	 points= "(160,40);(160,40);(160,60);(160,60)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.75"
%	 points= "(140,70);(140,70);(140,60);(140,60)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.75"
%	 points= "(125,40);(125,40);(160,40);(160,40)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.75"
%	 points= "(105,60);(105,60);(125,40);(125,40)"
%	 fill-style= "none"
%	 />
%<text text-vert-align= "center-v"
%	 stroke-width= "0.75"
%	 anchor-point= "(80,50)"
%	 text-frame= "noframe"
%	 fill-style= "none"
%	 text-hor-align= "center-h"
%	 >
%\EQLS
%</text>
%<multicurve stroke-width= "0.75"
%	 points= "(5,60);(5,60);(55,60);(55,60)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.75"
%	 points= "(55,40);(55,40);(55,60);(55,60)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.75"
%	 points= "(40,70);(40,70);(40,60);(40,60)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.75"
%	 points= "(25,40);(25,40);(55,40);(55,40)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.75"
%	 points= "(50,40);(50,40);(50,0);(50,0)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.75"
%	 points= "(15,50);(15,50);(8.75,43.75);(8.75,43.75)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.75"
%	 points= "(5,60);(5,60);(25,40);(25,40)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.75"
%	 points= "(30,40);(30,40);(30,0);(30,0)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.75"
%	 points= "(100,35);(100,35);(100,0);(100,0)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.75"
%	 points= "(0,32.5);(0,32.5);(0,52.5);(0,52.5)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.75"
%	 points= "(0,52.5);(0,52.5);(20,32.5);(20,32.5)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.75"
%	 points= "(0,32.5);(0,32.5);(20,12.5);(20,12.5)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.75"
%	 points= "(20,12.5);(20,12.5);(20,32.5);(20,32.5)"
%	 fill-style= "none"
%	 />
%<text text-vert-align= "center-v"
%	 anchor-point= "(10,32.5)"
%	 text-frame= "noframe"
%	 fill-style= "none"
%	 text-hor-align= "center-h"
%	 >
%$\suces$
%</text>
%<multicurve stroke-width= "0.75"
%	 points= "(5,27.5);(5,27.5);(5,0);(5,0)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.75"
%	 points= "(15,17.5);(15,17.5);(15,0);(15,0)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.75"
%	 points= "(115,50);(115,50);(100,35);(100,35)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-overstrike-width= "1"
%	 stroke-overstrike= "true"
%	 stroke-width= "0.75"
%	 points= "(122.5,20);(122.5,20);(112.5,10);(112.5,10)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.75"
%	 points= "(112.5,10);(112.5,10);(112.5,0);(112.5,0)"
%	 fill-style= "none"
%	 />
%</jpic>
%%End JPIC-XML
%PSTricks content-type (pstricks.sty package needed)
%Add \usepackage{pstricks} in the preamble of your LaTeX file
%You can rescale the whole picture (to 80% for instance) by using the command \def\JPicScale{0.8}
\ifx\JPicScale\undefined\def\JPicScale{1}\fi
\psset{unit=\JPicScale mm}
\psset{linewidth=0.3,dotsep=1,hatchwidth=0.3,hatchsep=1.5,shadowsize=1,dimen=middle}
\psset{dotsize=0.7 2.5,dotscale=1 1,fillcolor=black}
\psset{arrowsize=1 2,arrowlength=1,arrowinset=0.25,tbarsize=0.7 5,bracketlength=0.15,rbracketlength=0.15}
\begin{pspicture}(0,0)(160,70)
\psline[linewidth=0.75](112.5,30)(160,30)
\psline[linewidth=0.75](160,10)(160,30)
\psline[linewidth=0.75](140,40)(140,30)
\psline[linewidth=0.75](132.5,10)(160,10)
\psline[linewidth=0.75](140,10)(140,0)
\psline[linewidth=0.75](112.5,30)(132.5,10)
\psline[linewidth=0.75](105,60)(160,60)
\psline[linewidth=0.75](160,40)(160,60)
\psline[linewidth=0.75](140,70)(140,60)
\psline[linewidth=0.75](125,40)(160,40)
\psline[linewidth=0.75](105,60)(125,40)
\rput(80,50){\EQLS}
\psline[linewidth=0.75](5,60)(55,60)
\psline[linewidth=0.75](55,40)(55,60)
\psline[linewidth=0.75](40,70)(40,60)
\psline[linewidth=0.75](25,40)(55,40)
\psline[linewidth=0.75](50,40)(50,0)
\psline[linewidth=0.75](15,50)(8.75,43.75)
\psline[linewidth=0.75](5,60)(25,40)
\psline[linewidth=0.75](30,40)(30,0)
\psline[linewidth=0.75](100,35)(100,0)
\psline[linewidth=0.75](0,32.5)(0,52.5)
\psline[linewidth=0.75](0,52.5)(20,32.5)
\psline[linewidth=0.75](0,32.5)(20,12.5)
\psline[linewidth=0.75](20,12.5)(20,32.5)
\rput(10,32.5){$\suces$}
\psline[linewidth=0.75](5,27.5)(5,0)
\psline[linewidth=0.75](15,17.5)(15,0)
\psline[linewidth=0.75](115,50)(100,35)
\psline[linewidth=0.75,border=1](122.5,20)(112.5,10)
\psline[linewidth=0.75](112.5,10)(112.5,0)
\end{pspicture}


==> PIC/compositions.tex <==
%%Created by jPicEdt 1.4.1_03: mixed JPIC-XML/LaTeX format
%%Sat Sep 02 21:42:12 HST 2017
%%Begin JPIC-XML
%<?xml version="1.0" standalone="yes"?>
%<jpic x-min="0" x-max="127.5" y-min="-37.5" y-max="40" auto-bounding="true">
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(0,-10);(0,-10);(20,-10);(20,-10)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(0,-10);(0,-10);(0,-25);(0,-25)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(20,-25);(20,-25);(20,-10);(20,-10)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(10,10);(10,10);(10,-10);(10,-10)"
%	 />
%<text stroke-width= "0.75"
%	 text-vert-align= "center-v"
%	 anchor-point= "(7.5,0)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\nameslang$
%</text>
%<text stroke-width= "0.75"
%	 text-vert-align= "center-v"
%	 anchor-point= "(7.5,-35)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\inputt$
%</text>
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(0,-25);(0,-25);(20,-25);(20,-25)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(10,-25);(10,-25);(10,-37.5);(10,-37.5)"
%	 />
%<text stroke-width= "0.75"
%	 text-vert-align= "center-v"
%	 anchor-point= "(10,-17.5)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\machine
%</text>
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(0,25);(0,25);(20,25);(20,25)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(0,25);(0,25);(0,10);(0,10)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(20,10);(20,10);(20,25);(20,25)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(10,40);(10,40);(10,25);(10,25)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(0,10);(0,10);(20,10);(20,10)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(80,7.5);(80,7.5);(100,7.5);(100,7.5)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(80,7.5);(80,7.5);(80,-7.5);(80,-7.5)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(100,-7.5);(100,-7.5);(100,7.5);(100,7.5)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(90,22.5);(90,22.5);(90,7.5);(90,7.5)"
%	 />
%<text stroke-width= "0.75"
%	 text-vert-align= "center-v"
%	 anchor-point= "(87.5,17.5)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\nameslang$
%</text>
%<text stroke-width= "0.75"
%	 text-vert-align= "center-v"
%	 anchor-point= "(87.5,-17.5)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\inputt$
%</text>
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(80,-7.5);(80,-7.5);(100,-7.5);(100,-7.5)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(90,-7.5);(90,-7.5);(90,-22.5);(90,-22.5)"
%	 />
%<text stroke-width= "0.75"
%	 text-vert-align= "center-v"
%	 anchor-point= "(90,0)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\machine
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(7.5,37.5)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\outputt$
%</text>
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(107.5,7.5);(107.5,7.5);(127.5,7.5);(127.5,7.5)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(107.5,7.5);(107.5,7.5);(107.5,-7.5);(107.5,-7.5)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(127.5,-7.5);(127.5,-7.5);(127.5,7.5);(127.5,7.5)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(117.5,22.5);(117.5,22.5);(117.5,7.5);(117.5,7.5)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(107.5,-7.5);(107.5,-7.5);(127.5,-7.5);(127.5,-7.5)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(117.5,-7.5);(117.5,-7.5);(117.5,-22.5);(117.5,-22.5)"
%	 />
%<text text-vert-align= "center-v"
%	 anchor-point= "(117.5,0)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\michine$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(120,-20)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\inputtt$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(120,17.5)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\outputtt$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(10,17.5)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\muchine$
%</text>
%</jpic>
%%End JPIC-XML
%PSTricks content-type (pstricks.sty package needed)
%Add \usepackage{pstricks} in the preamble of your LaTeX file
%You can rescale the whole picture (to 80% for instance) by using the command \def\JPicScale{0.8}
\ifx\JPicScale\undefined\def\JPicScale{1}\fi
\psset{unit=\JPicScale mm}
\psset{linewidth=0.3,dotsep=1,hatchwidth=0.3,hatchsep=1.5,shadowsize=1,dimen=middle}
\psset{dotsize=0.7 2.5,dotscale=1 1,fillcolor=black}
\psset{arrowsize=1 2,arrowlength=1,arrowinset=0.25,tbarsize=0.7 5,bracketlength=0.15,rbracketlength=0.15}
\begin{pspicture}(0,0)(127.5,40)
\psline[linewidth=0.75](0,-10)(20,-10)
\psline[linewidth=0.75](0,-10)(0,-25)
\psline[linewidth=0.75](20,-25)(20,-10)
\psline[linewidth=0.75](10,10)(10,-10)
\rput[r](7.5,0){$\nameslang$}
\rput[r](7.5,-35){$\inputt$}
\psline[linewidth=0.75](0,-25)(20,-25)
\psline[linewidth=0.75](10,-25)(10,-37.5)
\rput(10,-17.5){\machine}
\psline[linewidth=0.75](0,25)(20,25)
\psline[linewidth=0.75](0,25)(0,10)
\psline[linewidth=0.75](20,10)(20,25)
\psline[linewidth=0.75](10,40)(10,25)
\psline[linewidth=0.75](0,10)(20,10)
\psline[linewidth=0.75](80,7.5)(100,7.5)
\psline[linewidth=0.75](80,7.5)(80,-7.5)
\psline[linewidth=0.75](100,-7.5)(100,7.5)
\psline[linewidth=0.75](90,22.5)(90,7.5)
\rput[r](87.5,17.5){$\nameslang$}
\rput[r](87.5,-17.5){$\inputt$}
\psline[linewidth=0.75](80,-7.5)(100,-7.5)
\psline[linewidth=0.75](90,-7.5)(90,-22.5)
\rput(90,0){\machine}
\rput[r](7.5,37.5){$\outputt$}
\psline[linewidth=0.75](107.5,7.5)(127.5,7.5)
\psline[linewidth=0.75](107.5,7.5)(107.5,-7.5)
\psline[linewidth=0.75](127.5,-7.5)(127.5,7.5)
\psline[linewidth=0.75](117.5,22.5)(117.5,7.5)
\psline[linewidth=0.75](107.5,-7.5)(127.5,-7.5)
\psline[linewidth=0.75](117.5,-7.5)(117.5,-22.5)
\rput(117.5,0){$\michine$}
\rput[l](120,-20){$\inputtt$}
\rput[l](120,17.5){$\outputtt$}
\rput(10,17.5){$\muchine$}
\end{pspicture}


==> PIC/computation-1.tex <==
%%Created by jPicEdt 1.4.1_03: mixed JPIC-XML/LaTeX format
%%Tue Sep 27 12:23:35 HST 2016
%%Begin JPIC-XML
%<?xml version="1.0" standalone="yes"?>
%<jpic x-min="-10" x-max="240" y-min="-1.25" y-max="120" auto-bounding="true">
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(106.25,50);(106.25,50);(106.25,5);(106.25,5)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(124.38,50);(124.38,50);(124.38,5);(124.38,5)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(96.24,50);(96.24,50);(76.24,70);(76.24,70)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(76.24,70);(76.24,70);(133.75,70);(133.75,70)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(96.24,50);(96.24,50);(133.12,50);(133.12,50)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(133.75,70);(133.75,70);(133.75,50);(133.75,50)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(117.5,88.75);(117.5,88.75);(117.5,70);(117.5,70)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(85.62,60);(85.62,60);(85.62,39.38);(85.62,39.38)"
%	 />
%<text stroke-width= "0.8"
%	 text-vert-align= "center-v"
%	 anchor-point= "(106.25,-1.25)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\Progk$
%</text>
%<text stroke-width= "0.8"
%	 text-vert-align= "center-v"
%	 anchor-point= "(123.75,-1.25)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\Progm$
%</text>
%<text stroke-width= "0.8"
%	 text-vert-align= "center-v"
%	 anchor-point= "(117.5,95)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\Progn$
%</text>
%<text stroke-width= "0.8"
%	 text-vert-align= "center-v"
%	 anchor-point= "(111.25,60)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\universalmkn$
%</text>
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(73.12,26.88);(73.12,26.88);(98.12,26.88);(98.12,26.88)"
%	 />
%<text stroke-width= "0.75"
%	 text-vert-align= "center-v"
%	 anchor-point= "(80.62,33.75)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\program
%</text>
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(73.12,51.88);(73.12,51.88);(98.12,26.88);(98.12,26.88)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(73.12,51.88);(73.12,51.88);(73.12,26.88);(73.12,26.88)"
%	 />
%<text stroke-width= "0.75"
%	 text-vert-align= "center-v"
%	 anchor-point= "(83.12,55.62)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\Progtype$
%</text>
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(10,50);(10,50);(10,5);(10,5)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(29.38,50);(29.38,50);(29.38,5);(29.38,5)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(-0,50);(-0,50);(0,70);(0,70)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(0,70);(0,70);(39.38,70);(39.38,70)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(-0,50);(-0,50);(39.38,50);(39.38,50)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(39.38,70);(39.38,70);(39.38,50);(39.38,50)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(18.12,88.75);(18.12,88.75);(18.12,70);(18.12,70)"
%	 />
%<text stroke-width= "0.8"
%	 text-vert-align= "center-v"
%	 anchor-point= "(10,-1.25)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\Progk$
%</text>
%<text stroke-width= "0.8"
%	 text-vert-align= "center-v"
%	 anchor-point= "(28.75,-0.62)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\Progm$
%</text>
%<text stroke-width= "0.8"
%	 text-vert-align= "center-v"
%	 anchor-point= "(18.12,93.75)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\Progn$
%</text>
%<text stroke-width= "0.75"
%	 text-vert-align= "center-v"
%	 anchor-point= "(55,59.38)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\EQLS
%</text>
%<text stroke-width= "0.8"
%	 text-vert-align= "center-v"
%	 anchor-point= "(20,60)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\gee
%</text>
%<text stroke-width= "0.8"
%	 text-vert-align= "center-v"
%	 anchor-point= "(-10,120)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%\computations
%</text>
%<text stroke-width= "0.8"
%	 text-vert-align= "center-v"
%	 anchor-point= "(95,120)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\programmed
%</text>
%<text stroke-width= "0.8"
%	 text-vert-align= "center-v"
%	 anchor-point= "(240,120)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%\evaluated
%</text>
%</jpic>
%%End JPIC-XML
%PSTricks content-type (pstricks.sty package needed)
%Add \usepackage{pstricks} in the preamble of your LaTeX file
%You can rescale the whole picture (to 80% for instance) by using the command \def\JPicScale{0.8}
\ifx\JPicScale\undefined\def\JPicScale{1}\fi
\psset{unit=\JPicScale mm}
\psset{linewidth=0.3,dotsep=1,hatchwidth=0.3,hatchsep=1.5,shadowsize=1,dimen=middle}
\psset{dotsize=0.7 2.5,dotscale=1 1,fillcolor=black}
\psset{arrowsize=1 2,arrowlength=1,arrowinset=0.25,tbarsize=0.7 5,bracketlength=0.15,rbracketlength=0.15}
\begin{pspicture}(0,0)(240,120)
\psline[linewidth=0.75](106.25,50)(106.25,5)
\psline[linewidth=0.75](124.38,50)(124.38,5)
\psline[linewidth=0.75](96.24,50)(76.24,70)
\psline[linewidth=0.75](76.24,70)(133.75,70)
\psline[linewidth=0.75](96.24,50)(133.12,50)
\psline[linewidth=0.75](133.75,70)(133.75,50)
\psline[linewidth=0.75](117.5,88.75)(117.5,70)
\psline[linewidth=0.75](85.62,60)(85.62,39.38)
\rput(106.25,-1.25){$\Progk$}
\rput(123.75,-1.25){$\Progm$}
\rput(117.5,95){$\Progn$}
\rput(111.25,60){$\universalmkn$}
\psline[linewidth=0.75](73.12,26.88)(98.12,26.88)
\rput(80.62,33.75){\program}
\psline[linewidth=0.75](73.12,51.88)(98.12,26.88)
\psline[linewidth=0.75](73.12,51.88)(73.12,26.88)
\rput[r](83.12,55.62){$\Progtype$}
\psline[linewidth=0.75](10,50)(10,5)
\psline[linewidth=0.75](29.38,50)(29.38,5)
\psline[linewidth=0.75](-0,50)(0,70)
\psline[linewidth=0.75](0,70)(39.38,70)
\psline[linewidth=0.75](-0,50)(39.38,50)
\psline[linewidth=0.75](39.38,70)(39.38,50)
\psline[linewidth=0.75](18.12,88.75)(18.12,70)
\rput(10,-1.25){$\Progk$}
\rput(28.75,-0.62){$\Progm$}
\rput(18.12,93.75){$\Progn$}
\rput(55,59.38){\EQLS}
\rput(20,60){\gee}
\rput[l](-10,120){\computations}
\rput(95,120){\programmed}
\rput[r](240,120){\evaluated}
\end{pspicture}


==> PIC/computation-2.tex <==
%%Created by jPicEdt 1.4.1_03: mixed JPIC-XML/LaTeX format
%%Tue Sep 27 12:22:33 HST 2016
%%Begin JPIC-XML
%<?xml version="1.0" standalone="yes"?>
%<jpic x-min="-10" x-max="240" y-min="-1.25" y-max="120" auto-bounding="true">
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(10,50);(10,50);(10,5);(10,5)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(29.38,50);(29.38,50);(29.38,5);(29.38,5)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(-0,50);(-0,50);(0,70);(0,70)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(0,70);(0,70);(39.38,70);(39.38,70)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(-0,50);(-0,50);(39.38,50);(39.38,50)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(39.38,70);(39.38,70);(39.38,50);(39.38,50)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(18.12,88.75);(18.12,88.75);(18.12,70);(18.12,70)"
%	 />
%<text stroke-width= "0.8"
%	 text-vert-align= "center-v"
%	 anchor-point= "(10,-1.25)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\Progk$
%</text>
%<text stroke-width= "0.8"
%	 text-vert-align= "center-v"
%	 anchor-point= "(29.38,-0.62)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\Progm$
%</text>
%<text stroke-width= "0.8"
%	 text-vert-align= "center-v"
%	 anchor-point= "(18.12,93.75)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\Progn$
%</text>
%<text stroke-width= "0.8"
%	 text-vert-align= "center-v"
%	 anchor-point= "(20,60)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\gee
%</text>
%<text stroke-width= "0.8"
%	 text-vert-align= "center-v"
%	 anchor-point= "(-10,120)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%\computations
%</text>
%<text stroke-width= "0.8"
%	 text-vert-align= "center-v"
%	 anchor-point= "(240,120)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%\evaluated
%</text>
%</jpic>
%%End JPIC-XML
%PSTricks content-type (pstricks.sty package needed)
%Add \usepackage{pstricks} in the preamble of your LaTeX file
%You can rescale the whole picture (to 80% for instance) by using the command \def\JPicScale{0.8}
\ifx\JPicScale\undefined\def\JPicScale{1}\fi
\psset{unit=\JPicScale mm}
\psset{linewidth=0.3,dotsep=1,hatchwidth=0.3,hatchsep=1.5,shadowsize=1,dimen=middle}
\psset{dotsize=0.7 2.5,dotscale=1 1,fillcolor=black}
\psset{arrowsize=1 2,arrowlength=1,arrowinset=0.25,tbarsize=0.7 5,bracketlength=0.15,rbracketlength=0.15}
\begin{pspicture}(0,0)(240,120)
\psline[linewidth=0.75](10,50)(10,5)
\psline[linewidth=0.75](29.38,50)(29.38,5)
\psline[linewidth=0.75](-0,50)(0,70)
\psline[linewidth=0.75](0,70)(39.38,70)
\psline[linewidth=0.75](-0,50)(39.38,50)
\psline[linewidth=0.75](39.38,70)(39.38,50)
\psline[linewidth=0.75](18.12,88.75)(18.12,70)
\rput(10,-1.25){$\Progk$}
\rput(29.38,-0.62){$\Progm$}
\rput(18.12,93.75){$\Progn$}
\rput(20,60){\gee}
\rput[l](-10,120){\computations}
\rput[r](240,120){\evaluated}
\end{pspicture}


==> PIC/computation-H-hat.tex <==
%%Created by jPicEdt 1.4.1_03: mixed JPIC-XML/LaTeX format
%%Fri Dec 27 09:16:36 GMT-10:00 2019
%%Begin JPIC-XML
%<?xml version="1.0" standalone="yes"?>
%<jpic x-min="0" x-max="360" y-min="-5" y-max="99.06" auto-bounding="true">
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(285,35);(285,35);(285,0);(285,0)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(275,35);(275,35);(255,55);(255,55)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(255,55);(255,55);(295,55);(295,55)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(275,35);(275,35);(295,35);(295,35)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(295,55);(295,55);(295,35);(295,35)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(285,90);(285,90);(285,55);(285,55)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(265,45);(265,45);(265,15);(265,15)"
%	 />
%<text fill-style= "none"
%	 stroke-width= "0.8"
%	 text-vert-align= "center-v"
%	 anchor-point= "(265,-5)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\Progk$
%</text>
%<text fill-style= "none"
%	 stroke-width= "0.8"
%	 text-vert-align= "center-v"
%	 anchor-point= "(285,-5)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\Progm$
%</text>
%<text fill-style= "none"
%	 stroke-width= "0.8"
%	 text-vert-align= "center-v"
%	 anchor-point= "(285,95)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\Progn$
%</text>
%<text fill-style= "none"
%	 stroke-width= "0.8"
%	 text-vert-align= "center-v"
%	 anchor-point= "(280,45)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\universalmkn$
%</text>
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(255,5);(255,5);(275,5);(275,5)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(255,25);(255,25);(275,5);(275,5)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(255,25);(255,25);(255,5);(255,5)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(10,35);(10,35);(10,5);(10,5)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(30,35);(30,35);(30,5);(30,5)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(0,35);(0,35);(0,55);(0,55)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(0,55);(0,55);(39.38,55);(39.38,55)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(0,35);(0,35);(39.38,35);(39.38,35)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(39.38,55);(39.38,55);(39.38,35);(39.38,35)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(30,90);(30,90);(30,55);(30,55)"
%	 />
%<text fill-style= "none"
%	 stroke-width= "0.8"
%	 text-vert-align= "center-v"
%	 anchor-point= "(10,0)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\Progk$
%</text>
%<text fill-style= "none"
%	 stroke-width= "0.8"
%	 text-vert-align= "center-v"
%	 anchor-point= "(30,0)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\Progm$
%</text>
%<text fill-style= "none"
%	 stroke-width= "0.8"
%	 text-vert-align= "center-v"
%	 anchor-point= "(30,95)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\Progn$
%</text>
%<text fill-style= "none"
%	 stroke-width= "0.75"
%	 text-vert-align= "center-v"
%	 anchor-point= "(55,44.38)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\EQLS
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(360,-5)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%
%</text>
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(95,35);(95,35);(95,5);(95,5)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(115,35);(115,35);(115,5);(115,5)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(85,35);(85,35);(85,55);(85,55)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(85.62,55);(85.62,55);(125,55);(125,55)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(85,35);(85,35);(124.38,35);(124.38,35)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(125,55);(125,55);(125,35);(125,35)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(115,90);(115,90);(115,55);(115,55)"
%	 />
%<text fill-style= "none"
%	 stroke-width= "0.8"
%	 text-vert-align= "center-v"
%	 anchor-point= "(95,0)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\Progk$
%</text>
%<text fill-style= "none"
%	 stroke-width= "0.8"
%	 text-vert-align= "center-v"
%	 anchor-point= "(115,0)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\Progm$
%</text>
%<text fill-style= "none"
%	 stroke-width= "0.8"
%	 text-vert-align= "center-v"
%	 anchor-point= "(115,95)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\Progn$
%</text>
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(75,50);(75,50);(75,40);(75,40)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(95,70);(95,70);(75,50);(75,50)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(95,20);(95,20);(75,40);(75,40)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(95,80);(95,80);(95,70);(95,70)"
%	 />
%<ellipse fill-style= "solid"
%	 p3= "(96.56,18.44)"
%	 p2= "(96.56,21.56)"
%	 p1= "(93.44,21.56)"
%	 closure= "open"
%	 angle-end= "0"
%	 angle-start= "0"
%	 />
%<ellipse fill-style= "solid"
%	 p3= "(96.56,78.44)"
%	 p2= "(96.56,81.56)"
%	 p1= "(93.44,81.56)"
%	 closure= "open"
%	 angle-end= "0"
%	 angle-start= "0"
%	 />
%<multicurve fill-style= "none"
%	 points= "(70,65);(70,65);(130,65);(130,65)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(70,15);(70,15);(130,15);(130,15)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(130,15);(130,15);(130,65);(130,65)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(70,15);(70,15);(70,65);(70,65)"
%	 />
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(125,23.75)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\geenohat$
%</text>
%<text fill-style= "none"
%	 stroke-width= "0.75"
%	 text-vert-align= "center-v"
%	 anchor-point= "(235,45)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\EQLS
%</text>
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(265,5);(265,5);(265,0);(265,0)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(265,70);(265,70);(265,55);(265,55)"
%	 />
%<ellipse fill-style= "solid"
%	 p3= "(266.56,68.44)"
%	 p2= "(266.56,71.56)"
%	 p1= "(263.44,71.56)"
%	 closure= "open"
%	 angle-end= "0"
%	 angle-start= "0"
%	 />
%<text fill-style= "none"
%	 stroke-width= "0.8"
%	 text-vert-align= "center-v"
%	 anchor-point= "(92.5,75)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\Progk$
%</text>
%<multicurve fill-style= "none"
%	 stroke-color= "#ff0066"
%	 points= "(250,75);(250,75);(300,75);(300,75)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-color= "#ff0066"
%	 points= "(270,30);(270,30);(300,30);(300,30)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-color= "#ff0066"
%	 points= "(300,30);(300,30);(300,75);(300,75)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-color= "#ff0066"
%	 points= "(250,50);(250,50);(250,75);(250,75)"
%	 />
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(295,65)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\ukk$
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(262.5,65)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\RRsmall$
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(267.5,22.5)"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\RRsmall$
%</text>
%<multicurve fill-style= "none"
%	 stroke-color= "#ff0066"
%	 points= "(250,50);(250,50);(270,30);(270,30)"
%	 />
%<text fill-style= "none"
%	 stroke-width= "0.75"
%	 text-vert-align= "center-v"
%	 anchor-point= "(145,44.38)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\EQLS
%</text>
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(185,35);(185,35);(185,5);(185,5)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(205,35);(205,35);(205,5);(205,5)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(175,35);(175,35);(175,55);(175,55)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(175.62,55);(175.62,55);(215,55);(215,55)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(175,35);(175,35);(214.38,35);(214.38,35)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(215,55);(215,55);(215,35);(215,35)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(205,90);(205,90);(205,55);(205,55)"
%	 />
%<text fill-style= "none"
%	 stroke-width= "0.8"
%	 text-vert-align= "center-v"
%	 anchor-point= "(185,0)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\Progk$
%</text>
%<text fill-style= "none"
%	 stroke-width= "0.8"
%	 text-vert-align= "center-v"
%	 anchor-point= "(205,0)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\Progm$
%</text>
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(165,50);(165,50);(165,40);(165,40)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(185,70);(185,70);(165,50);(165,50)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(185,20);(185,20);(165,40);(165,40)"
%	 />
%<ellipse fill-style= "solid"
%	 p3= "(186.56,18.44)"
%	 p2= "(186.56,21.56)"
%	 p1= "(183.44,21.56)"
%	 closure= "open"
%	 angle-end= "0"
%	 angle-start= "0"
%	 />
%<ellipse fill-style= "solid"
%	 p3= "(186.56,95.94)"
%	 p2= "(186.56,99.06)"
%	 p1= "(183.44,99.06)"
%	 closure= "open"
%	 angle-end= "0"
%	 angle-start= "0"
%	 />
%<multicurve fill-style= "none"
%	 points= "(160,65);(160,65);(220,65);(220,65)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(160,15);(160,15);(220,15);(220,15)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(220,15);(220,15);(220,65);(220,65)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(160,15);(160,15);(160,65);(160,65)"
%	 />
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(215,23.75)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\geenohat$
%</text>
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(185,97.5);(185,97.5);(185,85);(185,85)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(175,75);(175,75);(195,75);(195,75)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(175,95);(175,95);(195,75);(195,75)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(175,95);(175,95);(175,75);(175,75)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(185,75);(185,75);(185,70);(185,70)"
%	 />
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(187.5,90)"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\RRsmall$
%</text>
%<text fill-style= "none"
%	 stroke-width= "0.8"
%	 text-vert-align= "center-v"
%	 anchor-point= "(205,95)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\Progn$
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(260,10)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\pprogram
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(20,45)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\ggee
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(105,45)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\ggee
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(195,45)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\ggee
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(180,80)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\pprogram
%</text>
%</jpic>
%%End JPIC-XML
%PSTricks content-type (pstricks.sty package needed)
%Add \usepackage{pstricks} in the preamble of your LaTeX file
%You can rescale the whole picture (to 80% for instance) by using the command \def\JPicScale{0.8}
\ifx\JPicScale\undefined\def\JPicScale{1}\fi
\psset{unit=\JPicScale mm}
\psset{linewidth=0.3,dotsep=1,hatchwidth=0.3,hatchsep=1.5,shadowsize=1,dimen=middle}
\psset{dotsize=0.7 2.5,dotscale=1 1,fillcolor=black}
\psset{arrowsize=1 2,arrowlength=1,arrowinset=0.25,tbarsize=0.7 5,bracketlength=0.15,rbracketlength=0.15}
\begin{pspicture}(0,0)(360,99.06)
\psline[linewidth=0.75](285,35)(285,0)
\psline[linewidth=0.75](275,35)(255,55)
\psline[linewidth=0.75](255,55)(295,55)
\psline[linewidth=0.75](275,35)(295,35)
\psline[linewidth=0.75](295,55)(295,35)
\psline[linewidth=0.75](285,90)(285,55)
\psline[linewidth=0.75](265,45)(265,15)
\rput(265,-5){$\Progk$}
\rput(285,-5){$\Progm$}
\rput(285,95){$\Progn$}
\rput(280,45){$\universalmkn$}
\psline[linewidth=0.75](255,5)(275,5)
\psline[linewidth=0.75](255,25)(275,5)
\psline[linewidth=0.75](255,25)(255,5)
\psline[linewidth=0.75](10,35)(10,5)
\psline[linewidth=0.75](30,35)(30,5)
\psline[linewidth=0.75](0,35)(0,55)
\psline[linewidth=0.75](0,55)(39.38,55)
\psline[linewidth=0.75](0,35)(39.38,35)
\psline[linewidth=0.75](39.38,55)(39.38,35)
\psline[linewidth=0.75](30,90)(30,55)
\rput(10,0){$\Progk$}
\rput(30,0){$\Progm$}
\rput(30,95){$\Progn$}
\rput(55,44.38){\EQLS}
\rput(360,-5){}
\psline[linewidth=0.75](95,35)(95,5)
\psline[linewidth=0.75](115,35)(115,5)
\psline[linewidth=0.75](85,35)(85,55)
\psline[linewidth=0.75](85.62,55)(125,55)
\psline[linewidth=0.75](85,35)(124.38,35)
\psline[linewidth=0.75](125,55)(125,35)
\psline[linewidth=0.75](115,90)(115,55)
\rput(95,0){$\Progk$}
\rput(115,0){$\Progm$}
\rput(115,95){$\Progn$}
\psline[linewidth=0.75](75,50)(75,40)
\psline[linewidth=0.75](95,70)(75,50)
\psline[linewidth=0.75](95,20)(75,40)
\psline[linewidth=0.75](95,80)(95,70)
\rput{0}(95,20){\psellipse[fillstyle=solid](0,0)(1.56,-1.56)}
\rput{0}(95,80){\psellipse[fillstyle=solid](0,0)(1.56,-1.56)}
\psline(70,65)(130,65)
\psline(70,15)(130,15)
\psline(130,15)(130,65)
\psline(70,15)(70,65)
\rput(125,23.75){$\geenohat$}
\rput(235,45){\EQLS}
\psline[linewidth=0.75](265,5)(265,0)
\psline[linewidth=0.75](265,70)(265,55)
\rput{0}(265,70){\psellipse[fillstyle=solid](0,0)(1.56,-1.56)}
\rput[r](92.5,75){$\Progk$}
\newrgbcolor{userLineColour}{1 0 0.4}
\psline[linecolor=userLineColour](250,75)(300,75)
\newrgbcolor{userLineColour}{1 0 0.4}
\psline[linecolor=userLineColour](270,30)(300,30)
\newrgbcolor{userLineColour}{1 0 0.4}
\psline[linecolor=userLineColour](300,30)(300,75)
\newrgbcolor{userLineColour}{1 0 0.4}
\psline[linecolor=userLineColour](250,50)(250,75)
\rput(295,65){$\ukk$}
\rput[r](262.5,65){$\RRsmall$}
\rput[l](267.5,22.5){$\RRsmall$}
\newrgbcolor{userLineColour}{1 0 0.4}
\psline[linecolor=userLineColour](250,50)(270,30)
\rput(145,44.38){\EQLS}
\psline[linewidth=0.75](185,35)(185,5)
\psline[linewidth=0.75](205,35)(205,5)
\psline[linewidth=0.75](175,35)(175,55)
\psline[linewidth=0.75](175.62,55)(215,55)
\psline[linewidth=0.75](175,35)(214.38,35)
\psline[linewidth=0.75](215,55)(215,35)
\psline[linewidth=0.75](205,90)(205,55)
\rput(185,0){$\Progk$}
\rput(205,0){$\Progm$}
\psline[linewidth=0.75](165,50)(165,40)
\psline[linewidth=0.75](185,70)(165,50)
\psline[linewidth=0.75](185,20)(165,40)
\rput{0}(185,20){\psellipse[fillstyle=solid](0,0)(1.56,-1.56)}
\rput{0}(185,97.5){\psellipse[fillstyle=solid](0,0)(1.56,-1.56)}
\psline(160,65)(220,65)
\psline(160,15)(220,15)
\psline(220,15)(220,65)
\psline(160,15)(160,65)
\rput(215,23.75){$\geenohat$}
\psline[linewidth=0.75](185,97.5)(185,85)
\psline[linewidth=0.75](175,75)(195,75)
\psline[linewidth=0.75](175,95)(195,75)
\psline[linewidth=0.75](175,95)(175,75)
\psline[linewidth=0.75](185,75)(185,70)
\rput[l](187.5,90){$\RRsmall$}
\rput(205,95){$\Progn$}
\rput(260,10){\pprogram}
\rput(20,45){\ggee}
\rput(105,45){\ggee}
\rput(195,45){\ggee}
\rput(180,80){\pprogram}
\end{pspicture}


==> PIC/computation-all.tex <==
%%Created by jPicEdt 1.4.1_03: mixed JPIC-XML/LaTeX format
%%Sat Nov 11 12:36:56 HST 2017
%%Begin JPIC-XML
%<?xml version="1.0" standalone="yes"?>
%<jpic x-min="0" x-max="290.63" y-min="-10" y-max="95" auto-bounding="true">
%<multicurve stroke-width= "0.75"
%	 points= "(95,35);(95,35);(95,-10);(95,-10)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.75"
%	 points= "(115,35);(115,35);(115,-10);(115,-10)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.75"
%	 points= "(90,35);(90,35);(70,55);(70,55)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.75"
%	 points= "(70,55);(70,55);(125,55);(125,55)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.75"
%	 points= "(90,35);(90,35);(125,35);(125,35)"
%	 fill-style= "none"
%	 />
%<text text-vert-align= "center-v"
%	 anchor-point= "(140,45)"
%	 stroke-width= "0.75"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\EQLS
%</text>
%<multicurve stroke-width= "0.75"
%	 points= "(125,55);(125,55);(125,35);(125,35)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.75"
%	 points= "(105,75);(105,75);(105,55);(105,55)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.75"
%	 points= "(80,45);(80,45);(80,25);(80,25)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.75"
%	 points= "(170,30);(170,30);(170,15);(170,15)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.75"
%	 points= "(187.5,20);(187.5,20);(187.51,-8.12);(187.51,-8.12)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.75"
%	 points= "(160,40);(160,40);(180,40);(180,40)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.75"
%	 points= "(200,20);(200,20);(180,20);(180,20)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.75"
%	 points= "(200,35);(200,35);(180,55);(180,55)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.75"
%	 points= "(180,40);(180,40);(200,20);(200,20)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.75"
%	 points= "(180,55);(180,55);(214.38,55);(214.38,55)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.75"
%	 points= "(188.75,46.25);(188.75,46.25);(188.75,31.25);(188.75,31.25)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.75"
%	 points= "(200,35);(200,35);(214.38,35);(214.38,35)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.75"
%	 points= "(214.38,55);(214.38,55);(214.38,35);(214.38,35)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.75"
%	 points= "(160,40);(160,40);(180,20);(180,20)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.75"
%	 points= "(200,75);(200,75);(200,55);(200,55)"
%	 fill-style= "none"
%	 />
%<text text-vert-align= "center-v"
%	 anchor-point= "(186.25,42.5)"
%	 stroke-width= "0.75"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\Progtype$
%</text>
%<multicurve stroke-width= "0.75"
%	 points= "(207.5,35);(207.5,35);(207.5,-10);(207.5,-10)"
%	 fill-style= "none"
%	 />
%<text text-vert-align= "center-v"
%	 anchor-point= "(178.74,28.12)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\partial$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(205,45)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\universal$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(95,-7.5)"
%	 stroke-width= "0.8"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\Progk$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(115,-7.5)"
%	 stroke-width= "0.8"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\Progm$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(105,80)"
%	 stroke-width= "0.8"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\Progn$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(200,80)"
%	 stroke-width= "0.8"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\Progn$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(206.25,0)"
%	 stroke-width= "0.8"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\Progm$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(187.5,0)"
%	 stroke-width= "0.8"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\Progk$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(105,45)"
%	 stroke-width= "0.8"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\universalmkn$
%</text>
%<multicurve stroke-width= "0.75"
%	 points= "(160,25);(160,25);(160,5);(160,5)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.75"
%	 points= "(160,5);(160,5);(180,5);(180,5)"
%	 fill-style= "none"
%	 />
%<text text-vert-align= "center-v"
%	 anchor-point= "(167.5,10)"
%	 stroke-width= "0.75"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\program
%</text>
%<multicurve stroke-width= "0.75"
%	 points= "(160,25);(160,25);(180,5);(180,5)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.75"
%	 points= "(70,15);(70,15);(90,15);(90,15)"
%	 fill-style= "none"
%	 />
%<text text-vert-align= "center-v"
%	 anchor-point= "(77.5,20)"
%	 stroke-width= "0.75"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\program
%</text>
%<multicurve stroke-width= "0.75"
%	 points= "(70,35);(70,35);(90,15);(90,15)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.75"
%	 points= "(70,35);(70,35);(70,15);(70,15)"
%	 fill-style= "none"
%	 />
%<text text-vert-align= "center-v"
%	 anchor-point= "(166.88,23.75)"
%	 stroke-width= "0.75"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\Progtype$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(80.62,40.62)"
%	 stroke-width= "0.75"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\Progtype$
%</text>
%<multicurve stroke-width= "0.75"
%	 points= "(30,35);(30,35);(30,5);(30,5)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.75"
%	 points= "(0,35);(0,35);(0,55);(0,55)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.75"
%	 points= "(0,55);(0,55);(40,55);(40,55)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.75"
%	 points= "(0,35);(0,35);(39.38,35);(39.38,35)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.75"
%	 points= "(40,55);(40,55);(40,35);(40,35)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.75"
%	 points= "(20,90);(20,90);(20,55);(20,55)"
%	 fill-style= "none"
%	 />
%<text text-vert-align= "center-v"
%	 anchor-point= "(10,0)"
%	 stroke-width= "0.8"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\Progk$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(30,0)"
%	 stroke-width= "0.8"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\Progm$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(20,95)"
%	 stroke-width= "0.8"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\Progn$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(55,44.38)"
%	 stroke-width= "0.75"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\EQLS
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(20,45)"
%	 stroke-width= "0.8"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\gee
%</text>
%<multicurve stroke-width= "0.75"
%	 points= "(10,35);(10,35);(10,5);(10,5)"
%	 fill-style= "none"
%	 />
%<text text-vert-align= "center-v"
%	 anchor-point= "(228.75,45)"
%	 stroke-width= "0.75"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\EQLS
%</text>
%<multicurve stroke-width= "0.75"
%	 points= "(260,20);(260,20);(260.01,-8.12);(260.01,-8.12)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.75"
%	 points= "(242.5,40);(242.5,40);(256.25,40);(256.25,40)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.75"
%	 points= "(276.25,20);(276.25,20);(242.5,20);(242.5,20)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.75"
%	 points= "(276.25,35);(276.25,35);(256.25,55);(256.25,55)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.75"
%	 points= "(256.25,40);(256.25,40);(276.25,20);(276.25,20)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.75"
%	 points= "(256.25,55);(256.25,55);(290.63,55);(290.63,55)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.75"
%	 points= "(263.75,47.5);(263.75,47.5);(263.75,32.5);(263.75,32.5)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.75"
%	 points= "(276.25,35);(276.25,35);(290.63,35);(290.63,35)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.75"
%	 points= "(290.63,55);(290.63,55);(290.63,35);(290.63,35)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.75"
%	 points= "(276.25,75);(276.25,75);(276.25,55);(276.25,55)"
%	 fill-style= "none"
%	 />
%<text text-vert-align= "center-v"
%	 anchor-point= "(261.25,45)"
%	 stroke-width= "0.75"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\Progtype$
%</text>
%<multicurve stroke-width= "0.75"
%	 points= "(283.75,35);(283.75,35);(283.75,-10);(283.75,-10)"
%	 fill-style= "none"
%	 />
%<text text-vert-align= "center-v"
%	 anchor-point= "(280,45)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\universal$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(276.25,80)"
%	 stroke-width= "0.8"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\Progn$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(282.5,0)"
%	 stroke-width= "0.8"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\Progm$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(260,0)"
%	 stroke-width= "0.8"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\Progk$
%</text>
%<multicurve stroke-width= "0.75"
%	 points= "(242.5,40);(242.5,40);(242.5,20);(242.5,20)"
%	 fill-style= "none"
%	 />
%</jpic>
%%End JPIC-XML
%PSTricks content-type (pstricks.sty package needed)
%Add \usepackage{pstricks} in the preamble of your LaTeX file
%You can rescale the whole picture (to 80% for instance) by using the command \def\JPicScale{0.8}
\ifx\JPicScale\undefined\def\JPicScale{1}\fi
\psset{unit=\JPicScale mm}
\psset{linewidth=0.3,dotsep=1,hatchwidth=0.3,hatchsep=1.5,shadowsize=1,dimen=middle}
\psset{dotsize=0.7 2.5,dotscale=1 1,fillcolor=black}
\psset{arrowsize=1 2,arrowlength=1,arrowinset=0.25,tbarsize=0.7 5,bracketlength=0.15,rbracketlength=0.15}
\begin{pspicture}(0,0)(290.63,95)
\psline[linewidth=0.75](95,35)(95,-10)
\psline[linewidth=0.75](115,35)(115,-10)
\psline[linewidth=0.75](90,35)(70,55)
\psline[linewidth=0.75](70,55)(125,55)
\psline[linewidth=0.75](90,35)(125,35)
\rput(140,45){\EQLS}
\psline[linewidth=0.75](125,55)(125,35)
\psline[linewidth=0.75](105,75)(105,55)
\psline[linewidth=0.75](80,45)(80,25)
\psline[linewidth=0.75](170,30)(170,15)
\psline[linewidth=0.75](187.5,20)(187.51,-8.12)
\psline[linewidth=0.75](160,40)(180,40)
\psline[linewidth=0.75](200,20)(180,20)
\psline[linewidth=0.75](200,35)(180,55)
\psline[linewidth=0.75](180,40)(200,20)
\psline[linewidth=0.75](180,55)(214.38,55)
\psline[linewidth=0.75](188.75,46.25)(188.75,31.25)
\psline[linewidth=0.75](200,35)(214.38,35)
\psline[linewidth=0.75](214.38,55)(214.38,35)
\psline[linewidth=0.75](160,40)(180,20)
\psline[linewidth=0.75](200,75)(200,55)
\rput[r](186.25,42.5){$\Progtype$}
\psline[linewidth=0.75](207.5,35)(207.5,-10)
\rput(178.74,28.12){$\partial$}
\rput(205,45){$\universal$}
\rput(95,-7.5){$\Progk$}
\rput(115,-7.5){$\Progm$}
\rput(105,80){$\Progn$}
\rput(200,80){$\Progn$}
\rput(206.25,0){$\Progm$}
\rput(187.5,0){$\Progk$}
\rput(105,45){$\universalmkn$}
\psline[linewidth=0.75](160,25)(160,5)
\psline[linewidth=0.75](160,5)(180,5)
\rput(167.5,10){\program}
\psline[linewidth=0.75](160,25)(180,5)
\psline[linewidth=0.75](70,15)(90,15)
\rput(77.5,20){\program}
\psline[linewidth=0.75](70,35)(90,15)
\psline[linewidth=0.75](70,35)(70,15)
\rput[r](166.88,23.75){$\Progtype$}
\rput[r](80.62,40.62){$\Progtype$}
\psline[linewidth=0.75](30,35)(30,5)
\psline[linewidth=0.75](0,35)(0,55)
\psline[linewidth=0.75](0,55)(40,55)
\psline[linewidth=0.75](0,35)(39.38,35)
\psline[linewidth=0.75](40,55)(40,35)
\psline[linewidth=0.75](20,90)(20,55)
\rput(10,0){$\Progk$}
\rput(30,0){$\Progm$}
\rput(20,95){$\Progn$}
\rput(55,44.38){\EQLS}
\rput(20,45){\gee}
\psline[linewidth=0.75](10,35)(10,5)
\rput(228.75,45){\EQLS}
\psline[linewidth=0.75](260,20)(260.01,-8.12)
\psline[linewidth=0.75](242.5,40)(256.25,40)
\psline[linewidth=0.75](276.25,20)(242.5,20)
\psline[linewidth=0.75](276.25,35)(256.25,55)
\psline[linewidth=0.75](256.25,40)(276.25,20)
\psline[linewidth=0.75](256.25,55)(290.63,55)
\psline[linewidth=0.75](263.75,47.5)(263.75,32.5)
\psline[linewidth=0.75](276.25,35)(290.63,35)
\psline[linewidth=0.75](290.63,55)(290.63,35)
\psline[linewidth=0.75](276.25,75)(276.25,55)
\rput[r](261.25,45){$\Progtype$}
\psline[linewidth=0.75](283.75,35)(283.75,-10)
\rput(280,45){$\universal$}
\rput(276.25,80){$\Progn$}
\rput(282.5,0){$\Progm$}
\rput(260,0){$\Progk$}
\psline[linewidth=0.75](242.5,40)(242.5,20)
\end{pspicture}


==> PIC/computation-tight.tex <==
%%Created by jPicEdt 1.4.1_03: mixed JPIC-XML/LaTeX format
%%Sat Nov 11 15:59:46 HST 2017
%%Begin JPIC-XML
%<?xml version="1.0" standalone="yes"?>
%<jpic x-min="0" x-max="305" y-min="5" y-max="90" auto-bounding="true">
%<multicurve stroke-width= "0.75"
%	 points= "(100,60);(100,60);(100,30);(100,30)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.75"
%	 points= "(125,60);(125,60);(125,30);(125,30)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.75"
%	 points= "(95,60);(95,60);(75,80);(75,80)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.75"
%	 points= "(75,80);(75,80);(130,80);(130,80)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.75"
%	 points= "(95,60);(95,60);(130,60);(130,60)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.75"
%	 points= "(130,80);(130,80);(130,60);(130,60)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.75"
%	 points= "(110,90);(110,90);(110,80);(110,80)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.75"
%	 points= "(85,70);(85,70);(85,57.5);(85,57.5)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.75"
%	 points= "(167.5,57.5);(167.5,57.5);(167.5,45);(167.5,45)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.75"
%	 points= "(185,47.5);(185,47.5);(185,30);(185,30)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.75"
%	 points= "(157.5,67.5);(157.5,67.5);(177.5,67.5);(177.5,67.5)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.75"
%	 points= "(197.5,47.5);(197.5,47.5);(177.5,47.5);(177.5,47.5)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.75"
%	 points= "(197.5,60);(197.5,60);(177.5,80);(177.5,80)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.75"
%	 points= "(177.5,67.5);(177.5,67.5);(197.5,47.5);(197.5,47.5)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.75"
%	 points= "(177.5,80);(177.5,80);(217.5,80);(217.5,80)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.75"
%	 points= "(187.5,70);(187.5,70);(187.5,57.5);(187.5,57.5)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.75"
%	 points= "(197.5,60);(197.5,60);(217.5,60);(217.5,60)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.75"
%	 points= "(217.5,80);(217.5,80);(217.5,60);(217.5,60)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.75"
%	 points= "(157.5,67.5);(157.5,67.5);(177.5,47.5);(177.5,47.5)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.75"
%	 points= "(197.5,90);(197.5,90);(197.5,80);(197.5,80)"
%	 fill-style= "none"
%	 />
%<text text-vert-align= "center-v"
%	 anchor-point= "(185,67.5)"
%	 stroke-width= "0.75"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\Progtype$
%</text>
%<multicurve stroke-width= "0.75"
%	 points= "(207.5,60);(207.5,60);(207.5,30);(207.5,30)"
%	 fill-style= "none"
%	 />
%<text text-vert-align= "center-v"
%	 anchor-point= "(177.5,57.5)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\partial$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(205,70)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\universal$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(97.5,31.25)"
%	 stroke-width= "0.8"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\Progk$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(120,31.25)"
%	 stroke-width= "0.8"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\Progm$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(112.5,88.75)"
%	 stroke-width= "0.8"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\Progn$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(200,88.75)"
%	 stroke-width= "0.8"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\Progn$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(205,31.25)"
%	 stroke-width= "0.8"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\Progm$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(182.5,31.25)"
%	 stroke-width= "0.8"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\Progk$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(110,70)"
%	 stroke-width= "0.8"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\universalmkn$
%</text>
%<multicurve stroke-width= "0.75"
%	 points= "(157.5,55);(157.5,55);(157.5,35);(157.5,35)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.75"
%	 points= "(157.5,35);(157.5,35);(177.5,35);(177.5,35)"
%	 fill-style= "none"
%	 />
%<text text-vert-align= "center-v"
%	 anchor-point= "(165,40)"
%	 stroke-width= "0.75"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\program
%</text>
%<multicurve stroke-width= "0.75"
%	 points= "(157.5,55);(157.5,55);(177.5,35);(177.5,35)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.75"
%	 points= "(75,47.5);(75,47.5);(95,47.5);(95,47.5)"
%	 fill-style= "none"
%	 />
%<text text-vert-align= "center-v"
%	 anchor-point= "(82.5,52.5)"
%	 stroke-width= "0.75"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\program
%</text>
%<multicurve stroke-width= "0.75"
%	 points= "(75,67.5);(75,67.5);(95,47.5);(95,47.5)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.75"
%	 points= "(75,67.5);(75,67.5);(75,47.5);(75,47.5)"
%	 fill-style= "none"
%	 />
%<text text-vert-align= "center-v"
%	 anchor-point= "(165,55)"
%	 stroke-width= "0.75"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\Progtype$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(82.5,67.5)"
%	 stroke-width= "0.75"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\Progtype$
%</text>
%<multicurve stroke-width= "0.75"
%	 points= "(40,60);(40,60);(40,30);(40,30)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.75"
%	 points= "(0,60);(0,60);(0,80);(0,80)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.75"
%	 points= "(0,80);(0,80);(50,80);(50,80)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.75"
%	 points= "(0,60);(0,60);(50,60);(50,60)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.75"
%	 points= "(50,80);(50,80);(50,60);(50,60)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.75"
%	 points= "(25,88.75);(25,88.75);(25,80);(25,80)"
%	 fill-style= "none"
%	 />
%<text text-vert-align= "center-v"
%	 anchor-point= "(7.5,31.25)"
%	 stroke-width= "0.8"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\Progk$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(37.5,31.25)"
%	 stroke-width= "0.8"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\Progm$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(27.5,88.75)"
%	 stroke-width= "0.8"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\Progn$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(25,70)"
%	 stroke-width= "0.8"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\gee
%</text>
%<multicurve stroke-width= "0.75"
%	 points= "(10,60);(10,60);(10,30);(10,30)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.75"
%	 points= "(292.5,60);(292.5,60);(292.5,30);(292.5,30)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.75"
%	 points= "(245,47.5);(245,47.5);(245,67.5);(245,67.5)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.75"
%	 points= "(265,80);(265,80);(305,80);(305,80)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.75"
%	 points= "(285,60);(285,60);(305,60);(305,60)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.75"
%	 points= "(305,80);(305,80);(305,60);(305,60)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.75"
%	 points= "(287.5,90);(287.5,90);(287.5,80);(287.5,80)"
%	 fill-style= "none"
%	 />
%<text text-vert-align= "center-v"
%	 anchor-point= "(257.5,31.25)"
%	 stroke-width= "0.8"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\Progk$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(290,31.25)"
%	 stroke-width= "0.8"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\Progm$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(290,88.75)"
%	 stroke-width= "0.8"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\Progn$
%</text>
%<multicurve stroke-width= "0.75"
%	 points= "(260,47.5);(260,47.5);(260,30);(260,30)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.75"
%	 points= "(285,60);(285,60);(265,80);(265,80)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.75"
%	 points= "(245,47.5);(245,47.5);(285,47.5);(285,47.5)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.75"
%	 points= "(245,67.5);(245,67.5);(265,67.5);(265,67.5)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.75"
%	 points= "(285,47.5);(285,47.5);(265,67.5);(265,67.5)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.75"
%	 points= "(275,70);(275,70);(275,57.5);(275,57.5)"
%	 fill-style= "none"
%	 />
%<text text-vert-align= "center-v"
%	 anchor-point= "(272.5,67.5)"
%	 stroke-width= "0.75"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\Progtype$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(145,70)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\eqlsb$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(233.75,70)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\eqlsc$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(63.75,70)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\eqlsa$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(291.25,70)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\universal$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(105,5)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\ux$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(200,5)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\sx$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(145,5)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\eqlsb$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(63.75,5)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\eqlsa$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(261.25,57.5)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\Gx$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(25,5)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\gx$
%</text>
%</jpic>
%%End JPIC-XML
%PSTricks content-type (pstricks.sty package needed)
%Add \usepackage{pstricks} in the preamble of your LaTeX file
%You can rescale the whole picture (to 80% for instance) by using the command \def\JPicScale{0.8}
\ifx\JPicScale\undefined\def\JPicScale{1}\fi
\psset{unit=\JPicScale mm}
\psset{linewidth=0.3,dotsep=1,hatchwidth=0.3,hatchsep=1.5,shadowsize=1,dimen=middle}
\psset{dotsize=0.7 2.5,dotscale=1 1,fillcolor=black}
\psset{arrowsize=1 2,arrowlength=1,arrowinset=0.25,tbarsize=0.7 5,bracketlength=0.15,rbracketlength=0.15}
\begin{pspicture}(0,0)(305,90)
\psline[linewidth=0.75](100,60)(100,30)
\psline[linewidth=0.75](125,60)(125,30)
\psline[linewidth=0.75](95,60)(75,80)
\psline[linewidth=0.75](75,80)(130,80)
\psline[linewidth=0.75](95,60)(130,60)
\psline[linewidth=0.75](130,80)(130,60)
\psline[linewidth=0.75](110,90)(110,80)
\psline[linewidth=0.75](85,70)(85,57.5)
\psline[linewidth=0.75](167.5,57.5)(167.5,45)
\psline[linewidth=0.75](185,47.5)(185,30)
\psline[linewidth=0.75](157.5,67.5)(177.5,67.5)
\psline[linewidth=0.75](197.5,47.5)(177.5,47.5)
\psline[linewidth=0.75](197.5,60)(177.5,80)
\psline[linewidth=0.75](177.5,67.5)(197.5,47.5)
\psline[linewidth=0.75](177.5,80)(217.5,80)
\psline[linewidth=0.75](187.5,70)(187.5,57.5)
\psline[linewidth=0.75](197.5,60)(217.5,60)
\psline[linewidth=0.75](217.5,80)(217.5,60)
\psline[linewidth=0.75](157.5,67.5)(177.5,47.5)
\psline[linewidth=0.75](197.5,90)(197.5,80)
\rput[r](185,67.5){$\Progtype$}
\psline[linewidth=0.75](207.5,60)(207.5,30)
\rput(177.5,57.5){$\partial$}
\rput(205,70){$\universal$}
\rput[r](97.5,31.25){$\Progk$}
\rput[r](120,31.25){$\Progm$}
\rput[l](112.5,88.75){$\Progn$}
\rput[l](200,88.75){$\Progn$}
\rput[r](205,31.25){$\Progm$}
\rput[r](182.5,31.25){$\Progk$}
\rput(110,70){$\universalmkn$}
\psline[linewidth=0.75](157.5,55)(157.5,35)
\psline[linewidth=0.75](157.5,35)(177.5,35)
\rput(165,40){\program}
\psline[linewidth=0.75](157.5,55)(177.5,35)
\psline[linewidth=0.75](75,47.5)(95,47.5)
\rput(82.5,52.5){\program}
\psline[linewidth=0.75](75,67.5)(95,47.5)
\psline[linewidth=0.75](75,67.5)(75,47.5)
\rput[r](165,55){$\Progtype$}
\rput[r](82.5,67.5){$\Progtype$}
\psline[linewidth=0.75](40,60)(40,30)
\psline[linewidth=0.75](0,60)(0,80)
\psline[linewidth=0.75](0,80)(50,80)
\psline[linewidth=0.75](0,60)(50,60)
\psline[linewidth=0.75](50,80)(50,60)
\psline[linewidth=0.75](25,88.75)(25,80)
\rput[r](7.5,31.25){$\Progk$}
\rput[r](37.5,31.25){$\Progm$}
\rput[l](27.5,88.75){$\Progn$}
\rput(25,70){\gee}
\psline[linewidth=0.75](10,60)(10,30)
\psline[linewidth=0.75](292.5,60)(292.5,30)
\psline[linewidth=0.75](245,47.5)(245,67.5)
\psline[linewidth=0.75](265,80)(305,80)
\psline[linewidth=0.75](285,60)(305,60)
\psline[linewidth=0.75](305,80)(305,60)
\psline[linewidth=0.75](287.5,90)(287.5,80)
\rput[r](257.5,31.25){$\Progk$}
\rput[r](290,31.25){$\Progm$}
\rput[l](290,88.75){$\Progn$}
\psline[linewidth=0.75](260,47.5)(260,30)
\psline[linewidth=0.75](285,60)(265,80)
\psline[linewidth=0.75](245,47.5)(285,47.5)
\psline[linewidth=0.75](245,67.5)(265,67.5)
\psline[linewidth=0.75](285,47.5)(265,67.5)
\psline[linewidth=0.75](275,70)(275,57.5)
\rput[r](272.5,67.5){$\Progtype$}
\rput(145,70){$\eqlsb$}
\rput(233.75,70){$\eqlsc$}
\rput(63.75,70){$\eqlsa$}
\rput(291.25,70){$\universal$}
\rput(105,5){$\ux$}
\rput(200,5){$\sx$}
\rput(145,5){$\eqlsb$}
\rput(63.75,5){$\eqlsa$}
\rput(261.25,57.5){$\Gx$}
\rput(25,5){$\gx$}
\end{pspicture}


==> PIC/connective.tex <==
%%Created by jPicEdt 1.4.1_03: mixed JPIC-XML/LaTeX format
%%Sat Jun 05 15:40:20 GMT-10:00 2021
%%Begin JPIC-XML
%<?xml version="1.0" standalone="yes"?>
%<jpic x-min="0" x-max="225" y-min="0" y-max="162.5" auto-bounding="true">
%<multicurve fill-style= "none"
%	 points= "(160,152.5);(160,152.5);(225,152.5);(225,152.5)"
%	 stroke-width= "0.2"
%	 />
%<multicurve fill-style= "none"
%	 points= "(167.5,147.5);(167.5,147.5);(217.5,147.5);(217.5,147.5)"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(217.5,127.5);(217.5,127.5);(217.5,147.5);(217.5,147.5)"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(202.5,162.5);(202.5,162.5);(202.5,147.5);(202.5,147.5)"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(187.5,127.5);(187.5,127.5);(217.5,127.5);(217.5,127.5)"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(212.5,127.5);(212.5,127.5);(212.5,90);(212.5,90)"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(192.5,127.5);(192.5,127.5);(192.5,112.5);(192.5,112.5)"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(167.5,147.5);(167.5,147.5);(187.5,127.5);(187.5,127.5)"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(185,105);(185,105);(200,105);(200,105)"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(185,105);(185,105);(185,120);(185,120)"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(185,120);(185,120);(200,105);(200,105)"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(177.5,137.5);(177.5,137.5);(177.5,90);(177.5,90)"
%	 stroke-width= "0.35"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(188.75,108.75)"
%	 text-frame= "noframe"
%	 stroke-width= "0.35"
%	 text-hor-align= "center-h"
%	 >
%$\oone$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(197.5,137.5)"
%	 text-frame= "noframe"
%	 stroke-width= "0.35"
%	 text-hor-align= "center-h"
%	 >
%$\ueval$
%</text>
%<ellipse p3= "(195.08,109.92)"
%	 fill-style= "solid"
%	 p2= "(195.08,115.08)"
%	 fill-color= "#330033"
%	 p1= "(189.92,115.08)"
%	 closure= "open"
%	 angle-end= "0"
%	 stroke-width= "0.35"
%	 angle-start= "0"
%	 />
%<multicurve fill-style= "none"
%	 points= "(160,100);(160,100);(225,100);(225,100)"
%	 stroke-width= "0.2"
%	 />
%<multicurve fill-style= "none"
%	 points= "(160,100);(160,100);(160,152.5);(160,152.5)"
%	 stroke-width= "0.2"
%	 />
%<multicurve fill-style= "none"
%	 points= "(225,100);(225,100);(225,152.5);(225,152.5)"
%	 stroke-width= "0.2"
%	 />
%<multicurve fill-style= "none"
%	 points= "(160,62.5);(160,62.5);(225,62.5);(225,62.5)"
%	 stroke-width= "0.2"
%	 />
%<multicurve fill-style= "none"
%	 points= "(167.5,57.5);(167.5,57.5);(217.5,57.5);(217.5,57.5)"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(217.5,37.5);(217.5,37.5);(217.5,57.5);(217.5,57.5)"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(202.5,75);(202.5,75);(202.5,60);(202.5,60)"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(187.5,37.5);(187.5,37.5);(217.5,37.5);(217.5,37.5)"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(212.5,37.5);(212.5,37.5);(212.5,0);(212.5,0)"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(192.5,37.5);(192.5,37.5);(192.5,22.5);(192.5,22.5)"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(167.5,57.5);(167.5,57.5);(187.5,37.5);(187.5,37.5)"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(185,15);(185,15);(200,15);(200,15)"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(185,15);(185,15);(185,30);(185,30)"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(185,30);(185,30);(200,15);(200,15)"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(177.5,47.5);(177.5,47.5);(177.5,0);(177.5,0)"
%	 stroke-width= "0.35"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(188.75,18.75)"
%	 text-frame= "noframe"
%	 stroke-width= "0.35"
%	 text-hor-align= "center-h"
%	 >
%$\zzero$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(197.5,47.5)"
%	 text-frame= "noframe"
%	 stroke-width= "0.35"
%	 text-hor-align= "center-h"
%	 >
%$\ueval$
%</text>
%<ellipse p3= "(195.08,19.92)"
%	 fill-style= "solid"
%	 p2= "(195.08,25.08)"
%	 fill-color= "#330033"
%	 p1= "(189.92,25.08)"
%	 closure= "open"
%	 angle-end= "0"
%	 stroke-width= "0.35"
%	 angle-start= "0"
%	 />
%<multicurve fill-style= "none"
%	 points= "(160,10);(160,10);(225,10);(225,10)"
%	 stroke-width= "0.2"
%	 />
%<multicurve fill-style= "none"
%	 points= "(160,10);(160,10);(160,62.5);(160,62.5)"
%	 stroke-width= "0.2"
%	 />
%<multicurve fill-style= "none"
%	 points= "(225,10);(225,10);(225,62.5);(225,62.5)"
%	 stroke-width= "0.2"
%	 />
%<multicurve fill-style= "none"
%	 points= "(0,152.5);(0,152.5);(65,152.5);(65,152.5)"
%	 stroke-width= "0.2"
%	 />
%<multicurve fill-style= "none"
%	 points= "(7.5,147.5);(7.5,147.5);(57.5,147.5);(57.5,147.5)"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(57.5,127.5);(57.5,127.5);(57.5,147.5);(57.5,147.5)"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(42.5,162.5);(42.5,162.5);(42.5,147.5);(42.5,147.5)"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(27.5,127.5);(27.5,127.5);(57.5,127.5);(57.5,127.5)"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(32.5,127.5);(32.5,127.5);(32.5,90);(32.5,90)"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(52.5,127.5);(52.5,127.5);(52.5,112.5);(52.5,112.5)"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(7.5,147.5);(7.5,147.5);(27.5,127.5);(27.5,127.5)"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(45,105);(45,105);(60,105);(60,105)"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(45,105);(45,105);(45,120);(45,120)"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(45,120);(45,120);(60,105);(60,105)"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(17.5,137.5);(17.5,137.5);(17.5,90);(17.5,90)"
%	 stroke-width= "0.35"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(48.75,18.75)"
%	 text-frame= "noframe"
%	 stroke-width= "0.35"
%	 text-hor-align= "center-h"
%	 >
%$\oone$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(37.5,137.5)"
%	 text-frame= "noframe"
%	 stroke-width= "0.35"
%	 text-hor-align= "center-h"
%	 >
%$\ueval$
%</text>
%<ellipse p3= "(55.08,109.92)"
%	 fill-style= "solid"
%	 p2= "(55.08,115.08)"
%	 fill-color= "#330033"
%	 p1= "(49.92,115.08)"
%	 closure= "open"
%	 angle-end= "0"
%	 stroke-width= "0.35"
%	 angle-start= "0"
%	 />
%<multicurve fill-style= "none"
%	 points= "(0,100);(0,100);(65,100);(65,100)"
%	 stroke-width= "0.2"
%	 />
%<multicurve fill-style= "none"
%	 points= "(0,100);(0,100);(0,152.5);(0,152.5)"
%	 stroke-width= "0.2"
%	 />
%<multicurve fill-style= "none"
%	 points= "(65,100);(65,100);(65,152.5);(65,152.5)"
%	 stroke-width= "0.2"
%	 />
%<multicurve fill-style= "none"
%	 points= "(0,62.5);(0,62.5);(65,62.5);(65,62.5)"
%	 stroke-width= "0.2"
%	 />
%<multicurve fill-style= "none"
%	 points= "(7.5,57.5);(7.5,57.5);(57.5,57.5);(57.5,57.5)"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(57.5,37.5);(57.5,37.5);(57.5,57.5);(57.5,57.5)"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(42.5,75);(42.5,75);(42.5,60);(42.5,60)"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(27.5,37.5);(27.5,37.5);(57.5,37.5);(57.5,37.5)"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(32.5,37.5);(32.5,37.5);(32.5,0);(32.5,0)"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(52.5,37.5);(52.5,37.5);(52.5,22.5);(52.5,22.5)"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(7.5,57.5);(7.5,57.5);(27.5,37.5);(27.5,37.5)"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(45,15);(45,15);(60,15);(60,15)"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(45,15);(45,15);(45,30);(45,30)"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(45,30);(45,30);(60,15);(60,15)"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(17.5,47.5);(17.5,47.5);(17.5,0);(17.5,0)"
%	 stroke-width= "0.35"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(48.75,108.75)"
%	 text-frame= "noframe"
%	 stroke-width= "0.35"
%	 text-hor-align= "center-h"
%	 >
%$\zzero$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(37.5,47.5)"
%	 text-frame= "noframe"
%	 stroke-width= "0.35"
%	 text-hor-align= "center-h"
%	 >
%$\ueval$
%</text>
%<ellipse p3= "(55.08,19.92)"
%	 fill-style= "solid"
%	 p2= "(55.08,25.08)"
%	 fill-color= "#330033"
%	 p1= "(49.92,25.08)"
%	 closure= "open"
%	 angle-end= "0"
%	 stroke-width= "0.35"
%	 angle-start= "0"
%	 />
%<multicurve fill-style= "none"
%	 points= "(0,10);(0,10);(65,10);(65,10)"
%	 stroke-width= "0.2"
%	 />
%<multicurve fill-style= "none"
%	 points= "(0,10);(0,10);(0,62.5);(0,62.5)"
%	 stroke-width= "0.2"
%	 />
%<multicurve fill-style= "none"
%	 points= "(65,10);(65,10);(65,62.5);(65,62.5)"
%	 stroke-width= "0.2"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(7.5,107.5)"
%	 text-frame= "noframe"
%	 stroke-width= "0.35"
%	 text-hor-align= "center-h"
%	 >
%$\hand$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(167.5,107.5)"
%	 text-frame= "noframe"
%	 stroke-width= "0.35"
%	 text-hor-align= "center-h"
%	 >
%$\hor$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(7.5,17.5)"
%	 text-frame= "noframe"
%	 stroke-width= "0.35"
%	 text-hor-align= "center-h"
%	 >
%$\hthen$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(167.5,17.5)"
%	 text-frame= "noframe"
%	 stroke-width= "0.35"
%	 text-hor-align= "center-h"
%	 >
%$\hxand$
%</text>
%</jpic>
%%End JPIC-XML
%LaTeX-picture environment using emulated lines and arcs
%You can rescale the whole picture (to 80% for instance) by using the command \def\JPicScale{0.8}
\ifx\JPicScale\undefined\def\JPicScale{1}\fi
\unitlength \JPicScale mm
\begin{picture}(225,162.5)(0,0)
\linethickness{0.2mm}
\put(160,152.5){\line(1,0){65}}
\linethickness{0.35mm}
\put(167.5,147.5){\line(1,0){50}}
\linethickness{0.35mm}
\put(217.5,127.5){\line(0,1){20}}
\linethickness{0.35mm}
\put(202.5,147.5){\line(0,1){15}}
\linethickness{0.35mm}
\put(187.5,127.5){\line(1,0){30}}
\linethickness{0.35mm}
\put(212.5,90){\line(0,1){37.5}}
\linethickness{0.35mm}
\put(192.5,112.5){\line(0,1){15}}
\linethickness{0.35mm}
\multiput(167.5,147.5)(0.12,-0.12){167}{\line(1,0){0.12}}
\linethickness{0.35mm}
\put(185,105){\line(1,0){15}}
\linethickness{0.35mm}
\put(185,105){\line(0,1){15}}
\linethickness{0.35mm}
\multiput(185,120)(0.12,-0.12){125}{\line(1,0){0.12}}
\linethickness{0.35mm}
\put(177.5,90){\line(0,1){47.5}}
\put(188.75,108.75){\makebox(0,0)[cc]{$\oone$}}

\put(197.5,137.5){\makebox(0,0)[cc]{$\ueval$}}

\linethickness{0.35mm}
\put(192.5,112.5){\circle*{5.16}}

\linethickness{0.2mm}
\put(160,100){\line(1,0){65}}
\linethickness{0.2mm}
\put(160,100){\line(0,1){52.5}}
\linethickness{0.2mm}
\put(225,100){\line(0,1){52.5}}
\linethickness{0.2mm}
\put(160,62.5){\line(1,0){65}}
\linethickness{0.35mm}
\put(167.5,57.5){\line(1,0){50}}
\linethickness{0.35mm}
\put(217.5,37.5){\line(0,1){20}}
\linethickness{0.35mm}
\put(202.5,60){\line(0,1){15}}
\linethickness{0.35mm}
\put(187.5,37.5){\line(1,0){30}}
\linethickness{0.35mm}
\put(212.5,0){\line(0,1){37.5}}
\linethickness{0.35mm}
\put(192.5,22.5){\line(0,1){15}}
\linethickness{0.35mm}
\multiput(167.5,57.5)(0.12,-0.12){167}{\line(1,0){0.12}}
\linethickness{0.35mm}
\put(185,15){\line(1,0){15}}
\linethickness{0.35mm}
\put(185,15){\line(0,1){15}}
\linethickness{0.35mm}
\multiput(185,30)(0.12,-0.12){125}{\line(1,0){0.12}}
\linethickness{0.35mm}
\put(177.5,0){\line(0,1){47.5}}
\put(188.75,18.75){\makebox(0,0)[cc]{$\zzero$}}

\put(197.5,47.5){\makebox(0,0)[cc]{$\ueval$}}

\linethickness{0.35mm}
\put(192.5,22.5){\circle*{5.16}}

\linethickness{0.2mm}
\put(160,10){\line(1,0){65}}
\linethickness{0.2mm}
\put(160,10){\line(0,1){52.5}}
\linethickness{0.2mm}
\put(225,10){\line(0,1){52.5}}
\linethickness{0.2mm}
\put(0,152.5){\line(1,0){65}}
\linethickness{0.35mm}
\put(7.5,147.5){\line(1,0){50}}
\linethickness{0.35mm}
\put(57.5,127.5){\line(0,1){20}}
\linethickness{0.35mm}
\put(42.5,147.5){\line(0,1){15}}
\linethickness{0.35mm}
\put(27.5,127.5){\line(1,0){30}}
\linethickness{0.35mm}
\put(32.5,90){\line(0,1){37.5}}
\linethickness{0.35mm}
\put(52.5,112.5){\line(0,1){15}}
\linethickness{0.35mm}
\multiput(7.5,147.5)(0.12,-0.12){167}{\line(1,0){0.12}}
\linethickness{0.35mm}
\put(45,105){\line(1,0){15}}
\linethickness{0.35mm}
\put(45,105){\line(0,1){15}}
\linethickness{0.35mm}
\multiput(45,120)(0.12,-0.12){125}{\line(1,0){0.12}}
\linethickness{0.35mm}
\put(17.5,90){\line(0,1){47.5}}
\put(48.75,18.75){\makebox(0,0)[cc]{$\oone$}}

\put(37.5,137.5){\makebox(0,0)[cc]{$\ueval$}}

\linethickness{0.35mm}
\put(52.5,112.5){\circle*{5.16}}

\linethickness{0.2mm}
\put(0,100){\line(1,0){65}}
\linethickness{0.2mm}
\put(0,100){\line(0,1){52.5}}
\linethickness{0.2mm}
\put(65,100){\line(0,1){52.5}}
\linethickness{0.2mm}
\put(0,62.5){\line(1,0){65}}
\linethickness{0.35mm}
\put(7.5,57.5){\line(1,0){50}}
\linethickness{0.35mm}
\put(57.5,37.5){\line(0,1){20}}
\linethickness{0.35mm}
\put(42.5,60){\line(0,1){15}}
\linethickness{0.35mm}
\put(27.5,37.5){\line(1,0){30}}
\linethickness{0.35mm}
\put(32.5,0){\line(0,1){37.5}}
\linethickness{0.35mm}
\put(52.5,22.5){\line(0,1){15}}
\linethickness{0.35mm}
\multiput(7.5,57.5)(0.12,-0.12){167}{\line(1,0){0.12}}
\linethickness{0.35mm}
\put(45,15){\line(1,0){15}}
\linethickness{0.35mm}
\put(45,15){\line(0,1){15}}
\linethickness{0.35mm}
\multiput(45,30)(0.12,-0.12){125}{\line(1,0){0.12}}
\linethickness{0.35mm}
\put(17.5,0){\line(0,1){47.5}}
\put(48.75,108.75){\makebox(0,0)[cc]{$\zzero$}}

\put(37.5,47.5){\makebox(0,0)[cc]{$\ueval$}}

\linethickness{0.35mm}
\put(52.5,22.5){\circle*{5.16}}

\linethickness{0.2mm}
\put(0,10){\line(1,0){65}}
\linethickness{0.2mm}
\put(0,10){\line(0,1){52.5}}
\linethickness{0.2mm}
\put(65,10){\line(0,1){52.5}}
\put(7.5,107.5){\makebox(0,0)[cc]{$\hand$}}

\put(167.5,107.5){\makebox(0,0)[cc]{$\hor$}}

\put(7.5,17.5){\makebox(0,0)[cc]{$\hthen$}}

\put(167.5,17.5){\makebox(0,0)[cc]{$\hxand$}}

\end{picture}


==> PIC/convolution-and-split.tex <==
%%Created by jPicEdt 1.4.1_03: mixed JPIC-XML/LaTeX format
%%Wed Dec 28 22:53:42 GMT-10:00 2022
%%Begin JPIC-XML
%<?xml version="1.0" standalone="yes"?>
%<jpic x-min="0" x-max="227.5" y-min="0" y-max="140" auto-bounding="true">
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(135,52.5)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\Dottt
%</text>
%<multicurve fill-style= "none"
%	 points= "(155,32.5);(155,32.5);(115,32.5);(115,32.5)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(155,32.5);(155,32.5);(115,72.5);(115,72.5)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(115,32.5);(115,32.5);(115,72.5);(115,72.5)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(122.5,122.5);(122.5,122.5);(122.5,107.5);(122.5,107.5)"
%	 stroke-width= "1"
%	 />
%<multicurve fill-style= "none"
%	 points= "(147.5,32.5);(147.5,32.5);(147.5,17.5);(147.5,17.5)"
%	 stroke-width= "1"
%	 />
%<multicurve fill-style= "none"
%	 points= "(130,115);(130,115);(115,130);(115,130)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(115,130);(115,130);(130,130);(130,130)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(130,115);(130,115);(130,130);(130,130)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(135,87.5);(135,87.5);(135,52.5);(135,52.5)"
%	 stroke-width= "1"
%	 />
%<multicurve fill-style= "none"
%	 points= "(155,107.5);(155,107.5);(115,107.5);(115,107.5)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(155,67.5);(155,67.5);(115,107.5);(115,107.5)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(155,67.5);(155,67.5);(155,107.5);(155,107.5)"
%	 />
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(140,99.38)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\projjj$
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(128.12,41.25)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\pairrrr$
%</text>
%<multicurve fill-style= "none"
%	 points= "(122.5,140);(122.5,140);(122.5,130);(122.5,130)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(147.5,122.5);(147.5,122.5);(147.5,107.5);(147.5,107.5)"
%	 stroke-width= "1"
%	 />
%<multicurve fill-style= "none"
%	 points= "(155,115);(155,115);(140,130);(140,130)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(140,130);(140,130);(155,130);(155,130)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(155,115);(155,115);(155,130);(155,130)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(147.5,140);(147.5,140);(147.5,130);(147.5,130)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(155,10);(155,10);(140,25);(140,25)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(140,10);(140,10);(155,10);(155,10)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(140,10);(140,10);(140,25);(140,25)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(147.5,10);(147.5,10);(147.5,0);(147.5,0)"
%	 />
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(147.5,17.5)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\Dottt
%</text>
%<multicurve fill-style= "none"
%	 points= "(122.5,32.5);(122.5,32.5);(122.5,17.5);(122.5,17.5)"
%	 stroke-width= "1"
%	 />
%<multicurve fill-style= "none"
%	 points= "(130,10);(130,10);(115,25);(115,25)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(115,10);(115,10);(130,10);(130,10)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(115,10);(115,10);(115,25);(115,25)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(122.5,10);(122.5,10);(122.5,0);(122.5,0)"
%	 />
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(122.5,17.5)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\Dottt
%</text>
%<multicurve fill-style= "none"
%	 points= "(227.5,140);(227.5,140);(227.5,0);(227.5,0)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(202.5,140);(202.5,140);(202.5,0);(202.5,0)"
%	 />
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(177.5,70)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\EQLZ
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(200,70)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\AAh$
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(225,70)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\BAh$
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(120,1.25)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\AAh$
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(145,1.25)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\BAh$
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(125,138.75)"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\AAh$
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(150,138.75)"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\BAh$
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(125.62,125.62)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\quu$
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(118.75,13.75)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\iih$
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(150.62,125.62)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\quub$
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(144.38,13.75)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\iihb$
%</text>
%<multicurve fill-style= "none"
%	 points= "(20,140);(20,140);(20,115);(20,115)"
%	 stroke-width= "1"
%	 />
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(20,115)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\Dottt
%</text>
%<multicurve fill-style= "none"
%	 points= "(40,95);(40,95);(0,95);(0,95)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(40,95);(40,95);(0,135);(0,135)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(0,95);(0,95);(0,135);(0,135)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(20,25);(20,25);(20,0);(20,0)"
%	 stroke-width= "1"
%	 />
%<multicurve fill-style= "none"
%	 points= "(40,45);(40,45);(0,45);(0,45)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(40,5);(40,5);(0,45);(0,45)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(40,5);(40,5);(40,45);(40,45)"
%	 />
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(25,36.88)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\projjj$
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(13.12,103.75)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\pairrrr$
%</text>
%<multicurve fill-style= "none"
%	 points= "(7.5,57.5);(7.5,57.5);(7.5,45);(7.5,45)"
%	 stroke-width= "1"
%	 />
%<multicurve fill-style= "none"
%	 points= "(15,50);(15,50);(0,65);(0,65)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(0,65);(0,65);(15,65);(15,65)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(15,50);(15,50);(15,65);(15,65)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(7.5,75);(7.5,75);(7.5,65);(7.5,65)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(32.5,57.5);(32.5,57.5);(32.5,45);(32.5,45)"
%	 stroke-width= "1"
%	 />
%<multicurve fill-style= "none"
%	 points= "(40,50);(40,50);(25,65);(25,65)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(25,65);(25,65);(40,65);(40,65)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(40,50);(40,50);(40,65);(40,65)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(32.5,75);(32.5,75);(32.5,65);(32.5,65)"
%	 />
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(10.62,60.62)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\quu$
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(35.62,60.62)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\quub$
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(10,70)"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\AAh$
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(35,70)"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\BAh$
%</text>
%<multicurve fill-style= "none"
%	 points= "(32.5,95);(32.5,95);(32.5,82.5);(32.5,82.5)"
%	 stroke-width= "1"
%	 />
%<multicurve fill-style= "none"
%	 points= "(40,75);(40,75);(25,90);(25,90)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(25,75);(25,75);(40,75);(40,75)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(25,75);(25,75);(25,90);(25,90)"
%	 />
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(32.5,82.5)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\Dottt
%</text>
%<multicurve fill-style= "none"
%	 points= "(7.5,95);(7.5,95);(7.5,82.5);(7.5,82.5)"
%	 stroke-width= "1"
%	 />
%<multicurve fill-style= "none"
%	 points= "(15,75);(15,75);(0,90);(0,90)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(0,75);(0,75);(15,75);(15,75)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(0,75);(0,75);(0,90);(0,90)"
%	 />
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(7.5,82.5)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\Dottt
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(3.75,78.75)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\iih$
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(29.38,78.75)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\iihb$
%</text>
%</jpic>
%%End JPIC-XML
%LaTeX-picture environment using emulated lines and arcs
%You can rescale the whole picture (to 80% for instance) by using the command \def\JPicScale{0.8}
\ifx\JPicScale\undefined\def\JPicScale{1}\fi
\unitlength \JPicScale mm
\begin{picture}(227.5,140)(0,0)
\put(135,52.5){\makebox(0,0)[cc]{\Dottt}}

\linethickness{0.3mm}
\put(115,32.5){\line(1,0){40}}
\linethickness{0.3mm}
\multiput(115,72.5)(0.12,-0.12){333}{\line(1,0){0.12}}
\linethickness{0.3mm}
\put(115,32.5){\line(0,1){40}}
\linethickness{1mm}
\put(122.5,107.5){\line(0,1){15}}
\linethickness{1mm}
\put(147.5,17.5){\line(0,1){15}}
\linethickness{0.3mm}
\multiput(115,130)(0.12,-0.12){125}{\line(1,0){0.12}}
\linethickness{0.3mm}
\put(115,130){\line(1,0){15}}
\linethickness{0.3mm}
\put(130,115){\line(0,1){15}}
\linethickness{1mm}
\put(135,52.5){\line(0,1){35}}
\linethickness{0.3mm}
\put(115,107.5){\line(1,0){40}}
\linethickness{0.3mm}
\multiput(115,107.5)(0.12,-0.12){333}{\line(1,0){0.12}}
\linethickness{0.3mm}
\put(155,67.5){\line(0,1){40}}
\put(140,99.38){\makebox(0,0)[cc]{$\projjj$}}

\put(128.12,41.25){\makebox(0,0)[cc]{$\pairrrr$}}

\linethickness{0.3mm}
\put(122.5,130){\line(0,1){10}}
\linethickness{1mm}
\put(147.5,107.5){\line(0,1){15}}
\linethickness{0.3mm}
\multiput(140,130)(0.12,-0.12){125}{\line(1,0){0.12}}
\linethickness{0.3mm}
\put(140,130){\line(1,0){15}}
\linethickness{0.3mm}
\put(155,115){\line(0,1){15}}
\linethickness{0.3mm}
\put(147.5,130){\line(0,1){10}}
\linethickness{0.3mm}
\multiput(140,25)(0.12,-0.12){125}{\line(1,0){0.12}}
\linethickness{0.3mm}
\put(140,10){\line(1,0){15}}
\linethickness{0.3mm}
\put(140,10){\line(0,1){15}}
\linethickness{0.3mm}
\put(147.5,0){\line(0,1){10}}
\put(147.5,17.5){\makebox(0,0)[cc]{\Dottt}}

\linethickness{1mm}
\put(122.5,17.5){\line(0,1){15}}
\linethickness{0.3mm}
\multiput(115,25)(0.12,-0.12){125}{\line(1,0){0.12}}
\linethickness{0.3mm}
\put(115,10){\line(1,0){15}}
\linethickness{0.3mm}
\put(115,10){\line(0,1){15}}
\linethickness{0.3mm}
\put(122.5,0){\line(0,1){10}}
\put(122.5,17.5){\makebox(0,0)[cc]{\Dottt}}

\linethickness{0.3mm}
\put(227.5,0){\line(0,1){140}}
\linethickness{0.3mm}
\put(202.5,0){\line(0,1){140}}
\put(177.5,70){\makebox(0,0)[cc]{\EQLZ}}

\put(200,70){\makebox(0,0)[cr]{$\AAh$}}

\put(225,70){\makebox(0,0)[cr]{$\BAh$}}

\put(120,1.25){\makebox(0,0)[cr]{$\AAh$}}

\put(145,1.25){\makebox(0,0)[cr]{$\BAh$}}

\put(125,138.75){\makebox(0,0)[cl]{$\AAh$}}

\put(150,138.75){\makebox(0,0)[cl]{$\BAh$}}

\put(125.62,125.62){\makebox(0,0)[cc]{$\quu$}}

\put(118.75,13.75){\makebox(0,0)[cc]{$\iih$}}

\put(150.62,125.62){\makebox(0,0)[cc]{$\quub$}}

\put(144.38,13.75){\makebox(0,0)[cc]{$\iihb$}}

\linethickness{1mm}
\put(20,115){\line(0,1){25}}
\put(20,115){\makebox(0,0)[cc]{\Dottt}}

\linethickness{0.3mm}
\put(0,95){\line(1,0){40}}
\linethickness{0.3mm}
\multiput(0,135)(0.12,-0.12){333}{\line(1,0){0.12}}
\linethickness{0.3mm}
\put(0,95){\line(0,1){40}}
\linethickness{1mm}
\put(20,0){\line(0,1){25}}
\linethickness{0.3mm}
\put(0,45){\line(1,0){40}}
\linethickness{0.3mm}
\multiput(0,45)(0.12,-0.12){333}{\line(1,0){0.12}}
\linethickness{0.3mm}
\put(40,5){\line(0,1){40}}
\put(25,36.88){\makebox(0,0)[cc]{$\projjj$}}

\put(13.12,103.75){\makebox(0,0)[cc]{$\pairrrr$}}

\linethickness{1mm}
\put(7.5,45){\line(0,1){12.5}}
\linethickness{0.3mm}
\multiput(0,65)(0.12,-0.12){125}{\line(1,0){0.12}}
\linethickness{0.3mm}
\put(0,65){\line(1,0){15}}
\linethickness{0.3mm}
\put(15,50){\line(0,1){15}}
\linethickness{0.3mm}
\put(7.5,65){\line(0,1){10}}
\linethickness{1mm}
\put(32.5,45){\line(0,1){12.5}}
\linethickness{0.3mm}
\multiput(25,65)(0.12,-0.12){125}{\line(1,0){0.12}}
\linethickness{0.3mm}
\put(25,65){\line(1,0){15}}
\linethickness{0.3mm}
\put(40,50){\line(0,1){15}}
\linethickness{0.3mm}
\put(32.5,65){\line(0,1){10}}
\put(10.62,60.62){\makebox(0,0)[cc]{$\quu$}}

\put(35.62,60.62){\makebox(0,0)[cc]{$\quub$}}

\put(10,70){\makebox(0,0)[cl]{$\AAh$}}

\put(35,70){\makebox(0,0)[cl]{$\BAh$}}

\linethickness{1mm}
\put(32.5,82.5){\line(0,1){12.5}}
\linethickness{0.3mm}
\multiput(25,90)(0.12,-0.12){125}{\line(1,0){0.12}}
\linethickness{0.3mm}
\put(25,75){\line(1,0){15}}
\linethickness{0.3mm}
\put(25,75){\line(0,1){15}}
\put(32.5,82.5){\makebox(0,0)[cc]{\Dottt}}

\linethickness{1mm}
\put(7.5,82.5){\line(0,1){12.5}}
\linethickness{0.3mm}
\multiput(0,90)(0.12,-0.12){125}{\line(1,0){0.12}}
\linethickness{0.3mm}
\put(0,75){\line(1,0){15}}
\linethickness{0.3mm}
\put(0,75){\line(0,1){15}}
\put(7.5,82.5){\makebox(0,0)[cc]{\Dottt}}

\put(3.75,78.75){\makebox(0,0)[cc]{$\iih$}}

\put(29.38,78.75){\makebox(0,0)[cc]{$\iihb$}}

\end{picture}


==> PIC/convolution-split.tex <==
%%Created by jPicEdt 1.4.1_03: mixed JPIC-XML/LaTeX format
%%Wed Dec 28 22:37:47 GMT-10:00 2022
%%Begin JPIC-XML
%<?xml version="1.0" standalone="yes"?>
%<jpic x-min="0" x-max="112.5" y-min="0" y-max="135" auto-bounding="true">
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(20,52.5)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\Dottt
%</text>
%<multicurve fill-style= "none"
%	 points= "(40,32.5);(40,32.5);(0,32.5);(0,32.5)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(40,32.5);(40,32.5);(0,72.5);(0,72.5)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(0,32.5);(0,32.5);(0,72.5);(0,72.5)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(7.5,117.5);(7.5,117.5);(7.5,102.5);(7.5,102.5)"
%	 stroke-width= "1"
%	 />
%<multicurve fill-style= "none"
%	 points= "(32.5,32.5);(32.5,32.5);(32.5,17.5);(32.5,17.5)"
%	 stroke-width= "1"
%	 />
%<multicurve fill-style= "none"
%	 points= "(15,110);(15,110);(0,125);(0,125)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(0,125);(0,125);(15,125);(15,125)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(15,110);(15,110);(15,125);(15,125)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(20,82.5);(20,82.5);(20,52.5);(20,52.5)"
%	 stroke-width= "1"
%	 />
%<multicurve fill-style= "none"
%	 points= "(40,102.5);(40,102.5);(0,102.5);(0,102.5)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(40,62.5);(40,62.5);(0,102.5);(0,102.5)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(40,62.5);(40,62.5);(40,102.5);(40,102.5)"
%	 />
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(25,94.38)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\projjj$
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(13.12,41.25)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\pairrrr$
%</text>
%<multicurve fill-style= "none"
%	 points= "(7.5,135);(7.5,135);(7.5,125);(7.5,125)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(32.5,117.5);(32.5,117.5);(32.5,102.5);(32.5,102.5)"
%	 stroke-width= "1"
%	 />
%<multicurve fill-style= "none"
%	 points= "(40,110);(40,110);(25,125);(25,125)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(25,125);(25,125);(40,125);(40,125)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(40,110);(40,110);(40,125);(40,125)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(32.5,135);(32.5,135);(32.5,125);(32.5,125)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(40,10);(40,10);(25,25);(25,25)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(25,10);(25,10);(40,10);(40,10)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(25,10);(25,10);(25,25);(25,25)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(32.5,10);(32.5,10);(32.5,0);(32.5,0)"
%	 />
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(32.5,17.5)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\Dottt
%</text>
%<multicurve fill-style= "none"
%	 points= "(7.5,32.5);(7.5,32.5);(7.5,17.5);(7.5,17.5)"
%	 stroke-width= "1"
%	 />
%<multicurve fill-style= "none"
%	 points= "(15,10);(15,10);(0,25);(0,25)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(0,10);(0,10);(15,10);(15,10)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(0,10);(0,10);(0,25);(0,25)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(7.5,10);(7.5,10);(7.5,0);(7.5,0)"
%	 />
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(7.5,17.5)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\Dottt
%</text>
%<multicurve fill-style= "none"
%	 points= "(112.5,135);(112.5,135);(112.5,0);(112.5,0)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(87.5,135);(87.5,135);(87.5,0);(87.5,0)"
%	 />
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(62.5,65)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\EQLZ
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(85,65)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\AAh$
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(110,65)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\BAh$
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(5,1.25)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\AAh$
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(30,1.25)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\BAh$
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(10,133.75)"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\AAh$
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(35,133.75)"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\BAh$
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(10.62,120.62)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\quu$
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(3.75,13.75)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\iih$
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(35.62,120.62)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\quub$
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(29.38,13.75)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\iihb$
%</text>
%</jpic>
%%End JPIC-XML
%LaTeX-picture environment using emulated lines and arcs
%You can rescale the whole picture (to 80% for instance) by using the command \def\JPicScale{0.8}
\ifx\JPicScale\undefined\def\JPicScale{1}\fi
\unitlength \JPicScale mm
\begin{picture}(112.5,135)(0,0)
\put(20,52.5){\makebox(0,0)[cc]{\Dottt}}

\linethickness{0.3mm}
\put(0,32.5){\line(1,0){40}}
\linethickness{0.3mm}
\multiput(0,72.5)(0.12,-0.12){333}{\line(1,0){0.12}}
\linethickness{0.3mm}
\put(0,32.5){\line(0,1){40}}
\linethickness{1mm}
\put(7.5,102.5){\line(0,1){15}}
\linethickness{1mm}
\put(32.5,17.5){\line(0,1){15}}
\linethickness{0.3mm}
\multiput(0,125)(0.12,-0.12){125}{\line(1,0){0.12}}
\linethickness{0.3mm}
\put(0,125){\line(1,0){15}}
\linethickness{0.3mm}
\put(15,110){\line(0,1){15}}
\linethickness{1mm}
\put(20,52.5){\line(0,1){30}}
\linethickness{0.3mm}
\put(0,102.5){\line(1,0){40}}
\linethickness{0.3mm}
\multiput(0,102.5)(0.12,-0.12){333}{\line(1,0){0.12}}
\linethickness{0.3mm}
\put(40,62.5){\line(0,1){40}}
\put(25,94.38){\makebox(0,0)[cc]{$\projjj$}}

\put(13.12,41.25){\makebox(0,0)[cc]{$\pairrrr$}}

\linethickness{0.3mm}
\put(7.5,125){\line(0,1){10}}
\linethickness{1mm}
\put(32.5,102.5){\line(0,1){15}}
\linethickness{0.3mm}
\multiput(25,125)(0.12,-0.12){125}{\line(1,0){0.12}}
\linethickness{0.3mm}
\put(25,125){\line(1,0){15}}
\linethickness{0.3mm}
\put(40,110){\line(0,1){15}}
\linethickness{0.3mm}
\put(32.5,125){\line(0,1){10}}
\linethickness{0.3mm}
\multiput(25,25)(0.12,-0.12){125}{\line(1,0){0.12}}
\linethickness{0.3mm}
\put(25,10){\line(1,0){15}}
\linethickness{0.3mm}
\put(25,10){\line(0,1){15}}
\linethickness{0.3mm}
\put(32.5,0){\line(0,1){10}}
\put(32.5,17.5){\makebox(0,0)[cc]{\Dottt}}

\linethickness{1mm}
\put(7.5,17.5){\line(0,1){15}}
\linethickness{0.3mm}
\multiput(0,25)(0.12,-0.12){125}{\line(1,0){0.12}}
\linethickness{0.3mm}
\put(0,10){\line(1,0){15}}
\linethickness{0.3mm}
\put(0,10){\line(0,1){15}}
\linethickness{0.3mm}
\put(7.5,0){\line(0,1){10}}
\put(7.5,17.5){\makebox(0,0)[cc]{\Dottt}}

\linethickness{0.3mm}
\put(112.5,0){\line(0,1){135}}
\linethickness{0.3mm}
\put(87.5,0){\line(0,1){135}}
\put(62.5,65){\makebox(0,0)[cc]{\EQLZ}}

\put(85,65){\makebox(0,0)[cr]{$\AAh$}}

\put(110,65){\makebox(0,0)[cr]{$\BAh$}}

\put(5,1.25){\makebox(0,0)[cr]{$\AAh$}}

\put(30,1.25){\makebox(0,0)[cr]{$\BAh$}}

\put(10,133.75){\makebox(0,0)[cl]{$\AAh$}}

\put(35,133.75){\makebox(0,0)[cl]{$\BAh$}}

\put(10.62,120.62){\makebox(0,0)[cc]{$\quu$}}

\put(3.75,13.75){\makebox(0,0)[cc]{$\iih$}}

\put(35.62,120.62){\makebox(0,0)[cc]{$\quub$}}

\put(29.38,13.75){\makebox(0,0)[cc]{$\iihb$}}

\end{picture}


==> PIC/convolution.tex <==
%%Created by jPicEdt 1.4.1_03: mixed JPIC-XML/LaTeX format
%%Sun Dec 25 23:14:24 GMT-10:00 2022
%%Begin JPIC-XML
%<?xml version="1.0" standalone="yes"?>
%<jpic x-min="0" x-max="40" y-min="0" y-max="145" auto-bounding="true">
%<multicurve fill-style= "none"
%	 points= "(20,145);(20,145);(20,115);(20,115)"
%	 stroke-width= "1"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(20,115)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\Dottt
%</text>
%<multicurve fill-style= "none"
%	 points= "(40,95);(40,95);(0,95);(0,95)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(40,95);(40,95);(0,135);(0,135)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(0,95);(0,95);(0,135);(0,135)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(5,95);(5,95);(5,80);(5,80)"
%	 stroke-width= "1"
%	 />
%<multicurve fill-style= "none"
%	 points= "(35,65);(35,65);(35,50);(35,50)"
%	 stroke-width= "1"
%	 />
%<multicurve fill-style= "none"
%	 points= "(5,65);(5,65);(5,50);(5,50)"
%	 stroke-width= "1"
%	 />
%<multicurve fill-style= "none"
%	 points= "(35,95);(35,95);(35,80);(35,80)"
%	 stroke-width= "1"
%	 />
%<multicurve fill-style= "none"
%	 points= "(40,75);(40,75);(30,85);(30,85)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(40,60);(40,60);(30,70);(30,70)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(30,70);(30,70);(30,85);(30,85)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(40,60);(40,60);(40,75);(40,75)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(10,75);(10,75);(0,85);(0,85)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(10,60);(10,60);(0,70);(0,70)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(0,70);(0,70);(0,85);(0,85)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(10,60);(10,60);(10,75);(10,75)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(20,30);(20,30);(20,0);(20,0)"
%	 stroke-width= "1"
%	 />
%<multicurve fill-style= "none"
%	 points= "(40,50);(40,50);(0,50);(0,50)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(40,10);(40,10);(0,50);(0,50)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(40,10);(40,10);(40,50);(40,50)"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(25,41.88)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\projjj$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(5,72.5)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\varrhoo$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(35,72.5)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\varsigmaa$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(13.12,103.75)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\pairrrr$
%</text>
%</jpic>
%%End JPIC-XML
%LaTeX-picture environment using emulated lines and arcs
%You can rescale the whole picture (to 80% for instance) by using the command \def\JPicScale{0.8}
\ifx\JPicScale\undefined\def\JPicScale{1}\fi
\unitlength \JPicScale mm
\begin{picture}(40,145)(0,0)
\linethickness{1mm}
\put(20,115){\line(0,1){30}}
\put(20,115){\makebox(0,0)[cc]{\Dottt}}

\linethickness{0.3mm}
\put(0,95){\line(1,0){40}}
\linethickness{0.3mm}
\multiput(0,135)(0.12,-0.12){333}{\line(1,0){0.12}}
\linethickness{0.3mm}
\put(0,95){\line(0,1){40}}
\linethickness{1mm}
\put(5,80){\line(0,1){15}}
\linethickness{1mm}
\put(35,50){\line(0,1){15}}
\linethickness{1mm}
\put(5,50){\line(0,1){15}}
\linethickness{1mm}
\put(35,80){\line(0,1){15}}
\linethickness{0.3mm}
\multiput(30,85)(0.12,-0.12){83}{\line(1,0){0.12}}
\linethickness{0.3mm}
\multiput(30,70)(0.12,-0.12){83}{\line(1,0){0.12}}
\linethickness{0.3mm}
\put(30,70){\line(0,1){15}}
\linethickness{0.3mm}
\put(40,60){\line(0,1){15}}
\linethickness{0.3mm}
\multiput(0,85)(0.12,-0.12){83}{\line(1,0){0.12}}
\linethickness{0.3mm}
\multiput(0,70)(0.12,-0.12){83}{\line(1,0){0.12}}
\linethickness{0.3mm}
\put(0,70){\line(0,1){15}}
\linethickness{0.3mm}
\put(10,60){\line(0,1){15}}
\linethickness{1mm}
\put(20,0){\line(0,1){30}}
\linethickness{0.3mm}
\put(0,50){\line(1,0){40}}
\linethickness{0.3mm}
\multiput(0,50)(0.12,-0.12){333}{\line(1,0){0.12}}
\linethickness{0.3mm}
\put(40,10){\line(0,1){40}}
\put(25,41.88){\makebox(0,0)[cc]{$\projjj$}}

\put(5,72.5){\makebox(0,0)[cc]{$\varrhoo$}}

\put(35,72.5){\makebox(0,0)[cc]{$\varsigmaa$}}

\put(13.12,103.75){\makebox(0,0)[cc]{$\pairrrr$}}

\end{picture}


==> PIC/coper-add-def.tex <==
%%Created by jPicEdt 1.4.1_03: mixed JPIC-XML/LaTeX format
%%Sun Aug 21 15:30:06 GMT-10:00 2022
%%Begin JPIC-XML
%<?xml version="1.0" standalone="yes"?>
%<jpic x-min="0" x-max="160" y-min="0" y-max="97.5" auto-bounding="true">
%<multicurve fill-style= "none"
%	 points= "(112.5,40);(112.5,40);(160,40);(160,40)"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(160,20);(160,20);(160,40);(160,40)"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(155,67.5);(155,67.5);(155,40);(155,40)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(132.5,20);(132.5,20);(160,20);(160,20)"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(155,20);(155,20);(155,0);(155,0)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(135,20.01);(135,20.01);(135,0);(135,0)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(112.5,40);(112.5,40);(132.5,20);(132.5,20)"
%	 stroke-width= "0.35"
%	 />
%<ellipse p3= "(137.58,7.42)"
%	 fill-style= "solid"
%	 p2= "(137.58,12.58)"
%	 fill-color= "#330033"
%	 p1= "(132.42,12.58)"
%	 closure= "open"
%	 angle-end= "0"
%	 angle-start= "0"
%	 />
%<multicurve fill-style= "none"
%	 points= "(130,62.5);(130,62.5);(106.25,38.75);(106.25,38.75)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(106.25,38.75);(106.25,38.75);(135,10);(135,10)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(105,87.5);(105,87.5);(160,87.5);(160,87.5)"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(160,67.5);(160,67.5);(160,87.5);(160,87.5)"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(150,97.5);(150,97.5);(150,87.5);(150,87.5)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(125,67.5);(125,67.5);(160,67.5);(160,67.5)"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(130,67.5);(130,67.5);(130,62.5);(130,62.5)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(105,87.5);(105,87.5);(125,67.5);(125,67.5)"
%	 stroke-width= "0.35"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(80,67.5)"
%	 text-frame= "noframe"
%	 stroke-width= "0.75"
%	 text-hor-align= "center-h"
%	 >
%\EQLS
%</text>
%<multicurve fill-style= "none"
%	 points= "(5,87.5);(5,87.5);(55,87.5);(55,87.5)"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(55,67.5);(55,67.5);(55,87.5);(55,87.5)"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(40,97.5);(40,97.5);(40,87.5);(40,87.5)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(25,67.5);(25,67.5);(55,67.5);(55,67.5)"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(50,67.5);(50,67.5);(50,0);(50,0)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(15,77.5);(15,77.5);(10,72.5);(10,72.5)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(5,87.5);(5,87.5);(25,67.5);(25,67.5)"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(30,67.5);(30,67.5);(30,0);(30,0)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(100,62.5);(100,62.5);(100,0);(100,0)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(0,62.5);(0,62.5);(0,82.5);(0,82.5)"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(0,82.5);(0,82.5);(20,62.5);(20,62.5)"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(0,62.5);(0,62.5);(20,62.5);(20,62.5)"
%	 stroke-width= "0.35"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(5,66.25)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\suces$
%</text>
%<multicurve fill-style= "none"
%	 points= "(5,62.5);(5,62.5);(5,0);(5,0)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(15,62.5);(15,62.5);(15,0);(15,0)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(115,77.5);(115,77.5);(100,62.5);(100,62.5)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 stroke-overstrike-width= "1"
%	 points= "(122.5,30);(122.5,30);(112.5,20);(112.5,20)"
%	 stroke-overstrike= "true"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(112.5,20);(112.5,20);(112.5,0);(112.5,0)"
%	 stroke-width= "0.75"
%	 />
%<ellipse p3= "(11.33,69.92)"
%	 fill-style= "solid"
%	 p2= "(11.33,75.08)"
%	 fill-color= "#330033"
%	 p1= "(6.17,75.08)"
%	 closure= "open"
%	 angle-end= "0"
%	 angle-start= "0"
%	 />
%</jpic>
%%End JPIC-XML
%LaTeX-picture environment using emulated lines and arcs
%You can rescale the whole picture (to 80% for instance) by using the command \def\JPicScale{0.8}
\ifx\JPicScale\undefined\def\JPicScale{1}\fi
\unitlength \JPicScale mm
\begin{picture}(160,97.5)(0,0)
\linethickness{0.35mm}
\put(112.5,40){\line(1,0){47.5}}
\linethickness{0.35mm}
\put(160,20){\line(0,1){20}}
\linethickness{0.75mm}
\put(155,40){\line(0,1){27.5}}
\linethickness{0.35mm}
\put(132.5,20){\line(1,0){27.5}}
\linethickness{0.75mm}
\put(155,0){\line(0,1){20}}
\linethickness{0.75mm}
\put(135,0){\line(0,1){20.01}}
\linethickness{0.35mm}
\multiput(112.5,40)(0.12,-0.12){167}{\line(1,0){0.12}}
\linethickness{0.3mm}
\put(135,10){\circle*{5.16}}

\linethickness{0.75mm}
\multiput(106.25,38.75)(0.12,0.12){198}{\line(1,0){0.12}}
\linethickness{0.75mm}
\multiput(106.25,38.75)(0.12,-0.12){240}{\line(1,0){0.12}}
\linethickness{0.35mm}
\put(105,87.5){\line(1,0){55}}
\linethickness{0.35mm}
\put(160,67.5){\line(0,1){20}}
\linethickness{0.75mm}
\put(150,87.5){\line(0,1){10}}
\linethickness{0.35mm}
\put(125,67.5){\line(1,0){35}}
\linethickness{0.75mm}
\put(130,62.5){\line(0,1){5}}
\linethickness{0.35mm}
\multiput(105,87.5)(0.12,-0.12){167}{\line(1,0){0.12}}
\put(80,67.5){\makebox(0,0)[cc]{\EQLS}}

\linethickness{0.35mm}
\put(5,87.5){\line(1,0){50}}
\linethickness{0.35mm}
\put(55,67.5){\line(0,1){20}}
\linethickness{0.75mm}
\put(40,87.5){\line(0,1){10}}
\linethickness{0.35mm}
\put(25,67.5){\line(1,0){30}}
\linethickness{0.75mm}
\put(50,0){\line(0,1){67.5}}
\linethickness{0.75mm}
\multiput(10,72.5)(0.12,0.12){42}{\line(1,0){0.12}}
\linethickness{0.35mm}
\multiput(5,87.5)(0.12,-0.12){167}{\line(1,0){0.12}}
\linethickness{0.75mm}
\put(30,0){\line(0,1){67.5}}
\linethickness{0.75mm}
\put(100,0){\line(0,1){62.5}}
\linethickness{0.35mm}
\put(0,62.5){\line(0,1){20}}
\linethickness{0.35mm}
\multiput(0,82.5)(0.12,-0.12){167}{\line(1,0){0.12}}
\linethickness{0.35mm}
\put(0,62.5){\line(1,0){20}}
\put(5,66.25){\makebox(0,0)[cc]{$\suces$}}

\linethickness{0.75mm}
\put(5,0){\line(0,1){62.5}}
\linethickness{0.75mm}
\put(15,0){\line(0,1){62.5}}
\linethickness{0.75mm}
\multiput(100,62.5)(0.12,0.12){125}{\line(1,0){0.12}}
\linethickness{0.75mm}
\multiput(112.5,20)(0.12,0.12){83}{\line(1,0){0.12}}
\linethickness{0.75mm}
\put(112.5,0){\line(0,1){20}}
\linethickness{0.3mm}
\put(8.75,72.5){\circle*{5.16}}

\end{picture}


==> PIC/coper-add-prop.tex <==
%%Created by jPicEdt 1.4.1_03: mixed JPIC-XML/LaTeX format
%%Thu Oct 20 16:49:20 HST 2016
%%Begin JPIC-XML
%<?xml version="1.0" standalone="yes"?>
%<jpic x-min="-3.75" x-max="160" y-min="-11.25" y-max="70" auto-bounding="true">
%<multicurve stroke-width= "0.75"
%	 points= "(150,40);(150,40);(150,-10);(150,-10)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.75"
%	 points= "(105,60);(105,60);(160,60);(160,60)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.75"
%	 points= "(160,40);(160,40);(160,60);(160,60)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.75"
%	 points= "(150,70);(150,70);(150,60);(150,60)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.75"
%	 points= "(125,40);(125,40);(160,40);(160,40)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.75"
%	 points= "(130,40);(130,40);(130,-11.25);(130,-11.25)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.75"
%	 points= "(105,60);(105,60);(125,40);(125,40)"
%	 fill-style= "none"
%	 />
%<text text-vert-align= "center-v"
%	 stroke-width= "0.75"
%	 anchor-point= "(81.25,40)"
%	 text-frame= "noframe"
%	 fill-style= "none"
%	 text-hor-align= "center-h"
%	 >
%\EQLS
%</text>
%<multicurve stroke-width= "0.75"
%	 points= "(5,60);(5,60);(55,60);(55,60)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.75"
%	 points= "(55,40);(55,40);(55,60);(55,60)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.75"
%	 points= "(40,70);(40,70);(40,60);(40,60)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.75"
%	 points= "(25,40);(25,40);(55,40);(55,40)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.75"
%	 points= "(50,40);(50,40);(50,-10);(50,-10)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.75"
%	 points= "(15,50);(15,50);(10,45);(10,45)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.75"
%	 points= "(5,60);(5,60);(25,40);(25,40)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.75"
%	 points= "(30,40);(30,40);(30,-10);(30,-10)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.75"
%	 points= "(115,50);(115,50);(115,17.5);(115,17.5)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.75"
%	 points= "(0,35);(0,35);(0,55);(0,55)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.75"
%	 points= "(0,55);(0,55);(20,35);(20,35)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.75"
%	 points= "(0,35);(0,35);(20,15);(20,15)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.75"
%	 points= "(20,15);(20,15);(20,35);(20,35)"
%	 fill-style= "none"
%	 />
%<text text-vert-align= "center-v"
%	 anchor-point= "(10,35)"
%	 text-frame= "noframe"
%	 fill-style= "none"
%	 text-hor-align= "center-h"
%	 >
%$\suces$
%</text>
%<multicurve stroke-width= "0.75"
%	 points= "(100,5);(100,5);(127.5,5);(127.5,5)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.75"
%	 points= "(100,5);(100,5);(100,32.5);(100,32.5)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.75"
%	 points= "(100,32.5);(100,32.5);(127.5,5);(127.5,5)"
%	 fill-style= "none"
%	 />
%<text text-vert-align= "center-v"
%	 anchor-point= "(109.38,11.88)"
%	 text-frame= "noframe"
%	 fill-style= "none"
%	 text-hor-align= "center-h"
%	 >
%$\enplus$
%</text>
%<multicurve stroke-width= "0.75"
%	 points= "(15,20);(15,20);(15,2.5);(15,2.5)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.75"
%	 points= "(7.5,-5);(7.5,-5);(22.5,-5);(22.5,-5)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.75"
%	 points= "(7.5,-5);(7.5,-5);(7.5,10);(7.5,10)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.75"
%	 points= "(7.5,10);(7.5,10);(22.5,-5);(22.5,-5)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.75"
%	 points= "(3.75,31.25);(3.75,31.25);(3.75,21.25);(3.75,21.25)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.75"
%	 points= "(-3.75,13.75);(-3.75,13.75);(11.25,13.75);(11.25,13.75)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.75"
%	 points= "(-3.75,13.75);(-3.75,13.75);(-3.75,28.75);(-3.75,28.75)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.75"
%	 points= "(-3.75,28.75);(-3.75,28.75);(11.25,13.75);(11.25,13.75)"
%	 fill-style= "none"
%	 />
%<text text-vert-align= "center-v"
%	 anchor-point= "(0,17.5)"
%	 text-frame= "noframe"
%	 fill-style= "none"
%	 text-hor-align= "center-h"
%	 >
%$\een$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(12.5,-1.25)"
%	 text-frame= "noframe"
%	 fill-style= "none"
%	 text-hor-align= "center-h"
%	 >
%$\mee$
%</text>
%</jpic>
%%End JPIC-XML
%PSTricks content-type (pstricks.sty package needed)
%Add \usepackage{pstricks} in the preamble of your LaTeX file
%You can rescale the whole picture (to 80% for instance) by using the command \def\JPicScale{0.8}
\ifx\JPicScale\undefined\def\JPicScale{1}\fi
\psset{unit=\JPicScale mm}
\psset{linewidth=0.3,dotsep=1,hatchwidth=0.3,hatchsep=1.5,shadowsize=1,dimen=middle}
\psset{dotsize=0.7 2.5,dotscale=1 1,fillcolor=black}
\psset{arrowsize=1 2,arrowlength=1,arrowinset=0.25,tbarsize=0.7 5,bracketlength=0.15,rbracketlength=0.15}
\begin{pspicture}(0,0)(160,70)
\psline[linewidth=0.75](150,40)(150,-10)
\psline[linewidth=0.75](105,60)(160,60)
\psline[linewidth=0.75](160,40)(160,60)
\psline[linewidth=0.75](150,70)(150,60)
\psline[linewidth=0.75](125,40)(160,40)
\psline[linewidth=0.75](130,40)(130,-11.25)
\psline[linewidth=0.75](105,60)(125,40)
\rput(81.25,40){\EQLS}
\psline[linewidth=0.75](5,60)(55,60)
\psline[linewidth=0.75](55,40)(55,60)
\psline[linewidth=0.75](40,70)(40,60)
\psline[linewidth=0.75](25,40)(55,40)
\psline[linewidth=0.75](50,40)(50,-10)
\psline[linewidth=0.75](15,50)(10,45)
\psline[linewidth=0.75](5,60)(25,40)
\psline[linewidth=0.75](30,40)(30,-10)
\psline[linewidth=0.75](115,50)(115,17.5)
\psline[linewidth=0.75](0,35)(0,55)
\psline[linewidth=0.75](0,55)(20,35)
\psline[linewidth=0.75](0,35)(20,15)
\psline[linewidth=0.75](20,15)(20,35)
\rput(10,35){$\suces$}
\psline[linewidth=0.75](100,5)(127.5,5)
\psline[linewidth=0.75](100,5)(100,32.5)
\psline[linewidth=0.75](100,32.5)(127.5,5)
\rput(109.38,11.88){$\enplus$}
\psline[linewidth=0.75](15,20)(15,2.5)
\psline[linewidth=0.75](7.5,-5)(22.5,-5)
\psline[linewidth=0.75](7.5,-5)(7.5,10)
\psline[linewidth=0.75](7.5,10)(22.5,-5)
\psline[linewidth=0.75](3.75,31.25)(3.75,21.25)
\psline[linewidth=0.75](-3.75,13.75)(11.25,13.75)
\psline[linewidth=0.75](-3.75,13.75)(-3.75,28.75)
\psline[linewidth=0.75](-3.75,28.75)(11.25,13.75)
\rput(0,17.5){$\een$}
\rput(12.5,-1.25){$\mee$}
\end{pspicture}


==> PIC/coper-exp-def.tex <==
%%Created by jPicEdt 1.4.1_03: mixed JPIC-XML/LaTeX format
%%Sun Oct 23 19:52:35 HST 2016
%%Begin JPIC-XML
%<?xml version="1.0" standalone="yes"?>
%<jpic x-min="0" x-max="158.75" y-min="0" y-max="61.25" auto-bounding="true">
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(90,45);(90,45);(110,45);(110,45)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(155,30);(155,30);(155,0);(155,0)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(110,25);(110,25);(130,25);(130,25)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(120,25.01);(120,25.01);(120,0);(120,0)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(115,50);(115,50);(158.75,50);(158.75,50)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(158.75,30);(158.75,30);(158.75,50);(158.75,50)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(147.5,61.25);(147.5,61.25);(147.5,50);(147.5,50)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(135,30);(135,30);(158.75,30);(158.75,30)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(140,30);(140,30);(140,0);(140,0)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(115,50);(115,50);(135,30);(135,30)"
%	 />
%<text stroke-width= "0.75"
%	 text-vert-align= "center-v"
%	 anchor-point= "(70,40)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\EQLS
%</text>
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(5,50);(5,50);(50,50);(50,50)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(50,30);(50,30);(50,50);(50,50)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(40,61.25);(40,61.25);(40,50);(40,50)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(25,30);(25,30);(50,30);(50,30)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(45,30);(45,30);(45,0);(45,0)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(15,40);(15,40);(10,35);(10,35)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(5,50);(5,50);(25,30);(25,30)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(30,30);(30,30);(30,0);(30,0)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(0,25);(0,25);(0,45);(0,45)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(0,45);(0,45);(20,25);(20,25)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(0,25);(0,25);(20,5);(20,5)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(20,5);(20,5);(20,25);(20,25)"
%	 />
%<text text-vert-align= "center-v"
%	 anchor-point= "(10,25)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\suces$
%</text>
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(5,20);(5,20);(5,0);(5,0)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(15,10);(15,10);(15,0);(15,0)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(125,40);(125,40);(120,35);(120,35)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(100,35);(100,35);(100,0);(100,0)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(110,45);(110,45);(130,25);(130,25)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(90,45);(90,45);(110,25);(110,25)"
%	 />
%</jpic>
%%End JPIC-XML
%PSTricks content-type (pstricks.sty package needed)
%Add \usepackage{pstricks} in the preamble of your LaTeX file
%You can rescale the whole picture (to 80% for instance) by using the command \def\JPicScale{0.8}
\ifx\JPicScale\undefined\def\JPicScale{1}\fi
\psset{unit=\JPicScale mm}
\psset{linewidth=0.3,dotsep=1,hatchwidth=0.3,hatchsep=1.5,shadowsize=1,dimen=middle}
\psset{dotsize=0.7 2.5,dotscale=1 1,fillcolor=black}
\psset{arrowsize=1 2,arrowlength=1,arrowinset=0.25,tbarsize=0.7 5,bracketlength=0.15,rbracketlength=0.15}
\begin{pspicture}(0,0)(158.75,61.25)
\psline[linewidth=0.75](90,45)(110,45)
\psline[linewidth=0.75](155,30)(155,0)
\psline[linewidth=0.75](110,25)(130,25)
\psline[linewidth=0.75](120,25.01)(120,0)
\psline[linewidth=0.75](115,50)(158.75,50)
\psline[linewidth=0.75](158.75,30)(158.75,50)
\psline[linewidth=0.75](147.5,61.25)(147.5,50)
\psline[linewidth=0.75](135,30)(158.75,30)
\psline[linewidth=0.75](140,30)(140,0)
\psline[linewidth=0.75](115,50)(135,30)
\rput(70,40){\EQLS}
\psline[linewidth=0.75](5,50)(50,50)
\psline[linewidth=0.75](50,30)(50,50)
\psline[linewidth=0.75](40,61.25)(40,50)
\psline[linewidth=0.75](25,30)(50,30)
\psline[linewidth=0.75](45,30)(45,0)
\psline[linewidth=0.75](15,40)(10,35)
\psline[linewidth=0.75](5,50)(25,30)
\psline[linewidth=0.75](30,30)(30,0)
\psline[linewidth=0.75](0,25)(0,45)
\psline[linewidth=0.75](0,45)(20,25)
\psline[linewidth=0.75](0,25)(20,5)
\psline[linewidth=0.75](20,5)(20,25)
\rput(10,25){$\suces$}
\psline[linewidth=0.75](5,20)(5,0)
\psline[linewidth=0.75](15,10)(15,0)
\psline[linewidth=0.75](125,40)(120,35)
\psline[linewidth=0.75](100,35)(100,0)
\psline[linewidth=0.75](110,45)(130,25)
\psline[linewidth=0.75](90,45)(110,25)
\end{pspicture}


==> PIC/coper-exp-defexp.tex <==
%%Created by jPicEdt 1.4.1_03: mixed JPIC-XML/LaTeX format
%%Sun Oct 23 19:29:17 HST 2016
%%Begin JPIC-XML
%<?xml version="1.0" standalone="yes"?>
%<jpic x-min="-10" x-max="280" y-min="0" y-max="165" auto-bounding="true">
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(150,115);(150,115);(170,115);(170,115)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(195,110);(195,110);(195,60);(195,60)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(170.62,95);(170.62,95);(190,95);(190,95)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(180,95);(180,95);(180,80);(180,80)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(160,105.01);(160,105.01);(142.5,87.5);(142.5,87.5)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(150,115);(150,115);(170,95);(170,95)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(170,130);(170,130);(200,130);(200,130)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(200,110);(200,110);(200,130);(200,130)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(195,140);(195,140);(195,130);(195,130)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(190.62,110);(190.62,110);(200,110);(200,110)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(180,120.01);(180,120.01);(180,105);(180,105)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(170,130);(170,130);(190,110);(190,110)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(30,100);(30,100);(30,60);(30,60)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(10.62,80.01);(10.62,80.01);(10.62,60);(10.62,60)"
%	 />
%<ellipse p3= "(13.2,77.42)"
%	 p2= "(13.2,82.58)"
%	 p1= "(8.05,82.58)"
%	 closure= "open"
%	 fill-style= "solid"
%	 angle-end= "0"
%	 fill-color= "#330033"
%	 angle-start= "0"
%	 />
%<multicurve stroke-width= "0.6"
%	 fill-style= "none"
%	 points= "(0,90);(0,90);(40,90);(40,90)"
%	 />
%<multicurve stroke-width= "0.6"
%	 fill-style= "none"
%	 points= "(40,70);(40,70);(40,90);(40,90)"
%	 />
%<multicurve stroke-width= "0.6"
%	 fill-style= "none"
%	 points= "(0,70);(0,70);(40,70);(40,70)"
%	 />
%<multicurve stroke-width= "0.6"
%	 fill-style= "none"
%	 points= "(0,90);(0,90);(0,70);(0,70)"
%	 />
%<text stroke-width= "0.75"
%	 text-vert-align= "center-v"
%	 anchor-point= "(20,50)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\EQLS
%</text>
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(70,30);(70,30);(120,30);(120,30)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(120,10);(120,10);(120,30);(120,30)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(105,40);(105,40);(105,30);(105,30)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(90,10);(90,10);(120,10);(120,10)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(115,10);(115,10);(115,0);(115,0)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(80,20.01);(80,20.01);(80,10);(80,10)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(70,30);(70,30);(90,10);(90,10)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(70,0);(70,0);(90,0);(90,0)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(70,0);(70,0);(70,20);(70,20)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(70,20);(70,20);(90,0);(90,0)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(95,10);(95,10);(95,0);(95,0)"
%	 />
%<text stroke-width= "0.75"
%	 text-vert-align= "center-v"
%	 anchor-point= "(100,50)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\EQLS
%</text>
%<text stroke-width= "0.75"
%	 text-vert-align= "center-v"
%	 anchor-point= "(180,50)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\EQLS
%</text>
%<text stroke-width= "0.75"
%	 text-vert-align= "center-v"
%	 anchor-point= "(260,50)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\EQLS
%</text>
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(150,30);(150,30);(200,30);(200,30)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(200,10);(200,10);(200,30);(200,30)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(185,40);(185,40);(185,30);(185,30)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(170,10);(170,10);(200,10);(200,10)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(195,10);(195,10);(195,0);(195,0)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(160,20.01);(160,20.01);(160,10);(160,10)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(150,30);(150,30);(170,10);(170,10)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(150,0);(150,0);(170,0);(170,0)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(150,0);(150,0);(150,20);(150,20)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(150,20);(150,20);(170,0);(170,0)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(175,10);(175,10);(175,0);(175,0)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(230,30);(230,30);(280,30);(280,30)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(280,10);(280,10);(280,30);(280,30)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(265,40);(265,40);(265,30);(265,30)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(250,10);(250,10);(280,10);(280,10)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(275,10);(275,10);(275,0);(275,0)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(240,20.01);(240,20.01);(240,10);(240,10)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(230,30);(230,30);(250,10);(250,10)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(230,0);(230,0);(250,0);(250,0)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(230,0);(230,0);(230,20);(230,20)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(230,20);(230,20);(250,0);(250,0)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(255,10);(255,10);(255,0);(255,0)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(-10,30);(-10,30);(40,30);(40,30)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(40,10);(40,10);(40,30);(40,30)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(25,40);(25,40);(25,30);(25,30)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(10,10);(10,10);(40,10);(40,10)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(35,10);(35,10);(35,0);(35,0)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(0,20.01);(0,20.01);(0,10);(0,10)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(-10,30);(-10,30);(10,10);(10,10)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(-10,0);(-10,0);(10,0);(10,0)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(-10,0);(-10,0);(-10,20);(-10,20)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(-10,20);(-10,20);(10,0);(10,0)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(15,10);(15,10);(15,0);(15,0)"
%	 />
%<text text-vert-align= "center-v"
%	 anchor-point= "(75,5)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\oone$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(155,5)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\ttwo$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(-5,5)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\zzero$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(235,5)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\tthree$
%</text>
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(20.62,80.01);(20.62,80.01);(20.62,60);(20.62,60)"
%	 />
%<ellipse p3= "(23.2,77.42)"
%	 p2= "(23.2,82.58)"
%	 p1= "(18.05,82.58)"
%	 closure= "open"
%	 fill-style= "solid"
%	 angle-end= "0"
%	 fill-color= "#330033"
%	 angle-start= "0"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(25,10);(25,10);(25,0);(25,0)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(105,10);(105,10);(105,0);(105,0)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(185,10);(185,10);(185,0);(185,0)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(265,10);(265,10);(265,0);(265,0)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(170,115);(170,115);(190,95);(190,95)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(150,90);(150,90);(170,90);(170,90)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(170.62,70);(170.62,70);(190,70);(190,70)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(180,70);(180,70);(180,60);(180,60)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(160,80.01);(160,80.01);(155,75);(155,75)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(150,90);(150,90);(170,70);(170,70)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(170,90);(170,90);(190,70);(190,70)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(70,90);(70,90);(90,90);(90,90)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(115,85);(115,85);(115,65);(115,65)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(90.62,70);(90.62,70);(110,70);(110,70)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(100,70);(100,70);(100,60);(100,60)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(80,80.01);(80,80.01);(80,60);(80,60)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(70,90);(70,90);(90,70);(90,70)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(90,105);(90,105);(120,105);(120,105)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(120,85);(120,85);(120,105);(120,105)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(115,115);(115,115);(115,105);(115,105)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(110.62,85);(110.62,85);(120,85);(120,85)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(100,95.01);(100,95.01);(100,80);(100,80)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(90,105);(90,105);(110,85);(110,85)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(90,90);(90,90);(110,70);(110,70)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(142.5,87.5);(142.5,87.5);(155,75);(155,75)"
%	 />
%<ellipse p3= "(157.58,72.42)"
%	 p2= "(157.58,77.58)"
%	 p1= "(152.42,77.58)"
%	 closure= "open"
%	 fill-style= "solid"
%	 angle-end= "0"
%	 fill-color= "#330033"
%	 angle-start= "0"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(155,75);(155,75);(155,60);(155,60)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(230,140);(230,140);(250,140);(250,140)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(275,135);(275,135);(275,60);(275,60)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(250.62,120);(250.62,120);(270,120);(270,120)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(260,120);(260,120);(260,105);(260,105)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(240,130.01);(240,130.01);(222.5,112.5);(222.5,112.5)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(230,140);(230,140);(250,120);(250,120)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(250,155);(250,155);(280,155);(280,155)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(280,135);(280,135);(280,155);(280,155)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(275,165);(275,165);(275,155);(275,155)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(270.62,135);(270.62,135);(280,135);(280,135)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(260,145.01);(260,145.01);(260,130);(260,130)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(250,155);(250,155);(270,135);(270,135)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(250,140);(250,140);(270,120);(270,120)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(230,115);(230,115);(250,115);(250,115)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(250.62,95);(250.62,95);(270,95);(270,95)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(260,95);(260,95);(260,85);(260,85)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(240,105.01);(240,105.01);(235,100);(235,100)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(230,115);(230,115);(250,95);(250,95)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(250,115);(250,115);(270,95);(270,95)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(222.5,112.5);(222.5,112.5);(235,100);(235,100)"
%	 />
%<ellipse p3= "(237.58,97.42)"
%	 p2= "(237.58,102.58)"
%	 p1= "(232.42,102.58)"
%	 closure= "open"
%	 fill-style= "solid"
%	 angle-end= "0"
%	 fill-color= "#330033"
%	 angle-start= "0"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(260,95);(260,95);(260,80);(260,80)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(240,105.01);(240,105.01);(222.5,87.5);(222.5,87.5)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(230,90);(230,90);(250,90);(250,90)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(250.62,70);(250.62,70);(270,70);(270,70)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(260,70);(260,70);(260,60);(260,60)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(240,80.01);(240,80.01);(235,75);(235,75)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(230,90);(230,90);(250,70);(250,70)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(250,90);(250,90);(270,70);(270,70)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(222.5,87.5);(222.5,87.5);(235,75);(235,75)"
%	 />
%<ellipse p3= "(237.58,72.42)"
%	 p2= "(237.58,77.58)"
%	 p1= "(232.42,77.58)"
%	 closure= "open"
%	 fill-style= "solid"
%	 angle-end= "0"
%	 fill-color= "#330033"
%	 angle-start= "0"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(235,75);(235,75);(235,60);(235,60)"
%	 />
%</jpic>
%%End JPIC-XML
%PSTricks content-type (pstricks.sty package needed)
%Add \usepackage{pstricks} in the preamble of your LaTeX file
%You can rescale the whole picture (to 80% for instance) by using the command \def\JPicScale{0.8}
\ifx\JPicScale\undefined\def\JPicScale{1}\fi
\psset{unit=\JPicScale mm}
\psset{linewidth=0.3,dotsep=1,hatchwidth=0.3,hatchsep=1.5,shadowsize=1,dimen=middle}
\psset{dotsize=0.7 2.5,dotscale=1 1,fillcolor=black}
\psset{arrowsize=1 2,arrowlength=1,arrowinset=0.25,tbarsize=0.7 5,bracketlength=0.15,rbracketlength=0.15}
\begin{pspicture}(0,0)(280,165)
\psline[linewidth=0.75](150,115)(170,115)
\psline[linewidth=0.75](195,110)(195,60)
\psline[linewidth=0.75](170.62,95)(190,95)
\psline[linewidth=0.75](180,95)(180,80)
\psline[linewidth=0.75](160,105.01)(142.5,87.5)
\psline[linewidth=0.75](150,115)(170,95)
\psline[linewidth=0.75](170,130)(200,130)
\psline[linewidth=0.75](200,110)(200,130)
\psline[linewidth=0.75](195,140)(195,130)
\psline[linewidth=0.75](190.62,110)(200,110)
\psline[linewidth=0.75](180,120.01)(180,105)
\psline[linewidth=0.75](170,130)(190,110)
\psline[linewidth=0.75](30,100)(30,60)
\psline[linewidth=0.75](10.62,80.01)(10.62,60)
\newrgbcolor{userFillColour}{0.2 0 0.2}
\rput{90}(10.62,80){\psellipse[fillcolor=userFillColour,fillstyle=solid](0,0)(2.58,-2.58)}
\psline[linewidth=0.6](0,90)(40,90)
\psline[linewidth=0.6](40,70)(40,90)
\psline[linewidth=0.6](0,70)(40,70)
\psline[linewidth=0.6](0,90)(0,70)
\rput(20,50){\EQLS}
\psline[linewidth=0.75](70,30)(120,30)
\psline[linewidth=0.75](120,10)(120,30)
\psline[linewidth=0.75](105,40)(105,30)
\psline[linewidth=0.75](90,10)(120,10)
\psline[linewidth=0.75](115,10)(115,0)
\psline[linewidth=0.75](80,20.01)(80,10)
\psline[linewidth=0.75](70,30)(90,10)
\psline[linewidth=0.75](70,0)(90,0)
\psline[linewidth=0.75](70,0)(70,20)
\psline[linewidth=0.75](70,20)(90,0)
\psline[linewidth=0.75](95,10)(95,0)
\rput(100,50){\EQLS}
\rput(180,50){\EQLS}
\rput(260,50){\EQLS}
\psline[linewidth=0.75](150,30)(200,30)
\psline[linewidth=0.75](200,10)(200,30)
\psline[linewidth=0.75](185,40)(185,30)
\psline[linewidth=0.75](170,10)(200,10)
\psline[linewidth=0.75](195,10)(195,0)
\psline[linewidth=0.75](160,20.01)(160,10)
\psline[linewidth=0.75](150,30)(170,10)
\psline[linewidth=0.75](150,0)(170,0)
\psline[linewidth=0.75](150,0)(150,20)
\psline[linewidth=0.75](150,20)(170,0)
\psline[linewidth=0.75](175,10)(175,0)
\psline[linewidth=0.75](230,30)(280,30)
\psline[linewidth=0.75](280,10)(280,30)
\psline[linewidth=0.75](265,40)(265,30)
\psline[linewidth=0.75](250,10)(280,10)
\psline[linewidth=0.75](275,10)(275,0)
\psline[linewidth=0.75](240,20.01)(240,10)
\psline[linewidth=0.75](230,30)(250,10)
\psline[linewidth=0.75](230,0)(250,0)
\psline[linewidth=0.75](230,0)(230,20)
\psline[linewidth=0.75](230,20)(250,0)
\psline[linewidth=0.75](255,10)(255,0)
\psline[linewidth=0.75](-10,30)(40,30)
\psline[linewidth=0.75](40,10)(40,30)
\psline[linewidth=0.75](25,40)(25,30)
\psline[linewidth=0.75](10,10)(40,10)
\psline[linewidth=0.75](35,10)(35,0)
\psline[linewidth=0.75](0,20.01)(0,10)
\psline[linewidth=0.75](-10,30)(10,10)
\psline[linewidth=0.75](-10,0)(10,0)
\psline[linewidth=0.75](-10,0)(-10,20)
\psline[linewidth=0.75](-10,20)(10,0)
\psline[linewidth=0.75](15,10)(15,0)
\rput(75,5){$\oone$}
\rput(155,5){$\ttwo$}
\rput(-5,5){$\zzero$}
\rput(235,5){$\tthree$}
\psline[linewidth=0.75](20.62,80.01)(20.62,60)
\newrgbcolor{userFillColour}{0.2 0 0.2}
\rput{90}(20.62,80){\psellipse[fillcolor=userFillColour,fillstyle=solid](0,0)(2.58,-2.58)}
\psline[linewidth=0.75](25,10)(25,0)
\psline[linewidth=0.75](105,10)(105,0)
\psline[linewidth=0.75](185,10)(185,0)
\psline[linewidth=0.75](265,10)(265,0)
\psline[linewidth=0.75](170,115)(190,95)
\psline[linewidth=0.75](150,90)(170,90)
\psline[linewidth=0.75](170.62,70)(190,70)
\psline[linewidth=0.75](180,70)(180,60)
\psline[linewidth=0.75](160,80.01)(155,75)
\psline[linewidth=0.75](150,90)(170,70)
\psline[linewidth=0.75](170,90)(190,70)
\psline[linewidth=0.75](70,90)(90,90)
\psline[linewidth=0.75](115,85)(115,65)
\psline[linewidth=0.75](90.62,70)(110,70)
\psline[linewidth=0.75](100,70)(100,60)
\psline[linewidth=0.75](80,80.01)(80,60)
\psline[linewidth=0.75](70,90)(90,70)
\psline[linewidth=0.75](90,105)(120,105)
\psline[linewidth=0.75](120,85)(120,105)
\psline[linewidth=0.75](115,115)(115,105)
\psline[linewidth=0.75](110.62,85)(120,85)
\psline[linewidth=0.75](100,95.01)(100,80)
\psline[linewidth=0.75](90,105)(110,85)
\psline[linewidth=0.75](90,90)(110,70)
\psline[linewidth=0.75](142.5,87.5)(155,75)
\newrgbcolor{userFillColour}{0.2 0 0.2}
\rput{90}(155,75){\psellipse[fillcolor=userFillColour,fillstyle=solid](0,0)(2.58,-2.58)}
\psline[linewidth=0.75](155,75)(155,60)
\psline[linewidth=0.75](230,140)(250,140)
\psline[linewidth=0.75](275,135)(275,60)
\psline[linewidth=0.75](250.62,120)(270,120)
\psline[linewidth=0.75](260,120)(260,105)
\psline[linewidth=0.75](240,130.01)(222.5,112.5)
\psline[linewidth=0.75](230,140)(250,120)
\psline[linewidth=0.75](250,155)(280,155)
\psline[linewidth=0.75](280,135)(280,155)
\psline[linewidth=0.75](275,165)(275,155)
\psline[linewidth=0.75](270.62,135)(280,135)
\psline[linewidth=0.75](260,145.01)(260,130)
\psline[linewidth=0.75](250,155)(270,135)
\psline[linewidth=0.75](250,140)(270,120)
\psline[linewidth=0.75](230,115)(250,115)
\psline[linewidth=0.75](250.62,95)(270,95)
\psline[linewidth=0.75](260,95)(260,85)
\psline[linewidth=0.75](240,105.01)(235,100)
\psline[linewidth=0.75](230,115)(250,95)
\psline[linewidth=0.75](250,115)(270,95)
\psline[linewidth=0.75](222.5,112.5)(235,100)
\newrgbcolor{userFillColour}{0.2 0 0.2}
\rput{90}(235,100){\psellipse[fillcolor=userFillColour,fillstyle=solid](0,0)(2.58,-2.58)}
\psline[linewidth=0.75](260,95)(260,80)
\psline[linewidth=0.75](240,105.01)(222.5,87.5)
\psline[linewidth=0.75](230,90)(250,90)
\psline[linewidth=0.75](250.62,70)(270,70)
\psline[linewidth=0.75](260,70)(260,60)
\psline[linewidth=0.75](240,80.01)(235,75)
\psline[linewidth=0.75](230,90)(250,70)
\psline[linewidth=0.75](250,90)(270,70)
\psline[linewidth=0.75](222.5,87.5)(235,75)
\newrgbcolor{userFillColour}{0.2 0 0.2}
\rput{90}(235,75){\psellipse[fillcolor=userFillColour,fillstyle=solid](0,0)(2.58,-2.58)}
\psline[linewidth=0.75](235,75)(235,60)
\end{pspicture}


==> PIC/coper-mult-def.tex <==
%%Created by jPicEdt 1.4.1_03: mixed JPIC-XML/LaTeX format
%%Sun Aug 21 15:36:18 GMT-10:00 2022
%%Begin JPIC-XML
%<?xml version="1.0" standalone="yes"?>
%<jpic x-min="0" x-max="158.75" y-min="0" y-max="81.25" auto-bounding="true">
%<multicurve fill-style= "none"
%	 points= "(110,40);(110,40);(130,40);(130,40)"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(156.25,50);(156.25,50);(156.25,0);(156.25,0)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(130,20);(130,20);(150,20);(150,20)"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(137.5,20.01);(137.5,20.01);(137.5,0);(137.5,0)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(103.75,70);(103.75,70);(158.75,70);(158.75,70)"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(158.75,50);(158.75,50);(158.75,70);(158.75,70)"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(138.75,81.25);(138.75,81.25);(138.75,70);(138.75,70)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(123.75,50);(123.75,50);(158.75,50);(158.75,50)"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(137.5,50);(137.5,50);(137.5,32.5);(137.5,32.5)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(103.75,70);(103.75,70);(123.75,50);(123.75,50)"
%	 stroke-width= "0.35"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(80,67.5)"
%	 text-frame= "noframe"
%	 stroke-width= "0.75"
%	 text-hor-align= "center-h"
%	 >
%\EQLS
%</text>
%<multicurve fill-style= "none"
%	 points= "(5,70);(5,70);(58.75,70);(58.75,70)"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(58.75,50);(58.75,50);(58.75,70);(58.75,70)"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(40,81.25);(40,81.25);(40,70);(40,70)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(25,50);(25,50);(58.75,50);(58.75,50)"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(55,50);(55,50);(55,0);(55,0)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(15,60);(15,60);(10,55);(10,55)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(5,70);(5,70);(25,50);(25,50)"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(36.25,50);(36.25,50);(36.25,0);(36.25,0)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(100,46.25);(100,46.25);(100,0);(100,0)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(0,45);(0,45);(0,65);(0,65)"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(0,65);(0,65);(20,45);(20,45)"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(0,45);(0,45);(20,45);(20,45)"
%	 stroke-width= "0.35"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(6.25,48.75)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\suces$
%</text>
%<multicurve fill-style= "none"
%	 points= "(5,45);(5,45);(5,0);(5,0)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(15,45);(15,45);(15,0);(15,0)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(113.75,60);(113.75,60);(100,46.25);(100,46.25)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 stroke-overstrike-width= "1"
%	 points= "(120,30);(120,30);(110,20);(110,20)"
%	 stroke-overstrike= "true"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(110,20);(110,20);(110,0);(110,0)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(130,40);(130,40);(150,20);(150,20)"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(110,40);(110,40);(130,20);(130,20)"
%	 stroke-width= "0.35"
%	 />
%<ellipse p3= "(12.58,52.42)"
%	 fill-style= "solid"
%	 p2= "(12.58,57.58)"
%	 fill-color= "#330033"
%	 p1= "(7.42,57.58)"
%	 closure= "open"
%	 angle-end= "0"
%	 angle-start= "0"
%	 />
%<ellipse p3= "(140.08,29.92)"
%	 fill-style= "solid"
%	 p2= "(140.08,35.08)"
%	 fill-color= "#330033"
%	 p1= "(134.92,35.08)"
%	 closure= "open"
%	 angle-end= "0"
%	 angle-start= "0"
%	 />
%</jpic>
%%End JPIC-XML
%LaTeX-picture environment using emulated lines and arcs
%You can rescale the whole picture (to 80% for instance) by using the command \def\JPicScale{0.8}
\ifx\JPicScale\undefined\def\JPicScale{1}\fi
\unitlength \JPicScale mm
\begin{picture}(158.75,81.25)(0,0)
\linethickness{0.35mm}
\put(110,40){\line(1,0){20}}
\linethickness{0.75mm}
\put(156.25,0){\line(0,1){50}}
\linethickness{0.35mm}
\put(130,20){\line(1,0){20}}
\linethickness{0.75mm}
\put(137.5,0){\line(0,1){20.01}}
\linethickness{0.35mm}
\put(103.75,70){\line(1,0){55}}
\linethickness{0.35mm}
\put(158.75,50){\line(0,1){20}}
\linethickness{0.75mm}
\put(138.75,70){\line(0,1){11.25}}
\linethickness{0.35mm}
\put(123.75,50){\line(1,0){35}}
\linethickness{0.75mm}
\put(137.5,32.5){\line(0,1){17.5}}
\linethickness{0.35mm}
\multiput(103.75,70)(0.12,-0.12){167}{\line(1,0){0.12}}
\put(80,67.5){\makebox(0,0)[cc]{\EQLS}}

\linethickness{0.35mm}
\put(5,70){\line(1,0){53.75}}
\linethickness{0.35mm}
\put(58.75,50){\line(0,1){20}}
\linethickness{0.75mm}
\put(40,70){\line(0,1){11.25}}
\linethickness{0.35mm}
\put(25,50){\line(1,0){33.75}}
\linethickness{0.75mm}
\put(55,0){\line(0,1){50}}
\linethickness{0.75mm}
\multiput(10,55)(0.12,0.12){42}{\line(1,0){0.12}}
\linethickness{0.35mm}
\multiput(5,70)(0.12,-0.12){167}{\line(1,0){0.12}}
\linethickness{0.75mm}
\put(36.25,0){\line(0,1){50}}
\linethickness{0.75mm}
\put(100,0){\line(0,1){46.25}}
\linethickness{0.35mm}
\put(0,45){\line(0,1){20}}
\linethickness{0.35mm}
\multiput(0,65)(0.12,-0.12){167}{\line(1,0){0.12}}
\linethickness{0.35mm}
\put(0,45){\line(1,0){20}}
\put(6.25,48.75){\makebox(0,0)[cc]{$\suces$}}

\linethickness{0.75mm}
\put(5,0){\line(0,1){45}}
\linethickness{0.75mm}
\put(15,0){\line(0,1){45}}
\linethickness{0.75mm}
\multiput(100,46.25)(0.12,0.12){115}{\line(1,0){0.12}}
\linethickness{0.75mm}
\multiput(110,20)(0.12,0.12){83}{\line(1,0){0.12}}
\linethickness{0.75mm}
\put(110,0){\line(0,1){20}}
\linethickness{0.35mm}
\multiput(130,40)(0.12,-0.12){167}{\line(1,0){0.12}}
\linethickness{0.35mm}
\multiput(110,40)(0.12,-0.12){167}{\line(1,0){0.12}}
\linethickness{0.3mm}
\put(10,55){\circle*{5.16}}

\linethickness{0.3mm}
\put(137.5,32.5){\circle*{5.16}}

\end{picture}


==> PIC/coper-succ-def.tex <==
%%Created by jPicEdt 1.4.1_03: mixed JPIC-XML/LaTeX format
%%Sun Aug 21 15:20:31 GMT-10:00 2022
%%Begin JPIC-XML
%<?xml version="1.0" standalone="yes"?>
%<jpic x-min="0" x-max="160" y-min="0" y-max="75" auto-bounding="true">
%<multicurve fill-style= "none"
%	 points= "(125,30);(125,30);(160,30);(160,30)"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(160,10);(160,10);(160,30);(160,30)"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(150,45);(150,45);(150,30);(150,30)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(145,10);(145,10);(160,10);(160,10)"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(150,10);(150,10);(150,0);(150,0)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(135,20.01);(135,20.01);(135,0);(135,0)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(125,30);(125,30);(145,10);(145,10)"
%	 stroke-width= "0.35"
%	 />
%<ellipse p3= "(137.58,7.42)"
%	 fill-style= "solid"
%	 p2= "(137.58,12.58)"
%	 fill-color= "#330033"
%	 p1= "(132.42,12.58)"
%	 closure= "open"
%	 angle-end= "0"
%	 angle-start= "0"
%	 />
%<multicurve fill-style= "none"
%	 points= "(130,40);(130,40);(117.5,27.5);(117.5,27.5)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(117.5,27.5);(117.5,27.5);(135,10);(135,10)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(105,65);(105,65);(160,65);(160,65)"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(160,45);(160,45);(160,65);(160,65)"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(150,75);(150,75);(150,65);(150,65)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(125,45);(125,45);(160,45);(160,45)"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(130,45);(130,45);(130,40);(130,40)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(105,65);(105,65);(125,45);(125,45)"
%	 stroke-width= "0.35"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(80,50)"
%	 text-frame= "noframe"
%	 stroke-width= "0.75"
%	 text-hor-align= "center-h"
%	 >
%\EQLS
%</text>
%<multicurve fill-style= "none"
%	 points= "(5,65);(5,65);(55,65);(55,65)"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(55,45);(55,45);(55,65);(55,65)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(40,75);(40,75);(40,65);(40,65)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(25,45);(25,45);(55,45);(55,45)"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(50,45);(50,45);(50,0);(50,0)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(15,55);(15,55);(10,50);(10,50)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(5,65);(5,65);(25,45);(25,45)"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(30,45);(30,45);(30,0);(30,0)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(115,55);(115,55);(115,0);(115,0)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(0,40);(0,40);(0,60);(0,60)"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(0,60);(0,60);(20,40);(20,40)"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(0,40);(0,40);(20,40);(20,40)"
%	 stroke-width= "0.35"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(5,45)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\suces$
%</text>
%<multicurve fill-style= "none"
%	 points= "(10,40);(10,40);(10,0);(10,0)"
%	 stroke-width= "0.75"
%	 />
%<ellipse p3= "(12.58,47.42)"
%	 fill-style= "solid"
%	 p2= "(12.58,52.58)"
%	 fill-color= "#330033"
%	 p1= "(7.42,52.58)"
%	 closure= "open"
%	 angle-end= "0"
%	 angle-start= "0"
%	 />
%</jpic>
%%End JPIC-XML
%LaTeX-picture environment using emulated lines and arcs
%You can rescale the whole picture (to 80% for instance) by using the command \def\JPicScale{0.8}
\ifx\JPicScale\undefined\def\JPicScale{1}\fi
\unitlength \JPicScale mm
\begin{picture}(160,75)(0,0)
\linethickness{0.35mm}
\put(125,30){\line(1,0){35}}
\linethickness{0.35mm}
\put(160,10){\line(0,1){20}}
\linethickness{0.75mm}
\put(150,30){\line(0,1){15}}
\linethickness{0.35mm}
\put(145,10){\line(1,0){15}}
\linethickness{0.75mm}
\put(150,0){\line(0,1){10}}
\linethickness{0.75mm}
\put(135,0){\line(0,1){20.01}}
\linethickness{0.35mm}
\multiput(125,30)(0.12,-0.12){167}{\line(1,0){0.12}}
\linethickness{0.3mm}
\put(135,10){\circle*{5.16}}

\linethickness{0.75mm}
\multiput(117.5,27.5)(0.12,0.12){104}{\line(1,0){0.12}}
\linethickness{0.75mm}
\multiput(117.5,27.5)(0.12,-0.12){146}{\line(1,0){0.12}}
\linethickness{0.35mm}
\put(105,65){\line(1,0){55}}
\linethickness{0.35mm}
\put(160,45){\line(0,1){20}}
\linethickness{0.75mm}
\put(150,65){\line(0,1){10}}
\linethickness{0.35mm}
\put(125,45){\line(1,0){35}}
\linethickness{0.75mm}
\put(130,40){\line(0,1){5}}
\linethickness{0.35mm}
\multiput(105,65)(0.12,-0.12){167}{\line(1,0){0.12}}
\put(80,50){\makebox(0,0)[cc]{\EQLS}}

\linethickness{0.35mm}
\put(5,65){\line(1,0){50}}
\linethickness{0.75mm}
\put(55,45){\line(0,1){20}}
\linethickness{0.75mm}
\put(40,65){\line(0,1){10}}
\linethickness{0.35mm}
\put(25,45){\line(1,0){30}}
\linethickness{0.75mm}
\put(50,0){\line(0,1){45}}
\linethickness{0.75mm}
\multiput(10,50)(0.12,0.12){42}{\line(1,0){0.12}}
\linethickness{0.35mm}
\multiput(5,65)(0.12,-0.12){167}{\line(1,0){0.12}}
\linethickness{0.75mm}
\put(30,0){\line(0,1){45}}
\linethickness{0.75mm}
\put(115,0){\line(0,1){55}}
\linethickness{0.35mm}
\put(0,40){\line(0,1){20}}
\linethickness{0.35mm}
\multiput(0,60)(0.12,-0.12){167}{\line(1,0){0.12}}
\linethickness{0.35mm}
\put(0,40){\line(1,0){20}}
\put(5,45){\makebox(0,0)[cc]{$\suces$}}

\linethickness{0.75mm}
\put(10,0){\line(0,1){40}}
\linethickness{0.3mm}
\put(10,50){\circle*{5.16}}

\end{picture}


==> PIC/coper-succ-prop.tex <==
%%Created by jPicEdt 1.4.1_03: mixed JPIC-XML/LaTeX format
%%Thu Oct 20 16:04:42 HST 2016
%%Begin JPIC-XML
%<?xml version="1.0" standalone="yes"?>
%<jpic x-min="0" x-max="160" y-min="0" y-max="70" auto-bounding="true">
%<multicurve stroke-width= "0.75"
%	 points= "(150,40);(150,40);(150,0);(150,0)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.75"
%	 points= "(105,60);(105,60);(160,60);(160,60)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.75"
%	 points= "(160,40);(160,40);(160,60);(160,60)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.75"
%	 points= "(150,70);(150,70);(150,60);(150,60)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.75"
%	 points= "(125,40);(125,40);(160,40);(160,40)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.75"
%	 points= "(130,40);(130,40);(130,0);(130,0)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.75"
%	 points= "(105,60);(105,60);(125,40);(125,40)"
%	 fill-style= "none"
%	 />
%<text text-vert-align= "center-v"
%	 stroke-width= "0.75"
%	 anchor-point= "(80,45)"
%	 text-frame= "noframe"
%	 fill-style= "none"
%	 text-hor-align= "center-h"
%	 >
%\EQLS
%</text>
%<multicurve stroke-width= "0.75"
%	 points= "(5,60);(5,60);(55,60);(55,60)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.75"
%	 points= "(55,40);(55,40);(55,60);(55,60)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.75"
%	 points= "(40,70);(40,70);(40,60);(40,60)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.75"
%	 points= "(25,40);(25,40);(55,40);(55,40)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.75"
%	 points= "(50,40);(50,40);(50,0);(50,0)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.75"
%	 points= "(15,50);(15,50);(10,45);(10,45)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.75"
%	 points= "(5,60);(5,60);(25,40);(25,40)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.75"
%	 points= "(30,40);(30,40);(30,0);(30,0)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.75"
%	 points= "(115,50);(115,50);(115,25);(115,25)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.75"
%	 points= "(0,35);(0,35);(0,55);(0,55)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.75"
%	 points= "(0,55);(0,55);(20,35);(20,35)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.75"
%	 points= "(0,35);(0,35);(20,15);(20,15)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.75"
%	 points= "(20,15);(20,15);(20,35);(20,35)"
%	 fill-style= "none"
%	 />
%<text text-vert-align= "center-v"
%	 anchor-point= "(10,35)"
%	 text-frame= "noframe"
%	 fill-style= "none"
%	 text-hor-align= "center-h"
%	 >
%$\suces$
%</text>
%<multicurve stroke-width= "0.75"
%	 points= "(10,25);(10,25);(10,15);(10,15)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.75"
%	 points= "(102.5,12.5);(102.5,12.5);(127.5,12.5);(127.5,12.5)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.75"
%	 points= "(102.5,12.5);(102.5,12.5);(102.5,37.5);(102.5,37.5)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.75"
%	 points= "(102.5,37.5);(102.5,37.5);(127.5,12.5);(127.5,12.5)"
%	 fill-style= "none"
%	 />
%<text text-vert-align= "center-v"
%	 anchor-point= "(111.25,20)"
%	 text-frame= "noframe"
%	 fill-style= "none"
%	 text-hor-align= "center-h"
%	 >
%$\enplus$
%</text>
%<multicurve stroke-width= "0.75"
%	 points= "(0,5);(0,5);(20,5);(20,5)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.75"
%	 points= "(0,5);(0,5);(0,25);(0,25)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.75"
%	 points= "(0,25);(0,25);(20,5);(20,5)"
%	 fill-style= "none"
%	 />
%<text text-vert-align= "center-v"
%	 anchor-point= "(6.25,11.25)"
%	 text-frame= "noframe"
%	 fill-style= "none"
%	 text-hor-align= "center-h"
%	 >
%$\een$
%</text>
%</jpic>
%%End JPIC-XML
%PSTricks content-type (pstricks.sty package needed)
%Add \usepackage{pstricks} in the preamble of your LaTeX file
%You can rescale the whole picture (to 80% for instance) by using the command \def\JPicScale{0.8}
\ifx\JPicScale\undefined\def\JPicScale{1}\fi
\psset{unit=\JPicScale mm}
\psset{linewidth=0.3,dotsep=1,hatchwidth=0.3,hatchsep=1.5,shadowsize=1,dimen=middle}
\psset{dotsize=0.7 2.5,dotscale=1 1,fillcolor=black}
\psset{arrowsize=1 2,arrowlength=1,arrowinset=0.25,tbarsize=0.7 5,bracketlength=0.15,rbracketlength=0.15}
\begin{pspicture}(0,0)(160,70)
\psline[linewidth=0.75](150,40)(150,0)
\psline[linewidth=0.75](105,60)(160,60)
\psline[linewidth=0.75](160,40)(160,60)
\psline[linewidth=0.75](150,70)(150,60)
\psline[linewidth=0.75](125,40)(160,40)
\psline[linewidth=0.75](130,40)(130,0)
\psline[linewidth=0.75](105,60)(125,40)
\rput(80,45){\EQLS}
\psline[linewidth=0.75](5,60)(55,60)
\psline[linewidth=0.75](55,40)(55,60)
\psline[linewidth=0.75](40,70)(40,60)
\psline[linewidth=0.75](25,40)(55,40)
\psline[linewidth=0.75](50,40)(50,0)
\psline[linewidth=0.75](15,50)(10,45)
\psline[linewidth=0.75](5,60)(25,40)
\psline[linewidth=0.75](30,40)(30,0)
\psline[linewidth=0.75](115,50)(115,25)
\psline[linewidth=0.75](0,35)(0,55)
\psline[linewidth=0.75](0,55)(20,35)
\psline[linewidth=0.75](0,35)(20,15)
\psline[linewidth=0.75](20,15)(20,35)
\rput(10,35){$\suces$}
\psline[linewidth=0.75](10,25)(10,15)
\psline[linewidth=0.75](102.5,12.5)(127.5,12.5)
\psline[linewidth=0.75](102.5,12.5)(102.5,37.5)
\psline[linewidth=0.75](102.5,37.5)(127.5,12.5)
\rput(111.25,20){$\enplus$}
\psline[linewidth=0.75](0,5)(20,5)
\psline[linewidth=0.75](0,5)(0,25)
\psline[linewidth=0.75](0,25)(20,5)
\rput(6.25,11.25){$\een$}
\end{pspicture}


==> PIC/coper-succ.tex <==
%%Created by jPicEdt 1.4.1_03: mixed JPIC-XML/LaTeX format
%%Sun Aug 21 15:15:09 GMT-10:00 2022
%%Begin JPIC-XML
%<?xml version="1.0" standalone="yes"?>
%<jpic x-min="0" x-max="260" y-min="0" y-max="125" auto-bounding="true">
%<multicurve fill-style= "none"
%	 points= "(120,30);(120,30);(160,30);(160,30)"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(160,10);(160,10);(160,30);(160,30)"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(150,55);(150,55);(150,30);(150,30)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(140.62,10);(140.62,10);(160,10);(160,10)"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(150,10);(150,10);(150,0);(150,0)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(130,20.01);(130,20.01);(130,0);(130,0)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(120,30);(120,30);(140,10);(140,10)"
%	 stroke-width= "0.35"
%	 />
%<ellipse p3= "(132.58,7.42)"
%	 fill-style= "solid"
%	 p2= "(132.58,12.58)"
%	 fill-color= "#330033"
%	 p1= "(127.42,12.58)"
%	 closure= "open"
%	 angle-end= "0"
%	 angle-start= "0"
%	 />
%<multicurve fill-style= "none"
%	 points= "(130,50);(130,50);(110,30);(110,30)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(110,30);(110,30);(130,10);(130,10)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(105,75);(105,75);(160,75);(160,75)"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(160,55);(160,55);(160,75);(160,75)"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(150,125);(150,125);(150,75);(150,75)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(125,55);(125,55);(160,55);(160,55)"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(130,55);(130,55);(130,50);(130,50)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(105,75);(105,75);(125,55);(125,55)"
%	 stroke-width= "0.35"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(80,65)"
%	 text-frame= "noframe"
%	 stroke-width= "0.75"
%	 text-hor-align= "center-h"
%	 >
%\EQLS
%</text>
%<multicurve fill-style= "none"
%	 points= "(5,75);(5,75);(55,75);(55,75)"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(55,55);(55,55);(55,75);(55,75)"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(40,125);(40,125);(40,75);(40,75)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(25,55);(25,55);(55,55);(55,55)"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(50,55);(50,55);(50,0);(50,0)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(13.75,66.25);(13.75,66.25);(13.75,56.24);(13.75,56.24)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(5,75);(5,75);(25,55);(25,55)"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(0,45);(0,45);(25,45);(25,45)"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(0,45);(0,45);(0,70);(0,70)"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(0,70);(0,70);(25,45);(25,45)"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(30,55);(30,55);(30,0);(30,0)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(112.5,67.5);(112.5,67.5);(112.5,57.49);(112.5,57.49)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(102.5,47.5);(102.5,47.5);(122.5,47.5);(122.5,47.5)"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(102.5,47.5);(102.5,47.5);(102.5,67.5);(102.5,67.5)"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(102.5,67.5);(102.5,67.5);(122.5,47.5);(122.5,47.5)"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(220,115);(220,115);(260,115);(260,115)"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(260,95);(260,95);(260,115);(260,115)"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(250,125);(250,125);(250,115);(250,115)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(240.62,95);(240.62,95);(260,95);(260,95)"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(250,55);(250,55);(250,0);(250,0)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(220,115);(220,115);(240,95);(240,95)"
%	 stroke-width= "0.35"
%	 />
%<ellipse p3= "(232.58,39.92)"
%	 fill-style= "solid"
%	 p2= "(232.58,45.08)"
%	 fill-color= "#330033"
%	 p1= "(227.42,45.08)"
%	 closure= "open"
%	 angle-end= "0"
%	 angle-start= "0"
%	 />
%<multicurve fill-style= "none"
%	 points= "(230,105);(230,105);(198.75,73.75);(198.75,73.75)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(198.75,73.75);(198.75,73.75);(230,42.5);(230,42.5)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(205,75);(205,75);(260,75);(260,75)"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(260,55);(260,55);(260,75);(260,75)"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(250,95);(250,95);(250,75);(250,75)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(225,55);(225,55);(260,55);(260,55)"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(230,55);(230,55);(230,0);(230,0)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(205,75);(205,75);(225,55);(225,55)"
%	 stroke-width= "0.35"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(180,65)"
%	 text-frame= "noframe"
%	 stroke-width= "0.75"
%	 text-hor-align= "center-h"
%	 >
%\EQLS
%</text>
%<multicurve fill-style= "none"
%	 points= "(202.5,37.5);(202.5,37.5);(222.5,37.5);(222.5,37.5)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(202.5,37.5);(202.5,37.5);(202.5,57.5);(202.5,57.5)"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 stroke-overstrike-width= "1.35"
%	 points= "(215,65);(215,65);(215,45);(215,45)"
%	 stroke-overstrike= "true"
%	 stroke-width= "0.75"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(8.75,52.5)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\enplus$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(107.5,52.5)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\een$
%</text>
%<multicurve fill-style= "none"
%	 points= "(202.5,57.5);(202.5,57.5);(222.5,37.5);(222.5,37.5)"
%	 stroke-width= "0.35"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(207.5,42.5)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\een$
%</text>
%<ellipse p3= "(115.08,54.92)"
%	 fill-style= "solid"
%	 p2= "(115.08,60.08)"
%	 fill-color= "#330033"
%	 p1= "(109.92,60.08)"
%	 closure= "open"
%	 angle-end= "0"
%	 angle-start= "0"
%	 />
%<ellipse p3= "(217.58,42.42)"
%	 fill-style= "solid"
%	 p2= "(217.58,47.58)"
%	 fill-color= "#330033"
%	 p1= "(212.42,47.58)"
%	 closure= "open"
%	 angle-end= "0"
%	 angle-start= "0"
%	 />
%<ellipse p3= "(16.33,53.04)"
%	 fill-style= "solid"
%	 p2= "(16.33,58.2)"
%	 fill-color= "#330033"
%	 p1= "(11.17,58.2)"
%	 closure= "open"
%	 angle-end= "0"
%	 angle-start= "0"
%	 />
%</jpic>
%%End JPIC-XML
%LaTeX-picture environment using emulated lines and arcs
%You can rescale the whole picture (to 80% for instance) by using the command \def\JPicScale{0.8}
\ifx\JPicScale\undefined\def\JPicScale{1}\fi
\unitlength \JPicScale mm
\begin{picture}(260,125)(0,0)
\linethickness{0.35mm}
\put(120,30){\line(1,0){40}}
\linethickness{0.35mm}
\put(160,10){\line(0,1){20}}
\linethickness{0.75mm}
\put(150,30){\line(0,1){25}}
\linethickness{0.35mm}
\put(140.62,10){\line(1,0){19.38}}
\linethickness{0.75mm}
\put(150,0){\line(0,1){10}}
\linethickness{0.75mm}
\put(130,0){\line(0,1){20.01}}
\linethickness{0.35mm}
\multiput(120,30)(0.12,-0.12){167}{\line(1,0){0.12}}
\linethickness{0.3mm}
\put(130,10){\circle*{5.16}}

\linethickness{0.75mm}
\multiput(110,30)(0.12,0.12){167}{\line(1,0){0.12}}
\linethickness{0.75mm}
\multiput(110,30)(0.12,-0.12){167}{\line(1,0){0.12}}
\linethickness{0.35mm}
\put(105,75){\line(1,0){55}}
\linethickness{0.35mm}
\put(160,55){\line(0,1){20}}
\linethickness{0.75mm}
\put(150,75){\line(0,1){50}}
\linethickness{0.35mm}
\put(125,55){\line(1,0){35}}
\linethickness{0.75mm}
\put(130,50){\line(0,1){5}}
\linethickness{0.35mm}
\multiput(105,75)(0.12,-0.12){167}{\line(1,0){0.12}}
\put(80,65){\makebox(0,0)[cc]{\EQLS}}

\linethickness{0.35mm}
\put(5,75){\line(1,0){50}}
\linethickness{0.35mm}
\put(55,55){\line(0,1){20}}
\linethickness{0.75mm}
\put(40,75){\line(0,1){50}}
\linethickness{0.35mm}
\put(25,55){\line(1,0){30}}
\linethickness{0.75mm}
\put(50,0){\line(0,1){55}}
\linethickness{0.75mm}
\put(13.75,56.24){\line(0,1){10.01}}
\linethickness{0.35mm}
\multiput(5,75)(0.12,-0.12){167}{\line(1,0){0.12}}
\linethickness{0.35mm}
\put(0,45){\line(1,0){25}}
\linethickness{0.35mm}
\put(0,45){\line(0,1){25}}
\linethickness{0.35mm}
\multiput(0,70)(0.12,-0.12){208}{\line(1,0){0.12}}
\linethickness{0.75mm}
\put(30,0){\line(0,1){55}}
\linethickness{0.75mm}
\put(112.5,57.49){\line(0,1){10.01}}
\linethickness{0.35mm}
\put(102.5,47.5){\line(1,0){20}}
\linethickness{0.35mm}
\put(102.5,47.5){\line(0,1){20}}
\linethickness{0.35mm}
\multiput(102.5,67.5)(0.12,-0.12){167}{\line(1,0){0.12}}
\linethickness{0.35mm}
\put(220,115){\line(1,0){40}}
\linethickness{0.35mm}
\put(260,95){\line(0,1){20}}
\linethickness{0.75mm}
\put(250,115){\line(0,1){10}}
\linethickness{0.35mm}
\put(240.62,95){\line(1,0){19.38}}
\linethickness{0.75mm}
\put(250,0){\line(0,1){55}}
\linethickness{0.35mm}
\multiput(220,115)(0.12,-0.12){167}{\line(1,0){0.12}}
\linethickness{0.3mm}
\put(230,42.5){\circle*{5.16}}

\linethickness{0.75mm}
\multiput(198.75,73.75)(0.12,0.12){260}{\line(1,0){0.12}}
\linethickness{0.75mm}
\multiput(198.75,73.75)(0.12,-0.12){260}{\line(1,0){0.12}}
\linethickness{0.35mm}
\put(205,75){\line(1,0){55}}
\linethickness{0.35mm}
\put(260,55){\line(0,1){20}}
\linethickness{0.75mm}
\put(250,75){\line(0,1){20}}
\linethickness{0.35mm}
\put(225,55){\line(1,0){35}}
\linethickness{0.75mm}
\put(230,0){\line(0,1){55}}
\linethickness{0.35mm}
\multiput(205,75)(0.12,-0.12){167}{\line(1,0){0.12}}
\put(180,65){\makebox(0,0)[cc]{\EQLS}}

\linethickness{0.75mm}
\put(202.5,37.5){\line(1,0){20}}
\linethickness{0.35mm}
\put(202.5,37.5){\line(0,1){20}}
\linethickness{0.75mm}
\put(215,45){\line(0,1){20}}
\put(8.75,52.5){\makebox(0,0)[cc]{$\enplus$}}

\put(107.5,52.5){\makebox(0,0)[cc]{$\een$}}

\linethickness{0.35mm}
\multiput(202.5,57.5)(0.12,-0.12){167}{\line(1,0){0.12}}
\put(207.5,42.5){\makebox(0,0)[cc]{$\een$}}

\linethickness{0.3mm}
\put(112.5,57.5){\circle*{5.16}}

\linethickness{0.3mm}
\put(215,45){\circle*{5.16}}

\linethickness{0.3mm}
\put(13.75,55.62){\circle*{5.16}}

\end{picture}


==> PIC/copy.tex <==
%%Created by jPicEdt 1.4.1_03: mixed JPIC-XML/LaTeX format
%%Wed Sep 28 20:09:58 HST 2016
%%Begin JPIC-XML
%<?xml version="1.0" standalone="yes"?>
%<jpic x-min="8.75" x-max="31.88" y-min="7.5" y-max="40" auto-bounding="true">
%<text stroke-width= "0.75"
%	 text-vert-align= "center-v"
%	 anchor-point= "(16.88,9.38)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\inputt$
%</text>
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(20,20);(20,20);(20,7.5);(20,7.5)"
%	 />
%<ellipse p3= "(21.41,18.59)"
%	 p2= "(21.41,21.41)"
%	 p1= "(18.59,21.41)"
%	 closure= "open"
%	 fill-style= "solid"
%	 angle-end= "360"
%	 fill-color= "#330033"
%	 angle-start= "0"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(30,40);(30,40);(30,30);(30,30)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(10,39.38);(10,39.38);(10,29.38);(10,29.38)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(30,30);(30,30);(20,20);(20,20)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(10,29.38);(10,29.38);(20,19.38);(20,19.38)"
%	 />
%<text stroke-width= "0.75"
%	 text-vert-align= "center-v"
%	 anchor-point= "(8.75,37.5)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\inputt$
%</text>
%<text stroke-width= "0.75"
%	 text-vert-align= "center-v"
%	 anchor-point= "(31.88,38.12)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\inputt$
%</text>
%</jpic>
%%End JPIC-XML
%PSTricks content-type (pstricks.sty package needed)
%Add \usepackage{pstricks} in the preamble of your LaTeX file
%You can rescale the whole picture (to 80% for instance) by using the command \def\JPicScale{0.8}
\ifx\JPicScale\undefined\def\JPicScale{1}\fi
\psset{unit=\JPicScale mm}
\psset{linewidth=0.3,dotsep=1,hatchwidth=0.3,hatchsep=1.5,shadowsize=1,dimen=middle}
\psset{dotsize=0.7 2.5,dotscale=1 1,fillcolor=black}
\psset{arrowsize=1 2,arrowlength=1,arrowinset=0.25,tbarsize=0.7 5,bracketlength=0.15,rbracketlength=0.15}
\begin{pspicture}(0,0)(31.88,40)
\rput[r](16.88,9.38){$\inputt$}
\psline[linewidth=0.75](20,20)(20,7.5)
\newrgbcolor{userFillColour}{0.2 0 0.2}
\rput{0}(20,20){\psellipse[fillcolor=userFillColour,fillstyle=solid](0,0)(1.41,-1.41)}
\psline[linewidth=0.75](30,40)(30,30)
\psline[linewidth=0.75](10,39.38)(10,29.38)
\psline[linewidth=0.75](30,30)(20,20)
\psline[linewidth=0.75](10,29.38)(20,19.38)
\rput[r](8.75,37.5){$\inputt$}
\rput[l](31.88,38.12){$\inputt$}
\end{pspicture}


==> PIC/costless-domain.tex <==
%%Created by jPicEdt 1.4.1_03: mixed JPIC-XML/LaTeX format
%%Sat Nov 26 21:11:14 GMT-10:00 2022
%%Begin JPIC-XML
%<?xml version="1.0" standalone="yes"?>
%<jpic x-min="0" x-max="90" y-min="0" y-max="130" auto-bounding="true">
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(45,65)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\EQLS
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(12.5,1.25)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\Progtype$
%</text>
%<multicurve fill-style= "none"
%	 points= "(80,90);(80,90);(80,100);(80,100)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(70,90);(70,90);(80,90);(80,90)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(75,90);(75,90);(75,55);(75,55)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(75,115);(75,115);(65,105);(65,105)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(65,85);(65,85);(75,75);(75,75)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(65,105);(65,105);(65,85);(65,85)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(70,100);(70,100);(70,90);(70,90)"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(75,95)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\universal$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(77.5,65)"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\Progtype$
%</text>
%<multicurve fill-style= "none"
%	 points= "(70,100);(70,100);(80,100);(80,100)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(75,105);(75,105);(75,100);(75,100)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(75,130);(75,130);(75,115);(75,115)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.1"
%	 points= "(60,120);(60,120);(90,120);(90,120)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.1"
%	 points= "(90,120);(90,120);(90,70);(90,70)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.1"
%	 points= "(60,120);(60,120);(60,70);(60,70)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.1"
%	 points= "(60,70);(60,70);(90,70);(90,70)"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(85,115)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\nameiota$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(75,105)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\Dottt
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(75,75)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\Dottt
%</text>
%<multicurve fill-style= "none"
%	 points= "(20,60);(20,60);(20,70);(20,70)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(10,60);(10,60);(20,60);(20,60)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(15,60);(15,60);(15,0);(15,0)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(15,85);(15,85);(5,75);(5,75)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(5,55);(5,55);(15,45);(15,45)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(5,75);(5,75);(5,55);(5,55)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(10,70);(10,70);(10,60);(10,60)"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(15,65)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\universal$
%</text>
%<multicurve fill-style= "none"
%	 points= "(10,70);(10,70);(20,70);(20,70)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(15,75);(15,75);(15,70);(15,70)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(15,130);(15,130);(15,85);(15,85)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.1"
%	 points= "(0,90);(0,90);(30,90);(30,90)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.1"
%	 points= "(30,90);(30,90);(30,40);(30,40)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.1"
%	 points= "(0,90);(0,90);(0,40);(0,40)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.1"
%	 points= "(0,40);(0,40);(30,40);(30,40)"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(25,85)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\nameiota$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(15,75)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\Dottt
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(15,45)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\Dottt
%</text>
%<multicurve fill-style= "none"
%	 points= "(80,30);(80,30);(80,40);(80,40)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(70,30);(70,30);(80,30);(80,30)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(75,30);(75,30);(75,0);(75,0)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(75,55);(75,55);(65,45);(65,45)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(65,25);(65,25);(75,15);(75,15)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(65,45);(65,45);(65,25);(65,25)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(70,40);(70,40);(70,30);(70,30)"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(75,35)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\universal$
%</text>
%<multicurve fill-style= "none"
%	 points= "(70,40);(70,40);(80,40);(80,40)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(75,45);(75,45);(75,40);(75,40)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.1"
%	 points= "(60,60);(60,60);(90,60);(90,60)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.1"
%	 points= "(90,60);(90,60);(90,10);(90,10)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.1"
%	 points= "(60,60);(60,60);(60,10);(60,10)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.1"
%	 points= "(60,10);(60,10);(90,10);(90,10)"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(85,55)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\nameiota$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(75,45)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\Dottt
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(75,15)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\Dottt
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(72.5,1.25)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\Progtype$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(17.5,128.75)"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\Progtype$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(77.5,128.75)"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\Progtype$
%</text>
%</jpic>
%%End JPIC-XML
%LaTeX-picture environment using emulated lines and arcs
%You can rescale the whole picture (to 80% for instance) by using the command \def\JPicScale{0.8}
\ifx\JPicScale\undefined\def\JPicScale{1}\fi
\unitlength \JPicScale mm
\begin{picture}(90,130)(0,0)
\put(45,65){\makebox(0,0)[cc]{\EQLS}}

\put(12.5,1.25){\makebox(0,0)[cr]{$\Progtype$}}

\linethickness{0.3mm}
\put(80,90){\line(0,1){10}}
\linethickness{0.3mm}
\put(70,90){\line(1,0){10}}
\linethickness{0.3mm}
\put(75,55){\line(0,1){35}}
\linethickness{0.3mm}
\multiput(65,105)(0.12,0.12){83}{\line(1,0){0.12}}
\linethickness{0.3mm}
\multiput(65,85)(0.12,-0.12){83}{\line(1,0){0.12}}
\linethickness{0.3mm}
\put(65,85){\line(0,1){20}}
\linethickness{0.3mm}
\put(70,90){\line(0,1){10}}
\put(75,95){\makebox(0,0)[cc]{$\universal$}}

\put(77.5,65){\makebox(0,0)[cl]{$\Progtype$}}

\linethickness{0.3mm}
\put(70,100){\line(1,0){10}}
\linethickness{0.3mm}
\put(75,100){\line(0,1){5}}
\linethickness{0.3mm}
\put(75,115){\line(0,1){15}}
\linethickness{0.1mm}
\put(60,120){\line(1,0){30}}
\linethickness{0.1mm}
\put(90,70){\line(0,1){50}}
\linethickness{0.1mm}
\put(60,70){\line(0,1){50}}
\linethickness{0.1mm}
\put(60,70){\line(1,0){30}}
\put(85,115){\makebox(0,0)[cc]{$\nameiota$}}

\put(75,105){\makebox(0,0)[cc]{\Dottt}}

\put(75,75){\makebox(0,0)[cc]{\Dottt}}

\linethickness{0.3mm}
\put(20,60){\line(0,1){10}}
\linethickness{0.3mm}
\put(10,60){\line(1,0){10}}
\linethickness{0.3mm}
\put(15,0){\line(0,1){60}}
\linethickness{0.3mm}
\multiput(5,75)(0.12,0.12){83}{\line(1,0){0.12}}
\linethickness{0.3mm}
\multiput(5,55)(0.12,-0.12){83}{\line(1,0){0.12}}
\linethickness{0.3mm}
\put(5,55){\line(0,1){20}}
\linethickness{0.3mm}
\put(10,60){\line(0,1){10}}
\put(15,65){\makebox(0,0)[cc]{$\universal$}}

\linethickness{0.3mm}
\put(10,70){\line(1,0){10}}
\linethickness{0.3mm}
\put(15,70){\line(0,1){5}}
\linethickness{0.3mm}
\put(15,85){\line(0,1){45}}
\linethickness{0.1mm}
\put(0,90){\line(1,0){30}}
\linethickness{0.1mm}
\put(30,40){\line(0,1){50}}
\linethickness{0.1mm}
\put(0,40){\line(0,1){50}}
\linethickness{0.1mm}
\put(0,40){\line(1,0){30}}
\put(25,85){\makebox(0,0)[cc]{$\nameiota$}}

\put(15,75){\makebox(0,0)[cc]{\Dottt}}

\put(15,45){\makebox(0,0)[cc]{\Dottt}}

\linethickness{0.3mm}
\put(80,30){\line(0,1){10}}
\linethickness{0.3mm}
\put(70,30){\line(1,0){10}}
\linethickness{0.3mm}
\put(75,0){\line(0,1){30}}
\linethickness{0.3mm}
\multiput(65,45)(0.12,0.12){83}{\line(1,0){0.12}}
\linethickness{0.3mm}
\multiput(65,25)(0.12,-0.12){83}{\line(1,0){0.12}}
\linethickness{0.3mm}
\put(65,25){\line(0,1){20}}
\linethickness{0.3mm}
\put(70,30){\line(0,1){10}}
\put(75,35){\makebox(0,0)[cc]{$\universal$}}

\linethickness{0.3mm}
\put(70,40){\line(1,0){10}}
\linethickness{0.3mm}
\put(75,40){\line(0,1){5}}
\linethickness{0.1mm}
\put(60,60){\line(1,0){30}}
\linethickness{0.1mm}
\put(90,10){\line(0,1){50}}
\linethickness{0.1mm}
\put(60,10){\line(0,1){50}}
\linethickness{0.1mm}
\put(60,10){\line(1,0){30}}
\put(85,55){\makebox(0,0)[cc]{$\nameiota$}}

\put(75,45){\makebox(0,0)[cc]{\Dottt}}

\put(75,15){\makebox(0,0)[cc]{\Dottt}}

\put(72.5,1.25){\makebox(0,0)[cr]{$\Progtype$}}

\put(17.5,128.75){\makebox(0,0)[cl]{$\Progtype$}}

\put(77.5,128.75){\makebox(0,0)[cl]{$\Progtype$}}

\end{picture}


==> PIC/costless-order.tex <==
%%Created by jPicEdt 1.4.1_03: mixed JPIC-XML/LaTeX format
%%Sat Nov 26 21:27:04 GMT-10:00 2022
%%Begin JPIC-XML
%<?xml version="1.0" standalone="yes"?>
%<jpic x-min="0" x-max="150" y-min="0" y-max="60" auto-bounding="true">
%<multicurve fill-style= "none"
%	 stroke-width= "0.35"
%	 points= "(145,20);(145,20);(135,10);(135,10)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.35"
%	 points= "(135,10);(135,10);(135,0);(135,0)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.35"
%	 points= "(120,25);(120,25);(130,25);(130,25)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.35"
%	 points= "(125,25);(125,25);(125,20);(125,20)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.35"
%	 points= "(125,20);(125,20);(135,10);(135,10)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.35"
%	 points= "(145,25);(145,25);(145,20);(145,20)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.35"
%	 points= "(140,25);(140,25);(150,25);(150,25)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.35"
%	 points= "(140,35);(140,35);(150,35);(150,35)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.35"
%	 points= "(120,35);(120,35);(130,35);(130,35)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.35"
%	 points= "(130,35);(130,35);(130,25);(130,25)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.35"
%	 points= "(140,35);(140,35);(140,25);(140,25)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.35"
%	 points= "(150,35);(150,35);(150,25);(150,25)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.35"
%	 points= "(120,35);(120,35);(120,25);(120,25)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.35"
%	 points= "(125,40);(125,40);(125,35);(125,35)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.35"
%	 points= "(145,40);(145,40);(145,35);(145,35)"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 stroke-width= "0.35"
%	 anchor-point= "(132.5,1.25)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\AAh$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 stroke-width= "0.35"
%	 anchor-point= "(137.5,58.75)"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\BBh$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(145,40)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\Dottt
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(135,10)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\Dottt
%</text>
%<multicurve fill-style= "none"
%	 stroke-width= "0.35"
%	 points= "(135,50);(135,50);(125,40);(125,40)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.35"
%	 points= "(135,60);(135,60);(135,50);(135,50)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.35"
%	 points= "(95,25);(95,25);(105,25);(105,25)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.35"
%	 points= "(100,25);(100,25);(100,0);(100,0)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.35"
%	 points= "(95,35);(95,35);(105,35);(105,35)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.35"
%	 points= "(105,35);(105,35);(105,25);(105,25)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.35"
%	 points= "(95,35);(95,35);(95,25);(95,25)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.35"
%	 points= "(100,60);(100,60);(100,35);(100,35)"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 stroke-width= "0.35"
%	 anchor-point= "(100,30)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\aah$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 stroke-width= "0.35"
%	 anchor-point= "(97.5,1.25)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\AAh$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(112.5,30)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\EQLS
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 stroke-width= "0.35"
%	 anchor-point= "(145,30)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\aah$
%</text>
%<multicurve fill-style= "none"
%	 stroke-width= "0.35"
%	 points= "(0,25);(0,25);(10,25);(10,25)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.35"
%	 points= "(5,25);(5,25);(5,0);(5,0)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.35"
%	 points= "(0,35);(0,35);(10,35);(10,35)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.35"
%	 points= "(10,35);(10,35);(10,25);(10,25)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.35"
%	 points= "(0,35);(0,35);(0,25);(0,25)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.35"
%	 points= "(5,60);(5,60);(5,35);(5,35)"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 stroke-width= "0.35"
%	 anchor-point= "(5,30)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\aah$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 stroke-width= "0.35"
%	 anchor-point= "(2.5,1.25)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\AAh$
%</text>
%<multicurve fill-style= "none"
%	 stroke-width= "0.35"
%	 points= "(25,25);(25,25);(35,25);(35,25)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.35"
%	 points= "(30,25);(30,25);(30,0);(30,0)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.35"
%	 points= "(25,35);(25,35);(35,35);(35,35)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.35"
%	 points= "(35,35);(35,35);(35,25);(35,25)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.35"
%	 points= "(25,35);(25,35);(25,25);(25,25)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.35"
%	 points= "(30,60);(30,60);(30,35);(30,35)"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 stroke-width= "0.35"
%	 anchor-point= "(27.5,1.25)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\AAh$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(17.5,30)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\ILT$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(65,30)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\HIIF
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 stroke-width= "0.35"
%	 anchor-point= "(102.5,58.75)"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\BBh$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 stroke-width= "0.35"
%	 anchor-point= "(32.5,58.75)"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\BBh$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 stroke-width= "0.35"
%	 anchor-point= "(7.5,58.75)"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\BBh$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(30,30)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\baaah$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(125,30)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\baaah$
%</text>
%</jpic>
%%End JPIC-XML
%LaTeX-picture environment using emulated lines and arcs
%You can rescale the whole picture (to 80% for instance) by using the command \def\JPicScale{0.8}
\ifx\JPicScale\undefined\def\JPicScale{1}\fi
\unitlength \JPicScale mm
\begin{picture}(150,60)(0,0)
\linethickness{0.35mm}
\multiput(135,10)(0.12,0.12){83}{\line(1,0){0.12}}
\linethickness{0.35mm}
\put(135,0){\line(0,1){10}}
\linethickness{0.35mm}
\put(120,25){\line(1,0){10}}
\linethickness{0.35mm}
\put(125,20){\line(0,1){5}}
\linethickness{0.35mm}
\multiput(125,20)(0.12,-0.12){83}{\line(1,0){0.12}}
\linethickness{0.35mm}
\put(145,20){\line(0,1){5}}
\linethickness{0.35mm}
\put(140,25){\line(1,0){10}}
\linethickness{0.35mm}
\put(140,35){\line(1,0){10}}
\linethickness{0.35mm}
\put(120,35){\line(1,0){10}}
\linethickness{0.35mm}
\put(130,25){\line(0,1){10}}
\linethickness{0.35mm}
\put(140,25){\line(0,1){10}}
\linethickness{0.35mm}
\put(150,25){\line(0,1){10}}
\linethickness{0.35mm}
\put(120,25){\line(0,1){10}}
\linethickness{0.35mm}
\put(125,35){\line(0,1){5}}
\linethickness{0.35mm}
\put(145,35){\line(0,1){5}}
\put(132.5,1.25){\makebox(0,0)[cr]{$\AAh$}}

\put(137.5,58.75){\makebox(0,0)[cl]{$\BBh$}}

\put(145,40){\makebox(0,0)[cc]{\Dottt}}

\put(135,10){\makebox(0,0)[cc]{\Dottt}}

\linethickness{0.35mm}
\multiput(125,40)(0.12,0.12){83}{\line(1,0){0.12}}
\linethickness{0.35mm}
\put(135,50){\line(0,1){10}}
\linethickness{0.35mm}
\put(95,25){\line(1,0){10}}
\linethickness{0.35mm}
\put(100,0){\line(0,1){25}}
\linethickness{0.35mm}
\put(95,35){\line(1,0){10}}
\linethickness{0.35mm}
\put(105,25){\line(0,1){10}}
\linethickness{0.35mm}
\put(95,25){\line(0,1){10}}
\linethickness{0.35mm}
\put(100,35){\line(0,1){25}}
\put(100,30){\makebox(0,0)[cc]{$\aah$}}

\put(97.5,1.25){\makebox(0,0)[cr]{$\AAh$}}

\put(112.5,30){\makebox(0,0)[cc]{\EQLS}}

\put(145,30){\makebox(0,0)[cc]{$\aah$}}

\linethickness{0.35mm}
\put(0,25){\line(1,0){10}}
\linethickness{0.35mm}
\put(5,0){\line(0,1){25}}
\linethickness{0.35mm}
\put(0,35){\line(1,0){10}}
\linethickness{0.35mm}
\put(10,25){\line(0,1){10}}
\linethickness{0.35mm}
\put(0,25){\line(0,1){10}}
\linethickness{0.35mm}
\put(5,35){\line(0,1){25}}
\put(5,30){\makebox(0,0)[cc]{$\aah$}}

\put(2.5,1.25){\makebox(0,0)[cr]{$\AAh$}}

\linethickness{0.35mm}
\put(25,25){\line(1,0){10}}
\linethickness{0.35mm}
\put(30,0){\line(0,1){25}}
\linethickness{0.35mm}
\put(25,35){\line(1,0){10}}
\linethickness{0.35mm}
\put(35,25){\line(0,1){10}}
\linethickness{0.35mm}
\put(25,25){\line(0,1){10}}
\linethickness{0.35mm}
\put(30,35){\line(0,1){25}}
\put(27.5,1.25){\makebox(0,0)[cr]{$\AAh$}}

\put(17.5,30){\makebox(0,0)[cc]{$\ILT$}}

\put(65,30){\makebox(0,0)[cc]{\HIIF}}

\put(102.5,58.75){\makebox(0,0)[cl]{$\BBh$}}

\put(32.5,58.75){\makebox(0,0)[cl]{$\BBh$}}

\put(7.5,58.75){\makebox(0,0)[cl]{$\BBh$}}

\put(30,30){\makebox(0,0)[cc]{$\baaah$}}

\put(125,30){\makebox(0,0)[cc]{$\baaah$}}

\end{picture}


==> PIC/costless-trans-three.tex <==
%%Created by jPicEdt 1.4.1_03: mixed JPIC-XML/LaTeX format
%%Mon Nov 28 00:18:42 GMT-10:00 2022
%%Begin JPIC-XML
%<?xml version="1.0" standalone="yes"?>
%<jpic x-min="0" x-max="195" y-min="0" y-max="190" auto-bounding="true">
%<multicurve fill-style= "none"
%	 stroke-width= "0.35"
%	 points= "(135,135);(135,135);(125,125);(125,125)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.35"
%	 points= "(110,140);(110,140);(120,140);(120,140)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.35"
%	 points= "(115,140);(115,140);(115,135);(115,135)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.35"
%	 points= "(135,140);(135,140);(135,135);(135,135)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.35"
%	 points= "(130,140);(130,140);(140,140);(140,140)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.35"
%	 points= "(130,150);(130,150);(140,150);(140,150)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.35"
%	 points= "(110,150);(110,150);(120,150);(120,150)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.35"
%	 points= "(120,150);(120,150);(120,140);(120,140)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.35"
%	 points= "(130,150);(130,150);(130,140);(130,140)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.35"
%	 points= "(140,150);(140,150);(140,140);(140,140)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.35"
%	 points= "(110,150);(110,150);(110,140);(110,140)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.35"
%	 points= "(115,155);(115,155);(115,150);(115,150)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.35"
%	 points= "(135,155);(135,155);(135,150);(135,150)"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 stroke-width= "0.35"
%	 anchor-point= "(142.5,188.75)"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\BBh$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(135,155)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\Dottt
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(125,125)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\Dottt
%</text>
%<multicurve fill-style= "none"
%	 stroke-width= "0.35"
%	 points= "(140,180);(140,180);(115,155);(115,155)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.35"
%	 points= "(140,190);(140,190);(140,180);(140,180)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.35"
%	 points= "(0,140);(0,140);(10,140);(10,140)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.35"
%	 points= "(5,140);(5,140);(5,100);(5,100)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.35"
%	 points= "(0,150);(0,150);(10,150);(10,150)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.35"
%	 points= "(10,150);(10,150);(10,140);(10,140)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.35"
%	 points= "(0,150);(0,150);(0,140);(0,140)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.35"
%	 points= "(5,190);(5,190);(5,150);(5,150)"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 stroke-width= "0.35"
%	 anchor-point= "(5,145)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\aah$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 stroke-width= "0.35"
%	 anchor-point= "(2.5,101.25)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\AAh$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 stroke-width= "0.35"
%	 anchor-point= "(7.5,188.75)"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\BBh$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(135,145)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\baaah$
%</text>
%<multicurve fill-style= "none"
%	 stroke-width= "0.35"
%	 points= "(155,125);(155,125);(140,110);(140,110)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.35"
%	 points= "(140,110);(140,110);(140,100);(140,100)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.35"
%	 points= "(115,135);(115,135);(140,110);(140,110)"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 stroke-width= "0.35"
%	 anchor-point= "(137.5,101.25)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\AAh$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(140,110)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\Dottt
%</text>
%<multicurve fill-style= "none"
%	 stroke-width= "0.35"
%	 points= "(155,140);(155,140);(155,125);(155,125)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.35"
%	 points= "(150,140);(150,140);(160,140);(160,140)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.35"
%	 points= "(150,150);(150,150);(160,150);(160,150)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.35"
%	 points= "(150,150);(150,150);(150,140);(150,140)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.35"
%	 points= "(160,150);(160,150);(160,140);(160,140)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.35"
%	 points= "(155,165);(155,165);(155,150);(155,150)"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(155,165)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\Dottt
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 stroke-width= "0.35"
%	 anchor-point= "(155,145)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\aah$
%</text>
%<multicurve fill-style= "none"
%	 stroke-width= "0.35"
%	 points= "(40,140);(40,140);(50,140);(50,140)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.35"
%	 points= "(45,140);(45,140);(45,125);(45,125)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.35"
%	 points= "(40,150);(40,150);(50,150);(50,150)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.35"
%	 points= "(50,150);(50,150);(50,140);(50,140)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.35"
%	 points= "(40,150);(40,150);(40,140);(40,140)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.35"
%	 points= "(45,165);(45,165);(45,150);(45,150)"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 stroke-width= "0.35"
%	 anchor-point= "(62.5,188.75)"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\BBh$
%</text>
%<multicurve fill-style= "none"
%	 stroke-width= "0.35"
%	 points= "(60,180);(60,180);(45,165);(45,165)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.35"
%	 points= "(60,190);(60,190);(60,180);(60,180)"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(45,145)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\baaah$
%</text>
%<multicurve fill-style= "none"
%	 stroke-width= "0.35"
%	 points= "(75,125);(75,125);(60,110);(60,110)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.35"
%	 points= "(60,110);(60,110);(60,100);(60,100)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.35"
%	 points= "(45,125);(45,125);(60,110);(60,110)"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 stroke-width= "0.35"
%	 anchor-point= "(57.5,101.25)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\AAh$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(60,110)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\Dottt
%</text>
%<multicurve fill-style= "none"
%	 stroke-width= "0.35"
%	 points= "(75,140);(75,140);(75,125);(75,125)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.35"
%	 points= "(70,140);(70,140);(80,140);(80,140)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.35"
%	 points= "(70,150);(70,150);(80,150);(80,150)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.35"
%	 points= "(70,150);(70,150);(70,140);(70,140)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.35"
%	 points= "(80,150);(80,150);(80,140);(80,140)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.35"
%	 points= "(75,165);(75,165);(75,150);(75,150)"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(75,165)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\Dottt
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 stroke-width= "0.35"
%	 anchor-point= "(75,145)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\aah$
%</text>
%<multicurve fill-style= "none"
%	 stroke-width= "0.35"
%	 points= "(100,35);(100,35);(110,25);(110,25)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.35"
%	 points= "(95,40);(95,40);(105,40);(105,40)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.35"
%	 points= "(100,40);(100,40);(100,35);(100,35)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.35"
%	 points= "(120,40);(120,40);(120,35);(120,35)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.35"
%	 points= "(115,40);(115,40);(125,40);(125,40)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.35"
%	 points= "(115,50);(115,50);(125,50);(125,50)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.35"
%	 points= "(95,50);(95,50);(105,50);(105,50)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.35"
%	 points= "(105,50);(105,50);(105,40);(105,40)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.35"
%	 points= "(115,50);(115,50);(115,40);(115,40)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.35"
%	 points= "(125,50);(125,50);(125,40);(125,40)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.35"
%	 points= "(95,50);(95,50);(95,40);(95,40)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.35"
%	 points= "(100,65);(100,65);(100,50);(100,50)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.35"
%	 points= "(120,55);(120,55);(120,50);(120,50)"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 stroke-width= "0.35"
%	 anchor-point= "(97.5,88.75)"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\BBh$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(100,65)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\Dottt
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(110,25)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\Dottt
%</text>
%<multicurve fill-style= "none"
%	 stroke-width= "0.35"
%	 points= "(95,80);(95,80);(80,65);(80,65)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.35"
%	 points= "(95,90);(95,90);(95,80);(95,80)"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 stroke-width= "0.35"
%	 anchor-point= "(120,45)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\aah$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(100,45)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\baaah$
%</text>
%<multicurve fill-style= "none"
%	 stroke-width= "0.35"
%	 points= "(120,35);(120,35);(95,10);(95,10)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.35"
%	 points= "(95,10);(95,10);(95,0);(95,0)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.35"
%	 points= "(80,25);(80,25);(95,10);(95,10)"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 stroke-width= "0.35"
%	 anchor-point= "(92.5,1.25)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\AAh$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(95,10)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\Dottt
%</text>
%<multicurve fill-style= "none"
%	 stroke-width= "0.35"
%	 points= "(80,40);(80,40);(80,25);(80,25)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.35"
%	 points= "(75,40);(75,40);(85,40);(85,40)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.35"
%	 points= "(75,50);(75,50);(85,50);(85,50)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.35"
%	 points= "(75,50);(75,50);(75,40);(75,40)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.35"
%	 points= "(85,50);(85,50);(85,40);(85,40)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.35"
%	 points= "(80,65);(80,65);(80,50);(80,50)"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(120,55)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\Dottt
%</text>
%<multicurve fill-style= "none"
%	 stroke-width= "0.35"
%	 points= "(155,40);(155,40);(165,40);(165,40)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.35"
%	 points= "(160,40);(160,40);(160,25);(160,25)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.35"
%	 points= "(155,50);(155,50);(165,50);(165,50)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.35"
%	 points= "(165,50);(165,50);(165,40);(165,40)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.35"
%	 points= "(155,50);(155,50);(155,40);(155,40)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.35"
%	 points= "(160,65);(160,65);(160,50);(160,50)"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 stroke-width= "0.35"
%	 anchor-point= "(177.5,88.75)"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\BBh$
%</text>
%<multicurve fill-style= "none"
%	 stroke-width= "0.35"
%	 points= "(175,80);(175,80);(160,65);(160,65)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.35"
%	 points= "(175,90);(175,90);(175,80);(175,80)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.35"
%	 points= "(190,25);(190,25);(175,10);(175,10)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.35"
%	 points= "(175,10);(175,10);(175,0);(175,0)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.35"
%	 points= "(160,25);(160,25);(175,10);(175,10)"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 stroke-width= "0.35"
%	 anchor-point= "(172.5,1.25)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\AAh$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(175,10)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\Dottt
%</text>
%<multicurve fill-style= "none"
%	 stroke-width= "0.35"
%	 points= "(190,40);(190,40);(190,25);(190,25)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.35"
%	 points= "(185,40);(185,40);(195,40);(195,40)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.35"
%	 points= "(185,50);(185,50);(195,50);(195,50)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.35"
%	 points= "(185,50);(185,50);(185,40);(185,40)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.35"
%	 points= "(195,50);(195,50);(195,40);(195,40)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.35"
%	 points= "(190,65);(190,65);(190,50);(190,50)"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(190,65)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\Dottt
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 stroke-width= "0.35"
%	 anchor-point= "(190,45)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\aah$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(160,45)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\caaah$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(80,45)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\caaah$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(115,145)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\caaah$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(25,147.5)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\EQLSone
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(95,147.5)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\EQLStwo
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(180,147.5)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\EQLSthree
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(140,47.5)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\EQLSfour
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(55,47.5)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\EQLSthree
%</text>
%</jpic>
%%End JPIC-XML
%LaTeX-picture environment using emulated lines and arcs
%You can rescale the whole picture (to 80% for instance) by using the command \def\JPicScale{0.8}
\ifx\JPicScale\undefined\def\JPicScale{1}\fi
\unitlength \JPicScale mm
\begin{picture}(195,190)(0,0)
\linethickness{0.35mm}
\multiput(125,125)(0.12,0.12){83}{\line(1,0){0.12}}
\linethickness{0.35mm}
\put(110,140){\line(1,0){10}}
\linethickness{0.35mm}
\put(115,135){\line(0,1){5}}
\linethickness{0.35mm}
\put(135,135){\line(0,1){5}}
\linethickness{0.35mm}
\put(130,140){\line(1,0){10}}
\linethickness{0.35mm}
\put(130,150){\line(1,0){10}}
\linethickness{0.35mm}
\put(110,150){\line(1,0){10}}
\linethickness{0.35mm}
\put(120,140){\line(0,1){10}}
\linethickness{0.35mm}
\put(130,140){\line(0,1){10}}
\linethickness{0.35mm}
\put(140,140){\line(0,1){10}}
\linethickness{0.35mm}
\put(110,140){\line(0,1){10}}
\linethickness{0.35mm}
\put(115,150){\line(0,1){5}}
\linethickness{0.35mm}
\put(135,150){\line(0,1){5}}
\put(142.5,188.75){\makebox(0,0)[cl]{$\BBh$}}

\put(135,155){\makebox(0,0)[cc]{\Dottt}}

\put(125,125){\makebox(0,0)[cc]{\Dottt}}

\linethickness{0.35mm}
\multiput(115,155)(0.12,0.12){208}{\line(1,0){0.12}}
\linethickness{0.35mm}
\put(140,180){\line(0,1){10}}
\linethickness{0.35mm}
\put(0,140){\line(1,0){10}}
\linethickness{0.35mm}
\put(5,100){\line(0,1){40}}
\linethickness{0.35mm}
\put(0,150){\line(1,0){10}}
\linethickness{0.35mm}
\put(10,140){\line(0,1){10}}
\linethickness{0.35mm}
\put(0,140){\line(0,1){10}}
\linethickness{0.35mm}
\put(5,150){\line(0,1){40}}
\put(5,145){\makebox(0,0)[cc]{$\aah$}}

\put(2.5,101.25){\makebox(0,0)[cr]{$\AAh$}}

\put(7.5,188.75){\makebox(0,0)[cl]{$\BBh$}}

\put(135,145){\makebox(0,0)[cc]{$\baaah$}}

\linethickness{0.35mm}
\multiput(140,110)(0.12,0.12){125}{\line(1,0){0.12}}
\linethickness{0.35mm}
\put(140,100){\line(0,1){10}}
\linethickness{0.35mm}
\multiput(115,135)(0.12,-0.12){208}{\line(1,0){0.12}}
\put(137.5,101.25){\makebox(0,0)[cr]{$\AAh$}}

\put(140,110){\makebox(0,0)[cc]{\Dottt}}

\linethickness{0.35mm}
\put(155,125){\line(0,1){15}}
\linethickness{0.35mm}
\put(150,140){\line(1,0){10}}
\linethickness{0.35mm}
\put(150,150){\line(1,0){10}}
\linethickness{0.35mm}
\put(150,140){\line(0,1){10}}
\linethickness{0.35mm}
\put(160,140){\line(0,1){10}}
\linethickness{0.35mm}
\put(155,150){\line(0,1){15}}
\put(155,165){\makebox(0,0)[cc]{\Dottt}}

\put(155,145){\makebox(0,0)[cc]{$\aah$}}

\linethickness{0.35mm}
\put(40,140){\line(1,0){10}}
\linethickness{0.35mm}
\put(45,125){\line(0,1){15}}
\linethickness{0.35mm}
\put(40,150){\line(1,0){10}}
\linethickness{0.35mm}
\put(50,140){\line(0,1){10}}
\linethickness{0.35mm}
\put(40,140){\line(0,1){10}}
\linethickness{0.35mm}
\put(45,150){\line(0,1){15}}
\put(62.5,188.75){\makebox(0,0)[cl]{$\BBh$}}

\linethickness{0.35mm}
\multiput(45,165)(0.12,0.12){125}{\line(1,0){0.12}}
\linethickness{0.35mm}
\put(60,180){\line(0,1){10}}
\put(45,145){\makebox(0,0)[cc]{$\baaah$}}

\linethickness{0.35mm}
\multiput(60,110)(0.12,0.12){125}{\line(1,0){0.12}}
\linethickness{0.35mm}
\put(60,100){\line(0,1){10}}
\linethickness{0.35mm}
\multiput(45,125)(0.12,-0.12){125}{\line(1,0){0.12}}
\put(57.5,101.25){\makebox(0,0)[cr]{$\AAh$}}

\put(60,110){\makebox(0,0)[cc]{\Dottt}}

\linethickness{0.35mm}
\put(75,125){\line(0,1){15}}
\linethickness{0.35mm}
\put(70,140){\line(1,0){10}}
\linethickness{0.35mm}
\put(70,150){\line(1,0){10}}
\linethickness{0.35mm}
\put(70,140){\line(0,1){10}}
\linethickness{0.35mm}
\put(80,140){\line(0,1){10}}
\linethickness{0.35mm}
\put(75,150){\line(0,1){15}}
\put(75,165){\makebox(0,0)[cc]{\Dottt}}

\put(75,145){\makebox(0,0)[cc]{$\aah$}}

\linethickness{0.35mm}
\multiput(100,35)(0.12,-0.12){83}{\line(1,0){0.12}}
\linethickness{0.35mm}
\put(95,40){\line(1,0){10}}
\linethickness{0.35mm}
\put(100,35){\line(0,1){5}}
\linethickness{0.35mm}
\put(120,35){\line(0,1){5}}
\linethickness{0.35mm}
\put(115,40){\line(1,0){10}}
\linethickness{0.35mm}
\put(115,50){\line(1,0){10}}
\linethickness{0.35mm}
\put(95,50){\line(1,0){10}}
\linethickness{0.35mm}
\put(105,40){\line(0,1){10}}
\linethickness{0.35mm}
\put(115,40){\line(0,1){10}}
\linethickness{0.35mm}
\put(125,40){\line(0,1){10}}
\linethickness{0.35mm}
\put(95,40){\line(0,1){10}}
\linethickness{0.35mm}
\put(100,50){\line(0,1){15}}
\linethickness{0.35mm}
\put(120,50){\line(0,1){5}}
\put(97.5,88.75){\makebox(0,0)[cl]{$\BBh$}}

\put(100,65){\makebox(0,0)[cc]{\Dottt}}

\put(110,25){\makebox(0,0)[cc]{\Dottt}}

\linethickness{0.35mm}
\multiput(80,65)(0.12,0.12){125}{\line(1,0){0.12}}
\linethickness{0.35mm}
\put(95,80){\line(0,1){10}}
\put(120,45){\makebox(0,0)[cc]{$\aah$}}

\put(100,45){\makebox(0,0)[cc]{$\baaah$}}

\linethickness{0.35mm}
\multiput(95,10)(0.12,0.12){208}{\line(1,0){0.12}}
\linethickness{0.35mm}
\put(95,0){\line(0,1){10}}
\linethickness{0.35mm}
\multiput(80,25)(0.12,-0.12){125}{\line(1,0){0.12}}
\put(92.5,1.25){\makebox(0,0)[cr]{$\AAh$}}

\put(95,10){\makebox(0,0)[cc]{\Dottt}}

\linethickness{0.35mm}
\put(80,25){\line(0,1){15}}
\linethickness{0.35mm}
\put(75,40){\line(1,0){10}}
\linethickness{0.35mm}
\put(75,50){\line(1,0){10}}
\linethickness{0.35mm}
\put(75,40){\line(0,1){10}}
\linethickness{0.35mm}
\put(85,40){\line(0,1){10}}
\linethickness{0.35mm}
\put(80,50){\line(0,1){15}}
\put(120,55){\makebox(0,0)[cc]{\Dottt}}

\linethickness{0.35mm}
\put(155,40){\line(1,0){10}}
\linethickness{0.35mm}
\put(160,25){\line(0,1){15}}
\linethickness{0.35mm}
\put(155,50){\line(1,0){10}}
\linethickness{0.35mm}
\put(165,40){\line(0,1){10}}
\linethickness{0.35mm}
\put(155,40){\line(0,1){10}}
\linethickness{0.35mm}
\put(160,50){\line(0,1){15}}
\put(177.5,88.75){\makebox(0,0)[cl]{$\BBh$}}

\linethickness{0.35mm}
\multiput(160,65)(0.12,0.12){125}{\line(1,0){0.12}}
\linethickness{0.35mm}
\put(175,80){\line(0,1){10}}
\linethickness{0.35mm}
\multiput(175,10)(0.12,0.12){125}{\line(1,0){0.12}}
\linethickness{0.35mm}
\put(175,0){\line(0,1){10}}
\linethickness{0.35mm}
\multiput(160,25)(0.12,-0.12){125}{\line(1,0){0.12}}
\put(172.5,1.25){\makebox(0,0)[cr]{$\AAh$}}

\put(175,10){\makebox(0,0)[cc]{\Dottt}}

\linethickness{0.35mm}
\put(190,25){\line(0,1){15}}
\linethickness{0.35mm}
\put(185,40){\line(1,0){10}}
\linethickness{0.35mm}
\put(185,50){\line(1,0){10}}
\linethickness{0.35mm}
\put(185,40){\line(0,1){10}}
\linethickness{0.35mm}
\put(195,40){\line(0,1){10}}
\linethickness{0.35mm}
\put(190,50){\line(0,1){15}}
\put(190,65){\makebox(0,0)[cc]{\Dottt}}

\put(190,45){\makebox(0,0)[cc]{$\aah$}}

\put(160,45){\makebox(0,0)[cc]{$\caaah$}}

\put(80,45){\makebox(0,0)[cc]{$\caaah$}}

\put(115,145){\makebox(0,0)[cc]{$\caaah$}}

\put(25,147.5){\makebox(0,0)[cc]{\EQLSone}}

\put(95,147.5){\makebox(0,0)[cc]{\EQLStwo}}

\put(180,147.5){\makebox(0,0)[cc]{\EQLSthree}}

\put(140,47.5){\makebox(0,0)[cc]{\EQLSfour}}

\put(55,47.5){\makebox(0,0)[cc]{\EQLSthree}}

\end{picture}


==> PIC/costless-trans-two.tex <==
%%Created by jPicEdt 1.4.1_03: mixed JPIC-XML/LaTeX format
%%Sun Nov 27 16:55:57 GMT-10:00 2022
%%Begin JPIC-XML
%<?xml version="1.0" standalone="yes"?>
%<jpic x-min="0" x-max="210" y-min="0" y-max="200" auto-bounding="true">
%<multicurve fill-style= "none"
%	 stroke-width= "0.35"
%	 points= "(115,145);(115,145);(105,135);(105,135)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.35"
%	 points= "(90,150);(90,150);(100,150);(100,150)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.35"
%	 points= "(95,150);(95,150);(95,145);(95,145)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.35"
%	 points= "(115,150);(115,150);(115,145);(115,145)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.35"
%	 points= "(110,150);(110,150);(120,150);(120,150)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.35"
%	 points= "(110,160);(110,160);(120,160);(120,160)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.35"
%	 points= "(90,160);(90,160);(100,160);(100,160)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.35"
%	 points= "(100,160);(100,160);(100,150);(100,150)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.35"
%	 points= "(110,160);(110,160);(110,150);(110,150)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.35"
%	 points= "(120,160);(120,160);(120,150);(120,150)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.35"
%	 points= "(90,160);(90,160);(90,150);(90,150)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.35"
%	 points= "(95,165);(95,165);(95,160);(95,160)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.35"
%	 points= "(115,165);(115,165);(115,160);(115,160)"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 stroke-width= "0.35"
%	 anchor-point= "(122.5,198.75)"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\BBh$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(115,165)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\Dottt
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(105,135)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\Dottt
%</text>
%<multicurve fill-style= "none"
%	 stroke-width= "0.35"
%	 points= "(120,190);(120,190);(95,165);(95,165)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.35"
%	 points= "(120,200);(120,200);(120,190);(120,190)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.35"
%	 points= "(0,150);(0,150);(10,150);(10,150)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.35"
%	 points= "(5,150);(5,150);(5,110);(5,110)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.35"
%	 points= "(0,160);(0,160);(10,160);(10,160)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.35"
%	 points= "(10,160);(10,160);(10,150);(10,150)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.35"
%	 points= "(0,160);(0,160);(0,150);(0,150)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.35"
%	 points= "(5,200);(5,200);(5,160);(5,160)"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 stroke-width= "0.35"
%	 anchor-point= "(5,155)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\aah$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 stroke-width= "0.35"
%	 anchor-point= "(2.5,111.25)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\AAh$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 stroke-width= "0.35"
%	 anchor-point= "(7.5,198.75)"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\BBh$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(115,155)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\baaah$
%</text>
%<multicurve fill-style= "none"
%	 stroke-width= "0.35"
%	 points= "(135,135);(135,135);(120,120);(120,120)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.35"
%	 points= "(120,120);(120,120);(120,110);(120,110)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.35"
%	 points= "(95,145);(95,145);(120,120);(120,120)"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 stroke-width= "0.35"
%	 anchor-point= "(117.5,111.25)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\AAh$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(120,120)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\Dottt
%</text>
%<multicurve fill-style= "none"
%	 stroke-width= "0.35"
%	 points= "(135,150);(135,150);(135,135);(135,135)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.35"
%	 points= "(130,150);(130,150);(140,150);(140,150)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.35"
%	 points= "(130,160);(130,160);(140,160);(140,160)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.35"
%	 points= "(130,160);(130,160);(130,150);(130,150)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.35"
%	 points= "(140,160);(140,160);(140,150);(140,150)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.35"
%	 points= "(135,175);(135,175);(135,160);(135,160)"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(135,175)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\Dottt
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 stroke-width= "0.35"
%	 anchor-point= "(135,155)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\aah$
%</text>
%<multicurve fill-style= "none"
%	 stroke-width= "0.35"
%	 points= "(30,150);(30,150);(40,150);(40,150)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.35"
%	 points= "(35,150);(35,150);(35,135);(35,135)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.35"
%	 points= "(30,160);(30,160);(40,160);(40,160)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.35"
%	 points= "(40,160);(40,160);(40,150);(40,150)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.35"
%	 points= "(30,160);(30,160);(30,150);(30,150)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.35"
%	 points= "(35,175);(35,175);(35,160);(35,160)"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 stroke-width= "0.35"
%	 anchor-point= "(52.5,198.75)"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\BBh$
%</text>
%<multicurve fill-style= "none"
%	 stroke-width= "0.35"
%	 points= "(50,190);(50,190);(35,175);(35,175)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.35"
%	 points= "(50,200);(50,200);(50,190);(50,190)"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(35,155)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\baaah$
%</text>
%<multicurve fill-style= "none"
%	 stroke-width= "0.35"
%	 points= "(65,135);(65,135);(50,120);(50,120)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.35"
%	 points= "(50,120);(50,120);(50,110);(50,110)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.35"
%	 points= "(35,135);(35,135);(50,120);(50,120)"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 stroke-width= "0.35"
%	 anchor-point= "(47.5,111.25)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\AAh$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(50,120)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\Dottt
%</text>
%<multicurve fill-style= "none"
%	 stroke-width= "0.35"
%	 points= "(65,150);(65,150);(65,135);(65,135)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.35"
%	 points= "(60,150);(60,150);(70,150);(70,150)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.35"
%	 points= "(60,160);(60,160);(70,160);(70,160)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.35"
%	 points= "(60,160);(60,160);(60,150);(60,150)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.35"
%	 points= "(70,160);(70,160);(70,150);(70,150)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.35"
%	 points= "(65,175);(65,175);(65,160);(65,160)"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(65,175)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\Dottt
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 stroke-width= "0.35"
%	 anchor-point= "(65,155)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\aah$
%</text>
%<multicurve fill-style= "none"
%	 stroke-width= "0.35"
%	 points= "(125,35);(125,35);(135,25);(135,25)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.35"
%	 points= "(120,40);(120,40);(130,40);(130,40)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.35"
%	 points= "(125,40);(125,40);(125,35);(125,35)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.35"
%	 points= "(145,40);(145,40);(145,35);(145,35)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.35"
%	 points= "(140,40);(140,40);(150,40);(150,40)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.35"
%	 points= "(140,50);(140,50);(150,50);(150,50)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.35"
%	 points= "(120,50);(120,50);(130,50);(130,50)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.35"
%	 points= "(130,50);(130,50);(130,40);(130,40)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.35"
%	 points= "(140,50);(140,50);(140,40);(140,40)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.35"
%	 points= "(150,50);(150,50);(150,40);(150,40)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.35"
%	 points= "(120,50);(120,50);(120,40);(120,40)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.35"
%	 points= "(125,65);(125,65);(125,50);(125,50)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.35"
%	 points= "(145,55);(145,55);(145,50);(145,50)"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 stroke-width= "0.35"
%	 anchor-point= "(122.5,88.75)"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\BBh$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(125,65)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\Dottt
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(135,25)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\Dottt
%</text>
%<multicurve fill-style= "none"
%	 stroke-width= "0.35"
%	 points= "(120,80);(120,80);(105,65);(105,65)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.35"
%	 points= "(120,90);(120,90);(120,80);(120,80)"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 stroke-width= "0.35"
%	 anchor-point= "(145,45)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\aah$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(125,45)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\baaah$
%</text>
%<multicurve fill-style= "none"
%	 stroke-width= "0.35"
%	 points= "(145,35);(145,35);(120,10);(120,10)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.35"
%	 points= "(120,10);(120,10);(120,0);(120,0)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.35"
%	 points= "(105,25);(105,25);(120,10);(120,10)"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 stroke-width= "0.35"
%	 anchor-point= "(117.5,1.25)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\AAh$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(120,10)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\Dottt
%</text>
%<multicurve fill-style= "none"
%	 stroke-width= "0.35"
%	 points= "(105,40);(105,40);(105,25);(105,25)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.35"
%	 points= "(100,40);(100,40);(110,40);(110,40)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.35"
%	 points= "(100,50);(100,50);(110,50);(110,50)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.35"
%	 points= "(100,50);(100,50);(100,40);(100,40)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.35"
%	 points= "(110,50);(110,50);(110,40);(110,40)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.35"
%	 points= "(105,65);(105,65);(105,50);(105,50)"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(145,55)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\Dottt
%</text>
%<multicurve fill-style= "none"
%	 stroke-width= "0.35"
%	 points= "(170,40);(170,40);(180,40);(180,40)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.35"
%	 points= "(175,40);(175,40);(175,25);(175,25)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.35"
%	 points= "(170,50);(170,50);(180,50);(180,50)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.35"
%	 points= "(180,50);(180,50);(180,40);(180,40)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.35"
%	 points= "(170,50);(170,50);(170,40);(170,40)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.35"
%	 points= "(175,65);(175,65);(175,50);(175,50)"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 stroke-width= "0.35"
%	 anchor-point= "(192.5,88.75)"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\BBh$
%</text>
%<multicurve fill-style= "none"
%	 stroke-width= "0.35"
%	 points= "(190,80);(190,80);(175,65);(175,65)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.35"
%	 points= "(190,90);(190,90);(190,80);(190,80)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.35"
%	 points= "(205,25);(205,25);(190,10);(190,10)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.35"
%	 points= "(190,10);(190,10);(190,0);(190,0)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.35"
%	 points= "(175,25);(175,25);(190,10);(190,10)"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 stroke-width= "0.35"
%	 anchor-point= "(187.5,1.25)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\AAh$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(190,10)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\Dottt
%</text>
%<multicurve fill-style= "none"
%	 stroke-width= "0.35"
%	 points= "(205,40);(205,40);(205,25);(205,25)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.35"
%	 points= "(200,40);(200,40);(210,40);(210,40)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.35"
%	 points= "(200,50);(200,50);(210,50);(210,50)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.35"
%	 points= "(200,50);(200,50);(200,40);(200,40)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.35"
%	 points= "(210,50);(210,50);(210,40);(210,40)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.35"
%	 points= "(205,65);(205,65);(205,50);(205,50)"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(205,65)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\Dottt
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 stroke-width= "0.35"
%	 anchor-point= "(205,45)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\aah$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(175,45)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\caaah$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(105,45)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\caaah$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(95,155)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\caaah$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(20,155)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\EQLSone
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(80,155)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\EQLStwo
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(160,155)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\EQLSthree
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(160,45)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\EQLSfour
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(80,45)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\EQLSthree
%</text>
%</jpic>
%%End JPIC-XML
%LaTeX-picture environment using emulated lines and arcs
%You can rescale the whole picture (to 80% for instance) by using the command \def\JPicScale{0.8}
\ifx\JPicScale\undefined\def\JPicScale{1}\fi
\unitlength \JPicScale mm
\begin{picture}(210,200)(0,0)
\linethickness{0.35mm}
\multiput(105,135)(0.12,0.12){83}{\line(1,0){0.12}}
\linethickness{0.35mm}
\put(90,150){\line(1,0){10}}
\linethickness{0.35mm}
\put(95,145){\line(0,1){5}}
\linethickness{0.35mm}
\put(115,145){\line(0,1){5}}
\linethickness{0.35mm}
\put(110,150){\line(1,0){10}}
\linethickness{0.35mm}
\put(110,160){\line(1,0){10}}
\linethickness{0.35mm}
\put(90,160){\line(1,0){10}}
\linethickness{0.35mm}
\put(100,150){\line(0,1){10}}
\linethickness{0.35mm}
\put(110,150){\line(0,1){10}}
\linethickness{0.35mm}
\put(120,150){\line(0,1){10}}
\linethickness{0.35mm}
\put(90,150){\line(0,1){10}}
\linethickness{0.35mm}
\put(95,160){\line(0,1){5}}
\linethickness{0.35mm}
\put(115,160){\line(0,1){5}}
\put(122.5,198.75){\makebox(0,0)[cl]{$\BBh$}}

\put(115,165){\makebox(0,0)[cc]{\Dottt}}

\put(105,135){\makebox(0,0)[cc]{\Dottt}}

\linethickness{0.35mm}
\multiput(95,165)(0.12,0.12){208}{\line(1,0){0.12}}
\linethickness{0.35mm}
\put(120,190){\line(0,1){10}}
\linethickness{0.35mm}
\put(0,150){\line(1,0){10}}
\linethickness{0.35mm}
\put(5,110){\line(0,1){40}}
\linethickness{0.35mm}
\put(0,160){\line(1,0){10}}
\linethickness{0.35mm}
\put(10,150){\line(0,1){10}}
\linethickness{0.35mm}
\put(0,150){\line(0,1){10}}
\linethickness{0.35mm}
\put(5,160){\line(0,1){40}}
\put(5,155){\makebox(0,0)[cc]{$\aah$}}

\put(2.5,111.25){\makebox(0,0)[cr]{$\AAh$}}

\put(7.5,198.75){\makebox(0,0)[cl]{$\BBh$}}

\put(115,155){\makebox(0,0)[cc]{$\baaah$}}

\linethickness{0.35mm}
\multiput(120,120)(0.12,0.12){125}{\line(1,0){0.12}}
\linethickness{0.35mm}
\put(120,110){\line(0,1){10}}
\linethickness{0.35mm}
\multiput(95,145)(0.12,-0.12){208}{\line(1,0){0.12}}
\put(117.5,111.25){\makebox(0,0)[cr]{$\AAh$}}

\put(120,120){\makebox(0,0)[cc]{\Dottt}}

\linethickness{0.35mm}
\put(135,135){\line(0,1){15}}
\linethickness{0.35mm}
\put(130,150){\line(1,0){10}}
\linethickness{0.35mm}
\put(130,160){\line(1,0){10}}
\linethickness{0.35mm}
\put(130,150){\line(0,1){10}}
\linethickness{0.35mm}
\put(140,150){\line(0,1){10}}
\linethickness{0.35mm}
\put(135,160){\line(0,1){15}}
\put(135,175){\makebox(0,0)[cc]{\Dottt}}

\put(135,155){\makebox(0,0)[cc]{$\aah$}}

\linethickness{0.35mm}
\put(30,150){\line(1,0){10}}
\linethickness{0.35mm}
\put(35,135){\line(0,1){15}}
\linethickness{0.35mm}
\put(30,160){\line(1,0){10}}
\linethickness{0.35mm}
\put(40,150){\line(0,1){10}}
\linethickness{0.35mm}
\put(30,150){\line(0,1){10}}
\linethickness{0.35mm}
\put(35,160){\line(0,1){15}}
\put(52.5,198.75){\makebox(0,0)[cl]{$\BBh$}}

\linethickness{0.35mm}
\multiput(35,175)(0.12,0.12){125}{\line(1,0){0.12}}
\linethickness{0.35mm}
\put(50,190){\line(0,1){10}}
\put(35,155){\makebox(0,0)[cc]{$\baaah$}}

\linethickness{0.35mm}
\multiput(50,120)(0.12,0.12){125}{\line(1,0){0.12}}
\linethickness{0.35mm}
\put(50,110){\line(0,1){10}}
\linethickness{0.35mm}
\multiput(35,135)(0.12,-0.12){125}{\line(1,0){0.12}}
\put(47.5,111.25){\makebox(0,0)[cr]{$\AAh$}}

\put(50,120){\makebox(0,0)[cc]{\Dottt}}

\linethickness{0.35mm}
\put(65,135){\line(0,1){15}}
\linethickness{0.35mm}
\put(60,150){\line(1,0){10}}
\linethickness{0.35mm}
\put(60,160){\line(1,0){10}}
\linethickness{0.35mm}
\put(60,150){\line(0,1){10}}
\linethickness{0.35mm}
\put(70,150){\line(0,1){10}}
\linethickness{0.35mm}
\put(65,160){\line(0,1){15}}
\put(65,175){\makebox(0,0)[cc]{\Dottt}}

\put(65,155){\makebox(0,0)[cc]{$\aah$}}

\linethickness{0.35mm}
\multiput(125,35)(0.12,-0.12){83}{\line(1,0){0.12}}
\linethickness{0.35mm}
\put(120,40){\line(1,0){10}}
\linethickness{0.35mm}
\put(125,35){\line(0,1){5}}
\linethickness{0.35mm}
\put(145,35){\line(0,1){5}}
\linethickness{0.35mm}
\put(140,40){\line(1,0){10}}
\linethickness{0.35mm}
\put(140,50){\line(1,0){10}}
\linethickness{0.35mm}
\put(120,50){\line(1,0){10}}
\linethickness{0.35mm}
\put(130,40){\line(0,1){10}}
\linethickness{0.35mm}
\put(140,40){\line(0,1){10}}
\linethickness{0.35mm}
\put(150,40){\line(0,1){10}}
\linethickness{0.35mm}
\put(120,40){\line(0,1){10}}
\linethickness{0.35mm}
\put(125,50){\line(0,1){15}}
\linethickness{0.35mm}
\put(145,50){\line(0,1){5}}
\put(122.5,88.75){\makebox(0,0)[cl]{$\BBh$}}

\put(125,65){\makebox(0,0)[cc]{\Dottt}}

\put(135,25){\makebox(0,0)[cc]{\Dottt}}

\linethickness{0.35mm}
\multiput(105,65)(0.12,0.12){125}{\line(1,0){0.12}}
\linethickness{0.35mm}
\put(120,80){\line(0,1){10}}
\put(145,45){\makebox(0,0)[cc]{$\aah$}}

\put(125,45){\makebox(0,0)[cc]{$\baaah$}}

\linethickness{0.35mm}
\multiput(120,10)(0.12,0.12){208}{\line(1,0){0.12}}
\linethickness{0.35mm}
\put(120,0){\line(0,1){10}}
\linethickness{0.35mm}
\multiput(105,25)(0.12,-0.12){125}{\line(1,0){0.12}}
\put(117.5,1.25){\makebox(0,0)[cr]{$\AAh$}}

\put(120,10){\makebox(0,0)[cc]{\Dottt}}

\linethickness{0.35mm}
\put(105,25){\line(0,1){15}}
\linethickness{0.35mm}
\put(100,40){\line(1,0){10}}
\linethickness{0.35mm}
\put(100,50){\line(1,0){10}}
\linethickness{0.35mm}
\put(100,40){\line(0,1){10}}
\linethickness{0.35mm}
\put(110,40){\line(0,1){10}}
\linethickness{0.35mm}
\put(105,50){\line(0,1){15}}
\put(145,55){\makebox(0,0)[cc]{\Dottt}}

\linethickness{0.35mm}
\put(170,40){\line(1,0){10}}
\linethickness{0.35mm}
\put(175,25){\line(0,1){15}}
\linethickness{0.35mm}
\put(170,50){\line(1,0){10}}
\linethickness{0.35mm}
\put(180,40){\line(0,1){10}}
\linethickness{0.35mm}
\put(170,40){\line(0,1){10}}
\linethickness{0.35mm}
\put(175,50){\line(0,1){15}}
\put(192.5,88.75){\makebox(0,0)[cl]{$\BBh$}}

\linethickness{0.35mm}
\multiput(175,65)(0.12,0.12){125}{\line(1,0){0.12}}
\linethickness{0.35mm}
\put(190,80){\line(0,1){10}}
\linethickness{0.35mm}
\multiput(190,10)(0.12,0.12){125}{\line(1,0){0.12}}
\linethickness{0.35mm}
\put(190,0){\line(0,1){10}}
\linethickness{0.35mm}
\multiput(175,25)(0.12,-0.12){125}{\line(1,0){0.12}}
\put(187.5,1.25){\makebox(0,0)[cr]{$\AAh$}}

\put(190,10){\makebox(0,0)[cc]{\Dottt}}

\linethickness{0.35mm}
\put(205,25){\line(0,1){15}}
\linethickness{0.35mm}
\put(200,40){\line(1,0){10}}
\linethickness{0.35mm}
\put(200,50){\line(1,0){10}}
\linethickness{0.35mm}
\put(200,40){\line(0,1){10}}
\linethickness{0.35mm}
\put(210,40){\line(0,1){10}}
\linethickness{0.35mm}
\put(205,50){\line(0,1){15}}
\put(205,65){\makebox(0,0)[cc]{\Dottt}}

\put(205,45){\makebox(0,0)[cc]{$\aah$}}

\put(175,45){\makebox(0,0)[cc]{$\caaah$}}

\put(105,45){\makebox(0,0)[cc]{$\caaah$}}

\put(95,155){\makebox(0,0)[cc]{$\caaah$}}

\put(20,155){\makebox(0,0)[cc]{\EQLSone}}

\put(80,155){\makebox(0,0)[cc]{\EQLStwo}}

\put(160,155){\makebox(0,0)[cc]{\EQLSthree}}

\put(160,45){\makebox(0,0)[cc]{\EQLSfour}}

\put(80,45){\makebox(0,0)[cc]{\EQLSthree}}

\end{picture}


==> PIC/costless-trans.tex <==
%%Created by jPicEdt 1.4.1_03: mixed JPIC-XML/LaTeX format
%%Sun Nov 27 16:00:25 GMT-10:00 2022
%%Begin JPIC-XML
%<?xml version="1.0" standalone="yes"?>
%<jpic x-min="0" x-max="270" y-min="0" y-max="90" auto-bounding="true">
%<multicurve fill-style= "none"
%	 stroke-width= "0.35"
%	 points= "(115,35);(115,35);(105,25);(105,25)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.35"
%	 points= "(90,40);(90,40);(100,40);(100,40)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.35"
%	 points= "(95,40);(95,40);(95,35);(95,35)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.35"
%	 points= "(115,40);(115,40);(115,35);(115,35)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.35"
%	 points= "(110,40);(110,40);(120,40);(120,40)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.35"
%	 points= "(110,50);(110,50);(120,50);(120,50)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.35"
%	 points= "(90,50);(90,50);(100,50);(100,50)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.35"
%	 points= "(100,50);(100,50);(100,40);(100,40)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.35"
%	 points= "(110,50);(110,50);(110,40);(110,40)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.35"
%	 points= "(120,50);(120,50);(120,40);(120,40)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.35"
%	 points= "(90,50);(90,50);(90,40);(90,40)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.35"
%	 points= "(95,55);(95,55);(95,50);(95,50)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.35"
%	 points= "(115,55);(115,55);(115,50);(115,50)"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 stroke-width= "0.35"
%	 anchor-point= "(122.5,88.75)"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\BBh$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(115,55)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\Dottt
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(105,25)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\Dottt
%</text>
%<multicurve fill-style= "none"
%	 stroke-width= "0.35"
%	 points= "(120,80);(120,80);(95,55);(95,55)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.35"
%	 points= "(120,90);(120,90);(120,80);(120,80)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.35"
%	 points= "(0,40);(0,40);(10,40);(10,40)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.35"
%	 points= "(5,40);(5,40);(5,0);(5,0)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.35"
%	 points= "(0,50);(0,50);(10,50);(10,50)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.35"
%	 points= "(10,50);(10,50);(10,40);(10,40)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.35"
%	 points= "(0,50);(0,50);(0,40);(0,40)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.35"
%	 points= "(5,90);(5,90);(5,50);(5,50)"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 stroke-width= "0.35"
%	 anchor-point= "(5,45)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\aah$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 stroke-width= "0.35"
%	 anchor-point= "(2.5,1.25)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\AAh$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 stroke-width= "0.35"
%	 anchor-point= "(7.5,88.75)"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\BBh$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(115,45)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\baaah$
%</text>
%<multicurve fill-style= "none"
%	 stroke-width= "0.35"
%	 points= "(135,25);(135,25);(120,10);(120,10)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.35"
%	 points= "(120,10);(120,10);(120,0);(120,0)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.35"
%	 points= "(95,35);(95,35);(120,10);(120,10)"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 stroke-width= "0.35"
%	 anchor-point= "(117.5,1.25)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\AAh$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(120,10)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\Dottt
%</text>
%<multicurve fill-style= "none"
%	 stroke-width= "0.35"
%	 points= "(135,40);(135,40);(135,25);(135,25)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.35"
%	 points= "(130,40);(130,40);(140,40);(140,40)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.35"
%	 points= "(130,50);(130,50);(140,50);(140,50)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.35"
%	 points= "(130,50);(130,50);(130,40);(130,40)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.35"
%	 points= "(140,50);(140,50);(140,40);(140,40)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.35"
%	 points= "(135,65);(135,65);(135,50);(135,50)"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(135,65)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\Dottt
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 stroke-width= "0.35"
%	 anchor-point= "(135,45)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\aah$
%</text>
%<multicurve fill-style= "none"
%	 stroke-width= "0.35"
%	 points= "(30,40);(30,40);(40,40);(40,40)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.35"
%	 points= "(35,40);(35,40);(35,25);(35,25)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.35"
%	 points= "(30,50);(30,50);(40,50);(40,50)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.35"
%	 points= "(40,50);(40,50);(40,40);(40,40)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.35"
%	 points= "(30,50);(30,50);(30,40);(30,40)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.35"
%	 points= "(35,65);(35,65);(35,50);(35,50)"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 stroke-width= "0.35"
%	 anchor-point= "(52.5,88.75)"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\BBh$
%</text>
%<multicurve fill-style= "none"
%	 stroke-width= "0.35"
%	 points= "(50,80);(50,80);(35,65);(35,65)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.35"
%	 points= "(50,90);(50,90);(50,80);(50,80)"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(35,45)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\baaah$
%</text>
%<multicurve fill-style= "none"
%	 stroke-width= "0.35"
%	 points= "(65,25);(65,25);(50,10);(50,10)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.35"
%	 points= "(50,10);(50,10);(50,0);(50,0)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.35"
%	 points= "(35,25);(35,25);(50,10);(50,10)"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 stroke-width= "0.35"
%	 anchor-point= "(47.5,1.25)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\AAh$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(50,10)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\Dottt
%</text>
%<multicurve fill-style= "none"
%	 stroke-width= "0.35"
%	 points= "(65,40);(65,40);(65,25);(65,25)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.35"
%	 points= "(60,40);(60,40);(70,40);(70,40)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.35"
%	 points= "(60,50);(60,50);(70,50);(70,50)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.35"
%	 points= "(60,50);(60,50);(60,40);(60,40)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.35"
%	 points= "(70,50);(70,50);(70,40);(70,40)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.35"
%	 points= "(65,65);(65,65);(65,50);(65,50)"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(65,65)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\Dottt
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 stroke-width= "0.35"
%	 anchor-point= "(65,45)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\aah$
%</text>
%<multicurve fill-style= "none"
%	 stroke-width= "0.35"
%	 points= "(185,35);(185,35);(195,25);(195,25)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.35"
%	 points= "(180,40);(180,40);(190,40);(190,40)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.35"
%	 points= "(185,40);(185,40);(185,35);(185,35)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.35"
%	 points= "(205,40);(205,40);(205,35);(205,35)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.35"
%	 points= "(200,40);(200,40);(210,40);(210,40)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.35"
%	 points= "(200,50);(200,50);(210,50);(210,50)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.35"
%	 points= "(180,50);(180,50);(190,50);(190,50)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.35"
%	 points= "(190,50);(190,50);(190,40);(190,40)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.35"
%	 points= "(200,50);(200,50);(200,40);(200,40)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.35"
%	 points= "(210,50);(210,50);(210,40);(210,40)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.35"
%	 points= "(180,50);(180,50);(180,40);(180,40)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.35"
%	 points= "(185,65);(185,65);(185,50);(185,50)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.35"
%	 points= "(205,55);(205,55);(205,50);(205,50)"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 stroke-width= "0.35"
%	 anchor-point= "(182.5,88.75)"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\BBh$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(185,65)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\Dottt
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(195,25)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\Dottt
%</text>
%<multicurve fill-style= "none"
%	 stroke-width= "0.35"
%	 points= "(180,80);(180,80);(165,65);(165,65)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.35"
%	 points= "(180,90);(180,90);(180,80);(180,80)"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 stroke-width= "0.35"
%	 anchor-point= "(205,45)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\aah$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(185,45)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\baaah$
%</text>
%<multicurve fill-style= "none"
%	 stroke-width= "0.35"
%	 points= "(205,35);(205,35);(180,10);(180,10)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.35"
%	 points= "(180,10);(180,10);(180,0);(180,0)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.35"
%	 points= "(165,25);(165,25);(180,10);(180,10)"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 stroke-width= "0.35"
%	 anchor-point= "(177.5,1.25)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\AAh$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(180,10)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\Dottt
%</text>
%<multicurve fill-style= "none"
%	 stroke-width= "0.35"
%	 points= "(165,40);(165,40);(165,25);(165,25)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.35"
%	 points= "(160,40);(160,40);(170,40);(170,40)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.35"
%	 points= "(160,50);(160,50);(170,50);(170,50)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.35"
%	 points= "(160,50);(160,50);(160,40);(160,40)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.35"
%	 points= "(170,50);(170,50);(170,40);(170,40)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.35"
%	 points= "(165,65);(165,65);(165,50);(165,50)"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(205,55)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\Dottt
%</text>
%<multicurve fill-style= "none"
%	 stroke-width= "0.35"
%	 points= "(230,40);(230,40);(240,40);(240,40)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.35"
%	 points= "(235,40);(235,40);(235,25);(235,25)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.35"
%	 points= "(230,50);(230,50);(240,50);(240,50)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.35"
%	 points= "(240,50);(240,50);(240,40);(240,40)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.35"
%	 points= "(230,50);(230,50);(230,40);(230,40)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.35"
%	 points= "(235,65);(235,65);(235,50);(235,50)"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 stroke-width= "0.35"
%	 anchor-point= "(252.5,88.75)"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\BBh$
%</text>
%<multicurve fill-style= "none"
%	 stroke-width= "0.35"
%	 points= "(250,80);(250,80);(235,65);(235,65)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.35"
%	 points= "(250,90);(250,90);(250,80);(250,80)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.35"
%	 points= "(265,25);(265,25);(250,10);(250,10)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.35"
%	 points= "(250,10);(250,10);(250,0);(250,0)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.35"
%	 points= "(235,25);(235,25);(250,10);(250,10)"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 stroke-width= "0.35"
%	 anchor-point= "(247.5,1.25)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\AAh$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(250,10)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\Dottt
%</text>
%<multicurve fill-style= "none"
%	 stroke-width= "0.35"
%	 points= "(265,40);(265,40);(265,25);(265,25)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.35"
%	 points= "(260,40);(260,40);(270,40);(270,40)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.35"
%	 points= "(260,50);(260,50);(270,50);(270,50)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.35"
%	 points= "(260,50);(260,50);(260,40);(260,40)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.35"
%	 points= "(270,50);(270,50);(270,40);(270,40)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.35"
%	 points= "(265,65);(265,65);(265,50);(265,50)"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(265,65)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\Dottt
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 stroke-width= "0.35"
%	 anchor-point= "(265,45)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\aah$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(235,45)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\caaah$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(165,45)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\caaah$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(95,45)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\caaah$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(20,45)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\EQLSone
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(80,45)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\EQLStwo
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(150,45)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\EQLSthree
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(220,45)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\EQLSfour
%</text>
%</jpic>
%%End JPIC-XML
%LaTeX-picture environment using emulated lines and arcs
%You can rescale the whole picture (to 80% for instance) by using the command \def\JPicScale{0.8}
\ifx\JPicScale\undefined\def\JPicScale{1}\fi
\unitlength \JPicScale mm
\begin{picture}(270,90)(0,0)
\linethickness{0.35mm}
\multiput(105,25)(0.12,0.12){83}{\line(1,0){0.12}}
\linethickness{0.35mm}
\put(90,40){\line(1,0){10}}
\linethickness{0.35mm}
\put(95,35){\line(0,1){5}}
\linethickness{0.35mm}
\put(115,35){\line(0,1){5}}
\linethickness{0.35mm}
\put(110,40){\line(1,0){10}}
\linethickness{0.35mm}
\put(110,50){\line(1,0){10}}
\linethickness{0.35mm}
\put(90,50){\line(1,0){10}}
\linethickness{0.35mm}
\put(100,40){\line(0,1){10}}
\linethickness{0.35mm}
\put(110,40){\line(0,1){10}}
\linethickness{0.35mm}
\put(120,40){\line(0,1){10}}
\linethickness{0.35mm}
\put(90,40){\line(0,1){10}}
\linethickness{0.35mm}
\put(95,50){\line(0,1){5}}
\linethickness{0.35mm}
\put(115,50){\line(0,1){5}}
\put(122.5,88.75){\makebox(0,0)[cl]{$\BBh$}}

\put(115,55){\makebox(0,0)[cc]{\Dottt}}

\put(105,25){\makebox(0,0)[cc]{\Dottt}}

\linethickness{0.35mm}
\multiput(95,55)(0.12,0.12){208}{\line(1,0){0.12}}
\linethickness{0.35mm}
\put(120,80){\line(0,1){10}}
\linethickness{0.35mm}
\put(0,40){\line(1,0){10}}
\linethickness{0.35mm}
\put(5,0){\line(0,1){40}}
\linethickness{0.35mm}
\put(0,50){\line(1,0){10}}
\linethickness{0.35mm}
\put(10,40){\line(0,1){10}}
\linethickness{0.35mm}
\put(0,40){\line(0,1){10}}
\linethickness{0.35mm}
\put(5,50){\line(0,1){40}}
\put(5,45){\makebox(0,0)[cc]{$\aah$}}

\put(2.5,1.25){\makebox(0,0)[cr]{$\AAh$}}

\put(7.5,88.75){\makebox(0,0)[cl]{$\BBh$}}

\put(115,45){\makebox(0,0)[cc]{$\baaah$}}

\linethickness{0.35mm}
\multiput(120,10)(0.12,0.12){125}{\line(1,0){0.12}}
\linethickness{0.35mm}
\put(120,0){\line(0,1){10}}
\linethickness{0.35mm}
\multiput(95,35)(0.12,-0.12){208}{\line(1,0){0.12}}
\put(117.5,1.25){\makebox(0,0)[cr]{$\AAh$}}

\put(120,10){\makebox(0,0)[cc]{\Dottt}}

\linethickness{0.35mm}
\put(135,25){\line(0,1){15}}
\linethickness{0.35mm}
\put(130,40){\line(1,0){10}}
\linethickness{0.35mm}
\put(130,50){\line(1,0){10}}
\linethickness{0.35mm}
\put(130,40){\line(0,1){10}}
\linethickness{0.35mm}
\put(140,40){\line(0,1){10}}
\linethickness{0.35mm}
\put(135,50){\line(0,1){15}}
\put(135,65){\makebox(0,0)[cc]{\Dottt}}

\put(135,45){\makebox(0,0)[cc]{$\aah$}}

\linethickness{0.35mm}
\put(30,40){\line(1,0){10}}
\linethickness{0.35mm}
\put(35,25){\line(0,1){15}}
\linethickness{0.35mm}
\put(30,50){\line(1,0){10}}
\linethickness{0.35mm}
\put(40,40){\line(0,1){10}}
\linethickness{0.35mm}
\put(30,40){\line(0,1){10}}
\linethickness{0.35mm}
\put(35,50){\line(0,1){15}}
\put(52.5,88.75){\makebox(0,0)[cl]{$\BBh$}}

\linethickness{0.35mm}
\multiput(35,65)(0.12,0.12){125}{\line(1,0){0.12}}
\linethickness{0.35mm}
\put(50,80){\line(0,1){10}}
\put(35,45){\makebox(0,0)[cc]{$\baaah$}}

\linethickness{0.35mm}
\multiput(50,10)(0.12,0.12){125}{\line(1,0){0.12}}
\linethickness{0.35mm}
\put(50,0){\line(0,1){10}}
\linethickness{0.35mm}
\multiput(35,25)(0.12,-0.12){125}{\line(1,0){0.12}}
\put(47.5,1.25){\makebox(0,0)[cr]{$\AAh$}}

\put(50,10){\makebox(0,0)[cc]{\Dottt}}

\linethickness{0.35mm}
\put(65,25){\line(0,1){15}}
\linethickness{0.35mm}
\put(60,40){\line(1,0){10}}
\linethickness{0.35mm}
\put(60,50){\line(1,0){10}}
\linethickness{0.35mm}
\put(60,40){\line(0,1){10}}
\linethickness{0.35mm}
\put(70,40){\line(0,1){10}}
\linethickness{0.35mm}
\put(65,50){\line(0,1){15}}
\put(65,65){\makebox(0,0)[cc]{\Dottt}}

\put(65,45){\makebox(0,0)[cc]{$\aah$}}

\linethickness{0.35mm}
\multiput(185,35)(0.12,-0.12){83}{\line(1,0){0.12}}
\linethickness{0.35mm}
\put(180,40){\line(1,0){10}}
\linethickness{0.35mm}
\put(185,35){\line(0,1){5}}
\linethickness{0.35mm}
\put(205,35){\line(0,1){5}}
\linethickness{0.35mm}
\put(200,40){\line(1,0){10}}
\linethickness{0.35mm}
\put(200,50){\line(1,0){10}}
\linethickness{0.35mm}
\put(180,50){\line(1,0){10}}
\linethickness{0.35mm}
\put(190,40){\line(0,1){10}}
\linethickness{0.35mm}
\put(200,40){\line(0,1){10}}
\linethickness{0.35mm}
\put(210,40){\line(0,1){10}}
\linethickness{0.35mm}
\put(180,40){\line(0,1){10}}
\linethickness{0.35mm}
\put(185,50){\line(0,1){15}}
\linethickness{0.35mm}
\put(205,50){\line(0,1){5}}
\put(182.5,88.75){\makebox(0,0)[cl]{$\BBh$}}

\put(185,65){\makebox(0,0)[cc]{\Dottt}}

\put(195,25){\makebox(0,0)[cc]{\Dottt}}

\linethickness{0.35mm}
\multiput(165,65)(0.12,0.12){125}{\line(1,0){0.12}}
\linethickness{0.35mm}
\put(180,80){\line(0,1){10}}
\put(205,45){\makebox(0,0)[cc]{$\aah$}}

\put(185,45){\makebox(0,0)[cc]{$\baaah$}}

\linethickness{0.35mm}
\multiput(180,10)(0.12,0.12){208}{\line(1,0){0.12}}
\linethickness{0.35mm}
\put(180,0){\line(0,1){10}}
\linethickness{0.35mm}
\multiput(165,25)(0.12,-0.12){125}{\line(1,0){0.12}}
\put(177.5,1.25){\makebox(0,0)[cr]{$\AAh$}}

\put(180,10){\makebox(0,0)[cc]{\Dottt}}

\linethickness{0.35mm}
\put(165,25){\line(0,1){15}}
\linethickness{0.35mm}
\put(160,40){\line(1,0){10}}
\linethickness{0.35mm}
\put(160,50){\line(1,0){10}}
\linethickness{0.35mm}
\put(160,40){\line(0,1){10}}
\linethickness{0.35mm}
\put(170,40){\line(0,1){10}}
\linethickness{0.35mm}
\put(165,50){\line(0,1){15}}
\put(205,55){\makebox(0,0)[cc]{\Dottt}}

\linethickness{0.35mm}
\put(230,40){\line(1,0){10}}
\linethickness{0.35mm}
\put(235,25){\line(0,1){15}}
\linethickness{0.35mm}
\put(230,50){\line(1,0){10}}
\linethickness{0.35mm}
\put(240,40){\line(0,1){10}}
\linethickness{0.35mm}
\put(230,40){\line(0,1){10}}
\linethickness{0.35mm}
\put(235,50){\line(0,1){15}}
\put(252.5,88.75){\makebox(0,0)[cl]{$\BBh$}}

\linethickness{0.35mm}
\multiput(235,65)(0.12,0.12){125}{\line(1,0){0.12}}
\linethickness{0.35mm}
\put(250,80){\line(0,1){10}}
\linethickness{0.35mm}
\multiput(250,10)(0.12,0.12){125}{\line(1,0){0.12}}
\linethickness{0.35mm}
\put(250,0){\line(0,1){10}}
\linethickness{0.35mm}
\multiput(235,25)(0.12,-0.12){125}{\line(1,0){0.12}}
\put(247.5,1.25){\makebox(0,0)[cr]{$\AAh$}}

\put(250,10){\makebox(0,0)[cc]{\Dottt}}

\linethickness{0.35mm}
\put(265,25){\line(0,1){15}}
\linethickness{0.35mm}
\put(260,40){\line(1,0){10}}
\linethickness{0.35mm}
\put(260,50){\line(1,0){10}}
\linethickness{0.35mm}
\put(260,40){\line(0,1){10}}
\linethickness{0.35mm}
\put(270,40){\line(0,1){10}}
\linethickness{0.35mm}
\put(265,50){\line(0,1){15}}
\put(265,65){\makebox(0,0)[cc]{\Dottt}}

\put(265,45){\makebox(0,0)[cc]{$\aah$}}

\put(235,45){\makebox(0,0)[cc]{$\caaah$}}

\put(165,45){\makebox(0,0)[cc]{$\caaah$}}

\put(95,45){\makebox(0,0)[cc]{$\caaah$}}

\put(20,45){\makebox(0,0)[cc]{\EQLSone}}

\put(80,45){\makebox(0,0)[cc]{\EQLStwo}}

\put(150,45){\makebox(0,0)[cc]{\EQLSthree}}

\put(220,45){\makebox(0,0)[cc]{\EQLSfour}}

\end{picture}


==> PIC/costless.tex <==
%%Created by jPicEdt 1.4.1_03: mixed JPIC-XML/LaTeX format
%%Sat Nov 26 20:32:54 GMT-10:00 2022
%%Begin JPIC-XML
%<?xml version="1.0" standalone="yes"?>
%<jpic x-min="0" x-max="60" y-min="0" y-max="60" auto-bounding="true">
%<multicurve fill-style= "none"
%	 stroke-width= "0.35"
%	 points= "(25,20);(25,20);(15,10);(15,10)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.35"
%	 points= "(15,10);(15,10);(15,0);(15,0)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.35"
%	 points= "(0,25);(0,25);(10,25);(10,25)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.35"
%	 points= "(5,25);(5,25);(5,20);(5,20)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.35"
%	 points= "(5,20);(5,20);(15,10);(15,10)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.35"
%	 points= "(25,25);(25,25);(25,20);(25,20)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.35"
%	 points= "(20,25);(20,25);(30,25);(30,25)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.35"
%	 points= "(20,35);(20,35);(30,35);(30,35)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.35"
%	 points= "(0,35);(0,35);(10,35);(10,35)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.35"
%	 points= "(10,35);(10,35);(10,25);(10,25)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.35"
%	 points= "(20,35);(20,35);(20,25);(20,25)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.35"
%	 points= "(30,35);(30,35);(30,25);(30,25)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.35"
%	 points= "(0,35);(0,35);(0,25);(0,25)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.35"
%	 points= "(5,40);(5,40);(5,35);(5,35)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.35"
%	 points= "(25,40);(25,40);(25,35);(25,35)"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 stroke-width= "0.35"
%	 anchor-point= "(5,30)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\aah$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 stroke-width= "0.35"
%	 anchor-point= "(12.5,0)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\AAh$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 stroke-width= "0.35"
%	 anchor-point= "(17.5,60)"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\BBh$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(25,40)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\Dottt
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(15,10)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\Dottt
%</text>
%<multicurve fill-style= "none"
%	 stroke-width= "0.35"
%	 points= "(15,50);(15,50);(5,40);(5,40)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.35"
%	 points= "(15,60);(15,60);(15,50);(15,50)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.35"
%	 points= "(50,25);(50,25);(60,25);(60,25)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.35"
%	 points= "(55,25);(55,25);(55,0);(55,0)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.35"
%	 points= "(50,35);(50,35);(60,35);(60,35)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.35"
%	 points= "(60,35);(60,35);(60,25);(60,25)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.35"
%	 points= "(50,35);(50,35);(50,25);(50,25)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.35"
%	 points= "(55,60);(55,60);(55,35);(55,35)"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 stroke-width= "0.35"
%	 anchor-point= "(55,30)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\aah$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 stroke-width= "0.35"
%	 anchor-point= "(52.5,0)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\AAh$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(40,30)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\EQLS
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 stroke-width= "0.35"
%	 anchor-point= "(25,30)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\aah$
%</text>
%</jpic>
%%End JPIC-XML
%LaTeX-picture environment using emulated lines and arcs
%You can rescale the whole picture (to 80% for instance) by using the command \def\JPicScale{0.8}
\ifx\JPicScale\undefined\def\JPicScale{1}\fi
\unitlength \JPicScale mm
\begin{picture}(60,60)(0,0)
\linethickness{0.35mm}
\multiput(15,10)(0.12,0.12){83}{\line(1,0){0.12}}
\linethickness{0.35mm}
\put(15,0){\line(0,1){10}}
\linethickness{0.35mm}
\put(0,25){\line(1,0){10}}
\linethickness{0.35mm}
\put(5,20){\line(0,1){5}}
\linethickness{0.35mm}
\multiput(5,20)(0.12,-0.12){83}{\line(1,0){0.12}}
\linethickness{0.35mm}
\put(25,20){\line(0,1){5}}
\linethickness{0.35mm}
\put(20,25){\line(1,0){10}}
\linethickness{0.35mm}
\put(20,35){\line(1,0){10}}
\linethickness{0.35mm}
\put(0,35){\line(1,0){10}}
\linethickness{0.35mm}
\put(10,25){\line(0,1){10}}
\linethickness{0.35mm}
\put(20,25){\line(0,1){10}}
\linethickness{0.35mm}
\put(30,25){\line(0,1){10}}
\linethickness{0.35mm}
\put(0,25){\line(0,1){10}}
\linethickness{0.35mm}
\put(5,35){\line(0,1){5}}
\linethickness{0.35mm}
\put(25,35){\line(0,1){5}}
\put(5,30){\makebox(0,0)[cc]{$\aah$}}

\put(12.5,0){\makebox(0,0)[cr]{$\AAh$}}

\put(17.5,60){\makebox(0,0)[cl]{$\BBh$}}

\put(25,40){\makebox(0,0)[cc]{\Dottt}}

\put(15,10){\makebox(0,0)[cc]{\Dottt}}

\linethickness{0.35mm}
\multiput(5,40)(0.12,0.12){83}{\line(1,0){0.12}}
\linethickness{0.35mm}
\put(15,50){\line(0,1){10}}
\linethickness{0.35mm}
\put(50,25){\line(1,0){10}}
\linethickness{0.35mm}
\put(55,0){\line(0,1){25}}
\linethickness{0.35mm}
\put(50,35){\line(1,0){10}}
\linethickness{0.35mm}
\put(60,25){\line(0,1){10}}
\linethickness{0.35mm}
\put(50,25){\line(0,1){10}}
\linethickness{0.35mm}
\put(55,35){\line(0,1){25}}
\put(55,30){\makebox(0,0)[cc]{$\aah$}}

\put(52.5,0){\makebox(0,0)[cr]{$\AAh$}}

\put(40,30){\makebox(0,0)[cc]{\EQLS}}

\put(25,30){\makebox(0,0)[cc]{$\aah$}}

\end{picture}


==> PIC/cuml.tex <==
%%Created by jPicEdt 1.4.1_03: mixed JPIC-XML/LaTeX format
%%Sun Jan 12 20:00:08 GMT-10:00 2020
%%Begin JPIC-XML
%<?xml version="1.0" standalone="yes"?>
%<jpic x-min="0" x-max="155" y-min="0" y-max="95" auto-bounding="true">
%<multicurve fill-style= "none"
%	 points= "(110,50);(110,50);(155,50);(155,50)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(155,30);(155,30);(155,50);(155,50)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(130,30);(130,30);(155,30);(155,30)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(150,30);(150,30);(150,0);(150,0)"
%	 stroke-width= "0.75"
%	 />
%<ellipse fill-style= "solid"
%	 p3= "(122.58,27.42)"
%	 fill-color= "#330033"
%	 p2= "(122.58,32.58)"
%	 p1= "(117.42,32.58)"
%	 closure= "open"
%	 angle-end= "0"
%	 angle-start= "0"
%	 />
%<multicurve fill-style= "none"
%	 points= "(100,50);(100,50);(120,30);(120,30)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(120,40);(120,40);(120,0);(120,0)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(110,50);(110,50);(130,30);(130,30)"
%	 stroke-width= "0.75"
%	 />
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(140,40)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\universal$
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(147.5,1.25)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\Atype$
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(117.5,1.25)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\Progtype$
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(122.5,95)"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\Progtype$
%</text>
%<multicurve fill-style= "none"
%	 points= "(150,95);(150,95);(150,50);(150,50)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(100,95);(100,95);(100,50);(100,50)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(0,85);(0,85);(10,85);(10,85)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(10,75);(10,75);(10,85);(10,85)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(5,95);(5,95);(5,85);(5,85)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(0,75);(0,75);(10,75);(10,75)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(120,95);(120,95);(120,50);(120,50)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(0,85);(0,85);(0,75);(0,75)"
%	 stroke-width= "0.75"
%	 />
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(5,80)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\universallift$
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(102.5,95)"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\Progtype$
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(7.5,95)"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\Progtype$
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(152.5,95)"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\Btype$
%</text>
%<multicurve fill-style= "none"
%	 points= "(25,50);(25,50);(50,50);(50,50)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(50,30);(50,30);(50,50);(50,50)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(25,30);(25,30);(50,30);(50,30)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(45,30);(45,30);(45,0);(45,0)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(15,40);(15,40);(15,0);(15,0)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(5,50);(5,50);(25,30);(25,30)"
%	 stroke-width= "0.75"
%	 />
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(30,40)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\universal$
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(42.5,1.25)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\Atype$
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(12.5,1.25)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\Progtype$
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(17.5,65)"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\Progtype$
%</text>
%<multicurve fill-style= "none"
%	 points= "(45,95);(45,95);(45,50);(45,50)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(15,70);(15,70);(15,60);(15,60)"
%	 stroke-width= "0.75"
%	 />
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(47.5,95)"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\Btype$
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(75,40)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\EQLS
%</text>
%<multicurve fill-style= "none"
%	 points= "(5,70);(5,70);(25,50);(25,50)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(5,50);(5,50);(5,70);(5,70)"
%	 stroke-width= "0.75"
%	 />
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(27.5,95)"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\Progtype$
%</text>
%</jpic>
%%End JPIC-XML
%PSTricks content-type (pstricks.sty package needed)
%Add \usepackage{pstricks} in the preamble of your LaTeX file
%You can rescale the whole picture (to 80% for instance) by using the command \def\JPicScale{0.8}
\ifx\JPicScale\undefined\def\JPicScale{1}\fi
\psset{unit=\JPicScale mm}
\psset{linewidth=0.3,dotsep=1,hatchwidth=0.3,hatchsep=1.5,shadowsize=1,dimen=middle}
\psset{dotsize=0.7 2.5,dotscale=1 1,fillcolor=black}
\psset{arrowsize=1 2,arrowlength=1,arrowinset=0.25,tbarsize=0.7 5,bracketlength=0.15,rbracketlength=0.15}
\begin{pspicture}(0,0)(155,95)
\psline[linewidth=0.75](110,50)(155,50)
\psline[linewidth=0.75](155,30)(155,50)
\psline[linewidth=0.75](130,30)(155,30)
\psline[linewidth=0.75](150,30)(150,0)
\newrgbcolor{userFillColour}{0.2 0 0.2}
\rput{0}(120,30){\psellipse[fillcolor=userFillColour,fillstyle=solid](0,0)(2.58,-2.58)}
\psline[linewidth=0.75](100,50)(120,30)
\psline[linewidth=0.75](120,40)(120,0)
\psline[linewidth=0.75](110,50)(130,30)
\rput(140,40){$\universal$}
\rput[r](147.5,1.25){$\Atype$}
\rput[r](117.5,1.25){$\Progtype$}
\rput[l](122.5,95){$\Progtype$}
\psline[linewidth=0.75](150,95)(150,50)
\psline[linewidth=0.75](100,95)(100,50)
\psline[linewidth=0.75](0,85)(10,85)
\psline[linewidth=0.75](10,75)(10,85)
\psline[linewidth=0.75](5,95)(5,85)
\psline[linewidth=0.75](0,75)(10,75)
\psline[linewidth=0.75](120,95)(120,50)
\psline[linewidth=0.75](0,85)(0,75)
\rput(5,80){$\universallift$}
\rput[l](102.5,95){$\Progtype$}
\rput[l](7.5,95){$\Progtype$}
\rput[l](152.5,95){$\Btype$}
\psline[linewidth=0.75](25,50)(50,50)
\psline[linewidth=0.75](50,30)(50,50)
\psline[linewidth=0.75](25,30)(50,30)
\psline[linewidth=0.75](45,30)(45,0)
\psline[linewidth=0.75](15,40)(15,0)
\psline[linewidth=0.75](5,50)(25,30)
\rput(30,40){$\universal$}
\rput[r](42.5,1.25){$\Atype$}
\rput[r](12.5,1.25){$\Progtype$}
\rput[l](17.5,65){$\Progtype$}
\psline[linewidth=0.75](45,95)(45,50)
\psline[linewidth=0.75](15,70)(15,60)
\rput[l](47.5,95){$\Btype$}
\rput(75,40){\EQLS}
\psline[linewidth=0.75](5,70)(25,50)
\psline[linewidth=0.75](5,50)(5,70)
\rput[l](27.5,95){$\Progtype$}
\end{pspicture}


==> PIC/cumul.tex <==
%%Created by jPicEdt 1.4.1_03: mixed JPIC-XML/LaTeX format
%%Sun Jan 12 20:17:45 GMT-10:00 2020
%%Begin JPIC-XML
%<?xml version="1.0" standalone="yes"?>
%<jpic x-min="0" x-max="140" y-min="0" y-max="90" auto-bounding="true">
%<multicurve fill-style= "none"
%	 points= "(100,35);(100,35);(140,35);(140,35)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(140,15);(140,15);(140,35);(140,35)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(120,15);(120,15);(140,15);(140,15)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(130,15);(130,15);(130,0);(130,0)"
%	 stroke-width= "0.75"
%	 />
%<ellipse fill-style= "solid"
%	 p3= "(112.58,12.42)"
%	 fill-color= "#330033"
%	 p2= "(112.58,17.58)"
%	 p1= "(107.42,17.58)"
%	 closure= "open"
%	 angle-end= "0"
%	 angle-start= "0"
%	 />
%<multicurve fill-style= "none"
%	 points= "(90,35);(90,35);(110,15);(110,15)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(110,25);(110,25);(110,0);(110,0)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(100,35);(100,35);(120,15);(120,15)"
%	 stroke-width= "0.75"
%	 />
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(125,25)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\universal$
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(127.5,0)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\Atype$
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(107.5,0)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\Progtype$
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(112.5,90)"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\Progtype$
%</text>
%<multicurve fill-style= "none"
%	 points= "(130,90);(130,90);(130,35);(130,35)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(90,90);(90,90);(90,35);(90,35)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(0,80);(0,80);(10,80);(10,80)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(10,70);(10,70);(10,80);(10,80)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(5,90);(5,90);(5,80);(5,80)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(0,70);(0,70);(10,70);(10,70)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(110,90);(110,90);(110,35);(110,35)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(0,80);(0,80);(0,70);(0,70)"
%	 stroke-width= "0.75"
%	 />
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(5,75)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\universallift$
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(92.5,90)"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\Progtype$
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(7.5,90)"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\Progtype$
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(132.5,90)"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\Btype$
%</text>
%<multicurve fill-style= "none"
%	 points= "(22.5,35);(22.5,35);(50,35);(50,35)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(50,15);(50,15);(50,35);(50,35)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(22.5,15);(22.5,15);(50,15);(50,15)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(45,15);(45,15);(45,0);(45,0)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(15,22.5);(15,22.5);(15,0);(15,0)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(7.5,30);(7.5,30);(22.5,15);(22.5,15)"
%	 stroke-width= "0.75"
%	 />
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(42.5,0)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\Atype$
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(12.5,0)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\Progtype$
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(17.5,47.5)"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\Progtype$
%</text>
%<multicurve fill-style= "none"
%	 points= "(45,90);(45,90);(45,35);(45,35)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(15,52.5);(15,52.5);(15,42.5);(15,42.5)"
%	 stroke-width= "0.75"
%	 />
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(45,90)"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\Btype$
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(70,40)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\EQLS
%</text>
%<multicurve fill-style= "none"
%	 points= "(7.5,50);(7.5,50);(22.5,35);(22.5,35)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(7.5,30);(7.5,30);(7.5,50);(7.5,50)"
%	 stroke-width= "0.75"
%	 />
%<ellipse fill-style= "solid"
%	 p3= "(17.58,49.92)"
%	 fill-color= "#330033"
%	 p2= "(17.58,55.08)"
%	 p1= "(12.42,55.08)"
%	 closure= "open"
%	 angle-end= "0"
%	 angle-start= "0"
%	 />
%<multicurve fill-style= "none"
%	 points= "(5,62.5);(5,62.5);(15,52.5);(15,52.5)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(15,52.5);(15,52.5);(25,62.5);(25,62.5)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(25,62.5);(25,62.5);(25,70);(25,70)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(5,62.5);(5,62.5);(5,70);(5,70)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(20,80);(20,80);(30,80);(30,80)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(30,70);(30,70);(30,80);(30,80)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(25,90);(25,90);(25,80);(25,80)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(20,70);(20,70);(30,70);(30,70)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(20,80);(20,80);(20,70);(20,70)"
%	 stroke-width= "0.75"
%	 />
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(27.5,90)"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\Progtype$
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(25,75)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\secnd$
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(30,25)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\cumultv$
%</text>
%</jpic>
%%End JPIC-XML
%PSTricks content-type (pstricks.sty package needed)
%Add \usepackage{pstricks} in the preamble of your LaTeX file
%You can rescale the whole picture (to 80% for instance) by using the command \def\JPicScale{0.8}
\ifx\JPicScale\undefined\def\JPicScale{1}\fi
\psset{unit=\JPicScale mm}
\psset{linewidth=0.3,dotsep=1,hatchwidth=0.3,hatchsep=1.5,shadowsize=1,dimen=middle}
\psset{dotsize=0.7 2.5,dotscale=1 1,fillcolor=black}
\psset{arrowsize=1 2,arrowlength=1,arrowinset=0.25,tbarsize=0.7 5,bracketlength=0.15,rbracketlength=0.15}
\begin{pspicture}(0,0)(140,90)
\psline[linewidth=0.75](100,35)(140,35)
\psline[linewidth=0.75](140,15)(140,35)
\psline[linewidth=0.75](120,15)(140,15)
\psline[linewidth=0.75](130,15)(130,0)
\newrgbcolor{userFillColour}{0.2 0 0.2}
\rput{0}(110,15){\psellipse[fillcolor=userFillColour,fillstyle=solid](0,0)(2.58,-2.58)}
\psline[linewidth=0.75](90,35)(110,15)
\psline[linewidth=0.75](110,25)(110,0)
\psline[linewidth=0.75](100,35)(120,15)
\rput(125,25){$\universal$}
\rput[r](127.5,0){$\Atype$}
\rput[r](107.5,0){$\Progtype$}
\rput[l](112.5,90){$\Progtype$}
\psline[linewidth=0.75](130,90)(130,35)
\psline[linewidth=0.75](90,90)(90,35)
\psline[linewidth=0.75](0,80)(10,80)
\psline[linewidth=0.75](10,70)(10,80)
\psline[linewidth=0.75](5,90)(5,80)
\psline[linewidth=0.75](0,70)(10,70)
\psline[linewidth=0.75](110,90)(110,35)
\psline[linewidth=0.75](0,80)(0,70)
\rput(5,75){$\universallift$}
\rput[l](92.5,90){$\Progtype$}
\rput[l](7.5,90){$\Progtype$}
\rput[l](132.5,90){$\Btype$}
\psline[linewidth=0.75](22.5,35)(50,35)
\psline[linewidth=0.75](50,15)(50,35)
\psline[linewidth=0.75](22.5,15)(50,15)
\psline[linewidth=0.75](45,15)(45,0)
\psline[linewidth=0.75](15,22.5)(15,0)
\psline[linewidth=0.75](7.5,30)(22.5,15)
\rput[r](42.5,0){$\Atype$}
\rput[r](12.5,0){$\Progtype$}
\rput[l](17.5,47.5){$\Progtype$}
\psline[linewidth=0.75](45,90)(45,35)
\psline[linewidth=0.75](15,52.5)(15,42.5)
\rput[l](45,90){$\Btype$}
\rput(70,40){\EQLS}
\psline[linewidth=0.75](7.5,50)(22.5,35)
\psline[linewidth=0.75](7.5,30)(7.5,50)
\newrgbcolor{userFillColour}{0.2 0 0.2}
\rput{0}(15,52.5){\psellipse[fillcolor=userFillColour,fillstyle=solid](0,0)(2.58,-2.58)}
\psline[linewidth=0.75](5,62.5)(15,52.5)
\psline[linewidth=0.75](15,52.5)(25,62.5)
\psline[linewidth=0.75](25,62.5)(25,70)
\psline[linewidth=0.75](5,62.5)(5,70)
\psline[linewidth=0.75](20,80)(30,80)
\psline[linewidth=0.75](30,70)(30,80)
\psline[linewidth=0.75](25,90)(25,80)
\psline[linewidth=0.75](20,70)(30,70)
\psline[linewidth=0.75](20,80)(20,70)
\rput[l](27.5,90){$\Progtype$}
\rput(25,75){$\secnd$}
\rput(30,25){$\cumultv$}
\end{pspicture}


==> PIC/cun-left.tex <==
%%Created by jPicEdt 1.4.1_03: mixed JPIC-XML/LaTeX format
%%Sat Sep 02 17:29:59 HST 2017
%%Begin JPIC-XML
%<?xml version="1.0" standalone="yes"?>
%<jpic x-min="-2.19" x-max="10" y-min="-10.62" y-max="8.12" auto-bounding="true">
%<multicurve points= "(0.62,0);(0.62,0);(5.62,-5);(5.62,-5);(5.62,-5);(4.38,-5);
%	(4.38,-5);(4.38,-5);(5,-5);(5,-5)"
%	 fill-style= "none"
%	 />
%<ellipse p3= "(-2.19,2.81)"
%	 p2= "(-2.19,-0.31)"
%	 p1= "(0.94,-0.31)"
%	 closure= "open"
%	 angle-end= "0"
%	 fill-style= "solid"
%	 angle-start= "0"
%	 />
%<ellipse p3= "(3.75,-3.13)"
%	 p2= "(3.75,-6.25)"
%	 p1= "(6.88,-6.25)"
%	 closure= "open"
%	 angle-end= "0"
%	 fill-style= "solid"
%	 angle-start= "0"
%	 />
%<multicurve points= "(10,8.12);(10,8.12);(10,5.62);(10,5.62);(10,5.62);(10,0);
%	(10,0);(10,0);(6.25,-3.75);(6.25,-3.75)"
%	 fill-style= "none"
%	 />
%<multicurve points= "(5,-6.25);(5,-6.25);(5,-10);(5,-10);(5,-10);(5,-10.62);
%	(5,-10.62);(5,-10.62);(5,-10);(5,-10)"
%	 fill-style= "none"
%	 />
%</jpic>
%%End JPIC-XML
%PSTricks content-type (pstricks.sty package needed)
%Add \usepackage{pstricks} in the preamble of your LaTeX file
%You can rescale the whole picture (to 80% for instance) by using the command \def\JPicScale{0.8}
\ifx\JPicScale\undefined\def\JPicScale{1}\fi
\psset{unit=\JPicScale mm}
\psset{linewidth=0.3,dotsep=1,hatchwidth=0.3,hatchsep=1.5,shadowsize=1,dimen=middle}
\psset{dotsize=0.7 2.5,dotscale=1 1,fillcolor=black}
\psset{arrowsize=1 2,arrowlength=1,arrowinset=0.25,tbarsize=0.7 5,bracketlength=0.15,rbracketlength=0.15}
\begin{pspicture}(0,0)(10,8.12)
\psline(0.62,0)
(5.62,-5)
(4.38,-5)(5,-5)
\rput{0}(-0.62,1.25){\psellipse[fillstyle=solid](0,0)(1.57,-1.56)}
\rput{0}(5.31,-4.69){\psellipse[fillstyle=solid](0,0)(1.57,-1.56)}
\psline(10,8.12)
(10,5.62)
(10,0)(6.25,-3.75)
\psline(5,-6.25)
(5,-10)
(5,-10.62)(5,-10)
\end{pspicture}


==> PIC/cun-right.tex <==
%%Created by jPicEdt 1.4.1_03: mixed JPIC-XML/LaTeX format
%%Sat Sep 02 17:34:38 HST 2017
%%Begin JPIC-XML
%<?xml version="1.0" standalone="yes"?>
%<jpic x-min="-0.63" x-max="12.19" y-min="-10.62" y-max="8.12" auto-bounding="true">
%<ellipse p3= "(9.06,2.81)"
%	 p2= "(9.06,-0.31)"
%	 p1= "(12.19,-0.31)"
%	 closure= "open"
%	 angle-end= "0"
%	 fill-style= "solid"
%	 angle-start= "0"
%	 />
%<ellipse p3= "(2.81,-3.44)"
%	 p2= "(2.81,-6.56)"
%	 p1= "(5.94,-6.56)"
%	 closure= "open"
%	 angle-end= "0"
%	 fill-style= "solid"
%	 angle-start= "0"
%	 />
%<multicurve points= "(4.38,-6.25);(4.38,-6.25);(4.38,-10);(4.38,-10);(4.38,-10);(4.38,-10.62);
%	(4.38,-10.62);(4.38,-10.62);(4.38,-10);(4.38,-10)"
%	 fill-style= "none"
%	 />
%<multicurve points= "(-0.63,8.12);(-0.63,8.12);(-0.62,1.87);(-0.62,1.87);(-0.62,1.87);(-0.62,0);
%	(-0.62,0);(-0.62,0);(3.13,-3.75);(3.13,-3.75)"
%	 fill-style= "none"
%	 />
%<multicurve points= "(9.38,0);(9.38,0);(4.38,-5);(4.38,-5);(4.38,-5);(4.38,-5);
%	(4.38,-5);(4.38,-5);(4.38,-5);(4.38,-5)"
%	 fill-style= "none"
%	 />
%</jpic>
%%End JPIC-XML
%PSTricks content-type (pstricks.sty package needed)
%Add \usepackage{pstricks} in the preamble of your LaTeX file
%You can rescale the whole picture (to 80% for instance) by using the command \def\JPicScale{0.8}
\ifx\JPicScale\undefined\def\JPicScale{1}\fi
\psset{unit=\JPicScale mm}
\psset{linewidth=0.3,dotsep=1,hatchwidth=0.3,hatchsep=1.5,shadowsize=1,dimen=middle}
\psset{dotsize=0.7 2.5,dotscale=1 1,fillcolor=black}
\psset{arrowsize=1 2,arrowlength=1,arrowinset=0.25,tbarsize=0.7 5,bracketlength=0.15,rbracketlength=0.15}
\begin{pspicture}(0,0)(12.19,8.12)
\rput{0}(10.62,1.25){\psellipse[fillstyle=solid](0,0)(1.57,-1.56)}
\rput{0}(4.38,-5){\psellipse[fillstyle=solid](0,0)(1.57,-1.56)}
\psline(4.38,-6.25)
(4.38,-10)
(4.38,-10.62)(4.38,-10)
\psline(-0.63,8.12)
(-0.62,1.87)
(-0.62,0)(3.13,-3.75)
\pscustom[]{\psline(9.38,0)(4.38,-5)
\psbezier(4.38,-5)(4.38,-5)(4.38,-5)
\psbezier(4.38,-5)(4.38,-5)(4.38,-5)
}
\end{pspicture}


==> PIC/currying.tex <==
%%Created by jPicEdt 1.4.1_03: mixed JPIC-XML/LaTeX format
%%Tue Jan 31 16:19:58 GMT 2012
%%Begin JPIC-XML
%<?xml version="1.0" standalone="yes"?>
%<jpic x-min="9.38" x-max="80.62" y-min="-0.62" y-max="40.62" auto-bounding="true">
%<multicurve stroke-width= "0.4"
%	 fill-style= "none"
%	 arrow-head-width-minimum= "1.05"
%	 right-arrow= "head"
%	 points= "(10,35.62);(10,35.62);(10,3.75);(10,3.75)"
%	 arrow-head-length-scale= "2"
%	 />
%<multicurve stroke-width= "0.4"
%	 fill-style= "none"
%	 arrow-head-width-minimum= "1.05"
%	 right-arrow= "head"
%	 points= "(23.12,0);(23.12,0);(75,0);(75,0)"
%	 arrow-head-length-scale= "2"
%	 />
%<multicurve stroke-width= "0.4"
%	 fill-style= "none"
%	 arrow-head-width-minimum= "1.05"
%	 right-arrow= "head"
%	 points= "(80,35.62);(80,35.62);(80,23.12);(80,23.12)"
%	 arrow-head-length-scale= "2"
%	 />
%<text text-vert-align= "center-v"
%	 anchor-point= "(10,40)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\three$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(10,0)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\two$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(80,0)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\one$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(80,40)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\three$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(80,20)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\two$
%</text>
%<multicurve stroke-width= "0.4"
%	 fill-style= "none"
%	 arrow-head-width-minimum= "1.05"
%	 right-arrow= "head"
%	 points= "(80,16.25);(80,16.25);(80,3.12);(80,3.12)"
%	 arrow-head-length-scale= "2"
%	 />
%<multicurve stroke-width= "0.4"
%	 fill-style= "none"
%	 arrow-head-width-minimum= "1.05"
%	 right-arrow= "head"
%	 points= "(30,40);(30,40);(60.62,40);(60.62,40)"
%	 arrow-head-length-scale= "2"
%	 />
%<text text-vert-align= "bottom"
%	 anchor-point= "(44.38,40.62)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\up$
%</text>
%<text text-vert-align= "top"
%	 anchor-point= "(44.38,-0.62)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\down$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(80.62,30.62)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\rightup$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(80.62,11.25)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\rightdown$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(9.38,20)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\leftdown$
%</text>
%</jpic>
%%End JPIC-XML
%PSTricks content-type (pstricks.sty package needed)
%Add \usepackage{pstricks} in the preamble of your LaTeX file
%You can rescale the whole picture (to 80% for instance) by using the command \def\JPicScale{0.8}
\ifx\JPicScale\undefined\def\JPicScale{1}\fi
\psset{unit=\JPicScale mm}
\psset{linewidth=0.3,dotsep=1,hatchwidth=0.3,hatchsep=1.5,shadowsize=1,dimen=middle}
\psset{dotsize=0.7 2.5,dotscale=1 1,fillcolor=black}
\psset{arrowsize=1 2,arrowlength=1,arrowinset=0.25,tbarsize=0.7 5,bracketlength=0.15,rbracketlength=0.15}
\begin{pspicture}(0,0)(80.62,40.62)
\psline[linewidth=0.4,arrowsize=1.05 2,arrowlength=2]{->}(10,35.62)(10,3.75)
\psline[linewidth=0.4,arrowsize=1.05 2,arrowlength=2]{->}(23.12,0)(75,0)
\psline[linewidth=0.4,arrowsize=1.05 2,arrowlength=2]{->}(80,35.62)(80,23.12)
\rput(10,40){$\three$}
\rput(10,0){$\two$}
\rput(80,0){$\one$}
\rput(80,40){$\three$}
\rput(80,20){$\two$}
\psline[linewidth=0.4,arrowsize=1.05 2,arrowlength=2]{->}(80,16.25)(80,3.12)
\psline[linewidth=0.4,arrowsize=1.05 2,arrowlength=2]{->}(30,40)(60.62,40)
\rput[b](44.38,40.62){$\up$}
\rput[t](44.38,-0.62){$\down$}
\rput[l](80.62,30.62){$\rightup$}
\rput[l](80.62,11.25){$\rightdown$}
\rput[r](9.38,20){$\leftdown$}
\end{pspicture}


==> PIC/curved.tex <==
%%Created by jPicEdt 1.4.1_03: mixed JPIC-XML/LaTeX format
%%Sun Jan 08 11:25:32 GMT 2012
%%Begin JPIC-XML
%<?xml version="1.0" standalone="yes"?>
%<jpic x-min="10" x-max="140" y-min="0" y-max="45" auto-bounding="true">
%<multicurve stroke-width= "0.4"
%	 fill-style= "none"
%	 points= "(10,20);(10,20);(15,30);(20,25);(25,20);(25,0);
%	(35,10);(45,20);(55,20);(65,15);(75,10);(65,25);
%	(80,30);(95,35);(80,45);(100,45);(120,45);(105,45);
%	(120,40);(135,35);(125,45);(130,30);(135,15);(140,20);
%	(140,20);(140,20);(140,20);(140,20);(140,20);(140,20);
%	(140,20)"
%	 />
%</jpic>
%%End JPIC-XML
%PSTricks content-type (pstricks.sty package needed)
%Add \usepackage{pstricks} in the preamble of your LaTeX file
%You can rescale the whole picture (to 80% for instance) by using the command \def\JPicScale{0.8}
\ifx\JPicScale\undefined\def\JPicScale{1}\fi
\psset{unit=\JPicScale mm}
\psset{linewidth=0.3,dotsep=1,hatchwidth=0.3,hatchsep=1.5,shadowsize=1,dimen=middle}
\psset{dotsize=0.7 2.5,dotscale=1 1,fillcolor=black}
\psset{arrowsize=1 2,arrowlength=1,arrowinset=0.25,tbarsize=0.7 5,bracketlength=0.15,rbracketlength=0.15}
\begin{pspicture}(0,0)(140,45)
\pscustom[linewidth=0.4]{\psbezier(10,20)(10,20)(15,30)(20,25)
\psbezier(25,20)(25,0)(35,10)
\psbezier(45,20)(55,20)(65,15)
\psbezier(75,10)(65,25)(80,30)
\psbezier(95,35)(80,45)(100,45)
\psbezier(120,45)(105,45)(120,40)
\psbezier(135,35)(125,45)(130,30)
\psbezier(135,15)(140,20)(140,20)
\psbezier(140,20)(140,20)(140,20)
\psbezier(140,20)(140,20)(140,20)
}
\end{pspicture}


==> PIC/dataserv-cmn.tex <==
%%Created by jPicEdt 1.4.1_03: mixed JPIC-XML/LaTeX format
%%Mon Aug 31 15:03:16 GMT-10:00 2020
%%Begin JPIC-XML
%<?xml version="1.0" standalone="yes"?>
%<jpic x-min="0" x-max="32.5" y-min="1.25" y-max="62.5" auto-bounding="true">
%<multicurve fill-style= "none"
%	 points= "(30,40);(30,40);(15,25);(15,25)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(15,25);(15,25);(15,5);(15,5)"
%	 stroke-width= "0.75"
%	 />
%<ellipse p3= "(18.79,21.21)"
%	 fill-style= "solid"
%	 p2= "(18.79,28.79)"
%	 fill-color= "#330033"
%	 p1= "(11.21,28.79)"
%	 closure= "open"
%	 angle-end= "0"
%	 angle-start= "0"
%	 />
%<multicurve fill-style= "none"
%	 points= "(0,40);(0,40);(15,25);(15,25)"
%	 stroke-width= "0.75"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(12.5,13.75)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\AAh$
%</text>
%<multicurve fill-style= "none"
%	 points= "(0,57.5);(0,57.5);(0,40);(0,40)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(30,57.5);(30,57.5);(30,40);(30,40)"
%	 stroke-width= "0.75"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(32.5,45)"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\AAh$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(2.5,45)"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\AAh$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(21.25,25)"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\ccopy$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(15.62,1.25)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\eex$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(0,62.5)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\eex$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(30,62.5)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\eex$
%</text>
%</jpic>
%%End JPIC-XML
%PSTricks content-type (pstricks.sty package needed)
%Add \usepackage{pstricks} in the preamble of your LaTeX file
%You can rescale the whole picture (to 80% for instance) by using the command \def\JPicScale{0.8}
\ifx\JPicScale\undefined\def\JPicScale{1}\fi
\psset{unit=\JPicScale mm}
\psset{linewidth=0.3,dotsep=1,hatchwidth=0.3,hatchsep=1.5,shadowsize=1,dimen=middle}
\psset{dotsize=0.7 2.5,dotscale=1 1,fillcolor=black}
\psset{arrowsize=1 2,arrowlength=1,arrowinset=0.25,tbarsize=0.7 5,bracketlength=0.15,rbracketlength=0.15}
\begin{pspicture}(0,0)(32.5,62.5)
\psline[linewidth=0.75](30,40)(15,25)
\psline[linewidth=0.75](15,25)(15,5)
\newrgbcolor{userFillColour}{0.2 0 0.2}
\rput{0}(15,25){\psellipse[fillcolor=userFillColour,fillstyle=solid](0,0)(3.79,-3.79)}
\psline[linewidth=0.75](0,40)(15,25)
\rput[r](12.5,13.75){$\AAh$}
\psline[linewidth=0.75](0,57.5)(0,40)
\psline[linewidth=0.75](30,57.5)(30,40)
\rput[l](32.5,45){$\AAh$}
\rput[l](2.5,45){$\AAh$}
\rput[l](21.25,25){$\ccopy$}
\rput(15.62,1.25){$\eex$}
\rput(0,62.5){$\eex$}
\rput(30,62.5){$\eex$}
\end{pspicture}


==> PIC/dataserv-cun.tex <==
%%Created by jPicEdt 1.4.1_03: mixed JPIC-XML/LaTeX format
%%Mon Aug 31 15:54:20 GMT-10:00 2020
%%Begin JPIC-XML
%<?xml version="1.0" standalone="yes"?>
%<jpic x-min="5.93" x-max="17.5" y-min="1.25" y-max="59.07" auto-bounding="true">
%<multicurve fill-style= "none"
%	 points= "(10,55);(10,55);(10,5);(10,5)"
%	 stroke-width= "0.75"
%	 />
%<ellipse p3= "(14.07,50.93)"
%	 fill-style= "solid"
%	 p2= "(14.07,59.07)"
%	 fill-color= "#330033"
%	 p1= "(5.93,59.07)"
%	 closure= "open"
%	 angle-end= "0"
%	 angle-start= "0"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(7.5,25)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\AAh$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(17.5,55)"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\delete$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(10,1.25)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\eex$
%</text>
%</jpic>
%%End JPIC-XML
%PSTricks content-type (pstricks.sty package needed)
%Add \usepackage{pstricks} in the preamble of your LaTeX file
%You can rescale the whole picture (to 80% for instance) by using the command \def\JPicScale{0.8}
\ifx\JPicScale\undefined\def\JPicScale{1}\fi
\psset{unit=\JPicScale mm}
\psset{linewidth=0.3,dotsep=1,hatchwidth=0.3,hatchsep=1.5,shadowsize=1,dimen=middle}
\psset{dotsize=0.7 2.5,dotscale=1 1,fillcolor=black}
\psset{arrowsize=1 2,arrowlength=1,arrowinset=0.25,tbarsize=0.7 5,bracketlength=0.15,rbracketlength=0.15}
\begin{pspicture}(0,0)(17.5,59.07)
\psline[linewidth=0.75](10,55)(10,5)
\newrgbcolor{userFillColour}{0.2 0 0.2}
\rput{0}(10,55){\psellipse[fillcolor=userFillColour,fillstyle=solid](0,0)(4.07,-4.07)}
\rput[r](7.5,25){$\AAh$}
\rput[l](17.5,55){$\delete$}
\rput(10,1.25){$\eex$}
\end{pspicture}


==> PIC/dataserv-effect-eqns.tex <==
%%Created by jPicEdt 1.4.1_03: mixed JPIC-XML/LaTeX format
%%Mon Nov 04 16:49:19 GMT-10:00 2019
%%Begin JPIC-XML
%<?xml version="1.0" standalone="yes"?>
%<jpic x-min="0" x-max="100" y-min="0" y-max="80" auto-bounding="true">
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(90,20);(90,20);(90,0);(90,0)"
%	 />
%<ellipse p3= "(94.07,15.93)"
%	 p2= "(94.07,24.07)"
%	 fill-color= "#330033"
%	 p1= "(85.93,24.07)"
%	 closure= "open"
%	 fill-style= "solid"
%	 angle-end= "0"
%	 angle-start= "0"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(40,35);(40,35);(25,20);(25,20)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(25,20);(25,20);(25,0);(25,0)"
%	 />
%<ellipse p3= "(28.79,16.21)"
%	 p2= "(28.79,23.79)"
%	 fill-color= "#330033"
%	 p1= "(21.21,23.79)"
%	 closure= "open"
%	 fill-style= "solid"
%	 angle-end= "0"
%	 angle-start= "0"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(10,35);(10,35);(25,20);(25,20)"
%	 />
%<text text-vert-align= "center-v"
%	 anchor-point= "(22.5,0)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\AAh$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(87.5,0)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\AAh$
%</text>
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(10,43.75);(10,43.75);(10,35);(10,35)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(40,43.75);(40,43.75);(40,35);(40,35)"
%	 />
%<text text-vert-align= "center-v"
%	 anchor-point= "(90,35)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\delete$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(25,35)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\ccopy$
%</text>
%<parallelogram p3= "(45,45)"
%	 p2= "(45,55)"
%	 fill-color= "#ffffff"
%	 p1= "(35,55)"
%	 stroke-width= "0.75"
%	 fill-style= "solid"
%	 />
%<parallelogram p3= "(15,45)"
%	 p2= "(15,55)"
%	 fill-color= "#ffffff"
%	 p1= "(5,55)"
%	 stroke-width= "0.75"
%	 fill-style= "solid"
%	 />
%<text text-vert-align= "center-v"
%	 stroke-dasharray= "8;8"
%	 anchor-point= "(40,50)"
%	 stroke-width= "0.75"
%	 fill-style= "none"
%	 stroke-style= "dashed"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\unit$
%</text>
%<parallelogram p3= "(37.5,80)"
%	 p2= "(37.5,55)"
%	 fill-color= "#999999"
%	 p1= "(42.5,55)"
%	 stroke-color= "#999999"
%	 fill-style= "solid"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(40,80);(40,80);(40,55);(40,55)"
%	 />
%<text text-vert-align= "center-v"
%	 stroke-dasharray= "8;8"
%	 anchor-point= "(10,50)"
%	 stroke-width= "0.75"
%	 fill-style= "none"
%	 stroke-style= "dashed"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\unit$
%</text>
%<parallelogram p3= "(7.5,80)"
%	 p2= "(7.5,55)"
%	 fill-color= "#999999"
%	 p1= "(12.5,55)"
%	 stroke-color= "#999999"
%	 fill-style= "solid"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(10,80);(10,80);(10,55);(10,55)"
%	 />
%<parallelogram p3= "(87.5,80)"
%	 p2= "(87.5,55)"
%	 fill-color= "#999999"
%	 p1= "(92.5,55)"
%	 stroke-color= "#999999"
%	 fill-style= "solid"
%	 />
%<parallelogram p3= "(95,45)"
%	 p2= "(95,55)"
%	 fill-color= "#ffffff"
%	 p1= "(85,55)"
%	 stroke-width= "0.75"
%	 fill-style= "solid"
%	 />
%<text text-vert-align= "center-v"
%	 stroke-dasharray= "8;8"
%	 anchor-point= "(90,50)"
%	 stroke-width= "0.75"
%	 fill-style= "none"
%	 stroke-style= "dashed"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\unit$
%</text>
%<parallelogram p3= "(100,60)"
%	 p2= "(100,12.5)"
%	 p1= "(80,12.5)"
%	 stroke-width= "0.75"
%	 fill-style= "none"
%	 />
%<parallelogram p3= "(50,60)"
%	 p2= "(50,12.5)"
%	 p1= "(0,12.5)"
%	 stroke-width= "0.75"
%	 fill-style= "none"
%	 />
%<text text-vert-align= "center-v"
%	 anchor-point= "(15,78.75)"
%	 stroke-width= "0.7"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\MAAh$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(95,78.75)"
%	 stroke-width= "0.7"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\Miih$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(45,78.75)"
%	 stroke-width= "0.7"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\MAAh$
%</text>
%</jpic>
%%End JPIC-XML
%PSTricks content-type (pstricks.sty package needed)
%Add \usepackage{pstricks} in the preamble of your LaTeX file
%You can rescale the whole picture (to 80% for instance) by using the command \def\JPicScale{0.8}
\ifx\JPicScale\undefined\def\JPicScale{1}\fi
\psset{unit=\JPicScale mm}
\psset{linewidth=0.3,dotsep=1,hatchwidth=0.3,hatchsep=1.5,shadowsize=1,dimen=middle}
\psset{dotsize=0.7 2.5,dotscale=1 1,fillcolor=black}
\psset{arrowsize=1 2,arrowlength=1,arrowinset=0.25,tbarsize=0.7 5,bracketlength=0.15,rbracketlength=0.15}
\begin{pspicture}(0,0)(100,80)
\psline[linewidth=0.75](90,20)(90,0)
\newrgbcolor{userFillColour}{0.2 0 0.2}
\rput{0}(90,20){\psellipse[fillcolor=userFillColour,fillstyle=solid](0,0)(4.07,-4.07)}
\psline[linewidth=0.75](40,35)(25,20)
\psline[linewidth=0.75](25,20)(25,0)
\newrgbcolor{userFillColour}{0.2 0 0.2}
\rput{0}(25,20){\psellipse[fillcolor=userFillColour,fillstyle=solid](0,0)(3.79,-3.79)}
\psline[linewidth=0.75](10,35)(25,20)
\rput[r](22.5,0){$\AAh$}
\rput[r](87.5,0){$\AAh$}
\psline[linewidth=0.75](10,43.75)(10,35)
\psline[linewidth=0.75](40,43.75)(40,35)
\rput(90,35){$\delete$}
\rput(25,35){$\ccopy$}
\pspolygon[linewidth=0.75,fillcolor=white,fillstyle=solid](35,55)(45,55)(45,45)(35,45)
\pspolygon[linewidth=0.75,fillcolor=white,fillstyle=solid](5,55)(15,55)(15,45)(5,45)
\rput(40,50){$\unit$}
\newrgbcolor{userLineColour}{0.6 0.6 0.6}
\newrgbcolor{userFillColour}{0.6 0.6 0.6}
\pspolygon[linecolor=userLineColour,fillcolor=userFillColour,fillstyle=solid](42.5,55)(37.5,55)(37.5,80)(42.5,80)
\psline[linewidth=0.75](40,80)(40,55)
\rput(10,50){$\unit$}
\newrgbcolor{userLineColour}{0.6 0.6 0.6}
\newrgbcolor{userFillColour}{0.6 0.6 0.6}
\pspolygon[linecolor=userLineColour,fillcolor=userFillColour,fillstyle=solid](12.5,55)(7.5,55)(7.5,80)(12.5,80)
\psline[linewidth=0.75](10,80)(10,55)
\newrgbcolor{userLineColour}{0.6 0.6 0.6}
\newrgbcolor{userFillColour}{0.6 0.6 0.6}
\pspolygon[linecolor=userLineColour,fillcolor=userFillColour,fillstyle=solid](92.5,55)(87.5,55)(87.5,80)(92.5,80)
\pspolygon[linewidth=0.75,fillcolor=white,fillstyle=solid](85,55)(95,55)(95,45)(85,45)
\rput(90,50){$\unit$}
\pspolygon[linewidth=0.75](80,12.5)(100,12.5)(100,60)(80,60)
\pspolygon[linewidth=0.75](0,12.5)(50,12.5)(50,60)(0,60)
\rput[l](15,78.75){$\MAAh$}
\rput[l](95,78.75){$\Miih$}
\rput[l](45,78.75){$\MAAh$}
\end{pspicture}


==> PIC/dataserv-effect-free.tex <==
%%Created by jPicEdt 1.4.1_03: mixed JPIC-XML/LaTeX format
%%Mon Dec 30 10:27:27 GMT-10:00 2019
%%Begin JPIC-XML
%<?xml version="1.0" standalone="yes"?>
%<jpic x-min="-2.5" x-max="256.25" y-min="0" y-max="120" auto-bounding="true">
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(85,50);(85,50);(85,40);(85,40)"
%	 />
%<parallelogram fill-color= "#999999"
%	 fill-style= "solid"
%	 p3= "(82.5,120)"
%	 p2= "(82.5,100)"
%	 p1= "(117.5,100)"
%	 stroke-color= "#999999"
%	 />
%<parallelogram fill-color= "#999999"
%	 fill-style= "solid"
%	 p3= "(82.5,97.5)"
%	 p2= "(82.5,70)"
%	 p1= "(87.5,70)"
%	 stroke-color= "#999999"
%	 />
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(60,75)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\EQLS
%</text>
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(115,50);(115,50);(115,40);(115,40)"
%	 />
%<parallelogram fill-color= "#999999"
%	 fill-style= "solid"
%	 p3= "(112.5,95)"
%	 p2= "(112.5,70)"
%	 p1= "(117.5,70)"
%	 stroke-color= "#999999"
%	 />
%<parallelogram fill-color= "#ffffff"
%	 fill-style= "solid"
%	 stroke-width= "0.75"
%	 p3= "(120,90)"
%	 p2= "(120,100)"
%	 p1= "(80,100)"
%	 />
%<text fill-color= "#ffffff"
%	 fill-style= "solid"
%	 text-vert-align= "center-v"
%	 stroke-color= "#999999"
%	 anchor-point= "(100,95)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\ffubini$
%</text>
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(85,120);(85,120);(85,70);(85,70)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(115,120);(115,120);(115,70);(115,70)"
%	 />
%<parallelogram fill-color= "#ffffff"
%	 fill-style= "solid"
%	 stroke-width= "0.75"
%	 p3= "(95,50)"
%	 p2= "(95,70)"
%	 p1= "(75,70)"
%	 />
%<parallelogram fill-color= "#ffffff"
%	 fill-style= "solid"
%	 stroke-width= "0.75"
%	 p3= "(125,50)"
%	 p2= "(125,70)"
%	 p1= "(105,70)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(115,40);(115,40);(100,25);(100,25)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(100,25);(100,25);(100,0);(100,0)"
%	 />
%<ellipse fill-color= "#330033"
%	 fill-style= "solid"
%	 p3= "(103.79,21.21)"
%	 p2= "(103.79,28.79)"
%	 p1= "(96.21,28.79)"
%	 closure= "open"
%	 angle-end= "0"
%	 angle-start= "0"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(85,40);(85,40);(100,25);(100,25)"
%	 />
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(85,60)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\fee$
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(115,60)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\fee$
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(97.5,0)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\AAh$
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(120,80)"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\MBBh$
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(90,80)"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\MBBh$
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(118.75,120)"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\MBBBh$
%</text>
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(20,15);(20,15);(20,0);(20,0)"
%	 />
%<parallelogram fill-color= "#999999"
%	 fill-style= "solid"
%	 p3= "(17.5,52.5)"
%	 p2= "(17.5,35)"
%	 p1= "(22.5,35)"
%	 stroke-color= "#999999"
%	 />
%<parallelogram fill-color= "#999999"
%	 fill-style= "solid"
%	 p3= "(-2.5,102.5)"
%	 p2= "(-2.5,50)"
%	 p1= "(42.5,50)"
%	 stroke-color= "#999999"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(5,90);(5,90);(5,75);(5,75)"
%	 />
%<parallelogram fill-color= "#999999"
%	 fill-style= "solid"
%	 p3= "(2.5,120)"
%	 p2= "(2.5,100)"
%	 p1= "(37.5,100)"
%	 stroke-color= "#999999"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(35,90);(35,90);(35,75);(35,75)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(5,120);(5,120);(5,100);(5,100)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(35,120);(35,120);(35,100);(35,100)"
%	 />
%<parallelogram fill-color= "#ffffff"
%	 fill-style= "solid"
%	 stroke-width= "0.75"
%	 p3= "(40,90)"
%	 p2= "(40,100)"
%	 p1= "(0,100)"
%	 />
%<text fill-style= "none"
%	 stroke-width= "0.75"
%	 text-vert-align= "center-v"
%	 stroke-dasharray= "8;8"
%	 anchor-point= "(20,95)"
%	 text-frame= "noframe"
%	 stroke-style= "dashed"
%	 text-hor-align= "center-h"
%	 >
%$\unit$
%</text>
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(35,75);(35,75);(20,60);(20,60)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(20,60);(20,60);(20,35);(20,35)"
%	 />
%<ellipse fill-color= "#330033"
%	 fill-style= "solid"
%	 p3= "(23.79,56.21)"
%	 p2= "(23.79,63.79)"
%	 p1= "(16.21,63.79)"
%	 closure= "open"
%	 angle-end= "0"
%	 angle-start= "0"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(5,75);(5,75);(20,60);(20,60)"
%	 />
%<parallelogram fill-color= "#ffffff"
%	 fill-style= "solid"
%	 stroke-width= "0.75"
%	 p3= "(30,15)"
%	 p2= "(30,35)"
%	 p1= "(10,35)"
%	 />
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(20,25)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\fee$
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(17.5,0)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\AAh$
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(40,120)"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\MBBBh$
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(25,42.5)"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\MBBh$
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(20,75)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\MDDB$
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(106.25,25)"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\DDA$
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(235,75)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\EQLS
%</text>
%<parallelogram fill-color= "#999999"
%	 fill-style= "solid"
%	 p3= "(207.5,100)"
%	 p2= "(207.5,55)"
%	 p1= "(222.5,55)"
%	 stroke-color= "#999999"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(215,15);(215,15);(215,0);(215,0)"
%	 />
%<parallelogram fill-color= "#999999"
%	 fill-style= "solid"
%	 p3= "(212.5,55)"
%	 p2= "(212.5,35)"
%	 p1= "(217.5,35)"
%	 stroke-color= "#999999"
%	 />
%<parallelogram fill-color= "#999999"
%	 fill-style= "solid"
%	 p3= "(212.5,120)"
%	 p2= "(212.5,90)"
%	 p1= "(217.5,90)"
%	 stroke-color= "#999999"
%	 />
%<parallelogram fill-color= "#ffffff"
%	 fill-style= "solid"
%	 stroke-width= "0.75"
%	 p3= "(220,87.5)"
%	 p2= "(220,97.5)"
%	 p1= "(210,97.5)"
%	 />
%<text fill-style= "none"
%	 stroke-width= "0.75"
%	 text-vert-align= "center-v"
%	 stroke-dasharray= "8;8"
%	 anchor-point= "(215,92.5)"
%	 text-frame= "noframe"
%	 stroke-style= "dashed"
%	 text-hor-align= "center-h"
%	 >
%$\unit$
%</text>
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(215,60);(215,60);(215,35);(215,35)"
%	 />
%<ellipse fill-color= "#330033"
%	 fill-style= "solid"
%	 p3= "(218.79,56.21)"
%	 p2= "(218.79,63.79)"
%	 p1= "(211.21,63.79)"
%	 closure= "open"
%	 angle-end= "0"
%	 angle-start= "0"
%	 />
%<parallelogram fill-color= "#ffffff"
%	 fill-style= "solid"
%	 stroke-width= "0.75"
%	 p3= "(225,15)"
%	 p2= "(225,35)"
%	 p1= "(205,35)"
%	 />
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(215,25)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\fee$
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(212.5,0)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\AAh$
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(220,42.5)"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\MBBh$
%</text>
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(250,60);(250,60);(250,0);(250,0)"
%	 />
%<parallelogram fill-color= "#999999"
%	 fill-style= "solid"
%	 p3= "(247.5,120)"
%	 p2= "(247.5,90)"
%	 p1= "(252.5,90)"
%	 stroke-color= "#999999"
%	 />
%<parallelogram fill-color= "#ffffff"
%	 fill-style= "solid"
%	 stroke-width= "0.75"
%	 p3= "(255,87.5)"
%	 p2= "(255,97.5)"
%	 p1= "(245,97.5)"
%	 />
%<text fill-style= "none"
%	 stroke-width= "0.75"
%	 text-vert-align= "center-v"
%	 stroke-dasharray= "8;8"
%	 anchor-point= "(250,92.5)"
%	 text-frame= "noframe"
%	 stroke-style= "dashed"
%	 text-hor-align= "center-h"
%	 >
%$\unit$
%</text>
%<ellipse fill-color= "#330033"
%	 fill-style= "solid"
%	 p3= "(253.79,56.21)"
%	 p2= "(253.79,63.79)"
%	 p1= "(246.21,63.79)"
%	 closure= "open"
%	 angle-end= "0"
%	 angle-start= "0"
%	 />
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(247.5,0)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\AAh$
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(220,120)"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\Mii$
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(255,120)"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\Mii$
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(256.25,60)"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\Taa$
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(215,75)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\MTbb$
%</text>
%</jpic>
%%End JPIC-XML
%PSTricks content-type (pstricks.sty package needed)
%Add \usepackage{pstricks} in the preamble of your LaTeX file
%You can rescale the whole picture (to 80% for instance) by using the command \def\JPicScale{0.8}
\ifx\JPicScale\undefined\def\JPicScale{1}\fi
\psset{unit=\JPicScale mm}
\psset{linewidth=0.3,dotsep=1,hatchwidth=0.3,hatchsep=1.5,shadowsize=1,dimen=middle}
\psset{dotsize=0.7 2.5,dotscale=1 1,fillcolor=black}
\psset{arrowsize=1 2,arrowlength=1,arrowinset=0.25,tbarsize=0.7 5,bracketlength=0.15,rbracketlength=0.15}
\begin{pspicture}(0,0)(256.25,120)
\psline[linewidth=0.75](85,50)(85,40)
\newrgbcolor{userLineColour}{0.6 0.6 0.6}
\newrgbcolor{userFillColour}{0.6 0.6 0.6}
\pspolygon[linecolor=userLineColour,fillcolor=userFillColour,fillstyle=solid](117.5,100)(82.5,100)(82.5,120)(117.5,120)
\newrgbcolor{userLineColour}{0.6 0.6 0.6}
\newrgbcolor{userFillColour}{0.6 0.6 0.6}
\pspolygon[linecolor=userLineColour,fillcolor=userFillColour,fillstyle=solid](87.5,70)(82.5,70)(82.5,97.5)(87.5,97.5)
\rput(60,75){\EQLS}
\psline[linewidth=0.75](115,50)(115,40)
\newrgbcolor{userLineColour}{0.6 0.6 0.6}
\newrgbcolor{userFillColour}{0.6 0.6 0.6}
\pspolygon[linecolor=userLineColour,fillcolor=userFillColour,fillstyle=solid](117.5,70)(112.5,70)(112.5,95)(117.5,95)
\pspolygon[linewidth=0.75,fillcolor=white,fillstyle=solid](80,100)(120,100)(120,90)(80,90)
\newrgbcolor{userLineColour}{0.6 0.6 0.6}
\rput(100,95){$\ffubini$}
\psline[linewidth=0.75](85,120)(85,70)
\psline[linewidth=0.75](115,120)(115,70)
\pspolygon[linewidth=0.75,fillcolor=white,fillstyle=solid](75,70)(95,70)(95,50)(75,50)
\pspolygon[linewidth=0.75,fillcolor=white,fillstyle=solid](105,70)(125,70)(125,50)(105,50)
\psline[linewidth=0.75](115,40)(100,25)
\psline[linewidth=0.75](100,25)(100,0)
\newrgbcolor{userFillColour}{0.2 0 0.2}
\rput{0}(100,25){\psellipse[fillcolor=userFillColour,fillstyle=solid](0,0)(3.79,-3.79)}
\psline[linewidth=0.75](85,40)(100,25)
\rput(85,60){$\fee$}
\rput(115,60){$\fee$}
\rput[r](97.5,0){$\AAh$}
\rput[l](120,80){$\MBBh$}
\rput[l](90,80){$\MBBh$}
\rput[l](118.75,120){$\MBBBh$}
\psline[linewidth=0.75](20,15)(20,0)
\newrgbcolor{userLineColour}{0.6 0.6 0.6}
\newrgbcolor{userFillColour}{0.6 0.6 0.6}
\pspolygon[linecolor=userLineColour,fillcolor=userFillColour,fillstyle=solid](22.5,35)(17.5,35)(17.5,52.5)(22.5,52.5)
\newrgbcolor{userLineColour}{0.6 0.6 0.6}
\newrgbcolor{userFillColour}{0.6 0.6 0.6}
\pspolygon[linecolor=userLineColour,fillcolor=userFillColour,fillstyle=solid](42.5,50)(-2.5,50)(-2.5,102.5)(42.5,102.5)
\psline[linewidth=0.75](5,90)(5,75)
\newrgbcolor{userLineColour}{0.6 0.6 0.6}
\newrgbcolor{userFillColour}{0.6 0.6 0.6}
\pspolygon[linecolor=userLineColour,fillcolor=userFillColour,fillstyle=solid](37.5,100)(2.5,100)(2.5,120)(37.5,120)
\psline[linewidth=0.75](35,90)(35,75)
\psline[linewidth=0.75](5,120)(5,100)
\psline[linewidth=0.75](35,120)(35,100)
\pspolygon[linewidth=0.75,fillcolor=white,fillstyle=solid](0,100)(40,100)(40,90)(0,90)
\rput(20,95){$\unit$}
\psline[linewidth=0.75](35,75)(20,60)
\psline[linewidth=0.75](20,60)(20,35)
\newrgbcolor{userFillColour}{0.2 0 0.2}
\rput{0}(20,60){\psellipse[fillcolor=userFillColour,fillstyle=solid](0,0)(3.79,-3.79)}
\psline[linewidth=0.75](5,75)(20,60)
\pspolygon[linewidth=0.75,fillcolor=white,fillstyle=solid](10,35)(30,35)(30,15)(10,15)
\rput(20,25){$\fee$}
\rput[r](17.5,0){$\AAh$}
\rput[l](40,120){$\MBBBh$}
\rput[l](25,42.5){$\MBBh$}
\rput(20,75){$\MDDB$}
\rput[l](106.25,25){$\DDA$}
\rput(235,75){\EQLS}
\newrgbcolor{userLineColour}{0.6 0.6 0.6}
\newrgbcolor{userFillColour}{0.6 0.6 0.6}
\pspolygon[linecolor=userLineColour,fillcolor=userFillColour,fillstyle=solid](222.5,55)(207.5,55)(207.5,100)(222.5,100)
\psline[linewidth=0.75](215,15)(215,0)
\newrgbcolor{userLineColour}{0.6 0.6 0.6}
\newrgbcolor{userFillColour}{0.6 0.6 0.6}
\pspolygon[linecolor=userLineColour,fillcolor=userFillColour,fillstyle=solid](217.5,35)(212.5,35)(212.5,55)(217.5,55)
\newrgbcolor{userLineColour}{0.6 0.6 0.6}
\newrgbcolor{userFillColour}{0.6 0.6 0.6}
\pspolygon[linecolor=userLineColour,fillcolor=userFillColour,fillstyle=solid](217.5,90)(212.5,90)(212.5,120)(217.5,120)
\pspolygon[linewidth=0.75,fillcolor=white,fillstyle=solid](210,97.5)(220,97.5)(220,87.5)(210,87.5)
\rput(215,92.5){$\unit$}
\psline[linewidth=0.75](215,60)(215,35)
\newrgbcolor{userFillColour}{0.2 0 0.2}
\rput{0}(215,60){\psellipse[fillcolor=userFillColour,fillstyle=solid](0,0)(3.79,-3.79)}
\pspolygon[linewidth=0.75,fillcolor=white,fillstyle=solid](205,35)(225,35)(225,15)(205,15)
\rput(215,25){$\fee$}
\rput[r](212.5,0){$\AAh$}
\rput[l](220,42.5){$\MBBh$}
\psline[linewidth=0.75](250,60)(250,0)
\newrgbcolor{userLineColour}{0.6 0.6 0.6}
\newrgbcolor{userFillColour}{0.6 0.6 0.6}
\pspolygon[linecolor=userLineColour,fillcolor=userFillColour,fillstyle=solid](252.5,90)(247.5,90)(247.5,120)(252.5,120)
\pspolygon[linewidth=0.75,fillcolor=white,fillstyle=solid](245,97.5)(255,97.5)(255,87.5)(245,87.5)
\rput(250,92.5){$\unit$}
\newrgbcolor{userFillColour}{0.2 0 0.2}
\rput{0}(250,60){\psellipse[fillcolor=userFillColour,fillstyle=solid](0,0)(3.79,-3.79)}
\rput[r](247.5,0){$\AAh$}
\rput[l](220,120){$\Mii$}
\rput[l](255,120){$\Mii$}
\rput[l](256.25,60){$\Taa$}
\rput(215,75){$\MTbb$}
\end{pspicture}


==> PIC/dataserv-effect.tex <==
%%Created by jPicEdt 1.4.1_03: mixed JPIC-XML/LaTeX format
%%Thu Dec 26 13:51:22 GMT-10:00 2019
%%Begin JPIC-XML
%<?xml version="1.0" standalone="yes"?>
%<jpic x-min="0" x-max="100" y-min="0" y-max="80" auto-bounding="true">
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(90,20);(90,20);(90,0);(90,0)"
%	 />
%<ellipse fill-color= "#330033"
%	 fill-style= "solid"
%	 p3= "(94.07,15.93)"
%	 p2= "(94.07,24.07)"
%	 p1= "(85.93,24.07)"
%	 closure= "open"
%	 angle-end= "0"
%	 angle-start= "0"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(40,35);(40,35);(25,20);(25,20)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(25,20);(25,20);(25,0);(25,0)"
%	 />
%<ellipse fill-color= "#330033"
%	 fill-style= "solid"
%	 p3= "(28.79,16.21)"
%	 p2= "(28.79,23.79)"
%	 p1= "(21.21,23.79)"
%	 closure= "open"
%	 angle-end= "0"
%	 angle-start= "0"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(10,35);(10,35);(25,20);(25,20)"
%	 />
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(22.5,0)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\AAh$
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(87.5,0)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\AAh$
%</text>
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(10,43.75);(10,43.75);(10,35);(10,35)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(40,43.75);(40,43.75);(40,35);(40,35)"
%	 />
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(90,35)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\delete$
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(25,35)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\ccopy$
%</text>
%<parallelogram fill-color= "#ffffff"
%	 fill-style= "solid"
%	 stroke-width= "0.75"
%	 p3= "(45,45)"
%	 p2= "(45,55)"
%	 p1= "(35,55)"
%	 />
%<parallelogram fill-color= "#ffffff"
%	 fill-style= "solid"
%	 stroke-width= "0.75"
%	 p3= "(15,45)"
%	 p2= "(15,55)"
%	 p1= "(5,55)"
%	 />
%<text fill-style= "none"
%	 stroke-width= "0.75"
%	 text-vert-align= "center-v"
%	 stroke-dasharray= "8;8"
%	 anchor-point= "(40,50)"
%	 text-frame= "noframe"
%	 stroke-style= "dashed"
%	 text-hor-align= "center-h"
%	 >
%$\unit$
%</text>
%<parallelogram fill-color= "#999999"
%	 fill-style= "solid"
%	 p3= "(37.5,80)"
%	 p2= "(37.5,55)"
%	 p1= "(42.5,55)"
%	 stroke-color= "#999999"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(40,80);(40,80);(40,55);(40,55)"
%	 />
%<text fill-style= "none"
%	 stroke-width= "0.75"
%	 text-vert-align= "center-v"
%	 stroke-dasharray= "8;8"
%	 anchor-point= "(10,50)"
%	 text-frame= "noframe"
%	 stroke-style= "dashed"
%	 text-hor-align= "center-h"
%	 >
%$\unit$
%</text>
%<parallelogram fill-color= "#999999"
%	 fill-style= "solid"
%	 p3= "(7.5,80)"
%	 p2= "(7.5,55)"
%	 p1= "(12.5,55)"
%	 stroke-color= "#999999"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(10,80);(10,80);(10,55);(10,55)"
%	 />
%<parallelogram fill-color= "#999999"
%	 fill-style= "solid"
%	 p3= "(87.5,80)"
%	 p2= "(87.5,55)"
%	 p1= "(92.5,55)"
%	 stroke-color= "#999999"
%	 />
%<parallelogram fill-color= "#ffffff"
%	 fill-style= "solid"
%	 stroke-width= "0.75"
%	 p3= "(95,45)"
%	 p2= "(95,55)"
%	 p1= "(85,55)"
%	 />
%<text fill-style= "none"
%	 stroke-width= "0.75"
%	 text-vert-align= "center-v"
%	 stroke-dasharray= "8;8"
%	 anchor-point= "(90,50)"
%	 text-frame= "noframe"
%	 stroke-style= "dashed"
%	 text-hor-align= "center-h"
%	 >
%$\unit$
%</text>
%<parallelogram fill-style= "none"
%	 stroke-width= "0.75"
%	 p3= "(100,60)"
%	 p2= "(100,12.5)"
%	 p1= "(80,12.5)"
%	 />
%<parallelogram fill-style= "none"
%	 stroke-width= "0.75"
%	 p3= "(50,60)"
%	 p2= "(50,12.5)"
%	 p1= "(0,12.5)"
%	 />
%<text fill-style= "none"
%	 stroke-width= "0.7"
%	 text-vert-align= "center-v"
%	 anchor-point= "(15,78.75)"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\MAAh$
%</text>
%<text fill-style= "none"
%	 stroke-width= "0.7"
%	 text-vert-align= "center-v"
%	 anchor-point= "(95,78.75)"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\Miih$
%</text>
%<text fill-style= "none"
%	 stroke-width= "0.7"
%	 text-vert-align= "center-v"
%	 anchor-point= "(45,78.75)"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\MAAh$
%</text>
%</jpic>
%%End JPIC-XML
%PSTricks content-type (pstricks.sty package needed)
%Add \usepackage{pstricks} in the preamble of your LaTeX file
%You can rescale the whole picture (to 80% for instance) by using the command \def\JPicScale{0.8}
\ifx\JPicScale\undefined\def\JPicScale{1}\fi
\psset{unit=\JPicScale mm}
\psset{linewidth=0.3,dotsep=1,hatchwidth=0.3,hatchsep=1.5,shadowsize=1,dimen=middle}
\psset{dotsize=0.7 2.5,dotscale=1 1,fillcolor=black}
\psset{arrowsize=1 2,arrowlength=1,arrowinset=0.25,tbarsize=0.7 5,bracketlength=0.15,rbracketlength=0.15}
\begin{pspicture}(0,0)(100,80)
\psline[linewidth=0.75](90,20)(90,0)
\newrgbcolor{userFillColour}{0.2 0 0.2}
\rput{0}(90,20){\psellipse[fillcolor=userFillColour,fillstyle=solid](0,0)(4.07,-4.07)}
\psline[linewidth=0.75](40,35)(25,20)
\psline[linewidth=0.75](25,20)(25,0)
\newrgbcolor{userFillColour}{0.2 0 0.2}
\rput{0}(25,20){\psellipse[fillcolor=userFillColour,fillstyle=solid](0,0)(3.79,-3.79)}
\psline[linewidth=0.75](10,35)(25,20)
\rput[r](22.5,0){$\AAh$}
\rput[r](87.5,0){$\AAh$}
\psline[linewidth=0.75](10,43.75)(10,35)
\psline[linewidth=0.75](40,43.75)(40,35)
\rput(90,35){$\delete$}
\rput(25,35){$\ccopy$}
\pspolygon[linewidth=0.75,fillcolor=white,fillstyle=solid](35,55)(45,55)(45,45)(35,45)
\pspolygon[linewidth=0.75,fillcolor=white,fillstyle=solid](5,55)(15,55)(15,45)(5,45)
\rput(40,50){$\unit$}
\newrgbcolor{userLineColour}{0.6 0.6 0.6}
\newrgbcolor{userFillColour}{0.6 0.6 0.6}
\pspolygon[linecolor=userLineColour,fillcolor=userFillColour,fillstyle=solid](42.5,55)(37.5,55)(37.5,80)(42.5,80)
\psline[linewidth=0.75](40,80)(40,55)
\rput(10,50){$\unit$}
\newrgbcolor{userLineColour}{0.6 0.6 0.6}
\newrgbcolor{userFillColour}{0.6 0.6 0.6}
\pspolygon[linecolor=userLineColour,fillcolor=userFillColour,fillstyle=solid](12.5,55)(7.5,55)(7.5,80)(12.5,80)
\psline[linewidth=0.75](10,80)(10,55)
\newrgbcolor{userLineColour}{0.6 0.6 0.6}
\newrgbcolor{userFillColour}{0.6 0.6 0.6}
\pspolygon[linecolor=userLineColour,fillcolor=userFillColour,fillstyle=solid](92.5,55)(87.5,55)(87.5,80)(92.5,80)
\pspolygon[linewidth=0.75,fillcolor=white,fillstyle=solid](85,55)(95,55)(95,45)(85,45)
\rput(90,50){$\unit$}
\pspolygon[linewidth=0.75](80,12.5)(100,12.5)(100,60)(80,60)
\pspolygon[linewidth=0.75](0,12.5)(50,12.5)(50,60)(0,60)
\rput[l](15,78.75){$\MAAh$}
\rput[l](95,78.75){$\Miih$}
\rput[l](45,78.75){$\MAAh$}
\end{pspicture}


==> PIC/dataserv-eqns.tex <==
%%Created by jPicEdt 1.4.1_03: mixed JPIC-XML/LaTeX format
%%Sun Nov 03 14:11:15 GMT-10:00 2019
%%Begin JPIC-XML
%<?xml version="1.0" standalone="yes"?>
%<jpic x-min="0" x-max="77.5" y-min="0" y-max="54.07" auto-bounding="true">
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(70,50);(70,50);(70,0);(70,0)"
%	 />
%<ellipse fill-style= "solid"
%	 p3= "(74.07,45.93)"
%	 p2= "(74.07,54.07)"
%	 p1= "(65.93,54.07)"
%	 fill-color= "#330033"
%	 closure= "open"
%	 angle-end= "0"
%	 angle-start= "0"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(30,35);(30,35);(15,20);(15,20)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(15,20);(15,20);(15,0);(15,0)"
%	 />
%<ellipse fill-style= "solid"
%	 p3= "(18.79,16.21)"
%	 p2= "(18.79,23.79)"
%	 p1= "(11.21,23.79)"
%	 fill-color= "#330033"
%	 closure= "open"
%	 angle-end= "0"
%	 angle-start= "0"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(0,35);(0,35);(15,20);(15,20)"
%	 />
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(12.5,0)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\AAh$
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(67.5,0)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\AAh$
%</text>
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(0,52.5);(0,52.5);(0,35);(0,35)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(30,52.5);(30,52.5);(30,35);(30,35)"
%	 />
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(32.5,51.25)"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\AAh$
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(2.5,51.25)"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\AAh$
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(77.5,50)"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\delete$
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(21.25,20)"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\ccopy$
%</text>
%</jpic>
%%End JPIC-XML
%PSTricks content-type (pstricks.sty package needed)
%Add \usepackage{pstricks} in the preamble of your LaTeX file
%You can rescale the whole picture (to 80% for instance) by using the command \def\JPicScale{0.8}
\ifx\JPicScale\undefined\def\JPicScale{1}\fi
\psset{unit=\JPicScale mm}
\psset{linewidth=0.3,dotsep=1,hatchwidth=0.3,hatchsep=1.5,shadowsize=1,dimen=middle}
\psset{dotsize=0.7 2.5,dotscale=1 1,fillcolor=black}
\psset{arrowsize=1 2,arrowlength=1,arrowinset=0.25,tbarsize=0.7 5,bracketlength=0.15,rbracketlength=0.15}
\begin{pspicture}(0,0)(77.5,54.07)
\psline[linewidth=0.75](70,50)(70,0)
\newrgbcolor{userFillColour}{0.2 0 0.2}
\rput{0}(70,50){\psellipse[fillcolor=userFillColour,fillstyle=solid](0,0)(4.07,-4.07)}
\psline[linewidth=0.75](30,35)(15,20)
\psline[linewidth=0.75](15,20)(15,0)
\newrgbcolor{userFillColour}{0.2 0 0.2}
\rput{0}(15,20){\psellipse[fillcolor=userFillColour,fillstyle=solid](0,0)(3.79,-3.79)}
\psline[linewidth=0.75](0,35)(15,20)
\rput[r](12.5,0){$\AAh$}
\rput[r](67.5,0){$\AAh$}
\psline[linewidth=0.75](0,52.5)(0,35)
\psline[linewidth=0.75](30,52.5)(30,35)
\rput[l](32.5,51.25){$\AAh$}
\rput[l](2.5,51.25){$\AAh$}
\rput[l](77.5,50){$\delete$}
\rput[l](21.25,20){$\ccopy$}
\end{pspicture}


==> PIC/dataserv-op.tex <==
%%Created by jPicEdt 1.4.1_03: mixed JPIC-XML/LaTeX format
%%Tue Jan 05 06:10:11 GMT-10:00 2021
%%Begin JPIC-XML
%<?xml version="1.0" standalone="yes"?>
%<jpic x-min="2.5" x-max="82.5" y-min="0.93" y-max="46.25" auto-bounding="true">
%<multicurve fill-style= "none"
%	 points= "(75,46.25);(75,46.25);(75,5);(75,5)"
%	 stroke-width= "0.75"
%	 />
%<ellipse p3= "(79.07,0.93)"
%	 fill-style= "solid"
%	 p2= "(79.07,9.07)"
%	 p1= "(70.93,9.07)"
%	 closure= "open"
%	 angle-end= "0"
%	 stroke-width= "0.75"
%	 angle-start= "0"
%	 />
%<multicurve fill-style= "none"
%	 points= "(5,15);(5,15);(20,30);(20,30)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(20,30);(20,30);(20,46.25);(20,46.25)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(35,15);(35,15);(20,30);(20,30)"
%	 stroke-width= "0.75"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(22.5,46.25)"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\AAh$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(77.5,46.25)"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\AAh$
%</text>
%<multicurve fill-style= "none"
%	 points= "(35,2.5);(35,2.5);(35,15);(35,15)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(5,2.5);(5,2.5);(5,15);(5,15)"
%	 stroke-width= "0.75"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(2.5,3.75)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\AAh$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(32.5,3.75)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\AAh$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(82.5,3.75)"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\delete$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(27.5,30)"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\ccopy$
%</text>
%<ellipse p3= "(16.21,33.79)"
%	 fill-style= "solid"
%	 p2= "(16.21,26.21)"
%	 p1= "(23.79,26.21)"
%	 closure= "open"
%	 angle-end= "0"
%	 stroke-width= "0.75"
%	 angle-start= "0"
%	 />
%</jpic>
%%End JPIC-XML
%PSTricks content-type (pstricks.sty package needed)
%Add \usepackage{pstricks} in the preamble of your LaTeX file
%You can rescale the whole picture (to 80% for instance) by using the command \def\JPicScale{0.8}
\ifx\JPicScale\undefined\def\JPicScale{1}\fi
\psset{unit=\JPicScale mm}
\psset{linewidth=0.3,dotsep=1,hatchwidth=0.3,hatchsep=1.5,shadowsize=1,dimen=middle}
\psset{dotsize=0.7 2.5,dotscale=1 1,fillcolor=black}
\psset{arrowsize=1 2,arrowlength=1,arrowinset=0.25,tbarsize=0.7 5,bracketlength=0.15,rbracketlength=0.15}
\begin{pspicture}(0,0)(82.5,46.25)
\psline[linewidth=0.75](75,46.25)(75,5)
\rput{0}(75,5){\psellipse[linewidth=0.75,fillstyle=solid](0,0)(4.07,-4.07)}
\psline[linewidth=0.75](5,15)(20,30)
\psline[linewidth=0.75](20,30)(20,46.25)
\psline[linewidth=0.75](35,15)(20,30)
\rput[l](22.5,46.25){$\AAh$}
\rput[l](77.5,46.25){$\AAh$}
\psline[linewidth=0.75](35,2.5)(35,15)
\psline[linewidth=0.75](5,2.5)(5,15)
\rput[r](2.5,3.75){$\AAh$}
\rput[r](32.5,3.75){$\AAh$}
\rput[l](82.5,3.75){$\delete$}
\rput[l](27.5,30){$\ccopy$}
\rput{0}(20,30){\psellipse[linewidth=0.75,fillstyle=solid](0,0)(3.79,-3.79)}
\end{pspicture}


==> PIC/dataserv-white-strict.tex <==
%%Created by jPicEdt 1.4.1_03: mixed JPIC-XML/LaTeX format
%%Tue Jan 05 05:25:05 GMT-10:00 2021
%%Begin JPIC-XML
%<?xml version="1.0" standalone="yes"?>
%<jpic x-min="2.5" x-max="82.5" y-min="0.93" y-max="46.25" auto-bounding="true">
%<multicurve fill-style= "none"
%	 points= "(75,46.25);(75,46.25);(75,8.75);(75,8.75)"
%	 stroke-width= "0.75"
%	 />
%<ellipse p3= "(79.07,0.93)"
%	 fill-style= "solid"
%	 p2= "(79.07,9.07)"
%	 p1= "(70.93,9.07)"
%	 closure= "open"
%	 angle-end= "0"
%	 stroke-width= "0.75"
%	 angle-start= "0"
%	 />
%<multicurve fill-style= "none"
%	 points= "(5,15);(5,15);(20,30);(20,30)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(20,30);(20,30);(20,46.25);(20,46.25)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(35,15);(35,15);(20,30);(20,30)"
%	 stroke-width= "0.75"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(22.5,46.25)"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\AAh$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(77.5,46.25)"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\AAh$
%</text>
%<multicurve fill-style= "none"
%	 points= "(35,2.5);(35,2.5);(35,15);(35,15)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(5,2.5);(5,2.5);(5,15);(5,15)"
%	 stroke-width= "0.75"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(2.5,3.75)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\AAh$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(32.5,3.75)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\AAh$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(82.5,3.75)"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\delete$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(27.5,30)"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\ccopy$
%</text>
%<ellipse p3= "(16.21,33.79)"
%	 fill-style= "none"
%	 p2= "(16.21,26.21)"
%	 p1= "(23.79,26.21)"
%	 closure= "open"
%	 angle-end= "0"
%	 stroke-width= "0.75"
%	 angle-start= "0"
%	 />
%</jpic>
%%End JPIC-XML
%PSTricks content-type (pstricks.sty package needed)
%Add \usepackage{pstricks} in the preamble of your LaTeX file
%You can rescale the whole picture (to 80% for instance) by using the command \def\JPicScale{0.8}
\ifx\JPicScale\undefined\def\JPicScale{1}\fi
\psset{unit=\JPicScale mm}
\psset{linewidth=0.3,dotsep=1,hatchwidth=0.3,hatchsep=1.5,shadowsize=1,dimen=middle}
\psset{dotsize=0.7 2.5,dotscale=1 1,fillcolor=black}
\psset{arrowsize=1 2,arrowlength=1,arrowinset=0.25,tbarsize=0.7 5,bracketlength=0.15,rbracketlength=0.15}
\begin{pspicture}(0,0)(82.5,46.25)
\psline[linewidth=0.75](75,46.25)(75,8.75)
\rput{0}(75,5){\psellipse[linewidth=0.75,fillstyle=solid](0,0)(4.07,-4.07)}
\psline[linewidth=0.75](5,15)(20,30)
\psline[linewidth=0.75](20,30)(20,46.25)
\psline[linewidth=0.75](35,15)(20,30)
\rput[l](22.5,46.25){$\AAh$}
\rput[l](77.5,46.25){$\AAh$}
\psline[linewidth=0.75](35,2.5)(35,15)
\psline[linewidth=0.75](5,2.5)(5,15)
\rput[r](2.5,3.75){$\AAh$}
\rput[r](32.5,3.75){$\AAh$}
\rput[l](82.5,3.75){$\delete$}
\rput[l](27.5,30){$\ccopy$}
\rput{0}(20,30){\psellipse[linewidth=0.75](0,0)(3.79,-3.79)}
\end{pspicture}


==> PIC/dataserv-white.tex <==
%%Created by jPicEdt 1.4.1_03: mixed JPIC-XML/LaTeX format
%%Sat Dec 12 09:57:54 GMT-10:00 2020
%%Begin JPIC-XML
%<?xml version="1.0" standalone="yes"?>
%<jpic x-min="2.5" x-max="82.5" y-min="0.93" y-max="46.25" auto-bounding="true">
%<multicurve fill-style= "none"
%	 points= "(75,46.25);(75,46.25);(75,5);(75,5)"
%	 stroke-width= "0.75"
%	 />
%<ellipse p3= "(79.07,0.93)"
%	 fill-style= "solid"
%	 p2= "(79.07,9.07)"
%	 fill-color= "#ffffff"
%	 p1= "(70.93,9.07)"
%	 closure= "open"
%	 angle-end= "0"
%	 angle-start= "0"
%	 />
%<multicurve fill-style= "none"
%	 points= "(5,15);(5,15);(20,30);(20,30)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(20,30);(20,30);(20,46.25);(20,46.25)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(35,15);(35,15);(20,30);(20,30)"
%	 stroke-width= "0.75"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(22.5,46.25)"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\AAh$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(77.5,46.25)"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\AAh$
%</text>
%<multicurve fill-style= "none"
%	 points= "(35,2.5);(35,2.5);(35,15);(35,15)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(5,2.5);(5,2.5);(5,15);(5,15)"
%	 stroke-width= "0.75"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(2.5,3.75)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\AAh$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(32.5,3.75)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\AAh$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(82.5,3.75)"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\delete$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(27.5,30)"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\ccopy$
%</text>
%<ellipse p3= "(16.21,33.79)"
%	 fill-style= "solid"
%	 p2= "(16.21,26.21)"
%	 fill-color= "#ffffff"
%	 p1= "(23.79,26.21)"
%	 closure= "open"
%	 angle-end= "0"
%	 angle-start= "0"
%	 />
%</jpic>
%%End JPIC-XML
%PSTricks content-type (pstricks.sty package needed)
%Add \usepackage{pstricks} in the preamble of your LaTeX file
%You can rescale the whole picture (to 80% for instance) by using the command \def\JPicScale{0.8}
\ifx\JPicScale\undefined\def\JPicScale{1}\fi
\psset{unit=\JPicScale mm}
\psset{linewidth=0.3,dotsep=1,hatchwidth=0.3,hatchsep=1.5,shadowsize=1,dimen=middle}
\psset{dotsize=0.7 2.5,dotscale=1 1,fillcolor=black}
\psset{arrowsize=1 2,arrowlength=1,arrowinset=0.25,tbarsize=0.7 5,bracketlength=0.15,rbracketlength=0.15}
\begin{pspicture}(0,0)(82.5,46.25)
\psline[linewidth=0.75](75,46.25)(75,5)
\rput{0}(75,5){\psellipse[fillcolor=white,fillstyle=solid](0,0)(4.07,-4.07)}
\psline[linewidth=0.75](5,15)(20,30)
\psline[linewidth=0.75](20,30)(20,46.25)
\psline[linewidth=0.75](35,15)(20,30)
\rput[l](22.5,46.25){$\AAh$}
\rput[l](77.5,46.25){$\AAh$}
\psline[linewidth=0.75](35,2.5)(35,15)
\psline[linewidth=0.75](5,2.5)(5,15)
\rput[r](2.5,3.75){$\AAh$}
\rput[r](32.5,3.75){$\AAh$}
\rput[l](82.5,3.75){$\delete$}
\rput[l](27.5,30){$\ccopy$}
\rput{0}(20,30){\psellipse[fillcolor=white,fillstyle=solid](0,0)(3.79,-3.79)}
\end{pspicture}


==> PIC/dataserv.tex <==
%%Created by jPicEdt 1.4.1_03: mixed JPIC-XML/LaTeX format
%%Sat Nov 02 19:30:15 GMT-10:00 2019
%%Begin JPIC-XML
%<?xml version="1.0" standalone="yes"?>
%<jpic x-min="0" x-max="77.5" y-min="0" y-max="54.07" auto-bounding="true">
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(70,50);(70,50);(70,0);(70,0)"
%	 />
%<ellipse fill-style= "solid"
%	 p3= "(74.07,45.93)"
%	 p2= "(74.07,54.07)"
%	 p1= "(65.93,54.07)"
%	 fill-color= "#330033"
%	 closure= "open"
%	 angle-end= "0"
%	 angle-start= "0"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(30,35);(30,35);(15,20);(15,20)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(15,20);(15,20);(15,0);(15,0)"
%	 />
%<ellipse fill-style= "solid"
%	 p3= "(18.79,16.21)"
%	 p2= "(18.79,23.79)"
%	 p1= "(11.21,23.79)"
%	 fill-color= "#330033"
%	 closure= "open"
%	 angle-end= "0"
%	 angle-start= "0"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(0,35);(0,35);(15,20);(15,20)"
%	 />
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(12.5,0)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\AAh$
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(67.5,0)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\AAh$
%</text>
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(0,52.5);(0,52.5);(0,35);(0,35)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(30,52.5);(30,52.5);(30,35);(30,35)"
%	 />
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(32.5,51.25)"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\AAh$
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(2.5,51.25)"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\AAh$
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(77.5,50)"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\delete$
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(21.25,20)"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\ccopy$
%</text>
%</jpic>
%%End JPIC-XML
%PSTricks content-type (pstricks.sty package needed)
%Add \usepackage{pstricks} in the preamble of your LaTeX file
%You can rescale the whole picture (to 80% for instance) by using the command \def\JPicScale{0.8}
\ifx\JPicScale\undefined\def\JPicScale{1}\fi
\psset{unit=\JPicScale mm}
\psset{linewidth=0.3,dotsep=1,hatchwidth=0.3,hatchsep=1.5,shadowsize=1,dimen=middle}
\psset{dotsize=0.7 2.5,dotscale=1 1,fillcolor=black}
\psset{arrowsize=1 2,arrowlength=1,arrowinset=0.25,tbarsize=0.7 5,bracketlength=0.15,rbracketlength=0.15}
\begin{pspicture}(0,0)(77.5,54.07)
\psline[linewidth=0.75](70,50)(70,0)
\newrgbcolor{userFillColour}{0.2 0 0.2}
\rput{0}(70,50){\psellipse[fillcolor=userFillColour,fillstyle=solid](0,0)(4.07,-4.07)}
\psline[linewidth=0.75](30,35)(15,20)
\psline[linewidth=0.75](15,20)(15,0)
\newrgbcolor{userFillColour}{0.2 0 0.2}
\rput{0}(15,20){\psellipse[fillcolor=userFillColour,fillstyle=solid](0,0)(3.79,-3.79)}
\psline[linewidth=0.75](0,35)(15,20)
\rput[r](12.5,0){$\AAh$}
\rput[r](67.5,0){$\AAh$}
\psline[linewidth=0.75](0,52.5)(0,35)
\psline[linewidth=0.75](30,52.5)(30,35)
\rput[l](32.5,51.25){$\AAh$}
\rput[l](2.5,51.25){$\AAh$}
\rput[l](77.5,50){$\delete$}
\rput[l](21.25,20){$\ccopy$}
\end{pspicture}


==> PIC/decider-1.tex <==
%%Created by jPicEdt 1.4.1_03: mixed JPIC-XML/LaTeX format
%%Sun Jan 21 10:10:25 HST 2018
%%Begin JPIC-XML
%<?xml version="1.0" standalone="yes"?>
%<jpic x-min="0" x-max="220" y-min="-5" y-max="100" auto-bounding="true">
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(80,45);(80,45);(140,45);(140,45)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(140,20);(140,20);(140,45);(140,45)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(120,65);(120,65);(120,45);(120,45)"
%	 />
%<text stroke-width= "0.75"
%	 text-vert-align= "center-v"
%	 anchor-point= "(120,70)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\nameslang$
%</text>
%<text stroke-width= "0.75"
%	 text-vert-align= "center-v"
%	 anchor-point= "(120,-5)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\inputt$
%</text>
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(105,20);(105,20);(140,20);(140,20)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(120,20);(120,20);(120,0);(120,0)"
%	 />
%<text stroke-width= "0.75"
%	 text-vert-align= "center-v"
%	 anchor-point= "(118.12,31.88)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\universal
%</text>
%<text stroke-width= "0.75"
%	 text-vert-align= "center-v"
%	 anchor-point= "(65,30)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\EQLS
%</text>
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(92.5,32.5);(92.5,32.5);(92.5,5);(92.5,5)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(80,45);(80,45);(105,20);(105,20)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(0,45);(0,45);(50,45);(50,45)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(50,20);(50,20);(50,45);(50,45)"
%	 />
%<text stroke-width= "0.75"
%	 text-vert-align= "center-v"
%	 anchor-point= "(40,-5)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\inputt$
%</text>
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(0,20);(0,20);(50,20);(50,20)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(40,20);(40,20);(40,0);(40,0)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(10,20);(10,20);(10,5);(10,5)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(0,45);(0,45);(0,20);(0,20)"
%	 />
%<text text-vert-align= "center-v"
%	 anchor-point= "(25,31.88)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\gee$
%</text>
%<text stroke-width= "0.75"
%	 text-vert-align= "center-v"
%	 anchor-point= "(155,30)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\EQLS
%</text>
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(170,45);(170,45);(220,45);(220,45)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(220,20);(220,20);(220,45);(220,45)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(195,65);(195,65);(195,45);(195,45)"
%	 />
%<text stroke-width= "0.75"
%	 text-vert-align= "center-v"
%	 anchor-point= "(195,70)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\nameslang$
%</text>
%<text stroke-width= "0.75"
%	 text-vert-align= "center-v"
%	 anchor-point= "(210,-5)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\inputt$
%</text>
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(170,20);(170,20);(220,20);(220,20)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(210,20);(210,20);(210,0);(210,0)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(180,20);(180,20);(180,5);(180,5)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(170,45);(170,45);(170,20);(170,20)"
%	 />
%<text text-vert-align= "center-v"
%	 anchor-point= "(195,31.88)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\gee$
%</text>
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(25,60);(25,60);(25,45);(25,45)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(25,95);(25,95);(25,80);(25,80)"
%	 />
%<multicurve stroke-width= "0.6"
%	 fill-style= "none"
%	 points= "(15,80);(15,80);(35,80);(35,80)"
%	 />
%<multicurve stroke-width= "0.6"
%	 fill-style= "none"
%	 points= "(35,60);(35,60);(35,80);(35,80)"
%	 />
%<multicurve stroke-width= "0.6"
%	 fill-style= "none"
%	 points= "(15,60);(15,60);(35,60);(35,60)"
%	 />
%<multicurve stroke-width= "0.6"
%	 fill-style= "none"
%	 points= "(15,80);(15,80);(15,60);(15,60)"
%	 />
%<text text-vert-align= "center-v"
%	 anchor-point= "(25,70)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\nneg$
%</text>
%<text stroke-width= "0.75"
%	 text-vert-align= "center-v"
%	 anchor-point= "(25,100)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\nameslang$
%</text>
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(2.5,-5);(2.5,-5);(20,-5);(20,-5)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(2.5,-5);(2.5,-5);(2.5,12.5);(2.5,12.5)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(2.5,12.5);(2.5,12.5);(20,-5);(20,-5)"
%	 />
%<text text-vert-align= "center-v"
%	 anchor-point= "(7.5,0)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\zzero$
%</text>
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(85,-5);(85,-5);(102.5,-5);(102.5,-5)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(85,-5);(85,-5);(85,12.5);(85,12.5)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(85,12.5);(85,12.5);(102.5,-5);(102.5,-5)"
%	 />
%<text text-vert-align= "center-v"
%	 anchor-point= "(90,0)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\zzero$
%</text>
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(172.5,-5);(172.5,-5);(190,-5);(190,-5)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(172.5,-5);(172.5,-5);(172.5,12.5);(172.5,12.5)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(172.5,12.5);(172.5,12.5);(190,-5);(190,-5)"
%	 />
%<text text-vert-align= "center-v"
%	 anchor-point= "(177.5,0)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\zzero$
%</text>
%</jpic>
%%End JPIC-XML
%PSTricks content-type (pstricks.sty package needed)
%Add \usepackage{pstricks} in the preamble of your LaTeX file
%You can rescale the whole picture (to 80% for instance) by using the command \def\JPicScale{0.8}
\ifx\JPicScale\undefined\def\JPicScale{1}\fi
\psset{unit=\JPicScale mm}
\psset{linewidth=0.3,dotsep=1,hatchwidth=0.3,hatchsep=1.5,shadowsize=1,dimen=middle}
\psset{dotsize=0.7 2.5,dotscale=1 1,fillcolor=black}
\psset{arrowsize=1 2,arrowlength=1,arrowinset=0.25,tbarsize=0.7 5,bracketlength=0.15,rbracketlength=0.15}
\begin{pspicture}(0,0)(220,100)
\psline[linewidth=0.75](80,45)(140,45)
\psline[linewidth=0.75](140,20)(140,45)
\psline[linewidth=0.75](120,65)(120,45)
\rput(120,70){$\nameslang$}
\rput(120,-5){$\inputt$}
\psline[linewidth=0.75](105,20)(140,20)
\psline[linewidth=0.75](120,20)(120,0)
\rput(118.12,31.88){\universal}
\rput(65,30){\EQLS}
\psline[linewidth=0.75](92.5,32.5)(92.5,5)
\psline[linewidth=0.75](80,45)(105,20)
\psline[linewidth=0.75](0,45)(50,45)
\psline[linewidth=0.75](50,20)(50,45)
\rput(40,-5){$\inputt$}
\psline[linewidth=0.75](0,20)(50,20)
\psline[linewidth=0.75](40,20)(40,0)
\psline[linewidth=0.75](10,20)(10,5)
\psline[linewidth=0.75](0,45)(0,20)
\rput(25,31.88){$\gee$}
\rput(155,30){\EQLS}
\psline[linewidth=0.75](170,45)(220,45)
\psline[linewidth=0.75](220,20)(220,45)
\psline[linewidth=0.75](195,65)(195,45)
\rput(195,70){$\nameslang$}
\rput(210,-5){$\inputt$}
\psline[linewidth=0.75](170,20)(220,20)
\psline[linewidth=0.75](210,20)(210,0)
\psline[linewidth=0.75](180,20)(180,5)
\psline[linewidth=0.75](170,45)(170,20)
\rput(195,31.88){$\gee$}
\psline[linewidth=0.75](25,60)(25,45)
\psline[linewidth=0.75](25,95)(25,80)
\psline[linewidth=0.6](15,80)(35,80)
\psline[linewidth=0.6](35,60)(35,80)
\psline[linewidth=0.6](15,60)(35,60)
\psline[linewidth=0.6](15,80)(15,60)
\rput(25,70){$\nneg$}
\rput(25,100){$\nameslang$}
\psline[linewidth=0.75](2.5,-5)(20,-5)
\psline[linewidth=0.75](2.5,-5)(2.5,12.5)
\psline[linewidth=0.75](2.5,12.5)(20,-5)
\rput(7.5,0){$\zzero$}
\psline[linewidth=0.75](85,-5)(102.5,-5)
\psline[linewidth=0.75](85,-5)(85,12.5)
\psline[linewidth=0.75](85,12.5)(102.5,-5)
\rput(90,0){$\zzero$}
\psline[linewidth=0.75](172.5,-5)(190,-5)
\psline[linewidth=0.75](172.5,-5)(172.5,12.5)
\psline[linewidth=0.75](172.5,12.5)(190,-5)
\rput(177.5,0){$\zzero$}
\end{pspicture}


==> PIC/decider.tex <==
%%Created by jPicEdt 1.4.1_03: mixed JPIC-XML/LaTeX format
%%Sun Oct 30 12:15:07 HST 2016
%%Begin JPIC-XML
%<?xml version="1.0" standalone="yes"?>
%<jpic x-min="0" x-max="140" y-min="0" y-max="63.12" auto-bounding="true">
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(80,45);(80,45);(140,45);(140,45)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(140,20);(140,20);(140,45);(140,45)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(120,56.88);(120,56.88);(120,45);(120,45)"
%	 />
%<text stroke-width= "0.75"
%	 text-vert-align= "center-v"
%	 anchor-point= "(120,63.12)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\nameslang$
%</text>
%<text stroke-width= "0.75"
%	 text-vert-align= "center-v"
%	 anchor-point= "(120,0)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\inputt$
%</text>
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(105,20);(105,20);(140,20);(140,20)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(120,20);(120,20);(120,5);(120,5)"
%	 />
%<text stroke-width= "0.75"
%	 text-vert-align= "center-v"
%	 anchor-point= "(118.12,31.88)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\universal
%</text>
%<text stroke-width= "0.75"
%	 text-vert-align= "center-v"
%	 anchor-point= "(65,30)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\EQLS
%</text>
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(92.5,32.5);(92.5,32.5);(92.5,5);(92.5,5)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(80,45);(80,45);(105,20);(105,20)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(0,45);(0,45);(50,45);(50,45)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(50,20);(50,20);(50,45);(50,45)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(25,56.88);(25,56.88);(25,45);(25,45)"
%	 />
%<text stroke-width= "0.75"
%	 text-vert-align= "center-v"
%	 anchor-point= "(25,63.12)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\nameslang$
%</text>
%<text stroke-width= "0.75"
%	 text-vert-align= "center-v"
%	 anchor-point= "(40,0)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\inputt$
%</text>
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(0,20);(0,20);(50,20);(50,20)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(40,20);(40,20);(40,5);(40,5)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(10,20);(10,20);(10,5);(10,5)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(0,45);(0,45);(0,20);(0,20)"
%	 />
%<text text-vert-align= "center-v"
%	 anchor-point= "(25,31.88)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\gee$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(92.5,0)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\progtype$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(10,0)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\progtype$
%</text>
%</jpic>
%%End JPIC-XML
%PSTricks content-type (pstricks.sty package needed)
%Add \usepackage{pstricks} in the preamble of your LaTeX file
%You can rescale the whole picture (to 80% for instance) by using the command \def\JPicScale{0.8}
\ifx\JPicScale\undefined\def\JPicScale{1}\fi
\psset{unit=\JPicScale mm}
\psset{linewidth=0.3,dotsep=1,hatchwidth=0.3,hatchsep=1.5,shadowsize=1,dimen=middle}
\psset{dotsize=0.7 2.5,dotscale=1 1,fillcolor=black}
\psset{arrowsize=1 2,arrowlength=1,arrowinset=0.25,tbarsize=0.7 5,bracketlength=0.15,rbracketlength=0.15}
\begin{pspicture}(0,0)(140,63.12)
\psline[linewidth=0.75](80,45)(140,45)
\psline[linewidth=0.75](140,20)(140,45)
\psline[linewidth=0.75](120,56.88)(120,45)
\rput(120,63.12){$\nameslang$}
\rput(120,0){$\inputt$}
\psline[linewidth=0.75](105,20)(140,20)
\psline[linewidth=0.75](120,20)(120,5)
\rput(118.12,31.88){\universal}
\rput(65,30){\EQLS}
\psline[linewidth=0.75](92.5,32.5)(92.5,5)
\psline[linewidth=0.75](80,45)(105,20)
\psline[linewidth=0.75](0,45)(50,45)
\psline[linewidth=0.75](50,20)(50,45)
\psline[linewidth=0.75](25,56.88)(25,45)
\rput(25,63.12){$\nameslang$}
\rput(40,0){$\inputt$}
\psline[linewidth=0.75](0,20)(50,20)
\psline[linewidth=0.75](40,20)(40,5)
\psline[linewidth=0.75](10,20)(10,5)
\psline[linewidth=0.75](0,45)(0,20)
\rput(25,31.88){$\gee$}
\rput(92.5,0){$\progtype$}
\rput(10,0){$\progtype$}
\end{pspicture}


==> PIC/delete.tex <==
%%Created by jPicEdt 1.4.1_03: mixed JPIC-XML/LaTeX format
%%Wed Sep 28 20:13:51 HST 2016
%%Begin JPIC-XML
%<?xml version="1.0" standalone="yes"?>
%<jpic x-min="16.88" x-max="21.41" y-min="7.5" y-max="40.16" auto-bounding="true">
%<text stroke-width= "0.75"
%	 text-vert-align= "center-v"
%	 anchor-point= "(16.88,9.38)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\inputt$
%</text>
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(20,37.5);(20,37.5);(20,7.5);(20,7.5)"
%	 />
%<ellipse p3= "(21.41,37.34)"
%	 p2= "(21.41,40.16)"
%	 p1= "(18.59,40.16)"
%	 closure= "open"
%	 fill-style= "solid"
%	 angle-end= "360"
%	 fill-color= "#330033"
%	 angle-start= "0"
%	 />
%</jpic>
%%End JPIC-XML
%PSTricks content-type (pstricks.sty package needed)
%Add \usepackage{pstricks} in the preamble of your LaTeX file
%You can rescale the whole picture (to 80% for instance) by using the command \def\JPicScale{0.8}
\ifx\JPicScale\undefined\def\JPicScale{1}\fi
\psset{unit=\JPicScale mm}
\psset{linewidth=0.3,dotsep=1,hatchwidth=0.3,hatchsep=1.5,shadowsize=1,dimen=middle}
\psset{dotsize=0.7 2.5,dotscale=1 1,fillcolor=black}
\psset{arrowsize=1 2,arrowlength=1,arrowinset=0.25,tbarsize=0.7 5,bracketlength=0.15,rbracketlength=0.15}
\begin{pspicture}(0,0)(21.41,40.16)
\rput[r](16.88,9.38){$\inputt$}
\psline[linewidth=0.75](20,37.5)(20,7.5)
\newrgbcolor{userFillColour}{0.2 0 0.2}
\rput{0}(20,38.75){\psellipse[fillcolor=userFillColour,fillstyle=solid](0,0)(1.41,-1.41)}
\end{pspicture}


==> PIC/eqserv-1.tex <==
%%Created by jPicEdt 1.4.1_03: mixed JPIC-XML/LaTeX format
%%Sun Jun 06 16:13:38 GMT-10:00 2021
%%Begin JPIC-XML
%<?xml version="1.0" standalone="yes"?>
%<jpic x-min="0" x-max="65" y-min="0" y-max="100" auto-bounding="true">
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(20,55)"
%	 text-frame= "noframe"
%	 stroke-width= "0.35"
%	 text-hor-align= "center-h"
%	 >
%\DOTT
%</text>
%<multicurve fill-style= "none"
%	 points= "(20,55);(20,55);(0,35);(0,35)"
%	 stroke-width= "0.45"
%	 />
%<multicurve fill-style= "none"
%	 points= "(0,35);(0,35);(0,0);(0,0)"
%	 stroke-width= "0.45"
%	 />
%<multicurve fill-style= "none"
%	 points= "(40,35);(40,35);(20,55);(20,55)"
%	 stroke-width= "0.45"
%	 />
%<multicurve fill-style= "none"
%	 points= "(40,35);(40,35);(40,0);(40,0)"
%	 stroke-width= "0.45"
%	 />
%<multicurve fill-style= "none"
%	 points= "(20,100);(20,100);(20,55);(20,55)"
%	 stroke-width= "0.45"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(65,55)"
%	 stroke-color= "#ff0033"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\EQLS
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(30,60)"
%	 stroke-color= "#ff0033"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\compsn$
%</text>
%</jpic>
%%End JPIC-XML
%LaTeX-picture environment using emulated lines and arcs
%You can rescale the whole picture (to 80% for instance) by using the command \def\JPicScale{0.8}
\ifx\JPicScale\undefined\def\JPicScale{1}\fi
\unitlength \JPicScale mm
\begin{picture}(65,100)(0,0)
\put(20,55){\makebox(0,0)[cc]{\DOTT}}

\linethickness{0.45mm}
\multiput(0,35)(0.12,0.12){167}{\line(1,0){0.12}}
\linethickness{0.45mm}
\put(0,0){\line(0,1){35}}
\linethickness{0.45mm}
\multiput(20,55)(0.12,-0.12){167}{\line(1,0){0.12}}
\linethickness{0.45mm}
\put(40,0){\line(0,1){35}}
\linethickness{0.45mm}
\put(20,55){\line(0,1){45}}
\put(65,55){\makebox(0,0)[cc]{\EQLS}}

\put(30,60){\makebox(0,0)[cc]{$\compsn$}}

\end{picture}


==> PIC/eqserv.tex <==
%%Created by jPicEdt 1.4.1_03: mixed JPIC-XML/LaTeX format
%%Sun Jun 06 16:13:38 GMT-10:00 2021
%%Begin JPIC-XML
%<?xml version="1.0" standalone="yes"?>
%<jpic x-min="0" x-max="190" y-min="0" y-max="100" auto-bounding="true">
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(20,55)"
%	 text-frame= "noframe"
%	 stroke-width= "0.35"
%	 text-hor-align= "center-h"
%	 >
%\DOTT
%</text>
%<multicurve fill-style= "none"
%	 points= "(150,65);(150,65);(150,30);(150,30)"
%	 stroke-width= "0.45"
%	 />
%<multicurve fill-style= "none"
%	 points= "(115,75);(115,75);(115,55);(115,55)"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(105,35);(105,35);(125,35);(125,35)"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(105,35);(105,35);(105,55);(105,55)"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(105,55);(105,55);(125,55);(125,55)"
%	 stroke-width= "0.35"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(115,55)"
%	 text-frame= "noframe"
%	 stroke-width= "0.35"
%	 text-hor-align= "center-h"
%	 >
%\DOTT
%</text>
%<multicurve fill-style= "none"
%	 points= "(125,35);(125,35);(125,55);(125,55)"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(110,35);(110,35);(110,30);(110,30)"
%	 stroke-width= "0.45"
%	 />
%<multicurve fill-style= "none"
%	 points= "(120,35);(120,35);(120,30);(120,30)"
%	 stroke-width= "0.45"
%	 />
%<multicurve fill-style= "none"
%	 points= "(135,15);(135,15);(120,30);(120,30)"
%	 stroke-width= "0.45"
%	 />
%<multicurve fill-style= "none"
%	 points= "(110,30);(110,30);(95,15);(95,15)"
%	 stroke-width= "0.45"
%	 />
%<multicurve fill-style= "none"
%	 points= "(135,15);(135,15);(135,0);(135,0)"
%	 stroke-width= "0.45"
%	 />
%<multicurve fill-style= "none"
%	 points= "(125,65);(125,65);(185,65);(185,65)"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(105,85);(105,85);(185,85);(185,85)"
%	 stroke-width= "0.35"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(113.75,65)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\Baut$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(115,45)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\isequal$
%</text>
%<multicurve fill-style= "none"
%	 points= "(20,55);(20,55);(0,35);(0,35)"
%	 stroke-width= "0.45"
%	 />
%<multicurve fill-style= "none"
%	 points= "(0,35);(0,35);(0,0);(0,0)"
%	 stroke-width= "0.45"
%	 />
%<multicurve fill-style= "none"
%	 points= "(40,35);(40,35);(20,55);(20,55)"
%	 stroke-width= "0.45"
%	 />
%<multicurve fill-style= "none"
%	 points= "(40,35);(40,35);(40,0);(40,0)"
%	 stroke-width= "0.45"
%	 />
%<multicurve fill-style= "none"
%	 points= "(20,100);(20,100);(20,55);(20,55)"
%	 stroke-width= "0.45"
%	 />
%<multicurve fill-style= "none"
%	 points= "(95,15);(95,15);(95,0);(95,0)"
%	 stroke-width= "0.45"
%	 />
%<multicurve fill-style= "none"
%	 points= "(150,30);(150,30);(135,15);(135,15)"
%	 stroke-width= "0.45"
%	 />
%<multicurve fill-style= "none"
%	 points= "(105,85);(105,85);(125,65);(125,65)"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(150,100);(150,100);(150,85);(150,85)"
%	 stroke-width= "0.45"
%	 />
%<multicurve fill-style= "none"
%	 points= "(185,65);(185,65);(185,85);(185,85)"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(175,40);(175,40);(165,50);(165,50)"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(165,50);(165,50);(185,50);(185,50)"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(175,40);(175,40);(185,50);(185,50)"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(175,65);(175,65);(175,50);(175,50)"
%	 stroke-width= "0.45"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(175.62,45.62)"
%	 stroke-color= "#ff0033"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\divg$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(135,15)"
%	 text-frame= "noframe"
%	 stroke-width= "0.35"
%	 text-hor-align= "center-h"
%	 >
%\DOTT
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(65,55)"
%	 stroke-color= "#ff0033"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\EQLS
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(150,75)"
%	 stroke-color= "#ff0033"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\iiif$
%</text>
%<multicurve fill-style= "none"
%	 points= "(90,90);(90,90);(190,90);(190,90)"
%	 stroke-width= "0.2"
%	 />
%<multicurve fill-style= "none"
%	 points= "(90,10);(90,10);(190,10);(190,10)"
%	 stroke-width= "0.2"
%	 />
%<multicurve fill-style= "none"
%	 points= "(90,90);(90,90);(90,10);(90,10)"
%	 stroke-width= "0.2"
%	 />
%<multicurve fill-style= "none"
%	 points= "(190,90);(190,90);(190,10);(190,10)"
%	 stroke-width= "0.2"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(30,60)"
%	 stroke-color= "#ff0033"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\compsn$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(180,17.5)"
%	 stroke-color= "#ff0033"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\compsn$
%</text>
%</jpic>
%%End JPIC-XML
%LaTeX-picture environment using emulated lines and arcs
%You can rescale the whole picture (to 80% for instance) by using the command \def\JPicScale{0.8}
\ifx\JPicScale\undefined\def\JPicScale{1}\fi
\unitlength \JPicScale mm
\begin{picture}(190,100)(0,0)
\put(20,55){\makebox(0,0)[cc]{\DOTT}}

\linethickness{0.45mm}
\put(150,30){\line(0,1){35}}
\linethickness{0.35mm}
\put(115,55){\line(0,1){20}}
\linethickness{0.35mm}
\put(105,35){\line(1,0){20}}
\linethickness{0.35mm}
\put(105,35){\line(0,1){20}}
\linethickness{0.35mm}
\put(105,55){\line(1,0){20}}
\put(115,55){\makebox(0,0)[cc]{\DOTT}}

\linethickness{0.35mm}
\put(125,35){\line(0,1){20}}
\linethickness{0.45mm}
\put(110,30){\line(0,1){5}}
\linethickness{0.45mm}
\put(120,30){\line(0,1){5}}
\linethickness{0.45mm}
\multiput(120,30)(0.12,-0.12){125}{\line(1,0){0.12}}
\linethickness{0.45mm}
\multiput(95,15)(0.12,0.12){125}{\line(1,0){0.12}}
\linethickness{0.45mm}
\put(135,0){\line(0,1){15}}
\linethickness{0.35mm}
\put(125,65){\line(1,0){60}}
\linethickness{0.35mm}
\put(105,85){\line(1,0){80}}
\put(113.75,65){\makebox(0,0)[cr]{$\Baut$}}

\put(115,45){\makebox(0,0)[cc]{$\isequal$}}

\linethickness{0.45mm}
\multiput(0,35)(0.12,0.12){167}{\line(1,0){0.12}}
\linethickness{0.45mm}
\put(0,0){\line(0,1){35}}
\linethickness{0.45mm}
\multiput(20,55)(0.12,-0.12){167}{\line(1,0){0.12}}
\linethickness{0.45mm}
\put(40,0){\line(0,1){35}}
\linethickness{0.45mm}
\put(20,55){\line(0,1){45}}
\linethickness{0.45mm}
\put(95,0){\line(0,1){15}}
\linethickness{0.45mm}
\multiput(135,15)(0.12,0.12){125}{\line(1,0){0.12}}
\linethickness{0.35mm}
\multiput(105,85)(0.12,-0.12){167}{\line(1,0){0.12}}
\linethickness{0.45mm}
\put(150,85){\line(0,1){15}}
\linethickness{0.35mm}
\put(185,65){\line(0,1){20}}
\linethickness{0.35mm}
\multiput(165,50)(0.12,-0.12){83}{\line(1,0){0.12}}
\linethickness{0.35mm}
\put(165,50){\line(1,0){20}}
\linethickness{0.35mm}
\multiput(175,40)(0.12,0.12){83}{\line(1,0){0.12}}
\linethickness{0.45mm}
\put(175,50){\line(0,1){15}}
\put(175.62,45.62){\makebox(0,0)[cc]{$\divg$}}

\put(135,15){\makebox(0,0)[cc]{\DOTT}}

\put(65,55){\makebox(0,0)[cc]{\EQLS}}

\put(150,75){\makebox(0,0)[cc]{$\iiif$}}

\linethickness{0.2mm}
\put(90,90){\line(1,0){100}}
\linethickness{0.2mm}
\put(90,10){\line(1,0){100}}
\linethickness{0.2mm}
\put(90,10){\line(0,1){80}}
\linethickness{0.2mm}
\put(190,10){\line(0,1){80}}
\put(30,60){\makebox(0,0)[cc]{$\compsn$}}

\put(180,17.5){\makebox(0,0)[cc]{$\compsn$}}

\end{picture}


==> PIC/equal.tex <==
%%Created by jPicEdt 1.4.1_03: mixed JPIC-XML/LaTeX format
%%Sun Jun 06 15:21:04 GMT-10:00 2021
%%Begin JPIC-XML
%<?xml version="1.0" standalone="yes"?>
%<jpic x-min="0" x-max="80" y-min="0" y-max="155" auto-bounding="true">
%<multicurve fill-style= "none"
%	 points= "(15,100);(15,100);(15,95);(15,95)"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(5,80);(5,80);(25,80);(25,80)"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(5,80);(5,80);(5,95);(5,95)"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(5,95);(5,95);(25,95);(25,95)"
%	 stroke-width= "0.35"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(15,95)"
%	 text-frame= "noframe"
%	 stroke-width= "0.35"
%	 text-hor-align= "center-h"
%	 >
%\DOTT
%</text>
%<multicurve fill-style= "none"
%	 points= "(25,80);(25,80);(25,95);(25,95)"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(10,80);(10,80);(10,75);(10,75)"
%	 stroke-width= "0.65"
%	 />
%<multicurve fill-style= "none"
%	 points= "(20,80);(20,80);(20,75);(20,75)"
%	 stroke-width= "0.65"
%	 />
%<multicurve fill-style= "none"
%	 points= "(20,75);(20,75);(70,25);(70,25)"
%	 stroke-width= "0.65"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(15,87.5)"
%	 text-frame= "noframe"
%	 stroke-width= "0.35"
%	 text-hor-align= "center-h"
%	 >
%$\smaller$
%</text>
%<multicurve fill-style= "none"
%	 points= "(10,75);(10,75);(40,45);(40,45)"
%	 stroke-width= "0.65"
%	 />
%<multicurve fill-style= "none"
%	 points= "(65,100);(65,100);(65,95);(65,95)"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(55,80);(55,80);(75,80);(75,80)"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(55,80);(55,80);(55,95);(55,95)"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(55,95);(55,95);(75,95);(75,95)"
%	 stroke-width= "0.35"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(65,95)"
%	 text-frame= "noframe"
%	 stroke-width= "0.35"
%	 text-hor-align= "center-h"
%	 >
%\DOTT
%</text>
%<multicurve fill-style= "none"
%	 points= "(75,80);(75,80);(75,95);(75,95)"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(60,80);(60,80);(60,75);(60,75)"
%	 stroke-width= "0.65"
%	 />
%<multicurve fill-style= "none"
%	 points= "(70,80);(70,80);(70,75);(70,75)"
%	 stroke-width= "0.65"
%	 />
%<multicurve fill-style= "none"
%	 points= "(70,75);(70,75);(15,20);(15,20)"
%	 stroke-width= "0.65"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(65,87.5)"
%	 text-frame= "noframe"
%	 stroke-width= "0.35"
%	 text-hor-align= "center-h"
%	 >
%$\smaller$
%</text>
%<multicurve fill-style= "none"
%	 points= "(60,75);(60,75);(40,55);(40,55)"
%	 stroke-width= "0.65"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(40,55)"
%	 text-frame= "noframe"
%	 stroke-width= "0.65"
%	 text-hor-align= "center-h"
%	 >
%\DOTT
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(40,45)"
%	 text-frame= "noframe"
%	 stroke-width= "0.65"
%	 text-hor-align= "center-h"
%	 >
%\DOTT
%</text>
%<multicurve fill-style= "none"
%	 points= "(70,25);(70,25);(70,5);(70,5)"
%	 stroke-width= "0.65"
%	 />
%<multicurve fill-style= "none"
%	 points= "(15,20);(15,20);(15,5);(15,5)"
%	 stroke-width= "0.65"
%	 />
%<multicurve fill-style= "none"
%	 points= "(40,155);(40,155);(40,140);(40,140)"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(30,125);(30,125);(50,125);(50,125)"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(30,125);(30,125);(30,140);(30,140)"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(30,140);(30,140);(50,140);(50,140)"
%	 stroke-width= "0.35"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(40,140)"
%	 text-frame= "noframe"
%	 stroke-width= "0.35"
%	 text-hor-align= "center-h"
%	 >
%\DOTT
%</text>
%<multicurve fill-style= "none"
%	 points= "(50,125);(50,125);(50,140);(50,140)"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(35,125);(35,125);(35,120);(35,120)"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(45,125);(45,125);(45,120);(45,120)"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(45,120);(45,120);(65,100);(65,100)"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(35,120);(35,120);(15,100);(15,100)"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(80,145);(80,145);(80,15);(80,15)"
%	 stroke-width= "0.2"
%	 />
%<multicurve fill-style= "none"
%	 points= "(0,145);(0,145);(0,15);(0,15)"
%	 stroke-width= "0.2"
%	 />
%<multicurve fill-style= "none"
%	 points= "(80,145);(80,145);(0,145);(0,145)"
%	 stroke-width= "0.2"
%	 />
%<multicurve fill-style= "none"
%	 points= "(80,15);(80,15);(0,15);(0,15)"
%	 stroke-width= "0.2"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(40,132.5)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\hand$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(42.5,155)"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\Baut$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(15,0)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\heex$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(70,0)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\hwaai$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(10,35)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\isequal$
%</text>
%</jpic>
%%End JPIC-XML
%LaTeX-picture environment using emulated lines and arcs
%You can rescale the whole picture (to 80% for instance) by using the command \def\JPicScale{0.8}
\ifx\JPicScale\undefined\def\JPicScale{1}\fi
\unitlength \JPicScale mm
\begin{picture}(80,155)(0,0)
\linethickness{0.35mm}
\put(15,95){\line(0,1){5}}
\linethickness{0.35mm}
\put(5,80){\line(1,0){20}}
\linethickness{0.35mm}
\put(5,80){\line(0,1){15}}
\linethickness{0.35mm}
\put(5,95){\line(1,0){20}}
\put(15,95){\makebox(0,0)[cc]{\DOTT}}

\linethickness{0.35mm}
\put(25,80){\line(0,1){15}}
\linethickness{0.65mm}
\put(10,75){\line(0,1){5}}
\linethickness{0.65mm}
\put(20,75){\line(0,1){5}}
\linethickness{0.65mm}
\multiput(20,75)(0.12,-0.12){417}{\line(1,0){0.12}}
\put(15,87.5){\makebox(0,0)[cc]{$\smaller$}}

\linethickness{0.65mm}
\multiput(10,75)(0.12,-0.12){250}{\line(1,0){0.12}}
\linethickness{0.35mm}
\put(65,95){\line(0,1){5}}
\linethickness{0.35mm}
\put(55,80){\line(1,0){20}}
\linethickness{0.35mm}
\put(55,80){\line(0,1){15}}
\linethickness{0.35mm}
\put(55,95){\line(1,0){20}}
\put(65,95){\makebox(0,0)[cc]{\DOTT}}

\linethickness{0.35mm}
\put(75,80){\line(0,1){15}}
\linethickness{0.65mm}
\put(60,75){\line(0,1){5}}
\linethickness{0.65mm}
\put(70,75){\line(0,1){5}}
\linethickness{0.65mm}
\multiput(15,20)(0.12,0.12){458}{\line(1,0){0.12}}
\put(65,87.5){\makebox(0,0)[cc]{$\smaller$}}

\linethickness{0.65mm}
\multiput(40,55)(0.12,0.12){167}{\line(1,0){0.12}}
\put(40,55){\makebox(0,0)[cc]{\DOTT}}

\put(40,45){\makebox(0,0)[cc]{\DOTT}}

\linethickness{0.65mm}
\put(70,5){\line(0,1){20}}
\linethickness{0.65mm}
\put(15,5){\line(0,1){15}}
\linethickness{0.35mm}
\put(40,140){\line(0,1){15}}
\linethickness{0.35mm}
\put(30,125){\line(1,0){20}}
\linethickness{0.35mm}
\put(30,125){\line(0,1){15}}
\linethickness{0.35mm}
\put(30,140){\line(1,0){20}}
\put(40,140){\makebox(0,0)[cc]{\DOTT}}

\linethickness{0.35mm}
\put(50,125){\line(0,1){15}}
\linethickness{0.35mm}
\put(35,120){\line(0,1){5}}
\linethickness{0.35mm}
\put(45,120){\line(0,1){5}}
\linethickness{0.35mm}
\multiput(45,120)(0.12,-0.12){167}{\line(1,0){0.12}}
\linethickness{0.35mm}
\multiput(15,100)(0.12,0.12){167}{\line(1,0){0.12}}
\linethickness{0.2mm}
\put(80,15){\line(0,1){130}}
\linethickness{0.2mm}
\put(0,15){\line(0,1){130}}
\linethickness{0.2mm}
\put(0,145){\line(1,0){80}}
\linethickness{0.2mm}
\put(0,15){\line(1,0){80}}
\put(40,132.5){\makebox(0,0)[cc]{$\hand$}}

\put(42.5,155){\makebox(0,0)[cl]{$\Baut$}}

\put(15,0){\makebox(0,0)[cc]{$\heex$}}

\put(70,0){\makebox(0,0)[cc]{$\hwaai$}}

\put(10,35){\makebox(0,0)[cc]{$\isequal$}}

\end{picture}


==> PIC/equality.tex <==
%%Created by jPicEdt 1.4.1_03: mixed JPIC-XML/LaTeX format
%%Mon Dec 14 09:59:47 GMT-10:00 2020
%%Begin JPIC-XML
%<?xml version="1.0" standalone="yes"?>
%<jpic x-min="2.5" x-max="35" y-min="2.5" y-max="46.25" auto-bounding="true">
%<multicurve fill-style= "none"
%	 points= "(5,15);(5,15);(20,30);(20,30)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(20,30);(20,30);(20,46.25);(20,46.25)"
%	 stroke-width= "0.75"
%	 />
%<ellipse p3= "(16.21,33.79)"
%	 fill-style= "solid"
%	 p2= "(16.21,26.21)"
%	 fill-color= "#330033"
%	 p1= "(23.79,26.21)"
%	 closure= "open"
%	 angle-end= "0"
%	 angle-start= "0"
%	 />
%<multicurve fill-style= "none"
%	 points= "(35,15);(35,15);(20,30);(20,30)"
%	 stroke-width= "0.75"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(22.5,46.25)"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\AAh$
%</text>
%<multicurve fill-style= "none"
%	 points= "(35,2.5);(35,2.5);(35,15);(35,15)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(5,2.5);(5,2.5);(5,15);(5,15)"
%	 stroke-width= "0.75"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(2.5,3.75)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\AAh$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(32.5,3.75)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\AAh$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(27.5,30)"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\ccopy$
%</text>
%</jpic>
%%End JPIC-XML
%PSTricks content-type (pstricks.sty package needed)
%Add \usepackage{pstricks} in the preamble of your LaTeX file
%You can rescale the whole picture (to 80% for instance) by using the command \def\JPicScale{0.8}
\ifx\JPicScale\undefined\def\JPicScale{1}\fi
\psset{unit=\JPicScale mm}
\psset{linewidth=0.3,dotsep=1,hatchwidth=0.3,hatchsep=1.5,shadowsize=1,dimen=middle}
\psset{dotsize=0.7 2.5,dotscale=1 1,fillcolor=black}
\psset{arrowsize=1 2,arrowlength=1,arrowinset=0.25,tbarsize=0.7 5,bracketlength=0.15,rbracketlength=0.15}
\begin{pspicture}(0,0)(35,46.25)
\psline[linewidth=0.75](5,15)(20,30)
\psline[linewidth=0.75](20,30)(20,46.25)
\newrgbcolor{userFillColour}{0.2 0 0.2}
\rput{0}(20,30){\psellipse[fillcolor=userFillColour,fillstyle=solid](0,0)(3.79,-3.79)}
\psline[linewidth=0.75](35,15)(20,30)
\rput[l](22.5,46.25){$\AAh$}
\psline[linewidth=0.75](35,2.5)(35,15)
\psline[linewidth=0.75](5,2.5)(5,15)
\rput[r](2.5,3.75){$\AAh$}
\rput[r](32.5,3.75){$\AAh$}
\rput[l](27.5,30){$\ccopy$}
\end{pspicture}


==> PIC/eval-black.tex <==
%%Created by jPicEdt 1.4.1_03: mixed JPIC-XML/LaTeX format
%%Fri Jul 15 08:38:20 GMT+01:00 2022
%%Begin JPIC-XML
%<?xml version="1.0" standalone="yes"?>
%<jpic x-min="0" x-max="200" y-min="0" y-max="120" auto-bounding="true">
%<multicurve fill-style= "none"
%	 stroke-width= "0.5"
%	 points= "(140,20);(140,20);(140,0);(140,0)"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 stroke-width= "0.35"
%	 anchor-point= "(100,60)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\EQLS
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 stroke-width= "0.35"
%	 anchor-point= "(136.25,65)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\Code$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 stroke-width= "0.35"
%	 anchor-point= "(165,117.5)"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\Cee$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 stroke-width= "0.35"
%	 anchor-point= "(45,117.5)"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\Cee$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 stroke-width= "0.35"
%	 anchor-point= "(15,2.5)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\Aee$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 stroke-width= "0.35"
%	 anchor-point= "(55,2.5)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\Bee$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 stroke-width= "0.35"
%	 anchor-point= "(130,35)"
%	 text-rotation= "-45"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\Fee$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 stroke-width= "0.35"
%	 anchor-point= "(135,2.5)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\Aee$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 stroke-width= "0.35"
%	 anchor-point= "(175,2.5)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\Bee$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 stroke-width= "0.35"
%	 anchor-point= "(140,40)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\Dott$
%</text>
%<multicurve fill-style= "none"
%	 stroke-width= "0.35"
%	 points= "(200,100);(200,100);(200,60);(200,60)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.35"
%	 points= "(120,100);(120,100);(200,100);(200,100)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.35"
%	 points= "(200,60);(200,60);(160,60);(160,60)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.35"
%	 points= "(120,100);(120,100);(160,60);(160,60)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.35"
%	 points= "(160,20);(160,20);(120,20);(120,20)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.5"
%	 points= "(180,60);(180,60);(180,0);(180,0)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.5"
%	 points= "(160,120);(160,120);(160,100);(160,100)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.35"
%	 points= "(120,60);(120,60);(160,20);(160,20)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "1"
%	 points= "(140,40);(140,40);(140,80);(140,80)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.35"
%	 points= "(120,60);(120,60);(120,20);(120,20)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.35"
%	 points= "(80,80);(80,80);(80,40);(80,40)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.35"
%	 points= "(80,40);(80,40);(0,40);(0,40)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.35"
%	 points= "(0,80);(0,80);(80,80);(80,80)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.5"
%	 points= "(60,40);(60,40);(60,0);(60,0)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.5"
%	 points= "(40,120);(40,120);(40,80);(40,80)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.35"
%	 points= "(0,80);(0,80);(0,40);(0,40)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.5"
%	 points= "(20,40);(20,40);(20,0);(20,0)"
%	 />
%<parallelogram p3= "(80,40)"
%	 p2= "(80,80)"
%	 fill-style= "solid"
%	 p1= "(0,80)"
%	 />
%<multicurve fill-color= "#330033"
%	 fill-style= "solid"
%	 points= "(120,100);(120,100);(200,100);(200,100);(200,100);(200,60);
%	(200,60);(200,60);(160,60);(160,60);(160,60);(120,100)"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 stroke-width= "0.35"
%	 anchor-point= "(176.25,80)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\Univ$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 stroke-width= "0.35"
%	 anchor-point= "(40,60)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\fee$
%</text>
%</jpic>
%%End JPIC-XML
%PSTricks content-type (pstricks.sty package needed)
%Add \usepackage{pstricks} in the preamble of your LaTeX file
%You can rescale the whole picture (to 80% for instance) by using the command \def\JPicScale{0.8}
\ifx\JPicScale\undefined\def\JPicScale{1}\fi
\psset{unit=\JPicScale mm}
\psset{linewidth=0.3,dotsep=1,hatchwidth=0.3,hatchsep=1.5,shadowsize=1,dimen=middle}
\psset{dotsize=0.7 2.5,dotscale=1 1,fillcolor=black}
\psset{arrowsize=1 2,arrowlength=1,arrowinset=0.25,tbarsize=0.7 5,bracketlength=0.15,rbracketlength=0.15}
\begin{pspicture}(0,0)(200,120)
\psline[linewidth=0.5](140,20)(140,0)
\rput(100,60){\EQLS}
\rput[r](136.25,65){$\Code$}
\rput[l](165,117.5){$\Cee$}
\rput[l](45,117.5){$\Cee$}
\rput[r](15,2.5){$\Aee$}
\rput[r](55,2.5){$\Bee$}
\rput{-45}(130,35){$\Fee$}
\rput[r](135,2.5){$\Aee$}
\rput[r](175,2.5){$\Bee$}
\rput(140,40){$\Dott$}
\psline[linewidth=0.35](200,100)(200,60)
\psline[linewidth=0.35](120,100)(200,100)
\psline[linewidth=0.35](200,60)(160,60)
\psline[linewidth=0.35](120,100)(160,60)
\psline[linewidth=0.35](160,20)(120,20)
\psline[linewidth=0.5](180,60)(180,0)
\psline[linewidth=0.5](160,120)(160,100)
\psline[linewidth=0.35](120,60)(160,20)
\psline[linewidth=1](140,40)(140,80)
\psline[linewidth=0.35](120,60)(120,20)
\psline[linewidth=0.35](80,80)(80,40)
\psline[linewidth=0.35](80,40)(0,40)
\psline[linewidth=0.35](0,80)(80,80)
\psline[linewidth=0.5](60,40)(60,0)
\psline[linewidth=0.5](40,120)(40,80)
\psline[linewidth=0.35](0,80)(0,40)
\psline[linewidth=0.5](20,40)(20,0)
\pspolygon[fillstyle=solid](0,80)(80,80)(80,40)(0,40)
\newrgbcolor{userFillColour}{0.2 0 0.2}
\pspolygon[fillcolor=userFillColour,fillstyle=solid](120,100)
(200,100)
(200,60)
(160,60)(120,100)
\rput(176.25,80){$\Univ$}
\rput(40,60){$\fee$}
\end{pspicture}


==> PIC/eval-pev.tex <==
%%Created by jPicEdt 1.4.1_03: mixed JPIC-XML/LaTeX format
%%Sun Nov 22 17:03:22 GMT-10:00 2020
%%Begin JPIC-XML
%<?xml version="1.0" standalone="yes"?>
%<jpic x-min="0" x-max="220" y-min="0" y-max="110" auto-bounding="true">
%<text stroke-width= "0.35"
%	 fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(162.5,52.5)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\Progtype$
%</text>
%<text stroke-width= "0.35"
%	 fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(157.5,32.5)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\partial$
%</text>
%<text stroke-width= "0.35"
%	 fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(190,65)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\universal$
%</text>
%<text stroke-width= "0.35"
%	 fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(192.5,110)"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\Progn$
%</text>
%<text stroke-width= "0.35"
%	 fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(202.5,0)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\Progm$
%</text>
%<text stroke-width= "0.35"
%	 fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(172.5,0)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\Progk$
%</text>
%<text stroke-width= "0.35"
%	 fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(147.5,0)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\Progtype$
%</text>
%<text stroke-width= "0.35"
%	 fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(110,65)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\eqlsb$
%</text>
%<multicurve fill-style= "none"
%	 points= "(220,95);(220,95);(220,35);(220,35)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(220,35);(220,35);(190,35);(190,35)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(190,15);(190,15);(160,15);(160,15)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(160,15);(160,15);(140,35);(140,35)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(140,35);(140,35);(140,65);(140,65)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(140,65);(140,65);(190,15);(190,15)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(190,35);(190,35);(140,85);(140,85)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(140,85);(140,85);(140,95);(140,95)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(140,95);(140,95);(220,95);(220,95)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(150,25);(150,25);(150,0);(150,0)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(165,60);(165,60);(165,40);(165,40)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(175,15);(175,15);(175,0);(175,0)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(205,35);(205,35);(205,0);(205,0)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(190,110);(190,110);(190,95);(190,95)"
%	 />
%<text stroke-width= "0.35"
%	 fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(50,65)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\universal$
%</text>
%<text stroke-width= "0.35"
%	 fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(52.5,110)"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\Progn$
%</text>
%<text stroke-width= "0.35"
%	 fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(62.5,0)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\Progm$
%</text>
%<text stroke-width= "0.35"
%	 fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(32.5,0)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\Progk$
%</text>
%<text stroke-width= "0.35"
%	 fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(7.5,0)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\Progtype$
%</text>
%<multicurve fill-style= "none"
%	 points= "(80,95);(80,95);(80,35);(80,35)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(80,35);(80,35);(20,35);(20,35)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(20,35);(20,35);(0,55);(0,55)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(0,55);(0,55);(0,95);(0,95)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(0,95);(0,95);(80,95);(80,95)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(10,45);(10,45);(10,0);(10,0)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(35,35);(35,35);(35,0);(35,0)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(65,35);(65,35);(65,0);(65,0)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(50,110);(50,110);(50,95);(50,95)"
%	 />
%</jpic>
%%End JPIC-XML
%LaTeX-picture environment using emulated lines and arcs
%You can rescale the whole picture (to 80% for instance) by using the command \def\JPicScale{0.8}
\ifx\JPicScale\undefined\def\JPicScale{1}\fi
\unitlength \JPicScale mm
\begin{picture}(220,110)(0,0)
\put(162.5,52.5){\makebox(0,0)[cr]{$\Progtype$}}

\put(157.5,32.5){\makebox(0,0)[cc]{$\partial$}}

\put(190,65){\makebox(0,0)[cc]{$\universal$}}

\put(192.5,110){\makebox(0,0)[cl]{$\Progn$}}

\put(202.5,0){\makebox(0,0)[cr]{$\Progm$}}

\put(172.5,0){\makebox(0,0)[cr]{$\Progk$}}

\put(147.5,0){\makebox(0,0)[cr]{$\Progtype$}}

\put(110,65){\makebox(0,0)[cc]{$\eqlsb$}}

\linethickness{0.3mm}
\put(220,35){\line(0,1){60}}
\linethickness{0.3mm}
\put(190,35){\line(1,0){30}}
\linethickness{0.3mm}
\put(160,15){\line(1,0){30}}
\linethickness{0.3mm}
\multiput(140,35)(0.12,-0.12){167}{\line(1,0){0.12}}
\linethickness{0.3mm}
\put(140,35){\line(0,1){30}}
\linethickness{0.3mm}
\multiput(140,65)(0.12,-0.12){417}{\line(1,0){0.12}}
\linethickness{0.3mm}
\multiput(140,85)(0.12,-0.12){417}{\line(1,0){0.12}}
\linethickness{0.3mm}
\put(140,85){\line(0,1){10}}
\linethickness{0.3mm}
\put(140,95){\line(1,0){80}}
\linethickness{0.3mm}
\put(150,0){\line(0,1){25}}
\linethickness{0.3mm}
\put(165,40){\line(0,1){20}}
\linethickness{0.3mm}
\put(175,0){\line(0,1){15}}
\linethickness{0.3mm}
\put(205,0){\line(0,1){35}}
\linethickness{0.3mm}
\put(190,95){\line(0,1){15}}
\put(50,65){\makebox(0,0)[cc]{$\universal$}}

\put(52.5,110){\makebox(0,0)[cl]{$\Progn$}}

\put(62.5,0){\makebox(0,0)[cr]{$\Progm$}}

\put(32.5,0){\makebox(0,0)[cr]{$\Progk$}}

\put(7.5,0){\makebox(0,0)[cr]{$\Progtype$}}

\linethickness{0.3mm}
\put(80,35){\line(0,1){60}}
\linethickness{0.3mm}
\put(20,35){\line(1,0){60}}
\linethickness{0.3mm}
\multiput(0,55)(0.12,-0.12){167}{\line(1,0){0.12}}
\linethickness{0.3mm}
\put(0,55){\line(0,1){40}}
\linethickness{0.3mm}
\put(0,95){\line(1,0){80}}
\linethickness{0.3mm}
\put(10,0){\line(0,1){45}}
\linethickness{0.3mm}
\put(35,0){\line(0,1){35}}
\linethickness{0.3mm}
\put(65,0){\line(0,1){35}}
\linethickness{0.3mm}
\put(50,95){\line(0,1){15}}
\end{picture}


==> PIC/eval-proc.tex <==
%%Created by jPicEdt 1.4.1_03: mixed JPIC-XML/LaTeX format
%%Sun May 22 18:08:46 GMT+01:00 2022
%%Begin JPIC-XML
%<?xml version="1.0" standalone="yes"?>
%<jpic x-min="0" x-max="200" y-min="0" y-max="160" auto-bounding="true">
%<multicurve fill-style= "none"
%	 stroke-width= "0.4"
%	 points= "(80,80);(80,80);(80,40);(80,40)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.4"
%	 points= "(80,40);(80,40);(0,40);(0,40)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.4"
%	 points= "(0,80);(0,80);(80,80);(80,80)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.4"
%	 points= "(60,40);(60,40);(60,0);(60,0)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.4"
%	 points= "(60,120);(60,120);(60,80);(60,80)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.4"
%	 points= "(0,80);(0,80);(0,40);(0,40)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.4"
%	 points= "(20,40);(20,40);(20,0);(20,0)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.4"
%	 points= "(200,100);(200,100);(200,60);(200,60)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.4"
%	 points= "(160,20);(160,20);(120,20);(120,20)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.4"
%	 points= "(120,100);(120,100);(200,100);(200,100)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.4"
%	 points= "(180,60);(180,60);(180,0);(180,0)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.4"
%	 points= "(180,120);(180,120);(180,100);(180,100)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.4"
%	 points= "(120,60);(120,60);(120,20);(120,20)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.4"
%	 points= "(140,20);(140,20);(140,0);(140,0)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.4"
%	 points= "(200,60);(200,60);(160,60);(160,60)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.4"
%	 points= "(120,100);(120,100);(160,60);(160,60)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.4"
%	 points= "(120,60);(120,60);(160,20);(160,20)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "1.45"
%	 points= "(140,40);(140,40);(140,80);(140,80)"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 stroke-width= "0.4"
%	 anchor-point= "(170,80)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\Univ$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 stroke-width= "0.4"
%	 anchor-point= "(100,60)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\EQLS
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 stroke-width= "0.4"
%	 anchor-point= "(136.25,65)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\Code$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 stroke-width= "0.4"
%	 anchor-point= "(185,117.5)"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\Cee$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 stroke-width= "0.4"
%	 anchor-point= "(65,117.5)"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\Cee$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 stroke-width= "0.4"
%	 anchor-point= "(15,2.5)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\Aee$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 stroke-width= "0.4"
%	 anchor-point= "(55,2.5)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\Bee$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 stroke-width= "0.4"
%	 anchor-point= "(40,60)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\fee$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 stroke-width= "0.4"
%	 anchor-point= "(130,31.25)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\Fee$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 stroke-width= "0.4"
%	 anchor-point= "(135,2.5)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\Aee$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 stroke-width= "0.4"
%	 anchor-point= "(175,2.5)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\Bee$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 stroke-width= "0.4"
%	 anchor-point= "(100,140)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\EQLS
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 stroke-width= "0.4"
%	 anchor-point= "(60,140)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\LHS$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 stroke-width= "0.4"
%	 anchor-point= "(180,140)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\RHS$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 stroke-width= "0.4"
%	 anchor-point= "(140,40)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\Dott$
%</text>
%<multicurve fill-style= "none"
%	 stroke-width= "0.4"
%	 points= "(20,120);(20,120);(20,80);(20,80)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.4"
%	 points= "(140,120);(140,120);(140,100);(140,100)"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 stroke-width= "0.4"
%	 anchor-point= "(25,117.5)"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\Aee$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 stroke-width= "0.4"
%	 anchor-point= "(145,117.5)"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\Aee$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 stroke-width= "0.4"
%	 anchor-point= "(20,160)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\LHSP$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 stroke-width= "0.4"
%	 anchor-point= "(140,160)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\RHSP$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 stroke-width= "0.4"
%	 anchor-point= "(100,160)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\EQLS
%</text>
%</jpic>
%%End JPIC-XML
%PSTricks content-type (pstricks.sty package needed)
%Add \usepackage{pstricks} in the preamble of your LaTeX file
%You can rescale the whole picture (to 80% for instance) by using the command \def\JPicScale{0.8}
\ifx\JPicScale\undefined\def\JPicScale{1}\fi
\psset{unit=\JPicScale mm}
\psset{linewidth=0.3,dotsep=1,hatchwidth=0.3,hatchsep=1.5,shadowsize=1,dimen=middle}
\psset{dotsize=0.7 2.5,dotscale=1 1,fillcolor=black}
\psset{arrowsize=1 2,arrowlength=1,arrowinset=0.25,tbarsize=0.7 5,bracketlength=0.15,rbracketlength=0.15}
\begin{pspicture}(0,0)(200,160)
\psline[linewidth=0.4](80,80)(80,40)
\psline[linewidth=0.4](80,40)(0,40)
\psline[linewidth=0.4](0,80)(80,80)
\psline[linewidth=0.4](60,40)(60,0)
\psline[linewidth=0.4](60,120)(60,80)
\psline[linewidth=0.4](0,80)(0,40)
\psline[linewidth=0.4](20,40)(20,0)
\psline[linewidth=0.4](200,100)(200,60)
\psline[linewidth=0.4](160,20)(120,20)
\psline[linewidth=0.4](120,100)(200,100)
\psline[linewidth=0.4](180,60)(180,0)
\psline[linewidth=0.4](180,120)(180,100)
\psline[linewidth=0.4](120,60)(120,20)
\psline[linewidth=0.4](140,20)(140,0)
\psline[linewidth=0.4](200,60)(160,60)
\psline[linewidth=0.4](120,100)(160,60)
\psline[linewidth=0.4](120,60)(160,20)
\psline[linewidth=1.45](140,40)(140,80)
\rput(170,80){$\Univ$}
\rput(100,60){\EQLS}
\rput[r](136.25,65){$\Code$}
\rput[l](185,117.5){$\Cee$}
\rput[l](65,117.5){$\Cee$}
\rput[r](15,2.5){$\Aee$}
\rput[r](55,2.5){$\Bee$}
\rput(40,60){$\fee$}
\rput(130,31.25){$\Fee$}
\rput[r](135,2.5){$\Aee$}
\rput[r](175,2.5){$\Bee$}
\rput(100,140){\EQLS}
\rput(60,140){$\LHS$}
\rput(180,140){$\RHS$}
\rput(140,40){$\Dott$}
\psline[linewidth=0.4](20,120)(20,80)
\psline[linewidth=0.4](140,120)(140,100)
\rput[l](25,117.5){$\Aee$}
\rput[l](145,117.5){$\Aee$}
\rput(20,160){$\LHSP$}
\rput(140,160){$\RHSP$}
\rput(100,160){\EQLS}
\end{pspicture}


==> PIC/eval-procs.tex <==
%%Created by jPicEdt 1.4.1_03: mixed JPIC-XML/LaTeX format
%%Sun May 22 17:52:56 GMT+01:00 2022
%%Begin JPIC-XML
%<?xml version="1.0" standalone="yes"?>
%<jpic x-min="0" x-max="200" y-min="0" y-max="170" auto-bounding="true">
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(80,80);(80,80);(80,40);(80,40)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(80,40);(80,40);(0,40);(0,40)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(0,80);(0,80);(80,80);(80,80)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(60,40);(60,40);(60,0);(60,0)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(60,120);(60,120);(60,80);(60,80)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(0,80);(0,80);(0,40);(0,40)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(20,40);(20,40);(20,0);(20,0)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(200,100);(200,100);(200,60);(200,60)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(160,20);(160,20);(120,20);(120,20)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(120,100);(120,100);(200,100);(200,100)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(180,60);(180,60);(180,0);(180,0)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(180,120);(180,120);(180,100);(180,100)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(120,60);(120,60);(120,20);(120,20)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(140,20);(140,20);(140,0);(140,0)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(200,60);(200,60);(160,60);(160,60)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(120,100);(120,100);(160,60);(160,60)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(120,60);(120,60);(160,20);(160,20)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "1.4"
%	 points= "(140,40);(140,40);(140,80);(140,80)"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 stroke-width= "0.75"
%	 anchor-point= "(170,80)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\Univ$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 stroke-width= "0.75"
%	 anchor-point= "(100,60)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\EQLS
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 stroke-width= "0.75"
%	 anchor-point= "(136.25,65)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\Code$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 stroke-width= "0.75"
%	 anchor-point= "(185,117.5)"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\Cee$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 stroke-width= "0.75"
%	 anchor-point= "(65,117.5)"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\Cee$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 stroke-width= "0.75"
%	 anchor-point= "(15,2.5)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\Aee$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 stroke-width= "0.75"
%	 anchor-point= "(55,2.5)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\Bee$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 stroke-width= "0.75"
%	 anchor-point= "(40,60)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\fee$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 stroke-width= "0.75"
%	 anchor-point= "(130,31.25)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\Fee$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 stroke-width= "0.75"
%	 anchor-point= "(135,2.5)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\Aee$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 stroke-width= "0.75"
%	 anchor-point= "(175,2.5)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\Bee$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 stroke-width= "0.75"
%	 anchor-point= "(100,150)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\EQLS
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(60,150)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\LHS$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(180,150)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\RHS$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(140,40)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\Dott$
%</text>
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(20,120);(20,120);(20,80);(20,80)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(140,120);(140,120);(140,100);(140,100)"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 stroke-width= "0.75"
%	 anchor-point= "(25,117.5)"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\Aee$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 stroke-width= "0.75"
%	 anchor-point= "(145,117.5)"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\Aee$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(20,170)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\LHSP$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(140,170)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\RHSP$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 stroke-width= "0.75"
%	 anchor-point= "(100,170)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\EQLS
%</text>
%</jpic>
%%End JPIC-XML
%LaTeX-picture environment using emulated lines and arcs
%You can rescale the whole picture (to 80% for instance) by using the command \def\JPicScale{0.8}
\ifx\JPicScale\undefined\def\JPicScale{1}\fi
\unitlength \JPicScale mm
\begin{picture}(200,170)(0,0)
\linethickness{0.75mm}
\put(80,40){\line(0,1){40}}
\linethickness{0.75mm}
\put(0,40){\line(1,0){80}}
\linethickness{0.75mm}
\put(0,80){\line(1,0){80}}
\linethickness{0.75mm}
\put(60,0){\line(0,1){40}}
\linethickness{0.75mm}
\put(60,80){\line(0,1){40}}
\linethickness{0.75mm}
\put(0,40){\line(0,1){40}}
\linethickness{0.75mm}
\put(20,0){\line(0,1){40}}
\linethickness{0.75mm}
\put(200,60){\line(0,1){40}}
\linethickness{0.75mm}
\put(120,20){\line(1,0){40}}
\linethickness{0.75mm}
\put(120,100){\line(1,0){80}}
\linethickness{0.75mm}
\put(180,0){\line(0,1){60}}
\linethickness{0.75mm}
\put(180,100){\line(0,1){20}}
\linethickness{0.75mm}
\put(120,20){\line(0,1){40}}
\linethickness{0.75mm}
\put(140,0){\line(0,1){20}}
\linethickness{0.75mm}
\put(160,60){\line(1,0){40}}
\linethickness{0.75mm}
\multiput(120,100)(0.12,-0.12){333}{\line(1,0){0.12}}
\linethickness{0.75mm}
\multiput(120,60)(0.12,-0.12){333}{\line(1,0){0.12}}
\linethickness{1.4mm}
\put(140,40){\line(0,1){40}}
\put(170,80){\makebox(0,0)[cc]{$\Univ$}}

\put(100,60){\makebox(0,0)[cc]{\EQLS}}

\put(136.25,65){\makebox(0,0)[cr]{$\Code$}}

\put(185,117.5){\makebox(0,0)[cl]{$\Cee$}}

\put(65,117.5){\makebox(0,0)[cl]{$\Cee$}}

\put(15,2.5){\makebox(0,0)[cr]{$\Aee$}}

\put(55,2.5){\makebox(0,0)[cr]{$\Bee$}}

\put(40,60){\makebox(0,0)[cc]{$\fee$}}

\put(130,31.25){\makebox(0,0)[cc]{$\Fee$}}

\put(135,2.5){\makebox(0,0)[cr]{$\Aee$}}

\put(175,2.5){\makebox(0,0)[cr]{$\Bee$}}

\put(100,150){\makebox(0,0)[cc]{\EQLS}}

\put(60,150){\makebox(0,0)[cc]{$\LHS$}}

\put(180,150){\makebox(0,0)[cc]{$\RHS$}}

\put(140,40){\makebox(0,0)[cc]{$\Dott$}}

\linethickness{0.75mm}
\put(20,80){\line(0,1){40}}
\linethickness{0.75mm}
\put(140,100){\line(0,1){20}}
\put(25,117.5){\makebox(0,0)[cl]{$\Aee$}}

\put(145,117.5){\makebox(0,0)[cl]{$\Aee$}}

\put(20,170){\makebox(0,0)[cc]{$\LHSP$}}

\put(140,170){\makebox(0,0)[cc]{$\RHSP$}}

\put(100,170){\makebox(0,0)[cc]{\EQLS}}

\end{picture}


==> PIC/eval-uev-strict-thick.tex <==
%%Created by jPicEdt 1.4.1_03: mixed JPIC-XML/LaTeX format
%%Thu Dec 17 09:06:46 GMT-10:00 2020
%%Begin JPIC-XML
%<?xml version="1.0" standalone="yes"?>
%<jpic x-min="0" x-max="180" y-min="0" y-max="100" auto-bounding="true">
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(30,60)"
%	 text-frame= "noframe"
%	 stroke-width= "0.75"
%	 text-hor-align= "center-h"
%	 >
%\gee
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(90,60)"
%	 text-frame= "noframe"
%	 stroke-width= "0.75"
%	 text-hor-align= "center-h"
%	 >
%$\eqlsa$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(155,60)"
%	 text-frame= "noframe"
%	 stroke-width= "0.75"
%	 text-hor-align= "center-h"
%	 >
%$\universal$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(152.5,100)"
%	 text-frame= "noframe"
%	 stroke-width= "0.75"
%	 text-hor-align= "left"
%	 >
%$\Progn$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(167.5,0)"
%	 text-frame= "noframe"
%	 stroke-width= "0.75"
%	 text-hor-align= "right"
%	 >
%$\Progm$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(130,28.75)"
%	 text-frame= "noframe"
%	 stroke-width= "0.75"
%	 text-hor-align= "center-h"
%	 >
%\program
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(127.5,55)"
%	 text-frame= "noframe"
%	 stroke-width= "0.75"
%	 text-hor-align= "right"
%	 >
%$\Progtype$
%</text>
%<multicurve fill-style= "none"
%	 points= "(180,80);(180,80);(180,40);(180,40)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(180,40);(180,40);(150,40);(150,40)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(150,20);(150,20);(120,20);(120,20)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(120,50);(120,50);(120,20);(120,20)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(120,50);(120,50);(150,20);(150,20)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(150,40);(150,40);(120,70);(120,70)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(120,70);(120,70);(120,80);(120,80)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(120,80);(120,80);(180,80);(180,80)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(130,60);(130,60);(130,35);(130,35)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(170,40);(170,40);(170,0);(170,0)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(150,100);(150,100);(150,80);(150,80)"
%	 stroke-width= "0.75"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(32.5,100)"
%	 text-frame= "noframe"
%	 stroke-width= "0.75"
%	 text-hor-align= "left"
%	 >
%$\Progn$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(47.5,0)"
%	 text-frame= "noframe"
%	 stroke-width= "0.75"
%	 text-hor-align= "right"
%	 >
%$\Progm$
%</text>
%<multicurve fill-style= "none"
%	 points= "(60,80);(60,80);(60,40);(60,40)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(60,40);(60,40);(0,40);(0,40)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(0,80);(0,80);(60,80);(60,80)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(50,40);(50,40);(50,0);(50,0)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(30,100);(30,100);(30,80);(30,80)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(0,80);(0,80);(0,40);(0,40)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(10,40);(10,40);(10,0);(10,0)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(130,23.75);(130,23.75);(130,0);(130,0)"
%	 stroke-width= "0.75"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(127.5,0)"
%	 text-frame= "noframe"
%	 stroke-width= "0.75"
%	 text-hor-align= "right"
%	 >
%$\Param$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(7.5,0)"
%	 text-frame= "noframe"
%	 stroke-width= "0.75"
%	 text-hor-align= "right"
%	 >
%$\Param$
%</text>
%</jpic>
%%End JPIC-XML
%PSTricks content-type (pstricks.sty package needed)
%Add \usepackage{pstricks} in the preamble of your LaTeX file
%You can rescale the whole picture (to 80% for instance) by using the command \def\JPicScale{0.8}
\ifx\JPicScale\undefined\def\JPicScale{1}\fi
\psset{unit=\JPicScale mm}
\psset{linewidth=0.3,dotsep=1,hatchwidth=0.3,hatchsep=1.5,shadowsize=1,dimen=middle}
\psset{dotsize=0.7 2.5,dotscale=1 1,fillcolor=black}
\psset{arrowsize=1 2,arrowlength=1,arrowinset=0.25,tbarsize=0.7 5,bracketlength=0.15,rbracketlength=0.15}
\begin{pspicture}(0,0)(180,100)
\rput(30,60){\gee}
\rput(90,60){$\eqlsa$}
\rput(155,60){$\universal$}
\rput[l](152.5,100){$\Progn$}
\rput[r](167.5,0){$\Progm$}
\rput(130,28.75){\program}
\rput[r](127.5,55){$\Progtype$}
\psline[linewidth=0.75](180,80)(180,40)
\psline[linewidth=0.75](180,40)(150,40)
\psline[linewidth=0.75](150,20)(120,20)
\psline[linewidth=0.75](120,50)(120,20)
\psline[linewidth=0.75](120,50)(150,20)
\psline[linewidth=0.75](150,40)(120,70)
\psline[linewidth=0.75](120,70)(120,80)
\psline[linewidth=0.75](120,80)(180,80)
\psline[linewidth=0.75](130,60)(130,35)
\psline[linewidth=0.75](170,40)(170,0)
\psline[linewidth=0.75](150,100)(150,80)
\rput[l](32.5,100){$\Progn$}
\rput[r](47.5,0){$\Progm$}
\psline[linewidth=0.75](60,80)(60,40)
\psline[linewidth=0.75](60,40)(0,40)
\psline[linewidth=0.75](0,80)(60,80)
\psline[linewidth=0.75](50,40)(50,0)
\psline[linewidth=0.75](30,100)(30,80)
\psline[linewidth=0.75](0,80)(0,40)
\psline[linewidth=0.75](10,40)(10,0)
\psline[linewidth=0.75](130,23.75)(130,0)
\rput[r](127.5,0){$\Param$}
\rput[r](7.5,0){$\Param$}
\end{pspicture}


==> PIC/eval-uev-strict.tex <==
%%Created by jPicEdt 1.4.1_03: mixed JPIC-XML/LaTeX format
%%Sun Dec 13 13:06:05 GMT-10:00 2020
%%Begin JPIC-XML
%<?xml version="1.0" standalone="yes"?>
%<jpic x-min="0" x-max="180" y-min="0" y-max="100" auto-bounding="true">
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(30,60)"
%	 text-frame= "noframe"
%	 stroke-width= "0.35"
%	 text-hor-align= "center-h"
%	 >
%\gee
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(90,60)"
%	 text-frame= "noframe"
%	 stroke-width= "0.35"
%	 text-hor-align= "center-h"
%	 >
%$\eqlsa$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(155,60)"
%	 text-frame= "noframe"
%	 stroke-width= "0.35"
%	 text-hor-align= "center-h"
%	 >
%$\universal$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(152.5,100)"
%	 text-frame= "noframe"
%	 stroke-width= "0.35"
%	 text-hor-align= "left"
%	 >
%$\Progn$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(167.5,0)"
%	 text-frame= "noframe"
%	 stroke-width= "0.35"
%	 text-hor-align= "right"
%	 >
%$\Progm$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(130,28.75)"
%	 text-frame= "noframe"
%	 stroke-width= "0.35"
%	 text-hor-align= "center-h"
%	 >
%\program
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(127.5,55)"
%	 text-frame= "noframe"
%	 stroke-width= "0.35"
%	 text-hor-align= "right"
%	 >
%$\Progtype$
%</text>
%<multicurve fill-style= "none"
%	 points= "(180,80);(180,80);(180,40);(180,40)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(180,40);(180,40);(150,40);(150,40)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(150,20);(150,20);(120,20);(120,20)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(120,50);(120,50);(120,20);(120,20)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(120,50);(120,50);(150,20);(150,20)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(150,40);(150,40);(120,70);(120,70)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(120,70);(120,70);(120,80);(120,80)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(120,80);(120,80);(180,80);(180,80)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(130,60);(130,60);(130,35);(130,35)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(170,40);(170,40);(170,0);(170,0)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(150,100);(150,100);(150,80);(150,80)"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(32.5,100)"
%	 text-frame= "noframe"
%	 stroke-width= "0.35"
%	 text-hor-align= "left"
%	 >
%$\Progn$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(47.5,0)"
%	 text-frame= "noframe"
%	 stroke-width= "0.35"
%	 text-hor-align= "right"
%	 >
%$\Progm$
%</text>
%<multicurve fill-style= "none"
%	 points= "(60,80);(60,80);(60,40);(60,40)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(60,40);(60,40);(0,40);(0,40)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(0,80);(0,80);(60,80);(60,80)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(50,40);(50,40);(50,0);(50,0)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(30,100);(30,100);(30,80);(30,80)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(0,80);(0,80);(0,40);(0,40)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(10,40);(10,40);(10,0);(10,0)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(130,23.75);(130,23.75);(130,0);(130,0)"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(127.5,0)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\Param$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(7.5,0)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\Param$
%</text>
%</jpic>
%%End JPIC-XML
%PSTricks content-type (pstricks.sty package needed)
%Add \usepackage{pstricks} in the preamble of your LaTeX file
%You can rescale the whole picture (to 80% for instance) by using the command \def\JPicScale{0.8}
\ifx\JPicScale\undefined\def\JPicScale{1}\fi
\psset{unit=\JPicScale mm}
\psset{linewidth=0.3,dotsep=1,hatchwidth=0.3,hatchsep=1.5,shadowsize=1,dimen=middle}
\psset{dotsize=0.7 2.5,dotscale=1 1,fillcolor=black}
\psset{arrowsize=1 2,arrowlength=1,arrowinset=0.25,tbarsize=0.7 5,bracketlength=0.15,rbracketlength=0.15}
\begin{pspicture}(0,0)(180,100)
\rput(30,60){\gee}
\rput(90,60){$\eqlsa$}
\rput(155,60){$\universal$}
\rput[l](152.5,100){$\Progn$}
\rput[r](167.5,0){$\Progm$}
\rput(130,28.75){\program}
\rput[r](127.5,55){$\Progtype$}
\psline(180,80)(180,40)
\psline(180,40)(150,40)
\psline(150,20)(120,20)
\psline(120,50)(120,20)
\psline(120,50)(150,20)
\psline(150,40)(120,70)
\psline(120,70)(120,80)
\psline(120,80)(180,80)
\psline(130,60)(130,35)
\psline(170,40)(170,0)
\psline(150,100)(150,80)
\rput[l](32.5,100){$\Progn$}
\rput[r](47.5,0){$\Progm$}
\psline(60,80)(60,40)
\psline(60,40)(0,40)
\psline(0,80)(60,80)
\psline(50,40)(50,0)
\psline(30,100)(30,80)
\psline(0,80)(0,40)
\psline(10,40)(10,0)
\psline(130,23.75)(130,0)
\rput[r](127.5,0){$\Param$}
\rput[r](7.5,0){$\Param$}
\end{pspicture}


==> PIC/eval-uev.tex <==
%%Created by jPicEdt 1.4.1_03: mixed JPIC-XML/LaTeX format
%%Sun Nov 22 17:55:47 GMT-10:00 2020
%%Begin JPIC-XML
%<?xml version="1.0" standalone="yes"?>
%<jpic x-min="0" x-max="200" y-min="0" y-max="120" auto-bounding="true">
%<text stroke-width= "0.35"
%	 fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(30,75)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\gee
%</text>
%<text stroke-width= "0.35"
%	 fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(90,75)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\eqlsa$
%</text>
%<text stroke-width= "0.35"
%	 fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(170,75)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\universal$
%</text>
%<text stroke-width= "0.35"
%	 fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(172.5,120)"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\Progn$
%</text>
%<text stroke-width= "0.35"
%	 fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(172.5,0)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\Progm$
%</text>
%<text stroke-width= "0.35"
%	 fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(127.5,23.75)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\program
%</text>
%<text stroke-width= "0.35"
%	 fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(132.5,50)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\Progtype$
%</text>
%<multicurve fill-style= "none"
%	 points= "(200,105);(200,105);(200,45);(200,45)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(200,45);(200,45);(150,45);(150,45)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(150,15);(150,15);(120,15);(120,15)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(120,45);(120,45);(120,15);(120,15)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(120,45);(120,45);(150,15);(150,15)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(150,45);(150,45);(120,75);(120,75)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(120,75);(120,75);(120,105);(120,105)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(120,105);(120,105);(200,105);(200,105)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(135,60);(135,60);(135,30);(135,30)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(175,45);(175,45);(175,0);(175,0)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(170,120);(170,120);(170,105);(170,105)"
%	 />
%<text stroke-width= "0.35"
%	 fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(32.5,120)"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\Progn$
%</text>
%<text stroke-width= "0.35"
%	 fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(27.5,0)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\Progm$
%</text>
%<multicurve fill-style= "none"
%	 points= "(60,105);(60,105);(60,45);(60,45)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(60,45);(60,45);(0,45);(0,45)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(0,105);(0,105);(60,105);(60,105)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(30,45);(30,45);(30,0);(30,0)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(30,120);(30,120);(30,105);(30,105)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(0,105);(0,105);(0,45);(0,45)"
%	 />
%</jpic>
%%End JPIC-XML
%LaTeX-picture environment using emulated lines and arcs
%You can rescale the whole picture (to 80% for instance) by using the command \def\JPicScale{0.8}
\ifx\JPicScale\undefined\def\JPicScale{1}\fi
\unitlength \JPicScale mm
\begin{picture}(200,120)(0,0)
\put(30,75){\makebox(0,0)[cc]{\gee}}

\put(90,75){\makebox(0,0)[cc]{$\eqlsa$}}

\put(170,75){\makebox(0,0)[cc]{$\universal$}}

\put(172.5,120){\makebox(0,0)[cl]{$\Progn$}}

\put(172.5,0){\makebox(0,0)[cr]{$\Progm$}}

\put(127.5,23.75){\makebox(0,0)[cc]{\program}}

\put(132.5,50){\makebox(0,0)[cr]{$\Progtype$}}

\linethickness{0.3mm}
\put(200,45){\line(0,1){60}}
\linethickness{0.3mm}
\put(150,45){\line(1,0){50}}
\linethickness{0.3mm}
\put(120,15){\line(1,0){30}}
\linethickness{0.3mm}
\put(120,15){\line(0,1){30}}
\linethickness{0.3mm}
\multiput(120,45)(0.12,-0.12){250}{\line(1,0){0.12}}
\linethickness{0.3mm}
\multiput(120,75)(0.12,-0.12){250}{\line(1,0){0.12}}
\linethickness{0.3mm}
\put(120,75){\line(0,1){30}}
\linethickness{0.3mm}
\put(120,105){\line(1,0){80}}
\linethickness{0.3mm}
\put(135,30){\line(0,1){30}}
\linethickness{0.3mm}
\put(175,0){\line(0,1){45}}
\linethickness{0.3mm}
\put(170,105){\line(0,1){15}}
\put(32.5,120){\makebox(0,0)[cl]{$\Progn$}}

\put(27.5,0){\makebox(0,0)[cr]{$\Progm$}}

\linethickness{0.3mm}
\put(60,45){\line(0,1){60}}
\linethickness{0.3mm}
\put(0,45){\line(1,0){60}}
\linethickness{0.3mm}
\put(0,105){\line(1,0){60}}
\linethickness{0.3mm}
\put(30,0){\line(0,1){45}}
\linethickness{0.3mm}
\put(30,105){\line(0,1){15}}
\linethickness{0.3mm}
\put(0,45){\line(0,1){60}}
\end{picture}


==> PIC/evalff.tex <==
%%Created by jPicEdt 1.4.1_03: mixed JPIC-XML/LaTeX format
%%Mon May 17 23:14:52 GMT-10:00 2021
%%Begin JPIC-XML
%<?xml version="1.0" standalone="yes"?>
%<jpic x-min="0" x-max="240" y-min="0" y-max="150" auto-bounding="true">
%<multicurve fill-style= "none"
%	 points= "(40,80);(40,80);(40,40);(40,40)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(40,40);(40,40);(0,40);(0,40)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(0,80);(0,80);(40,80);(40,80)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(20,40);(20,40);(20,0);(20,0)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(20,120);(20,120);(20,80);(20,80)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(0,80);(0,80);(0,40);(0,40)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(240,100);(240,100);(240,60);(240,60)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(200,20);(200,20);(160,20);(160,20)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(160,100);(160,100);(240,100);(240,100)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(220,60);(220,60);(220,0);(220,0)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(220,120);(220,120);(220,100);(220,100)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(160,60);(160,60);(160,20);(160,20)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(240,60);(240,60);(200,60);(200,60)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(160,100);(160,100);(200,60);(200,60)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(160,60);(160,60);(200,20);(200,20)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(180,40);(180,40);(180,80);(180,80)"
%	 stroke-width= "1.4"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(220,80)"
%	 text-frame= "noframe"
%	 stroke-width= "0.75"
%	 text-hor-align= "center-h"
%	 >
%$\Univ$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(140,60)"
%	 text-frame= "noframe"
%	 stroke-width= "0.75"
%	 text-hor-align= "center-h"
%	 >
%\EQLS
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(176.25,65)"
%	 text-frame= "noframe"
%	 stroke-width= "0.75"
%	 text-hor-align= "right"
%	 >
%$\Code$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(225,117.5)"
%	 text-frame= "noframe"
%	 stroke-width= "0.75"
%	 text-hor-align= "left"
%	 >
%$\Cee$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(25,117.5)"
%	 text-frame= "noframe"
%	 stroke-width= "0.75"
%	 text-hor-align= "left"
%	 >
%$\Cee$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(15,2.5)"
%	 text-frame= "noframe"
%	 stroke-width= "0.75"
%	 text-hor-align= "right"
%	 >
%$\Bee$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(20,60)"
%	 text-frame= "noframe"
%	 stroke-width= "0.75"
%	 text-hor-align= "center-h"
%	 >
%$\fee$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(170,31.25)"
%	 text-frame= "noframe"
%	 stroke-width= "0.75"
%	 text-hor-align= "center-h"
%	 >
%$\Fee$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(215,2.5)"
%	 text-frame= "noframe"
%	 stroke-width= "0.75"
%	 text-hor-align= "right"
%	 >
%$\Bee$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(180,40)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\Dott$
%</text>
%<multicurve fill-style= "none"
%	 points= "(120,100);(120,100);(120,60);(120,60)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(120,20);(120,20);(80,20);(80,20)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(80,100);(80,100);(120,100);(120,100)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(100,20);(100,20);(100,0);(100,0)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(100,120);(100,120);(100,100);(100,100)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(80,60);(80,60);(80,20);(80,20)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(80,100);(80,100);(120,60);(120,60)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(80,60);(80,60);(120,20);(120,20)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(100,40);(100,40);(100,80);(100,80)"
%	 stroke-width= "1.4"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(110,85)"
%	 text-frame= "noframe"
%	 stroke-width= "0.75"
%	 text-hor-align= "center-h"
%	 >
%$\Univ$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(60,60)"
%	 text-frame= "noframe"
%	 stroke-width= "0.75"
%	 text-hor-align= "center-h"
%	 >
%\EQLS
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(96.25,65)"
%	 text-frame= "noframe"
%	 stroke-width= "0.75"
%	 text-hor-align= "right"
%	 >
%$\Code$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(105,117.5)"
%	 text-frame= "noframe"
%	 stroke-width= "0.75"
%	 text-hor-align= "left"
%	 >
%$\Cee$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(95,2.5)"
%	 text-frame= "noframe"
%	 stroke-width= "0.75"
%	 text-hor-align= "right"
%	 >
%$\Bee$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(100,40)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\Dott$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(20,150)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\fleft$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(100,150)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\fmid$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(190,150)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\fright$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(140,150)"
%	 text-frame= "noframe"
%	 stroke-width= "0.75"
%	 text-hor-align= "center-h"
%	 >
%\EQLS
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(60,150)"
%	 text-frame= "noframe"
%	 stroke-width= "0.75"
%	 text-hor-align= "center-h"
%	 >
%\EQLS
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(90,30)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\Fei$
%</text>
%</jpic>
%%End JPIC-XML
%LaTeX-picture environment using emulated lines and arcs
%You can rescale the whole picture (to 80% for instance) by using the command \def\JPicScale{0.8}
\ifx\JPicScale\undefined\def\JPicScale{1}\fi
\unitlength \JPicScale mm
\begin{picture}(240,150)(0,0)
\linethickness{0.75mm}
\put(40,40){\line(0,1){40}}
\linethickness{0.75mm}
\put(0,40){\line(1,0){40}}
\linethickness{0.75mm}
\put(0,80){\line(1,0){40}}
\linethickness{0.75mm}
\put(20,0){\line(0,1){40}}
\linethickness{0.75mm}
\put(20,80){\line(0,1){40}}
\linethickness{0.75mm}
\put(0,40){\line(0,1){40}}
\linethickness{0.75mm}
\put(240,60){\line(0,1){40}}
\linethickness{0.75mm}
\put(160,20){\line(1,0){40}}
\linethickness{0.75mm}
\put(160,100){\line(1,0){80}}
\linethickness{0.75mm}
\put(220,0){\line(0,1){60}}
\linethickness{0.75mm}
\put(220,100){\line(0,1){20}}
\linethickness{0.75mm}
\put(160,20){\line(0,1){40}}
\linethickness{0.75mm}
\put(200,60){\line(1,0){40}}
\linethickness{0.75mm}
\multiput(160,100)(0.12,-0.12){333}{\line(1,0){0.12}}
\linethickness{0.75mm}
\multiput(160,60)(0.12,-0.12){333}{\line(1,0){0.12}}
\linethickness{1.4mm}
\put(180,40){\line(0,1){40}}
\put(220,80){\makebox(0,0)[cc]{$\Univ$}}

\put(140,60){\makebox(0,0)[cc]{\EQLS}}

\put(176.25,65){\makebox(0,0)[cr]{$\Code$}}

\put(225,117.5){\makebox(0,0)[cl]{$\Cee$}}

\put(25,117.5){\makebox(0,0)[cl]{$\Cee$}}

\put(15,2.5){\makebox(0,0)[cr]{$\Bee$}}

\put(20,60){\makebox(0,0)[cc]{$\fee$}}

\put(170,31.25){\makebox(0,0)[cc]{$\Fee$}}

\put(215,2.5){\makebox(0,0)[cr]{$\Bee$}}

\put(180,40){\makebox(0,0)[cc]{$\Dott$}}

\linethickness{0.75mm}
\put(120,60){\line(0,1){40}}
\linethickness{0.75mm}
\put(80,20){\line(1,0){40}}
\linethickness{0.75mm}
\put(80,100){\line(1,0){40}}
\linethickness{0.75mm}
\put(100,0){\line(0,1){20}}
\linethickness{0.75mm}
\put(100,100){\line(0,1){20}}
\linethickness{0.75mm}
\put(80,20){\line(0,1){40}}
\linethickness{0.75mm}
\multiput(80,100)(0.12,-0.12){333}{\line(1,0){0.12}}
\linethickness{0.75mm}
\multiput(80,60)(0.12,-0.12){333}{\line(1,0){0.12}}
\linethickness{1.4mm}
\put(100,40){\line(0,1){40}}
\put(110,85){\makebox(0,0)[cc]{$\Univ$}}

\put(60,60){\makebox(0,0)[cc]{\EQLS}}

\put(96.25,65){\makebox(0,0)[cr]{$\Code$}}

\put(105,117.5){\makebox(0,0)[cl]{$\Cee$}}

\put(95,2.5){\makebox(0,0)[cr]{$\Bee$}}

\put(100,40){\makebox(0,0)[cc]{$\Dott$}}

\put(20,150){\makebox(0,0)[cc]{$\fleft$}}

\put(100,150){\makebox(0,0)[cc]{$\fmid$}}

\put(190,150){\makebox(0,0)[cc]{$\fright$}}

\put(140,150){\makebox(0,0)[cc]{\EQLS}}

\put(60,150){\makebox(0,0)[cc]{\EQLS}}

\put(90,30){\makebox(0,0)[cc]{$\Fei$}}

\end{picture}


==> PIC/exec-tight.tex <==
%%Created by jPicEdt 1.4.1_03: mixed JPIC-XML/LaTeX format
%%Tue May 24 19:53:27 GMT+01:00 2022
%%Begin JPIC-XML
%<?xml version="1.0" standalone="yes"?>
%<jpic x-min="0" x-max="200" y-min="0" y-max="185" auto-bounding="true">
%<multicurve fill-style= "none"
%	 points= "(80,60);(80,60);(80,20);(80,20)"
%	 stroke-width= "0.4"
%	 />
%<multicurve fill-style= "none"
%	 points= "(80,20);(80,20);(0,20);(0,20)"
%	 stroke-width= "0.4"
%	 />
%<multicurve fill-style= "none"
%	 points= "(0,60);(0,60);(80,60);(80,60)"
%	 stroke-width= "0.4"
%	 />
%<multicurve fill-style= "none"
%	 points= "(60,20);(60,20);(60,0);(60,0)"
%	 stroke-width= "0.4"
%	 />
%<multicurve fill-style= "none"
%	 points= "(60,135);(60,135);(60,60);(60,60)"
%	 stroke-width= "0.4"
%	 />
%<multicurve fill-style= "none"
%	 points= "(0,60);(0,60);(0,20);(0,20)"
%	 stroke-width= "0.4"
%	 />
%<multicurve fill-style= "none"
%	 points= "(20,20);(20,20);(20,0);(20,0)"
%	 stroke-width= "0.4"
%	 />
%<multicurve fill-style= "none"
%	 points= "(200,80);(200,80);(200,40);(200,40)"
%	 stroke-width= "0.4"
%	 />
%<multicurve fill-style= "none"
%	 points= "(160,20);(160,20);(120,20);(120,20)"
%	 stroke-width= "0.4"
%	 />
%<multicurve fill-style= "none"
%	 points= "(160,80);(160,80);(200,80);(200,80)"
%	 stroke-width= "0.4"
%	 />
%<multicurve fill-style= "none"
%	 points= "(180,40);(180,40);(180,0);(180,0)"
%	 stroke-width= "0.4"
%	 />
%<multicurve fill-style= "none"
%	 points= "(180,135);(180,135);(180,80);(180,80)"
%	 stroke-width= "0.4"
%	 />
%<multicurve fill-style= "none"
%	 points= "(120,60);(120,60);(120,20);(120,20)"
%	 stroke-width= "0.4"
%	 />
%<multicurve fill-style= "none"
%	 points= "(140,20);(140,20);(140,0);(140,0)"
%	 stroke-width= "0.4"
%	 />
%<multicurve fill-style= "none"
%	 points= "(200,40);(200,40);(160,40);(160,40)"
%	 stroke-width= "0.4"
%	 />
%<multicurve fill-style= "none"
%	 points= "(120,80);(120,80);(160,40);(160,40)"
%	 stroke-width= "0.4"
%	 />
%<multicurve fill-style= "none"
%	 points= "(120,60);(120,60);(160,20);(160,20)"
%	 stroke-width= "0.4"
%	 />
%<multicurve fill-style= "none"
%	 points= "(140,40);(140,40);(140,60);(140,60)"
%	 stroke-width= "1.45"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(170,60)"
%	 text-frame= "noframe"
%	 stroke-width= "0.4"
%	 text-hor-align= "center-h"
%	 >
%$\Univ$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(100,40)"
%	 text-frame= "noframe"
%	 stroke-width= "0.4"
%	 text-hor-align= "center-h"
%	 >
%\EQLS
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(135,56.25)"
%	 text-frame= "noframe"
%	 stroke-width= "0.4"
%	 text-hor-align= "right"
%	 >
%$\Code$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(185,130)"
%	 text-frame= "noframe"
%	 stroke-width= "0.4"
%	 text-hor-align= "left"
%	 >
%$\Cee$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(65,130)"
%	 text-frame= "noframe"
%	 stroke-width= "0.4"
%	 text-hor-align= "left"
%	 >
%$\Cee$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(15,2.5)"
%	 text-frame= "noframe"
%	 stroke-width= "0.4"
%	 text-hor-align= "right"
%	 >
%$\Aee$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(55,2.5)"
%	 text-frame= "noframe"
%	 stroke-width= "0.4"
%	 text-hor-align= "right"
%	 >
%$\Bee$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(40,40)"
%	 text-frame= "noframe"
%	 stroke-width= "0.4"
%	 text-hor-align= "center-h"
%	 >
%$\fee$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(130,31.25)"
%	 text-frame= "noframe"
%	 stroke-width= "0.4"
%	 text-hor-align= "center-h"
%	 >
%$\Fee$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(135,2.5)"
%	 text-frame= "noframe"
%	 stroke-width= "0.4"
%	 text-hor-align= "right"
%	 >
%$\Aee$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(175,2.5)"
%	 text-frame= "noframe"
%	 stroke-width= "0.4"
%	 text-hor-align= "right"
%	 >
%$\Bee$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(100,185)"
%	 text-frame= "noframe"
%	 stroke-width= "0.4"
%	 text-hor-align= "center-h"
%	 >
%\EQLS
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(60,185)"
%	 text-frame= "noframe"
%	 stroke-width= "0.4"
%	 text-hor-align= "center-h"
%	 >
%$\LHS$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(180,185)"
%	 text-frame= "noframe"
%	 stroke-width= "0.4"
%	 text-hor-align= "center-h"
%	 >
%$\RHS$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(140,40)"
%	 text-frame= "noframe"
%	 stroke-width= "0.4"
%	 text-hor-align= "center-h"
%	 >
%$\Dott$
%</text>
%<multicurve fill-style= "none"
%	 points= "(20,80);(20,80);(20,60);(20,60)"
%	 stroke-width= "0.4"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(25,70)"
%	 text-frame= "noframe"
%	 stroke-width= "0.4"
%	 text-hor-align= "left"
%	 >
%$\Aee$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(20,165)"
%	 text-frame= "noframe"
%	 stroke-width= "0.4"
%	 text-hor-align= "center-h"
%	 >
%$\LHSP$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(140,165)"
%	 text-frame= "noframe"
%	 stroke-width= "0.4"
%	 text-hor-align= "center-h"
%	 >
%$\RHSP$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(100,165)"
%	 text-frame= "noframe"
%	 stroke-width= "0.4"
%	 text-hor-align= "center-h"
%	 >
%\EQLS
%</text>
%<multicurve fill-style= "none"
%	 points= "(40,80);(40,80);(0,80);(0,80)"
%	 stroke-width= "0.4"
%	 />
%<multicurve fill-style= "none"
%	 points= "(0,120);(0,120);(0,80);(0,80)"
%	 stroke-width= "0.4"
%	 />
%<multicurve fill-style= "none"
%	 points= "(20,100);(20,100);(20,135);(20,135)"
%	 stroke-width= "1.45"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(10,91.25)"
%	 text-frame= "noframe"
%	 stroke-width= "0.4"
%	 text-hor-align= "center-h"
%	 >
%$\Fee$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(20,100)"
%	 text-frame= "noframe"
%	 stroke-width= "0.4"
%	 text-hor-align= "center-h"
%	 >
%$\Dott$
%</text>
%<multicurve fill-style= "none"
%	 points= "(0,120);(0,120);(40,80);(40,80)"
%	 stroke-width= "0.4"
%	 />
%<multicurve fill-style= "none"
%	 points= "(120,120);(120,120);(160,80);(160,80)"
%	 stroke-width= "0.4"
%	 />
%<multicurve fill-style= "none"
%	 points= "(120,120);(120,120);(120,80);(120,80)"
%	 stroke-width= "0.4"
%	 />
%<multicurve fill-style= "none"
%	 points= "(140,100);(140,100);(140,135);(140,135)"
%	 stroke-width= "1.45"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(145,130)"
%	 text-frame= "noframe"
%	 stroke-width= "0.4"
%	 text-hor-align= "left"
%	 >
%$\Code$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(25,130)"
%	 text-frame= "noframe"
%	 stroke-width= "0.4"
%	 text-hor-align= "left"
%	 >
%$\Code$
%</text>
%</jpic>
%%End JPIC-XML
%PSTricks content-type (pstricks.sty package needed)
%Add \usepackage{pstricks} in the preamble of your LaTeX file
%You can rescale the whole picture (to 80% for instance) by using the command \def\JPicScale{0.8}
\ifx\JPicScale\undefined\def\JPicScale{1}\fi
\psset{unit=\JPicScale mm}
\psset{linewidth=0.3,dotsep=1,hatchwidth=0.3,hatchsep=1.5,shadowsize=1,dimen=middle}
\psset{dotsize=0.7 2.5,dotscale=1 1,fillcolor=black}
\psset{arrowsize=1 2,arrowlength=1,arrowinset=0.25,tbarsize=0.7 5,bracketlength=0.15,rbracketlength=0.15}
\begin{pspicture}(0,0)(200,185)
\psline[linewidth=0.4](80,60)(80,20)
\psline[linewidth=0.4](80,20)(0,20)
\psline[linewidth=0.4](0,60)(80,60)
\psline[linewidth=0.4](60,20)(60,0)
\psline[linewidth=0.4](60,135)(60,60)
\psline[linewidth=0.4](0,60)(0,20)
\psline[linewidth=0.4](20,20)(20,0)
\psline[linewidth=0.4](200,80)(200,40)
\psline[linewidth=0.4](160,20)(120,20)
\psline[linewidth=0.4](160,80)(200,80)
\psline[linewidth=0.4](180,40)(180,0)
\psline[linewidth=0.4](180,135)(180,80)
\psline[linewidth=0.4](120,60)(120,20)
\psline[linewidth=0.4](140,20)(140,0)
\psline[linewidth=0.4](200,40)(160,40)
\psline[linewidth=0.4](120,80)(160,40)
\psline[linewidth=0.4](120,60)(160,20)
\psline[linewidth=1.45](140,40)(140,60)
\rput(170,60){$\Univ$}
\rput(100,40){\EQLS}
\rput[r](135,56.25){$\Code$}
\rput[l](185,130){$\Cee$}
\rput[l](65,130){$\Cee$}
\rput[r](15,2.5){$\Aee$}
\rput[r](55,2.5){$\Bee$}
\rput(40,40){$\fee$}
\rput(130,31.25){$\Fee$}
\rput[r](135,2.5){$\Aee$}
\rput[r](175,2.5){$\Bee$}
\rput(100,185){\EQLS}
\rput(60,185){$\LHS$}
\rput(180,185){$\RHS$}
\rput(140,40){$\Dott$}
\psline[linewidth=0.4](20,80)(20,60)
\rput[l](25,70){$\Aee$}
\rput(20,165){$\LHSP$}
\rput(140,165){$\RHSP$}
\rput(100,165){\EQLS}
\psline[linewidth=0.4](40,80)(0,80)
\psline[linewidth=0.4](0,120)(0,80)
\psline[linewidth=1.45](20,100)(20,135)
\rput(10,91.25){$\Fee$}
\rput(20,100){$\Dott$}
\psline[linewidth=0.4](0,120)(40,80)
\psline[linewidth=0.4](120,120)(160,80)
\psline[linewidth=0.4](120,120)(120,80)
\psline[linewidth=1.45](140,100)(140,135)
\rput[l](145,130){$\Code$}
\rput[l](25,130){$\Code$}
\end{pspicture}


==> PIC/exec.tex <==
%%Created by jPicEdt 1.4.1_03: mixed JPIC-XML/LaTeX format
%%Sun May 22 18:25:54 GMT+01:00 2022
%%Begin JPIC-XML
%<?xml version="1.0" standalone="yes"?>
%<jpic x-min="0" x-max="200" y-min="0" y-max="205" auto-bounding="true">
%<multicurve fill-style= "none"
%	 stroke-width= "0.4"
%	 points= "(80,80);(80,80);(80,40);(80,40)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.4"
%	 points= "(80,40);(80,40);(0,40);(0,40)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.4"
%	 points= "(0,80);(0,80);(80,80);(80,80)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.4"
%	 points= "(60,40);(60,40);(60,0);(60,0)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.4"
%	 points= "(60,160);(60,160);(60,80);(60,80)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.4"
%	 points= "(0,80);(0,80);(0,40);(0,40)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.4"
%	 points= "(20,40);(20,40);(20,0);(20,0)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.4"
%	 points= "(200,100);(200,100);(200,60);(200,60)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.4"
%	 points= "(160,20);(160,20);(120,20);(120,20)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.4"
%	 points= "(160,100);(160,100);(200,100);(200,100)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.4"
%	 points= "(180,60);(180,60);(180,0);(180,0)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.4"
%	 points= "(180,160);(180,160);(180,100);(180,100)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.4"
%	 points= "(120,60);(120,60);(120,20);(120,20)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.4"
%	 points= "(140,20);(140,20);(140,0);(140,0)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.4"
%	 points= "(200,60);(200,60);(160,60);(160,60)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.4"
%	 points= "(120,100);(120,100);(160,60);(160,60)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.4"
%	 points= "(120,60);(120,60);(160,20);(160,20)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "1.45"
%	 points= "(140,40);(140,40);(140,80);(140,80)"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 stroke-width= "0.4"
%	 anchor-point= "(170,80)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\Univ$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 stroke-width= "0.4"
%	 anchor-point= "(100,60)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\EQLS
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 stroke-width= "0.4"
%	 anchor-point= "(136.25,65)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\Code$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 stroke-width= "0.4"
%	 anchor-point= "(185,155)"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\Cee$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 stroke-width= "0.4"
%	 anchor-point= "(65,155)"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\Cee$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 stroke-width= "0.4"
%	 anchor-point= "(15,2.5)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\Aee$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 stroke-width= "0.4"
%	 anchor-point= "(55,2.5)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\Bee$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 stroke-width= "0.4"
%	 anchor-point= "(40,60)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\fee$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 stroke-width= "0.4"
%	 anchor-point= "(130,31.25)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\Fee$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 stroke-width= "0.4"
%	 anchor-point= "(135,2.5)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\Aee$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 stroke-width= "0.4"
%	 anchor-point= "(175,2.5)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\Bee$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 stroke-width= "0.4"
%	 anchor-point= "(100,205)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\EQLS
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 stroke-width= "0.4"
%	 anchor-point= "(60,205)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\LHS$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 stroke-width= "0.4"
%	 anchor-point= "(180,205)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\RHS$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 stroke-width= "0.4"
%	 anchor-point= "(140,40)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\Dott$
%</text>
%<multicurve fill-style= "none"
%	 stroke-width= "0.4"
%	 points= "(20,100);(20,100);(20,80);(20,80)"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 stroke-width= "0.4"
%	 anchor-point= "(25,90)"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\Aee$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 stroke-width= "0.4"
%	 anchor-point= "(20,185)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\LHSP$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 stroke-width= "0.4"
%	 anchor-point= "(140,185)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\RHSP$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 stroke-width= "0.4"
%	 anchor-point= "(100,185)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\EQLS
%</text>
%<multicurve fill-style= "none"
%	 stroke-width= "0.4"
%	 points= "(40,100);(40,100);(0,100);(0,100)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.4"
%	 points= "(0,140);(0,140);(0,100);(0,100)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "1.45"
%	 points= "(20,120);(20,120);(20,160);(20,160)"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 stroke-width= "0.4"
%	 anchor-point= "(10,111.25)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\Fee$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 stroke-width= "0.4"
%	 anchor-point= "(20,120)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\Dott$
%</text>
%<multicurve fill-style= "none"
%	 stroke-width= "0.4"
%	 points= "(0,140);(0,140);(40,100);(40,100)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.4"
%	 points= "(120,140);(120,140);(160,100);(160,100)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.4"
%	 points= "(120,140);(120,140);(120,100);(120,100)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "1.45"
%	 points= "(140,120);(140,120);(140,160);(140,160)"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 stroke-width= "0.4"
%	 anchor-point= "(145,155)"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\Code$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 stroke-width= "0.4"
%	 anchor-point= "(25,155)"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\Code$
%</text>
%</jpic>
%%End JPIC-XML
%PSTricks content-type (pstricks.sty package needed)
%Add \usepackage{pstricks} in the preamble of your LaTeX file
%You can rescale the whole picture (to 80% for instance) by using the command \def\JPicScale{0.8}
\ifx\JPicScale\undefined\def\JPicScale{1}\fi
\psset{unit=\JPicScale mm}
\psset{linewidth=0.3,dotsep=1,hatchwidth=0.3,hatchsep=1.5,shadowsize=1,dimen=middle}
\psset{dotsize=0.7 2.5,dotscale=1 1,fillcolor=black}
\psset{arrowsize=1 2,arrowlength=1,arrowinset=0.25,tbarsize=0.7 5,bracketlength=0.15,rbracketlength=0.15}
\begin{pspicture}(0,0)(200,205)
\psline[linewidth=0.4](80,80)(80,40)
\psline[linewidth=0.4](80,40)(0,40)
\psline[linewidth=0.4](0,80)(80,80)
\psline[linewidth=0.4](60,40)(60,0)
\psline[linewidth=0.4](60,160)(60,80)
\psline[linewidth=0.4](0,80)(0,40)
\psline[linewidth=0.4](20,40)(20,0)
\psline[linewidth=0.4](200,100)(200,60)
\psline[linewidth=0.4](160,20)(120,20)
\psline[linewidth=0.4](160,100)(200,100)
\psline[linewidth=0.4](180,60)(180,0)
\psline[linewidth=0.4](180,160)(180,100)
\psline[linewidth=0.4](120,60)(120,20)
\psline[linewidth=0.4](140,20)(140,0)
\psline[linewidth=0.4](200,60)(160,60)
\psline[linewidth=0.4](120,100)(160,60)
\psline[linewidth=0.4](120,60)(160,20)
\psline[linewidth=1.45](140,40)(140,80)
\rput(170,80){$\Univ$}
\rput(100,60){\EQLS}
\rput[r](136.25,65){$\Code$}
\rput[l](185,155){$\Cee$}
\rput[l](65,155){$\Cee$}
\rput[r](15,2.5){$\Aee$}
\rput[r](55,2.5){$\Bee$}
\rput(40,60){$\fee$}
\rput(130,31.25){$\Fee$}
\rput[r](135,2.5){$\Aee$}
\rput[r](175,2.5){$\Bee$}
\rput(100,205){\EQLS}
\rput(60,205){$\LHS$}
\rput(180,205){$\RHS$}
\rput(140,40){$\Dott$}
\psline[linewidth=0.4](20,100)(20,80)
\rput[l](25,90){$\Aee$}
\rput(20,185){$\LHSP$}
\rput(140,185){$\RHSP$}
\rput(100,185){\EQLS}
\psline[linewidth=0.4](40,100)(0,100)
\psline[linewidth=0.4](0,140)(0,100)
\psline[linewidth=1.45](20,120)(20,160)
\rput(10,111.25){$\Fee$}
\rput(20,120){$\Dott$}
\psline[linewidth=0.4](0,140)(40,100)
\psline[linewidth=0.4](120,140)(160,100)
\psline[linewidth=0.4](120,140)(120,100)
\psline[linewidth=1.45](140,120)(140,160)
\rput[l](145,155){$\Code$}
\rput[l](25,155){$\Code$}
\end{pspicture}


==> PIC/f.tex <==
%%Created by jPicEdt 1.4.1_03: mixed JPIC-XML/LaTeX format
%%Wed Sep 28 19:51:42 HST 2016
%%Begin JPIC-XML
%<?xml version="1.0" standalone="yes"?>
%<jpic x-min="0" x-max="40" y-min="1.25" y-max="71.25" auto-bounding="true">
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(0,47.5);(0,47.5);(40,47.5);(40,47.5)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(0,47.5);(0,47.5);(0,22.5);(0,22.5)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(40,22.5);(40,22.5);(40,47.5);(40,47.5)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(20,65);(20,65);(20,47.5);(20,47.5)"
%	 />
%<text stroke-width= "0.75"
%	 text-vert-align= "center-v"
%	 anchor-point= "(20,71.25)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\nameslang$
%</text>
%<text stroke-width= "0.75"
%	 text-vert-align= "center-v"
%	 anchor-point= "(20,1.25)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\inputt$
%</text>
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(0,22.5);(0,22.5);(40,22.5);(40,22.5)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(20,22.5);(20,22.5);(20,7.5);(20,7.5)"
%	 />
%<text stroke-width= "0.75"
%	 text-vert-align= "center-v"
%	 anchor-point= "(20,35)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\machine
%</text>
%</jpic>
%%End JPIC-XML
%PSTricks content-type (pstricks.sty package needed)
%Add \usepackage{pstricks} in the preamble of your LaTeX file
%You can rescale the whole picture (to 80% for instance) by using the command \def\JPicScale{0.8}
\ifx\JPicScale\undefined\def\JPicScale{1}\fi
\psset{unit=\JPicScale mm}
\psset{linewidth=0.3,dotsep=1,hatchwidth=0.3,hatchsep=1.5,shadowsize=1,dimen=middle}
\psset{dotsize=0.7 2.5,dotscale=1 1,fillcolor=black}
\psset{arrowsize=1 2,arrowlength=1,arrowinset=0.25,tbarsize=0.7 5,bracketlength=0.15,rbracketlength=0.15}
\begin{pspicture}(0,0)(40,71.25)
\psline[linewidth=0.75](0,47.5)(40,47.5)
\psline[linewidth=0.75](0,47.5)(0,22.5)
\psline[linewidth=0.75](40,22.5)(40,47.5)
\psline[linewidth=0.75](20,65)(20,47.5)
\rput(20,71.25){$\nameslang$}
\rput(20,1.25){$\inputt$}
\psline[linewidth=0.75](0,22.5)(40,22.5)
\psline[linewidth=0.75](20,22.5)(20,7.5)
\rput(20,35){\machine}
\end{pspicture}


==> PIC/fixp-1.tex <==
%%Created by jPicEdt 1.4.1_03: mixed JPIC-XML/LaTeX format
%%Wed Dec 02 13:17:48 GMT-10:00 2020
%%Begin JPIC-XML
%<?xml version="1.0" standalone="yes"?>
%<jpic x-min="0" x-max="515" y-min="-5" y-max="165" auto-bounding="true">
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(30,130)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\gee$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(122.5,165)"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\nameslang$
%</text>
%<multicurve fill-style= "none"
%	 points= "(110,110);(110,110);(140,110);(140,110)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(90,130);(90,130);(110,110);(110,110)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(120,110);(120,110);(120,10);(120,10)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(100,120);(100,120);(100,90);(100,90)"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(120,130)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\universal
%</text>
%<multicurve fill-style= "none"
%	 points= "(90,150);(90,150);(140,150);(140,150)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(90,150);(90,150);(90,130);(90,130)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(120,165);(120,165);(120,150);(120,150)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(140,110);(140,110);(140,150);(140,150)"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(70,130)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\EQLS
%</text>
%<multicurve fill-style= "none"
%	 points= "(90,100);(90,100);(90,80);(90,80)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(90,80);(90,80);(110,80);(110,80)"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(96.25,86.25)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\program
%</text>
%<multicurve fill-style= "none"
%	 points= "(90,100);(90,100);(110,80);(110,80)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(50,110);(50,110);(50,150);(50,150)"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(32.5,165)"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\nameslang$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(27.5,100)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\inputt$
%</text>
%<multicurve fill-style= "none"
%	 points= "(10,110);(10,110);(50,110);(50,110)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(30,110);(30,110);(30,90);(30,90)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(0,70);(0,70);(0,90);(0,90)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(50,50);(50,50);(20,50);(20,50)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(0,90);(0,90);(50,90);(50,90)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(0,70);(0,70);(20,50);(20,50)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(30,50);(30,50);(30,45);(30,45)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(10,60);(10,60);(10,10);(10,10)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(30,45);(30,45);(10,25);(10,25)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(10,150);(10,150);(50,150);(50,150)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(10,150);(10,150);(10,110);(10,110)"
%	 />
%<ellipse p3= "(12.5,22.5)"
%	 fill-style= "solid"
%	 p2= "(12.5,27.5)"
%	 fill-color= "#333333"
%	 p1= "(7.5,27.5)"
%	 closure= "open"
%	 angle-end= "0"
%	 stroke-overstrike= "true"
%	 stroke-width= "1.3"
%	 angle-start= "0"
%	 />
%<multicurve fill-style= "none"
%	 points= "(30,165);(30,165);(30,150);(30,150)"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(117.5,10)"
%	 text-frame= "noframe"
%	 stroke-width= "0.35"
%	 text-hor-align= "right"
%	 >
%$\progtype$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(97.5,110)"
%	 text-frame= "noframe"
%	 stroke-width= "0.35"
%	 text-hor-align= "right"
%	 >
%$\progtype$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(7.5,10)"
%	 text-frame= "noframe"
%	 stroke-width= "0.35"
%	 text-hor-align= "right"
%	 >
%$\progtype$
%</text>
%<multicurve fill-style= "none"
%	 points= "(50,50);(50,50);(50,90);(50,90)"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(30,68.75)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\universal
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(310,130)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\gee$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(402.5,165)"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\nameslang$
%</text>
%<multicurve fill-style= "none"
%	 points= "(390,110);(390,110);(420,110);(420,110)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(370,130);(370,130);(390,110);(390,110)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(400,110);(400,110);(400,10);(400,10)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(380,120);(380,120);(380,90);(380,90)"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(400,130)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\universal
%</text>
%<multicurve fill-style= "none"
%	 points= "(370,150);(370,150);(420,150);(420,150)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(370,150);(370,150);(370,130);(370,130)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(400,165);(400,165);(400,150);(400,150)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(420,110);(420,110);(420,150);(420,150)"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(350,130)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\EQLS
%</text>
%<multicurve fill-style= "none"
%	 points= "(370,100);(370,100);(370,80);(370,80)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(370,80);(370,80);(390,80);(390,80)"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(376.25,86.25)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\program
%</text>
%<multicurve fill-style= "none"
%	 points= "(370,100);(370,100);(390,80);(390,80)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(330,110);(330,110);(330,150);(330,150)"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(312.5,165)"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\nameslang$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(307.5,102.5)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\inputt$
%</text>
%<multicurve fill-style= "none"
%	 points= "(290,110);(290,110);(330,110);(330,110)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(310,110);(310,110);(310,90);(310,90)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(280,70);(280,70);(280,90);(280,90)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(330,50);(330,50);(300,50);(300,50)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(280,90);(280,90);(330,90);(330,90)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(280,70);(280,70);(300,50);(300,50)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(310,50);(310,50);(310,45);(310,45)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(290,60);(290,60);(290,10);(290,10)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(310,45);(310,45);(290,25);(290,25)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(290,150);(290,150);(330,150);(330,150)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(290,150);(290,150);(290,110);(290,110)"
%	 />
%<ellipse p3= "(292.5,22.5)"
%	 fill-style= "solid"
%	 p2= "(292.5,27.5)"
%	 fill-color= "#333333"
%	 p1= "(287.5,27.5)"
%	 closure= "open"
%	 angle-end= "0"
%	 stroke-overstrike= "true"
%	 stroke-width= "1.3"
%	 angle-start= "0"
%	 />
%<multicurve fill-style= "none"
%	 points= "(310,165);(310,165);(310,150);(310,150)"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(377.5,110)"
%	 text-frame= "noframe"
%	 stroke-width= "0.35"
%	 text-hor-align= "right"
%	 >
%$\progtype$
%</text>
%<multicurve fill-style= "none"
%	 points= "(330,50);(330,50);(330,90);(330,90)"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(310,68.75)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\universal
%</text>
%<multicurve fill-style= "none"
%	 points= "(390,20);(390,20);(390,0);(390,0)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(390,0);(390,0);(410,0);(410,0)"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(396.25,6.25)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\program
%</text>
%<multicurve fill-style= "none"
%	 points= "(390,20);(390,20);(410,0);(410,0)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(280,20);(280,20);(280,0);(280,0)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(280,0);(280,0);(300,0);(300,0)"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(286.25,6.25)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\program
%</text>
%<multicurve fill-style= "none"
%	 points= "(280,20);(280,20);(300,0);(300,0)"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(397.5,40)"
%	 text-frame= "noframe"
%	 stroke-width= "0.35"
%	 text-hor-align= "right"
%	 >
%$\progtype$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(492.5,165)"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\nameslang$
%</text>
%<multicurve fill-style= "none"
%	 points= "(480,110);(480,110);(510,110);(510,110)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(460,130);(460,130);(480,110);(480,110)"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(490,130)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\universal
%</text>
%<multicurve fill-style= "none"
%	 points= "(460,150);(460,150);(510,150);(510,150)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(460,150);(460,150);(460,130);(460,130)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(490,165);(490,165);(490,150);(490,150)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(510,110);(510,110);(510,150);(510,150)"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(440,130)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\EQLS
%</text>
%<multicurve fill-style= "none"
%	 points= "(490,110);(490,110);(490,105);(490,105)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(470,120);(470,120);(470,70);(470,70)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(490,105);(490,105);(470,85);(470,85)"
%	 />
%<ellipse p3= "(472.5,82.5)"
%	 fill-style= "solid"
%	 p2= "(472.5,87.5)"
%	 fill-color= "#333333"
%	 p1= "(467.5,87.5)"
%	 closure= "open"
%	 angle-end= "0"
%	 stroke-overstrike= "true"
%	 stroke-width= "1.3"
%	 angle-start= "0"
%	 />
%<multicurve fill-style= "none"
%	 points= "(460,80);(460,80);(460,60);(460,60)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(460,60);(460,60);(480,60);(480,60)"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(465,66.25)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\program
%</text>
%<multicurve fill-style= "none"
%	 points= "(460,80);(460,80);(480,60);(480,60)"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(215,130)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\thennn
%</text>
%<multicurve fill-style= "none"
%	 points= "(275,95);(275,95);(335,95);(335,95)"
%	 stroke-width= "0.15"
%	 />
%<multicurve fill-style= "none"
%	 points= "(275,-5);(275,-5);(275,95);(275,95)"
%	 stroke-width= "0.15"
%	 />
%<multicurve fill-style= "none"
%	 points= "(335,25);(335,25);(335,95);(335,95)"
%	 stroke-width= "0.15"
%	 />
%<multicurve fill-style= "none"
%	 points= "(305,-5);(305,-5);(335,25);(335,25)"
%	 stroke-width= "0.15"
%	 />
%<multicurve fill-style= "none"
%	 points= "(275,-5);(275,-5);(305,-5);(305,-5)"
%	 stroke-width= "0.15"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(310,20)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\aahh$
%</text>
%<multicurve fill-style= "none"
%	 points= "(455,155);(455,155);(515,155);(515,155)"
%	 stroke-width= "0.15"
%	 />
%<multicurve fill-style= "none"
%	 points= "(455,55);(455,55);(455,155);(455,155)"
%	 stroke-width= "0.15"
%	 />
%<multicurve fill-style= "none"
%	 points= "(515,85);(515,85);(515,155);(515,155)"
%	 stroke-width= "0.15"
%	 />
%<multicurve fill-style= "none"
%	 points= "(485,55);(485,55);(515,85);(515,85)"
%	 stroke-width= "0.15"
%	 />
%<multicurve fill-style= "none"
%	 points= "(455,55);(455,55);(485,55);(485,55)"
%	 stroke-width= "0.15"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(490,80)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\aahh$
%</text>
%</jpic>
%%End JPIC-XML
%LaTeX-picture environment using emulated lines and arcs
%You can rescale the whole picture (to 80% for instance) by using the command \def\JPicScale{0.8}
\ifx\JPicScale\undefined\def\JPicScale{1}\fi
\unitlength \JPicScale mm
\begin{picture}(515,165)(0,0)
\put(30,130){\makebox(0,0)[cc]{$\gee$}}

\put(122.5,165){\makebox(0,0)[cl]{$\nameslang$}}

\linethickness{0.3mm}
\put(110,110){\line(1,0){30}}
\linethickness{0.3mm}
\multiput(90,130)(0.12,-0.12){167}{\line(1,0){0.12}}
\linethickness{0.3mm}
\put(120,10){\line(0,1){100}}
\linethickness{0.3mm}
\put(100,90){\line(0,1){30}}
\put(120,130){\makebox(0,0)[cc]{\universal}}

\linethickness{0.3mm}
\put(90,150){\line(1,0){50}}
\linethickness{0.3mm}
\put(90,130){\line(0,1){20}}
\linethickness{0.3mm}
\put(120,150){\line(0,1){15}}
\linethickness{0.3mm}
\put(140,110){\line(0,1){40}}
\put(70,130){\makebox(0,0)[cc]{\EQLS}}

\linethickness{0.3mm}
\put(90,80){\line(0,1){20}}
\linethickness{0.3mm}
\put(90,80){\line(1,0){20}}
\put(96.25,86.25){\makebox(0,0)[cc]{\program}}

\linethickness{0.3mm}
\multiput(90,100)(0.12,-0.12){167}{\line(1,0){0.12}}
\linethickness{0.3mm}
\put(50,110){\line(0,1){40}}
\put(32.5,165){\makebox(0,0)[cl]{$\nameslang$}}

\put(27.5,100){\makebox(0,0)[cr]{$\inputt$}}

\linethickness{0.3mm}
\put(10,110){\line(1,0){40}}
\linethickness{0.3mm}
\put(30,90){\line(0,1){20}}
\linethickness{0.3mm}
\put(0,70){\line(0,1){20}}
\linethickness{0.3mm}
\put(20,50){\line(1,0){30}}
\linethickness{0.3mm}
\put(0,90){\line(1,0){50}}
\linethickness{0.3mm}
\multiput(0,70)(0.12,-0.12){167}{\line(1,0){0.12}}
\linethickness{0.3mm}
\put(30,45){\line(0,1){5}}
\linethickness{0.3mm}
\put(10,10){\line(0,1){50}}
\linethickness{0.3mm}
\multiput(10,25)(0.12,0.12){167}{\line(1,0){0.12}}
\linethickness{0.3mm}
\put(10,150){\line(1,0){40}}
\linethickness{0.3mm}
\put(10,110){\line(0,1){40}}
\linethickness{1.3mm}
\put(10,25){\circle*{5}}

\linethickness{0.3mm}
\put(30,150){\line(0,1){15}}
\put(117.5,10){\makebox(0,0)[cr]{$\progtype$}}

\put(97.5,110){\makebox(0,0)[cr]{$\progtype$}}

\put(7.5,10){\makebox(0,0)[cr]{$\progtype$}}

\linethickness{0.3mm}
\put(50,50){\line(0,1){40}}
\put(30,68.75){\makebox(0,0)[cc]{\universal}}

\put(310,130){\makebox(0,0)[cc]{$\gee$}}

\put(402.5,165){\makebox(0,0)[cl]{$\nameslang$}}

\linethickness{0.3mm}
\put(390,110){\line(1,0){30}}
\linethickness{0.3mm}
\multiput(370,130)(0.12,-0.12){167}{\line(1,0){0.12}}
\linethickness{0.3mm}
\put(400,10){\line(0,1){100}}
\linethickness{0.3mm}
\put(380,90){\line(0,1){30}}
\put(400,130){\makebox(0,0)[cc]{\universal}}

\linethickness{0.3mm}
\put(370,150){\line(1,0){50}}
\linethickness{0.3mm}
\put(370,130){\line(0,1){20}}
\linethickness{0.3mm}
\put(400,150){\line(0,1){15}}
\linethickness{0.3mm}
\put(420,110){\line(0,1){40}}
\put(350,130){\makebox(0,0)[cc]{\EQLS}}

\linethickness{0.3mm}
\put(370,80){\line(0,1){20}}
\linethickness{0.3mm}
\put(370,80){\line(1,0){20}}
\put(376.25,86.25){\makebox(0,0)[cc]{\program}}

\linethickness{0.3mm}
\multiput(370,100)(0.12,-0.12){167}{\line(1,0){0.12}}
\linethickness{0.3mm}
\put(330,110){\line(0,1){40}}
\put(312.5,165){\makebox(0,0)[cl]{$\nameslang$}}

\put(307.5,102.5){\makebox(0,0)[cr]{$\inputt$}}

\linethickness{0.3mm}
\put(290,110){\line(1,0){40}}
\linethickness{0.3mm}
\put(310,90){\line(0,1){20}}
\linethickness{0.3mm}
\put(280,70){\line(0,1){20}}
\linethickness{0.3mm}
\put(300,50){\line(1,0){30}}
\linethickness{0.3mm}
\put(280,90){\line(1,0){50}}
\linethickness{0.3mm}
\multiput(280,70)(0.12,-0.12){167}{\line(1,0){0.12}}
\linethickness{0.3mm}
\put(310,45){\line(0,1){5}}
\linethickness{0.3mm}
\put(290,10){\line(0,1){50}}
\linethickness{0.3mm}
\multiput(290,25)(0.12,0.12){167}{\line(1,0){0.12}}
\linethickness{0.3mm}
\put(290,150){\line(1,0){40}}
\linethickness{0.3mm}
\put(290,110){\line(0,1){40}}
\linethickness{1.3mm}
\put(290,25){\circle*{5}}

\linethickness{0.3mm}
\put(310,150){\line(0,1){15}}
\put(377.5,110){\makebox(0,0)[cr]{$\progtype$}}

\linethickness{0.3mm}
\put(330,50){\line(0,1){40}}
\put(310,68.75){\makebox(0,0)[cc]{\universal}}

\linethickness{0.3mm}
\put(390,0){\line(0,1){20}}
\linethickness{0.3mm}
\put(390,0){\line(1,0){20}}
\put(396.25,6.25){\makebox(0,0)[cc]{\program}}

\linethickness{0.3mm}
\multiput(390,20)(0.12,-0.12){167}{\line(1,0){0.12}}
\linethickness{0.3mm}
\put(280,0){\line(0,1){20}}
\linethickness{0.3mm}
\put(280,0){\line(1,0){20}}
\put(286.25,6.25){\makebox(0,0)[cc]{\program}}

\linethickness{0.3mm}
\multiput(280,20)(0.12,-0.12){167}{\line(1,0){0.12}}
\put(397.5,40){\makebox(0,0)[cr]{$\progtype$}}

\put(492.5,165){\makebox(0,0)[cl]{$\nameslang$}}

\linethickness{0.3mm}
\put(480,110){\line(1,0){30}}
\linethickness{0.3mm}
\multiput(460,130)(0.12,-0.12){167}{\line(1,0){0.12}}
\put(490,130){\makebox(0,0)[cc]{\universal}}

\linethickness{0.3mm}
\put(460,150){\line(1,0){50}}
\linethickness{0.3mm}
\put(460,130){\line(0,1){20}}
\linethickness{0.3mm}
\put(490,150){\line(0,1){15}}
\linethickness{0.3mm}
\put(510,110){\line(0,1){40}}
\put(440,130){\makebox(0,0)[cc]{\EQLS}}

\linethickness{0.3mm}
\put(490,105){\line(0,1){5}}
\linethickness{0.3mm}
\put(470,70){\line(0,1){50}}
\linethickness{0.3mm}
\multiput(470,85)(0.12,0.12){167}{\line(1,0){0.12}}
\linethickness{1.3mm}
\put(470,85){\circle*{5}}

\linethickness{0.3mm}
\put(460,60){\line(0,1){20}}
\linethickness{0.3mm}
\put(460,60){\line(1,0){20}}
\put(465,66.25){\makebox(0,0)[cc]{\program}}

\linethickness{0.3mm}
\multiput(460,80)(0.12,-0.12){167}{\line(1,0){0.12}}
\put(215,130){\makebox(0,0)[cc]{\thennn}}

\linethickness{0.15mm}
\put(275,95){\line(1,0){60}}
\linethickness{0.15mm}
\put(275,-5){\line(0,1){100}}
\linethickness{0.15mm}
\put(335,25){\line(0,1){70}}
\linethickness{0.15mm}
\multiput(305,-5)(0.12,0.12){250}{\line(1,0){0.12}}
\linethickness{0.15mm}
\put(275,-5){\line(1,0){30}}
\put(310,20){\makebox(0,0)[cc]{$\aahh$}}

\linethickness{0.15mm}
\put(455,155){\line(1,0){60}}
\linethickness{0.15mm}
\put(455,55){\line(0,1){100}}
\linethickness{0.15mm}
\put(515,85){\line(0,1){70}}
\linethickness{0.15mm}
\multiput(485,55)(0.12,0.12){250}{\line(1,0){0.12}}
\linethickness{0.15mm}
\put(455,55){\line(1,0){30}}
\put(490,80){\makebox(0,0)[cc]{$\aahh$}}

\end{picture}


==> PIC/fixp-2.tex <==
%%Created by jPicEdt 1.4.1_03: mixed JPIC-XML/LaTeX format
%%Mon Dec 28 10:14:06 GMT-10:00 2020
%%Begin JPIC-XML
%<?xml version="1.0" standalone="yes"?>
%<jpic x-min="0" x-max="510" y-min="-5" y-max="165" auto-bounding="true">
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(30,130)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\gee$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(122.5,165)"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\nameslang$
%</text>
%<multicurve fill-style= "none"
%	 points= "(110,110);(110,110);(140,110);(140,110)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(90,130);(90,130);(110,110);(110,110)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(120,110);(120,110);(120,10);(120,10)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(100,120);(100,120);(100,90);(100,90)"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(120,130)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\universal
%</text>
%<multicurve fill-style= "none"
%	 points= "(90,150);(90,150);(140,150);(140,150)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(90,150);(90,150);(90,130);(90,130)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(120,165);(120,165);(120,150);(120,150)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(140,110);(140,110);(140,150);(140,150)"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(70,130)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\EQLS
%</text>
%<multicurve fill-style= "none"
%	 points= "(90,100);(90,100);(90,80);(90,80)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(90,80);(90,80);(110,80);(110,80)"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(96.25,86.25)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\program
%</text>
%<multicurve fill-style= "none"
%	 points= "(90,100);(90,100);(110,80);(110,80)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(50,110);(50,110);(50,150);(50,150)"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(32.5,165)"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\nameslang$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(27.5,100)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\inputt$
%</text>
%<multicurve fill-style= "none"
%	 points= "(10,110);(10,110);(50,110);(50,110)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(30,110);(30,110);(30,90);(30,90)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(0,70);(0,70);(0,90);(0,90)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(50,50);(50,50);(20,50);(20,50)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(0,90);(0,90);(50,90);(50,90)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(0,70);(0,70);(20,50);(20,50)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(30,50);(30,50);(30,45);(30,45)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(10,60);(10,60);(10,10);(10,10)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(30,45);(30,45);(10,25);(10,25)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(10,150);(10,150);(50,150);(50,150)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(10,150);(10,150);(10,110);(10,110)"
%	 />
%<ellipse p3= "(12.5,22.5)"
%	 fill-style= "solid"
%	 p2= "(12.5,27.5)"
%	 fill-color= "#333333"
%	 p1= "(7.5,27.5)"
%	 closure= "open"
%	 angle-end= "0"
%	 stroke-overstrike= "true"
%	 stroke-width= "1.3"
%	 angle-start= "0"
%	 />
%<multicurve fill-style= "none"
%	 points= "(30,165);(30,165);(30,150);(30,150)"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(117.5,10)"
%	 text-frame= "noframe"
%	 stroke-width= "0.35"
%	 text-hor-align= "right"
%	 >
%$\progtype$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(97.5,110)"
%	 text-frame= "noframe"
%	 stroke-width= "0.35"
%	 text-hor-align= "right"
%	 >
%$\progtype$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(7.5,10)"
%	 text-frame= "noframe"
%	 stroke-width= "0.35"
%	 text-hor-align= "right"
%	 >
%$\progtype$
%</text>
%<multicurve fill-style= "none"
%	 points= "(50,50);(50,50);(50,90);(50,90)"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(30,68.75)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\universal
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(485,130)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\gee$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(402.5,165)"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\nameslang$
%</text>
%<multicurve fill-style= "none"
%	 points= "(390,110);(390,110);(420,110);(420,110)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(370,130);(370,130);(390,110);(390,110)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(400,110);(400,110);(400,10);(400,10)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(380,120);(380,120);(380,90);(380,90)"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(400,130)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\universal
%</text>
%<multicurve fill-style= "none"
%	 points= "(370,150);(370,150);(420,150);(420,150)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(370,150);(370,150);(370,130);(370,130)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(400,165);(400,165);(400,150);(400,150)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(420,110);(420,110);(420,150);(420,150)"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(350,130)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\EQLS
%</text>
%<multicurve fill-style= "none"
%	 points= "(370,100);(370,100);(370,80);(370,80)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(370,80);(370,80);(390,80);(390,80)"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(376.25,86.25)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\program
%</text>
%<multicurve fill-style= "none"
%	 points= "(370,100);(370,100);(390,80);(390,80)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(505,110);(505,110);(505,150);(505,150)"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(487.5,165)"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\nameslang$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(482.5,102.5)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\inputt$
%</text>
%<multicurve fill-style= "none"
%	 points= "(465,110);(465,110);(505,110);(505,110)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(485,110);(485,110);(485,90);(485,90)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(455,70);(455,70);(455,90);(455,90)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(505,50);(505,50);(475,50);(475,50)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(455,90);(455,90);(505,90);(505,90)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(455,70);(455,70);(475,50);(475,50)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(485,50);(485,50);(485,45);(485,45)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(465,60);(465,60);(465,10);(465,10)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(485,45);(485,45);(465,25);(465,25)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(465,150);(465,150);(505,150);(505,150)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(465,150);(465,150);(465,110);(465,110)"
%	 />
%<ellipse p3= "(467.5,22.5)"
%	 fill-style= "solid"
%	 p2= "(467.5,27.5)"
%	 fill-color= "#333333"
%	 p1= "(462.5,27.5)"
%	 closure= "open"
%	 angle-end= "0"
%	 stroke-overstrike= "true"
%	 stroke-width= "1.3"
%	 angle-start= "0"
%	 />
%<multicurve fill-style= "none"
%	 points= "(485,165);(485,165);(485,150);(485,150)"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(377.5,110)"
%	 text-frame= "noframe"
%	 stroke-width= "0.35"
%	 text-hor-align= "right"
%	 >
%$\progtype$
%</text>
%<multicurve fill-style= "none"
%	 points= "(505,50);(505,50);(505,90);(505,90)"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(485,68.75)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\universal
%</text>
%<multicurve fill-style= "none"
%	 points= "(390,20);(390,20);(390,0);(390,0)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(390,0);(390,0);(410,0);(410,0)"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(396.25,6.25)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\program
%</text>
%<multicurve fill-style= "none"
%	 points= "(390,20);(390,20);(410,0);(410,0)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(455,20);(455,20);(455,0);(455,0)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(455,0);(455,0);(475,0);(475,0)"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(461.25,6.25)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\program
%</text>
%<multicurve fill-style= "none"
%	 points= "(455,20);(455,20);(475,0);(475,0)"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(397.5,40)"
%	 text-frame= "noframe"
%	 stroke-width= "0.35"
%	 text-hor-align= "right"
%	 >
%$\progtype$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(307.5,165)"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\nameslang$
%</text>
%<multicurve fill-style= "none"
%	 points= "(295,110);(295,110);(325,110);(325,110)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(275,130);(275,130);(295,110);(295,110)"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(305,130)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\universal
%</text>
%<multicurve fill-style= "none"
%	 points= "(275,150);(275,150);(325,150);(325,150)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(275,150);(275,150);(275,130);(275,130)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(305,165);(305,165);(305,150);(305,150)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(325,110);(325,110);(325,150);(325,150)"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(440,130)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\EQLS
%</text>
%<multicurve fill-style= "none"
%	 points= "(305,110);(305,110);(305,105);(305,105)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(285,120);(285,120);(285,70);(285,70)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(305,105);(305,105);(285,85);(285,85)"
%	 />
%<ellipse p3= "(287.5,82.5)"
%	 fill-style= "solid"
%	 p2= "(287.5,87.5)"
%	 fill-color= "#333333"
%	 p1= "(282.5,87.5)"
%	 closure= "open"
%	 angle-end= "0"
%	 stroke-overstrike= "true"
%	 stroke-width= "1.3"
%	 angle-start= "0"
%	 />
%<multicurve fill-style= "none"
%	 points= "(275,80);(275,80);(275,60);(275,60)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(275,60);(275,60);(295,60);(295,60)"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(280,66.25)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\program
%</text>
%<multicurve fill-style= "none"
%	 points= "(275,80);(275,80);(295,60);(295,60)"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(215,130)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\thennn
%</text>
%<multicurve fill-style= "none"
%	 points= "(450,95);(450,95);(510,95);(510,95)"
%	 stroke-width= "0.15"
%	 />
%<multicurve fill-style= "none"
%	 points= "(450,-5);(450,-5);(450,95);(450,95)"
%	 stroke-width= "0.15"
%	 />
%<multicurve fill-style= "none"
%	 points= "(510,25);(510,25);(510,95);(510,95)"
%	 stroke-width= "0.15"
%	 />
%<multicurve fill-style= "none"
%	 points= "(480,-5);(480,-5);(510,25);(510,25)"
%	 stroke-width= "0.15"
%	 />
%<multicurve fill-style= "none"
%	 points= "(450,-5);(450,-5);(480,-5);(480,-5)"
%	 stroke-width= "0.15"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(485,20)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\aahh$
%</text>
%<multicurve fill-style= "none"
%	 points= "(270,155);(270,155);(330,155);(330,155)"
%	 stroke-width= "0.15"
%	 />
%<multicurve fill-style= "none"
%	 points= "(270,55);(270,55);(270,155);(270,155)"
%	 stroke-width= "0.15"
%	 />
%<multicurve fill-style= "none"
%	 points= "(330,85);(330,85);(330,155);(330,155)"
%	 stroke-width= "0.15"
%	 />
%<multicurve fill-style= "none"
%	 points= "(300,55);(300,55);(330,85);(330,85)"
%	 stroke-width= "0.15"
%	 />
%<multicurve fill-style= "none"
%	 points= "(270,55);(270,55);(300,55);(300,55)"
%	 stroke-width= "0.15"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(305,80)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\aahh$
%</text>
%</jpic>
%%End JPIC-XML
%PSTricks content-type (pstricks.sty package needed)
%Add \usepackage{pstricks} in the preamble of your LaTeX file
%You can rescale the whole picture (to 80% for instance) by using the command \def\JPicScale{0.8}
\ifx\JPicScale\undefined\def\JPicScale{1}\fi
\psset{unit=\JPicScale mm}
\psset{linewidth=0.3,dotsep=1,hatchwidth=0.3,hatchsep=1.5,shadowsize=1,dimen=middle}
\psset{dotsize=0.7 2.5,dotscale=1 1,fillcolor=black}
\psset{arrowsize=1 2,arrowlength=1,arrowinset=0.25,tbarsize=0.7 5,bracketlength=0.15,rbracketlength=0.15}
\begin{pspicture}(0,0)(510,165)
\rput(30,130){$\gee$}
\rput[l](122.5,165){$\nameslang$}
\psline(110,110)(140,110)
\psline(90,130)(110,110)
\psline(120,110)(120,10)
\psline(100,120)(100,90)
\rput(120,130){\universal}
\psline(90,150)(140,150)
\psline(90,150)(90,130)
\psline(120,165)(120,150)
\psline(140,110)(140,150)
\rput(70,130){\EQLS}
\psline(90,100)(90,80)
\psline(90,80)(110,80)
\rput(96.25,86.25){\program}
\psline(90,100)(110,80)
\psline(50,110)(50,150)
\rput[l](32.5,165){$\nameslang$}
\rput[r](27.5,100){$\inputt$}
\psline(10,110)(50,110)
\psline(30,110)(30,90)
\psline(0,70)(0,90)
\psline(50,50)(20,50)
\psline(0,90)(50,90)
\psline(0,70)(20,50)
\psline(30,50)(30,45)
\psline(10,60)(10,10)
\psline(30,45)(10,25)
\psline(10,150)(50,150)
\psline(10,150)(10,110)
\newrgbcolor{userFillColour}{0.2 0.2 0.2}
\rput{0}(10,25){\psellipse[linewidth=1.3,border=0.3,fillcolor=userFillColour,fillstyle=solid](0,0)(2.5,-2.5)}
\psline(30,165)(30,150)
\rput[r](117.5,10){$\progtype$}
\rput[r](97.5,110){$\progtype$}
\rput[r](7.5,10){$\progtype$}
\psline(50,50)(50,90)
\rput(30,68.75){\universal}
\rput(485,130){$\gee$}
\rput[l](402.5,165){$\nameslang$}
\psline(390,110)(420,110)
\psline(370,130)(390,110)
\psline(400,110)(400,10)
\psline(380,120)(380,90)
\rput(400,130){\universal}
\psline(370,150)(420,150)
\psline(370,150)(370,130)
\psline(400,165)(400,150)
\psline(420,110)(420,150)
\rput(350,130){\EQLS}
\psline(370,100)(370,80)
\psline(370,80)(390,80)
\rput(376.25,86.25){\program}
\psline(370,100)(390,80)
\psline(505,110)(505,150)
\rput[l](487.5,165){$\nameslang$}
\rput[r](482.5,102.5){$\inputt$}
\psline(465,110)(505,110)
\psline(485,110)(485,90)
\psline(455,70)(455,90)
\psline(505,50)(475,50)
\psline(455,90)(505,90)
\psline(455,70)(475,50)
\psline(485,50)(485,45)
\psline(465,60)(465,10)
\psline(485,45)(465,25)
\psline(465,150)(505,150)
\psline(465,150)(465,110)
\newrgbcolor{userFillColour}{0.2 0.2 0.2}
\rput{0}(465,25){\psellipse[linewidth=1.3,border=0.3,fillcolor=userFillColour,fillstyle=solid](0,0)(2.5,-2.5)}
\psline(485,165)(485,150)
\rput[r](377.5,110){$\progtype$}
\psline(505,50)(505,90)
\rput(485,68.75){\universal}
\psline(390,20)(390,0)
\psline(390,0)(410,0)
\rput(396.25,6.25){\program}
\psline(390,20)(410,0)
\psline(455,20)(455,0)
\psline(455,0)(475,0)
\rput(461.25,6.25){\program}
\psline(455,20)(475,0)
\rput[r](397.5,40){$\progtype$}
\rput[l](307.5,165){$\nameslang$}
\psline(295,110)(325,110)
\psline(275,130)(295,110)
\rput(305,130){\universal}
\psline(275,150)(325,150)
\psline(275,150)(275,130)
\psline(305,165)(305,150)
\psline(325,110)(325,150)
\rput(440,130){\EQLS}
\psline(305,110)(305,105)
\psline(285,120)(285,70)
\psline(305,105)(285,85)
\newrgbcolor{userFillColour}{0.2 0.2 0.2}
\rput{0}(285,85){\psellipse[linewidth=1.3,border=0.3,fillcolor=userFillColour,fillstyle=solid](0,0)(2.5,-2.5)}
\psline(275,80)(275,60)
\psline(275,60)(295,60)
\rput(280,66.25){\program}
\psline(275,80)(295,60)
\rput(215,130){\thennn}
\psline[linewidth=0.15](450,95)(510,95)
\psline[linewidth=0.15](450,-5)(450,95)
\psline[linewidth=0.15](510,25)(510,95)
\psline[linewidth=0.15](480,-5)(510,25)
\psline[linewidth=0.15](450,-5)(480,-5)
\rput(485,20){$\aahh$}
\psline[linewidth=0.15](270,155)(330,155)
\psline[linewidth=0.15](270,55)(270,155)
\psline[linewidth=0.15](330,85)(330,155)
\psline[linewidth=0.15](300,55)(330,85)
\psline[linewidth=0.15](270,55)(300,55)
\rput(305,80){$\aahh$}
\end{pspicture}


==> PIC/fixp-3.tex <==
%%Created by jPicEdt 1.4.1_03: mixed JPIC-XML/LaTeX format
%%Mon Dec 28 11:17:11 GMT-10:00 2020
%%Begin JPIC-XML
%<?xml version="1.0" standalone="yes"?>
%<jpic x-min="0" x-max="385" y-min="5" y-max="355" auto-bounding="true">
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(122.5,195)"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\nameslang$
%</text>
%<multicurve fill-style= "none"
%	 points= "(130,140);(130,140);(160,140);(160,140)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(110,160);(110,160);(130,140);(130,140)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(120,150);(120,150);(120,100);(120,100)"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(140,160)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\universal
%</text>
%<multicurve fill-style= "none"
%	 points= "(110,180);(110,180);(160,180);(160,180)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(110,180);(110,180);(110,160);(110,160)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(120,195);(120,195);(120,180);(120,180)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(160,140);(160,140);(160,180);(160,180)"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(85,160)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\EQLS
%</text>
%<multicurve fill-style= "none"
%	 points= "(110,80);(110,80);(110,100);(110,100)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(160,60);(160,60);(130,60);(130,60)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(110,100);(110,100);(160,100);(160,100)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(110,80);(110,80);(130,60);(130,60)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(140,60);(140,60);(140,55);(140,55)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(120,70);(120,70);(120,20);(120,20)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(140,55);(140,55);(120,35);(120,35)"
%	 />
%<ellipse p3= "(122.5,32.5)"
%	 fill-style= "solid"
%	 p2= "(122.5,37.5)"
%	 fill-color= "#333333"
%	 p1= "(117.5,37.5)"
%	 closure= "open"
%	 angle-end= "0"
%	 stroke-overstrike= "true"
%	 stroke-width= "1.3"
%	 angle-start= "0"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(117.5,130)"
%	 text-frame= "noframe"
%	 stroke-width= "0.35"
%	 text-hor-align= "right"
%	 >
%$\progtype$
%</text>
%<multicurve fill-style= "none"
%	 points= "(160,60);(160,60);(160,100);(160,100)"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(140,78.75)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\universal
%</text>
%<multicurve fill-style= "none"
%	 points= "(110,30);(110,30);(110,10);(110,10)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(110,10);(110,10);(130,10);(130,10)"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(116.25,16.25)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\program
%</text>
%<multicurve fill-style= "none"
%	 points= "(110,30);(110,30);(130,10);(130,10)"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(17.5,195)"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\nameslang$
%</text>
%<multicurve fill-style= "none"
%	 points= "(25,140);(25,140);(55,140);(55,140)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(5,160);(5,160);(25,140);(25,140)"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(35,160)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\universal
%</text>
%<multicurve fill-style= "none"
%	 points= "(5,180);(5,180);(55,180);(55,180)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(5,180);(5,180);(5,160);(5,160)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(15,195);(15,195);(15,180);(15,180)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(55,140);(55,140);(55,180);(55,180)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(35,140);(35,140);(35,135);(35,135)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(15,150);(15,150);(15,100);(15,100)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(35,135);(35,135);(15,115);(15,115)"
%	 />
%<ellipse p3= "(17.5,112.5)"
%	 fill-style= "solid"
%	 p2= "(17.5,117.5)"
%	 fill-color= "#333333"
%	 p1= "(12.5,117.5)"
%	 closure= "open"
%	 angle-end= "0"
%	 stroke-overstrike= "true"
%	 stroke-width= "1.3"
%	 angle-start= "0"
%	 />
%<multicurve fill-style= "none"
%	 points= "(5,110);(5,110);(5,90);(5,90)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(5,90);(5,90);(25,90);(25,90)"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(10,96.25)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\program
%</text>
%<multicurve fill-style= "none"
%	 points= "(5,110);(5,110);(25,90);(25,90)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(105,105);(105,105);(165,105);(165,105)"
%	 stroke-width= "0.15"
%	 />
%<multicurve fill-style= "none"
%	 points= "(105,5);(105,5);(105,105);(105,105)"
%	 stroke-width= "0.15"
%	 />
%<multicurve fill-style= "none"
%	 points= "(165,35);(165,35);(165,105);(165,105)"
%	 stroke-width= "0.15"
%	 />
%<multicurve fill-style= "none"
%	 points= "(135,5);(135,5);(165,35);(165,35)"
%	 stroke-width= "0.15"
%	 />
%<multicurve fill-style= "none"
%	 points= "(105,5);(105,5);(135,5);(135,5)"
%	 stroke-width= "0.15"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(140,30)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\aahh$
%</text>
%<multicurve fill-style= "none"
%	 points= "(0,185);(0,185);(60,185);(60,185)"
%	 stroke-width= "0.15"
%	 />
%<multicurve fill-style= "none"
%	 points= "(0,85);(0,85);(0,185);(0,185)"
%	 stroke-width= "0.15"
%	 />
%<multicurve fill-style= "none"
%	 points= "(60,115);(60,115);(60,185);(60,185)"
%	 stroke-width= "0.15"
%	 />
%<multicurve fill-style= "none"
%	 points= "(30,85);(30,85);(60,115);(60,115)"
%	 stroke-width= "0.15"
%	 />
%<multicurve fill-style= "none"
%	 points= "(0,85);(0,85);(30,85);(30,85)"
%	 stroke-width= "0.15"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(35,110)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\aahh$
%</text>
%<multicurve fill-style= "none"
%	 points= "(140,140);(140,140);(140,135);(140,135)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(140,135);(140,135);(120,115);(120,115)"
%	 />
%<ellipse p3= "(122.5,112.5)"
%	 fill-style= "solid"
%	 p2= "(122.5,117.5)"
%	 fill-color= "#333333"
%	 p1= "(117.5,117.5)"
%	 closure= "open"
%	 angle-end= "0"
%	 stroke-overstrike= "true"
%	 stroke-width= "1.3"
%	 angle-start= "0"
%	 />
%<multicurve fill-style= "none"
%	 points= "(230,140);(230,140);(260,140);(260,140)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(210,160);(210,160);(230,140);(230,140)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(220,150);(220,150);(220,100);(220,100)"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(240,160)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\universal
%</text>
%<multicurve fill-style= "none"
%	 points= "(210,180);(210,180);(260,180);(260,180)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(210,180);(210,180);(210,160);(210,160)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(260,140);(260,140);(260,180);(260,180)"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(185,160)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\EQLS
%</text>
%<multicurve fill-style= "none"
%	 points= "(210,80);(210,80);(210,100);(210,100)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(260,60);(260,60);(230,60);(230,60)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(210,100);(210,100);(260,100);(260,100)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(210,80);(210,80);(230,60);(230,60)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(240,60);(240,60);(240,55);(240,55)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(220,70);(220,70);(220,20);(220,20)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(240,55);(240,55);(220,35);(220,35)"
%	 />
%<ellipse p3= "(222.5,32.5)"
%	 fill-style= "solid"
%	 p2= "(222.5,37.5)"
%	 fill-color= "#333333"
%	 p1= "(217.5,37.5)"
%	 closure= "open"
%	 angle-end= "0"
%	 stroke-overstrike= "true"
%	 stroke-width= "1.3"
%	 angle-start= "0"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(217.5,130)"
%	 text-frame= "noframe"
%	 stroke-width= "0.35"
%	 text-hor-align= "right"
%	 >
%$\progtype$
%</text>
%<multicurve fill-style= "none"
%	 points= "(260,60);(260,60);(260,100);(260,100)"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(240,78.75)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\universal
%</text>
%<multicurve fill-style= "none"
%	 points= "(210,30);(210,30);(210,10);(210,10)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(210,10);(210,10);(230,10);(230,10)"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(216.25,16.25)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\program
%</text>
%<multicurve fill-style= "none"
%	 points= "(210,30);(210,30);(230,10);(230,10)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(205,105);(205,105);(265,105);(265,105)"
%	 stroke-width= "0.15"
%	 />
%<multicurve fill-style= "none"
%	 points= "(205,5);(205,5);(205,105);(205,105)"
%	 stroke-width= "0.15"
%	 />
%<multicurve fill-style= "none"
%	 points= "(265,35);(265,35);(265,105);(265,105)"
%	 stroke-width= "0.15"
%	 />
%<multicurve fill-style= "none"
%	 points= "(235,5);(235,5);(265,35);(265,35)"
%	 stroke-width= "0.15"
%	 />
%<multicurve fill-style= "none"
%	 points= "(205,5);(205,5);(235,5);(235,5)"
%	 stroke-width= "0.15"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(240,30)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\aahh$
%</text>
%<multicurve fill-style= "none"
%	 points= "(240,140);(240,140);(240,135);(240,135)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(240,135);(240,135);(220,115);(220,115)"
%	 />
%<ellipse p3= "(222.5,112.5)"
%	 fill-style= "solid"
%	 p2= "(222.5,117.5)"
%	 fill-color= "#333333"
%	 p1= "(217.5,117.5)"
%	 closure= "open"
%	 angle-end= "0"
%	 stroke-overstrike= "true"
%	 stroke-width= "1.3"
%	 angle-start= "0"
%	 />
%<multicurve fill-style= "none"
%	 points= "(230,220);(230,220);(260,220);(260,220)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(210,240);(210,240);(230,220);(230,220)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(220,230);(220,230);(220,180);(220,180)"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(240,240)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\universal
%</text>
%<multicurve fill-style= "none"
%	 points= "(210,260);(210,260);(260,260);(260,260)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(210,260);(210,260);(210,240);(210,240)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(260,220);(260,220);(260,260);(260,260)"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(217.5,210)"
%	 text-frame= "noframe"
%	 stroke-width= "0.35"
%	 text-hor-align= "right"
%	 >
%$\progtype$
%</text>
%<multicurve fill-style= "none"
%	 points= "(240,220);(240,220);(240,215);(240,215)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(240,215);(240,215);(220,195);(220,195)"
%	 />
%<ellipse p3= "(222.5,192.5)"
%	 fill-style= "solid"
%	 p2= "(222.5,197.5)"
%	 fill-color= "#333333"
%	 p1= "(217.5,197.5)"
%	 closure= "open"
%	 angle-end= "0"
%	 stroke-overstrike= "true"
%	 stroke-width= "1.3"
%	 angle-start= "0"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(222.5,275)"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\nameslang$
%</text>
%<multicurve fill-style= "none"
%	 points= "(220,275);(220,275);(220,260);(220,260)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(330,300);(330,300);(360,300);(360,300)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(310,320);(310,320);(330,300);(330,300)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(320,310);(320,310);(320,260);(320,260)"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(340,320)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\universal
%</text>
%<multicurve fill-style= "none"
%	 points= "(310,340);(310,340);(360,340);(360,340)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(310,340);(310,340);(310,320);(310,320)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(360,300);(360,300);(360,340);(360,340)"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(317.5,290)"
%	 text-frame= "noframe"
%	 stroke-width= "0.35"
%	 text-hor-align= "right"
%	 >
%$\progtype$
%</text>
%<multicurve fill-style= "none"
%	 points= "(340,300);(340,300);(340,295);(340,295)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(340,295);(340,295);(320,275);(320,275)"
%	 />
%<ellipse p3= "(322.5,272.5)"
%	 fill-style= "solid"
%	 p2= "(322.5,277.5)"
%	 fill-color= "#333333"
%	 p1= "(317.5,277.5)"
%	 closure= "open"
%	 angle-end= "0"
%	 stroke-overstrike= "true"
%	 stroke-width= "1.3"
%	 angle-start= "0"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(322.5,355)"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\nameslang$
%</text>
%<multicurve fill-style= "none"
%	 points= "(320,355);(320,355);(320,340);(320,340)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(330,140);(330,140);(360,140);(360,140)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(310,160);(310,160);(330,140);(330,140)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(320,150);(320,150);(320,100);(320,100)"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(340,160)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\universal
%</text>
%<multicurve fill-style= "none"
%	 points= "(310,180);(310,180);(360,180);(360,180)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(310,180);(310,180);(310,160);(310,160)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(360,140);(360,140);(360,180);(360,180)"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(285,160)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\EQLS
%</text>
%<multicurve fill-style= "none"
%	 points= "(310,80);(310,80);(310,100);(310,100)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(360,60);(360,60);(330,60);(330,60)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(310,100);(310,100);(360,100);(360,100)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(310,80);(310,80);(330,60);(330,60)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(340,60);(340,60);(340,55);(340,55)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(320,70);(320,70);(320,20);(320,20)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(340,55);(340,55);(320,35);(320,35)"
%	 />
%<ellipse p3= "(322.5,32.5)"
%	 fill-style= "solid"
%	 p2= "(322.5,37.5)"
%	 fill-color= "#333333"
%	 p1= "(317.5,37.5)"
%	 closure= "open"
%	 angle-end= "0"
%	 stroke-overstrike= "true"
%	 stroke-width= "1.3"
%	 angle-start= "0"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(317.5,130)"
%	 text-frame= "noframe"
%	 stroke-width= "0.35"
%	 text-hor-align= "right"
%	 >
%$\progtype$
%</text>
%<multicurve fill-style= "none"
%	 points= "(360,60);(360,60);(360,100);(360,100)"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(340,78.75)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\universal
%</text>
%<multicurve fill-style= "none"
%	 points= "(310,30);(310,30);(310,10);(310,10)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(310,10);(310,10);(330,10);(330,10)"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(316.25,16.25)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\program
%</text>
%<multicurve fill-style= "none"
%	 points= "(310,30);(310,30);(330,10);(330,10)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(305,105);(305,105);(365,105);(365,105)"
%	 stroke-width= "0.15"
%	 />
%<multicurve fill-style= "none"
%	 points= "(305,5);(305,5);(305,105);(305,105)"
%	 stroke-width= "0.15"
%	 />
%<multicurve fill-style= "none"
%	 points= "(365,35);(365,35);(365,105);(365,105)"
%	 stroke-width= "0.15"
%	 />
%<multicurve fill-style= "none"
%	 points= "(335,5);(335,5);(365,35);(365,35)"
%	 stroke-width= "0.15"
%	 />
%<multicurve fill-style= "none"
%	 points= "(305,5);(305,5);(335,5);(335,5)"
%	 stroke-width= "0.15"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(340,30)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\aahh$
%</text>
%<multicurve fill-style= "none"
%	 points= "(340,140);(340,140);(340,135);(340,135)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(340,135);(340,135);(320,115);(320,115)"
%	 />
%<ellipse p3= "(322.5,112.5)"
%	 fill-style= "solid"
%	 p2= "(322.5,117.5)"
%	 fill-color= "#333333"
%	 p1= "(317.5,117.5)"
%	 closure= "open"
%	 angle-end= "0"
%	 stroke-overstrike= "true"
%	 stroke-width= "1.3"
%	 angle-start= "0"
%	 />
%<multicurve fill-style= "none"
%	 points= "(330,220);(330,220);(360,220);(360,220)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(310,240);(310,240);(330,220);(330,220)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(320,230);(320,230);(320,180);(320,180)"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(340,240)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\universal
%</text>
%<multicurve fill-style= "none"
%	 points= "(310,260);(310,260);(360,260);(360,260)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(310,260);(310,260);(310,240);(310,240)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(360,220);(360,220);(360,260);(360,260)"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(317.5,210)"
%	 text-frame= "noframe"
%	 stroke-width= "0.35"
%	 text-hor-align= "right"
%	 >
%$\progtype$
%</text>
%<multicurve fill-style= "none"
%	 points= "(340,220);(340,220);(340,215);(340,215)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(340,215);(340,215);(320,195);(320,195)"
%	 />
%<ellipse p3= "(322.5,192.5)"
%	 fill-style= "solid"
%	 p2= "(322.5,197.5)"
%	 fill-color= "#333333"
%	 p1= "(317.5,197.5)"
%	 closure= "open"
%	 angle-end= "0"
%	 stroke-overstrike= "true"
%	 stroke-width= "1.3"
%	 angle-start= "0"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(385,160)"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%\EQLSETC
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(12.5,130)"
%	 text-frame= "noframe"
%	 stroke-width= "0.35"
%	 text-hor-align= "right"
%	 >
%$\progtype$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(117.5,50)"
%	 text-frame= "noframe"
%	 stroke-width= "0.35"
%	 text-hor-align= "right"
%	 >
%$\progtype$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(217.5,50)"
%	 text-frame= "noframe"
%	 stroke-width= "0.35"
%	 text-hor-align= "right"
%	 >
%$\progtype$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(317.5,50)"
%	 text-frame= "noframe"
%	 stroke-width= "0.35"
%	 text-hor-align= "right"
%	 >
%$\progtype$
%</text>
%</jpic>
%%End JPIC-XML
%PSTricks content-type (pstricks.sty package needed)
%Add \usepackage{pstricks} in the preamble of your LaTeX file
%You can rescale the whole picture (to 80% for instance) by using the command \def\JPicScale{0.8}
\ifx\JPicScale\undefined\def\JPicScale{1}\fi
\psset{unit=\JPicScale mm}
\psset{linewidth=0.3,dotsep=1,hatchwidth=0.3,hatchsep=1.5,shadowsize=1,dimen=middle}
\psset{dotsize=0.7 2.5,dotscale=1 1,fillcolor=black}
\psset{arrowsize=1 2,arrowlength=1,arrowinset=0.25,tbarsize=0.7 5,bracketlength=0.15,rbracketlength=0.15}
\begin{pspicture}(0,0)(385,355)
\rput[l](122.5,195){$\nameslang$}
\psline(130,140)(160,140)
\psline(110,160)(130,140)
\psline(120,150)(120,100)
\rput(140,160){\universal}
\psline(110,180)(160,180)
\psline(110,180)(110,160)
\psline(120,195)(120,180)
\psline(160,140)(160,180)
\rput(85,160){\EQLS}
\psline(110,80)(110,100)
\psline(160,60)(130,60)
\psline(110,100)(160,100)
\psline(110,80)(130,60)
\psline(140,60)(140,55)
\psline(120,70)(120,20)
\psline(140,55)(120,35)
\newrgbcolor{userFillColour}{0.2 0.2 0.2}
\rput{0}(120,35){\psellipse[linewidth=1.3,border=0.3,fillcolor=userFillColour,fillstyle=solid](0,0)(2.5,-2.5)}
\rput[r](117.5,130){$\progtype$}
\psline(160,60)(160,100)
\rput(140,78.75){\universal}
\psline(110,30)(110,10)
\psline(110,10)(130,10)
\rput(116.25,16.25){\program}
\psline(110,30)(130,10)
\rput[l](17.5,195){$\nameslang$}
\psline(25,140)(55,140)
\psline(5,160)(25,140)
\rput(35,160){\universal}
\psline(5,180)(55,180)
\psline(5,180)(5,160)
\psline(15,195)(15,180)
\psline(55,140)(55,180)
\psline(35,140)(35,135)
\psline(15,150)(15,100)
\psline(35,135)(15,115)
\newrgbcolor{userFillColour}{0.2 0.2 0.2}
\rput{0}(15,115){\psellipse[linewidth=1.3,border=0.3,fillcolor=userFillColour,fillstyle=solid](0,0)(2.5,-2.5)}
\psline(5,110)(5,90)
\psline(5,90)(25,90)
\rput(10,96.25){\program}
\psline(5,110)(25,90)
\psline[linewidth=0.15](105,105)(165,105)
\psline[linewidth=0.15](105,5)(105,105)
\psline[linewidth=0.15](165,35)(165,105)
\psline[linewidth=0.15](135,5)(165,35)
\psline[linewidth=0.15](105,5)(135,5)
\rput(140,30){$\aahh$}
\psline[linewidth=0.15](0,185)(60,185)
\psline[linewidth=0.15](0,85)(0,185)
\psline[linewidth=0.15](60,115)(60,185)
\psline[linewidth=0.15](30,85)(60,115)
\psline[linewidth=0.15](0,85)(30,85)
\rput(35,110){$\aahh$}
\psline(140,140)(140,135)
\psline(140,135)(120,115)
\newrgbcolor{userFillColour}{0.2 0.2 0.2}
\rput{0}(120,115){\psellipse[linewidth=1.3,border=0.3,fillcolor=userFillColour,fillstyle=solid](0,0)(2.5,-2.5)}
\psline(230,140)(260,140)
\psline(210,160)(230,140)
\psline(220,150)(220,100)
\rput(240,160){\universal}
\psline(210,180)(260,180)
\psline(210,180)(210,160)
\psline(260,140)(260,180)
\rput(185,160){\EQLS}
\psline(210,80)(210,100)
\psline(260,60)(230,60)
\psline(210,100)(260,100)
\psline(210,80)(230,60)
\psline(240,60)(240,55)
\psline(220,70)(220,20)
\psline(240,55)(220,35)
\newrgbcolor{userFillColour}{0.2 0.2 0.2}
\rput{0}(220,35){\psellipse[linewidth=1.3,border=0.3,fillcolor=userFillColour,fillstyle=solid](0,0)(2.5,-2.5)}
\rput[r](217.5,130){$\progtype$}
\psline(260,60)(260,100)
\rput(240,78.75){\universal}
\psline(210,30)(210,10)
\psline(210,10)(230,10)
\rput(216.25,16.25){\program}
\psline(210,30)(230,10)
\psline[linewidth=0.15](205,105)(265,105)
\psline[linewidth=0.15](205,5)(205,105)
\psline[linewidth=0.15](265,35)(265,105)
\psline[linewidth=0.15](235,5)(265,35)
\psline[linewidth=0.15](205,5)(235,5)
\rput(240,30){$\aahh$}
\psline(240,140)(240,135)
\psline(240,135)(220,115)
\newrgbcolor{userFillColour}{0.2 0.2 0.2}
\rput{0}(220,115){\psellipse[linewidth=1.3,border=0.3,fillcolor=userFillColour,fillstyle=solid](0,0)(2.5,-2.5)}
\psline(230,220)(260,220)
\psline(210,240)(230,220)
\psline(220,230)(220,180)
\rput(240,240){\universal}
\psline(210,260)(260,260)
\psline(210,260)(210,240)
\psline(260,220)(260,260)
\rput[r](217.5,210){$\progtype$}
\psline(240,220)(240,215)
\psline(240,215)(220,195)
\newrgbcolor{userFillColour}{0.2 0.2 0.2}
\rput{0}(220,195){\psellipse[linewidth=1.3,border=0.3,fillcolor=userFillColour,fillstyle=solid](0,0)(2.5,-2.5)}
\rput[l](222.5,275){$\nameslang$}
\psline(220,275)(220,260)
\psline(330,300)(360,300)
\psline(310,320)(330,300)
\psline(320,310)(320,260)
\rput(340,320){\universal}
\psline(310,340)(360,340)
\psline(310,340)(310,320)
\psline(360,300)(360,340)
\rput[r](317.5,290){$\progtype$}
\psline(340,300)(340,295)
\psline(340,295)(320,275)
\newrgbcolor{userFillColour}{0.2 0.2 0.2}
\rput{0}(320,275){\psellipse[linewidth=1.3,border=0.3,fillcolor=userFillColour,fillstyle=solid](0,0)(2.5,-2.5)}
\rput[l](322.5,355){$\nameslang$}
\psline(320,355)(320,340)
\psline(330,140)(360,140)
\psline(310,160)(330,140)
\psline(320,150)(320,100)
\rput(340,160){\universal}
\psline(310,180)(360,180)
\psline(310,180)(310,160)
\psline(360,140)(360,180)
\rput(285,160){\EQLS}
\psline(310,80)(310,100)
\psline(360,60)(330,60)
\psline(310,100)(360,100)
\psline(310,80)(330,60)
\psline(340,60)(340,55)
\psline(320,70)(320,20)
\psline(340,55)(320,35)
\newrgbcolor{userFillColour}{0.2 0.2 0.2}
\rput{0}(320,35){\psellipse[linewidth=1.3,border=0.3,fillcolor=userFillColour,fillstyle=solid](0,0)(2.5,-2.5)}
\rput[r](317.5,130){$\progtype$}
\psline(360,60)(360,100)
\rput(340,78.75){\universal}
\psline(310,30)(310,10)
\psline(310,10)(330,10)
\rput(316.25,16.25){\program}
\psline(310,30)(330,10)
\psline[linewidth=0.15](305,105)(365,105)
\psline[linewidth=0.15](305,5)(305,105)
\psline[linewidth=0.15](365,35)(365,105)
\psline[linewidth=0.15](335,5)(365,35)
\psline[linewidth=0.15](305,5)(335,5)
\rput(340,30){$\aahh$}
\psline(340,140)(340,135)
\psline(340,135)(320,115)
\newrgbcolor{userFillColour}{0.2 0.2 0.2}
\rput{0}(320,115){\psellipse[linewidth=1.3,border=0.3,fillcolor=userFillColour,fillstyle=solid](0,0)(2.5,-2.5)}
\psline(330,220)(360,220)
\psline(310,240)(330,220)
\psline(320,230)(320,180)
\rput(340,240){\universal}
\psline(310,260)(360,260)
\psline(310,260)(310,240)
\psline(360,220)(360,260)
\rput[r](317.5,210){$\progtype$}
\psline(340,220)(340,215)
\psline(340,215)(320,195)
\newrgbcolor{userFillColour}{0.2 0.2 0.2}
\rput{0}(320,195){\psellipse[linewidth=1.3,border=0.3,fillcolor=userFillColour,fillstyle=solid](0,0)(2.5,-2.5)}
\rput[l](385,160){\EQLSETC}
\rput[r](12.5,130){$\progtype$}
\rput[r](117.5,50){$\progtype$}
\rput[r](217.5,50){$\progtype$}
\rput[r](317.5,50){$\progtype$}
\end{pspicture}


==> PIC/fixp-4.tex <==
%%Created by jPicEdt 1.4.1_03: mixed JPIC-XML/LaTeX format
%%Mon Dec 28 12:51:14 GMT-10:00 2020
%%Begin JPIC-XML
%<?xml version="1.0" standalone="yes"?>
%<jpic x-min="0" x-max="500" y-min="-5" y-max="165" auto-bounding="true">
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(135,130)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\gee$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(32.5,165)"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\nameslang$
%</text>
%<multicurve fill-style= "none"
%	 points= "(20,110);(20,110);(50,110);(50,110)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(0,130);(0,130);(20,110);(20,110)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(30,110);(30,110);(30,10);(30,10)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(10,120);(10,120);(10,90);(10,90)"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(30,130)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\universal
%</text>
%<multicurve fill-style= "none"
%	 points= "(0,150);(0,150);(50,150);(50,150)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(0,150);(0,150);(0,130);(0,130)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(30,165);(30,165);(30,150);(30,150)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(50,110);(50,110);(50,150);(50,150)"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(80,130)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\EQLS
%</text>
%<multicurve fill-style= "none"
%	 points= "(0,100);(0,100);(0,80);(0,80)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(0,80);(0,80);(20,80);(20,80)"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(6.25,86.25)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\program
%</text>
%<multicurve fill-style= "none"
%	 points= "(0,100);(0,100);(20,80);(20,80)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(155,110);(155,110);(155,150);(155,150)"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(137.5,165)"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\nameslang$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(132.5,100)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\inputt$
%</text>
%<multicurve fill-style= "none"
%	 points= "(115,110);(115,110);(155,110);(155,110)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(135,110);(135,110);(135,90);(135,90)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(105,70);(105,70);(105,90);(105,90)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(155,50);(155,50);(125,50);(125,50)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(105,90);(105,90);(155,90);(155,90)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(105,70);(105,70);(125,50);(125,50)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(135,50);(135,50);(135,45);(135,45)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(115,60);(115,60);(115,10);(115,10)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(135,45);(135,45);(115,25);(115,25)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(115,150);(115,150);(155,150);(155,150)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(115,150);(115,150);(115,110);(115,110)"
%	 />
%<ellipse p3= "(117.5,22.5)"
%	 fill-style= "solid"
%	 p2= "(117.5,27.5)"
%	 fill-color= "#333333"
%	 p1= "(112.5,27.5)"
%	 closure= "open"
%	 angle-end= "0"
%	 stroke-overstrike= "true"
%	 stroke-width= "1.3"
%	 angle-start= "0"
%	 />
%<multicurve fill-style= "none"
%	 points= "(135,165);(135,165);(135,150);(135,150)"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(27.5,10)"
%	 text-frame= "noframe"
%	 stroke-width= "0.35"
%	 text-hor-align= "right"
%	 >
%$\progtype$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(7.5,110)"
%	 text-frame= "noframe"
%	 stroke-width= "0.35"
%	 text-hor-align= "right"
%	 >
%$\progtype$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(112.5,10)"
%	 text-frame= "noframe"
%	 stroke-width= "0.35"
%	 text-hor-align= "right"
%	 >
%$\progtype$
%</text>
%<multicurve fill-style= "none"
%	 points= "(155,50);(155,50);(155,90);(155,90)"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(135,68.75)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\universal
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(475,130)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\gee$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(392.5,165)"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\nameslang$
%</text>
%<multicurve fill-style= "none"
%	 points= "(380,110);(380,110);(410,110);(410,110)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(360,130);(360,130);(380,110);(380,110)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(390,110);(390,110);(390,10);(390,10)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(370,120);(370,120);(370,90);(370,90)"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(390,130)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\universal
%</text>
%<multicurve fill-style= "none"
%	 points= "(360,150);(360,150);(410,150);(410,150)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(360,150);(360,150);(360,130);(360,130)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(390,165);(390,165);(390,150);(390,150)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(410,110);(410,110);(410,150);(410,150)"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(340,130)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\EQLS
%</text>
%<multicurve fill-style= "none"
%	 points= "(360,100);(360,100);(360,80);(360,80)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(360,80);(360,80);(380,80);(380,80)"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(366.25,86.25)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\program
%</text>
%<multicurve fill-style= "none"
%	 points= "(360,100);(360,100);(380,80);(380,80)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(495,110);(495,110);(495,150);(495,150)"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(477.5,165)"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\nameslang$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(472.5,102.5)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\inputt$
%</text>
%<multicurve fill-style= "none"
%	 points= "(455,110);(455,110);(495,110);(495,110)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(475,110);(475,110);(475,90);(475,90)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(445,70);(445,70);(445,90);(445,90)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(495,50);(495,50);(465,50);(465,50)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(445,90);(445,90);(495,90);(495,90)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(445,70);(445,70);(465,50);(465,50)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(475,50);(475,50);(475,45);(475,45)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(455,60);(455,60);(455,10);(455,10)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(475,45);(475,45);(455,25);(455,25)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(455,150);(455,150);(495,150);(495,150)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(455,150);(455,150);(455,110);(455,110)"
%	 />
%<ellipse p3= "(457.5,22.5)"
%	 fill-style= "solid"
%	 p2= "(457.5,27.5)"
%	 fill-color= "#333333"
%	 p1= "(452.5,27.5)"
%	 closure= "open"
%	 angle-end= "0"
%	 stroke-overstrike= "true"
%	 stroke-width= "1.3"
%	 angle-start= "0"
%	 />
%<multicurve fill-style= "none"
%	 points= "(475,165);(475,165);(475,150);(475,150)"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(367.5,110)"
%	 text-frame= "noframe"
%	 stroke-width= "0.35"
%	 text-hor-align= "right"
%	 >
%$\progtype$
%</text>
%<multicurve fill-style= "none"
%	 points= "(495,50);(495,50);(495,90);(495,90)"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(475,68.75)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\universal
%</text>
%<multicurve fill-style= "none"
%	 points= "(380,20);(380,20);(380,0);(380,0)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(380,0);(380,0);(400,0);(400,0)"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(386.25,6.25)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\program
%</text>
%<multicurve fill-style= "none"
%	 points= "(380,20);(380,20);(400,0);(400,0)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(445,20);(445,20);(445,0);(445,0)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(445,0);(445,0);(465,0);(465,0)"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(451.25,6.25)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\program
%</text>
%<multicurve fill-style= "none"
%	 points= "(445,20);(445,20);(465,0);(465,0)"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(387.5,40)"
%	 text-frame= "noframe"
%	 stroke-width= "0.35"
%	 text-hor-align= "right"
%	 >
%$\progtype$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(297.5,165)"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\nameslang$
%</text>
%<multicurve fill-style= "none"
%	 points= "(285,110);(285,110);(315,110);(315,110)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(265,130);(265,130);(285,110);(285,110)"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(295,130)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\universal
%</text>
%<multicurve fill-style= "none"
%	 points= "(265,150);(265,150);(315,150);(315,150)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(265,150);(265,150);(265,130);(265,130)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(295,165);(295,165);(295,150);(295,150)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(315,110);(315,110);(315,150);(315,150)"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(430,130)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\EQLS
%</text>
%<multicurve fill-style= "none"
%	 points= "(295,110);(295,110);(295,105);(295,105)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(275,120);(275,120);(275,70);(275,70)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(295,105);(295,105);(275,85);(275,85)"
%	 />
%<ellipse p3= "(277.5,82.5)"
%	 fill-style= "solid"
%	 p2= "(277.5,87.5)"
%	 fill-color= "#333333"
%	 p1= "(272.5,87.5)"
%	 closure= "open"
%	 angle-end= "0"
%	 stroke-overstrike= "true"
%	 stroke-width= "1.3"
%	 angle-start= "0"
%	 />
%<multicurve fill-style= "none"
%	 points= "(265,80);(265,80);(265,60);(265,60)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(265,60);(265,60);(285,60);(285,60)"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(270,66.25)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\program
%</text>
%<multicurve fill-style= "none"
%	 points= "(265,80);(265,80);(285,60);(285,60)"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(205,130)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\thennn
%</text>
%<multicurve fill-style= "none"
%	 points= "(440,95);(440,95);(500,95);(500,95)"
%	 stroke-width= "0.15"
%	 />
%<multicurve fill-style= "none"
%	 points= "(440,-5);(440,-5);(440,95);(440,95)"
%	 stroke-width= "0.15"
%	 />
%<multicurve fill-style= "none"
%	 points= "(500,25);(500,25);(500,95);(500,95)"
%	 stroke-width= "0.15"
%	 />
%<multicurve fill-style= "none"
%	 points= "(470,-5);(470,-5);(500,25);(500,25)"
%	 stroke-width= "0.15"
%	 />
%<multicurve fill-style= "none"
%	 points= "(440,-5);(440,-5);(470,-5);(470,-5)"
%	 stroke-width= "0.15"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(475,20)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\aahh$
%</text>
%<multicurve fill-style= "none"
%	 points= "(260,155);(260,155);(320,155);(320,155)"
%	 stroke-width= "0.15"
%	 />
%<multicurve fill-style= "none"
%	 points= "(260,55);(260,55);(260,155);(260,155)"
%	 stroke-width= "0.15"
%	 />
%<multicurve fill-style= "none"
%	 points= "(320,85);(320,85);(320,155);(320,155)"
%	 stroke-width= "0.15"
%	 />
%<multicurve fill-style= "none"
%	 points= "(290,55);(290,55);(320,85);(320,85)"
%	 stroke-width= "0.15"
%	 />
%<multicurve fill-style= "none"
%	 points= "(260,55);(260,55);(290,55);(290,55)"
%	 stroke-width= "0.15"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(295,80)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\aahh$
%</text>
%</jpic>
%%End JPIC-XML
%PSTricks content-type (pstricks.sty package needed)
%Add \usepackage{pstricks} in the preamble of your LaTeX file
%You can rescale the whole picture (to 80% for instance) by using the command \def\JPicScale{0.8}
\ifx\JPicScale\undefined\def\JPicScale{1}\fi
\psset{unit=\JPicScale mm}
\psset{linewidth=0.3,dotsep=1,hatchwidth=0.3,hatchsep=1.5,shadowsize=1,dimen=middle}
\psset{dotsize=0.7 2.5,dotscale=1 1,fillcolor=black}
\psset{arrowsize=1 2,arrowlength=1,arrowinset=0.25,tbarsize=0.7 5,bracketlength=0.15,rbracketlength=0.15}
\begin{pspicture}(0,0)(500,165)
\rput(135,130){$\gee$}
\rput[l](32.5,165){$\nameslang$}
\psline(20,110)(50,110)
\psline(0,130)(20,110)
\psline(30,110)(30,10)
\psline(10,120)(10,90)
\rput(30,130){\universal}
\psline(0,150)(50,150)
\psline(0,150)(0,130)
\psline(30,165)(30,150)
\psline(50,110)(50,150)
\rput(80,130){\EQLS}
\psline(0,100)(0,80)
\psline(0,80)(20,80)
\rput(6.25,86.25){\program}
\psline(0,100)(20,80)
\psline(155,110)(155,150)
\rput[l](137.5,165){$\nameslang$}
\rput[r](132.5,100){$\inputt$}
\psline(115,110)(155,110)
\psline(135,110)(135,90)
\psline(105,70)(105,90)
\psline(155,50)(125,50)
\psline(105,90)(155,90)
\psline(105,70)(125,50)
\psline(135,50)(135,45)
\psline(115,60)(115,10)
\psline(135,45)(115,25)
\psline(115,150)(155,150)
\psline(115,150)(115,110)
\newrgbcolor{userFillColour}{0.2 0.2 0.2}
\rput{0}(115,25){\psellipse[linewidth=1.3,border=0.3,fillcolor=userFillColour,fillstyle=solid](0,0)(2.5,-2.5)}
\psline(135,165)(135,150)
\rput[r](27.5,10){$\progtype$}
\rput[r](7.5,110){$\progtype$}
\rput[r](112.5,10){$\progtype$}
\psline(155,50)(155,90)
\rput(135,68.75){\universal}
\rput(475,130){$\gee$}
\rput[l](392.5,165){$\nameslang$}
\psline(380,110)(410,110)
\psline(360,130)(380,110)
\psline(390,110)(390,10)
\psline(370,120)(370,90)
\rput(390,130){\universal}
\psline(360,150)(410,150)
\psline(360,150)(360,130)
\psline(390,165)(390,150)
\psline(410,110)(410,150)
\rput(340,130){\EQLS}
\psline(360,100)(360,80)
\psline(360,80)(380,80)
\rput(366.25,86.25){\program}
\psline(360,100)(380,80)
\psline(495,110)(495,150)
\rput[l](477.5,165){$\nameslang$}
\rput[r](472.5,102.5){$\inputt$}
\psline(455,110)(495,110)
\psline(475,110)(475,90)
\psline(445,70)(445,90)
\psline(495,50)(465,50)
\psline(445,90)(495,90)
\psline(445,70)(465,50)
\psline(475,50)(475,45)
\psline(455,60)(455,10)
\psline(475,45)(455,25)
\psline(455,150)(495,150)
\psline(455,150)(455,110)
\newrgbcolor{userFillColour}{0.2 0.2 0.2}
\rput{0}(455,25){\psellipse[linewidth=1.3,border=0.3,fillcolor=userFillColour,fillstyle=solid](0,0)(2.5,-2.5)}
\psline(475,165)(475,150)
\rput[r](367.5,110){$\progtype$}
\psline(495,50)(495,90)
\rput(475,68.75){\universal}
\psline(380,20)(380,0)
\psline(380,0)(400,0)
\rput(386.25,6.25){\program}
\psline(380,20)(400,0)
\psline(445,20)(445,0)
\psline(445,0)(465,0)
\rput(451.25,6.25){\program}
\psline(445,20)(465,0)
\rput[r](387.5,40){$\progtype$}
\rput[l](297.5,165){$\nameslang$}
\psline(285,110)(315,110)
\psline(265,130)(285,110)
\rput(295,130){\universal}
\psline(265,150)(315,150)
\psline(265,150)(265,130)
\psline(295,165)(295,150)
\psline(315,110)(315,150)
\rput(430,130){\EQLS}
\psline(295,110)(295,105)
\psline(275,120)(275,70)
\psline(295,105)(275,85)
\newrgbcolor{userFillColour}{0.2 0.2 0.2}
\rput{0}(275,85){\psellipse[linewidth=1.3,border=0.3,fillcolor=userFillColour,fillstyle=solid](0,0)(2.5,-2.5)}
\psline(265,80)(265,60)
\psline(265,60)(285,60)
\rput(270,66.25){\program}
\psline(265,80)(285,60)
\rput(205,130){\thennn}
\psline[linewidth=0.15](440,95)(500,95)
\psline[linewidth=0.15](440,-5)(440,95)
\psline[linewidth=0.15](500,25)(500,95)
\psline[linewidth=0.15](470,-5)(500,25)
\psline[linewidth=0.15](440,-5)(470,-5)
\rput(475,20){$\aahh$}
\psline[linewidth=0.15](260,155)(320,155)
\psline[linewidth=0.15](260,55)(260,155)
\psline[linewidth=0.15](320,85)(320,155)
\psline[linewidth=0.15](290,55)(320,85)
\psline[linewidth=0.15](260,55)(290,55)
\rput(295,80){$\aahh$}
\end{pspicture}


==> PIC/fixp-6.tex <==
%%Created by jPicEdt 1.4.1_03: mixed JPIC-XML/LaTeX format
%%Sat May 22 13:50:03 GMT-10:00 2021
%%Begin JPIC-XML
%<?xml version="1.0" standalone="yes"?>
%<jpic x-min="0" x-max="350" y-min="5" y-max="198.75" auto-bounding="true">
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(92.5,135)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\gee$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(32.5,158.75)"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\nameslang$
%</text>
%<multicurve fill-style= "none"
%	 points= "(20,110);(20,110);(40,110);(40,110)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(0,130);(0,130);(20,110);(20,110)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(30,110);(30,110);(30,50);(30,50)"
%	 stroke-width= "0.6"
%	 />
%<multicurve fill-style= "none"
%	 points= "(10,120);(10,120);(10,90);(10,90)"
%	 stroke-width= "0.6"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(30,120)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\universal
%</text>
%<multicurve fill-style= "none"
%	 points= "(0,130);(0,130);(40,130);(40,130)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(30,160);(30,160);(30,130);(30,130)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(40,110);(40,110);(40,130);(40,130)"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(55,120)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\EQLS
%</text>
%<multicurve fill-style= "none"
%	 points= "(0,100);(0,100);(0,80);(0,80)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(0,80);(0,80);(20,80);(20,80)"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(5,85)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\program
%</text>
%<multicurve fill-style= "none"
%	 points= "(0,100);(0,100);(20,80);(20,80)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(102.5,125);(102.5,125);(102.5,145);(102.5,145)"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(95,158.75)"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\nameslang$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(90,120)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\inputt$
%</text>
%<multicurve fill-style= "none"
%	 points= "(82.5,125);(82.5,125);(102.5,125);(102.5,125)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(92.5,125);(92.5,125);(92.5,115);(92.5,115)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(102.5,95);(102.5,95);(82.5,95);(82.5,95)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(62.5,115);(62.5,115);(102.5,115);(102.5,115)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(62.5,115);(62.5,115);(82.5,95);(82.5,95)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(92.5,95);(92.5,95);(92.5,90);(92.5,90)"
%	 stroke-width= "0.6"
%	 />
%<multicurve fill-style= "none"
%	 points= "(72.5,105);(72.5,105);(72.5,55);(72.5,55)"
%	 stroke-width= "0.6"
%	 />
%<multicurve fill-style= "none"
%	 points= "(92.5,90);(92.5,90);(72.5,70);(72.5,70)"
%	 stroke-width= "0.6"
%	 />
%<multicurve fill-style= "none"
%	 points= "(82.5,145);(82.5,145);(102.5,145);(102.5,145)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(82.5,145);(82.5,145);(82.5,125);(82.5,125)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(92.5,155);(92.5,155);(92.5,145);(92.5,145)"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(27.5,50)"
%	 text-frame= "noframe"
%	 stroke-width= "0.35"
%	 text-hor-align= "right"
%	 >
%$\progtype$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(7.5,110)"
%	 text-frame= "noframe"
%	 stroke-width= "0.35"
%	 text-hor-align= "right"
%	 >
%$\progtype$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(70,55)"
%	 text-frame= "noframe"
%	 stroke-width= "0.35"
%	 text-hor-align= "right"
%	 >
%$\progtype$
%</text>
%<multicurve fill-style= "none"
%	 points= "(102.5,95);(102.5,95);(102.5,115);(102.5,115)"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(92.5,105)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\universal
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(130,120)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\thennn
%</text>
%<multicurve fill-style= "none"
%	 points= "(155,135);(155,135);(205,135);(205,135)"
%	 stroke-width= "0.15"
%	 />
%<multicurve fill-style= "none"
%	 points= "(155,55);(155,55);(155,135);(155,135)"
%	 stroke-width= "0.15"
%	 />
%<multicurve fill-style= "none"
%	 points= "(205,75);(205,75);(205,135);(205,135)"
%	 stroke-width= "0.15"
%	 />
%<multicurve fill-style= "none"
%	 points= "(185,55);(185,55);(205,75);(205,75)"
%	 stroke-width= "0.15"
%	 />
%<multicurve fill-style= "none"
%	 points= "(155,55);(155,55);(185,55);(185,55)"
%	 stroke-width= "0.15"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(190,80)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\aahh$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(72.5,70)"
%	 text-frame= "noframe"
%	 stroke-width= "0.2"
%	 text-hor-align= "center-h"
%	 >
%\DOTT
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(10,90)"
%	 text-frame= "noframe"
%	 stroke-width= "0.2"
%	 text-hor-align= "center-h"
%	 >
%\DOTT
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(187.5,140)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\inputt$
%</text>
%<multicurve fill-style= "none"
%	 points= "(190,150);(190,150);(190,130);(190,130)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(200,110);(200,110);(180,110);(180,110)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(160,130);(160,130);(200,130);(200,130)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(160,130);(160,130);(180,110);(180,110)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(190,110);(190,110);(190,105);(190,105)"
%	 stroke-width= "0.6"
%	 />
%<multicurve fill-style= "none"
%	 points= "(170,120);(170,120);(170,70);(170,70)"
%	 stroke-width= "0.6"
%	 />
%<multicurve fill-style= "none"
%	 points= "(190,105);(190,105);(170,85);(170,85)"
%	 stroke-width= "0.6"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(167.5,110)"
%	 text-frame= "noframe"
%	 stroke-width= "0.35"
%	 text-hor-align= "right"
%	 >
%$\progtype$
%</text>
%<multicurve fill-style= "none"
%	 points= "(200,110);(200,110);(200,130);(200,130)"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(190,120)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\universal
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(170,85)"
%	 text-frame= "noframe"
%	 stroke-width= "0.2"
%	 text-hor-align= "center-h"
%	 >
%\DOTT
%</text>
%<multicurve fill-style= "none"
%	 points= "(160,80);(160,80);(160,60);(160,60)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(160,60);(160,60);(180,60);(180,60)"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(165,65)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\program
%</text>
%<multicurve fill-style= "none"
%	 points= "(160,80);(160,80);(180,60);(180,60)"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(170,70)"
%	 text-frame= "noframe"
%	 stroke-width= "0.2"
%	 text-hor-align= "center-h"
%	 >
%\DOTT
%</text>
%<multicurve fill-style= "none"
%	 points= "(255,110);(255,110);(275,110);(275,110)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(235,130);(235,130);(255,110);(255,110)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(265,110);(265,110);(265,55);(265,55)"
%	 stroke-width= "0.6"
%	 />
%<multicurve fill-style= "none"
%	 points= "(245,120);(245,120);(245,90);(245,90)"
%	 stroke-width= "0.6"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(265,120)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\universal
%</text>
%<multicurve fill-style= "none"
%	 points= "(235,130);(235,130);(275,130);(275,130)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(265,160);(265,160);(265,130);(265,130)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(275,110);(275,110);(275,130);(275,130)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(235,100);(235,100);(235,80);(235,80)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(235,80);(235,80);(255,80);(255,80)"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(240,85)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\program
%</text>
%<multicurve fill-style= "none"
%	 points= "(235,100);(235,100);(255,80);(255,80)"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(260,100)"
%	 text-frame= "noframe"
%	 stroke-width= "0.35"
%	 text-hor-align= "right"
%	 >
%$\progtype$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(242.5,110)"
%	 text-frame= "noframe"
%	 stroke-width= "0.35"
%	 text-hor-align= "right"
%	 >
%$\progtype$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(245,90)"
%	 text-frame= "noframe"
%	 stroke-width= "0.2"
%	 text-hor-align= "center-h"
%	 >
%\DOTT
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(220,120)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\EQLS
%</text>
%<multicurve fill-style= "none"
%	 points= "(200,180);(200,180);(200,160);(200,160)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(200,160);(200,160);(220,160);(220,160)"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(205,165)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\program
%</text>
%<multicurve fill-style= "none"
%	 points= "(200,180);(200,180);(220,160);(220,160)"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(210,170)"
%	 text-frame= "noframe"
%	 stroke-width= "0.2"
%	 text-hor-align= "center-h"
%	 >
%\DOTT
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(290,120)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\EQLS
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(337.5,135)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\gee$
%</text>
%<multicurve fill-style= "none"
%	 points= "(347.5,125);(347.5,125);(347.5,145);(347.5,145)"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(335,198.75)"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\nameslang$
%</text>
%<multicurve fill-style= "none"
%	 points= "(327.5,125);(327.5,125);(347.5,125);(347.5,125)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(327.5,145);(327.5,145);(347.5,145);(347.5,145)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(327.5,145);(327.5,145);(327.5,125);(327.5,125)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(337.5,155);(337.5,155);(337.5,145);(337.5,145)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(270,25);(270,25);(270,5);(270,5)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(270,5);(270,5);(290,5);(290,5)"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(275,10)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\program
%</text>
%<multicurve fill-style= "none"
%	 points= "(270,25);(270,25);(290,5);(290,5)"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(280,15)"
%	 text-frame= "noframe"
%	 stroke-width= "0.2"
%	 text-hor-align= "center-h"
%	 >
%\DOTT
%</text>
%<multicurve fill-style= "none"
%	 points= "(300,120);(300,120);(350,120);(350,120)"
%	 stroke-width= "0.15"
%	 />
%<multicurve fill-style= "none"
%	 points= "(300,40);(300,40);(300,120);(300,120)"
%	 stroke-width= "0.15"
%	 />
%<multicurve fill-style= "none"
%	 points= "(350,60);(350,60);(350,120);(350,120)"
%	 stroke-width= "0.15"
%	 />
%<multicurve fill-style= "none"
%	 points= "(330,40);(330,40);(350,60);(350,60)"
%	 stroke-width= "0.15"
%	 />
%<multicurve fill-style= "none"
%	 points= "(300,40);(300,40);(330,40);(330,40)"
%	 stroke-width= "0.15"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(335,65)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\aahh$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(300,160)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\inputt$
%</text>
%<multicurve fill-style= "none"
%	 points= "(335,125);(335,125);(335,115);(335,115)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(345,95);(345,95);(325,95);(325,95)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(305,115);(305,115);(345,115);(345,115)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(305,115);(305,115);(325,95);(325,95)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(335,95);(335,95);(335,90);(335,90)"
%	 stroke-width= "0.6"
%	 />
%<multicurve fill-style= "none"
%	 points= "(315,105);(315,105);(315,55);(315,55)"
%	 stroke-width= "0.6"
%	 />
%<multicurve fill-style= "none"
%	 points= "(335,90);(335,90);(315,70);(315,70)"
%	 stroke-width= "0.6"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(312.5,95)"
%	 text-frame= "noframe"
%	 stroke-width= "0.35"
%	 text-hor-align= "right"
%	 >
%$\progtype$
%</text>
%<multicurve fill-style= "none"
%	 points= "(345,95);(345,95);(345,115);(345,115)"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(335,105)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\universal
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(315,70)"
%	 text-frame= "noframe"
%	 stroke-width= "0.2"
%	 text-hor-align= "center-h"
%	 >
%\DOTT
%</text>
%<multicurve fill-style= "none"
%	 points= "(305,65);(305,65);(305,45);(305,45)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(305,45);(305,45);(325,45);(325,45)"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(310,50)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\program
%</text>
%<multicurve fill-style= "none"
%	 points= "(305,65);(305,65);(325,45);(325,45)"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(315,55)"
%	 text-frame= "noframe"
%	 stroke-width= "0.2"
%	 text-hor-align= "center-h"
%	 >
%\DOTT
%</text>
%</jpic>
%%End JPIC-XML
%LaTeX-picture environment using emulated lines and arcs
%You can rescale the whole picture (to 80% for instance) by using the command \def\JPicScale{0.8}
\ifx\JPicScale\undefined\def\JPicScale{1}\fi
\unitlength \JPicScale mm
\begin{picture}(350,198.75)(0,0)
\put(92.5,135){\makebox(0,0)[cc]{$\gee$}}

\put(32.5,158.75){\makebox(0,0)[cl]{$\nameslang$}}

\linethickness{0.3mm}
\put(20,110){\line(1,0){20}}
\linethickness{0.3mm}
\multiput(0,130)(0.12,-0.12){167}{\line(1,0){0.12}}
\linethickness{0.6mm}
\put(30,50){\line(0,1){60}}
\linethickness{0.6mm}
\put(10,90){\line(0,1){30}}
\put(30,120){\makebox(0,0)[cc]{\universal}}

\linethickness{0.3mm}
\put(0,130){\line(1,0){40}}
\linethickness{0.3mm}
\put(30,130){\line(0,1){30}}
\linethickness{0.3mm}
\put(40,110){\line(0,1){20}}
\put(55,120){\makebox(0,0)[cc]{\EQLS}}

\linethickness{0.3mm}
\put(0,80){\line(0,1){20}}
\linethickness{0.3mm}
\put(0,80){\line(1,0){20}}
\put(5,85){\makebox(0,0)[cc]{\program}}

\linethickness{0.3mm}
\multiput(0,100)(0.12,-0.12){167}{\line(1,0){0.12}}
\linethickness{0.3mm}
\put(102.5,125){\line(0,1){20}}
\put(95,158.75){\makebox(0,0)[cl]{$\nameslang$}}

\put(90,120){\makebox(0,0)[cr]{$\inputt$}}

\linethickness{0.3mm}
\put(82.5,125){\line(1,0){20}}
\linethickness{0.3mm}
\put(92.5,115){\line(0,1){10}}
\linethickness{0.3mm}
\put(82.5,95){\line(1,0){20}}
\linethickness{0.3mm}
\put(62.5,115){\line(1,0){40}}
\linethickness{0.3mm}
\multiput(62.5,115)(0.12,-0.12){167}{\line(1,0){0.12}}
\linethickness{0.6mm}
\put(92.5,90){\line(0,1){5}}
\linethickness{0.6mm}
\put(72.5,55){\line(0,1){50}}
\linethickness{0.6mm}
\multiput(72.5,70)(0.12,0.12){167}{\line(1,0){0.12}}
\linethickness{0.3mm}
\put(82.5,145){\line(1,0){20}}
\linethickness{0.3mm}
\put(82.5,125){\line(0,1){20}}
\linethickness{0.3mm}
\put(92.5,145){\line(0,1){10}}
\put(27.5,50){\makebox(0,0)[cr]{$\progtype$}}

\put(7.5,110){\makebox(0,0)[cr]{$\progtype$}}

\put(70,55){\makebox(0,0)[cr]{$\progtype$}}

\linethickness{0.3mm}
\put(102.5,95){\line(0,1){20}}
\put(92.5,105){\makebox(0,0)[cc]{\universal}}

\put(130,120){\makebox(0,0)[cc]{\thennn}}

\linethickness{0.15mm}
\put(155,135){\line(1,0){50}}
\linethickness{0.15mm}
\put(155,55){\line(0,1){80}}
\linethickness{0.15mm}
\put(205,75){\line(0,1){60}}
\linethickness{0.15mm}
\multiput(185,55)(0.12,0.12){167}{\line(1,0){0.12}}
\linethickness{0.15mm}
\put(155,55){\line(1,0){30}}
\put(190,80){\makebox(0,0)[cc]{$\aahh$}}

\put(72.5,70){\makebox(0,0)[cc]{\DOTT}}

\put(10,90){\makebox(0,0)[cc]{\DOTT}}

\put(187.5,140){\makebox(0,0)[cr]{$\inputt$}}

\linethickness{0.3mm}
\put(190,130){\line(0,1){20}}
\linethickness{0.3mm}
\put(180,110){\line(1,0){20}}
\linethickness{0.3mm}
\put(160,130){\line(1,0){40}}
\linethickness{0.3mm}
\multiput(160,130)(0.12,-0.12){167}{\line(1,0){0.12}}
\linethickness{0.6mm}
\put(190,105){\line(0,1){5}}
\linethickness{0.6mm}
\put(170,70){\line(0,1){50}}
\linethickness{0.6mm}
\multiput(170,85)(0.12,0.12){167}{\line(1,0){0.12}}
\put(167.5,110){\makebox(0,0)[cr]{$\progtype$}}

\linethickness{0.3mm}
\put(200,110){\line(0,1){20}}
\put(190,120){\makebox(0,0)[cc]{\universal}}

\put(170,85){\makebox(0,0)[cc]{\DOTT}}

\linethickness{0.3mm}
\put(160,60){\line(0,1){20}}
\linethickness{0.3mm}
\put(160,60){\line(1,0){20}}
\put(165,65){\makebox(0,0)[cc]{\program}}

\linethickness{0.3mm}
\multiput(160,80)(0.12,-0.12){167}{\line(1,0){0.12}}
\put(170,70){\makebox(0,0)[cc]{\DOTT}}

\linethickness{0.3mm}
\put(255,110){\line(1,0){20}}
\linethickness{0.3mm}
\multiput(235,130)(0.12,-0.12){167}{\line(1,0){0.12}}
\linethickness{0.6mm}
\put(265,55){\line(0,1){55}}
\linethickness{0.6mm}
\put(245,90){\line(0,1){30}}
\put(265,120){\makebox(0,0)[cc]{\universal}}

\linethickness{0.3mm}
\put(235,130){\line(1,0){40}}
\linethickness{0.3mm}
\put(265,130){\line(0,1){30}}
\linethickness{0.3mm}
\put(275,110){\line(0,1){20}}
\linethickness{0.3mm}
\put(235,80){\line(0,1){20}}
\linethickness{0.3mm}
\put(235,80){\line(1,0){20}}
\put(240,85){\makebox(0,0)[cc]{\program}}

\linethickness{0.3mm}
\multiput(235,100)(0.12,-0.12){167}{\line(1,0){0.12}}
\put(260,100){\makebox(0,0)[cr]{$\progtype$}}

\put(242.5,110){\makebox(0,0)[cr]{$\progtype$}}

\put(245,90){\makebox(0,0)[cc]{\DOTT}}

\put(220,120){\makebox(0,0)[cc]{\EQLS}}

\linethickness{0.3mm}
\put(200,160){\line(0,1){20}}
\linethickness{0.3mm}
\put(200,160){\line(1,0){20}}
\put(205,165){\makebox(0,0)[cc]{\program}}

\linethickness{0.3mm}
\multiput(200,180)(0.12,-0.12){167}{\line(1,0){0.12}}
\put(210,170){\makebox(0,0)[cc]{\DOTT}}

\put(290,120){\makebox(0,0)[cc]{\EQLS}}

\put(337.5,135){\makebox(0,0)[cc]{$\gee$}}

\linethickness{0.3mm}
\put(347.5,125){\line(0,1){20}}
\put(335,198.75){\makebox(0,0)[cl]{$\nameslang$}}

\linethickness{0.3mm}
\put(327.5,125){\line(1,0){20}}
\linethickness{0.3mm}
\put(327.5,145){\line(1,0){20}}
\linethickness{0.3mm}
\put(327.5,125){\line(0,1){20}}
\linethickness{0.3mm}
\put(337.5,145){\line(0,1){10}}
\linethickness{0.3mm}
\put(270,5){\line(0,1){20}}
\linethickness{0.3mm}
\put(270,5){\line(1,0){20}}
\put(275,10){\makebox(0,0)[cc]{\program}}

\linethickness{0.3mm}
\multiput(270,25)(0.12,-0.12){167}{\line(1,0){0.12}}
\put(280,15){\makebox(0,0)[cc]{\DOTT}}

\linethickness{0.15mm}
\put(300,120){\line(1,0){50}}
\linethickness{0.15mm}
\put(300,40){\line(0,1){80}}
\linethickness{0.15mm}
\put(350,60){\line(0,1){60}}
\linethickness{0.15mm}
\multiput(330,40)(0.12,0.12){167}{\line(1,0){0.12}}
\linethickness{0.15mm}
\put(300,40){\line(1,0){30}}
\put(335,65){\makebox(0,0)[cc]{$\aahh$}}

\put(300,160){\makebox(0,0)[cr]{$\inputt$}}

\linethickness{0.3mm}
\put(335,115){\line(0,1){10}}
\linethickness{0.3mm}
\put(325,95){\line(1,0){20}}
\linethickness{0.3mm}
\put(305,115){\line(1,0){40}}
\linethickness{0.3mm}
\multiput(305,115)(0.12,-0.12){167}{\line(1,0){0.12}}
\linethickness{0.6mm}
\put(335,90){\line(0,1){5}}
\linethickness{0.6mm}
\put(315,55){\line(0,1){50}}
\linethickness{0.6mm}
\multiput(315,70)(0.12,0.12){167}{\line(1,0){0.12}}
\put(312.5,95){\makebox(0,0)[cr]{$\progtype$}}

\linethickness{0.3mm}
\put(345,95){\line(0,1){20}}
\put(335,105){\makebox(0,0)[cc]{\universal}}

\put(315,70){\makebox(0,0)[cc]{\DOTT}}

\linethickness{0.3mm}
\put(305,45){\line(0,1){20}}
\linethickness{0.3mm}
\put(305,45){\line(1,0){20}}
\put(310,50){\makebox(0,0)[cc]{\program}}

\linethickness{0.3mm}
\multiput(305,65)(0.12,-0.12){167}{\line(1,0){0.12}}
\put(315,55){\makebox(0,0)[cc]{\DOTT}}

\end{picture}


==> PIC/fixp-kleene-noM.tex <==
%%Created by jPicEdt 1.4.1_03: mixed JPIC-XML/LaTeX format
%%Tue Nov 05 19:27:16 GMT-10:00 2019
%%Begin JPIC-XML
%<?xml version="1.0" standalone="yes"?>
%<jpic x-min="0" x-max="270" y-min="0" y-max="115.62" auto-bounding="true">
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(65,45);(65,45);(65,65);(65,65)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(30,45);(30,45);(65,45);(65,45)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(40,45);(40,45);(40,0);(40,0)"
%	 />
%<ellipse p3= "(42.58,22.42)"
%	 p2= "(42.58,27.58)"
%	 fill-color= "#330033"
%	 p1= "(37.42,27.58)"
%	 closure= "open"
%	 fill-style= "solid"
%	 angle-end= "0"
%	 angle-start= "0"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(30,95);(30,95);(0,65);(0,65)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(0,65);(0,65);(40,25);(40,25)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(60,85);(60,85);(60,105);(60,105)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(40,85);(40,85);(60,85);(60,85)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(20,105);(20,105);(40,85);(40,85)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(165,45);(165,45);(165,65);(165,65)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(130,45);(130,45);(165,45);(165,45)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(140,45);(140,45);(140,0);(140,0)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(120,55.01);(120,55.01);(120,25);(120,25)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(110,65);(110,65);(130,45);(130,45)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(10,35);(10,35);(10,15);(10,15)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(30,15);(30,15);(10,15);(10,15)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(110,35);(110,35);(110,15);(110,15)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(110,35);(110,35);(130,15);(130,15)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(130,15);(130,15);(110,15);(110,15)"
%	 />
%<multicurve stroke-overstrike= "true"
%	 stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(20,55);(20,55);(20,25);(20,25)"
%	 stroke-overstrike-width= "1"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(10,35);(10,35);(30,15);(30,15)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(10,65);(10,65);(30,45);(30,45)"
%	 />
%<text text-vert-align= "center-v"
%	 anchor-point= "(85,55)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\EQLS
%</text>
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(270,55);(270,55);(270,75);(270,75)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(232.5,35);(232.5,35);(252.5,35);(252.5,35)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(242.5,35);(242.5,35);(242.5,0);(242.5,0)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(222.5,45);(222.5,45);(222.5,25);(222.5,25)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(212.5,55);(212.5,55);(232.5,35);(232.5,35)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(212.5,35);(212.5,35);(212.5,15);(212.5,15)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(212.5,35);(212.5,35);(232.5,15);(232.5,15)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(232.5,15);(232.5,15);(212.5,15);(212.5,15)"
%	 />
%<text text-vert-align= "center-v"
%	 anchor-point= "(185,55)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\EQLS
%</text>
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(212.5,55);(212.5,55);(232.5,55);(232.5,55)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(232.5,55);(232.5,55);(252.5,35);(252.5,35)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(232.5,75);(232.5,75);(252.5,55);(252.5,55)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(242.5,65);(242.5,65);(242.5,45);(242.5,45)"
%	 />
%<multicurve stroke-width= "0.5"
%	 fill-style= "none"
%	 points= "(235,62.5);(235,62.5);(257.5,40);(257.5,40)"
%	 />
%<multicurve stroke-width= "0.5"
%	 fill-style= "none"
%	 points= "(205,62.5);(205,62.5);(205,10);(205,10)"
%	 />
%<multicurve stroke-width= "0.5"
%	 fill-style= "none"
%	 points= "(235,62.5);(235,62.5);(205,62.5);(205,62.5)"
%	 />
%<multicurve stroke-width= "0.5"
%	 fill-style= "none"
%	 points= "(257.5,10);(257.5,10);(205,10);(205,10)"
%	 />
%<multicurve stroke-width= "0.5"
%	 fill-style= "none"
%	 points= "(257.5,10);(257.5,10);(257.5,40);(257.5,40)"
%	 />
%<text text-vert-align= "center-v"
%	 anchor-point= "(16.25,21.25)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\PsiT$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(116.25,21.25)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\PsiT$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(218.75,21.25)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\PsiT$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(251.25,16.25)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\psiT$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(47.5,55)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\universal$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(147.5,55)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\universal$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(255,65)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\smalluniversal$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(232.5,45)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\partev$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(137.5,2.5)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\Progtype$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(240,2.5)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\Progtype$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(267.5,85)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\Atype$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(152.5,82.5)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\Atype$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(52.5,113.75)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\Atype$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(52.5,73.75)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\Atype$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(37.5,2.5)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\Progtype$
%</text>
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(57.5,45);(57.5,45);(57.5,0);(57.5,0)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(157.5,45);(157.5,45);(157.5,0);(157.5,0)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(252.5,55);(252.5,55);(270,55);(270,55)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(265,55);(265,55);(265,0);(265,0)"
%	 />
%<text text-vert-align= "center-v"
%	 anchor-point= "(262.5,2.5)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\Atype$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(155,2.5)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\Atype$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(55,2.5)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\Atype$
%</text>
%<parallelogram p3= "(47.5,115.62)"
%	 p2= "(47.5,105)"
%	 fill-color= "#999999"
%	 p1= "(52.5,105)"
%	 stroke-color= "#999999"
%	 fill-style= "solid"
%	 />
%<parallelogram p3= "(47.5,84.38)"
%	 p2= "(47.5,65.62)"
%	 fill-color= "#999999"
%	 p1= "(52.5,65.62)"
%	 stroke-color= "#999999"
%	 fill-style= "solid"
%	 />
%<parallelogram p3= "(147.5,85)"
%	 p2= "(147.5,65.62)"
%	 fill-color= "#999999"
%	 p1= "(152.5,65.62)"
%	 stroke-color= "#999999"
%	 fill-style= "solid"
%	 />
%<parallelogram p3= "(262.5,86.88)"
%	 p2= "(262.5,75)"
%	 fill-color= "#999999"
%	 p1= "(267.5,75)"
%	 stroke-color= "#999999"
%	 fill-style= "solid"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(10,65);(10,65);(65,65);(65,65)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(20,105);(20,105);(60,105);(60,105)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(50,115);(50,115);(50,105);(50,105)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(110,65);(110,65);(165,65);(165,65)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(150,85);(150,85);(150,65);(150,65)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(232.5,75);(232.5,75);(270,75);(270,75)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(265,86.25);(265,86.25);(265,75);(265,75)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(50,85);(50,85);(50,65);(50,65)"
%	 />
%<text text-vert-align= "center-v"
%	 anchor-point= "(48.12,96.25)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\universallift$
%</text>
%</jpic>
%%End JPIC-XML
%PSTricks content-type (pstricks.sty package needed)
%Add \usepackage{pstricks} in the preamble of your LaTeX file
%You can rescale the whole picture (to 80% for instance) by using the command \def\JPicScale{0.8}
\ifx\JPicScale\undefined\def\JPicScale{1}\fi
\psset{unit=\JPicScale mm}
\psset{linewidth=0.3,dotsep=1,hatchwidth=0.3,hatchsep=1.5,shadowsize=1,dimen=middle}
\psset{dotsize=0.7 2.5,dotscale=1 1,fillcolor=black}
\psset{arrowsize=1 2,arrowlength=1,arrowinset=0.25,tbarsize=0.7 5,bracketlength=0.15,rbracketlength=0.15}
\begin{pspicture}(0,0)(270,115.62)
\psline[linewidth=0.75](65,45)(65,65)
\psline[linewidth=0.75](30,45)(65,45)
\psline[linewidth=0.75](40,45)(40,0)
\newrgbcolor{userFillColour}{0.2 0 0.2}
\rput{0}(40,25){\psellipse[fillcolor=userFillColour,fillstyle=solid](0,0)(2.58,-2.58)}
\psline[linewidth=0.75](30,95)(0,65)
\psline[linewidth=0.75](0,65)(40,25)
\psline[linewidth=0.75](60,85)(60,105)
\psline[linewidth=0.75](40,85)(60,85)
\psline[linewidth=0.75](20,105)(40,85)
\psline[linewidth=0.75](165,45)(165,65)
\psline[linewidth=0.75](130,45)(165,45)
\psline[linewidth=0.75](140,45)(140,0)
\psline[linewidth=0.75](120,55.01)(120,25)
\psline[linewidth=0.75](110,65)(130,45)
\psline[linewidth=0.75](10,35)(10,15)
\psline[linewidth=0.75](30,15)(10,15)
\psline[linewidth=0.75](110,35)(110,15)
\psline[linewidth=0.75](110,35)(130,15)
\psline[linewidth=0.75](130,15)(110,15)
\psline[linewidth=0.75,border=1](20,55)(20,25)
\psline[linewidth=0.75](10,35)(30,15)
\psline[linewidth=0.75](10,65)(30,45)
\rput(85,55){\EQLS}
\psline[linewidth=0.75](270,55)(270,75)
\psline[linewidth=0.75](232.5,35)(252.5,35)
\psline[linewidth=0.75](242.5,35)(242.5,0)
\psline[linewidth=0.75](222.5,45)(222.5,25)
\psline[linewidth=0.75](212.5,55)(232.5,35)
\psline[linewidth=0.75](212.5,35)(212.5,15)
\psline[linewidth=0.75](212.5,35)(232.5,15)
\psline[linewidth=0.75](232.5,15)(212.5,15)
\rput(185,55){\EQLS}
\psline[linewidth=0.75](212.5,55)(232.5,55)
\psline[linewidth=0.75](232.5,55)(252.5,35)
\psline[linewidth=0.75](232.5,75)(252.5,55)
\psline[linewidth=0.75](242.5,65)(242.5,45)
\psline[linewidth=0.5](235,62.5)(257.5,40)
\psline[linewidth=0.5](205,62.5)(205,10)
\psline[linewidth=0.5](235,62.5)(205,62.5)
\psline[linewidth=0.5](257.5,10)(205,10)
\psline[linewidth=0.5](257.5,10)(257.5,40)
\rput(16.25,21.25){$\PsiT$}
\rput(116.25,21.25){$\PsiT$}
\rput(218.75,21.25){$\PsiT$}
\rput(251.25,16.25){$\psiT$}
\rput(47.5,55){$\universal$}
\rput(147.5,55){$\universal$}
\rput(255,65){$\smalluniversal$}
\rput(232.5,45){$\partev$}
\rput[r](137.5,2.5){$\Progtype$}
\rput[r](240,2.5){$\Progtype$}
\rput[l](267.5,85){$\Atype$}
\rput[l](152.5,82.5){$\Atype$}
\rput[l](52.5,113.75){$\Atype$}
\rput[l](52.5,73.75){$\Atype$}
\rput[r](37.5,2.5){$\Progtype$}
\psline[linewidth=0.75](57.5,45)(57.5,0)
\psline[linewidth=0.75](157.5,45)(157.5,0)
\psline[linewidth=0.75](252.5,55)(270,55)
\psline[linewidth=0.75](265,55)(265,0)
\rput[r](262.5,2.5){$\Atype$}
\rput[r](155,2.5){$\Atype$}
\rput[r](55,2.5){$\Atype$}
\newrgbcolor{userLineColour}{0.6 0.6 0.6}
\newrgbcolor{userFillColour}{0.6 0.6 0.6}
\newrgbcolor{userLineColour}{0.6 0.6 0.6}
\newrgbcolor{userFillColour}{0.6 0.6 0.6}
\newrgbcolor{userLineColour}{0.6 0.6 0.6}
\newrgbcolor{userFillColour}{0.6 0.6 0.6}
\newrgbcolor{userLineColour}{0.6 0.6 0.6}
\newrgbcolor{userFillColour}{0.6 0.6 0.6}
\psline[linewidth=0.75](10,65)(65,65)
\psline[linewidth=0.75](20,105)(60,105)
\psline[linewidth=0.75](50,115)(50,105)
\psline[linewidth=0.75](110,65)(165,65)
\psline[linewidth=0.75](150,85)(150,65)
\psline[linewidth=0.75](232.5,75)(270,75)
\psline[linewidth=0.75](265,86.25)(265,75)
\psline[linewidth=0.75](50,85)(50,65)
\rput(48.12,96.25){$\universallift$}
\end{pspicture}


==> PIC/fixp-turing-1.tex <==
%%Created by jPicEdt 1.4.1_03: mixed JPIC-XML/LaTeX format
%%Sun May 23 15:38:22 GMT-10:00 2021
%%Begin JPIC-XML
%<?xml version="1.0" standalone="yes"?>
%<jpic x-min="0" x-max="130" y-min="-1.25" y-max="105" auto-bounding="true">
%<multicurve fill-style= "none"
%	 points= "(50,35);(50,35);(50,55);(50,55)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(30,35);(30,35);(50,35);(50,35)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(40,35);(40,35);(40,0);(40,0)"
%	 />
%<ellipse fill-color= "#330033"
%	 fill-style= "solid"
%	 p3= "(42.58,12.42)"
%	 p2= "(42.58,17.58)"
%	 p1= "(37.42,17.58)"
%	 closure= "open"
%	 angle-end= "0"
%	 angle-start= "0"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(20,75);(20,75);(0,55);(0,55)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(50,75);(50,75);(50,95);(50,95)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(20,85.01);(20,85.01);(20,75);(20,75)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(10,95);(10,95);(30,75);(30,75)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(130,35);(130,35);(130,55);(130,55)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(110,35);(110,35);(130,35);(130,35)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(120,35);(120,35);(120,0);(120,0)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(100,45.01);(100,45.01);(100,15);(100,15)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(90,55);(90,55);(110,35);(110,35)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(10,25);(10,25);(10,5);(10,5)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(30,5);(30,5);(10,5);(10,5)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(90,25);(90,25);(90,5);(90,5)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(90,25);(90,25);(110,5);(110,5)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(110,5);(110,5);(90,5);(90,5)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(10,25);(10,25);(30,5);(30,5)"
%	 />
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(70,45)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\EQLS
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(15,10)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\PsiT$
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(95,10)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\PsiT$
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(37.5,45)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\universal$
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(117.5,45)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\universal$
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(117.5,-1.25)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\Progtype$
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(125,75)"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\Atype$
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(44.38,105)"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\Atype$
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(44.38,64.38)"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\Atype$
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(37.5,-1.25)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\Progtype$
%</text>
%<multicurve fill-style= "none"
%	 points= "(90,55);(90,55);(130,55);(130,55)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(120,75);(120,75);(120,55);(120,55)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(30,75);(30,75);(50,75);(50,75)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(10,55);(10,55);(50,55);(50,55)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(40,75);(40,75);(40,55);(40,55)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(10,95);(10,95);(50,95);(50,95)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(40,105);(40,105);(40,95);(40,95)"
%	 />
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(38.75,86.25)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\universallift$
%</text>
%<ellipse fill-color= "#330033"
%	 fill-style= "solid"
%	 p3= "(102.58,12.42)"
%	 p2= "(102.58,17.58)"
%	 p1= "(97.42,17.58)"
%	 closure= "open"
%	 angle-end= "0"
%	 angle-start= "0"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(0,55);(0,55);(40,15);(40,15)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(20,45);(20,45);(20,15);(20,15)"
%	 stroke-overstrike= "true"
%	 stroke-overstrike-width= "1.3"
%	 />
%<ellipse fill-color= "#330033"
%	 fill-style= "solid"
%	 p3= "(22.58,12.42)"
%	 p2= "(22.58,17.58)"
%	 p1= "(17.42,17.58)"
%	 closure= "open"
%	 angle-end= "0"
%	 angle-start= "0"
%	 />
%<multicurve fill-style= "none"
%	 points= "(10,55);(10,55);(30,35);(30,35)"
%	 />
%</jpic>
%%End JPIC-XML
%PSTricks content-type (pstricks.sty package needed)
%Add \usepackage{pstricks} in the preamble of your LaTeX file
%You can rescale the whole picture (to 80% for instance) by using the command \def\JPicScale{0.8}
\ifx\JPicScale\undefined\def\JPicScale{1}\fi
\psset{unit=\JPicScale mm}
\psset{linewidth=0.3,dotsep=1,hatchwidth=0.3,hatchsep=1.5,shadowsize=1,dimen=middle}
\psset{dotsize=0.7 2.5,dotscale=1 1,fillcolor=black}
\psset{arrowsize=1 2,arrowlength=1,arrowinset=0.25,tbarsize=0.7 5,bracketlength=0.15,rbracketlength=0.15}
\begin{pspicture}(0,0)(130,105)
\psline(50,35)(50,55)
\psline(30,35)(50,35)
\psline[linewidth=0.75](40,35)(40,0)
\newrgbcolor{userFillColour}{0.2 0 0.2}
\rput{0}(40,15){\psellipse[fillcolor=userFillColour,fillstyle=solid](0,0)(2.58,-2.58)}
\psline[linewidth=0.75](20,75)(0,55)
\psline(50,75)(50,95)
\psline[linewidth=0.75](20,85.01)(20,75)
\psline(10,95)(30,75)
\psline(130,35)(130,55)
\psline(110,35)(130,35)
\psline(120,35)(120,0)
\psline[linewidth=0.75](100,45.01)(100,15)
\psline(90,55)(110,35)
\psline(10,25)(10,5)
\psline(30,5)(10,5)
\psline(90,25)(90,5)
\psline(90,25)(110,5)
\psline(110,5)(90,5)
\psline(10,25)(30,5)
\rput(70,45){\EQLS}
\rput(15,10){$\PsiT$}
\rput(95,10){$\PsiT$}
\rput(37.5,45){$\universal$}
\rput(117.5,45){$\universal$}
\rput[r](117.5,-1.25){$\Progtype$}
\rput[l](125,75){$\Atype$}
\rput[l](44.38,105){$\Atype$}
\rput[l](44.38,64.38){$\Atype$}
\rput[r](37.5,-1.25){$\Progtype$}
\psline(90,55)(130,55)
\psline(120,75)(120,55)
\psline(30,75)(50,75)
\psline(10,55)(50,55)
\psline(40,75)(40,55)
\psline(10,95)(50,95)
\psline(40,105)(40,95)
\rput(38.75,86.25){$\universallift$}
\newrgbcolor{userFillColour}{0.2 0 0.2}
\rput{0}(100,15){\psellipse[fillcolor=userFillColour,fillstyle=solid](0,0)(2.58,-2.58)}
\psline[linewidth=0.75](0,55)(40,15)
\psline[linewidth=0.75,border=1.3](20,45)(20,15)
\newrgbcolor{userFillColour}{0.2 0 0.2}
\rput{0}(20,15){\psellipse[fillcolor=userFillColour,fillstyle=solid](0,0)(2.58,-2.58)}
\psline(10,55)(30,35)
\end{pspicture}


==> PIC/fixp-turing-clas-noM.tex <==
%%Created by jPicEdt 1.4.1_03: mixed JPIC-XML/LaTeX format
%%Tue Nov 05 19:39:36 GMT-10:00 2019
%%Begin JPIC-XML
%<?xml version="1.0" standalone="yes"?>
%<jpic x-min="0" x-max="250" y-min="0" y-max="101.25" auto-bounding="true">
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(10,50);(10,50);(50,50);(50,50)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(50,30);(50,30);(50,50);(50,50)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(30,30);(30,30);(50,30);(50,30)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(40,30);(40,30);(40,0);(40,0)"
%	 />
%<ellipse p3= "(42.58,7.42)"
%	 p2= "(42.58,12.58)"
%	 fill-color= "#330033"
%	 p1= "(37.42,12.58)"
%	 closure= "open"
%	 fill-style= "solid"
%	 angle-end= "0"
%	 angle-start= "0"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(0,50);(0,50);(40,10);(40,10)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(90,40);(90,40);(90,20);(90,20)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(90,40);(90,40);(110,20);(110,20)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(110,20);(110,20);(90,20);(90,20)"
%	 />
%<multicurve stroke-overstrike= "true"
%	 stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(20,40);(20,40);(20,0);(20,0)"
%	 stroke-overstrike-width= "1"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(10,50);(10,50);(30,30);(30,30)"
%	 />
%<text text-vert-align= "center-v"
%	 anchor-point= "(70,60)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\EQLS
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(96.25,26.25)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\PsiT$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(37.5,40)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\universal$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(45,58.75)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\Atype$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(37.5,0)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\Progtype$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(17.5,0)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\Progtype$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(137.5,0)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\Progtype$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(117.5,0)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\Progtype$
%</text>
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(220,40);(220,40);(220,0);(220,0)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(200,50);(200,50);(200,30);(200,30)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(190,60);(190,60);(210,40);(210,40)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(190,40);(190,40);(190,20);(190,20)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(190,40);(190,40);(210,20);(210,20)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(210,20);(210,20);(190,20);(190,20)"
%	 />
%<text text-vert-align= "center-v"
%	 anchor-point= "(170,60)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\EQLS
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(196.25,26.25)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\PsiT$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(237.5,0)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\Progtype$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(217.5,0)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\Progtype$
%</text>
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(210,40);(210,40);(230,40);(230,40)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(210,60);(210,60);(230,40);(230,40)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(190,60);(190,60);(210,60);(210,60)"
%	 />
%<multicurve stroke-width= "0.5"
%	 fill-style= "none"
%	 points= "(215,66.25);(215,66.25);(235,46.25);(235,46.25)"
%	 />
%<multicurve stroke-width= "0.5"
%	 fill-style= "none"
%	 points= "(185,66.25);(185,66.25);(185,13.75);(185,13.75)"
%	 />
%<multicurve stroke-width= "0.5"
%	 fill-style= "none"
%	 points= "(215,66.25);(215,66.25);(185,66.25);(185,66.25)"
%	 />
%<multicurve stroke-width= "0.5"
%	 fill-style= "none"
%	 points= "(235,13.75);(235,13.75);(185,13.75);(185,13.75)"
%	 />
%<multicurve stroke-width= "0.5"
%	 fill-style= "none"
%	 points= "(235,13.75);(235,13.75);(235,46.25);(235,46.25)"
%	 />
%<text text-vert-align= "center-v"
%	 anchor-point= "(228.75,18.75)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\psiT$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(210,50)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\partev$
%</text>
%<parallelogram p3= "(37.5,70.78)"
%	 p2= "(37.5,50.47)"
%	 fill-color= "#999999"
%	 p1= "(42.5,50.47)"
%	 stroke-color= "#999999"
%	 fill-style= "solid"
%	 />
%<parallelogram p3= "(137.5,100)"
%	 p2= "(137.5,90.47)"
%	 fill-color= "#999999"
%	 p1= "(142.5,90.47)"
%	 stroke-color= "#999999"
%	 fill-style= "solid"
%	 />
%<parallelogram p3= "(237.5,100)"
%	 p2= "(237.5,90.47)"
%	 fill-color= "#999999"
%	 p1= "(242.5,90.47)"
%	 stroke-color= "#999999"
%	 fill-style= "solid"
%	 />
%<parallelogram p3= "(37.5,101.25)"
%	 p2= "(37.5,91.09)"
%	 fill-color= "#999999"
%	 p1= "(42.5,91.09)"
%	 stroke-color= "#999999"
%	 fill-style= "solid"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(40,70.62);(40,70.62);(40,50.62);(40,50.62)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(20,70.62);(20,70.62);(0,50.62);(0,50.62)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(10,90.62);(10,90.62);(50,90.62);(50,90.62)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(50,70.62);(50,70.62);(50,90.62);(50,90.62)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(40,100.62);(40,100.62);(40,90.62);(40,90.62)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(30,70.62);(30,70.62);(50,70.62);(50,70.62)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(20,80.64);(20,80.64);(20,70.62);(20,70.62)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(10,90.62);(10,90.62);(30,70.62);(30,70.62)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(90,90.62);(90,90.62);(150,90.62);(150,90.62)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(150,70.62);(150,70.62);(150,90.62);(150,90.62)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(140,99.38);(140,99.38);(140,90.62);(140,90.62)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(110,70.62);(110,70.62);(150,70.62);(150,70.62)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(120,70.62);(120,70.62);(120,0.62);(120,0.62)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(100,80.62);(100,80.62);(100,30.62);(100,30.62)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(90,90.62);(90,90.62);(110,70.62);(110,70.62)"
%	 />
%<text text-vert-align= "center-v"
%	 anchor-point= "(130,80.62)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\universal$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(144.38,99.38)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\Atype$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(44.38,100.62)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\Atype$
%</text>
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(140,70.62);(140,70.62);(140,0.62);(140,0.62)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(210,90.62);(210,90.62);(250,90.62);(250,90.62)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(250,70.62);(250,70.62);(250,90.62);(250,90.62)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(240,99.38);(240,99.38);(240,90.62);(240,90.62)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(230,70.62);(230,70.62);(250,70.62);(250,70.62)"
%	 />
%<text text-vert-align= "center-v"
%	 anchor-point= "(236.25,80.62)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\universal$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(244.38,99.38)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\Atype$
%</text>
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(240,70.62);(240,70.62);(240,0.62);(240,0.62)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(220,80.62);(220,80.62);(220,50.62);(220,50.62)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(210,90.62);(210,90.62);(230,70.62);(230,70.62)"
%	 />
%<text text-vert-align= "center-v"
%	 anchor-point= "(217.5,73.12)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\Progtype$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(37.5,81.88)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\universallift$
%</text>
%</jpic>
%%End JPIC-XML
%PSTricks content-type (pstricks.sty package needed)
%Add \usepackage{pstricks} in the preamble of your LaTeX file
%You can rescale the whole picture (to 80% for instance) by using the command \def\JPicScale{0.8}
\ifx\JPicScale\undefined\def\JPicScale{1}\fi
\psset{unit=\JPicScale mm}
\psset{linewidth=0.3,dotsep=1,hatchwidth=0.3,hatchsep=1.5,shadowsize=1,dimen=middle}
\psset{dotsize=0.7 2.5,dotscale=1 1,fillcolor=black}
\psset{arrowsize=1 2,arrowlength=1,arrowinset=0.25,tbarsize=0.7 5,bracketlength=0.15,rbracketlength=0.15}
\begin{pspicture}(0,0)(250,101.25)
\psline[linewidth=0.75](10,50)(50,50)
\psline[linewidth=0.75](50,30)(50,50)
\psline[linewidth=0.75](30,30)(50,30)
\psline[linewidth=0.75](40,30)(40,0)
\newrgbcolor{userFillColour}{0.2 0 0.2}
\rput{0}(40,10){\psellipse[fillcolor=userFillColour,fillstyle=solid](0,0)(2.58,-2.58)}
\psline[linewidth=0.75](0,50)(40,10)
\psline[linewidth=0.75](90,40)(90,20)
\psline[linewidth=0.75](90,40)(110,20)
\psline[linewidth=0.75](110,20)(90,20)
\psline[linewidth=0.75,border=1](20,40)(20,0)
\psline[linewidth=0.75](10,50)(30,30)
\rput(70,60){\EQLS}
\rput(96.25,26.25){$\PsiT$}
\rput(37.5,40){$\universal$}
\rput[l](45,58.75){$\Atype$}
\rput[r](37.5,0){$\Progtype$}
\rput[r](17.5,0){$\Progtype$}
\rput[r](137.5,0){$\Progtype$}
\rput[r](117.5,0){$\Progtype$}
\psline[linewidth=0.75](220,40)(220,0)
\psline[linewidth=0.75](200,50)(200,30)
\psline[linewidth=0.75](190,60)(210,40)
\psline[linewidth=0.75](190,40)(190,20)
\psline[linewidth=0.75](190,40)(210,20)
\psline[linewidth=0.75](210,20)(190,20)
\rput(170,60){\EQLS}
\rput(196.25,26.25){$\PsiT$}
\rput[r](237.5,0){$\Progtype$}
\rput[r](217.5,0){$\Progtype$}
\psline[linewidth=0.75](210,40)(230,40)
\psline[linewidth=0.75](210,60)(230,40)
\psline[linewidth=0.75](190,60)(210,60)
\psline[linewidth=0.5](215,66.25)(235,46.25)
\psline[linewidth=0.5](185,66.25)(185,13.75)
\psline[linewidth=0.5](215,66.25)(185,66.25)
\psline[linewidth=0.5](235,13.75)(185,13.75)
\psline[linewidth=0.5](235,13.75)(235,46.25)
\rput(228.75,18.75){$\psiT$}
\rput(210,50){$\partev$}
\newrgbcolor{userLineColour}{0.6 0.6 0.6}
\newrgbcolor{userFillColour}{0.6 0.6 0.6}
\newrgbcolor{userLineColour}{0.6 0.6 0.6}
\newrgbcolor{userFillColour}{0.6 0.6 0.6}
\newrgbcolor{userLineColour}{0.6 0.6 0.6}
\newrgbcolor{userFillColour}{0.6 0.6 0.6}
\newrgbcolor{userLineColour}{0.6 0.6 0.6}
\newrgbcolor{userFillColour}{0.6 0.6 0.6}
\psline[linewidth=0.75](40,70.62)(40,50.62)
\psline[linewidth=0.75](20,70.62)(0,50.62)
\psline[linewidth=0.75](10,90.62)(50,90.62)
\psline[linewidth=0.75](50,70.62)(50,90.62)
\psline[linewidth=0.75](40,100.62)(40,90.62)
\psline[linewidth=0.75](30,70.62)(50,70.62)
\psline[linewidth=0.75](20,80.64)(20,70.62)
\psline[linewidth=0.75](10,90.62)(30,70.62)
\psline[linewidth=0.75](90,90.62)(150,90.62)
\psline[linewidth=0.75](150,70.62)(150,90.62)
\psline[linewidth=0.75](140,99.38)(140,90.62)
\psline[linewidth=0.75](110,70.62)(150,70.62)
\psline[linewidth=0.75](120,70.62)(120,0.62)
\psline[linewidth=0.75](100,80.62)(100,30.62)
\psline[linewidth=0.75](90,90.62)(110,70.62)
\rput(130,80.62){$\universal$}
\rput[l](144.38,99.38){$\Atype$}
\rput[l](44.38,100.62){$\Atype$}
\psline[linewidth=0.75](140,70.62)(140,0.62)
\psline[linewidth=0.75](210,90.62)(250,90.62)
\psline[linewidth=0.75](250,70.62)(250,90.62)
\psline[linewidth=0.75](240,99.38)(240,90.62)
\psline[linewidth=0.75](230,70.62)(250,70.62)
\rput(236.25,80.62){$\universal$}
\rput[l](244.38,99.38){$\Atype$}
\psline[linewidth=0.75](240,70.62)(240,0.62)
\psline[linewidth=0.75](220,80.62)(220,50.62)
\psline[linewidth=0.75](210,90.62)(230,70.62)
\rput[r](217.5,73.12){$\Progtype$}
\rput(37.5,81.88){$\universallift$}
\end{pspicture}


==> PIC/fixp-turing-clas.tex <==
%%Created by jPicEdt 1.4.1_03: mixed JPIC-XML/LaTeX format
%%Tue Nov 05 19:39:36 GMT-10:00 2019
%%Begin JPIC-XML
%<?xml version="1.0" standalone="yes"?>
%<jpic x-min="0" x-max="250" y-min="0" y-max="101.25" auto-bounding="true">
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(10,50);(10,50);(50,50);(50,50)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(50,30);(50,30);(50,50);(50,50)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(30,30);(30,30);(50,30);(50,30)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(40,30);(40,30);(40,0);(40,0)"
%	 />
%<ellipse p3= "(42.58,7.42)"
%	 p2= "(42.58,12.58)"
%	 fill-color= "#330033"
%	 p1= "(37.42,12.58)"
%	 closure= "open"
%	 fill-style= "solid"
%	 angle-end= "0"
%	 angle-start= "0"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(0,50);(0,50);(40,10);(40,10)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(90,40);(90,40);(90,20);(90,20)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(90,40);(90,40);(110,20);(110,20)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(110,20);(110,20);(90,20);(90,20)"
%	 />
%<multicurve stroke-overstrike= "true"
%	 stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(20,40);(20,40);(20,0);(20,0)"
%	 stroke-overstrike-width= "1"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(10,50);(10,50);(30,30);(30,30)"
%	 />
%<text text-vert-align= "center-v"
%	 anchor-point= "(70,60)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\EQLS
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(96.25,26.25)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\PsiT$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(37.5,40)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\universal$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(45,58.75)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\Atype$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(37.5,0)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\Progtype$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(17.5,0)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\Progtype$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(137.5,0)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\Progtype$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(117.5,0)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\Progtype$
%</text>
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(220,40);(220,40);(220,0);(220,0)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(200,50);(200,50);(200,30);(200,30)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(190,60);(190,60);(210,40);(210,40)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(190,40);(190,40);(190,20);(190,20)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(190,40);(190,40);(210,20);(210,20)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(210,20);(210,20);(190,20);(190,20)"
%	 />
%<text text-vert-align= "center-v"
%	 anchor-point= "(170,60)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\EQLS
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(196.25,26.25)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\PsiT$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(237.5,0)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\Progtype$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(217.5,0)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\Progtype$
%</text>
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(210,40);(210,40);(230,40);(230,40)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(210,60);(210,60);(230,40);(230,40)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(190,60);(190,60);(210,60);(210,60)"
%	 />
%<multicurve stroke-width= "0.5"
%	 fill-style= "none"
%	 points= "(215,66.25);(215,66.25);(235,46.25);(235,46.25)"
%	 />
%<multicurve stroke-width= "0.5"
%	 fill-style= "none"
%	 points= "(185,66.25);(185,66.25);(185,13.75);(185,13.75)"
%	 />
%<multicurve stroke-width= "0.5"
%	 fill-style= "none"
%	 points= "(215,66.25);(215,66.25);(185,66.25);(185,66.25)"
%	 />
%<multicurve stroke-width= "0.5"
%	 fill-style= "none"
%	 points= "(235,13.75);(235,13.75);(185,13.75);(185,13.75)"
%	 />
%<multicurve stroke-width= "0.5"
%	 fill-style= "none"
%	 points= "(235,13.75);(235,13.75);(235,46.25);(235,46.25)"
%	 />
%<text text-vert-align= "center-v"
%	 anchor-point= "(228.75,18.75)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\psiT$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(210,50)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\partev$
%</text>
%<parallelogram p3= "(37.5,70.78)"
%	 p2= "(37.5,50.47)"
%	 fill-color= "#999999"
%	 p1= "(42.5,50.47)"
%	 stroke-color= "#999999"
%	 fill-style= "solid"
%	 />
%<parallelogram p3= "(137.5,100)"
%	 p2= "(137.5,90.47)"
%	 fill-color= "#999999"
%	 p1= "(142.5,90.47)"
%	 stroke-color= "#999999"
%	 fill-style= "solid"
%	 />
%<parallelogram p3= "(237.5,100)"
%	 p2= "(237.5,90.47)"
%	 fill-color= "#999999"
%	 p1= "(242.5,90.47)"
%	 stroke-color= "#999999"
%	 fill-style= "solid"
%	 />
%<parallelogram p3= "(37.5,101.25)"
%	 p2= "(37.5,91.09)"
%	 fill-color= "#999999"
%	 p1= "(42.5,91.09)"
%	 stroke-color= "#999999"
%	 fill-style= "solid"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(40,70.62);(40,70.62);(40,50.62);(40,50.62)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(20,70.62);(20,70.62);(0,50.62);(0,50.62)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(10,90.62);(10,90.62);(50,90.62);(50,90.62)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(50,70.62);(50,70.62);(50,90.62);(50,90.62)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(40,100.62);(40,100.62);(40,90.62);(40,90.62)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(30,70.62);(30,70.62);(50,70.62);(50,70.62)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(20,80.64);(20,80.64);(20,70.62);(20,70.62)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(10,90.62);(10,90.62);(30,70.62);(30,70.62)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(90,90.62);(90,90.62);(150,90.62);(150,90.62)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(150,70.62);(150,70.62);(150,90.62);(150,90.62)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(140,99.38);(140,99.38);(140,90.62);(140,90.62)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(110,70.62);(110,70.62);(150,70.62);(150,70.62)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(120,70.62);(120,70.62);(120,0.62);(120,0.62)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(100,80.62);(100,80.62);(100,30.62);(100,30.62)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(90,90.62);(90,90.62);(110,70.62);(110,70.62)"
%	 />
%<text text-vert-align= "center-v"
%	 anchor-point= "(130,80.62)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\universal$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(144.38,99.38)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\Atype$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(44.38,100.62)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\Atype$
%</text>
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(140,70.62);(140,70.62);(140,0.62);(140,0.62)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(210,90.62);(210,90.62);(250,90.62);(250,90.62)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(250,70.62);(250,70.62);(250,90.62);(250,90.62)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(240,99.38);(240,99.38);(240,90.62);(240,90.62)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(230,70.62);(230,70.62);(250,70.62);(250,70.62)"
%	 />
%<text text-vert-align= "center-v"
%	 anchor-point= "(236.25,80.62)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\universal$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(244.38,99.38)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\Atype$
%</text>
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(240,70.62);(240,70.62);(240,0.62);(240,0.62)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(220,80.62);(220,80.62);(220,50.62);(220,50.62)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(210,90.62);(210,90.62);(230,70.62);(230,70.62)"
%	 />
%<text text-vert-align= "center-v"
%	 anchor-point= "(217.5,73.12)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\Progtype$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(37.5,81.88)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\universallift$
%</text>
%</jpic>
%%End JPIC-XML
%PSTricks content-type (pstricks.sty package needed)
%Add \usepackage{pstricks} in the preamble of your LaTeX file
%You can rescale the whole picture (to 80% for instance) by using the command \def\JPicScale{0.8}
\ifx\JPicScale\undefined\def\JPicScale{1}\fi
\psset{unit=\JPicScale mm}
\psset{linewidth=0.3,dotsep=1,hatchwidth=0.3,hatchsep=1.5,shadowsize=1,dimen=middle}
\psset{dotsize=0.7 2.5,dotscale=1 1,fillcolor=black}
\psset{arrowsize=1 2,arrowlength=1,arrowinset=0.25,tbarsize=0.7 5,bracketlength=0.15,rbracketlength=0.15}
\begin{pspicture}(0,0)(250,101.25)
\psline[linewidth=0.75](10,50)(50,50)
\psline[linewidth=0.75](50,30)(50,50)
\psline[linewidth=0.75](30,30)(50,30)
\psline[linewidth=0.75](40,30)(40,0)
\newrgbcolor{userFillColour}{0.2 0 0.2}
\rput{0}(40,10){\psellipse[fillcolor=userFillColour,fillstyle=solid](0,0)(2.58,-2.58)}
\psline[linewidth=0.75](0,50)(40,10)
\psline[linewidth=0.75](90,40)(90,20)
\psline[linewidth=0.75](90,40)(110,20)
\psline[linewidth=0.75](110,20)(90,20)
\psline[linewidth=0.75,border=1](20,40)(20,0)
\psline[linewidth=0.75](10,50)(30,30)
\rput(70,60){\EQLS}
\rput(96.25,26.25){$\PsiT$}
\rput(37.5,40){$\universal$}
\rput[l](45,58.75){$\Atype$}
\rput[r](37.5,0){$\Progtype$}
\rput[r](17.5,0){$\Progtype$}
\rput[r](137.5,0){$\Progtype$}
\rput[r](117.5,0){$\Progtype$}
\psline[linewidth=0.75](220,40)(220,0)
\psline[linewidth=0.75](200,50)(200,30)
\psline[linewidth=0.75](190,60)(210,40)
\psline[linewidth=0.75](190,40)(190,20)
\psline[linewidth=0.75](190,40)(210,20)
\psline[linewidth=0.75](210,20)(190,20)
\rput(170,60){\EQLS}
\rput(196.25,26.25){$\PsiT$}
\rput[r](237.5,0){$\Progtype$}
\rput[r](217.5,0){$\Progtype$}
\psline[linewidth=0.75](210,40)(230,40)
\psline[linewidth=0.75](210,60)(230,40)
\psline[linewidth=0.75](190,60)(210,60)
\psline[linewidth=0.5](215,66.25)(235,46.25)
\psline[linewidth=0.5](185,66.25)(185,13.75)
\psline[linewidth=0.5](215,66.25)(185,66.25)
\psline[linewidth=0.5](235,13.75)(185,13.75)
\psline[linewidth=0.5](235,13.75)(235,46.25)
\rput(228.75,18.75){$\psiT$}
\rput(210,50){$\partev$}
\newrgbcolor{userLineColour}{0.6 0.6 0.6}
\newrgbcolor{userFillColour}{0.6 0.6 0.6}
\pspolygon[linecolor=userLineColour,fillcolor=userFillColour,fillstyle=solid](42.5,50.47)(37.5,50.47)(37.5,70.78)(42.5,70.78)
\newrgbcolor{userLineColour}{0.6 0.6 0.6}
\newrgbcolor{userFillColour}{0.6 0.6 0.6}
\pspolygon[linecolor=userLineColour,fillcolor=userFillColour,fillstyle=solid](142.5,90.47)(137.5,90.47)(137.5,100)(142.5,100)
\newrgbcolor{userLineColour}{0.6 0.6 0.6}
\newrgbcolor{userFillColour}{0.6 0.6 0.6}
\pspolygon[linecolor=userLineColour,fillcolor=userFillColour,fillstyle=solid](242.5,90.47)(237.5,90.47)(237.5,100)(242.5,100)
\newrgbcolor{userLineColour}{0.6 0.6 0.6}
\newrgbcolor{userFillColour}{0.6 0.6 0.6}
\pspolygon[linecolor=userLineColour,fillcolor=userFillColour,fillstyle=solid](42.5,91.09)(37.5,91.09)(37.5,101.25)(42.5,101.25)
\psline[linewidth=0.75](40,70.62)(40,50.62)
\psline[linewidth=0.75](20,70.62)(0,50.62)
\psline[linewidth=0.75](10,90.62)(50,90.62)
\psline[linewidth=0.75](50,70.62)(50,90.62)
\psline[linewidth=0.75](40,100.62)(40,90.62)
\psline[linewidth=0.75](30,70.62)(50,70.62)
\psline[linewidth=0.75](20,80.64)(20,70.62)
\psline[linewidth=0.75](10,90.62)(30,70.62)
\psline[linewidth=0.75](90,90.62)(150,90.62)
\psline[linewidth=0.75](150,70.62)(150,90.62)
\psline[linewidth=0.75](140,99.38)(140,90.62)
\psline[linewidth=0.75](110,70.62)(150,70.62)
\psline[linewidth=0.75](120,70.62)(120,0.62)
\psline[linewidth=0.75](100,80.62)(100,30.62)
\psline[linewidth=0.75](90,90.62)(110,70.62)
\rput(130,80.62){$\universal$}
\rput[l](144.38,99.38){$\Atype$}
\rput[l](44.38,100.62){$\Atype$}
\psline[linewidth=0.75](140,70.62)(140,0.62)
\psline[linewidth=0.75](210,90.62)(250,90.62)
\psline[linewidth=0.75](250,70.62)(250,90.62)
\psline[linewidth=0.75](240,99.38)(240,90.62)
\psline[linewidth=0.75](230,70.62)(250,70.62)
\rput(236.25,80.62){$\universal$}
\rput[l](244.38,99.38){$\Atype$}
\psline[linewidth=0.75](240,70.62)(240,0.62)
\psline[linewidth=0.75](220,80.62)(220,50.62)
\psline[linewidth=0.75](210,90.62)(230,70.62)
\rput[r](217.5,73.12){$\Progtype$}
\rput(37.5,81.88){$\universallift$}
\end{pspicture}


==> PIC/fixp-turing-noM.tex <==
%%Created by jPicEdt 1.4.1_03: mixed JPIC-XML/LaTeX format
%%Sun May 23 15:24:30 GMT-10:00 2021
%%Begin JPIC-XML
%<?xml version="1.0" standalone="yes"?>
%<jpic x-min="0" x-max="130" y-min="-1.25" y-max="105" auto-bounding="true">
%<multicurve fill-style= "none"
%	 points= "(50,35);(50,35);(50,55);(50,55)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(30,35);(30,35);(50,35);(50,35)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(40,35);(40,35);(40,0);(40,0)"
%	 />
%<ellipse fill-color= "#330033"
%	 fill-style= "solid"
%	 p3= "(42.58,12.42)"
%	 p2= "(42.58,17.58)"
%	 p1= "(37.42,17.58)"
%	 closure= "open"
%	 angle-end= "0"
%	 angle-start= "0"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(20,75);(20,75);(0,55);(0,55)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(0,55);(0,55);(40,15);(40,15)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(50,75);(50,75);(50,95);(50,95)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(20,85.01);(20,85.01);(20,75);(20,75)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(10,95);(10,95);(30,75);(30,75)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(130,35);(130,35);(130,55);(130,55)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(110,35);(110,35);(130,35);(130,35)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(120,35);(120,35);(120,0);(120,0)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(100,45.01);(100,45.01);(100,15);(100,15)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(90,55);(90,55);(110,35);(110,35)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(10,25);(10,25);(10,5);(10,5)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(30,5);(30,5);(10,5);(10,5)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(90,25);(90,25);(90,5);(90,5)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(90,25);(90,25);(110,5);(110,5)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(110,5);(110,5);(90,5);(90,5)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(20,45);(20,45);(20,15);(20,15)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(10,25);(10,25);(30,5);(30,5)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(10,55);(10,55);(30,35);(30,35)"
%	 />
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(70,45)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\EQLS
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(15,10)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\PsiT$
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(95,10)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\PsiT$
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(37.5,45)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\universal$
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(117.5,45)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\universal$
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(117.5,-1.25)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\Progtype$
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(125,75)"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\Atype$
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(44.38,105)"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\Atype$
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(44.38,64.38)"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\Atype$
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(37.5,-1.25)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\Progtype$
%</text>
%<multicurve fill-style= "none"
%	 points= "(90,55);(90,55);(130,55);(130,55)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(120,75);(120,75);(120,55);(120,55)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(30,75);(30,75);(50,75);(50,75)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(10,55);(10,55);(50,55);(50,55)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(40,75);(40,75);(40,55);(40,55)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(10,95);(10,95);(50,95);(50,95)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(40,105);(40,105);(40,95);(40,95)"
%	 />
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(38.75,86.25)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\universallift$
%</text>
%<ellipse fill-color= "#330033"
%	 fill-style= "solid"
%	 p3= "(22.58,12.42)"
%	 p2= "(22.58,17.58)"
%	 p1= "(17.42,17.58)"
%	 closure= "open"
%	 angle-end= "0"
%	 angle-start= "0"
%	 />
%<ellipse fill-color= "#330033"
%	 fill-style= "solid"
%	 p3= "(102.58,12.42)"
%	 p2= "(102.58,17.58)"
%	 p1= "(97.42,17.58)"
%	 closure= "open"
%	 angle-end= "0"
%	 angle-start= "0"
%	 />
%</jpic>
%%End JPIC-XML
%LaTeX-picture environment using emulated lines and arcs
%You can rescale the whole picture (to 80% for instance) by using the command \def\JPicScale{0.8}
\ifx\JPicScale\undefined\def\JPicScale{1}\fi
\unitlength \JPicScale mm
\begin{picture}(130,105)(0,0)
\linethickness{0.3mm}
\put(50,35){\line(0,1){20}}
\linethickness{0.3mm}
\put(30,35){\line(1,0){20}}
\linethickness{0.75mm}
\put(40,0){\line(0,1){35}}
\linethickness{0.3mm}
\put(40,15){\circle*{5.16}}

\linethickness{0.75mm}
\multiput(0,55)(0.12,0.12){167}{\line(1,0){0.12}}
\linethickness{0.75mm}
\multiput(0,55)(0.12,-0.12){333}{\line(1,0){0.12}}
\linethickness{0.3mm}
\put(50,75){\line(0,1){20}}
\linethickness{0.75mm}
\put(20,75){\line(0,1){10.01}}
\linethickness{0.3mm}
\multiput(10,95)(0.12,-0.12){167}{\line(1,0){0.12}}
\linethickness{0.3mm}
\put(130,35){\line(0,1){20}}
\linethickness{0.3mm}
\put(110,35){\line(1,0){20}}
\linethickness{0.3mm}
\put(120,0){\line(0,1){35}}
\linethickness{0.75mm}
\put(100,15){\line(0,1){30.01}}
\linethickness{0.3mm}
\multiput(90,55)(0.12,-0.12){167}{\line(1,0){0.12}}
\linethickness{0.3mm}
\put(10,5){\line(0,1){20}}
\linethickness{0.3mm}
\put(10,5){\line(1,0){20}}
\linethickness{0.3mm}
\put(90,5){\line(0,1){20}}
\linethickness{0.3mm}
\multiput(90,25)(0.12,-0.12){167}{\line(1,0){0.12}}
\linethickness{0.3mm}
\put(90,5){\line(1,0){20}}
\linethickness{0.75mm}
\put(20,15){\line(0,1){30}}
\linethickness{0.3mm}
\multiput(10,25)(0.12,-0.12){167}{\line(1,0){0.12}}
\linethickness{0.3mm}
\multiput(10,55)(0.12,-0.12){167}{\line(1,0){0.12}}
\put(70,45){\makebox(0,0)[cc]{\EQLS}}

\put(15,10){\makebox(0,0)[cc]{$\PsiT$}}

\put(95,10){\makebox(0,0)[cc]{$\PsiT$}}

\put(37.5,45){\makebox(0,0)[cc]{$\universal$}}

\put(117.5,45){\makebox(0,0)[cc]{$\universal$}}

\put(117.5,-1.25){\makebox(0,0)[cr]{$\Progtype$}}

\put(125,75){\makebox(0,0)[cl]{$\Atype$}}

\put(44.38,105){\makebox(0,0)[cl]{$\Atype$}}

\put(44.38,64.38){\makebox(0,0)[cl]{$\Atype$}}

\put(37.5,-1.25){\makebox(0,0)[cr]{$\Progtype$}}

\linethickness{0.3mm}
\put(90,55){\line(1,0){40}}
\linethickness{0.3mm}
\put(120,55){\line(0,1){20}}
\linethickness{0.3mm}
\put(30,75){\line(1,0){20}}
\linethickness{0.3mm}
\put(10,55){\line(1,0){40}}
\linethickness{0.3mm}
\put(40,55){\line(0,1){20}}
\linethickness{0.3mm}
\put(10,95){\line(1,0){40}}
\linethickness{0.3mm}
\put(40,95){\line(0,1){10}}
\put(38.75,86.25){\makebox(0,0)[cc]{$\universallift$}}

\linethickness{0.3mm}
\put(20,15){\circle*{5.16}}

\linethickness{0.3mm}
\put(100,15){\circle*{5.16}}

\end{picture}


==> PIC/fixp-turing.tex <==
%%Created by jPicEdt 1.4.1_03: mixed JPIC-XML/LaTeX format
%%Sun May 23 15:36:31 GMT-10:00 2021
%%Begin JPIC-XML
%<?xml version="1.0" standalone="yes"?>
%<jpic x-min="0" x-max="130" y-min="-1.25" y-max="105" auto-bounding="true">
%<multicurve fill-style= "none"
%	 points= "(50,35);(50,35);(50,55);(50,55)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(30,35);(30,35);(50,35);(50,35)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(40,35);(40,35);(40,0);(40,0)"
%	 />
%<ellipse fill-color= "#330033"
%	 fill-style= "solid"
%	 p3= "(42.58,12.42)"
%	 p2= "(42.58,17.58)"
%	 p1= "(37.42,17.58)"
%	 closure= "open"
%	 angle-end= "0"
%	 angle-start= "0"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(20,75);(20,75);(0,55);(0,55)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(50,75);(50,75);(50,95);(50,95)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(20,85.01);(20,85.01);(20,75);(20,75)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(10,95);(10,95);(30,75);(30,75)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(130,35);(130,35);(130,55);(130,55)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(110,35);(110,35);(130,35);(130,35)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(120,35);(120,35);(120,0);(120,0)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(100,45.01);(100,45.01);(100,15);(100,15)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(90,55);(90,55);(110,35);(110,35)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(10,25);(10,25);(10,5);(10,5)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(30,5);(30,5);(10,5);(10,5)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(90,25);(90,25);(90,5);(90,5)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(90,25);(90,25);(110,5);(110,5)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(110,5);(110,5);(90,5);(90,5)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(10,25);(10,25);(30,5);(30,5)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(10,55);(10,55);(30,35);(30,35)"
%	 />
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(70,45)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\EQLS
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(15,10)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\PsiT$
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(95,10)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\PsiT$
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(37.5,45)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\universal$
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(117.5,45)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\universal$
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(117.5,-1.25)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\Progtype$
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(125,75)"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\Atype$
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(44.38,105)"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\Atype$
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(44.38,64.38)"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\Atype$
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(37.5,-1.25)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\Progtype$
%</text>
%<multicurve fill-style= "none"
%	 points= "(90,55);(90,55);(130,55);(130,55)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(120,75);(120,75);(120,55);(120,55)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(30,75);(30,75);(50,75);(50,75)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(10,55);(10,55);(50,55);(50,55)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(40,75);(40,75);(40,55);(40,55)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(10,95);(10,95);(50,95);(50,95)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(40,105);(40,105);(40,95);(40,95)"
%	 />
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(38.75,86.25)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\universallift$
%</text>
%<ellipse fill-color= "#330033"
%	 fill-style= "solid"
%	 p3= "(22.58,12.42)"
%	 p2= "(22.58,17.58)"
%	 p1= "(17.42,17.58)"
%	 closure= "open"
%	 angle-end= "0"
%	 angle-start= "0"
%	 />
%<ellipse fill-color= "#330033"
%	 fill-style= "solid"
%	 p3= "(102.58,12.42)"
%	 p2= "(102.58,17.58)"
%	 p1= "(97.42,17.58)"
%	 closure= "open"
%	 angle-end= "0"
%	 angle-start= "0"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(20,45);(20,45);(20,15);(20,15)"
%	 stroke-overstrike= "true"
%	 stroke-overstrike-width= "1.3"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(0,55);(0,55);(40,15);(40,15)"
%	 />
%</jpic>
%%End JPIC-XML
%LaTeX-picture environment using emulated lines and arcs
%You can rescale the whole picture (to 80% for instance) by using the command \def\JPicScale{0.8}
\ifx\JPicScale\undefined\def\JPicScale{1}\fi
\unitlength \JPicScale mm
\begin{picture}(130,105)(0,0)
\linethickness{0.3mm}
\put(50,35){\line(0,1){20}}
\linethickness{0.3mm}
\put(30,35){\line(1,0){20}}
\linethickness{0.75mm}
\put(40,0){\line(0,1){35}}
\linethickness{0.3mm}
\put(40,15){\circle*{5.16}}

\linethickness{0.75mm}
\multiput(0,55)(0.12,0.12){167}{\line(1,0){0.12}}
\linethickness{0.3mm}
\put(50,75){\line(0,1){20}}
\linethickness{0.75mm}
\put(20,75){\line(0,1){10.01}}
\linethickness{0.3mm}
\multiput(10,95)(0.12,-0.12){167}{\line(1,0){0.12}}
\linethickness{0.3mm}
\put(130,35){\line(0,1){20}}
\linethickness{0.3mm}
\put(110,35){\line(1,0){20}}
\linethickness{0.3mm}
\put(120,0){\line(0,1){35}}
\linethickness{0.75mm}
\put(100,15){\line(0,1){30.01}}
\linethickness{0.3mm}
\multiput(90,55)(0.12,-0.12){167}{\line(1,0){0.12}}
\linethickness{0.3mm}
\put(10,5){\line(0,1){20}}
\linethickness{0.3mm}
\put(10,5){\line(1,0){20}}
\linethickness{0.3mm}
\put(90,5){\line(0,1){20}}
\linethickness{0.3mm}
\multiput(90,25)(0.12,-0.12){167}{\line(1,0){0.12}}
\linethickness{0.3mm}
\put(90,5){\line(1,0){20}}
\linethickness{0.3mm}
\multiput(10,25)(0.12,-0.12){167}{\line(1,0){0.12}}
\linethickness{0.3mm}
\multiput(10,55)(0.12,-0.12){167}{\line(1,0){0.12}}
\put(70,45){\makebox(0,0)[cc]{\EQLS}}

\put(15,10){\makebox(0,0)[cc]{$\PsiT$}}

\put(95,10){\makebox(0,0)[cc]{$\PsiT$}}

\put(37.5,45){\makebox(0,0)[cc]{$\universal$}}

\put(117.5,45){\makebox(0,0)[cc]{$\universal$}}

\put(117.5,-1.25){\makebox(0,0)[cr]{$\Progtype$}}

\put(125,75){\makebox(0,0)[cl]{$\Atype$}}

\put(44.38,105){\makebox(0,0)[cl]{$\Atype$}}

\put(44.38,64.38){\makebox(0,0)[cl]{$\Atype$}}

\put(37.5,-1.25){\makebox(0,0)[cr]{$\Progtype$}}

\linethickness{0.3mm}
\put(90,55){\line(1,0){40}}
\linethickness{0.3mm}
\put(120,55){\line(0,1){20}}
\linethickness{0.3mm}
\put(30,75){\line(1,0){20}}
\linethickness{0.3mm}
\put(10,55){\line(1,0){40}}
\linethickness{0.3mm}
\put(40,55){\line(0,1){20}}
\linethickness{0.3mm}
\put(10,95){\line(1,0){40}}
\linethickness{0.3mm}
\put(40,95){\line(0,1){10}}
\put(38.75,86.25){\makebox(0,0)[cc]{$\universallift$}}

\linethickness{0.3mm}
\put(20,15){\circle*{5.16}}

\linethickness{0.3mm}
\put(100,15){\circle*{5.16}}

\linethickness{0.75mm}
\put(20,15){\line(0,1){30}}
\linethickness{0.75mm}
\multiput(0,55)(0.12,-0.12){333}{\line(1,0){0.12}}
\end{picture}


==> PIC/fixp-univ-noM.tex <==
%%Created by jPicEdt 1.4.1_03: mixed JPIC-XML/LaTeX format
%%Tue Nov 05 19:34:49 GMT-10:00 2019
%%Begin JPIC-XML
%<?xml version="1.0" standalone="yes"?>
%<jpic x-min="5" x-max="280" y-min="0" y-max="118.12" auto-bounding="true">
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(20,65);(20,65);(40,65);(40,65)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(50,85);(50,85);(50,55);(50,55)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(40,45);(40,45);(60,45);(60,45)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(50,45);(50,45);(50,0);(50,0)"
%	 />
%<ellipse p3= "(52.58,22.42)"
%	 p2= "(52.58,27.58)"
%	 fill-color= "#330033"
%	 p1= "(47.42,27.58)"
%	 closure= "open"
%	 fill-style= "solid"
%	 angle-end= "0"
%	 angle-start= "0"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(30,95);(30,95);(5,70);(5,70)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(5,70);(5,70);(50,25);(50,25)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(77.5,85);(77.5,85);(77.5,105);(77.5,105)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(40,85);(40,85);(77.5,85);(77.5,85)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(20,105);(20,105);(40,85);(40,85)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(175,45);(175,45);(175,65);(175,65)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(140,45);(140,45);(175,45);(175,45)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(150,45);(150,45);(150,0);(150,0)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(130,55.01);(130,55.01);(130,25);(130,25)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(120,65);(120,65);(140,45);(140,45)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(20,35);(20,35);(20,15);(20,15)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(40,15);(40,15);(20,15);(20,15)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(120,35);(120,35);(120,15);(120,15)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(120,35);(120,35);(140,15);(140,15)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(140,15);(140,15);(120,15);(120,15)"
%	 />
%<multicurve stroke-overstrike= "true"
%	 stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(30,55);(30,55);(30,25);(30,25)"
%	 stroke-overstrike-width= "1"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(20,35);(20,35);(40,15);(40,15)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(20,65);(20,65);(40,45);(40,45)"
%	 />
%<text text-vert-align= "center-v"
%	 anchor-point= "(95,55)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\EQLS
%</text>
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(280,55);(280,55);(280,75);(280,75)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(242.5,35);(242.5,35);(262.5,35);(262.5,35)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(252.5,35);(252.5,35);(252.5,0);(252.5,0)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(232.5,45);(232.5,45);(232.5,25);(232.5,25)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(222.5,55);(222.5,55);(242.5,35);(242.5,35)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(222.5,35);(222.5,35);(222.5,15);(222.5,15)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(222.5,35);(222.5,35);(242.5,15);(242.5,15)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(242.5,15);(242.5,15);(222.5,15);(222.5,15)"
%	 />
%<text text-vert-align= "center-v"
%	 anchor-point= "(195,55)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\EQLS
%</text>
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(222.5,55);(222.5,55);(242.5,55);(242.5,55)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(242.5,55);(242.5,55);(262.5,35);(262.5,35)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(242.5,75);(242.5,75);(262.5,55);(262.5,55)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(252.5,65);(252.5,65);(252.5,45);(252.5,45)"
%	 />
%<multicurve stroke-width= "0.5"
%	 fill-style= "none"
%	 points= "(245,62.5);(245,62.5);(267.5,40);(267.5,40)"
%	 />
%<multicurve stroke-width= "0.5"
%	 fill-style= "none"
%	 points= "(215,62.5);(215,62.5);(215,10);(215,10)"
%	 />
%<multicurve stroke-width= "0.5"
%	 fill-style= "none"
%	 points= "(245,62.5);(245,62.5);(215,62.5);(215,62.5)"
%	 />
%<multicurve stroke-width= "0.5"
%	 fill-style= "none"
%	 points= "(267.5,10);(267.5,10);(215,10);(215,10)"
%	 />
%<multicurve stroke-width= "0.5"
%	 fill-style= "none"
%	 points= "(267.5,10);(267.5,10);(267.5,40);(267.5,40)"
%	 />
%<text text-vert-align= "center-v"
%	 anchor-point= "(26.25,21.25)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\PsiT$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(126.25,21.25)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\PsiT$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(228.75,21.25)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\PsiT$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(261.25,16.25)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\psiT$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(57.5,95)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\universal$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(157.5,55)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\universal$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(265,65)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\smalluniversal$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(242.5,45)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\partev$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(147.5,2.5)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\Progtype$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(250,2.5)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\Progtype$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(47.5,2.5)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\Progtype$
%</text>
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(67.5,85);(67.5,85);(67.5,0);(67.5,0)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(167.5,45);(167.5,45);(167.5,0);(167.5,0)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(262.5,55);(262.5,55);(280,55);(280,55)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(275,55);(275,55);(275,0);(275,0)"
%	 />
%<text text-vert-align= "center-v"
%	 anchor-point= "(272.5,2.5)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\Atype$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(165,2.5)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\Atype$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(65,2.5)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\Atype$
%</text>
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(40,65);(40,65);(60,45);(60,45)"
%	 />
%<text text-vert-align= "center-v"
%	 anchor-point= "(40,55)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\partev$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(52.5,70)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\Progtype$
%</text>
%<parallelogram p3= "(65,118.12)"
%	 p2= "(65,105.47)"
%	 fill-color= "#999999"
%	 p1= "(70,105.47)"
%	 stroke-color= "#999999"
%	 fill-style= "solid"
%	 />
%<parallelogram p3= "(272.5,86.88)"
%	 p2= "(272.5,75.47)"
%	 fill-color= "#999999"
%	 p1= "(277.5,75.47)"
%	 stroke-color= "#999999"
%	 fill-style= "solid"
%	 />
%<parallelogram p3= "(157.5,85.78)"
%	 p2= "(157.5,65.47)"
%	 fill-color= "#999999"
%	 p1= "(162.5,65.47)"
%	 stroke-color= "#999999"
%	 fill-style= "solid"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(20,105);(20,105);(77.5,105);(77.5,105)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(67.5,117.5);(67.5,117.5);(67.5,105);(67.5,105)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(120,65);(120,65);(175,65);(175,65)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(160,85);(160,85);(160,65);(160,65)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(242.5,75);(242.5,75);(280,75);(280,75)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(275,86.25);(275,86.25);(275,75);(275,75)"
%	 />
%<text text-vert-align= "center-v"
%	 anchor-point= "(71.88,118.12)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\Btype$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(164.38,85.62)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\Btype$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(280,86.88)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\Btype$
%</text>
%</jpic>
%%End JPIC-XML
%PSTricks content-type (pstricks.sty package needed)
%Add \usepackage{pstricks} in the preamble of your LaTeX file
%You can rescale the whole picture (to 80% for instance) by using the command \def\JPicScale{0.8}
\ifx\JPicScale\undefined\def\JPicScale{1}\fi
\psset{unit=\JPicScale mm}
\psset{linewidth=0.3,dotsep=1,hatchwidth=0.3,hatchsep=1.5,shadowsize=1,dimen=middle}
\psset{dotsize=0.7 2.5,dotscale=1 1,fillcolor=black}
\psset{arrowsize=1 2,arrowlength=1,arrowinset=0.25,tbarsize=0.7 5,bracketlength=0.15,rbracketlength=0.15}
\begin{pspicture}(0,0)(280,118.12)
\psline[linewidth=0.75](20,65)(40,65)
\psline[linewidth=0.75](50,85)(50,55)
\psline[linewidth=0.75](40,45)(60,45)
\psline[linewidth=0.75](50,45)(50,0)
\newrgbcolor{userFillColour}{0.2 0 0.2}
\rput{0}(50,25){\psellipse[fillcolor=userFillColour,fillstyle=solid](0,0)(2.58,-2.58)}
\psline[linewidth=0.75](30,95)(5,70)
\psline[linewidth=0.75](5,70)(50,25)
\psline[linewidth=0.75](77.5,85)(77.5,105)
\psline[linewidth=0.75](40,85)(77.5,85)
\psline[linewidth=0.75](20,105)(40,85)
\psline[linewidth=0.75](175,45)(175,65)
\psline[linewidth=0.75](140,45)(175,45)
\psline[linewidth=0.75](150,45)(150,0)
\psline[linewidth=0.75](130,55.01)(130,25)
\psline[linewidth=0.75](120,65)(140,45)
\psline[linewidth=0.75](20,35)(20,15)
\psline[linewidth=0.75](40,15)(20,15)
\psline[linewidth=0.75](120,35)(120,15)
\psline[linewidth=0.75](120,35)(140,15)
\psline[linewidth=0.75](140,15)(120,15)
\psline[linewidth=0.75,border=1](30,55)(30,25)
\psline[linewidth=0.75](20,35)(40,15)
\psline[linewidth=0.75](20,65)(40,45)
\rput(95,55){\EQLS}
\psline[linewidth=0.75](280,55)(280,75)
\psline[linewidth=0.75](242.5,35)(262.5,35)
\psline[linewidth=0.75](252.5,35)(252.5,0)
\psline[linewidth=0.75](232.5,45)(232.5,25)
\psline[linewidth=0.75](222.5,55)(242.5,35)
\psline[linewidth=0.75](222.5,35)(222.5,15)
\psline[linewidth=0.75](222.5,35)(242.5,15)
\psline[linewidth=0.75](242.5,15)(222.5,15)
\rput(195,55){\EQLS}
\psline[linewidth=0.75](222.5,55)(242.5,55)
\psline[linewidth=0.75](242.5,55)(262.5,35)
\psline[linewidth=0.75](242.5,75)(262.5,55)
\psline[linewidth=0.75](252.5,65)(252.5,45)
\psline[linewidth=0.5](245,62.5)(267.5,40)
\psline[linewidth=0.5](215,62.5)(215,10)
\psline[linewidth=0.5](245,62.5)(215,62.5)
\psline[linewidth=0.5](267.5,10)(215,10)
\psline[linewidth=0.5](267.5,10)(267.5,40)
\rput(26.25,21.25){$\PsiT$}
\rput(126.25,21.25){$\PsiT$}
\rput(228.75,21.25){$\PsiT$}
\rput(261.25,16.25){$\psiT$}
\rput(57.5,95){$\universal$}
\rput(157.5,55){$\universal$}
\rput(265,65){$\smalluniversal$}
\rput(242.5,45){$\partev$}
\rput[r](147.5,2.5){$\Progtype$}
\rput[r](250,2.5){$\Progtype$}
\rput[r](47.5,2.5){$\Progtype$}
\psline[linewidth=0.75](67.5,85)(67.5,0)
\psline[linewidth=0.75](167.5,45)(167.5,0)
\psline[linewidth=0.75](262.5,55)(280,55)
\psline[linewidth=0.75](275,55)(275,0)
\rput[r](272.5,2.5){$\Atype$}
\rput[r](165,2.5){$\Atype$}
\rput[r](65,2.5){$\Atype$}
\psline[linewidth=0.75](40,65)(60,45)
\rput(40,55){$\partev$}
\rput[l](52.5,70){$\Progtype$}
\newrgbcolor{userLineColour}{0.6 0.6 0.6}
\newrgbcolor{userFillColour}{0.6 0.6 0.6}
\newrgbcolor{userLineColour}{0.6 0.6 0.6}
\newrgbcolor{userFillColour}{0.6 0.6 0.6}
\newrgbcolor{userLineColour}{0.6 0.6 0.6}
\newrgbcolor{userFillColour}{0.6 0.6 0.6}
\psline[linewidth=0.75](20,105)(77.5,105)
\psline[linewidth=0.75](67.5,117.5)(67.5,105)
\psline[linewidth=0.75](120,65)(175,65)
\psline[linewidth=0.75](160,85)(160,65)
\psline[linewidth=0.75](242.5,75)(280,75)
\psline[linewidth=0.75](275,86.25)(275,75)
\rput[l](71.88,118.12){$\Btype$}
\rput[l](164.38,85.62){$\Btype$}
\rput[l](280,86.88){$\Btype$}
\end{pspicture}


==> PIC/fmn-left.tex <==
%%Created by jPicEdt 1.4.1_03: mixed JPIC-XML/LaTeX format
%%Sat Nov 11 18:57:20 HST 2017
%%Begin JPIC-XML
%<?xml version="1.0" standalone="yes"?>
%<jpic x-min="-1.87" x-max="6.87" y-min="-7.5" y-max="12.5" auto-bounding="true">
%<parallelogram p3= "(4.37,-3.12)"
%	 p2= "(4.37,0.62)"
%	 p1= "(0.63,0.62)"
%	 fill-style= "none"
%	 />
%<text text-vert-align= "center-v"
%	 anchor-point= "(2.5,-1.26)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\fun$
%</text>
%<ellipse p3= "(4.06,4.06)"
%	 p2= "(4.06,7.19)"
%	 p1= "(0.94,7.19)"
%	 closure= "open"
%	 angle-end= "0"
%	 fill-style= "solid"
%	 angle-start= "0"
%	 />
%<multicurve points= "(2.5,1.24);(2.5,1.24);(2.5,0.62);(2.5,0.62);(2.5,0.62);(2.5,0.62);
%	(2.5,0.62);(2.5,0.62);(2.5,4.38);(2.5,4.38)"
%	 fill-style= "none"
%	 />
%<multicurve points= "(2.5,-6.88);(2.5,-6.88);(2.5,-7.5);(2.5,-7.5);(2.5,-7.5);(2.5,-7.5);
%	(2.5,-7.5);(2.5,-7.5);(2.5,-3.12);(2.5,-3.12)"
%	 fill-style= "none"
%	 />
%<multicurve points= "(2.5,5.01);(2.5,5.01);(-0.63,8.12);(-0.63,8.12);(-0.63,8.12);(-1.87,9.38);
%	(-1.87,9.38);(-1.87,9.38);(-1.87,12.5);(-1.87,12.5)"
%	 fill-style= "none"
%	 />
%<multicurve points= "(3.13,5.62);(3.13,5.62);(6.87,9.38);(6.87,9.38);(6.87,9.38);(6.87,10.62);
%	(6.87,10.62);(6.87,10.62);(6.87,12.5);(6.87,12.5)"
%	 fill-style= "none"
%	 />
%</jpic>
%%End JPIC-XML
%PSTricks content-type (pstricks.sty package needed)
%Add \usepackage{pstricks} in the preamble of your LaTeX file
%You can rescale the whole picture (to 80% for instance) by using the command \def\JPicScale{0.8}
\ifx\JPicScale\undefined\def\JPicScale{1}\fi
\psset{unit=\JPicScale mm}
\psset{linewidth=0.3,dotsep=1,hatchwidth=0.3,hatchsep=1.5,shadowsize=1,dimen=middle}
\psset{dotsize=0.7 2.5,dotscale=1 1,fillcolor=black}
\psset{arrowsize=1 2,arrowlength=1,arrowinset=0.25,tbarsize=0.7 5,bracketlength=0.15,rbracketlength=0.15}
\begin{pspicture}(0,0)(6.87,12.5)
\pspolygon[](0.63,0.62)(4.37,0.62)(4.37,-3.12)(0.63,-3.12)
\rput(2.5,-1.26){$\fun$}
\rput{0}(2.5,5.62){\psellipse[fillstyle=solid](0,0)(1.56,-1.56)}
\pscustom[]{\psline(2.5,1.24)(2.5,0.62)
\psbezier(2.5,0.62)(2.5,0.62)(2.5,0.62)
\psline(2.5,0.62)(2.5,4.38)
}
\pscustom[]{\psline(2.5,-6.88)(2.5,-7.5)
\psbezier(2.5,-7.5)(2.5,-7.5)(2.5,-7.5)
\psline(2.5,-7.5)(2.5,-3.12)
}
\psline(2.5,5.01)
(-0.63,8.12)
(-1.87,9.38)(-1.87,12.5)
\psline(3.13,5.62)
(6.87,9.38)
(6.87,10.62)(6.87,12.5)
\end{pspicture}


==> PIC/fmn-right.tex <==
%%Created by jPicEdt 1.4.1_03: mixed JPIC-XML/LaTeX format
%%Thu Aug 30 10:15:26 GMT-10:00 2018
%%Begin JPIC-XML
%<?xml version="1.0" standalone="yes"?>
%<jpic x-min="-3.74" x-max="8.75" y-min="-6.88" y-max="13.13" auto-bounding="true">
%<parallelogram p3= "(-0,5)"
%	 p2= "(-0,8.75)"
%	 fill-style= "none"
%	 p1= "(-3.74,8.75)"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(-1.88,6.86)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\fun$
%</text>
%<ellipse p3= "(4.06,-3.44)"
%	 p2= "(4.06,-0.31)"
%	 fill-style= "solid"
%	 p1= "(0.94,-0.31)"
%	 closure= "open"
%	 angle-end= "0"
%	 angle-start= "0"
%	 />
%<multicurve fill-style= "none"
%	 points= "(2.5,-6.26);(2.5,-6.26);(2.5,-6.88);(2.5,-6.88);(2.5,-6.88);(2.5,-6.88);
%	(2.5,-6.88);(2.5,-6.88);(2.5,-3.12);(2.5,-3.12)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(6.88,9.38);(6.88,9.38);(6.88,8.75);(6.88,8.75);(6.88,8.75);(6.88,8.75);
%	(6.88,8.75);(6.88,8.75);(6.88,13.13);(6.88,13.13)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(2.5,-2.49);(2.5,-2.49);(-0.63,0.62);(-0.63,0.62);(-0.63,0.62);(-1.87,1.88);
%	(-1.87,1.88);(-1.87,1.88);(-1.87,5);(-1.87,5)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(3.13,-1.88);(3.13,-1.88);(6.87,1.88);(6.87,1.88);(6.87,1.88);(6.87,3.12);
%	(6.87,3.12);(6.87,3.12);(6.87,5);(6.87,5)"
%	 />
%<parallelogram p3= "(8.75,5)"
%	 p2= "(8.75,8.75)"
%	 fill-style= "none"
%	 p1= "(5,8.75)"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(6.88,6.86)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\fun$
%</text>
%<multicurve fill-style= "none"
%	 points= "(-1.88,9.38);(-1.88,9.38);(-1.88,8.75);(-1.88,8.75);(-1.88,8.75);(-1.88,8.75);
%	(-1.88,8.75);(-1.88,8.75);(-1.88,13.13);(-1.88,13.13)"
%	 />
%</jpic>
%%End JPIC-XML
%PSTricks content-type (pstricks.sty package needed)
%Add \usepackage{pstricks} in the preamble of your LaTeX file
%You can rescale the whole picture (to 80% for instance) by using the command \def\JPicScale{0.8}
\ifx\JPicScale\undefined\def\JPicScale{1}\fi
\psset{unit=\JPicScale mm}
\psset{linewidth=0.3,dotsep=1,hatchwidth=0.3,hatchsep=1.5,shadowsize=1,dimen=middle}
\psset{dotsize=0.7 2.5,dotscale=1 1,fillcolor=black}
\psset{arrowsize=1 2,arrowlength=1,arrowinset=0.25,tbarsize=0.7 5,bracketlength=0.15,rbracketlength=0.15}
\begin{pspicture}(0,0)(8.75,13.13)
\pspolygon[](-3.74,8.75)(-0,8.75)(-0,5)(-3.74,5)
\rput(-1.88,6.86){$\fun$}
\rput{90}(2.5,-1.88){\psellipse[fillstyle=solid](0,0)(1.57,-1.56)}
\pscustom[]{\psline(2.5,-6.26)(2.5,-6.88)
\psbezier(2.5,-6.88)(2.5,-6.88)(2.5,-6.88)
\psline(2.5,-6.88)(2.5,-3.12)
}
\pscustom[]{\psline(6.88,9.38)(6.88,8.75)
\psbezier(6.88,8.75)(6.88,8.75)(6.88,8.75)
\psline(6.88,8.75)(6.88,13.13)
}
\psline(2.5,-2.49)
(-0.63,0.62)
(-1.87,1.88)(-1.87,5)
\psline(3.13,-1.88)
(6.87,1.88)
(6.87,3.12)(6.87,5)
\pspolygon[](5,8.75)(8.75,8.75)(8.75,5)(5,5)
\rput(6.88,6.86){$\fun$}
\pscustom[]{\psline(-1.88,9.38)(-1.88,8.75)
\psbezier(-1.88,8.75)(-1.88,8.75)(-1.88,8.75)
\psline(-1.88,8.75)(-1.88,13.13)
}
\end{pspicture}


==> PIC/frob-WF.tex <==
%%Created by jPicEdt 1.4.1_03: mixed JPIC-XML/LaTeX format
%%Thu Dec 17 15:32:01 GMT-10:00 2020
%%Begin JPIC-XML
%<?xml version="1.0" standalone="yes"?>
%<jpic x-min="0" x-max="41.57" y-min="1.25" y-max="35" auto-bounding="true">
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(22.5,17.5)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\EQLS
%</text>
%<ellipse p3= "(4.06,12.19)"
%	 fill-style= "solid"
%	 p2= "(4.07,15.31)"
%	 p1= "(0.94,15.31)"
%	 closure= "open"
%	 angle-end= "0"
%	 angle-start= "0"
%	 />
%<multicurve fill-style= "none"
%	 points= "(2.5,13.75);(2.5,13.75);(10,21.25);(10,21.25);(10,21.25);(10,21.25);
%	(10,21.25);(10,21.25);(10,21.25);(10,21.25)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(10,21.25);(10,21.25);(10,32.5);(10,32.5)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(10,21.25);(10,21.25);(12.5,18.75);(12.5,18.75)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(12.5,15);(12.5,15);(12.5,18.75);(12.5,18.75)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(2.5,5);(2.5,5);(2.5,13.75);(2.5,13.75)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(0,16.25);(0,16.25);(2.5,13.75);(2.5,13.75)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(0,16.25);(0,16.25);(0,32.5);(0,32.5)"
%	 />
%<ellipse p3= "(11.57,19.69)"
%	 fill-style= "none"
%	 p2= "(11.56,22.81)"
%	 p1= "(8.43,22.81)"
%	 closure= "open"
%	 angle-end= "0"
%	 angle-start= "0"
%	 />
%<ellipse p3= "(36.56,22.19)"
%	 fill-style= "solid"
%	 p2= "(36.57,25.31)"
%	 p1= "(33.44,25.31)"
%	 closure= "open"
%	 stroke-overstrike-width= "2"
%	 angle-end= "0"
%	 stroke-overstrike= "true"
%	 angle-start= "0"
%	 />
%<multicurve fill-style= "none"
%	 points= "(30,28.75);(30,28.75);(35,23.75);(35,23.75)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(30,28.75);(30,28.75);(30,32.5);(30,32.5)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(40,4.38);(40,4.38);(40,6.25);(40,6.25)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(35,20);(35,20);(35,23.75);(35,23.75)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(30,5);(30,5);(30,6.25);(30,6.25)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(40,28.75);(40,28.75);(35,23.75);(35,23.75)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(40,28.75);(40,28.75);(40,32.5);(40,32.5)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(32.5,22.5);(32.5,22.5);(37.5,17.5);(37.5,17.5)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(37.5,17.5);(37.5,17.5);(37.5,12.5);(37.5,12.5)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(32.5,22.5);(32.5,22.5);(32.5,17.5);(32.5,17.5)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(32.5,17.5);(32.5,17.5);(37.5,12.5);(37.5,12.5)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(10,17.5);(10,17.5);(15,12.5);(15,12.5)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(10,17.5);(10,17.5);(10,12.5);(10,12.5)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(10,12.5);(10,12.5);(15,7.5);(15,7.5)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(12.5,3.75);(12.5,3.75);(12.5,10);(12.5,10)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(15,12.5);(15,12.5);(15,7.5);(15,7.5)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(0,5);(0,5);(5,5);(5,5)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(5,5);(5,5);(2.5,2.5);(2.5,2.5)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(2.5,2.5);(2.5,2.5);(0,5);(0,5)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(27.5,5);(27.5,5);(32.5,5);(32.5,5)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(32.5,5);(32.5,5);(30,2.5);(30,2.5)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(30,2.5);(30,2.5);(27.5,5);(27.5,5)"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(35,17.5)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\Aah$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(12.5,12.5)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\Aah$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(30,1.25)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\aah$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(2.5,1.25)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\aah$
%</text>
%<ellipse p3= "(36.57,9.69)"
%	 fill-style= "none"
%	 p2= "(36.56,12.81)"
%	 p1= "(33.43,12.81)"
%	 closure= "open"
%	 angle-end= "0"
%	 angle-start= "0"
%	 />
%<multicurve fill-style= "none"
%	 points= "(35,11.25);(35,11.25);(40,6.25);(40,6.25)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(35,11.25);(35,11.25);(35,15);(35,15)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(35,11.25);(35,11.25);(30,6.25);(30,6.25)"
%	 />
%<ellipse p3= "(14.06,1.56)"
%	 fill-style= "solid"
%	 p2= "(14.07,4.69)"
%	 fill-color= "#ffffff"
%	 p1= "(10.94,4.69)"
%	 closure= "open"
%	 angle-end= "0"
%	 angle-start= "0"
%	 />
%<ellipse p3= "(41.56,2.19)"
%	 fill-style= "solid"
%	 p2= "(41.57,5.31)"
%	 fill-color= "#ffffff"
%	 p1= "(38.44,5.31)"
%	 closure= "open"
%	 angle-end= "0"
%	 angle-start= "0"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(0,35)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\aah$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(28.75,35)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\Aaah$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(10,35)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\aAxh$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(41.25,35)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\Aaah$
%</text>
%</jpic>
%%End JPIC-XML
%PSTricks content-type (pstricks.sty package needed)
%Add \usepackage{pstricks} in the preamble of your LaTeX file
%You can rescale the whole picture (to 80% for instance) by using the command \def\JPicScale{0.8}
\ifx\JPicScale\undefined\def\JPicScale{1}\fi
\psset{unit=\JPicScale mm}
\psset{linewidth=0.3,dotsep=1,hatchwidth=0.3,hatchsep=1.5,shadowsize=1,dimen=middle}
\psset{dotsize=0.7 2.5,dotscale=1 1,fillcolor=black}
\psset{arrowsize=1 2,arrowlength=1,arrowinset=0.25,tbarsize=0.7 5,bracketlength=0.15,rbracketlength=0.15}
\begin{pspicture}(0,0)(41.57,35)
\rput(22.5,17.5){\EQLS}
\rput{22.45}(2.5,13.75){\psellipse[fillstyle=solid](0,0)(1.57,-1.56)}
\pscustom[]{\psline(2.5,13.75)(10,21.25)
\psbezier(10,21.25)(10,21.25)(10,21.25)
\psbezier(10,21.25)(10,21.25)(10,21.25)
}
\psline(10,21.25)(10,32.5)
\psline(10,21.25)(12.5,18.75)
\psline(12.5,15)(12.5,18.75)
\psline(2.5,5)(2.5,13.75)
\psline(0,16.25)(2.5,13.75)
\psline(0,16.25)(0,32.5)
\rput{-22.45}(10,21.25){\psellipse[](0,0)(1.57,-1.56)}
\rput{22.45}(35,23.75){\psellipse[border=2,fillstyle=solid](0,0)(1.57,-1.56)}
\psline(30,28.75)(35,23.75)
\psline(30,28.75)(30,32.5)
\psline(40,4.38)(40,6.25)
\psline(35,20)(35,23.75)
\psline(30,5)(30,6.25)
\psline(40,28.75)(35,23.75)
\psline(40,28.75)(40,32.5)
\psline(32.5,22.5)(37.5,17.5)
\psline(37.5,17.5)(37.5,12.5)
\psline(32.5,22.5)(32.5,17.5)
\psline(32.5,17.5)(37.5,12.5)
\psline(10,17.5)(15,12.5)
\psline(10,17.5)(10,12.5)
\psline(10,12.5)(15,7.5)
\psline(12.5,3.75)(12.5,10)
\psline(15,12.5)(15,7.5)
\psline(0,5)(5,5)
\psline(5,5)(2.5,2.5)
\psline(2.5,2.5)(0,5)
\psline(27.5,5)(32.5,5)
\psline(32.5,5)(30,2.5)
\psline(30,2.5)(27.5,5)
\rput(35,17.5){$\Aah$}
\rput(12.5,12.5){$\Aah$}
\rput(30,1.25){$\aah$}
\rput(2.5,1.25){$\aah$}
\rput{-22.45}(35,11.25){\psellipse[](0,0)(1.57,-1.56)}
\psline(35,11.25)(40,6.25)
\psline(35,11.25)(35,15)
\psline(35,11.25)(30,6.25)
\rput{22.45}(12.5,3.12){\psellipse[fillcolor=white,fillstyle=solid](0,0)(1.57,-1.56)}
\rput{22.45}(40,3.75){\psellipse[fillcolor=white,fillstyle=solid](0,0)(1.57,-1.56)}
\rput(0,35){$\aah$}
\rput(28.75,35){$\Aaah$}
\rput(10,35){$\aAxh$}
\rput(41.25,35){$\Aaah$}
\end{pspicture}


==> PIC/frob-WO.tex <==
%%Created by jPicEdt 1.4.1_03: mixed JPIC-XML/LaTeX format
%%Mon Dec 21 23:56:04 GMT-10:00 2020
%%Begin JPIC-XML
%<?xml version="1.0" standalone="yes"?>
%<jpic x-min="0" x-max="237.5" y-min="1.25" y-max="60" auto-bounding="true">
%<ellipse p3= "(6.56,44.69)"
%	 fill-style= "solid"
%	 p2= "(6.57,47.81)"
%	 p1= "(3.44,47.81)"
%	 closure= "open"
%	 stroke-overstrike-width= "2"
%	 angle-end= "0"
%	 stroke-overstrike= "true"
%	 angle-start= "0"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(120,42.5)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\EQLS
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(20,35)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\EQLS
%</text>
%<ellipse p3= "(104.06,37.19)"
%	 fill-style= "solid"
%	 p2= "(104.07,40.31)"
%	 p1= "(100.94,40.31)"
%	 closure= "open"
%	 angle-end= "0"
%	 angle-start= "0"
%	 />
%<ellipse p3= "(38.43,40.31)"
%	 fill-style= "solid"
%	 p2= "(38.44,37.19)"
%	 p1= "(41.57,37.19)"
%	 closure= "open"
%	 angle-end= "0"
%	 angle-start= "0"
%	 />
%<multicurve fill-style= "none"
%	 points= "(40,38.75);(40,38.75);(42.5,41.25);(42.5,41.25)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(42.5,41.25);(42.5,41.25);(42.5,55);(42.5,55)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(40,30);(40,30);(40,38.75);(40,38.75)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(30,21.25);(30,21.25);(30,43.75);(30,43.75)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(112.5,30);(112.5,30);(112.5,43.75);(112.5,43.75)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(102.5,21.25);(102.5,21.25);(102.5,38.75);(102.5,38.75)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(100,41.25);(100,41.25);(102.5,38.75);(102.5,38.75)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(100,41.25);(100,41.25);(100,55);(100,55)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(0,51.25);(0,51.25);(5,46.25);(5,46.25)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(0,51.25);(0,51.25);(0,55);(0,55)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(10,30);(10,30);(10,33.75);(10,33.75)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(0,21.25);(0,21.25);(0,33.75);(0,33.75)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(10,51.25);(10,51.25);(5,46.25);(5,46.25)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(40,21.25);(40,21.25);(40,25);(40,25)"
%	 />
%<ellipse p3= "(6.57,37.19)"
%	 fill-style= "solid"
%	 p2= "(6.56,40.31)"
%	 fill-color= "#ffffff"
%	 p1= "(3.43,40.31)"
%	 closure= "open"
%	 angle-end= "0"
%	 angle-start= "0"
%	 />
%<ellipse p3= "(111.57,44.69)"
%	 fill-style= "solid"
%	 p2= "(111.56,47.81)"
%	 fill-color= "#ffffff"
%	 p1= "(108.43,47.81)"
%	 closure= "open"
%	 angle-end= "0"
%	 angle-start= "0"
%	 />
%<ellipse p3= "(30.94,47.81)"
%	 fill-style= "solid"
%	 p2= "(30.94,44.69)"
%	 fill-color= "#ffffff"
%	 p1= "(34.07,44.69)"
%	 closure= "open"
%	 angle-end= "0"
%	 angle-start= "0"
%	 />
%<ellipse p3= "(131.56,44.69)"
%	 fill-style= "solid"
%	 p2= "(131.57,47.81)"
%	 p1= "(128.44,47.81)"
%	 closure= "open"
%	 stroke-overstrike-width= "2"
%	 angle-end= "0"
%	 stroke-overstrike= "true"
%	 angle-start= "0"
%	 />
%<multicurve fill-style= "none"
%	 points= "(125,51.25);(125,51.25);(130,46.25);(130,46.25)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(125,51.25);(125,51.25);(125,55);(125,55)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(135,30);(135,30);(135,33.75);(135,33.75)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(125,21.25);(125,21.25);(125,33.75);(125,33.75)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(135,51.25);(135,51.25);(130,46.25);(130,46.25)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(135,51.25);(135,51.25);(135,55);(135,55)"
%	 />
%<ellipse p3= "(131.57,37.19)"
%	 fill-style= "solid"
%	 p2= "(131.56,40.31)"
%	 fill-color= "#ffffff"
%	 p1= "(128.43,40.31)"
%	 closure= "open"
%	 angle-end= "0"
%	 angle-start= "0"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(140,40)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\ORR
%</text>
%<multicurve fill-style= "none"
%	 points= "(200,20);(200,20);(205,20);(205,20)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(200,20);(200,20);(202.5,17.5);(202.5,17.5)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(202.5,17.5);(202.5,17.5);(205,20);(205,20)"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(202.5,15)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\xee$
%</text>
%<multicurve fill-style= "none"
%	 points= "(222.5,20);(222.5,20);(227.5,20);(227.5,20)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(222.5,20);(222.5,20);(225,17.5);(225,17.5)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(225,17.5);(225,17.5);(227.5,20);(227.5,20)"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(225,15)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\xee$
%</text>
%<multicurve fill-style= "none"
%	 points= "(127.5,60);(127.5,60);(132.5,60);(132.5,60)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(127.5,60);(127.5,60);(130,57.5);(130,57.5)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(130,57.5);(130,57.5);(132.5,60);(132.5,60)"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(130,55)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\xee$
%</text>
%<multicurve fill-style= "none"
%	 points= "(37.5,25);(37.5,25);(42.5,25);(42.5,25)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(150,60);(150,60);(152.5,57.5);(152.5,57.5)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(35,1.25);(35,1.25);(35,16.25);(35,16.25)"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(152.5,55)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\xee$
%</text>
%<multicurve fill-style= "none"
%	 points= "(37.5,30);(37.5,30);(42.5,30);(42.5,30)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(37.5,30);(37.5,30);(37.5,25);(37.5,25)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(42.5,25);(42.5,25);(42.5,30);(42.5,30)"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(162.5,55)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\yee$
%</text>
%<multicurve fill-style= "none"
%	 points= "(137.5,60);(137.5,60);(142.5,60);(142.5,60)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(137.5,60);(137.5,60);(140,57.5);(140,57.5)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(140,57.5);(140,57.5);(142.5,60);(142.5,60)"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(140,55)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\yee$
%</text>
%<multicurve fill-style= "none"
%	 points= "(232.5,20);(232.5,20);(237.5,20);(237.5,20)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(232.5,20);(232.5,20);(235,17.5);(235,17.5)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(235,17.5);(235,17.5);(237.5,20);(237.5,20)"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(235,15)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\yee$
%</text>
%<multicurve fill-style= "none"
%	 points= "(210,20);(210,20);(215,20);(215,20)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(210,20);(210,20);(212.5,17.5);(212.5,17.5)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(212.5,17.5);(212.5,17.5);(215,20);(215,20)"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(212.5,15)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\yee$
%</text>
%<multicurve fill-style= "none"
%	 points= "(102.5,38.75);(102.5,38.75);(110,46.25);(110,46.25);(110,46.25);(110,46.25);
%	(110,46.25);(110,46.25);(110,46.25);(110,46.25)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(32.5,46.25);(32.5,46.25);(40,38.75);(40,38.75);(40,38.75);(40,38.75);
%	(40,38.75);(40,38.75);(40,38.75);(40,38.75)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(30,43.75);(30,43.75);(32.5,46.25);(32.5,46.25)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(110,46.25);(110,46.25);(110,55);(110,55)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(32.5,46.25);(32.5,46.25);(32.5,55);(32.5,55)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(110,46.25);(110,46.25);(112.5,43.75);(112.5,43.75)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(5,38.75);(5,38.75);(10,33.75);(10,33.75)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(5,38.75);(5,38.75);(5,46.25);(5,46.25)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(5,38.75);(5,38.75);(0,33.75);(0,33.75)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(130,38.75);(130,38.75);(135,33.75);(135,33.75)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(130,38.75);(130,38.75);(130,46.25);(130,46.25)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(130,38.75);(130,38.75);(125,33.75);(125,33.75)"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(100,57.5)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\xee$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(110,57.5)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\xyee$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(125,57.5)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\xyee$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(135,57.5)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\xyee$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(0,57.5)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\xyee$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(10,57.5)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\xyee$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(32.5,57.5)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\xyee$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(42.5,57.5)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\yee$
%</text>
%<ellipse p3= "(36.56,14.69)"
%	 fill-style= "solid"
%	 p2= "(36.57,17.81)"
%	 p1= "(33.44,17.81)"
%	 closure= "open"
%	 angle-end= "0"
%	 angle-start= "0"
%	 />
%<multicurve fill-style= "none"
%	 points= "(30,21.25);(30,21.25);(35,16.25);(35,16.25)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(40,21.25);(40,21.25);(35,16.25);(35,16.25)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(10,51.25);(10,51.25);(10,55);(10,55)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(7.5,25);(7.5,25);(12.5,25);(12.5,25)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(7.5,30);(7.5,30);(12.5,30);(12.5,30)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(7.5,30);(7.5,30);(7.5,25);(7.5,25)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(12.5,25);(12.5,25);(12.5,30);(12.5,30)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(10,21.25);(10,21.25);(10,25);(10,25)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(5,1.25);(5,1.25);(5,16.25);(5,16.25)"
%	 />
%<ellipse p3= "(6.56,14.69)"
%	 fill-style= "solid"
%	 p2= "(6.57,17.81)"
%	 p1= "(3.44,17.81)"
%	 closure= "open"
%	 angle-end= "0"
%	 angle-start= "0"
%	 />
%<multicurve fill-style= "none"
%	 points= "(0,21.25);(0,21.25);(5,16.25);(5,16.25)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(10,21.25);(10,21.25);(5,16.25);(5,16.25)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(127.5,6.25);(127.5,6.25);(132.5,6.25);(132.5,6.25)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(127.5,11.25);(127.5,11.25);(132.5,11.25);(132.5,11.25)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(127.5,11.25);(127.5,11.25);(127.5,6.25);(127.5,6.25)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(132.5,6.25);(132.5,6.25);(132.5,11.25);(132.5,11.25)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(112.5,21.25);(112.5,21.25);(112.5,25);(112.5,25)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(110,25);(110,25);(115,25);(115,25)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(107.5,11.25);(107.5,11.25);(107.5,16.25);(107.5,16.25)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(110,30);(110,30);(115,30);(115,30)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(110,30);(110,30);(110,25);(110,25)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(115,25);(115,25);(115,30);(115,30)"
%	 />
%<ellipse p3= "(109.06,14.69)"
%	 fill-style= "solid"
%	 p2= "(109.07,17.81)"
%	 p1= "(105.94,17.81)"
%	 closure= "open"
%	 angle-end= "0"
%	 angle-start= "0"
%	 />
%<multicurve fill-style= "none"
%	 points= "(102.5,21.25);(102.5,21.25);(107.5,16.25);(107.5,16.25)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(112.5,21.25);(112.5,21.25);(107.5,16.25);(107.5,16.25)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(132.5,25);(132.5,25);(137.5,25);(137.5,25)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(132.5,30);(132.5,30);(137.5,30);(137.5,30)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(132.5,30);(132.5,30);(132.5,25);(132.5,25)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(137.5,25);(137.5,25);(137.5,30);(137.5,30)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(135,21.25);(135,21.25);(135,25);(135,25)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(130,11.25);(130,11.25);(130,16.25);(130,16.25)"
%	 />
%<ellipse p3= "(131.56,14.69)"
%	 fill-style= "solid"
%	 p2= "(131.57,17.81)"
%	 p1= "(128.44,17.81)"
%	 closure= "open"
%	 angle-end= "0"
%	 angle-start= "0"
%	 />
%<multicurve fill-style= "none"
%	 points= "(125,21.25);(125,21.25);(130,16.25);(130,16.25)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(135,21.25);(135,21.25);(130,16.25);(130,16.25)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(105,6.25);(105,6.25);(110,6.25);(110,6.25)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(105,11.25);(105,11.25);(110,11.25);(110,11.25)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(105,11.25);(105,11.25);(105,6.25);(105,6.25)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(110,6.25);(110,6.25);(110,11.25);(110,11.25)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(130,1.25);(130,1.25);(130,6.25);(130,6.25)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(107.5,1.25);(107.5,1.25);(107.5,6.25);(107.5,6.25)"
%	 />
%</jpic>
%%End JPIC-XML
%PSTricks content-type (pstricks.sty package needed)
%Add \usepackage{pstricks} in the preamble of your LaTeX file
%You can rescale the whole picture (to 80% for instance) by using the command \def\JPicScale{0.8}
\ifx\JPicScale\undefined\def\JPicScale{1}\fi
\psset{unit=\JPicScale mm}
\psset{linewidth=0.3,dotsep=1,hatchwidth=0.3,hatchsep=1.5,shadowsize=1,dimen=middle}
\psset{dotsize=0.7 2.5,dotscale=1 1,fillcolor=black}
\psset{arrowsize=1 2,arrowlength=1,arrowinset=0.25,tbarsize=0.7 5,bracketlength=0.15,rbracketlength=0.15}
\begin{pspicture}(0,0)(237.5,60)
\rput{22.45}(5,46.25){\psellipse[border=2,fillstyle=solid](0,0)(1.57,-1.56)}
\rput(120,42.5){\EQLS}
\rput(20,35){\EQLS}
\rput{22.45}(102.5,38.75){\psellipse[fillstyle=solid](0,0)(1.57,-1.56)}
\rput{-22.45}(40,38.75){\psellipse[fillstyle=solid](0,0)(1.57,-1.56)}
\psline(40,38.75)(42.5,41.25)
\psline(42.5,41.25)(42.5,55)
\psline(40,30)(40,38.75)
\psline(30,21.25)(30,43.75)
\psline(112.5,30)(112.5,43.75)
\psline(102.5,21.25)(102.5,38.75)
\psline(100,41.25)(102.5,38.75)
\psline(100,41.25)(100,55)
\psline(0,51.25)(5,46.25)
\psline(0,51.25)(0,55)
\psline(10,30)(10,33.75)
\psline(0,21.25)(0,33.75)
\psline(10,51.25)(5,46.25)
\psline(40,21.25)(40,25)
\rput{-22.45}(5,38.75){\psellipse[fillcolor=white,fillstyle=solid](0,0)(1.57,-1.56)}
\rput{-22.45}(110,46.25){\psellipse[fillcolor=white,fillstyle=solid](0,0)(1.57,-1.56)}
\rput{0}(32.5,46.25){\psellipse[fillcolor=white,fillstyle=solid](0,0)(1.57,-1.56)}
\rput{22.45}(130,46.25){\psellipse[border=2,fillstyle=solid](0,0)(1.57,-1.56)}
\psline(125,51.25)(130,46.25)
\psline(125,51.25)(125,55)
\psline(135,30)(135,33.75)
\psline(125,21.25)(125,33.75)
\psline(135,51.25)(130,46.25)
\psline(135,51.25)(135,55)
\rput{-22.45}(130,38.75){\psellipse[fillcolor=white,fillstyle=solid](0,0)(1.57,-1.56)}
\rput(140,40){\ORR}
\psline(200,20)(205,20)
\psline(200,20)(202.5,17.5)
\psline(202.5,17.5)(205,20)
\rput(202.5,15){$\xee$}
\psline(222.5,20)(227.5,20)
\psline(222.5,20)(225,17.5)
\psline(225,17.5)(227.5,20)
\rput(225,15){$\xee$}
\psline(127.5,60)(132.5,60)
\psline(127.5,60)(130,57.5)
\psline(130,57.5)(132.5,60)
\rput(130,55){$\xee$}
\psline(37.5,25)(42.5,25)
\psline(150,60)(152.5,57.5)
\psline(35,1.25)(35,16.25)
\rput(152.5,55){$\xee$}
\psline(37.5,30)(42.5,30)
\psline(37.5,30)(37.5,25)
\psline(42.5,25)(42.5,30)
\rput(162.5,55){$\yee$}
\psline(137.5,60)(142.5,60)
\psline(137.5,60)(140,57.5)
\psline(140,57.5)(142.5,60)
\rput(140,55){$\yee$}
\psline(232.5,20)(237.5,20)
\psline(232.5,20)(235,17.5)
\psline(235,17.5)(237.5,20)
\rput(235,15){$\yee$}
\psline(210,20)(215,20)
\psline(210,20)(212.5,17.5)
\psline(212.5,17.5)(215,20)
\rput(212.5,15){$\yee$}
\pscustom[]{\psline(102.5,38.75)(110,46.25)
\psbezier(110,46.25)(110,46.25)(110,46.25)
\psbezier(110,46.25)(110,46.25)(110,46.25)
}
\pscustom[]{\psline(32.5,46.25)(40,38.75)
\psbezier(40,38.75)(40,38.75)(40,38.75)
\psbezier(40,38.75)(40,38.75)(40,38.75)
}
\psline(30,43.75)(32.5,46.25)
\psline(110,46.25)(110,55)
\psline(32.5,46.25)(32.5,55)
\psline(110,46.25)(112.5,43.75)
\psline(5,38.75)(10,33.75)
\psline(5,38.75)(5,46.25)
\psline(5,38.75)(0,33.75)
\psline(130,38.75)(135,33.75)
\psline(130,38.75)(130,46.25)
\psline(130,38.75)(125,33.75)
\rput(100,57.5){$\xee$}
\rput(110,57.5){$\xyee$}
\rput(125,57.5){$\xyee$}
\rput(135,57.5){$\xyee$}
\rput(0,57.5){$\xyee$}
\rput(10,57.5){$\xyee$}
\rput(32.5,57.5){$\xyee$}
\rput(42.5,57.5){$\yee$}
\rput{22.45}(35,16.25){\psellipse[fillstyle=solid](0,0)(1.57,-1.56)}
\psline(30,21.25)(35,16.25)
\psline(40,21.25)(35,16.25)
\psline(10,51.25)(10,55)
\psline(7.5,25)(12.5,25)
\psline(7.5,30)(12.5,30)
\psline(7.5,30)(7.5,25)
\psline(12.5,25)(12.5,30)
\psline(10,21.25)(10,25)
\psline(5,1.25)(5,16.25)
\rput{22.45}(5,16.25){\psellipse[fillstyle=solid](0,0)(1.57,-1.56)}
\psline(0,21.25)(5,16.25)
\psline(10,21.25)(5,16.25)
\psline(127.5,6.25)(132.5,6.25)
\psline(127.5,11.25)(132.5,11.25)
\psline(127.5,11.25)(127.5,6.25)
\psline(132.5,6.25)(132.5,11.25)
\psline(112.5,21.25)(112.5,25)
\psline(110,25)(115,25)
\psline(107.5,11.25)(107.5,16.25)
\psline(110,30)(115,30)
\psline(110,30)(110,25)
\psline(115,25)(115,30)
\rput{22.45}(107.5,16.25){\psellipse[fillstyle=solid](0,0)(1.57,-1.56)}
\psline(102.5,21.25)(107.5,16.25)
\psline(112.5,21.25)(107.5,16.25)
\psline(132.5,25)(137.5,25)
\psline(132.5,30)(137.5,30)
\psline(132.5,30)(132.5,25)
\psline(137.5,25)(137.5,30)
\psline(135,21.25)(135,25)
\psline(130,11.25)(130,16.25)
\rput{22.45}(130,16.25){\psellipse[fillstyle=solid](0,0)(1.57,-1.56)}
\psline(125,21.25)(130,16.25)
\psline(135,21.25)(130,16.25)
\psline(105,6.25)(110,6.25)
\psline(105,11.25)(110,11.25)
\psline(105,11.25)(105,6.25)
\psline(110,6.25)(110,11.25)
\psline(130,1.25)(130,6.25)
\psline(107.5,1.25)(107.5,6.25)
\end{pspicture}


==> PIC/frob-def.tex <==
%%Created by jPicEdt 1.4.1_03: mixed JPIC-XML/LaTeX format
%%Sat Jun 05 21:48:21 GMT-10:00 2021
%%Begin JPIC-XML
%<?xml version="1.0" standalone="yes"?>
%<jpic x-min="25" x-max="60" y-min="0" y-max="25" auto-bounding="true">
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(40,12.5)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\EQLS
%</text>
%<multicurve fill-style= "none"
%	 points= "(50,16.25);(50,16.25);(57.5,8.75);(57.5,8.75);(57.5,8.75);(57.5,8.75);
%	(57.5,8.75);(57.5,8.75);(57.5,8.75);(57.5,8.75)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(57.5,8.75);(57.5,8.75);(60,11.25);(60,11.25)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(60,11.25);(60,11.25);(60,25);(60,25)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(57.5,0);(57.5,0);(57.5,8.75);(57.5,8.75)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(47.5,13.75);(47.5,13.75);(50,16.25);(50,16.25)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(47.5,0);(47.5,0);(47.5,13.75);(47.5,13.75)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(50,16.25);(50,16.25);(50,25);(50,25)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(25,21.25);(25,21.25);(30,16.25);(30,16.25)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(25,21.25);(25,21.25);(25,25);(25,25)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(30,8.75);(30,8.75);(35,3.75);(35,3.75)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(35,0);(35,0);(35,3.75);(35,3.75)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(30,8.75);(30,8.75);(30,16.25);(30,16.25)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(30,8.75);(30,8.75);(25,3.75);(25,3.75)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(25,0);(25,0);(25,3.75);(25,3.75)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(35,21.25);(35,21.25);(30,16.25);(30,16.25)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(35,21.25);(35,21.25);(35,25);(35,25)"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(30,16.25)"
%	 stroke-color= "#ff0033"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\DOTT
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(30,8.75)"
%	 stroke-color= "#ff0033"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\DOTT
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(50,16.25)"
%	 stroke-color= "#ff0033"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\DOTT
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(57.5,8.75)"
%	 stroke-color= "#ff0033"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\DOTT
%</text>
%</jpic>
%%End JPIC-XML
%LaTeX-picture environment using emulated lines and arcs
%You can rescale the whole picture (to 80% for instance) by using the command \def\JPicScale{0.8}
\ifx\JPicScale\undefined\def\JPicScale{1}\fi
\unitlength \JPicScale mm
\begin{picture}(60,25)(0,0)
\put(40,12.5){\makebox(0,0)[cc]{\EQLS}}

\linethickness{0.3mm}
\multiput(50,16.25)(0.12,-0.12){63}{\line(1,0){0.12}}
\linethickness{0.3mm}
\multiput(57.5,8.75)(0.12,0.12){21}{\line(1,0){0.12}}
\linethickness{0.3mm}
\put(60,11.25){\line(0,1){13.75}}
\linethickness{0.3mm}
\put(57.5,0){\line(0,1){8.75}}
\linethickness{0.3mm}
\multiput(47.5,13.75)(0.12,0.12){21}{\line(1,0){0.12}}
\linethickness{0.3mm}
\put(47.5,0){\line(0,1){13.75}}
\linethickness{0.3mm}
\put(50,16.25){\line(0,1){8.75}}
\linethickness{0.3mm}
\multiput(25,21.25)(0.12,-0.12){42}{\line(1,0){0.12}}
\linethickness{0.3mm}
\put(25,21.25){\line(0,1){3.75}}
\linethickness{0.3mm}
\multiput(30,8.75)(0.12,-0.12){42}{\line(1,0){0.12}}
\linethickness{0.3mm}
\put(35,0){\line(0,1){3.75}}
\linethickness{0.3mm}
\put(30,8.75){\line(0,1){7.5}}
\linethickness{0.3mm}
\multiput(25,3.75)(0.12,0.12){42}{\line(1,0){0.12}}
\linethickness{0.3mm}
\put(25,0){\line(0,1){3.75}}
\linethickness{0.3mm}
\multiput(30,16.25)(0.12,0.12){42}{\line(1,0){0.12}}
\linethickness{0.3mm}
\put(35,21.25){\line(0,1){3.75}}
\put(30,16.25){\makebox(0,0)[cc]{\DOTT}}

\put(30,8.75){\makebox(0,0)[cc]{\DOTT}}

\put(50,16.25){\makebox(0,0)[cc]{\DOTT}}

\put(57.5,8.75){\makebox(0,0)[cc]{\DOTT}}

\end{picture}


==> PIC/frob-law-3-white.tex <==
%%Created by jPicEdt 1.4.1_03: mixed JPIC-XML/LaTeX format
%%Sat Dec 12 10:19:00 GMT-10:00 2020
%%Begin JPIC-XML
%<?xml version="1.0" standalone="yes"?>
%<jpic x-min="0" x-max="152.5" y-min="0" y-max="25" auto-bounding="true">
%<ellipse p3= "(74.06,14.69)"
%	 fill-style= "solid"
%	 p2= "(74.07,17.81)"
%	 p1= "(70.94,17.81)"
%	 closure= "open"
%	 stroke-overstrike-width= "2"
%	 angle-end= "0"
%	 stroke-overstrike= "true"
%	 angle-start= "0"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(20,12.5)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\EQLS
%</text>
%<ellipse p3= "(141.56,3.44)"
%	 fill-style= "solid"
%	 p2= "(141.56,6.56)"
%	 p1= "(138.44,6.56)"
%	 closure= "open"
%	 angle-end= "0"
%	 angle-start= "0"
%	 />
%<multicurve fill-style= "none"
%	 points= "(140,0);(140,0);(140,5);(140,5)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(140,5);(140,5);(142.5,7.5);(142.5,7.5)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(140,5);(140,5);(137.5,7.5);(137.5,7.5)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(152.5,0);(152.5,0);(152.5,25);(152.5,25)"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(147.5,12.5)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\EQLS
%</text>
%<multicurve fill-style= "none"
%	 points= "(140,20);(140,20);(140,25);(140,25)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(137.5,17.5);(137.5,17.5);(140,20);(140,20)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(142.5,17.5);(142.5,17.5);(140,20);(140,20)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(137.5,7.5);(137.5,7.5);(137.5,17.5);(137.5,17.5)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(142.5,7.5);(142.5,7.5);(142.5,17.5);(142.5,17.5)"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(82.5,12.5)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\EQLS
%</text>
%<ellipse p3= "(4.06,7.19)"
%	 fill-style= "solid"
%	 p2= "(4.07,10.31)"
%	 p1= "(0.94,10.31)"
%	 closure= "open"
%	 angle-end= "0"
%	 angle-start= "0"
%	 />
%<multicurve fill-style= "none"
%	 points= "(2.5,8.75);(2.5,8.75);(10,16.25);(10,16.25);(10,16.25);(10,16.25);
%	(10,16.25);(10,16.25);(10,16.25);(10,16.25)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(92.5,16.25);(92.5,16.25);(100,8.75);(100,8.75);(100,8.75);(100,8.75);
%	(100,8.75);(100,8.75);(100,8.75);(100,8.75)"
%	 />
%<ellipse p3= "(98.43,10.31)"
%	 fill-style= "solid"
%	 p2= "(98.44,7.19)"
%	 p1= "(101.57,7.19)"
%	 closure= "open"
%	 angle-end= "0"
%	 angle-start= "0"
%	 />
%<multicurve fill-style= "none"
%	 points= "(100,8.75);(100,8.75);(102.5,11.25);(102.5,11.25)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(102.5,11.25);(102.5,11.25);(102.5,25);(102.5,25)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(100,0);(100,0);(100,8.75);(100,8.75)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(90,13.75);(90,13.75);(92.5,16.25);(92.5,16.25)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(90,0);(90,0);(90,13.75);(90,13.75)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(10,16.25);(10,16.25);(10,25);(10,25)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(92.5,16.25);(92.5,16.25);(92.5,25);(92.5,25)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(10,16.25);(10,16.25);(12.5,13.75);(12.5,13.75)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(12.5,0);(12.5,0);(12.5,13.75);(12.5,13.75)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(2.5,0);(2.5,0);(2.5,8.75);(2.5,8.75)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(0,11.25);(0,11.25);(2.5,8.75);(2.5,8.75)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(0,11.25);(0,11.25);(0,25);(0,25)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(67.5,21.25);(67.5,21.25);(72.5,16.25);(72.5,16.25)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(67.5,21.25);(67.5,21.25);(67.5,25);(67.5,25)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(72.5,8.75);(72.5,8.75);(77.5,3.75);(77.5,3.75)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(77.5,0);(77.5,0);(77.5,3.75);(77.5,3.75)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(72.5,8.75);(72.5,8.75);(72.5,16.25);(72.5,16.25)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(72.5,8.75);(72.5,8.75);(67.5,3.75);(67.5,3.75)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(67.5,0);(67.5,0);(67.5,3.75);(67.5,3.75)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(77.5,21.25);(77.5,21.25);(72.5,16.25);(72.5,16.25)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(77.5,21.25);(77.5,21.25);(77.5,25);(77.5,25)"
%	 />
%<ellipse p3= "(74.07,7.19)"
%	 fill-style= "solid"
%	 p2= "(74.06,10.31)"
%	 fill-color= "#ffffff"
%	 p1= "(70.93,10.31)"
%	 closure= "open"
%	 angle-end= "0"
%	 angle-start= "0"
%	 />
%<ellipse p3= "(141.57,18.44)"
%	 fill-style= "solid"
%	 p2= "(141.57,21.56)"
%	 fill-color= "#ffffff"
%	 p1= "(138.44,21.56)"
%	 closure= "open"
%	 angle-end= "0"
%	 angle-start= "0"
%	 />
%<ellipse p3= "(11.57,14.69)"
%	 fill-style= "solid"
%	 p2= "(11.56,17.81)"
%	 fill-color= "#ffffff"
%	 p1= "(8.43,17.81)"
%	 closure= "open"
%	 angle-end= "0"
%	 angle-start= "0"
%	 />
%<ellipse p3= "(90.94,17.81)"
%	 fill-style= "solid"
%	 p2= "(90.94,14.69)"
%	 fill-color= "#ffffff"
%	 p1= "(94.07,14.69)"
%	 closure= "open"
%	 angle-end= "0"
%	 angle-start= "0"
%	 />
%<ellipse p3= "(31.56,14.69)"
%	 fill-style= "solid"
%	 p2= "(31.57,17.81)"
%	 p1= "(28.44,17.81)"
%	 closure= "open"
%	 stroke-overstrike-width= "2"
%	 angle-end= "0"
%	 stroke-overstrike= "true"
%	 angle-start= "0"
%	 />
%<multicurve fill-style= "none"
%	 points= "(25,21.25);(25,21.25);(30,16.25);(30,16.25)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(25,21.25);(25,21.25);(25,25);(25,25)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(30,8.75);(30,8.75);(35,3.75);(35,3.75)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(35,0);(35,0);(35,3.75);(35,3.75)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(30,8.75);(30,8.75);(30,16.25);(30,16.25)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(30,8.75);(30,8.75);(25,3.75);(25,3.75)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(25,0);(25,0);(25,3.75);(25,3.75)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(35,21.25);(35,21.25);(30,16.25);(30,16.25)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(35,21.25);(35,21.25);(35,25);(35,25)"
%	 />
%<ellipse p3= "(31.57,7.19)"
%	 fill-style= "solid"
%	 p2= "(31.56,10.31)"
%	 fill-color= "#ffffff"
%	 p1= "(28.43,10.31)"
%	 closure= "open"
%	 angle-end= "0"
%	 angle-start= "0"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(51.25,12.5)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\ORR
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(120,12.5)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\ANDD
%</text>
%</jpic>
%%End JPIC-XML
%PSTricks content-type (pstricks.sty package needed)
%Add \usepackage{pstricks} in the preamble of your LaTeX file
%You can rescale the whole picture (to 80% for instance) by using the command \def\JPicScale{0.8}
\ifx\JPicScale\undefined\def\JPicScale{1}\fi
\psset{unit=\JPicScale mm}
\psset{linewidth=0.3,dotsep=1,hatchwidth=0.3,hatchsep=1.5,shadowsize=1,dimen=middle}
\psset{dotsize=0.7 2.5,dotscale=1 1,fillcolor=black}
\psset{arrowsize=1 2,arrowlength=1,arrowinset=0.25,tbarsize=0.7 5,bracketlength=0.15,rbracketlength=0.15}
\begin{pspicture}(0,0)(152.5,25)
\rput{0}(72.5,16.25){\psellipse[border=2,fillstyle=solid](0,0)(1.57,-1.56)}
\rput(20,12.5){\EQLS}
\rput{-0}(140,5){\psellipse[fillstyle=solid](0,0)(1.57,-1.56)}
\psline(140,0)(140,5)
\psline(140,5)(142.5,7.5)
\psline(140,5)(137.5,7.5)
\psline(152.5,0)(152.5,25)
\rput(147.5,12.5){\EQLS}
\psline(140,20)(140,25)
\psline(137.5,17.5)(140,20)
\psline(142.5,17.5)(140,20)
\psline(137.5,7.5)(137.5,17.5)
\psline(142.5,7.5)(142.5,17.5)
\rput(82.5,12.5){\EQLS}
\rput{0}(2.5,8.75){\psellipse[fillstyle=solid](0,0)(1.57,-1.56)}
\pscustom[]{\psline(2.5,8.75)(10,16.25)
\psbezier(10,16.25)(10,16.25)(10,16.25)
\psbezier(10,16.25)(10,16.25)(10,16.25)
}
\pscustom[]{\psline(92.5,16.25)(100,8.75)
\psbezier(100,8.75)(100,8.75)(100,8.75)
\psbezier(100,8.75)(100,8.75)(100,8.75)
}
\rput{0}(100,8.75){\psellipse[fillstyle=solid](0,0)(1.57,-1.56)}
\psline(100,8.75)(102.5,11.25)
\psline(102.5,11.25)(102.5,25)
\psline(100,0)(100,8.75)
\psline(90,13.75)(92.5,16.25)
\psline(90,0)(90,13.75)
\psline(10,16.25)(10,25)
\psline(92.5,16.25)(92.5,25)
\psline(10,16.25)(12.5,13.75)
\psline(12.5,0)(12.5,13.75)
\psline(2.5,0)(2.5,8.75)
\psline(0,11.25)(2.5,8.75)
\psline(0,11.25)(0,25)
\psline(67.5,21.25)(72.5,16.25)
\psline(67.5,21.25)(67.5,25)
\psline(72.5,8.75)(77.5,3.75)
\psline(77.5,0)(77.5,3.75)
\psline(72.5,8.75)(72.5,16.25)
\psline(72.5,8.75)(67.5,3.75)
\psline(67.5,0)(67.5,3.75)
\psline(77.5,21.25)(72.5,16.25)
\psline(77.5,21.25)(77.5,25)
\rput{0}(72.5,8.75){\psellipse[fillcolor=white,fillstyle=solid](0,0)(1.57,-1.56)}
\rput{-0}(140.01,20){\psellipse[fillcolor=white,fillstyle=solid](0,0)(1.56,-1.56)}
\rput{0}(10,16.25){\psellipse[fillcolor=white,fillstyle=solid](0,0)(1.57,-1.56)}
\rput{0}(92.5,16.25){\psellipse[fillcolor=white,fillstyle=solid](0,0)(1.57,-1.56)}
\rput{0}(30,16.25){\psellipse[border=2,fillstyle=solid](0,0)(1.57,-1.56)}
\psline(25,21.25)(30,16.25)
\psline(25,21.25)(25,25)
\psline(30,8.75)(35,3.75)
\psline(35,0)(35,3.75)
\psline(30,8.75)(30,16.25)
\psline(30,8.75)(25,3.75)
\psline(25,0)(25,3.75)
\psline(35,21.25)(30,16.25)
\psline(35,21.25)(35,25)
\rput{0}(30,8.75){\psellipse[fillcolor=white,fillstyle=solid](0,0)(1.57,-1.56)}
\rput(51.25,12.5){\ORR}
\rput(120,12.5){\ANDD}
\end{pspicture}


==> PIC/frob-law-3.tex <==
%%Created by jPicEdt 1.4.1_03: mixed JPIC-XML/LaTeX format
%%Tue Jan 05 06:13:38 GMT-10:00 2021
%%Begin JPIC-XML
%<?xml version="1.0" standalone="yes"?>
%<jpic x-min="0" x-max="132.5" y-min="0" y-max="25" auto-bounding="true">
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(20,12.5)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\EQLS
%</text>
%<multicurve fill-style= "none"
%	 points= "(120,0);(120,0);(120,5);(120,5)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(120,5);(120,5);(122.5,7.5);(122.5,7.5)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(120,5);(120,5);(117.5,7.5);(117.5,7.5)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(132.5,0);(132.5,0);(132.5,25);(132.5,25)"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(127.5,12.5)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\EQLS
%</text>
%<multicurve fill-style= "none"
%	 points= "(120,20);(120,20);(120,25);(120,25)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(117.5,17.5);(117.5,17.5);(120,20);(120,20)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(122.5,17.5);(122.5,17.5);(120,20);(120,20)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(117.5,7.5);(117.5,7.5);(117.5,17.5);(117.5,17.5)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(122.5,7.5);(122.5,7.5);(122.5,17.5);(122.5,17.5)"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(40,12.5)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\EQLS
%</text>
%<multicurve fill-style= "none"
%	 points= "(2.5,8.75);(2.5,8.75);(10,16.25);(10,16.25);(10,16.25);(10,16.25);
%	(10,16.25);(10,16.25);(10,16.25);(10,16.25)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(50,16.25);(50,16.25);(57.5,8.75);(57.5,8.75);(57.5,8.75);(57.5,8.75);
%	(57.5,8.75);(57.5,8.75);(57.5,8.75);(57.5,8.75)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(57.5,8.75);(57.5,8.75);(60,11.25);(60,11.25)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(60,11.25);(60,11.25);(60,25);(60,25)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(57.5,0);(57.5,0);(57.5,8.75);(57.5,8.75)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(47.5,13.75);(47.5,13.75);(50,16.25);(50,16.25)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(47.5,0);(47.5,0);(47.5,13.75);(47.5,13.75)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(10,16.25);(10,16.25);(10,25);(10,25)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(50,16.25);(50,16.25);(50,25);(50,25)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(10,16.25);(10,16.25);(12.5,13.75);(12.5,13.75)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(12.5,0);(12.5,0);(12.5,13.75);(12.5,13.75)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(2.5,0);(2.5,0);(2.5,8.75);(2.5,8.75)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(0,11.25);(0,11.25);(2.5,8.75);(2.5,8.75)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(0,11.25);(0,11.25);(0,25);(0,25)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(25,21.25);(25,21.25);(30,16.25);(30,16.25)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(25,21.25);(25,21.25);(25,25);(25,25)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(30,8.75);(30,8.75);(35,3.75);(35,3.75)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(35,0);(35,0);(35,3.75);(35,3.75)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(30,8.75);(30,8.75);(30,16.25);(30,16.25)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(30,8.75);(30,8.75);(25,3.75);(25,3.75)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(25,0);(25,0);(25,3.75);(25,3.75)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(35,21.25);(35,21.25);(30,16.25);(30,16.25)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(35,21.25);(35,21.25);(35,25);(35,25)"
%	 />
%<ellipse p3= "(31.57,7.19)"
%	 fill-style= "solid"
%	 p2= "(31.56,10.31)"
%	 p1= "(28.43,10.31)"
%	 closure= "open"
%	 angle-end= "0"
%	 angle-start= "0"
%	 />
%<ellipse p3= "(31.56,14.69)"
%	 fill-style= "solid"
%	 p2= "(31.57,17.81)"
%	 p1= "(28.44,17.81)"
%	 closure= "open"
%	 angle-end= "0"
%	 angle-start= "0"
%	 />
%<ellipse p3= "(121.56,3.44)"
%	 fill-style= "solid"
%	 p2= "(121.56,6.56)"
%	 p1= "(118.44,6.56)"
%	 closure= "open"
%	 angle-end= "0"
%	 angle-start= "0"
%	 />
%<ellipse p3= "(121.57,18.44)"
%	 fill-style= "solid"
%	 p2= "(121.57,21.56)"
%	 p1= "(118.44,21.56)"
%	 closure= "open"
%	 angle-end= "0"
%	 angle-start= "0"
%	 />
%<ellipse p3= "(4.06,7.19)"
%	 fill-style= "solid"
%	 p2= "(4.07,10.31)"
%	 p1= "(0.94,10.31)"
%	 closure= "open"
%	 angle-end= "0"
%	 angle-start= "0"
%	 />
%<ellipse p3= "(11.57,14.69)"
%	 fill-style= "solid"
%	 p2= "(11.56,17.81)"
%	 p1= "(8.43,17.81)"
%	 closure= "open"
%	 angle-end= "0"
%	 angle-start= "0"
%	 />
%<ellipse p3= "(48.44,17.81)"
%	 fill-style= "solid"
%	 p2= "(48.44,14.69)"
%	 p1= "(51.57,14.69)"
%	 closure= "open"
%	 angle-end= "0"
%	 angle-start= "0"
%	 />
%<ellipse p3= "(55.93,10.31)"
%	 fill-style= "solid"
%	 p2= "(55.94,7.19)"
%	 p1= "(59.07,7.19)"
%	 closure= "open"
%	 angle-end= "0"
%	 angle-start= "0"
%	 />
%</jpic>
%%End JPIC-XML
%PSTricks content-type (pstricks.sty package needed)
%Add \usepackage{pstricks} in the preamble of your LaTeX file
%You can rescale the whole picture (to 80% for instance) by using the command \def\JPicScale{0.8}
\ifx\JPicScale\undefined\def\JPicScale{1}\fi
\psset{unit=\JPicScale mm}
\psset{linewidth=0.3,dotsep=1,hatchwidth=0.3,hatchsep=1.5,shadowsize=1,dimen=middle}
\psset{dotsize=0.7 2.5,dotscale=1 1,fillcolor=black}
\psset{arrowsize=1 2,arrowlength=1,arrowinset=0.25,tbarsize=0.7 5,bracketlength=0.15,rbracketlength=0.15}
\begin{pspicture}(0,0)(132.5,25)
\rput(20,12.5){\EQLS}
\psline(120,0)(120,5)
\psline(120,5)(122.5,7.5)
\psline(120,5)(117.5,7.5)
\psline(132.5,0)(132.5,25)
\rput(127.5,12.5){\EQLS}
\psline(120,20)(120,25)
\psline(117.5,17.5)(120,20)
\psline(122.5,17.5)(120,20)
\psline(117.5,7.5)(117.5,17.5)
\psline(122.5,7.5)(122.5,17.5)
\rput(40,12.5){\EQLS}
\pscustom[]{\psline(2.5,8.75)(10,16.25)
\psbezier(10,16.25)(10,16.25)(10,16.25)
\psbezier(10,16.25)(10,16.25)(10,16.25)
}
\pscustom[]{\psline(50,16.25)(57.5,8.75)
\psbezier(57.5,8.75)(57.5,8.75)(57.5,8.75)
\psbezier(57.5,8.75)(57.5,8.75)(57.5,8.75)
}
\psline(57.5,8.75)(60,11.25)
\psline(60,11.25)(60,25)
\psline(57.5,0)(57.5,8.75)
\psline(47.5,13.75)(50,16.25)
\psline(47.5,0)(47.5,13.75)
\psline(10,16.25)(10,25)
\psline(50,16.25)(50,25)
\psline(10,16.25)(12.5,13.75)
\psline(12.5,0)(12.5,13.75)
\psline(2.5,0)(2.5,8.75)
\psline(0,11.25)(2.5,8.75)
\psline(0,11.25)(0,25)
\psline(25,21.25)(30,16.25)
\psline(25,21.25)(25,25)
\psline(30,8.75)(35,3.75)
\psline(35,0)(35,3.75)
\psline(30,8.75)(30,16.25)
\psline(30,8.75)(25,3.75)
\psline(25,0)(25,3.75)
\psline(35,21.25)(30,16.25)
\psline(35,21.25)(35,25)
\rput{-22.45}(30,8.75){\psellipse[fillstyle=solid](0,0)(1.57,-1.56)}
\rput{22.45}(30,16.25){\psellipse[fillstyle=solid](0,0)(1.57,-1.56)}
\rput{0}(120,5){\psellipse[fillstyle=solid](0,0)(1.56,-1.56)}
\rput{0}(120,20){\psellipse[fillstyle=solid](0,0)(1.57,-1.56)}
\rput{22.45}(2.5,8.75){\psellipse[fillstyle=solid](0,0)(1.57,-1.56)}
\rput{-22.45}(10,16.25){\psellipse[fillstyle=solid](0,0)(1.57,-1.56)}
\rput{0}(50,16.25){\psellipse[fillstyle=solid](0,0)(1.57,-1.56)}
\rput{-22.45}(57.5,8.75){\psellipse[fillstyle=solid](0,0)(1.57,-1.56)}
\end{pspicture}


==> PIC/frob-law-33.tex <==
%%Created by jPicEdt 1.4.1_03: mixed JPIC-XML/LaTeX format
%%Mon Jun 07 13:21:56 GMT-10:00 2021
%%Begin JPIC-XML
%<?xml version="1.0" standalone="yes"?>
%<jpic x-min="0" x-max="107.5" y-min="0" y-max="25" auto-bounding="true">
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(20,12.5)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\EQLS
%</text>
%<multicurve fill-style= "none"
%	 points= "(95,0);(95,0);(95,5);(95,5)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(95,5);(95,5);(97.5,7.5);(97.5,7.5)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(95,5);(95,5);(92.5,7.5);(92.5,7.5)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(107.5,0);(107.5,0);(107.5,25);(107.5,25)"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(102.5,12.5)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\EQLS
%</text>
%<multicurve fill-style= "none"
%	 points= "(95,20);(95,20);(95,25);(95,25)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(92.5,17.5);(92.5,17.5);(95,20);(95,20)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(97.5,17.5);(97.5,17.5);(95,20);(95,20)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(92.5,7.5);(92.5,7.5);(92.5,17.5);(92.5,17.5)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(97.5,7.5);(97.5,7.5);(97.5,17.5);(97.5,17.5)"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(40,12.5)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\EQLS
%</text>
%<multicurve fill-style= "none"
%	 points= "(2.5,8.75);(2.5,8.75);(10,16.25);(10,16.25);(10,16.25);(10,16.25);
%	(10,16.25);(10,16.25);(10,16.25);(10,16.25)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(50,16.25);(50,16.25);(57.5,8.75);(57.5,8.75);(57.5,8.75);(57.5,8.75);
%	(57.5,8.75);(57.5,8.75);(57.5,8.75);(57.5,8.75)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(57.5,8.75);(57.5,8.75);(60,11.25);(60,11.25)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(60,11.25);(60,11.25);(60,25);(60,25)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(57.5,0);(57.5,0);(57.5,8.75);(57.5,8.75)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(47.5,13.75);(47.5,13.75);(50,16.25);(50,16.25)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(47.5,0);(47.5,0);(47.5,13.75);(47.5,13.75)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(10,16.25);(10,16.25);(10,25);(10,25)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(50,16.25);(50,16.25);(50,25);(50,25)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(10,16.25);(10,16.25);(12.5,13.75);(12.5,13.75)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(12.5,0);(12.5,0);(12.5,13.75);(12.5,13.75)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(2.5,0);(2.5,0);(2.5,8.75);(2.5,8.75)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(0,11.25);(0,11.25);(2.5,8.75);(2.5,8.75)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(0,11.25);(0,11.25);(0,25);(0,25)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(25,21.25);(25,21.25);(30,16.25);(30,16.25)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(25,21.25);(25,21.25);(25,25);(25,25)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(30,8.75);(30,8.75);(35,3.75);(35,3.75)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(35,0);(35,0);(35,3.75);(35,3.75)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(30,8.75);(30,8.75);(30,16.25);(30,16.25)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(30,8.75);(30,8.75);(25,3.75);(25,3.75)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(25,0);(25,0);(25,3.75);(25,3.75)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(35,21.25);(35,21.25);(30,16.25);(30,16.25)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(35,21.25);(35,21.25);(35,25);(35,25)"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(95,20)"
%	 stroke-color= "#ff0033"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\DOTT
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(95,5)"
%	 stroke-color= "#ff0033"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\DOTT
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(57.5,8.75)"
%	 stroke-color= "#ff0033"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\DOTT
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(50,16.25)"
%	 stroke-color= "#ff0033"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\DOTT
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(30,16.25)"
%	 stroke-color= "#ff0033"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\DOTT
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(30,8.75)"
%	 stroke-color= "#ff0033"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\DOTT
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(10,16.25)"
%	 stroke-color= "#ff0033"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\DOTT
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(2.5,8.75)"
%	 stroke-color= "#ff0033"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\DOTT
%</text>
%</jpic>
%%End JPIC-XML
%LaTeX-picture environment using emulated lines and arcs
%You can rescale the whole picture (to 80% for instance) by using the command \def\JPicScale{0.8}
\ifx\JPicScale\undefined\def\JPicScale{1}\fi
\unitlength \JPicScale mm
\begin{picture}(107.5,25)(0,0)
\put(20,12.5){\makebox(0,0)[cc]{\EQLS}}

\linethickness{0.3mm}
\put(95,0){\line(0,1){5}}
\linethickness{0.3mm}
\multiput(95,5)(0.12,0.12){21}{\line(1,0){0.12}}
\linethickness{0.3mm}
\multiput(92.5,7.5)(0.12,-0.12){21}{\line(1,0){0.12}}
\linethickness{0.3mm}
\put(107.5,0){\line(0,1){25}}
\put(102.5,12.5){\makebox(0,0)[cc]{\EQLS}}

\linethickness{0.3mm}
\put(95,20){\line(0,1){5}}
\linethickness{0.3mm}
\multiput(92.5,17.5)(0.12,0.12){21}{\line(1,0){0.12}}
\linethickness{0.3mm}
\multiput(95,20)(0.12,-0.12){21}{\line(1,0){0.12}}
\linethickness{0.3mm}
\put(92.5,7.5){\line(0,1){10}}
\linethickness{0.3mm}
\put(97.5,7.5){\line(0,1){10}}
\put(40,12.5){\makebox(0,0)[cc]{\EQLS}}

\linethickness{0.3mm}
\multiput(2.5,8.75)(0.12,0.12){63}{\line(1,0){0.12}}
\linethickness{0.3mm}
\multiput(50,16.25)(0.12,-0.12){63}{\line(1,0){0.12}}
\linethickness{0.3mm}
\multiput(57.5,8.75)(0.12,0.12){21}{\line(1,0){0.12}}
\linethickness{0.3mm}
\put(60,11.25){\line(0,1){13.75}}
\linethickness{0.3mm}
\put(57.5,0){\line(0,1){8.75}}
\linethickness{0.3mm}
\multiput(47.5,13.75)(0.12,0.12){21}{\line(1,0){0.12}}
\linethickness{0.3mm}
\put(47.5,0){\line(0,1){13.75}}
\linethickness{0.3mm}
\put(10,16.25){\line(0,1){8.75}}
\linethickness{0.3mm}
\put(50,16.25){\line(0,1){8.75}}
\linethickness{0.3mm}
\multiput(10,16.25)(0.12,-0.12){21}{\line(1,0){0.12}}
\linethickness{0.3mm}
\put(12.5,0){\line(0,1){13.75}}
\linethickness{0.3mm}
\put(2.5,0){\line(0,1){8.75}}
\linethickness{0.3mm}
\multiput(0,11.25)(0.12,-0.12){21}{\line(1,0){0.12}}
\linethickness{0.3mm}
\put(0,11.25){\line(0,1){13.75}}
\linethickness{0.3mm}
\multiput(25,21.25)(0.12,-0.12){42}{\line(1,0){0.12}}
\linethickness{0.3mm}
\put(25,21.25){\line(0,1){3.75}}
\linethickness{0.3mm}
\multiput(30,8.75)(0.12,-0.12){42}{\line(1,0){0.12}}
\linethickness{0.3mm}
\put(35,0){\line(0,1){3.75}}
\linethickness{0.3mm}
\put(30,8.75){\line(0,1){7.5}}
\linethickness{0.3mm}
\multiput(25,3.75)(0.12,0.12){42}{\line(1,0){0.12}}
\linethickness{0.3mm}
\put(25,0){\line(0,1){3.75}}
\linethickness{0.3mm}
\multiput(30,16.25)(0.12,0.12){42}{\line(1,0){0.12}}
\linethickness{0.3mm}
\put(35,21.25){\line(0,1){3.75}}
\put(95,20){\makebox(0,0)[cc]{\DOTT}}

\put(95,5){\makebox(0,0)[cc]{\DOTT}}

\put(57.5,8.75){\makebox(0,0)[cc]{\DOTT}}

\put(50,16.25){\makebox(0,0)[cc]{\DOTT}}

\put(30,16.25){\makebox(0,0)[cc]{\DOTT}}

\put(30,8.75){\makebox(0,0)[cc]{\DOTT}}

\put(10,16.25){\makebox(0,0)[cc]{\DOTT}}

\put(2.5,8.75){\makebox(0,0)[cc]{\DOTT}}

\end{picture}


==> PIC/frob-law-333.tex <==
%%Created by jPicEdt 1.4.1_03: mixed JPIC-XML/LaTeX format
%%Mon Jun 07 14:42:58 GMT-10:00 2021
%%Begin JPIC-XML
%<?xml version="1.0" standalone="yes"?>
%<jpic x-min="0" x-max="107.5" y-min="0" y-max="25" auto-bounding="true">
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(20,12.5)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\EQLS
%</text>
%<multicurve fill-style= "none"
%	 points= "(95,0);(95,0);(95,5);(95,5)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(95,5);(95,5);(97.5,7.5);(97.5,7.5)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(95,5);(95,5);(92.5,7.5);(92.5,7.5)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(107.5,0);(107.5,0);(107.5,25);(107.5,25)"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(102.5,12.5)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\EQLS
%</text>
%<multicurve fill-style= "none"
%	 points= "(95,20);(95,20);(95,25);(95,25)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(92.5,17.5);(92.5,17.5);(95,20);(95,20)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(97.5,17.5);(97.5,17.5);(95,20);(95,20)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(92.5,7.5);(92.5,7.5);(92.5,17.5);(92.5,17.5)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(97.5,7.5);(97.5,7.5);(97.5,17.5);(97.5,17.5)"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(40,12.5)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\EQLS
%</text>
%<multicurve fill-style= "none"
%	 points= "(2.5,8.75);(2.5,8.75);(10,16.25);(10,16.25);(10,16.25);(10,16.25);
%	(10,16.25);(10,16.25);(10,16.25);(10,16.25)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(50,16.25);(50,16.25);(57.5,8.75);(57.5,8.75);(57.5,8.75);(57.5,8.75);
%	(57.5,8.75);(57.5,8.75);(57.5,8.75);(57.5,8.75)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(57.5,8.75);(57.5,8.75);(60,11.25);(60,11.25)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(60,11.25);(60,11.25);(60,25);(60,25)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(57.5,0);(57.5,0);(57.5,8.75);(57.5,8.75)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(47.5,13.75);(47.5,13.75);(50,16.25);(50,16.25)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(47.5,0);(47.5,0);(47.5,13.75);(47.5,13.75)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(10,16.25);(10,16.25);(10,25);(10,25)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(50,16.25);(50,16.25);(50,25);(50,25)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(10,16.25);(10,16.25);(12.5,13.75);(12.5,13.75)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(12.5,0);(12.5,0);(12.5,13.75);(12.5,13.75)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(2.5,0);(2.5,0);(2.5,8.75);(2.5,8.75)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(0,11.25);(0,11.25);(2.5,8.75);(2.5,8.75)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(0,11.25);(0,11.25);(0,25);(0,25)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(25,21.25);(25,21.25);(30,16.25);(30,16.25)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(25,21.25);(25,21.25);(25,25);(25,25)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(30,8.75);(30,8.75);(35,3.75);(35,3.75)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(35,0);(35,0);(35,3.75);(35,3.75)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(30,8.75);(30,8.75);(30,16.25);(30,16.25)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(30,8.75);(30,8.75);(25,3.75);(25,3.75)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(25,0);(25,0);(25,3.75);(25,3.75)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(35,21.25);(35,21.25);(30,16.25);(30,16.25)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(35,21.25);(35,21.25);(35,25);(35,25)"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(95,20)"
%	 stroke-color= "#ff0033"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\DOTT
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(95,5)"
%	 stroke-color= "#ff0033"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\DOTT
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(57.5,8.75)"
%	 stroke-color= "#ff0033"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\DOTT
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(50,16.25)"
%	 stroke-color= "#ff0033"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\DOTT
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(30,16.25)"
%	 stroke-color= "#ff0033"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\DOTT
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(30,8.75)"
%	 stroke-color= "#ff0033"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\DOTT
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(10,16.25)"
%	 stroke-color= "#ff0033"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\DOTT
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(2.5,8.75)"
%	 stroke-color= "#ff0033"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\DOTT
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(95,8.75)"
%	 stroke-color= "#ff0033"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\cpy$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(95,16.25)"
%	 stroke-color= "#ff0033"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\cpr$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(57.5,12.5)"
%	 stroke-color= "#ff0033"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\cpy$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(30,20)"
%	 stroke-color= "#ff0033"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\cpy$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(2.5,12.5)"
%	 stroke-color= "#ff0033"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\cpy$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(50,12.5)"
%	 stroke-color= "#ff0033"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\cpr$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(30,5)"
%	 stroke-color= "#ff0033"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\cpr$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(10,12.5)"
%	 stroke-color= "#ff0033"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\cpr$
%</text>
%</jpic>
%%End JPIC-XML
%LaTeX-picture environment using emulated lines and arcs
%You can rescale the whole picture (to 80% for instance) by using the command \def\JPicScale{0.8}
\ifx\JPicScale\undefined\def\JPicScale{1}\fi
\unitlength \JPicScale mm
\begin{picture}(107.5,25)(0,0)
\put(20,12.5){\makebox(0,0)[cc]{\EQLS}}

\linethickness{0.3mm}
\put(95,0){\line(0,1){5}}
\linethickness{0.3mm}
\multiput(95,5)(0.12,0.12){21}{\line(1,0){0.12}}
\linethickness{0.3mm}
\multiput(92.5,7.5)(0.12,-0.12){21}{\line(1,0){0.12}}
\linethickness{0.3mm}
\put(107.5,0){\line(0,1){25}}
\put(102.5,12.5){\makebox(0,0)[cc]{\EQLS}}

\linethickness{0.3mm}
\put(95,20){\line(0,1){5}}
\linethickness{0.3mm}
\multiput(92.5,17.5)(0.12,0.12){21}{\line(1,0){0.12}}
\linethickness{0.3mm}
\multiput(95,20)(0.12,-0.12){21}{\line(1,0){0.12}}
\linethickness{0.3mm}
\put(92.5,7.5){\line(0,1){10}}
\linethickness{0.3mm}
\put(97.5,7.5){\line(0,1){10}}
\put(40,12.5){\makebox(0,0)[cc]{\EQLS}}

\linethickness{0.3mm}
\multiput(2.5,8.75)(0.12,0.12){63}{\line(1,0){0.12}}
\linethickness{0.3mm}
\multiput(50,16.25)(0.12,-0.12){63}{\line(1,0){0.12}}
\linethickness{0.3mm}
\multiput(57.5,8.75)(0.12,0.12){21}{\line(1,0){0.12}}
\linethickness{0.3mm}
\put(60,11.25){\line(0,1){13.75}}
\linethickness{0.3mm}
\put(57.5,0){\line(0,1){8.75}}
\linethickness{0.3mm}
\multiput(47.5,13.75)(0.12,0.12){21}{\line(1,0){0.12}}
\linethickness{0.3mm}
\put(47.5,0){\line(0,1){13.75}}
\linethickness{0.3mm}
\put(10,16.25){\line(0,1){8.75}}
\linethickness{0.3mm}
\put(50,16.25){\line(0,1){8.75}}
\linethickness{0.3mm}
\multiput(10,16.25)(0.12,-0.12){21}{\line(1,0){0.12}}
\linethickness{0.3mm}
\put(12.5,0){\line(0,1){13.75}}
\linethickness{0.3mm}
\put(2.5,0){\line(0,1){8.75}}
\linethickness{0.3mm}
\multiput(0,11.25)(0.12,-0.12){21}{\line(1,0){0.12}}
\linethickness{0.3mm}
\put(0,11.25){\line(0,1){13.75}}
\linethickness{0.3mm}
\multiput(25,21.25)(0.12,-0.12){42}{\line(1,0){0.12}}
\linethickness{0.3mm}
\put(25,21.25){\line(0,1){3.75}}
\linethickness{0.3mm}
\multiput(30,8.75)(0.12,-0.12){42}{\line(1,0){0.12}}
\linethickness{0.3mm}
\put(35,0){\line(0,1){3.75}}
\linethickness{0.3mm}
\put(30,8.75){\line(0,1){7.5}}
\linethickness{0.3mm}
\multiput(25,3.75)(0.12,0.12){42}{\line(1,0){0.12}}
\linethickness{0.3mm}
\put(25,0){\line(0,1){3.75}}
\linethickness{0.3mm}
\multiput(30,16.25)(0.12,0.12){42}{\line(1,0){0.12}}
\linethickness{0.3mm}
\put(35,21.25){\line(0,1){3.75}}
\put(95,20){\makebox(0,0)[cc]{\DOTT}}

\put(95,5){\makebox(0,0)[cc]{\DOTT}}

\put(57.5,8.75){\makebox(0,0)[cc]{\DOTT}}

\put(50,16.25){\makebox(0,0)[cc]{\DOTT}}

\put(30,16.25){\makebox(0,0)[cc]{\DOTT}}

\put(30,8.75){\makebox(0,0)[cc]{\DOTT}}

\put(10,16.25){\makebox(0,0)[cc]{\DOTT}}

\put(2.5,8.75){\makebox(0,0)[cc]{\DOTT}}

\put(95,8.75){\makebox(0,0)[cc]{$\cpy$}}

\put(95,16.25){\makebox(0,0)[cc]{$\cpr$}}

\put(57.5,12.5){\makebox(0,0)[cc]{$\cpy$}}

\put(30,20){\makebox(0,0)[cc]{$\cpy$}}

\put(2.5,12.5){\makebox(0,0)[cc]{$\cpy$}}

\put(50,12.5){\makebox(0,0)[cc]{$\cpr$}}

\put(30,5){\makebox(0,0)[cc]{$\cpr$}}

\put(10,12.5){\makebox(0,0)[cc]{$\cpr$}}

\end{picture}


==> PIC/frob-law-4-white.tex <==
%%Created by jPicEdt 1.4.1_03: mixed JPIC-XML/LaTeX format
%%Sat Dec 12 15:58:40 GMT-10:00 2020
%%Begin JPIC-XML
%<?xml version="1.0" standalone="yes"?>
%<jpic x-min="0" x-max="132.5" y-min="1.25" y-max="32.5" auto-bounding="true">
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(20,17.5)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\EQLS
%</text>
%<ellipse p3= "(121.56,8.44)"
%	 fill-style= "solid"
%	 p2= "(121.56,11.56)"
%	 p1= "(118.44,11.56)"
%	 closure= "open"
%	 angle-end= "0"
%	 angle-start= "0"
%	 />
%<multicurve fill-style= "none"
%	 points= "(120,2.5);(120,2.5);(120,10);(120,10)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(120,10);(120,10);(122.5,12.5);(122.5,12.5)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(120,10);(120,10);(117.5,12.5);(117.5,12.5)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(132.5,2.5);(132.5,2.5);(132.5,32.5);(132.5,32.5)"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(127.5,17.5)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\EQLS
%</text>
%<multicurve fill-style= "none"
%	 points= "(120,25);(120,25);(120,32.5);(120,32.5)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(117.5,22.5);(117.5,22.5);(120,25);(120,25)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(122.5,22.5);(122.5,22.5);(120,25);(120,25)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(117.5,12.5);(117.5,12.5);(117.5,22.5);(117.5,22.5)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(122.5,12.5);(122.5,12.5);(122.5,22.5);(122.5,22.5)"
%	 />
%<ellipse p3= "(4.06,12.19)"
%	 fill-style= "solid"
%	 p2= "(4.07,15.31)"
%	 p1= "(0.94,15.31)"
%	 closure= "open"
%	 angle-end= "0"
%	 angle-start= "0"
%	 />
%<multicurve fill-style= "none"
%	 points= "(2.5,13.75);(2.5,13.75);(10,21.25);(10,21.25);(10,21.25);(10,21.25);
%	(10,21.25);(10,21.25);(10,21.25);(10,21.25)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(10,21.25);(10,21.25);(10,32.5);(10,32.5)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(10,21.25);(10,21.25);(12.5,18.75);(12.5,18.75)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(12.5,15);(12.5,15);(12.5,18.75);(12.5,18.75)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(2.5,5);(2.5,5);(2.5,13.75);(2.5,13.75)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(0,16.25);(0,16.25);(2.5,13.75);(2.5,13.75)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(0,16.25);(0,16.25);(0,32.5);(0,32.5)"
%	 />
%<ellipse p3= "(121.57,23.44)"
%	 fill-style= "solid"
%	 p2= "(121.57,26.56)"
%	 fill-color= "#ffffff"
%	 p1= "(118.44,26.56)"
%	 closure= "open"
%	 angle-end= "0"
%	 angle-start= "0"
%	 />
%<ellipse p3= "(11.57,19.69)"
%	 fill-style= "solid"
%	 p2= "(11.56,22.81)"
%	 fill-color= "#ffffff"
%	 p1= "(8.43,22.81)"
%	 closure= "open"
%	 angle-end= "0"
%	 angle-start= "0"
%	 />
%<ellipse p3= "(31.56,22.19)"
%	 fill-style= "solid"
%	 p2= "(31.57,25.31)"
%	 p1= "(28.44,25.31)"
%	 closure= "open"
%	 stroke-overstrike-width= "2"
%	 angle-end= "0"
%	 stroke-overstrike= "true"
%	 angle-start= "0"
%	 />
%<multicurve fill-style= "none"
%	 points= "(25,28.75);(25,28.75);(30,23.75);(30,23.75)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(25,28.75);(25,28.75);(25,32.5);(25,32.5)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(30,11.25);(30,11.25);(35,6.25);(35,6.25)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(35,2.5);(35,2.5);(35,6.25);(35,6.25)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(30,20);(30,20);(30,23.75);(30,23.75)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(30,11.25);(30,11.25);(25,6.25);(25,6.25)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(25,5);(25,5);(25,6.25);(25,6.25)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(35,28.75);(35,28.75);(30,23.75);(30,23.75)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(35,28.75);(35,28.75);(35,32.5);(35,32.5)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(30,11.25);(30,11.25);(30,15);(30,15)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(27.5,22.5);(27.5,22.5);(32.5,17.5);(32.5,17.5)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(32.5,17.5);(32.5,17.5);(32.5,12.5);(32.5,12.5)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(27.5,22.5);(27.5,22.5);(27.5,17.5);(27.5,17.5)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(27.5,17.5);(27.5,17.5);(32.5,12.5);(32.5,12.5)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(10,17.5);(10,17.5);(15,12.5);(15,12.5)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(10,17.5);(10,17.5);(10,12.5);(10,12.5)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(10,12.5);(10,12.5);(15,7.5);(15,7.5)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(12.5,2.5);(12.5,2.5);(12.5,10);(12.5,10)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(15,12.5);(15,12.5);(15,7.5);(15,7.5)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(0,5);(0,5);(5,5);(5,5)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(5,5);(5,5);(2.5,2.5);(2.5,2.5)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(2.5,2.5);(2.5,2.5);(0,5);(0,5)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(22.5,5);(22.5,5);(27.5,5);(27.5,5)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(27.5,5);(27.5,5);(25,2.5);(25,2.5)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(25,2.5);(25,2.5);(22.5,5);(22.5,5)"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(30,17.5)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\Aah$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(12.5,12.5)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\Aah$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(25,1.25)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\aah$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(2.5,1.25)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\aah$
%</text>
%<ellipse p3= "(31.57,9.69)"
%	 fill-style= "solid"
%	 p2= "(31.56,12.81)"
%	 fill-color= "#ffffff"
%	 p1= "(28.43,12.81)"
%	 closure= "open"
%	 angle-end= "0"
%	 angle-start= "0"
%	 />
%</jpic>
%%End JPIC-XML
%PSTricks content-type (pstricks.sty package needed)
%Add \usepackage{pstricks} in the preamble of your LaTeX file
%You can rescale the whole picture (to 80% for instance) by using the command \def\JPicScale{0.8}
\ifx\JPicScale\undefined\def\JPicScale{1}\fi
\psset{unit=\JPicScale mm}
\psset{linewidth=0.3,dotsep=1,hatchwidth=0.3,hatchsep=1.5,shadowsize=1,dimen=middle}
\psset{dotsize=0.7 2.5,dotscale=1 1,fillcolor=black}
\psset{arrowsize=1 2,arrowlength=1,arrowinset=0.25,tbarsize=0.7 5,bracketlength=0.15,rbracketlength=0.15}
\begin{pspicture}(0,0)(132.5,32.5)
\rput(20,17.5){\EQLS}
\rput{-0}(120,10){\psellipse[fillstyle=solid](0,0)(1.57,-1.56)}
\psline(120,2.5)(120,10)
\psline(120,10)(122.5,12.5)
\psline(120,10)(117.5,12.5)
\psline(132.5,2.5)(132.5,32.5)
\rput(127.5,17.5){\EQLS}
\psline(120,25)(120,32.5)
\psline(117.5,22.5)(120,25)
\psline(122.5,22.5)(120,25)
\psline(117.5,12.5)(117.5,22.5)
\psline(122.5,12.5)(122.5,22.5)
\rput{0}(2.5,13.75){\psellipse[fillstyle=solid](0,0)(1.57,-1.56)}
\pscustom[]{\psline(2.5,13.75)(10,21.25)
\psbezier(10,21.25)(10,21.25)(10,21.25)
\psbezier(10,21.25)(10,21.25)(10,21.25)
}
\psline(10,21.25)(10,32.5)
\psline(10,21.25)(12.5,18.75)
\psline(12.5,15)(12.5,18.75)
\psline(2.5,5)(2.5,13.75)
\psline(0,16.25)(2.5,13.75)
\psline(0,16.25)(0,32.5)
\rput{-0}(120.01,25){\psellipse[fillcolor=white,fillstyle=solid](0,0)(1.56,-1.56)}
\rput{0}(10,21.25){\psellipse[fillcolor=white,fillstyle=solid](0,0)(1.57,-1.56)}
\rput{0}(30,23.75){\psellipse[border=2,fillstyle=solid](0,0)(1.57,-1.56)}
\psline(25,28.75)(30,23.75)
\psline(25,28.75)(25,32.5)
\psline(30,11.25)(35,6.25)
\psline(35,2.5)(35,6.25)
\psline(30,20)(30,23.75)
\psline(30,11.25)(25,6.25)
\psline(25,5)(25,6.25)
\psline(35,28.75)(30,23.75)
\psline(35,28.75)(35,32.5)
\psline(30,11.25)(30,15)
\psline(27.5,22.5)(32.5,17.5)
\psline(32.5,17.5)(32.5,12.5)
\psline(27.5,22.5)(27.5,17.5)
\psline(27.5,17.5)(32.5,12.5)
\psline(10,17.5)(15,12.5)
\psline(10,17.5)(10,12.5)
\psline(10,12.5)(15,7.5)
\psline(12.5,2.5)(12.5,10)
\psline(15,12.5)(15,7.5)
\psline(0,5)(5,5)
\psline(5,5)(2.5,2.5)
\psline(2.5,2.5)(0,5)
\psline(22.5,5)(27.5,5)
\psline(27.5,5)(25,2.5)
\psline(25,2.5)(22.5,5)
\rput(30,17.5){$\Aah$}
\rput(12.5,12.5){$\Aah$}
\rput(25,1.25){$\aah$}
\rput(2.5,1.25){$\aah$}
\rput{0}(30,11.25){\psellipse[fillcolor=white,fillstyle=solid](0,0)(1.57,-1.56)}
\end{pspicture}


==> PIC/frob-law-4.tex <==
%%Created by jPicEdt 1.4.1_03: mixed JPIC-XML/LaTeX format
%%Sat Dec 12 12:47:57 GMT-10:00 2020
%%Begin JPIC-XML
%<?xml version="1.0" standalone="yes"?>
%<jpic x-min="0" x-max="137.5" y-min="0" y-max="25" auto-bounding="true">
%<ellipse p3= "(36.57,7.19)"
%	 fill-style= "solid"
%	 p2= "(36.56,10.31)"
%	 p1= "(33.43,10.31)"
%	 closure= "open"
%	 angle-end= "0"
%	 angle-start= "0"
%	 />
%<ellipse p3= "(36.56,14.69)"
%	 fill-style= "solid"
%	 p2= "(36.57,17.81)"
%	 p1= "(33.44,17.81)"
%	 closure= "open"
%	 stroke-overstrike-width= "2"
%	 angle-end= "0"
%	 stroke-overstrike= "true"
%	 angle-start= "0"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(22.5,12.5)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\EQLS
%</text>
%<ellipse p3= "(121.56,3.44)"
%	 fill-style= "solid"
%	 p2= "(121.56,6.56)"
%	 p1= "(118.44,6.56)"
%	 closure= "open"
%	 angle-end= "0"
%	 angle-start= "0"
%	 />
%<multicurve fill-style= "none"
%	 points= "(120,0);(120,0);(120,5);(120,5)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(120,5);(120,5);(122.5,7.5);(122.5,7.5)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(120,5);(120,5);(117.5,7.5);(117.5,7.5)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(137.5,0);(137.5,0);(137.5,25);(137.5,25)"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(130,12.5)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\EQLS
%</text>
%<ellipse p3= "(121.57,18.44)"
%	 fill-style= "solid"
%	 p2= "(121.57,21.56)"
%	 p1= "(118.44,21.56)"
%	 closure= "open"
%	 angle-end= "0"
%	 angle-start= "0"
%	 />
%<multicurve fill-style= "none"
%	 points= "(120,20);(120,20);(120,25);(120,25)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(117.5,17.5);(117.5,17.5);(120,20);(120,20)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(122.5,17.5);(122.5,17.5);(120,20);(120,20)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(117.5,7.5);(117.5,7.5);(117.5,17.5);(117.5,17.5)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(122.5,7.5);(122.5,7.5);(122.5,17.5);(122.5,17.5)"
%	 />
%<ellipse p3= "(4.06,7.19)"
%	 fill-style= "solid"
%	 p2= "(4.07,10.31)"
%	 p1= "(0.94,10.31)"
%	 closure= "open"
%	 angle-end= "0"
%	 angle-start= "0"
%	 />
%<multicurve fill-style= "none"
%	 points= "(2.5,8.75);(2.5,8.75);(10,16.25);(10,16.25);(10,16.25);(10,16.25);
%	(10,16.25);(10,16.25);(10,16.25);(10,16.25)"
%	 />
%<ellipse p3= "(11.57,14.69)"
%	 fill-style= "solid"
%	 p2= "(11.56,17.81)"
%	 p1= "(8.43,17.81)"
%	 closure= "open"
%	 angle-end= "0"
%	 angle-start= "0"
%	 />
%<multicurve fill-style= "none"
%	 points= "(10,16.25);(10,16.25);(10,25);(10,25)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(10,16.25);(10,16.25);(12.5,13.75);(12.5,13.75)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(12.5,0);(12.5,0);(12.5,13.75);(12.5,13.75)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(2.5,0);(2.5,0);(2.5,8.75);(2.5,8.75)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(0,11.25);(0,11.25);(2.5,8.75);(2.5,8.75)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(0,11.25);(0,11.25);(0,25);(0,25)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(30,21.25);(30,21.25);(35,16.25);(35,16.25)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(30,21.25);(30,21.25);(30,25);(30,25)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(35,8.75);(35,8.75);(40,3.75);(40,3.75)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(40,0);(40,0);(40,3.75);(40,3.75)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(35,8.75);(35,8.75);(35,16.25);(35,16.25)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(35,8.75);(35,8.75);(30,3.75);(30,3.75)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(30,0);(30,0);(30,3.75);(30,3.75)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(40,21.25);(40,21.25);(35,16.25);(35,16.25)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(40,21.25);(40,21.25);(40,25);(40,25)"
%	 />
%</jpic>
%%End JPIC-XML
%PSTricks content-type (pstricks.sty package needed)
%Add \usepackage{pstricks} in the preamble of your LaTeX file
%You can rescale the whole picture (to 80% for instance) by using the command \def\JPicScale{0.8}
\ifx\JPicScale\undefined\def\JPicScale{1}\fi
\psset{unit=\JPicScale mm}
\psset{linewidth=0.3,dotsep=1,hatchwidth=0.3,hatchsep=1.5,shadowsize=1,dimen=middle}
\psset{dotsize=0.7 2.5,dotscale=1 1,fillcolor=black}
\psset{arrowsize=1 2,arrowlength=1,arrowinset=0.25,tbarsize=0.7 5,bracketlength=0.15,rbracketlength=0.15}
\begin{pspicture}(0,0)(137.5,25)
\rput{-22.45}(35,8.75){\psellipse[fillstyle=solid](0,0)(1.57,-1.56)}
\rput{22.45}(35,16.25){\psellipse[border=2,fillstyle=solid](0,0)(1.57,-1.56)}
\rput(22.5,12.5){\EQLS}
\rput{0}(120,5){\psellipse[fillstyle=solid](0,0)(1.56,-1.56)}
\psline(120,0)(120,5)
\psline(120,5)(122.5,7.5)
\psline(120,5)(117.5,7.5)
\psline(137.5,0)(137.5,25)
\rput(130,12.5){\EQLS}
\rput{0}(120,20){\psellipse[fillstyle=solid](0,0)(1.57,-1.56)}
\psline(120,20)(120,25)
\psline(117.5,17.5)(120,20)
\psline(122.5,17.5)(120,20)
\psline(117.5,7.5)(117.5,17.5)
\psline(122.5,7.5)(122.5,17.5)
\rput{22.45}(2.5,8.75){\psellipse[fillstyle=solid](0,0)(1.57,-1.56)}
\pscustom[]{\psline(2.5,8.75)(10,16.25)
\psbezier(10,16.25)(10,16.25)(10,16.25)
\psbezier(10,16.25)(10,16.25)(10,16.25)
}
\rput{-22.45}(10,16.25){\psellipse[fillstyle=solid](0,0)(1.57,-1.56)}
\psline(10,16.25)(10,25)
\psline(10,16.25)(12.5,13.75)
\psline(12.5,0)(12.5,13.75)
\psline(2.5,0)(2.5,8.75)
\psline(0,11.25)(2.5,8.75)
\psline(0,11.25)(0,25)
\psline(30,21.25)(35,16.25)
\psline(30,21.25)(30,25)
\psline(35,8.75)(40,3.75)
\psline(40,0)(40,3.75)
\psline(35,8.75)(35,16.25)
\psline(35,8.75)(30,3.75)
\psline(30,0)(30,3.75)
\psline(40,21.25)(35,16.25)
\psline(40,21.25)(40,25)
\end{pspicture}


==> PIC/frob-law-white-strict.tex <==
%%Created by jPicEdt 1.4.1_03: mixed JPIC-XML/LaTeX format
%%Sun Dec 13 15:55:41 GMT-10:00 2020
%%Begin JPIC-XML
%<?xml version="1.0" standalone="yes"?>
%<jpic x-min="2.5" x-max="82.5" y-min="0.93" y-max="46.25" auto-bounding="true">
%<multicurve fill-style= "none"
%	 points= "(75,46.25);(75,46.25);(75,5);(75,5)"
%	 stroke-width= "0.75"
%	 />
%<ellipse p3= "(79.07,0.93)"
%	 fill-style= "none"
%	 p2= "(79.07,9.07)"
%	 p1= "(70.93,9.07)"
%	 closure= "open"
%	 angle-end= "0"
%	 angle-start= "0"
%	 />
%<multicurve fill-style= "none"
%	 points= "(5,15);(5,15);(20,30);(20,30)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(20,30);(20,30);(20,46.25);(20,46.25)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(35,15);(35,15);(20,30);(20,30)"
%	 stroke-width= "0.75"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(22.5,46.25)"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\AAh$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(77.5,46.25)"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\AAh$
%</text>
%<multicurve fill-style= "none"
%	 points= "(35,2.5);(35,2.5);(35,15);(35,15)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(5,2.5);(5,2.5);(5,15);(5,15)"
%	 stroke-width= "0.75"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(2.5,3.75)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\AAh$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(32.5,3.75)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\AAh$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(82.5,3.75)"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\delete$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(27.5,30)"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\ccopy$
%</text>
%<ellipse p3= "(16.21,33.79)"
%	 fill-style= "none"
%	 p2= "(16.21,26.21)"
%	 p1= "(23.79,26.21)"
%	 closure= "open"
%	 angle-end= "0"
%	 angle-start= "0"
%	 />
%</jpic>
%%End JPIC-XML
%LaTeX-picture environment using emulated lines and arcs
%You can rescale the whole picture (to 80% for instance) by using the command \def\JPicScale{0.8}
\ifx\JPicScale\undefined\def\JPicScale{1}\fi
\unitlength \JPicScale mm
\begin{picture}(82.5,46.25)(0,0)
\linethickness{0.75mm}
\put(75,5){\line(0,1){41.25}}
\linethickness{0.3mm}
\put(75,5){\circle{8.14}}

\linethickness{0.75mm}
\multiput(5,15)(0.12,0.12){125}{\line(1,0){0.12}}
\linethickness{0.75mm}
\put(20,30){\line(0,1){16.25}}
\linethickness{0.75mm}
\multiput(20,30)(0.12,-0.12){125}{\line(1,0){0.12}}
\put(22.5,46.25){\makebox(0,0)[cl]{$\AAh$}}

\put(77.5,46.25){\makebox(0,0)[cl]{$\AAh$}}

\linethickness{0.75mm}
\put(35,2.5){\line(0,1){12.5}}
\linethickness{0.75mm}
\put(5,2.5){\line(0,1){12.5}}
\put(2.5,3.75){\makebox(0,0)[cr]{$\AAh$}}

\put(32.5,3.75){\makebox(0,0)[cr]{$\AAh$}}

\put(82.5,3.75){\makebox(0,0)[cl]{$\delete$}}

\put(27.5,30){\makebox(0,0)[cl]{$\ccopy$}}

\linethickness{0.3mm}
\put(20,30){\circle{7.58}}

\end{picture}


==> PIC/frob-law.tex <==
%%Created by jPicEdt 1.4.1_03: mixed JPIC-XML/LaTeX format
%%Fri Dec 11 22:01:57 GMT-10:00 2020
%%Begin JPIC-XML
%<?xml version="1.0" standalone="yes"?>
%<jpic x-min="0" x-max="137.5" y-min="0" y-max="25" auto-bounding="true">
%<multicurve fill-style= "none"
%	 points= "(40,0);(40,0);(40,0);(40,0);(40,0);(40,3.75);
%	(40,3.75);(40,3.75);(35,8.75);(35,8.75)"
%	 />
%<ellipse p3= "(36.57,7.19)"
%	 fill-style= "solid"
%	 p2= "(36.56,10.31)"
%	 p1= "(33.43,10.31)"
%	 closure= "open"
%	 angle-end= "0"
%	 angle-start= "0"
%	 />
%<multicurve fill-style= "none"
%	 points= "(30,0);(30,0);(30,3.75);(30,3.75);(30,3.75);(30,3.75);
%	(30,3.75);(30,3.75);(33.75,7.5);(33.75,7.5)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(35,10);(35,10);(35,13.75);(35,13.75);(35,13.75);(35,16.25);
%	(35,16.25);(35,16.25);(35,13.75);(35,13.75)"
%	 />
%<ellipse p3= "(36.56,14.69)"
%	 fill-style= "solid"
%	 p2= "(36.57,17.81)"
%	 p1= "(33.44,17.81)"
%	 closure= "open"
%	 angle-end= "0"
%	 angle-start= "0"
%	 />
%<multicurve fill-style= "none"
%	 points= "(35,16.25);(35,16.25);(30,21.25);(30,21.25);(30,21.25);(30,25);
%	(30,25);(30,25);(30,25);(30,25)"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(22.5,12.5)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\EQLS
%</text>
%<ellipse p3= "(121.56,3.44)"
%	 fill-style= "solid"
%	 p2= "(121.56,6.56)"
%	 p1= "(118.44,6.56)"
%	 closure= "open"
%	 angle-end= "0"
%	 angle-start= "0"
%	 />
%<multicurve fill-style= "none"
%	 points= "(120,0);(120,0);(120,5);(120,5)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(120,5);(120,5);(122.5,7.5);(122.5,7.5)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(120,5);(120,5);(117.5,7.5);(117.5,7.5)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(137.5,0);(137.5,0);(137.5,25);(137.5,25)"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(130,12.5)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\EQLS
%</text>
%<ellipse p3= "(121.57,18.44)"
%	 fill-style= "solid"
%	 p2= "(121.57,21.56)"
%	 p1= "(118.44,21.56)"
%	 closure= "open"
%	 angle-end= "0"
%	 angle-start= "0"
%	 />
%<multicurve fill-style= "none"
%	 points= "(120,20);(120,20);(120,25);(120,25)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(117.5,17.5);(117.5,17.5);(120,20);(120,20)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(122.5,17.5);(122.5,17.5);(120,20);(120,20)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(117.5,7.5);(117.5,7.5);(117.5,17.5);(117.5,17.5)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(122.5,7.5);(122.5,7.5);(122.5,17.5);(122.5,17.5)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(35,16.25);(35,16.25);(40,21.25);(40,21.25);(40,21.25);(40,25);
%	(40,25);(40,25);(40,25);(40,25)"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(47.5,12.5)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\EQLS
%</text>
%<multicurve fill-style= "none"
%	 points= "(2.5,0);(2.5,0);(2.5,6.25);(2.5,6.25);(2.5,6.25);(2.5,8.75);
%	(2.5,8.75);(2.5,8.75);(2.5,6.25);(2.5,6.25)"
%	 />
%<ellipse p3= "(4.06,7.19)"
%	 fill-style= "solid"
%	 p2= "(4.07,10.31)"
%	 p1= "(0.94,10.31)"
%	 closure= "open"
%	 angle-end= "0"
%	 angle-start= "0"
%	 />
%<multicurve fill-style= "none"
%	 points= "(2.5,8.75);(2.5,8.75);(0,11.25);(0,11.25);(0,11.25);(0,25);
%	(0,25);(0,25);(0,18.75);(0,18.75)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(2.5,8.75);(2.5,8.75);(10,16.25);(10,16.25);(10,16.25);(10,16.25);
%	(10,16.25);(10,16.25);(10,16.25);(10,16.25)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(12.5,0);(12.5,0);(12.5,6.25);(12.5,6.25);(12.5,6.25);(12.5,13.75);
%	(12.5,13.75);(12.5,13.75);(10,16.25);(10,16.25)"
%	 />
%<ellipse p3= "(11.57,14.69)"
%	 fill-style= "solid"
%	 p2= "(11.56,17.81)"
%	 p1= "(8.43,17.81)"
%	 closure= "open"
%	 angle-end= "0"
%	 angle-start= "0"
%	 />
%<multicurve fill-style= "none"
%	 points= "(10,17.5);(10,17.5);(10,21.25);(10,21.25);(10,21.25);(10,25);
%	(10,25);(10,25);(10,21.25);(10,21.25)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(60,25);(60,25);(60,20);(60,20);(60,20);(60,17.5);
%	(60,17.5);(60,17.5);(60,20);(60,20)"
%	 />
%<ellipse p3= "(58.44,19.06)"
%	 fill-style= "solid"
%	 p2= "(58.44,15.94)"
%	 p1= "(61.57,15.94)"
%	 closure= "open"
%	 angle-end= "0"
%	 angle-start= "0"
%	 />
%<multicurve fill-style= "none"
%	 points= "(60,17.5);(60,17.5);(57.5,15);(57.5,15);(57.5,15);(57.5,0);
%	(57.5,0);(57.5,0);(57.5,7.5);(57.5,7.5)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(60,17.5);(60,17.5);(67.5,10);(67.5,10);(67.5,10);(67.5,10);
%	(67.5,10);(67.5,10);(67.5,10);(67.5,10)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(70,25);(70,25);(70,20);(70,20);(70,20);(70,12.5);
%	(70,12.5);(70,12.5);(67.5,10);(67.5,10)"
%	 />
%<ellipse p3= "(65.93,11.56)"
%	 fill-style= "solid"
%	 p2= "(65.94,8.44)"
%	 p1= "(69.07,8.44)"
%	 closure= "open"
%	 angle-end= "0"
%	 angle-start= "0"
%	 />
%<multicurve fill-style= "none"
%	 points= "(67.5,8.75);(67.5,8.75);(67.5,5);(67.5,5);(67.5,5);(67.5,0);
%	(67.5,0);(67.5,0);(67.5,5);(67.5,5)"
%	 />
%</jpic>
%%End JPIC-XML
%PSTricks content-type (pstricks.sty package needed)
%Add \usepackage{pstricks} in the preamble of your LaTeX file
%You can rescale the whole picture (to 80% for instance) by using the command \def\JPicScale{0.8}
\ifx\JPicScale\undefined\def\JPicScale{1}\fi
\psset{unit=\JPicScale mm}
\psset{linewidth=0.3,dotsep=1,hatchwidth=0.3,hatchsep=1.5,shadowsize=1,dimen=middle}
\psset{dotsize=0.7 2.5,dotscale=1 1,fillcolor=black}
\psset{arrowsize=1 2,arrowlength=1,arrowinset=0.25,tbarsize=0.7 5,bracketlength=0.15,rbracketlength=0.15}
\begin{pspicture}(0,0)(137.5,25)
\pscustom[]{\psbezier(40,0)(40,0)(40,0)(40,0)
\psline(40,0)(40,3.75)
\psline(40,3.75)(35,8.75)
}
\rput{0}(35,8.75){\psellipse[fillstyle=solid](0,0)(1.57,-1.56)}
\psline(30,0)
(30,3.75)
(30,3.75)(33.75,7.5)
\psline(35,10)
(35,13.75)
(35,16.25)(35,13.75)
\rput{0}(35,16.25){\psellipse[fillstyle=solid](0,0)(1.57,-1.56)}
\pscustom[]{\psline(35,16.25)(30,21.25)
\psline(30,21.25)(30,25)
\psbezier(30,25)(30,25)(30,25)
}
\rput(22.5,12.5){\EQLS}
\rput{-0}(120,5){\psellipse[fillstyle=solid](0,0)(1.57,-1.56)}
\psline(120,0)(120,5)
\psline(120,5)(122.5,7.5)
\psline(120,5)(117.5,7.5)
\psline(137.5,0)(137.5,25)
\rput(130,12.5){\EQLS}
\rput{-0}(120.01,20){\psellipse[fillstyle=solid](0,0)(1.56,-1.56)}
\psline(120,20)(120,25)
\psline(117.5,17.5)(120,20)
\psline(122.5,17.5)(120,20)
\psline(117.5,7.5)(117.5,17.5)
\psline(122.5,7.5)(122.5,17.5)
\pscustom[]{\psline(35,16.25)(40,21.25)
\psline(40,21.25)(40,25)
\psbezier(40,25)(40,25)(40,25)
}
\rput(47.5,12.5){\EQLS}
\psline(2.5,0)
(2.5,6.25)
(2.5,8.75)(2.5,6.25)
\rput{0}(2.5,8.75){\psellipse[fillstyle=solid](0,0)(1.57,-1.56)}
\psline(2.5,8.75)
(0,11.25)
(0,25)(0,18.75)
\pscustom[]{\psline(2.5,8.75)(10,16.25)
\psbezier(10,16.25)(10,16.25)(10,16.25)
\psbezier(10,16.25)(10,16.25)(10,16.25)
}
\psline(12.5,0)
(12.5,6.25)
(12.5,13.75)(10,16.25)
\rput{0}(10,16.25){\psellipse[fillstyle=solid](0,0)(1.57,-1.56)}
\psline(10,17.5)
(10,21.25)
(10,25)(10,21.25)
\psline(60,25)
(60,20)
(60,17.5)(60,20)
\rput{0}(60,17.5){\psellipse[fillstyle=solid](0,0)(1.57,-1.56)}
\psline(60,17.5)
(57.5,15)
(57.5,0)(57.5,7.5)
\pscustom[]{\psline(60,17.5)(67.5,10)
\psbezier(67.5,10)(67.5,10)(67.5,10)
\psbezier(67.5,10)(67.5,10)(67.5,10)
}
\psline(70,25)
(70,20)
(70,12.5)(67.5,10)
\rput{0}(67.5,10){\psellipse[fillstyle=solid](0,0)(1.57,-1.56)}
\psline(67.5,8.75)
(67.5,5)
(67.5,0)(67.5,5)
\end{pspicture}


==> PIC/frob-monoid-1.tex <==
%%Created by jPicEdt 1.4.1_03: mixed JPIC-XML/LaTeX format
%%Fri Dec 11 22:23:20 GMT-10:00 2020
%%Begin JPIC-XML
%<?xml version="1.0" standalone="yes"?>
%<jpic x-min="-0.63" x-max="160" y-min="1.88" y-max="20.62" auto-bounding="true">
%<multicurve fill-style= "none"
%	 points= "(39.38,10.62);(39.38,10.62);(34.38,15.62);(34.38,15.62);(34.38,15.62);(35.62,15.62);
%	(35.62,15.62);(35.62,15.62);(35,15.62);(35,15.62)"
%	 />
%<ellipse p3= "(42.19,7.81)"
%	 fill-style= "solid"
%	 p2= "(42.19,10.94)"
%	 p1= "(39.06,10.94)"
%	 closure= "open"
%	 angle-end= "0"
%	 angle-start= "0"
%	 />
%<ellipse p3= "(36.25,13.75)"
%	 fill-style= "solid"
%	 p2= "(36.25,16.88)"
%	 p1= "(33.12,16.88)"
%	 closure= "open"
%	 angle-end= "0"
%	 angle-start= "0"
%	 />
%<multicurve fill-style= "none"
%	 points= "(30,2.5);(30,2.5);(30,5);(30,5);(30,5);(30,10.63);
%	(30,10.63);(30,10.63);(33.75,14.38);(33.75,14.38)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(35.63,2.5);(35.63,2.5);(35.63,3.13);(35.63,3.13);(35.63,3.13);(35.62,5);
%	(35.62,5);(35.62,5);(39.37,8.75);(39.37,8.75)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(45.63,2.5);(45.63,2.5);(45.63,3.13);(45.63,3.13);(45.63,3.13);(45.62,5);
%	(45.62,5);(45.62,5);(41.87,8.75);(41.87,8.75)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(35,16.88);(35,16.88);(35,20);(35,20);(35,20);(35,20.62);
%	(35,20.62);(35,20.62);(35,20);(35,20)"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(22.5,10)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\EQLS
%</text>
%<ellipse p3= "(5.94,7.81)"
%	 fill-style= "solid"
%	 p2= "(5.94,10.94)"
%	 p1= "(2.81,10.94)"
%	 closure= "open"
%	 angle-end= "0"
%	 angle-start= "0"
%	 />
%<multicurve fill-style= "none"
%	 points= "(-0.62,1.88);(-0.62,1.88);(-0.62,2.5);(-0.62,2.5);(-0.62,2.5);(-0.63,4.38);
%	(-0.63,4.38);(-0.63,4.38);(3.12,8.13);(3.12,8.13)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(9.38,1.88);(9.38,1.88);(9.38,2.5);(9.38,2.5);(9.38,2.5);(9.37,4.38);
%	(9.37,4.38);(9.37,4.38);(5.62,8.13);(5.62,8.13)"
%	 />
%<ellipse p3= "(12.19,14.06)"
%	 fill-style= "solid"
%	 p2= "(12.19,17.19)"
%	 p1= "(9.06,17.19)"
%	 closure= "open"
%	 angle-end= "0"
%	 angle-start= "0"
%	 />
%<multicurve fill-style= "none"
%	 points= "(15.63,2.5);(15.63,2.5);(15.62,8.75);(15.62,8.75);(15.62,8.75);(15.62,10.63);
%	(15.62,10.63);(15.62,10.63);(11.87,14.38);(11.87,14.38)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(5.62,10.62);(5.62,10.62);(10.62,15.62);(10.62,15.62);(10.62,15.62);(10.62,15.62);
%	(10.62,15.62);(10.62,15.62);(10.62,15.62);(10.62,15.62)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(10.62,16.88);(10.62,16.88);(10.62,20);(10.62,20);(10.62,20);(10.62,20.62);
%	(10.62,20.62);(10.62,20.62);(10.62,20);(10.62,20)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(114.38,10);(114.38,10);(109.38,15);(109.38,15);(109.38,15);(110.62,15);
%	(110.62,15);(110.62,15);(110,15);(110,15)"
%	 />
%<ellipse p3= "(117.19,7.19)"
%	 fill-style= "solid"
%	 p2= "(117.19,10.31)"
%	 p1= "(114.06,10.31)"
%	 closure= "open"
%	 angle-end= "0"
%	 angle-start= "0"
%	 />
%<ellipse p3= "(111.25,13.13)"
%	 fill-style= "solid"
%	 p2= "(111.25,16.25)"
%	 p1= "(108.12,16.25)"
%	 closure= "open"
%	 angle-end= "0"
%	 angle-start= "0"
%	 />
%<multicurve fill-style= "none"
%	 points= "(105,1.88);(105,1.88);(105,4.38);(105,4.38);(105,4.38);(105,10);
%	(105,10);(105,10);(108.75,13.75);(108.75,13.75)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(110,16.25);(110,16.25);(110,20);(110,20);(110,20);(110,20.62);
%	(110,20.62);(110,20.62);(110,20);(110,20)"
%	 />
%<ellipse p3= "(65.94,7.19)"
%	 fill-style= "solid"
%	 p2= "(65.94,10.31)"
%	 p1= "(62.81,10.31)"
%	 closure= "open"
%	 angle-end= "0"
%	 angle-start= "0"
%	 />
%<ellipse p3= "(72.19,13.44)"
%	 fill-style= "solid"
%	 p2= "(72.19,16.56)"
%	 p1= "(69.06,16.56)"
%	 closure= "open"
%	 angle-end= "0"
%	 angle-start= "0"
%	 />
%<multicurve fill-style= "none"
%	 points= "(70.62,16.25);(70.62,16.25);(70.62,20);(70.62,20);(70.62,20);(70.62,20.62);
%	(70.62,20.62);(70.62,20.62);(70.62,20);(70.62,20)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(75.63,1.88);(75.63,1.88);(75.62,8.13);(75.62,8.13);(75.62,8.13);(75.62,10);
%	(75.62,10);(75.62,10);(71.87,13.75);(71.87,13.75)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(65.62,10);(65.62,10);(70.62,15);(70.62,15);(70.62,15);(70.62,15);
%	(70.62,15);(70.62,15);(70.62,15);(70.62,15)"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(97.5,10)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\EQLS
%</text>
%<ellipse p3= "(139.07,13.44)"
%	 fill-style= "solid"
%	 p2= "(139.07,16.56)"
%	 p1= "(135.94,16.56)"
%	 closure= "open"
%	 angle-end= "0"
%	 angle-start= "0"
%	 />
%<multicurve fill-style= "none"
%	 points= "(137.5,15);(137.5,15);(137.5,20);(137.5,20)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(135,12.5);(135,12.5);(137.5,15);(137.5,15)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(140,12.5);(140,12.5);(137.5,15);(137.5,15)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(135,10);(135,10);(135,12.5);(135,12.5)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(140,10);(140,10);(140,12.5);(140,12.5)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(140,5);(140,5);(135,10);(135,10)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(140,10);(140,10);(135,5);(135,5)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(135,2.5);(135,2.5);(135,5);(135,5)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(140,2.5);(140,2.5);(140,5);(140,5)"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(147.5,10)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\EQLS
%</text>
%<ellipse p3= "(159.07,13.44)"
%	 fill-style= "solid"
%	 p2= "(159.07,16.56)"
%	 p1= "(155.94,16.56)"
%	 closure= "open"
%	 angle-end= "0"
%	 angle-start= "0"
%	 />
%<multicurve fill-style= "none"
%	 points= "(157.5,15);(157.5,15);(157.5,20);(157.5,20)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(155,12.5);(155,12.5);(157.5,15);(157.5,15)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(160,12.5);(160,12.5);(157.5,15);(157.5,15)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(155,2.5);(155,2.5);(155,12.5);(155,12.5)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(160,2.5);(160,2.5);(160,12.5);(160,12.5)"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(82.5,10)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\EQLS
%</text>
%<multicurve fill-style= "none"
%	 points= "(90,2.5);(90,2.5);(90,19.38);(90,19.38);(90,19.38);(90,20);
%	(90,20);(90,20);(90,19.38);(90,19.38)"
%	 />
%</jpic>
%%End JPIC-XML
%PSTricks content-type (pstricks.sty package needed)
%Add \usepackage{pstricks} in the preamble of your LaTeX file
%You can rescale the whole picture (to 80% for instance) by using the command \def\JPicScale{0.8}
\ifx\JPicScale\undefined\def\JPicScale{1}\fi
\psset{unit=\JPicScale mm}
\psset{linewidth=0.3,dotsep=1,hatchwidth=0.3,hatchsep=1.5,shadowsize=1,dimen=middle}
\psset{dotsize=0.7 2.5,dotscale=1 1,fillcolor=black}
\psset{arrowsize=1 2,arrowlength=1,arrowinset=0.25,tbarsize=0.7 5,bracketlength=0.15,rbracketlength=0.15}
\begin{pspicture}(0,0)(160,20.62)
\psline(39.38,10.62)
(34.38,15.62)
(35.62,15.62)(35,15.62)
\rput{90}(40.62,9.38){\psellipse[fillstyle=solid](0,0)(1.57,-1.56)}
\rput{0}(34.68,15.32){\psellipse[fillstyle=solid](0,0)(1.56,-1.57)}
\psline(30,2.5)
(30,5)
(30,10.63)(33.75,14.38)
\psline(35.63,2.5)
(35.63,3.13)
(35.62,5)(39.37,8.75)
\psline(45.63,2.5)
(45.63,3.13)
(45.62,5)(41.87,8.75)
\psline(35,16.88)
(35,20)
(35,20.62)(35,20)
\rput(22.5,10){\EQLS}
\rput{0}(4.38,9.38){\psellipse[fillstyle=solid](0,0)(1.56,-1.57)}
\psline(-0.62,1.88)
(-0.62,2.5)
(-0.63,4.38)(3.12,8.13)
\psline(9.38,1.88)
(9.38,2.5)
(9.37,4.38)(5.62,8.13)
\rput{0}(10.62,15.62){\psellipse[fillstyle=solid](0,0)(1.57,-1.56)}
\psline(15.63,2.5)
(15.62,8.75)
(15.62,10.63)(11.87,14.38)
\pscustom[]{\psline(5.62,10.62)(10.62,15.62)
\psbezier(10.62,15.62)(10.62,15.62)(10.62,15.62)
\psbezier(10.62,15.62)(10.62,15.62)(10.62,15.62)
}
\psline(10.62,16.88)
(10.62,20)
(10.62,20.62)(10.62,20)
\psline(114.38,10)
(109.38,15)
(110.62,15)(110,15)
\rput{0}(115.62,8.75){\psellipse[fillstyle=solid](0,0)(1.56,-1.56)}
\rput{0}(109.68,14.69){\psellipse[fillstyle=solid](0,0)(1.56,-1.56)}
\psline(105,1.88)
(105,4.38)
(105,10)(108.75,13.75)
\psline(110,16.25)
(110,20)
(110,20.62)(110,20)
\rput{0}(64.38,8.75){\psellipse[fillstyle=solid](0,0)(1.56,-1.56)}
\rput{0}(70.62,15){\psellipse[fillstyle=solid](0,0)(1.56,-1.56)}
\psline(70.62,16.25)
(70.62,20)
(70.62,20.62)(70.62,20)
\psline(75.63,1.88)
(75.62,8.13)
(75.62,10)(71.87,13.75)
\pscustom[]{\psline(65.62,10)(70.62,15)
\psbezier(70.62,15)(70.62,15)(70.62,15)
\psbezier(70.62,15)(70.62,15)(70.62,15)
}
\rput(97.5,10){\EQLS}
\rput{0}(137.5,15){\psellipse[fillstyle=solid](0,0)(1.56,-1.56)}
\psline(137.5,15)(137.5,20)
\psline(135,12.5)(137.5,15)
\psline(140,12.5)(137.5,15)
\psline(135,10)(135,12.5)
\psline(140,10)(140,12.5)
\psline(140,5)(135,10)
\psline(140,10)(135,5)
\psline(135,2.5)(135,5)
\psline(140,2.5)(140,5)
\rput(147.5,10){\EQLS}
\rput{0}(157.5,15){\psellipse[fillstyle=solid](0,0)(1.56,-1.56)}
\psline(157.5,15)(157.5,20)
\psline(155,12.5)(157.5,15)
\psline(160,12.5)(157.5,15)
\psline(155,2.5)(155,12.5)
\psline(160,2.5)(160,12.5)
\rput(82.5,10){\EQLS}
\psline(90,2.5)
(90,19.38)
(90,20)(90,19.38)
\end{pspicture}


==> PIC/frob-monoid-white-strict.tex <==
%%Created by jPicEdt 1.4.1_03: mixed JPIC-XML/LaTeX format
%%Thu Dec 17 11:45:44 GMT-10:00 2020
%%Begin JPIC-XML
%<?xml version="1.0" standalone="yes"?>
%<jpic x-min="0" x-max="198.75" y-min="0" y-max="20" auto-bounding="true">
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(22.5,10)"
%	 text-frame= "noframe"
%	 stroke-width= "0.35"
%	 text-hor-align= "center-h"
%	 >
%\EQLS
%</text>
%<ellipse p3= "(6.56,5.94)"
%	 fill-style= "none"
%	 p2= "(6.56,9.06)"
%	 p1= "(3.44,9.06)"
%	 closure= "open"
%	 angle-end= "0"
%	 stroke-width= "0.35"
%	 angle-start= "0"
%	 />
%<ellipse p3= "(111.56,6.57)"
%	 fill-style= "none"
%	 p2= "(111.56,9.68)"
%	 p1= "(108.44,9.68)"
%	 closure= "open"
%	 angle-end= "0"
%	 stroke-width= "0.35"
%	 angle-start= "0"
%	 />
%<ellipse p3= "(106.56,11.56)"
%	 fill-style= "none"
%	 p2= "(106.56,14.68)"
%	 p1= "(103.44,14.68)"
%	 closure= "open"
%	 angle-end= "0"
%	 stroke-width= "0.35"
%	 angle-start= "0"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(95,10)"
%	 text-frame= "noframe"
%	 stroke-width= "0.35"
%	 text-hor-align= "center-h"
%	 >
%\EQLS
%</text>
%<multicurve fill-style= "none"
%	 points= "(140,13.75);(140,13.75);(140,20);(140,20)"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(137.5,11.25);(137.5,11.25);(140,13.75);(140,13.75)"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(142.5,11.25);(142.5,11.25);(140,13.75);(140,13.75)"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(137.5,8.75);(137.5,8.75);(137.5,11.25);(137.5,11.25)"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(142.5,8.75);(142.5,8.75);(142.5,11.25);(142.5,11.25)"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(142.5,3.75);(142.5,3.75);(137.5,8.75);(137.5,8.75)"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(142.5,8.75);(142.5,8.75);(137.5,3.75);(137.5,3.75)"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(137.5,0);(137.5,0);(137.5,3.75);(137.5,3.75)"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(142.5,0);(142.5,0);(142.5,3.75);(142.5,3.75)"
%	 stroke-width= "0.35"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(147.5,10)"
%	 text-frame= "noframe"
%	 stroke-width= "0.35"
%	 text-hor-align= "center-h"
%	 >
%\EQLS
%</text>
%<multicurve fill-style= "none"
%	 points= "(155,13.75);(155,13.75);(155,20);(155,20)"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(152.5,11.25);(152.5,11.25);(155,13.75);(155,13.75)"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(157.5,11.25);(157.5,11.25);(155,13.75);(155,13.75)"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(152.5,0);(152.5,0);(152.5,11.25);(152.5,11.25)"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(157.5,0);(157.5,0);(157.5,11.25);(157.5,11.25)"
%	 stroke-width= "0.35"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(85,10)"
%	 text-frame= "noframe"
%	 stroke-width= "0.35"
%	 text-hor-align= "center-h"
%	 >
%\EQLS
%</text>
%<ellipse p3= "(141.56,12.19)"
%	 fill-style= "none"
%	 p2= "(141.56,15.31)"
%	 p1= "(138.44,15.31)"
%	 closure= "open"
%	 angle-end= "0"
%	 stroke-width= "0.35"
%	 angle-start= "0"
%	 />
%<ellipse p3= "(156.56,12.19)"
%	 fill-style= "none"
%	 p2= "(156.56,15.31)"
%	 p1= "(153.44,15.31)"
%	 closure= "open"
%	 angle-end= "0"
%	 stroke-width= "0.35"
%	 angle-start= "0"
%	 />
%<ellipse p3= "(12.81,12.18)"
%	 fill-style= "none"
%	 p2= "(12.81,15.31)"
%	 p1= "(9.69,15.31)"
%	 closure= "open"
%	 angle-end= "0"
%	 stroke-width= "0.35"
%	 angle-start= "0"
%	 />
%<multicurve fill-style= "none"
%	 points= "(90,20);(90,20);(90,0);(90,0)"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(105,13.12);(105,13.12);(108.75,9.38);(108.75,9.38)"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(105,13.12);(105,13.12);(100,8.12);(100,8.12)"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(100,8.12);(100,8.12);(100,0);(100,0)"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(105,20);(105,20);(105,13.12);(105,13.12)"
%	 stroke-width= "0.35"
%	 />
%<ellipse p3= "(71.56,6.56)"
%	 fill-style= "none"
%	 p2= "(71.56,9.68)"
%	 p1= "(68.44,9.68)"
%	 closure= "open"
%	 angle-end= "0"
%	 stroke-width= "0.35"
%	 angle-start= "0"
%	 />
%<ellipse p3= "(76.56,11.56)"
%	 fill-style= "none"
%	 p2= "(76.56,14.68)"
%	 p1= "(73.44,14.68)"
%	 closure= "open"
%	 angle-end= "0"
%	 stroke-width= "0.35"
%	 angle-start= "0"
%	 />
%<multicurve fill-style= "none"
%	 points= "(75,13.12);(75,13.12);(80,8.12);(80,8.12)"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(75,13.12);(75,13.12);(71.25,9.38);(71.25,9.38)"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(80,8.12);(80,8.12);(80,0);(80,0)"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(75,20);(75,20);(75,13.12);(75,13.12)"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(0,2.5);(0,2.5);(0,0);(0,0)"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(11.25,13.75);(11.25,13.75);(0,2.5);(0,2.5)"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(17.5,7.5);(17.5,7.5);(17.5,0);(17.5,0)"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(17.5,7.5);(17.5,7.5);(11.25,13.75);(11.25,13.75)"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(11.25,20);(11.25,20);(11.25,13.75);(11.25,13.75)"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(10,2.5);(10,2.5);(5,7.5);(5,7.5)"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(10,2.5);(10,2.5);(10,0);(10,0)"
%	 stroke-width= "0.35"
%	 />
%<ellipse p3= "(41.56,5.94)"
%	 fill-style= "none"
%	 p2= "(41.56,9.06)"
%	 p1= "(38.44,9.06)"
%	 closure= "open"
%	 angle-end= "0"
%	 stroke-width= "0.35"
%	 angle-start= "0"
%	 />
%<ellipse p3= "(35.32,12.18)"
%	 fill-style= "none"
%	 p2= "(35.32,15.31)"
%	 p1= "(32.18,15.31)"
%	 closure= "open"
%	 angle-end= "0"
%	 stroke-width= "0.35"
%	 angle-start= "0"
%	 />
%<multicurve fill-style= "none"
%	 points= "(45,2.5);(45,2.5);(45,0);(45,0)"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(33.75,13.75);(33.75,13.75);(45,2.5);(45,2.5)"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(27.5,7.5);(27.5,7.5);(27.5,0);(27.5,0)"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(27.5,7.5);(27.5,7.5);(33.75,13.75);(33.75,13.75)"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(33.75,20);(33.75,20);(33.75,13.75);(33.75,13.75)"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(35,2.5);(35,2.5);(40,7.5);(40,7.5)"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(35,2.5);(35,2.5);(35,0);(35,0)"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(186.25,0);(186.25,0);(186.25,5);(186.25,5)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(186.25,5);(186.25,5);(188.75,7.5);(188.75,7.5)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(186.25,5);(186.25,5);(183.75,7.5);(183.75,7.5)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(198.75,0);(198.75,0);(198.75,20);(198.75,20)"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(193.75,10)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\EQLS
%</text>
%<multicurve fill-style= "none"
%	 points= "(183.75,7.5);(183.75,7.5);(183.75,11.25);(183.75,11.25)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(188.75,7.5);(188.75,7.5);(188.75,11.25);(188.75,11.25)"
%	 />
%<ellipse p3= "(187.81,3.44)"
%	 fill-style= "solid"
%	 p2= "(187.81,6.56)"
%	 p1= "(184.69,6.56)"
%	 closure= "open"
%	 angle-end= "0"
%	 angle-start= "0"
%	 />
%<ellipse p3= "(187.82,12.19)"
%	 fill-style= "solid"
%	 p2= "(187.82,15.31)"
%	 fill-color= "#ffffff"
%	 p1= "(184.69,15.31)"
%	 closure= "open"
%	 angle-end= "0"
%	 angle-start= "0"
%	 />
%<multicurve fill-style= "none"
%	 points= "(186.25,13.75);(186.25,13.75);(186.25,20);(186.25,20)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(183.75,11.25);(183.75,11.25);(186.25,13.75);(186.25,13.75)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(188.75,11.25);(188.75,11.25);(186.25,13.75);(186.25,13.75)"
%	 />
%</jpic>
%%End JPIC-XML
%PSTricks content-type (pstricks.sty package needed)
%Add \usepackage{pstricks} in the preamble of your LaTeX file
%You can rescale the whole picture (to 80% for instance) by using the command \def\JPicScale{0.8}
\ifx\JPicScale\undefined\def\JPicScale{1}\fi
\psset{unit=\JPicScale mm}
\psset{linewidth=0.3,dotsep=1,hatchwidth=0.3,hatchsep=1.5,shadowsize=1,dimen=middle}
\psset{dotsize=0.7 2.5,dotscale=1 1,fillcolor=black}
\psset{arrowsize=1 2,arrowlength=1,arrowinset=0.25,tbarsize=0.7 5,bracketlength=0.15,rbracketlength=0.15}
\begin{pspicture}(0,0)(198.75,20)
\rput(22.5,10){\EQLS}
\rput{0}(5,7.5){\psellipse[linewidth=0.35](0,0)(1.56,-1.56)}
\rput{0}(110,8.12){\psellipse[linewidth=0.35](0,0)(1.56,-1.55)}
\rput{0}(105,13.12){\psellipse[linewidth=0.35](0,0)(1.56,-1.56)}
\rput(95,10){\EQLS}
\psline[linewidth=0.35](140,13.75)(140,20)
\psline[linewidth=0.35](137.5,11.25)(140,13.75)
\psline[linewidth=0.35](142.5,11.25)(140,13.75)
\psline[linewidth=0.35](137.5,8.75)(137.5,11.25)
\psline[linewidth=0.35](142.5,8.75)(142.5,11.25)
\psline[linewidth=0.35](142.5,3.75)(137.5,8.75)
\psline[linewidth=0.35](142.5,8.75)(137.5,3.75)
\psline[linewidth=0.35](137.5,0)(137.5,3.75)
\psline[linewidth=0.35](142.5,0)(142.5,3.75)
\rput(147.5,10){\EQLS}
\psline[linewidth=0.35](155,13.75)(155,20)
\psline[linewidth=0.35](152.5,11.25)(155,13.75)
\psline[linewidth=0.35](157.5,11.25)(155,13.75)
\psline[linewidth=0.35](152.5,0)(152.5,11.25)
\psline[linewidth=0.35](157.5,0)(157.5,11.25)
\rput(85,10){\EQLS}
\rput{0}(140,13.75){\psellipse[linewidth=0.35](0,0)(1.56,-1.56)}
\rput{0}(155,13.75){\psellipse[linewidth=0.35](0,0)(1.56,-1.56)}
\rput{90}(11.25,13.75){\psellipse[linewidth=0.35](0,0)(1.56,-1.56)}
\psline[linewidth=0.35](90,20)(90,0)
\psline[linewidth=0.35](105,13.12)(108.75,9.38)
\psline[linewidth=0.35](105,13.12)(100,8.12)
\psline[linewidth=0.35](100,8.12)(100,0)
\psline[linewidth=0.35](105,20)(105,13.12)
\rput{0}(70,8.12){\psellipse[linewidth=0.35](0,0)(1.56,-1.56)}
\rput{0}(75,13.12){\psellipse[linewidth=0.35](0,0)(1.56,-1.56)}
\psline[linewidth=0.35](75,13.12)(80,8.12)
\psline[linewidth=0.35](75,13.12)(71.25,9.38)
\psline[linewidth=0.35](80,8.12)(80,0)
\psline[linewidth=0.35](75,20)(75,13.12)
\psline[linewidth=0.35](0,2.5)(0,0)
\psline[linewidth=0.35](11.25,13.75)(0,2.5)
\psline[linewidth=0.35](17.5,7.5)(17.5,0)
\psline[linewidth=0.35](17.5,7.5)(11.25,13.75)
\psline[linewidth=0.35](11.25,20)(11.25,13.75)
\psline[linewidth=0.35](10,2.5)(5,7.5)
\psline[linewidth=0.35](10,2.5)(10,0)
\rput{0}(40,7.5){\psellipse[linewidth=0.35](0,0)(1.56,-1.56)}
\rput{0}(33.75,13.75){\psellipse[linewidth=0.35](0,0)(1.57,-1.57)}
\psline[linewidth=0.35](45,2.5)(45,0)
\psline[linewidth=0.35](33.75,13.75)(45,2.5)
\psline[linewidth=0.35](27.5,7.5)(27.5,0)
\psline[linewidth=0.35](27.5,7.5)(33.75,13.75)
\psline[linewidth=0.35](33.75,20)(33.75,13.75)
\psline[linewidth=0.35](35,2.5)(40,7.5)
\psline[linewidth=0.35](35,2.5)(35,0)
\psline(186.25,0)(186.25,5)
\psline(186.25,5)(188.75,7.5)
\psline(186.25,5)(183.75,7.5)
\psline(198.75,0)(198.75,20)
\rput(193.75,10){\EQLS}
\psline(183.75,7.5)(183.75,11.25)
\psline(188.75,7.5)(188.75,11.25)
\rput{0}(186.25,5){\psellipse[fillstyle=solid](0,0)(1.56,-1.56)}
\rput{0}(186.26,13.75){\psellipse[fillcolor=white,fillstyle=solid](0,0)(1.57,-1.56)}
\psline(186.25,13.75)(186.25,20)
\psline(183.75,11.25)(186.25,13.75)
\psline(188.75,11.25)(186.25,13.75)
\end{pspicture}


==> PIC/frob-monoid-white.tex <==
%%Created by jPicEdt 1.4.1_03: mixed JPIC-XML/LaTeX format
%%Sat Dec 12 10:03:34 GMT-10:00 2020
%%Begin JPIC-XML
%<?xml version="1.0" standalone="yes"?>
%<jpic x-min="-0.63" x-max="160" y-min="1.88" y-max="20.62" auto-bounding="true">
%<multicurve fill-style= "none"
%	 points= "(39.38,10.62);(39.38,10.62);(34.38,15.62);(34.38,15.62);(34.38,15.62);(35.62,15.62);
%	(35.62,15.62);(35.62,15.62);(35,15.62);(35,15.62)"
%	 />
%<ellipse p3= "(42.19,7.81)"
%	 fill-style= "solid"
%	 p2= "(42.19,10.94)"
%	 fill-color= "#ffffff"
%	 p1= "(39.06,10.94)"
%	 closure= "open"
%	 angle-end= "0"
%	 angle-start= "0"
%	 />
%<ellipse p3= "(36.25,13.75)"
%	 fill-style= "solid"
%	 p2= "(36.25,16.88)"
%	 fill-color= "#ffffff"
%	 p1= "(33.12,16.88)"
%	 closure= "open"
%	 angle-end= "0"
%	 angle-start= "0"
%	 />
%<multicurve fill-style= "none"
%	 points= "(30,2.5);(30,2.5);(30,5);(30,5);(30,5);(30,10.63);
%	(30,10.63);(30,10.63);(33.75,14.38);(33.75,14.38)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(35.63,2.5);(35.63,2.5);(35.63,3.13);(35.63,3.13);(35.63,3.13);(35.62,5);
%	(35.62,5);(35.62,5);(39.37,8.75);(39.37,8.75)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(45.63,2.5);(45.63,2.5);(45.63,3.13);(45.63,3.13);(45.63,3.13);(45.62,5);
%	(45.62,5);(45.62,5);(41.87,8.75);(41.87,8.75)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(35,16.88);(35,16.88);(35,20);(35,20);(35,20);(35,20.62);
%	(35,20.62);(35,20.62);(35,20);(35,20)"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(22.5,10)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\EQLS
%</text>
%<ellipse p3= "(5.94,7.81)"
%	 fill-style= "solid"
%	 p2= "(5.94,10.94)"
%	 fill-color= "#ffffff"
%	 p1= "(2.81,10.94)"
%	 closure= "open"
%	 angle-end= "0"
%	 angle-start= "0"
%	 />
%<multicurve fill-style= "none"
%	 points= "(-0.62,1.88);(-0.62,1.88);(-0.62,2.5);(-0.62,2.5);(-0.62,2.5);(-0.63,4.38);
%	(-0.63,4.38);(-0.63,4.38);(3.12,8.13);(3.12,8.13)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(9.38,1.88);(9.38,1.88);(9.38,2.5);(9.38,2.5);(9.38,2.5);(9.37,4.38);
%	(9.37,4.38);(9.37,4.38);(5.62,8.13);(5.62,8.13)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(15.63,2.5);(15.63,2.5);(15.62,8.75);(15.62,8.75);(15.62,8.75);(15.62,10.63);
%	(15.62,10.63);(15.62,10.63);(10.62,15.62);(10.62,15.62)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(5.62,10.62);(5.62,10.62);(10.62,15.62);(10.62,15.62);(10.62,15.62);(10.62,15.62);
%	(10.62,15.62);(10.62,15.62);(10.62,15.62);(10.62,15.62)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(10.62,15.62);(10.62,15.62);(10.62,20);(10.62,20);(10.62,20);(10.62,20.62);
%	(10.62,20.62);(10.62,20.62);(10.62,20);(10.62,20)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(114.38,10);(114.38,10);(109.38,15);(109.38,15);(109.38,15);(110.62,15);
%	(110.62,15);(110.62,15);(110,15);(110,15)"
%	 />
%<ellipse p3= "(117.19,7.19)"
%	 fill-style= "solid"
%	 p2= "(117.19,10.31)"
%	 fill-color= "#ffffff"
%	 p1= "(114.06,10.31)"
%	 closure= "open"
%	 angle-end= "0"
%	 angle-start= "0"
%	 />
%<ellipse p3= "(111.25,13.13)"
%	 fill-style= "solid"
%	 p2= "(111.25,16.25)"
%	 fill-color= "#ffffff"
%	 p1= "(108.12,16.25)"
%	 closure= "open"
%	 angle-end= "0"
%	 angle-start= "0"
%	 />
%<multicurve fill-style= "none"
%	 points= "(105,1.88);(105,1.88);(105,4.38);(105,4.38);(105,4.38);(105,10);
%	(105,10);(105,10);(108.75,13.75);(108.75,13.75)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(110,16.25);(110,16.25);(110,20);(110,20);(110,20);(110,20.62);
%	(110,20.62);(110,20.62);(110,20);(110,20)"
%	 />
%<ellipse p3= "(65.94,7.19)"
%	 fill-style= "solid"
%	 p2= "(65.94,10.31)"
%	 fill-color= "#ffffff"
%	 p1= "(62.81,10.31)"
%	 closure= "open"
%	 angle-end= "0"
%	 angle-start= "0"
%	 />
%<multicurve fill-style= "none"
%	 points= "(70.62,16.25);(70.62,16.25);(70.62,20);(70.62,20);(70.62,20);(70.62,20.62);
%	(70.62,20.62);(70.62,20.62);(70.62,20);(70.62,20)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(75.63,1.88);(75.63,1.88);(75.62,8.13);(75.62,8.13);(75.62,8.13);(75.62,10);
%	(75.62,10);(75.62,10);(71.87,13.75);(71.87,13.75)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(65.62,10);(65.62,10);(70.62,15);(70.62,15);(70.62,15);(70.62,15);
%	(70.62,15);(70.62,15);(70.62,15);(70.62,15)"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(97.5,10)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\EQLS
%</text>
%<multicurve fill-style= "none"
%	 points= "(137.5,15);(137.5,15);(137.5,20);(137.5,20)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(135,12.5);(135,12.5);(137.5,15);(137.5,15)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(140,12.5);(140,12.5);(137.5,15);(137.5,15)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(135,10);(135,10);(135,12.5);(135,12.5)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(140,10);(140,10);(140,12.5);(140,12.5)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(140,5);(140,5);(135,10);(135,10)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(140,10);(140,10);(135,5);(135,5)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(135,2.5);(135,2.5);(135,5);(135,5)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(140,2.5);(140,2.5);(140,5);(140,5)"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(147.5,10)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\EQLS
%</text>
%<multicurve fill-style= "none"
%	 points= "(157.5,15);(157.5,15);(157.5,20);(157.5,20)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(155,12.5);(155,12.5);(157.5,15);(157.5,15)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(160,12.5);(160,12.5);(157.5,15);(157.5,15)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(155,2.5);(155,2.5);(155,12.5);(155,12.5)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(160,2.5);(160,2.5);(160,12.5);(160,12.5)"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(82.5,10)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\EQLS
%</text>
%<multicurve fill-style= "none"
%	 points= "(90,2.5);(90,2.5);(90,19.38);(90,19.38);(90,19.38);(90,20);
%	(90,20);(90,20);(90,19.38);(90,19.38)"
%	 />
%<ellipse p3= "(139.06,13.44)"
%	 fill-style= "solid"
%	 p2= "(139.06,16.56)"
%	 fill-color= "#ffffff"
%	 p1= "(135.94,16.56)"
%	 closure= "open"
%	 angle-end= "0"
%	 angle-start= "0"
%	 />
%<ellipse p3= "(159.06,13.44)"
%	 fill-style= "solid"
%	 p2= "(159.06,16.56)"
%	 fill-color= "#ffffff"
%	 p1= "(155.94,16.56)"
%	 closure= "open"
%	 angle-end= "0"
%	 angle-start= "0"
%	 />
%<ellipse p3= "(12.19,14.06)"
%	 fill-style= "solid"
%	 p2= "(12.19,17.19)"
%	 fill-color= "#ffffff"
%	 p1= "(9.06,17.19)"
%	 closure= "open"
%	 angle-end= "0"
%	 angle-start= "0"
%	 />
%<ellipse p3= "(72.19,13.44)"
%	 fill-style= "solid"
%	 p2= "(72.19,16.56)"
%	 fill-color= "#ffffff"
%	 p1= "(69.06,16.56)"
%	 closure= "open"
%	 angle-end= "0"
%	 angle-start= "0"
%	 />
%</jpic>
%%End JPIC-XML
%PSTricks content-type (pstricks.sty package needed)
%Add \usepackage{pstricks} in the preamble of your LaTeX file
%You can rescale the whole picture (to 80% for instance) by using the command \def\JPicScale{0.8}
\ifx\JPicScale\undefined\def\JPicScale{1}\fi
\psset{unit=\JPicScale mm}
\psset{linewidth=0.3,dotsep=1,hatchwidth=0.3,hatchsep=1.5,shadowsize=1,dimen=middle}
\psset{dotsize=0.7 2.5,dotscale=1 1,fillcolor=black}
\psset{arrowsize=1 2,arrowlength=1,arrowinset=0.25,tbarsize=0.7 5,bracketlength=0.15,rbracketlength=0.15}
\begin{pspicture}(0,0)(160,20.62)
\psline(39.38,10.62)
(34.38,15.62)
(35.62,15.62)(35,15.62)
\rput{90}(40.62,9.38){\psellipse[fillcolor=white,fillstyle=solid](0,0)(1.57,-1.56)}
\rput{0}(34.68,15.32){\psellipse[fillcolor=white,fillstyle=solid](0,0)(1.56,-1.57)}
\psline(30,2.5)
(30,5)
(30,10.63)(33.75,14.38)
\psline(35.63,2.5)
(35.63,3.13)
(35.62,5)(39.37,8.75)
\psline(45.63,2.5)
(45.63,3.13)
(45.62,5)(41.87,8.75)
\psline(35,16.88)
(35,20)
(35,20.62)(35,20)
\rput(22.5,10){\EQLS}
\rput{0}(4.38,9.38){\psellipse[fillcolor=white,fillstyle=solid](0,0)(1.56,-1.57)}
\psline(-0.62,1.88)
(-0.62,2.5)
(-0.63,4.38)(3.12,8.13)
\psline(9.38,1.88)
(9.38,2.5)
(9.37,4.38)(5.62,8.13)
\psline(15.63,2.5)
(15.62,8.75)
(15.62,10.63)(10.62,15.62)
\pscustom[]{\psline(5.62,10.62)(10.62,15.62)
\psbezier(10.62,15.62)(10.62,15.62)(10.62,15.62)
\psbezier(10.62,15.62)(10.62,15.62)(10.62,15.62)
}
\psline(10.62,15.62)
(10.62,20)
(10.62,20.62)(10.62,20)
\psline(114.38,10)
(109.38,15)
(110.62,15)(110,15)
\rput{0}(115.62,8.75){\psellipse[fillcolor=white,fillstyle=solid](0,0)(1.56,-1.56)}
\rput{0}(109.68,14.69){\psellipse[fillcolor=white,fillstyle=solid](0,0)(1.56,-1.56)}
\psline(105,1.88)
(105,4.38)
(105,10)(108.75,13.75)
\psline(110,16.25)
(110,20)
(110,20.62)(110,20)
\rput{0}(64.38,8.75){\psellipse[fillcolor=white,fillstyle=solid](0,0)(1.56,-1.56)}
\psline(70.62,16.25)
(70.62,20)
(70.62,20.62)(70.62,20)
\psline(75.63,1.88)
(75.62,8.13)
(75.62,10)(71.87,13.75)
\pscustom[]{\psline(65.62,10)(70.62,15)
\psbezier(70.62,15)(70.62,15)(70.62,15)
\psbezier(70.62,15)(70.62,15)(70.62,15)
}
\rput(97.5,10){\EQLS}
\psline(137.5,15)(137.5,20)
\psline(135,12.5)(137.5,15)
\psline(140,12.5)(137.5,15)
\psline(135,10)(135,12.5)
\psline(140,10)(140,12.5)
\psline(140,5)(135,10)
\psline(140,10)(135,5)
\psline(135,2.5)(135,5)
\psline(140,2.5)(140,5)
\rput(147.5,10){\EQLS}
\psline(157.5,15)(157.5,20)
\psline(155,12.5)(157.5,15)
\psline(160,12.5)(157.5,15)
\psline(155,2.5)(155,12.5)
\psline(160,2.5)(160,12.5)
\rput(82.5,10){\EQLS}
\psline(90,2.5)
(90,19.38)
(90,20)(90,19.38)
\rput{0}(137.5,15){\psellipse[fillcolor=white,fillstyle=solid](0,0)(1.56,-1.56)}
\rput{0}(157.5,15){\psellipse[fillcolor=white,fillstyle=solid](0,0)(1.56,-1.56)}
\rput{0}(10.62,15.62){\psellipse[fillcolor=white,fillstyle=solid](0,0)(1.56,-1.56)}
\rput{0}(70.62,15){\psellipse[fillcolor=white,fillstyle=solid](0,0)(1.56,-1.56)}
\end{pspicture}


==> PIC/frob-monoid.tex <==
%%Created by jPicEdt 1.4.1_03: mixed JPIC-XML/LaTeX format
%%Tue Jan 05 06:12:30 GMT-10:00 2021
%%Begin JPIC-XML
%<?xml version="1.0" standalone="yes"?>
%<jpic x-min="-0.63" x-max="160" y-min="1.88" y-max="20.62" auto-bounding="true">
%<multicurve fill-style= "none"
%	 points= "(34.38,10.62);(34.38,10.62);(29.38,15.62);(29.38,15.62);(29.38,15.62);(30.62,15.62);
%	(30.62,15.62);(30.62,15.62);(30,15.62);(30,15.62)"
%	 />
%<ellipse p3= "(31.25,13.75)"
%	 fill-style= "solid"
%	 p2= "(31.25,16.88)"
%	 p1= "(28.12,16.88)"
%	 closure= "open"
%	 angle-end= "0"
%	 angle-start= "0"
%	 />
%<multicurve fill-style= "none"
%	 points= "(25,2.5);(25,2.5);(25,5);(25,5);(25,5);(25,10.63);
%	(25,10.63);(25,10.63);(28.75,14.38);(28.75,14.38)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(30.63,2.5);(30.63,2.5);(30.63,3.13);(30.63,3.13);(30.63,3.13);(30.62,5);
%	(30.62,5);(30.62,5);(34.37,8.75);(34.37,8.75)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(40.63,2.5);(40.63,2.5);(40.63,3.13);(40.63,3.13);(40.63,3.13);(40.62,5);
%	(40.62,5);(40.62,5);(36.87,8.75);(36.87,8.75)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(30,16.88);(30,16.88);(30,20);(30,20);(30,20);(30,20.62);
%	(30,20.62);(30,20.62);(30,20);(30,20)"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(20,10)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\EQLS
%</text>
%<multicurve fill-style= "none"
%	 points= "(-0.62,1.88);(-0.62,1.88);(-0.62,2.5);(-0.62,2.5);(-0.62,2.5);(-0.63,4.38);
%	(-0.63,4.38);(-0.63,4.38);(3.12,8.13);(3.12,8.13)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(9.38,1.88);(9.38,1.88);(9.38,2.5);(9.38,2.5);(9.38,2.5);(9.37,4.38);
%	(9.37,4.38);(9.37,4.38);(5.62,8.13);(5.62,8.13)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(15.63,2.5);(15.63,2.5);(15.62,8.75);(15.62,8.75);(15.62,8.75);(15.62,10.63);
%	(15.62,10.63);(15.62,10.63);(11.87,14.38);(11.87,14.38)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(5.62,10.62);(5.62,10.62);(10.62,15.62);(10.62,15.62);(10.62,15.62);(10.62,15.62);
%	(10.62,15.62);(10.62,15.62);(10.62,15.62);(10.62,15.62)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(10.62,16.88);(10.62,16.88);(10.62,20);(10.62,20);(10.62,20);(10.62,20.62);
%	(10.62,20.62);(10.62,20.62);(10.62,20);(10.62,20)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(109.38,10);(109.38,10);(104.38,15);(104.38,15);(104.38,15);(105.62,15);
%	(105.62,15);(105.62,15);(105,15);(105,15)"
%	 />
%<ellipse p3= "(112.19,7.19)"
%	 fill-style= "solid"
%	 p2= "(112.19,10.31)"
%	 p1= "(109.06,10.31)"
%	 closure= "open"
%	 angle-end= "0"
%	 angle-start= "0"
%	 />
%<multicurve fill-style= "none"
%	 points= "(100,1.88);(100,1.88);(100,4.38);(100,4.38);(100,4.38);(100,10);
%	(100,10);(100,10);(103.75,13.75);(103.75,13.75)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(105,16.25);(105,16.25);(105,20);(105,20);(105,20);(105,20.62);
%	(105,20.62);(105,20.62);(105,20);(105,20)"
%	 />
%<ellipse p3= "(70.94,7.19)"
%	 fill-style= "solid"
%	 p2= "(70.94,10.31)"
%	 p1= "(67.81,10.31)"
%	 closure= "open"
%	 angle-end= "0"
%	 angle-start= "0"
%	 />
%<multicurve fill-style= "none"
%	 points= "(75.62,16.25);(75.62,16.25);(75.62,20);(75.62,20);(75.62,20);(75.62,20.62);
%	(75.62,20.62);(75.62,20.62);(75.62,20);(75.62,20)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(80.63,1.88);(80.63,1.88);(80.62,8.13);(80.62,8.13);(80.62,8.13);(80.62,10);
%	(80.62,10);(80.62,10);(76.87,13.75);(76.87,13.75)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(70.62,10);(70.62,10);(75.62,15);(75.62,15);(75.62,15);(75.62,15);
%	(75.62,15);(75.62,15);(75.62,15);(75.62,15)"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(95,10)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\EQLS
%</text>
%<multicurve fill-style= "none"
%	 points= "(142.5,15);(142.5,15);(142.5,20);(142.5,20)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(140,12.5);(140,12.5);(142.5,15);(142.5,15)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(145,12.5);(145,12.5);(142.5,15);(142.5,15)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(140,10);(140,10);(140,12.5);(140,12.5)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(145,10);(145,10);(145,12.5);(145,12.5)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(145,5);(145,5);(140,10);(140,10)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(145,10);(145,10);(140,5);(140,5)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(140,2.5);(140,2.5);(140,5);(140,5)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(145,2.5);(145,2.5);(145,5);(145,5)"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(150,10)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\EQLS
%</text>
%<multicurve fill-style= "none"
%	 points= "(157.5,15);(157.5,15);(157.5,20);(157.5,20)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(155,12.5);(155,12.5);(157.5,15);(157.5,15)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(160,12.5);(160,12.5);(157.5,15);(157.5,15)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(155,2.5);(155,2.5);(155,12.5);(155,12.5)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(160,2.5);(160,2.5);(160,12.5);(160,12.5)"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(85,10)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\EQLS
%</text>
%<multicurve fill-style= "none"
%	 points= "(90,2.5);(90,2.5);(90,19.38);(90,19.38);(90,19.38);(90,20);
%	(90,20);(90,20);(90,19.38);(90,19.38)"
%	 />
%<ellipse p3= "(37.19,7.81)"
%	 fill-style= "solid"
%	 p2= "(37.19,10.94)"
%	 p1= "(34.06,10.94)"
%	 closure= "open"
%	 angle-end= "0"
%	 angle-start= "0"
%	 />
%<ellipse p3= "(5.94,7.81)"
%	 fill-style= "solid"
%	 p2= "(5.94,10.94)"
%	 p1= "(2.81,10.94)"
%	 closure= "open"
%	 angle-end= "0"
%	 angle-start= "0"
%	 />
%<ellipse p3= "(12.19,14.06)"
%	 fill-style= "solid"
%	 p2= "(12.19,17.19)"
%	 p1= "(9.06,17.19)"
%	 closure= "open"
%	 angle-end= "0"
%	 angle-start= "0"
%	 />
%<ellipse p3= "(106.25,13.13)"
%	 fill-style= "solid"
%	 p2= "(106.25,16.25)"
%	 p1= "(103.12,16.25)"
%	 closure= "open"
%	 angle-end= "0"
%	 angle-start= "0"
%	 />
%<ellipse p3= "(77.19,13.44)"
%	 fill-style= "solid"
%	 p2= "(77.19,16.56)"
%	 p1= "(74.06,16.56)"
%	 closure= "open"
%	 angle-end= "0"
%	 angle-start= "0"
%	 />
%<ellipse p3= "(144.07,13.44)"
%	 fill-style= "solid"
%	 p2= "(144.07,16.56)"
%	 p1= "(140.94,16.56)"
%	 closure= "open"
%	 angle-end= "0"
%	 angle-start= "0"
%	 />
%<ellipse p3= "(159.07,13.44)"
%	 fill-style= "solid"
%	 p2= "(159.07,16.56)"
%	 p1= "(155.94,16.56)"
%	 closure= "open"
%	 angle-end= "0"
%	 angle-start= "0"
%	 />
%</jpic>
%%End JPIC-XML
%PSTricks content-type (pstricks.sty package needed)
%Add \usepackage{pstricks} in the preamble of your LaTeX file
%You can rescale the whole picture (to 80% for instance) by using the command \def\JPicScale{0.8}
\ifx\JPicScale\undefined\def\JPicScale{1}\fi
\psset{unit=\JPicScale mm}
\psset{linewidth=0.3,dotsep=1,hatchwidth=0.3,hatchsep=1.5,shadowsize=1,dimen=middle}
\psset{dotsize=0.7 2.5,dotscale=1 1,fillcolor=black}
\psset{arrowsize=1 2,arrowlength=1,arrowinset=0.25,tbarsize=0.7 5,bracketlength=0.15,rbracketlength=0.15}
\begin{pspicture}(0,0)(160,20.62)
\psline(34.38,10.62)
(29.38,15.62)
(30.62,15.62)(30,15.62)
\rput{0}(29.69,15.32){\psellipse[fillstyle=solid](0,0)(1.56,-1.56)}
\psline(25,2.5)
(25,5)
(25,10.63)(28.75,14.38)
\psline(30.63,2.5)
(30.63,3.13)
(30.62,5)(34.37,8.75)
\psline(40.63,2.5)
(40.63,3.13)
(40.62,5)(36.87,8.75)
\psline(30,16.88)
(30,20)
(30,20.62)(30,20)
\rput(20,10){\EQLS}
\psline(-0.62,1.88)
(-0.62,2.5)
(-0.63,4.38)(3.12,8.13)
\psline(9.38,1.88)
(9.38,2.5)
(9.37,4.38)(5.62,8.13)
\psline(15.63,2.5)
(15.62,8.75)
(15.62,10.63)(11.87,14.38)
\pscustom[]{\psline(5.62,10.62)(10.62,15.62)
\psbezier(10.62,15.62)(10.62,15.62)(10.62,15.62)
\psbezier(10.62,15.62)(10.62,15.62)(10.62,15.62)
}
\psline(10.62,16.88)
(10.62,20)
(10.62,20.62)(10.62,20)
\psline(109.38,10)
(104.38,15)
(105.62,15)(105,15)
\rput{0}(110.62,8.75){\psellipse[fillstyle=solid](0,0)(1.56,-1.56)}
\psline(100,1.88)
(100,4.38)
(100,10)(103.75,13.75)
\psline(105,16.25)
(105,20)
(105,20.62)(105,20)
\rput{0}(69.38,8.75){\psellipse[fillstyle=solid](0,0)(1.56,-1.56)}
\psline(75.62,16.25)
(75.62,20)
(75.62,20.62)(75.62,20)
\psline(80.63,1.88)
(80.62,8.13)
(80.62,10)(76.87,13.75)
\pscustom[]{\psline(70.62,10)(75.62,15)
\psbezier(75.62,15)(75.62,15)(75.62,15)
\psbezier(75.62,15)(75.62,15)(75.62,15)
}
\rput(95,10){\EQLS}
\psline(142.5,15)(142.5,20)
\psline(140,12.5)(142.5,15)
\psline(145,12.5)(142.5,15)
\psline(140,10)(140,12.5)
\psline(145,10)(145,12.5)
\psline(145,5)(140,10)
\psline(145,10)(140,5)
\psline(140,2.5)(140,5)
\psline(145,2.5)(145,5)
\rput(150,10){\EQLS}
\psline(157.5,15)(157.5,20)
\psline(155,12.5)(157.5,15)
\psline(160,12.5)(157.5,15)
\psline(155,2.5)(155,12.5)
\psline(160,2.5)(160,12.5)
\rput(85,10){\EQLS}
\psline(90,2.5)
(90,19.38)
(90,20)(90,19.38)
\rput{90}(35.62,9.38){\psellipse[fillstyle=solid](0,0)(1.57,-1.56)}
\rput{0}(4.38,9.38){\psellipse[fillstyle=solid](0,0)(1.56,-1.57)}
\rput{0}(10.62,15.62){\psellipse[fillstyle=solid](0,0)(1.57,-1.56)}
\rput{0}(104.68,14.69){\psellipse[fillstyle=solid](0,0)(1.56,-1.56)}
\rput{0}(75.62,15){\psellipse[fillstyle=solid](0,0)(1.56,-1.56)}
\rput{0}(142.5,15){\psellipse[fillstyle=solid](0,0)(1.56,-1.56)}
\rput{0}(157.5,15){\psellipse[fillstyle=solid](0,0)(1.56,-1.56)}
\end{pspicture}


==> PIC/frob-semigroup.tex <==
%%Created by jPicEdt 1.4.1_03: mixed JPIC-XML/LaTeX format
%%Mon Dec 14 10:03:23 GMT-10:00 2020
%%Begin JPIC-XML
%<?xml version="1.0" standalone="yes"?>
%<jpic x-min="-0.63" x-max="150" y-min="1.88" y-max="20.62" auto-bounding="true">
%<multicurve fill-style= "none"
%	 points= "(39.38,10.62);(39.38,10.62);(34.38,15.62);(34.38,15.62);(34.38,15.62);(35.62,15.62);
%	(35.62,15.62);(35.62,15.62);(35,15.62);(35,15.62)"
%	 />
%<ellipse p3= "(42.19,7.81)"
%	 fill-style= "solid"
%	 p2= "(42.19,10.94)"
%	 p1= "(39.06,10.94)"
%	 closure= "open"
%	 angle-end= "0"
%	 angle-start= "0"
%	 />
%<ellipse p3= "(36.25,13.75)"
%	 fill-style= "solid"
%	 p2= "(36.25,16.88)"
%	 p1= "(33.12,16.88)"
%	 closure= "open"
%	 angle-end= "0"
%	 angle-start= "0"
%	 />
%<multicurve fill-style= "none"
%	 points= "(30,2.5);(30,2.5);(30,5);(30,5);(30,5);(30,10.63);
%	(30,10.63);(30,10.63);(33.75,14.38);(33.75,14.38)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(35.63,2.5);(35.63,2.5);(35.63,3.13);(35.63,3.13);(35.63,3.13);(35.62,5);
%	(35.62,5);(35.62,5);(39.37,8.75);(39.37,8.75)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(45.63,2.5);(45.63,2.5);(45.63,3.13);(45.63,3.13);(45.63,3.13);(45.62,5);
%	(45.62,5);(45.62,5);(41.87,8.75);(41.87,8.75)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(35,16.88);(35,16.88);(35,20);(35,20);(35,20);(35,20.62);
%	(35,20.62);(35,20.62);(35,20);(35,20)"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(22.5,10)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\EQLS
%</text>
%<ellipse p3= "(5.94,7.81)"
%	 fill-style= "solid"
%	 p2= "(5.94,10.94)"
%	 p1= "(2.81,10.94)"
%	 closure= "open"
%	 angle-end= "0"
%	 angle-start= "0"
%	 />
%<multicurve fill-style= "none"
%	 points= "(-0.62,1.88);(-0.62,1.88);(-0.62,2.5);(-0.62,2.5);(-0.62,2.5);(-0.63,4.38);
%	(-0.63,4.38);(-0.63,4.38);(3.12,8.13);(3.12,8.13)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(9.38,1.88);(9.38,1.88);(9.38,2.5);(9.38,2.5);(9.38,2.5);(9.37,4.38);
%	(9.37,4.38);(9.37,4.38);(5.62,8.13);(5.62,8.13)"
%	 />
%<ellipse p3= "(12.19,14.06)"
%	 fill-style= "solid"
%	 p2= "(12.19,17.19)"
%	 p1= "(9.06,17.19)"
%	 closure= "open"
%	 angle-end= "0"
%	 angle-start= "0"
%	 />
%<multicurve fill-style= "none"
%	 points= "(15.63,2.5);(15.63,2.5);(15.62,8.75);(15.62,8.75);(15.62,8.75);(15.62,10.63);
%	(15.62,10.63);(15.62,10.63);(11.87,14.38);(11.87,14.38)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(5.62,10.62);(5.62,10.62);(10.62,15.62);(10.62,15.62);(10.62,15.62);(10.62,15.62);
%	(10.62,15.62);(10.62,15.62);(10.62,15.62);(10.62,15.62)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(10.62,16.88);(10.62,16.88);(10.62,20);(10.62,20);(10.62,20);(10.62,20.62);
%	(10.62,20.62);(10.62,20.62);(10.62,20);(10.62,20)"
%	 />
%<ellipse p3= "(129.07,13.44)"
%	 fill-style= "solid"
%	 p2= "(129.07,16.56)"
%	 p1= "(125.94,16.56)"
%	 closure= "open"
%	 angle-end= "0"
%	 angle-start= "0"
%	 />
%<multicurve fill-style= "none"
%	 points= "(127.5,15);(127.5,15);(127.5,20);(127.5,20)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(125,12.5);(125,12.5);(127.5,15);(127.5,15)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(130,12.5);(130,12.5);(127.5,15);(127.5,15)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(125,10);(125,10);(125,12.5);(125,12.5)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(130,10);(130,10);(130,12.5);(130,12.5)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(130,5);(130,5);(125,10);(125,10)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(130,10);(130,10);(125,5);(125,5)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(125,2.5);(125,2.5);(125,5);(125,5)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(130,2.5);(130,2.5);(130,5);(130,5)"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(137.5,10)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\EQLS
%</text>
%<ellipse p3= "(149.07,13.44)"
%	 fill-style= "solid"
%	 p2= "(149.07,16.56)"
%	 p1= "(145.94,16.56)"
%	 closure= "open"
%	 angle-end= "0"
%	 angle-start= "0"
%	 />
%<multicurve fill-style= "none"
%	 points= "(147.5,15);(147.5,15);(147.5,20);(147.5,20)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(145,12.5);(145,12.5);(147.5,15);(147.5,15)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(150,12.5);(150,12.5);(147.5,15);(147.5,15)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(145,2.5);(145,2.5);(145,12.5);(145,12.5)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(150,2.5);(150,2.5);(150,12.5);(150,12.5)"
%	 />
%</jpic>
%%End JPIC-XML
%PSTricks content-type (pstricks.sty package needed)
%Add \usepackage{pstricks} in the preamble of your LaTeX file
%You can rescale the whole picture (to 80% for instance) by using the command \def\JPicScale{0.8}
\ifx\JPicScale\undefined\def\JPicScale{1}\fi
\psset{unit=\JPicScale mm}
\psset{linewidth=0.3,dotsep=1,hatchwidth=0.3,hatchsep=1.5,shadowsize=1,dimen=middle}
\psset{dotsize=0.7 2.5,dotscale=1 1,fillcolor=black}
\psset{arrowsize=1 2,arrowlength=1,arrowinset=0.25,tbarsize=0.7 5,bracketlength=0.15,rbracketlength=0.15}
\begin{pspicture}(0,0)(150,20.62)
\psline(39.38,10.62)
(34.38,15.62)
(35.62,15.62)(35,15.62)
\rput{90}(40.62,9.38){\psellipse[fillstyle=solid](0,0)(1.57,-1.56)}
\rput{0}(34.68,15.32){\psellipse[fillstyle=solid](0,0)(1.56,-1.57)}
\psline(30,2.5)
(30,5)
(30,10.63)(33.75,14.38)
\psline(35.63,2.5)
(35.63,3.13)
(35.62,5)(39.37,8.75)
\psline(45.63,2.5)
(45.63,3.13)
(45.62,5)(41.87,8.75)
\psline(35,16.88)
(35,20)
(35,20.62)(35,20)
\rput(22.5,10){\EQLS}
\rput{0}(4.38,9.38){\psellipse[fillstyle=solid](0,0)(1.56,-1.57)}
\psline(-0.62,1.88)
(-0.62,2.5)
(-0.63,4.38)(3.12,8.13)
\psline(9.38,1.88)
(9.38,2.5)
(9.37,4.38)(5.62,8.13)
\rput{0}(10.62,15.62){\psellipse[fillstyle=solid](0,0)(1.57,-1.56)}
\psline(15.63,2.5)
(15.62,8.75)
(15.62,10.63)(11.87,14.38)
\pscustom[]{\psline(5.62,10.62)(10.62,15.62)
\psbezier(10.62,15.62)(10.62,15.62)(10.62,15.62)
\psbezier(10.62,15.62)(10.62,15.62)(10.62,15.62)
}
\psline(10.62,16.88)
(10.62,20)
(10.62,20.62)(10.62,20)
\rput{0}(127.5,15){\psellipse[fillstyle=solid](0,0)(1.56,-1.56)}
\psline(127.5,15)(127.5,20)
\psline(125,12.5)(127.5,15)
\psline(130,12.5)(127.5,15)
\psline(125,10)(125,12.5)
\psline(130,10)(130,12.5)
\psline(130,5)(125,10)
\psline(130,10)(125,5)
\psline(125,2.5)(125,5)
\psline(130,2.5)(130,5)
\rput(137.5,10){\EQLS}
\rput{0}(147.5,15){\psellipse[fillstyle=solid](0,0)(1.56,-1.56)}
\psline(147.5,15)(147.5,20)
\psline(145,12.5)(147.5,15)
\psline(150,12.5)(147.5,15)
\psline(145,2.5)(145,12.5)
\psline(150,2.5)(150,12.5)
\end{pspicture}


==> PIC/frob-semilat-OR.tex <==
%%Created by jPicEdt 1.4.1_03: mixed JPIC-XML/LaTeX format
%%Thu Dec 17 15:01:06 GMT-10:00 2020
%%Begin JPIC-XML
%<?xml version="1.0" standalone="yes"?>
%<jpic x-min="0" x-max="122.5" y-min="0" y-max="32.5" auto-bounding="true">
%<ellipse p3= "(94.06,19.69)"
%	 fill-style= "solid"
%	 p2= "(94.07,22.81)"
%	 p1= "(90.94,22.81)"
%	 closure= "open"
%	 stroke-overstrike-width= "2"
%	 angle-end= "0"
%	 stroke-overstrike= "true"
%	 angle-start= "0"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(20,17.5)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\EQLS
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(102.5,17.5)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\EQLS
%</text>
%<ellipse p3= "(4.06,12.19)"
%	 fill-style= "solid"
%	 p2= "(4.07,15.31)"
%	 p1= "(0.94,15.31)"
%	 closure= "open"
%	 angle-end= "0"
%	 angle-start= "0"
%	 />
%<ellipse p3= "(118.43,15.31)"
%	 fill-style= "solid"
%	 p2= "(118.44,12.19)"
%	 p1= "(121.57,12.19)"
%	 closure= "open"
%	 angle-end= "0"
%	 angle-start= "0"
%	 />
%<multicurve fill-style= "none"
%	 points= "(120,13.75);(120,13.75);(122.5,16.25);(122.5,16.25)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(122.5,16.25);(122.5,16.25);(122.5,30);(122.5,30)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(120,5);(120,5);(120,13.75);(120,13.75)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(110,5);(110,5);(110,18.75);(110,18.75)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(12.5,5);(12.5,5);(12.5,18.75);(12.5,18.75)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(2.5,5);(2.5,5);(2.5,13.75);(2.5,13.75)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(0,16.25);(0,16.25);(2.5,13.75);(2.5,13.75)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(0,16.25);(0,16.25);(0,30);(0,30)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(87.5,26.25);(87.5,26.25);(92.5,21.25);(92.5,21.25)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(87.5,26.25);(87.5,26.25);(87.5,30);(87.5,30)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(97.5,5);(97.5,5);(97.5,8.75);(97.5,8.75)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(87.5,5);(87.5,5);(87.5,8.75);(87.5,8.75)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(97.5,26.25);(97.5,26.25);(92.5,21.25);(92.5,21.25)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(97.5,26.25);(97.5,26.25);(97.5,30);(97.5,30)"
%	 />
%<ellipse p3= "(94.07,12.19)"
%	 fill-style= "solid"
%	 p2= "(94.06,15.31)"
%	 fill-color= "#ffffff"
%	 p1= "(90.93,15.31)"
%	 closure= "open"
%	 angle-end= "0"
%	 angle-start= "0"
%	 />
%<ellipse p3= "(11.57,19.69)"
%	 fill-style= "solid"
%	 p2= "(11.56,22.81)"
%	 fill-color= "#ffffff"
%	 p1= "(8.43,22.81)"
%	 closure= "open"
%	 angle-end= "0"
%	 angle-start= "0"
%	 />
%<ellipse p3= "(110.94,22.81)"
%	 fill-style= "solid"
%	 p2= "(110.94,19.69)"
%	 fill-color= "#ffffff"
%	 p1= "(114.07,19.69)"
%	 closure= "open"
%	 angle-end= "0"
%	 angle-start= "0"
%	 />
%<ellipse p3= "(31.56,19.69)"
%	 fill-style= "solid"
%	 p2= "(31.57,22.81)"
%	 p1= "(28.44,22.81)"
%	 closure= "open"
%	 stroke-overstrike-width= "2"
%	 angle-end= "0"
%	 stroke-overstrike= "true"
%	 angle-start= "0"
%	 />
%<multicurve fill-style= "none"
%	 points= "(25,26.25);(25,26.25);(30,21.25);(30,21.25)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(25,26.25);(25,26.25);(25,30);(25,30)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(35,5);(35,5);(35,8.75);(35,8.75)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(25,5);(25,5);(25,8.75);(25,8.75)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(35,26.25);(35,26.25);(30,21.25);(30,21.25)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(35,26.25);(35,26.25);(35,30);(35,30)"
%	 />
%<ellipse p3= "(31.57,12.19)"
%	 fill-style= "solid"
%	 p2= "(31.56,15.31)"
%	 fill-color= "#ffffff"
%	 p1= "(28.43,15.31)"
%	 closure= "open"
%	 angle-end= "0"
%	 angle-start= "0"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(60,17.5)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\ORR
%</text>
%<multicurve fill-style= "none"
%	 points= "(0,5);(0,5);(5,5);(5,5)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(0,5);(0,5);(2.5,2.5);(2.5,2.5)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(2.5,2.5);(2.5,2.5);(5,5);(5,5)"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(2.5,0)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\xee$
%</text>
%<multicurve fill-style= "none"
%	 points= "(22.5,5);(22.5,5);(27.5,5);(27.5,5)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(22.5,5);(22.5,5);(25,2.5);(25,2.5)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(25,2.5);(25,2.5);(27.5,5);(27.5,5)"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(25,0)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\xee$
%</text>
%<multicurve fill-style= "none"
%	 points= "(85,5);(85,5);(90,5);(90,5)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(85,5);(85,5);(87.5,2.5);(87.5,2.5)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(87.5,2.5);(87.5,2.5);(90,5);(90,5)"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(87.5,0)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\xee$
%</text>
%<multicurve fill-style= "none"
%	 points= "(107.5,5);(107.5,5);(112.5,5);(112.5,5)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(107.5,5);(107.5,5);(110,2.5);(110,2.5)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(110,2.5);(110,2.5);(112.5,5);(112.5,5)"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(110,0)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\xee$
%</text>
%<multicurve fill-style= "none"
%	 points= "(117.5,5);(117.5,5);(122.5,5);(122.5,5)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(117.5,5);(117.5,5);(120,2.5);(120,2.5)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(120,2.5);(120,2.5);(122.5,5);(122.5,5)"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(120,0)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\yee$
%</text>
%<multicurve fill-style= "none"
%	 points= "(95,5);(95,5);(100,5);(100,5)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(95,5);(95,5);(97.5,2.5);(97.5,2.5)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(97.5,2.5);(97.5,2.5);(100,5);(100,5)"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(97.5,0)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\yee$
%</text>
%<multicurve fill-style= "none"
%	 points= "(32.5,5);(32.5,5);(37.5,5);(37.5,5)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(32.5,5);(32.5,5);(35,2.5);(35,2.5)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(35,2.5);(35,2.5);(37.5,5);(37.5,5)"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(35,0)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\yee$
%</text>
%<multicurve fill-style= "none"
%	 points= "(10,5);(10,5);(15,5);(15,5)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(10,5);(10,5);(12.5,2.5);(12.5,2.5)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(12.5,2.5);(12.5,2.5);(15,5);(15,5)"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(12.5,0)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\yee$
%</text>
%<multicurve fill-style= "none"
%	 points= "(2.5,13.75);(2.5,13.75);(10,21.25);(10,21.25);(10,21.25);(10,21.25);
%	(10,21.25);(10,21.25);(10,21.25);(10,21.25)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(112.5,21.25);(112.5,21.25);(120,13.75);(120,13.75);(120,13.75);(120,13.75);
%	(120,13.75);(120,13.75);(120,13.75);(120,13.75)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(110,18.75);(110,18.75);(112.5,21.25);(112.5,21.25)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(10,21.25);(10,21.25);(10,30);(10,30)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(112.5,21.25);(112.5,21.25);(112.5,30);(112.5,30)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(10,21.25);(10,21.25);(12.5,18.75);(12.5,18.75)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(92.5,13.75);(92.5,13.75);(97.5,8.75);(97.5,8.75)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(92.5,13.75);(92.5,13.75);(92.5,21.25);(92.5,21.25)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(92.5,13.75);(92.5,13.75);(87.5,8.75);(87.5,8.75)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(30,13.75);(30,13.75);(35,8.75);(35,8.75)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(30,13.75);(30,13.75);(30,21.25);(30,21.25)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(30,13.75);(30,13.75);(25,8.75);(25,8.75)"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(0,32.5)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\xee$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(10,32.5)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\xyee$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(25,32.5)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\xyee$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(35,32.5)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\xyee$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(87.5,32.5)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\xyee$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(97.5,32.5)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\xyee$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(112.5,32.5)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\xyee$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(122.5,32.5)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\yee$
%</text>
%</jpic>
%%End JPIC-XML
%PSTricks content-type (pstricks.sty package needed)
%Add \usepackage{pstricks} in the preamble of your LaTeX file
%You can rescale the whole picture (to 80% for instance) by using the command \def\JPicScale{0.8}
\ifx\JPicScale\undefined\def\JPicScale{1}\fi
\psset{unit=\JPicScale mm}
\psset{linewidth=0.3,dotsep=1,hatchwidth=0.3,hatchsep=1.5,shadowsize=1,dimen=middle}
\psset{dotsize=0.7 2.5,dotscale=1 1,fillcolor=black}
\psset{arrowsize=1 2,arrowlength=1,arrowinset=0.25,tbarsize=0.7 5,bracketlength=0.15,rbracketlength=0.15}
\begin{pspicture}(0,0)(122.5,32.5)
\rput{22.45}(92.5,21.25){\psellipse[border=2,fillstyle=solid](0,0)(1.57,-1.56)}
\rput(20,17.5){\EQLS}
\rput(102.5,17.5){\EQLS}
\rput{22.45}(2.5,13.75){\psellipse[fillstyle=solid](0,0)(1.57,-1.56)}
\rput{-22.45}(120,13.75){\psellipse[fillstyle=solid](0,0)(1.57,-1.56)}
\psline(120,13.75)(122.5,16.25)
\psline(122.5,16.25)(122.5,30)
\psline(120,5)(120,13.75)
\psline(110,5)(110,18.75)
\psline(12.5,5)(12.5,18.75)
\psline(2.5,5)(2.5,13.75)
\psline(0,16.25)(2.5,13.75)
\psline(0,16.25)(0,30)
\psline(87.5,26.25)(92.5,21.25)
\psline(87.5,26.25)(87.5,30)
\psline(97.5,5)(97.5,8.75)
\psline(87.5,5)(87.5,8.75)
\psline(97.5,26.25)(92.5,21.25)
\psline(97.5,26.25)(97.5,30)
\rput{-22.45}(92.5,13.75){\psellipse[fillcolor=white,fillstyle=solid](0,0)(1.57,-1.56)}
\rput{-22.45}(10,21.25){\psellipse[fillcolor=white,fillstyle=solid](0,0)(1.57,-1.56)}
\rput{0}(112.5,21.25){\psellipse[fillcolor=white,fillstyle=solid](0,0)(1.56,-1.56)}
\rput{22.45}(30,21.25){\psellipse[border=2,fillstyle=solid](0,0)(1.57,-1.56)}
\psline(25,26.25)(30,21.25)
\psline(25,26.25)(25,30)
\psline(35,5)(35,8.75)
\psline(25,5)(25,8.75)
\psline(35,26.25)(30,21.25)
\psline(35,26.25)(35,30)
\rput{-22.45}(30,13.75){\psellipse[fillcolor=white,fillstyle=solid](0,0)(1.57,-1.56)}
\rput(60,17.5){\ORR}
\psline(0,5)(5,5)
\psline(0,5)(2.5,2.5)
\psline(2.5,2.5)(5,5)
\rput(2.5,0){$\xee$}
\psline(22.5,5)(27.5,5)
\psline(22.5,5)(25,2.5)
\psline(25,2.5)(27.5,5)
\rput(25,0){$\xee$}
\psline(85,5)(90,5)
\psline(85,5)(87.5,2.5)
\psline(87.5,2.5)(90,5)
\rput(87.5,0){$\xee$}
\psline(107.5,5)(112.5,5)
\psline(107.5,5)(110,2.5)
\psline(110,2.5)(112.5,5)
\rput(110,0){$\xee$}
\psline(117.5,5)(122.5,5)
\psline(117.5,5)(120,2.5)
\psline(120,2.5)(122.5,5)
\rput(120,0){$\yee$}
\psline(95,5)(100,5)
\psline(95,5)(97.5,2.5)
\psline(97.5,2.5)(100,5)
\rput(97.5,0){$\yee$}
\psline(32.5,5)(37.5,5)
\psline(32.5,5)(35,2.5)
\psline(35,2.5)(37.5,5)
\rput(35,0){$\yee$}
\psline(10,5)(15,5)
\psline(10,5)(12.5,2.5)
\psline(12.5,2.5)(15,5)
\rput(12.5,0){$\yee$}
\pscustom[]{\psline(2.5,13.75)(10,21.25)
\psbezier(10,21.25)(10,21.25)(10,21.25)
\psbezier(10,21.25)(10,21.25)(10,21.25)
}
\pscustom[]{\psline(112.5,21.25)(120,13.75)
\psbezier(120,13.75)(120,13.75)(120,13.75)
\psbezier(120,13.75)(120,13.75)(120,13.75)
}
\psline(110,18.75)(112.5,21.25)
\psline(10,21.25)(10,30)
\psline(112.5,21.25)(112.5,30)
\psline(10,21.25)(12.5,18.75)
\psline(92.5,13.75)(97.5,8.75)
\psline(92.5,13.75)(92.5,21.25)
\psline(92.5,13.75)(87.5,8.75)
\psline(30,13.75)(35,8.75)
\psline(30,13.75)(30,21.25)
\psline(30,13.75)(25,8.75)
\rput(0,32.5){$\xee$}
\rput(10,32.5){$\xyee$}
\rput(25,32.5){$\xyee$}
\rput(35,32.5){$\xyee$}
\rput(87.5,32.5){$\xyee$}
\rput(97.5,32.5){$\xyee$}
\rput(112.5,32.5){$\xyee$}
\rput(122.5,32.5){$\yee$}
\end{pspicture}


==> PIC/frob-semilat.tex <==
%%Created by jPicEdt 1.4.1_03: mixed JPIC-XML/LaTeX format
%%Tue Jan 05 05:24:00 GMT-10:00 2021
%%Begin JPIC-XML
%<?xml version="1.0" standalone="yes"?>
%<jpic x-min="0" x-max="183.75" y-min="0" y-max="20" auto-bounding="true">
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(22.5,10)"
%	 text-frame= "noframe"
%	 stroke-width= "0.35"
%	 text-hor-align= "center-h"
%	 >
%\EQLS
%</text>
%<ellipse p3= "(6.56,5.94)"
%	 fill-style= "none"
%	 p2= "(6.56,9.06)"
%	 p1= "(3.44,9.06)"
%	 closure= "open"
%	 angle-end= "0"
%	 stroke-width= "0.35"
%	 angle-start= "0"
%	 />
%<ellipse p3= "(106.56,6.57)"
%	 fill-style= "solid"
%	 p2= "(106.56,9.68)"
%	 p1= "(103.44,9.68)"
%	 closure= "open"
%	 angle-end= "0"
%	 stroke-width= "0.35"
%	 angle-start= "0"
%	 />
%<ellipse p3= "(101.56,11.56)"
%	 fill-style= "none"
%	 p2= "(101.56,14.68)"
%	 p1= "(98.44,14.68)"
%	 closure= "open"
%	 angle-end= "0"
%	 stroke-width= "0.35"
%	 angle-start= "0"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(90,10)"
%	 text-frame= "noframe"
%	 stroke-width= "0.35"
%	 text-hor-align= "center-h"
%	 >
%\EQLS
%</text>
%<multicurve fill-style= "none"
%	 points= "(130,13.75);(130,13.75);(130,20);(130,20)"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(127.5,11.25);(127.5,11.25);(130,13.75);(130,13.75)"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(132.5,11.25);(132.5,11.25);(130,13.75);(130,13.75)"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(127.5,8.75);(127.5,8.75);(127.5,11.25);(127.5,11.25)"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(132.5,8.75);(132.5,8.75);(132.5,11.25);(132.5,11.25)"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(132.5,3.75);(132.5,3.75);(127.5,8.75);(127.5,8.75)"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(132.5,8.75);(132.5,8.75);(127.5,3.75);(127.5,3.75)"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(127.5,0);(127.5,0);(127.5,3.75);(127.5,3.75)"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(132.5,0);(132.5,0);(132.5,3.75);(132.5,3.75)"
%	 stroke-width= "0.35"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(137.5,10)"
%	 text-frame= "noframe"
%	 stroke-width= "0.35"
%	 text-hor-align= "center-h"
%	 >
%\EQLS
%</text>
%<multicurve fill-style= "none"
%	 points= "(145,13.75);(145,13.75);(145,20);(145,20)"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(142.5,11.25);(142.5,11.25);(145,13.75);(145,13.75)"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(147.5,11.25);(147.5,11.25);(145,13.75);(145,13.75)"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(142.5,0);(142.5,0);(142.5,11.25);(142.5,11.25)"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(147.5,0);(147.5,0);(147.5,11.25);(147.5,11.25)"
%	 stroke-width= "0.35"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(80,10)"
%	 text-frame= "noframe"
%	 stroke-width= "0.35"
%	 text-hor-align= "center-h"
%	 >
%\EQLS
%</text>
%<ellipse p3= "(131.56,12.19)"
%	 fill-style= "none"
%	 p2= "(131.56,15.31)"
%	 p1= "(128.44,15.31)"
%	 closure= "open"
%	 angle-end= "0"
%	 stroke-width= "0.35"
%	 angle-start= "0"
%	 />
%<ellipse p3= "(146.56,12.19)"
%	 fill-style= "none"
%	 p2= "(146.56,15.31)"
%	 p1= "(143.44,15.31)"
%	 closure= "open"
%	 angle-end= "0"
%	 stroke-width= "0.35"
%	 angle-start= "0"
%	 />
%<ellipse p3= "(12.81,12.18)"
%	 fill-style= "none"
%	 p2= "(12.81,15.31)"
%	 p1= "(9.69,15.31)"
%	 closure= "open"
%	 angle-end= "0"
%	 stroke-width= "0.35"
%	 angle-start= "0"
%	 />
%<multicurve fill-style= "none"
%	 points= "(85,20);(85,20);(85,0);(85,0)"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(100,13.12);(100,13.12);(103.75,9.38);(103.75,9.38)"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(100,13.12);(100,13.12);(95,8.12);(95,8.12)"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(95,8.12);(95,8.12);(95,0);(95,0)"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(100,20);(100,20);(100,13.12);(100,13.12)"
%	 stroke-width= "0.35"
%	 />
%<ellipse p3= "(66.56,6.56)"
%	 fill-style= "solid"
%	 p2= "(66.56,9.68)"
%	 p1= "(63.44,9.68)"
%	 closure= "open"
%	 angle-end= "0"
%	 stroke-width= "0.35"
%	 angle-start= "0"
%	 />
%<ellipse p3= "(71.56,11.56)"
%	 fill-style= "none"
%	 p2= "(71.56,14.68)"
%	 p1= "(68.44,14.68)"
%	 closure= "open"
%	 angle-end= "0"
%	 stroke-width= "0.35"
%	 angle-start= "0"
%	 />
%<multicurve fill-style= "none"
%	 points= "(70,13.12);(70,13.12);(75,8.12);(75,8.12)"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(70,13.12);(70,13.12);(66.25,9.38);(66.25,9.38)"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(75,8.12);(75,8.12);(75,0);(75,0)"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(70,20);(70,20);(70,13.12);(70,13.12)"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(0,2.5);(0,2.5);(0,0);(0,0)"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(11.25,13.75);(11.25,13.75);(0,2.5);(0,2.5)"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(17.5,7.5);(17.5,7.5);(17.5,0);(17.5,0)"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(17.5,7.5);(17.5,7.5);(11.25,13.75);(11.25,13.75)"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(11.25,20);(11.25,20);(11.25,13.75);(11.25,13.75)"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(10,2.5);(10,2.5);(5,7.5);(5,7.5)"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(10,2.5);(10,2.5);(10,0);(10,0)"
%	 stroke-width= "0.35"
%	 />
%<ellipse p3= "(41.56,5.94)"
%	 fill-style= "none"
%	 p2= "(41.56,9.06)"
%	 p1= "(38.44,9.06)"
%	 closure= "open"
%	 angle-end= "0"
%	 stroke-width= "0.35"
%	 angle-start= "0"
%	 />
%<ellipse p3= "(35.32,12.18)"
%	 fill-style= "none"
%	 p2= "(35.32,15.31)"
%	 p1= "(32.18,15.31)"
%	 closure= "open"
%	 angle-end= "0"
%	 stroke-width= "0.35"
%	 angle-start= "0"
%	 />
%<multicurve fill-style= "none"
%	 points= "(45,2.5);(45,2.5);(45,0);(45,0)"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(33.75,13.75);(33.75,13.75);(45,2.5);(45,2.5)"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(27.5,7.5);(27.5,7.5);(27.5,0);(27.5,0)"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(27.5,7.5);(27.5,7.5);(33.75,13.75);(33.75,13.75)"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(33.75,20);(33.75,20);(33.75,13.75);(33.75,13.75)"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(35,2.5);(35,2.5);(40,7.5);(40,7.5)"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(35,2.5);(35,2.5);(35,0);(35,0)"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(171.25,0);(171.25,0);(171.25,5);(171.25,5)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(171.25,5);(171.25,5);(173.75,7.5);(173.75,7.5)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(171.25,5);(171.25,5);(168.75,7.5);(168.75,7.5)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(183.75,0);(183.75,0);(183.75,20);(183.75,20)"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(178.75,10)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\EQLS
%</text>
%<multicurve fill-style= "none"
%	 points= "(168.75,7.5);(168.75,7.5);(168.75,11.25);(168.75,11.25)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(173.75,7.5);(173.75,7.5);(173.75,11.25);(173.75,11.25)"
%	 />
%<ellipse p3= "(172.81,3.44)"
%	 fill-style= "solid"
%	 p2= "(172.81,6.56)"
%	 p1= "(169.69,6.56)"
%	 closure= "open"
%	 angle-end= "0"
%	 angle-start= "0"
%	 />
%<ellipse p3= "(172.82,12.19)"
%	 fill-style= "solid"
%	 p2= "(172.82,15.31)"
%	 fill-color= "#ffffff"
%	 p1= "(169.69,15.31)"
%	 closure= "open"
%	 angle-end= "0"
%	 angle-start= "0"
%	 />
%<multicurve fill-style= "none"
%	 points= "(171.25,13.75);(171.25,13.75);(171.25,20);(171.25,20)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(168.75,11.25);(168.75,11.25);(171.25,13.75);(171.25,13.75)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(173.75,11.25);(173.75,11.25);(171.25,13.75);(171.25,13.75)"
%	 />
%</jpic>
%%End JPIC-XML
%PSTricks content-type (pstricks.sty package needed)
%Add \usepackage{pstricks} in the preamble of your LaTeX file
%You can rescale the whole picture (to 80% for instance) by using the command \def\JPicScale{0.8}
\ifx\JPicScale\undefined\def\JPicScale{1}\fi
\psset{unit=\JPicScale mm}
\psset{linewidth=0.3,dotsep=1,hatchwidth=0.3,hatchsep=1.5,shadowsize=1,dimen=middle}
\psset{dotsize=0.7 2.5,dotscale=1 1,fillcolor=black}
\psset{arrowsize=1 2,arrowlength=1,arrowinset=0.25,tbarsize=0.7 5,bracketlength=0.15,rbracketlength=0.15}
\begin{pspicture}(0,0)(183.75,20)
\rput(22.5,10){\EQLS}
\rput{0}(5,7.5){\psellipse[linewidth=0.35](0,0)(1.56,-1.56)}
\rput{0}(105,8.12){\psellipse[linewidth=0.35,fillstyle=solid](0,0)(1.56,-1.55)}
\rput{0}(100,13.12){\psellipse[linewidth=0.35](0,0)(1.56,-1.56)}
\rput(90,10){\EQLS}
\psline[linewidth=0.35](130,13.75)(130,20)
\psline[linewidth=0.35](127.5,11.25)(130,13.75)
\psline[linewidth=0.35](132.5,11.25)(130,13.75)
\psline[linewidth=0.35](127.5,8.75)(127.5,11.25)
\psline[linewidth=0.35](132.5,8.75)(132.5,11.25)
\psline[linewidth=0.35](132.5,3.75)(127.5,8.75)
\psline[linewidth=0.35](132.5,8.75)(127.5,3.75)
\psline[linewidth=0.35](127.5,0)(127.5,3.75)
\psline[linewidth=0.35](132.5,0)(132.5,3.75)
\rput(137.5,10){\EQLS}
\psline[linewidth=0.35](145,13.75)(145,20)
\psline[linewidth=0.35](142.5,11.25)(145,13.75)
\psline[linewidth=0.35](147.5,11.25)(145,13.75)
\psline[linewidth=0.35](142.5,0)(142.5,11.25)
\psline[linewidth=0.35](147.5,0)(147.5,11.25)
\rput(80,10){\EQLS}
\rput{0}(130,13.75){\psellipse[linewidth=0.35](0,0)(1.56,-1.56)}
\rput{0}(145,13.75){\psellipse[linewidth=0.35](0,0)(1.56,-1.56)}
\rput{90}(11.25,13.75){\psellipse[linewidth=0.35](0,0)(1.56,-1.56)}
\psline[linewidth=0.35](85,20)(85,0)
\psline[linewidth=0.35](100,13.12)(103.75,9.38)
\psline[linewidth=0.35](100,13.12)(95,8.12)
\psline[linewidth=0.35](95,8.12)(95,0)
\psline[linewidth=0.35](100,20)(100,13.12)
\rput{0}(65,8.12){\psellipse[linewidth=0.35,fillstyle=solid](0,0)(1.56,-1.56)}
\rput{0}(70,13.12){\psellipse[linewidth=0.35](0,0)(1.56,-1.56)}
\psline[linewidth=0.35](70,13.12)(75,8.12)
\psline[linewidth=0.35](70,13.12)(66.25,9.38)
\psline[linewidth=0.35](75,8.12)(75,0)
\psline[linewidth=0.35](70,20)(70,13.12)
\psline[linewidth=0.35](0,2.5)(0,0)
\psline[linewidth=0.35](11.25,13.75)(0,2.5)
\psline[linewidth=0.35](17.5,7.5)(17.5,0)
\psline[linewidth=0.35](17.5,7.5)(11.25,13.75)
\psline[linewidth=0.35](11.25,20)(11.25,13.75)
\psline[linewidth=0.35](10,2.5)(5,7.5)
\psline[linewidth=0.35](10,2.5)(10,0)
\rput{0}(40,7.5){\psellipse[linewidth=0.35](0,0)(1.56,-1.56)}
\rput{0}(33.75,13.75){\psellipse[linewidth=0.35](0,0)(1.57,-1.57)}
\psline[linewidth=0.35](45,2.5)(45,0)
\psline[linewidth=0.35](33.75,13.75)(45,2.5)
\psline[linewidth=0.35](27.5,7.5)(27.5,0)
\psline[linewidth=0.35](27.5,7.5)(33.75,13.75)
\psline[linewidth=0.35](33.75,20)(33.75,13.75)
\psline[linewidth=0.35](35,2.5)(40,7.5)
\psline[linewidth=0.35](35,2.5)(35,0)
\psline(171.25,0)(171.25,5)
\psline(171.25,5)(173.75,7.5)
\psline(171.25,5)(168.75,7.5)
\psline(183.75,0)(183.75,20)
\rput(178.75,10){\EQLS}
\psline(168.75,7.5)(168.75,11.25)
\psline(173.75,7.5)(173.75,11.25)
\rput{0}(171.25,5){\psellipse[fillstyle=solid](0,0)(1.56,-1.56)}
\rput{0}(171.26,13.75){\psellipse[fillcolor=white,fillstyle=solid](0,0)(1.57,-1.56)}
\psline(171.25,13.75)(171.25,20)
\psline(168.75,11.25)(171.25,13.75)
\psline(173.75,11.25)(171.25,13.75)
\end{pspicture}


==> PIC/frob.tex <==
%%Created by jPicEdt 1.4.1_03: mixed JPIC-XML/LaTeX format
%%Mon Jun 07 15:06:30 GMT-10:00 2021
%%Begin JPIC-XML
%<?xml version="1.0" standalone="yes"?>
%<jpic x-min="0" x-max="107.5" y-min="0" y-max="25" auto-bounding="true">
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(20,12.5)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\EQLS
%</text>
%<multicurve fill-style= "none"
%	 points= "(92.5,0);(92.5,0);(92.5,5);(92.5,5)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(92.5,5);(92.5,5);(96.25,8.75);(96.25,8.75)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(92.5,5);(92.5,5);(88.75,8.75);(88.75,8.75)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(107.5,0);(107.5,0);(107.5,25);(107.5,25)"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(101.25,12.5)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\EQLS
%</text>
%<multicurve fill-style= "none"
%	 points= "(92.5,20);(92.5,20);(92.5,25);(92.5,25)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(88.75,16.25);(88.75,16.25);(92.5,20);(92.5,20)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(96.25,16.25);(96.25,16.25);(92.5,20);(92.5,20)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(88.75,8.75);(88.75,8.75);(88.75,16.25);(88.75,16.25)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(96.25,8.75);(96.25,8.75);(96.25,16.25);(96.25,16.25)"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(40,12.5)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\EQLS
%</text>
%<multicurve fill-style= "none"
%	 points= "(2.5,8.75);(2.5,8.75);(10,16.25);(10,16.25);(10,16.25);(10,16.25);
%	(10,16.25);(10,16.25);(10,16.25);(10,16.25)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(50,16.25);(50,16.25);(57.5,8.75);(57.5,8.75);(57.5,8.75);(57.5,8.75);
%	(57.5,8.75);(57.5,8.75);(57.5,8.75);(57.5,8.75)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(57.5,8.75);(57.5,8.75);(60,11.25);(60,11.25)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(60,11.25);(60,11.25);(60,25);(60,25)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(57.5,0);(57.5,0);(57.5,8.75);(57.5,8.75)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(47.5,13.75);(47.5,13.75);(50,16.25);(50,16.25)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(47.5,0);(47.5,0);(47.5,13.75);(47.5,13.75)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(10,16.25);(10,16.25);(10,25);(10,25)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(50,16.25);(50,16.25);(50,25);(50,25)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(10,16.25);(10,16.25);(12.5,13.75);(12.5,13.75)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(12.5,0);(12.5,0);(12.5,13.75);(12.5,13.75)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(2.5,0);(2.5,0);(2.5,8.75);(2.5,8.75)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(0,11.25);(0,11.25);(2.5,8.75);(2.5,8.75)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(0,11.25);(0,11.25);(0,25);(0,25)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(25,21.25);(25,21.25);(30,16.25);(30,16.25)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(25,21.25);(25,21.25);(25,25);(25,25)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(30,8.75);(30,8.75);(35,3.75);(35,3.75)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(35,0);(35,0);(35,3.75);(35,3.75)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(30,8.75);(30,8.75);(30,16.25);(30,16.25)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(30,8.75);(30,8.75);(25,3.75);(25,3.75)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(25,0);(25,0);(25,3.75);(25,3.75)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(35,21.25);(35,21.25);(30,16.25);(30,16.25)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(35,21.25);(35,21.25);(35,25);(35,25)"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(92.5,20)"
%	 stroke-color= "#ff0033"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\DOTT
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(92.5,5)"
%	 stroke-color= "#ff0033"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\DOTT
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(57.5,8.75)"
%	 stroke-color= "#ff0033"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\DOTT
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(50,16.25)"
%	 stroke-color= "#ff0033"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\DOTT
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(30,16.25)"
%	 stroke-color= "#ff0033"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\DOTT
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(30,8.75)"
%	 stroke-color= "#ff0033"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\DOTT
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(10,16.25)"
%	 stroke-color= "#ff0033"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\DOTT
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(2.5,8.75)"
%	 stroke-color= "#ff0033"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\DOTT
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(92.5,8.75)"
%	 stroke-color= "#ff0033"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\cpy$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(92.5,16.25)"
%	 stroke-color= "#ff0033"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\cpr$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(57.5,12.5)"
%	 stroke-color= "#ff0033"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\cpy$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(30,20)"
%	 stroke-color= "#ff0033"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\cpy$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(2.5,12.5)"
%	 stroke-color= "#ff0033"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\cpy$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(50,12.5)"
%	 stroke-color= "#ff0033"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\cpr$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(30,5)"
%	 stroke-color= "#ff0033"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\cpr$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(10,12.5)"
%	 stroke-color= "#ff0033"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\cpr$
%</text>
%</jpic>
%%End JPIC-XML
%LaTeX-picture environment using emulated lines and arcs
%You can rescale the whole picture (to 80% for instance) by using the command \def\JPicScale{0.8}
\ifx\JPicScale\undefined\def\JPicScale{1}\fi
\unitlength \JPicScale mm
\begin{picture}(107.5,25)(0,0)
\put(20,12.5){\makebox(0,0)[cc]{\EQLS}}

\linethickness{0.3mm}
\put(92.5,0){\line(0,1){5}}
\linethickness{0.3mm}
\multiput(92.5,5)(0.12,0.12){31}{\line(1,0){0.12}}
\linethickness{0.3mm}
\multiput(88.75,8.75)(0.12,-0.12){31}{\line(1,0){0.12}}
\linethickness{0.3mm}
\put(107.5,0){\line(0,1){25}}
\put(101.25,12.5){\makebox(0,0)[cc]{\EQLS}}

\linethickness{0.3mm}
\put(92.5,20){\line(0,1){5}}
\linethickness{0.3mm}
\multiput(88.75,16.25)(0.12,0.12){31}{\line(1,0){0.12}}
\linethickness{0.3mm}
\multiput(92.5,20)(0.12,-0.12){31}{\line(1,0){0.12}}
\linethickness{0.3mm}
\put(88.75,8.75){\line(0,1){7.5}}
\linethickness{0.3mm}
\put(96.25,8.75){\line(0,1){7.5}}
\put(40,12.5){\makebox(0,0)[cc]{\EQLS}}

\linethickness{0.3mm}
\multiput(2.5,8.75)(0.12,0.12){63}{\line(1,0){0.12}}
\linethickness{0.3mm}
\multiput(50,16.25)(0.12,-0.12){63}{\line(1,0){0.12}}
\linethickness{0.3mm}
\multiput(57.5,8.75)(0.12,0.12){21}{\line(1,0){0.12}}
\linethickness{0.3mm}
\put(60,11.25){\line(0,1){13.75}}
\linethickness{0.3mm}
\put(57.5,0){\line(0,1){8.75}}
\linethickness{0.3mm}
\multiput(47.5,13.75)(0.12,0.12){21}{\line(1,0){0.12}}
\linethickness{0.3mm}
\put(47.5,0){\line(0,1){13.75}}
\linethickness{0.3mm}
\put(10,16.25){\line(0,1){8.75}}
\linethickness{0.3mm}
\put(50,16.25){\line(0,1){8.75}}
\linethickness{0.3mm}
\multiput(10,16.25)(0.12,-0.12){21}{\line(1,0){0.12}}
\linethickness{0.3mm}
\put(12.5,0){\line(0,1){13.75}}
\linethickness{0.3mm}
\put(2.5,0){\line(0,1){8.75}}
\linethickness{0.3mm}
\multiput(0,11.25)(0.12,-0.12){21}{\line(1,0){0.12}}
\linethickness{0.3mm}
\put(0,11.25){\line(0,1){13.75}}
\linethickness{0.3mm}
\multiput(25,21.25)(0.12,-0.12){42}{\line(1,0){0.12}}
\linethickness{0.3mm}
\put(25,21.25){\line(0,1){3.75}}
\linethickness{0.3mm}
\multiput(30,8.75)(0.12,-0.12){42}{\line(1,0){0.12}}
\linethickness{0.3mm}
\put(35,0){\line(0,1){3.75}}
\linethickness{0.3mm}
\put(30,8.75){\line(0,1){7.5}}
\linethickness{0.3mm}
\multiput(25,3.75)(0.12,0.12){42}{\line(1,0){0.12}}
\linethickness{0.3mm}
\put(25,0){\line(0,1){3.75}}
\linethickness{0.3mm}
\multiput(30,16.25)(0.12,0.12){42}{\line(1,0){0.12}}
\linethickness{0.3mm}
\put(35,21.25){\line(0,1){3.75}}
\put(92.5,20){\makebox(0,0)[cc]{\DOTT}}

\put(92.5,5){\makebox(0,0)[cc]{\DOTT}}

\put(57.5,8.75){\makebox(0,0)[cc]{\DOTT}}

\put(50,16.25){\makebox(0,0)[cc]{\DOTT}}

\put(30,16.25){\makebox(0,0)[cc]{\DOTT}}

\put(30,8.75){\makebox(0,0)[cc]{\DOTT}}

\put(10,16.25){\makebox(0,0)[cc]{\DOTT}}

\put(2.5,8.75){\makebox(0,0)[cc]{\DOTT}}

\put(92.5,8.75){\makebox(0,0)[cc]{$\cpy$}}

\put(92.5,16.25){\makebox(0,0)[cc]{$\cpr$}}

\put(57.5,12.5){\makebox(0,0)[cc]{$\cpy$}}

\put(30,20){\makebox(0,0)[cc]{$\cpy$}}

\put(2.5,12.5){\makebox(0,0)[cc]{$\cpy$}}

\put(50,12.5){\makebox(0,0)[cc]{$\cpr$}}

\put(30,5){\makebox(0,0)[cc]{$\cpr$}}

\put(10,12.5){\makebox(0,0)[cc]{$\cpr$}}

\end{picture}


==> PIC/fstar-domain.tex <==
%%Created by jPicEdt 1.4.1_03: mixed JPIC-XML/LaTeX format
%%Wed Dec 16 09:55:28 GMT-10:00 2020
%%Begin JPIC-XML
%<?xml version="1.0" standalone="yes"?>
%<jpic x-min="5" x-max="385" y-min="0" y-max="165" auto-bounding="true">
%<multicurve fill-style= "none"
%	 points= "(275,70);(275,70);(275,90);(275,90)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(255,70);(255,70);(275,70);(275,70)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(265,70);(265,70);(265,0);(265,0)"
%	 />
%<ellipse p3= "(267.58,47.42)"
%	 fill-style= "solid"
%	 p2= "(267.58,52.58)"
%	 fill-color= "#330033"
%	 p1= "(262.42,52.58)"
%	 closure= "open"
%	 angle-end= "0"
%	 angle-start= "0"
%	 />
%<multicurve fill-style= "none"
%	 points= "(265,110);(265,110);(250,95);(250,95)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(250,65);(250,65);(265,50);(265,50)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(250,95);(250,95);(250,65);(250,65)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(255,90);(255,90);(255,70);(255,70)"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(220,90)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\EQLS
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(265,80)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\universal$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(268.75,95)"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\Atype$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(262.5,0)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\Progtype$
%</text>
%<multicurve fill-style= "none"
%	 points= "(255,90);(255,90);(275,90);(275,90)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(265,100);(265,100);(265,90);(265,90)"
%	 />
%<ellipse p3= "(267.58,97.42)"
%	 fill-style= "solid"
%	 p2= "(267.58,102.58)"
%	 fill-color= "#330033"
%	 p1= "(262.42,102.58)"
%	 closure= "open"
%	 angle-end= "0"
%	 angle-start= "0"
%	 />
%<multicurve fill-style= "none"
%	 points= "(265,165);(265,165);(265,110);(265,110)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(50,50);(50,50);(50,70);(50,70)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(30,50);(30,50);(50,50);(50,50)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(210,125);(210,125);(210,95);(210,95)"
%	 />
%<ellipse p3= "(162.58,57.42)"
%	 fill-style= "solid"
%	 p2= "(162.58,62.58)"
%	 fill-color= "#330033"
%	 p1= "(157.42,62.58)"
%	 closure= "open"
%	 angle-end= "0"
%	 angle-start= "0"
%	 />
%<multicurve fill-style= "none"
%	 points= "(25,95);(25,95);(10,80);(10,80)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(25,95);(25,95);(40,80);(40,80)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(40,80);(40,80);(40,70);(40,70)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(30,70);(30,70);(30,50);(30,50)"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(40,60)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\universal$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(7.5,0)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\Atype$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(72.5,120)"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\Progtype$
%</text>
%<multicurve fill-style= "none"
%	 points= "(30,70);(30,70);(50,70);(50,70)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(10,80);(10,80);(10,0);(10,0)"
%	 />
%<ellipse p3= "(27.58,92.42)"
%	 fill-style= "solid"
%	 p2= "(27.58,97.58)"
%	 fill-color= "#330033"
%	 p1= "(22.42,97.58)"
%	 closure= "open"
%	 angle-end= "0"
%	 angle-start= "0"
%	 />
%<multicurve fill-style= "none"
%	 points= "(180,110);(180,110);(180,130);(180,130)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(160,110);(160,110);(180,110);(180,110)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(25,105);(25,105);(25,95);(25,95)"
%	 />
%<ellipse p3= "(172.58,87.42)"
%	 fill-style= "solid"
%	 p2= "(172.58,92.58)"
%	 fill-color= "#330033"
%	 p1= "(167.42,92.58)"
%	 closure= "open"
%	 angle-end= "0"
%	 angle-start= "0"
%	 />
%<multicurve fill-style= "none"
%	 points= "(170,150);(170,150);(155,135);(155,135)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(155,105);(155,105);(170,90);(170,90)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(155,135);(155,135);(155,105);(155,105)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(160,130);(160,130);(160,110);(160,110)"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(170,120)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\universal$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(173.75,135)"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\Atype$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(225,140)"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\Progtype$
%</text>
%<multicurve fill-style= "none"
%	 points= "(160,130);(160,130);(180,130);(180,130)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(170,140);(170,140);(170,130);(170,130)"
%	 />
%<ellipse p3= "(172.58,137.42)"
%	 fill-style= "solid"
%	 p2= "(172.58,142.58)"
%	 fill-color= "#330033"
%	 p1= "(167.42,142.58)"
%	 closure= "open"
%	 angle-end= "0"
%	 angle-start= "0"
%	 />
%<multicurve fill-style= "none"
%	 points= "(170,165);(170,165);(170,150);(170,150)"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(87.5,165)"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\Progtype$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(22.5,165)"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\Progtype$
%</text>
%<multicurve fill-style= "none"
%	 points= "(245,115);(245,115);(280,115);(280,115)"
%	 stroke-width= "0.1"
%	 />
%<multicurve fill-style= "none"
%	 points= "(280,115);(280,115);(280,45);(280,45)"
%	 stroke-width= "0.1"
%	 />
%<multicurve fill-style= "none"
%	 points= "(245,115);(245,115);(245,45);(245,45)"
%	 stroke-width= "0.1"
%	 />
%<multicurve fill-style= "none"
%	 points= "(245,45);(245,45);(280,45);(280,45)"
%	 stroke-width= "0.1"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(272.5,60)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\nameiota$
%</text>
%<multicurve fill-style= "none"
%	 points= "(150,155);(150,155);(185,155);(185,155)"
%	 stroke-width= "0.1"
%	 />
%<multicurve fill-style= "none"
%	 points= "(185,155);(185,155);(185,85);(185,85)"
%	 stroke-width= "0.1"
%	 />
%<multicurve fill-style= "none"
%	 points= "(150,155);(150,155);(150,85);(150,85)"
%	 stroke-width= "0.1"
%	 />
%<multicurve fill-style= "none"
%	 points= "(150,85);(150,85);(185,85);(185,85)"
%	 stroke-width= "0.1"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(177.5,100)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\nameiota$
%</text>
%<multicurve fill-style= "none"
%	 points= "(5,112.5);(5,112.5);(75,112.5);(75,112.5)"
%	 stroke-width= "0.1"
%	 />
%<multicurve fill-style= "none"
%	 points= "(75,112.5);(75,112.5);(75,7.5);(75,7.5)"
%	 stroke-width= "0.1"
%	 />
%<multicurve fill-style= "none"
%	 points= "(5,112.5);(5,112.5);(5,7.5);(5,7.5)"
%	 stroke-width= "0.1"
%	 />
%<multicurve fill-style= "none"
%	 points= "(5,7.5);(5,7.5);(75,7.5);(75,7.5)"
%	 stroke-width= "0.1"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(175,50)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\nameiota$
%</text>
%<multicurve fill-style= "none"
%	 points= "(315,70);(315,70);(315,90);(315,90)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(295,70);(295,70);(315,70);(315,70)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(305,50);(305,50);(305,0);(305,0)"
%	 />
%<ellipse p3= "(307.58,107.42)"
%	 fill-style= "solid"
%	 p2= "(307.58,112.58)"
%	 fill-color= "#330033"
%	 p1= "(302.42,112.58)"
%	 closure= "open"
%	 angle-end= "0"
%	 angle-start= "0"
%	 />
%<multicurve fill-style= "none"
%	 points= "(305,110);(305,110);(290,95);(290,95)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(290,65);(290,65);(305,50);(305,50)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(290,95);(290,95);(290,65);(290,65)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(295,90);(295,90);(295,70);(295,70)"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(335,80)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\EQLS
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(305,80)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\universal$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(302.5,0)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\Atype$
%</text>
%<multicurve fill-style= "none"
%	 points= "(295,90);(295,90);(315,90);(315,90)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(305,70);(305,70);(305,60);(305,60)"
%	 />
%<ellipse p3= "(307.58,57.42)"
%	 fill-style= "solid"
%	 p2= "(307.58,62.58)"
%	 fill-color= "#330033"
%	 p1= "(302.42,62.58)"
%	 closure= "open"
%	 angle-end= "0"
%	 angle-start= "0"
%	 />
%<multicurve fill-style= "none"
%	 points= "(305,165);(305,165);(305,90);(305,90)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(380,30);(380,30);(380,50);(380,50)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(360,30);(360,30);(380,30);(380,30)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(370,10);(370,10);(370,0);(370,0)"
%	 />
%<ellipse p3= "(372.58,17.42)"
%	 fill-style= "solid"
%	 p2= "(372.58,22.58)"
%	 fill-color= "#330033"
%	 p1= "(367.42,22.58)"
%	 closure= "open"
%	 angle-end= "0"
%	 angle-start= "0"
%	 />
%<multicurve fill-style= "none"
%	 points= "(370,70);(370,70);(355,55);(355,55)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(355,25);(355,25);(370,10);(370,10)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(355,55);(355,55);(355,25);(355,25)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(360,50);(360,50);(360,30);(360,30)"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(370,40)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\universal$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(367.5,55)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\Atype$
%</text>
%<multicurve fill-style= "none"
%	 points= "(360,50);(360,50);(380,50);(380,50)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(370,30);(370,30);(370,20);(370,20)"
%	 />
%<ellipse p3= "(372.58,67.42)"
%	 fill-style= "solid"
%	 p2= "(372.58,72.58)"
%	 fill-color= "#330033"
%	 p1= "(367.42,72.58)"
%	 closure= "open"
%	 angle-end= "0"
%	 angle-start= "0"
%	 />
%<multicurve fill-style= "none"
%	 points= "(380,110);(380,110);(380,130);(380,130)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(360,110);(360,110);(380,110);(380,110)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(370,90);(370,90);(370,50);(370,50)"
%	 />
%<ellipse p3= "(372.58,97.42)"
%	 fill-style= "solid"
%	 p2= "(372.58,102.58)"
%	 fill-color= "#330033"
%	 p1= "(367.42,102.58)"
%	 closure= "open"
%	 angle-end= "0"
%	 angle-start= "0"
%	 />
%<multicurve fill-style= "none"
%	 points= "(370,150);(370,150);(355,135);(355,135)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(355,105);(355,105);(370,90);(370,90)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(355,135);(355,135);(355,105);(355,105)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(360,130);(360,130);(360,110);(360,110)"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(370,120)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\universal$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(367.5,0)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\Atype$
%</text>
%<multicurve fill-style= "none"
%	 points= "(360,130);(360,130);(380,130);(380,130)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(370,110);(370,110);(370,100);(370,100)"
%	 />
%<ellipse p3= "(372.58,147.42)"
%	 fill-style= "solid"
%	 p2= "(372.58,152.58)"
%	 fill-color= "#330033"
%	 p1= "(367.42,152.58)"
%	 closure= "open"
%	 angle-end= "0"
%	 angle-start= "0"
%	 />
%<multicurve fill-style= "none"
%	 points= "(370,165);(370,165);(370,130);(370,130)"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(367.5,105)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\Progtype$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(302.5,65)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\Progtype$
%</text>
%<multicurve fill-style= "none"
%	 points= "(285,115);(285,115);(320,115);(320,115)"
%	 stroke-width= "0.1"
%	 />
%<multicurve fill-style= "none"
%	 points= "(320,115);(320,115);(320,45);(320,45)"
%	 stroke-width= "0.1"
%	 />
%<multicurve fill-style= "none"
%	 points= "(285,115);(285,115);(285,45);(285,45)"
%	 stroke-width= "0.1"
%	 />
%<multicurve fill-style= "none"
%	 points= "(285,45);(285,45);(320,45);(320,45)"
%	 stroke-width= "0.1"
%	 />
%<multicurve fill-style= "none"
%	 points= "(350,155);(350,155);(385,155);(385,155)"
%	 stroke-width= "0.1"
%	 />
%<multicurve fill-style= "none"
%	 points= "(385,155);(385,155);(385,85);(385,85)"
%	 stroke-width= "0.1"
%	 />
%<multicurve fill-style= "none"
%	 points= "(350,155);(350,155);(350,85);(350,85)"
%	 stroke-width= "0.1"
%	 />
%<multicurve fill-style= "none"
%	 points= "(350,85);(350,85);(385,85);(385,85)"
%	 stroke-width= "0.1"
%	 />
%<multicurve fill-style= "none"
%	 points= "(350,75);(350,75);(385,75);(385,75)"
%	 stroke-width= "0.1"
%	 />
%<multicurve fill-style= "none"
%	 points= "(385,75);(385,75);(385,5);(385,5)"
%	 stroke-width= "0.1"
%	 />
%<multicurve fill-style= "none"
%	 points= "(350,75);(350,75);(350,5);(350,5)"
%	 stroke-width= "0.1"
%	 />
%<multicurve fill-style= "none"
%	 points= "(350,5);(350,5);(385,5);(385,5)"
%	 stroke-width= "0.1"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(312.5,100)"
%	 text-frame= "noframe"
%	 stroke-width= "0.2"
%	 text-hor-align= "center-h"
%	 >
%$\nametau$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(377.5,60)"
%	 text-frame= "noframe"
%	 stroke-width= "0.2"
%	 text-hor-align= "center-h"
%	 >
%$\nametau$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(377.5,140)"
%	 text-frame= "noframe"
%	 stroke-width= "0.2"
%	 text-hor-align= "center-h"
%	 >
%$\nametau$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(367.5,25)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\Progtype$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(242.5,165)"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\Atype$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(307.5,165)"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\Atype$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(367.5,135)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\Atype$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(302.5,95)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\Atype$
%</text>
%<ellipse p3= "(27.58,102.42)"
%	 fill-style= "solid"
%	 p2= "(27.58,107.58)"
%	 fill-color= "#330033"
%	 p1= "(22.42,107.58)"
%	 closure= "open"
%	 angle-end= "0"
%	 angle-start= "0"
%	 />
%<multicurve fill-style= "none"
%	 points= "(40,50);(40,50);(40,40);(40,40)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(70,40);(70,40);(55,25);(55,25)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(40,40);(40,40);(55,25);(55,25)"
%	 />
%<ellipse p3= "(57.58,12.42)"
%	 fill-style= "solid"
%	 p2= "(57.58,17.58)"
%	 fill-color= "#330033"
%	 p1= "(52.42,17.58)"
%	 closure= "open"
%	 angle-end= "0"
%	 angle-start= "0"
%	 />
%<multicurve fill-style= "none"
%	 points= "(55,25);(55,25);(55,15);(55,15)"
%	 />
%<ellipse p3= "(57.58,22.42)"
%	 fill-style= "solid"
%	 p2= "(57.58,27.58)"
%	 fill-color= "#330033"
%	 p1= "(52.42,27.58)"
%	 closure= "open"
%	 angle-end= "0"
%	 angle-start= "0"
%	 />
%<multicurve fill-style= "none"
%	 points= "(70,120);(70,120);(70,40);(70,40)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(200,85);(200,85);(200,15);(200,15)"
%	 />
%</jpic>
%%End JPIC-XML
%PSTricks content-type (pstricks.sty package needed)
%Add \usepackage{pstricks} in the preamble of your LaTeX file
%You can rescale the whole picture (to 80% for instance) by using the command \def\JPicScale{0.8}
\ifx\JPicScale\undefined\def\JPicScale{1}\fi
\psset{unit=\JPicScale mm}
\psset{linewidth=0.3,dotsep=1,hatchwidth=0.3,hatchsep=1.5,shadowsize=1,dimen=middle}
\psset{dotsize=0.7 2.5,dotscale=1 1,fillcolor=black}
\psset{arrowsize=1 2,arrowlength=1,arrowinset=0.25,tbarsize=0.7 5,bracketlength=0.15,rbracketlength=0.15}
\begin{pspicture}(0,0)(385,165)
\psline(275,70)(275,90)
\psline(255,70)(275,70)
\psline(265,70)(265,0)
\newrgbcolor{userFillColour}{0.2 0 0.2}
\rput{0}(265,50){\psellipse[fillcolor=userFillColour,fillstyle=solid](0,0)(2.58,-2.58)}
\psline(265,110)(250,95)
\psline(250,65)(265,50)
\psline(250,95)(250,65)
\psline(255,90)(255,70)
\rput(220,90){\EQLS}
\rput(265,80){$\universal$}
\rput[l](268.75,95){$\Atype$}
\rput[r](262.5,0){$\Progtype$}
\psline(255,90)(275,90)
\psline(265,100)(265,90)
\newrgbcolor{userFillColour}{0.2 0 0.2}
\rput{0}(265,100){\psellipse[fillcolor=userFillColour,fillstyle=solid](0,0)(2.58,-2.58)}
\psline(265,165)(265,110)
\psline(50,50)(50,70)
\psline(30,50)(50,50)
\psline(210,125)(210,95)
\newrgbcolor{userFillColour}{0.2 0 0.2}
\rput{0}(160,60){\psellipse[fillcolor=userFillColour,fillstyle=solid](0,0)(2.58,-2.58)}
\psline(25,95)(10,80)
\psline(25,95)(40,80)
\psline(40,80)(40,70)
\psline(30,70)(30,50)
\rput(40,60){$\universal$}
\rput[r](7.5,0){$\Atype$}
\rput[l](72.5,120){$\Progtype$}
\psline(30,70)(50,70)
\psline(10,80)(10,0)
\newrgbcolor{userFillColour}{0.2 0 0.2}
\rput{0}(25,95){\psellipse[fillcolor=userFillColour,fillstyle=solid](0,0)(2.58,-2.58)}
\psline(180,110)(180,130)
\psline(160,110)(180,110)
\psline(25,105)(25,95)
\newrgbcolor{userFillColour}{0.2 0 0.2}
\rput{0}(170,90){\psellipse[fillcolor=userFillColour,fillstyle=solid](0,0)(2.58,-2.58)}
\psline(170,150)(155,135)
\psline(155,105)(170,90)
\psline(155,135)(155,105)
\psline(160,130)(160,110)
\rput(170,120){$\universal$}
\rput[l](173.75,135){$\Atype$}
\rput[l](225,140){$\Progtype$}
\psline(160,130)(180,130)
\psline(170,140)(170,130)
\newrgbcolor{userFillColour}{0.2 0 0.2}
\rput{0}(170,140){\psellipse[fillcolor=userFillColour,fillstyle=solid](0,0)(2.58,-2.58)}
\psline(170,165)(170,150)
\rput[l](87.5,165){$\Progtype$}
\rput[l](22.5,165){$\Progtype$}
\psline[linewidth=0.1](245,115)(280,115)
\psline[linewidth=0.1](280,115)(280,45)
\psline[linewidth=0.1](245,115)(245,45)
\psline[linewidth=0.1](245,45)(280,45)
\rput(272.5,60){$\nameiota$}
\psline[linewidth=0.1](150,155)(185,155)
\psline[linewidth=0.1](185,155)(185,85)
\psline[linewidth=0.1](150,155)(150,85)
\psline[linewidth=0.1](150,85)(185,85)
\rput(177.5,100){$\nameiota$}
\psline[linewidth=0.1](5,112.5)(75,112.5)
\psline[linewidth=0.1](75,112.5)(75,7.5)
\psline[linewidth=0.1](5,112.5)(5,7.5)
\psline[linewidth=0.1](5,7.5)(75,7.5)
\rput(175,50){$\nameiota$}
\psline(315,70)(315,90)
\psline(295,70)(315,70)
\psline(305,50)(305,0)
\newrgbcolor{userFillColour}{0.2 0 0.2}
\rput{0}(305,110){\psellipse[fillcolor=userFillColour,fillstyle=solid](0,0)(2.58,-2.58)}
\psline(305,110)(290,95)
\psline(290,65)(305,50)
\psline(290,95)(290,65)
\psline(295,90)(295,70)
\rput(335,80){\EQLS}
\rput(305,80){$\universal$}
\rput[r](302.5,0){$\Atype$}
\psline(295,90)(315,90)
\psline(305,70)(305,60)
\newrgbcolor{userFillColour}{0.2 0 0.2}
\rput{0}(305,60){\psellipse[fillcolor=userFillColour,fillstyle=solid](0,0)(2.58,-2.58)}
\psline(305,165)(305,90)
\psline(380,30)(380,50)
\psline(360,30)(380,30)
\psline(370,10)(370,0)
\newrgbcolor{userFillColour}{0.2 0 0.2}
\rput{0}(370,20){\psellipse[fillcolor=userFillColour,fillstyle=solid](0,0)(2.58,-2.58)}
\psline(370,70)(355,55)
\psline(355,25)(370,10)
\psline(355,55)(355,25)
\psline(360,50)(360,30)
\rput(370,40){$\universal$}
\rput[r](367.5,55){$\Atype$}
\psline(360,50)(380,50)
\psline(370,30)(370,20)
\newrgbcolor{userFillColour}{0.2 0 0.2}
\rput{0}(370,70){\psellipse[fillcolor=userFillColour,fillstyle=solid](0,0)(2.58,-2.58)}
\psline(380,110)(380,130)
\psline(360,110)(380,110)
\psline(370,90)(370,50)
\newrgbcolor{userFillColour}{0.2 0 0.2}
\rput{0}(370,100){\psellipse[fillcolor=userFillColour,fillstyle=solid](0,0)(2.58,-2.58)}
\psline(370,150)(355,135)
\psline(355,105)(370,90)
\psline(355,135)(355,105)
\psline(360,130)(360,110)
\rput(370,120){$\universal$}
\rput[r](367.5,0){$\Atype$}
\psline(360,130)(380,130)
\psline(370,110)(370,100)
\newrgbcolor{userFillColour}{0.2 0 0.2}
\rput{0}(370,150){\psellipse[fillcolor=userFillColour,fillstyle=solid](0,0)(2.58,-2.58)}
\psline(370,165)(370,130)
\rput[r](367.5,105){$\Progtype$}
\rput[r](302.5,65){$\Progtype$}
\psline[linewidth=0.1](285,115)(320,115)
\psline[linewidth=0.1](320,115)(320,45)
\psline[linewidth=0.1](285,115)(285,45)
\psline[linewidth=0.1](285,45)(320,45)
\psline[linewidth=0.1](350,155)(385,155)
\psline[linewidth=0.1](385,155)(385,85)
\psline[linewidth=0.1](350,155)(350,85)
\psline[linewidth=0.1](350,85)(385,85)
\psline[linewidth=0.1](350,75)(385,75)
\psline[linewidth=0.1](385,75)(385,5)
\psline[linewidth=0.1](350,75)(350,5)
\psline[linewidth=0.1](350,5)(385,5)
\rput(312.5,100){$\nametau$}
\rput(377.5,60){$\nametau$}
\rput(377.5,140){$\nametau$}
\rput[r](367.5,25){$\Progtype$}
\rput[l](242.5,165){$\Atype$}
\rput[l](307.5,165){$\Atype$}
\rput[r](367.5,135){$\Atype$}
\rput[r](302.5,95){$\Atype$}
\newrgbcolor{userFillColour}{0.2 0 0.2}
\rput{0}(25,105){\psellipse[fillcolor=userFillColour,fillstyle=solid](0,0)(2.58,-2.58)}
\psline(40,50)(40,40)
\psline(70,40)(55,25)
\psline(40,40)(55,25)
\newrgbcolor{userFillColour}{0.2 0 0.2}
\rput{0}(55,15){\psellipse[fillcolor=userFillColour,fillstyle=solid](0,0)(2.58,-2.58)}
\psline(55,25)(55,15)
\newrgbcolor{userFillColour}{0.2 0 0.2}
\rput{0}(55,25){\psellipse[fillcolor=userFillColour,fillstyle=solid](0,0)(2.58,-2.58)}
\psline(70,120)(70,40)
\psline(200,85)(200,15)
\end{pspicture}


==> PIC/fstar.tex <==
%%Created by jPicEdt 1.4.1_03: mixed JPIC-XML/LaTeX format
%%Wed Dec 16 10:42:31 GMT-10:00 2020
%%Begin JPIC-XML
%<?xml version="1.0" standalone="yes"?>
%<jpic x-min="5" x-max="75" y-min="0" y-max="140" auto-bounding="true">
%<multicurve fill-style= "none"
%	 points= "(50,60);(50,60);(50,80);(50,80)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(30,60);(30,60);(50,60);(50,60)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(25,105);(25,105);(10,90);(10,90)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(25,105);(25,105);(40,90);(40,90)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(40,90);(40,90);(40,80);(40,80)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(30,80);(30,80);(30,60);(30,60)"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(40,70)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\universal$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(7.5,0)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\Atype$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(72.5,140)"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\Progtype$
%</text>
%<multicurve fill-style= "none"
%	 points= "(30,80);(30,80);(50,80);(50,80)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(10,90);(10,90);(10,0);(10,0)"
%	 />
%<ellipse p3= "(27.58,102.42)"
%	 fill-style= "solid"
%	 p2= "(27.58,107.58)"
%	 fill-color= "#330033"
%	 p1= "(22.42,107.58)"
%	 closure= "open"
%	 angle-end= "0"
%	 angle-start= "0"
%	 />
%<multicurve fill-style= "none"
%	 points= "(25,115);(25,115);(25,105);(25,105)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(5,122.5);(5,122.5);(75,122.5);(75,122.5)"
%	 stroke-width= "0.1"
%	 />
%<multicurve fill-style= "none"
%	 points= "(75,122.5);(75,122.5);(75,17.5);(75,17.5)"
%	 stroke-width= "0.1"
%	 />
%<multicurve fill-style= "none"
%	 points= "(5,122.5);(5,122.5);(5,17.5);(5,17.5)"
%	 stroke-width= "0.1"
%	 />
%<multicurve fill-style= "none"
%	 points= "(5,17.5);(5,17.5);(75,17.5);(75,17.5)"
%	 stroke-width= "0.1"
%	 />
%<ellipse p3= "(27.58,112.42)"
%	 fill-style= "solid"
%	 p2= "(27.58,117.58)"
%	 fill-color= "#330033"
%	 p1= "(22.42,117.58)"
%	 closure= "open"
%	 angle-end= "0"
%	 angle-start= "0"
%	 />
%<multicurve fill-style= "none"
%	 points= "(40,60);(40,60);(40,50);(40,50)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(70,50);(70,50);(55,35);(55,35)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(40,50);(40,50);(55,35);(55,35)"
%	 />
%<ellipse p3= "(57.58,22.42)"
%	 fill-style= "solid"
%	 p2= "(57.58,27.58)"
%	 fill-color= "#330033"
%	 p1= "(52.42,27.58)"
%	 closure= "open"
%	 angle-end= "0"
%	 angle-start= "0"
%	 />
%<multicurve fill-style= "none"
%	 points= "(55,35);(55,35);(55,25);(55,25)"
%	 />
%<ellipse p3= "(57.58,32.42)"
%	 fill-style= "solid"
%	 p2= "(57.58,37.58)"
%	 fill-color= "#330033"
%	 p1= "(52.42,37.58)"
%	 closure= "open"
%	 angle-end= "0"
%	 angle-start= "0"
%	 />
%<multicurve fill-style= "none"
%	 points= "(70,140);(70,140);(70,50);(70,50)"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(25,40)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\fstar$
%</text>
%</jpic>
%%End JPIC-XML
%LaTeX-picture environment using emulated lines and arcs
%You can rescale the whole picture (to 80% for instance) by using the command \def\JPicScale{0.8}
\ifx\JPicScale\undefined\def\JPicScale{1}\fi
\unitlength \JPicScale mm
\begin{picture}(75,140)(0,0)
\linethickness{0.3mm}
\put(50,60){\line(0,1){20}}
\linethickness{0.3mm}
\put(30,60){\line(1,0){20}}
\linethickness{0.3mm}
\multiput(10,90)(0.12,0.12){125}{\line(1,0){0.12}}
\linethickness{0.3mm}
\multiput(25,105)(0.12,-0.12){125}{\line(1,0){0.12}}
\linethickness{0.3mm}
\put(40,80){\line(0,1){10}}
\linethickness{0.3mm}
\put(30,60){\line(0,1){20}}
\put(40,70){\makebox(0,0)[cc]{$\universal$}}

\put(7.5,0){\makebox(0,0)[cr]{$\Atype$}}

\put(72.5,140){\makebox(0,0)[cl]{$\Progtype$}}

\linethickness{0.3mm}
\put(30,80){\line(1,0){20}}
\linethickness{0.3mm}
\put(10,0){\line(0,1){90}}
\linethickness{0.3mm}
\put(25,105){\circle*{5.16}}

\linethickness{0.3mm}
\put(25,105){\line(0,1){10}}
\linethickness{0.1mm}
\put(5,122.5){\line(1,0){70}}
\linethickness{0.1mm}
\put(75,17.5){\line(0,1){105}}
\linethickness{0.1mm}
\put(5,17.5){\line(0,1){105}}
\linethickness{0.1mm}
\put(5,17.5){\line(1,0){70}}
\linethickness{0.3mm}
\put(25,115){\circle*{5.16}}

\linethickness{0.3mm}
\put(40,50){\line(0,1){10}}
\linethickness{0.3mm}
\multiput(55,35)(0.12,0.12){125}{\line(1,0){0.12}}
\linethickness{0.3mm}
\multiput(40,50)(0.12,-0.12){125}{\line(1,0){0.12}}
\linethickness{0.3mm}
\put(55,25){\circle*{5.16}}

\linethickness{0.3mm}
\put(55,25){\line(0,1){10}}
\linethickness{0.3mm}
\put(55,35){\circle*{5.16}}

\linethickness{0.3mm}
\put(70,50){\line(0,1){90}}
\put(25,40){\makebox(0,0)[cc]{$\fstar$}}

\end{picture}


==> PIC/fun-consistent-1.tex <==
%%Created by jPicEdt 1.4.1_03: mixed JPIC-XML/LaTeX format
%%Thu Dec 17 07:38:14 GMT-10:00 2020
%%Begin JPIC-XML
%<?xml version="1.0" standalone="yes"?>
%<jpic x-min="15" x-max="35" y-min="-35" y-max="48.79" auto-bounding="true">
%<multicurve fill-style= "none"
%	 points= "(25,10);(25,10);(25,-35);(25,-35)"
%	 stroke-width= "0.75"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(22.5,-35)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\AAh$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(27.5,35)"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\BBh$
%</text>
%<multicurve fill-style= "none"
%	 points= "(25,45);(25,45);(25,30);(25,30)"
%	 stroke-width= "0.75"
%	 />
%<parallelogram p3= "(35,10)"
%	 fill-style= "solid"
%	 p2= "(35,30)"
%	 fill-color= "#ffffff"
%	 p1= "(15,30)"
%	 stroke-width= "0.7"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(25,20)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\aah$
%</text>
%<ellipse p3= "(28.79,41.21)"
%	 fill-style= "solid"
%	 p2= "(28.79,48.79)"
%	 fill-color= "#330033"
%	 p1= "(21.21,48.79)"
%	 closure= "open"
%	 angle-end= "0"
%	 angle-start= "0"
%	 />
%</jpic>
%%End JPIC-XML
%PSTricks content-type (pstricks.sty package needed)
%Add \usepackage{pstricks} in the preamble of your LaTeX file
%You can rescale the whole picture (to 80% for instance) by using the command \def\JPicScale{0.8}
\ifx\JPicScale\undefined\def\JPicScale{1}\fi
\psset{unit=\JPicScale mm}
\psset{linewidth=0.3,dotsep=1,hatchwidth=0.3,hatchsep=1.5,shadowsize=1,dimen=middle}
\psset{dotsize=0.7 2.5,dotscale=1 1,fillcolor=black}
\psset{arrowsize=1 2,arrowlength=1,arrowinset=0.25,tbarsize=0.7 5,bracketlength=0.15,rbracketlength=0.15}
\begin{pspicture}(0,0)(35,48.79)
\psline[linewidth=0.75](25,10)(25,-35)
\rput[r](22.5,-35){$\AAh$}
\rput[l](27.5,35){$\BBh$}
\psline[linewidth=0.75](25,45)(25,30)
\pspolygon[linewidth=0.7,fillcolor=white,fillstyle=solid](15,30)(35,30)(35,10)(15,10)
\rput(25,20){$\aah$}
\newrgbcolor{userFillColour}{0.2 0 0.2}
\rput{0}(25,45){\psellipse[fillcolor=userFillColour,fillstyle=solid](0,0)(3.79,-3.79)}
\end{pspicture}


==> PIC/fun-consistent-2.tex <==
%%Created by jPicEdt 1.4.1_03: mixed JPIC-XML/LaTeX format
%%Thu Dec 17 07:35:43 GMT-10:00 2020
%%Begin JPIC-XML
%<?xml version="1.0" standalone="yes"?>
%<jpic x-min="20" x-max="70" y-min="-35" y-max="48.79" auto-bounding="true">
%<multicurve fill-style= "none"
%	 points= "(60,0);(60,0);(45,-15);(45,-15)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(45,-15);(45,-15);(45,-35);(45,-35)"
%	 stroke-width= "0.75"
%	 />
%<ellipse p3= "(48.79,-18.79)"
%	 fill-style= "solid"
%	 p2= "(48.79,-11.21)"
%	 fill-color= "#330033"
%	 p1= "(41.21,-11.21)"
%	 closure= "open"
%	 angle-end= "0"
%	 angle-start= "0"
%	 />
%<multicurve fill-style= "none"
%	 points= "(30,10);(30,10);(30,0);(30,0)"
%	 stroke-width= "0.6"
%	 />
%<multicurve fill-style= "none"
%	 points= "(30,0);(30,0);(45,-15);(45,-15)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(60,10);(60,10);(60,0);(60,0)"
%	 stroke-width= "0.6"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(42.5,-35)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\AAh$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(62.5,35)"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\BBh$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(32.5,35)"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\BBh$
%</text>
%<multicurve fill-style= "none"
%	 points= "(30,45);(30,45);(30,30);(30,30)"
%	 stroke-width= "0.75"
%	 />
%<parallelogram p3= "(40,10)"
%	 fill-style= "solid"
%	 p2= "(40,30)"
%	 fill-color= "#ffffff"
%	 p1= "(20,30)"
%	 stroke-width= "0.7"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(30,20)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\aah$
%</text>
%<parallelogram p3= "(70,10)"
%	 fill-style= "solid"
%	 p2= "(70,30)"
%	 fill-color= "#ffffff"
%	 p1= "(50,30)"
%	 stroke-width= "0.7"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(60,20)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\aah$
%</text>
%<multicurve fill-style= "none"
%	 points= "(60,45);(60,45);(60,30);(60,30)"
%	 stroke-width= "0.75"
%	 />
%<ellipse p3= "(63.79,41.21)"
%	 fill-style= "solid"
%	 p2= "(63.79,48.79)"
%	 fill-color= "#330033"
%	 p1= "(56.21,48.79)"
%	 closure= "open"
%	 angle-end= "0"
%	 angle-start= "0"
%	 />
%<ellipse p3= "(33.79,41.21)"
%	 fill-style= "solid"
%	 p2= "(33.79,48.79)"
%	 fill-color= "#330033"
%	 p1= "(26.21,48.79)"
%	 closure= "open"
%	 angle-end= "0"
%	 angle-start= "0"
%	 />
%</jpic>
%%End JPIC-XML
%PSTricks content-type (pstricks.sty package needed)
%Add \usepackage{pstricks} in the preamble of your LaTeX file
%You can rescale the whole picture (to 80% for instance) by using the command \def\JPicScale{0.8}
\ifx\JPicScale\undefined\def\JPicScale{1}\fi
\psset{unit=\JPicScale mm}
\psset{linewidth=0.3,dotsep=1,hatchwidth=0.3,hatchsep=1.5,shadowsize=1,dimen=middle}
\psset{dotsize=0.7 2.5,dotscale=1 1,fillcolor=black}
\psset{arrowsize=1 2,arrowlength=1,arrowinset=0.25,tbarsize=0.7 5,bracketlength=0.15,rbracketlength=0.15}
\begin{pspicture}(0,0)(70,48.79)
\psline[linewidth=0.75](60,0)(45,-15)
\psline[linewidth=0.75](45,-15)(45,-35)
\newrgbcolor{userFillColour}{0.2 0 0.2}
\rput{0}(45,-15){\psellipse[fillcolor=userFillColour,fillstyle=solid](0,0)(3.79,-3.79)}
\psline[linewidth=0.6](30,10)(30,0)
\psline[linewidth=0.75](30,0)(45,-15)
\psline[linewidth=0.6](60,10)(60,0)
\rput[r](42.5,-35){$\AAh$}
\rput[l](62.5,35){$\BBh$}
\rput[l](32.5,35){$\BBh$}
\psline[linewidth=0.75](30,45)(30,30)
\pspolygon[linewidth=0.7,fillcolor=white,fillstyle=solid](20,30)(40,30)(40,10)(20,10)
\rput(30,20){$\aah$}
\pspolygon[linewidth=0.7,fillcolor=white,fillstyle=solid](50,30)(70,30)(70,10)(50,10)
\rput(60,20){$\aah$}
\psline[linewidth=0.75](60,45)(60,30)
\newrgbcolor{userFillColour}{0.2 0 0.2}
\rput{0}(60,45){\psellipse[fillcolor=userFillColour,fillstyle=solid](0,0)(3.79,-3.79)}
\newrgbcolor{userFillColour}{0.2 0 0.2}
\rput{0}(30,45){\psellipse[fillcolor=userFillColour,fillstyle=solid](0,0)(3.79,-3.79)}
\end{pspicture}


==> PIC/fun-consistent-3.tex <==
%%Created by jPicEdt 1.4.1_03: mixed JPIC-XML/LaTeX format
%%Fri Dec 18 16:16:59 GMT-10:00 2020
%%Begin JPIC-XML
%<?xml version="1.0" standalone="yes"?>
%<jpic x-min="-0" x-max="20" y-min="-38.79" y-max="40" auto-bounding="true">
%<multicurve fill-style= "none"
%	 points= "(10,0);(10,0);(10,40);(10,40)"
%	 stroke-width= "0.75"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(6.25,-26.25)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\AAh$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(13.75,40)"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\BBh$
%</text>
%<multicurve fill-style= "none"
%	 points= "(10,-35);(10,-35);(10,-20);(10,-20)"
%	 stroke-width= "0.75"
%	 />
%<parallelogram p3= "(-0,0)"
%	 fill-style= "solid"
%	 p2= "(0,-20)"
%	 fill-color= "#ffffff"
%	 p1= "(20,-20)"
%	 stroke-width= "0.7"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(10,-10)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\aah$
%</text>
%<ellipse p3= "(6.21,-31.21)"
%	 fill-style= "solid"
%	 p2= "(6.21,-38.79)"
%	 fill-color= "#330033"
%	 p1= "(13.79,-38.79)"
%	 closure= "open"
%	 angle-end= "0"
%	 angle-start= "0"
%	 />
%</jpic>
%%End JPIC-XML
%PSTricks content-type (pstricks.sty package needed)
%Add \usepackage{pstricks} in the preamble of your LaTeX file
%You can rescale the whole picture (to 80% for instance) by using the command \def\JPicScale{0.8}
\ifx\JPicScale\undefined\def\JPicScale{1}\fi
\psset{unit=\JPicScale mm}
\psset{linewidth=0.3,dotsep=1,hatchwidth=0.3,hatchsep=1.5,shadowsize=1,dimen=middle}
\psset{dotsize=0.7 2.5,dotscale=1 1,fillcolor=black}
\psset{arrowsize=1 2,arrowlength=1,arrowinset=0.25,tbarsize=0.7 5,bracketlength=0.15,rbracketlength=0.15}
\begin{pspicture}(0,0)(20,40)
\psline[linewidth=0.75](10,0)(10,40)
\rput[r](6.25,-26.25){$\AAh$}
\rput[l](13.75,40){$\BBh$}
\psline[linewidth=0.75](10,-35)(10,-20)
\pspolygon[linewidth=0.7,fillcolor=white,fillstyle=solid](20,-20)(0,-20)(-0,0)(20,0)
\rput(10,-10){$\aah$}
\newrgbcolor{userFillColour}{0.2 0 0.2}
\rput{0}(10,-35){\psellipse[fillcolor=userFillColour,fillstyle=solid](0,0)(3.79,-3.79)}
\end{pspicture}


==> PIC/fun-consistent-4.tex <==
%%Created by jPicEdt 1.4.1_03: mixed JPIC-XML/LaTeX format
%%Fri Dec 18 16:19:23 GMT-10:00 2020
%%Begin JPIC-XML
%<?xml version="1.0" standalone="yes"?>
%<jpic x-min="50" x-max="100" y-min="-38.79" y-max="40" auto-bounding="true">
%<multicurve fill-style= "none"
%	 points= "(60,10);(60,10);(75,25);(75,25)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(75,25);(75,25);(75,40);(75,40)"
%	 stroke-width= "0.75"
%	 />
%<ellipse p3= "(71.21,28.79)"
%	 fill-style= "solid"
%	 p2= "(71.21,21.21)"
%	 fill-color= "#330033"
%	 p1= "(78.79,21.21)"
%	 closure= "open"
%	 angle-end= "0"
%	 angle-start= "0"
%	 />
%<multicurve fill-style= "none"
%	 points= "(90,0);(90,0);(90,10);(90,10)"
%	 stroke-width= "0.6"
%	 />
%<multicurve fill-style= "none"
%	 points= "(90,10);(90,10);(75,25);(75,25)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(60,-0);(60,-0);(60,10);(60,10)"
%	 stroke-width= "0.6"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(86.25,-26.25)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\AAh$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(78.75,40)"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\BBh$
%</text>
%<multicurve fill-style= "none"
%	 points= "(90,-35);(90,-35);(90,-20);(90,-20)"
%	 stroke-width= "0.75"
%	 />
%<parallelogram p3= "(80,-0)"
%	 fill-style= "solid"
%	 p2= "(80,-20)"
%	 fill-color= "#ffffff"
%	 p1= "(100,-20)"
%	 stroke-width= "0.7"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(90,-10)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\aah$
%</text>
%<parallelogram p3= "(50,-0)"
%	 fill-style= "solid"
%	 p2= "(50,-20)"
%	 fill-color= "#ffffff"
%	 p1= "(70,-20)"
%	 stroke-width= "0.7"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(60,-10)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\aah$
%</text>
%<multicurve fill-style= "none"
%	 points= "(60,-35);(60,-35);(60,-20);(60,-20)"
%	 stroke-width= "0.75"
%	 />
%<ellipse p3= "(56.21,-31.21)"
%	 fill-style= "solid"
%	 p2= "(56.21,-38.79)"
%	 fill-color= "#330033"
%	 p1= "(63.79,-38.79)"
%	 closure= "open"
%	 angle-end= "0"
%	 angle-start= "0"
%	 />
%<ellipse p3= "(86.21,-31.21)"
%	 fill-style= "solid"
%	 p2= "(86.21,-38.79)"
%	 fill-color= "#330033"
%	 p1= "(93.79,-38.79)"
%	 closure= "open"
%	 angle-end= "0"
%	 angle-start= "0"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(56.25,-26.25)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\AAh$
%</text>
%</jpic>
%%End JPIC-XML
%PSTricks content-type (pstricks.sty package needed)
%Add \usepackage{pstricks} in the preamble of your LaTeX file
%You can rescale the whole picture (to 80% for instance) by using the command \def\JPicScale{0.8}
\ifx\JPicScale\undefined\def\JPicScale{1}\fi
\psset{unit=\JPicScale mm}
\psset{linewidth=0.3,dotsep=1,hatchwidth=0.3,hatchsep=1.5,shadowsize=1,dimen=middle}
\psset{dotsize=0.7 2.5,dotscale=1 1,fillcolor=black}
\psset{arrowsize=1 2,arrowlength=1,arrowinset=0.25,tbarsize=0.7 5,bracketlength=0.15,rbracketlength=0.15}
\begin{pspicture}(0,0)(100,40)
\psline[linewidth=0.75](60,10)(75,25)
\psline[linewidth=0.75](75,25)(75,40)
\newrgbcolor{userFillColour}{0.2 0 0.2}
\rput{0}(75,25){\psellipse[fillcolor=userFillColour,fillstyle=solid](0,0)(3.79,-3.79)}
\psline[linewidth=0.6](90,0)(90,10)
\psline[linewidth=0.75](90,10)(75,25)
\psline[linewidth=0.6](60,-0)(60,10)
\rput[r](86.25,-26.25){$\AAh$}
\rput[l](78.75,40){$\BBh$}
\psline[linewidth=0.75](90,-35)(90,-20)
\pspolygon[linewidth=0.7,fillcolor=white,fillstyle=solid](100,-20)(80,-20)(80,-0)(100,0)
\rput(90,-10){$\aah$}
\pspolygon[linewidth=0.7,fillcolor=white,fillstyle=solid](70,-20)(50,-20)(50,-0)(70,-0)
\rput(60,-10){$\aah$}
\psline[linewidth=0.75](60,-35)(60,-20)
\newrgbcolor{userFillColour}{0.2 0 0.2}
\rput{0}(60,-35){\psellipse[fillcolor=userFillColour,fillstyle=solid](0,0)(3.79,-3.79)}
\newrgbcolor{userFillColour}{0.2 0 0.2}
\rput{0}(90,-35){\psellipse[fillcolor=userFillColour,fillstyle=solid](0,0)(3.79,-3.79)}
\rput[r](56.25,-26.25){$\AAh$}
\end{pspicture}


==> PIC/fun-consistent.tex <==
%%Created by jPicEdt 1.4.1_03: mixed JPIC-XML/LaTeX format
%%Thu Dec 17 07:15:27 GMT-10:00 2020
%%Begin JPIC-XML
%<?xml version="1.0" standalone="yes"?>
%<jpic x-min="-10" x-max="22.5" y-min="-35" y-max="38.75" auto-bounding="true">
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(2.5,-35)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\AAh$
%</text>
%<multicurve fill-style= "none"
%	 points= "(5,-25);(5,-25);(5,-35);(5,-35)"
%	 stroke-width= "0.75"
%	 />
%<parallelogram p3= "(15,-25)"
%	 fill-style= "solid"
%	 p2= "(15,-5)"
%	 fill-color= "#ffffff"
%	 p1= "(-5,-5)"
%	 stroke-width= "0.7"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(5,-15)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\aah$
%</text>
%<multicurve fill-style= "none"
%	 points= "(20,20);(20,20);(5,5);(5,5)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(5,5);(5,5);(5,-5);(5,-5)"
%	 stroke-width= "0.75"
%	 />
%<ellipse p3= "(8.79,1.21)"
%	 fill-style= "solid"
%	 p2= "(8.79,8.79)"
%	 fill-color= "#330033"
%	 p1= "(1.21,8.79)"
%	 closure= "open"
%	 angle-end= "0"
%	 angle-start= "0"
%	 />
%<multicurve fill-style= "none"
%	 points= "(-10,38.75);(-10,38.75);(-10,20);(-10,20)"
%	 stroke-width= "0.6"
%	 />
%<multicurve fill-style= "none"
%	 points= "(-10,20);(-10,20);(5,5);(5,5)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(20,38.75);(20,38.75);(20,20);(20,20)"
%	 stroke-width= "0.6"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(22.5,37.5)"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\BBh$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(-7.5,37.5)"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\BBh$
%</text>
%</jpic>
%%End JPIC-XML
%PSTricks content-type (pstricks.sty package needed)
%Add \usepackage{pstricks} in the preamble of your LaTeX file
%You can rescale the whole picture (to 80% for instance) by using the command \def\JPicScale{0.8}
\ifx\JPicScale\undefined\def\JPicScale{1}\fi
\psset{unit=\JPicScale mm}
\psset{linewidth=0.3,dotsep=1,hatchwidth=0.3,hatchsep=1.5,shadowsize=1,dimen=middle}
\psset{dotsize=0.7 2.5,dotscale=1 1,fillcolor=black}
\psset{arrowsize=1 2,arrowlength=1,arrowinset=0.25,tbarsize=0.7 5,bracketlength=0.15,rbracketlength=0.15}
\begin{pspicture}(0,0)(22.5,38.75)
\rput[r](2.5,-35){$\AAh$}
\psline[linewidth=0.75](5,-25)(5,-35)
\pspolygon[linewidth=0.7,fillcolor=white,fillstyle=solid](-5,-5)(15,-5)(15,-25)(-5,-25)
\rput(5,-15){$\aah$}
\psline[linewidth=0.75](20,20)(5,5)
\psline[linewidth=0.75](5,5)(5,-5)
\newrgbcolor{userFillColour}{0.2 0 0.2}
\rput{0}(5,5){\psellipse[fillcolor=userFillColour,fillstyle=solid](0,0)(3.79,-3.79)}
\psline[linewidth=0.6](-10,38.75)(-10,20)
\psline[linewidth=0.75](-10,20)(5,5)
\psline[linewidth=0.6](20,38.75)(20,20)
\rput[l](22.5,37.5){$\BBh$}
\rput[l](-7.5,37.5){$\BBh$}
\end{pspicture}


==> PIC/fun-left.tex <==
%%Created by jPicEdt 1.4.1_03: mixed JPIC-XML/LaTeX format
%%Thu Aug 30 10:29:57 GMT-10:00 2018
%%Begin JPIC-XML
%<?xml version="1.0" standalone="yes"?>
%<jpic x-min="-1.87" x-max="1.87" y-min="-4.38" y-max="11.56" auto-bounding="true">
%<ellipse p3= "(1.56,8.43)"
%	 p2= "(1.56,11.56)"
%	 fill-style= "solid"
%	 p1= "(-1.56,11.56)"
%	 closure= "open"
%	 angle-end= "0"
%	 angle-start= "0"
%	 />
%<multicurve fill-style= "none"
%	 points= "(0,5.62);(0,5.62);(0,3.75);(0,3.75);(0,3.75);(0,5);
%	(0,5);(0,5);(0,8.75);(0,8.75)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(0,-3.76);(0,-3.76);(0,-4.38);(0,-4.38);(0,-4.38);(0,-4.38);
%	(0,-4.38);(0,-4.38);(0,0);(0,0)"
%	 />
%<parallelogram p3= "(1.87,0)"
%	 p2= "(1.87,3.75)"
%	 fill-style= "none"
%	 p1= "(-1.87,3.75)"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(0,1.87)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\fun$
%</text>
%</jpic>
%%End JPIC-XML
%PSTricks content-type (pstricks.sty package needed)
%Add \usepackage{pstricks} in the preamble of your LaTeX file
%You can rescale the whole picture (to 80% for instance) by using the command \def\JPicScale{0.8}
\ifx\JPicScale\undefined\def\JPicScale{1}\fi
\psset{unit=\JPicScale mm}
\psset{linewidth=0.3,dotsep=1,hatchwidth=0.3,hatchsep=1.5,shadowsize=1,dimen=middle}
\psset{dotsize=0.7 2.5,dotscale=1 1,fillcolor=black}
\psset{arrowsize=1 2,arrowlength=1,arrowinset=0.25,tbarsize=0.7 5,bracketlength=0.15,rbracketlength=0.15}
\begin{pspicture}(0,0)(1.87,11.56)
\rput{90}(0,10){\psellipse[fillstyle=solid](0,0)(1.57,-1.56)}
\psline(0,5.62)
(0,3.75)
(0,5)(0,8.75)
\pscustom[]{\psline(0,-3.76)(0,-4.38)
\psbezier(0,-4.38)(0,-4.38)(0,-4.38)
\psline(0,-4.38)(0,0)
}
\pspolygon[](-1.87,3.75)(1.87,3.75)(1.87,0)(-1.87,0)
\rput(0,1.87){$\fun$}
\end{pspicture}


==> PIC/fun-right.tex <==
%%Created by jPicEdt 1.4.1_03: mixed JPIC-XML/LaTeX format
%%Thu Aug 30 10:30:45 GMT-10:00 2018
%%Begin JPIC-XML
%<?xml version="1.0" standalone="yes"?>
%<jpic x-min="-1.56" x-max="1.56" y-min="-4.38" y-max="11.56" auto-bounding="true">
%<ellipse p3= "(1.56,8.43)"
%	 p2= "(1.56,11.56)"
%	 fill-style= "solid"
%	 p1= "(-1.56,11.56)"
%	 closure= "open"
%	 angle-end= "0"
%	 angle-start= "0"
%	 />
%<multicurve fill-style= "none"
%	 points= "(0,5.62);(0,5.62);(0,-4.38);(0,-4.38);(0,-4.38);(0,5);
%	(0,5);(0,5);(0,8.75);(0,8.75)"
%	 />
%</jpic>
%%End JPIC-XML
%PSTricks content-type (pstricks.sty package needed)
%Add \usepackage{pstricks} in the preamble of your LaTeX file
%You can rescale the whole picture (to 80% for instance) by using the command \def\JPicScale{0.8}
\ifx\JPicScale\undefined\def\JPicScale{1}\fi
\psset{unit=\JPicScale mm}
\psset{linewidth=0.3,dotsep=1,hatchwidth=0.3,hatchsep=1.5,shadowsize=1,dimen=middle}
\psset{dotsize=0.7 2.5,dotscale=1 1,fillcolor=black}
\psset{arrowsize=1 2,arrowlength=1,arrowinset=0.25,tbarsize=0.7 5,bracketlength=0.15,rbracketlength=0.15}
\begin{pspicture}(0,0)(1.56,11.56)
\rput{90}(0,10){\psellipse[fillstyle=solid](0,0)(1.57,-1.56)}
\psline(0,5.62)
(0,-4.38)
(0,5)(0,8.75)
\end{pspicture}


==> PIC/fun-strict.tex <==
%%Created by jPicEdt 1.4.1_03: mixed JPIC-XML/LaTeX format
%%Sun Dec 13 12:03:40 GMT-10:00 2020
%%Begin JPIC-XML
%<?xml version="1.0" standalone="yes"?>
%<jpic x-min="0" x-max="20" y-min="0" y-max="40" auto-bounding="true">
%<multicurve fill-style= "none"
%	 points= "(0,30);(0,30);(20,30);(20,30)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(0,30);(0,30);(0,10);(0,10)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(20,10);(20,10);(20,30);(20,30)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(10,40);(10,40);(10,25);(10,25)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(0,10);(0,10);(20,10);(20,10)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(10,15);(10,15);(10,0);(10,0)"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(10,20)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\see$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(11.25,38.75)"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\Beh$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(8.75,0)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\Aah$
%</text>
%</jpic>
%%End JPIC-XML
%PSTricks content-type (pstricks.sty package needed)
%Add \usepackage{pstricks} in the preamble of your LaTeX file
%You can rescale the whole picture (to 80% for instance) by using the command \def\JPicScale{0.8}
\ifx\JPicScale\undefined\def\JPicScale{1}\fi
\psset{unit=\JPicScale mm}
\psset{linewidth=0.3,dotsep=1,hatchwidth=0.3,hatchsep=1.5,shadowsize=1,dimen=middle}
\psset{dotsize=0.7 2.5,dotscale=1 1,fillcolor=black}
\psset{arrowsize=1 2,arrowlength=1,arrowinset=0.25,tbarsize=0.7 5,bracketlength=0.15,rbracketlength=0.15}
\begin{pspicture}(0,0)(20,40)
\psline(0,30)(20,30)
\psline(0,30)(0,10)
\psline(20,10)(20,30)
\psline(10,40)(10,25)
\psline(0,10)(20,10)
\psline(10,15)(10,0)
\rput(10,20){$\see$}
\rput[l](11.25,38.75){$\Beh$}
\rput[r](8.75,0){$\Aah$}
\end{pspicture}


==> PIC/fun.tex <==
%%Created by jPicEdt 1.4.1_03: mixed JPIC-XML/LaTeX format
%%Sat Sep 02 21:38:10 HST 2017
%%Begin JPIC-XML
%<?xml version="1.0" standalone="yes"?>
%<jpic x-min="0" x-max="20" y-min="-20" y-max="20" auto-bounding="true">
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(0,7.5);(0,7.5);(20,7.5);(20,7.5)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(0,7.5);(0,7.5);(0,-7.5);(0,-7.5)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(20,-7.5);(20,-7.5);(20,7.5);(20,7.5)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(10,20);(10,20);(10,7.5);(10,7.5)"
%	 />
%<text stroke-width= "0.75"
%	 text-vert-align= "center-v"
%	 anchor-point= "(7.5,17.5)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\nameslang$
%</text>
%<text stroke-width= "0.75"
%	 text-vert-align= "center-v"
%	 anchor-point= "(7.5,-17.5)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\inputt$
%</text>
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(0,-7.5);(0,-7.5);(20,-7.5);(20,-7.5)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(10,-7.5);(10,-7.5);(10,-20);(10,-20)"
%	 />
%<text stroke-width= "0.75"
%	 text-vert-align= "center-v"
%	 anchor-point= "(10,0)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\machine
%</text>
%</jpic>
%%End JPIC-XML
%PSTricks content-type (pstricks.sty package needed)
%Add \usepackage{pstricks} in the preamble of your LaTeX file
%You can rescale the whole picture (to 80% for instance) by using the command \def\JPicScale{0.8}
\ifx\JPicScale\undefined\def\JPicScale{1}\fi
\psset{unit=\JPicScale mm}
\psset{linewidth=0.3,dotsep=1,hatchwidth=0.3,hatchsep=1.5,shadowsize=1,dimen=middle}
\psset{dotsize=0.7 2.5,dotscale=1 1,fillcolor=black}
\psset{arrowsize=1 2,arrowlength=1,arrowinset=0.25,tbarsize=0.7 5,bracketlength=0.15,rbracketlength=0.15}
\begin{pspicture}(0,0)(20,20)
\psline[linewidth=0.75](0,7.5)(20,7.5)
\psline[linewidth=0.75](0,7.5)(0,-7.5)
\psline[linewidth=0.75](20,-7.5)(20,7.5)
\psline[linewidth=0.75](10,20)(10,7.5)
\rput[r](7.5,17.5){$\nameslang$}
\rput[r](7.5,-17.5){$\inputt$}
\psline[linewidth=0.75](0,-7.5)(20,-7.5)
\psline[linewidth=0.75](10,-7.5)(10,-20)
\rput(10,0){\machine}
\end{pspicture}


==> PIC/functor.tex <==
%%Created by jPicEdt 1.4.1_03: mixed JPIC-XML/LaTeX format
%%Sat Jan 02 00:15:29 GMT-10:00 2021
%%Begin JPIC-XML
%<?xml version="1.0" standalone="yes"?>
%<jpic x-min="0" x-max="145" y-min="0" y-max="152.5" auto-bounding="true">
%<multicurve fill-style= "none"
%	 points= "(0,80);(0,80);(0,60);(0,60)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(20,80);(20,80);(20,60);(20,60)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(10,90);(10,90);(10,80);(10,80)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(10,60);(10,60);(10,50);(10,50)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(0,80);(0,80);(20,80);(20,80)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(0,60);(0,60);(20,60);(20,60)"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(10,70)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\eef$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(7.5,50)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\Aah$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(12.5,90)"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\Beh$
%</text>
%<multicurve fill-style= "none"
%	 points= "(90,80);(90,80);(90,60);(90,60)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(110,80);(110,80);(110,60);(110,60)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(100,90);(100,90);(100,80);(100,80)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(100,60);(100,60);(100,50);(100,50)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(90,80);(90,80);(110,80);(110,80)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(90,60);(90,60);(110,60);(110,60)"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(100,70)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\eef$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(97.5,50)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\Aah$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(102.5,90)"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\Beh$
%</text>
%<multicurve fill-style= "none"
%	 points= "(120,80);(120,80);(120,60);(120,60)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(140,80);(140,80);(140,60);(140,60)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(130,90);(130,90);(130,80);(130,80)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(130,60);(130,60);(130,50);(130,50)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(120,80);(120,80);(140,80);(140,80)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(120,60);(120,60);(140,60);(140,60)"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(130,70)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\eef$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(127.5,50)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\Aah$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(132.5,90)"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\Beh$
%</text>
%<multicurve fill-style= "none"
%	 points= "(67.5,30);(67.5,30);(67.5,10);(67.5,10)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(87.5,30);(87.5,30);(87.5,10);(87.5,10)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(77.5,40);(77.5,40);(77.5,30);(77.5,30)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(77.5,10);(77.5,10);(77.5,0);(77.5,0)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(67.5,30);(67.5,30);(87.5,30);(87.5,30)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(67.5,10);(67.5,10);(87.5,10);(87.5,10)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(75,142.5);(75,142.5);(75,122.5);(75,122.5)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(95,142.5);(95,142.5);(95,122.5);(95,122.5)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(85,152.5);(85,152.5);(85,142.5);(85,142.5)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(85,122.5);(85,122.5);(85,112.5);(85,112.5)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(75,142.5);(75,142.5);(95,142.5);(95,142.5)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(75,122.5);(75,122.5);(95,122.5);(95,122.5)"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(85,132.5)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\eef$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(82.5,112.5)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\Aah$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(87.5,152.5)"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\Beh$
%</text>
%<multicurve fill-style= "none"
%	 points= "(65,152.5);(65,152.5);(65,112.5);(65,112.5)"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 arrow-head-inset-scale= "0"
%	 anchor-point= "(62.5,112.5)"
%	 text-frame= "noframe"
%	 stroke-width= "0.95"
%	 text-hor-align= "right"
%	 right-arrow= "head"
%	 >
%$\Eeh$
%</text>
%<multicurve fill-style= "none"
%	 points= "(60,147.5);(60,147.5);(100,147.5);(100,147.5)"
%	 stroke-width= "0.15"
%	 />
%<multicurve fill-style= "none"
%	 points= "(60,117.5);(60,117.5);(100,117.5);(100,117.5)"
%	 stroke-width= "0.15"
%	 />
%<multicurve fill-style= "none"
%	 points= "(60,147.5);(60,147.5);(60,117.5);(60,117.5)"
%	 stroke-width= "0.15"
%	 />
%<multicurve fill-style= "none"
%	 points= "(100,147.5);(100,147.5);(100,117.5);(100,117.5)"
%	 stroke-width= "0.15"
%	 />
%<multicurve fill-style= "none"
%	 points= "(35,70);(35,70);(75,70);(75,70)"
%	 stroke-width= "0.5"
%	 />
%<multicurve fill-style= "none"
%	 points= "(35,67.5);(35,67.5);(35,72.5);(35,72.5)"
%	 stroke-width= "0.5"
%	 />
%<multicurve fill-style= "none"
%	 points= "(75,70);(75,70);(70,72.5);(70,72.5)"
%	 stroke-width= "0.5"
%	 />
%<multicurve fill-style= "none"
%	 points= "(75,70);(75,70);(70,67.5);(70,67.5)"
%	 stroke-width= "0.5"
%	 />
%<multicurve fill-style= "none"
%	 points= "(85,85);(85,85);(145,85);(145,85)"
%	 stroke-width= "0.15"
%	 />
%<multicurve fill-style= "none"
%	 points= "(85,55);(85,55);(145,55);(145,55)"
%	 stroke-width= "0.15"
%	 />
%<multicurve fill-style= "none"
%	 points= "(85,85);(85,85);(85,55);(85,55)"
%	 stroke-width= "0.15"
%	 />
%<multicurve fill-style= "none"
%	 points= "(145,85);(145,85);(145,55);(145,55)"
%	 stroke-width= "0.15"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 arrow-head-inset-scale= "0"
%	 anchor-point= "(77.5,20)"
%	 text-frame= "noframe"
%	 stroke-width= "0.95"
%	 text-hor-align= "center-h"
%	 right-arrow= "head"
%	 >
%$\Teef$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 arrow-head-inset-scale= "0"
%	 anchor-point= "(80,40)"
%	 text-frame= "noframe"
%	 stroke-width= "0.95"
%	 text-hor-align= "left"
%	 right-arrow= "head"
%	 >
%$\TBeh$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 arrow-head-inset-scale= "0"
%	 anchor-point= "(75,0)"
%	 text-frame= "noframe"
%	 stroke-width= "0.95"
%	 text-hor-align= "right"
%	 right-arrow= "head"
%	 >
%$\TAah$
%</text>
%<multicurve fill-style= "none"
%	 points= "(32.5,77.5);(32.5,77.5);(60.78,105.78);(60.78,105.78)"
%	 stroke-width= "0.6"
%	 />
%<multicurve fill-style= "none"
%	 points= "(34.27,75.73);(34.27,75.73);(30.73,79.27);(30.73,79.27)"
%	 stroke-width= "0.6"
%	 />
%<multicurve fill-style= "none"
%	 points= "(60.78,105.78);(60.78,105.78);(55.48,104.02);(55.48,104.02)"
%	 stroke-width= "0.6"
%	 />
%<multicurve fill-style= "none"
%	 points= "(60.78,105.78);(60.78,105.78);(59.02,100.48);(59.02,100.48)"
%	 stroke-width= "0.6"
%	 />
%<multicurve fill-style= "none"
%	 points= "(32.5,62.5);(32.5,62.5);(60.78,34.22);(60.78,34.22)"
%	 stroke-width= "0.6"
%	 />
%<multicurve fill-style= "none"
%	 points= "(30.73,60.73);(30.73,60.73);(34.27,64.27);(34.27,64.27)"
%	 stroke-width= "0.6"
%	 />
%<multicurve fill-style= "none"
%	 points= "(60.78,34.22);(60.78,34.22);(59.02,39.52);(59.02,39.52)"
%	 stroke-width= "0.6"
%	 />
%<multicurve fill-style= "none"
%	 points= "(60.78,34.22);(60.78,34.22);(55.48,35.98);(55.48,35.98)"
%	 stroke-width= "0.6"
%	 />
%<text text-vert-align= "bottom"
%	 fill-style= "none"
%	 arrow-head-inset-scale= "0"
%	 anchor-point= "(45,92.5)"
%	 text-rotation= "45"
%	 text-frame= "noframe"
%	 stroke-width= "0.95"
%	 text-hor-align= "right"
%	 right-arrow= "head"
%	 >
%$\Toone$
%</text>
%<text text-vert-align= "bottom"
%	 fill-style= "none"
%	 arrow-head-inset-scale= "0"
%	 anchor-point= "(55,72.5)"
%	 text-frame= "noframe"
%	 stroke-width= "0.95"
%	 text-hor-align= "center-h"
%	 right-arrow= "head"
%	 >
%$\Ttwo$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 arrow-head-inset-scale= "0"
%	 anchor-point= "(45,47.5)"
%	 text-rotation= "-45"
%	 text-frame= "noframe"
%	 stroke-width= "0.95"
%	 text-hor-align= "right"
%	 right-arrow= "head"
%	 >
%$\Tthree$
%</text>
%</jpic>
%%End JPIC-XML
%LaTeX-picture environment using emulated lines and arcs
%You can rescale the whole picture (to 80% for instance) by using the command \def\JPicScale{0.8}
\ifx\JPicScale\undefined\def\JPicScale{1}\fi
\unitlength \JPicScale mm
\begin{picture}(145,152.5)(0,0)
\linethickness{0.3mm}
\put(0,60){\line(0,1){20}}
\linethickness{0.3mm}
\put(20,60){\line(0,1){20}}
\linethickness{0.3mm}
\put(10,80){\line(0,1){10}}
\linethickness{0.3mm}
\put(10,50){\line(0,1){10}}
\linethickness{0.3mm}
\put(0,80){\line(1,0){20}}
\linethickness{0.3mm}
\put(0,60){\line(1,0){20}}
\put(10,70){\makebox(0,0)[cc]{$\eef$}}

\put(7.5,50){\makebox(0,0)[cr]{$\Aah$}}

\put(12.5,90){\makebox(0,0)[cl]{$\Beh$}}

\linethickness{0.3mm}
\put(90,60){\line(0,1){20}}
\linethickness{0.3mm}
\put(110,60){\line(0,1){20}}
\linethickness{0.3mm}
\put(100,80){\line(0,1){10}}
\linethickness{0.3mm}
\put(100,50){\line(0,1){10}}
\linethickness{0.3mm}
\put(90,80){\line(1,0){20}}
\linethickness{0.3mm}
\put(90,60){\line(1,0){20}}
\put(100,70){\makebox(0,0)[cc]{$\eef$}}

\put(97.5,50){\makebox(0,0)[cr]{$\Aah$}}

\put(102.5,90){\makebox(0,0)[cl]{$\Beh$}}

\linethickness{0.3mm}
\put(120,60){\line(0,1){20}}
\linethickness{0.3mm}
\put(140,60){\line(0,1){20}}
\linethickness{0.3mm}
\put(130,80){\line(0,1){10}}
\linethickness{0.3mm}
\put(130,50){\line(0,1){10}}
\linethickness{0.3mm}
\put(120,80){\line(1,0){20}}
\linethickness{0.3mm}
\put(120,60){\line(1,0){20}}
\put(130,70){\makebox(0,0)[cc]{$\eef$}}

\put(127.5,50){\makebox(0,0)[cr]{$\Aah$}}

\put(132.5,90){\makebox(0,0)[cl]{$\Beh$}}

\linethickness{0.3mm}
\put(67.5,10){\line(0,1){20}}
\linethickness{0.3mm}
\put(87.5,10){\line(0,1){20}}
\linethickness{0.3mm}
\put(77.5,30){\line(0,1){10}}
\linethickness{0.3mm}
\put(77.5,0){\line(0,1){10}}
\linethickness{0.3mm}
\put(67.5,30){\line(1,0){20}}
\linethickness{0.3mm}
\put(67.5,10){\line(1,0){20}}
\linethickness{0.3mm}
\put(75,122.5){\line(0,1){20}}
\linethickness{0.3mm}
\put(95,122.5){\line(0,1){20}}
\linethickness{0.3mm}
\put(85,142.5){\line(0,1){10}}
\linethickness{0.3mm}
\put(85,112.5){\line(0,1){10}}
\linethickness{0.3mm}
\put(75,142.5){\line(1,0){20}}
\linethickness{0.3mm}
\put(75,122.5){\line(1,0){20}}
\put(85,132.5){\makebox(0,0)[cc]{$\eef$}}

\put(82.5,112.5){\makebox(0,0)[cr]{$\Aah$}}

\put(87.5,152.5){\makebox(0,0)[cl]{$\Beh$}}

\linethickness{0.3mm}
\put(65,112.5){\line(0,1){40}}
\put(62.5,112.5){\makebox(0,0)[cr]{$\Eeh$}}

\linethickness{0.15mm}
\put(60,147.5){\line(1,0){40}}
\linethickness{0.15mm}
\put(60,117.5){\line(1,0){40}}
\linethickness{0.15mm}
\put(60,117.5){\line(0,1){30}}
\linethickness{0.15mm}
\put(100,117.5){\line(0,1){30}}
\linethickness{0.5mm}
\put(35,70){\line(1,0){40}}
\linethickness{0.5mm}
\put(35,67.5){\line(0,1){5}}
\linethickness{0.5mm}
\multiput(70,72.5)(0.24,-0.12){21}{\line(1,0){0.24}}
\linethickness{0.5mm}
\multiput(70,67.5)(0.24,0.12){21}{\line(1,0){0.24}}
\linethickness{0.15mm}
\put(85,85){\line(1,0){60}}
\linethickness{0.15mm}
\put(85,55){\line(1,0){60}}
\linethickness{0.15mm}
\put(85,55){\line(0,1){30}}
\linethickness{0.15mm}
\put(145,55){\line(0,1){30}}
\put(77.5,20){\makebox(0,0)[cc]{$\Teef$}}

\put(80,40){\makebox(0,0)[cl]{$\TBeh$}}

\put(75,0){\makebox(0,0)[cr]{$\TAah$}}

\linethickness{0.6mm}
\multiput(32.5,77.5)(0.12,0.12){236}{\line(1,0){0.12}}
\linethickness{0.6mm}
\multiput(30.73,79.27)(0.12,-0.12){29}{\line(1,0){0.12}}
\linethickness{0.6mm}
\multiput(55.48,104.02)(0.35,0.12){15}{\line(1,0){0.35}}
\linethickness{0.6mm}
\multiput(59.02,100.48)(0.12,0.35){15}{\line(0,1){0.35}}
\linethickness{0.6mm}
\multiput(32.5,62.5)(0.12,-0.12){236}{\line(1,0){0.12}}
\linethickness{0.6mm}
\multiput(30.73,60.73)(0.12,0.12){29}{\line(0,1){0.12}}
\linethickness{0.6mm}
\multiput(59.02,39.52)(0.12,-0.35){15}{\line(0,-1){0.35}}
\linethickness{0.6mm}
\multiput(55.48,35.98)(0.35,-0.12){15}{\line(1,0){0.35}}
\put(45,92.5){\makebox(0,0)[br]{$\Toone$}}

\put(55,72.5){\makebox(0,0)[bc]{$\Ttwo$}}

\put(45,47.5){\makebox(0,0)[cr]{$\Tthree$}}

\end{picture}


==> PIC/futamura-0.tex <==
%%Created by jPicEdt 1.4.1_03: mixed JPIC-XML/LaTeX format
%%Wed Nov 23 19:43:06 HST 2016
%%Begin JPIC-XML
%<?xml version="1.0" standalone="yes"?>
%<jpic x-min="0" x-max="125" y-min="0" y-max="245" auto-bounding="true">
%<multicurve stroke-width= "0.95"
%	 points= "(80,230);(80,230);(125,230);(125,230)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.95"
%	 points= "(125,210);(125,210);(125,230);(125,230)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.95"
%	 points= "(115,245);(115,245);(115,230);(115,230)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.95"
%	 points= "(100,210);(100,210);(125,210);(125,210)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.95"
%	 points= "(115,210);(115,210);(115,0);(115,0)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.95"
%	 points= "(80,230);(80,230);(100,210);(100,210)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.95"
%	 points= "(55,200);(55,200);(100,200);(100,200)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.95"
%	 points= "(55,67.5);(55,67.5);(55,47.5);(55,47.5)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.95"
%	 points= "(100,180);(100,180);(100,200);(100,200)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.95"
%	 points= "(90,220);(90,220);(90,200);(90,200)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.95"
%	 points= "(75,180);(75,180);(100,180);(100,180)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.95"
%	 points= "(90,180);(90,180);(90,0);(90,0)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.95"
%	 points= "(55,47.5);(55,47.5);(75,47.5);(75,47.5)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.95"
%	 points= "(55,67.5);(55,67.5);(75,47.5);(75,47.5)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.95"
%	 points= "(65,190);(65,190);(65,170);(65,170)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.95"
%	 points= "(55,200);(55,200);(75,180);(75,180)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.95"
%	 points= "(20,100);(20,100);(20,80);(20,80)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.95"
%	 points= "(20,80);(20,80);(40,80);(40,80)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.95"
%	 points= "(20,100);(20,100);(40,80);(40,80)"
%	 fill-style= "none"
%	 />
%<text text-vert-align= "center-v"
%	 anchor-point= "(60,52.5)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\itag$
%</text>
%<multicurve stroke-width= "0.95"
%	 points= "(30,170);(30,170);(75,170);(75,170)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.95"
%	 points= "(75,150);(75,150);(75,170);(75,170)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.95"
%	 points= "(50,150);(50,150);(75,150);(75,150)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.95"
%	 points= "(65,150);(65,150);(65,57.5);(65,57.5)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.95"
%	 points= "(40,160);(40,160);(40,130);(40,130)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.95"
%	 points= "(30,170);(30,170);(50,150);(50,150)"
%	 fill-style= "none"
%	 />
%<text text-vert-align= "center-v"
%	 anchor-point= "(62.5,75)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\Lprogtype$
%</text>
%<multicurve stroke-width= "0.95"
%	 points= "(10,140);(10,140);(30,140);(30,140)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.95"
%	 points= "(50,120);(50,120);(30,140);(30,140)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.95"
%	 points= "(30,120);(30,120);(50,120);(50,120)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.95"
%	 points= "(40,120);(40,120);(40,110);(40,110)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.95"
%	 points= "(20,130);(20,130);(20,110);(20,110)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.95"
%	 points= "(10,140);(10,140);(30,120);(30,120)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.95"
%	 points= "(40,110);(40,110);(30,100);(30,100)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.95"
%	 points= "(20,110);(20,110);(30,100);(30,100)"
%	 fill-style= "none"
%	 />
%<ellipse p3= "(32.57,97.42)"
%	 p2= "(32.57,102.58)"
%	 p1= "(27.43,102.58)"
%	 closure= "open"
%	 angle-end= "0"
%	 fill-style= "solid"
%	 angle-start= "0"
%	 fill-color= "#330033"
%	 />
%<multicurve stroke-width= "0.95"
%	 points= "(30,100);(30,100);(30,90);(30,90)"
%	 fill-style= "none"
%	 />
%<text text-vert-align= "center-v"
%	 anchor-point= "(62.5,182.5)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\Lprogtype$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(86.25,210)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\Lprogtype$
%</text>
%<multicurve points= "(7.5,145);(7.5,145);(52.5,145);(52.5,145)"
%	 fill-style= "none"
%	 />
%<multicurve points= "(7.5,145);(7.5,145);(7.5,80);(7.5,80)"
%	 fill-style= "none"
%	 />
%<multicurve points= "(52.5,145);(52.5,145);(52.5,80);(52.5,80)"
%	 fill-style= "none"
%	 />
%<multicurve points= "(7.5,80);(7.5,80);(30,57.5);(30,57.5)"
%	 fill-style= "none"
%	 />
%<multicurve points= "(52.5,80);(52.5,80);(30,57.5);(30,57.5)"
%	 fill-style= "none"
%	 />
%<multicurve points= "(0,175);(0,175);(0,45);(0,45)"
%	 fill-style= "none"
%	 />
%<multicurve points= "(80,175);(80,175);(80,45);(80,45)"
%	 fill-style= "none"
%	 />
%<multicurve points= "(0,45);(0,45);(40,5);(40,5)"
%	 fill-style= "none"
%	 />
%<multicurve points= "(80,45);(80,45);(40,5);(40,5)"
%	 fill-style= "none"
%	 />
%<multicurve points= "(0,175);(0,175);(80,175);(80,175)"
%	 fill-style= "none"
%	 />
%<text text-vert-align= "center-v"
%	 anchor-point= "(115,220)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\ltag$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(40,15)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\Cprog$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(30,67.5)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\Gprog$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(25,85)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\Sprog$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(30,130)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\stag$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(90,190)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\ltag$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(65,160)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\ltag$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(87.5,5)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\Hprogtype$
%</text>
%</jpic>
%%End JPIC-XML
%PSTricks content-type (pstricks.sty package needed)
%Add \usepackage{pstricks} in the preamble of your LaTeX file
%You can rescale the whole picture (to 80% for instance) by using the command \def\JPicScale{0.8}
\ifx\JPicScale\undefined\def\JPicScale{1}\fi
\psset{unit=\JPicScale mm}
\psset{linewidth=0.3,dotsep=1,hatchwidth=0.3,hatchsep=1.5,shadowsize=1,dimen=middle}
\psset{dotsize=0.7 2.5,dotscale=1 1,fillcolor=black}
\psset{arrowsize=1 2,arrowlength=1,arrowinset=0.25,tbarsize=0.7 5,bracketlength=0.15,rbracketlength=0.15}
\begin{pspicture}(0,0)(125,245)
\psline[linewidth=0.95](80,230)(125,230)
\psline[linewidth=0.95](125,210)(125,230)
\psline[linewidth=0.95](115,245)(115,230)
\psline[linewidth=0.95](100,210)(125,210)
\psline[linewidth=0.95](115,210)(115,0)
\psline[linewidth=0.95](80,230)(100,210)
\psline[linewidth=0.95](55,200)(100,200)
\psline[linewidth=0.95](55,67.5)(55,47.5)
\psline[linewidth=0.95](100,180)(100,200)
\psline[linewidth=0.95](90,220)(90,200)
\psline[linewidth=0.95](75,180)(100,180)
\psline[linewidth=0.95](90,180)(90,0)
\psline[linewidth=0.95](55,47.5)(75,47.5)
\psline[linewidth=0.95](55,67.5)(75,47.5)
\psline[linewidth=0.95](65,190)(65,170)
\psline[linewidth=0.95](55,200)(75,180)
\psline[linewidth=0.95](20,100)(20,80)
\psline[linewidth=0.95](20,80)(40,80)
\psline[linewidth=0.95](20,100)(40,80)
\rput(60,52.5){$\itag$}
\psline[linewidth=0.95](30,170)(75,170)
\psline[linewidth=0.95](75,150)(75,170)
\psline[linewidth=0.95](50,150)(75,150)
\psline[linewidth=0.95](65,150)(65,57.5)
\psline[linewidth=0.95](40,160)(40,130)
\psline[linewidth=0.95](30,170)(50,150)
\rput[r](62.5,75){$\Lprogtype$}
\psline[linewidth=0.95](10,140)(30,140)
\psline[linewidth=0.95](50,120)(30,140)
\psline[linewidth=0.95](30,120)(50,120)
\psline[linewidth=0.95](40,120)(40,110)
\psline[linewidth=0.95](20,130)(20,110)
\psline[linewidth=0.95](10,140)(30,120)
\psline[linewidth=0.95](40,110)(30,100)
\psline[linewidth=0.95](20,110)(30,100)
\newrgbcolor{userFillColour}{0.2 0 0.2}
\rput{90}(30,100){\psellipse[fillcolor=userFillColour,fillstyle=solid](0,0)(2.58,-2.57)}
\psline[linewidth=0.95](30,100)(30,90)
\rput[r](62.5,182.5){$\Lprogtype$}
\rput[r](86.25,210){$\Lprogtype$}
\psline(7.5,145)(52.5,145)
\psline(7.5,145)(7.5,80)
\psline(52.5,145)(52.5,80)
\psline(7.5,80)(30,57.5)
\psline(52.5,80)(30,57.5)
\psline(0,175)(0,45)
\psline(80,175)(80,45)
\psline(0,45)(40,5)
\psline(80,45)(40,5)
\psline(0,175)(80,175)
\rput(115,220){$\ltag$}
\rput(40,15){$\Cprog$}
\rput(30,67.5){$\Gprog$}
\rput(25,85){$\Sprog$}
\rput(30,130){$\stag$}
\rput(90,190){$\ltag$}
\rput(65,160){$\ltag$}
\rput[r](87.5,5){$\Hprogtype$}
\end{pspicture}


==> PIC/futamura-1.tex <==
%%Created by jPicEdt 1.4.1_03: mixed JPIC-XML/LaTeX format
%%Tue Nov 29 09:19:46 HST 2016
%%Begin JPIC-XML
%<?xml version="1.0" standalone="yes"?>
%<jpic x-min="0" x-max="125" y-min="0" y-max="245" auto-bounding="true">
%<multicurve stroke-width= "0.95"
%	 points= "(80,230);(80,230);(125,230);(125,230)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.95"
%	 points= "(125,210);(125,210);(125,230);(125,230)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.95"
%	 points= "(115,245);(115,245);(115,230);(115,230)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.95"
%	 points= "(100,210);(100,210);(125,210);(125,210)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.95"
%	 points= "(115,210);(115,210);(115,0);(115,0)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.95"
%	 points= "(80,230);(80,230);(100,210);(100,210)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.95"
%	 points= "(55,200);(55,200);(100,200);(100,200)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.95"
%	 points= "(55,67.5);(55,67.5);(55,47.5);(55,47.5)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.95"
%	 points= "(100,180);(100,180);(100,200);(100,200)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.95"
%	 points= "(90,220);(90,220);(90,200);(90,200)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.95"
%	 points= "(75,180);(75,180);(100,180);(100,180)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.95"
%	 points= "(90,180);(90,180);(90,0);(90,0)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.95"
%	 points= "(55,47.5);(55,47.5);(75,47.5);(75,47.5)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.95"
%	 points= "(55,67.5);(55,67.5);(75,47.5);(75,47.5)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.95"
%	 points= "(65,190);(65,190);(65,170);(65,170)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.95"
%	 points= "(55,200);(55,200);(75,180);(75,180)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.95"
%	 points= "(10,120);(10,120);(10,100);(10,100)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.95"
%	 points= "(10,100);(10,100);(30,100);(30,100)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.95"
%	 points= "(10,120);(10,120);(30,100);(30,100)"
%	 fill-style= "none"
%	 />
%<text text-vert-align= "center-v"
%	 anchor-point= "(60,52.5)"
%	 text-frame= "noframe"
%	 fill-style= "none"
%	 text-hor-align= "center-h"
%	 >
%$\itag$
%</text>
%<multicurve stroke-width= "0.95"
%	 points= "(30,170);(30,170);(75,170);(75,170)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.95"
%	 points= "(75,150);(75,150);(75,170);(75,170)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.95"
%	 points= "(50,150);(50,150);(75,150);(75,150)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.95"
%	 points= "(65,150);(65,150);(65,57.5);(65,57.5)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.95"
%	 points= "(40,160);(40,160);(40,130);(40,130)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.95"
%	 points= "(30,170);(30,170);(50,150);(50,150)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.95"
%	 points= "(10,140);(10,140);(30,140);(30,140)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.95"
%	 points= "(50,120);(50,120);(30,140);(30,140)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.95"
%	 points= "(30,120);(30,120);(50,120);(50,120)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.95"
%	 points= "(40,120);(40,120);(40,83.75);(40,83.75)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.95"
%	 points= "(20,130);(20,130);(20,110);(20,110)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.95"
%	 points= "(10,140);(10,140);(30,120);(30,120)"
%	 fill-style= "none"
%	 />
%<text text-vert-align= "center-v"
%	 anchor-point= "(62.5,182.5)"
%	 text-frame= "noframe"
%	 fill-style= "none"
%	 text-hor-align= "right"
%	 >
%$\Lprogtype$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(86.25,210)"
%	 text-frame= "noframe"
%	 fill-style= "none"
%	 text-hor-align= "right"
%	 >
%$\Lprogtype$
%</text>
%<multicurve points= "(5,175);(5,175);(5,45);(5,45)"
%	 fill-style= "none"
%	 />
%<multicurve points= "(80,175);(80,175);(80,45);(80,45)"
%	 fill-style= "none"
%	 />
%<multicurve points= "(5,45);(5,45);(42.5,7.5);(42.5,7.5)"
%	 fill-style= "none"
%	 />
%<multicurve points= "(80,45);(80,45);(42.5,7.5);(42.5,7.5)"
%	 fill-style= "none"
%	 />
%<multicurve points= "(5,175);(5,175);(80,175);(80,175)"
%	 fill-style= "none"
%	 />
%<text text-vert-align= "center-v"
%	 anchor-point= "(115,220)"
%	 text-frame= "noframe"
%	 fill-style= "none"
%	 text-hor-align= "center-h"
%	 >
%$\ltag$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(42.5,16.25)"
%	 text-frame= "noframe"
%	 fill-style= "none"
%	 text-hor-align= "center-h"
%	 >
%$\Cprog$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(15,105)"
%	 text-frame= "noframe"
%	 fill-style= "none"
%	 text-hor-align= "center-h"
%	 >
%$\Sprog$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(30,130)"
%	 text-frame= "noframe"
%	 fill-style= "none"
%	 text-hor-align= "center-h"
%	 >
%$\stag$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(90,190)"
%	 text-frame= "noframe"
%	 fill-style= "none"
%	 text-hor-align= "center-h"
%	 >
%$\ltag$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(65,160)"
%	 text-frame= "noframe"
%	 fill-style= "none"
%	 text-hor-align= "center-h"
%	 >
%$\ltag$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(87.5,5)"
%	 text-frame= "noframe"
%	 fill-style= "none"
%	 text-hor-align= "right"
%	 >
%$\Hprogtype$
%</text>
%<multicurve stroke-width= "0.95"
%	 points= "(30,93.75);(30,93.75);(30,73.75);(30,73.75)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.95"
%	 points= "(30,73.75);(30,73.75);(50,73.75);(50,73.75)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.95"
%	 points= "(30,93.75);(30,93.75);(50,73.75);(50,73.75)"
%	 fill-style= "none"
%	 />
%<text text-vert-align= "center-v"
%	 anchor-point= "(35,78.75)"
%	 text-frame= "noframe"
%	 fill-style= "none"
%	 text-hor-align= "center-h"
%	 >
%$\Sprog$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(0,220)"
%	 text-frame= "noframe"
%	 fill-style= "none"
%	 text-hor-align= "center-h"
%	 >
%\nothing
%</text>
%</jpic>
%%End JPIC-XML
%PSTricks content-type (pstricks.sty package needed)
%Add \usepackage{pstricks} in the preamble of your LaTeX file
%You can rescale the whole picture (to 80% for instance) by using the command \def\JPicScale{0.8}
\ifx\JPicScale\undefined\def\JPicScale{1}\fi
\psset{unit=\JPicScale mm}
\psset{linewidth=0.3,dotsep=1,hatchwidth=0.3,hatchsep=1.5,shadowsize=1,dimen=middle}
\psset{dotsize=0.7 2.5,dotscale=1 1,fillcolor=black}
\psset{arrowsize=1 2,arrowlength=1,arrowinset=0.25,tbarsize=0.7 5,bracketlength=0.15,rbracketlength=0.15}
\begin{pspicture}(0,0)(125,245)
\psline[linewidth=0.95](80,230)(125,230)
\psline[linewidth=0.95](125,210)(125,230)
\psline[linewidth=0.95](115,245)(115,230)
\psline[linewidth=0.95](100,210)(125,210)
\psline[linewidth=0.95](115,210)(115,0)
\psline[linewidth=0.95](80,230)(100,210)
\psline[linewidth=0.95](55,200)(100,200)
\psline[linewidth=0.95](55,67.5)(55,47.5)
\psline[linewidth=0.95](100,180)(100,200)
\psline[linewidth=0.95](90,220)(90,200)
\psline[linewidth=0.95](75,180)(100,180)
\psline[linewidth=0.95](90,180)(90,0)
\psline[linewidth=0.95](55,47.5)(75,47.5)
\psline[linewidth=0.95](55,67.5)(75,47.5)
\psline[linewidth=0.95](65,190)(65,170)
\psline[linewidth=0.95](55,200)(75,180)
\psline[linewidth=0.95](10,120)(10,100)
\psline[linewidth=0.95](10,100)(30,100)
\psline[linewidth=0.95](10,120)(30,100)
\rput(60,52.5){$\itag$}
\psline[linewidth=0.95](30,170)(75,170)
\psline[linewidth=0.95](75,150)(75,170)
\psline[linewidth=0.95](50,150)(75,150)
\psline[linewidth=0.95](65,150)(65,57.5)
\psline[linewidth=0.95](40,160)(40,130)
\psline[linewidth=0.95](30,170)(50,150)
\psline[linewidth=0.95](10,140)(30,140)
\psline[linewidth=0.95](50,120)(30,140)
\psline[linewidth=0.95](30,120)(50,120)
\psline[linewidth=0.95](40,120)(40,83.75)
\psline[linewidth=0.95](20,130)(20,110)
\psline[linewidth=0.95](10,140)(30,120)
\rput[r](62.5,182.5){$\Lprogtype$}
\rput[r](86.25,210){$\Lprogtype$}
\psline(5,175)(5,45)
\psline(80,175)(80,45)
\psline(5,45)(42.5,7.5)
\psline(80,45)(42.5,7.5)
\psline(5,175)(80,175)
\rput(115,220){$\ltag$}
\rput(42.5,16.25){$\Cprog$}
\rput(15,105){$\Sprog$}
\rput(30,130){$\stag$}
\rput(90,190){$\ltag$}
\rput(65,160){$\ltag$}
\rput[r](87.5,5){$\Hprogtype$}
\psline[linewidth=0.95](30,93.75)(30,73.75)
\psline[linewidth=0.95](30,73.75)(50,73.75)
\psline[linewidth=0.95](30,93.75)(50,73.75)
\rput(35,78.75){$\Sprog$}
\rput(0,220){\nothing}
\end{pspicture}


==> PIC/futamura-1A.tex <==
%%Created by jPicEdt 1.4.1_03: mixed JPIC-XML/LaTeX format
%%Tue Nov 29 09:18:41 HST 2016
%%Begin JPIC-XML
%<?xml version="1.0" standalone="yes"?>
%<jpic x-min="0" x-max="125" y-min="0" y-max="245" auto-bounding="true">
%<multicurve stroke-width= "0.95"
%	 points= "(80,230);(80,230);(125,230);(125,230)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.95"
%	 points= "(125,210);(125,210);(125,230);(125,230)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.95"
%	 points= "(115,245);(115,245);(115,230);(115,230)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.95"
%	 points= "(100,210);(100,210);(125,210);(125,210)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.95"
%	 points= "(115,210);(115,210);(115,27.5);(115,27.5)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.95"
%	 points= "(80,230);(80,230);(100,210);(100,210)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.95"
%	 points= "(55,200);(55,200);(100,200);(100,200)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.95"
%	 points= "(55,97.5);(55,97.5);(55,77.5);(55,77.5)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.95"
%	 points= "(100,180);(100,180);(100,200);(100,200)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.95"
%	 points= "(90,220);(90,220);(90,200);(90,200)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.95"
%	 points= "(75,180);(75,180);(100,180);(100,180)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.95"
%	 points= "(90,180);(90,180);(90,27.5);(90,27.5)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.95"
%	 points= "(55,77.5);(55,77.5);(75,77.5);(75,77.5)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.95"
%	 points= "(55,97.5);(55,97.5);(75,77.5);(75,77.5)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.95"
%	 points= "(65,190);(65,190);(65,170);(65,170)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.95"
%	 points= "(55,200);(55,200);(75,180);(75,180)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.95"
%	 points= "(10,150);(10,150);(10,130);(10,130)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.95"
%	 points= "(10,130);(10,130);(30,130);(30,130)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.95"
%	 points= "(10,150);(10,150);(30,130);(30,130)"
%	 fill-style= "none"
%	 />
%<text text-vert-align= "center-v"
%	 anchor-point= "(60,82.5)"
%	 text-frame= "noframe"
%	 fill-style= "none"
%	 text-hor-align= "center-h"
%	 >
%$\itag$
%</text>
%<multicurve stroke-width= "0.95"
%	 points= "(10,170);(10,170);(75,170);(75,170)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.95"
%	 points= "(75,150);(75,150);(75,170);(75,170)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.95"
%	 points= "(30,150);(30,150);(75,150);(75,150)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.95"
%	 points= "(65,150);(65,150);(65,87.5);(65,87.5)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.95"
%	 points= "(40,150);(40,150);(40,115);(40,115)"
%	 fill-style= "none"
%	 />
%<text text-vert-align= "center-v"
%	 anchor-point= "(62.5,102.5)"
%	 text-frame= "noframe"
%	 fill-style= "none"
%	 text-hor-align= "right"
%	 >
%$\Lprogtype$
%</text>
%<multicurve stroke-width= "0.95"
%	 points= "(20,160);(20,160);(20,140);(20,140)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.95"
%	 points= "(10,170);(10,170);(30,150);(30,150)"
%	 fill-style= "none"
%	 />
%<text text-vert-align= "center-v"
%	 anchor-point= "(62.5,182.5)"
%	 text-frame= "noframe"
%	 fill-style= "none"
%	 text-hor-align= "right"
%	 >
%$\Lprogtype$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(86.25,210)"
%	 text-frame= "noframe"
%	 fill-style= "none"
%	 text-hor-align= "right"
%	 >
%$\Lprogtype$
%</text>
%<multicurve points= "(5,175);(5,175);(5,77.5);(5,77.5)"
%	 fill-style= "none"
%	 />
%<multicurve points= "(80,175);(80,175);(80,77.5);(80,77.5)"
%	 fill-style= "none"
%	 />
%<multicurve points= "(5,77.5);(5,77.5);(42.5,40);(42.5,40)"
%	 fill-style= "none"
%	 />
%<multicurve points= "(80,77.5);(80,77.5);(42.5,40);(42.5,40)"
%	 fill-style= "none"
%	 />
%<multicurve points= "(5,175);(5,175);(80,175);(80,175)"
%	 fill-style= "none"
%	 />
%<text text-vert-align= "center-v"
%	 anchor-point= "(115,220)"
%	 text-frame= "noframe"
%	 fill-style= "none"
%	 text-hor-align= "center-h"
%	 >
%$\ltag$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(42.5,50)"
%	 text-frame= "noframe"
%	 fill-style= "none"
%	 text-hor-align= "center-h"
%	 >
%$\Cprog$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(15,135)"
%	 text-frame= "noframe"
%	 fill-style= "none"
%	 text-hor-align= "center-h"
%	 >
%$\Sprog$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(90,190)"
%	 text-frame= "noframe"
%	 fill-style= "none"
%	 text-hor-align= "center-h"
%	 >
%$\ltag$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(65,160)"
%	 text-frame= "noframe"
%	 fill-style= "none"
%	 text-hor-align= "center-h"
%	 >
%$\ltag$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(87.5,37.5)"
%	 text-frame= "noframe"
%	 fill-style= "none"
%	 text-hor-align= "right"
%	 >
%$\Hprogtype$
%</text>
%<multicurve stroke-width= "0.95"
%	 points= "(30,125);(30,125);(30,105);(30,105)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.95"
%	 points= "(30,105);(30,105);(50,105);(50,105)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.95"
%	 points= "(30,125);(30,125);(50,105);(50,105)"
%	 fill-style= "none"
%	 />
%<text text-vert-align= "center-v"
%	 anchor-point= "(35,110)"
%	 text-frame= "noframe"
%	 fill-style= "none"
%	 text-hor-align= "center-h"
%	 >
%$\Sprog$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(0,220)"
%	 text-frame= "noframe"
%	 fill-style= "none"
%	 text-hor-align= "center-h"
%	 >
%\nothing
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(40,0)"
%	 text-frame= "noframe"
%	 fill-style= "none"
%	 text-hor-align= "center-h"
%	 >
%\nothing
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(37.5,127.5)"
%	 text-frame= "noframe"
%	 fill-style= "none"
%	 text-hor-align= "right"
%	 >
%$\Lprogtype$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(17.5,155)"
%	 text-frame= "noframe"
%	 fill-style= "none"
%	 text-hor-align= "right"
%	 >
%$\Lprogtype$
%</text>
%</jpic>
%%End JPIC-XML
%PSTricks content-type (pstricks.sty package needed)
%Add \usepackage{pstricks} in the preamble of your LaTeX file
%You can rescale the whole picture (to 80% for instance) by using the command \def\JPicScale{0.8}
\ifx\JPicScale\undefined\def\JPicScale{1}\fi
\psset{unit=\JPicScale mm}
\psset{linewidth=0.3,dotsep=1,hatchwidth=0.3,hatchsep=1.5,shadowsize=1,dimen=middle}
\psset{dotsize=0.7 2.5,dotscale=1 1,fillcolor=black}
\psset{arrowsize=1 2,arrowlength=1,arrowinset=0.25,tbarsize=0.7 5,bracketlength=0.15,rbracketlength=0.15}
\begin{pspicture}(0,0)(125,245)
\psline[linewidth=0.95](80,230)(125,230)
\psline[linewidth=0.95](125,210)(125,230)
\psline[linewidth=0.95](115,245)(115,230)
\psline[linewidth=0.95](100,210)(125,210)
\psline[linewidth=0.95](115,210)(115,27.5)
\psline[linewidth=0.95](80,230)(100,210)
\psline[linewidth=0.95](55,200)(100,200)
\psline[linewidth=0.95](55,97.5)(55,77.5)
\psline[linewidth=0.95](100,180)(100,200)
\psline[linewidth=0.95](90,220)(90,200)
\psline[linewidth=0.95](75,180)(100,180)
\psline[linewidth=0.95](90,180)(90,27.5)
\psline[linewidth=0.95](55,77.5)(75,77.5)
\psline[linewidth=0.95](55,97.5)(75,77.5)
\psline[linewidth=0.95](65,190)(65,170)
\psline[linewidth=0.95](55,200)(75,180)
\psline[linewidth=0.95](10,150)(10,130)
\psline[linewidth=0.95](10,130)(30,130)
\psline[linewidth=0.95](10,150)(30,130)
\rput(60,82.5){$\itag$}
\psline[linewidth=0.95](10,170)(75,170)
\psline[linewidth=0.95](75,150)(75,170)
\psline[linewidth=0.95](30,150)(75,150)
\psline[linewidth=0.95](65,150)(65,87.5)
\psline[linewidth=0.95](40,150)(40,115)
\rput[r](62.5,102.5){$\Lprogtype$}
\psline[linewidth=0.95](20,160)(20,140)
\psline[linewidth=0.95](10,170)(30,150)
\rput[r](62.5,182.5){$\Lprogtype$}
\rput[r](86.25,210){$\Lprogtype$}
\psline(5,175)(5,77.5)
\psline(80,175)(80,77.5)
\psline(5,77.5)(42.5,40)
\psline(80,77.5)(42.5,40)
\psline(5,175)(80,175)
\rput(115,220){$\ltag$}
\rput(42.5,50){$\Cprog$}
\rput(15,135){$\Sprog$}
\rput(90,190){$\ltag$}
\rput(65,160){$\ltag$}
\rput[r](87.5,37.5){$\Hprogtype$}
\psline[linewidth=0.95](30,125)(30,105)
\psline[linewidth=0.95](30,105)(50,105)
\psline[linewidth=0.95](30,125)(50,105)
\rput(35,110){$\Sprog$}
\rput(0,220){\nothing}
\rput(40,0){\nothing}
\rput[r](37.5,127.5){$\Lprogtype$}
\rput[r](17.5,155){$\Lprogtype$}
\end{pspicture}


==> PIC/futamura-2.tex <==
%%Created by jPicEdt 1.4.1_03: mixed JPIC-XML/LaTeX format
%%Tue Nov 29 09:07:16 HST 2016
%%Begin JPIC-XML
%<?xml version="1.0" standalone="yes"?>
%<jpic x-min="0" x-max="125" y-min="0" y-max="245" auto-bounding="true">
%<multicurve stroke-width= "0.95"
%	 points= "(80,230);(80,230);(125,230);(125,230)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.95"
%	 points= "(125,210);(125,210);(125,230);(125,230)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.95"
%	 points= "(115,245);(115,245);(115,230);(115,230)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.95"
%	 points= "(100,210);(100,210);(125,210);(125,210)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.95"
%	 points= "(115,210);(115,210);(115,60);(115,60)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.95"
%	 points= "(80,230);(80,230);(100,210);(100,210)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.95"
%	 points= "(55,200);(55,200);(100,200);(100,200)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.95"
%	 points= "(55,120);(55,120);(55,100);(55,100)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.95"
%	 points= "(100,180);(100,180);(100,200);(100,200)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.95"
%	 points= "(90,220);(90,220);(90,200);(90,200)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.95"
%	 points= "(75,180);(75,180);(100,180);(100,180)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.95"
%	 points= "(90,180);(90,180);(90,60);(90,60)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.95"
%	 points= "(55,100);(55,100);(75,100);(75,100)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.95"
%	 points= "(55,120);(55,120);(75,100);(75,100)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.95"
%	 points= "(65,190);(65,190);(65,160);(65,160)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.95"
%	 points= "(55,200);(55,200);(75,180);(75,180)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.95"
%	 points= "(30,150);(30,150);(30,130);(30,130)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.95"
%	 points= "(30,130);(30,130);(50,130);(50,130)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.95"
%	 points= "(30,150);(30,150);(50,130);(50,130)"
%	 fill-style= "none"
%	 />
%<text text-vert-align= "center-v"
%	 anchor-point= "(60,105)"
%	 text-frame= "noframe"
%	 fill-style= "none"
%	 text-hor-align= "center-h"
%	 >
%$\itag$
%</text>
%<multicurve stroke-width= "0.95"
%	 points= "(65,150);(65,150);(65,110);(65,110)"
%	 fill-style= "none"
%	 />
%<text text-vert-align= "center-v"
%	 anchor-point= "(62.5,125)"
%	 text-frame= "noframe"
%	 fill-style= "none"
%	 text-hor-align= "right"
%	 >
%$\Lprogtype$
%</text>
%<multicurve stroke-width= "0.95"
%	 points= "(30,170);(30,170);(55,170);(55,170)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.95"
%	 points= "(75,150);(75,150);(55,170);(55,170)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.95"
%	 points= "(50,150);(50,150);(75,150);(75,150)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.95"
%	 points= "(40,160);(40,160);(40,140);(40,140)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.95"
%	 points= "(30,170);(30,170);(50,150);(50,150)"
%	 fill-style= "none"
%	 />
%<text text-vert-align= "center-v"
%	 anchor-point= "(62.5,182.5)"
%	 text-frame= "noframe"
%	 fill-style= "none"
%	 text-hor-align= "right"
%	 >
%$\Lprogtype$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(86.25,210)"
%	 text-frame= "noframe"
%	 fill-style= "none"
%	 text-hor-align= "right"
%	 >
%$\Lprogtype$
%</text>
%<multicurve points= "(25,175);(25,175);(25,100);(25,100)"
%	 fill-style= "none"
%	 />
%<multicurve points= "(80,175);(80,175);(80,100);(80,100)"
%	 fill-style= "none"
%	 />
%<multicurve points= "(25,100);(25,100);(52.5,72.5);(52.5,72.5)"
%	 fill-style= "none"
%	 />
%<multicurve points= "(80,100);(80,100);(52.5,72.5);(52.5,72.5)"
%	 fill-style= "none"
%	 />
%<multicurve points= "(25,175);(25,175);(80,175);(80,175)"
%	 fill-style= "none"
%	 />
%<text text-vert-align= "center-v"
%	 anchor-point= "(115,220)"
%	 text-frame= "noframe"
%	 fill-style= "none"
%	 text-hor-align= "center-h"
%	 >
%$\ltag$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(52.5,83.75)"
%	 text-frame= "noframe"
%	 fill-style= "none"
%	 text-hor-align= "center-h"
%	 >
%$\Cprog$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(35,135)"
%	 text-frame= "noframe"
%	 fill-style= "none"
%	 text-hor-align= "center-h"
%	 >
%$\Sprog$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(52.5,160)"
%	 text-frame= "noframe"
%	 fill-style= "none"
%	 text-hor-align= "center-h"
%	 >
%$\stag$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(90,190)"
%	 text-frame= "noframe"
%	 fill-style= "none"
%	 text-hor-align= "center-h"
%	 >
%$\ltag$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(87.5,70)"
%	 text-frame= "noframe"
%	 fill-style= "none"
%	 text-hor-align= "right"
%	 >
%$\Hprogtype$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(60,0)"
%	 text-frame= "noframe"
%	 fill-style= "none"
%	 text-hor-align= "center-h"
%	 >
%\nothing
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(0,220)"
%	 text-frame= "noframe"
%	 fill-style= "none"
%	 text-hor-align= "center-h"
%	 >
%\nothing
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(37.5,155)"
%	 text-frame= "noframe"
%	 fill-style= "none"
%	 text-hor-align= "right"
%	 >
%$\Lprogtype$
%</text>
%</jpic>
%%End JPIC-XML
%PSTricks content-type (pstricks.sty package needed)
%Add \usepackage{pstricks} in the preamble of your LaTeX file
%You can rescale the whole picture (to 80% for instance) by using the command \def\JPicScale{0.8}
\ifx\JPicScale\undefined\def\JPicScale{1}\fi
\psset{unit=\JPicScale mm}
\psset{linewidth=0.3,dotsep=1,hatchwidth=0.3,hatchsep=1.5,shadowsize=1,dimen=middle}
\psset{dotsize=0.7 2.5,dotscale=1 1,fillcolor=black}
\psset{arrowsize=1 2,arrowlength=1,arrowinset=0.25,tbarsize=0.7 5,bracketlength=0.15,rbracketlength=0.15}
\begin{pspicture}(0,0)(125,245)
\psline[linewidth=0.95](80,230)(125,230)
\psline[linewidth=0.95](125,210)(125,230)
\psline[linewidth=0.95](115,245)(115,230)
\psline[linewidth=0.95](100,210)(125,210)
\psline[linewidth=0.95](115,210)(115,60)
\psline[linewidth=0.95](80,230)(100,210)
\psline[linewidth=0.95](55,200)(100,200)
\psline[linewidth=0.95](55,120)(55,100)
\psline[linewidth=0.95](100,180)(100,200)
\psline[linewidth=0.95](90,220)(90,200)
\psline[linewidth=0.95](75,180)(100,180)
\psline[linewidth=0.95](90,180)(90,60)
\psline[linewidth=0.95](55,100)(75,100)
\psline[linewidth=0.95](55,120)(75,100)
\psline[linewidth=0.95](65,190)(65,160)
\psline[linewidth=0.95](55,200)(75,180)
\psline[linewidth=0.95](30,150)(30,130)
\psline[linewidth=0.95](30,130)(50,130)
\psline[linewidth=0.95](30,150)(50,130)
\rput(60,105){$\itag$}
\psline[linewidth=0.95](65,150)(65,110)
\rput[r](62.5,125){$\Lprogtype$}
\psline[linewidth=0.95](30,170)(55,170)
\psline[linewidth=0.95](75,150)(55,170)
\psline[linewidth=0.95](50,150)(75,150)
\psline[linewidth=0.95](40,160)(40,140)
\psline[linewidth=0.95](30,170)(50,150)
\rput[r](62.5,182.5){$\Lprogtype$}
\rput[r](86.25,210){$\Lprogtype$}
\psline(25,175)(25,100)
\psline(80,175)(80,100)
\psline(25,100)(52.5,72.5)
\psline(80,100)(52.5,72.5)
\psline(25,175)(80,175)
\rput(115,220){$\ltag$}
\rput(52.5,83.75){$\Cprog$}
\rput(35,135){$\Sprog$}
\rput(52.5,160){$\stag$}
\rput(90,190){$\ltag$}
\rput[r](87.5,70){$\Hprogtype$}
\rput(60,0){\nothing}
\rput(0,220){\nothing}
\rput[r](37.5,155){$\Lprogtype$}
\end{pspicture}


==> PIC/futamura-3.tex <==
%%Created by jPicEdt 1.4.1_03: mixed JPIC-XML/LaTeX format
%%Tue Nov 29 09:06:08 HST 2016
%%Begin JPIC-XML
%<?xml version="1.0" standalone="yes"?>
%<jpic x-min="0" x-max="125" y-min="0" y-max="245" auto-bounding="true">
%<multicurve stroke-width= "0.95"
%	 points= "(80,230);(80,230);(125,230);(125,230)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.95"
%	 points= "(125,210);(125,210);(125,230);(125,230)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.95"
%	 points= "(115,245);(115,245);(115,230);(115,230)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.95"
%	 points= "(100,210);(100,210);(125,210);(125,210)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.95"
%	 points= "(115,210);(115,210);(115,100);(115,100)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.95"
%	 points= "(80,230);(80,230);(100,210);(100,210)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.95"
%	 points= "(30,200);(30,200);(100,200);(100,200)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.95"
%	 points= "(55,150);(55,150);(55,130);(55,130)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.95"
%	 points= "(100,180);(100,180);(100,200);(100,200)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.95"
%	 points= "(90,220);(90,220);(90,200);(90,200)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.95"
%	 points= "(50,180);(50,180);(100,180);(100,180)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.95"
%	 points= "(90,180);(90,180);(90,100);(90,100)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.95"
%	 points= "(55,130);(55,130);(75,130);(75,130)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.95"
%	 points= "(55,150);(55,150);(75,130);(75,130)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.95"
%	 points= "(30,180);(30,180);(30,160);(30,160)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.95"
%	 points= "(30,160);(30,160);(50,160);(50,160)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.95"
%	 points= "(30,180);(30,180);(50,160);(50,160)"
%	 fill-style= "none"
%	 />
%<text text-vert-align= "center-v"
%	 anchor-point= "(60,135)"
%	 text-frame= "noframe"
%	 fill-style= "none"
%	 text-hor-align= "center-h"
%	 >
%$\itag$
%</text>
%<multicurve stroke-width= "0.95"
%	 points= "(65,180);(65,180);(65,140);(65,140)"
%	 fill-style= "none"
%	 />
%<text text-vert-align= "center-v"
%	 anchor-point= "(62.5,155)"
%	 text-frame= "noframe"
%	 fill-style= "none"
%	 text-hor-align= "right"
%	 >
%$\Lprogtype$
%</text>
%<multicurve stroke-width= "0.95"
%	 points= "(40,190);(40,190);(40,170);(40,170)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.95"
%	 points= "(30,200);(30,200);(50,180);(50,180)"
%	 fill-style= "none"
%	 />
%<text text-vert-align= "center-v"
%	 anchor-point= "(86.25,210)"
%	 text-frame= "noframe"
%	 fill-style= "none"
%	 text-hor-align= "right"
%	 >
%$\Lprogtype$
%</text>
%<multicurve points= "(20,205);(20,205);(20,125);(20,125)"
%	 fill-style= "none"
%	 />
%<multicurve points= "(105,205);(105,205);(105,125);(105,125)"
%	 fill-style= "none"
%	 />
%<multicurve points= "(105,125);(105,125);(20,125);(20,125)"
%	 fill-style= "none"
%	 />
%<multicurve points= "(20,205);(20,205);(105,205);(105,205)"
%	 fill-style= "none"
%	 />
%<text text-vert-align= "center-v"
%	 anchor-point= "(115,220)"
%	 text-frame= "noframe"
%	 fill-style= "none"
%	 text-hor-align= "center-h"
%	 >
%$\ltag$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(100,130)"
%	 text-frame= "noframe"
%	 fill-style= "none"
%	 text-hor-align= "center-h"
%	 >
%$\Cprog$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(35,165)"
%	 text-frame= "noframe"
%	 fill-style= "none"
%	 text-hor-align= "center-h"
%	 >
%$\Sprog$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(90,190)"
%	 text-frame= "noframe"
%	 fill-style= "none"
%	 text-hor-align= "center-h"
%	 >
%$\ltag$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(87.5,110)"
%	 text-frame= "noframe"
%	 fill-style= "none"
%	 text-hor-align= "right"
%	 >
%$\Hprogtype$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(60,0)"
%	 text-frame= "noframe"
%	 fill-style= "none"
%	 text-hor-align= "center-h"
%	 >
%\nothing
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(0,205)"
%	 text-frame= "noframe"
%	 fill-style= "none"
%	 text-hor-align= "left"
%	 >
%\nothing
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(37.5,183.75)"
%	 text-frame= "noframe"
%	 fill-style= "none"
%	 text-hor-align= "right"
%	 >
%$\Lprogtype$
%</text>
%</jpic>
%%End JPIC-XML
%PSTricks content-type (pstricks.sty package needed)
%Add \usepackage{pstricks} in the preamble of your LaTeX file
%You can rescale the whole picture (to 80% for instance) by using the command \def\JPicScale{0.8}
\ifx\JPicScale\undefined\def\JPicScale{1}\fi
\psset{unit=\JPicScale mm}
\psset{linewidth=0.3,dotsep=1,hatchwidth=0.3,hatchsep=1.5,shadowsize=1,dimen=middle}
\psset{dotsize=0.7 2.5,dotscale=1 1,fillcolor=black}
\psset{arrowsize=1 2,arrowlength=1,arrowinset=0.25,tbarsize=0.7 5,bracketlength=0.15,rbracketlength=0.15}
\begin{pspicture}(0,0)(125,245)
\psline[linewidth=0.95](80,230)(125,230)
\psline[linewidth=0.95](125,210)(125,230)
\psline[linewidth=0.95](115,245)(115,230)
\psline[linewidth=0.95](100,210)(125,210)
\psline[linewidth=0.95](115,210)(115,100)
\psline[linewidth=0.95](80,230)(100,210)
\psline[linewidth=0.95](30,200)(100,200)
\psline[linewidth=0.95](55,150)(55,130)
\psline[linewidth=0.95](100,180)(100,200)
\psline[linewidth=0.95](90,220)(90,200)
\psline[linewidth=0.95](50,180)(100,180)
\psline[linewidth=0.95](90,180)(90,100)
\psline[linewidth=0.95](55,130)(75,130)
\psline[linewidth=0.95](55,150)(75,130)
\psline[linewidth=0.95](30,180)(30,160)
\psline[linewidth=0.95](30,160)(50,160)
\psline[linewidth=0.95](30,180)(50,160)
\rput(60,135){$\itag$}
\psline[linewidth=0.95](65,180)(65,140)
\rput[r](62.5,155){$\Lprogtype$}
\psline[linewidth=0.95](40,190)(40,170)
\psline[linewidth=0.95](30,200)(50,180)
\rput[r](86.25,210){$\Lprogtype$}
\psline(20,205)(20,125)
\psline(105,205)(105,125)
\psline(105,125)(20,125)
\psline(20,205)(105,205)
\rput(115,220){$\ltag$}
\rput(100,130){$\Cprog$}
\rput(35,165){$\Sprog$}
\rput(90,190){$\ltag$}
\rput[r](87.5,110){$\Hprogtype$}
\rput(60,0){\nothing}
\rput[l](0,205){\nothing}
\rput[r](37.5,183.75){$\Lprogtype$}
\end{pspicture}


==> PIC/futamura-4.tex <==
%%Created by jPicEdt 1.4.1_03: mixed JPIC-XML/LaTeX format
%%Wed Nov 23 18:41:38 HST 2016
%%Begin JPIC-XML
%<?xml version="1.0" standalone="yes"?>
%<jpic x-min="0" x-max="125" y-min="0" y-max="245" auto-bounding="true">
%<multicurve stroke-width= "0.95"
%	 points= "(80,230);(80,230);(125,230);(125,230)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.95"
%	 points= "(125,210);(125,210);(125,230);(125,230)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.95"
%	 points= "(115,245);(115,245);(115,230);(115,230)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.95"
%	 points= "(100,210);(100,210);(125,210);(125,210)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.95"
%	 points= "(115,210);(115,210);(115,130);(115,130)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.95"
%	 points= "(80,230);(80,230);(100,210);(100,210)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.95"
%	 points= "(55,180);(55,180);(55,160);(55,160)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.95"
%	 points= "(90,220);(90,220);(90,190);(90,190)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.95"
%	 points= "(90,180);(90,180);(90,130);(90,130)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.95"
%	 points= "(55,160);(55,160);(75,160);(75,160)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.95"
%	 points= "(55,180);(55,180);(75,160);(75,160)"
%	 fill-style= "none"
%	 />
%<text text-vert-align= "center-v"
%	 anchor-point= "(60,165)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\itag$
%</text>
%<multicurve stroke-width= "0.95"
%	 points= "(65,190);(65,190);(65,170);(65,170)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.95"
%	 points= "(55,200);(55,200);(80,200);(80,200)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.95"
%	 points= "(100,180);(100,180);(80,200);(80,200)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.95"
%	 points= "(75,180);(75,180);(100,180);(100,180)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.95"
%	 points= "(55,200);(55,200);(75,180);(75,180)"
%	 fill-style= "none"
%	 />
%<text text-vert-align= "center-v"
%	 anchor-point= "(62.5,185)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\Lprogtype$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(86.25,210)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\Lprogtype$
%</text>
%<multicurve points= "(50,203.75);(50,203.75);(50,155);(50,155)"
%	 fill-style= "none"
%	 />
%<multicurve points= "(105,203.75);(105,203.75);(105,155);(105,155)"
%	 fill-style= "none"
%	 />
%<multicurve points= "(50,155);(50,155);(105,155);(105,155)"
%	 fill-style= "none"
%	 />
%<multicurve points= "(50,203.75);(50,203.75);(105,203.75);(105,203.75)"
%	 fill-style= "none"
%	 />
%<text text-vert-align= "center-v"
%	 anchor-point= "(115,220)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\ltag$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(100,160)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\Cprog$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(77.5,190)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\stag$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(87.5,140)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\Hprogtype$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(0,210)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%\nothing
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(40,0)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\nothing
%</text>
%</jpic>
%%End JPIC-XML
%PSTricks content-type (pstricks.sty package needed)
%Add \usepackage{pstricks} in the preamble of your LaTeX file
%You can rescale the whole picture (to 80% for instance) by using the command \def\JPicScale{0.8}
\ifx\JPicScale\undefined\def\JPicScale{1}\fi
\psset{unit=\JPicScale mm}
\psset{linewidth=0.3,dotsep=1,hatchwidth=0.3,hatchsep=1.5,shadowsize=1,dimen=middle}
\psset{dotsize=0.7 2.5,dotscale=1 1,fillcolor=black}
\psset{arrowsize=1 2,arrowlength=1,arrowinset=0.25,tbarsize=0.7 5,bracketlength=0.15,rbracketlength=0.15}
\begin{pspicture}(0,0)(125,245)
\psline[linewidth=0.95](80,230)(125,230)
\psline[linewidth=0.95](125,210)(125,230)
\psline[linewidth=0.95](115,245)(115,230)
\psline[linewidth=0.95](100,210)(125,210)
\psline[linewidth=0.95](115,210)(115,130)
\psline[linewidth=0.95](80,230)(100,210)
\psline[linewidth=0.95](55,180)(55,160)
\psline[linewidth=0.95](90,220)(90,190)
\psline[linewidth=0.95](90,180)(90,130)
\psline[linewidth=0.95](55,160)(75,160)
\psline[linewidth=0.95](55,180)(75,160)
\rput(60,165){$\itag$}
\psline[linewidth=0.95](65,190)(65,170)
\psline[linewidth=0.95](55,200)(80,200)
\psline[linewidth=0.95](100,180)(80,200)
\psline[linewidth=0.95](75,180)(100,180)
\psline[linewidth=0.95](55,200)(75,180)
\rput[r](62.5,185){$\Lprogtype$}
\rput[r](86.25,210){$\Lprogtype$}
\psline(50,203.75)(50,155)
\psline(105,203.75)(105,155)
\psline(50,155)(105,155)
\psline(50,203.75)(105,203.75)
\rput(115,220){$\ltag$}
\rput(100,160){$\Cprog$}
\rput(77.5,190){$\stag$}
\rput[r](87.5,140){$\Hprogtype$}
\rput[l](0,210){\nothing}
\rput(40,0){\nothing}
\end{pspicture}


==> PIC/futamura-5.tex <==
%%Created by jPicEdt 1.4.1_03: mixed JPIC-XML/LaTeX format
%%Wed Nov 23 19:46:53 HST 2016
%%Begin JPIC-XML
%<?xml version="1.0" standalone="yes"?>
%<jpic x-min="0" x-max="125" y-min="0" y-max="245" auto-bounding="true">
%<multicurve stroke-width= "0.95"
%	 points= "(55,230);(55,230);(125,230);(125,230)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.95"
%	 points= "(125,210);(125,210);(125,230);(125,230)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.95"
%	 points= "(115,245);(115,245);(115,230);(115,230)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.95"
%	 points= "(75,210);(75,210);(125,210);(125,210)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.95"
%	 points= "(115,210);(115,210);(115,175);(115,175)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.95"
%	 points= "(55,210);(55,210);(55,190);(55,190)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.95"
%	 points= "(90,210);(90,210);(90,175);(90,175)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.95"
%	 points= "(55,190);(55,190);(75,190);(75,190)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.95"
%	 points= "(55,210);(55,210);(75,190);(75,190)"
%	 fill-style= "none"
%	 />
%<text text-vert-align= "center-v"
%	 anchor-point= "(60,195)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\itag$
%</text>
%<multicurve stroke-width= "0.95"
%	 points= "(65,220);(65,220);(65,200);(65,200)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.95"
%	 points= "(55,230);(55,230);(75,210);(75,210)"
%	 fill-style= "none"
%	 />
%<text text-vert-align= "center-v"
%	 anchor-point= "(62.5,213.75)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\Lprogtype$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(115,220)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\ltag$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(87.5,180)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\Hprogtype$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(0,210)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%\nothing
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(40,0)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\nothing
%</text>
%</jpic>
%%End JPIC-XML
%PSTricks content-type (pstricks.sty package needed)
%Add \usepackage{pstricks} in the preamble of your LaTeX file
%You can rescale the whole picture (to 80% for instance) by using the command \def\JPicScale{0.8}
\ifx\JPicScale\undefined\def\JPicScale{1}\fi
\psset{unit=\JPicScale mm}
\psset{linewidth=0.3,dotsep=1,hatchwidth=0.3,hatchsep=1.5,shadowsize=1,dimen=middle}
\psset{dotsize=0.7 2.5,dotscale=1 1,fillcolor=black}
\psset{arrowsize=1 2,arrowlength=1,arrowinset=0.25,tbarsize=0.7 5,bracketlength=0.15,rbracketlength=0.15}
\begin{pspicture}(0,0)(125,245)
\psline[linewidth=0.95](55,230)(125,230)
\psline[linewidth=0.95](125,210)(125,230)
\psline[linewidth=0.95](115,245)(115,230)
\psline[linewidth=0.95](75,210)(125,210)
\psline[linewidth=0.95](115,210)(115,175)
\psline[linewidth=0.95](55,210)(55,190)
\psline[linewidth=0.95](90,210)(90,175)
\psline[linewidth=0.95](55,190)(75,190)
\psline[linewidth=0.95](55,210)(75,190)
\rput(60,195){$\itag$}
\psline[linewidth=0.95](65,220)(65,200)
\psline[linewidth=0.95](55,230)(75,210)
\rput[r](62.5,213.75){$\Lprogtype$}
\rput(115,220){$\ltag$}
\rput[r](87.5,180){$\Hprogtype$}
\rput[l](0,210){\nothing}
\rput(40,0){\nothing}
\end{pspicture}


==> PIC/futamura-6.tex <==
%%Created by jPicEdt 1.4.1_03: mixed JPIC-XML/LaTeX format
%%Wed Nov 23 17:31:12 HST 2016
%%Begin JPIC-XML
%<?xml version="1.0" standalone="yes"?>
%<jpic x-min="0" x-max="125" y-min="0" y-max="245" auto-bounding="true">
%<multicurve stroke-width= "0.95"
%	 points= "(80,230);(80,230);(125,230);(125,230)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.95"
%	 points= "(125,210);(125,210);(125,230);(125,230)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.95"
%	 points= "(115,245);(115,245);(115,230);(115,230)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.95"
%	 points= "(100,210);(100,210);(125,210);(125,210)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.95"
%	 points= "(115,210);(115,210);(115,175);(115,175)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.95"
%	 points= "(90,220);(90,220);(90,175);(90,175)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.95"
%	 points= "(80,230);(80,230);(100,210);(100,210)"
%	 fill-style= "none"
%	 />
%<text text-vert-align= "center-v"
%	 anchor-point= "(115,220)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\ltag$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(87.5,180)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\Hprogtype$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(0,210)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%\nothing
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(40,0)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\nothing
%</text>
%</jpic>
%%End JPIC-XML
%PSTricks content-type (pstricks.sty package needed)
%Add \usepackage{pstricks} in the preamble of your LaTeX file
%You can rescale the whole picture (to 80% for instance) by using the command \def\JPicScale{0.8}
\ifx\JPicScale\undefined\def\JPicScale{1}\fi
\psset{unit=\JPicScale mm}
\psset{linewidth=0.3,dotsep=1,hatchwidth=0.3,hatchsep=1.5,shadowsize=1,dimen=middle}
\psset{dotsize=0.7 2.5,dotscale=1 1,fillcolor=black}
\psset{arrowsize=1 2,arrowlength=1,arrowinset=0.25,tbarsize=0.7 5,bracketlength=0.15,rbracketlength=0.15}
\begin{pspicture}(0,0)(125,245)
\psline[linewidth=0.95](80,230)(125,230)
\psline[linewidth=0.95](125,210)(125,230)
\psline[linewidth=0.95](115,245)(115,230)
\psline[linewidth=0.95](100,210)(125,210)
\psline[linewidth=0.95](115,210)(115,175)
\psline[linewidth=0.95](90,220)(90,175)
\psline[linewidth=0.95](80,230)(100,210)
\rput(115,220){$\ltag$}
\rput[r](87.5,180){$\Hprogtype$}
\rput[l](0,210){\nothing}
\rput(40,0){\nothing}
\end{pspicture}


==> PIC/futamura-exercise.tex <==
%%Created by jPicEdt 1.4.1_03: mixed JPIC-XML/LaTeX format
%%Fri Dec 08 00:09:44 HST 2017
%%Begin JPIC-XML
%<?xml version="1.0" standalone="yes"?>
%<jpic x-min="0" x-max="340" y-min="0" y-max="120" auto-bounding="true">
%<multicurve stroke-width= "0.95"
%	 points= "(40,20);(40,20);(40,0);(40,0)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.95"
%	 points= "(40,0);(40,0);(60,0);(60,0)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.95"
%	 points= "(40,20);(40,20);(60,0);(60,0)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.95"
%	 points= "(50,100);(50,100);(50,80);(50,80)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.95"
%	 points= "(10,20);(10,20);(10,0);(10,0)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.95"
%	 points= "(10,0);(10,0);(30,0);(30,0)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.95"
%	 points= "(10,20);(10,20);(30,0);(30,0)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.95"
%	 points= "(20,80);(20,80);(60,80);(60,80)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.95"
%	 points= "(60,60);(60,60);(60,80);(60,80)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.95"
%	 points= "(40,60);(40,60);(60,60);(60,60)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.95"
%	 points= "(50,60);(50,60);(50,10);(50,10)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.95"
%	 points= "(30,70);(30,70);(30,50);(30,50)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.95"
%	 points= "(20,80);(20,80);(40,60);(40,60)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.95"
%	 points= "(0,60);(0,60);(20,60);(20,60)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.95"
%	 points= "(40,40);(40,40);(20,60);(20,60)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.95"
%	 points= "(20,40);(20,40);(40,40);(40,40)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.95"
%	 points= "(30,40);(30,40);(30,30);(30,30)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.95"
%	 points= "(10,50);(10,50);(10,30);(10,30)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.95"
%	 points= "(0,60);(0,60);(20,40);(20,40)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.95"
%	 points= "(30,30);(30,30);(20,20);(20,20)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.95"
%	 points= "(10,30);(10,30);(20,20);(20,20)"
%	 fill-style= "none"
%	 />
%<ellipse p3= "(22.57,17.42)"
%	 p2= "(22.57,22.58)"
%	 p1= "(17.43,22.58)"
%	 closure= "open"
%	 fill-color= "#330033"
%	 angle-end= "0"
%	 fill-style= "solid"
%	 angle-start= "0"
%	 />
%<multicurve stroke-width= "0.95"
%	 points= "(20,20);(20,20);(20,10);(20,10)"
%	 fill-style= "none"
%	 />
%<text text-vert-align= "center-v"
%	 anchor-point= "(15,5)"
%	 text-frame= "noframe"
%	 fill-style= "none"
%	 text-hor-align= "center-h"
%	 >
%$\Sprog$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(20,50)"
%	 text-frame= "noframe"
%	 fill-style= "none"
%	 text-hor-align= "center-h"
%	 >
%$\stag$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(45,70)"
%	 text-frame= "noframe"
%	 fill-style= "none"
%	 text-hor-align= "center-h"
%	 >
%$\ltag$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(85,60)"
%	 text-frame= "noframe"
%	 fill-style= "none"
%	 text-hor-align= "center-h"
%	 >
%\EQLS
%</text>
%<multicurve stroke-width= "0.95"
%	 points= "(310,20);(310,20);(310,0);(310,0)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.95"
%	 points= "(310,0);(310,0);(330,0);(330,0)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.95"
%	 points= "(310,20);(310,20);(330,0);(330,0)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.95"
%	 points= "(330,100);(330,100);(330,50);(330,50)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.95"
%	 points= "(300,60);(300,60);(320,60);(320,60)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.95"
%	 points= "(340,40);(340,40);(320,60);(320,60)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.95"
%	 points= "(320,40);(320,40);(340,40);(340,40)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.95"
%	 points= "(330,40);(330,40);(330,30);(330,30)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.95"
%	 points= "(310,50);(310,50);(310,30);(310,30)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.95"
%	 points= "(300,60);(300,60);(320,40);(320,40)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.95"
%	 points= "(330,30);(330,30);(320,20);(320,20)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.95"
%	 points= "(310,30);(310,30);(320,20);(320,20)"
%	 fill-style= "none"
%	 />
%<ellipse p3= "(322.57,17.42)"
%	 p2= "(322.57,22.58)"
%	 p1= "(317.43,22.58)"
%	 closure= "open"
%	 fill-color= "#330033"
%	 angle-end= "0"
%	 fill-style= "solid"
%	 angle-start= "0"
%	 />
%<multicurve stroke-width= "0.95"
%	 points= "(320,20);(320,20);(320,10);(320,10)"
%	 fill-style= "none"
%	 />
%<text text-vert-align= "center-v"
%	 anchor-point= "(315,5)"
%	 text-frame= "noframe"
%	 fill-style= "none"
%	 text-hor-align= "center-h"
%	 >
%$\Sprog$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(320,50)"
%	 text-frame= "noframe"
%	 fill-style= "none"
%	 text-hor-align= "center-h"
%	 >
%$\stag$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(46.25,5)"
%	 text-frame= "noframe"
%	 fill-style= "none"
%	 text-hor-align= "center-h"
%	 >
%$\Sprog$
%</text>
%<multicurve stroke-width= "0.95"
%	 points= "(150,100);(150,100);(150,80);(150,80)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.95"
%	 points= "(120,20);(120,20);(120,0);(120,0)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.95"
%	 points= "(120,0);(120,0);(140,0);(140,0)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.95"
%	 points= "(120,20);(120,20);(140,0);(140,0)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.95"
%	 points= "(100,80);(100,80);(160,80);(160,80)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.95"
%	 points= "(160,60);(160,60);(160,80);(160,80)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.95"
%	 points= "(120,60);(120,60);(160,60);(160,60)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.95"
%	 points= "(150,60);(150,60);(150,40);(150,40)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.95"
%	 points= "(100,80);(100,80);(120,60);(120,60)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.95"
%	 points= "(130,60);(130,60);(130,10);(130,10)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.95"
%	 points= "(110,70);(110,70);(110,40);(110,40)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.95"
%	 points= "(150,40);(150,40);(130,20);(130,20)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.95"
%	 points= "(110,40);(110,40);(130,20);(130,20)"
%	 fill-style= "none"
%	 />
%<ellipse p3= "(132.57,17.42)"
%	 p2= "(132.57,22.58)"
%	 p1= "(127.43,22.58)"
%	 closure= "open"
%	 fill-color= "#330033"
%	 angle-end= "0"
%	 fill-style= "solid"
%	 angle-start= "0"
%	 />
%<text text-vert-align= "center-v"
%	 anchor-point= "(125,5)"
%	 text-frame= "noframe"
%	 fill-style= "none"
%	 text-hor-align= "center-h"
%	 >
%$\Sprog$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(135,70)"
%	 text-frame= "noframe"
%	 fill-style= "none"
%	 text-hor-align= "center-h"
%	 >
%$\ltag$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(185,60)"
%	 text-frame= "noframe"
%	 fill-style= "none"
%	 text-hor-align= "center-h"
%	 >
%\EQLS
%</text>
%<multicurve stroke-width= "0.95"
%	 points= "(250,100);(250,100);(250,80);(250,80)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.95"
%	 points= "(200,20);(200,20);(200,0);(200,0)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.95"
%	 points= "(200,0);(200,0);(220,0);(220,0)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.95"
%	 points= "(200,20);(200,20);(220,0);(220,0)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.95"
%	 points= "(200,80);(200,80);(260,80);(260,80)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.95"
%	 points= "(260,60);(260,60);(260,80);(260,80)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.95"
%	 points= "(220,60);(220,60);(260,60);(260,60)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.95"
%	 points= "(250,60);(250,60);(250,40);(250,40)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.95"
%	 points= "(200,80);(200,80);(220,60);(220,60)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.95"
%	 points= "(230,60);(230,60);(230,40);(230,40)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.95"
%	 points= "(210,70);(210,70);(210,10);(210,10)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.95"
%	 points= "(250,40);(250,40);(240,30);(240,30)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.95"
%	 points= "(230,40);(230,40);(240,30);(240,30)"
%	 fill-style= "none"
%	 />
%<ellipse p3= "(242.57,27.42)"
%	 p2= "(242.57,32.58)"
%	 p1= "(237.43,32.58)"
%	 closure= "open"
%	 fill-color= "#330033"
%	 angle-end= "0"
%	 fill-style= "solid"
%	 angle-start= "0"
%	 />
%<text text-vert-align= "center-v"
%	 anchor-point= "(205,5)"
%	 text-frame= "noframe"
%	 fill-style= "none"
%	 text-hor-align= "center-h"
%	 >
%$\Sprog$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(235,70)"
%	 text-frame= "noframe"
%	 fill-style= "none"
%	 text-hor-align= "center-h"
%	 >
%$\ltag$
%</text>
%<multicurve stroke-width= "0.95"
%	 points= "(230,20);(230,20);(230,0);(230,0)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.95"
%	 points= "(230,0);(230,0);(250,0);(250,0)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.95"
%	 points= "(230,20);(230,20);(250,0);(250,0)"
%	 fill-style= "none"
%	 />
%<text text-vert-align= "center-v"
%	 anchor-point= "(235,5)"
%	 text-frame= "noframe"
%	 fill-style= "none"
%	 text-hor-align= "center-h"
%	 >
%$\Sprog$
%</text>
%<multicurve stroke-width= "0.95"
%	 points= "(240,30);(240,30);(240,10);(240,10)"
%	 fill-style= "none"
%	 />
%<text text-vert-align= "center-v"
%	 anchor-point= "(280,60)"
%	 text-frame= "noframe"
%	 fill-style= "none"
%	 text-hor-align= "center-h"
%	 >
%\EQLS
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(40,120)"
%	 text-frame= "noframe"
%	 fill-style= "none"
%	 text-hor-align= "center-h"
%	 >
%$\LLHS$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(185,120)"
%	 text-frame= "noframe"
%	 fill-style= "none"
%	 text-hor-align= "center-h"
%	 >
%$\LMHS$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(320,120)"
%	 text-frame= "noframe"
%	 fill-style= "none"
%	 text-hor-align= "center-h"
%	 >
%$\RRHS$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(85,120)"
%	 text-frame= "noframe"
%	 fill-style= "none"
%	 text-hor-align= "center-h"
%	 >
%$\EQLSone$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(280,120)"
%	 text-frame= "noframe"
%	 fill-style= "none"
%	 text-hor-align= "center-h"
%	 >
%$\EQLStwo$
%</text>
%</jpic>
%%End JPIC-XML
%PSTricks content-type (pstricks.sty package needed)
%Add \usepackage{pstricks} in the preamble of your LaTeX file
%You can rescale the whole picture (to 80% for instance) by using the command \def\JPicScale{0.8}
\ifx\JPicScale\undefined\def\JPicScale{1}\fi
\psset{unit=\JPicScale mm}
\psset{linewidth=0.3,dotsep=1,hatchwidth=0.3,hatchsep=1.5,shadowsize=1,dimen=middle}
\psset{dotsize=0.7 2.5,dotscale=1 1,fillcolor=black}
\psset{arrowsize=1 2,arrowlength=1,arrowinset=0.25,tbarsize=0.7 5,bracketlength=0.15,rbracketlength=0.15}
\begin{pspicture}(0,0)(340,120)
\psline[linewidth=0.95](40,20)(40,0)
\psline[linewidth=0.95](40,0)(60,0)
\psline[linewidth=0.95](40,20)(60,0)
\psline[linewidth=0.95](50,100)(50,80)
\psline[linewidth=0.95](10,20)(10,0)
\psline[linewidth=0.95](10,0)(30,0)
\psline[linewidth=0.95](10,20)(30,0)
\psline[linewidth=0.95](20,80)(60,80)
\psline[linewidth=0.95](60,60)(60,80)
\psline[linewidth=0.95](40,60)(60,60)
\psline[linewidth=0.95](50,60)(50,10)
\psline[linewidth=0.95](30,70)(30,50)
\psline[linewidth=0.95](20,80)(40,60)
\psline[linewidth=0.95](0,60)(20,60)
\psline[linewidth=0.95](40,40)(20,60)
\psline[linewidth=0.95](20,40)(40,40)
\psline[linewidth=0.95](30,40)(30,30)
\psline[linewidth=0.95](10,50)(10,30)
\psline[linewidth=0.95](0,60)(20,40)
\psline[linewidth=0.95](30,30)(20,20)
\psline[linewidth=0.95](10,30)(20,20)
\newrgbcolor{userFillColour}{0.2 0 0.2}
\rput{90}(20,20){\psellipse[fillcolor=userFillColour,fillstyle=solid](0,0)(2.58,-2.57)}
\psline[linewidth=0.95](20,20)(20,10)
\rput(15,5){$\Sprog$}
\rput(20,50){$\stag$}
\rput(45,70){$\ltag$}
\rput(85,60){\EQLS}
\psline[linewidth=0.95](310,20)(310,0)
\psline[linewidth=0.95](310,0)(330,0)
\psline[linewidth=0.95](310,20)(330,0)
\psline[linewidth=0.95](330,100)(330,50)
\psline[linewidth=0.95](300,60)(320,60)
\psline[linewidth=0.95](340,40)(320,60)
\psline[linewidth=0.95](320,40)(340,40)
\psline[linewidth=0.95](330,40)(330,30)
\psline[linewidth=0.95](310,50)(310,30)
\psline[linewidth=0.95](300,60)(320,40)
\psline[linewidth=0.95](330,30)(320,20)
\psline[linewidth=0.95](310,30)(320,20)
\newrgbcolor{userFillColour}{0.2 0 0.2}
\rput{90}(320,20){\psellipse[fillcolor=userFillColour,fillstyle=solid](0,0)(2.58,-2.57)}
\psline[linewidth=0.95](320,20)(320,10)
\rput(315,5){$\Sprog$}
\rput(320,50){$\stag$}
\rput(46.25,5){$\Sprog$}
\psline[linewidth=0.95](150,100)(150,80)
\psline[linewidth=0.95](120,20)(120,0)
\psline[linewidth=0.95](120,0)(140,0)
\psline[linewidth=0.95](120,20)(140,0)
\psline[linewidth=0.95](100,80)(160,80)
\psline[linewidth=0.95](160,60)(160,80)
\psline[linewidth=0.95](120,60)(160,60)
\psline[linewidth=0.95](150,60)(150,40)
\psline[linewidth=0.95](100,80)(120,60)
\psline[linewidth=0.95](130,60)(130,10)
\psline[linewidth=0.95](110,70)(110,40)
\psline[linewidth=0.95](150,40)(130,20)
\psline[linewidth=0.95](110,40)(130,20)
\newrgbcolor{userFillColour}{0.2 0 0.2}
\rput{90}(130,20){\psellipse[fillcolor=userFillColour,fillstyle=solid](0,0)(2.58,-2.57)}
\rput(125,5){$\Sprog$}
\rput(135,70){$\ltag$}
\rput(185,60){\EQLS}
\psline[linewidth=0.95](250,100)(250,80)
\psline[linewidth=0.95](200,20)(200,0)
\psline[linewidth=0.95](200,0)(220,0)
\psline[linewidth=0.95](200,20)(220,0)
\psline[linewidth=0.95](200,80)(260,80)
\psline[linewidth=0.95](260,60)(260,80)
\psline[linewidth=0.95](220,60)(260,60)
\psline[linewidth=0.95](250,60)(250,40)
\psline[linewidth=0.95](200,80)(220,60)
\psline[linewidth=0.95](230,60)(230,40)
\psline[linewidth=0.95](210,70)(210,10)
\psline[linewidth=0.95](250,40)(240,30)
\psline[linewidth=0.95](230,40)(240,30)
\newrgbcolor{userFillColour}{0.2 0 0.2}
\rput{90}(240,30){\psellipse[fillcolor=userFillColour,fillstyle=solid](0,0)(2.58,-2.57)}
\rput(205,5){$\Sprog$}
\rput(235,70){$\ltag$}
\psline[linewidth=0.95](230,20)(230,0)
\psline[linewidth=0.95](230,0)(250,0)
\psline[linewidth=0.95](230,20)(250,0)
\rput(235,5){$\Sprog$}
\psline[linewidth=0.95](240,30)(240,10)
\rput(280,60){\EQLS}
\rput(40,120){$\LLHS$}
\rput(185,120){$\LMHS$}
\rput(320,120){$\RRHS$}
\rput(85,120){$\EQLSone$}
\rput(280,120){$\EQLStwo$}
\end{pspicture}


==> PIC/futamura-fst.tex <==
%%Created by jPicEdt 1.4.1_03: mixed JPIC-XML/LaTeX format
%%Sat Nov 24 15:51:42 GMT-10:00 2018
%%Begin JPIC-XML
%<?xml version="1.0" standalone="yes"?>
%<jpic x-min="10" x-max="300" y-min="0" y-max="115" auto-bounding="true">
%<multicurve fill-style= "none"
%	 points= "(235,100);(235,100);(280,100);(280,100)"
%	 stroke-width= "0.95"
%	 />
%<multicurve fill-style= "none"
%	 points= "(280,80);(280,80);(280,100);(280,100)"
%	 stroke-width= "0.95"
%	 />
%<multicurve fill-style= "none"
%	 points= "(270,115);(270,115);(270,100);(270,100)"
%	 stroke-width= "0.95"
%	 />
%<multicurve fill-style= "none"
%	 points= "(255,80);(255,80);(280,80);(280,80)"
%	 stroke-width= "0.95"
%	 />
%<multicurve fill-style= "none"
%	 points= "(270,80);(270,80);(270,0);(270,0)"
%	 stroke-width= "0.95"
%	 />
%<multicurve fill-style= "none"
%	 points= "(235,100);(235,100);(255,80);(255,80)"
%	 stroke-width= "0.95"
%	 />
%<multicurve fill-style= "none"
%	 points= "(210,50);(210,50);(210,30);(210,30)"
%	 stroke-width= "0.95"
%	 />
%<multicurve fill-style= "none"
%	 points= "(245,90);(245,90);(245,60);(245,60)"
%	 stroke-width= "0.95"
%	 />
%<multicurve fill-style= "none"
%	 points= "(245,50);(245,50);(245,0);(245,0)"
%	 stroke-width= "0.95"
%	 />
%<multicurve fill-style= "none"
%	 points= "(210,30);(210,30);(230,30);(230,30)"
%	 stroke-width= "0.95"
%	 />
%<multicurve fill-style= "none"
%	 points= "(210,50);(210,50);(230,30);(230,30)"
%	 stroke-width= "0.95"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(215,35)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\itag$
%</text>
%<multicurve fill-style= "none"
%	 points= "(220,60);(220,60);(220,40);(220,40)"
%	 stroke-width= "0.95"
%	 />
%<multicurve fill-style= "none"
%	 points= "(210,70);(210,70);(235,70);(235,70)"
%	 stroke-width= "0.95"
%	 />
%<multicurve fill-style= "none"
%	 points= "(255,50);(255,50);(235,70);(235,70)"
%	 stroke-width= "0.95"
%	 />
%<multicurve fill-style= "none"
%	 points= "(230,50);(230,50);(255,50);(255,50)"
%	 stroke-width= "0.95"
%	 />
%<multicurve fill-style= "none"
%	 points= "(210,70);(210,70);(230,50);(230,50)"
%	 stroke-width= "0.95"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(217.5,55)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\Lprogtype$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(241.25,80)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\Lprogtype$
%</text>
%<multicurve fill-style= "none"
%	 points= "(205,73.75);(205,73.75);(205,25);(205,25)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(260,73.75);(260,73.75);(260,25);(260,25)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(205,25);(205,25);(260,25);(260,25)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(205,73.75);(205,73.75);(260,73.75);(260,73.75)"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(270,90)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\ltag$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(255,30)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\Cprog$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(232.5,60)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\stag$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(242.5,10)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\Hprogtype$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(300,90)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\EQLStwo
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(195,90)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\EQLSone
%</text>
%<multicurve fill-style= "none"
%	 points= "(105,100);(105,100);(175,100);(175,100)"
%	 stroke-width= "0.95"
%	 />
%<multicurve fill-style= "none"
%	 points= "(175,80);(175,80);(175,100);(175,100)"
%	 stroke-width= "0.95"
%	 />
%<multicurve fill-style= "none"
%	 points= "(165,115);(165,115);(165,100);(165,100)"
%	 stroke-width= "0.95"
%	 />
%<multicurve fill-style= "none"
%	 points= "(125,80);(125,80);(175,80);(175,80)"
%	 stroke-width= "0.95"
%	 />
%<multicurve fill-style= "none"
%	 points= "(165,80);(165,80);(165,0);(165,0)"
%	 stroke-width= "0.95"
%	 />
%<multicurve fill-style= "none"
%	 points= "(105,80);(105,80);(105,60);(105,60)"
%	 stroke-width= "0.95"
%	 />
%<multicurve fill-style= "none"
%	 points= "(140,80);(140,80);(140,0);(140,0)"
%	 stroke-width= "0.95"
%	 />
%<multicurve fill-style= "none"
%	 points= "(105,60);(105,60);(125,60);(125,60)"
%	 stroke-width= "0.95"
%	 />
%<multicurve fill-style= "none"
%	 points= "(105,80);(105,80);(125,60);(125,60)"
%	 stroke-width= "0.95"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(110,65)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\itag$
%</text>
%<multicurve fill-style= "none"
%	 points= "(115,90);(115,90);(115,70);(115,70)"
%	 stroke-width= "0.95"
%	 />
%<multicurve fill-style= "none"
%	 points= "(105,100);(105,100);(125,80);(125,80)"
%	 stroke-width= "0.95"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(112.5,83.75)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\Lprogtype$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(165,90)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\ltag$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(137.5,10)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\Hprogtype$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(75,90)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\EQLSzero
%</text>
%<multicurve fill-style= "none"
%	 points= "(10,100);(10,100);(55,100);(55,100)"
%	 stroke-width= "0.95"
%	 />
%<multicurve fill-style= "none"
%	 points= "(55,80);(55,80);(55,100);(55,100)"
%	 stroke-width= "0.95"
%	 />
%<multicurve fill-style= "none"
%	 points= "(45,115);(45,115);(45,100);(45,100)"
%	 stroke-width= "0.95"
%	 />
%<multicurve fill-style= "none"
%	 points= "(30,80);(30,80);(55,80);(55,80)"
%	 stroke-width= "0.95"
%	 />
%<multicurve fill-style= "none"
%	 points= "(45,80);(45,80);(45,0);(45,0)"
%	 stroke-width= "0.95"
%	 />
%<multicurve fill-style= "none"
%	 points= "(20,90);(20,90);(20,0);(20,0)"
%	 stroke-width= "0.95"
%	 />
%<multicurve fill-style= "none"
%	 points= "(10,100);(10,100);(30,80);(30,80)"
%	 stroke-width= "0.95"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(17.5,10)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\Hprogtype$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(45,90)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\htag$
%</text>
%</jpic>
%%End JPIC-XML
%PSTricks content-type (pstricks.sty package needed)
%Add \usepackage{pstricks} in the preamble of your LaTeX file
%You can rescale the whole picture (to 80% for instance) by using the command \def\JPicScale{0.8}
\ifx\JPicScale\undefined\def\JPicScale{1}\fi
\psset{unit=\JPicScale mm}
\psset{linewidth=0.3,dotsep=1,hatchwidth=0.3,hatchsep=1.5,shadowsize=1,dimen=middle}
\psset{dotsize=0.7 2.5,dotscale=1 1,fillcolor=black}
\psset{arrowsize=1 2,arrowlength=1,arrowinset=0.25,tbarsize=0.7 5,bracketlength=0.15,rbracketlength=0.15}
\begin{pspicture}(0,0)(300,115)
\psline[linewidth=0.95](235,100)(280,100)
\psline[linewidth=0.95](280,80)(280,100)
\psline[linewidth=0.95](270,115)(270,100)
\psline[linewidth=0.95](255,80)(280,80)
\psline[linewidth=0.95](270,80)(270,0)
\psline[linewidth=0.95](235,100)(255,80)
\psline[linewidth=0.95](210,50)(210,30)
\psline[linewidth=0.95](245,90)(245,60)
\psline[linewidth=0.95](245,50)(245,0)
\psline[linewidth=0.95](210,30)(230,30)
\psline[linewidth=0.95](210,50)(230,30)
\rput(215,35){$\itag$}
\psline[linewidth=0.95](220,60)(220,40)
\psline[linewidth=0.95](210,70)(235,70)
\psline[linewidth=0.95](255,50)(235,70)
\psline[linewidth=0.95](230,50)(255,50)
\psline[linewidth=0.95](210,70)(230,50)
\rput[r](217.5,55){$\Lprogtype$}
\rput[r](241.25,80){$\Lprogtype$}
\psline(205,73.75)(205,25)
\psline(260,73.75)(260,25)
\psline(205,25)(260,25)
\psline(205,73.75)(260,73.75)
\rput(270,90){$\ltag$}
\rput(255,30){$\Cprog$}
\rput(232.5,60){$\stag$}
\rput[r](242.5,10){$\Hprogtype$}
\rput(300,90){\EQLStwo}
\rput(195,90){\EQLSone}
\psline[linewidth=0.95](105,100)(175,100)
\psline[linewidth=0.95](175,80)(175,100)
\psline[linewidth=0.95](165,115)(165,100)
\psline[linewidth=0.95](125,80)(175,80)
\psline[linewidth=0.95](165,80)(165,0)
\psline[linewidth=0.95](105,80)(105,60)
\psline[linewidth=0.95](140,80)(140,0)
\psline[linewidth=0.95](105,60)(125,60)
\psline[linewidth=0.95](105,80)(125,60)
\rput(110,65){$\itag$}
\psline[linewidth=0.95](115,90)(115,70)
\psline[linewidth=0.95](105,100)(125,80)
\rput[r](112.5,83.75){$\Lprogtype$}
\rput(165,90){$\ltag$}
\rput[r](137.5,10){$\Hprogtype$}
\rput(75,90){\EQLSzero}
\psline[linewidth=0.95](10,100)(55,100)
\psline[linewidth=0.95](55,80)(55,100)
\psline[linewidth=0.95](45,115)(45,100)
\psline[linewidth=0.95](30,80)(55,80)
\psline[linewidth=0.95](45,80)(45,0)
\psline[linewidth=0.95](20,90)(20,0)
\psline[linewidth=0.95](10,100)(30,80)
\rput[r](17.5,10){$\Hprogtype$}
\rput(45,90){$\htag$}
\end{pspicture}


==> PIC/futamura-prop.tex <==
%%Created by jPicEdt 1.4.1_03: mixed JPIC-XML/LaTeX format
%%Wed Nov 23 22:43:24 HST 2016
%%Begin JPIC-XML
%<?xml version="1.0" standalone="yes"?>
%<jpic x-min="0" x-max="146.25" y-min="0" y-max="100" auto-bounding="true">
%<multicurve stroke-width= "0.95"
%	 points= "(45,20);(45,20);(45,0);(45,0)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.95"
%	 points= "(45,0);(45,0);(65,0);(65,0)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.95"
%	 points= "(45,20);(45,20);(65,0);(65,0)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.95"
%	 points= "(55,100);(55,100);(55,80);(55,80)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.95"
%	 points= "(10,20);(10,20);(10,0);(10,0)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.95"
%	 points= "(10,0);(10,0);(30,0);(30,0)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.95"
%	 points= "(10,20);(10,20);(30,0);(30,0)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.95"
%	 points= "(20,80);(20,80);(65,80);(65,80)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.95"
%	 points= "(65,60);(65,60);(65,80);(65,80)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.95"
%	 points= "(40,60);(40,60);(65,60);(65,60)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.95"
%	 points= "(55,60);(55,60);(55,10);(55,10)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.95"
%	 points= "(30,70);(30,70);(30,50);(30,50)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.95"
%	 points= "(20,80);(20,80);(40,60);(40,60)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.95"
%	 points= "(0,60);(0,60);(20,60);(20,60)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.95"
%	 points= "(40,40);(40,40);(20,60);(20,60)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.95"
%	 points= "(20,40);(20,40);(40,40);(40,40)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.95"
%	 points= "(30,40);(30,40);(30,30);(30,30)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.95"
%	 points= "(10,50);(10,50);(10,30);(10,30)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.95"
%	 points= "(0,60);(0,60);(20,40);(20,40)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.95"
%	 points= "(30,30);(30,30);(20,20);(20,20)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.95"
%	 points= "(10,30);(10,30);(20,20);(20,20)"
%	 fill-style= "none"
%	 />
%<ellipse p3= "(22.57,17.42)"
%	 p2= "(22.57,22.58)"
%	 p1= "(17.43,22.58)"
%	 closure= "open"
%	 angle-end= "0"
%	 fill-style= "solid"
%	 angle-start= "0"
%	 fill-color= "#330033"
%	 />
%<multicurve stroke-width= "0.95"
%	 points= "(20,20);(20,20);(20,10);(20,10)"
%	 fill-style= "none"
%	 />
%<text text-vert-align= "center-v"
%	 anchor-point= "(15,5)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\Sprog$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(20,50)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\stag$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(55,70)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\ltag$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(87.5,70)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\EQLS
%</text>
%<multicurve stroke-width= "0.95"
%	 points= "(116.25,20);(116.25,20);(116.25,0);(116.25,0)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.95"
%	 points= "(116.25,0);(116.25,0);(136.25,0);(136.25,0)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.95"
%	 points= "(116.25,20);(116.25,20);(136.25,0);(136.25,0)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.95"
%	 points= "(136.25,100);(136.25,100);(136.25,50);(136.25,50)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.95"
%	 points= "(106.25,60);(106.25,60);(126.25,60);(126.25,60)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.95"
%	 points= "(146.25,40);(146.25,40);(126.25,60);(126.25,60)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.95"
%	 points= "(126.25,40);(126.25,40);(146.25,40);(146.25,40)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.95"
%	 points= "(136.25,40);(136.25,40);(136.25,30);(136.25,30)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.95"
%	 points= "(116.25,50);(116.25,50);(116.25,30);(116.25,30)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.95"
%	 points= "(106.25,60);(106.25,60);(126.25,40);(126.25,40)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.95"
%	 points= "(136.25,30);(136.25,30);(126.25,20);(126.25,20)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.95"
%	 points= "(116.25,30);(116.25,30);(126.25,20);(126.25,20)"
%	 fill-style= "none"
%	 />
%<ellipse p3= "(128.82,17.42)"
%	 p2= "(128.82,22.58)"
%	 p1= "(123.68,22.58)"
%	 closure= "open"
%	 angle-end= "0"
%	 fill-style= "solid"
%	 angle-start= "0"
%	 fill-color= "#330033"
%	 />
%<multicurve stroke-width= "0.95"
%	 points= "(126.25,20);(126.25,20);(126.25,10);(126.25,10)"
%	 fill-style= "none"
%	 />
%<text text-vert-align= "center-v"
%	 anchor-point= "(121.25,5)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\Sprog$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(126.25,50)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\stag$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(51.25,5)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\Sprog$
%</text>
%</jpic>
%%End JPIC-XML
%PSTricks content-type (pstricks.sty package needed)
%Add \usepackage{pstricks} in the preamble of your LaTeX file
%You can rescale the whole picture (to 80% for instance) by using the command \def\JPicScale{0.8}
\ifx\JPicScale\undefined\def\JPicScale{1}\fi
\psset{unit=\JPicScale mm}
\psset{linewidth=0.3,dotsep=1,hatchwidth=0.3,hatchsep=1.5,shadowsize=1,dimen=middle}
\psset{dotsize=0.7 2.5,dotscale=1 1,fillcolor=black}
\psset{arrowsize=1 2,arrowlength=1,arrowinset=0.25,tbarsize=0.7 5,bracketlength=0.15,rbracketlength=0.15}
\begin{pspicture}(0,0)(146.25,100)
\psline[linewidth=0.95](45,20)(45,0)
\psline[linewidth=0.95](45,0)(65,0)
\psline[linewidth=0.95](45,20)(65,0)
\psline[linewidth=0.95](55,100)(55,80)
\psline[linewidth=0.95](10,20)(10,0)
\psline[linewidth=0.95](10,0)(30,0)
\psline[linewidth=0.95](10,20)(30,0)
\psline[linewidth=0.95](20,80)(65,80)
\psline[linewidth=0.95](65,60)(65,80)
\psline[linewidth=0.95](40,60)(65,60)
\psline[linewidth=0.95](55,60)(55,10)
\psline[linewidth=0.95](30,70)(30,50)
\psline[linewidth=0.95](20,80)(40,60)
\psline[linewidth=0.95](0,60)(20,60)
\psline[linewidth=0.95](40,40)(20,60)
\psline[linewidth=0.95](20,40)(40,40)
\psline[linewidth=0.95](30,40)(30,30)
\psline[linewidth=0.95](10,50)(10,30)
\psline[linewidth=0.95](0,60)(20,40)
\psline[linewidth=0.95](30,30)(20,20)
\psline[linewidth=0.95](10,30)(20,20)
\newrgbcolor{userFillColour}{0.2 0 0.2}
\rput{90}(20,20){\psellipse[fillcolor=userFillColour,fillstyle=solid](0,0)(2.58,-2.57)}
\psline[linewidth=0.95](20,20)(20,10)
\rput(15,5){$\Sprog$}
\rput(20,50){$\stag$}
\rput(55,70){$\ltag$}
\rput(87.5,70){\EQLS}
\psline[linewidth=0.95](116.25,20)(116.25,0)
\psline[linewidth=0.95](116.25,0)(136.25,0)
\psline[linewidth=0.95](116.25,20)(136.25,0)
\psline[linewidth=0.95](136.25,100)(136.25,50)
\psline[linewidth=0.95](106.25,60)(126.25,60)
\psline[linewidth=0.95](146.25,40)(126.25,60)
\psline[linewidth=0.95](126.25,40)(146.25,40)
\psline[linewidth=0.95](136.25,40)(136.25,30)
\psline[linewidth=0.95](116.25,50)(116.25,30)
\psline[linewidth=0.95](106.25,60)(126.25,40)
\psline[linewidth=0.95](136.25,30)(126.25,20)
\psline[linewidth=0.95](116.25,30)(126.25,20)
\newrgbcolor{userFillColour}{0.2 0 0.2}
\rput{90}(126.25,20){\psellipse[fillcolor=userFillColour,fillstyle=solid](0,0)(2.58,-2.57)}
\psline[linewidth=0.95](126.25,20)(126.25,10)
\rput(121.25,5){$\Sprog$}
\rput(126.25,50){$\stag$}
\rput(51.25,5){$\Sprog$}
\end{pspicture}


==> PIC/futamura-snd.tex <==
%%Created by jPicEdt 1.4.1_03: mixed JPIC-XML/LaTeX format
%%Sat Nov 24 16:55:55 GMT-10:00 2018
%%Begin JPIC-XML
%<?xml version="1.0" standalone="yes"?>
%<jpic x-min="0" x-max="280" y-min="0" y-max="185" auto-bounding="true">
%<multicurve fill-style= "none"
%	 points= "(210,170);(210,170);(255,170);(255,170)"
%	 stroke-width= "0.95"
%	 />
%<multicurve fill-style= "none"
%	 points= "(255,150);(255,150);(255,170);(255,170)"
%	 stroke-width= "0.95"
%	 />
%<multicurve fill-style= "none"
%	 points= "(245,185);(245,185);(245,170);(245,170)"
%	 stroke-width= "0.95"
%	 />
%<multicurve fill-style= "none"
%	 points= "(230,150);(230,150);(255,150);(255,150)"
%	 stroke-width= "0.95"
%	 />
%<multicurve fill-style= "none"
%	 points= "(245,150);(245,150);(245,0);(245,0)"
%	 stroke-width= "0.95"
%	 />
%<multicurve fill-style= "none"
%	 points= "(210,170);(210,170);(230,150);(230,150)"
%	 stroke-width= "0.95"
%	 />
%<multicurve fill-style= "none"
%	 points= "(185,140);(185,140);(230,140);(230,140)"
%	 stroke-width= "0.95"
%	 />
%<multicurve fill-style= "none"
%	 points= "(185,60);(185,60);(185,40);(185,40)"
%	 stroke-width= "0.95"
%	 />
%<multicurve fill-style= "none"
%	 points= "(230,120);(230,120);(230,140);(230,140)"
%	 stroke-width= "0.95"
%	 />
%<multicurve fill-style= "none"
%	 points= "(220,160);(220,160);(220,140);(220,140)"
%	 stroke-width= "0.95"
%	 />
%<multicurve fill-style= "none"
%	 points= "(205,120);(205,120);(230,120);(230,120)"
%	 stroke-width= "0.95"
%	 />
%<multicurve fill-style= "none"
%	 points= "(220,120);(220,120);(220,0);(220,0)"
%	 stroke-width= "0.95"
%	 />
%<multicurve fill-style= "none"
%	 points= "(185,40);(185,40);(205,40);(205,40)"
%	 stroke-width= "0.95"
%	 />
%<multicurve fill-style= "none"
%	 points= "(185,60);(185,60);(205,40);(205,40)"
%	 stroke-width= "0.95"
%	 />
%<multicurve fill-style= "none"
%	 points= "(195,130);(195,130);(195,100);(195,100)"
%	 stroke-width= "0.95"
%	 />
%<multicurve fill-style= "none"
%	 points= "(185,140);(185,140);(205,120);(205,120)"
%	 stroke-width= "0.95"
%	 />
%<multicurve fill-style= "none"
%	 points= "(160,90);(160,90);(160,70);(160,70)"
%	 stroke-width= "0.95"
%	 />
%<multicurve fill-style= "none"
%	 points= "(160,70);(160,70);(180,70);(180,70)"
%	 stroke-width= "0.95"
%	 />
%<multicurve fill-style= "none"
%	 points= "(160,90);(160,90);(180,70);(180,70)"
%	 stroke-width= "0.95"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(190,45)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\itag$
%</text>
%<multicurve fill-style= "none"
%	 points= "(195,90);(195,90);(195,50);(195,50)"
%	 stroke-width= "0.95"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(192.5,65)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\Lprogtype$
%</text>
%<multicurve fill-style= "none"
%	 points= "(160,110);(160,110);(185,110);(185,110)"
%	 stroke-width= "0.95"
%	 />
%<multicurve fill-style= "none"
%	 points= "(205,90);(205,90);(185,110);(185,110)"
%	 stroke-width= "0.95"
%	 />
%<multicurve fill-style= "none"
%	 points= "(180,90);(180,90);(205,90);(205,90)"
%	 stroke-width= "0.95"
%	 />
%<multicurve fill-style= "none"
%	 points= "(170,100);(170,100);(170,80);(170,80)"
%	 stroke-width= "0.95"
%	 />
%<multicurve fill-style= "none"
%	 points= "(160,110);(160,110);(180,90);(180,90)"
%	 stroke-width= "0.95"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(192.5,122.5)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\Lprogtype$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(216.25,150)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\Lprogtype$
%</text>
%<multicurve fill-style= "none"
%	 points= "(155,115);(155,115);(155,40);(155,40)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(210,92.5);(210,92.5);(210,40);(210,40)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(155,40);(155,40);(182.5,12.5);(182.5,12.5)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(210,40);(210,40);(182.5,12.5);(182.5,12.5)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(187.5,115);(187.5,115);(210,92.5);(210,92.5)"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(245,160)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\ltag$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(165,75)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\Sprog$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(182.5,100)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\stag$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(220,130)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\ltag$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(217.5,10)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\Hprogtype$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(167.5,95)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\Lprogtype$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(145,160)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\EQLSthree
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(280,160)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\EQLSfour
%</text>
%<multicurve fill-style= "none"
%	 points= "(70,170);(70,170);(115,170);(115,170)"
%	 stroke-width= "0.95"
%	 />
%<multicurve fill-style= "none"
%	 points= "(115,150);(115,150);(115,170);(115,170)"
%	 stroke-width= "0.95"
%	 />
%<multicurve fill-style= "none"
%	 points= "(105,185);(105,185);(105,170);(105,170)"
%	 stroke-width= "0.95"
%	 />
%<multicurve fill-style= "none"
%	 points= "(90,150);(90,150);(115,150);(115,150)"
%	 stroke-width= "0.95"
%	 />
%<multicurve fill-style= "none"
%	 points= "(105,150);(105,150);(105,0);(105,0)"
%	 stroke-width= "0.95"
%	 />
%<multicurve fill-style= "none"
%	 points= "(70,170);(70,170);(90,150);(90,150)"
%	 stroke-width= "0.95"
%	 />
%<multicurve fill-style= "none"
%	 points= "(20,140);(20,140);(90,140);(90,140)"
%	 stroke-width= "0.95"
%	 />
%<multicurve fill-style= "none"
%	 points= "(45,90);(45,90);(45,70);(45,70)"
%	 stroke-width= "0.95"
%	 />
%<multicurve fill-style= "none"
%	 points= "(90,120);(90,120);(90,140);(90,140)"
%	 stroke-width= "0.95"
%	 />
%<multicurve fill-style= "none"
%	 points= "(80,160);(80,160);(80,140);(80,140)"
%	 stroke-width= "0.95"
%	 />
%<multicurve fill-style= "none"
%	 points= "(40,120);(40,120);(90,120);(90,120)"
%	 stroke-width= "0.95"
%	 />
%<multicurve fill-style= "none"
%	 points= "(80,120);(80,120);(80,0);(80,0)"
%	 stroke-width= "0.95"
%	 />
%<multicurve fill-style= "none"
%	 points= "(45,70);(45,70);(65,70);(65,70)"
%	 stroke-width= "0.95"
%	 />
%<multicurve fill-style= "none"
%	 points= "(45,90);(45,90);(65,70);(65,70)"
%	 stroke-width= "0.95"
%	 />
%<multicurve fill-style= "none"
%	 points= "(20,120);(20,120);(20,100);(20,100)"
%	 stroke-width= "0.95"
%	 />
%<multicurve fill-style= "none"
%	 points= "(20,100);(20,100);(40,100);(40,100)"
%	 stroke-width= "0.95"
%	 />
%<multicurve fill-style= "none"
%	 points= "(20,120);(20,120);(40,100);(40,100)"
%	 stroke-width= "0.95"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(50,75)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\itag$
%</text>
%<multicurve fill-style= "none"
%	 points= "(55,120);(55,120);(55,80);(55,80)"
%	 stroke-width= "0.95"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(52.5,95)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\Lprogtype$
%</text>
%<multicurve fill-style= "none"
%	 points= "(30,130);(30,130);(30,110);(30,110)"
%	 stroke-width= "0.95"
%	 />
%<multicurve fill-style= "none"
%	 points= "(20,140);(20,140);(40,120);(40,120)"
%	 stroke-width= "0.95"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(76.25,150)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\Lprogtype$
%</text>
%<multicurve fill-style= "none"
%	 points= "(10,145);(10,145);(10,65);(10,65)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(95,145);(95,145);(95,65);(95,65)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(95,65);(95,65);(10,65);(10,65)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(10,145);(10,145);(95,145);(95,145)"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(105,160)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\ltag$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(90,70)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\Cprog$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(25,105)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\Sprog$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(80,130)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\ltag$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(77.5,50)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\Hprogtype$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(27.5,123.75)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\Lprogtype$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(0,160)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\EQLStwo
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(182.5,22.5)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\Gprog$
%</text>
%<multicurve fill-style= "none"
%	 points= "(155,115);(155,115);(187.5,115);(187.5,115)"
%	 />
%</jpic>
%%End JPIC-XML
%PSTricks content-type (pstricks.sty package needed)
%Add \usepackage{pstricks} in the preamble of your LaTeX file
%You can rescale the whole picture (to 80% for instance) by using the command \def\JPicScale{0.8}
\ifx\JPicScale\undefined\def\JPicScale{1}\fi
\psset{unit=\JPicScale mm}
\psset{linewidth=0.3,dotsep=1,hatchwidth=0.3,hatchsep=1.5,shadowsize=1,dimen=middle}
\psset{dotsize=0.7 2.5,dotscale=1 1,fillcolor=black}
\psset{arrowsize=1 2,arrowlength=1,arrowinset=0.25,tbarsize=0.7 5,bracketlength=0.15,rbracketlength=0.15}
\begin{pspicture}(0,0)(280,185)
\psline[linewidth=0.95](210,170)(255,170)
\psline[linewidth=0.95](255,150)(255,170)
\psline[linewidth=0.95](245,185)(245,170)
\psline[linewidth=0.95](230,150)(255,150)
\psline[linewidth=0.95](245,150)(245,0)
\psline[linewidth=0.95](210,170)(230,150)
\psline[linewidth=0.95](185,140)(230,140)
\psline[linewidth=0.95](185,60)(185,40)
\psline[linewidth=0.95](230,120)(230,140)
\psline[linewidth=0.95](220,160)(220,140)
\psline[linewidth=0.95](205,120)(230,120)
\psline[linewidth=0.95](220,120)(220,0)
\psline[linewidth=0.95](185,40)(205,40)
\psline[linewidth=0.95](185,60)(205,40)
\psline[linewidth=0.95](195,130)(195,100)
\psline[linewidth=0.95](185,140)(205,120)
\psline[linewidth=0.95](160,90)(160,70)
\psline[linewidth=0.95](160,70)(180,70)
\psline[linewidth=0.95](160,90)(180,70)
\rput(190,45){$\itag$}
\psline[linewidth=0.95](195,90)(195,50)
\rput[r](192.5,65){$\Lprogtype$}
\psline[linewidth=0.95](160,110)(185,110)
\psline[linewidth=0.95](205,90)(185,110)
\psline[linewidth=0.95](180,90)(205,90)
\psline[linewidth=0.95](170,100)(170,80)
\psline[linewidth=0.95](160,110)(180,90)
\rput[r](192.5,122.5){$\Lprogtype$}
\rput[r](216.25,150){$\Lprogtype$}
\psline(155,115)(155,40)
\psline(210,92.5)(210,40)
\psline(155,40)(182.5,12.5)
\psline(210,40)(182.5,12.5)
\psline(187.5,115)(210,92.5)
\rput(245,160){$\ltag$}
\rput(165,75){$\Sprog$}
\rput(182.5,100){$\stag$}
\rput(220,130){$\ltag$}
\rput[r](217.5,10){$\Hprogtype$}
\rput[r](167.5,95){$\Lprogtype$}
\rput(145,160){\EQLSthree}
\rput(280,160){\EQLSfour}
\psline[linewidth=0.95](70,170)(115,170)
\psline[linewidth=0.95](115,150)(115,170)
\psline[linewidth=0.95](105,185)(105,170)
\psline[linewidth=0.95](90,150)(115,150)
\psline[linewidth=0.95](105,150)(105,0)
\psline[linewidth=0.95](70,170)(90,150)
\psline[linewidth=0.95](20,140)(90,140)
\psline[linewidth=0.95](45,90)(45,70)
\psline[linewidth=0.95](90,120)(90,140)
\psline[linewidth=0.95](80,160)(80,140)
\psline[linewidth=0.95](40,120)(90,120)
\psline[linewidth=0.95](80,120)(80,0)
\psline[linewidth=0.95](45,70)(65,70)
\psline[linewidth=0.95](45,90)(65,70)
\psline[linewidth=0.95](20,120)(20,100)
\psline[linewidth=0.95](20,100)(40,100)
\psline[linewidth=0.95](20,120)(40,100)
\rput(50,75){$\itag$}
\psline[linewidth=0.95](55,120)(55,80)
\rput[r](52.5,95){$\Lprogtype$}
\psline[linewidth=0.95](30,130)(30,110)
\psline[linewidth=0.95](20,140)(40,120)
\rput[r](76.25,150){$\Lprogtype$}
\psline(10,145)(10,65)
\psline(95,145)(95,65)
\psline(95,65)(10,65)
\psline(10,145)(95,145)
\rput(105,160){$\ltag$}
\rput(90,70){$\Cprog$}
\rput(25,105){$\Sprog$}
\rput(80,130){$\ltag$}
\rput[r](77.5,50){$\Hprogtype$}
\rput[r](27.5,123.75){$\Lprogtype$}
\rput(0,160){\EQLStwo}
\rput(182.5,22.5){$\Gprog$}
\psline(155,115)(187.5,115)
\end{pspicture}


==> PIC/futamura-trd-1.tex <==
%%Created by jPicEdt 1.4.1_03: mixed JPIC-XML/LaTeX format
%%Tue Nov 22 11:56:06 GMT-10:00 2022
%%Begin JPIC-XML
%<?xml version="1.0" standalone="yes"?>
%<jpic x-min="-5" x-max="430" y-min="0" y-max="245" auto-bounding="true">
%<multicurve fill-style= "none"
%	 stroke-width= "0.95"
%	 points= "(385,230);(385,230);(430,230);(430,230)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.95"
%	 points= "(430,210);(430,210);(430,230);(430,230)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.95"
%	 points= "(420,245);(420,245);(420,230);(420,230)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.95"
%	 points= "(405,210);(405,210);(430,210);(430,210)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.95"
%	 points= "(420,210);(420,210);(420,0);(420,0)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.95"
%	 points= "(385,230);(385,230);(405,210);(405,210)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.95"
%	 points= "(360,200);(360,200);(405,200);(405,200)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.95"
%	 points= "(360,67.5);(360,67.5);(360,47.5);(360,47.5)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.95"
%	 points= "(405,180);(405,180);(405,200);(405,200)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.95"
%	 points= "(395,220);(395,220);(395,200);(395,200)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.95"
%	 points= "(380,180);(380,180);(405,180);(405,180)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.95"
%	 points= "(395,180);(395,180);(395,0);(395,0)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.95"
%	 points= "(360,47.5);(360,47.5);(380,47.5);(380,47.5)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.95"
%	 points= "(360,67.5);(360,67.5);(380,47.5);(380,47.5)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.95"
%	 points= "(370,190);(370,190);(370,170);(370,170)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.95"
%	 points= "(360,200);(360,200);(380,180);(380,180)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.95"
%	 points= "(325,100);(325,100);(325,80);(325,80)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.95"
%	 points= "(325,80);(325,80);(345,80);(345,80)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.95"
%	 points= "(325,100);(325,100);(345,80);(345,80)"
%	 />
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(365,52.5)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\itag$
%</text>
%<multicurve fill-style= "none"
%	 stroke-width= "0.95"
%	 points= "(335,170);(335,170);(380,170);(380,170)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.95"
%	 points= "(380,150);(380,150);(380,170);(380,170)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.95"
%	 points= "(355,150);(355,150);(380,150);(380,150)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.95"
%	 points= "(370,150);(370,150);(370,57.5);(370,57.5)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.95"
%	 points= "(345,160);(345,160);(345,130);(345,130)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.95"
%	 points= "(335,170);(335,170);(355,150);(355,150)"
%	 />
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(367.5,75)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\Lprogtype$
%</text>
%<multicurve fill-style= "none"
%	 stroke-width= "0.95"
%	 points= "(315,140);(315,140);(335,140);(335,140)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.95"
%	 points= "(355,120);(355,120);(335,140);(335,140)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.95"
%	 points= "(335,120);(335,120);(355,120);(355,120)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.95"
%	 points= "(345,120);(345,120);(345,110);(345,110)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.95"
%	 points= "(325,130);(325,130);(325,110);(325,110)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.95"
%	 points= "(315,140);(315,140);(335,120);(335,120)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.95"
%	 points= "(345,110);(345,110);(335,100);(335,100)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.95"
%	 points= "(325,110);(325,110);(335,100);(335,100)"
%	 />
%<ellipse fill-color= "#330033"
%	 fill-style= "solid"
%	 p3= "(337.57,97.42)"
%	 p2= "(337.57,102.58)"
%	 p1= "(332.43,102.58)"
%	 closure= "open"
%	 angle-end= "0"
%	 angle-start= "0"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.95"
%	 points= "(335,100);(335,100);(335,90);(335,90)"
%	 />
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(367.5,182.5)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\Lprogtype$
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(391.25,210)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\Lprogtype$
%</text>
%<multicurve fill-style= "none"
%	 points= "(336.88,143.75);(336.88,143.75);(357.5,123.12);(357.5,123.12)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(312.5,143.75);(312.5,143.75);(312.5,80);(312.5,80)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(357.5,123.12);(357.5,123.12);(357.5,80);(357.5,80)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(312.5,80);(312.5,80);(335,57.5);(335,57.5)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(357.5,80);(357.5,80);(335,57.5);(335,57.5)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(305,175);(305,175);(305,45);(305,45)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(385,175);(385,175);(385,45);(385,45)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(305,45);(305,45);(345,5);(345,5)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(385,45);(385,45);(345,5);(345,5)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(305,175);(305,175);(385,175);(385,175)"
%	 />
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(420,220)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\ltag$
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(345,15)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\Cprog$
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(335,67.5)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\Gprog$
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(330,85)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\Sprog$
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(335,130)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\stag$
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(395,190)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\ltag$
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(370,160)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\ltag$
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(392.5,5)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\Hprogtype$
%</text>
%<multicurve fill-style= "none"
%	 stroke-width= "0.95"
%	 points= "(225,230);(225,230);(270,230);(270,230)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.95"
%	 points= "(270,210);(270,210);(270,230);(270,230)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.95"
%	 points= "(260,245);(260,245);(260,230);(260,230)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.95"
%	 points= "(245,210);(245,210);(270,210);(270,210)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.95"
%	 points= "(260,210);(260,210);(260,0);(260,0)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.95"
%	 points= "(225,230);(225,230);(245,210);(245,210)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.95"
%	 points= "(200,200);(200,200);(245,200);(245,200)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.95"
%	 points= "(200,67.5);(200,67.5);(200,47.5);(200,47.5)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.95"
%	 points= "(245,180);(245,180);(245,200);(245,200)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.95"
%	 points= "(235,220);(235,220);(235,200);(235,200)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.95"
%	 points= "(220,180);(220,180);(245,180);(245,180)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.95"
%	 points= "(235,180);(235,180);(235,0);(235,0)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.95"
%	 points= "(200,47.5);(200,47.5);(220,47.5);(220,47.5)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.95"
%	 points= "(200,67.5);(200,67.5);(220,47.5);(220,47.5)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.95"
%	 points= "(210,190);(210,190);(210,170);(210,170)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.95"
%	 points= "(200,200);(200,200);(220,180);(220,180)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.95"
%	 points= "(155,120);(155,120);(155,100);(155,100)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.95"
%	 points= "(155,100);(155,100);(175,100);(175,100)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.95"
%	 points= "(155,120);(155,120);(175,100);(175,100)"
%	 />
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(205,52.5)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\itag$
%</text>
%<multicurve fill-style= "none"
%	 stroke-width= "0.95"
%	 points= "(175,170);(175,170);(220,170);(220,170)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.95"
%	 points= "(220,150);(220,150);(220,170);(220,170)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.95"
%	 points= "(195,150);(195,150);(220,150);(220,150)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.95"
%	 points= "(210,150);(210,150);(210,57.5);(210,57.5)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.95"
%	 points= "(185,160);(185,160);(185,130);(185,130)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.95"
%	 points= "(175,170);(175,170);(195,150);(195,150)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.95"
%	 points= "(155,140);(155,140);(175,140);(175,140)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.95"
%	 points= "(195,120);(195,120);(175,140);(175,140)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.95"
%	 points= "(175,120);(175,120);(195,120);(195,120)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.95"
%	 points= "(185,120);(185,120);(185,83.75);(185,83.75)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.95"
%	 points= "(165,130);(165,130);(165,110);(165,110)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.95"
%	 points= "(155,140);(155,140);(175,120);(175,120)"
%	 />
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(207.5,182.5)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\Lprogtype$
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(231.25,210)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\Lprogtype$
%</text>
%<multicurve fill-style= "none"
%	 points= "(150,175);(150,175);(150,45);(150,45)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(225,175);(225,175);(225,45);(225,45)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(150,45);(150,45);(187.5,7.5);(187.5,7.5)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(225,45);(225,45);(187.5,7.5);(187.5,7.5)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(150,175);(150,175);(225,175);(225,175)"
%	 />
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(260,220)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\ltag$
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(187.5,16.25)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\Cprog$
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(160,105)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\Sprog$
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(175,130)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\stag$
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(235,190)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\ltag$
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(210,160)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\ltag$
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(232.5,5)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\Hprogtype$
%</text>
%<multicurve fill-style= "none"
%	 stroke-width= "0.95"
%	 points= "(175,93.75);(175,93.75);(175,73.75);(175,73.75)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.95"
%	 points= "(175,73.75);(175,73.75);(195,73.75);(195,73.75)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.95"
%	 points= "(175,93.75);(175,93.75);(195,73.75);(195,73.75)"
%	 />
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(180,78.75)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\Sprog$
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(295,210)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\EQLSsix
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(145,210)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\EQLSfive
%</text>
%<multicurve fill-style= "none"
%	 stroke-width= "0.95"
%	 points= "(70,230);(70,230);(115,230);(115,230)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.95"
%	 points= "(115,210);(115,210);(115,230);(115,230)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.95"
%	 points= "(105,245);(105,245);(105,230);(105,230)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.95"
%	 points= "(90,210);(90,210);(115,210);(115,210)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.95"
%	 points= "(105,210);(105,210);(105,27.5);(105,27.5)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.95"
%	 points= "(70,230);(70,230);(90,210);(90,210)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.95"
%	 points= "(45,200);(45,200);(90,200);(90,200)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.95"
%	 points= "(45,97.5);(45,97.5);(45,77.5);(45,77.5)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.95"
%	 points= "(90,180);(90,180);(90,200);(90,200)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.95"
%	 points= "(80,220);(80,220);(80,200);(80,200)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.95"
%	 points= "(65,180);(65,180);(90,180);(90,180)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.95"
%	 points= "(80,180);(80,180);(80,27.5);(80,27.5)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.95"
%	 points= "(45,77.5);(45,77.5);(65,77.5);(65,77.5)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.95"
%	 points= "(45,97.5);(45,97.5);(65,77.5);(65,77.5)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.95"
%	 points= "(55,190);(55,190);(55,170);(55,170)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.95"
%	 points= "(45,200);(45,200);(65,180);(65,180)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.95"
%	 points= "(0,150);(0,150);(0,130);(0,130)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.95"
%	 points= "(0,130);(0,130);(20,130);(20,130)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.95"
%	 points= "(0,150);(0,150);(20,130);(20,130)"
%	 />
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(50,82.5)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\itag$
%</text>
%<multicurve fill-style= "none"
%	 stroke-width= "0.95"
%	 points= "(0,170);(0,170);(65,170);(65,170)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.95"
%	 points= "(65,150);(65,150);(65,170);(65,170)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.95"
%	 points= "(20,150);(20,150);(65,150);(65,150)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.95"
%	 points= "(55,150);(55,150);(55,87.5);(55,87.5)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.95"
%	 points= "(30,150);(30,150);(30,115);(30,115)"
%	 />
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(52.5,102.5)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\Lprogtype$
%</text>
%<multicurve fill-style= "none"
%	 stroke-width= "0.95"
%	 points= "(10,160);(10,160);(10,140);(10,140)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.95"
%	 points= "(0,170);(0,170);(20,150);(20,150)"
%	 />
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(52.5,182.5)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\Lprogtype$
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(76.25,210)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\Lprogtype$
%</text>
%<multicurve fill-style= "none"
%	 points= "(-5,175);(-5,175);(-5,77.5);(-5,77.5)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(70,175);(70,175);(70,77.5);(70,77.5)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(-5,77.5);(-5,77.5);(32.5,40);(32.5,40)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(70,77.5);(70,77.5);(32.5,40);(32.5,40)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(-5,175);(-5,175);(70,175);(70,175)"
%	 />
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(105,220)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\ltag$
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(32.5,50)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\Cprog$
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(5,135)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\Sprog$
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(80,190)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\ltag$
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(55,160)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\ltag$
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(77.5,37.5)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\Hprogtype$
%</text>
%<multicurve fill-style= "none"
%	 stroke-width= "0.95"
%	 points= "(20,125);(20,125);(20,105);(20,105)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.95"
%	 points= "(20,105);(20,105);(40,105);(40,105)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.95"
%	 points= "(20,125);(20,125);(40,105);(40,105)"
%	 />
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(25,110)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\Sprog$
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(27.5,127.5)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\Lprogtype$
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(7.5,155)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\Lprogtype$
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(-5,210)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\EQLSfour
%</text>
%<multicurve fill-style= "none"
%	 points= "(312.5,143.75);(312.5,143.75);(336.88,143.75);(336.88,143.75)"
%	 />
%<ellipse fill-color= "#330033"
%	 fill-style= "solid"
%	 p3= "(337.57,87.42)"
%	 p2= "(337.57,92.58)"
%	 p1= "(332.43,92.58)"
%	 closure= "open"
%	 angle-end= "0"
%	 angle-start= "0"
%	 />
%<ellipse fill-color= "#330033"
%	 fill-style= "solid"
%	 p3= "(372.57,54.92)"
%	 p2= "(372.57,60.08)"
%	 p1= "(367.43,60.08)"
%	 closure= "open"
%	 angle-end= "0"
%	 angle-start= "0"
%	 />
%</jpic>
%%End JPIC-XML
%LaTeX-picture environment using emulated lines and arcs
%You can rescale the whole picture (to 80% for instance) by using the command \def\JPicScale{0.8}
\ifx\JPicScale\undefined\def\JPicScale{1}\fi
\unitlength \JPicScale mm
\begin{picture}(430,245)(0,0)
\linethickness{0.95mm}
\put(385,230){\line(1,0){45}}
\linethickness{0.95mm}
\put(430,210){\line(0,1){20}}
\linethickness{0.95mm}
\put(420,230){\line(0,1){15}}
\linethickness{0.95mm}
\put(405,210){\line(1,0){25}}
\linethickness{0.95mm}
\put(420,0){\line(0,1){210}}
\linethickness{0.95mm}
\multiput(385,230)(0.12,-0.12){167}{\line(1,0){0.12}}
\linethickness{0.95mm}
\put(360,200){\line(1,0){45}}
\linethickness{0.95mm}
\put(360,47.5){\line(0,1){20}}
\linethickness{0.95mm}
\put(405,180){\line(0,1){20}}
\linethickness{0.95mm}
\put(395,200){\line(0,1){20}}
\linethickness{0.95mm}
\put(380,180){\line(1,0){25}}
\linethickness{0.95mm}
\put(395,0){\line(0,1){180}}
\linethickness{0.95mm}
\put(360,47.5){\line(1,0){20}}
\linethickness{0.95mm}
\multiput(360,67.5)(0.12,-0.12){167}{\line(1,0){0.12}}
\linethickness{0.95mm}
\put(370,170){\line(0,1){20}}
\linethickness{0.95mm}
\multiput(360,200)(0.12,-0.12){167}{\line(1,0){0.12}}
\linethickness{0.95mm}
\put(325,80){\line(0,1){20}}
\linethickness{0.95mm}
\put(325,80){\line(1,0){20}}
\linethickness{0.95mm}
\multiput(325,100)(0.12,-0.12){167}{\line(1,0){0.12}}
\put(365,52.5){\makebox(0,0)[cc]{$\itag$}}

\linethickness{0.95mm}
\put(335,170){\line(1,0){45}}
\linethickness{0.95mm}
\put(380,150){\line(0,1){20}}
\linethickness{0.95mm}
\put(355,150){\line(1,0){25}}
\linethickness{0.95mm}
\put(370,57.5){\line(0,1){92.5}}
\linethickness{0.95mm}
\put(345,130){\line(0,1){30}}
\linethickness{0.95mm}
\multiput(335,170)(0.12,-0.12){167}{\line(1,0){0.12}}
\put(367.5,75){\makebox(0,0)[cr]{$\Lprogtype$}}

\linethickness{0.95mm}
\put(315,140){\line(1,0){20}}
\linethickness{0.95mm}
\multiput(335,140)(0.12,-0.12){167}{\line(1,0){0.12}}
\linethickness{0.95mm}
\put(335,120){\line(1,0){20}}
\linethickness{0.95mm}
\put(345,110){\line(0,1){10}}
\linethickness{0.95mm}
\put(325,110){\line(0,1){20}}
\linethickness{0.95mm}
\multiput(315,140)(0.12,-0.12){167}{\line(1,0){0.12}}
\linethickness{0.95mm}
\multiput(335,100)(0.12,0.12){83}{\line(1,0){0.12}}
\linethickness{0.95mm}
\multiput(325,110)(0.12,-0.12){83}{\line(1,0){0.12}}
\linethickness{0.3mm}
\put(337.56,99.75){\line(0,1){0.51}}
\multiput(337.46,99.25)(0.1,0.5){1}{\line(0,1){0.5}}
\multiput(337.27,98.78)(0.1,0.23){2}{\line(0,1){0.23}}
\multiput(336.99,98.36)(0.14,0.21){2}{\line(0,1){0.21}}
\multiput(336.63,98.01)(0.12,0.12){3}{\line(0,1){0.12}}
\multiput(336.21,97.72)(0.21,0.14){2}{\line(1,0){0.21}}
\multiput(335.75,97.53)(0.23,0.1){2}{\line(1,0){0.23}}
\multiput(335.25,97.43)(0.49,0.1){1}{\line(1,0){0.49}}
\put(334.75,97.43){\line(1,0){0.5}}
\multiput(334.25,97.53)(0.49,-0.1){1}{\line(1,0){0.49}}
\multiput(333.79,97.72)(0.23,-0.1){2}{\line(1,0){0.23}}
\multiput(333.37,98.01)(0.21,-0.14){2}{\line(1,0){0.21}}
\multiput(333.01,98.36)(0.12,-0.12){3}{\line(0,-1){0.12}}
\multiput(332.73,98.78)(0.14,-0.21){2}{\line(0,-1){0.21}}
\multiput(332.54,99.25)(0.1,-0.23){2}{\line(0,-1){0.23}}
\multiput(332.44,99.75)(0.1,-0.5){1}{\line(0,-1){0.5}}
\put(332.44,99.75){\line(0,1){0.51}}
\multiput(332.44,100.25)(0.1,0.5){1}{\line(0,1){0.5}}
\multiput(332.54,100.75)(0.1,0.23){2}{\line(0,1){0.23}}
\multiput(332.73,101.22)(0.14,0.21){2}{\line(0,1){0.21}}
\multiput(333.01,101.64)(0.12,0.12){3}{\line(0,1){0.12}}
\multiput(333.37,101.99)(0.21,0.14){2}{\line(1,0){0.21}}
\multiput(333.79,102.28)(0.23,0.1){2}{\line(1,0){0.23}}
\multiput(334.25,102.47)(0.49,0.1){1}{\line(1,0){0.49}}
\put(334.75,102.57){\line(1,0){0.5}}
\multiput(335.25,102.57)(0.49,-0.1){1}{\line(1,0){0.49}}
\multiput(335.75,102.47)(0.23,-0.1){2}{\line(1,0){0.23}}
\multiput(336.21,102.28)(0.21,-0.14){2}{\line(1,0){0.21}}
\multiput(336.63,101.99)(0.12,-0.12){3}{\line(0,-1){0.12}}
\multiput(336.99,101.64)(0.14,-0.21){2}{\line(0,-1){0.21}}
\multiput(337.27,101.22)(0.1,-0.23){2}{\line(0,-1){0.23}}
\multiput(337.46,100.75)(0.1,-0.5){1}{\line(0,-1){0.5}}

\linethickness{0.95mm}
\put(335,90){\line(0,1){10}}
\put(367.5,182.5){\makebox(0,0)[cr]{$\Lprogtype$}}

\put(391.25,210){\makebox(0,0)[cr]{$\Lprogtype$}}

\linethickness{0.3mm}
\multiput(336.88,143.75)(0.12,-0.12){172}{\line(0,-1){0.12}}
\linethickness{0.3mm}
\put(312.5,80){\line(0,1){63.75}}
\linethickness{0.3mm}
\put(357.5,80){\line(0,1){43.12}}
\linethickness{0.3mm}
\multiput(312.5,80)(0.12,-0.12){188}{\line(1,0){0.12}}
\linethickness{0.3mm}
\multiput(335,57.5)(0.12,0.12){188}{\line(1,0){0.12}}
\linethickness{0.3mm}
\put(305,45){\line(0,1){130}}
\linethickness{0.3mm}
\put(385,45){\line(0,1){130}}
\linethickness{0.3mm}
\multiput(305,45)(0.12,-0.12){333}{\line(1,0){0.12}}
\linethickness{0.3mm}
\multiput(345,5)(0.12,0.12){333}{\line(1,0){0.12}}
\linethickness{0.3mm}
\put(305,175){\line(1,0){80}}
\put(420,220){\makebox(0,0)[cc]{$\ltag$}}

\put(345,15){\makebox(0,0)[cc]{$\Cprog$}}

\put(335,67.5){\makebox(0,0)[cc]{$\Gprog$}}

\put(330,85){\makebox(0,0)[cc]{$\Sprog$}}

\put(335,130){\makebox(0,0)[cc]{$\stag$}}

\put(395,190){\makebox(0,0)[cc]{$\ltag$}}

\put(370,160){\makebox(0,0)[cc]{$\ltag$}}

\put(392.5,5){\makebox(0,0)[cr]{$\Hprogtype$}}

\linethickness{0.95mm}
\put(225,230){\line(1,0){45}}
\linethickness{0.95mm}
\put(270,210){\line(0,1){20}}
\linethickness{0.95mm}
\put(260,230){\line(0,1){15}}
\linethickness{0.95mm}
\put(245,210){\line(1,0){25}}
\linethickness{0.95mm}
\put(260,0){\line(0,1){210}}
\linethickness{0.95mm}
\multiput(225,230)(0.12,-0.12){167}{\line(1,0){0.12}}
\linethickness{0.95mm}
\put(200,200){\line(1,0){45}}
\linethickness{0.95mm}
\put(200,47.5){\line(0,1){20}}
\linethickness{0.95mm}
\put(245,180){\line(0,1){20}}
\linethickness{0.95mm}
\put(235,200){\line(0,1){20}}
\linethickness{0.95mm}
\put(220,180){\line(1,0){25}}
\linethickness{0.95mm}
\put(235,0){\line(0,1){180}}
\linethickness{0.95mm}
\put(200,47.5){\line(1,0){20}}
\linethickness{0.95mm}
\multiput(200,67.5)(0.12,-0.12){167}{\line(1,0){0.12}}
\linethickness{0.95mm}
\put(210,170){\line(0,1){20}}
\linethickness{0.95mm}
\multiput(200,200)(0.12,-0.12){167}{\line(1,0){0.12}}
\linethickness{0.95mm}
\put(155,100){\line(0,1){20}}
\linethickness{0.95mm}
\put(155,100){\line(1,0){20}}
\linethickness{0.95mm}
\multiput(155,120)(0.12,-0.12){167}{\line(1,0){0.12}}
\put(205,52.5){\makebox(0,0)[cc]{$\itag$}}

\linethickness{0.95mm}
\put(175,170){\line(1,0){45}}
\linethickness{0.95mm}
\put(220,150){\line(0,1){20}}
\linethickness{0.95mm}
\put(195,150){\line(1,0){25}}
\linethickness{0.95mm}
\put(210,57.5){\line(0,1){92.5}}
\linethickness{0.95mm}
\put(185,130){\line(0,1){30}}
\linethickness{0.95mm}
\multiput(175,170)(0.12,-0.12){167}{\line(1,0){0.12}}
\linethickness{0.95mm}
\put(155,140){\line(1,0){20}}
\linethickness{0.95mm}
\multiput(175,140)(0.12,-0.12){167}{\line(1,0){0.12}}
\linethickness{0.95mm}
\put(175,120){\line(1,0){20}}
\linethickness{0.95mm}
\put(185,83.75){\line(0,1){36.25}}
\linethickness{0.95mm}
\put(165,110){\line(0,1){20}}
\linethickness{0.95mm}
\multiput(155,140)(0.12,-0.12){167}{\line(1,0){0.12}}
\put(207.5,182.5){\makebox(0,0)[cr]{$\Lprogtype$}}

\put(231.25,210){\makebox(0,0)[cr]{$\Lprogtype$}}

\linethickness{0.3mm}
\put(150,45){\line(0,1){130}}
\linethickness{0.3mm}
\put(225,45){\line(0,1){130}}
\linethickness{0.3mm}
\multiput(150,45)(0.12,-0.12){313}{\line(1,0){0.12}}
\linethickness{0.3mm}
\multiput(187.5,7.5)(0.12,0.12){313}{\line(1,0){0.12}}
\linethickness{0.3mm}
\put(150,175){\line(1,0){75}}
\put(260,220){\makebox(0,0)[cc]{$\ltag$}}

\put(187.5,16.25){\makebox(0,0)[cc]{$\Cprog$}}

\put(160,105){\makebox(0,0)[cc]{$\Sprog$}}

\put(175,130){\makebox(0,0)[cc]{$\stag$}}

\put(235,190){\makebox(0,0)[cc]{$\ltag$}}

\put(210,160){\makebox(0,0)[cc]{$\ltag$}}

\put(232.5,5){\makebox(0,0)[cr]{$\Hprogtype$}}

\linethickness{0.95mm}
\put(175,73.75){\line(0,1){20}}
\linethickness{0.95mm}
\put(175,73.75){\line(1,0){20}}
\linethickness{0.95mm}
\multiput(175,93.75)(0.12,-0.12){167}{\line(1,0){0.12}}
\put(180,78.75){\makebox(0,0)[cc]{$\Sprog$}}

\put(295,210){\makebox(0,0)[cc]{\EQLSsix}}

\put(145,210){\makebox(0,0)[cc]{\EQLSfive}}

\linethickness{0.95mm}
\put(70,230){\line(1,0){45}}
\linethickness{0.95mm}
\put(115,210){\line(0,1){20}}
\linethickness{0.95mm}
\put(105,230){\line(0,1){15}}
\linethickness{0.95mm}
\put(90,210){\line(1,0){25}}
\linethickness{0.95mm}
\put(105,27.5){\line(0,1){182.5}}
\linethickness{0.95mm}
\multiput(70,230)(0.12,-0.12){167}{\line(1,0){0.12}}
\linethickness{0.95mm}
\put(45,200){\line(1,0){45}}
\linethickness{0.95mm}
\put(45,77.5){\line(0,1){20}}
\linethickness{0.95mm}
\put(90,180){\line(0,1){20}}
\linethickness{0.95mm}
\put(80,200){\line(0,1){20}}
\linethickness{0.95mm}
\put(65,180){\line(1,0){25}}
\linethickness{0.95mm}
\put(80,27.5){\line(0,1){152.5}}
\linethickness{0.95mm}
\put(45,77.5){\line(1,0){20}}
\linethickness{0.95mm}
\multiput(45,97.5)(0.12,-0.12){167}{\line(1,0){0.12}}
\linethickness{0.95mm}
\put(55,170){\line(0,1){20}}
\linethickness{0.95mm}
\multiput(45,200)(0.12,-0.12){167}{\line(1,0){0.12}}
\linethickness{0.95mm}
\put(0,130){\line(0,1){20}}
\linethickness{0.95mm}
\put(0,130){\line(1,0){20}}
\linethickness{0.95mm}
\multiput(0,150)(0.12,-0.12){167}{\line(1,0){0.12}}
\put(50,82.5){\makebox(0,0)[cc]{$\itag$}}

\linethickness{0.95mm}
\put(0,170){\line(1,0){65}}
\linethickness{0.95mm}
\put(65,150){\line(0,1){20}}
\linethickness{0.95mm}
\put(20,150){\line(1,0){45}}
\linethickness{0.95mm}
\put(55,87.5){\line(0,1){62.5}}
\linethickness{0.95mm}
\put(30,115){\line(0,1){35}}
\put(52.5,102.5){\makebox(0,0)[cr]{$\Lprogtype$}}

\linethickness{0.95mm}
\put(10,140){\line(0,1){20}}
\linethickness{0.95mm}
\multiput(0,170)(0.12,-0.12){167}{\line(1,0){0.12}}
\put(52.5,182.5){\makebox(0,0)[cr]{$\Lprogtype$}}

\put(76.25,210){\makebox(0,0)[cr]{$\Lprogtype$}}

\linethickness{0.3mm}
\put(-5,77.5){\line(0,1){97.5}}
\linethickness{0.3mm}
\put(70,77.5){\line(0,1){97.5}}
\linethickness{0.3mm}
\multiput(-5,77.5)(0.12,-0.12){313}{\line(1,0){0.12}}
\linethickness{0.3mm}
\multiput(32.5,40)(0.12,0.12){313}{\line(1,0){0.12}}
\linethickness{0.3mm}
\put(-5,175){\line(1,0){75}}
\put(105,220){\makebox(0,0)[cc]{$\ltag$}}

\put(32.5,50){\makebox(0,0)[cc]{$\Cprog$}}

\put(5,135){\makebox(0,0)[cc]{$\Sprog$}}

\put(80,190){\makebox(0,0)[cc]{$\ltag$}}

\put(55,160){\makebox(0,0)[cc]{$\ltag$}}

\put(77.5,37.5){\makebox(0,0)[cr]{$\Hprogtype$}}

\linethickness{0.95mm}
\put(20,105){\line(0,1){20}}
\linethickness{0.95mm}
\put(20,105){\line(1,0){20}}
\linethickness{0.95mm}
\multiput(20,125)(0.12,-0.12){167}{\line(1,0){0.12}}
\put(25,110){\makebox(0,0)[cc]{$\Sprog$}}

\put(27.5,127.5){\makebox(0,0)[cr]{$\Lprogtype$}}

\put(7.5,155){\makebox(0,0)[cr]{$\Lprogtype$}}

\put(-5,210){\makebox(0,0)[cc]{\EQLSfour}}

\linethickness{0.3mm}
\put(312.5,143.75){\line(1,0){24.38}}
\linethickness{0.3mm}
\put(337.56,89.75){\line(0,1){0.51}}
\multiput(337.46,89.25)(0.1,0.5){1}{\line(0,1){0.5}}
\multiput(337.27,88.78)(0.1,0.23){2}{\line(0,1){0.23}}
\multiput(336.99,88.36)(0.14,0.21){2}{\line(0,1){0.21}}
\multiput(336.63,88.01)(0.12,0.12){3}{\line(0,1){0.12}}
\multiput(336.21,87.72)(0.21,0.14){2}{\line(1,0){0.21}}
\multiput(335.75,87.53)(0.23,0.1){2}{\line(1,0){0.23}}
\multiput(335.25,87.43)(0.49,0.1){1}{\line(1,0){0.49}}
\put(334.75,87.43){\line(1,0){0.5}}
\multiput(334.25,87.53)(0.49,-0.1){1}{\line(1,0){0.49}}
\multiput(333.79,87.72)(0.23,-0.1){2}{\line(1,0){0.23}}
\multiput(333.37,88.01)(0.21,-0.14){2}{\line(1,0){0.21}}
\multiput(333.01,88.36)(0.12,-0.12){3}{\line(0,-1){0.12}}
\multiput(332.73,88.78)(0.14,-0.21){2}{\line(0,-1){0.21}}
\multiput(332.54,89.25)(0.1,-0.23){2}{\line(0,-1){0.23}}
\multiput(332.44,89.75)(0.1,-0.5){1}{\line(0,-1){0.5}}
\put(332.44,89.75){\line(0,1){0.51}}
\multiput(332.44,90.25)(0.1,0.5){1}{\line(0,1){0.5}}
\multiput(332.54,90.75)(0.1,0.23){2}{\line(0,1){0.23}}
\multiput(332.73,91.22)(0.14,0.21){2}{\line(0,1){0.21}}
\multiput(333.01,91.64)(0.12,0.12){3}{\line(0,1){0.12}}
\multiput(333.37,91.99)(0.21,0.14){2}{\line(1,0){0.21}}
\multiput(333.79,92.28)(0.23,0.1){2}{\line(1,0){0.23}}
\multiput(334.25,92.47)(0.49,0.1){1}{\line(1,0){0.49}}
\put(334.75,92.57){\line(1,0){0.5}}
\multiput(335.25,92.57)(0.49,-0.1){1}{\line(1,0){0.49}}
\multiput(335.75,92.47)(0.23,-0.1){2}{\line(1,0){0.23}}
\multiput(336.21,92.28)(0.21,-0.14){2}{\line(1,0){0.21}}
\multiput(336.63,91.99)(0.12,-0.12){3}{\line(0,-1){0.12}}
\multiput(336.99,91.64)(0.14,-0.21){2}{\line(0,-1){0.21}}
\multiput(337.27,91.22)(0.1,-0.23){2}{\line(0,-1){0.23}}
\multiput(337.46,90.75)(0.1,-0.5){1}{\line(0,-1){0.5}}

\linethickness{0.3mm}
\put(372.56,57.25){\line(0,1){0.51}}
\multiput(372.46,56.75)(0.1,0.5){1}{\line(0,1){0.5}}
\multiput(372.27,56.28)(0.1,0.23){2}{\line(0,1){0.23}}
\multiput(371.99,55.86)(0.14,0.21){2}{\line(0,1){0.21}}
\multiput(371.63,55.51)(0.12,0.12){3}{\line(0,1){0.12}}
\multiput(371.21,55.22)(0.21,0.14){2}{\line(1,0){0.21}}
\multiput(370.75,55.03)(0.23,0.1){2}{\line(1,0){0.23}}
\multiput(370.25,54.93)(0.49,0.1){1}{\line(1,0){0.49}}
\put(369.75,54.93){\line(1,0){0.5}}
\multiput(369.25,55.03)(0.49,-0.1){1}{\line(1,0){0.49}}
\multiput(368.79,55.22)(0.23,-0.1){2}{\line(1,0){0.23}}
\multiput(368.37,55.51)(0.21,-0.14){2}{\line(1,0){0.21}}
\multiput(368.01,55.86)(0.12,-0.12){3}{\line(0,-1){0.12}}
\multiput(367.73,56.28)(0.14,-0.21){2}{\line(0,-1){0.21}}
\multiput(367.54,56.75)(0.1,-0.23){2}{\line(0,-1){0.23}}
\multiput(367.44,57.25)(0.1,-0.5){1}{\line(0,-1){0.5}}
\put(367.44,57.25){\line(0,1){0.51}}
\multiput(367.44,57.75)(0.1,0.5){1}{\line(0,1){0.5}}
\multiput(367.54,58.25)(0.1,0.23){2}{\line(0,1){0.23}}
\multiput(367.73,58.72)(0.14,0.21){2}{\line(0,1){0.21}}
\multiput(368.01,59.14)(0.12,0.12){3}{\line(0,1){0.12}}
\multiput(368.37,59.49)(0.21,0.14){2}{\line(1,0){0.21}}
\multiput(368.79,59.78)(0.23,0.1){2}{\line(1,0){0.23}}
\multiput(369.25,59.97)(0.49,0.1){1}{\line(1,0){0.49}}
\put(369.75,60.07){\line(1,0){0.5}}
\multiput(370.25,60.07)(0.49,-0.1){1}{\line(1,0){0.49}}
\multiput(370.75,59.97)(0.23,-0.1){2}{\line(1,0){0.23}}
\multiput(371.21,59.78)(0.21,-0.14){2}{\line(1,0){0.21}}
\multiput(371.63,59.49)(0.12,-0.12){3}{\line(0,-1){0.12}}
\multiput(371.99,59.14)(0.14,-0.21){2}{\line(0,-1){0.21}}
\multiput(372.27,58.72)(0.1,-0.23){2}{\line(0,-1){0.23}}
\multiput(372.46,58.25)(0.1,-0.5){1}{\line(0,-1){0.5}}

\end{picture}


==> PIC/futamura-trd.tex <==
%%Created by jPicEdt 1.4.1_03: mixed JPIC-XML/LaTeX format
%%Sat Nov 24 16:54:43 GMT-10:00 2018
%%Begin JPIC-XML
%<?xml version="1.0" standalone="yes"?>
%<jpic x-min="-5" x-max="430" y-min="0" y-max="245" auto-bounding="true">
%<multicurve fill-style= "none"
%	 points= "(385,230);(385,230);(430,230);(430,230)"
%	 stroke-width= "0.95"
%	 />
%<multicurve fill-style= "none"
%	 points= "(430,210);(430,210);(430,230);(430,230)"
%	 stroke-width= "0.95"
%	 />
%<multicurve fill-style= "none"
%	 points= "(420,245);(420,245);(420,230);(420,230)"
%	 stroke-width= "0.95"
%	 />
%<multicurve fill-style= "none"
%	 points= "(405,210);(405,210);(430,210);(430,210)"
%	 stroke-width= "0.95"
%	 />
%<multicurve fill-style= "none"
%	 points= "(420,210);(420,210);(420,0);(420,0)"
%	 stroke-width= "0.95"
%	 />
%<multicurve fill-style= "none"
%	 points= "(385,230);(385,230);(405,210);(405,210)"
%	 stroke-width= "0.95"
%	 />
%<multicurve fill-style= "none"
%	 points= "(360,200);(360,200);(405,200);(405,200)"
%	 stroke-width= "0.95"
%	 />
%<multicurve fill-style= "none"
%	 points= "(360,67.5);(360,67.5);(360,47.5);(360,47.5)"
%	 stroke-width= "0.95"
%	 />
%<multicurve fill-style= "none"
%	 points= "(405,180);(405,180);(405,200);(405,200)"
%	 stroke-width= "0.95"
%	 />
%<multicurve fill-style= "none"
%	 points= "(395,220);(395,220);(395,200);(395,200)"
%	 stroke-width= "0.95"
%	 />
%<multicurve fill-style= "none"
%	 points= "(380,180);(380,180);(405,180);(405,180)"
%	 stroke-width= "0.95"
%	 />
%<multicurve fill-style= "none"
%	 points= "(395,180);(395,180);(395,0);(395,0)"
%	 stroke-width= "0.95"
%	 />
%<multicurve fill-style= "none"
%	 points= "(360,47.5);(360,47.5);(380,47.5);(380,47.5)"
%	 stroke-width= "0.95"
%	 />
%<multicurve fill-style= "none"
%	 points= "(360,67.5);(360,67.5);(380,47.5);(380,47.5)"
%	 stroke-width= "0.95"
%	 />
%<multicurve fill-style= "none"
%	 points= "(370,190);(370,190);(370,170);(370,170)"
%	 stroke-width= "0.95"
%	 />
%<multicurve fill-style= "none"
%	 points= "(360,200);(360,200);(380,180);(380,180)"
%	 stroke-width= "0.95"
%	 />
%<multicurve fill-style= "none"
%	 points= "(325,100);(325,100);(325,80);(325,80)"
%	 stroke-width= "0.95"
%	 />
%<multicurve fill-style= "none"
%	 points= "(325,80);(325,80);(345,80);(345,80)"
%	 stroke-width= "0.95"
%	 />
%<multicurve fill-style= "none"
%	 points= "(325,100);(325,100);(345,80);(345,80)"
%	 stroke-width= "0.95"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(365,52.5)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\itag$
%</text>
%<multicurve fill-style= "none"
%	 points= "(335,170);(335,170);(380,170);(380,170)"
%	 stroke-width= "0.95"
%	 />
%<multicurve fill-style= "none"
%	 points= "(380,150);(380,150);(380,170);(380,170)"
%	 stroke-width= "0.95"
%	 />
%<multicurve fill-style= "none"
%	 points= "(355,150);(355,150);(380,150);(380,150)"
%	 stroke-width= "0.95"
%	 />
%<multicurve fill-style= "none"
%	 points= "(370,150);(370,150);(370,57.5);(370,57.5)"
%	 stroke-width= "0.95"
%	 />
%<multicurve fill-style= "none"
%	 points= "(345,160);(345,160);(345,130);(345,130)"
%	 stroke-width= "0.95"
%	 />
%<multicurve fill-style= "none"
%	 points= "(335,170);(335,170);(355,150);(355,150)"
%	 stroke-width= "0.95"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(367.5,75)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\Lprogtype$
%</text>
%<multicurve fill-style= "none"
%	 points= "(315,140);(315,140);(335,140);(335,140)"
%	 stroke-width= "0.95"
%	 />
%<multicurve fill-style= "none"
%	 points= "(355,120);(355,120);(335,140);(335,140)"
%	 stroke-width= "0.95"
%	 />
%<multicurve fill-style= "none"
%	 points= "(335,120);(335,120);(355,120);(355,120)"
%	 stroke-width= "0.95"
%	 />
%<multicurve fill-style= "none"
%	 points= "(345,120);(345,120);(345,110);(345,110)"
%	 stroke-width= "0.95"
%	 />
%<multicurve fill-style= "none"
%	 points= "(325,130);(325,130);(325,110);(325,110)"
%	 stroke-width= "0.95"
%	 />
%<multicurve fill-style= "none"
%	 points= "(315,140);(315,140);(335,120);(335,120)"
%	 stroke-width= "0.95"
%	 />
%<multicurve fill-style= "none"
%	 points= "(345,110);(345,110);(335,100);(335,100)"
%	 stroke-width= "0.95"
%	 />
%<multicurve fill-style= "none"
%	 points= "(325,110);(325,110);(335,100);(335,100)"
%	 stroke-width= "0.95"
%	 />
%<ellipse p3= "(337.57,97.42)"
%	 fill-style= "solid"
%	 p2= "(337.57,102.58)"
%	 fill-color= "#330033"
%	 p1= "(332.43,102.58)"
%	 closure= "open"
%	 angle-end= "0"
%	 angle-start= "0"
%	 />
%<multicurve fill-style= "none"
%	 points= "(335,100);(335,100);(335,90);(335,90)"
%	 stroke-width= "0.95"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(367.5,182.5)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\Lprogtype$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(391.25,210)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\Lprogtype$
%</text>
%<multicurve fill-style= "none"
%	 points= "(336.88,143.75);(336.88,143.75);(357.5,123.12);(357.5,123.12)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(312.5,143.75);(312.5,143.75);(312.5,80);(312.5,80)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(357.5,123.12);(357.5,123.12);(357.5,80);(357.5,80)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(312.5,80);(312.5,80);(335,57.5);(335,57.5)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(357.5,80);(357.5,80);(335,57.5);(335,57.5)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(305,175);(305,175);(305,45);(305,45)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(385,175);(385,175);(385,45);(385,45)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(305,45);(305,45);(345,5);(345,5)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(385,45);(385,45);(345,5);(345,5)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(305,175);(305,175);(385,175);(385,175)"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(420,220)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\ltag$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(345,15)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\Cprog$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(335,67.5)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\Gprog$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(330,85)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\Sprog$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(335,130)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\stag$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(395,190)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\ltag$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(370,160)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\ltag$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(392.5,5)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\Hprogtype$
%</text>
%<multicurve fill-style= "none"
%	 points= "(225,230);(225,230);(270,230);(270,230)"
%	 stroke-width= "0.95"
%	 />
%<multicurve fill-style= "none"
%	 points= "(270,210);(270,210);(270,230);(270,230)"
%	 stroke-width= "0.95"
%	 />
%<multicurve fill-style= "none"
%	 points= "(260,245);(260,245);(260,230);(260,230)"
%	 stroke-width= "0.95"
%	 />
%<multicurve fill-style= "none"
%	 points= "(245,210);(245,210);(270,210);(270,210)"
%	 stroke-width= "0.95"
%	 />
%<multicurve fill-style= "none"
%	 points= "(260,210);(260,210);(260,0);(260,0)"
%	 stroke-width= "0.95"
%	 />
%<multicurve fill-style= "none"
%	 points= "(225,230);(225,230);(245,210);(245,210)"
%	 stroke-width= "0.95"
%	 />
%<multicurve fill-style= "none"
%	 points= "(200,200);(200,200);(245,200);(245,200)"
%	 stroke-width= "0.95"
%	 />
%<multicurve fill-style= "none"
%	 points= "(200,67.5);(200,67.5);(200,47.5);(200,47.5)"
%	 stroke-width= "0.95"
%	 />
%<multicurve fill-style= "none"
%	 points= "(245,180);(245,180);(245,200);(245,200)"
%	 stroke-width= "0.95"
%	 />
%<multicurve fill-style= "none"
%	 points= "(235,220);(235,220);(235,200);(235,200)"
%	 stroke-width= "0.95"
%	 />
%<multicurve fill-style= "none"
%	 points= "(220,180);(220,180);(245,180);(245,180)"
%	 stroke-width= "0.95"
%	 />
%<multicurve fill-style= "none"
%	 points= "(235,180);(235,180);(235,0);(235,0)"
%	 stroke-width= "0.95"
%	 />
%<multicurve fill-style= "none"
%	 points= "(200,47.5);(200,47.5);(220,47.5);(220,47.5)"
%	 stroke-width= "0.95"
%	 />
%<multicurve fill-style= "none"
%	 points= "(200,67.5);(200,67.5);(220,47.5);(220,47.5)"
%	 stroke-width= "0.95"
%	 />
%<multicurve fill-style= "none"
%	 points= "(210,190);(210,190);(210,170);(210,170)"
%	 stroke-width= "0.95"
%	 />
%<multicurve fill-style= "none"
%	 points= "(200,200);(200,200);(220,180);(220,180)"
%	 stroke-width= "0.95"
%	 />
%<multicurve fill-style= "none"
%	 points= "(155,120);(155,120);(155,100);(155,100)"
%	 stroke-width= "0.95"
%	 />
%<multicurve fill-style= "none"
%	 points= "(155,100);(155,100);(175,100);(175,100)"
%	 stroke-width= "0.95"
%	 />
%<multicurve fill-style= "none"
%	 points= "(155,120);(155,120);(175,100);(175,100)"
%	 stroke-width= "0.95"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(205,52.5)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\itag$
%</text>
%<multicurve fill-style= "none"
%	 points= "(175,170);(175,170);(220,170);(220,170)"
%	 stroke-width= "0.95"
%	 />
%<multicurve fill-style= "none"
%	 points= "(220,150);(220,150);(220,170);(220,170)"
%	 stroke-width= "0.95"
%	 />
%<multicurve fill-style= "none"
%	 points= "(195,150);(195,150);(220,150);(220,150)"
%	 stroke-width= "0.95"
%	 />
%<multicurve fill-style= "none"
%	 points= "(210,150);(210,150);(210,57.5);(210,57.5)"
%	 stroke-width= "0.95"
%	 />
%<multicurve fill-style= "none"
%	 points= "(185,160);(185,160);(185,130);(185,130)"
%	 stroke-width= "0.95"
%	 />
%<multicurve fill-style= "none"
%	 points= "(175,170);(175,170);(195,150);(195,150)"
%	 stroke-width= "0.95"
%	 />
%<multicurve fill-style= "none"
%	 points= "(155,140);(155,140);(175,140);(175,140)"
%	 stroke-width= "0.95"
%	 />
%<multicurve fill-style= "none"
%	 points= "(195,120);(195,120);(175,140);(175,140)"
%	 stroke-width= "0.95"
%	 />
%<multicurve fill-style= "none"
%	 points= "(175,120);(175,120);(195,120);(195,120)"
%	 stroke-width= "0.95"
%	 />
%<multicurve fill-style= "none"
%	 points= "(185,120);(185,120);(185,83.75);(185,83.75)"
%	 stroke-width= "0.95"
%	 />
%<multicurve fill-style= "none"
%	 points= "(165,130);(165,130);(165,110);(165,110)"
%	 stroke-width= "0.95"
%	 />
%<multicurve fill-style= "none"
%	 points= "(155,140);(155,140);(175,120);(175,120)"
%	 stroke-width= "0.95"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(207.5,182.5)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\Lprogtype$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(231.25,210)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\Lprogtype$
%</text>
%<multicurve fill-style= "none"
%	 points= "(150,175);(150,175);(150,45);(150,45)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(225,175);(225,175);(225,45);(225,45)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(150,45);(150,45);(187.5,7.5);(187.5,7.5)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(225,45);(225,45);(187.5,7.5);(187.5,7.5)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(150,175);(150,175);(225,175);(225,175)"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(260,220)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\ltag$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(187.5,16.25)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\Cprog$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(160,105)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\Sprog$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(175,130)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\stag$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(235,190)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\ltag$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(210,160)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\ltag$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(232.5,5)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\Hprogtype$
%</text>
%<multicurve fill-style= "none"
%	 points= "(175,93.75);(175,93.75);(175,73.75);(175,73.75)"
%	 stroke-width= "0.95"
%	 />
%<multicurve fill-style= "none"
%	 points= "(175,73.75);(175,73.75);(195,73.75);(195,73.75)"
%	 stroke-width= "0.95"
%	 />
%<multicurve fill-style= "none"
%	 points= "(175,93.75);(175,93.75);(195,73.75);(195,73.75)"
%	 stroke-width= "0.95"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(180,78.75)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\Sprog$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(295,210)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\EQLSsix
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(145,210)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\EQLSfive
%</text>
%<multicurve fill-style= "none"
%	 points= "(70,230);(70,230);(115,230);(115,230)"
%	 stroke-width= "0.95"
%	 />
%<multicurve fill-style= "none"
%	 points= "(115,210);(115,210);(115,230);(115,230)"
%	 stroke-width= "0.95"
%	 />
%<multicurve fill-style= "none"
%	 points= "(105,245);(105,245);(105,230);(105,230)"
%	 stroke-width= "0.95"
%	 />
%<multicurve fill-style= "none"
%	 points= "(90,210);(90,210);(115,210);(115,210)"
%	 stroke-width= "0.95"
%	 />
%<multicurve fill-style= "none"
%	 points= "(105,210);(105,210);(105,27.5);(105,27.5)"
%	 stroke-width= "0.95"
%	 />
%<multicurve fill-style= "none"
%	 points= "(70,230);(70,230);(90,210);(90,210)"
%	 stroke-width= "0.95"
%	 />
%<multicurve fill-style= "none"
%	 points= "(45,200);(45,200);(90,200);(90,200)"
%	 stroke-width= "0.95"
%	 />
%<multicurve fill-style= "none"
%	 points= "(45,97.5);(45,97.5);(45,77.5);(45,77.5)"
%	 stroke-width= "0.95"
%	 />
%<multicurve fill-style= "none"
%	 points= "(90,180);(90,180);(90,200);(90,200)"
%	 stroke-width= "0.95"
%	 />
%<multicurve fill-style= "none"
%	 points= "(80,220);(80,220);(80,200);(80,200)"
%	 stroke-width= "0.95"
%	 />
%<multicurve fill-style= "none"
%	 points= "(65,180);(65,180);(90,180);(90,180)"
%	 stroke-width= "0.95"
%	 />
%<multicurve fill-style= "none"
%	 points= "(80,180);(80,180);(80,27.5);(80,27.5)"
%	 stroke-width= "0.95"
%	 />
%<multicurve fill-style= "none"
%	 points= "(45,77.5);(45,77.5);(65,77.5);(65,77.5)"
%	 stroke-width= "0.95"
%	 />
%<multicurve fill-style= "none"
%	 points= "(45,97.5);(45,97.5);(65,77.5);(65,77.5)"
%	 stroke-width= "0.95"
%	 />
%<multicurve fill-style= "none"
%	 points= "(55,190);(55,190);(55,170);(55,170)"
%	 stroke-width= "0.95"
%	 />
%<multicurve fill-style= "none"
%	 points= "(45,200);(45,200);(65,180);(65,180)"
%	 stroke-width= "0.95"
%	 />
%<multicurve fill-style= "none"
%	 points= "(0,150);(0,150);(0,130);(0,130)"
%	 stroke-width= "0.95"
%	 />
%<multicurve fill-style= "none"
%	 points= "(0,130);(0,130);(20,130);(20,130)"
%	 stroke-width= "0.95"
%	 />
%<multicurve fill-style= "none"
%	 points= "(0,150);(0,150);(20,130);(20,130)"
%	 stroke-width= "0.95"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(50,82.5)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\itag$
%</text>
%<multicurve fill-style= "none"
%	 points= "(0,170);(0,170);(65,170);(65,170)"
%	 stroke-width= "0.95"
%	 />
%<multicurve fill-style= "none"
%	 points= "(65,150);(65,150);(65,170);(65,170)"
%	 stroke-width= "0.95"
%	 />
%<multicurve fill-style= "none"
%	 points= "(20,150);(20,150);(65,150);(65,150)"
%	 stroke-width= "0.95"
%	 />
%<multicurve fill-style= "none"
%	 points= "(55,150);(55,150);(55,87.5);(55,87.5)"
%	 stroke-width= "0.95"
%	 />
%<multicurve fill-style= "none"
%	 points= "(30,150);(30,150);(30,115);(30,115)"
%	 stroke-width= "0.95"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(52.5,102.5)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\Lprogtype$
%</text>
%<multicurve fill-style= "none"
%	 points= "(10,160);(10,160);(10,140);(10,140)"
%	 stroke-width= "0.95"
%	 />
%<multicurve fill-style= "none"
%	 points= "(0,170);(0,170);(20,150);(20,150)"
%	 stroke-width= "0.95"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(52.5,182.5)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\Lprogtype$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(76.25,210)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\Lprogtype$
%</text>
%<multicurve fill-style= "none"
%	 points= "(-5,175);(-5,175);(-5,77.5);(-5,77.5)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(70,175);(70,175);(70,77.5);(70,77.5)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(-5,77.5);(-5,77.5);(32.5,40);(32.5,40)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(70,77.5);(70,77.5);(32.5,40);(32.5,40)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(-5,175);(-5,175);(70,175);(70,175)"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(105,220)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\ltag$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(32.5,50)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\Cprog$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(5,135)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\Sprog$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(80,190)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\ltag$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(55,160)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\ltag$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(77.5,37.5)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\Hprogtype$
%</text>
%<multicurve fill-style= "none"
%	 points= "(20,125);(20,125);(20,105);(20,105)"
%	 stroke-width= "0.95"
%	 />
%<multicurve fill-style= "none"
%	 points= "(20,105);(20,105);(40,105);(40,105)"
%	 stroke-width= "0.95"
%	 />
%<multicurve fill-style= "none"
%	 points= "(20,125);(20,125);(40,105);(40,105)"
%	 stroke-width= "0.95"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(25,110)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\Sprog$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(27.5,127.5)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\Lprogtype$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(7.5,155)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\Lprogtype$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(-5,210)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\EQLSfour
%</text>
%<multicurve fill-style= "none"
%	 points= "(312.5,143.75);(312.5,143.75);(336.88,143.75);(336.88,143.75)"
%	 />
%</jpic>
%%End JPIC-XML
%PSTricks content-type (pstricks.sty package needed)
%Add \usepackage{pstricks} in the preamble of your LaTeX file
%You can rescale the whole picture (to 80% for instance) by using the command \def\JPicScale{0.8}
\ifx\JPicScale\undefined\def\JPicScale{1}\fi
\psset{unit=\JPicScale mm}
\psset{linewidth=0.3,dotsep=1,hatchwidth=0.3,hatchsep=1.5,shadowsize=1,dimen=middle}
\psset{dotsize=0.7 2.5,dotscale=1 1,fillcolor=black}
\psset{arrowsize=1 2,arrowlength=1,arrowinset=0.25,tbarsize=0.7 5,bracketlength=0.15,rbracketlength=0.15}
\begin{pspicture}(0,0)(430,245)
\psline[linewidth=0.95](385,230)(430,230)
\psline[linewidth=0.95](430,210)(430,230)
\psline[linewidth=0.95](420,245)(420,230)
\psline[linewidth=0.95](405,210)(430,210)
\psline[linewidth=0.95](420,210)(420,0)
\psline[linewidth=0.95](385,230)(405,210)
\psline[linewidth=0.95](360,200)(405,200)
\psline[linewidth=0.95](360,67.5)(360,47.5)
\psline[linewidth=0.95](405,180)(405,200)
\psline[linewidth=0.95](395,220)(395,200)
\psline[linewidth=0.95](380,180)(405,180)
\psline[linewidth=0.95](395,180)(395,0)
\psline[linewidth=0.95](360,47.5)(380,47.5)
\psline[linewidth=0.95](360,67.5)(380,47.5)
\psline[linewidth=0.95](370,190)(370,170)
\psline[linewidth=0.95](360,200)(380,180)
\psline[linewidth=0.95](325,100)(325,80)
\psline[linewidth=0.95](325,80)(345,80)
\psline[linewidth=0.95](325,100)(345,80)
\rput(365,52.5){$\itag$}
\psline[linewidth=0.95](335,170)(380,170)
\psline[linewidth=0.95](380,150)(380,170)
\psline[linewidth=0.95](355,150)(380,150)
\psline[linewidth=0.95](370,150)(370,57.5)
\psline[linewidth=0.95](345,160)(345,130)
\psline[linewidth=0.95](335,170)(355,150)
\rput[r](367.5,75){$\Lprogtype$}
\psline[linewidth=0.95](315,140)(335,140)
\psline[linewidth=0.95](355,120)(335,140)
\psline[linewidth=0.95](335,120)(355,120)
\psline[linewidth=0.95](345,120)(345,110)
\psline[linewidth=0.95](325,130)(325,110)
\psline[linewidth=0.95](315,140)(335,120)
\psline[linewidth=0.95](345,110)(335,100)
\psline[linewidth=0.95](325,110)(335,100)
\newrgbcolor{userFillColour}{0.2 0 0.2}
\rput{90}(335,100){\psellipse[fillcolor=userFillColour,fillstyle=solid](0,0)(2.58,-2.57)}
\psline[linewidth=0.95](335,100)(335,90)
\rput[r](367.5,182.5){$\Lprogtype$}
\rput[r](391.25,210){$\Lprogtype$}
\psline(336.88,143.75)(357.5,123.12)
\psline(312.5,143.75)(312.5,80)
\psline(357.5,123.12)(357.5,80)
\psline(312.5,80)(335,57.5)
\psline(357.5,80)(335,57.5)
\psline(305,175)(305,45)
\psline(385,175)(385,45)
\psline(305,45)(345,5)
\psline(385,45)(345,5)
\psline(305,175)(385,175)
\rput(420,220){$\ltag$}
\rput(345,15){$\Cprog$}
\rput(335,67.5){$\Gprog$}
\rput(330,85){$\Sprog$}
\rput(335,130){$\stag$}
\rput(395,190){$\ltag$}
\rput(370,160){$\ltag$}
\rput[r](392.5,5){$\Hprogtype$}
\psline[linewidth=0.95](225,230)(270,230)
\psline[linewidth=0.95](270,210)(270,230)
\psline[linewidth=0.95](260,245)(260,230)
\psline[linewidth=0.95](245,210)(270,210)
\psline[linewidth=0.95](260,210)(260,0)
\psline[linewidth=0.95](225,230)(245,210)
\psline[linewidth=0.95](200,200)(245,200)
\psline[linewidth=0.95](200,67.5)(200,47.5)
\psline[linewidth=0.95](245,180)(245,200)
\psline[linewidth=0.95](235,220)(235,200)
\psline[linewidth=0.95](220,180)(245,180)
\psline[linewidth=0.95](235,180)(235,0)
\psline[linewidth=0.95](200,47.5)(220,47.5)
\psline[linewidth=0.95](200,67.5)(220,47.5)
\psline[linewidth=0.95](210,190)(210,170)
\psline[linewidth=0.95](200,200)(220,180)
\psline[linewidth=0.95](155,120)(155,100)
\psline[linewidth=0.95](155,100)(175,100)
\psline[linewidth=0.95](155,120)(175,100)
\rput(205,52.5){$\itag$}
\psline[linewidth=0.95](175,170)(220,170)
\psline[linewidth=0.95](220,150)(220,170)
\psline[linewidth=0.95](195,150)(220,150)
\psline[linewidth=0.95](210,150)(210,57.5)
\psline[linewidth=0.95](185,160)(185,130)
\psline[linewidth=0.95](175,170)(195,150)
\psline[linewidth=0.95](155,140)(175,140)
\psline[linewidth=0.95](195,120)(175,140)
\psline[linewidth=0.95](175,120)(195,120)
\psline[linewidth=0.95](185,120)(185,83.75)
\psline[linewidth=0.95](165,130)(165,110)
\psline[linewidth=0.95](155,140)(175,120)
\rput[r](207.5,182.5){$\Lprogtype$}
\rput[r](231.25,210){$\Lprogtype$}
\psline(150,175)(150,45)
\psline(225,175)(225,45)
\psline(150,45)(187.5,7.5)
\psline(225,45)(187.5,7.5)
\psline(150,175)(225,175)
\rput(260,220){$\ltag$}
\rput(187.5,16.25){$\Cprog$}
\rput(160,105){$\Sprog$}
\rput(175,130){$\stag$}
\rput(235,190){$\ltag$}
\rput(210,160){$\ltag$}
\rput[r](232.5,5){$\Hprogtype$}
\psline[linewidth=0.95](175,93.75)(175,73.75)
\psline[linewidth=0.95](175,73.75)(195,73.75)
\psline[linewidth=0.95](175,93.75)(195,73.75)
\rput(180,78.75){$\Sprog$}
\rput(295,210){\EQLSsix}
\rput(145,210){\EQLSfive}
\psline[linewidth=0.95](70,230)(115,230)
\psline[linewidth=0.95](115,210)(115,230)
\psline[linewidth=0.95](105,245)(105,230)
\psline[linewidth=0.95](90,210)(115,210)
\psline[linewidth=0.95](105,210)(105,27.5)
\psline[linewidth=0.95](70,230)(90,210)
\psline[linewidth=0.95](45,200)(90,200)
\psline[linewidth=0.95](45,97.5)(45,77.5)
\psline[linewidth=0.95](90,180)(90,200)
\psline[linewidth=0.95](80,220)(80,200)
\psline[linewidth=0.95](65,180)(90,180)
\psline[linewidth=0.95](80,180)(80,27.5)
\psline[linewidth=0.95](45,77.5)(65,77.5)
\psline[linewidth=0.95](45,97.5)(65,77.5)
\psline[linewidth=0.95](55,190)(55,170)
\psline[linewidth=0.95](45,200)(65,180)
\psline[linewidth=0.95](0,150)(0,130)
\psline[linewidth=0.95](0,130)(20,130)
\psline[linewidth=0.95](0,150)(20,130)
\rput(50,82.5){$\itag$}
\psline[linewidth=0.95](0,170)(65,170)
\psline[linewidth=0.95](65,150)(65,170)
\psline[linewidth=0.95](20,150)(65,150)
\psline[linewidth=0.95](55,150)(55,87.5)
\psline[linewidth=0.95](30,150)(30,115)
\rput[r](52.5,102.5){$\Lprogtype$}
\psline[linewidth=0.95](10,160)(10,140)
\psline[linewidth=0.95](0,170)(20,150)
\rput[r](52.5,182.5){$\Lprogtype$}
\rput[r](76.25,210){$\Lprogtype$}
\psline(-5,175)(-5,77.5)
\psline(70,175)(70,77.5)
\psline(-5,77.5)(32.5,40)
\psline(70,77.5)(32.5,40)
\psline(-5,175)(70,175)
\rput(105,220){$\ltag$}
\rput(32.5,50){$\Cprog$}
\rput(5,135){$\Sprog$}
\rput(80,190){$\ltag$}
\rput(55,160){$\ltag$}
\rput[r](77.5,37.5){$\Hprogtype$}
\psline[linewidth=0.95](20,125)(20,105)
\psline[linewidth=0.95](20,105)(40,105)
\psline[linewidth=0.95](20,125)(40,105)
\rput(25,110){$\Sprog$}
\rput[r](27.5,127.5){$\Lprogtype$}
\rput[r](7.5,155){$\Lprogtype$}
\rput(-5,210){\EQLSfour}
\psline(312.5,143.75)(336.88,143.75)
\end{pspicture}


==> PIC/futamura.tex <==
%%Created by jPicEdt 1.4.1_03: mixed JPIC-XML/LaTeX format
%%Thu Nov 22 06:03:01 GMT-10:00 2018
%%Begin JPIC-XML
%<?xml version="1.0" standalone="yes"?>
%<jpic x-min="-5" x-max="430" y-min="0" y-max="245" auto-bounding="true">
%<multicurve fill-style= "none"
%	 points= "(385,230);(385,230);(430,230);(430,230)"
%	 stroke-width= "0.95"
%	 />
%<multicurve fill-style= "none"
%	 points= "(430,210);(430,210);(430,230);(430,230)"
%	 stroke-width= "0.95"
%	 />
%<multicurve fill-style= "none"
%	 points= "(420,245);(420,245);(420,230);(420,230)"
%	 stroke-width= "0.95"
%	 />
%<multicurve fill-style= "none"
%	 points= "(405,210);(405,210);(430,210);(430,210)"
%	 stroke-width= "0.95"
%	 />
%<multicurve fill-style= "none"
%	 points= "(420,210);(420,210);(420,0);(420,0)"
%	 stroke-width= "0.95"
%	 />
%<multicurve fill-style= "none"
%	 points= "(385,230);(385,230);(405,210);(405,210)"
%	 stroke-width= "0.95"
%	 />
%<multicurve fill-style= "none"
%	 points= "(360,200);(360,200);(405,200);(405,200)"
%	 stroke-width= "0.95"
%	 />
%<multicurve fill-style= "none"
%	 points= "(360,67.5);(360,67.5);(360,47.5);(360,47.5)"
%	 stroke-width= "0.95"
%	 />
%<multicurve fill-style= "none"
%	 points= "(405,180);(405,180);(405,200);(405,200)"
%	 stroke-width= "0.95"
%	 />
%<multicurve fill-style= "none"
%	 points= "(395,220);(395,220);(395,200);(395,200)"
%	 stroke-width= "0.95"
%	 />
%<multicurve fill-style= "none"
%	 points= "(380,180);(380,180);(405,180);(405,180)"
%	 stroke-width= "0.95"
%	 />
%<multicurve fill-style= "none"
%	 points= "(395,180);(395,180);(395,0);(395,0)"
%	 stroke-width= "0.95"
%	 />
%<multicurve fill-style= "none"
%	 points= "(360,47.5);(360,47.5);(380,47.5);(380,47.5)"
%	 stroke-width= "0.95"
%	 />
%<multicurve fill-style= "none"
%	 points= "(360,67.5);(360,67.5);(380,47.5);(380,47.5)"
%	 stroke-width= "0.95"
%	 />
%<multicurve fill-style= "none"
%	 points= "(370,190);(370,190);(370,170);(370,170)"
%	 stroke-width= "0.95"
%	 />
%<multicurve fill-style= "none"
%	 points= "(360,200);(360,200);(380,180);(380,180)"
%	 stroke-width= "0.95"
%	 />
%<multicurve fill-style= "none"
%	 points= "(325,100);(325,100);(325,80);(325,80)"
%	 stroke-width= "0.95"
%	 />
%<multicurve fill-style= "none"
%	 points= "(325,80);(325,80);(345,80);(345,80)"
%	 stroke-width= "0.95"
%	 />
%<multicurve fill-style= "none"
%	 points= "(325,100);(325,100);(345,80);(345,80)"
%	 stroke-width= "0.95"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(365,52.5)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\itag$
%</text>
%<multicurve fill-style= "none"
%	 points= "(335,170);(335,170);(380,170);(380,170)"
%	 stroke-width= "0.95"
%	 />
%<multicurve fill-style= "none"
%	 points= "(380,150);(380,150);(380,170);(380,170)"
%	 stroke-width= "0.95"
%	 />
%<multicurve fill-style= "none"
%	 points= "(355,150);(355,150);(380,150);(380,150)"
%	 stroke-width= "0.95"
%	 />
%<multicurve fill-style= "none"
%	 points= "(370,150);(370,150);(370,57.5);(370,57.5)"
%	 stroke-width= "0.95"
%	 />
%<multicurve fill-style= "none"
%	 points= "(345,160);(345,160);(345,130);(345,130)"
%	 stroke-width= "0.95"
%	 />
%<multicurve fill-style= "none"
%	 points= "(335,170);(335,170);(355,150);(355,150)"
%	 stroke-width= "0.95"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(367.5,75)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\Lprogtype$
%</text>
%<multicurve fill-style= "none"
%	 points= "(315,140);(315,140);(335,140);(335,140)"
%	 stroke-width= "0.95"
%	 />
%<multicurve fill-style= "none"
%	 points= "(355,120);(355,120);(335,140);(335,140)"
%	 stroke-width= "0.95"
%	 />
%<multicurve fill-style= "none"
%	 points= "(335,120);(335,120);(355,120);(355,120)"
%	 stroke-width= "0.95"
%	 />
%<multicurve fill-style= "none"
%	 points= "(345,120);(345,120);(345,110);(345,110)"
%	 stroke-width= "0.95"
%	 />
%<multicurve fill-style= "none"
%	 points= "(325,130);(325,130);(325,110);(325,110)"
%	 stroke-width= "0.95"
%	 />
%<multicurve fill-style= "none"
%	 points= "(315,140);(315,140);(335,120);(335,120)"
%	 stroke-width= "0.95"
%	 />
%<multicurve fill-style= "none"
%	 points= "(345,110);(345,110);(335,100);(335,100)"
%	 stroke-width= "0.95"
%	 />
%<multicurve fill-style= "none"
%	 points= "(325,110);(325,110);(335,100);(335,100)"
%	 stroke-width= "0.95"
%	 />
%<ellipse p3= "(337.57,97.42)"
%	 fill-style= "solid"
%	 p2= "(337.57,102.58)"
%	 fill-color= "#330033"
%	 p1= "(332.43,102.58)"
%	 closure= "open"
%	 angle-end= "0"
%	 angle-start= "0"
%	 />
%<multicurve fill-style= "none"
%	 points= "(335,100);(335,100);(335,90);(335,90)"
%	 stroke-width= "0.95"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(367.5,182.5)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\Lprogtype$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(391.25,210)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\Lprogtype$
%</text>
%<multicurve fill-style= "none"
%	 points= "(312.5,145);(312.5,145);(357.5,145);(357.5,145)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(312.5,145);(312.5,145);(312.5,80);(312.5,80)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(357.5,145);(357.5,145);(357.5,80);(357.5,80)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(312.5,80);(312.5,80);(335,57.5);(335,57.5)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(357.5,80);(357.5,80);(335,57.5);(335,57.5)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(305,175);(305,175);(305,45);(305,45)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(385,175);(385,175);(385,45);(385,45)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(305,45);(305,45);(345,5);(345,5)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(385,45);(385,45);(345,5);(345,5)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(305,175);(305,175);(385,175);(385,175)"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(420,220)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\ltag$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(345,15)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\Cprog$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(335,67.5)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\Gprog$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(330,85)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\Sprog$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(335,130)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\stag$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(395,190)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\ltag$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(370,160)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\ltag$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(392.5,5)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\Hprogtype$
%</text>
%<multicurve fill-style= "none"
%	 points= "(225,230);(225,230);(270,230);(270,230)"
%	 stroke-width= "0.95"
%	 />
%<multicurve fill-style= "none"
%	 points= "(270,210);(270,210);(270,230);(270,230)"
%	 stroke-width= "0.95"
%	 />
%<multicurve fill-style= "none"
%	 points= "(260,245);(260,245);(260,230);(260,230)"
%	 stroke-width= "0.95"
%	 />
%<multicurve fill-style= "none"
%	 points= "(245,210);(245,210);(270,210);(270,210)"
%	 stroke-width= "0.95"
%	 />
%<multicurve fill-style= "none"
%	 points= "(260,210);(260,210);(260,0);(260,0)"
%	 stroke-width= "0.95"
%	 />
%<multicurve fill-style= "none"
%	 points= "(225,230);(225,230);(245,210);(245,210)"
%	 stroke-width= "0.95"
%	 />
%<multicurve fill-style= "none"
%	 points= "(200,200);(200,200);(245,200);(245,200)"
%	 stroke-width= "0.95"
%	 />
%<multicurve fill-style= "none"
%	 points= "(200,67.5);(200,67.5);(200,47.5);(200,47.5)"
%	 stroke-width= "0.95"
%	 />
%<multicurve fill-style= "none"
%	 points= "(245,180);(245,180);(245,200);(245,200)"
%	 stroke-width= "0.95"
%	 />
%<multicurve fill-style= "none"
%	 points= "(235,220);(235,220);(235,200);(235,200)"
%	 stroke-width= "0.95"
%	 />
%<multicurve fill-style= "none"
%	 points= "(220,180);(220,180);(245,180);(245,180)"
%	 stroke-width= "0.95"
%	 />
%<multicurve fill-style= "none"
%	 points= "(235,180);(235,180);(235,0);(235,0)"
%	 stroke-width= "0.95"
%	 />
%<multicurve fill-style= "none"
%	 points= "(200,47.5);(200,47.5);(220,47.5);(220,47.5)"
%	 stroke-width= "0.95"
%	 />
%<multicurve fill-style= "none"
%	 points= "(200,67.5);(200,67.5);(220,47.5);(220,47.5)"
%	 stroke-width= "0.95"
%	 />
%<multicurve fill-style= "none"
%	 points= "(210,190);(210,190);(210,170);(210,170)"
%	 stroke-width= "0.95"
%	 />
%<multicurve fill-style= "none"
%	 points= "(200,200);(200,200);(220,180);(220,180)"
%	 stroke-width= "0.95"
%	 />
%<multicurve fill-style= "none"
%	 points= "(155,120);(155,120);(155,100);(155,100)"
%	 stroke-width= "0.95"
%	 />
%<multicurve fill-style= "none"
%	 points= "(155,100);(155,100);(175,100);(175,100)"
%	 stroke-width= "0.95"
%	 />
%<multicurve fill-style= "none"
%	 points= "(155,120);(155,120);(175,100);(175,100)"
%	 stroke-width= "0.95"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(205,52.5)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\itag$
%</text>
%<multicurve fill-style= "none"
%	 points= "(175,170);(175,170);(220,170);(220,170)"
%	 stroke-width= "0.95"
%	 />
%<multicurve fill-style= "none"
%	 points= "(220,150);(220,150);(220,170);(220,170)"
%	 stroke-width= "0.95"
%	 />
%<multicurve fill-style= "none"
%	 points= "(195,150);(195,150);(220,150);(220,150)"
%	 stroke-width= "0.95"
%	 />
%<multicurve fill-style= "none"
%	 points= "(210,150);(210,150);(210,57.5);(210,57.5)"
%	 stroke-width= "0.95"
%	 />
%<multicurve fill-style= "none"
%	 points= "(185,160);(185,160);(185,130);(185,130)"
%	 stroke-width= "0.95"
%	 />
%<multicurve fill-style= "none"
%	 points= "(175,170);(175,170);(195,150);(195,150)"
%	 stroke-width= "0.95"
%	 />
%<multicurve fill-style= "none"
%	 points= "(155,140);(155,140);(175,140);(175,140)"
%	 stroke-width= "0.95"
%	 />
%<multicurve fill-style= "none"
%	 points= "(195,120);(195,120);(175,140);(175,140)"
%	 stroke-width= "0.95"
%	 />
%<multicurve fill-style= "none"
%	 points= "(175,120);(175,120);(195,120);(195,120)"
%	 stroke-width= "0.95"
%	 />
%<multicurve fill-style= "none"
%	 points= "(185,120);(185,120);(185,83.75);(185,83.75)"
%	 stroke-width= "0.95"
%	 />
%<multicurve fill-style= "none"
%	 points= "(165,130);(165,130);(165,110);(165,110)"
%	 stroke-width= "0.95"
%	 />
%<multicurve fill-style= "none"
%	 points= "(155,140);(155,140);(175,120);(175,120)"
%	 stroke-width= "0.95"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(207.5,182.5)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\Lprogtype$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(231.25,210)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\Lprogtype$
%</text>
%<multicurve fill-style= "none"
%	 points= "(150,175);(150,175);(150,45);(150,45)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(225,175);(225,175);(225,45);(225,45)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(150,45);(150,45);(187.5,7.5);(187.5,7.5)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(225,45);(225,45);(187.5,7.5);(187.5,7.5)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(150,175);(150,175);(225,175);(225,175)"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(260,220)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\ltag$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(187.5,16.25)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\Cprog$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(160,105)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\Sprog$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(175,130)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\stag$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(235,190)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\ltag$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(210,160)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\ltag$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(232.5,5)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\Hprogtype$
%</text>
%<multicurve fill-style= "none"
%	 points= "(175,93.75);(175,93.75);(175,73.75);(175,73.75)"
%	 stroke-width= "0.95"
%	 />
%<multicurve fill-style= "none"
%	 points= "(175,73.75);(175,73.75);(195,73.75);(195,73.75)"
%	 stroke-width= "0.95"
%	 />
%<multicurve fill-style= "none"
%	 points= "(175,93.75);(175,93.75);(195,73.75);(195,73.75)"
%	 stroke-width= "0.95"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(180,78.75)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\Sprog$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(295,210)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\EQLSsix
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(145,210)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\EQLSfive
%</text>
%<multicurve fill-style= "none"
%	 points= "(70,230);(70,230);(115,230);(115,230)"
%	 stroke-width= "0.95"
%	 />
%<multicurve fill-style= "none"
%	 points= "(115,210);(115,210);(115,230);(115,230)"
%	 stroke-width= "0.95"
%	 />
%<multicurve fill-style= "none"
%	 points= "(105,245);(105,245);(105,230);(105,230)"
%	 stroke-width= "0.95"
%	 />
%<multicurve fill-style= "none"
%	 points= "(90,210);(90,210);(115,210);(115,210)"
%	 stroke-width= "0.95"
%	 />
%<multicurve fill-style= "none"
%	 points= "(105,210);(105,210);(105,27.5);(105,27.5)"
%	 stroke-width= "0.95"
%	 />
%<multicurve fill-style= "none"
%	 points= "(70,230);(70,230);(90,210);(90,210)"
%	 stroke-width= "0.95"
%	 />
%<multicurve fill-style= "none"
%	 points= "(45,200);(45,200);(90,200);(90,200)"
%	 stroke-width= "0.95"
%	 />
%<multicurve fill-style= "none"
%	 points= "(45,97.5);(45,97.5);(45,77.5);(45,77.5)"
%	 stroke-width= "0.95"
%	 />
%<multicurve fill-style= "none"
%	 points= "(90,180);(90,180);(90,200);(90,200)"
%	 stroke-width= "0.95"
%	 />
%<multicurve fill-style= "none"
%	 points= "(80,220);(80,220);(80,200);(80,200)"
%	 stroke-width= "0.95"
%	 />
%<multicurve fill-style= "none"
%	 points= "(65,180);(65,180);(90,180);(90,180)"
%	 stroke-width= "0.95"
%	 />
%<multicurve fill-style= "none"
%	 points= "(80,180);(80,180);(80,27.5);(80,27.5)"
%	 stroke-width= "0.95"
%	 />
%<multicurve fill-style= "none"
%	 points= "(45,77.5);(45,77.5);(65,77.5);(65,77.5)"
%	 stroke-width= "0.95"
%	 />
%<multicurve fill-style= "none"
%	 points= "(45,97.5);(45,97.5);(65,77.5);(65,77.5)"
%	 stroke-width= "0.95"
%	 />
%<multicurve fill-style= "none"
%	 points= "(55,190);(55,190);(55,170);(55,170)"
%	 stroke-width= "0.95"
%	 />
%<multicurve fill-style= "none"
%	 points= "(45,200);(45,200);(65,180);(65,180)"
%	 stroke-width= "0.95"
%	 />
%<multicurve fill-style= "none"
%	 points= "(0,150);(0,150);(0,130);(0,130)"
%	 stroke-width= "0.95"
%	 />
%<multicurve fill-style= "none"
%	 points= "(0,130);(0,130);(20,130);(20,130)"
%	 stroke-width= "0.95"
%	 />
%<multicurve fill-style= "none"
%	 points= "(0,150);(0,150);(20,130);(20,130)"
%	 stroke-width= "0.95"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(50,82.5)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\itag$
%</text>
%<multicurve fill-style= "none"
%	 points= "(0,170);(0,170);(65,170);(65,170)"
%	 stroke-width= "0.95"
%	 />
%<multicurve fill-style= "none"
%	 points= "(65,150);(65,150);(65,170);(65,170)"
%	 stroke-width= "0.95"
%	 />
%<multicurve fill-style= "none"
%	 points= "(20,150);(20,150);(65,150);(65,150)"
%	 stroke-width= "0.95"
%	 />
%<multicurve fill-style= "none"
%	 points= "(55,150);(55,150);(55,87.5);(55,87.5)"
%	 stroke-width= "0.95"
%	 />
%<multicurve fill-style= "none"
%	 points= "(30,150);(30,150);(30,115);(30,115)"
%	 stroke-width= "0.95"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(52.5,102.5)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\Lprogtype$
%</text>
%<multicurve fill-style= "none"
%	 points= "(10,160);(10,160);(10,140);(10,140)"
%	 stroke-width= "0.95"
%	 />
%<multicurve fill-style= "none"
%	 points= "(0,170);(0,170);(20,150);(20,150)"
%	 stroke-width= "0.95"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(52.5,182.5)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\Lprogtype$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(76.25,210)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\Lprogtype$
%</text>
%<multicurve fill-style= "none"
%	 points= "(-5,175);(-5,175);(-5,77.5);(-5,77.5)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(70,175);(70,175);(70,77.5);(70,77.5)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(-5,77.5);(-5,77.5);(32.5,40);(32.5,40)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(70,77.5);(70,77.5);(32.5,40);(32.5,40)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(-5,175);(-5,175);(70,175);(70,175)"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(105,220)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\ltag$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(32.5,50)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\Cprog$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(5,135)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\Sprog$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(80,190)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\ltag$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(55,160)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\ltag$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(77.5,37.5)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\Hprogtype$
%</text>
%<multicurve fill-style= "none"
%	 points= "(20,125);(20,125);(20,105);(20,105)"
%	 stroke-width= "0.95"
%	 />
%<multicurve fill-style= "none"
%	 points= "(20,105);(20,105);(40,105);(40,105)"
%	 stroke-width= "0.95"
%	 />
%<multicurve fill-style= "none"
%	 points= "(20,125);(20,125);(40,105);(40,105)"
%	 stroke-width= "0.95"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(25,110)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\Sprog$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(27.5,127.5)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\Lprogtype$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(7.5,155)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\Lprogtype$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(-5,210)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\EQLSfour
%</text>
%</jpic>
%%End JPIC-XML
%PSTricks content-type (pstricks.sty package needed)
%Add \usepackage{pstricks} in the preamble of your LaTeX file
%You can rescale the whole picture (to 80% for instance) by using the command \def\JPicScale{0.8}
\ifx\JPicScale\undefined\def\JPicScale{1}\fi
\psset{unit=\JPicScale mm}
\psset{linewidth=0.3,dotsep=1,hatchwidth=0.3,hatchsep=1.5,shadowsize=1,dimen=middle}
\psset{dotsize=0.7 2.5,dotscale=1 1,fillcolor=black}
\psset{arrowsize=1 2,arrowlength=1,arrowinset=0.25,tbarsize=0.7 5,bracketlength=0.15,rbracketlength=0.15}
\begin{pspicture}(0,0)(430,245)
\psline[linewidth=0.95](385,230)(430,230)
\psline[linewidth=0.95](430,210)(430,230)
\psline[linewidth=0.95](420,245)(420,230)
\psline[linewidth=0.95](405,210)(430,210)
\psline[linewidth=0.95](420,210)(420,0)
\psline[linewidth=0.95](385,230)(405,210)
\psline[linewidth=0.95](360,200)(405,200)
\psline[linewidth=0.95](360,67.5)(360,47.5)
\psline[linewidth=0.95](405,180)(405,200)
\psline[linewidth=0.95](395,220)(395,200)
\psline[linewidth=0.95](380,180)(405,180)
\psline[linewidth=0.95](395,180)(395,0)
\psline[linewidth=0.95](360,47.5)(380,47.5)
\psline[linewidth=0.95](360,67.5)(380,47.5)
\psline[linewidth=0.95](370,190)(370,170)
\psline[linewidth=0.95](360,200)(380,180)
\psline[linewidth=0.95](325,100)(325,80)
\psline[linewidth=0.95](325,80)(345,80)
\psline[linewidth=0.95](325,100)(345,80)
\rput(365,52.5){$\itag$}
\psline[linewidth=0.95](335,170)(380,170)
\psline[linewidth=0.95](380,150)(380,170)
\psline[linewidth=0.95](355,150)(380,150)
\psline[linewidth=0.95](370,150)(370,57.5)
\psline[linewidth=0.95](345,160)(345,130)
\psline[linewidth=0.95](335,170)(355,150)
\rput[r](367.5,75){$\Lprogtype$}
\psline[linewidth=0.95](315,140)(335,140)
\psline[linewidth=0.95](355,120)(335,140)
\psline[linewidth=0.95](335,120)(355,120)
\psline[linewidth=0.95](345,120)(345,110)
\psline[linewidth=0.95](325,130)(325,110)
\psline[linewidth=0.95](315,140)(335,120)
\psline[linewidth=0.95](345,110)(335,100)
\psline[linewidth=0.95](325,110)(335,100)
\newrgbcolor{userFillColour}{0.2 0 0.2}
\rput{90}(335,100){\psellipse[fillcolor=userFillColour,fillstyle=solid](0,0)(2.58,-2.57)}
\psline[linewidth=0.95](335,100)(335,90)
\rput[r](367.5,182.5){$\Lprogtype$}
\rput[r](391.25,210){$\Lprogtype$}
\psline(312.5,145)(357.5,145)
\psline(312.5,145)(312.5,80)
\psline(357.5,145)(357.5,80)
\psline(312.5,80)(335,57.5)
\psline(357.5,80)(335,57.5)
\psline(305,175)(305,45)
\psline(385,175)(385,45)
\psline(305,45)(345,5)
\psline(385,45)(345,5)
\psline(305,175)(385,175)
\rput(420,220){$\ltag$}
\rput(345,15){$\Cprog$}
\rput(335,67.5){$\Gprog$}
\rput(330,85){$\Sprog$}
\rput(335,130){$\stag$}
\rput(395,190){$\ltag$}
\rput(370,160){$\ltag$}
\rput[r](392.5,5){$\Hprogtype$}
\psline[linewidth=0.95](225,230)(270,230)
\psline[linewidth=0.95](270,210)(270,230)
\psline[linewidth=0.95](260,245)(260,230)
\psline[linewidth=0.95](245,210)(270,210)
\psline[linewidth=0.95](260,210)(260,0)
\psline[linewidth=0.95](225,230)(245,210)
\psline[linewidth=0.95](200,200)(245,200)
\psline[linewidth=0.95](200,67.5)(200,47.5)
\psline[linewidth=0.95](245,180)(245,200)
\psline[linewidth=0.95](235,220)(235,200)
\psline[linewidth=0.95](220,180)(245,180)
\psline[linewidth=0.95](235,180)(235,0)
\psline[linewidth=0.95](200,47.5)(220,47.5)
\psline[linewidth=0.95](200,67.5)(220,47.5)
\psline[linewidth=0.95](210,190)(210,170)
\psline[linewidth=0.95](200,200)(220,180)
\psline[linewidth=0.95](155,120)(155,100)
\psline[linewidth=0.95](155,100)(175,100)
\psline[linewidth=0.95](155,120)(175,100)
\rput(205,52.5){$\itag$}
\psline[linewidth=0.95](175,170)(220,170)
\psline[linewidth=0.95](220,150)(220,170)
\psline[linewidth=0.95](195,150)(220,150)
\psline[linewidth=0.95](210,150)(210,57.5)
\psline[linewidth=0.95](185,160)(185,130)
\psline[linewidth=0.95](175,170)(195,150)
\psline[linewidth=0.95](155,140)(175,140)
\psline[linewidth=0.95](195,120)(175,140)
\psline[linewidth=0.95](175,120)(195,120)
\psline[linewidth=0.95](185,120)(185,83.75)
\psline[linewidth=0.95](165,130)(165,110)
\psline[linewidth=0.95](155,140)(175,120)
\rput[r](207.5,182.5){$\Lprogtype$}
\rput[r](231.25,210){$\Lprogtype$}
\psline(150,175)(150,45)
\psline(225,175)(225,45)
\psline(150,45)(187.5,7.5)
\psline(225,45)(187.5,7.5)
\psline(150,175)(225,175)
\rput(260,220){$\ltag$}
\rput(187.5,16.25){$\Cprog$}
\rput(160,105){$\Sprog$}
\rput(175,130){$\stag$}
\rput(235,190){$\ltag$}
\rput(210,160){$\ltag$}
\rput[r](232.5,5){$\Hprogtype$}
\psline[linewidth=0.95](175,93.75)(175,73.75)
\psline[linewidth=0.95](175,73.75)(195,73.75)
\psline[linewidth=0.95](175,93.75)(195,73.75)
\rput(180,78.75){$\Sprog$}
\rput(295,210){\EQLSsix}
\rput(145,210){\EQLSfive}
\psline[linewidth=0.95](70,230)(115,230)
\psline[linewidth=0.95](115,210)(115,230)
\psline[linewidth=0.95](105,245)(105,230)
\psline[linewidth=0.95](90,210)(115,210)
\psline[linewidth=0.95](105,210)(105,27.5)
\psline[linewidth=0.95](70,230)(90,210)
\psline[linewidth=0.95](45,200)(90,200)
\psline[linewidth=0.95](45,97.5)(45,77.5)
\psline[linewidth=0.95](90,180)(90,200)
\psline[linewidth=0.95](80,220)(80,200)
\psline[linewidth=0.95](65,180)(90,180)
\psline[linewidth=0.95](80,180)(80,27.5)
\psline[linewidth=0.95](45,77.5)(65,77.5)
\psline[linewidth=0.95](45,97.5)(65,77.5)
\psline[linewidth=0.95](55,190)(55,170)
\psline[linewidth=0.95](45,200)(65,180)
\psline[linewidth=0.95](0,150)(0,130)
\psline[linewidth=0.95](0,130)(20,130)
\psline[linewidth=0.95](0,150)(20,130)
\rput(50,82.5){$\itag$}
\psline[linewidth=0.95](0,170)(65,170)
\psline[linewidth=0.95](65,150)(65,170)
\psline[linewidth=0.95](20,150)(65,150)
\psline[linewidth=0.95](55,150)(55,87.5)
\psline[linewidth=0.95](30,150)(30,115)
\rput[r](52.5,102.5){$\Lprogtype$}
\psline[linewidth=0.95](10,160)(10,140)
\psline[linewidth=0.95](0,170)(20,150)
\rput[r](52.5,182.5){$\Lprogtype$}
\rput[r](76.25,210){$\Lprogtype$}
\psline(-5,175)(-5,77.5)
\psline(70,175)(70,77.5)
\psline(-5,77.5)(32.5,40)
\psline(70,77.5)(32.5,40)
\psline(-5,175)(70,175)
\rput(105,220){$\ltag$}
\rput(32.5,50){$\Cprog$}
\rput(5,135){$\Sprog$}
\rput(80,190){$\ltag$}
\rput(55,160){$\ltag$}
\rput[r](77.5,37.5){$\Hprogtype$}
\psline[linewidth=0.95](20,125)(20,105)
\psline[linewidth=0.95](20,105)(40,105)
\psline[linewidth=0.95](20,125)(40,105)
\rput(25,110){$\Sprog$}
\rput[r](27.5,127.5){$\Lprogtype$}
\rput[r](7.5,155){$\Lprogtype$}
\rput(-5,210){\EQLSfour}
\end{pspicture}


==> PIC/godement-par.tex <==
%%Created by jPicEdt 1.4.1_03: mixed JPIC-XML/LaTeX format
%%Tue Sep 01 07:34:09 GMT-10:00 2020
%%Begin JPIC-XML
%<?xml version="1.0" standalone="yes"?>
%<jpic x-min="-5" x-max="115" y-min="0" y-max="60" auto-bounding="true">
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(15,40);(15,40);(45,40);(45,40)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(15,40);(15,40);(15,20);(15,20)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(45,20);(45,20);(45,40);(45,40)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(30,60);(30,60);(30,40);(30,40)"
%	 />
%<text fill-style= "none"
%	 stroke-width= "0.75"
%	 text-vert-align= "center-v"
%	 anchor-point= "(27.5,55)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\nameslang$
%</text>
%<text fill-style= "none"
%	 stroke-width= "0.75"
%	 text-vert-align= "center-v"
%	 anchor-point= "(27.5,5)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\inputt$
%</text>
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(15,20);(15,20);(45,20);(45,20)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(30,20);(30,20);(30,0);(30,0)"
%	 />
%<text fill-style= "none"
%	 stroke-width= "0.75"
%	 text-vert-align= "center-v"
%	 anchor-point= "(30,30)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\machine
%</text>
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(65,40);(65,40);(95,40);(95,40)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(65,40);(65,40);(65,20);(65,20)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(95,20);(95,20);(95,40);(95,40)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(80,60);(80,60);(80,40);(80,40)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(65,20);(65,20);(95,20);(95,20)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(80,20);(80,20);(80,0);(80,0)"
%	 />
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(77.5,5)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\otherinputt$
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(77.5,55)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\otheroutpt$
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(80,30)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\hee$
%</text>
%<parallelogram fill-style= "none"
%	 p3= "(115,15)"
%	 p2= "(115,45)"
%	 p1= "(-5,45)"
%	 stroke-color= "#3300ff"
%	 />
%<text fill-style= "none"
%	 text-vert-align= "bottom"
%	 anchor-point= "(113.75,16.25)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\parcompp$
%</text>
%</jpic>
%%End JPIC-XML
%PSTricks content-type (pstricks.sty package needed)
%Add \usepackage{pstricks} in the preamble of your LaTeX file
%You can rescale the whole picture (to 80% for instance) by using the command \def\JPicScale{0.8}
\ifx\JPicScale\undefined\def\JPicScale{1}\fi
\psset{unit=\JPicScale mm}
\psset{linewidth=0.3,dotsep=1,hatchwidth=0.3,hatchsep=1.5,shadowsize=1,dimen=middle}
\psset{dotsize=0.7 2.5,dotscale=1 1,fillcolor=black}
\psset{arrowsize=1 2,arrowlength=1,arrowinset=0.25,tbarsize=0.7 5,bracketlength=0.15,rbracketlength=0.15}
\begin{pspicture}(0,0)(115,60)
\psline[linewidth=0.75](15,40)(45,40)
\psline[linewidth=0.75](15,40)(15,20)
\psline[linewidth=0.75](45,20)(45,40)
\psline[linewidth=0.75](30,60)(30,40)
\rput[r](27.5,55){$\nameslang$}
\rput[r](27.5,5){$\inputt$}
\psline[linewidth=0.75](15,20)(45,20)
\psline[linewidth=0.75](30,20)(30,0)
\rput(30,30){\machine}
\psline[linewidth=0.75](65,40)(95,40)
\psline[linewidth=0.75](65,40)(65,20)
\psline[linewidth=0.75](95,20)(95,40)
\psline[linewidth=0.75](80,60)(80,40)
\psline[linewidth=0.75](65,20)(95,20)
\psline[linewidth=0.75](80,20)(80,0)
\rput[r](77.5,5){$\otherinputt$}
\rput[r](77.5,55){$\otheroutpt$}
\rput(80,30){$\hee$}
\newrgbcolor{userLineColour}{0.2 0 1}
\pspolygon[linecolor=userLineColour](-5,45)(115,45)(115,15)(-5,15)
\rput[br](113.75,16.25){$\parcompp$}
\end{pspicture}


==> PIC/godement-seq.tex <==
%%Created by jPicEdt 1.4.1_03: mixed JPIC-XML/LaTeX format
%%Tue Sep 01 07:25:15 GMT-10:00 2020
%%Begin JPIC-XML
%<?xml version="1.0" standalone="yes"?>
%<jpic x-min="0" x-max="40" y-min="-60" y-max="60" auto-bounding="true">
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(5,-15);(5,-15);(35,-15);(35,-15)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(5,-15);(5,-15);(5,-35);(5,-35)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(35,-35);(35,-35);(35,-15);(35,-15)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(20,15);(20,15);(20,-15);(20,-15)"
%	 />
%<text fill-style= "none"
%	 stroke-width= "0.75"
%	 text-vert-align= "center-v"
%	 anchor-point= "(17.5,0)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\nameslang$
%</text>
%<text fill-style= "none"
%	 stroke-width= "0.75"
%	 text-vert-align= "center-v"
%	 anchor-point= "(18.75,-58.75)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\inputt$
%</text>
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(5,-35);(5,-35);(35,-35);(35,-35)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(20,-35);(20,-35);(20,-60);(20,-60)"
%	 />
%<text fill-style= "none"
%	 stroke-width= "0.75"
%	 text-vert-align= "center-v"
%	 anchor-point= "(20,-25)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\machine
%</text>
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(5,35);(5,35);(35,35);(35,35)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(5,35);(5,35);(5,15);(5,15)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(35,15);(35,15);(35,35);(35,35)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(20,60);(20,60);(20,35);(20,35)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(5,15);(5,15);(35,15);(35,15)"
%	 />
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(20,25)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\gee
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(22.5,58.75)"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%\outpt
%</text>
%<parallelogram fill-style= "none"
%	 p3= "(40,-50)"
%	 p2= "(40,50)"
%	 p1= "(0,50)"
%	 stroke-color= "#ff0066"
%	 />
%<text fill-style= "none"
%	 text-vert-align= "top"
%	 anchor-point= "(38.75,48.12)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\seqcompp$
%</text>
%</jpic>
%%End JPIC-XML
%PSTricks content-type (pstricks.sty package needed)
%Add \usepackage{pstricks} in the preamble of your LaTeX file
%You can rescale the whole picture (to 80% for instance) by using the command \def\JPicScale{0.8}
\ifx\JPicScale\undefined\def\JPicScale{1}\fi
\psset{unit=\JPicScale mm}
\psset{linewidth=0.3,dotsep=1,hatchwidth=0.3,hatchsep=1.5,shadowsize=1,dimen=middle}
\psset{dotsize=0.7 2.5,dotscale=1 1,fillcolor=black}
\psset{arrowsize=1 2,arrowlength=1,arrowinset=0.25,tbarsize=0.7 5,bracketlength=0.15,rbracketlength=0.15}
\begin{pspicture}(0,0)(40,60)
\psline[linewidth=0.75](5,-15)(35,-15)
\psline[linewidth=0.75](5,-15)(5,-35)
\psline[linewidth=0.75](35,-35)(35,-15)
\psline[linewidth=0.75](20,15)(20,-15)
\rput[r](17.5,0){$\nameslang$}
\rput[r](18.75,-58.75){$\inputt$}
\psline[linewidth=0.75](5,-35)(35,-35)
\psline[linewidth=0.75](20,-35)(20,-60)
\rput(20,-25){\machine}
\psline[linewidth=0.75](5,35)(35,35)
\psline[linewidth=0.75](5,35)(5,15)
\psline[linewidth=0.75](35,15)(35,35)
\psline[linewidth=0.75](20,60)(20,35)
\psline[linewidth=0.75](5,15)(35,15)
\rput(20,25){\gee}
\rput[l](22.5,58.75){\outpt}
\newrgbcolor{userLineColour}{1 0 0.4}
\pspolygon[linecolor=userLineColour](0,50)(40,50)(40,-50)(0,-50)
\rput[tr](38.75,48.12){$\seqcompp$}
\end{pspicture}


==> PIC/halt-all.tex <==
%%Created by jPicEdt 1.4.1_03: mixed JPIC-XML/LaTeX format
%%Mon Oct 31 13:46:19 HST 2016
%%Begin JPIC-XML
%<?xml version="1.0" standalone="yes"?>
%<jpic x-min="0" x-max="78.12" y-min="0" y-max="62.58" auto-bounding="true">
%<multicurve stroke-width= "0.75"
%	 points= "(0,40);(0,40);(30,40);(30,40)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.75"
%	 points= "(30,20);(30,20);(30,40);(30,40)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.75"
%	 points= "(0,20);(0,20);(30,20);(30,20)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "1.1"
%	 points= "(15,20);(15,20);(15,0);(15,0)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.75"
%	 points= "(0,40);(0,40);(0,20);(0,20)"
%	 fill-style= "none"
%	 />
%<text text-vert-align= "center-v"
%	 stroke-width= "0.75"
%	 anchor-point= "(50,30)"
%	 text-frame= "noframe"
%	 fill-style= "none"
%	 text-hor-align= "center-h"
%	 >
%\EQLS
%</text>
%<multicurve stroke-width= "1.1"
%	 points= "(75,60);(75,60);(75,0);(75,0)"
%	 fill-style= "none"
%	 />
%<ellipse p3= "(77.58,57.42)"
%	 p2= "(77.58,62.58)"
%	 p1= "(72.42,62.58)"
%	 closure= "open"
%	 fill-color= "#330033"
%	 angle-end= "0"
%	 fill-style= "solid"
%	 angle-start= "0"
%	 />
%<ellipse p3= "(17.58,57.42)"
%	 p2= "(17.58,62.58)"
%	 p1= "(12.42,62.58)"
%	 closure= "open"
%	 fill-color= "#330033"
%	 angle-end= "0"
%	 fill-style= "solid"
%	 angle-start= "0"
%	 />
%<multicurve stroke-width= "1.1"
%	 points= "(15,60);(15,60);(15,40);(15,40)"
%	 fill-style= "none"
%	 />
%<text text-vert-align= "center-v"
%	 anchor-point= "(16.88,10)"
%	 text-frame= "noframe"
%	 fill-style= "none"
%	 text-hor-align= "left"
%	 >
%$\medput$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(78.12,10)"
%	 text-frame= "noframe"
%	 fill-style= "none"
%	 text-hor-align= "left"
%	 >
%$\medput$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(15,30)"
%	 text-frame= "noframe"
%	 fill-style= "none"
%	 text-hor-align= "center-h"
%	 >
%$\eef$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(18.12,50)"
%	 text-frame= "noframe"
%	 fill-style= "none"
%	 text-hor-align= "left"
%	 >
%$\outputt$
%</text>
%</jpic>
%%End JPIC-XML
%PSTricks content-type (pstricks.sty package needed)
%Add \usepackage{pstricks} in the preamble of your LaTeX file
%You can rescale the whole picture (to 80% for instance) by using the command \def\JPicScale{0.8}
\ifx\JPicScale\undefined\def\JPicScale{1}\fi
\psset{unit=\JPicScale mm}
\psset{linewidth=0.3,dotsep=1,hatchwidth=0.3,hatchsep=1.5,shadowsize=1,dimen=middle}
\psset{dotsize=0.7 2.5,dotscale=1 1,fillcolor=black}
\psset{arrowsize=1 2,arrowlength=1,arrowinset=0.25,tbarsize=0.7 5,bracketlength=0.15,rbracketlength=0.15}
\begin{pspicture}(0,0)(78.12,62.58)
\psline[linewidth=0.75](0,40)(30,40)
\psline[linewidth=0.75](30,20)(30,40)
\psline[linewidth=0.75](0,20)(30,20)
\psline[linewidth=1.1](15,20)(15,0)
\psline[linewidth=0.75](0,40)(0,20)
\rput(50,30){\EQLS}
\psline[linewidth=1.1](75,60)(75,0)
\newrgbcolor{userFillColour}{0.2 0 0.2}
\rput{0}(75,60){\psellipse[fillcolor=userFillColour,fillstyle=solid](0,0)(2.58,-2.58)}
\newrgbcolor{userFillColour}{0.2 0 0.2}
\rput{0}(15,60){\psellipse[fillcolor=userFillColour,fillstyle=solid](0,0)(2.58,-2.58)}
\psline[linewidth=1.1](15,60)(15,40)
\rput[l](16.88,10){$\medput$}
\rput[l](78.12,10){$\medput$}
\rput(15,30){$\eef$}
\rput[l](18.12,50){$\outputt$}
\end{pspicture}


==> PIC/halt.tex <==
%%Created by jPicEdt 1.4.1_03: mixed JPIC-XML/LaTeX format
%%Mon Oct 31 13:08:29 HST 2016
%%Begin JPIC-XML
%<?xml version="1.0" standalone="yes"?>
%<jpic x-min="0" x-max="90" y-min="0.62" y-max="102.58" auto-bounding="true">
%<multicurve stroke-width= "0.75"
%	 points= "(0,80);(0,80);(30,80);(30,80)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.75"
%	 points= "(30,60);(30,60);(30,80);(30,80)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.75"
%	 points= "(0,60);(0,60);(30,60);(30,60)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "1.1"
%	 points= "(15,60);(15,60);(15,40);(15,40)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.75"
%	 points= "(0,80);(0,80);(0,60);(0,60)"
%	 fill-style= "none"
%	 />
%<text text-vert-align= "center-v"
%	 stroke-width= "0.75"
%	 anchor-point= "(50,50)"
%	 text-frame= "noframe"
%	 fill-style= "none"
%	 text-hor-align= "center-h"
%	 >
%\EQLS
%</text>
%<multicurve stroke-width= "1.1"
%	 points= "(75,100);(75,100);(75,40);(75,40)"
%	 fill-style= "none"
%	 />
%<ellipse p3= "(77.58,97.42)"
%	 p2= "(77.58,102.58)"
%	 p1= "(72.42,102.58)"
%	 closure= "open"
%	 fill-color= "#330033"
%	 angle-end= "0"
%	 fill-style= "solid"
%	 angle-start= "0"
%	 />
%<ellipse p3= "(17.58,97.42)"
%	 p2= "(17.58,102.58)"
%	 p1= "(12.42,102.58)"
%	 closure= "open"
%	 fill-color= "#330033"
%	 angle-end= "0"
%	 fill-style= "solid"
%	 angle-start= "0"
%	 />
%<multicurve stroke-width= "1.1"
%	 points= "(15,100);(15,100);(15,80);(15,80)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.75"
%	 points= "(0,40);(0,40);(30,40);(30,40)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.75"
%	 points= "(30,20);(30,20);(30,40);(30,40)"
%	 fill-style= "none"
%	 />
%<text text-vert-align= "center-v"
%	 stroke-width= "0.75"
%	 anchor-point= "(17.5,10)"
%	 text-frame= "noframe"
%	 fill-style= "none"
%	 text-hor-align= "left"
%	 >
%$\inputt$
%</text>
%<multicurve stroke-width= "0.75"
%	 points= "(0,20);(0,20);(30,20);(30,20)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "1.1"
%	 points= "(15,20);(15,20);(15,0.62);(15,0.62)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.75"
%	 points= "(0,40);(0,40);(0,20);(0,20)"
%	 fill-style= "none"
%	 />
%<text text-vert-align= "center-v"
%	 anchor-point= "(15,30)"
%	 text-frame= "noframe"
%	 fill-style= "none"
%	 text-hor-align= "center-h"
%	 >
%$\gee$
%</text>
%<multicurve stroke-width= "0.75"
%	 points= "(60,40);(60,40);(90,40);(90,40)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.75"
%	 points= "(90,20);(90,20);(90,40);(90,40)"
%	 fill-style= "none"
%	 />
%<text text-vert-align= "center-v"
%	 stroke-width= "0.75"
%	 anchor-point= "(77.5,10)"
%	 text-frame= "noframe"
%	 fill-style= "none"
%	 text-hor-align= "left"
%	 >
%$\inputt$
%</text>
%<multicurve stroke-width= "0.75"
%	 points= "(60,20);(60,20);(90,20);(90,20)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "1.1"
%	 points= "(75,20);(75,20);(75,0.62);(75,0.62)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.75"
%	 points= "(60,40);(60,40);(60,20);(60,20)"
%	 fill-style= "none"
%	 />
%<text text-vert-align= "center-v"
%	 anchor-point= "(75,30)"
%	 text-frame= "noframe"
%	 fill-style= "none"
%	 text-hor-align= "center-h"
%	 >
%$\gee$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(16.88,50)"
%	 text-frame= "noframe"
%	 fill-style= "none"
%	 text-hor-align= "left"
%	 >
%$\medput$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(78.12,50)"
%	 text-frame= "noframe"
%	 fill-style= "none"
%	 text-hor-align= "left"
%	 >
%$\medput$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(15,70)"
%	 text-frame= "noframe"
%	 fill-style= "none"
%	 text-hor-align= "center-h"
%	 >
%$\eef$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(18.12,90)"
%	 text-frame= "noframe"
%	 fill-style= "none"
%	 text-hor-align= "left"
%	 >
%$\outputt$
%</text>
%</jpic>
%%End JPIC-XML
%PSTricks content-type (pstricks.sty package needed)
%Add \usepackage{pstricks} in the preamble of your LaTeX file
%You can rescale the whole picture (to 80% for instance) by using the command \def\JPicScale{0.8}
\ifx\JPicScale\undefined\def\JPicScale{1}\fi
\psset{unit=\JPicScale mm}
\psset{linewidth=0.3,dotsep=1,hatchwidth=0.3,hatchsep=1.5,shadowsize=1,dimen=middle}
\psset{dotsize=0.7 2.5,dotscale=1 1,fillcolor=black}
\psset{arrowsize=1 2,arrowlength=1,arrowinset=0.25,tbarsize=0.7 5,bracketlength=0.15,rbracketlength=0.15}
\begin{pspicture}(0,0)(90,102.58)
\psline[linewidth=0.75](0,80)(30,80)
\psline[linewidth=0.75](30,60)(30,80)
\psline[linewidth=0.75](0,60)(30,60)
\psline[linewidth=1.1](15,60)(15,40)
\psline[linewidth=0.75](0,80)(0,60)
\rput(50,50){\EQLS}
\psline[linewidth=1.1](75,100)(75,40)
\newrgbcolor{userFillColour}{0.2 0 0.2}
\rput{0}(75,100){\psellipse[fillcolor=userFillColour,fillstyle=solid](0,0)(2.58,-2.58)}
\newrgbcolor{userFillColour}{0.2 0 0.2}
\rput{0}(15,100){\psellipse[fillcolor=userFillColour,fillstyle=solid](0,0)(2.58,-2.58)}
\psline[linewidth=1.1](15,100)(15,80)
\psline[linewidth=0.75](0,40)(30,40)
\psline[linewidth=0.75](30,20)(30,40)
\rput[l](17.5,10){$\inputt$}
\psline[linewidth=0.75](0,20)(30,20)
\psline[linewidth=1.1](15,20)(15,0.62)
\psline[linewidth=0.75](0,40)(0,20)
\rput(15,30){$\gee$}
\psline[linewidth=0.75](60,40)(90,40)
\psline[linewidth=0.75](90,20)(90,40)
\rput[l](77.5,10){$\inputt$}
\psline[linewidth=0.75](60,20)(90,20)
\psline[linewidth=1.1](75,20)(75,0.62)
\psline[linewidth=0.75](60,40)(60,20)
\rput(75,30){$\gee$}
\rput[l](16.88,50){$\medput$}
\rput[l](78.12,50){$\medput$}
\rput(15,70){$\eef$}
\rput[l](18.12,90){$\outputt$}
\end{pspicture}


==> PIC/halter-1.tex <==
%%Created by jPicEdt 1.4.1_03: mixed JPIC-XML/LaTeX format
%%Tue Dec 18 13:14:53 GMT-08:00 2018
%%Begin JPIC-XML
%<?xml version="1.0" standalone="yes"?>
%<jpic x-min="25" x-max="262.5" y-min="-5" y-max="120" auto-bounding="true">
%<multicurve fill-style= "none"
%	 points= "(110,45);(110,45);(170,45);(170,45)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(170,20);(170,20);(170,45);(170,45)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(150,82.5);(150,82.5);(150,45);(150,45)"
%	 stroke-width= "0.75"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(150,-5)"
%	 text-frame= "noframe"
%	 stroke-width= "0.75"
%	 text-hor-align= "center-h"
%	 >
%$\inputt$
%</text>
%<multicurve fill-style= "none"
%	 points= "(135,20);(135,20);(170,20);(170,20)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(150,20);(150,20);(150,0);(150,0)"
%	 stroke-width= "0.75"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(148.12,31.88)"
%	 text-frame= "noframe"
%	 stroke-width= "0.75"
%	 text-hor-align= "center-h"
%	 >
%\universal
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(90,30)"
%	 text-frame= "noframe"
%	 stroke-width= "0.75"
%	 text-hor-align= "center-h"
%	 >
%\EQLS
%</text>
%<multicurve fill-style= "none"
%	 points= "(122.5,32.5);(122.5,32.5);(122.5,5);(122.5,5)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(110,45);(110,45);(135,20);(135,20)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(25,45);(25,45);(75,45);(75,45)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(75,20);(75,20);(75,45);(75,45)"
%	 stroke-width= "0.75"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(65,-5)"
%	 text-frame= "noframe"
%	 stroke-width= "0.75"
%	 text-hor-align= "center-h"
%	 >
%$\inputt$
%</text>
%<multicurve fill-style= "none"
%	 points= "(25,20);(25,20);(75,20);(75,20)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(65,20);(65,20);(65,0);(65,0)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(35,20);(35,20);(35,5);(35,5)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(25,45);(25,45);(25,20);(25,20)"
%	 stroke-width= "0.75"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(197.5,30)"
%	 text-frame= "noframe"
%	 stroke-width= "0.75"
%	 text-hor-align= "center-h"
%	 >
%\EQLS
%</text>
%<multicurve fill-style= "none"
%	 points= "(212.5,45);(212.5,45);(262.5,45);(262.5,45)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(262.5,20);(262.5,20);(262.5,45);(262.5,45)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(237.5,115);(237.5,115);(237.5,45);(237.5,45)"
%	 stroke-width= "0.75"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(237.5,120)"
%	 text-frame= "noframe"
%	 stroke-width= "0.75"
%	 text-hor-align= "center-h"
%	 >
%$\nameslang$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(252.5,-5)"
%	 text-frame= "noframe"
%	 stroke-width= "0.75"
%	 text-hor-align= "center-h"
%	 >
%$\inputt$
%</text>
%<multicurve fill-style= "none"
%	 points= "(212.5,20);(212.5,20);(262.5,20);(262.5,20)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(252.5,20);(252.5,20);(252.5,0);(252.5,0)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(222.5,20);(222.5,20);(222.5,5);(222.5,5)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(212.5,45);(212.5,45);(212.5,20);(212.5,20)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(50,52.5);(50,52.5);(50,45);(50,45)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(50,82.5);(50,82.5);(50,72.5);(50,72.5)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(40,72.5);(40,72.5);(60,72.5);(60,72.5)"
%	 stroke-width= "0.6"
%	 />
%<multicurve fill-style= "none"
%	 points= "(60,52.5);(60,52.5);(60,72.5);(60,72.5)"
%	 stroke-width= "0.6"
%	 />
%<multicurve fill-style= "none"
%	 points= "(40,52.5);(40,52.5);(60,52.5);(60,52.5)"
%	 stroke-width= "0.6"
%	 />
%<multicurve fill-style= "none"
%	 points= "(40,72.5);(40,72.5);(40,52.5);(40,52.5)"
%	 stroke-width= "0.6"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(50,62.5)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\nneg$
%</text>
%<multicurve fill-style= "none"
%	 points= "(27.5,-5);(27.5,-5);(45,-5);(45,-5)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(27.5,-5);(27.5,-5);(27.5,12.5);(27.5,12.5)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(27.5,12.5);(27.5,12.5);(45,-5);(45,-5)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(115,-5);(115,-5);(132.5,-5);(132.5,-5)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(115,-5);(115,-5);(115,12.5);(115,12.5)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(115,12.5);(115,12.5);(132.5,-5);(132.5,-5)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(215,-5);(215,-5);(232.5,-5);(232.5,-5)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(215,-5);(215,-5);(215,12.5);(215,12.5)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(215,12.5);(215,12.5);(232.5,-5);(232.5,-5)"
%	 stroke-width= "0.75"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(50,120)"
%	 text-frame= "noframe"
%	 stroke-width= "0.75"
%	 text-hor-align= "center-h"
%	 >
%$\nameslang$
%</text>
%<multicurve fill-style= "none"
%	 points= "(50,115);(50,115);(50,102.5);(50,102.5)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(42.5,92.5);(42.5,92.5);(60,92.5);(60,92.5)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(42.5,92.5);(42.5,92.5);(42.5,110);(42.5,110)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(42.5,110);(42.5,110);(60,92.5);(60,92.5)"
%	 stroke-width= "0.75"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "solid"
%	 anchor-point= "(47.5,97.5)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\tttrue$
%</text>
%<ellipse p3= "(153.75,78.75)"
%	 fill-style= "solid"
%	 p2= "(153.75,86.25)"
%	 p1= "(146.25,86.25)"
%	 closure= "open"
%	 angle-end= "0"
%	 angle-start= "0"
%	 />
%<ellipse p3= "(53.75,78.75)"
%	 fill-style= "solid"
%	 p2= "(53.75,86.25)"
%	 p1= "(46.25,86.25)"
%	 closure= "open"
%	 angle-end= "0"
%	 angle-start= "0"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(150,120)"
%	 text-frame= "noframe"
%	 stroke-width= "0.75"
%	 text-hor-align= "center-h"
%	 >
%$\nameslang$
%</text>
%<multicurve fill-style= "none"
%	 points= "(150,115);(150,115);(150,102.5);(150,102.5)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(142.5,92.5);(142.5,92.5);(160,92.5);(160,92.5)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(142.5,92.5);(142.5,92.5);(142.5,110);(142.5,110)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(142.5,110);(142.5,110);(160,92.5);(160,92.5)"
%	 stroke-width= "0.75"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "solid"
%	 anchor-point= "(147.5,97.5)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\tttrue$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(221.25,0)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\hfixp$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(50,32.5)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\hee$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(237.5,32.5)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\hee$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(120.62,0)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\hfixp$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(32.5,0)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\hfixp$
%</text>
%</jpic>
%%End JPIC-XML
%PSTricks content-type (pstricks.sty package needed)
%Add \usepackage{pstricks} in the preamble of your LaTeX file
%You can rescale the whole picture (to 80% for instance) by using the command \def\JPicScale{0.8}
\ifx\JPicScale\undefined\def\JPicScale{1}\fi
\psset{unit=\JPicScale mm}
\psset{linewidth=0.3,dotsep=1,hatchwidth=0.3,hatchsep=1.5,shadowsize=1,dimen=middle}
\psset{dotsize=0.7 2.5,dotscale=1 1,fillcolor=black}
\psset{arrowsize=1 2,arrowlength=1,arrowinset=0.25,tbarsize=0.7 5,bracketlength=0.15,rbracketlength=0.15}
\begin{pspicture}(0,0)(262.5,120)
\psline[linewidth=0.75](110,45)(170,45)
\psline[linewidth=0.75](170,20)(170,45)
\psline[linewidth=0.75](150,82.5)(150,45)
\rput(150,-5){$\inputt$}
\psline[linewidth=0.75](135,20)(170,20)
\psline[linewidth=0.75](150,20)(150,0)
\rput(148.12,31.88){\universal}
\rput(90,30){\EQLS}
\psline[linewidth=0.75](122.5,32.5)(122.5,5)
\psline[linewidth=0.75](110,45)(135,20)
\psline[linewidth=0.75](25,45)(75,45)
\psline[linewidth=0.75](75,20)(75,45)
\rput(65,-5){$\inputt$}
\psline[linewidth=0.75](25,20)(75,20)
\psline[linewidth=0.75](65,20)(65,0)
\psline[linewidth=0.75](35,20)(35,5)
\psline[linewidth=0.75](25,45)(25,20)
\rput(197.5,30){\EQLS}
\psline[linewidth=0.75](212.5,45)(262.5,45)
\psline[linewidth=0.75](262.5,20)(262.5,45)
\psline[linewidth=0.75](237.5,115)(237.5,45)
\rput(237.5,120){$\nameslang$}
\rput(252.5,-5){$\inputt$}
\psline[linewidth=0.75](212.5,20)(262.5,20)
\psline[linewidth=0.75](252.5,20)(252.5,0)
\psline[linewidth=0.75](222.5,20)(222.5,5)
\psline[linewidth=0.75](212.5,45)(212.5,20)
\psline[linewidth=0.75](50,52.5)(50,45)
\psline[linewidth=0.75](50,82.5)(50,72.5)
\psline[linewidth=0.6](40,72.5)(60,72.5)
\psline[linewidth=0.6](60,52.5)(60,72.5)
\psline[linewidth=0.6](40,52.5)(60,52.5)
\psline[linewidth=0.6](40,72.5)(40,52.5)
\rput(50,62.5){$\nneg$}
\psline[linewidth=0.75](27.5,-5)(45,-5)
\psline[linewidth=0.75](27.5,-5)(27.5,12.5)
\psline[linewidth=0.75](27.5,12.5)(45,-5)
\psline[linewidth=0.75](115,-5)(132.5,-5)
\psline[linewidth=0.75](115,-5)(115,12.5)
\psline[linewidth=0.75](115,12.5)(132.5,-5)
\psline[linewidth=0.75](215,-5)(232.5,-5)
\psline[linewidth=0.75](215,-5)(215,12.5)
\psline[linewidth=0.75](215,12.5)(232.5,-5)
\rput(50,120){$\nameslang$}
\psline[linewidth=0.75](50,115)(50,102.5)
\psline[linewidth=0.75](42.5,92.5)(60,92.5)
\psline[linewidth=0.75](42.5,92.5)(42.5,110)
\psline[linewidth=0.75](42.5,110)(60,92.5)
\rput(47.5,97.5){$\tttrue$}
\rput{0}(150,82.5){\psellipse[fillstyle=solid](0,0)(3.75,-3.75)}
\rput{0}(50,82.5){\psellipse[fillstyle=solid](0,0)(3.75,-3.75)}
\rput(150,120){$\nameslang$}
\psline[linewidth=0.75](150,115)(150,102.5)
\psline[linewidth=0.75](142.5,92.5)(160,92.5)
\psline[linewidth=0.75](142.5,92.5)(142.5,110)
\psline[linewidth=0.75](142.5,110)(160,92.5)
\rput(147.5,97.5){$\tttrue$}
\rput(221.25,0){$\hfixp$}
\rput(50,32.5){$\hee$}
\rput(237.5,32.5){$\hee$}
\rput(120.62,0){$\hfixp$}
\rput(32.5,0){$\hfixp$}
\end{pspicture}


==> PIC/halter-2.tex <==
%%Created by jPicEdt 1.4.1_03: mixed JPIC-XML/LaTeX format
%%Thu Dec 19 19:43:58 GMT-10:00 2019
%%Begin JPIC-XML
%<?xml version="1.0" standalone="yes"?>
%<jpic x-min="0" x-max="145" y-min="0" y-max="115" auto-bounding="true">
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(90,45);(90,45);(145,45);(145,45)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(145,20);(145,20);(145,45);(145,45)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(130,65);(130,65);(130,45);(130,45)"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 stroke-width= "0.75"
%	 anchor-point= "(127.5,1.25)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\inputt$
%</text>
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(115,20);(115,20);(145,20);(145,20)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(130,20);(130,20);(130,0);(130,0)"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 stroke-width= "0.75"
%	 anchor-point= "(128.12,31.88)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\universal
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 stroke-width= "0.75"
%	 anchor-point= "(75,30)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\EQLS
%</text>
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(102.5,32.5);(102.5,32.5);(102.5,0);(102.5,0)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(90,45);(90,45);(115,20);(115,20)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(0,45);(0,45);(50,45);(50,45)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(50,20);(50,20);(50,45);(50,45)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(25,115);(25,115);(25,45);(25,45)"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 stroke-width= "0.75"
%	 anchor-point= "(28.75,113.75)"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\nameslang$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 stroke-width= "0.75"
%	 anchor-point= "(37.5,1.25)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\inputt$
%</text>
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(0,20);(0,20);(50,20);(50,20)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(40,20);(40,20);(40,0);(40,0)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(10,20);(10,20);(10,0);(10,0)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(0,45);(0,45);(0,20);(0,20)"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(25,31.88)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\gee$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(100,1.25)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\progtype$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(7.5,1.25)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\progtype$
%</text>
%<ellipse p3= "(133.75,61.25)"
%	 p2= "(133.75,68.75)"
%	 fill-style= "solid"
%	 p1= "(126.25,68.75)"
%	 closure= "open"
%	 angle-end= "0"
%	 angle-start= "0"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 stroke-width= "0.75"
%	 anchor-point= "(133.75,113.75)"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\nameslang$
%</text>
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(130,115);(130,115);(130,85);(130,85)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(122.5,75);(122.5,75);(140,75);(140,75)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(122.5,75);(122.5,75);(122.5,92.5);(122.5,92.5)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(122.5,92.5);(122.5,92.5);(140,75);(140,75)"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "solid"
%	 anchor-point= "(127.5,80)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\tttrue$
%</text>
%</jpic>
%%End JPIC-XML
%PSTricks content-type (pstricks.sty package needed)
%Add \usepackage{pstricks} in the preamble of your LaTeX file
%You can rescale the whole picture (to 80% for instance) by using the command \def\JPicScale{0.8}
\ifx\JPicScale\undefined\def\JPicScale{1}\fi
\psset{unit=\JPicScale mm}
\psset{linewidth=0.3,dotsep=1,hatchwidth=0.3,hatchsep=1.5,shadowsize=1,dimen=middle}
\psset{dotsize=0.7 2.5,dotscale=1 1,fillcolor=black}
\psset{arrowsize=1 2,arrowlength=1,arrowinset=0.25,tbarsize=0.7 5,bracketlength=0.15,rbracketlength=0.15}
\begin{pspicture}(0,0)(145,115)
\psline[linewidth=0.75](90,45)(145,45)
\psline[linewidth=0.75](145,20)(145,45)
\psline[linewidth=0.75](130,65)(130,45)
\rput[r](127.5,1.25){$\inputt$}
\psline[linewidth=0.75](115,20)(145,20)
\psline[linewidth=0.75](130,20)(130,0)
\rput(128.12,31.88){\universal}
\rput(75,30){\EQLS}
\psline[linewidth=0.75](102.5,32.5)(102.5,0)
\psline[linewidth=0.75](90,45)(115,20)
\psline[linewidth=0.75](0,45)(50,45)
\psline[linewidth=0.75](50,20)(50,45)
\psline[linewidth=0.75](25,115)(25,45)
\rput[l](28.75,113.75){$\nameslang$}
\rput[r](37.5,1.25){$\inputt$}
\psline[linewidth=0.75](0,20)(50,20)
\psline[linewidth=0.75](40,20)(40,0)
\psline[linewidth=0.75](10,20)(10,0)
\psline[linewidth=0.75](0,45)(0,20)
\rput(25,31.88){$\gee$}
\rput[r](100,1.25){$\progtype$}
\rput[r](7.5,1.25){$\progtype$}
\rput{0}(130,65){\psellipse[fillstyle=solid](0,0)(3.75,-3.75)}
\rput[l](133.75,113.75){$\nameslang$}
\psline[linewidth=0.75](130,115)(130,85)
\psline[linewidth=0.75](122.5,75)(140,75)
\psline[linewidth=0.75](122.5,75)(122.5,92.5)
\psline[linewidth=0.75](122.5,92.5)(140,75)
\rput(127.5,80){$\tttrue$}
\end{pspicture}


==> PIC/homom-fun-uni.tex <==
%%Created by jPicEdt 1.4.1_03: mixed JPIC-XML/LaTeX format
%%Wed Jan 25 17:34:06 GMT-10:00 2023
%%Begin JPIC-XML
%<?xml version="1.0" standalone="yes"?>
%<jpic x-min="2.5" x-max="65.62" y-min="-1.25" y-max="45.62" auto-bounding="true">
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(54.38,21.88)"
%	 text-frame= "noframe"
%	 stroke-width= "0.15"
%	 text-hor-align= "center-h"
%	 >
%$\ahh$
%</text>
%<multicurve fill-style= "none"
%	 points= "(20.62,-1.25);(20.62,-1.25);(20.62,16.88);(20.62,16.88)"
%	 stroke-width= "0.15"
%	 />
%<multicurve fill-style= "none"
%	 points= "(8.12,-1.25);(8.12,-1.25);(8.12,16.88);(8.12,16.88)"
%	 stroke-width= "0.15"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(6.88,-0.62)"
%	 text-frame= "noframe"
%	 stroke-width= "0.15"
%	 text-hor-align= "right"
%	 >
%$\xxh$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(33.75,22.5)"
%	 text-frame= "noframe"
%	 stroke-width= "0.15"
%	 text-hor-align= "center-h"
%	 >
%\EQLS
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(14.38,21.88)"
%	 text-frame= "noframe"
%	 stroke-width= "0.15"
%	 text-hor-align= "center-h"
%	 >
%$\bhh$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(19.38,-0.62)"
%	 text-frame= "noframe"
%	 stroke-width= "0.15"
%	 text-hor-align= "right"
%	 >
%$\ah$
%</text>
%<multicurve fill-style= "none"
%	 points= "(13.75,26.88);(13.75,26.88);(13.75,45.62);(13.75,45.62)"
%	 stroke-width= "0.15"
%	 />
%<multicurve fill-style= "none"
%	 points= "(60.62,-1.25);(60.62,-1.25);(60.62,16.88);(60.62,16.88)"
%	 stroke-width= "0.15"
%	 />
%<multicurve fill-style= "none"
%	 points= "(48.12,10);(48.12,10);(48.12,16.88);(48.12,16.88)"
%	 stroke-width= "0.15"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(46.88,-0.62)"
%	 text-frame= "noframe"
%	 stroke-width= "0.15"
%	 text-hor-align= "right"
%	 >
%$\xxh$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(59.38,-0.62)"
%	 text-frame= "noframe"
%	 stroke-width= "0.15"
%	 text-hor-align= "right"
%	 >
%$\ah$
%</text>
%<multicurve fill-style= "none"
%	 points= "(53.75,26.88);(53.75,26.88);(53.75,45.62);(53.75,45.62)"
%	 stroke-width= "0.15"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(48.12,7.5)"
%	 text-frame= "noframe"
%	 stroke-width= "0.15"
%	 text-hor-align= "center-h"
%	 >
%$\aah$
%</text>
%<parallelogram p3= "(53.12,5)"
%	 fill-style= "none"
%	 p2= "(53.12,10)"
%	 p1= "(43.12,10)"
%	 stroke-width= "0.15"
%	 />
%<multicurve fill-style= "none"
%	 points= "(48.12,-1.25);(48.12,-1.25);(48.12,5);(48.12,5)"
%	 stroke-width= "0.15"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(55,44.38)"
%	 text-frame= "noframe"
%	 stroke-width= "0.15"
%	 text-hor-align= "left"
%	 >
%$\xxbbh$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(15,44.38)"
%	 text-frame= "noframe"
%	 stroke-width= "0.15"
%	 text-hor-align= "left"
%	 >
%$\xxbbh$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(46.88,13.12)"
%	 text-frame= "noframe"
%	 stroke-width= "0.15"
%	 text-hor-align= "right"
%	 >
%$\ssbbh$
%</text>
%<multicurve fill-style= "none"
%	 points= "(2.5,26.88);(2.5,26.88);(26.25,26.88);(26.25,26.88)"
%	 stroke-width= "0.15"
%	 />
%<multicurve fill-style= "none"
%	 points= "(2.5,16.88);(2.5,16.88);(26.25,16.88);(26.25,16.88)"
%	 stroke-width= "0.15"
%	 />
%<multicurve fill-style= "none"
%	 points= "(41.88,26.88);(41.88,26.88);(65.62,26.88);(65.62,26.88)"
%	 stroke-width= "0.15"
%	 />
%<multicurve fill-style= "none"
%	 points= "(41.88,16.88);(41.88,16.88);(65.62,16.88);(65.62,16.88)"
%	 stroke-width= "0.15"
%	 />
%<multicurve fill-style= "none"
%	 points= "(65.62,26.88);(65.62,26.88);(65.62,16.88);(65.62,16.88)"
%	 stroke-width= "0.15"
%	 />
%<multicurve fill-style= "none"
%	 points= "(2.5,26.88);(2.5,26.88);(2.5,16.88);(2.5,16.88)"
%	 stroke-width= "0.15"
%	 />
%<multicurve fill-style= "none"
%	 points= "(26.25,26.88);(26.25,26.88);(26.25,16.88);(26.25,16.88)"
%	 stroke-width= "0.15"
%	 />
%<multicurve fill-style= "none"
%	 points= "(41.88,26.88);(41.88,26.88);(51.88,16.88);(51.88,16.88)"
%	 stroke-width= "0.15"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(48.12,10)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\Dott$
%</text>
%</jpic>
%%End JPIC-XML
%LaTeX-picture environment using emulated lines and arcs
%You can rescale the whole picture (to 80% for instance) by using the command \def\JPicScale{0.8}
\ifx\JPicScale\undefined\def\JPicScale{1}\fi
\unitlength \JPicScale mm
\begin{picture}(65.62,45.62)(0,0)
\put(54.38,21.88){\makebox(0,0)[cc]{$\ahh$}}

\linethickness{0.15mm}
\put(20.62,-1.25){\line(0,1){18.13}}
\linethickness{0.15mm}
\put(8.12,-1.25){\line(0,1){18.13}}
\put(6.88,-0.62){\makebox(0,0)[cr]{$\xxh$}}

\put(33.75,22.5){\makebox(0,0)[cc]{\EQLS}}

\put(14.38,21.88){\makebox(0,0)[cc]{$\bhh$}}

\put(19.38,-0.62){\makebox(0,0)[cr]{$\ah$}}

\linethickness{0.15mm}
\put(13.75,26.88){\line(0,1){18.74}}
\linethickness{0.15mm}
\put(60.62,-1.25){\line(0,1){18.13}}
\linethickness{0.15mm}
\put(48.12,10){\line(0,1){6.88}}
\put(46.88,-0.62){\makebox(0,0)[cr]{$\xxh$}}

\put(59.38,-0.62){\makebox(0,0)[cr]{$\ah$}}

\linethickness{0.15mm}
\put(53.75,26.88){\line(0,1){18.74}}
\put(48.12,7.5){\makebox(0,0)[cc]{$\aah$}}

\linethickness{0.15mm}
\put(43.12,10){\line(1,0){10}}
\put(43.12,5){\line(0,1){5}}
\put(53.12,5){\line(0,1){5}}
\put(43.12,5){\line(1,0){10}}
\linethickness{0.15mm}
\put(48.12,-1.25){\line(0,1){6.25}}
\put(55,44.38){\makebox(0,0)[cl]{$\xxbbh$}}

\put(15,44.38){\makebox(0,0)[cl]{$\xxbbh$}}

\put(46.88,13.12){\makebox(0,0)[cr]{$\ssbbh$}}

\linethickness{0.15mm}
\put(2.5,26.88){\line(1,0){23.75}}
\linethickness{0.15mm}
\put(2.5,16.88){\line(1,0){23.75}}
\linethickness{0.15mm}
\put(41.88,26.88){\line(1,0){23.74}}
\linethickness{0.15mm}
\put(41.88,16.88){\line(1,0){23.74}}
\linethickness{0.15mm}
\put(65.62,16.88){\line(0,1){10}}
\linethickness{0.15mm}
\put(2.5,16.88){\line(0,1){10}}
\linethickness{0.15mm}
\put(26.25,16.88){\line(0,1){10}}
\linethickness{0.15mm}
\multiput(41.88,26.88)(0.12,-0.12){83}{\line(0,-1){0.12}}
\put(48.12,10){\makebox(0,0)[cc]{$\Dott$}}

\end{picture}


==> PIC/id.tex <==
%%Created by jPicEdt 1.4.1_03: mixed JPIC-XML/LaTeX format
%%Wed Sep 28 20:00:59 HST 2016
%%Begin JPIC-XML
%<?xml version="1.0" standalone="yes"?>
%<jpic x-min="16.88" x-max="20" y-min="7.5" y-max="50" auto-bounding="true">
%<text stroke-width= "0.75"
%	 text-vert-align= "center-v"
%	 anchor-point= "(16.88,9.38)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\inputt$
%</text>
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(20,50);(20,50);(20,7.5);(20,7.5)"
%	 />
%</jpic>
%%End JPIC-XML
%PSTricks content-type (pstricks.sty package needed)
%Add \usepackage{pstricks} in the preamble of your LaTeX file
%You can rescale the whole picture (to 80% for instance) by using the command \def\JPicScale{0.8}
\ifx\JPicScale\undefined\def\JPicScale{1}\fi
\psset{unit=\JPicScale mm}
\psset{linewidth=0.3,dotsep=1,hatchwidth=0.3,hatchsep=1.5,shadowsize=1,dimen=middle}
\psset{dotsize=0.7 2.5,dotscale=1 1,fillcolor=black}
\psset{arrowsize=1 2,arrowlength=1,arrowinset=0.25,tbarsize=0.7 5,bracketlength=0.15,rbracketlength=0.15}
\begin{pspicture}(0,0)(20,50)
\rput[r](16.88,9.38){$\inputt$}
\psline[linewidth=0.75](20,50)(20,7.5)
\end{pspicture}


==> PIC/idem-HEX.tex <==
%%Created by jPicEdt 1.4.1_03: mixed JPIC-XML/LaTeX format
%%Sun Nov 22 07:47:07 GMT-10:00 2020
%%Begin JPIC-XML
%<?xml version="1.0" standalone="yes"?>
%<jpic x-min="0" x-max="356.25" y-min="0" y-max="100" auto-bounding="true">
%<multicurve fill-style= "none"
%	 points= "(0,80);(0,80);(30,80);(30,80)"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(220,30);(220,30);(220,70);(220,70)"
%	 stroke-width= "0.2"
%	 />
%<multicurve fill-style= "none"
%	 points= "(15,60);(15,60);(15,40);(15,40)"
%	 stroke-width= "1"
%	 />
%<multicurve fill-style= "none"
%	 points= "(0,60);(0,60);(30,60);(30,60)"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(15,20);(15,20);(15,0);(15,0)"
%	 stroke-width= "1"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(40,50)"
%	 text-frame= "noframe"
%	 stroke-width= "0.35"
%	 text-hor-align= "center-h"
%	 >
%\EQLS
%</text>
%<multicurve fill-style= "none"
%	 points= "(0,80);(0,80);(10,70);(10,70)"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(10,70);(10,70);(0,60);(0,60)"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(30,80);(30,80);(20,70);(20,70)"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(20,70);(20,70);(30,60);(30,60)"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(0,40);(0,40);(30,40);(30,40)"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(0,20);(0,20);(30,20);(30,20)"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(0,40);(0,40);(10,30);(10,30)"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(10,30);(10,30);(0,20);(0,20)"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(30,40);(30,40);(20,30);(20,30)"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(20,30);(20,30);(30,20);(30,20)"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(15,100);(15,100);(15,80);(15,80)"
%	 stroke-width= "1"
%	 />
%<multicurve fill-style= "none"
%	 points= "(50,60);(50,60);(80,60);(80,60)"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(65,40);(65,40);(65,0);(65,0)"
%	 stroke-width= "1"
%	 />
%<multicurve fill-style= "none"
%	 points= "(50,40);(50,40);(80,40);(80,40)"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(50,60);(50,60);(60,50);(60,50)"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(60,50);(60,50);(50,40);(50,40)"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(80,60);(80,60);(70,50);(70,50)"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(70,50);(70,50);(80,40);(80,40)"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(65,100);(65,100);(65,60);(65,60)"
%	 stroke-width= "1"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(120,50)"
%	 text-frame= "noframe"
%	 stroke-width= "0.35"
%	 text-hor-align= "center-h"
%	 >
%\thenword
%</text>
%<multicurve fill-style= "none"
%	 points= "(160,60);(160,60);(190,60);(190,60)"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(175,40);(175,40);(175,0);(175,0)"
%	 stroke-width= "1"
%	 />
%<multicurve fill-style= "none"
%	 points= "(160,40);(160,40);(190,40);(190,40)"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(160,60);(160,60);(170,50);(170,50)"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(170,50);(170,50);(160,40);(160,40)"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(190,60);(190,60);(180,50);(180,50)"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(180,50);(180,50);(190,40);(190,40)"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(175,100);(175,100);(175,60);(175,60)"
%	 stroke-width= "1"
%	 />
%<multicurve fill-style= "none"
%	 points= "(205,80);(205,80);(235,80);(235,80)"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(215,70);(215,70);(225,70);(225,70)"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(220,20);(220,20);(220,0);(220,0)"
%	 stroke-width= "1"
%	 />
%<multicurve fill-style= "none"
%	 points= "(205,80);(205,80);(215,70);(215,70)"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(235,80);(235,80);(225,70);(225,70)"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(215,30);(215,30);(225,30);(225,30)"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(205,20);(205,20);(235,20);(235,20)"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(215,30);(215,30);(205,20);(205,20)"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(225,30);(225,30);(235,20);(235,20)"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(220,100);(220,100);(220,80);(220,80)"
%	 stroke-width= "1"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(200,50)"
%	 text-frame= "noframe"
%	 stroke-width= "0.35"
%	 text-hor-align= "center-h"
%	 >
%\EQLS
%</text>
%<multicurve fill-style= "none"
%	 points= "(355,0);(355,0);(355,100);(355,100)"
%	 stroke-width= "0.2"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(340,50)"
%	 text-frame= "noframe"
%	 stroke-width= "0.35"
%	 text-hor-align= "center-h"
%	 >
%\EQLS
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(270,50)"
%	 text-frame= "noframe"
%	 stroke-width= "0.35"
%	 text-hor-align= "center-h"
%	 >
%\withword
%</text>
%<multicurve fill-style= "none"
%	 points= "(320,80);(320,80);(320,100);(320,100)"
%	 stroke-width= "0.2"
%	 />
%<multicurve fill-style= "none"
%	 points= "(305,30);(305,30);(335,30);(335,30)"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(315,20);(315,20);(325,20);(325,20)"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(305,30);(305,30);(315,20);(315,20)"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(335,30);(335,30);(325,20);(325,20)"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(315,80);(315,80);(325,80);(325,80)"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(305,70);(305,70);(335,70);(335,70)"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(315,80);(315,80);(305,70);(305,70)"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(325,80);(325,80);(335,70);(335,70)"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(320,70);(320,70);(320,30);(320,30)"
%	 stroke-width= "1"
%	 />
%<multicurve fill-style= "none"
%	 points= "(320,0);(320,0);(320,20);(320,20)"
%	 stroke-width= "0.2"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(15,70)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\pee$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(15,30)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\pee$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(65,50)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\pee$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(175,50)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\pee$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(220,75)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\iee$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(220,25)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\qee$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(320,75)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\qee$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(320,25)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\iee$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(12.5,0)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\Aee$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(62.5,0)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\Aee$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(12.5,50)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\Aee$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(17.5,100)"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\Aee$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(67.5,100)"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\Aee$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(177.5,100)"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\Aee$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(172.5,0)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\Aee$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(217.5,0)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\Aee$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(222.5,100)"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\Aee$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(317.5,50)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\Aee$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(352.5,0)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\Ree$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(317.5,0)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\Ree$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(356.25,100)"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\Ree$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(321.25,100)"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\Ree$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(222.5,50)"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\Ree$
%</text>
%</jpic>
%%End JPIC-XML
%LaTeX-picture environment using emulated lines and arcs
%You can rescale the whole picture (to 80% for instance) by using the command \def\JPicScale{0.8}
\ifx\JPicScale\undefined\def\JPicScale{1}\fi
\unitlength \JPicScale mm
\begin{picture}(356.25,100)(0,0)
\linethickness{0.35mm}
\put(0,80){\line(1,0){30}}
\linethickness{0.2mm}
\put(220,30){\line(0,1){40}}
\linethickness{1mm}
\put(15,40){\line(0,1){20}}
\linethickness{0.35mm}
\put(0,60){\line(1,0){30}}
\linethickness{1mm}
\put(15,0){\line(0,1){20}}
\put(40,50){\makebox(0,0)[cc]{\EQLS}}

\linethickness{0.35mm}
\multiput(0,80)(0.12,-0.12){83}{\line(1,0){0.12}}
\linethickness{0.35mm}
\multiput(0,60)(0.12,0.12){83}{\line(1,0){0.12}}
\linethickness{0.35mm}
\multiput(20,70)(0.12,0.12){83}{\line(1,0){0.12}}
\linethickness{0.35mm}
\multiput(20,70)(0.12,-0.12){83}{\line(1,0){0.12}}
\linethickness{0.35mm}
\put(0,40){\line(1,0){30}}
\linethickness{0.35mm}
\put(0,20){\line(1,0){30}}
\linethickness{0.35mm}
\multiput(0,40)(0.12,-0.12){83}{\line(1,0){0.12}}
\linethickness{0.35mm}
\multiput(0,20)(0.12,0.12){83}{\line(1,0){0.12}}
\linethickness{0.35mm}
\multiput(20,30)(0.12,0.12){83}{\line(1,0){0.12}}
\linethickness{0.35mm}
\multiput(20,30)(0.12,-0.12){83}{\line(1,0){0.12}}
\linethickness{1mm}
\put(15,80){\line(0,1){20}}
\linethickness{0.35mm}
\put(50,60){\line(1,0){30}}
\linethickness{1mm}
\put(65,0){\line(0,1){40}}
\linethickness{0.35mm}
\put(50,40){\line(1,0){30}}
\linethickness{0.35mm}
\multiput(50,60)(0.12,-0.12){83}{\line(1,0){0.12}}
\linethickness{0.35mm}
\multiput(50,40)(0.12,0.12){83}{\line(1,0){0.12}}
\linethickness{0.35mm}
\multiput(70,50)(0.12,0.12){83}{\line(1,0){0.12}}
\linethickness{0.35mm}
\multiput(70,50)(0.12,-0.12){83}{\line(1,0){0.12}}
\linethickness{1mm}
\put(65,60){\line(0,1){40}}
\put(120,50){\makebox(0,0)[cc]{\thenword}}

\linethickness{0.35mm}
\put(160,60){\line(1,0){30}}
\linethickness{1mm}
\put(175,0){\line(0,1){40}}
\linethickness{0.35mm}
\put(160,40){\line(1,0){30}}
\linethickness{0.35mm}
\multiput(160,60)(0.12,-0.12){83}{\line(1,0){0.12}}
\linethickness{0.35mm}
\multiput(160,40)(0.12,0.12){83}{\line(1,0){0.12}}
\linethickness{0.35mm}
\multiput(180,50)(0.12,0.12){83}{\line(1,0){0.12}}
\linethickness{0.35mm}
\multiput(180,50)(0.12,-0.12){83}{\line(1,0){0.12}}
\linethickness{1mm}
\put(175,60){\line(0,1){40}}
\linethickness{0.35mm}
\put(205,80){\line(1,0){30}}
\linethickness{0.35mm}
\put(215,70){\line(1,0){10}}
\linethickness{1mm}
\put(220,0){\line(0,1){20}}
\linethickness{0.35mm}
\multiput(205,80)(0.12,-0.12){83}{\line(1,0){0.12}}
\linethickness{0.35mm}
\multiput(225,70)(0.12,0.12){83}{\line(1,0){0.12}}
\linethickness{0.35mm}
\put(215,30){\line(1,0){10}}
\linethickness{0.35mm}
\put(205,20){\line(1,0){30}}
\linethickness{0.35mm}
\multiput(205,20)(0.12,0.12){83}{\line(1,0){0.12}}
\linethickness{0.35mm}
\multiput(225,30)(0.12,-0.12){83}{\line(1,0){0.12}}
\linethickness{1mm}
\put(220,80){\line(0,1){20}}
\put(200,50){\makebox(0,0)[cc]{\EQLS}}

\linethickness{0.2mm}
\put(355,0){\line(0,1){100}}
\put(340,50){\makebox(0,0)[cc]{\EQLS}}

\put(270,50){\makebox(0,0)[cc]{\withword}}

\linethickness{0.2mm}
\put(320,80){\line(0,1){20}}
\linethickness{0.35mm}
\put(305,30){\line(1,0){30}}
\linethickness{0.35mm}
\put(315,20){\line(1,0){10}}
\linethickness{0.35mm}
\multiput(305,30)(0.12,-0.12){83}{\line(1,0){0.12}}
\linethickness{0.35mm}
\multiput(325,20)(0.12,0.12){83}{\line(1,0){0.12}}
\linethickness{0.35mm}
\put(315,80){\line(1,0){10}}
\linethickness{0.35mm}
\put(305,70){\line(1,0){30}}
\linethickness{0.35mm}
\multiput(305,70)(0.12,0.12){83}{\line(1,0){0.12}}
\linethickness{0.35mm}
\multiput(325,80)(0.12,-0.12){83}{\line(1,0){0.12}}
\linethickness{1mm}
\put(320,30){\line(0,1){40}}
\linethickness{0.2mm}
\put(320,0){\line(0,1){20}}
\put(15,70){\makebox(0,0)[cc]{$\pee$}}

\put(15,30){\makebox(0,0)[cc]{$\pee$}}

\put(65,50){\makebox(0,0)[cc]{$\pee$}}

\put(175,50){\makebox(0,0)[cc]{$\pee$}}

\put(220,75){\makebox(0,0)[cc]{$\iee$}}

\put(220,25){\makebox(0,0)[cc]{$\qee$}}

\put(320,75){\makebox(0,0)[cc]{$\qee$}}

\put(320,25){\makebox(0,0)[cc]{$\iee$}}

\put(12.5,0){\makebox(0,0)[cr]{$\Aee$}}

\put(62.5,0){\makebox(0,0)[cr]{$\Aee$}}

\put(12.5,50){\makebox(0,0)[cr]{$\Aee$}}

\put(17.5,100){\makebox(0,0)[cl]{$\Aee$}}

\put(67.5,100){\makebox(0,0)[cl]{$\Aee$}}

\put(177.5,100){\makebox(0,0)[cl]{$\Aee$}}

\put(172.5,0){\makebox(0,0)[cr]{$\Aee$}}

\put(217.5,0){\makebox(0,0)[cr]{$\Aee$}}

\put(222.5,100){\makebox(0,0)[cl]{$\Aee$}}

\put(317.5,50){\makebox(0,0)[cr]{$\Aee$}}

\put(352.5,0){\makebox(0,0)[cr]{$\Ree$}}

\put(317.5,0){\makebox(0,0)[cr]{$\Ree$}}

\put(356.25,100){\makebox(0,0)[cl]{$\Ree$}}

\put(321.25,100){\makebox(0,0)[cl]{$\Ree$}}

\put(222.5,50){\makebox(0,0)[cl]{$\Ree$}}

\end{picture}


==> PIC/idem-fun-HEX.tex <==
%%Created by jPicEdt 1.4.1_03: mixed JPIC-XML/LaTeX format
%%Sun Nov 22 07:59:27 GMT-10:00 2020
%%Begin JPIC-XML
%<?xml version="1.0" standalone="yes"?>
%<jpic x-min="0" x-max="195" y-min="0" y-max="140" auto-bounding="true">
%<multicurve fill-style= "none"
%	 points= "(80,120);(80,120);(110,120);(110,120)"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(175,100);(175,100);(175,120);(175,120)"
%	 stroke-width= "0.2"
%	 />
%<multicurve fill-style= "none"
%	 points= "(95,60);(95,60);(95,40);(95,40)"
%	 stroke-width= "1"
%	 />
%<multicurve fill-style= "none"
%	 points= "(80,100);(80,100);(110,100);(110,100)"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(95,20);(95,20);(95,0);(95,0)"
%	 stroke-width= "1"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(135,70)"
%	 text-frame= "noframe"
%	 stroke-width= "0.35"
%	 text-hor-align= "center-h"
%	 >
%\EQLS
%</text>
%<multicurve fill-style= "none"
%	 points= "(80,120);(80,120);(90,110);(90,110)"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(90,110);(90,110);(80,100);(80,100)"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(110,120);(110,120);(100,110);(100,110)"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(100,110);(100,110);(110,100);(110,100)"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(80,40);(80,40);(110,40);(110,40)"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(80,20);(80,20);(110,20);(110,20)"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(80,40);(80,40);(90,30);(90,30)"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(90,30);(90,30);(80,20);(80,20)"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(110,40);(110,40);(100,30);(100,30)"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(100,30);(100,30);(110,20);(110,20)"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(95,140);(95,140);(95,120);(95,120)"
%	 stroke-width= "1"
%	 />
%<multicurve fill-style= "none"
%	 points= "(80,80);(80,80);(110,80);(110,80)"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(95,100);(95,100);(95,80);(95,80)"
%	 stroke-width= "1"
%	 />
%<multicurve fill-style= "none"
%	 points= "(80,60);(80,60);(110,60);(110,60)"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(80,80);(80,80);(80,60);(80,60)"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(110,80);(110,80);(110,60);(110,60)"
%	 stroke-width= "0.35"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(95,110)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\pee$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(92.5,0)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\Aee$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(92.5,50)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\Aee$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(177.5,115)"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\Ree$
%</text>
%<multicurve fill-style= "none"
%	 points= "(160,130);(160,130);(190,130);(190,130)"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(175,60);(175,60);(175,50);(175,50)"
%	 stroke-width= "1"
%	 />
%<multicurve fill-style= "none"
%	 points= "(160,90);(160,90);(190,90);(190,90)"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(175,10);(175,10);(175,0);(175,0)"
%	 stroke-width= "1"
%	 />
%<multicurve fill-style= "none"
%	 points= "(160,130);(160,130);(170,120);(170,120)"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(170,100);(170,100);(160,90);(160,90)"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(190,130);(190,130);(180,120);(180,120)"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(180,100);(180,100);(190,90);(190,90)"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(160,50);(160,50);(190,50);(190,50)"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(160,10);(160,10);(190,10);(190,10)"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(160,50);(160,50);(170,40);(170,40)"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(170,20);(170,20);(160,10);(160,10)"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(190,50);(190,50);(180,40);(180,40)"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(180,20);(180,20);(190,10);(190,10)"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(175,140);(175,140);(175,130);(175,130)"
%	 stroke-width= "1"
%	 />
%<multicurve fill-style= "none"
%	 points= "(160,80);(160,80);(190,80);(190,80)"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(175,90);(175,90);(175,80);(175,80)"
%	 stroke-width= "1"
%	 />
%<multicurve fill-style= "none"
%	 points= "(160,60);(160,60);(190,60);(190,60)"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(160,80);(160,80);(160,60);(160,60)"
%	 stroke-width= "0.35"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(172.5,0)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\Aee$
%</text>
%<multicurve fill-style= "none"
%	 points= "(190,80);(190,80);(190,60);(190,60)"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(170,40);(170,40);(180,40);(180,40)"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(170,20);(170,20);(180,20);(180,20)"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(170,120);(170,120);(180,120);(180,120)"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(170,100);(170,100);(180,100);(180,100)"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(175,20);(175,20);(175,40);(175,40)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(155,110);(155,110);(195,110);(195,110)"
%	 stroke-width= "0.2"
%	 />
%<multicurve fill-style= "none"
%	 points= "(155,30);(155,30);(195,30);(195,30)"
%	 stroke-width= "0.2"
%	 />
%<multicurve fill-style= "none"
%	 points= "(195,110);(195,110);(195,30);(195,30)"
%	 stroke-width= "0.2"
%	 />
%<multicurve fill-style= "none"
%	 points= "(155,110);(155,110);(155,30);(155,30)"
%	 stroke-width= "0.2"
%	 />
%<multicurve fill-style= "none"
%	 points= "(15,60);(15,60);(15,0);(15,0)"
%	 stroke-width= "1"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(55,70)"
%	 text-frame= "noframe"
%	 stroke-width= "0.35"
%	 text-hor-align= "center-h"
%	 >
%\EQLS
%</text>
%<multicurve fill-style= "none"
%	 points= "(0,80);(0,80);(30,80);(30,80)"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(15,140);(15,140);(15,80);(15,80)"
%	 stroke-width= "1"
%	 />
%<multicurve fill-style= "none"
%	 points= "(0,60);(0,60);(30,60);(30,60)"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(0,80);(0,80);(0,60);(0,60)"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(30,80);(30,80);(30,60);(30,60)"
%	 stroke-width= "0.35"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(12.5,0)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\Aee$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(172.5,53.75)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\Aee$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(160,35)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\feef$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(15,70)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\heeh$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(95,70)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\heeh$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(175,70)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\heeh$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(172.5,25)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\ReeA$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(17.5,140)"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\Bee$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(97.5,140)"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\Bee$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(177.5,140)"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\Bee$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(97.5,90)"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\Bee$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(177.5,85)"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\Bee$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(95,30)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\peeA$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(175,15)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\qeeA$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(175,45)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\ieeA$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(175,95)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\qeeB$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(175,125)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\ieeB$
%</text>
%</jpic>
%%End JPIC-XML
%LaTeX-picture environment using emulated lines and arcs
%You can rescale the whole picture (to 80% for instance) by using the command \def\JPicScale{0.8}
\ifx\JPicScale\undefined\def\JPicScale{1}\fi
\unitlength \JPicScale mm
\begin{picture}(195,140)(0,0)
\linethickness{0.35mm}
\put(80,120){\line(1,0){30}}
\linethickness{0.2mm}
\put(175,100){\line(0,1){20}}
\linethickness{1mm}
\put(95,40){\line(0,1){20}}
\linethickness{0.35mm}
\put(80,100){\line(1,0){30}}
\linethickness{1mm}
\put(95,0){\line(0,1){20}}
\put(135,70){\makebox(0,0)[cc]{\EQLS}}

\linethickness{0.35mm}
\multiput(80,120)(0.12,-0.12){83}{\line(1,0){0.12}}
\linethickness{0.35mm}
\multiput(80,100)(0.12,0.12){83}{\line(1,0){0.12}}
\linethickness{0.35mm}
\multiput(100,110)(0.12,0.12){83}{\line(1,0){0.12}}
\linethickness{0.35mm}
\multiput(100,110)(0.12,-0.12){83}{\line(1,0){0.12}}
\linethickness{0.35mm}
\put(80,40){\line(1,0){30}}
\linethickness{0.35mm}
\put(80,20){\line(1,0){30}}
\linethickness{0.35mm}
\multiput(80,40)(0.12,-0.12){83}{\line(1,0){0.12}}
\linethickness{0.35mm}
\multiput(80,20)(0.12,0.12){83}{\line(1,0){0.12}}
\linethickness{0.35mm}
\multiput(100,30)(0.12,0.12){83}{\line(1,0){0.12}}
\linethickness{0.35mm}
\multiput(100,30)(0.12,-0.12){83}{\line(1,0){0.12}}
\linethickness{1mm}
\put(95,120){\line(0,1){20}}
\linethickness{0.35mm}
\put(80,80){\line(1,0){30}}
\linethickness{1mm}
\put(95,80){\line(0,1){20}}
\linethickness{0.35mm}
\put(80,60){\line(1,0){30}}
\linethickness{0.35mm}
\put(80,60){\line(0,1){20}}
\linethickness{0.35mm}
\put(110,60){\line(0,1){20}}
\put(95,110){\makebox(0,0)[cc]{$\pee$}}

\put(92.5,0){\makebox(0,0)[cr]{$\Aee$}}

\put(92.5,50){\makebox(0,0)[cr]{$\Aee$}}

\put(177.5,115){\makebox(0,0)[cl]{$\Ree$}}

\linethickness{0.35mm}
\put(160,130){\line(1,0){30}}
\linethickness{1mm}
\put(175,50){\line(0,1){10}}
\linethickness{0.35mm}
\put(160,90){\line(1,0){30}}
\linethickness{1mm}
\put(175,0){\line(0,1){10}}
\linethickness{0.35mm}
\multiput(160,130)(0.12,-0.12){83}{\line(1,0){0.12}}
\linethickness{0.35mm}
\multiput(160,90)(0.12,0.12){83}{\line(1,0){0.12}}
\linethickness{0.35mm}
\multiput(180,120)(0.12,0.12){83}{\line(1,0){0.12}}
\linethickness{0.35mm}
\multiput(180,100)(0.12,-0.12){83}{\line(1,0){0.12}}
\linethickness{0.35mm}
\put(160,50){\line(1,0){30}}
\linethickness{0.35mm}
\put(160,10){\line(1,0){30}}
\linethickness{0.35mm}
\multiput(160,50)(0.12,-0.12){83}{\line(1,0){0.12}}
\linethickness{0.35mm}
\multiput(160,10)(0.12,0.12){83}{\line(1,0){0.12}}
\linethickness{0.35mm}
\multiput(180,40)(0.12,0.12){83}{\line(1,0){0.12}}
\linethickness{0.35mm}
\multiput(180,20)(0.12,-0.12){83}{\line(1,0){0.12}}
\linethickness{1mm}
\put(175,130){\line(0,1){10}}
\linethickness{0.35mm}
\put(160,80){\line(1,0){30}}
\linethickness{1mm}
\put(175,80){\line(0,1){10}}
\linethickness{0.35mm}
\put(160,60){\line(1,0){30}}
\linethickness{0.35mm}
\put(160,60){\line(0,1){20}}
\put(172.5,0){\makebox(0,0)[cr]{$\Aee$}}

\linethickness{0.35mm}
\put(190,60){\line(0,1){20}}
\linethickness{0.35mm}
\put(170,40){\line(1,0){10}}
\linethickness{0.35mm}
\put(170,20){\line(1,0){10}}
\linethickness{0.35mm}
\put(170,120){\line(1,0){10}}
\linethickness{0.35mm}
\put(170,100){\line(1,0){10}}
\linethickness{0.3mm}
\put(175,20){\line(0,1){20}}
\linethickness{0.2mm}
\put(155,110){\line(1,0){40}}
\linethickness{0.2mm}
\put(155,30){\line(1,0){40}}
\linethickness{0.2mm}
\put(195,30){\line(0,1){80}}
\linethickness{0.2mm}
\put(155,30){\line(0,1){80}}
\linethickness{1mm}
\put(15,0){\line(0,1){60}}
\put(55,70){\makebox(0,0)[cc]{\EQLS}}

\linethickness{0.35mm}
\put(0,80){\line(1,0){30}}
\linethickness{1mm}
\put(15,80){\line(0,1){60}}
\linethickness{0.35mm}
\put(0,60){\line(1,0){30}}
\linethickness{0.35mm}
\put(0,60){\line(0,1){20}}
\linethickness{0.35mm}
\put(30,60){\line(0,1){20}}
\put(12.5,0){\makebox(0,0)[cr]{$\Aee$}}

\put(172.5,53.75){\makebox(0,0)[cr]{$\Aee$}}

\put(160,35){\makebox(0,0)[cc]{$\feef$}}

\put(15,70){\makebox(0,0)[cc]{$\heeh$}}

\put(95,70){\makebox(0,0)[cc]{$\heeh$}}

\put(175,70){\makebox(0,0)[cc]{$\heeh$}}

\put(172.5,25){\makebox(0,0)[cr]{$\ReeA$}}

\put(17.5,140){\makebox(0,0)[cl]{$\Bee$}}

\put(97.5,140){\makebox(0,0)[cl]{$\Bee$}}

\put(177.5,140){\makebox(0,0)[cl]{$\Bee$}}

\put(97.5,90){\makebox(0,0)[cl]{$\Bee$}}

\put(177.5,85){\makebox(0,0)[cl]{$\Bee$}}

\put(95,30){\makebox(0,0)[cc]{$\peeA$}}

\put(175,15){\makebox(0,0)[cc]{$\qeeA$}}

\put(175,45){\makebox(0,0)[cc]{$\ieeA$}}

\put(175,95){\makebox(0,0)[cc]{$\qeeB$}}

\put(175,125){\makebox(0,0)[cc]{$\ieeB$}}

\end{picture}


==> PIC/idem-fun.tex <==
%%Created by jPicEdt 1.4.1_03: mixed JPIC-XML/LaTeX format
%%Sun Nov 22 08:14:00 GMT-10:00 2020
%%Begin JPIC-XML
%<?xml version="1.0" standalone="yes"?>
%<jpic x-min="0" x-max="195" y-min="0" y-max="140" auto-bounding="true">
%<multicurve fill-style= "none"
%	 points= "(175,105);(175,105);(175,120);(175,120)"
%	 stroke-width= "0.2"
%	 />
%<multicurve fill-style= "none"
%	 points= "(95,60);(95,60);(95,40);(95,40)"
%	 stroke-width= "1"
%	 />
%<multicurve fill-style= "none"
%	 points= "(95,20);(95,20);(95,0);(95,0)"
%	 stroke-width= "1"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(135,70)"
%	 text-frame= "noframe"
%	 stroke-width= "0.35"
%	 text-hor-align= "center-h"
%	 >
%\EQLS
%</text>
%<multicurve fill-style= "none"
%	 points= "(95,140);(95,140);(95,120);(95,120)"
%	 stroke-width= "1"
%	 />
%<multicurve fill-style= "none"
%	 points= "(80,80);(80,80);(110,80);(110,80)"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(95,100);(95,100);(95,80);(95,80)"
%	 stroke-width= "1"
%	 />
%<multicurve fill-style= "none"
%	 points= "(80,60);(80,60);(110,60);(110,60)"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(80,80);(80,80);(80,60);(80,60)"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(110,80);(110,80);(110,60);(110,60)"
%	 stroke-width= "0.35"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(95,110)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\pee$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(92.5,0)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\Aee$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(100,50)"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\Aee$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(177.5,115)"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\Ree$
%</text>
%<multicurve fill-style= "none"
%	 points= "(175,60);(175,60);(175,45);(175,45)"
%	 stroke-width= "1"
%	 />
%<multicurve fill-style= "none"
%	 points= "(175,10);(175,10);(175,0);(175,0)"
%	 stroke-width= "1"
%	 />
%<multicurve fill-style= "none"
%	 points= "(175,140);(175,140);(175,130);(175,130)"
%	 stroke-width= "1"
%	 />
%<multicurve fill-style= "none"
%	 points= "(160,80);(160,80);(190,80);(190,80)"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(175,95);(175,95);(175,80);(175,80)"
%	 stroke-width= "1"
%	 />
%<multicurve fill-style= "none"
%	 points= "(160,60);(160,60);(190,60);(190,60)"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(160,80);(160,80);(160,60);(160,60)"
%	 stroke-width= "0.35"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(172.5,0)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\Aee$
%</text>
%<multicurve fill-style= "none"
%	 points= "(190,80);(190,80);(190,60);(190,60)"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(175,20);(175,20);(175,35);(175,35)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(155,110);(155,110);(195,110);(195,110)"
%	 stroke-width= "0.2"
%	 />
%<multicurve fill-style= "none"
%	 points= "(155,30);(155,30);(195,30);(195,30)"
%	 stroke-width= "0.2"
%	 />
%<multicurve fill-style= "none"
%	 points= "(195,110);(195,110);(195,30);(195,30)"
%	 stroke-width= "0.2"
%	 />
%<multicurve fill-style= "none"
%	 points= "(155,110);(155,110);(155,30);(155,30)"
%	 stroke-width= "0.2"
%	 />
%<multicurve fill-style= "none"
%	 points= "(15,60);(15,60);(15,0);(15,0)"
%	 stroke-width= "1"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(55,70)"
%	 text-frame= "noframe"
%	 stroke-width= "0.35"
%	 text-hor-align= "center-h"
%	 >
%\EQLS
%</text>
%<multicurve fill-style= "none"
%	 points= "(0,80);(0,80);(30,80);(30,80)"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(15,140);(15,140);(15,80);(15,80)"
%	 stroke-width= "1"
%	 />
%<multicurve fill-style= "none"
%	 points= "(0,60);(0,60);(30,60);(30,60)"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(0,80);(0,80);(0,60);(0,60)"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(30,80);(30,80);(30,60);(30,60)"
%	 stroke-width= "0.35"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(12.5,0)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\Aee$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(177.5,52.5)"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\Aee$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(160,95)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\feef$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(15,70)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\heeh$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(95,70)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\heeh$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(175,70)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\heeh$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(172.5,25)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\ReeA$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(17.5,140)"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\Bee$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(97.5,140)"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\Bee$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(177.5,140)"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\Bee$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(92.5,90)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\Bee$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(172.5,85)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\Bee$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(95,30)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\peeA$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(180,15)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\qeeA$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(172.5,40)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\ieeA$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(180,100)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\qeeB$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(175,125)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\ieeB$
%</text>
%<multicurve fill-style= "none"
%	 points= "(85,130);(85,130);(105,110);(105,110)"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(85,110);(85,110);(105,90);(105,90)"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(85,130);(85,130);(85,110);(85,110)"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(105,110);(105,110);(105,90);(105,90)"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(165,140);(165,140);(185,120);(185,120)"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(165,120);(165,120);(185,120);(185,120)"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(165,140);(165,140);(165,120);(165,120)"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(165,20);(165,20);(185,20);(185,20)"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(165,20);(165,20);(185,0);(185,0)"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(185,20);(185,20);(185,0);(185,0)"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(85,50);(85,50);(105,30);(105,30)"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(85,30);(85,30);(105,10);(105,10)"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(85,50);(85,50);(85,30);(85,30)"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(105,30);(105,30);(105,10);(105,10)"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(165,55);(165,55);(185,35);(185,35)"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(165,35);(165,35);(185,35);(185,35)"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(165,55);(165,55);(165,35);(165,35)"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(165,105);(165,105);(185,105);(185,105)"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(165,105);(165,105);(185,85);(185,85)"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(185,105);(185,105);(185,85);(185,85)"
%	 stroke-width= "0.35"
%	 />
%</jpic>
%%End JPIC-XML
%LaTeX-picture environment using emulated lines and arcs
%You can rescale the whole picture (to 80% for instance) by using the command \def\JPicScale{0.8}
\ifx\JPicScale\undefined\def\JPicScale{1}\fi
\unitlength \JPicScale mm
\begin{picture}(195,140)(0,0)
\linethickness{0.2mm}
\put(175,105){\line(0,1){15}}
\linethickness{1mm}
\put(95,40){\line(0,1){20}}
\linethickness{1mm}
\put(95,0){\line(0,1){20}}
\put(135,70){\makebox(0,0)[cc]{\EQLS}}

\linethickness{1mm}
\put(95,120){\line(0,1){20}}
\linethickness{0.35mm}
\put(80,80){\line(1,0){30}}
\linethickness{1mm}
\put(95,80){\line(0,1){20}}
\linethickness{0.35mm}
\put(80,60){\line(1,0){30}}
\linethickness{0.35mm}
\put(80,60){\line(0,1){20}}
\linethickness{0.35mm}
\put(110,60){\line(0,1){20}}
\put(95,110){\makebox(0,0)[cc]{$\pee$}}

\put(92.5,0){\makebox(0,0)[cr]{$\Aee$}}

\put(100,50){\makebox(0,0)[cl]{$\Aee$}}

\put(177.5,115){\makebox(0,0)[cl]{$\Ree$}}

\linethickness{1mm}
\put(175,45){\line(0,1){15}}
\linethickness{1mm}
\put(175,0){\line(0,1){10}}
\linethickness{1mm}
\put(175,130){\line(0,1){10}}
\linethickness{0.35mm}
\put(160,80){\line(1,0){30}}
\linethickness{1mm}
\put(175,80){\line(0,1){15}}
\linethickness{0.35mm}
\put(160,60){\line(1,0){30}}
\linethickness{0.35mm}
\put(160,60){\line(0,1){20}}
\put(172.5,0){\makebox(0,0)[cr]{$\Aee$}}

\linethickness{0.35mm}
\put(190,60){\line(0,1){20}}
\linethickness{0.3mm}
\put(175,20){\line(0,1){15}}
\linethickness{0.2mm}
\put(155,110){\line(1,0){40}}
\linethickness{0.2mm}
\put(155,30){\line(1,0){40}}
\linethickness{0.2mm}
\put(195,30){\line(0,1){80}}
\linethickness{0.2mm}
\put(155,30){\line(0,1){80}}
\linethickness{1mm}
\put(15,0){\line(0,1){60}}
\put(55,70){\makebox(0,0)[cc]{\EQLS}}

\linethickness{0.35mm}
\put(0,80){\line(1,0){30}}
\linethickness{1mm}
\put(15,80){\line(0,1){60}}
\linethickness{0.35mm}
\put(0,60){\line(1,0){30}}
\linethickness{0.35mm}
\put(0,60){\line(0,1){20}}
\linethickness{0.35mm}
\put(30,60){\line(0,1){20}}
\put(12.5,0){\makebox(0,0)[cr]{$\Aee$}}

\put(177.5,52.5){\makebox(0,0)[cl]{$\Aee$}}

\put(160,95){\makebox(0,0)[cc]{$\feef$}}

\put(15,70){\makebox(0,0)[cc]{$\heeh$}}

\put(95,70){\makebox(0,0)[cc]{$\heeh$}}

\put(175,70){\makebox(0,0)[cc]{$\heeh$}}

\put(172.5,25){\makebox(0,0)[cr]{$\ReeA$}}

\put(17.5,140){\makebox(0,0)[cl]{$\Bee$}}

\put(97.5,140){\makebox(0,0)[cl]{$\Bee$}}

\put(177.5,140){\makebox(0,0)[cl]{$\Bee$}}

\put(92.5,90){\makebox(0,0)[cr]{$\Bee$}}

\put(172.5,85){\makebox(0,0)[cr]{$\Bee$}}

\put(95,30){\makebox(0,0)[cc]{$\peeA$}}

\put(180,15){\makebox(0,0)[cc]{$\qeeA$}}

\put(172.5,40){\makebox(0,0)[cc]{$\ieeA$}}

\put(180,100){\makebox(0,0)[cc]{$\qeeB$}}

\put(175,125){\makebox(0,0)[cc]{$\ieeB$}}

\linethickness{0.35mm}
\multiput(85,130)(0.12,-0.12){167}{\line(1,0){0.12}}
\linethickness{0.35mm}
\multiput(85,110)(0.12,-0.12){167}{\line(1,0){0.12}}
\linethickness{0.35mm}
\put(85,110){\line(0,1){20}}
\linethickness{0.35mm}
\put(105,90){\line(0,1){20}}
\linethickness{0.35mm}
\multiput(165,140)(0.12,-0.12){167}{\line(1,0){0.12}}
\linethickness{0.35mm}
\put(165,120){\line(1,0){20}}
\linethickness{0.35mm}
\put(165,120){\line(0,1){20}}
\linethickness{0.35mm}
\put(165,20){\line(1,0){20}}
\linethickness{0.35mm}
\multiput(165,20)(0.12,-0.12){167}{\line(1,0){0.12}}
\linethickness{0.35mm}
\put(185,0){\line(0,1){20}}
\linethickness{0.35mm}
\multiput(85,50)(0.12,-0.12){167}{\line(1,0){0.12}}
\linethickness{0.35mm}
\multiput(85,30)(0.12,-0.12){167}{\line(1,0){0.12}}
\linethickness{0.35mm}
\put(85,30){\line(0,1){20}}
\linethickness{0.35mm}
\put(105,10){\line(0,1){20}}
\linethickness{0.35mm}
\multiput(165,55)(0.12,-0.12){167}{\line(1,0){0.12}}
\linethickness{0.35mm}
\put(165,35){\line(1,0){20}}
\linethickness{0.35mm}
\put(165,35){\line(0,1){20}}
\linethickness{0.35mm}
\put(165,105){\line(1,0){20}}
\linethickness{0.35mm}
\multiput(165,105)(0.12,-0.12){167}{\line(1,0){0.12}}
\linethickness{0.35mm}
\put(185,85){\line(0,1){20}}
\end{picture}


==> PIC/idem-moncom-def.tex <==
%%Created by jPicEdt 1.4.1_03: mixed JPIC-XML/LaTeX format
%%Sun Dec 13 10:41:59 GMT-10:00 2020
%%Begin JPIC-XML
%<?xml version="1.0" standalone="yes"?>
%<jpic x-min="0" x-max="231.25" y-min="0" y-max="100" auto-bounding="true">
%<multicurve fill-style= "none"
%	 points= "(55,30);(55,30);(55,70);(55,70)"
%	 stroke-width= "0.2"
%	 />
%<multicurve fill-style= "none"
%	 points= "(10,40);(10,40);(10,0);(10,0)"
%	 stroke-width= "1"
%	 />
%<multicurve fill-style= "none"
%	 points= "(10,100);(10,100);(10,60);(10,60)"
%	 stroke-width= "1"
%	 />
%<multicurve fill-style= "none"
%	 points= "(55,20);(55,20);(55,0);(55,0)"
%	 stroke-width= "1"
%	 />
%<multicurve fill-style= "none"
%	 points= "(55,100);(55,100);(55,80);(55,80)"
%	 stroke-width= "1"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(35,50)"
%	 text-frame= "noframe"
%	 stroke-width= "0.35"
%	 text-hor-align= "center-h"
%	 >
%\EQLS
%</text>
%<multicurve fill-style= "none"
%	 points= "(230,0);(230,0);(230,100);(230,100)"
%	 stroke-width= "0.2"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(215,50)"
%	 text-frame= "noframe"
%	 stroke-width= "0.35"
%	 text-hor-align= "center-h"
%	 >
%\EQLS
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(125,50)"
%	 text-frame= "noframe"
%	 stroke-width= "0.35"
%	 text-hor-align= "center-h"
%	 >
%\withword
%</text>
%<multicurve fill-style= "none"
%	 points= "(195,80);(195,80);(195,100);(195,100)"
%	 stroke-width= "0.2"
%	 />
%<multicurve fill-style= "none"
%	 points= "(195,70);(195,70);(195,30);(195,30)"
%	 stroke-width= "1"
%	 />
%<multicurve fill-style= "none"
%	 points= "(195,0);(195,0);(195,20);(195,20)"
%	 stroke-width= "0.2"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(10,50)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\pee$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(52.5,75)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\iee$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(57.5,25)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\qee$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(197.5,75)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\qee$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(192.5,25)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\iee$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(12.5,100)"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\Aee$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(7.5,0)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\Aee$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(52.5,0)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\Aee$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(57.5,100)"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\Aee$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(192.5,50)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\Aee$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(227.5,0)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\Ree$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(192.5,0)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\Ree$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(231.25,100)"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\Ree$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(196.25,100)"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\Ree$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(57.5,50)"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\Ree$
%</text>
%<multicurve fill-style= "none"
%	 points= "(0,70);(0,70);(20,50);(20,50)"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(0,50);(0,50);(20,30);(20,30)"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(0,70);(0,70);(0,50);(0,50)"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(20,50);(20,50);(20,30);(20,30)"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(45,90);(45,90);(65,70);(65,70)"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(45,70);(45,70);(65,70);(65,70)"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(45,90);(45,90);(45,70);(45,70)"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(45,30);(45,30);(65,30);(65,30)"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(45,30);(45,30);(65,10);(65,10)"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(65,30);(65,30);(65,10);(65,10)"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(185,40);(185,40);(205,20);(205,20)"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(185,20);(185,20);(205,20);(205,20)"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(185,40);(185,40);(185,20);(185,20)"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(185,80);(185,80);(205,80);(205,80)"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(185,80);(185,80);(205,60);(205,60)"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(205,80);(205,80);(205,60);(205,60)"
%	 stroke-width= "0.35"
%	 />
%</jpic>
%%End JPIC-XML
%PSTricks content-type (pstricks.sty package needed)
%Add \usepackage{pstricks} in the preamble of your LaTeX file
%You can rescale the whole picture (to 80% for instance) by using the command \def\JPicScale{0.8}
\ifx\JPicScale\undefined\def\JPicScale{1}\fi
\psset{unit=\JPicScale mm}
\psset{linewidth=0.3,dotsep=1,hatchwidth=0.3,hatchsep=1.5,shadowsize=1,dimen=middle}
\psset{dotsize=0.7 2.5,dotscale=1 1,fillcolor=black}
\psset{arrowsize=1 2,arrowlength=1,arrowinset=0.25,tbarsize=0.7 5,bracketlength=0.15,rbracketlength=0.15}
\begin{pspicture}(0,0)(231.25,100)
\psline[linewidth=0.2](55,30)(55,70)
\psline[linewidth=1](10,40)(10,0)
\psline[linewidth=1](10,100)(10,60)
\psline[linewidth=1](55,20)(55,0)
\psline[linewidth=1](55,100)(55,80)
\rput(35,50){\EQLS}
\psline[linewidth=0.2](230,0)(230,100)
\rput(215,50){\EQLS}
\rput(125,50){\withword}
\psline[linewidth=0.2](195,80)(195,100)
\psline[linewidth=1](195,70)(195,30)
\psline[linewidth=0.2](195,0)(195,20)
\rput(10,50){$\pee$}
\rput(52.5,75){$\iee$}
\rput(57.5,25){$\qee$}
\rput(197.5,75){$\qee$}
\rput(192.5,25){$\iee$}
\rput[l](12.5,100){$\Aee$}
\rput[r](7.5,0){$\Aee$}
\rput[r](52.5,0){$\Aee$}
\rput[l](57.5,100){$\Aee$}
\rput[r](192.5,50){$\Aee$}
\rput[r](227.5,0){$\Ree$}
\rput[r](192.5,0){$\Ree$}
\rput[l](231.25,100){$\Ree$}
\rput[l](196.25,100){$\Ree$}
\rput[l](57.5,50){$\Ree$}
\psline[linewidth=0.35](0,70)(20,50)
\psline[linewidth=0.35](0,50)(20,30)
\psline[linewidth=0.35](0,70)(0,50)
\psline[linewidth=0.35](20,50)(20,30)
\psline[linewidth=0.35](45,90)(65,70)
\psline[linewidth=0.35](45,70)(65,70)
\psline[linewidth=0.35](45,90)(45,70)
\psline[linewidth=0.35](45,30)(65,30)
\psline[linewidth=0.35](45,30)(65,10)
\psline[linewidth=0.35](65,30)(65,10)
\psline[linewidth=0.35](185,40)(205,20)
\psline[linewidth=0.35](185,20)(205,20)
\psline[linewidth=0.35](185,40)(185,20)
\psline[linewidth=0.35](185,80)(205,80)
\psline[linewidth=0.35](185,80)(205,60)
\psline[linewidth=0.35](205,80)(205,60)
\end{pspicture}


==> PIC/idem-quot-1.tex <==
%%Created by jPicEdt 1.4.1_03: mixed JPIC-XML/LaTeX format
%%Tue Jun 01 16:10:21 GMT-10:00 2021
%%Begin JPIC-XML
%<?xml version="1.0" standalone="yes"?>
%<jpic x-min="0" x-max="250" y-min="-15" y-max="205" auto-bounding="true">
%<multicurve fill-style= "none"
%	 points= "(215,5);(215,5);(245,5);(245,5)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(215,5);(215,5);(215,35);(215,35)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(215,35);(215,35);(245,5);(245,5)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(215,185);(215,185);(245,185);(245,185)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(245,155);(245,155);(245,185);(245,185)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(215,185);(215,185);(245,155);(245,155)"
%	 stroke-width= "0.75"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(230,20)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\DOTT
%</text>
%<multicurve fill-style= "none"
%	 points= "(10,105);(10,105);(10,165);(10,165)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(0,95);(0,95);(0,115);(0,115)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(0,115);(0,115);(20,95);(20,95)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(20,75);(20,75);(20,95);(20,95)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(0,95);(0,95);(20,75);(20,75)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(10,25);(10,25);(10,85);(10,85)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(230,185);(230,185);(230,205);(230,205)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(230,-15);(230,-15);(230,5);(230,5)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(120,62.5);(120,62.5);(152.5,30);(152.5,30)"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(120,160);(120,160);(120,127.5);(120,127.5)"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(140,175);(140,175);(140,147.5);(140,147.5)"
%	 stroke-width= "1.2"
%	 />
%<multicurve fill-style= "none"
%	 points= "(140,42.5);(140,42.5);(140,15);(140,15)"
%	 stroke-width= "1.2"
%	 />
%<multicurve fill-style= "none"
%	 points= "(127.5,160);(127.5,160);(160,127.5);(160,127.5)"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(160,62.5);(160,62.5);(160,30);(160,30)"
%	 stroke-width= "0.35"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(140,147.5)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\DOTT
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(142.5,93.75)"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\Ree$
%</text>
%<multicurve fill-style= "none"
%	 points= "(160,30);(160,30);(152.5,30);(152.5,30)"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(127.5,160);(127.5,160);(120,160);(120,160)"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(140,127.5);(140,127.5);(140,62.5);(140,62.5)"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(160,127.5);(160,127.5);(120,127.5);(120,127.5)"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(160,62.5);(160,62.5);(120,62.5);(120,62.5)"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(80,105);(80,105);(80,125);(80,125)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(70,95);(70,95);(70,115);(70,115)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(70,115);(70,115);(90,95);(90,95)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(90,75);(90,75);(90,95);(90,95)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(70,95);(70,95);(90,75);(90,75)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(80,65);(80,65);(80,85);(80,85)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(80,175);(80,175);(80,140);(80,140)"
%	 stroke-width= "1.2"
%	 />
%<multicurve fill-style= "none"
%	 points= "(65,125);(65,125);(95,125);(95,125)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(65,125);(65,125);(65,155);(65,155)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(65,155);(65,155);(95,125);(95,125)"
%	 stroke-width= "0.75"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(80,140)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\DOTT
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(75,132.5)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\encobool$
%</text>
%<multicurve fill-style= "none"
%	 points= "(80,50);(80,50);(80,15);(80,15)"
%	 stroke-width= "1.2"
%	 />
%<multicurve fill-style= "none"
%	 points= "(65,65);(65,65);(95,65);(95,65)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(95,35);(95,35);(95,65);(95,65)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(65,65);(65,65);(95,35);(95,35)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(100,30);(100,30);(92.5,30);(92.5,30)"
%	 stroke-width= "0.35"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(83.75,56.25)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\booleval$
%</text>
%<multicurve fill-style= "none"
%	 points= "(60,160);(60,160);(60,62.5);(60,62.5)"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(67.5,160);(67.5,160);(100,127.5);(100,127.5)"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(67.5,160);(67.5,160);(60,160);(60,160)"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(100,127.5);(100,127.5);(100,30);(100,30)"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(60,62.5);(60,62.5);(92.5,30);(92.5,30)"
%	 stroke-width= "0.35"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(112.5,90)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\EQLS
%</text>
%<multicurve fill-style= "none"
%	 points= "(210,62.5);(210,62.5);(242.5,30);(242.5,30)"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(210,160);(210,160);(210,127.5);(210,127.5)"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(230,170);(230,170);(230,147.5);(230,147.5)"
%	 stroke-width= "1.2"
%	 />
%<multicurve fill-style= "none"
%	 points= "(230,42.5);(230,42.5);(230,20);(230,20)"
%	 stroke-width= "1.2"
%	 />
%<multicurve fill-style= "none"
%	 points= "(217.5,160);(217.5,160);(250,127.5);(250,127.5)"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(250,62.5);(250,62.5);(250,30);(250,30)"
%	 stroke-width= "0.35"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(230,147.5)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\DOTT
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(232.5,93.75)"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\Ree$
%</text>
%<multicurve fill-style= "none"
%	 points= "(250,30);(250,30);(242.5,30);(242.5,30)"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(217.5,160);(217.5,160);(210,160);(210,160)"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(230,127.5);(230,127.5);(230,62.5);(230,62.5)"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(250,127.5);(250,127.5);(210,127.5);(210,127.5)"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(250,62.5);(250,62.5);(210,62.5);(210,62.5)"
%	 stroke-width= "0.35"
%	 />
%</jpic>
%%End JPIC-XML
%LaTeX-picture environment using emulated lines and arcs
%You can rescale the whole picture (to 80% for instance) by using the command \def\JPicScale{0.8}
\ifx\JPicScale\undefined\def\JPicScale{1}\fi
\unitlength \JPicScale mm
\begin{picture}(250,205)(0,0)
\linethickness{0.75mm}
\put(215,5){\line(1,0){30}}
\linethickness{0.75mm}
\put(215,5){\line(0,1){30}}
\linethickness{0.75mm}
\multiput(215,35)(0.12,-0.12){250}{\line(1,0){0.12}}
\linethickness{0.75mm}
\put(215,185){\line(1,0){30}}
\linethickness{0.75mm}
\put(245,155){\line(0,1){30}}
\linethickness{0.75mm}
\multiput(215,185)(0.12,-0.12){250}{\line(1,0){0.12}}
\put(230,20){\makebox(0,0)[cc]{\DOTT}}

\linethickness{0.75mm}
\put(10,105){\line(0,1){60}}
\linethickness{0.75mm}
\put(0,95){\line(0,1){20}}
\linethickness{0.75mm}
\multiput(0,115)(0.12,-0.12){167}{\line(1,0){0.12}}
\linethickness{0.75mm}
\put(20,75){\line(0,1){20}}
\linethickness{0.75mm}
\multiput(0,95)(0.12,-0.12){167}{\line(1,0){0.12}}
\linethickness{0.75mm}
\put(10,25){\line(0,1){60}}
\linethickness{0.75mm}
\put(230,185){\line(0,1){20}}
\linethickness{0.75mm}
\put(230,-15){\line(0,1){20}}
\linethickness{0.35mm}
\multiput(120,62.5)(0.12,-0.12){271}{\line(1,0){0.12}}
\linethickness{0.35mm}
\put(120,127.5){\line(0,1){32.5}}
\linethickness{1.2mm}
\put(140,147.5){\line(0,1){27.5}}
\linethickness{1.2mm}
\put(140,15){\line(0,1){27.5}}
\linethickness{0.35mm}
\multiput(127.5,160)(0.12,-0.12){271}{\line(1,0){0.12}}
\linethickness{0.35mm}
\put(160,30){\line(0,1){32.5}}
\put(140,147.5){\makebox(0,0)[cc]{\DOTT}}

\put(142.5,93.75){\makebox(0,0)[cl]{$\Ree$}}

\linethickness{0.35mm}
\put(152.5,30){\line(1,0){7.5}}
\linethickness{0.35mm}
\put(120,160){\line(1,0){7.5}}
\linethickness{0.35mm}
\put(140,62.5){\line(0,1){65}}
\linethickness{0.35mm}
\put(120,127.5){\line(1,0){40}}
\linethickness{0.35mm}
\put(120,62.5){\line(1,0){40}}
\linethickness{0.75mm}
\put(80,105){\line(0,1){20}}
\linethickness{0.75mm}
\put(70,95){\line(0,1){20}}
\linethickness{0.75mm}
\multiput(70,115)(0.12,-0.12){167}{\line(1,0){0.12}}
\linethickness{0.75mm}
\put(90,75){\line(0,1){20}}
\linethickness{0.75mm}
\multiput(70,95)(0.12,-0.12){167}{\line(1,0){0.12}}
\linethickness{0.75mm}
\put(80,65){\line(0,1){20}}
\linethickness{1.2mm}
\put(80,140){\line(0,1){35}}
\linethickness{0.75mm}
\put(65,125){\line(1,0){30}}
\linethickness{0.75mm}
\put(65,125){\line(0,1){30}}
\linethickness{0.75mm}
\multiput(65,155)(0.12,-0.12){250}{\line(1,0){0.12}}
\put(80,140){\makebox(0,0)[cc]{\DOTT}}

\put(75,132.5){\makebox(0,0)[cc]{$\encobool$}}

\linethickness{1.2mm}
\put(80,15){\line(0,1){35}}
\linethickness{0.75mm}
\put(65,65){\line(1,0){30}}
\linethickness{0.75mm}
\put(95,35){\line(0,1){30}}
\linethickness{0.75mm}
\multiput(65,65)(0.12,-0.12){250}{\line(1,0){0.12}}
\linethickness{0.35mm}
\put(92.5,30){\line(1,0){7.5}}
\put(83.75,56.25){\makebox(0,0)[cc]{$\booleval$}}

\linethickness{0.35mm}
\put(60,62.5){\line(0,1){97.5}}
\linethickness{0.35mm}
\multiput(67.5,160)(0.12,-0.12){271}{\line(1,0){0.12}}
\linethickness{0.35mm}
\put(60,160){\line(1,0){7.5}}
\linethickness{0.35mm}
\put(100,30){\line(0,1){97.5}}
\linethickness{0.35mm}
\multiput(60,62.5)(0.12,-0.12){271}{\line(1,0){0.12}}
\put(112.5,90){\makebox(0,0)[cc]{\EQLS}}

\linethickness{0.35mm}
\multiput(210,62.5)(0.12,-0.12){271}{\line(1,0){0.12}}
\linethickness{0.35mm}
\put(210,127.5){\line(0,1){32.5}}
\linethickness{1.2mm}
\put(230,147.5){\line(0,1){22.5}}
\linethickness{1.2mm}
\put(230,20){\line(0,1){22.5}}
\linethickness{0.35mm}
\multiput(217.5,160)(0.12,-0.12){271}{\line(1,0){0.12}}
\linethickness{0.35mm}
\put(250,30){\line(0,1){32.5}}
\put(230,147.5){\makebox(0,0)[cc]{\DOTT}}

\put(232.5,93.75){\makebox(0,0)[cl]{$\Ree$}}

\linethickness{0.35mm}
\put(242.5,30){\line(1,0){7.5}}
\linethickness{0.35mm}
\put(210,160){\line(1,0){7.5}}
\linethickness{0.35mm}
\put(230,62.5){\line(0,1){65}}
\linethickness{0.35mm}
\put(210,127.5){\line(1,0){40}}
\linethickness{0.35mm}
\put(210,62.5){\line(1,0){40}}
\end{picture}


==> PIC/idem.tex <==
%%Created by jPicEdt 1.4.1_03: mixed JPIC-XML/LaTeX format
%%Mon May 31 22:14:38 GMT-10:00 2021
%%Begin JPIC-XML
%<?xml version="1.0" standalone="yes"?>
%<jpic x-min="5" x-max="356.25" y-min="0" y-max="100" auto-bounding="true">
%<multicurve fill-style= "none"
%	 points= "(5,90);(5,90);(25,70);(25,70)"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(220,30);(220,30);(220,70);(220,70)"
%	 stroke-width= "0.2"
%	 />
%<multicurve fill-style= "none"
%	 points= "(15,60);(15,60);(15,40);(15,40)"
%	 stroke-width= "1"
%	 />
%<multicurve fill-style= "none"
%	 points= "(5,70);(5,70);(25,50);(25,50)"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(15,20);(15,20);(15,0);(15,0)"
%	 stroke-width= "1"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(40,50)"
%	 text-frame= "noframe"
%	 stroke-width= "0.35"
%	 text-hor-align= "center-h"
%	 >
%\EQLS
%</text>
%<multicurve fill-style= "none"
%	 points= "(5,90);(5,90);(5,70);(5,70)"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(25,70);(25,70);(25,50);(25,50)"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(15,100);(15,100);(15,80);(15,80)"
%	 stroke-width= "1"
%	 />
%<multicurve fill-style= "none"
%	 points= "(65,40);(65,40);(65,0);(65,0)"
%	 stroke-width= "1"
%	 />
%<multicurve fill-style= "none"
%	 points= "(65,100);(65,100);(65,60);(65,60)"
%	 stroke-width= "1"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(120,50)"
%	 text-frame= "noframe"
%	 stroke-width= "0.35"
%	 text-hor-align= "center-h"
%	 >
%\thenword
%</text>
%<multicurve fill-style= "none"
%	 points= "(175,40);(175,40);(175,0);(175,0)"
%	 stroke-width= "1"
%	 />
%<multicurve fill-style= "none"
%	 points= "(175,100);(175,100);(175,60);(175,60)"
%	 stroke-width= "1"
%	 />
%<multicurve fill-style= "none"
%	 points= "(220,20);(220,20);(220,0);(220,0)"
%	 stroke-width= "1"
%	 />
%<multicurve fill-style= "none"
%	 points= "(220,100);(220,100);(220,80);(220,80)"
%	 stroke-width= "1"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(200,50)"
%	 text-frame= "noframe"
%	 stroke-width= "0.35"
%	 text-hor-align= "center-h"
%	 >
%\EQLS
%</text>
%<multicurve fill-style= "none"
%	 points= "(355,0);(355,0);(355,100);(355,100)"
%	 stroke-width= "0.2"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(340,50)"
%	 text-frame= "noframe"
%	 stroke-width= "0.35"
%	 text-hor-align= "center-h"
%	 >
%\EQLS
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(270,50)"
%	 text-frame= "noframe"
%	 stroke-width= "0.35"
%	 text-hor-align= "center-h"
%	 >
%\withword
%</text>
%<multicurve fill-style= "none"
%	 points= "(320,80);(320,80);(320,100);(320,100)"
%	 stroke-width= "0.2"
%	 />
%<multicurve fill-style= "none"
%	 points= "(320,70);(320,70);(320,30);(320,30)"
%	 stroke-width= "1"
%	 />
%<multicurve fill-style= "none"
%	 points= "(320,0);(320,0);(320,20);(320,20)"
%	 stroke-width= "0.2"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(15,70)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\pee$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(15,30)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\pee$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(65,50)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\pee$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(175,50)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\pee$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(217.5,75)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\iee$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(222.5,25)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\qee$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(322.5,75)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\qee$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(317.5,25)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\iee$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(12.5,0)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\Aee$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(62.5,0)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\Aee$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(17.5,46.25)"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\Aee$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(17.5,100)"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\Aee$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(67.5,100)"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\Aee$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(177.5,100)"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\Aee$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(172.5,0)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\Aee$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(217.5,0)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\Aee$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(222.5,100)"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\Aee$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(317.5,50)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\Aee$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(352.5,0)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\Ree$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(317.5,0)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\Ree$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(356.25,100)"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\Ree$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(321.25,100)"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\Ree$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(222.5,50)"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\Ree$
%</text>
%<multicurve fill-style= "none"
%	 points= "(5,50);(5,50);(25,30);(25,30)"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(5,30);(5,30);(25,10);(25,10)"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(5,50);(5,50);(5,30);(5,30)"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(25,30);(25,30);(25,10);(25,10)"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(55,70);(55,70);(75,50);(75,50)"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(55,50);(55,50);(75,30);(75,30)"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(55,70);(55,70);(55,50);(55,50)"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(75,50);(75,50);(75,30);(75,30)"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(165,70);(165,70);(185,50);(185,50)"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(165,50);(165,50);(185,30);(185,30)"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(165,70);(165,70);(165,50);(165,50)"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(185,50);(185,50);(185,30);(185,30)"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(210,90);(210,90);(230,70);(230,70)"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(210,70);(210,70);(230,70);(230,70)"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(210,90);(210,90);(210,70);(210,70)"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(210,30);(210,30);(230,30);(230,30)"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(210,30);(210,30);(230,10);(230,10)"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(230,30);(230,30);(230,10);(230,10)"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(310,40);(310,40);(330,20);(330,20)"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(310,20);(310,20);(330,20);(330,20)"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(310,40);(310,40);(310,20);(310,20)"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(310,80);(310,80);(330,80);(330,80)"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(310,80);(310,80);(330,60);(330,60)"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(330,80);(330,80);(330,60);(330,60)"
%	 stroke-width= "0.35"
%	 />
%<ellipse p3= "(222.58,77.42)"
%	 fill-style= "solid"
%	 p2= "(222.58,82.58)"
%	 fill-color= "#330033"
%	 p1= "(217.42,82.58)"
%	 closure= "open"
%	 angle-end= "0"
%	 angle-start= "0"
%	 />
%<ellipse p3= "(322.58,27.42)"
%	 fill-style= "solid"
%	 p2= "(322.58,32.58)"
%	 fill-color= "#330033"
%	 p1= "(317.42,32.58)"
%	 closure= "open"
%	 angle-end= "0"
%	 angle-start= "0"
%	 />
%</jpic>
%%End JPIC-XML
%PSTricks content-type (pstricks.sty package needed)
%Add \usepackage{pstricks} in the preamble of your LaTeX file
%You can rescale the whole picture (to 80% for instance) by using the command \def\JPicScale{0.8}
\ifx\JPicScale\undefined\def\JPicScale{1}\fi
\psset{unit=\JPicScale mm}
\psset{linewidth=0.3,dotsep=1,hatchwidth=0.3,hatchsep=1.5,shadowsize=1,dimen=middle}
\psset{dotsize=0.7 2.5,dotscale=1 1,fillcolor=black}
\psset{arrowsize=1 2,arrowlength=1,arrowinset=0.25,tbarsize=0.7 5,bracketlength=0.15,rbracketlength=0.15}
\begin{pspicture}(0,0)(356.25,100)
\psline[linewidth=0.35](5,90)(25,70)
\psline[linewidth=0.2](220,30)(220,70)
\psline[linewidth=1](15,60)(15,40)
\psline[linewidth=0.35](5,70)(25,50)
\psline[linewidth=1](15,20)(15,0)
\rput(40,50){\EQLS}
\psline[linewidth=0.35](5,90)(5,70)
\psline[linewidth=0.35](25,70)(25,50)
\psline[linewidth=1](15,100)(15,80)
\psline[linewidth=1](65,40)(65,0)
\psline[linewidth=1](65,100)(65,60)
\rput(120,50){\thenword}
\psline[linewidth=1](175,40)(175,0)
\psline[linewidth=1](175,100)(175,60)
\psline[linewidth=1](220,20)(220,0)
\psline[linewidth=1](220,100)(220,80)
\rput(200,50){\EQLS}
\psline[linewidth=0.2](355,0)(355,100)
\rput(340,50){\EQLS}
\rput(270,50){\withword}
\psline[linewidth=0.2](320,80)(320,100)
\psline[linewidth=1](320,70)(320,30)
\psline[linewidth=0.2](320,0)(320,20)
\rput(15,70){$\pee$}
\rput(15,30){$\pee$}
\rput(65,50){$\pee$}
\rput(175,50){$\pee$}
\rput(217.5,75){$\iee$}
\rput(222.5,25){$\qee$}
\rput(322.5,75){$\qee$}
\rput(317.5,25){$\iee$}
\rput[r](12.5,0){$\Aee$}
\rput[r](62.5,0){$\Aee$}
\rput[l](17.5,46.25){$\Aee$}
\rput[l](17.5,100){$\Aee$}
\rput[l](67.5,100){$\Aee$}
\rput[l](177.5,100){$\Aee$}
\rput[r](172.5,0){$\Aee$}
\rput[r](217.5,0){$\Aee$}
\rput[l](222.5,100){$\Aee$}
\rput[r](317.5,50){$\Aee$}
\rput[r](352.5,0){$\Ree$}
\rput[r](317.5,0){$\Ree$}
\rput[l](356.25,100){$\Ree$}
\rput[l](321.25,100){$\Ree$}
\rput[l](222.5,50){$\Ree$}
\psline[linewidth=0.35](5,50)(25,30)
\psline[linewidth=0.35](5,30)(25,10)
\psline[linewidth=0.35](5,50)(5,30)
\psline[linewidth=0.35](25,30)(25,10)
\psline[linewidth=0.35](55,70)(75,50)
\psline[linewidth=0.35](55,50)(75,30)
\psline[linewidth=0.35](55,70)(55,50)
\psline[linewidth=0.35](75,50)(75,30)
\psline[linewidth=0.35](165,70)(185,50)
\psline[linewidth=0.35](165,50)(185,30)
\psline[linewidth=0.35](165,70)(165,50)
\psline[linewidth=0.35](185,50)(185,30)
\psline[linewidth=0.35](210,90)(230,70)
\psline[linewidth=0.35](210,70)(230,70)
\psline[linewidth=0.35](210,90)(210,70)
\psline[linewidth=0.35](210,30)(230,30)
\psline[linewidth=0.35](210,30)(230,10)
\psline[linewidth=0.35](230,30)(230,10)
\psline[linewidth=0.35](310,40)(330,20)
\psline[linewidth=0.35](310,20)(330,20)
\psline[linewidth=0.35](310,40)(310,20)
\psline[linewidth=0.35](310,80)(330,80)
\psline[linewidth=0.35](310,80)(330,60)
\psline[linewidth=0.35](330,80)(330,60)
\newrgbcolor{userFillColour}{0.2 0 0.2}
\rput{0}(220,80){\psellipse[fillcolor=userFillColour,fillstyle=solid](0,0)(2.58,-2.58)}
\newrgbcolor{userFillColour}{0.2 0 0.2}
\rput{0}(320,30){\psellipse[fillcolor=userFillColour,fillstyle=solid](0,0)(2.58,-2.58)}
\end{pspicture}


==> PIC/imFunDom.tex <==
%%Created by jPicEdt 1.4.1_03: mixed JPIC-XML/LaTeX format
%%Tue Dec 15 23:31:39 GMT-10:00 2020
%%Begin JPIC-XML
%<?xml version="1.0" standalone="yes"?>
%<jpic x-min="0" x-max="320" y-min="0" y-max="165" auto-bounding="true">
%<multicurve fill-style= "none"
%	 points= "(30,70);(30,70);(30,90);(30,90)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(10,70);(10,70);(30,70);(30,70)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(20,70);(20,70);(20,0);(20,0)"
%	 />
%<ellipse p3= "(22.58,47.42)"
%	 fill-style= "solid"
%	 p2= "(22.58,52.58)"
%	 fill-color= "#330033"
%	 p1= "(17.42,52.58)"
%	 closure= "open"
%	 angle-end= "0"
%	 angle-start= "0"
%	 />
%<multicurve fill-style= "none"
%	 points= "(20,110);(20,110);(5,95);(5,95)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(5,65);(5,65);(20,50);(20,50)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(5,95);(5,95);(5,65);(5,65)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(10,90);(10,90);(10,70);(10,70)"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(50,80)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\EQLS
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(20,80)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\universal$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(23.75,95)"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\Atype$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(17.5,0)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\Progtype$
%</text>
%<multicurve fill-style= "none"
%	 points= "(10,90);(10,90);(30,90);(30,90)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(20,100);(20,100);(20,90);(20,90)"
%	 />
%<ellipse p3= "(22.58,97.42)"
%	 fill-style= "solid"
%	 p2= "(22.58,102.58)"
%	 fill-color= "#330033"
%	 p1= "(17.42,102.58)"
%	 closure= "open"
%	 angle-end= "0"
%	 angle-start= "0"
%	 />
%<multicurve fill-style= "none"
%	 points= "(20,165);(20,165);(20,110);(20,110)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(95,30);(95,30);(95,50);(95,50)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(75,30);(75,30);(95,30);(95,30)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(85,30);(85,30);(85,0);(85,0)"
%	 />
%<ellipse p3= "(87.58,7.42)"
%	 fill-style= "solid"
%	 p2= "(87.58,12.58)"
%	 fill-color= "#330033"
%	 p1= "(82.42,12.58)"
%	 closure= "open"
%	 angle-end= "0"
%	 angle-start= "0"
%	 />
%<multicurve fill-style= "none"
%	 points= "(85,70);(85,70);(70,55);(70,55)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(70,25);(70,25);(85,10);(85,10)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(70,55);(70,55);(70,25);(70,25)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(75,50);(75,50);(75,30);(75,30)"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(85,40)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\universal$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(88.75,55)"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\Atype$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(82.5,0)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\Progtype$
%</text>
%<multicurve fill-style= "none"
%	 points= "(75,50);(75,50);(95,50);(95,50)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(85,60);(85,60);(85,50);(85,50)"
%	 />
%<ellipse p3= "(87.58,57.42)"
%	 fill-style= "solid"
%	 p2= "(87.58,62.58)"
%	 fill-color= "#330033"
%	 p1= "(82.42,62.58)"
%	 closure= "open"
%	 angle-end= "0"
%	 angle-start= "0"
%	 />
%<multicurve fill-style= "none"
%	 points= "(95,110);(95,110);(95,130);(95,130)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(75,110);(75,110);(95,110);(95,110)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(85,110);(85,110);(85,70);(85,70)"
%	 />
%<ellipse p3= "(87.58,87.42)"
%	 fill-style= "solid"
%	 p2= "(87.58,92.58)"
%	 fill-color= "#330033"
%	 p1= "(82.42,92.58)"
%	 closure= "open"
%	 angle-end= "0"
%	 angle-start= "0"
%	 />
%<multicurve fill-style= "none"
%	 points= "(85,150);(85,150);(70,135);(70,135)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(70,105);(70,105);(85,90);(85,90)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(70,135);(70,135);(70,105);(70,105)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(75,130);(75,130);(75,110);(75,110)"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(85,120)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\universal$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(88.75,135)"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\Atype$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(87.5,80)"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\Progtype$
%</text>
%<multicurve fill-style= "none"
%	 points= "(75,130);(75,130);(95,130);(95,130)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(85,140);(85,140);(85,130);(85,130)"
%	 />
%<ellipse p3= "(87.58,137.42)"
%	 fill-style= "solid"
%	 p2= "(87.58,142.58)"
%	 fill-color= "#330033"
%	 p1= "(82.42,142.58)"
%	 closure= "open"
%	 angle-end= "0"
%	 angle-start= "0"
%	 />
%<multicurve fill-style= "none"
%	 points= "(85,165);(85,165);(85,150);(85,150)"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(87.5,165)"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\Progtype$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(22.5,165)"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\Progtype$
%</text>
%<multicurve fill-style= "none"
%	 points= "(0,115);(0,115);(35,115);(35,115)"
%	 stroke-width= "0.1"
%	 />
%<multicurve fill-style= "none"
%	 points= "(35,115);(35,115);(35,45);(35,45)"
%	 stroke-width= "0.1"
%	 />
%<multicurve fill-style= "none"
%	 points= "(0,115);(0,115);(0,45);(0,45)"
%	 stroke-width= "0.1"
%	 />
%<multicurve fill-style= "none"
%	 points= "(0,45);(0,45);(35,45);(35,45)"
%	 stroke-width= "0.1"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(27.5,60)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\nameiota$
%</text>
%<multicurve fill-style= "none"
%	 points= "(65,155);(65,155);(100,155);(100,155)"
%	 stroke-width= "0.1"
%	 />
%<multicurve fill-style= "none"
%	 points= "(100,155);(100,155);(100,85);(100,85)"
%	 stroke-width= "0.1"
%	 />
%<multicurve fill-style= "none"
%	 points= "(65,155);(65,155);(65,85);(65,85)"
%	 stroke-width= "0.1"
%	 />
%<multicurve fill-style= "none"
%	 points= "(65,85);(65,85);(100,85);(100,85)"
%	 stroke-width= "0.1"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(92.5,100)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\nameiota$
%</text>
%<multicurve fill-style= "none"
%	 points= "(65,75);(65,75);(100,75);(100,75)"
%	 stroke-width= "0.1"
%	 />
%<multicurve fill-style= "none"
%	 points= "(100,75);(100,75);(100,5);(100,5)"
%	 stroke-width= "0.1"
%	 />
%<multicurve fill-style= "none"
%	 points= "(65,75);(65,75);(65,5);(65,5)"
%	 stroke-width= "0.1"
%	 />
%<multicurve fill-style= "none"
%	 points= "(65,5);(65,5);(100,5);(100,5)"
%	 stroke-width= "0.1"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(92.5,20)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\nameiota$
%</text>
%<multicurve fill-style= "none"
%	 points= "(250,70);(250,70);(250,90);(250,90)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(230,70);(230,70);(250,70);(250,70)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(240,50);(240,50);(240,0);(240,0)"
%	 />
%<ellipse p3= "(242.58,107.42)"
%	 fill-style= "solid"
%	 p2= "(242.58,112.58)"
%	 fill-color= "#330033"
%	 p1= "(237.42,112.58)"
%	 closure= "open"
%	 angle-end= "0"
%	 angle-start= "0"
%	 />
%<multicurve fill-style= "none"
%	 points= "(240,110);(240,110);(225,95);(225,95)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(225,65);(225,65);(240,50);(240,50)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(225,95);(225,95);(225,65);(225,65)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(230,90);(230,90);(230,70);(230,70)"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(270,80)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\EQLS
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(240,80)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\universal$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(237.5,0)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\Atype$
%</text>
%<multicurve fill-style= "none"
%	 points= "(230,90);(230,90);(250,90);(250,90)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(240,70);(240,70);(240,60);(240,60)"
%	 />
%<ellipse p3= "(242.58,57.42)"
%	 fill-style= "solid"
%	 p2= "(242.58,62.58)"
%	 fill-color= "#330033"
%	 p1= "(237.42,62.58)"
%	 closure= "open"
%	 angle-end= "0"
%	 angle-start= "0"
%	 />
%<multicurve fill-style= "none"
%	 points= "(240,165);(240,165);(240,90);(240,90)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(315,30);(315,30);(315,50);(315,50)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(295,30);(295,30);(315,30);(315,30)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(305,10);(305,10);(305,0);(305,0)"
%	 />
%<ellipse p3= "(307.58,17.42)"
%	 fill-style= "solid"
%	 p2= "(307.58,22.58)"
%	 fill-color= "#330033"
%	 p1= "(302.42,22.58)"
%	 closure= "open"
%	 angle-end= "0"
%	 angle-start= "0"
%	 />
%<multicurve fill-style= "none"
%	 points= "(305,70);(305,70);(290,55);(290,55)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(290,25);(290,25);(305,10);(305,10)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(290,55);(290,55);(290,25);(290,25)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(295,50);(295,50);(295,30);(295,30)"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(305,40)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\universal$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(302.5,55)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\Atype$
%</text>
%<multicurve fill-style= "none"
%	 points= "(295,50);(295,50);(315,50);(315,50)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(305,30);(305,30);(305,20);(305,20)"
%	 />
%<ellipse p3= "(307.58,67.42)"
%	 fill-style= "solid"
%	 p2= "(307.58,72.58)"
%	 fill-color= "#330033"
%	 p1= "(302.42,72.58)"
%	 closure= "open"
%	 angle-end= "0"
%	 angle-start= "0"
%	 />
%<multicurve fill-style= "none"
%	 points= "(315,110);(315,110);(315,130);(315,130)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(295,110);(295,110);(315,110);(315,110)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(305,90);(305,90);(305,50);(305,50)"
%	 />
%<ellipse p3= "(307.58,97.42)"
%	 fill-style= "solid"
%	 p2= "(307.58,102.58)"
%	 fill-color= "#330033"
%	 p1= "(302.42,102.58)"
%	 closure= "open"
%	 angle-end= "0"
%	 angle-start= "0"
%	 />
%<multicurve fill-style= "none"
%	 points= "(305,150);(305,150);(290,135);(290,135)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(290,105);(290,105);(305,90);(305,90)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(290,135);(290,135);(290,105);(290,105)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(295,130);(295,130);(295,110);(295,110)"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(305,120)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\universal$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(302.5,0)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\Atype$
%</text>
%<multicurve fill-style= "none"
%	 points= "(295,130);(295,130);(315,130);(315,130)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(305,110);(305,110);(305,100);(305,100)"
%	 />
%<ellipse p3= "(307.58,147.42)"
%	 fill-style= "solid"
%	 p2= "(307.58,152.58)"
%	 fill-color= "#330033"
%	 p1= "(302.42,152.58)"
%	 closure= "open"
%	 angle-end= "0"
%	 angle-start= "0"
%	 />
%<multicurve fill-style= "none"
%	 points= "(305,165);(305,165);(305,130);(305,130)"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(302.5,105)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\Progtype$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(237.5,65)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\Progtype$
%</text>
%<multicurve fill-style= "none"
%	 points= "(220,115);(220,115);(255,115);(255,115)"
%	 stroke-width= "0.1"
%	 />
%<multicurve fill-style= "none"
%	 points= "(255,115);(255,115);(255,45);(255,45)"
%	 stroke-width= "0.1"
%	 />
%<multicurve fill-style= "none"
%	 points= "(220,115);(220,115);(220,45);(220,45)"
%	 stroke-width= "0.1"
%	 />
%<multicurve fill-style= "none"
%	 points= "(220,45);(220,45);(255,45);(255,45)"
%	 stroke-width= "0.1"
%	 />
%<multicurve fill-style= "none"
%	 points= "(285,155);(285,155);(320,155);(320,155)"
%	 stroke-width= "0.1"
%	 />
%<multicurve fill-style= "none"
%	 points= "(320,155);(320,155);(320,85);(320,85)"
%	 stroke-width= "0.1"
%	 />
%<multicurve fill-style= "none"
%	 points= "(285,155);(285,155);(285,85);(285,85)"
%	 stroke-width= "0.1"
%	 />
%<multicurve fill-style= "none"
%	 points= "(285,85);(285,85);(320,85);(320,85)"
%	 stroke-width= "0.1"
%	 />
%<multicurve fill-style= "none"
%	 points= "(285,75);(285,75);(320,75);(320,75)"
%	 stroke-width= "0.1"
%	 />
%<multicurve fill-style= "none"
%	 points= "(320,75);(320,75);(320,5);(320,5)"
%	 stroke-width= "0.1"
%	 />
%<multicurve fill-style= "none"
%	 points= "(285,75);(285,75);(285,5);(285,5)"
%	 stroke-width= "0.1"
%	 />
%<multicurve fill-style= "none"
%	 points= "(285,5);(285,5);(320,5);(320,5)"
%	 stroke-width= "0.1"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(247.5,100)"
%	 text-frame= "noframe"
%	 stroke-width= "0.2"
%	 text-hor-align= "center-h"
%	 >
%$\nametau$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(312.5,60)"
%	 text-frame= "noframe"
%	 stroke-width= "0.2"
%	 text-hor-align= "center-h"
%	 >
%$\nametau$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(312.5,140)"
%	 text-frame= "noframe"
%	 stroke-width= "0.2"
%	 text-hor-align= "center-h"
%	 >
%$\nametau$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(302.5,25)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\Progtype$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(242.5,165)"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\Atype$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(307.5,165)"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\Atype$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(302.5,135)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\Atype$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(237.5,95)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\Atype$
%</text>
%</jpic>
%%End JPIC-XML
%PSTricks content-type (pstricks.sty package needed)
%Add \usepackage{pstricks} in the preamble of your LaTeX file
%You can rescale the whole picture (to 80% for instance) by using the command \def\JPicScale{0.8}
\ifx\JPicScale\undefined\def\JPicScale{1}\fi
\psset{unit=\JPicScale mm}
\psset{linewidth=0.3,dotsep=1,hatchwidth=0.3,hatchsep=1.5,shadowsize=1,dimen=middle}
\psset{dotsize=0.7 2.5,dotscale=1 1,fillcolor=black}
\psset{arrowsize=1 2,arrowlength=1,arrowinset=0.25,tbarsize=0.7 5,bracketlength=0.15,rbracketlength=0.15}
\begin{pspicture}(0,0)(320,165)
\psline(30,70)(30,90)
\psline(10,70)(30,70)
\psline(20,70)(20,0)
\newrgbcolor{userFillColour}{0.2 0 0.2}
\rput{0}(20,50){\psellipse[fillcolor=userFillColour,fillstyle=solid](0,0)(2.58,-2.58)}
\psline(20,110)(5,95)
\psline(5,65)(20,50)
\psline(5,95)(5,65)
\psline(10,90)(10,70)
\rput(50,80){\EQLS}
\rput(20,80){$\universal$}
\rput[l](23.75,95){$\Atype$}
\rput[r](17.5,0){$\Progtype$}
\psline(10,90)(30,90)
\psline(20,100)(20,90)
\newrgbcolor{userFillColour}{0.2 0 0.2}
\rput{0}(20,100){\psellipse[fillcolor=userFillColour,fillstyle=solid](0,0)(2.58,-2.58)}
\psline(20,165)(20,110)
\psline(95,30)(95,50)
\psline(75,30)(95,30)
\psline(85,30)(85,0)
\newrgbcolor{userFillColour}{0.2 0 0.2}
\rput{0}(85,10){\psellipse[fillcolor=userFillColour,fillstyle=solid](0,0)(2.58,-2.58)}
\psline(85,70)(70,55)
\psline(70,25)(85,10)
\psline(70,55)(70,25)
\psline(75,50)(75,30)
\rput(85,40){$\universal$}
\rput[l](88.75,55){$\Atype$}
\rput[r](82.5,0){$\Progtype$}
\psline(75,50)(95,50)
\psline(85,60)(85,50)
\newrgbcolor{userFillColour}{0.2 0 0.2}
\rput{0}(85,60){\psellipse[fillcolor=userFillColour,fillstyle=solid](0,0)(2.58,-2.58)}
\psline(95,110)(95,130)
\psline(75,110)(95,110)
\psline(85,110)(85,70)
\newrgbcolor{userFillColour}{0.2 0 0.2}
\rput{0}(85,90){\psellipse[fillcolor=userFillColour,fillstyle=solid](0,0)(2.58,-2.58)}
\psline(85,150)(70,135)
\psline(70,105)(85,90)
\psline(70,135)(70,105)
\psline(75,130)(75,110)
\rput(85,120){$\universal$}
\rput[l](88.75,135){$\Atype$}
\rput[l](87.5,80){$\Progtype$}
\psline(75,130)(95,130)
\psline(85,140)(85,130)
\newrgbcolor{userFillColour}{0.2 0 0.2}
\rput{0}(85,140){\psellipse[fillcolor=userFillColour,fillstyle=solid](0,0)(2.58,-2.58)}
\psline(85,165)(85,150)
\rput[l](87.5,165){$\Progtype$}
\rput[l](22.5,165){$\Progtype$}
\psline[linewidth=0.1](0,115)(35,115)
\psline[linewidth=0.1](35,115)(35,45)
\psline[linewidth=0.1](0,115)(0,45)
\psline[linewidth=0.1](0,45)(35,45)
\rput(27.5,60){$\nameiota$}
\psline[linewidth=0.1](65,155)(100,155)
\psline[linewidth=0.1](100,155)(100,85)
\psline[linewidth=0.1](65,155)(65,85)
\psline[linewidth=0.1](65,85)(100,85)
\rput(92.5,100){$\nameiota$}
\psline[linewidth=0.1](65,75)(100,75)
\psline[linewidth=0.1](100,75)(100,5)
\psline[linewidth=0.1](65,75)(65,5)
\psline[linewidth=0.1](65,5)(100,5)
\rput(92.5,20){$\nameiota$}
\psline(250,70)(250,90)
\psline(230,70)(250,70)
\psline(240,50)(240,0)
\newrgbcolor{userFillColour}{0.2 0 0.2}
\rput{0}(240,110){\psellipse[fillcolor=userFillColour,fillstyle=solid](0,0)(2.58,-2.58)}
\psline(240,110)(225,95)
\psline(225,65)(240,50)
\psline(225,95)(225,65)
\psline(230,90)(230,70)
\rput(270,80){\EQLS}
\rput(240,80){$\universal$}
\rput[r](237.5,0){$\Atype$}
\psline(230,90)(250,90)
\psline(240,70)(240,60)
\newrgbcolor{userFillColour}{0.2 0 0.2}
\rput{0}(240,60){\psellipse[fillcolor=userFillColour,fillstyle=solid](0,0)(2.58,-2.58)}
\psline(240,165)(240,90)
\psline(315,30)(315,50)
\psline(295,30)(315,30)
\psline(305,10)(305,0)
\newrgbcolor{userFillColour}{0.2 0 0.2}
\rput{0}(305,20){\psellipse[fillcolor=userFillColour,fillstyle=solid](0,0)(2.58,-2.58)}
\psline(305,70)(290,55)
\psline(290,25)(305,10)
\psline(290,55)(290,25)
\psline(295,50)(295,30)
\rput(305,40){$\universal$}
\rput[r](302.5,55){$\Atype$}
\psline(295,50)(315,50)
\psline(305,30)(305,20)
\newrgbcolor{userFillColour}{0.2 0 0.2}
\rput{0}(305,70){\psellipse[fillcolor=userFillColour,fillstyle=solid](0,0)(2.58,-2.58)}
\psline(315,110)(315,130)
\psline(295,110)(315,110)
\psline(305,90)(305,50)
\newrgbcolor{userFillColour}{0.2 0 0.2}
\rput{0}(305,100){\psellipse[fillcolor=userFillColour,fillstyle=solid](0,0)(2.58,-2.58)}
\psline(305,150)(290,135)
\psline(290,105)(305,90)
\psline(290,135)(290,105)
\psline(295,130)(295,110)
\rput(305,120){$\universal$}
\rput[r](302.5,0){$\Atype$}
\psline(295,130)(315,130)
\psline(305,110)(305,100)
\newrgbcolor{userFillColour}{0.2 0 0.2}
\rput{0}(305,150){\psellipse[fillcolor=userFillColour,fillstyle=solid](0,0)(2.58,-2.58)}
\psline(305,165)(305,130)
\rput[r](302.5,105){$\Progtype$}
\rput[r](237.5,65){$\Progtype$}
\psline[linewidth=0.1](220,115)(255,115)
\psline[linewidth=0.1](255,115)(255,45)
\psline[linewidth=0.1](220,115)(220,45)
\psline[linewidth=0.1](220,45)(255,45)
\psline[linewidth=0.1](285,155)(320,155)
\psline[linewidth=0.1](320,155)(320,85)
\psline[linewidth=0.1](285,155)(285,85)
\psline[linewidth=0.1](285,85)(320,85)
\psline[linewidth=0.1](285,75)(320,75)
\psline[linewidth=0.1](320,75)(320,5)
\psline[linewidth=0.1](285,75)(285,5)
\psline[linewidth=0.1](285,5)(320,5)
\rput(247.5,100){$\nametau$}
\rput(312.5,60){$\nametau$}
\rput(312.5,140){$\nametau$}
\rput[r](302.5,25){$\Progtype$}
\rput[l](242.5,165){$\Atype$}
\rput[l](307.5,165){$\Atype$}
\rput[r](302.5,135){$\Atype$}
\rput[r](237.5,95){$\Atype$}
\end{pspicture}


==> PIC/imfun.tex <==
%%Created by jPicEdt 1.4.1_03: mixed JPIC-XML/LaTeX format
%%Fri Dec 11 16:03:23 GMT-10:00 2020
%%Begin JPIC-XML
%<?xml version="1.0" standalone="yes"?>
%<jpic x-min="0" x-max="100" y-min="0" y-max="165" auto-bounding="true">
%<multicurve fill-style= "none"
%	 points= "(30,70);(30,70);(30,90);(30,90)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(10,70);(10,70);(30,70);(30,70)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(20,70);(20,70);(20,0);(20,0)"
%	 />
%<ellipse p3= "(22.58,47.42)"
%	 fill-style= "solid"
%	 p2= "(22.58,52.58)"
%	 fill-color= "#330033"
%	 p1= "(17.42,52.58)"
%	 closure= "open"
%	 angle-end= "0"
%	 angle-start= "0"
%	 />
%<multicurve fill-style= "none"
%	 points= "(20,110);(20,110);(5,95);(5,95)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(5,65);(5,65);(20,50);(20,50)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(5,95);(5,95);(5,65);(5,65)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(10,90);(10,90);(10,70);(10,70)"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(50,80)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\EQLS
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(20,80)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\universal$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(23.75,95)"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\Atype$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(17.5,0)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\Progtype$
%</text>
%<multicurve fill-style= "none"
%	 points= "(10,90);(10,90);(30,90);(30,90)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(20,100);(20,100);(20,90);(20,90)"
%	 />
%<ellipse p3= "(22.58,97.42)"
%	 fill-style= "solid"
%	 p2= "(22.58,102.58)"
%	 fill-color= "#330033"
%	 p1= "(17.42,102.58)"
%	 closure= "open"
%	 angle-end= "0"
%	 angle-start= "0"
%	 />
%<multicurve fill-style= "none"
%	 points= "(20,165);(20,165);(20,110);(20,110)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(95,30);(95,30);(95,50);(95,50)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(75,30);(75,30);(95,30);(95,30)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(85,30);(85,30);(85,0);(85,0)"
%	 />
%<ellipse p3= "(87.58,7.42)"
%	 fill-style= "solid"
%	 p2= "(87.58,12.58)"
%	 fill-color= "#330033"
%	 p1= "(82.42,12.58)"
%	 closure= "open"
%	 angle-end= "0"
%	 angle-start= "0"
%	 />
%<multicurve fill-style= "none"
%	 points= "(85,70);(85,70);(70,55);(70,55)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(70,25);(70,25);(85,10);(85,10)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(70,55);(70,55);(70,25);(70,25)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(75,50);(75,50);(75,30);(75,30)"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(85,40)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\universal$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(88.75,55)"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\Atype$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(82.5,0)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\Progtype$
%</text>
%<multicurve fill-style= "none"
%	 points= "(75,50);(75,50);(95,50);(95,50)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(85,60);(85,60);(85,50);(85,50)"
%	 />
%<ellipse p3= "(87.58,57.42)"
%	 fill-style= "solid"
%	 p2= "(87.58,62.58)"
%	 fill-color= "#330033"
%	 p1= "(82.42,62.58)"
%	 closure= "open"
%	 angle-end= "0"
%	 angle-start= "0"
%	 />
%<multicurve fill-style= "none"
%	 points= "(95,110);(95,110);(95,130);(95,130)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(75,110);(75,110);(95,110);(95,110)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(85,110);(85,110);(85,70);(85,70)"
%	 />
%<ellipse p3= "(87.58,87.42)"
%	 fill-style= "solid"
%	 p2= "(87.58,92.58)"
%	 fill-color= "#330033"
%	 p1= "(82.42,92.58)"
%	 closure= "open"
%	 angle-end= "0"
%	 angle-start= "0"
%	 />
%<multicurve fill-style= "none"
%	 points= "(85,150);(85,150);(70,135);(70,135)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(70,105);(70,105);(85,90);(85,90)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(70,135);(70,135);(70,105);(70,105)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(75,130);(75,130);(75,110);(75,110)"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(85,120)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\universal$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(88.75,135)"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\Atype$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(87.5,80)"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\Progtype$
%</text>
%<multicurve fill-style= "none"
%	 points= "(75,130);(75,130);(95,130);(95,130)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(85,140);(85,140);(85,130);(85,130)"
%	 />
%<ellipse p3= "(87.58,137.42)"
%	 fill-style= "solid"
%	 p2= "(87.58,142.58)"
%	 fill-color= "#330033"
%	 p1= "(82.42,142.58)"
%	 closure= "open"
%	 angle-end= "0"
%	 angle-start= "0"
%	 />
%<multicurve fill-style= "none"
%	 points= "(85,165);(85,165);(85,150);(85,150)"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(87.5,165)"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\Progtype$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(22.5,165)"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\Progtype$
%</text>
%<multicurve fill-style= "none"
%	 points= "(0,115);(0,115);(35,115);(35,115)"
%	 stroke-width= "0.1"
%	 />
%<multicurve fill-style= "none"
%	 points= "(35,115);(35,115);(35,45);(35,45)"
%	 stroke-width= "0.1"
%	 />
%<multicurve fill-style= "none"
%	 points= "(0,115);(0,115);(0,45);(0,45)"
%	 stroke-width= "0.1"
%	 />
%<multicurve fill-style= "none"
%	 points= "(0,45);(0,45);(35,45);(35,45)"
%	 stroke-width= "0.1"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(27.5,55)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\nameiota$
%</text>
%<multicurve fill-style= "none"
%	 points= "(65,155);(65,155);(100,155);(100,155)"
%	 stroke-width= "0.1"
%	 />
%<multicurve fill-style= "none"
%	 points= "(100,155);(100,155);(100,85);(100,85)"
%	 stroke-width= "0.1"
%	 />
%<multicurve fill-style= "none"
%	 points= "(65,155);(65,155);(65,85);(65,85)"
%	 stroke-width= "0.1"
%	 />
%<multicurve fill-style= "none"
%	 points= "(65,85);(65,85);(100,85);(100,85)"
%	 stroke-width= "0.1"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(92.5,95)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\nameiota$
%</text>
%<multicurve fill-style= "none"
%	 points= "(65,75);(65,75);(100,75);(100,75)"
%	 stroke-width= "0.1"
%	 />
%<multicurve fill-style= "none"
%	 points= "(100,75);(100,75);(100,5);(100,5)"
%	 stroke-width= "0.1"
%	 />
%<multicurve fill-style= "none"
%	 points= "(65,75);(65,75);(65,5);(65,5)"
%	 stroke-width= "0.1"
%	 />
%<multicurve fill-style= "none"
%	 points= "(65,5);(65,5);(100,5);(100,5)"
%	 stroke-width= "0.1"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(92.5,15)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\nameiota$
%</text>
%</jpic>
%%End JPIC-XML
%LaTeX-picture environment using emulated lines and arcs
%You can rescale the whole picture (to 80% for instance) by using the command \def\JPicScale{0.8}
\ifx\JPicScale\undefined\def\JPicScale{1}\fi
\unitlength \JPicScale mm
\begin{picture}(100,165)(0,0)
\linethickness{0.3mm}
\put(30,70){\line(0,1){20}}
\linethickness{0.3mm}
\put(10,70){\line(1,0){20}}
\linethickness{0.3mm}
\put(20,0){\line(0,1){70}}
\linethickness{0.3mm}
\put(20,50){\circle*{5.16}}

\linethickness{0.3mm}
\multiput(5,95)(0.12,0.12){125}{\line(1,0){0.12}}
\linethickness{0.3mm}
\multiput(5,65)(0.12,-0.12){125}{\line(1,0){0.12}}
\linethickness{0.3mm}
\put(5,65){\line(0,1){30}}
\linethickness{0.3mm}
\put(10,70){\line(0,1){20}}
\put(50,80){\makebox(0,0)[cc]{\EQLS}}

\put(20,80){\makebox(0,0)[cc]{$\universal$}}

\put(23.75,95){\makebox(0,0)[cl]{$\Atype$}}

\put(17.5,0){\makebox(0,0)[cr]{$\Progtype$}}

\linethickness{0.3mm}
\put(10,90){\line(1,0){20}}
\linethickness{0.3mm}
\put(20,90){\line(0,1){10}}
\linethickness{0.3mm}
\put(20,100){\circle*{5.16}}

\linethickness{0.3mm}
\put(20,110){\line(0,1){55}}
\linethickness{0.3mm}
\put(95,30){\line(0,1){20}}
\linethickness{0.3mm}
\put(75,30){\line(1,0){20}}
\linethickness{0.3mm}
\put(85,0){\line(0,1){30}}
\linethickness{0.3mm}
\put(85,10){\circle*{5.16}}

\linethickness{0.3mm}
\multiput(70,55)(0.12,0.12){125}{\line(1,0){0.12}}
\linethickness{0.3mm}
\multiput(70,25)(0.12,-0.12){125}{\line(1,0){0.12}}
\linethickness{0.3mm}
\put(70,25){\line(0,1){30}}
\linethickness{0.3mm}
\put(75,30){\line(0,1){20}}
\put(85,40){\makebox(0,0)[cc]{$\universal$}}

\put(88.75,55){\makebox(0,0)[cl]{$\Atype$}}

\put(82.5,0){\makebox(0,0)[cr]{$\Progtype$}}

\linethickness{0.3mm}
\put(75,50){\line(1,0){20}}
\linethickness{0.3mm}
\put(85,50){\line(0,1){10}}
\linethickness{0.3mm}
\put(85,60){\circle*{5.16}}

\linethickness{0.3mm}
\put(95,110){\line(0,1){20}}
\linethickness{0.3mm}
\put(75,110){\line(1,0){20}}
\linethickness{0.3mm}
\put(85,70){\line(0,1){40}}
\linethickness{0.3mm}
\put(85,90){\circle*{5.16}}

\linethickness{0.3mm}
\multiput(70,135)(0.12,0.12){125}{\line(1,0){0.12}}
\linethickness{0.3mm}
\multiput(70,105)(0.12,-0.12){125}{\line(1,0){0.12}}
\linethickness{0.3mm}
\put(70,105){\line(0,1){30}}
\linethickness{0.3mm}
\put(75,110){\line(0,1){20}}
\put(85,120){\makebox(0,0)[cc]{$\universal$}}

\put(88.75,135){\makebox(0,0)[cl]{$\Atype$}}

\put(87.5,80){\makebox(0,0)[cl]{$\Progtype$}}

\linethickness{0.3mm}
\put(75,130){\line(1,0){20}}
\linethickness{0.3mm}
\put(85,130){\line(0,1){10}}
\linethickness{0.3mm}
\put(85,140){\circle*{5.16}}

\linethickness{0.3mm}
\put(85,150){\line(0,1){15}}
\put(87.5,165){\makebox(0,0)[cl]{$\Progtype$}}

\put(22.5,165){\makebox(0,0)[cl]{$\Progtype$}}

\linethickness{0.1mm}
\put(0,115){\line(1,0){35}}
\linethickness{0.1mm}
\put(35,45){\line(0,1){70}}
\linethickness{0.1mm}
\put(0,45){\line(0,1){70}}
\linethickness{0.1mm}
\put(0,45){\line(1,0){35}}
\put(27.5,55){\makebox(0,0)[cc]{$\nameiota$}}

\linethickness{0.1mm}
\put(65,155){\line(1,0){35}}
\linethickness{0.1mm}
\put(100,85){\line(0,1){70}}
\linethickness{0.1mm}
\put(65,85){\line(0,1){70}}
\linethickness{0.1mm}
\put(65,85){\line(1,0){35}}
\put(92.5,95){\makebox(0,0)[cc]{$\nameiota$}}

\linethickness{0.1mm}
\put(65,75){\line(1,0){35}}
\linethickness{0.1mm}
\put(100,5){\line(0,1){70}}
\linethickness{0.1mm}
\put(65,5){\line(0,1){70}}
\linethickness{0.1mm}
\put(65,5){\line(1,0){35}}
\put(92.5,15){\makebox(0,0)[cc]{$\nameiota$}}

\end{picture}


==> PIC/induction-step.tex <==
%%Created by jPicEdt 1.4.1_03: mixed JPIC-XML/LaTeX format
%%Sun Sep 27 15:09:26 GMT-10:00 2020
%%Begin JPIC-XML
%<?xml version="1.0" standalone="yes"?>
%<jpic x-min="0" x-max="20" y-min="-25" y-max="25" auto-bounding="true">
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(10,10)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\ahh$
%</text>
%<multicurve fill-style= "none"
%	 points= "(10,15);(10,15);(10,25);(10,25)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(10,-5);(10,-5);(10,5);(10,5)"
%	 />
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(7.5,20)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\bhh$
%</text>
%<multicurve fill-style= "none"
%	 points= "(5,-5);(5,-5);(15,-5);(15,-5)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(5,-5);(5,-5);(5,-15);(5,-15)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(15,-5);(15,-5);(15,-15);(15,-15)"
%	 />
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(7.5,0)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\Nhh$
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(10,-10)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\zhh$
%</text>
%<multicurve fill-style= "none"
%	 points= "(5,-15);(5,-15);(15,-15);(15,-15)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(10,-25);(10,-25);(10,-15);(10,-15)"
%	 />
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(7.5,-22.5)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\Nhh$
%</text>
%<multicurve fill-style= "none"
%	 points= "(5,5);(5,5);(15,5);(15,5)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(5,15);(5,15);(15,15);(15,15)"
%	 />
%<ellipse fill-style= "none"
%	 p3= "(20,5)"
%	 p2= "(20,15)"
%	 p1= "(10,15)"
%	 closure= "open"
%	 angle-end= "90"
%	 angle-start= "-90"
%	 />
%<ellipse fill-style= "none"
%	 p3= "(0,5)"
%	 p2= "(0,15)"
%	 p1= "(10,15)"
%	 closure= "open"
%	 angle-end= "90"
%	 angle-start= "-90"
%	 />
%</jpic>
%%End JPIC-XML
%PSTricks content-type (pstricks.sty package needed)
%Add \usepackage{pstricks} in the preamble of your LaTeX file
%You can rescale the whole picture (to 80% for instance) by using the command \def\JPicScale{0.8}
\ifx\JPicScale\undefined\def\JPicScale{1}\fi
\psset{unit=\JPicScale mm}
\psset{linewidth=0.3,dotsep=1,hatchwidth=0.3,hatchsep=1.5,shadowsize=1,dimen=middle}
\psset{dotsize=0.7 2.5,dotscale=1 1,fillcolor=black}
\psset{arrowsize=1 2,arrowlength=1,arrowinset=0.25,tbarsize=0.7 5,bracketlength=0.15,rbracketlength=0.15}
\begin{pspicture}(0,0)(20,25)
\rput(10,10){$\ahh$}
\psline(10,15)(10,25)
\psline(10,-5)(10,5)
\rput[r](7.5,20){$\bhh$}
\psline(5,-5)(15,-5)
\psline(5,-5)(5,-15)
\psline(15,-5)(15,-15)
\rput[r](7.5,0){$\Nhh$}
\rput(10,-10){$\zhh$}
\psline(5,-15)(15,-15)
\psline(10,-25)(10,-15)
\rput[r](7.5,-22.5){$\Nhh$}
\psline(5,5)(15,5)
\psline(5,15)(15,15)
\rput{0}(15,10){\psellipticarc[](0,0)(5,-5){-90}{90}}
\rput{0}(5,10){\psellipticarc[](0,0)(5,5){90}{270}}
\end{pspicture}


==> PIC/intersection.tex <==
%%Created by jPicEdt 1.4.1_03: mixed JPIC-XML/LaTeX format
%%Mon Jun 07 15:28:51 GMT-10:00 2021
%%Begin JPIC-XML
%<?xml version="1.0" standalone="yes"?>
%<jpic x-min="0" x-max="70" y-min="0" y-max="60" auto-bounding="true">
%<multicurve fill-style= "none"
%	 points= "(10,0);(10,0);(10,25);(10,25)"
%	 stroke-color= "#ff0033"
%	 />
%<multicurve fill-style= "none"
%	 points= "(10,35);(10,35);(10,60);(10,60)"
%	 stroke-color= "#ff0033"
%	 />
%<multicurve fill-style= "none"
%	 points= "(20,25);(20,25);(20,35);(20,35)"
%	 stroke-color= "#ff0033"
%	 />
%<multicurve fill-style= "none"
%	 points= "(0,25);(0,25);(0,35);(0,35)"
%	 stroke-color= "#ff0033"
%	 />
%<multicurve fill-style= "none"
%	 points= "(0,35);(0,35);(20,35);(20,35)"
%	 stroke-color= "#ff0033"
%	 />
%<multicurve fill-style= "none"
%	 points= "(0,25);(0,25);(20,25);(20,25)"
%	 stroke-color= "#ff0033"
%	 />
%<multicurve fill-style= "none"
%	 points= "(45,20);(45,20);(45,25);(45,25)"
%	 stroke-color= "#ff0033"
%	 />
%<multicurve fill-style= "none"
%	 points= "(45,35);(45,35);(45,40);(45,40)"
%	 stroke-color= "#ff0033"
%	 />
%<multicurve fill-style= "none"
%	 points= "(50,25);(50,25);(50,35);(50,35)"
%	 stroke-color= "#ff0033"
%	 />
%<multicurve fill-style= "none"
%	 points= "(40,25);(40,25);(40,35);(40,35)"
%	 stroke-color= "#ff0033"
%	 />
%<multicurve fill-style= "none"
%	 points= "(40,35);(40,35);(50,35);(50,35)"
%	 stroke-color= "#ff0033"
%	 />
%<multicurve fill-style= "none"
%	 points= "(40,25);(40,25);(50,25);(50,25)"
%	 stroke-color= "#ff0033"
%	 />
%<multicurve fill-style= "none"
%	 points= "(65,20);(65,20);(65,25);(65,25)"
%	 stroke-color= "#ff0033"
%	 />
%<multicurve fill-style= "none"
%	 points= "(65,35);(65,35);(65,40);(65,40)"
%	 stroke-color= "#ff0033"
%	 />
%<multicurve fill-style= "none"
%	 points= "(70,25);(70,25);(70,35);(70,35)"
%	 stroke-color= "#ff0033"
%	 />
%<multicurve fill-style= "none"
%	 points= "(60,25);(60,25);(60,35);(60,35)"
%	 stroke-color= "#ff0033"
%	 />
%<multicurve fill-style= "none"
%	 points= "(60,35);(60,35);(70,35);(70,35)"
%	 stroke-color= "#ff0033"
%	 />
%<multicurve fill-style= "none"
%	 points= "(60,25);(60,25);(70,25);(70,25)"
%	 stroke-color= "#ff0033"
%	 />
%<multicurve fill-style= "none"
%	 points= "(45,40);(45,40);(55,50);(55,50)"
%	 stroke-color= "#ff0033"
%	 />
%<multicurve fill-style= "none"
%	 points= "(55,10);(55,10);(65,20);(65,20)"
%	 stroke-color= "#ff0033"
%	 />
%<multicurve fill-style= "none"
%	 points= "(55,50);(55,50);(65,40);(65,40)"
%	 stroke-color= "#ff0033"
%	 />
%<multicurve fill-style= "none"
%	 points= "(45,20);(45,20);(55,10);(55,10)"
%	 stroke-color= "#ff0033"
%	 />
%<multicurve fill-style= "none"
%	 points= "(55,60);(55,60);(55,50);(55,50)"
%	 stroke-color= "#ff0033"
%	 />
%<multicurve fill-style= "none"
%	 points= "(55,10);(55,10);(55,0);(55,0)"
%	 stroke-color= "#ff0033"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(30,30)"
%	 stroke-color= "#ff0033"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\EQLS
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(10,30)"
%	 stroke-color= "#ff0033"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\intrsc$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(45,30)"
%	 stroke-color= "#ff0033"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\fintr$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(65,30)"
%	 stroke-color= "#ff0033"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\gintr$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(55,10)"
%	 stroke-color= "#ff0033"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\DOTT
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(55,50)"
%	 stroke-color= "#ff0033"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\DOTT
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(8.75,0)"
%	 stroke-color= "#ff0033"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\Haa$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(53.75,0)"
%	 stroke-color= "#ff0033"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\Haa$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(11.25,60)"
%	 stroke-color= "#ff0033"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\Hbb$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(56.25,60)"
%	 stroke-color= "#ff0033"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\Hbb$
%</text>
%</jpic>
%%End JPIC-XML
%LaTeX-picture environment using emulated lines and arcs
%You can rescale the whole picture (to 80% for instance) by using the command \def\JPicScale{0.8}
\ifx\JPicScale\undefined\def\JPicScale{1}\fi
\unitlength \JPicScale mm
\begin{picture}(70,60)(0,0)
\linethickness{0.3mm}
\put(10,0){\line(0,1){25}}
\linethickness{0.3mm}
\put(10,35){\line(0,1){25}}
\linethickness{0.3mm}
\put(20,25){\line(0,1){10}}
\linethickness{0.3mm}
\put(0,25){\line(0,1){10}}
\linethickness{0.3mm}
\put(0,35){\line(1,0){20}}
\linethickness{0.3mm}
\put(0,25){\line(1,0){20}}
\linethickness{0.3mm}
\put(45,20){\line(0,1){5}}
\linethickness{0.3mm}
\put(45,35){\line(0,1){5}}
\linethickness{0.3mm}
\put(50,25){\line(0,1){10}}
\linethickness{0.3mm}
\put(40,25){\line(0,1){10}}
\linethickness{0.3mm}
\put(40,35){\line(1,0){10}}
\linethickness{0.3mm}
\put(40,25){\line(1,0){10}}
\linethickness{0.3mm}
\put(65,20){\line(0,1){5}}
\linethickness{0.3mm}
\put(65,35){\line(0,1){5}}
\linethickness{0.3mm}
\put(70,25){\line(0,1){10}}
\linethickness{0.3mm}
\put(60,25){\line(0,1){10}}
\linethickness{0.3mm}
\put(60,35){\line(1,0){10}}
\linethickness{0.3mm}
\put(60,25){\line(1,0){10}}
\linethickness{0.3mm}
\multiput(45,40)(0.12,0.12){83}{\line(1,0){0.12}}
\linethickness{0.3mm}
\multiput(55,10)(0.12,0.12){83}{\line(1,0){0.12}}
\linethickness{0.3mm}
\multiput(55,50)(0.12,-0.12){83}{\line(1,0){0.12}}
\linethickness{0.3mm}
\multiput(45,20)(0.12,-0.12){83}{\line(1,0){0.12}}
\linethickness{0.3mm}
\put(55,50){\line(0,1){10}}
\linethickness{0.3mm}
\put(55,0){\line(0,1){10}}
\put(30,30){\makebox(0,0)[cc]{\EQLS}}

\put(10,30){\makebox(0,0)[cc]{$\intrsc$}}

\put(45,30){\makebox(0,0)[cc]{$\fintr$}}

\put(65,30){\makebox(0,0)[cc]{$\gintr$}}

\put(55,10){\makebox(0,0)[cc]{\DOTT}}

\put(55,50){\makebox(0,0)[cc]{\DOTT}}

\put(8.75,0){\makebox(0,0)[cr]{$\Haa$}}

\put(53.75,0){\makebox(0,0)[cr]{$\Haa$}}

\put(11.25,60){\makebox(0,0)[cl]{$\Hbb$}}

\put(56.25,60){\makebox(0,0)[cl]{$\Hbb$}}

\end{picture}


==> PIC/isome.tex <==
%%Created by jPicEdt 1.4.1_03: mixed JPIC-XML/LaTeX format
%%Mon Jan 04 19:33:39 GMT-10:00 2021
%%Begin JPIC-XML
%<?xml version="1.0" standalone="yes"?>
%<jpic x-min="0" x-max="155" y-min="0" y-max="170" auto-bounding="true">
%<multicurve fill-style= "none"
%	 points= "(0,0);(0,0);(20,0);(20,0)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(0,20);(0,20);(20,0);(20,0)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(0,20);(0,20);(0,0);(0,0)"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(6.25,5)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\fhhh$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(100,90)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\EQLS
%</text>
%<multicurve fill-style= "none"
%	 points= "(30,50);(30,50);(30,40);(30,40)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(25,40);(25,40);(55,10);(55,10)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(25,40);(25,40);(55,40);(55,40)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(55,40);(55,40);(55,10);(55,10)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(40,0);(40,0);(40,25);(40,25)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(0,100);(0,100);(20,100);(20,100)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(0,80);(0,80);(20,80);(20,80)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(20,100);(20,100);(20,80);(20,80)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(10,100);(10,100);(10,110);(10,110)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(10,70);(10,70);(10,80);(10,80)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(0,100);(0,100);(0,80);(0,80)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(50,50);(50,50);(50,40);(50,40)"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(45,30)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\khee$
%</text>
%<multicurve fill-style= "none"
%	 points= "(70,70);(70,70);(50,50);(50,50)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(25,160);(25,160);(55,160);(55,160)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(25,140);(25,140);(55,140);(55,140)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(55,160);(55,160);(55,140);(55,140)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(40,160);(40,160);(40,170);(40,170)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(25,160);(25,160);(25,140);(25,140)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(30,130);(30,130);(10,110);(10,110)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(30,140);(30,140);(30,130);(30,130)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(45,100);(45,100);(80,100);(80,100)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(60,80);(60,80);(80,80);(80,80)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(80,100);(80,100);(80,80);(80,80)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(70,100);(70,100);(70,110);(70,110)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(70,70);(70,70);(70,80);(70,80)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(45,95);(45,95);(60,80);(60,80)"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(70,90)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\predor$
%</text>
%<multicurve fill-style= "none"
%	 points= "(50,130);(50,130);(70,110);(70,110)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(50,140);(50,140);(50,130);(50,130)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(45,95);(45,95);(45,100);(45,100)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(52.5,87.5);(52.5,87.5);(10,45);(10,45)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(10,10);(10,10);(10,45);(10,45)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-overstrike-width= "1.3"
%	 points= "(10,70);(10,70);(30,50);(30,50)"
%	 stroke-overstrike= "true"
%	 />
%<multicurve fill-style= "none"
%	 points= "(120,100);(120,100);(155,100);(155,100)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(135,80);(135,80);(155,80);(155,80)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(155,100);(155,100);(155,80);(155,80)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(145,100);(145,100);(145,170);(145,170)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(145,0);(145,0);(145,80);(145,80)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(120,95);(120,95);(135,80);(135,80)"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(145,90)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\predor$
%</text>
%<multicurve fill-style= "none"
%	 points= "(120,95);(120,95);(120,100);(120,100)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(127.5,87.5);(127.5,87.5);(127.5,10);(127.5,10)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(117.5,0);(117.5,0);(137.5,0);(137.5,0)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(117.5,20);(117.5,20);(137.5,0);(137.5,0)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(117.5,20);(117.5,20);(117.5,0);(117.5,0)"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(123.75,5)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\fhhh$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(40,150)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\conjunction$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(10,90)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\negation$
%</text>
%</jpic>
%%End JPIC-XML
%PSTricks content-type (pstricks.sty package needed)
%Add \usepackage{pstricks} in the preamble of your LaTeX file
%You can rescale the whole picture (to 80% for instance) by using the command \def\JPicScale{0.8}
\ifx\JPicScale\undefined\def\JPicScale{1}\fi
\psset{unit=\JPicScale mm}
\psset{linewidth=0.3,dotsep=1,hatchwidth=0.3,hatchsep=1.5,shadowsize=1,dimen=middle}
\psset{dotsize=0.7 2.5,dotscale=1 1,fillcolor=black}
\psset{arrowsize=1 2,arrowlength=1,arrowinset=0.25,tbarsize=0.7 5,bracketlength=0.15,rbracketlength=0.15}
\begin{pspicture}(0,0)(155,170)
\psline(0,0)(20,0)
\psline(0,20)(20,0)
\psline(0,20)(0,0)
\rput(6.25,5){$\fhhh$}
\rput(100,90){\EQLS}
\psline(30,50)(30,40)
\psline(25,40)(55,10)
\psline(25,40)(55,40)
\psline(55,40)(55,10)
\psline(40,0)(40,25)
\psline(0,100)(20,100)
\psline(0,80)(20,80)
\psline(20,100)(20,80)
\psline(10,100)(10,110)
\psline(10,70)(10,80)
\psline(0,100)(0,80)
\psline(50,50)(50,40)
\rput(45,30){$\khee$}
\psline(70,70)(50,50)
\psline(25,160)(55,160)
\psline(25,140)(55,140)
\psline(55,160)(55,140)
\psline(40,160)(40,170)
\psline(25,160)(25,140)
\psline(30,130)(10,110)
\psline(30,140)(30,130)
\psline(45,100)(80,100)
\psline(60,80)(80,80)
\psline(80,100)(80,80)
\psline(70,100)(70,110)
\psline(70,70)(70,80)
\psline(45,95)(60,80)
\rput(70,90){$\predor$}
\psline(50,130)(70,110)
\psline(50,140)(50,130)
\psline(45,95)(45,100)
\psline(52.5,87.5)(10,45)
\psline(10,10)(10,45)
\psline[border=1.3](10,70)(30,50)
\psline(120,100)(155,100)
\psline(135,80)(155,80)
\psline(155,100)(155,80)
\psline(145,100)(145,170)
\psline(145,0)(145,80)
\psline(120,95)(135,80)
\rput(145,90){$\predor$}
\psline(120,95)(120,100)
\psline(127.5,87.5)(127.5,10)
\psline(117.5,0)(137.5,0)
\psline(117.5,20)(137.5,0)
\psline(117.5,20)(117.5,0)
\rput(123.75,5){$\fhhh$}
\rput(40,150){$\conjunction$}
\rput(10,90){$\negation$}
\end{pspicture}


==> PIC/kleene-1.tex <==
%%Created by jPicEdt 1.4.1_03: mixed JPIC-XML/LaTeX format
%%Tue Nov 05 18:39:18 GMT-10:00 2019
%%Begin JPIC-XML
%<?xml version="1.0" standalone="yes"?>
%<jpic x-min="13.75" x-max="173.75" y-min="-1.25" y-max="112.5" auto-bounding="true">
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(113.75,60);(113.75,60);(113.75,35);(113.75,35)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(173.75,69.37);(173.75,69.37);(173.75,94.37);(173.75,94.37)"
%	 />
%<text text-vert-align= "center-v"
%	 anchor-point= "(153.75,112.5)"
%	 stroke-width= "0.75"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\nameslang$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(165.62,-1.25)"
%	 stroke-width= "0.75"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\inputt$
%</text>
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(138.75,69.37);(138.75,69.37);(173.75,69.37);(173.75,69.37)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(165,69.37);(165,69.37);(165,3.75);(165,3.75)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(113.75,35);(113.75,35);(138.75,35);(138.75,35)"
%	 />
%<text text-vert-align= "center-v"
%	 anchor-point= "(151.87,81.25)"
%	 stroke-width= "0.75"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\universal
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(121.25,41.87)"
%	 stroke-width= "0.75"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\program
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(98.75,76.25)"
%	 stroke-width= "0.75"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\EQLS
%</text>
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(113.75,60);(113.75,60);(138.75,35);(138.75,35)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(126.25,81.88);(126.25,81.88);(126.25,48.12);(126.25,48.12)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(113.75,94.37);(113.75,94.37);(138.75,69.37);(138.75,69.37)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(83.75,69.37);(83.75,69.37);(83.75,94.37);(83.75,94.37)"
%	 />
%<text text-vert-align= "center-v"
%	 anchor-point= "(58.75,112.5)"
%	 stroke-width= "0.75"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\nameslang$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(74.38,-1.25)"
%	 stroke-width= "0.75"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\inputt$
%</text>
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(33.75,69.38);(33.75,69.38);(83.75,69.37);(83.75,69.37)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(73.75,69.37);(73.75,69.37);(73.75,3.75);(73.75,3.75)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(43.75,69.38);(43.75,69.38);(43.75,48.12);(43.75,48.12)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(33.75,94.38);(33.75,94.38);(33.75,69.38);(33.75,69.38)"
%	 />
%<text text-vert-align= "center-v"
%	 anchor-point= "(58.75,81.25)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\gee$
%</text>
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(13.75,56.24);(13.75,56.24);(35,56.24);(35,56.24)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(55,36.25);(55,36.25);(33.75,36.25);(33.75,36.25)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(35,56.24);(35,56.24);(55,36.25);(55,36.25)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(13.75,56.24);(13.75,56.24);(33.75,36.25);(33.75,36.25)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(34.38,14.38);(34.38,14.38);(34.38,3.75);(34.38,3.75)"
%	 />
%<ellipse p3= "(35.78,12.96)"
%	 p2= "(35.78,15.78)"
%	 fill-color= "#330033"
%	 p1= "(32.96,15.78)"
%	 closure= "open"
%	 fill-style= "solid"
%	 angle-end= "0"
%	 angle-start= "0"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(45,36.25);(45,36.25);(45,25);(45,25)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(24.38,45);(24.38,45);(24.38,23.76);(24.38,23.76)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(45,25);(45,25);(34.38,14.38);(34.38,14.38)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(24.38,23.76);(24.38,23.76);(34.38,13.75);(34.38,13.75)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(145,69.37);(145,69.37);(145,3.75);(145,3.75)"
%	 />
%<text text-vert-align= "center-v"
%	 anchor-point= "(145,-0.62)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\progtype$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(34.38,-1.25)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\progtype$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(35,45)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\parteval$
%</text>
%<parallelogram p3= "(56.25,106.88)"
%	 p2= "(56.25,94.38)"
%	 fill-color= "#999999"
%	 p1= "(61.25,94.38)"
%	 stroke-color= "#999999"
%	 fill-style= "solid"
%	 />
%<parallelogram p3= "(151.25,106.88)"
%	 p2= "(151.25,95)"
%	 fill-color= "#999999"
%	 p1= "(156.25,95)"
%	 stroke-color= "#999999"
%	 fill-style= "solid"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(113.75,94.37);(113.75,94.37);(173.75,94.37);(173.75,94.37)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(153.75,106.25);(153.75,106.25);(153.75,94.37);(153.75,94.37)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(33.75,94.38);(33.75,94.38);(83.75,94.37);(83.75,94.37)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(58.75,106.25);(58.75,106.25);(58.75,94.37);(58.75,94.37)"
%	 />
%</jpic>
%%End JPIC-XML
%PSTricks content-type (pstricks.sty package needed)
%Add \usepackage{pstricks} in the preamble of your LaTeX file
%You can rescale the whole picture (to 80% for instance) by using the command \def\JPicScale{0.8}
\ifx\JPicScale\undefined\def\JPicScale{1}\fi
\psset{unit=\JPicScale mm}
\psset{linewidth=0.3,dotsep=1,hatchwidth=0.3,hatchsep=1.5,shadowsize=1,dimen=middle}
\psset{dotsize=0.7 2.5,dotscale=1 1,fillcolor=black}
\psset{arrowsize=1 2,arrowlength=1,arrowinset=0.25,tbarsize=0.7 5,bracketlength=0.15,rbracketlength=0.15}
\begin{pspicture}(0,0)(173.75,112.5)
\psline[linewidth=0.75](113.75,60)(113.75,35)
\psline[linewidth=0.75](173.75,69.37)(173.75,94.37)
\rput(153.75,112.5){$\nameslang$}
\rput(165.62,-1.25){$\inputt$}
\psline[linewidth=0.75](138.75,69.37)(173.75,69.37)
\psline[linewidth=0.75](165,69.37)(165,3.75)
\psline[linewidth=0.75](113.75,35)(138.75,35)
\rput(151.87,81.25){\universal}
\rput(121.25,41.87){\program}
\rput(98.75,76.25){\EQLS}
\psline[linewidth=0.75](113.75,60)(138.75,35)
\psline[linewidth=0.75](126.25,81.88)(126.25,48.12)
\psline[linewidth=0.75](113.75,94.37)(138.75,69.37)
\psline[linewidth=0.75](83.75,69.37)(83.75,94.37)
\rput(58.75,112.5){$\nameslang$}
\rput(74.38,-1.25){$\inputt$}
\psline[linewidth=0.75](33.75,69.38)(83.75,69.37)
\psline[linewidth=0.75](73.75,69.37)(73.75,3.75)
\psline[linewidth=0.75](43.75,69.38)(43.75,48.12)
\psline[linewidth=0.75](33.75,94.38)(33.75,69.38)
\rput(58.75,81.25){$\gee$}
\psline[linewidth=0.75](13.75,56.24)(35,56.24)
\psline[linewidth=0.75](55,36.25)(33.75,36.25)
\psline[linewidth=0.75](35,56.24)(55,36.25)
\psline[linewidth=0.75](13.75,56.24)(33.75,36.25)
\psline[linewidth=0.75](34.38,14.38)(34.38,3.75)
\newrgbcolor{userFillColour}{0.2 0 0.2}
\rput{0}(34.37,14.37){\psellipse[fillcolor=userFillColour,fillstyle=solid](0,0)(1.41,-1.41)}
\psline[linewidth=0.75](45,36.25)(45,25)
\psline[linewidth=0.75](24.38,45)(24.38,23.76)
\psline[linewidth=0.75](45,25)(34.38,14.38)
\psline[linewidth=0.75](24.38,23.76)(34.38,13.75)
\psline[linewidth=0.75](145,69.37)(145,3.75)
\rput(145,-0.62){$\progtype$}
\rput(34.38,-1.25){$\progtype$}
\rput(35,45){$\parteval$}
\newrgbcolor{userLineColour}{0.6 0.6 0.6}
\newrgbcolor{userFillColour}{0.6 0.6 0.6}
\pspolygon[linecolor=userLineColour,fillcolor=userFillColour,fillstyle=solid](61.25,94.38)(56.25,94.38)(56.25,106.88)(61.25,106.88)
\newrgbcolor{userLineColour}{0.6 0.6 0.6}
\newrgbcolor{userFillColour}{0.6 0.6 0.6}
\pspolygon[linecolor=userLineColour,fillcolor=userFillColour,fillstyle=solid](156.25,95)(151.25,95)(151.25,106.88)(156.25,106.88)
\psline[linewidth=0.75](113.75,94.37)(173.75,94.37)
\psline[linewidth=0.75](153.75,106.25)(153.75,94.37)
\psline[linewidth=0.75](33.75,94.38)(83.75,94.37)
\psline[linewidth=0.75](58.75,106.25)(58.75,94.37)
\end{pspicture}


==> PIC/kleene-2.tex <==
%%Created by jPicEdt 1.4.1_03: mixed JPIC-XML/LaTeX format
%%Tue Nov 05 18:34:22 GMT-10:00 2019
%%Begin JPIC-XML
%<?xml version="1.0" standalone="yes"?>
%<jpic x-min="25" x-max="368.75" y-min="0.62" y-max="131.25" auto-bounding="true">
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(125,78.75);(125,78.75);(125,53.75);(125,53.75)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(185,88.12);(185,88.12);(185,113.12);(185,113.12)"
%	 />
%<text text-vert-align= "center-v"
%	 anchor-point= "(165,131.25)"
%	 stroke-width= "0.75"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\nameslang$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(176.25,1.25)"
%	 stroke-width= "0.75"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\inputt$
%</text>
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(150,88.12);(150,88.12);(185,88.12);(185,88.12)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(176.25,88.12);(176.25,88.12);(176.25,7.5);(176.25,7.5)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(125,53.75);(125,53.75);(150,53.75);(150,53.75)"
%	 />
%<text text-vert-align= "center-v"
%	 anchor-point= "(163.12,100)"
%	 stroke-width= "0.75"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\universal
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(132.5,60.62)"
%	 stroke-width= "0.75"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\program
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(110,95)"
%	 stroke-width= "0.75"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\EQLS
%</text>
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(125,78.75);(125,78.75);(150,53.75);(150,53.75)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(137.5,100.62);(137.5,100.62);(137.5,66.88);(137.5,66.88)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(125,113.12);(125,113.12);(150,88.12);(150,88.12)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(95,88.12);(95,88.12);(95,113.12);(95,113.12)"
%	 />
%<text text-vert-align= "center-v"
%	 anchor-point= "(70,131.25)"
%	 stroke-width= "0.75"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\nameslang$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(85,1.25)"
%	 stroke-width= "0.75"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\inputt$
%</text>
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(45,88.12);(45,88.12);(95,88.12);(95,88.12)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(85,88.12);(85,88.12);(85,6.88);(85,6.88)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(55,88.12);(55,88.12);(55,66.87);(55,66.87)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(45,113.12);(45,113.12);(45,88.12);(45,88.12)"
%	 />
%<text text-vert-align= "center-v"
%	 anchor-point= "(70,100)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\gee$
%</text>
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(25,75);(25,75);(46.25,75);(46.25,75)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(66.25,55);(66.25,55);(45,55);(45,55)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(46.25,75);(46.25,75);(66.25,55);(66.25,55)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(25,75);(25,75);(45,55);(45,55)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(45.62,33.12);(45.62,33.12);(45.62,22.5);(45.62,22.5)"
%	 />
%<ellipse p3= "(47.04,31.72)"
%	 p2= "(47.04,34.54)"
%	 fill-color= "#330033"
%	 p1= "(44.22,34.54)"
%	 closure= "open"
%	 fill-style= "solid"
%	 angle-end= "0"
%	 angle-start= "0"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(56.25,55);(56.25,55);(56.25,43.75);(56.25,43.75)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(35.62,63.75);(35.62,63.75);(35.62,42.5);(35.62,42.5)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(56.25,43.75);(56.25,43.75);(45.62,33.12);(45.62,33.12)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(35.62,42.5);(35.62,42.5);(45.62,32.5);(45.62,32.5)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(156.25,88.12);(156.25,88.12);(156.25,22.5);(156.25,22.5)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(35,33.75);(35,33.75);(35,8.75);(35,8.75)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(35,8.75);(35,8.75);(60,8.75);(60,8.75)"
%	 />
%<text text-vert-align= "center-v"
%	 anchor-point= "(42.5,15.62)"
%	 stroke-width= "0.75"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\program
%</text>
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(35,33.75);(35,33.75);(60,8.75);(60,8.75)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(144.38,34.38);(144.38,34.38);(144.38,9.38);(144.38,9.38)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(144.38,9.38);(144.38,9.38);(169.38,9.38);(169.38,9.38)"
%	 />
%<text text-vert-align= "center-v"
%	 anchor-point= "(151.88,16.25)"
%	 stroke-width= "0.75"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\program
%</text>
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(144.38,34.38);(144.38,34.38);(169.38,9.38);(169.38,9.38)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(275.62,87.5);(275.62,87.5);(275.62,112.5);(275.62,112.5)"
%	 />
%<text text-vert-align= "center-v"
%	 anchor-point= "(255.62,130.62)"
%	 stroke-width= "0.75"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\nameslang$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(266.88,0.62)"
%	 stroke-width= "0.75"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\inputt$
%</text>
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(240.62,87.5);(240.62,87.5);(275.62,87.5);(275.62,87.5)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(266.88,87.5);(266.88,87.5);(266.88,6.88);(266.88,6.88)"
%	 />
%<text text-vert-align= "center-v"
%	 anchor-point= "(253.74,99.38)"
%	 stroke-width= "0.75"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\universal
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(200.62,94.38)"
%	 stroke-width= "0.75"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\EQLS
%</text>
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(215.62,112.5);(215.62,112.5);(240.62,87.5);(240.62,87.5)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(237.5,35);(237.5,35);(237.5,24.38);(237.5,24.38)"
%	 />
%<ellipse p3= "(238.91,33.59)"
%	 p2= "(238.91,36.41)"
%	 fill-color= "#330033"
%	 p1= "(236.09,36.41)"
%	 closure= "open"
%	 fill-style= "solid"
%	 angle-end= "0"
%	 angle-start= "0"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(248.12,87.5);(248.12,87.5);(248.12,45.62);(248.12,45.62)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(227.5,100.62);(227.5,100.62);(227.5,44.38);(227.5,44.38)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(248.12,45.62);(248.12,45.62);(237.5,35);(237.5,35)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(227.5,44.38);(227.5,44.38);(237.5,34.38);(237.5,34.38)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(226.88,35.62);(226.88,35.62);(226.88,10.62);(226.88,10.62)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(226.88,10.62);(226.88,10.62);(251.88,10.62);(251.88,10.62)"
%	 />
%<text text-vert-align= "center-v"
%	 anchor-point= "(234.38,17.5)"
%	 stroke-width= "0.75"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\program
%</text>
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(226.88,35.62);(226.88,35.62);(251.88,10.62);(251.88,10.62)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(368.75,88.12);(368.75,88.12);(368.75,113.12);(368.75,113.12)"
%	 />
%<text text-vert-align= "center-v"
%	 anchor-point= "(343.75,131.25)"
%	 stroke-width= "0.75"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\nameslang$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(358.75,1.25)"
%	 stroke-width= "0.75"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\inputt$
%</text>
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(340.62,88.12);(340.62,88.12);(368.75,88.12);(368.75,88.12)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(358.75,88.12);(358.75,88.12);(358.75,6.88);(358.75,6.88)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(328.75,99.38);(328.75,99.38);(328.75,66.87);(328.75,66.87)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(315.62,113.12);(315.62,113.12);(340.62,88.12);(340.62,88.12)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(298.75,75);(298.75,75);(320,75);(320,75)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(340,55);(340,55);(318.75,55);(318.75,55)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(320,75);(320,75);(340,55);(340,55)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(298.75,75);(298.75,75);(318.75,55);(318.75,55)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(319.38,33.12);(319.38,33.12);(319.38,22.5);(319.38,22.5)"
%	 />
%<ellipse p3= "(320.78,31.72)"
%	 p2= "(320.78,34.54)"
%	 fill-color= "#330033"
%	 p1= "(317.97,34.54)"
%	 closure= "open"
%	 fill-style= "solid"
%	 angle-end= "0"
%	 angle-start= "0"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(330,55);(330,55);(330,43.75);(330,43.75)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(309.38,63.75);(309.38,63.75);(309.38,42.5);(309.38,42.5)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(330,43.75);(330,43.75);(319.38,33.12);(319.38,33.12)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(309.38,42.5);(309.38,42.5);(319.38,32.5);(319.38,32.5)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(308.75,33.75);(308.75,33.75);(308.75,8.75);(308.75,8.75)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(308.75,8.75);(308.75,8.75);(333.75,8.75);(333.75,8.75)"
%	 />
%<text text-vert-align= "center-v"
%	 anchor-point= "(316.25,15.62)"
%	 stroke-width= "0.75"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\program
%</text>
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(308.75,33.75);(308.75,33.75);(333.75,8.75);(333.75,8.75)"
%	 />
%<text text-vert-align= "center-v"
%	 anchor-point= "(350.62,100.62)"
%	 stroke-width= "0.75"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\universal
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(291.88,95)"
%	 stroke-width= "0.75"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\EQLS
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(44.38,65)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\parteval$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(319.38,65)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\parteval$
%</text>
%<parallelogram p3= "(67.5,125.62)"
%	 p2= "(67.5,113.75)"
%	 fill-color= "#999999"
%	 p1= "(72.5,113.75)"
%	 stroke-color= "#999999"
%	 fill-style= "solid"
%	 />
%<parallelogram p3= "(162.5,125.62)"
%	 p2= "(162.5,113.75)"
%	 fill-color= "#999999"
%	 p1= "(167.5,113.75)"
%	 stroke-color= "#999999"
%	 fill-style= "solid"
%	 />
%<parallelogram p3= "(253.12,125)"
%	 p2= "(253.12,112.5)"
%	 fill-color= "#999999"
%	 p1= "(258.12,112.5)"
%	 stroke-color= "#999999"
%	 fill-style= "solid"
%	 />
%<parallelogram p3= "(341.25,125.62)"
%	 p2= "(341.25,113.12)"
%	 fill-color= "#999999"
%	 p1= "(346.25,113.12)"
%	 stroke-color= "#999999"
%	 fill-style= "solid"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(125,113.12);(125,113.12);(185,113.12);(185,113.12)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(165,125);(165,125);(165,113.12);(165,113.12)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(45,113.12);(45,113.12);(95,113.12);(95,113.12)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(70,125);(70,125);(70,113.12);(70,113.12)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(215.62,112.5);(215.62,112.5);(275.62,112.5);(275.62,112.5)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(255.62,124.38);(255.62,124.38);(255.62,112.5);(255.62,112.5)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(315.62,113.12);(315.62,113.12);(368.75,113.12);(368.75,113.12)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(343.75,125);(343.75,125);(343.75,113.12);(343.75,113.12)"
%	 />
%</jpic>
%%End JPIC-XML
%PSTricks content-type (pstricks.sty package needed)
%Add \usepackage{pstricks} in the preamble of your LaTeX file
%You can rescale the whole picture (to 80% for instance) by using the command \def\JPicScale{0.8}
\ifx\JPicScale\undefined\def\JPicScale{1}\fi
\psset{unit=\JPicScale mm}
\psset{linewidth=0.3,dotsep=1,hatchwidth=0.3,hatchsep=1.5,shadowsize=1,dimen=middle}
\psset{dotsize=0.7 2.5,dotscale=1 1,fillcolor=black}
\psset{arrowsize=1 2,arrowlength=1,arrowinset=0.25,tbarsize=0.7 5,bracketlength=0.15,rbracketlength=0.15}
\begin{pspicture}(0,0)(368.75,131.25)
\psline[linewidth=0.75](125,78.75)(125,53.75)
\psline[linewidth=0.75](185,88.12)(185,113.12)
\rput(165,131.25){$\nameslang$}
\rput(176.25,1.25){$\inputt$}
\psline[linewidth=0.75](150,88.12)(185,88.12)
\psline[linewidth=0.75](176.25,88.12)(176.25,7.5)
\psline[linewidth=0.75](125,53.75)(150,53.75)
\rput(163.12,100){\universal}
\rput(132.5,60.62){\program}
\rput(110,95){\EQLS}
\psline[linewidth=0.75](125,78.75)(150,53.75)
\psline[linewidth=0.75](137.5,100.62)(137.5,66.88)
\psline[linewidth=0.75](125,113.12)(150,88.12)
\psline[linewidth=0.75](95,88.12)(95,113.12)
\rput(70,131.25){$\nameslang$}
\rput(85,1.25){$\inputt$}
\psline[linewidth=0.75](45,88.12)(95,88.12)
\psline[linewidth=0.75](85,88.12)(85,6.88)
\psline[linewidth=0.75](55,88.12)(55,66.87)
\psline[linewidth=0.75](45,113.12)(45,88.12)
\rput(70,100){$\gee$}
\psline[linewidth=0.75](25,75)(46.25,75)
\psline[linewidth=0.75](66.25,55)(45,55)
\psline[linewidth=0.75](46.25,75)(66.25,55)
\psline[linewidth=0.75](25,75)(45,55)
\psline[linewidth=0.75](45.62,33.12)(45.62,22.5)
\newrgbcolor{userFillColour}{0.2 0 0.2}
\rput{0}(45.63,33.13){\psellipse[fillcolor=userFillColour,fillstyle=solid](0,0)(1.41,-1.41)}
\psline[linewidth=0.75](56.25,55)(56.25,43.75)
\psline[linewidth=0.75](35.62,63.75)(35.62,42.5)
\psline[linewidth=0.75](56.25,43.75)(45.62,33.12)
\psline[linewidth=0.75](35.62,42.5)(45.62,32.5)
\psline[linewidth=0.75](156.25,88.12)(156.25,22.5)
\psline[linewidth=0.75](35,33.75)(35,8.75)
\psline[linewidth=0.75](35,8.75)(60,8.75)
\rput(42.5,15.62){\program}
\psline[linewidth=0.75](35,33.75)(60,8.75)
\psline[linewidth=0.75](144.38,34.38)(144.38,9.38)
\psline[linewidth=0.75](144.38,9.38)(169.38,9.38)
\rput(151.88,16.25){\program}
\psline[linewidth=0.75](144.38,34.38)(169.38,9.38)
\psline[linewidth=0.75](275.62,87.5)(275.62,112.5)
\rput(255.62,130.62){$\nameslang$}
\rput(266.88,0.62){$\inputt$}
\psline[linewidth=0.75](240.62,87.5)(275.62,87.5)
\psline[linewidth=0.75](266.88,87.5)(266.88,6.88)
\rput(253.74,99.38){\universal}
\rput(200.62,94.38){\EQLS}
\psline[linewidth=0.75](215.62,112.5)(240.62,87.5)
\psline[linewidth=0.75](237.5,35)(237.5,24.38)
\newrgbcolor{userFillColour}{0.2 0 0.2}
\rput{0}(237.5,35){\psellipse[fillcolor=userFillColour,fillstyle=solid](0,0)(1.41,-1.41)}
\psline[linewidth=0.75](248.12,87.5)(248.12,45.62)
\psline[linewidth=0.75](227.5,100.62)(227.5,44.38)
\psline[linewidth=0.75](248.12,45.62)(237.5,35)
\psline[linewidth=0.75](227.5,44.38)(237.5,34.38)
\psline[linewidth=0.75](226.88,35.62)(226.88,10.62)
\psline[linewidth=0.75](226.88,10.62)(251.88,10.62)
\rput(234.38,17.5){\program}
\psline[linewidth=0.75](226.88,35.62)(251.88,10.62)
\psline[linewidth=0.75](368.75,88.12)(368.75,113.12)
\rput(343.75,131.25){$\nameslang$}
\rput(358.75,1.25){$\inputt$}
\psline[linewidth=0.75](340.62,88.12)(368.75,88.12)
\psline[linewidth=0.75](358.75,88.12)(358.75,6.88)
\psline[linewidth=0.75](328.75,99.38)(328.75,66.87)
\psline[linewidth=0.75](315.62,113.12)(340.62,88.12)
\psline[linewidth=0.75](298.75,75)(320,75)
\psline[linewidth=0.75](340,55)(318.75,55)
\psline[linewidth=0.75](320,75)(340,55)
\psline[linewidth=0.75](298.75,75)(318.75,55)
\psline[linewidth=0.75](319.38,33.12)(319.38,22.5)
\newrgbcolor{userFillColour}{0.2 0 0.2}
\rput{90}(319.38,33.13){\psellipse[fillcolor=userFillColour,fillstyle=solid](0,0)(1.41,-1.4)}
\psline[linewidth=0.75](330,55)(330,43.75)
\psline[linewidth=0.75](309.38,63.75)(309.38,42.5)
\psline[linewidth=0.75](330,43.75)(319.38,33.12)
\psline[linewidth=0.75](309.38,42.5)(319.38,32.5)
\psline[linewidth=0.75](308.75,33.75)(308.75,8.75)
\psline[linewidth=0.75](308.75,8.75)(333.75,8.75)
\rput(316.25,15.62){\program}
\psline[linewidth=0.75](308.75,33.75)(333.75,8.75)
\rput(350.62,100.62){\universal}
\rput(291.88,95){\EQLS}
\rput(44.38,65){$\parteval$}
\rput(319.38,65){$\parteval$}
\newrgbcolor{userLineColour}{0.6 0.6 0.6}
\newrgbcolor{userFillColour}{0.6 0.6 0.6}
\pspolygon[linecolor=userLineColour,fillcolor=userFillColour,fillstyle=solid](72.5,113.75)(67.5,113.75)(67.5,125.62)(72.5,125.62)
\newrgbcolor{userLineColour}{0.6 0.6 0.6}
\newrgbcolor{userFillColour}{0.6 0.6 0.6}
\pspolygon[linecolor=userLineColour,fillcolor=userFillColour,fillstyle=solid](167.5,113.75)(162.5,113.75)(162.5,125.62)(167.5,125.62)
\newrgbcolor{userLineColour}{0.6 0.6 0.6}
\newrgbcolor{userFillColour}{0.6 0.6 0.6}
\pspolygon[linecolor=userLineColour,fillcolor=userFillColour,fillstyle=solid](258.12,112.5)(253.12,112.5)(253.12,125)(258.12,125)
\newrgbcolor{userLineColour}{0.6 0.6 0.6}
\newrgbcolor{userFillColour}{0.6 0.6 0.6}
\pspolygon[linecolor=userLineColour,fillcolor=userFillColour,fillstyle=solid](346.25,113.12)(341.25,113.12)(341.25,125.62)(346.25,125.62)
\psline[linewidth=0.75](125,113.12)(185,113.12)
\psline[linewidth=0.75](165,125)(165,113.12)
\psline[linewidth=0.75](45,113.12)(95,113.12)
\psline[linewidth=0.75](70,125)(70,113.12)
\psline[linewidth=0.75](215.62,112.5)(275.62,112.5)
\psline[linewidth=0.75](255.62,124.38)(255.62,112.5)
\psline[linewidth=0.75](315.62,113.12)(368.75,113.12)
\psline[linewidth=0.75](343.75,125)(343.75,113.12)
\end{pspicture}


==> PIC/kleene-3.tex <==
%%Created by jPicEdt 1.4.1_03: mixed JPIC-XML/LaTeX format
%%Tue Nov 05 19:04:53 GMT-10:00 2019
%%Begin JPIC-XML
%<?xml version="1.0" standalone="yes"?>
%<jpic x-min="23.75" x-max="173.75" y-min="0" y-max="102.5" auto-bounding="true">
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(113.75,35.62);(113.75,35.62);(113.75,10.62);(113.75,10.62)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(173.75,59.37);(173.75,59.37);(173.75,84.37);(173.75,84.37)"
%	 />
%<text text-vert-align= "center-v"
%	 anchor-point= "(150,102.5)"
%	 stroke-width= "0.75"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\nameslang$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(150,0)"
%	 stroke-width= "0.75"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\inputt$
%</text>
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(138.75,59.37);(138.75,59.37);(173.75,59.37);(173.75,59.37)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(150,59.37);(150,59.37);(150,5);(150,5)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(113.75,10.62);(113.75,10.62);(138.75,10.62);(138.75,10.62)"
%	 />
%<text text-vert-align= "center-v"
%	 anchor-point= "(150.62,70.62)"
%	 stroke-width= "0.75"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\universal
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(121.25,17.49)"
%	 stroke-width= "0.75"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\program
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(98.75,66.25)"
%	 stroke-width= "0.75"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\EQLS
%</text>
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(113.75,35.62);(113.75,35.62);(138.75,10.62);(138.75,10.62)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(126.25,71.88);(126.25,71.88);(126.25,23.74);(126.25,23.74)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(113.75,84.37);(113.75,84.37);(138.75,59.37);(138.75,59.37)"
%	 />
%<text text-vert-align= "center-v"
%	 anchor-point= "(60,102.5)"
%	 stroke-width= "0.75"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\nameslang$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(60,0)"
%	 stroke-width= "0.75"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\inputt$
%</text>
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(60,59.37);(60,59.37);(60,4.38);(60,4.38)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(23.75,48.75);(23.75,48.75);(23.75,69.38);(23.75,69.38)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(48.12,45.62);(48.12,45.62);(48.12,25);(48.12,25)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(23.75,70);(23.75,70);(48.12,45.62);(48.12,45.62)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(23.75,48.75);(23.75,48.75);(48.12,24.38);(48.12,24.38)"
%	 />
%<text text-vert-align= "center-v"
%	 anchor-point= "(35,48.75)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\parteval$
%</text>
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(83.75,59.37);(83.75,59.37);(83.75,84.37);(83.75,84.37)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(48.75,59.37);(48.75,59.37);(83.75,59.37);(83.75,59.37)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(23.75,84.37);(23.75,84.37);(48.75,59.37);(48.75,59.37)"
%	 />
%<text text-vert-align= "center-v"
%	 anchor-point= "(59.38,70.62)"
%	 stroke-width= "0.75"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\universal
%</text>
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(35,73.12);(35,73.12);(35,58.75);(35,58.75)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(35,37.5);(35,37.5);(35,25);(35,25)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(24.38,35.62);(24.38,35.62);(24.38,10.62);(24.38,10.62)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(24.38,10.62);(24.38,10.62);(49.38,10.62);(49.38,10.62)"
%	 />
%<text text-vert-align= "center-v"
%	 anchor-point= "(31.88,17.49)"
%	 stroke-width= "0.75"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\program
%</text>
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(24.38,35.62);(24.38,35.62);(49.38,10.62);(49.38,10.62)"
%	 />
%<parallelogram p3= "(56.88,96.88)"
%	 p2= "(56.88,84.38)"
%	 fill-color= "#999999"
%	 p1= "(61.88,84.38)"
%	 stroke-color= "#999999"
%	 fill-style= "solid"
%	 />
%<parallelogram p3= "(147.5,96.88)"
%	 p2= "(147.5,84.38)"
%	 fill-color= "#999999"
%	 p1= "(152.5,84.38)"
%	 stroke-color= "#999999"
%	 fill-style= "solid"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(113.75,84.37);(113.75,84.37);(173.75,84.37);(173.75,84.37)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(150,96.25);(150,96.25);(150,84.37);(150,84.37)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(59.38,96.25);(59.38,96.25);(59.38,84.37);(59.38,84.37)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(23.75,84.37);(23.75,84.37);(83.75,84.37);(83.75,84.37)"
%	 />
%</jpic>
%%End JPIC-XML
%PSTricks content-type (pstricks.sty package needed)
%Add \usepackage{pstricks} in the preamble of your LaTeX file
%You can rescale the whole picture (to 80% for instance) by using the command \def\JPicScale{0.8}
\ifx\JPicScale\undefined\def\JPicScale{1}\fi
\psset{unit=\JPicScale mm}
\psset{linewidth=0.3,dotsep=1,hatchwidth=0.3,hatchsep=1.5,shadowsize=1,dimen=middle}
\psset{dotsize=0.7 2.5,dotscale=1 1,fillcolor=black}
\psset{arrowsize=1 2,arrowlength=1,arrowinset=0.25,tbarsize=0.7 5,bracketlength=0.15,rbracketlength=0.15}
\begin{pspicture}(0,0)(173.75,102.5)
\psline[linewidth=0.75](113.75,35.62)(113.75,10.62)
\psline[linewidth=0.75](173.75,59.37)(173.75,84.37)
\rput(150,102.5){$\nameslang$}
\rput(150,0){$\inputt$}
\psline[linewidth=0.75](138.75,59.37)(173.75,59.37)
\psline[linewidth=0.75](150,59.37)(150,5)
\psline[linewidth=0.75](113.75,10.62)(138.75,10.62)
\rput(150.62,70.62){\universal}
\rput(121.25,17.49){\program}
\rput(98.75,66.25){\EQLS}
\psline[linewidth=0.75](113.75,35.62)(138.75,10.62)
\psline[linewidth=0.75](126.25,71.88)(126.25,23.74)
\psline[linewidth=0.75](113.75,84.37)(138.75,59.37)
\rput(60,102.5){$\nameslang$}
\rput(60,0){$\inputt$}
\psline[linewidth=0.75](60,59.37)(60,4.38)
\psline[linewidth=0.75](23.75,48.75)(23.75,69.38)
\psline[linewidth=0.75](48.12,45.62)(48.12,25)
\psline[linewidth=0.75](23.75,70)(48.12,45.62)
\psline[linewidth=0.75](23.75,48.75)(48.12,24.38)
\rput(35,48.75){$\parteval$}
\psline[linewidth=0.75](83.75,59.37)(83.75,84.37)
\psline[linewidth=0.75](48.75,59.37)(83.75,59.37)
\psline[linewidth=0.75](23.75,84.37)(48.75,59.37)
\rput(59.38,70.62){\universal}
\psline[linewidth=0.75](35,73.12)(35,58.75)
\psline[linewidth=0.75](35,37.5)(35,25)
\psline[linewidth=0.75](24.38,35.62)(24.38,10.62)
\psline[linewidth=0.75](24.38,10.62)(49.38,10.62)
\rput(31.88,17.49){\program}
\psline[linewidth=0.75](24.38,35.62)(49.38,10.62)
\newrgbcolor{userLineColour}{0.6 0.6 0.6}
\newrgbcolor{userFillColour}{0.6 0.6 0.6}
\pspolygon[linecolor=userLineColour,fillcolor=userFillColour,fillstyle=solid](61.88,84.38)(56.88,84.38)(56.88,96.88)(61.88,96.88)
\newrgbcolor{userLineColour}{0.6 0.6 0.6}
\newrgbcolor{userFillColour}{0.6 0.6 0.6}
\pspolygon[linecolor=userLineColour,fillcolor=userFillColour,fillstyle=solid](152.5,84.38)(147.5,84.38)(147.5,96.88)(152.5,96.88)
\psline[linewidth=0.75](113.75,84.37)(173.75,84.37)
\psline[linewidth=0.75](150,96.25)(150,84.37)
\psline[linewidth=0.75](59.38,96.25)(59.38,84.37)
\psline[linewidth=0.75](23.75,84.37)(83.75,84.37)
\end{pspicture}


==> PIC/kleene-31.tex <==
%%Created by jPicEdt 1.4.1_03: mixed JPIC-XML/LaTeX format
%%Sun Nov 29 16:44:04 GMT-10:00 2020
%%Begin JPIC-XML
%<?xml version="1.0" standalone="yes"?>
%<jpic x-min="23.75" x-max="173.75" y-min="0" y-max="102.5" auto-bounding="true">
%<multicurve fill-style= "none"
%	 stroke-width= "0.35"
%	 points= "(113.75,35.62);(113.75,35.62);(113.75,10.62);(113.75,10.62)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.35"
%	 points= "(173.75,59.37);(173.75,59.37);(173.75,84.37);(173.75,84.37)"
%	 />
%<text fill-style= "none"
%	 stroke-width= "0.35"
%	 text-vert-align= "center-v"
%	 anchor-point= "(150,102.5)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\nameslang$
%</text>
%<text fill-style= "none"
%	 stroke-width= "0.35"
%	 text-vert-align= "center-v"
%	 anchor-point= "(150,0)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\inputt$
%</text>
%<multicurve fill-style= "none"
%	 stroke-width= "0.35"
%	 points= "(138.75,59.37);(138.75,59.37);(173.75,59.37);(173.75,59.37)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.35"
%	 points= "(150,59.37);(150,59.37);(150,5);(150,5)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.35"
%	 points= "(113.75,10.62);(113.75,10.62);(138.75,10.62);(138.75,10.62)"
%	 />
%<text fill-style= "none"
%	 stroke-width= "0.35"
%	 text-vert-align= "center-v"
%	 anchor-point= "(150.62,70.62)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\universal
%</text>
%<text fill-style= "none"
%	 stroke-width= "0.35"
%	 text-vert-align= "center-v"
%	 anchor-point= "(121.25,17.49)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\program
%</text>
%<text fill-style= "none"
%	 stroke-width= "0.35"
%	 text-vert-align= "center-v"
%	 anchor-point= "(98.75,66.25)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\EQLS
%</text>
%<multicurve fill-style= "none"
%	 stroke-width= "0.35"
%	 points= "(113.75,35.62);(113.75,35.62);(138.75,10.62);(138.75,10.62)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.35"
%	 points= "(126.25,71.88);(126.25,71.88);(126.25,23.74);(126.25,23.74)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.35"
%	 points= "(113.75,84.37);(113.75,84.37);(138.75,59.37);(138.75,59.37)"
%	 />
%<text fill-style= "none"
%	 stroke-width= "0.35"
%	 text-vert-align= "center-v"
%	 anchor-point= "(60,102.5)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\nameslang$
%</text>
%<text fill-style= "none"
%	 stroke-width= "0.35"
%	 text-vert-align= "center-v"
%	 anchor-point= "(60,0)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\inputt$
%</text>
%<multicurve fill-style= "none"
%	 stroke-width= "0.35"
%	 points= "(60,59.37);(60,59.37);(60,4.38);(60,4.38)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.35"
%	 points= "(23.75,48.75);(23.75,48.75);(23.75,69.38);(23.75,69.38)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.35"
%	 points= "(48.12,45.62);(48.12,45.62);(48.12,25);(48.12,25)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.35"
%	 points= "(23.75,70);(23.75,70);(48.12,45.62);(48.12,45.62)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.35"
%	 points= "(23.75,48.75);(23.75,48.75);(48.12,24.38);(48.12,24.38)"
%	 />
%<text fill-style= "none"
%	 stroke-width= "0.35"
%	 text-vert-align= "center-v"
%	 anchor-point= "(35,48.75)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\parteval$
%</text>
%<multicurve fill-style= "none"
%	 stroke-width= "0.35"
%	 points= "(83.75,59.37);(83.75,59.37);(83.75,84.37);(83.75,84.37)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.35"
%	 points= "(48.75,59.37);(48.75,59.37);(83.75,59.37);(83.75,59.37)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.35"
%	 points= "(23.75,84.37);(23.75,84.37);(48.75,59.37);(48.75,59.37)"
%	 />
%<text fill-style= "none"
%	 stroke-width= "0.35"
%	 text-vert-align= "center-v"
%	 anchor-point= "(59.38,70.62)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\universal
%</text>
%<multicurve fill-style= "none"
%	 stroke-width= "0.35"
%	 points= "(35,73.12);(35,73.12);(35,58.75);(35,58.75)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.35"
%	 points= "(35,37.5);(35,37.5);(35,25);(35,25)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.35"
%	 points= "(24.38,35.62);(24.38,35.62);(24.38,10.62);(24.38,10.62)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.35"
%	 points= "(24.38,10.62);(24.38,10.62);(49.38,10.62);(49.38,10.62)"
%	 />
%<text fill-style= "none"
%	 stroke-width= "0.35"
%	 text-vert-align= "center-v"
%	 anchor-point= "(31.88,17.49)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\program
%</text>
%<multicurve fill-style= "none"
%	 stroke-width= "0.35"
%	 points= "(24.38,35.62);(24.38,35.62);(49.38,10.62);(49.38,10.62)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.35"
%	 points= "(113.75,84.37);(113.75,84.37);(173.75,84.37);(173.75,84.37)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.35"
%	 points= "(150,96.25);(150,96.25);(150,84.37);(150,84.37)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.35"
%	 points= "(59.38,96.25);(59.38,96.25);(59.38,84.37);(59.38,84.37)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.35"
%	 points= "(23.75,84.37);(23.75,84.37);(83.75,84.37);(83.75,84.37)"
%	 />
%</jpic>
%%End JPIC-XML
%LaTeX-picture environment using emulated lines and arcs
%You can rescale the whole picture (to 80% for instance) by using the command \def\JPicScale{0.8}
\ifx\JPicScale\undefined\def\JPicScale{1}\fi
\unitlength \JPicScale mm
\begin{picture}(173.75,102.5)(0,0)
\linethickness{0.35mm}
\put(113.75,10.62){\line(0,1){25}}
\linethickness{0.35mm}
\put(173.75,59.37){\line(0,1){25}}
\put(150,102.5){\makebox(0,0)[cc]{$\nameslang$}}

\put(150,0){\makebox(0,0)[cc]{$\inputt$}}

\linethickness{0.35mm}
\put(138.75,59.37){\line(1,0){35}}
\linethickness{0.35mm}
\put(150,5){\line(0,1){54.37}}
\linethickness{0.35mm}
\put(113.75,10.62){\line(1,0){25}}
\put(150.62,70.62){\makebox(0,0)[cc]{\universal}}

\put(121.25,17.49){\makebox(0,0)[cc]{\program}}

\put(98.75,66.25){\makebox(0,0)[cc]{\EQLS}}

\linethickness{0.35mm}
\multiput(113.75,35.62)(0.12,-0.12){208}{\line(1,0){0.12}}
\linethickness{0.35mm}
\put(126.25,23.74){\line(0,1){48.14}}
\linethickness{0.35mm}
\multiput(113.75,84.37)(0.12,-0.12){208}{\line(0,-1){0.12}}
\put(60,102.5){\makebox(0,0)[cc]{$\nameslang$}}

\put(60,0){\makebox(0,0)[cc]{$\inputt$}}

\linethickness{0.35mm}
\put(60,4.38){\line(0,1){54.99}}
\linethickness{0.35mm}
\put(23.75,48.75){\line(0,1){20.63}}
\linethickness{0.35mm}
\put(48.12,25){\line(0,1){20.62}}
\linethickness{0.35mm}
\multiput(23.75,70)(0.12,-0.12){203}{\line(0,-1){0.12}}
\linethickness{0.35mm}
\multiput(23.75,48.75)(0.12,-0.12){203}{\line(0,-1){0.12}}
\put(35,48.75){\makebox(0,0)[cc]{$\parteval$}}

\linethickness{0.35mm}
\put(83.75,59.37){\line(0,1){25}}
\linethickness{0.35mm}
\put(48.75,59.37){\line(1,0){35}}
\linethickness{0.35mm}
\multiput(23.75,84.37)(0.12,-0.12){208}{\line(0,-1){0.12}}
\put(59.38,70.62){\makebox(0,0)[cc]{\universal}}

\linethickness{0.35mm}
\put(35,58.75){\line(0,1){14.37}}
\linethickness{0.35mm}
\put(35,25){\line(0,1){12.5}}
\linethickness{0.35mm}
\put(24.38,10.62){\line(0,1){25}}
\linethickness{0.35mm}
\put(24.38,10.62){\line(1,0){25}}
\put(31.88,17.49){\makebox(0,0)[cc]{\program}}

\linethickness{0.35mm}
\multiput(24.38,35.62)(0.12,-0.12){208}{\line(1,0){0.12}}
\linethickness{0.35mm}
\put(113.75,84.37){\line(1,0){60}}
\linethickness{0.35mm}
\put(150,84.37){\line(0,1){11.88}}
\linethickness{0.35mm}
\put(59.38,84.37){\line(0,1){11.88}}
\linethickness{0.35mm}
\put(23.75,84.37){\line(1,0){60}}
\end{picture}


==> PIC/kleene-4.tex <==
%%Created by jPicEdt 1.4.1_03: mixed JPIC-XML/LaTeX format
%%Thu Sep 29 09:57:58 HST 2016
%%Begin JPIC-XML
%<?xml version="1.0" standalone="yes"?>
%<jpic x-min="0" x-max="185" y-min="2.5" y-max="92.5" auto-bounding="true">
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(0,75);(0,75);(50,75);(50,75)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(0,40.62);(0,40.62);(0,15.62);(0,15.62)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(50,50);(50,50);(50,75);(50,75)"
%	 />
%<multicurve stroke-width= "1.1"
%	 fill-style= "none"
%	 points= "(30,86.88);(30,86.88);(30,75);(30,75)"
%	 />
%<text stroke-width= "0.75"
%	 text-vert-align= "center-v"
%	 anchor-point= "(30,92.5)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\nameslang$
%</text>
%<text stroke-width= "0.75"
%	 text-vert-align= "center-v"
%	 anchor-point= "(40,3.12)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\inputt$
%</text>
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(25,50);(25,50);(50,50);(50,50)"
%	 />
%<multicurve stroke-width= "1.1"
%	 fill-style= "none"
%	 points= "(40,50);(40,50);(40,9.38);(40,9.38)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(0,15.62);(0,15.62);(25,15.62);(25,15.62)"
%	 />
%<text stroke-width= "0.75"
%	 text-vert-align= "center-v"
%	 anchor-point= "(31.25,62.5)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\universal
%</text>
%<text stroke-width= "0.75"
%	 text-vert-align= "center-v"
%	 anchor-point= "(7.5,22.5)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\program
%</text>
%<text stroke-width= "0.75"
%	 text-vert-align= "center-v"
%	 anchor-point= "(65,60)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\EQLS
%</text>
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(0,40.62);(0,40.62);(25,15.62);(25,15.62)"
%	 />
%<multicurve stroke-width= "1.1"
%	 fill-style= "none"
%	 points= "(12.5,62.5);(12.5,62.5);(12.5,28.75);(12.5,28.75)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(0,75);(0,75);(25,50);(25,50)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(80,75);(80,75);(130,75);(130,75)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(77.5,40.62);(77.5,40.62);(77.5,15.62);(77.5,15.62)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(130,50);(130,50);(130,75);(130,75)"
%	 />
%<text stroke-width= "0.75"
%	 text-vert-align= "center-v"
%	 anchor-point= "(90,92.5)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\nameslang$
%</text>
%<text stroke-width= "0.75"
%	 text-vert-align= "center-v"
%	 anchor-point= "(120,3.12)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\inputt$
%</text>
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(80,50);(80,50);(130,50);(130,50)"
%	 />
%<multicurve stroke-width= "1.1"
%	 fill-style= "none"
%	 points= "(120,62.5);(120,62.5);(120,9.38);(120,9.38)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(77.5,15.62);(77.5,15.62);(102.5,15.62);(102.5,15.62)"
%	 />
%<text stroke-width= "0.75"
%	 text-vert-align= "center-v"
%	 anchor-point= "(85,22.5)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\program
%</text>
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(77.5,40.62);(77.5,40.62);(102.5,15.62);(102.5,15.62)"
%	 />
%<multicurve stroke-width= "1.1"
%	 fill-style= "none"
%	 points= "(90,87.5);(90,87.5);(90,28.75);(90,28.75)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(80,75);(80,75);(80,50);(80,50)"
%	 />
%<text text-vert-align= "center-v"
%	 anchor-point= "(105,62.5)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\gee$
%</text>
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(160,75.62);(160,75.62);(160,50.62);(160,50.62)"
%	 />
%<text stroke-width= "0.75"
%	 text-vert-align= "center-v"
%	 anchor-point= "(172.5,92.5)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\nameslang$
%</text>
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(160,50.62);(160,50.62);(185,50.62);(185,50.62)"
%	 />
%<text stroke-width= "0.75"
%	 text-vert-align= "center-v"
%	 anchor-point= "(167.5,57.5)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\program
%</text>
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(160,75.62);(160,75.62);(185,50.62);(185,50.62)"
%	 />
%<multicurve stroke-width= "1.1"
%	 fill-style= "none"
%	 points= "(172.5,87.5);(172.5,87.5);(172.5,63.75);(172.5,63.75)"
%	 />
%<text stroke-width= "0.75"
%	 text-vert-align= "center-v"
%	 anchor-point= "(145,60)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\EQLS
%</text>
%<text stroke-width= "0.75"
%	 text-vert-align= "center-v"
%	 anchor-point= "(170,2.5)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\inputt$
%</text>
%<multicurve stroke-width= "1.1"
%	 fill-style= "none"
%	 points= "(170,40);(170,40);(170,10);(170,10)"
%	 />
%<ellipse p3= "(172.58,37.42)"
%	 p2= "(172.58,42.58)"
%	 p1= "(167.42,42.58)"
%	 closure= "open"
%	 fill-style= "solid"
%	 angle-end= "0"
%	 fill-color= "#330033"
%	 angle-start= "0"
%	 />
%<ellipse p3= "(122.58,59.92)"
%	 p2= "(122.58,65.08)"
%	 p1= "(117.42,65.08)"
%	 closure= "open"
%	 fill-style= "solid"
%	 angle-end= "0"
%	 fill-color= "#330033"
%	 angle-start= "0"
%	 />
%</jpic>
%%End JPIC-XML
%PSTricks content-type (pstricks.sty package needed)
%Add \usepackage{pstricks} in the preamble of your LaTeX file
%You can rescale the whole picture (to 80% for instance) by using the command \def\JPicScale{0.8}
\ifx\JPicScale\undefined\def\JPicScale{1}\fi
\psset{unit=\JPicScale mm}
\psset{linewidth=0.3,dotsep=1,hatchwidth=0.3,hatchsep=1.5,shadowsize=1,dimen=middle}
\psset{dotsize=0.7 2.5,dotscale=1 1,fillcolor=black}
\psset{arrowsize=1 2,arrowlength=1,arrowinset=0.25,tbarsize=0.7 5,bracketlength=0.15,rbracketlength=0.15}
\begin{pspicture}(0,0)(185,92.5)
\psline[linewidth=0.75](0,75)(50,75)
\psline[linewidth=0.75](0,40.62)(0,15.62)
\psline[linewidth=0.75](50,50)(50,75)
\psline[linewidth=1.1](30,86.88)(30,75)
\rput(30,92.5){$\nameslang$}
\rput(40,3.12){$\inputt$}
\psline[linewidth=0.75](25,50)(50,50)
\psline[linewidth=1.1](40,50)(40,9.38)
\psline[linewidth=0.75](0,15.62)(25,15.62)
\rput(31.25,62.5){\universal}
\rput(7.5,22.5){\program}
\rput(65,60){\EQLS}
\psline[linewidth=0.75](0,40.62)(25,15.62)
\psline[linewidth=1.1](12.5,62.5)(12.5,28.75)
\psline[linewidth=0.75](0,75)(25,50)
\psline[linewidth=0.75](80,75)(130,75)
\psline[linewidth=0.75](77.5,40.62)(77.5,15.62)
\psline[linewidth=0.75](130,50)(130,75)
\rput(90,92.5){$\nameslang$}
\rput(120,3.12){$\inputt$}
\psline[linewidth=0.75](80,50)(130,50)
\psline[linewidth=1.1](120,62.5)(120,9.38)
\psline[linewidth=0.75](77.5,15.62)(102.5,15.62)
\rput(85,22.5){\program}
\psline[linewidth=0.75](77.5,40.62)(102.5,15.62)
\psline[linewidth=1.1](90,87.5)(90,28.75)
\psline[linewidth=0.75](80,75)(80,50)
\rput(105,62.5){$\gee$}
\psline[linewidth=0.75](160,75.62)(160,50.62)
\rput(172.5,92.5){$\nameslang$}
\psline[linewidth=0.75](160,50.62)(185,50.62)
\rput(167.5,57.5){\program}
\psline[linewidth=0.75](160,75.62)(185,50.62)
\psline[linewidth=1.1](172.5,87.5)(172.5,63.75)
\rput(145,60){\EQLS}
\rput(170,2.5){$\inputt$}
\psline[linewidth=1.1](170,40)(170,10)
\newrgbcolor{userFillColour}{0.2 0 0.2}
\rput{0}(170,40){\psellipse[fillcolor=userFillColour,fillstyle=solid](0,0)(2.58,-2.58)}
\newrgbcolor{userFillColour}{0.2 0 0.2}
\rput{0}(120,62.5){\psellipse[fillcolor=userFillColour,fillstyle=solid](0,0)(2.58,-2.58)}
\end{pspicture}


==> PIC/kleene-5.tex <==
%%Created by jPicEdt 1.4.1_03: mixed JPIC-XML/LaTeX format
%%Thu Sep 29 10:30:47 HST 2016
%%Begin JPIC-XML
%<?xml version="1.0" standalone="yes"?>
%<jpic x-min="0" x-max="239.38" y-min="3.12" y-max="92.5" auto-bounding="true">
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(0,77.5);(0,77.5);(50,77.5);(50,77.5)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(0,40.62);(0,40.62);(0,15.62);(0,15.62)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(50,52.5);(50,52.5);(50,77.5);(50,77.5)"
%	 />
%<multicurve stroke-width= "1.1"
%	 fill-style= "none"
%	 points= "(40,87.5);(40,87.5);(40,78.12);(40,78.12)"
%	 />
%<text stroke-width= "0.75"
%	 text-vert-align= "center-v"
%	 anchor-point= "(21.25,92.5)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\nameslang$
%</text>
%<text stroke-width= "0.75"
%	 text-vert-align= "center-v"
%	 anchor-point= "(40,3.12)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\inputt$
%</text>
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(25,52.5);(25,52.5);(50,52.5);(50,52.5)"
%	 />
%<multicurve stroke-width= "1.1"
%	 fill-style= "none"
%	 points= "(40,52.5);(40,52.5);(40,9.38);(40,9.38)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(0,15.62);(0,15.62);(25,15.62);(25,15.62)"
%	 />
%<text stroke-width= "0.75"
%	 text-vert-align= "center-v"
%	 anchor-point= "(31.25,65)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\universal
%</text>
%<text stroke-width= "0.75"
%	 text-vert-align= "center-v"
%	 anchor-point= "(7.5,22.5)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\program
%</text>
%<text stroke-width= "0.75"
%	 text-vert-align= "center-v"
%	 anchor-point= "(60,65)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\EQLS
%</text>
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(0,40.62);(0,40.62);(25,15.62);(25,15.62)"
%	 />
%<multicurve stroke-width= "1.1"
%	 fill-style= "none"
%	 points= "(12.5,64.38);(12.5,64.38);(12.5,28.75);(12.5,28.75)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(0,77.5);(0,77.5);(25,52.5);(25,52.5)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(70,80);(70,80);(140,80);(140,80)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(77.5,40.62);(77.5,40.62);(77.5,15.62);(77.5,15.62)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(140,50);(140,50);(140,80);(140,80)"
%	 />
%<text stroke-width= "0.75"
%	 text-vert-align= "center-v"
%	 anchor-point= "(78.12,91.88)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\nameslang$
%</text>
%<text stroke-width= "0.75"
%	 text-vert-align= "center-v"
%	 anchor-point= "(120,3.12)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\inputt$
%</text>
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(70,50);(70,50);(140,50);(140,50)"
%	 />
%<multicurve stroke-width= "1.1"
%	 fill-style= "none"
%	 points= "(120,56.88);(120,56.88);(120,9.38);(120,9.38)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(77.5,15.62);(77.5,15.62);(102.5,15.62);(102.5,15.62)"
%	 />
%<text stroke-width= "0.75"
%	 text-vert-align= "center-v"
%	 anchor-point= "(85,22.5)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\program
%</text>
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(77.5,40.62);(77.5,40.62);(102.5,15.62);(102.5,15.62)"
%	 />
%<multicurve stroke-width= "1.1"
%	 fill-style= "none"
%	 points= "(90,61.25);(90,61.25);(90,28.75);(90,28.75)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(70,80);(70,80);(70,50);(70,50)"
%	 />
%<text text-vert-align= "center-v"
%	 anchor-point= "(78.12,57.5)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\gee$
%</text>
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(155,41.87);(155,41.87);(155,16.87);(155,16.87)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(155,16.87);(155,16.87);(180,16.87);(180,16.87)"
%	 />
%<text stroke-width= "0.75"
%	 text-vert-align= "center-v"
%	 anchor-point= "(162.5,23.75)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\program
%</text>
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(155,41.87);(155,41.87);(180,16.87);(180,16.87)"
%	 />
%<multicurve stroke-width= "1.1"
%	 fill-style= "none"
%	 points= "(167.5,87.5);(167.5,87.5);(167.5,30);(167.5,30)"
%	 />
%<text stroke-width= "0.75"
%	 text-vert-align= "center-v"
%	 anchor-point= "(150.62,65.62)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\EQLS
%</text>
%<ellipse p3= "(92.58,58.67)"
%	 p2= "(92.58,63.83)"
%	 p1= "(87.42,63.83)"
%	 closure= "open"
%	 fill-style= "solid"
%	 angle-end= "0"
%	 fill-color= "#330033"
%	 angle-start= "0"
%	 />
%<multicurve stroke-width= "1.1"
%	 fill-style= "none"
%	 points= "(5,87.5);(5,87.5);(5,78.12);(5,78.12)"
%	 />
%<multicurve stroke-width= "1.1"
%	 fill-style= "none"
%	 points= "(21.25,87.5);(21.25,87.5);(21.25,78.12);(21.25,78.12)"
%	 />
%<text stroke-width= "0.75"
%	 text-vert-align= "center-v"
%	 anchor-point= "(5.62,92.5)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\nameslang$
%</text>
%<multicurve stroke-width= "1.1"
%	 fill-style= "none"
%	 points= "(78.12,86.88);(78.12,86.88);(78.12,73.12);(78.12,73.12)"
%	 />
%<multicurve stroke-width= "0.9"
%	 fill-style= "none"
%	 points= "(108.75,71.88);(108.75,71.88);(133.75,71.88);(133.75,71.88)"
%	 />
%<multicurve stroke-width= "0.9"
%	 fill-style= "none"
%	 points= "(108.75,56.88);(108.75,56.88);(133.75,56.88);(133.75,56.88)"
%	 />
%<multicurve stroke-width= "0.9"
%	 fill-style= "none"
%	 points= "(108.75,71.88);(108.75,71.88);(108.75,56.88);(108.75,56.88)"
%	 />
%<multicurve stroke-width= "0.9"
%	 fill-style= "none"
%	 points= "(133.75,71.88);(133.75,71.88);(133.75,56.87);(133.75,56.87)"
%	 />
%<text stroke-width= "0.9"
%	 text-vert-align= "center-v"
%	 anchor-point= "(120.62,64.38)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\eff
%</text>
%<multicurve stroke-width= "1.1"
%	 fill-style= "none"
%	 points= "(120,86.88);(120,86.88);(120,71.88);(120,71.88)"
%	 />
%<multicurve stroke-width= "1.1"
%	 fill-style= "none"
%	 points= "(78.12,73.12);(78.12,73.12);(90,61.25);(90,61.25)"
%	 />
%<multicurve stroke-width= "1.1"
%	 fill-style= "none"
%	 points= "(102.5,87.5);(102.5,87.5);(102.5,73.75);(102.5,73.75)"
%	 />
%<multicurve stroke-width= "1.1"
%	 fill-style= "none"
%	 points= "(102.5,73.75);(102.5,73.75);(90,61.25);(90,61.25)"
%	 />
%<text stroke-width= "0.75"
%	 text-vert-align= "center-v"
%	 anchor-point= "(102.5,91.88)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\nameslang$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(120.62,91.88)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\outputt$
%</text>
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(185,41.25);(185,41.25);(185,16.24);(185,16.24)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(185,16.24);(185,16.24);(210,16.24);(210,16.24)"
%	 />
%<text stroke-width= "0.75"
%	 text-vert-align= "center-v"
%	 anchor-point= "(192.5,23.12)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\program
%</text>
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(185,41.25);(185,41.25);(210,16.24);(210,16.24)"
%	 />
%<multicurve stroke-width= "1.1"
%	 fill-style= "none"
%	 points= "(197.5,86.88);(197.5,86.88);(197.5,29.38);(197.5,29.38)"
%	 />
%<text stroke-width= "0.75"
%	 text-vert-align= "center-v"
%	 anchor-point= "(225.62,3.12)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\inputt$
%</text>
%<multicurve stroke-width= "1.1"
%	 fill-style= "none"
%	 points= "(225.62,56.88);(225.62,56.88);(225.62,9.38);(225.62,9.38)"
%	 />
%<multicurve stroke-width= "0.9"
%	 fill-style= "none"
%	 points= "(214.38,71.88);(214.38,71.88);(239.38,71.88);(239.38,71.88)"
%	 />
%<multicurve stroke-width= "0.9"
%	 fill-style= "none"
%	 points= "(214.38,56.88);(214.38,56.88);(239.38,56.88);(239.38,56.88)"
%	 />
%<multicurve stroke-width= "0.9"
%	 fill-style= "none"
%	 points= "(214.38,71.88);(214.38,71.88);(214.38,56.88);(214.38,56.88)"
%	 />
%<multicurve stroke-width= "0.9"
%	 fill-style= "none"
%	 points= "(239.38,71.88);(239.38,71.88);(239.38,56.87);(239.38,56.87)"
%	 />
%<text stroke-width= "0.9"
%	 text-vert-align= "center-v"
%	 anchor-point= "(226.25,64.38)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\eff
%</text>
%<multicurve stroke-width= "1.1"
%	 fill-style= "none"
%	 points= "(225.62,86.88);(225.62,86.88);(225.62,71.88);(225.62,71.88)"
%	 />
%</jpic>
%%End JPIC-XML
%PSTricks content-type (pstricks.sty package needed)
%Add \usepackage{pstricks} in the preamble of your LaTeX file
%You can rescale the whole picture (to 80% for instance) by using the command \def\JPicScale{0.8}
\ifx\JPicScale\undefined\def\JPicScale{1}\fi
\psset{unit=\JPicScale mm}
\psset{linewidth=0.3,dotsep=1,hatchwidth=0.3,hatchsep=1.5,shadowsize=1,dimen=middle}
\psset{dotsize=0.7 2.5,dotscale=1 1,fillcolor=black}
\psset{arrowsize=1 2,arrowlength=1,arrowinset=0.25,tbarsize=0.7 5,bracketlength=0.15,rbracketlength=0.15}
\begin{pspicture}(0,0)(239.38,92.5)
\psline[linewidth=0.75](0,77.5)(50,77.5)
\psline[linewidth=0.75](0,40.62)(0,15.62)
\psline[linewidth=0.75](50,52.5)(50,77.5)
\psline[linewidth=1.1](40,87.5)(40,78.12)
\rput(21.25,92.5){$\nameslang$}
\rput(40,3.12){$\inputt$}
\psline[linewidth=0.75](25,52.5)(50,52.5)
\psline[linewidth=1.1](40,52.5)(40,9.38)
\psline[linewidth=0.75](0,15.62)(25,15.62)
\rput(31.25,65){\universal}
\rput(7.5,22.5){\program}
\rput(60,65){\EQLS}
\psline[linewidth=0.75](0,40.62)(25,15.62)
\psline[linewidth=1.1](12.5,64.38)(12.5,28.75)
\psline[linewidth=0.75](0,77.5)(25,52.5)
\psline[linewidth=0.75](70,80)(140,80)
\psline[linewidth=0.75](77.5,40.62)(77.5,15.62)
\psline[linewidth=0.75](140,50)(140,80)
\rput(78.12,91.88){$\nameslang$}
\rput(120,3.12){$\inputt$}
\psline[linewidth=0.75](70,50)(140,50)
\psline[linewidth=1.1](120,56.88)(120,9.38)
\psline[linewidth=0.75](77.5,15.62)(102.5,15.62)
\rput(85,22.5){\program}
\psline[linewidth=0.75](77.5,40.62)(102.5,15.62)
\psline[linewidth=1.1](90,61.25)(90,28.75)
\psline[linewidth=0.75](70,80)(70,50)
\rput(78.12,57.5){$\gee$}
\psline[linewidth=0.75](155,41.87)(155,16.87)
\psline[linewidth=0.75](155,16.87)(180,16.87)
\rput(162.5,23.75){\program}
\psline[linewidth=0.75](155,41.87)(180,16.87)
\psline[linewidth=1.1](167.5,87.5)(167.5,30)
\rput(150.62,65.62){\EQLS}
\newrgbcolor{userFillColour}{0.2 0 0.2}
\rput{0}(90,61.25){\psellipse[fillcolor=userFillColour,fillstyle=solid](0,0)(2.58,-2.58)}
\psline[linewidth=1.1](5,87.5)(5,78.12)
\psline[linewidth=1.1](21.25,87.5)(21.25,78.12)
\rput(5.62,92.5){$\nameslang$}
\psline[linewidth=1.1](78.12,86.88)(78.12,73.12)
\psline[linewidth=0.9](108.75,71.88)(133.75,71.88)
\psline[linewidth=0.9](108.75,56.88)(133.75,56.88)
\psline[linewidth=0.9](108.75,71.88)(108.75,56.88)
\psline[linewidth=0.9](133.75,71.88)(133.75,56.87)
\rput(120.62,64.38){\eff}
\psline[linewidth=1.1](120,86.88)(120,71.88)
\psline[linewidth=1.1](78.12,73.12)(90,61.25)
\psline[linewidth=1.1](102.5,87.5)(102.5,73.75)
\psline[linewidth=1.1](102.5,73.75)(90,61.25)
\rput(102.5,91.88){$\nameslang$}
\rput(120.62,91.88){$\outputt$}
\psline[linewidth=0.75](185,41.25)(185,16.24)
\psline[linewidth=0.75](185,16.24)(210,16.24)
\rput(192.5,23.12){\program}
\psline[linewidth=0.75](185,41.25)(210,16.24)
\psline[linewidth=1.1](197.5,86.88)(197.5,29.38)
\rput(225.62,3.12){$\inputt$}
\psline[linewidth=1.1](225.62,56.88)(225.62,9.38)
\psline[linewidth=0.9](214.38,71.88)(239.38,71.88)
\psline[linewidth=0.9](214.38,56.88)(239.38,56.88)
\psline[linewidth=0.9](214.38,71.88)(214.38,56.88)
\psline[linewidth=0.9](239.38,71.88)(239.38,56.87)
\rput(226.25,64.38){\eff}
\psline[linewidth=1.1](225.62,86.88)(225.62,71.88)
\end{pspicture}


==> PIC/kleene-6.tex <==
%%Created by jPicEdt 1.4.1_03: mixed JPIC-XML/LaTeX format
%%Sat Dec 14 12:10:50 GMT-10:00 2019
%%Begin JPIC-XML
%<?xml version="1.0" standalone="yes"?>
%<jpic x-min="-1.25" x-max="543.75" y-min="-3.12" y-max="117.5" auto-bounding="true">
%<multicurve fill-style= "none"
%	 points= "(91.25,69.38);(91.25,69.38);(91.25,44.38);(91.25,44.38)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(151.25,78.74);(151.25,78.74);(151.25,103.74);(151.25,103.74)"
%	 stroke-width= "0.75"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(136.25,114.38)"
%	 text-frame= "noframe"
%	 stroke-width= "0.75"
%	 text-hor-align= "left"
%	 >
%$\nameslang$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(140,-1.88)"
%	 text-frame= "noframe"
%	 stroke-width= "0.75"
%	 text-hor-align= "right"
%	 >
%$\inputt$
%</text>
%<multicurve fill-style= "none"
%	 points= "(116.25,78.74);(116.25,78.74);(151.25,78.74);(151.25,78.74)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(142.5,78.74);(142.5,78.74);(142.5,-1.88);(142.5,-1.88)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(91.25,44.38);(91.25,44.38);(116.25,44.38);(116.25,44.38)"
%	 stroke-width= "0.75"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(129.37,90.62)"
%	 text-frame= "noframe"
%	 stroke-width= "0.75"
%	 text-hor-align= "center-h"
%	 >
%\universal
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(98.75,51.24)"
%	 text-frame= "noframe"
%	 stroke-width= "0.75"
%	 text-hor-align= "center-h"
%	 >
%\program
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(81.25,85.62)"
%	 text-frame= "noframe"
%	 stroke-width= "0.75"
%	 text-hor-align= "center-h"
%	 >
%\EQLS
%</text>
%<multicurve fill-style= "none"
%	 points= "(91.25,69.38);(91.25,69.38);(116.25,44.38);(116.25,44.38)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(103.75,91.26);(103.75,91.26);(103.75,57.5);(103.75,57.5)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(91.25,103.74);(91.25,103.74);(116.25,78.74);(116.25,78.74)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(68.75,78.74);(68.75,78.74);(68.75,103.74);(68.75,103.74)"
%	 stroke-width= "0.75"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(48.75,114.38)"
%	 text-frame= "noframe"
%	 stroke-width= "0.75"
%	 text-hor-align= "left"
%	 >
%$\nameslang$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(56.25,-1.88)"
%	 text-frame= "noframe"
%	 stroke-width= "0.75"
%	 text-hor-align= "right"
%	 >
%$\inputt$
%</text>
%<multicurve fill-style= "none"
%	 points= "(18.75,78.76);(18.75,78.76);(68.75,78.74);(68.75,78.74)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(58.75,78.74);(58.75,78.74);(58.75,-3.12);(58.75,-3.12)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(28.75,78.76);(28.75,78.76);(28.75,57.5);(28.75,57.5)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(18.75,103.76);(18.75,103.76);(18.75,78.76);(18.75,78.76)"
%	 stroke-width= "0.75"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(43.75,90.62)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\gee$
%</text>
%<multicurve fill-style= "none"
%	 points= "(-1.25,65.62);(-1.25,65.62);(20,65.62);(20,65.62)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(40,45.62);(40,45.62);(18.75,45.62);(18.75,45.62)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(20,65.62);(20,65.62);(40,45.62);(40,45.62)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(-1.25,65.62);(-1.25,65.62);(18.75,45.62);(18.75,45.62)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(19.38,23.76);(19.38,23.76);(19.38,-1.24);(19.38,-1.24)"
%	 stroke-width= "0.75"
%	 />
%<ellipse p3= "(20.78,22.34)"
%	 fill-style= "solid"
%	 p2= "(20.78,25.16)"
%	 fill-color= "#330033"
%	 p1= "(17.96,25.16)"
%	 closure= "open"
%	 angle-end= "0"
%	 angle-start= "0"
%	 />
%<multicurve fill-style= "none"
%	 points= "(30,45.62);(30,45.62);(30,34.38);(30,34.38)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(9.38,54.38);(9.38,54.38);(9.38,33.14);(9.38,33.14)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(30,34.38);(30,34.38);(19.38,23.76);(19.38,23.76)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(9.38,33.14);(9.38,33.14);(19.38,23.12);(19.38,23.12)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(122.5,78.74);(122.5,78.74);(122.5,-1.88);(122.5,-1.88)"
%	 stroke-width= "0.75"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(120,-1.88)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\progtype$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(16.88,-1.24)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\progtype$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(20,54.38)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\parteval$
%</text>
%<parallelogram p3= "(41.25,116.26)"
%	 fill-style= "solid"
%	 p2= "(41.25,103.76)"
%	 fill-color= "#999999"
%	 p1= "(46.25,103.76)"
%	 stroke-color= "#999999"
%	 />
%<parallelogram p3= "(128.75,116.26)"
%	 fill-style= "solid"
%	 p2= "(128.75,104.38)"
%	 fill-color= "#999999"
%	 p1= "(133.75,104.38)"
%	 stroke-color= "#999999"
%	 />
%<multicurve fill-style= "none"
%	 points= "(91.25,103.74);(91.25,103.74);(151.25,103.74);(151.25,103.74)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(131.25,115.62);(131.25,115.62);(131.25,103.74);(131.25,103.74)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(18.75,103.76);(18.75,103.76);(68.75,103.74);(68.75,103.74)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(43.75,115.62);(43.75,115.62);(43.75,103.74);(43.75,103.74)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(315,70.62);(315,70.62);(315,45.62);(315,45.62)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(375,80);(375,80);(375,105);(375,105)"
%	 stroke-width= "0.75"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(360,115.62)"
%	 text-frame= "noframe"
%	 stroke-width= "0.75"
%	 text-hor-align= "left"
%	 >
%$\nameslang$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(363.75,-1.88)"
%	 text-frame= "noframe"
%	 stroke-width= "0.75"
%	 text-hor-align= "right"
%	 >
%$\inputt$
%</text>
%<multicurve fill-style= "none"
%	 points= "(340,80);(340,80);(375,80);(375,80)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(366.25,80);(366.25,80);(366.25,-0.62);(366.25,-0.62)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(315,45.62);(315,45.62);(340,45.62);(340,45.62)"
%	 stroke-width= "0.75"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(353.12,91.88)"
%	 text-frame= "noframe"
%	 stroke-width= "0.75"
%	 text-hor-align= "center-h"
%	 >
%\universal
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(322.5,52.5)"
%	 text-frame= "noframe"
%	 stroke-width= "0.75"
%	 text-hor-align= "center-h"
%	 >
%\program
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(305,86.88)"
%	 text-frame= "noframe"
%	 stroke-width= "0.75"
%	 text-hor-align= "center-h"
%	 >
%\EQLS
%</text>
%<multicurve fill-style= "none"
%	 points= "(315,70.62);(315,70.62);(340,45.62);(340,45.62)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(327.5,92.5);(327.5,92.5);(327.5,58.76);(327.5,58.76)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(315,105);(315,105);(340,80);(340,80)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(295,80);(295,80);(295,105);(295,105)"
%	 stroke-width= "0.75"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(275,115.62)"
%	 text-frame= "noframe"
%	 stroke-width= "0.75"
%	 text-hor-align= "left"
%	 >
%$\nameslang$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(282.5,-1.88)"
%	 text-frame= "noframe"
%	 stroke-width= "0.75"
%	 text-hor-align= "right"
%	 >
%$\inputt$
%</text>
%<multicurve fill-style= "none"
%	 points= "(245,80);(245,80);(295,80);(295,80)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(285,80);(285,80);(285,-1.24);(285,-1.24)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(255,80);(255,80);(255,58.74);(255,58.74)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(245,105);(245,105);(245,80);(245,80)"
%	 stroke-width= "0.75"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(270,91.88)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\gee$
%</text>
%<multicurve fill-style= "none"
%	 points= "(225,66.88);(225,66.88);(246.25,66.88);(246.25,66.88)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(266.25,46.88);(266.25,46.88);(245,46.88);(245,46.88)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(246.25,66.88);(246.25,66.88);(266.25,46.88);(266.25,46.88)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(225,66.88);(225,66.88);(245,46.88);(245,46.88)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(245.62,25);(245.62,25);(245.62,14.38);(245.62,14.38)"
%	 stroke-width= "0.75"
%	 />
%<ellipse p3= "(247.04,23.6)"
%	 fill-style= "solid"
%	 p2= "(247.04,26.42)"
%	 fill-color= "#330033"
%	 p1= "(244.22,26.42)"
%	 closure= "open"
%	 angle-end= "0"
%	 angle-start= "0"
%	 />
%<multicurve fill-style= "none"
%	 points= "(256.25,46.88);(256.25,46.88);(256.25,35.62);(256.25,35.62)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(235.62,55.62);(235.62,55.62);(235.62,34.38);(235.62,34.38)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(256.25,35.62);(256.25,35.62);(245.62,25);(245.62,25)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(235.62,34.38);(235.62,34.38);(245.62,24.38);(245.62,24.38)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(346.25,80);(346.25,80);(346.25,14.38);(346.25,14.38)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(235,25.62);(235,25.62);(235,0.62);(235,0.62)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(235,0.62);(235,0.62);(260,0.62);(260,0.62)"
%	 stroke-width= "0.75"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(242.5,7.49)"
%	 text-frame= "noframe"
%	 stroke-width= "0.75"
%	 text-hor-align= "center-h"
%	 >
%\program
%</text>
%<multicurve fill-style= "none"
%	 points= "(235,25.62);(235,25.62);(260,0.62);(260,0.62)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(334.38,26.26);(334.38,26.26);(334.38,1.26);(334.38,1.26)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(334.38,1.26);(334.38,1.26);(359.38,1.26);(359.38,1.26)"
%	 stroke-width= "0.75"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(341.88,8.12)"
%	 text-frame= "noframe"
%	 stroke-width= "0.75"
%	 text-hor-align= "center-h"
%	 >
%\program
%</text>
%<multicurve fill-style= "none"
%	 points= "(334.38,26.26);(334.38,26.26);(359.38,1.26);(359.38,1.26)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(455.62,79.38);(455.62,79.38);(455.62,104.38);(455.62,104.38)"
%	 stroke-width= "0.75"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(440.62,115)"
%	 text-frame= "noframe"
%	 stroke-width= "0.75"
%	 text-hor-align= "left"
%	 >
%$\nameslang$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(444.38,-2.5)"
%	 text-frame= "noframe"
%	 stroke-width= "0.75"
%	 text-hor-align= "right"
%	 >
%$\inputt$
%</text>
%<multicurve fill-style= "none"
%	 points= "(420.62,79.38);(420.62,79.38);(455.62,79.38);(455.62,79.38)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(446.88,79.38);(446.88,79.38);(446.88,-1.24);(446.88,-1.24)"
%	 stroke-width= "0.75"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(433.74,91.26)"
%	 text-frame= "noframe"
%	 stroke-width= "0.75"
%	 text-hor-align= "center-h"
%	 >
%\universal
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(385.62,86.26)"
%	 text-frame= "noframe"
%	 stroke-width= "0.75"
%	 text-hor-align= "center-h"
%	 >
%\EQLS
%</text>
%<multicurve fill-style= "none"
%	 points= "(395.62,104.38);(395.62,104.38);(420.62,79.38);(420.62,79.38)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(417.5,26.88);(417.5,26.88);(417.5,16.26);(417.5,16.26)"
%	 stroke-width= "0.75"
%	 />
%<ellipse p3= "(418.91,25.46)"
%	 fill-style= "solid"
%	 p2= "(418.91,28.28)"
%	 fill-color= "#330033"
%	 p1= "(416.09,28.28)"
%	 closure= "open"
%	 angle-end= "0"
%	 angle-start= "0"
%	 />
%<multicurve fill-style= "none"
%	 points= "(428.12,79.38);(428.12,79.38);(428.12,37.5);(428.12,37.5)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(407.5,92.5);(407.5,92.5);(407.5,36.26);(407.5,36.26)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(428.12,37.5);(428.12,37.5);(417.5,26.88);(417.5,26.88)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(407.5,36.26);(407.5,36.26);(417.5,26.26);(417.5,26.26)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(406.88,27.5);(406.88,27.5);(406.88,2.5);(406.88,2.5)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(406.88,2.5);(406.88,2.5);(431.88,2.5);(431.88,2.5)"
%	 stroke-width= "0.75"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(414.38,9.38)"
%	 text-frame= "noframe"
%	 stroke-width= "0.75"
%	 text-hor-align= "center-h"
%	 >
%\program
%</text>
%<multicurve fill-style= "none"
%	 points= "(406.88,27.5);(406.88,27.5);(431.88,2.5);(431.88,2.5)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(543.75,80);(543.75,80);(543.75,105);(543.75,105)"
%	 stroke-width= "0.75"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(523.75,115.62)"
%	 text-frame= "noframe"
%	 stroke-width= "0.75"
%	 text-hor-align= "left"
%	 >
%$\nameslang$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(531.25,-1.88)"
%	 text-frame= "noframe"
%	 stroke-width= "0.75"
%	 text-hor-align= "right"
%	 >
%$\inputt$
%</text>
%<multicurve fill-style= "none"
%	 points= "(515.62,80);(515.62,80);(543.75,80);(543.75,80)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(533.75,80);(533.75,80);(533.75,-1.24);(533.75,-1.24)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(503.75,91.26);(503.75,91.26);(503.75,58.74);(503.75,58.74)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(490.62,105);(490.62,105);(515.62,80);(515.62,80)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(473.75,66.88);(473.75,66.88);(495,66.88);(495,66.88)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(515,46.88);(515,46.88);(493.75,46.88);(493.75,46.88)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(495,66.88);(495,66.88);(515,46.88);(515,46.88)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(473.75,66.88);(473.75,66.88);(493.75,46.88);(493.75,46.88)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(494.38,25);(494.38,25);(494.38,14.38);(494.38,14.38)"
%	 stroke-width= "0.75"
%	 />
%<ellipse p3= "(495.78,23.6)"
%	 fill-style= "solid"
%	 p2= "(495.78,26.42)"
%	 fill-color= "#330033"
%	 p1= "(492.97,26.42)"
%	 closure= "open"
%	 angle-end= "0"
%	 angle-start= "0"
%	 />
%<multicurve fill-style= "none"
%	 points= "(505,46.88);(505,46.88);(505,35.62);(505,35.62)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(484.38,55.62);(484.38,55.62);(484.38,34.38);(484.38,34.38)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(505,35.62);(505,35.62);(494.38,25);(494.38,25)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(484.38,34.38);(484.38,34.38);(494.38,24.38);(494.38,24.38)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(483.75,25.62);(483.75,25.62);(483.75,0.62);(483.75,0.62)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(483.75,0.62);(483.75,0.62);(508.75,0.62);(508.75,0.62)"
%	 stroke-width= "0.75"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(491.25,7.49)"
%	 text-frame= "noframe"
%	 stroke-width= "0.75"
%	 text-hor-align= "center-h"
%	 >
%\program
%</text>
%<multicurve fill-style= "none"
%	 points= "(483.75,25.62);(483.75,25.62);(508.75,0.62);(508.75,0.62)"
%	 stroke-width= "0.75"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(525.62,92.5)"
%	 text-frame= "noframe"
%	 stroke-width= "0.75"
%	 text-hor-align= "center-h"
%	 >
%\universal
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(466.88,86.88)"
%	 text-frame= "noframe"
%	 stroke-width= "0.75"
%	 text-hor-align= "center-h"
%	 >
%\EQLS
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(244.38,56.88)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\parteval$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(494.38,56.88)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\parteval$
%</text>
%<parallelogram p3= "(267.5,117.5)"
%	 fill-style= "solid"
%	 p2= "(267.5,105.62)"
%	 fill-color= "#999999"
%	 p1= "(272.5,105.62)"
%	 stroke-color= "#999999"
%	 />
%<parallelogram p3= "(352.5,117.5)"
%	 fill-style= "solid"
%	 p2= "(352.5,105.62)"
%	 fill-color= "#999999"
%	 p1= "(357.5,105.62)"
%	 stroke-color= "#999999"
%	 />
%<parallelogram p3= "(433.12,116.88)"
%	 fill-style= "solid"
%	 p2= "(433.12,104.38)"
%	 fill-color= "#999999"
%	 p1= "(438.12,104.38)"
%	 stroke-color= "#999999"
%	 />
%<parallelogram p3= "(516.25,117.5)"
%	 fill-style= "solid"
%	 p2= "(516.25,105)"
%	 fill-color= "#999999"
%	 p1= "(521.25,105)"
%	 stroke-color= "#999999"
%	 />
%<multicurve fill-style= "none"
%	 points= "(315,105);(315,105);(375,105);(375,105)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(355,116.88);(355,116.88);(355,105);(355,105)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(245,105);(245,105);(295,105);(295,105)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(270,116.88);(270,116.88);(270,105);(270,105)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(395.62,104.38);(395.62,104.38);(455.62,104.38);(455.62,104.38)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(435.62,116.26);(435.62,116.26);(435.62,104.38);(435.62,104.38)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(490.62,105);(490.62,105);(543.75,105);(543.75,105)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(518.75,116.88);(518.75,116.88);(518.75,105);(518.75,105)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(222.5,71.88);(222.5,71.88);(250,71.88);(250,71.88)"
%	 stroke-color= "#ff3333"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(250,71.88);(250,71.88);(272.5,49.38);(272.5,49.38)"
%	 stroke-color= "#ff3333"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(272.5,49.38);(272.5,49.38);(272.5,-3.12);(272.5,-3.12)"
%	 stroke-color= "#ff3333"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(222.5,71.88);(222.5,71.88);(222.5,-3.12);(222.5,-3.12)"
%	 stroke-color= "#ff3333"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(272.5,-3.12);(272.5,-3.12);(222.5,-3.12);(222.5,-3.12)"
%	 stroke-color= "#ff3333"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(470,71.88);(470,71.88);(497.5,71.88);(497.5,71.88)"
%	 stroke-color= "#ff3333"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(497.5,71.88);(497.5,71.88);(520,49.38);(520,49.38)"
%	 stroke-color= "#ff3333"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(520,49.38);(520,49.38);(520,-3.12);(520,-3.12)"
%	 stroke-color= "#ff3333"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(470,71.88);(470,71.88);(470,-3.12);(470,-3.12)"
%	 stroke-color= "#ff3333"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(520,-3.12);(520,-3.12);(470,-3.12);(470,-3.12)"
%	 stroke-color= "#ff3333"
%	 stroke-width= "0.75"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(265,19.38)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\Peeg$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(512.5,19.38)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\Peeg$
%</text>
%</jpic>
%%End JPIC-XML
%PSTricks content-type (pstricks.sty package needed)
%Add \usepackage{pstricks} in the preamble of your LaTeX file
%You can rescale the whole picture (to 80% for instance) by using the command \def\JPicScale{0.8}
\ifx\JPicScale\undefined\def\JPicScale{1}\fi
\psset{unit=\JPicScale mm}
\psset{linewidth=0.3,dotsep=1,hatchwidth=0.3,hatchsep=1.5,shadowsize=1,dimen=middle}
\psset{dotsize=0.7 2.5,dotscale=1 1,fillcolor=black}
\psset{arrowsize=1 2,arrowlength=1,arrowinset=0.25,tbarsize=0.7 5,bracketlength=0.15,rbracketlength=0.15}
\begin{pspicture}(0,0)(543.75,117.5)
\psline[linewidth=0.75](91.25,69.38)(91.25,44.38)
\psline[linewidth=0.75](151.25,78.74)(151.25,103.74)
\rput[l](136.25,114.38){$\nameslang$}
\rput[r](140,-1.88){$\inputt$}
\psline[linewidth=0.75](116.25,78.74)(151.25,78.74)
\psline[linewidth=0.75](142.5,78.74)(142.5,-1.88)
\psline[linewidth=0.75](91.25,44.38)(116.25,44.38)
\rput(129.37,90.62){\universal}
\rput(98.75,51.24){\program}
\rput(81.25,85.62){\EQLS}
\psline[linewidth=0.75](91.25,69.38)(116.25,44.38)
\psline[linewidth=0.75](103.75,91.26)(103.75,57.5)
\psline[linewidth=0.75](91.25,103.74)(116.25,78.74)
\psline[linewidth=0.75](68.75,78.74)(68.75,103.74)
\rput[l](48.75,114.38){$\nameslang$}
\rput[r](56.25,-1.88){$\inputt$}
\psline[linewidth=0.75](18.75,78.76)(68.75,78.74)
\psline[linewidth=0.75](58.75,78.74)(58.75,-3.12)
\psline[linewidth=0.75](28.75,78.76)(28.75,57.5)
\psline[linewidth=0.75](18.75,103.76)(18.75,78.76)
\rput(43.75,90.62){$\gee$}
\psline[linewidth=0.75](-1.25,65.62)(20,65.62)
\psline[linewidth=0.75](40,45.62)(18.75,45.62)
\psline[linewidth=0.75](20,65.62)(40,45.62)
\psline[linewidth=0.75](-1.25,65.62)(18.75,45.62)
\psline[linewidth=0.75](19.38,23.76)(19.38,-1.24)
\newrgbcolor{userFillColour}{0.2 0 0.2}
\rput{0}(19.37,23.74){\psellipse[fillcolor=userFillColour,fillstyle=solid](0,0)(1.41,-1.41)}
\psline[linewidth=0.75](30,45.62)(30,34.38)
\psline[linewidth=0.75](9.38,54.38)(9.38,33.14)
\psline[linewidth=0.75](30,34.38)(19.38,23.76)
\psline[linewidth=0.75](9.38,33.14)(19.38,23.12)
\psline[linewidth=0.75](122.5,78.74)(122.5,-1.88)
\rput[r](120,-1.88){$\progtype$}
\rput[r](16.88,-1.24){$\progtype$}
\rput(20,54.38){$\parteval$}
\newrgbcolor{userLineColour}{0.6 0.6 0.6}
\newrgbcolor{userFillColour}{0.6 0.6 0.6}
\pspolygon[linecolor=userLineColour,fillcolor=userFillColour,fillstyle=solid](46.25,103.76)(41.25,103.76)(41.25,116.26)(46.25,116.26)
\newrgbcolor{userLineColour}{0.6 0.6 0.6}
\newrgbcolor{userFillColour}{0.6 0.6 0.6}
\pspolygon[linecolor=userLineColour,fillcolor=userFillColour,fillstyle=solid](133.75,104.38)(128.75,104.38)(128.75,116.26)(133.75,116.26)
\psline[linewidth=0.75](91.25,103.74)(151.25,103.74)
\psline[linewidth=0.75](131.25,115.62)(131.25,103.74)
\psline[linewidth=0.75](18.75,103.76)(68.75,103.74)
\psline[linewidth=0.75](43.75,115.62)(43.75,103.74)
\psline[linewidth=0.75](315,70.62)(315,45.62)
\psline[linewidth=0.75](375,80)(375,105)
\rput[l](360,115.62){$\nameslang$}
\rput[r](363.75,-1.88){$\inputt$}
\psline[linewidth=0.75](340,80)(375,80)
\psline[linewidth=0.75](366.25,80)(366.25,-0.62)
\psline[linewidth=0.75](315,45.62)(340,45.62)
\rput(353.12,91.88){\universal}
\rput(322.5,52.5){\program}
\rput(305,86.88){\EQLS}
\psline[linewidth=0.75](315,70.62)(340,45.62)
\psline[linewidth=0.75](327.5,92.5)(327.5,58.76)
\psline[linewidth=0.75](315,105)(340,80)
\psline[linewidth=0.75](295,80)(295,105)
\rput[l](275,115.62){$\nameslang$}
\rput[r](282.5,-1.88){$\inputt$}
\psline[linewidth=0.75](245,80)(295,80)
\psline[linewidth=0.75](285,80)(285,-1.24)
\psline[linewidth=0.75](255,80)(255,58.74)
\psline[linewidth=0.75](245,105)(245,80)
\rput(270,91.88){$\gee$}
\psline[linewidth=0.75](225,66.88)(246.25,66.88)
\psline[linewidth=0.75](266.25,46.88)(245,46.88)
\psline[linewidth=0.75](246.25,66.88)(266.25,46.88)
\psline[linewidth=0.75](225,66.88)(245,46.88)
\psline[linewidth=0.75](245.62,25)(245.62,14.38)
\newrgbcolor{userFillColour}{0.2 0 0.2}
\rput{0}(245.63,25){\psellipse[fillcolor=userFillColour,fillstyle=solid](0,0)(1.41,-1.41)}
\psline[linewidth=0.75](256.25,46.88)(256.25,35.62)
\psline[linewidth=0.75](235.62,55.62)(235.62,34.38)
\psline[linewidth=0.75](256.25,35.62)(245.62,25)
\psline[linewidth=0.75](235.62,34.38)(245.62,24.38)
\psline[linewidth=0.75](346.25,80)(346.25,14.38)
\psline[linewidth=0.75](235,25.62)(235,0.62)
\psline[linewidth=0.75](235,0.62)(260,0.62)
\rput(242.5,7.49){\program}
\psline[linewidth=0.75](235,25.62)(260,0.62)
\psline[linewidth=0.75](334.38,26.26)(334.38,1.26)
\psline[linewidth=0.75](334.38,1.26)(359.38,1.26)
\rput(341.88,8.12){\program}
\psline[linewidth=0.75](334.38,26.26)(359.38,1.26)
\psline[linewidth=0.75](455.62,79.38)(455.62,104.38)
\rput[l](440.62,115){$\nameslang$}
\rput[r](444.38,-2.5){$\inputt$}
\psline[linewidth=0.75](420.62,79.38)(455.62,79.38)
\psline[linewidth=0.75](446.88,79.38)(446.88,-1.24)
\rput(433.74,91.26){\universal}
\rput(385.62,86.26){\EQLS}
\psline[linewidth=0.75](395.62,104.38)(420.62,79.38)
\psline[linewidth=0.75](417.5,26.88)(417.5,16.26)
\newrgbcolor{userFillColour}{0.2 0 0.2}
\rput{0}(417.5,26.88){\psellipse[fillcolor=userFillColour,fillstyle=solid](0,0)(1.41,-1.41)}
\psline[linewidth=0.75](428.12,79.38)(428.12,37.5)
\psline[linewidth=0.75](407.5,92.5)(407.5,36.26)
\psline[linewidth=0.75](428.12,37.5)(417.5,26.88)
\psline[linewidth=0.75](407.5,36.26)(417.5,26.26)
\psline[linewidth=0.75](406.88,27.5)(406.88,2.5)
\psline[linewidth=0.75](406.88,2.5)(431.88,2.5)
\rput(414.38,9.38){\program}
\psline[linewidth=0.75](406.88,27.5)(431.88,2.5)
\psline[linewidth=0.75](543.75,80)(543.75,105)
\rput[l](523.75,115.62){$\nameslang$}
\rput[r](531.25,-1.88){$\inputt$}
\psline[linewidth=0.75](515.62,80)(543.75,80)
\psline[linewidth=0.75](533.75,80)(533.75,-1.24)
\psline[linewidth=0.75](503.75,91.26)(503.75,58.74)
\psline[linewidth=0.75](490.62,105)(515.62,80)
\psline[linewidth=0.75](473.75,66.88)(495,66.88)
\psline[linewidth=0.75](515,46.88)(493.75,46.88)
\psline[linewidth=0.75](495,66.88)(515,46.88)
\psline[linewidth=0.75](473.75,66.88)(493.75,46.88)
\psline[linewidth=0.75](494.38,25)(494.38,14.38)
\newrgbcolor{userFillColour}{0.2 0 0.2}
\rput{90}(494.38,25){\psellipse[fillcolor=userFillColour,fillstyle=solid](0,0)(1.41,-1.4)}
\psline[linewidth=0.75](505,46.88)(505,35.62)
\psline[linewidth=0.75](484.38,55.62)(484.38,34.38)
\psline[linewidth=0.75](505,35.62)(494.38,25)
\psline[linewidth=0.75](484.38,34.38)(494.38,24.38)
\psline[linewidth=0.75](483.75,25.62)(483.75,0.62)
\psline[linewidth=0.75](483.75,0.62)(508.75,0.62)
\rput(491.25,7.49){\program}
\psline[linewidth=0.75](483.75,25.62)(508.75,0.62)
\rput(525.62,92.5){\universal}
\rput(466.88,86.88){\EQLS}
\rput(244.38,56.88){$\parteval$}
\rput(494.38,56.88){$\parteval$}
\newrgbcolor{userLineColour}{0.6 0.6 0.6}
\newrgbcolor{userFillColour}{0.6 0.6 0.6}
\pspolygon[linecolor=userLineColour,fillcolor=userFillColour,fillstyle=solid](272.5,105.62)(267.5,105.62)(267.5,117.5)(272.5,117.5)
\newrgbcolor{userLineColour}{0.6 0.6 0.6}
\newrgbcolor{userFillColour}{0.6 0.6 0.6}
\pspolygon[linecolor=userLineColour,fillcolor=userFillColour,fillstyle=solid](357.5,105.62)(352.5,105.62)(352.5,117.5)(357.5,117.5)
\newrgbcolor{userLineColour}{0.6 0.6 0.6}
\newrgbcolor{userFillColour}{0.6 0.6 0.6}
\pspolygon[linecolor=userLineColour,fillcolor=userFillColour,fillstyle=solid](438.12,104.38)(433.12,104.38)(433.12,116.88)(438.12,116.88)
\newrgbcolor{userLineColour}{0.6 0.6 0.6}
\newrgbcolor{userFillColour}{0.6 0.6 0.6}
\pspolygon[linecolor=userLineColour,fillcolor=userFillColour,fillstyle=solid](521.25,105)(516.25,105)(516.25,117.5)(521.25,117.5)
\psline[linewidth=0.75](315,105)(375,105)
\psline[linewidth=0.75](355,116.88)(355,105)
\psline[linewidth=0.75](245,105)(295,105)
\psline[linewidth=0.75](270,116.88)(270,105)
\psline[linewidth=0.75](395.62,104.38)(455.62,104.38)
\psline[linewidth=0.75](435.62,116.26)(435.62,104.38)
\psline[linewidth=0.75](490.62,105)(543.75,105)
\psline[linewidth=0.75](518.75,116.88)(518.75,105)
\newrgbcolor{userLineColour}{1 0.2 0.2}
\psline[linewidth=0.75,linecolor=userLineColour](222.5,71.88)(250,71.88)
\newrgbcolor{userLineColour}{1 0.2 0.2}
\psline[linewidth=0.75,linecolor=userLineColour](250,71.88)(272.5,49.38)
\newrgbcolor{userLineColour}{1 0.2 0.2}
\psline[linewidth=0.75,linecolor=userLineColour](272.5,49.38)(272.5,-3.12)
\newrgbcolor{userLineColour}{1 0.2 0.2}
\psline[linewidth=0.75,linecolor=userLineColour](222.5,71.88)(222.5,-3.12)
\newrgbcolor{userLineColour}{1 0.2 0.2}
\psline[linewidth=0.75,linecolor=userLineColour](272.5,-3.12)(222.5,-3.12)
\newrgbcolor{userLineColour}{1 0.2 0.2}
\psline[linewidth=0.75,linecolor=userLineColour](470,71.88)(497.5,71.88)
\newrgbcolor{userLineColour}{1 0.2 0.2}
\psline[linewidth=0.75,linecolor=userLineColour](497.5,71.88)(520,49.38)
\newrgbcolor{userLineColour}{1 0.2 0.2}
\psline[linewidth=0.75,linecolor=userLineColour](520,49.38)(520,-3.12)
\newrgbcolor{userLineColour}{1 0.2 0.2}
\psline[linewidth=0.75,linecolor=userLineColour](470,71.88)(470,-3.12)
\newrgbcolor{userLineColour}{1 0.2 0.2}
\psline[linewidth=0.75,linecolor=userLineColour](520,-3.12)(470,-3.12)
\rput(265,19.38){$\Peeg$}
\rput(512.5,19.38){$\Peeg$}
\end{pspicture}


==> PIC/kleene-7.tex <==
%%Created by jPicEdt 1.4.1_03: mixed JPIC-XML/LaTeX format
%%Tue Nov 24 19:37:18 GMT-10:00 2020
%%Begin JPIC-XML
%<?xml version="1.0" standalone="yes"?>
%<jpic x-min="0" x-max="435" y-min="0" y-max="180" auto-bounding="true">
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(45,140)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\gee$
%</text>
%<multicurve fill-style= "none"
%	 points= "(435,115);(435,115);(435,165);(435,165)"
%	 />
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(412.5,180)"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\nameslang$
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(422.5,0)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\inputt$
%</text>
%<multicurve fill-style= "none"
%	 points= "(405,115);(405,115);(435,115);(435,115)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(425,115);(425,115);(425,0);(425,0)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(385,135);(385,135);(385,85);(385,85)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(365,155);(365,155);(405,115);(405,115)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(365,85);(365,85);(365,105);(365,105)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(405,65);(405,65);(385,65);(385,65)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(365,105);(365,105);(405,65);(405,65)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(365,85);(365,85);(385,65);(385,65)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(395,65);(395,65);(395,60);(395,60)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(375,75);(375,75);(375,30);(375,30)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(395,60);(395,60);(375,40);(375,40)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(365,40);(365,40);(365,20);(365,20)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(365,20);(365,20);(385,20);(385,20)"
%	 />
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(370,26.25)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\program
%</text>
%<multicurve fill-style= "none"
%	 points= "(365,40);(365,40);(385,20);(385,20)"
%	 />
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(410,145)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\universal
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(340,105)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\EQLS
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(380,80)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\parteval$
%</text>
%<multicurve fill-style= "none"
%	 points= "(365,165);(365,165);(435,165);(435,165)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(365,165);(365,165);(365,155);(365,155)"
%	 />
%<multicurve stroke-width= "0.2"
%	 fill-style= "none"
%	 stroke-color= "#ff3333"
%	 points= "(370,110);(370,110);(410,70);(410,70)"
%	 />
%<multicurve stroke-width= "0.2"
%	 fill-style= "none"
%	 stroke-color= "#ff3333"
%	 points= "(410,70);(410,70);(410,15);(410,15)"
%	 />
%<multicurve stroke-width= "0.2"
%	 fill-style= "none"
%	 stroke-color= "#ff3333"
%	 points= "(360,110);(360,110);(360,15);(360,15)"
%	 />
%<multicurve stroke-width= "0.2"
%	 fill-style= "none"
%	 stroke-color= "#ff3333"
%	 points= "(410,15);(410,15);(360,15);(360,15)"
%	 />
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(400,25)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\Peeg$
%</text>
%<ellipse stroke-width= "1.3"
%	 fill-style= "solid"
%	 p3= "(377.5,37.5)"
%	 p2= "(377.5,42.5)"
%	 p1= "(372.5,42.5)"
%	 closure= "open"
%	 angle-end= "0"
%	 fill-color= "#333333"
%	 angle-start= "0"
%	 stroke-overstrike= "true"
%	 />
%<multicurve fill-style= "none"
%	 points= "(410,180);(410,180);(410,165);(410,165)"
%	 />
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(292.5,180)"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\nameslang$
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(302.5,0)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\inputt$
%</text>
%<multicurve fill-style= "none"
%	 points= "(265,115);(265,115);(315,115);(315,115)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(305,115);(305,115);(305,0);(305,0)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(245,135);(245,135);(265,115);(265,115)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(275,115);(275,115);(275,60);(275,60)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(255,125);(255,125);(255,30);(255,30)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(275,60);(275,60);(255,40);(255,40)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(245,40);(245,40);(245,20);(245,20)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(245,20);(245,20);(265,20);(265,20)"
%	 />
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(250,26.25)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\program
%</text>
%<multicurve fill-style= "none"
%	 points= "(245,40);(245,40);(265,20);(265,20)"
%	 />
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(290,142.5)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\universal
%</text>
%<multicurve fill-style= "none"
%	 points= "(245,165);(245,165);(315,165);(315,165)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(245,165);(245,165);(245,135);(245,135)"
%	 />
%<ellipse stroke-width= "1.3"
%	 fill-style= "solid"
%	 p3= "(257.5,37.5)"
%	 p2= "(257.5,42.5)"
%	 p1= "(252.5,42.5)"
%	 closure= "open"
%	 angle-end= "0"
%	 fill-color= "#333333"
%	 angle-start= "0"
%	 stroke-overstrike= "true"
%	 />
%<multicurve fill-style= "none"
%	 points= "(290,180);(290,180);(290,165);(290,165)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(315,115);(315,115);(315,165);(315,165)"
%	 />
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(221.25,105)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\EQLS
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(172.5,180)"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\nameslang$
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(182.5,0)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\inputt$
%</text>
%<multicurve fill-style= "none"
%	 points= "(145,115);(145,115);(195,115);(195,115)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(185,115);(185,115);(185,0);(185,0)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(125,135);(125,135);(145,115);(145,115)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(155,115);(155,115);(155,30);(155,30)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(135,125);(135,125);(135,105);(135,105)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(145,40);(145,40);(145,20);(145,20)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(145,20);(145,20);(165,20);(165,20)"
%	 />
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(150,26.25)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\program
%</text>
%<multicurve fill-style= "none"
%	 points= "(145,40);(145,40);(165,20);(165,20)"
%	 />
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(170,142.5)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\universal
%</text>
%<multicurve fill-style= "none"
%	 points= "(125,165);(125,165);(195,165);(195,165)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(125,165);(125,165);(125,135);(125,135)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(170,180);(170,180);(170,165);(170,165)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(195,115);(195,115);(195,165);(195,165)"
%	 />
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(100,105)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\EQLS
%</text>
%<multicurve fill-style= "none"
%	 points= "(125,115);(125,115);(125,95);(125,95)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(125,95);(125,95);(145,95);(145,95)"
%	 />
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(130,101.25)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\program
%</text>
%<multicurve fill-style= "none"
%	 points= "(125,115);(125,115);(145,95);(145,95)"
%	 />
%<multicurve stroke-width= "0.2"
%	 fill-style= "none"
%	 stroke-color= "#ff3333"
%	 points= "(360,110);(360,110);(370,110);(370,110)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(75,115);(75,115);(75,165);(75,165)"
%	 />
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(47.5,180)"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\nameslang$
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(62.5,0)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\inputt$
%</text>
%<multicurve fill-style= "none"
%	 points= "(15,115);(15,115);(75,115);(75,115)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(65,115);(65,115);(65,0);(65,0)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(25,115);(25,115);(25,85);(25,85)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(5,85);(5,85);(5,105);(5,105)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(45,65);(45,65);(25,65);(25,65)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(5,105);(5,105);(45,65);(45,65)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(5,85);(5,85);(25,65);(25,65)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(35,65);(35,65);(35,60);(35,60)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(15,75);(15,75);(15,30);(15,30)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(35,60);(35,60);(15,40);(15,40)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(5,40);(5,40);(5,20);(5,20)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(5,20);(5,20);(25,20);(25,20)"
%	 />
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(10,26.25)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\program
%</text>
%<multicurve fill-style= "none"
%	 points= "(5,40);(5,40);(25,20);(25,20)"
%	 />
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(20,80)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\parteval$
%</text>
%<multicurve fill-style= "none"
%	 points= "(15,165);(15,165);(75,165);(75,165)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(15,165);(15,165);(15,115);(15,115)"
%	 />
%<multicurve stroke-width= "0.2"
%	 fill-style= "none"
%	 stroke-color= "#ff3333"
%	 points= "(10,110);(10,110);(50,70);(50,70)"
%	 />
%<multicurve stroke-width= "0.2"
%	 fill-style= "none"
%	 stroke-color= "#ff3333"
%	 points= "(50,70);(50,70);(50,15);(50,15)"
%	 />
%<multicurve stroke-width= "0.2"
%	 fill-style= "none"
%	 stroke-color= "#ff3333"
%	 points= "(0,110);(0,110);(0,15);(0,15)"
%	 />
%<multicurve stroke-width= "0.2"
%	 fill-style= "none"
%	 stroke-color= "#ff3333"
%	 points= "(50,15);(50,15);(0,15);(0,15)"
%	 />
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(41.25,25)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\Peeg$
%</text>
%<ellipse stroke-width= "1.3"
%	 fill-style= "solid"
%	 p3= "(17.5,37.5)"
%	 p2= "(17.5,42.5)"
%	 p1= "(12.5,42.5)"
%	 closure= "open"
%	 angle-end= "0"
%	 fill-color= "#333333"
%	 angle-start= "0"
%	 stroke-overstrike= "true"
%	 />
%<multicurve fill-style= "none"
%	 points= "(45,180);(45,180);(45,165);(45,165)"
%	 />
%<multicurve stroke-width= "0.2"
%	 fill-style= "none"
%	 stroke-color= "#ff3333"
%	 points= "(0,110);(0,110);(10,110);(10,110)"
%	 />
%<text stroke-width= "0.35"
%	 fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(27.5,105)"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\progtype$
%</text>
%<text stroke-width= "0.35"
%	 fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(157.5,105)"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\progtype$
%</text>
%<text stroke-width= "0.35"
%	 fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(132.5,118.75)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\progtype$
%</text>
%<text stroke-width= "0.35"
%	 fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(277.5,80)"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\progtype$
%</text>
%<text stroke-width= "0.35"
%	 fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(252.5,80)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\progtype$
%</text>
%<text stroke-width= "0.35"
%	 fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(27.5,47.5)"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\progtype$
%</text>
%<text stroke-width= "0.35"
%	 fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(12.5,60)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\progtype$
%</text>
%<text stroke-width= "0.35"
%	 fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(387.5,105)"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\progtype$
%</text>
%<text stroke-width= "0.35"
%	 fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(387.5,47.5)"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\progtype$
%</text>
%<text stroke-width= "0.35"
%	 fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(372.5,60)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\progtype$
%</text>
%</jpic>
%%End JPIC-XML
%LaTeX-picture environment using emulated lines and arcs
%You can rescale the whole picture (to 80% for instance) by using the command \def\JPicScale{0.8}
\ifx\JPicScale\undefined\def\JPicScale{1}\fi
\unitlength \JPicScale mm
\begin{picture}(435,180)(0,0)
\put(45,140){\makebox(0,0)[cc]{$\gee$}}

\linethickness{0.3mm}
\put(435,115){\line(0,1){50}}
\put(412.5,180){\makebox(0,0)[cl]{$\nameslang$}}

\put(422.5,0){\makebox(0,0)[cr]{$\inputt$}}

\linethickness{0.3mm}
\put(405,115){\line(1,0){30}}
\linethickness{0.3mm}
\put(425,0){\line(0,1){115}}
\linethickness{0.3mm}
\put(385,85){\line(0,1){50}}
\linethickness{0.3mm}
\multiput(365,155)(0.12,-0.12){333}{\line(1,0){0.12}}
\linethickness{0.3mm}
\put(365,85){\line(0,1){20}}
\linethickness{0.3mm}
\put(385,65){\line(1,0){20}}
\linethickness{0.3mm}
\multiput(365,105)(0.12,-0.12){333}{\line(1,0){0.12}}
\linethickness{0.3mm}
\multiput(365,85)(0.12,-0.12){167}{\line(1,0){0.12}}
\linethickness{0.3mm}
\put(395,60){\line(0,1){5}}
\linethickness{0.3mm}
\put(375,30){\line(0,1){45}}
\linethickness{0.3mm}
\multiput(375,40)(0.12,0.12){167}{\line(1,0){0.12}}
\linethickness{0.3mm}
\put(365,20){\line(0,1){20}}
\linethickness{0.3mm}
\put(365,20){\line(1,0){20}}
\put(370,26.25){\makebox(0,0)[cc]{\program}}

\linethickness{0.3mm}
\multiput(365,40)(0.12,-0.12){167}{\line(1,0){0.12}}
\put(410,145){\makebox(0,0)[cc]{\universal}}

\put(340,105){\makebox(0,0)[cc]{\EQLS}}

\put(380,80){\makebox(0,0)[cc]{$\parteval$}}

\linethickness{0.3mm}
\put(365,165){\line(1,0){70}}
\linethickness{0.3mm}
\put(365,155){\line(0,1){10}}
\linethickness{0.2mm}
\multiput(370,110)(0.12,-0.12){333}{\line(1,0){0.12}}
\linethickness{0.2mm}
\put(410,15){\line(0,1){55}}
\linethickness{0.2mm}
\put(360,15){\line(0,1){95}}
\linethickness{0.2mm}
\put(360,15){\line(1,0){50}}
\put(400,25){\makebox(0,0)[cc]{$\Peeg$}}

\linethickness{1.3mm}
\put(375,40){\circle*{5}}

\linethickness{0.3mm}
\put(410,165){\line(0,1){15}}
\put(292.5,180){\makebox(0,0)[cl]{$\nameslang$}}

\put(302.5,0){\makebox(0,0)[cr]{$\inputt$}}

\linethickness{0.3mm}
\put(265,115){\line(1,0){50}}
\linethickness{0.3mm}
\put(305,0){\line(0,1){115}}
\linethickness{0.3mm}
\multiput(245,135)(0.12,-0.12){167}{\line(1,0){0.12}}
\linethickness{0.3mm}
\put(275,60){\line(0,1){55}}
\linethickness{0.3mm}
\put(255,30){\line(0,1){95}}
\linethickness{0.3mm}
\multiput(255,40)(0.12,0.12){167}{\line(1,0){0.12}}
\linethickness{0.3mm}
\put(245,20){\line(0,1){20}}
\linethickness{0.3mm}
\put(245,20){\line(1,0){20}}
\put(250,26.25){\makebox(0,0)[cc]{\program}}

\linethickness{0.3mm}
\multiput(245,40)(0.12,-0.12){167}{\line(1,0){0.12}}
\put(290,142.5){\makebox(0,0)[cc]{\universal}}

\linethickness{0.3mm}
\put(245,165){\line(1,0){70}}
\linethickness{0.3mm}
\put(245,135){\line(0,1){30}}
\linethickness{1.3mm}
\put(255,40){\circle*{5}}

\linethickness{0.3mm}
\put(290,165){\line(0,1){15}}
\linethickness{0.3mm}
\put(315,115){\line(0,1){50}}
\put(221.25,105){\makebox(0,0)[cc]{\EQLS}}

\put(172.5,180){\makebox(0,0)[cl]{$\nameslang$}}

\put(182.5,0){\makebox(0,0)[cr]{$\inputt$}}

\linethickness{0.3mm}
\put(145,115){\line(1,0){50}}
\linethickness{0.3mm}
\put(185,0){\line(0,1){115}}
\linethickness{0.3mm}
\multiput(125,135)(0.12,-0.12){167}{\line(1,0){0.12}}
\linethickness{0.3mm}
\put(155,30){\line(0,1){85}}
\linethickness{0.3mm}
\put(135,105){\line(0,1){20}}
\linethickness{0.3mm}
\put(145,20){\line(0,1){20}}
\linethickness{0.3mm}
\put(145,20){\line(1,0){20}}
\put(150,26.25){\makebox(0,0)[cc]{\program}}

\linethickness{0.3mm}
\multiput(145,40)(0.12,-0.12){167}{\line(1,0){0.12}}
\put(170,142.5){\makebox(0,0)[cc]{\universal}}

\linethickness{0.3mm}
\put(125,165){\line(1,0){70}}
\linethickness{0.3mm}
\put(125,135){\line(0,1){30}}
\linethickness{0.3mm}
\put(170,165){\line(0,1){15}}
\linethickness{0.3mm}
\put(195,115){\line(0,1){50}}
\put(100,105){\makebox(0,0)[cc]{\EQLS}}

\linethickness{0.3mm}
\put(125,95){\line(0,1){20}}
\linethickness{0.3mm}
\put(125,95){\line(1,0){20}}
\put(130,101.25){\makebox(0,0)[cc]{\program}}

\linethickness{0.3mm}
\multiput(125,115)(0.12,-0.12){167}{\line(1,0){0.12}}
\linethickness{0.2mm}
\put(360,110){\line(1,0){10}}
\linethickness{0.3mm}
\put(75,115){\line(0,1){50}}
\put(47.5,180){\makebox(0,0)[cl]{$\nameslang$}}

\put(62.5,0){\makebox(0,0)[cr]{$\inputt$}}

\linethickness{0.3mm}
\put(15,115){\line(1,0){60}}
\linethickness{0.3mm}
\put(65,0){\line(0,1){115}}
\linethickness{0.3mm}
\put(25,85){\line(0,1){30}}
\linethickness{0.3mm}
\put(5,85){\line(0,1){20}}
\linethickness{0.3mm}
\put(25,65){\line(1,0){20}}
\linethickness{0.3mm}
\multiput(5,105)(0.12,-0.12){333}{\line(1,0){0.12}}
\linethickness{0.3mm}
\multiput(5,85)(0.12,-0.12){167}{\line(1,0){0.12}}
\linethickness{0.3mm}
\put(35,60){\line(0,1){5}}
\linethickness{0.3mm}
\put(15,30){\line(0,1){45}}
\linethickness{0.3mm}
\multiput(15,40)(0.12,0.12){167}{\line(1,0){0.12}}
\linethickness{0.3mm}
\put(5,20){\line(0,1){20}}
\linethickness{0.3mm}
\put(5,20){\line(1,0){20}}
\put(10,26.25){\makebox(0,0)[cc]{\program}}

\linethickness{0.3mm}
\multiput(5,40)(0.12,-0.12){167}{\line(1,0){0.12}}
\put(20,80){\makebox(0,0)[cc]{$\parteval$}}

\linethickness{0.3mm}
\put(15,165){\line(1,0){60}}
\linethickness{0.3mm}
\put(15,115){\line(0,1){50}}
\linethickness{0.2mm}
\multiput(10,110)(0.12,-0.12){333}{\line(1,0){0.12}}
\linethickness{0.2mm}
\put(50,15){\line(0,1){55}}
\linethickness{0.2mm}
\put(0,15){\line(0,1){95}}
\linethickness{0.2mm}
\put(0,15){\line(1,0){50}}
\put(41.25,25){\makebox(0,0)[cc]{$\Peeg$}}

\linethickness{1.3mm}
\put(15,40){\circle*{5}}

\linethickness{0.3mm}
\put(45,165){\line(0,1){15}}
\linethickness{0.2mm}
\put(0,110){\line(1,0){10}}
\put(27.5,105){\makebox(0,0)[cl]{$\progtype$}}

\put(157.5,105){\makebox(0,0)[cl]{$\progtype$}}

\put(132.5,118.75){\makebox(0,0)[cr]{$\progtype$}}

\put(277.5,80){\makebox(0,0)[cl]{$\progtype$}}

\put(252.5,80){\makebox(0,0)[cr]{$\progtype$}}

\put(27.5,47.5){\makebox(0,0)[cl]{$\progtype$}}

\put(12.5,60){\makebox(0,0)[cr]{$\progtype$}}

\put(387.5,105){\makebox(0,0)[cl]{$\progtype$}}

\put(387.5,47.5){\makebox(0,0)[cl]{$\progtype$}}

\put(372.5,60){\makebox(0,0)[cr]{$\progtype$}}

\end{picture}


==> PIC/kleene-8.tex <==
%%Created by jPicEdt 1.4.1_03: mixed JPIC-XML/LaTeX format
%%Tue Nov 24 18:55:04 GMT-10:00 2020
%%Begin JPIC-XML
%<?xml version="1.0" standalone="yes"?>
%<jpic x-min="0" x-max="190" y-min="0" y-max="155" auto-bounding="true">
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(40,115)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\gee$
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(167.5,155)"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\nameslang$
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(177.5,0)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\inputt$
%</text>
%<multicurve fill-style= "none"
%	 points= "(140,90);(140,90);(190,90);(190,90)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(180,90);(180,90);(180,0);(180,0)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(120,110);(120,110);(140,90);(140,90)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(150,90);(150,90);(150,0);(150,0)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(130,100);(130,100);(130,80);(130,80)"
%	 />
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(165,117.5)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\universal
%</text>
%<multicurve fill-style= "none"
%	 points= "(120,140);(120,140);(190,140);(190,140)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(120,140);(120,140);(120,110);(120,110)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(165,155);(165,155);(165,140);(165,140)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(190,90);(190,90);(190,140);(190,140)"
%	 />
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(95,80)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\EQLS
%</text>
%<multicurve fill-style= "none"
%	 points= "(120,90);(120,90);(120,70);(120,70)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(120,70);(120,70);(140,70);(140,70)"
%	 />
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(125,76.25)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\program
%</text>
%<multicurve fill-style= "none"
%	 points= "(120,90);(120,90);(140,70);(140,70)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(70,90);(70,90);(70,140);(70,140)"
%	 />
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(42.5,155)"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\nameslang$
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(57.5,0)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\inputt$
%</text>
%<multicurve fill-style= "none"
%	 points= "(10,90);(10,90);(70,90);(70,90)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(60,90);(60,90);(60,0);(60,0)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(20,90);(20,90);(20,60);(20,60)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(0,60);(0,60);(0,80);(0,80)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(40,40);(40,40);(20,40);(20,40)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(0,80);(0,80);(40,40);(40,40)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(0,60);(0,60);(20,40);(20,40)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(30,40);(30,40);(30,35);(30,35)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(10,50);(10,50);(10,0);(10,0)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(30,35);(30,35);(10,15);(10,15)"
%	 />
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(15,55)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\parteval$
%</text>
%<multicurve fill-style= "none"
%	 points= "(10,140);(10,140);(70,140);(70,140)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(10,140);(10,140);(10,90);(10,90)"
%	 />
%<ellipse stroke-width= "1.3"
%	 fill-style= "solid"
%	 p3= "(12.5,12.5)"
%	 p2= "(12.5,17.5)"
%	 p1= "(7.5,17.5)"
%	 closure= "open"
%	 angle-end= "360"
%	 fill-color= "#333333"
%	 angle-start= "0"
%	 stroke-overstrike= "true"
%	 />
%<multicurve fill-style= "none"
%	 points= "(40,155);(40,155);(40,140);(40,140)"
%	 />
%<text stroke-width= "0.35"
%	 fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(22.5,80)"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\progtype$
%</text>
%<text stroke-width= "0.35"
%	 fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(147.5,0)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\progtype$
%</text>
%<text stroke-width= "0.35"
%	 fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(127.5,93.75)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\progtype$
%</text>
%<text stroke-width= "0.35"
%	 fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(7.5,0)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\progtype$
%</text>
%</jpic>
%%End JPIC-XML
%LaTeX-picture environment using emulated lines and arcs
%You can rescale the whole picture (to 80% for instance) by using the command \def\JPicScale{0.8}
\ifx\JPicScale\undefined\def\JPicScale{1}\fi
\unitlength \JPicScale mm
\begin{picture}(190,155)(0,0)
\put(40,115){\makebox(0,0)[cc]{$\gee$}}

\put(167.5,155){\makebox(0,0)[cl]{$\nameslang$}}

\put(177.5,0){\makebox(0,0)[cr]{$\inputt$}}

\linethickness{0.3mm}
\put(140,90){\line(1,0){50}}
\linethickness{0.3mm}
\put(180,0){\line(0,1){90}}
\linethickness{0.3mm}
\multiput(120,110)(0.12,-0.12){167}{\line(1,0){0.12}}
\linethickness{0.3mm}
\put(150,0){\line(0,1){90}}
\linethickness{0.3mm}
\put(130,80){\line(0,1){20}}
\put(165,117.5){\makebox(0,0)[cc]{\universal}}

\linethickness{0.3mm}
\put(120,140){\line(1,0){70}}
\linethickness{0.3mm}
\put(120,110){\line(0,1){30}}
\linethickness{0.3mm}
\put(165,140){\line(0,1){15}}
\linethickness{0.3mm}
\put(190,90){\line(0,1){50}}
\put(95,80){\makebox(0,0)[cc]{\EQLS}}

\linethickness{0.3mm}
\put(120,70){\line(0,1){20}}
\linethickness{0.3mm}
\put(120,70){\line(1,0){20}}
\put(125,76.25){\makebox(0,0)[cc]{\program}}

\linethickness{0.3mm}
\multiput(120,90)(0.12,-0.12){167}{\line(1,0){0.12}}
\linethickness{0.3mm}
\put(70,90){\line(0,1){50}}
\put(42.5,155){\makebox(0,0)[cl]{$\nameslang$}}

\put(57.5,0){\makebox(0,0)[cr]{$\inputt$}}

\linethickness{0.3mm}
\put(10,90){\line(1,0){60}}
\linethickness{0.3mm}
\put(60,0){\line(0,1){90}}
\linethickness{0.3mm}
\put(20,60){\line(0,1){30}}
\linethickness{0.3mm}
\put(0,60){\line(0,1){20}}
\linethickness{0.3mm}
\put(20,40){\line(1,0){20}}
\linethickness{0.3mm}
\multiput(0,80)(0.12,-0.12){333}{\line(1,0){0.12}}
\linethickness{0.3mm}
\multiput(0,60)(0.12,-0.12){167}{\line(1,0){0.12}}
\linethickness{0.3mm}
\put(30,35){\line(0,1){5}}
\linethickness{0.3mm}
\put(10,0){\line(0,1){50}}
\linethickness{0.3mm}
\multiput(10,15)(0.12,0.12){167}{\line(1,0){0.12}}
\put(15,55){\makebox(0,0)[cc]{$\parteval$}}

\linethickness{0.3mm}
\put(10,140){\line(1,0){60}}
\linethickness{0.3mm}
\put(10,90){\line(0,1){50}}
\linethickness{1.3mm}
\put(10,15){\circle*{5}}

\linethickness{0.3mm}
\put(40,140){\line(0,1){15}}
\put(22.5,80){\makebox(0,0)[cl]{$\progtype$}}

\put(147.5,0){\makebox(0,0)[cr]{$\progtype$}}

\put(127.5,93.75){\makebox(0,0)[cr]{$\progtype$}}

\put(7.5,0){\makebox(0,0)[cr]{$\progtype$}}

\end{picture}


==> PIC/kleene-9.tex <==
%%Created by jPicEdt 1.4.1_03: mixed JPIC-XML/LaTeX format
%%Tue Nov 24 19:01:55 GMT-10:00 2020
%%Begin JPIC-XML
%<?xml version="1.0" standalone="yes"?>
%<jpic x-min="0" x-max="190" y-min="0" y-max="130" auto-bounding="true">
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(40,90)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\gee$
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(167.5,130)"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\nameslang$
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(177.5,0)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\inputt$
%</text>
%<multicurve fill-style= "none"
%	 points= "(160,65);(160,65);(190,65);(190,65)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(180,65);(180,65);(180,0);(180,0)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(120,105);(120,105);(160,65);(160,65)"
%	 />
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(165,92.5)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\universal
%</text>
%<multicurve fill-style= "none"
%	 points= "(120,115);(120,115);(190,115);(190,115)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(120,115);(120,115);(120,105);(120,105)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(165,130);(165,130);(165,115);(165,115)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(190,65);(190,65);(190,115);(190,115)"
%	 />
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(95,90)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\EQLS
%</text>
%<multicurve fill-style= "none"
%	 points= "(70,65);(70,65);(70,115);(70,115)"
%	 />
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(42.5,130)"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\nameslang$
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(57.5,0)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\inputt$
%</text>
%<multicurve fill-style= "none"
%	 points= "(10,65);(10,65);(70,65);(70,65)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(60,65);(60,65);(60,0);(60,0)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(20,65);(20,65);(20,35);(20,35)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(0,15);(0,15);(0,55);(0,55)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(40,15);(40,15);(0,15);(0,15)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(0,55);(0,55);(40,15);(40,15)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(10,115);(10,115);(70,115);(70,115)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(10,115);(10,115);(10,65);(10,65)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(40,130);(40,130);(40,115);(40,115)"
%	 />
%<text stroke-width= "0.35"
%	 fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(22.5,50)"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\progtype$
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(12.5,27.5)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\Peeg$
%</text>
%<multicurve fill-style= "none"
%	 points= "(140,85);(140,85);(140,35);(140,35)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(120,15);(120,15);(120,55);(120,55)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(160,15);(160,15);(120,15);(120,15)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(120,55);(120,55);(160,15);(160,15)"
%	 />
%<text stroke-width= "0.35"
%	 fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(142.5,50)"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\progtype$
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(132.5,27.5)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\Peeg$
%</text>
%</jpic>
%%End JPIC-XML
%LaTeX-picture environment using emulated lines and arcs
%You can rescale the whole picture (to 80% for instance) by using the command \def\JPicScale{0.8}
\ifx\JPicScale\undefined\def\JPicScale{1}\fi
\unitlength \JPicScale mm
\begin{picture}(190,130)(0,0)
\put(40,90){\makebox(0,0)[cc]{$\gee$}}

\put(167.5,130){\makebox(0,0)[cl]{$\nameslang$}}

\put(177.5,0){\makebox(0,0)[cr]{$\inputt$}}

\linethickness{0.3mm}
\put(160,65){\line(1,0){30}}
\linethickness{0.3mm}
\put(180,0){\line(0,1){65}}
\linethickness{0.3mm}
\multiput(120,105)(0.12,-0.12){333}{\line(1,0){0.12}}
\put(165,92.5){\makebox(0,0)[cc]{\universal}}

\linethickness{0.3mm}
\put(120,115){\line(1,0){70}}
\linethickness{0.3mm}
\put(120,105){\line(0,1){10}}
\linethickness{0.3mm}
\put(165,115){\line(0,1){15}}
\linethickness{0.3mm}
\put(190,65){\line(0,1){50}}
\put(95,90){\makebox(0,0)[cc]{\EQLS}}

\linethickness{0.3mm}
\put(70,65){\line(0,1){50}}
\put(42.5,130){\makebox(0,0)[cl]{$\nameslang$}}

\put(57.5,0){\makebox(0,0)[cr]{$\inputt$}}

\linethickness{0.3mm}
\put(10,65){\line(1,0){60}}
\linethickness{0.3mm}
\put(60,0){\line(0,1){65}}
\linethickness{0.3mm}
\put(20,35){\line(0,1){30}}
\linethickness{0.3mm}
\put(0,15){\line(0,1){40}}
\linethickness{0.3mm}
\put(0,15){\line(1,0){40}}
\linethickness{0.3mm}
\multiput(0,55)(0.12,-0.12){333}{\line(1,0){0.12}}
\linethickness{0.3mm}
\put(10,115){\line(1,0){60}}
\linethickness{0.3mm}
\put(10,65){\line(0,1){50}}
\linethickness{0.3mm}
\put(40,115){\line(0,1){15}}
\put(22.5,50){\makebox(0,0)[cl]{$\progtype$}}

\put(12.5,27.5){\makebox(0,0)[cc]{$\Peeg$}}

\linethickness{0.3mm}
\put(140,35){\line(0,1){50}}
\linethickness{0.3mm}
\put(120,15){\line(0,1){40}}
\linethickness{0.3mm}
\put(120,15){\line(1,0){40}}
\linethickness{0.3mm}
\multiput(120,55)(0.12,-0.12){333}{\line(1,0){0.12}}
\put(142.5,50){\makebox(0,0)[cl]{$\progtype$}}

\put(132.5,27.5){\makebox(0,0)[cc]{$\Peeg$}}

\end{picture}


==> PIC/kleene-set-1.tex <==
%%Created by jPicEdt 1.4.1_03: mixed JPIC-XML/LaTeX format
%%Sat May 22 20:36:17 GMT-10:00 2021
%%Begin JPIC-XML
%<?xml version="1.0" standalone="yes"?>
%<jpic x-min="0" x-max="140" y-min="0" y-max="100" auto-bounding="true">
%<multicurve fill-style= "none"
%	 points= "(20,80);(20,80);(60,80);(60,80)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(60,80);(60,80);(60,60);(60,60)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(60,60);(60,60);(20,60);(20,60)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(20,60);(20,60);(20,80);(20,80)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(40,80);(40,80);(40,100);(40,100)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.65"
%	 points= "(30,60);(30,60);(30,40);(30,40)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(50,60);(50,60);(50,0);(50,0)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(20,50);(20,50);(40,30);(40,30)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(40,30);(40,30);(20,30);(20,30)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(20,30);(20,30);(0,50);(0,50)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(0,50);(0,50);(20,50);(20,50)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.65"
%	 points= "(30,30);(30,30);(30,0);(30,0)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(80,80);(80,80);(140,80);(140,80)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(140,80);(140,80);(140,60);(140,60)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(140,60);(140,60);(100,60);(100,60)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(100,60);(100,60);(80,80);(80,80)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(120,80);(120,80);(120,100);(120,100)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.65"
%	 points= "(110,60);(110,60);(110,0);(110,0)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(130,60);(130,60);(130,0);(130,0)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(100,30);(100,30);(80,50);(80,50)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(80,30);(80,30);(100,30);(100,30)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(80,50);(80,50);(80,30);(80,30)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.65"
%	 points= "(90,70);(90,70);(90,40);(90,40)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.65"
%	 points= "(10,40);(10,40);(10,30);(10,30)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.65"
%	 points= "(10,30);(10,30);(30,10);(30,10)"
%	 />
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(30,10)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\DOTT
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(30,40)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\DOTT
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(90,40)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\DOTT
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(47.5,0)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\Aah$
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(127.5,0)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\Aah$
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(20,40)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\PK$
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(40,70)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\grr$
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(42.5,100)"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\Bah$
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(122.5,100)"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\Bah$
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(120,70)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\UK$
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(70,70)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\EQLS
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(85,35)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\Grr$
%</text>
%</jpic>
%%End JPIC-XML
%LaTeX-picture environment using emulated lines and arcs
%You can rescale the whole picture (to 80% for instance) by using the command \def\JPicScale{0.8}
\ifx\JPicScale\undefined\def\JPicScale{1}\fi
\unitlength \JPicScale mm
\begin{picture}(140,100)(0,0)
\linethickness{0.3mm}
\put(20,80){\line(1,0){40}}
\linethickness{0.3mm}
\put(60,60){\line(0,1){20}}
\linethickness{0.3mm}
\put(20,60){\line(1,0){40}}
\linethickness{0.3mm}
\put(20,60){\line(0,1){20}}
\linethickness{0.3mm}
\put(40,80){\line(0,1){20}}
\linethickness{0.65mm}
\put(30,40){\line(0,1){20}}
\linethickness{0.3mm}
\put(50,0){\line(0,1){60}}
\linethickness{0.3mm}
\multiput(20,50)(0.12,-0.12){167}{\line(1,0){0.12}}
\linethickness{0.3mm}
\put(20,30){\line(1,0){20}}
\linethickness{0.3mm}
\multiput(0,50)(0.12,-0.12){167}{\line(1,0){0.12}}
\linethickness{0.3mm}
\put(0,50){\line(1,0){20}}
\linethickness{0.65mm}
\put(30,0){\line(0,1){30}}
\linethickness{0.3mm}
\put(80,80){\line(1,0){60}}
\linethickness{0.3mm}
\put(140,60){\line(0,1){20}}
\linethickness{0.3mm}
\put(100,60){\line(1,0){40}}
\linethickness{0.3mm}
\multiput(80,80)(0.12,-0.12){167}{\line(1,0){0.12}}
\linethickness{0.3mm}
\put(120,80){\line(0,1){20}}
\linethickness{0.65mm}
\put(110,0){\line(0,1){60}}
\linethickness{0.3mm}
\put(130,0){\line(0,1){60}}
\linethickness{0.3mm}
\multiput(80,50)(0.12,-0.12){167}{\line(1,0){0.12}}
\linethickness{0.3mm}
\put(80,30){\line(1,0){20}}
\linethickness{0.3mm}
\put(80,30){\line(0,1){20}}
\linethickness{0.65mm}
\put(90,40){\line(0,1){30}}
\linethickness{0.65mm}
\put(10,30){\line(0,1){10}}
\linethickness{0.65mm}
\multiput(10,30)(0.12,-0.12){167}{\line(1,0){0.12}}
\put(30,10){\makebox(0,0)[cc]{\DOTT}}

\put(30,40){\makebox(0,0)[cc]{\DOTT}}

\put(90,40){\makebox(0,0)[cc]{\DOTT}}

\put(47.5,0){\makebox(0,0)[cr]{$\Aah$}}

\put(127.5,0){\makebox(0,0)[cr]{$\Aah$}}

\put(20,40){\makebox(0,0)[cc]{$\PK$}}

\put(40,70){\makebox(0,0)[cc]{$\grr$}}

\put(42.5,100){\makebox(0,0)[cl]{$\Bah$}}

\put(122.5,100){\makebox(0,0)[cl]{$\Bah$}}

\put(120,70){\makebox(0,0)[cc]{$\UK$}}

\put(70,70){\makebox(0,0)[cc]{\EQLS}}

\put(85,35){\makebox(0,0)[cc]{$\Grr$}}

\end{picture}


==> PIC/kleene-tape.tex <==
%%Created by jPicEdt 1.4.1_03: mixed JPIC-XML/LaTeX format
%%Tue Nov 05 18:41:12 GMT-10:00 2019
%%Begin JPIC-XML
%<?xml version="1.0" standalone="yes"?>
%<jpic x-min="12.5" x-max="155" y-min="-1.88" y-max="88.12" auto-bounding="true">
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(95,35.62);(95,35.62);(95,10.62);(95,10.62)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(155,45);(155,45);(155,70);(155,70)"
%	 />
%<text text-vert-align= "center-v"
%	 anchor-point= "(135,88.12)"
%	 stroke-width= "0.75"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\nameslang$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(135,-1.88)"
%	 stroke-width= "0.75"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\inputt$
%</text>
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(120,45);(120,45);(155,45);(155,45)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(135,45);(135,45);(135,4.38);(135,4.38)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(95,10.62);(95,10.62);(120,10.62);(120,10.62)"
%	 />
%<text text-vert-align= "center-v"
%	 anchor-point= "(133.12,56.88)"
%	 stroke-width= "0.75"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\universal
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(102.5,17.5)"
%	 stroke-width= "0.75"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\program
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(80,51.88)"
%	 stroke-width= "0.75"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\EQLS
%</text>
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(95,35.62);(95,35.62);(120,10.62);(120,10.62)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(107.5,57.5);(107.5,57.5);(107.5,23.75);(107.5,23.75)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(95,70);(95,70);(120,45);(120,45)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(12.5,35.62);(12.5,35.62);(12.5,10.62);(12.5,10.62)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(65,45);(65,45);(65,70);(65,70)"
%	 />
%<text text-vert-align= "center-v"
%	 anchor-point= "(40,88.12)"
%	 stroke-width= "0.75"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\nameslang$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(55,-1.88)"
%	 stroke-width= "0.75"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\inputt$
%</text>
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(15,45);(15,45);(65,45);(65,45)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(55,45);(55,45);(55,4.38);(55,4.38)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(12.5,10.62);(12.5,10.62);(37.5,10.62);(37.5,10.62)"
%	 />
%<text text-vert-align= "center-v"
%	 anchor-point= "(20,17.5)"
%	 stroke-width= "0.75"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\program
%</text>
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(12.5,35.62);(12.5,35.62);(37.5,10.62);(37.5,10.62)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(25,45);(25,45);(25,23.75);(25,23.75)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(15,70);(15,70);(15,45);(15,45)"
%	 />
%<text text-vert-align= "center-v"
%	 anchor-point= "(40,56.88)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\gee$
%</text>
%<parallelogram p3= "(132.5,82.5)"
%	 p2= "(132.5,70)"
%	 fill-color= "#999999"
%	 p1= "(137.5,70)"
%	 stroke-color= "#999999"
%	 fill-style= "solid"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(95,70);(95,70);(155,70);(155,70)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(135,81.88);(135,81.88);(135,70);(135,70)"
%	 />
%<parallelogram p3= "(37.5,82.5)"
%	 p2= "(37.5,70)"
%	 fill-color= "#999999"
%	 p1= "(42.5,70)"
%	 stroke-color= "#999999"
%	 fill-style= "solid"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(15,70);(15,70);(65,70);(65,70)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(40,81.88);(40,81.88);(40,70);(40,70)"
%	 />
%</jpic>
%%End JPIC-XML
%PSTricks content-type (pstricks.sty package needed)
%Add \usepackage{pstricks} in the preamble of your LaTeX file
%You can rescale the whole picture (to 80% for instance) by using the command \def\JPicScale{0.8}
\ifx\JPicScale\undefined\def\JPicScale{1}\fi
\psset{unit=\JPicScale mm}
\psset{linewidth=0.3,dotsep=1,hatchwidth=0.3,hatchsep=1.5,shadowsize=1,dimen=middle}
\psset{dotsize=0.7 2.5,dotscale=1 1,fillcolor=black}
\psset{arrowsize=1 2,arrowlength=1,arrowinset=0.25,tbarsize=0.7 5,bracketlength=0.15,rbracketlength=0.15}
\begin{pspicture}(0,0)(155,88.12)
\psline[linewidth=0.75](95,35.62)(95,10.62)
\psline[linewidth=0.75](155,45)(155,70)
\rput(135,88.12){$\nameslang$}
\rput(135,-1.88){$\inputt$}
\psline[linewidth=0.75](120,45)(155,45)
\psline[linewidth=0.75](135,45)(135,4.38)
\psline[linewidth=0.75](95,10.62)(120,10.62)
\rput(133.12,56.88){\universal}
\rput(102.5,17.5){\program}
\rput(80,51.88){\EQLS}
\psline[linewidth=0.75](95,35.62)(120,10.62)
\psline[linewidth=0.75](107.5,57.5)(107.5,23.75)
\psline[linewidth=0.75](95,70)(120,45)
\psline[linewidth=0.75](12.5,35.62)(12.5,10.62)
\psline[linewidth=0.75](65,45)(65,70)
\rput(40,88.12){$\nameslang$}
\rput(55,-1.88){$\inputt$}
\psline[linewidth=0.75](15,45)(65,45)
\psline[linewidth=0.75](55,45)(55,4.38)
\psline[linewidth=0.75](12.5,10.62)(37.5,10.62)
\rput(20,17.5){\program}
\psline[linewidth=0.75](12.5,35.62)(37.5,10.62)
\psline[linewidth=0.75](25,45)(25,23.75)
\psline[linewidth=0.75](15,70)(15,45)
\rput(40,56.88){$\gee$}
\newrgbcolor{userLineColour}{0.6 0.6 0.6}
\newrgbcolor{userFillColour}{0.6 0.6 0.6}
\pspolygon[linecolor=userLineColour,fillcolor=userFillColour,fillstyle=solid](137.5,70)(132.5,70)(132.5,82.5)(137.5,82.5)
\psline[linewidth=0.75](95,70)(155,70)
\psline[linewidth=0.75](135,81.88)(135,70)
\newrgbcolor{userLineColour}{0.6 0.6 0.6}
\newrgbcolor{userFillColour}{0.6 0.6 0.6}
\pspolygon[linecolor=userLineColour,fillcolor=userFillColour,fillstyle=solid](42.5,70)(37.5,70)(37.5,82.5)(42.5,82.5)
\psline[linewidth=0.75](15,70)(65,70)
\psline[linewidth=0.75](40,81.88)(40,70)
\end{pspicture}


==> PIC/losless-0.tex <==
%%Created by jPicEdt 1.4.1_03: mixed JPIC-XML/LaTeX format
%%Sun Jan 22 15:11:19 GMT-10:00 2023
%%Begin JPIC-XML
%<?xml version="1.0" standalone="yes"?>
%<jpic x-min="0" x-max="165" y-min="0" y-max="180" auto-bounding="true">
%<multicurve fill-style= "none"
%	 points= "(70,160);(70,160);(70,140);(70,140)"
%	 stroke-width= "0.4"
%	 />
%<multicurve fill-style= "none"
%	 points= "(35,135);(35,135);(15,135);(15,135)"
%	 stroke-width= "0.4"
%	 />
%<multicurve fill-style= "none"
%	 points= "(20,160);(20,160);(70,160);(70,160)"
%	 stroke-width= "0.4"
%	 />
%<multicurve fill-style= "none"
%	 points= "(60,140);(60,140);(60,0);(60,0)"
%	 stroke-width= "0.4"
%	 />
%<multicurve fill-style= "none"
%	 points= "(60,180);(60,180);(60,160);(60,160)"
%	 stroke-width= "0.4"
%	 />
%<multicurve fill-style= "none"
%	 points= "(35,135);(35,135);(35,115);(35,115)"
%	 stroke-width= "0.4"
%	 />
%<multicurve fill-style= "none"
%	 points= "(20,145);(20,145);(20,135);(20,135)"
%	 stroke-width= "0.4"
%	 />
%<multicurve fill-style= "none"
%	 points= "(70,140);(70,140);(40,140);(40,140)"
%	 stroke-width= "0.4"
%	 />
%<multicurve fill-style= "none"
%	 points= "(20,160);(20,160);(40,140);(40,140)"
%	 stroke-width= "0.4"
%	 />
%<multicurve fill-style= "none"
%	 points= "(15,135);(15,135);(35,115);(35,115)"
%	 stroke-width= "0.4"
%	 />
%<multicurve fill-style= "none"
%	 points= "(30,135);(30,135);(30,150);(30,150)"
%	 stroke-width= "1.45"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(50,150)"
%	 text-frame= "noframe"
%	 stroke-width= "0.4"
%	 text-hor-align= "center-h"
%	 >
%$\Univ$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(63.75,178.75)"
%	 text-frame= "noframe"
%	 stroke-width= "0.4"
%	 text-hor-align= "left"
%	 >
%$\Cee$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(55,2.5)"
%	 text-frame= "noframe"
%	 stroke-width= "0.4"
%	 text-hor-align= "right"
%	 >
%$\Bee$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(20,145)"
%	 text-frame= "noframe"
%	 stroke-width= "0.4"
%	 text-hor-align= "center-h"
%	 >
%$\Dott$
%</text>
%<multicurve fill-style= "none"
%	 points= "(30,160);(30,160);(30,180);(30,180)"
%	 stroke-width= "1.45"
%	 />
%<multicurve fill-style= "none"
%	 points= "(25,90);(25,90);(25,125);(25,125)"
%	 stroke-width= "1.45"
%	 />
%<multicurve fill-style= "none"
%	 points= "(11.25,132.5);(11.25,132.5);(35,108.75);(35,108.75)"
%	 stroke-color= "#ff0000"
%	 stroke-width= "0.2"
%	 />
%<multicurve fill-style= "none"
%	 points= "(35,108.75);(35,108.75);(75,108.75);(75,108.75)"
%	 stroke-color= "#ff0000"
%	 stroke-width= "0.2"
%	 />
%<multicurve fill-style= "none"
%	 points= "(75,108.75);(75,108.75);(75,166.25);(75,166.25)"
%	 stroke-color= "#ff0000"
%	 stroke-width= "0.2"
%	 />
%<multicurve fill-style= "none"
%	 points= "(21.25,166.25);(21.25,166.25);(75,166.25);(75,166.25)"
%	 stroke-color= "#ff0000"
%	 stroke-width= "0.2"
%	 />
%<multicurve fill-style= "none"
%	 points= "(11.25,156.25);(11.25,156.25);(21.25,166.25);(21.25,166.25)"
%	 stroke-color= "#ff0000"
%	 stroke-width= "0.2"
%	 />
%<multicurve fill-style= "none"
%	 points= "(11.25,132.5);(11.25,132.5);(11.25,156.25);(11.25,156.25)"
%	 stroke-color= "#ff0000"
%	 stroke-width= "0.2"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(30,42.5)"
%	 text-frame= "noframe"
%	 stroke-width= "0.4"
%	 text-hor-align= "center-h"
%	 >
%$\Dott$
%</text>
%<multicurve fill-style= "none"
%	 points= "(40,32.5);(40,32.5);(20,32.5);(20,32.5)"
%	 stroke-width= "0.4"
%	 />
%<multicurve fill-style= "none"
%	 points= "(20,52.5);(20,52.5);(40,32.5);(40,32.5)"
%	 stroke-width= "0.4"
%	 />
%<multicurve fill-style= "none"
%	 points= "(30,32.5);(30,32.5);(30,0);(30,0)"
%	 stroke-width= "0.4"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(20,80)"
%	 text-frame= "noframe"
%	 stroke-width= "0.4"
%	 text-hor-align= "center-h"
%	 >
%$\Dott$
%</text>
%<multicurve fill-style= "none"
%	 points= "(5,95);(5,95);(35,65);(35,65)"
%	 stroke-width= "0.4"
%	 />
%<multicurve fill-style= "none"
%	 points= "(5,95);(5,95);(5,65);(5,65)"
%	 stroke-width= "0.4"
%	 />
%<multicurve fill-style= "none"
%	 points= "(30,42.5);(30,42.5);(30,65);(30,65)"
%	 stroke-width= "1.45"
%	 />
%<multicurve fill-style= "none"
%	 points= "(35,65);(35,65);(5,65);(5,65)"
%	 stroke-width= "0.4"
%	 />
%<multicurve fill-style= "none"
%	 points= "(10,65);(10,65);(10,35);(10,35)"
%	 stroke-width= "0.4"
%	 />
%<multicurve fill-style= "none"
%	 points= "(10,35);(10,35);(30,15);(30,15)"
%	 stroke-width= "0.4"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(30,15)"
%	 text-frame= "noframe"
%	 stroke-width= "0.4"
%	 text-hor-align= "center-h"
%	 >
%$\Dott$
%</text>
%<multicurve fill-style= "none"
%	 points= "(10,100);(10,100);(45,65);(45,65)"
%	 stroke-color= "#ff0033"
%	 stroke-width= "0.2"
%	 />
%<multicurve fill-style= "none"
%	 points= "(45,10);(45,10);(45,65);(45,65)"
%	 stroke-color= "#ff0033"
%	 stroke-width= "0.2"
%	 />
%<multicurve fill-style= "none"
%	 points= "(0,10);(0,10);(0,100);(0,100)"
%	 stroke-color= "#ff0033"
%	 stroke-width= "0.2"
%	 />
%<multicurve fill-style= "none"
%	 points= "(45,10);(45,10);(0,10);(0,10)"
%	 stroke-color= "#ff0033"
%	 stroke-width= "0.2"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(13.75,72.5)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\prrrr$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(27.5,128.75)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\pjjjj$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(25,121.25)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(17.5,140)"
%	 text-frame= "noframe"
%	 stroke-width= "0.4"
%	 text-hor-align= "right"
%	 >
%$\Aee$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(48.75,120)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\PadUniv$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(8.75,18.75)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\PadFee$
%</text>
%<multicurve fill-style= "none"
%	 points= "(20,52.5);(20,52.5);(20,32.5);(20,32.5)"
%	 stroke-width= "0.4"
%	 />
%<multicurve fill-style= "none"
%	 points= "(0,100);(0,100);(10,100);(10,100)"
%	 stroke-color= "#ff0033"
%	 stroke-width= "0.2"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(26.25,2.5)"
%	 text-frame= "noframe"
%	 stroke-width= "0.4"
%	 text-hor-align= "right"
%	 >
%$\Aee$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(33.75,179.38)"
%	 text-frame= "noframe"
%	 stroke-width= "0.4"
%	 text-hor-align= "left"
%	 >
%$\Code$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(100,140)"
%	 text-frame= "noframe"
%	 stroke-width= "0.4"
%	 text-hor-align= "center-h"
%	 >
%\EQLS
%</text>
%<multicurve fill-style= "none"
%	 points= "(165,160);(165,160);(165,140);(165,140)"
%	 stroke-width= "0.4"
%	 />
%<multicurve fill-style= "none"
%	 points= "(115,160);(115,160);(165,160);(165,160)"
%	 stroke-width= "0.4"
%	 />
%<multicurve fill-style= "none"
%	 points= "(155,140);(155,140);(155,0);(155,0)"
%	 stroke-width= "0.4"
%	 />
%<multicurve fill-style= "none"
%	 points= "(155,180);(155,180);(155,160);(155,160)"
%	 stroke-width= "0.4"
%	 />
%<multicurve fill-style= "none"
%	 points= "(165,140);(165,140);(135,140);(135,140)"
%	 stroke-width= "0.4"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(160,178.75)"
%	 text-frame= "noframe"
%	 stroke-width= "0.4"
%	 text-hor-align= "left"
%	 >
%$\Cee$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(116.25,2.5)"
%	 text-frame= "noframe"
%	 stroke-width= "0.4"
%	 text-hor-align= "right"
%	 >
%$\Aee$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(151.25,2.5)"
%	 text-frame= "noframe"
%	 stroke-width= "0.4"
%	 text-hor-align= "right"
%	 >
%$\Bee$
%</text>
%<multicurve fill-style= "none"
%	 points= "(115,160);(115,160);(135,140);(135,140)"
%	 stroke-width= "0.4"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(129.38,179.38)"
%	 text-frame= "noframe"
%	 stroke-width= "0.4"
%	 text-hor-align= "left"
%	 >
%$\Code$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(125,42.5)"
%	 text-frame= "noframe"
%	 stroke-width= "0.4"
%	 text-hor-align= "center-h"
%	 >
%$\Dott$
%</text>
%<multicurve fill-style= "none"
%	 points= "(135,32.5);(135,32.5);(115,32.5);(115,32.5)"
%	 stroke-width= "0.4"
%	 />
%<multicurve fill-style= "none"
%	 points= "(115,52.5);(115,52.5);(135,32.5);(135,32.5)"
%	 stroke-width= "0.4"
%	 />
%<multicurve fill-style= "none"
%	 points= "(125,32.5);(125,32.5);(125,0);(125,0)"
%	 stroke-width= "0.4"
%	 />
%<multicurve fill-style= "none"
%	 points= "(125,42.5);(125,42.5);(125,150);(125,150)"
%	 stroke-width= "1.45"
%	 />
%<multicurve fill-style= "none"
%	 points= "(115,52.5);(115,52.5);(115,32.5);(115,32.5)"
%	 stroke-width= "0.4"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(121.25,37.5)"
%	 text-frame= "noframe"
%	 stroke-width= "0.35"
%	 text-hor-align= "center-h"
%	 >
%$\programm$
%</text>
%<multicurve fill-style= "none"
%	 points= "(125,160);(125,160);(125,180);(125,180)"
%	 stroke-width= "1.45"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(145,150)"
%	 text-frame= "noframe"
%	 stroke-width= "0.4"
%	 text-hor-align= "center-h"
%	 >
%$\Univ$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(26.25,37.5)"
%	 text-frame= "noframe"
%	 stroke-width= "0.35"
%	 text-hor-align= "center-h"
%	 >
%$\programm$
%</text>
%</jpic>
%%End JPIC-XML
%PSTricks content-type (pstricks.sty package needed)
%Add \usepackage{pstricks} in the preamble of your LaTeX file
%You can rescale the whole picture (to 80% for instance) by using the command \def\JPicScale{0.8}
\ifx\JPicScale\undefined\def\JPicScale{1}\fi
\psset{unit=\JPicScale mm}
\psset{linewidth=0.3,dotsep=1,hatchwidth=0.3,hatchsep=1.5,shadowsize=1,dimen=middle}
\psset{dotsize=0.7 2.5,dotscale=1 1,fillcolor=black}
\psset{arrowsize=1 2,arrowlength=1,arrowinset=0.25,tbarsize=0.7 5,bracketlength=0.15,rbracketlength=0.15}
\begin{pspicture}(0,0)(165,180)
\psline[linewidth=0.4](70,160)(70,140)
\psline[linewidth=0.4](35,135)(15,135)
\psline[linewidth=0.4](20,160)(70,160)
\psline[linewidth=0.4](60,140)(60,0)
\psline[linewidth=0.4](60,180)(60,160)
\psline[linewidth=0.4](35,135)(35,115)
\psline[linewidth=0.4](20,145)(20,135)
\psline[linewidth=0.4](70,140)(40,140)
\psline[linewidth=0.4](20,160)(40,140)
\psline[linewidth=0.4](15,135)(35,115)
\psline[linewidth=1.45](30,135)(30,150)
\rput(50,150){$\Univ$}
\rput[l](63.75,178.75){$\Cee$}
\rput[r](55,2.5){$\Bee$}
\rput(20,145){$\Dott$}
\psline[linewidth=1.45](30,160)(30,180)
\psline[linewidth=1.45](25,90)(25,125)
\psline[linewidth=0.2,linecolor=red](11.25,132.5)(35,108.75)
\psline[linewidth=0.2,linecolor=red](35,108.75)(75,108.75)
\psline[linewidth=0.2,linecolor=red](75,108.75)(75,166.25)
\psline[linewidth=0.2,linecolor=red](21.25,166.25)(75,166.25)
\psline[linewidth=0.2,linecolor=red](11.25,156.25)(21.25,166.25)
\psline[linewidth=0.2,linecolor=red](11.25,132.5)(11.25,156.25)
\rput(30,42.5){$\Dott$}
\psline[linewidth=0.4](40,32.5)(20,32.5)
\psline[linewidth=0.4](20,52.5)(40,32.5)
\psline[linewidth=0.4](30,32.5)(30,0)
\rput(20,80){$\Dott$}
\psline[linewidth=0.4](5,95)(35,65)
\psline[linewidth=0.4](5,95)(5,65)
\psline[linewidth=1.45](30,42.5)(30,65)
\psline[linewidth=0.4](35,65)(5,65)
\psline[linewidth=0.4](10,65)(10,35)
\psline[linewidth=0.4](10,35)(30,15)
\rput(30,15){$\Dott$}
\newrgbcolor{userLineColour}{1 0 0.2}
\psline[linewidth=0.2,linecolor=userLineColour](10,100)(45,65)
\newrgbcolor{userLineColour}{1 0 0.2}
\psline[linewidth=0.2,linecolor=userLineColour](45,10)(45,65)
\newrgbcolor{userLineColour}{1 0 0.2}
\psline[linewidth=0.2,linecolor=userLineColour](0,10)(0,100)
\newrgbcolor{userLineColour}{1 0 0.2}
\psline[linewidth=0.2,linecolor=userLineColour](45,10)(0,10)
\rput(13.75,72.5){$\prrrr$}
\rput(27.5,128.75){$\pjjjj$}
\rput(25,121.25){}
\rput[r](17.5,140){$\Aee$}
\rput(48.75,120){$\PadUniv$}
\rput(8.75,18.75){$\PadFee$}
\psline[linewidth=0.4](20,52.5)(20,32.5)
\newrgbcolor{userLineColour}{1 0 0.2}
\psline[linewidth=0.2,linecolor=userLineColour](0,100)(10,100)
\rput[r](26.25,2.5){$\Aee$}
\rput[l](33.75,179.38){$\Code$}
\rput(100,140){\EQLS}
\psline[linewidth=0.4](165,160)(165,140)
\psline[linewidth=0.4](115,160)(165,160)
\psline[linewidth=0.4](155,140)(155,0)
\psline[linewidth=0.4](155,180)(155,160)
\psline[linewidth=0.4](165,140)(135,140)
\rput[l](160,178.75){$\Cee$}
\rput[r](116.25,2.5){$\Aee$}
\rput[r](151.25,2.5){$\Bee$}
\psline[linewidth=0.4](115,160)(135,140)
\rput[l](129.38,179.38){$\Code$}
\rput(125,42.5){$\Dott$}
\psline[linewidth=0.4](135,32.5)(115,32.5)
\psline[linewidth=0.4](115,52.5)(135,32.5)
\psline[linewidth=0.4](125,32.5)(125,0)
\psline[linewidth=1.45](125,42.5)(125,150)
\psline[linewidth=0.4](115,52.5)(115,32.5)
\rput(121.25,37.5){$\programm$}
\psline[linewidth=1.45](125,160)(125,180)
\rput(145,150){$\Univ$}
\rput(26.25,37.5){$\programm$}
\end{pspicture}


==> PIC/losless-1.tex <==
%%Created by jPicEdt 1.4.1_03: mixed JPIC-XML/LaTeX format
%%Sun Jan 22 15:36:21 GMT-10:00 2023
%%Begin JPIC-XML
%<?xml version="1.0" standalone="yes"?>
%<jpic x-min="0" x-max="70" y-min="0" y-max="90" auto-bounding="true">
%<multicurve fill-style= "none"
%	 points= "(30,70);(30,70);(0,70);(0,70)"
%	 stroke-width= "0.4"
%	 />
%<multicurve fill-style= "none"
%	 points= "(30,70);(30,70);(30,40);(30,40)"
%	 stroke-width= "0.4"
%	 />
%<multicurve fill-style= "none"
%	 points= "(5,75);(5,75);(5,70);(5,70)"
%	 stroke-width= "0.4"
%	 />
%<multicurve fill-style= "none"
%	 points= "(0,70);(0,70);(30,40);(30,40)"
%	 stroke-width= "0.4"
%	 />
%<multicurve fill-style= "none"
%	 points= "(25,70);(25,70);(25,80);(25,80)"
%	 stroke-width= "1.45"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(25,80)"
%	 text-frame= "noframe"
%	 stroke-width= "0.4"
%	 text-hor-align= "center-h"
%	 >
%$\Dott$
%</text>
%<multicurve fill-style= "none"
%	 points= "(15,35);(15,35);(15,55);(15,55)"
%	 stroke-width= "1.45"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(15,35)"
%	 text-frame= "noframe"
%	 stroke-width= "0.4"
%	 text-hor-align= "center-h"
%	 >
%$\Dott$
%</text>
%<multicurve fill-style= "none"
%	 points= "(0,50);(0,50);(30,20);(30,20)"
%	 stroke-width= "0.4"
%	 />
%<multicurve fill-style= "none"
%	 points= "(0,50);(0,50);(0,20);(0,20)"
%	 stroke-width= "0.4"
%	 />
%<multicurve fill-style= "none"
%	 points= "(30,20);(30,20);(0,20);(0,20)"
%	 stroke-width= "0.4"
%	 />
%<multicurve fill-style= "none"
%	 points= "(15,20);(15,20);(15,0);(15,0)"
%	 stroke-width= "0.4"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(8.75,27.5)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\prrrr$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(18.12,65)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\pjjjj$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(20,61.25)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(18.75,88.75)"
%	 text-frame= "noframe"
%	 stroke-width= "0.4"
%	 text-hor-align= "left"
%	 >
%$\Aee$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(12.5,1.25)"
%	 text-frame= "noframe"
%	 stroke-width= "0.4"
%	 text-hor-align= "right"
%	 >
%$\Aee$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(50,50)"
%	 text-frame= "noframe"
%	 stroke-width= "0.4"
%	 text-hor-align= "center-h"
%	 >
%\EQLS
%</text>
%<multicurve fill-style= "none"
%	 points= "(70,90);(70,90);(70,0);(70,0)"
%	 stroke-width= "0.4"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(66.25,1.25)"
%	 text-frame= "noframe"
%	 stroke-width= "0.4"
%	 text-hor-align= "right"
%	 >
%$\Aee$
%</text>
%<multicurve fill-style= "none"
%	 points= "(15,85);(15,85);(5,75);(5,75)"
%	 stroke-width= "0.4"
%	 />
%<multicurve fill-style= "none"
%	 points= "(15,90);(15,90);(15,85);(15,85)"
%	 stroke-width= "0.4"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(11.25,47.5)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\Code$
%</text>
%</jpic>
%%End JPIC-XML
%PSTricks content-type (pstricks.sty package needed)
%Add \usepackage{pstricks} in the preamble of your LaTeX file
%You can rescale the whole picture (to 80% for instance) by using the command \def\JPicScale{0.8}
\ifx\JPicScale\undefined\def\JPicScale{1}\fi
\psset{unit=\JPicScale mm}
\psset{linewidth=0.3,dotsep=1,hatchwidth=0.3,hatchsep=1.5,shadowsize=1,dimen=middle}
\psset{dotsize=0.7 2.5,dotscale=1 1,fillcolor=black}
\psset{arrowsize=1 2,arrowlength=1,arrowinset=0.25,tbarsize=0.7 5,bracketlength=0.15,rbracketlength=0.15}
\begin{pspicture}(0,0)(70,90)
\psline[linewidth=0.4](30,70)(0,70)
\psline[linewidth=0.4](30,70)(30,40)
\psline[linewidth=0.4](5,75)(5,70)
\psline[linewidth=0.4](0,70)(30,40)
\psline[linewidth=1.45](25,70)(25,80)
\rput(25,80){$\Dott$}
\psline[linewidth=1.45](15,35)(15,55)
\rput(15,35){$\Dott$}
\psline[linewidth=0.4](0,50)(30,20)
\psline[linewidth=0.4](0,50)(0,20)
\psline[linewidth=0.4](30,20)(0,20)
\psline[linewidth=0.4](15,20)(15,0)
\rput(8.75,27.5){$\prrrr$}
\rput(18.12,65){$\pjjjj$}
\rput(20,61.25){}
\rput[l](18.75,88.75){$\Aee$}
\rput[r](12.5,1.25){$\Aee$}
\rput(50,50){\EQLS}
\psline[linewidth=0.4](70,90)(70,0)
\rput[r](66.25,1.25){$\Aee$}
\psline[linewidth=0.4](15,85)(5,75)
\psline[linewidth=0.4](15,90)(15,85)
\rput[r](11.25,47.5){$\Code$}
\end{pspicture}


==> PIC/losless-11.tex <==
%%Created by jPicEdt 1.4.1_03: mixed JPIC-XML/LaTeX format
%%Sun Jan 22 15:34:13 GMT-10:00 2023
%%Begin JPIC-XML
%<?xml version="1.0" standalone="yes"?>
%<jpic x-min="-5" x-max="185" y-min="-0" y-max="190" auto-bounding="true">
%<multicurve fill-style= "none"
%	 points= "(65,100);(65,100);(65,80);(65,80)"
%	 stroke-width= "0.4"
%	 />
%<multicurve fill-style= "none"
%	 points= "(30,75);(30,75);(0,75);(0,75)"
%	 stroke-width= "0.4"
%	 />
%<multicurve fill-style= "none"
%	 points= "(15,100);(15,100);(65,100);(65,100)"
%	 stroke-width= "0.4"
%	 />
%<multicurve fill-style= "none"
%	 points= "(55,80);(55,80);(55,-0);(55,-0)"
%	 stroke-width= "0.4"
%	 />
%<multicurve fill-style= "none"
%	 points= "(55,190);(55,190);(55,100);(55,100)"
%	 stroke-width= "0.4"
%	 />
%<multicurve fill-style= "none"
%	 points= "(30,75);(30,75);(30,45);(30,45)"
%	 stroke-width= "0.4"
%	 />
%<multicurve fill-style= "none"
%	 points= "(5,85);(5,85);(5,75);(5,75)"
%	 stroke-width= "0.4"
%	 />
%<multicurve fill-style= "none"
%	 points= "(65,80);(65,80);(35,80);(35,80)"
%	 stroke-width= "0.4"
%	 />
%<multicurve fill-style= "none"
%	 points= "(15,100);(15,100);(35,80);(35,80)"
%	 stroke-width= "0.4"
%	 />
%<multicurve fill-style= "none"
%	 points= "(0,75);(0,75);(30,45);(30,45)"
%	 stroke-width= "0.4"
%	 />
%<multicurve fill-style= "none"
%	 points= "(25,75);(25,75);(25,90);(25,90)"
%	 stroke-width= "1.45"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(45,90)"
%	 text-frame= "noframe"
%	 stroke-width= "0.4"
%	 text-hor-align= "center-h"
%	 >
%$\Univ$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(58.75,188.75)"
%	 text-frame= "noframe"
%	 stroke-width= "0.4"
%	 text-hor-align= "left"
%	 >
%$\Cee$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(52.5,1.25)"
%	 text-frame= "noframe"
%	 stroke-width= "0.4"
%	 text-hor-align= "right"
%	 >
%$\Bee$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(5,85)"
%	 text-frame= "noframe"
%	 stroke-width= "0.4"
%	 text-hor-align= "center-h"
%	 >
%$\Dott$
%</text>
%<multicurve fill-style= "none"
%	 points= "(25,100);(25,100);(25,120);(25,120)"
%	 stroke-width= "1.45"
%	 />
%<multicurve fill-style= "none"
%	 points= "(15,35);(15,35);(15,60);(15,60)"
%	 stroke-width= "1.45"
%	 />
%<multicurve fill-style= "none"
%	 points= "(-5,70);(-5,70);(25,40);(25,40)"
%	 stroke-color= "#ff0000"
%	 stroke-width= "0.2"
%	 />
%<multicurve fill-style= "none"
%	 points= "(25,40);(25,40);(70,40);(70,40)"
%	 stroke-color= "#ff0000"
%	 stroke-width= "0.2"
%	 />
%<multicurve fill-style= "none"
%	 points= "(70,40);(70,40);(70,106.25);(70,106.25)"
%	 stroke-color= "#ff0000"
%	 stroke-width= "0.2"
%	 />
%<multicurve fill-style= "none"
%	 points= "(15,106.25);(15,106.25);(70,106.25);(70,106.25)"
%	 stroke-color= "#ff0000"
%	 stroke-width= "0.2"
%	 />
%<multicurve fill-style= "none"
%	 points= "(-5,86.25);(-5,86.25);(15,106.25);(15,106.25)"
%	 stroke-color= "#ff0000"
%	 stroke-width= "0.2"
%	 />
%<multicurve fill-style= "none"
%	 points= "(-5,70);(-5,70);(-5,86.25);(-5,86.25)"
%	 stroke-color= "#ff0000"
%	 stroke-width= "0.2"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(15,35)"
%	 text-frame= "noframe"
%	 stroke-width= "0.4"
%	 text-hor-align= "center-h"
%	 >
%$\Dott$
%</text>
%<multicurve fill-style= "none"
%	 points= "(0,50);(0,50);(30,20);(30,20)"
%	 stroke-width= "0.4"
%	 />
%<multicurve fill-style= "none"
%	 points= "(0,50);(0,50);(0,20);(0,20)"
%	 stroke-width= "0.4"
%	 />
%<multicurve fill-style= "none"
%	 points= "(30,20);(30,20);(0,20);(0,20)"
%	 stroke-width= "0.4"
%	 />
%<multicurve fill-style= "none"
%	 points= "(15,20);(15,20);(15,0);(15,0)"
%	 stroke-width= "0.4"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(8.75,27.5)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\prrrr$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(18.12,70)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\pjjjj$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(20,66.25)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(7.5,80)"
%	 text-frame= "noframe"
%	 stroke-width= "0.4"
%	 text-hor-align= "left"
%	 >
%$\Aee$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(43.75,60)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\PadUniv$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(12.5,1.25)"
%	 text-frame= "noframe"
%	 stroke-width= "0.4"
%	 text-hor-align= "right"
%	 >
%$\Aee$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(22.5,112.5)"
%	 text-frame= "noframe"
%	 stroke-width= "0.4"
%	 text-hor-align= "right"
%	 >
%$\Code$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(90,80)"
%	 text-frame= "noframe"
%	 stroke-width= "0.4"
%	 text-hor-align= "center-h"
%	 >
%\EQLS
%</text>
%<multicurve fill-style= "none"
%	 points= "(180,100);(180,100);(180,80);(180,80)"
%	 stroke-width= "0.4"
%	 />
%<multicurve fill-style= "none"
%	 points= "(145,75);(145,75);(115,75);(115,75)"
%	 stroke-width= "0.4"
%	 />
%<multicurve fill-style= "none"
%	 points= "(130,100);(130,100);(180,100);(180,100)"
%	 stroke-width= "0.4"
%	 />
%<multicurve fill-style= "none"
%	 points= "(170,80);(170,80);(170,-0);(170,-0)"
%	 stroke-width= "0.4"
%	 />
%<multicurve fill-style= "none"
%	 points= "(170,190);(170,190);(170,100);(170,100)"
%	 stroke-width= "0.4"
%	 />
%<multicurve fill-style= "none"
%	 points= "(145,75);(145,75);(145,45);(145,45)"
%	 stroke-width= "0.4"
%	 />
%<multicurve fill-style= "none"
%	 points= "(120,85);(120,85);(120,75);(120,75)"
%	 stroke-width= "0.4"
%	 />
%<multicurve fill-style= "none"
%	 points= "(180,80);(180,80);(150,80);(150,80)"
%	 stroke-width= "0.4"
%	 />
%<multicurve fill-style= "none"
%	 points= "(130,100);(130,100);(150,80);(150,80)"
%	 stroke-width= "0.4"
%	 />
%<multicurve fill-style= "none"
%	 points= "(115,75);(115,75);(145,45);(145,45)"
%	 stroke-width= "0.4"
%	 />
%<multicurve fill-style= "none"
%	 points= "(140,75);(140,75);(140,90);(140,90)"
%	 stroke-width= "1.45"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(160,90)"
%	 text-frame= "noframe"
%	 stroke-width= "0.4"
%	 text-hor-align= "center-h"
%	 >
%$\Univ$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(173.75,188.75)"
%	 text-frame= "noframe"
%	 stroke-width= "0.4"
%	 text-hor-align= "left"
%	 >
%$\Cee$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(168.75,1.25)"
%	 text-frame= "noframe"
%	 stroke-width= "0.4"
%	 text-hor-align= "right"
%	 >
%$\Bee$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(120,85)"
%	 text-frame= "noframe"
%	 stroke-width= "0.4"
%	 text-hor-align= "center-h"
%	 >
%$\Dott$
%</text>
%<multicurve fill-style= "none"
%	 points= "(140,100);(140,100);(140,190);(140,190)"
%	 stroke-width= "1.45"
%	 />
%<multicurve fill-style= "none"
%	 points= "(130,35);(130,35);(130,60);(130,60)"
%	 stroke-width= "1.45"
%	 />
%<multicurve fill-style= "none"
%	 points= "(110,70);(110,70);(140,40);(140,40)"
%	 stroke-color= "#ff0000"
%	 stroke-width= "0.2"
%	 />
%<multicurve fill-style= "none"
%	 points= "(140,40);(140,40);(185,40);(185,40)"
%	 stroke-color= "#ff0000"
%	 stroke-width= "0.2"
%	 />
%<multicurve fill-style= "none"
%	 points= "(185,40);(185,40);(185,106.25);(185,106.25)"
%	 stroke-color= "#ff0000"
%	 stroke-width= "0.2"
%	 />
%<multicurve fill-style= "none"
%	 points= "(130,106.25);(130,106.25);(185,106.25);(185,106.25)"
%	 stroke-color= "#ff0000"
%	 stroke-width= "0.2"
%	 />
%<multicurve fill-style= "none"
%	 points= "(110,86.25);(110,86.25);(130,106.25);(130,106.25)"
%	 stroke-color= "#ff0000"
%	 stroke-width= "0.2"
%	 />
%<multicurve fill-style= "none"
%	 points= "(110,70);(110,70);(110,86.25);(110,86.25)"
%	 stroke-color= "#ff0000"
%	 stroke-width= "0.2"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(130,35)"
%	 text-frame= "noframe"
%	 stroke-width= "0.4"
%	 text-hor-align= "center-h"
%	 >
%$\Dott$
%</text>
%<multicurve fill-style= "none"
%	 points= "(115,50);(115,50);(145,20);(145,20)"
%	 stroke-width= "0.4"
%	 />
%<multicurve fill-style= "none"
%	 points= "(115,50);(115,50);(115,20);(115,20)"
%	 stroke-width= "0.4"
%	 />
%<multicurve fill-style= "none"
%	 points= "(145,20);(145,20);(115,20);(115,20)"
%	 stroke-width= "0.4"
%	 />
%<multicurve fill-style= "none"
%	 points= "(130,20);(130,20);(130,0);(130,0)"
%	 stroke-width= "0.4"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(123.75,27.5)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\prrrr$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(133.12,70)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\pjjjj$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(135,66.25)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(123.75,80)"
%	 text-frame= "noframe"
%	 stroke-width= "0.4"
%	 text-hor-align= "left"
%	 >
%$\Aee$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(158.75,60)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\PadUniv$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(128.75,1.25)"
%	 text-frame= "noframe"
%	 stroke-width= "0.4"
%	 text-hor-align= "right"
%	 >
%$\Aee$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(143.75,189.38)"
%	 text-frame= "noframe"
%	 stroke-width= "0.4"
%	 text-hor-align= "left"
%	 >
%$\Code$
%</text>
%<multicurve fill-style= "none"
%	 points= "(40,135);(40,135);(10,135);(10,135)"
%	 stroke-width= "0.4"
%	 />
%<multicurve fill-style= "none"
%	 points= "(40,135);(40,135);(40,105);(40,105)"
%	 stroke-width= "0.4"
%	 />
%<multicurve fill-style= "none"
%	 points= "(15,140);(15,140);(15,135);(15,135)"
%	 stroke-width= "0.4"
%	 />
%<multicurve fill-style= "none"
%	 points= "(10,135);(10,135);(40,105);(40,105)"
%	 stroke-width= "0.4"
%	 />
%<multicurve fill-style= "none"
%	 points= "(35,135);(35,135);(35,145);(35,145)"
%	 stroke-width= "1.45"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(35,145)"
%	 text-frame= "noframe"
%	 stroke-width= "0.4"
%	 text-hor-align= "center-h"
%	 >
%$\Dott$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(28.12,130)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\pjjjj$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(30,126.25)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%
%</text>
%<multicurve fill-style= "none"
%	 points= "(25,150);(25,150);(15,140);(15,140)"
%	 stroke-width= "0.4"
%	 />
%<multicurve fill-style= "none"
%	 points= "(25,155);(25,155);(25,150);(25,150)"
%	 stroke-width= "0.4"
%	 />
%<multicurve fill-style= "none"
%	 points= "(25,170);(25,170);(25,190);(25,190)"
%	 stroke-width= "1.45"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(25,170)"
%	 text-frame= "noframe"
%	 stroke-width= "0.4"
%	 text-hor-align= "center-h"
%	 >
%$\Dott$
%</text>
%<multicurve fill-style= "none"
%	 points= "(10,185);(10,185);(40,155);(40,155)"
%	 stroke-width= "0.4"
%	 />
%<multicurve fill-style= "none"
%	 points= "(10,185);(10,185);(10,155);(10,155)"
%	 stroke-width= "0.4"
%	 />
%<multicurve fill-style= "none"
%	 points= "(40,155);(40,155);(10,155);(10,155)"
%	 stroke-width= "0.4"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(18.75,162.5)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\prrrr$
%</text>
%<text text-vert-align= "bottom"
%	 fill-style= "none"
%	 anchor-point= "(18.75,146.25)"
%	 text-frame= "noframe"
%	 stroke-width= "0.4"
%	 text-hor-align= "right"
%	 >
%$\Aee$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(28.75,188.75)"
%	 text-frame= "noframe"
%	 stroke-width= "0.4"
%	 text-hor-align= "left"
%	 >
%$\Code$
%</text>
%</jpic>
%%End JPIC-XML
%PSTricks content-type (pstricks.sty package needed)
%Add \usepackage{pstricks} in the preamble of your LaTeX file
%You can rescale the whole picture (to 80% for instance) by using the command \def\JPicScale{0.8}
\ifx\JPicScale\undefined\def\JPicScale{1}\fi
\psset{unit=\JPicScale mm}
\psset{linewidth=0.3,dotsep=1,hatchwidth=0.3,hatchsep=1.5,shadowsize=1,dimen=middle}
\psset{dotsize=0.7 2.5,dotscale=1 1,fillcolor=black}
\psset{arrowsize=1 2,arrowlength=1,arrowinset=0.25,tbarsize=0.7 5,bracketlength=0.15,rbracketlength=0.15}
\begin{pspicture}(0,0)(185,190)
\psline[linewidth=0.4](65,100)(65,80)
\psline[linewidth=0.4](30,75)(0,75)
\psline[linewidth=0.4](15,100)(65,100)
\psline[linewidth=0.4](55,80)(55,-0)
\psline[linewidth=0.4](55,190)(55,100)
\psline[linewidth=0.4](30,75)(30,45)
\psline[linewidth=0.4](5,85)(5,75)
\psline[linewidth=0.4](65,80)(35,80)
\psline[linewidth=0.4](15,100)(35,80)
\psline[linewidth=0.4](0,75)(30,45)
\psline[linewidth=1.45](25,75)(25,90)
\rput(45,90){$\Univ$}
\rput[l](58.75,188.75){$\Cee$}
\rput[r](52.5,1.25){$\Bee$}
\rput(5,85){$\Dott$}
\psline[linewidth=1.45](25,100)(25,120)
\psline[linewidth=1.45](15,35)(15,60)
\psline[linewidth=0.2,linecolor=red](-5,70)(25,40)
\psline[linewidth=0.2,linecolor=red](25,40)(70,40)
\psline[linewidth=0.2,linecolor=red](70,40)(70,106.25)
\psline[linewidth=0.2,linecolor=red](15,106.25)(70,106.25)
\psline[linewidth=0.2,linecolor=red](-5,86.25)(15,106.25)
\psline[linewidth=0.2,linecolor=red](-5,70)(-5,86.25)
\rput(15,35){$\Dott$}
\psline[linewidth=0.4](0,50)(30,20)
\psline[linewidth=0.4](0,50)(0,20)
\psline[linewidth=0.4](30,20)(0,20)
\psline[linewidth=0.4](15,20)(15,0)
\rput(8.75,27.5){$\prrrr$}
\rput(18.12,70){$\pjjjj$}
\rput(20,66.25){}
\rput[l](7.5,80){$\Aee$}
\rput(43.75,60){$\PadUniv$}
\rput[r](12.5,1.25){$\Aee$}
\rput[r](22.5,112.5){$\Code$}
\rput(90,80){\EQLS}
\psline[linewidth=0.4](180,100)(180,80)
\psline[linewidth=0.4](145,75)(115,75)
\psline[linewidth=0.4](130,100)(180,100)
\psline[linewidth=0.4](170,80)(170,-0)
\psline[linewidth=0.4](170,190)(170,100)
\psline[linewidth=0.4](145,75)(145,45)
\psline[linewidth=0.4](120,85)(120,75)
\psline[linewidth=0.4](180,80)(150,80)
\psline[linewidth=0.4](130,100)(150,80)
\psline[linewidth=0.4](115,75)(145,45)
\psline[linewidth=1.45](140,75)(140,90)
\rput(160,90){$\Univ$}
\rput[l](173.75,188.75){$\Cee$}
\rput[r](168.75,1.25){$\Bee$}
\rput(120,85){$\Dott$}
\psline[linewidth=1.45](140,100)(140,190)
\psline[linewidth=1.45](130,35)(130,60)
\psline[linewidth=0.2,linecolor=red](110,70)(140,40)
\psline[linewidth=0.2,linecolor=red](140,40)(185,40)
\psline[linewidth=0.2,linecolor=red](185,40)(185,106.25)
\psline[linewidth=0.2,linecolor=red](130,106.25)(185,106.25)
\psline[linewidth=0.2,linecolor=red](110,86.25)(130,106.25)
\psline[linewidth=0.2,linecolor=red](110,70)(110,86.25)
\rput(130,35){$\Dott$}
\psline[linewidth=0.4](115,50)(145,20)
\psline[linewidth=0.4](115,50)(115,20)
\psline[linewidth=0.4](145,20)(115,20)
\psline[linewidth=0.4](130,20)(130,0)
\rput(123.75,27.5){$\prrrr$}
\rput(133.12,70){$\pjjjj$}
\rput(135,66.25){}
\rput[l](123.75,80){$\Aee$}
\rput(158.75,60){$\PadUniv$}
\rput[r](128.75,1.25){$\Aee$}
\rput[l](143.75,189.38){$\Code$}
\psline[linewidth=0.4](40,135)(10,135)
\psline[linewidth=0.4](40,135)(40,105)
\psline[linewidth=0.4](15,140)(15,135)
\psline[linewidth=0.4](10,135)(40,105)
\psline[linewidth=1.45](35,135)(35,145)
\rput(35,145){$\Dott$}
\rput(28.12,130){$\pjjjj$}
\rput(30,126.25){}
\psline[linewidth=0.4](25,150)(15,140)
\psline[linewidth=0.4](25,155)(25,150)
\psline[linewidth=1.45](25,170)(25,190)
\rput(25,170){$\Dott$}
\psline[linewidth=0.4](10,185)(40,155)
\psline[linewidth=0.4](10,185)(10,155)
\psline[linewidth=0.4](40,155)(10,155)
\rput(18.75,162.5){$\prrrr$}
\rput[br](18.75,146.25){$\Aee$}
\rput[l](28.75,188.75){$\Code$}
\end{pspicture}


==> PIC/losless-2.tex <==
%%Created by jPicEdt 1.4.1_03: mixed JPIC-XML/LaTeX format
%%Sat Jan 21 19:44:22 GMT-10:00 2023
%%Begin JPIC-XML
%<?xml version="1.0" standalone="yes"?>
%<jpic x-min="0" x-max="165" y-min="0" y-max="180" auto-bounding="true">
%<multicurve fill-style= "none"
%	 points= "(70,160);(70,160);(70,140);(70,140)"
%	 stroke-width= "0.4"
%	 />
%<multicurve fill-style= "none"
%	 points= "(35,130);(35,130);(5,130);(5,130)"
%	 stroke-width= "0.4"
%	 />
%<multicurve fill-style= "none"
%	 points= "(20,160);(20,160);(70,160);(70,160)"
%	 stroke-width= "0.4"
%	 />
%<multicurve fill-style= "none"
%	 points= "(60,140);(60,140);(60,0);(60,0)"
%	 stroke-width= "0.4"
%	 />
%<multicurve fill-style= "none"
%	 points= "(60,180);(60,180);(60,160);(60,160)"
%	 stroke-width= "0.4"
%	 />
%<multicurve fill-style= "none"
%	 points= "(35,130);(35,130);(35,100);(35,100)"
%	 stroke-width= "0.4"
%	 />
%<multicurve fill-style= "none"
%	 points= "(10,140);(10,140);(10,130);(10,130)"
%	 stroke-width= "0.4"
%	 />
%<multicurve fill-style= "none"
%	 points= "(70,140);(70,140);(40,140);(40,140)"
%	 stroke-width= "0.4"
%	 />
%<multicurve fill-style= "none"
%	 points= "(20,160);(20,160);(40,140);(40,140)"
%	 stroke-width= "0.4"
%	 />
%<multicurve fill-style= "none"
%	 points= "(5,130);(5,130);(35,100);(35,100)"
%	 stroke-width= "0.4"
%	 />
%<multicurve fill-style= "none"
%	 points= "(30,130);(30,130);(30,150);(30,150)"
%	 stroke-width= "1.45"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(50,150)"
%	 text-frame= "noframe"
%	 stroke-width= "0.4"
%	 text-hor-align= "center-h"
%	 >
%$\Univ$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(63.75,178.75)"
%	 text-frame= "noframe"
%	 stroke-width= "0.4"
%	 text-hor-align= "left"
%	 >
%$\Cee$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(55,2.5)"
%	 text-frame= "noframe"
%	 stroke-width= "0.4"
%	 text-hor-align= "right"
%	 >
%$\Bee$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(10,140)"
%	 text-frame= "noframe"
%	 stroke-width= "0.4"
%	 text-hor-align= "center-h"
%	 >
%$\Dott$
%</text>
%<multicurve fill-style= "none"
%	 points= "(30,160);(30,160);(30,180);(30,180)"
%	 stroke-width= "1.45"
%	 />
%<multicurve fill-style= "none"
%	 points= "(20,80);(20,80);(20,115);(20,115)"
%	 stroke-width= "1.45"
%	 />
%<multicurve fill-style= "none"
%	 points= "(0,125);(0,125);(30,95);(30,95)"
%	 stroke-color= "#ff0000"
%	 stroke-width= "0.2"
%	 />
%<multicurve fill-style= "none"
%	 points= "(30,95);(30,95);(75,95);(75,95)"
%	 stroke-color= "#ff0000"
%	 stroke-width= "0.2"
%	 />
%<multicurve fill-style= "none"
%	 points= "(75,95);(75,95);(75,166.25);(75,166.25)"
%	 stroke-color= "#ff0000"
%	 stroke-width= "0.2"
%	 />
%<multicurve fill-style= "none"
%	 points= "(20,166.25);(20,166.25);(75,166.25);(75,166.25)"
%	 stroke-color= "#ff0000"
%	 stroke-width= "0.2"
%	 />
%<multicurve fill-style= "none"
%	 points= "(0,146.25);(0,146.25);(20,166.25);(20,166.25)"
%	 stroke-color= "#ff0000"
%	 stroke-width= "0.2"
%	 />
%<multicurve fill-style= "none"
%	 points= "(0,125);(0,125);(0,146.25);(0,146.25)"
%	 stroke-color= "#ff0000"
%	 stroke-width= "0.2"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(30,42.5)"
%	 text-frame= "noframe"
%	 stroke-width= "0.4"
%	 text-hor-align= "center-h"
%	 >
%$\Dott$
%</text>
%<multicurve fill-style= "none"
%	 points= "(40,32.5);(40,32.5);(20,32.5);(20,32.5)"
%	 stroke-width= "0.4"
%	 />
%<multicurve fill-style= "none"
%	 points= "(20,52.5);(20,52.5);(40,32.5);(40,32.5)"
%	 stroke-width= "0.4"
%	 />
%<multicurve fill-style= "none"
%	 points= "(30,32.5);(30,32.5);(30,0);(30,0)"
%	 stroke-width= "0.4"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(20,80)"
%	 text-frame= "noframe"
%	 stroke-width= "0.4"
%	 text-hor-align= "center-h"
%	 >
%$\Dott$
%</text>
%<multicurve fill-style= "none"
%	 points= "(5,95);(5,95);(35,65);(35,65)"
%	 stroke-width= "0.4"
%	 />
%<multicurve fill-style= "none"
%	 points= "(5,95);(5,95);(5,65);(5,65)"
%	 stroke-width= "0.4"
%	 />
%<multicurve fill-style= "none"
%	 points= "(30,42.5);(30,42.5);(30,65);(30,65)"
%	 stroke-width= "1.45"
%	 />
%<multicurve fill-style= "none"
%	 points= "(35,65);(35,65);(5,65);(5,65)"
%	 stroke-width= "0.4"
%	 />
%<multicurve fill-style= "none"
%	 points= "(10,65);(10,65);(10,35);(10,35)"
%	 stroke-width= "0.4"
%	 />
%<multicurve fill-style= "none"
%	 points= "(10,35);(10,35);(30,15);(30,15)"
%	 stroke-width= "0.4"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(30,15)"
%	 text-frame= "noframe"
%	 stroke-width= "0.4"
%	 text-hor-align= "center-h"
%	 >
%$\Dott$
%</text>
%<multicurve fill-style= "none"
%	 points= "(10,100);(10,100);(45,65);(45,65)"
%	 stroke-color= "#ff0033"
%	 stroke-width= "0.2"
%	 />
%<multicurve fill-style= "none"
%	 points= "(45,10);(45,10);(45,65);(45,65)"
%	 stroke-color= "#ff0033"
%	 stroke-width= "0.2"
%	 />
%<multicurve fill-style= "none"
%	 points= "(0,10);(0,10);(0,100);(0,100)"
%	 stroke-color= "#ff0033"
%	 stroke-width= "0.2"
%	 />
%<multicurve fill-style= "none"
%	 points= "(45,10);(45,10);(0,10);(0,10)"
%	 stroke-color= "#ff0033"
%	 stroke-width= "0.2"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(13.75,72.5)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\prrrr$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(23.12,125)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\pjjjj$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(25,121.25)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(13.75,135)"
%	 text-frame= "noframe"
%	 stroke-width= "0.4"
%	 text-hor-align= "left"
%	 >
%$\Aee$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(48.75,120)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\PadUniv$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(8.75,18.75)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\PadFee$
%</text>
%<multicurve fill-style= "none"
%	 points= "(20,52.5);(20,52.5);(20,32.5);(20,32.5)"
%	 stroke-width= "0.4"
%	 />
%<multicurve fill-style= "none"
%	 points= "(0,100);(0,100);(10,100);(10,100)"
%	 stroke-color= "#ff0033"
%	 stroke-width= "0.2"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(26.25,2.5)"
%	 text-frame= "noframe"
%	 stroke-width= "0.4"
%	 text-hor-align= "right"
%	 >
%$\Aee$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(33.75,179.38)"
%	 text-frame= "noframe"
%	 stroke-width= "0.4"
%	 text-hor-align= "left"
%	 >
%$\Code$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(100,140)"
%	 text-frame= "noframe"
%	 stroke-width= "0.4"
%	 text-hor-align= "center-h"
%	 >
%\EQLS
%</text>
%<multicurve fill-style= "none"
%	 points= "(165,160);(165,160);(165,140);(165,140)"
%	 stroke-width= "0.4"
%	 />
%<multicurve fill-style= "none"
%	 points= "(115,160);(115,160);(165,160);(165,160)"
%	 stroke-width= "0.4"
%	 />
%<multicurve fill-style= "none"
%	 points= "(155,140);(155,140);(155,0);(155,0)"
%	 stroke-width= "0.4"
%	 />
%<multicurve fill-style= "none"
%	 points= "(155,180);(155,180);(155,160);(155,160)"
%	 stroke-width= "0.4"
%	 />
%<multicurve fill-style= "none"
%	 points= "(165,140);(165,140);(135,140);(135,140)"
%	 stroke-width= "0.4"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(160,178.75)"
%	 text-frame= "noframe"
%	 stroke-width= "0.4"
%	 text-hor-align= "left"
%	 >
%$\Cee$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(116.25,2.5)"
%	 text-frame= "noframe"
%	 stroke-width= "0.4"
%	 text-hor-align= "right"
%	 >
%$\Aee$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(151.25,2.5)"
%	 text-frame= "noframe"
%	 stroke-width= "0.4"
%	 text-hor-align= "right"
%	 >
%$\Bee$
%</text>
%<multicurve fill-style= "none"
%	 points= "(115,160);(115,160);(135,140);(135,140)"
%	 stroke-width= "0.4"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(129.38,179.38)"
%	 text-frame= "noframe"
%	 stroke-width= "0.4"
%	 text-hor-align= "left"
%	 >
%$\Code$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(125,42.5)"
%	 text-frame= "noframe"
%	 stroke-width= "0.4"
%	 text-hor-align= "center-h"
%	 >
%$\Dott$
%</text>
%<multicurve fill-style= "none"
%	 points= "(135,32.5);(135,32.5);(115,32.5);(115,32.5)"
%	 stroke-width= "0.4"
%	 />
%<multicurve fill-style= "none"
%	 points= "(115,52.5);(115,52.5);(135,32.5);(135,32.5)"
%	 stroke-width= "0.4"
%	 />
%<multicurve fill-style= "none"
%	 points= "(125,32.5);(125,32.5);(125,0);(125,0)"
%	 stroke-width= "0.4"
%	 />
%<multicurve fill-style= "none"
%	 points= "(125,42.5);(125,42.5);(125,150);(125,150)"
%	 stroke-width= "1.45"
%	 />
%<multicurve fill-style= "none"
%	 points= "(115,52.5);(115,52.5);(115,32.5);(115,32.5)"
%	 stroke-width= "0.4"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(121.25,37.5)"
%	 text-frame= "noframe"
%	 stroke-width= "0.35"
%	 text-hor-align= "center-h"
%	 >
%$\programm$
%</text>
%<multicurve fill-style= "none"
%	 points= "(125,160);(125,160);(125,180);(125,180)"
%	 stroke-width= "1.45"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(145,150)"
%	 text-frame= "noframe"
%	 stroke-width= "0.4"
%	 text-hor-align= "center-h"
%	 >
%$\Univ$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(26.25,37.5)"
%	 text-frame= "noframe"
%	 stroke-width= "0.35"
%	 text-hor-align= "center-h"
%	 >
%$\programm$
%</text>
%</jpic>
%%End JPIC-XML
%PSTricks content-type (pstricks.sty package needed)
%Add \usepackage{pstricks} in the preamble of your LaTeX file
%You can rescale the whole picture (to 80% for instance) by using the command \def\JPicScale{0.8}
\ifx\JPicScale\undefined\def\JPicScale{1}\fi
\psset{unit=\JPicScale mm}
\psset{linewidth=0.3,dotsep=1,hatchwidth=0.3,hatchsep=1.5,shadowsize=1,dimen=middle}
\psset{dotsize=0.7 2.5,dotscale=1 1,fillcolor=black}
\psset{arrowsize=1 2,arrowlength=1,arrowinset=0.25,tbarsize=0.7 5,bracketlength=0.15,rbracketlength=0.15}
\begin{pspicture}(0,0)(165,180)
\psline[linewidth=0.4](70,160)(70,140)
\psline[linewidth=0.4](35,130)(5,130)
\psline[linewidth=0.4](20,160)(70,160)
\psline[linewidth=0.4](60,140)(60,0)
\psline[linewidth=0.4](60,180)(60,160)
\psline[linewidth=0.4](35,130)(35,100)
\psline[linewidth=0.4](10,140)(10,130)
\psline[linewidth=0.4](70,140)(40,140)
\psline[linewidth=0.4](20,160)(40,140)
\psline[linewidth=0.4](5,130)(35,100)
\psline[linewidth=1.45](30,130)(30,150)
\rput(50,150){$\Univ$}
\rput[l](63.75,178.75){$\Cee$}
\rput[r](55,2.5){$\Bee$}
\rput(10,140){$\Dott$}
\psline[linewidth=1.45](30,160)(30,180)
\psline[linewidth=1.45](20,80)(20,115)
\psline[linewidth=0.2,linecolor=red](0,125)(30,95)
\psline[linewidth=0.2,linecolor=red](30,95)(75,95)
\psline[linewidth=0.2,linecolor=red](75,95)(75,166.25)
\psline[linewidth=0.2,linecolor=red](20,166.25)(75,166.25)
\psline[linewidth=0.2,linecolor=red](0,146.25)(20,166.25)
\psline[linewidth=0.2,linecolor=red](0,125)(0,146.25)
\rput(30,42.5){$\Dott$}
\psline[linewidth=0.4](40,32.5)(20,32.5)
\psline[linewidth=0.4](20,52.5)(40,32.5)
\psline[linewidth=0.4](30,32.5)(30,0)
\rput(20,80){$\Dott$}
\psline[linewidth=0.4](5,95)(35,65)
\psline[linewidth=0.4](5,95)(5,65)
\psline[linewidth=1.45](30,42.5)(30,65)
\psline[linewidth=0.4](35,65)(5,65)
\psline[linewidth=0.4](10,65)(10,35)
\psline[linewidth=0.4](10,35)(30,15)
\rput(30,15){$\Dott$}
\newrgbcolor{userLineColour}{1 0 0.2}
\psline[linewidth=0.2,linecolor=userLineColour](10,100)(45,65)
\newrgbcolor{userLineColour}{1 0 0.2}
\psline[linewidth=0.2,linecolor=userLineColour](45,10)(45,65)
\newrgbcolor{userLineColour}{1 0 0.2}
\psline[linewidth=0.2,linecolor=userLineColour](0,10)(0,100)
\newrgbcolor{userLineColour}{1 0 0.2}
\psline[linewidth=0.2,linecolor=userLineColour](45,10)(0,10)
\rput(13.75,72.5){$\prrrr$}
\rput(23.12,125){$\pjjjj$}
\rput(25,121.25){}
\rput[l](13.75,135){$\Aee$}
\rput(48.75,120){$\PadUniv$}
\rput(8.75,18.75){$\PadFee$}
\psline[linewidth=0.4](20,52.5)(20,32.5)
\newrgbcolor{userLineColour}{1 0 0.2}
\psline[linewidth=0.2,linecolor=userLineColour](0,100)(10,100)
\rput[r](26.25,2.5){$\Aee$}
\rput[l](33.75,179.38){$\Code$}
\rput(100,140){\EQLS}
\psline[linewidth=0.4](165,160)(165,140)
\psline[linewidth=0.4](115,160)(165,160)
\psline[linewidth=0.4](155,140)(155,0)
\psline[linewidth=0.4](155,180)(155,160)
\psline[linewidth=0.4](165,140)(135,140)
\rput[l](160,178.75){$\Cee$}
\rput[r](116.25,2.5){$\Aee$}
\rput[r](151.25,2.5){$\Bee$}
\psline[linewidth=0.4](115,160)(135,140)
\rput[l](129.38,179.38){$\Code$}
\rput(125,42.5){$\Dott$}
\psline[linewidth=0.4](135,32.5)(115,32.5)
\psline[linewidth=0.4](115,52.5)(135,32.5)
\psline[linewidth=0.4](125,32.5)(125,0)
\psline[linewidth=1.45](125,42.5)(125,150)
\psline[linewidth=0.4](115,52.5)(115,32.5)
\rput(121.25,37.5){$\programm$}
\psline[linewidth=1.45](125,160)(125,180)
\rput(145,150){$\Univ$}
\rput(26.25,37.5){$\programm$}
\end{pspicture}


==> PIC/losless-feed.tex <==
%%Created by jPicEdt 1.4.1_03: mixed JPIC-XML/LaTeX format
%%Mon Jan 09 21:03:45 GMT-10:00 2023
%%Begin JPIC-XML
%<?xml version="1.0" standalone="yes"?>
%<jpic x-min="6.25" x-max="300" y-min="0" y-max="255" auto-bounding="true">
%<multicurve fill-style= "none"
%	 points= "(295,160);(295,160);(295,140);(295,140)"
%	 stroke-width= "0.4"
%	 />
%<multicurve fill-style= "none"
%	 points= "(260,130);(260,130);(230,130);(230,130)"
%	 stroke-width= "0.4"
%	 />
%<multicurve fill-style= "none"
%	 points= "(245,160);(245,160);(295,160);(295,160)"
%	 stroke-width= "0.4"
%	 />
%<multicurve fill-style= "none"
%	 points= "(285,140);(285,140);(285,0);(285,0)"
%	 stroke-width= "0.4"
%	 />
%<multicurve fill-style= "none"
%	 points= "(285,255);(285,255);(285,160);(285,160)"
%	 stroke-width= "0.4"
%	 />
%<multicurve fill-style= "none"
%	 points= "(260,130);(260,130);(260,100);(260,100)"
%	 stroke-width= "0.4"
%	 />
%<multicurve fill-style= "none"
%	 points= "(235,170);(235,170);(235,130);(235,130)"
%	 stroke-width= "0.4"
%	 />
%<multicurve fill-style= "none"
%	 points= "(295,140);(295,140);(265,140);(265,140)"
%	 stroke-width= "0.4"
%	 />
%<multicurve fill-style= "none"
%	 points= "(245,160);(245,160);(265,140);(265,140)"
%	 stroke-width= "0.4"
%	 />
%<multicurve fill-style= "none"
%	 points= "(230,130);(230,130);(260,100);(260,100)"
%	 stroke-width= "0.4"
%	 />
%<multicurve fill-style= "none"
%	 points= "(255,130);(255,130);(255,150);(255,150)"
%	 stroke-width= "1.45"
%	 />
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(275,150)"
%	 stroke-width= "0.4"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\Univ$
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(288.75,253.75)"
%	 stroke-width= "0.4"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\Cee$
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(245,42.5)"
%	 stroke-width= "0.4"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\Fee$
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(280,2.5)"
%	 stroke-width= "0.4"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\Bee$
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(245,185)"
%	 stroke-width= "0.4"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\Dott$
%</text>
%<multicurve fill-style= "none"
%	 points= "(255,160);(255,160);(255,170);(255,170)"
%	 stroke-width= "1.45"
%	 />
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(241.25,212.5)"
%	 stroke-width= "0.4"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\Code$
%</text>
%<multicurve fill-style= "none"
%	 points= "(260,170);(260,170);(230,170);(230,170)"
%	 stroke-width= "0.4"
%	 />
%<multicurve fill-style= "none"
%	 points= "(245,80);(245,80);(245,115);(245,115)"
%	 stroke-width= "1.45"
%	 />
%<multicurve fill-style= "none"
%	 points= "(230,200);(230,200);(260,170);(260,170)"
%	 stroke-width= "0.4"
%	 />
%<multicurve fill-style= "none"
%	 points= "(230,200);(230,200);(230,170);(230,170)"
%	 stroke-width= "0.4"
%	 />
%<multicurve fill-style= "none"
%	 points= "(245,185);(245,185);(245,215);(245,215)"
%	 stroke-width= "1.45"
%	 />
%<multicurve fill-style= "none"
%	 stroke-color= "#ff0000"
%	 points= "(225,125);(225,125);(255,95);(255,95)"
%	 stroke-width= "0.2"
%	 />
%<multicurve fill-style= "none"
%	 stroke-color= "#ff0000"
%	 points= "(255,95);(255,95);(300,95);(300,95)"
%	 stroke-width= "0.2"
%	 />
%<multicurve fill-style= "none"
%	 stroke-color= "#ff0000"
%	 points= "(300,95);(300,95);(300,185);(300,185)"
%	 stroke-width= "0.2"
%	 />
%<multicurve fill-style= "none"
%	 stroke-color= "#ff0000"
%	 points= "(255,185);(255,185);(300,185);(300,185)"
%	 stroke-width= "0.2"
%	 />
%<multicurve fill-style= "none"
%	 stroke-color= "#ff0000"
%	 points= "(225,215);(225,215);(255,185);(255,185)"
%	 stroke-width= "0.2"
%	 />
%<multicurve fill-style= "none"
%	 stroke-color= "#ff0000"
%	 points= "(225,125);(225,125);(225,215);(225,215)"
%	 stroke-width= "0.2"
%	 />
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(255,42.5)"
%	 stroke-width= "0.4"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\Dott$
%</text>
%<multicurve fill-style= "none"
%	 points= "(265,32.5);(265,32.5);(245,32.5);(245,32.5)"
%	 stroke-width= "0.4"
%	 />
%<multicurve fill-style= "none"
%	 points= "(245,52.5);(245,52.5);(265,32.5);(265,32.5)"
%	 stroke-width= "0.4"
%	 />
%<multicurve fill-style= "none"
%	 points= "(225,52.5);(225,52.5);(245,32.5);(245,32.5)"
%	 stroke-width= "0.4"
%	 />
%<multicurve fill-style= "none"
%	 points= "(255,32.5);(255,32.5);(255,0);(255,0)"
%	 stroke-width= "0.4"
%	 />
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(245,80)"
%	 stroke-width= "0.4"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\Dott$
%</text>
%<multicurve fill-style= "none"
%	 points= "(230,95);(230,95);(260,65);(260,65)"
%	 stroke-width= "0.4"
%	 />
%<multicurve fill-style= "none"
%	 points= "(230,95);(230,95);(230,65);(230,65)"
%	 stroke-width= "0.4"
%	 />
%<multicurve fill-style= "none"
%	 points= "(255,42.5);(255,42.5);(255,65);(255,65)"
%	 stroke-width= "1.45"
%	 />
%<multicurve fill-style= "none"
%	 points= "(260,65);(260,65);(230,65);(230,65)"
%	 stroke-width= "0.4"
%	 />
%<multicurve fill-style= "none"
%	 points= "(235,65);(235,65);(235,60);(235,60)"
%	 stroke-width= "0.4"
%	 />
%<multicurve fill-style= "none"
%	 points= "(220,50);(220,50);(255,15);(255,15)"
%	 stroke-width= "0.4"
%	 />
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(255,15)"
%	 stroke-width= "0.4"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\Dott$
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(105,140)"
%	 stroke-width= "0.4"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\EQLS
%</text>
%<multicurve fill-style= "none"
%	 points= "(90,150);(90,150);(90,130);(90,130)"
%	 stroke-width= "0.4"
%	 />
%<multicurve fill-style= "none"
%	 points= "(40,150);(40,150);(90,150);(90,150)"
%	 stroke-width= "0.4"
%	 />
%<multicurve fill-style= "none"
%	 points= "(80,130);(80,130);(80,0);(80,0)"
%	 stroke-width= "0.4"
%	 />
%<multicurve fill-style= "none"
%	 points= "(80,255);(80,255);(80,150);(80,150)"
%	 stroke-width= "0.4"
%	 />
%<multicurve fill-style= "none"
%	 points= "(90,130);(90,130);(40,130);(40,130)"
%	 stroke-width= "0.4"
%	 />
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(85,253.75)"
%	 stroke-width= "0.4"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\Cee$
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(46.25,2.5)"
%	 stroke-width= "0.4"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\Aee$
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(75,2.5)"
%	 stroke-width= "0.4"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\Bee$
%</text>
%<multicurve fill-style= "none"
%	 points= "(40,150);(40,150);(40,130);(40,130)"
%	 stroke-width= "0.4"
%	 />
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(43.75,253.75)"
%	 stroke-width= "0.4"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\Code$
%</text>
%<multicurve fill-style= "none"
%	 points= "(50,130);(50,130);(50,0);(50,0)"
%	 stroke-width= "0.4"
%	 />
%<multicurve fill-style= "none"
%	 stroke-color= "#ff0033"
%	 points= "(235,100);(235,100);(270,65);(270,65)"
%	 stroke-width= "0.2"
%	 />
%<multicurve fill-style= "none"
%	 stroke-color= "#ff0033"
%	 points= "(270,10);(270,10);(270,65);(270,65)"
%	 stroke-width= "0.2"
%	 />
%<multicurve fill-style= "none"
%	 stroke-color= "#ff0033"
%	 points= "(211.25,10);(211.25,10);(211.25,100);(211.25,100)"
%	 stroke-width= "0.2"
%	 />
%<multicurve fill-style= "none"
%	 stroke-color= "#ff0033"
%	 points= "(270,10);(270,10);(211.25,10);(211.25,10)"
%	 stroke-width= "0.2"
%	 />
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(65,140)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\quu$
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(238.75,72.5)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\prrrr$
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(238.75,176.25)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\prrrr$
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(248.12,125)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\pjjjj$
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(250,121.25)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(232.5,160)"
%	 stroke-width= "0.4"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\Aee$
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(273.75,173.75)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\PadUniv$
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(263.75,51.25)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\PadFee$
%</text>
%<multicurve fill-style= "none"
%	 points= "(245,52.5);(245,52.5);(225,52.5);(225,52.5)"
%	 stroke-width= "0.4"
%	 />
%<multicurve fill-style= "none"
%	 points= "(235,60);(235,60);(220,55);(220,55)"
%	 stroke-width= "0.4"
%	 />
%<multicurve fill-style= "none"
%	 points= "(220,55);(220,55);(220,50);(220,50)"
%	 stroke-width= "0.4"
%	 />
%<multicurve stroke-overstrike= "true"
%	 fill-style= "none"
%	 points= "(228.75,33.75);(228.75,33.75);(236.25,41.25);(236.25,41.25)"
%	 stroke-width= "1.45"
%	 stroke-overstrike-width= "0.65"
%	 />
%<multicurve fill-style= "none"
%	 points= "(237.5,23.75);(237.5,23.75);(217.5,23.75);(217.5,23.75)"
%	 stroke-width= "0.4"
%	 />
%<multicurve fill-style= "none"
%	 points= "(217.5,43.75);(217.5,43.75);(237.5,23.75);(237.5,23.75)"
%	 stroke-width= "0.4"
%	 />
%<multicurve fill-style= "none"
%	 points= "(217.5,43.75);(217.5,43.75);(217.5,23.75);(217.5,23.75)"
%	 stroke-width= "0.4"
%	 />
%<multicurve fill-style= "none"
%	 stroke-color= "#ff0033"
%	 points= "(211.25,100);(211.25,100);(235,100);(235,100)"
%	 stroke-width= "0.2"
%	 />
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(223.75,30)"
%	 stroke-width= "0.35"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\programm$
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(251.25,2.5)"
%	 stroke-width= "0.4"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\Aee$
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(40,192.5)"
%	 stroke-width= "0.4"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\Fee$
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(53.75,172.5)"
%	 stroke-width= "0.4"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\Aee$
%</text>
%<multicurve fill-style= "none"
%	 points= "(40,230);(40,230);(40,255);(40,255)"
%	 stroke-width= "1.45"
%	 />
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(50,192.5)"
%	 stroke-width= "0.4"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\Dott$
%</text>
%<multicurve fill-style= "none"
%	 points= "(60,182.5);(60,182.5);(40,182.5);(40,182.5)"
%	 stroke-width= "0.4"
%	 />
%<multicurve fill-style= "none"
%	 points= "(40,202.5);(40,202.5);(60,182.5);(60,182.5)"
%	 stroke-width= "0.4"
%	 />
%<multicurve fill-style= "none"
%	 points= "(20,202.5);(20,202.5);(40,182.5);(40,182.5)"
%	 stroke-width= "0.4"
%	 />
%<multicurve fill-style= "none"
%	 points= "(50,182.5);(50,182.5);(50,150);(50,150)"
%	 stroke-width= "0.4"
%	 />
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(40,230)"
%	 stroke-width= "0.4"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\Dott$
%</text>
%<multicurve fill-style= "none"
%	 points= "(25,245);(25,245);(55,215);(55,215)"
%	 stroke-width= "0.4"
%	 />
%<multicurve fill-style= "none"
%	 points= "(25,245);(25,245);(25,215);(25,215)"
%	 stroke-width= "0.4"
%	 />
%<multicurve fill-style= "none"
%	 points= "(50,192.5);(50,192.5);(50,215);(50,215)"
%	 stroke-width= "1.45"
%	 />
%<multicurve fill-style= "none"
%	 points= "(55,215);(55,215);(25,215);(25,215)"
%	 stroke-width= "0.4"
%	 />
%<multicurve fill-style= "none"
%	 points= "(30,215);(30,215);(30,210);(30,210)"
%	 stroke-width= "0.4"
%	 />
%<multicurve fill-style= "none"
%	 points= "(15,200);(15,200);(50,165);(50,165)"
%	 stroke-width= "0.4"
%	 />
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(50,165)"
%	 stroke-width= "0.4"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\Dott$
%</text>
%<multicurve fill-style= "none"
%	 stroke-color= "#ff0033"
%	 points= "(30,250);(30,250);(65,215);(65,215)"
%	 stroke-width= "0.2"
%	 />
%<multicurve fill-style= "none"
%	 stroke-color= "#ff0033"
%	 points= "(65,160);(65,160);(65,215);(65,215)"
%	 stroke-width= "0.2"
%	 />
%<multicurve fill-style= "none"
%	 stroke-color= "#ff0033"
%	 points= "(6.25,160);(6.25,160);(6.25,250);(6.25,250)"
%	 stroke-width= "0.2"
%	 />
%<multicurve fill-style= "none"
%	 stroke-color= "#ff0033"
%	 points= "(65,160);(65,160);(6.25,160);(6.25,160)"
%	 stroke-width= "0.2"
%	 />
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(33.75,222.5)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\prrrr$
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(58.75,201.25)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\PadFee$
%</text>
%<multicurve fill-style= "none"
%	 points= "(40,202.5);(40,202.5);(20,202.5);(20,202.5)"
%	 stroke-width= "0.4"
%	 />
%<multicurve fill-style= "none"
%	 points= "(30,210);(30,210);(15,205);(15,205)"
%	 stroke-width= "0.4"
%	 />
%<multicurve fill-style= "none"
%	 points= "(15,205);(15,205);(15,200);(15,200)"
%	 stroke-width= "0.4"
%	 />
%<multicurve stroke-overstrike= "true"
%	 fill-style= "none"
%	 points= "(23.75,183.75);(23.75,183.75);(31.25,191.25);(31.25,191.25)"
%	 stroke-width= "1.45"
%	 stroke-overstrike-width= "0.65"
%	 />
%<multicurve fill-style= "none"
%	 points= "(32.5,173.75);(32.5,173.75);(12.5,173.75);(12.5,173.75)"
%	 stroke-width= "0.4"
%	 />
%<multicurve fill-style= "none"
%	 points= "(12.5,193.75);(12.5,193.75);(32.5,173.75);(32.5,173.75)"
%	 stroke-width= "0.4"
%	 />
%<multicurve fill-style= "none"
%	 points= "(12.5,193.75);(12.5,193.75);(12.5,173.75);(12.5,173.75)"
%	 stroke-width= "0.4"
%	 />
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(18.75,180)"
%	 stroke-width= "0.35"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\programm$
%</text>
%<multicurve fill-style= "none"
%	 stroke-color= "#ff0033"
%	 points= "(6.25,250);(6.25,250);(30,250);(30,250)"
%	 stroke-width= "0.2"
%	 />
%<multicurve fill-style= "none"
%	 points= "(260,230);(260,230);(230,230);(230,230)"
%	 stroke-width= "0.4"
%	 />
%<multicurve fill-style= "none"
%	 points= "(260,230);(260,230);(260,200);(260,200)"
%	 stroke-width= "0.4"
%	 />
%<multicurve fill-style= "none"
%	 points= "(230,230);(230,230);(260,200);(260,200)"
%	 stroke-width= "0.4"
%	 />
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(248.12,225)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\pjjjj$
%</text>
%<multicurve fill-style= "none"
%	 points= "(235,235);(235,235);(235,230);(235,230)"
%	 stroke-width= "0.4"
%	 />
%<multicurve fill-style= "none"
%	 points= "(255,230);(255,230);(255,255);(255,255)"
%	 stroke-width= "1.45"
%	 />
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(235,235)"
%	 stroke-width= "0.4"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\Dott$
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(258.75,254.38)"
%	 stroke-width= "0.4"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\Code$
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(205,140)"
%	 stroke-width= "0.4"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\EQLS
%</text>
%<multicurve fill-style= "none"
%	 points= "(190,160);(190,160);(190,140);(190,140)"
%	 stroke-width= "0.4"
%	 />
%<multicurve fill-style= "none"
%	 points= "(140,160);(140,160);(190,160);(190,160)"
%	 stroke-width= "0.4"
%	 />
%<multicurve fill-style= "none"
%	 points= "(180,140);(180,140);(180,0);(180,0)"
%	 stroke-width= "0.4"
%	 />
%<multicurve fill-style= "none"
%	 points= "(180,255);(180,255);(180,160);(180,160)"
%	 stroke-width= "0.4"
%	 />
%<multicurve fill-style= "none"
%	 points= "(190,140);(190,140);(160,140);(160,140)"
%	 stroke-width= "0.4"
%	 />
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(185,253.75)"
%	 stroke-width= "0.4"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\Cee$
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(141.25,2.5)"
%	 stroke-width= "0.4"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\Aee$
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(176.25,2.5)"
%	 stroke-width= "0.4"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\Bee$
%</text>
%<multicurve fill-style= "none"
%	 points= "(140,160);(140,160);(160,140);(160,140)"
%	 stroke-width= "0.4"
%	 />
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(154.38,254.38)"
%	 stroke-width= "0.4"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\Code$
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(140,130)"
%	 stroke-width= "0.4"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\Fee$
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(150,130)"
%	 stroke-width= "0.4"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\Dott$
%</text>
%<multicurve fill-style= "none"
%	 points= "(160,120);(160,120);(140,120);(140,120)"
%	 stroke-width= "0.4"
%	 />
%<multicurve fill-style= "none"
%	 points= "(140,140);(140,140);(160,120);(160,120)"
%	 stroke-width= "0.4"
%	 />
%<multicurve fill-style= "none"
%	 points= "(120,140);(120,140);(140,120);(140,120)"
%	 stroke-width= "0.4"
%	 />
%<multicurve fill-style= "none"
%	 points= "(150,120);(150,120);(150,0);(150,0)"
%	 stroke-width= "0.4"
%	 />
%<multicurve fill-style= "none"
%	 points= "(150,130);(150,130);(150,150);(150,150)"
%	 stroke-width= "1.45"
%	 />
%<multicurve fill-style= "none"
%	 points= "(140,140);(140,140);(120,140);(120,140)"
%	 stroke-width= "0.4"
%	 />
%<multicurve fill-style= "none"
%	 points= "(130,110);(130,110);(130,130);(130,130)"
%	 stroke-width= "1.45"
%	 />
%<multicurve fill-style= "none"
%	 points= "(140,100);(140,100);(120,100);(120,100)"
%	 stroke-width= "0.4"
%	 />
%<multicurve fill-style= "none"
%	 points= "(120,120);(120,120);(140,100);(140,100)"
%	 stroke-width= "0.4"
%	 />
%<multicurve fill-style= "none"
%	 points= "(120,120);(120,120);(120,100);(120,100)"
%	 stroke-width= "0.4"
%	 />
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(126.25,106.25)"
%	 stroke-width= "0.35"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\programm$
%</text>
%<multicurve fill-style= "none"
%	 points= "(150,160);(150,160);(150,255);(150,255)"
%	 stroke-width= "1.45"
%	 />
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(228.12,33.12)"
%	 stroke-width= "0.4"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\Dott$
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(130,110)"
%	 stroke-width= "0.4"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\Dott$
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(23.12,183.12)"
%	 stroke-width= "0.4"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\Dott$
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(170,150)"
%	 stroke-width= "0.4"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\Univ$
%</text>
%</jpic>
%%End JPIC-XML
%PSTricks content-type (pstricks.sty package needed)
%Add \usepackage{pstricks} in the preamble of your LaTeX file
%You can rescale the whole picture (to 80% for instance) by using the command \def\JPicScale{0.8}
\ifx\JPicScale\undefined\def\JPicScale{1}\fi
\psset{unit=\JPicScale mm}
\psset{linewidth=0.3,dotsep=1,hatchwidth=0.3,hatchsep=1.5,shadowsize=1,dimen=middle}
\psset{dotsize=0.7 2.5,dotscale=1 1,fillcolor=black}
\psset{arrowsize=1 2,arrowlength=1,arrowinset=0.25,tbarsize=0.7 5,bracketlength=0.15,rbracketlength=0.15}
\begin{pspicture}(0,0)(300,255)
\psline[linewidth=0.4](295,160)(295,140)
\psline[linewidth=0.4](260,130)(230,130)
\psline[linewidth=0.4](245,160)(295,160)
\psline[linewidth=0.4](285,140)(285,0)
\psline[linewidth=0.4](285,255)(285,160)
\psline[linewidth=0.4](260,130)(260,100)
\psline[linewidth=0.4](235,170)(235,130)
\psline[linewidth=0.4](295,140)(265,140)
\psline[linewidth=0.4](245,160)(265,140)
\psline[linewidth=0.4](230,130)(260,100)
\psline[linewidth=1.45](255,130)(255,150)
\rput(275,150){$\Univ$}
\rput[l](288.75,253.75){$\Cee$}
\rput(245,42.5){$\Fee$}
\rput[r](280,2.5){$\Bee$}
\rput(245,185){$\Dott$}
\psline[linewidth=1.45](255,160)(255,170)
\rput[r](241.25,212.5){$\Code$}
\psline[linewidth=0.4](260,170)(230,170)
\psline[linewidth=1.45](245,80)(245,115)
\psline[linewidth=0.4](230,200)(260,170)
\psline[linewidth=0.4](230,200)(230,170)
\psline[linewidth=1.45](245,185)(245,215)
\psline[linewidth=0.2,linecolor=red](225,125)(255,95)
\psline[linewidth=0.2,linecolor=red](255,95)(300,95)
\psline[linewidth=0.2,linecolor=red](300,95)(300,185)
\psline[linewidth=0.2,linecolor=red](255,185)(300,185)
\psline[linewidth=0.2,linecolor=red](225,215)(255,185)
\psline[linewidth=0.2,linecolor=red](225,125)(225,215)
\rput(255,42.5){$\Dott$}
\psline[linewidth=0.4](265,32.5)(245,32.5)
\psline[linewidth=0.4](245,52.5)(265,32.5)
\psline[linewidth=0.4](225,52.5)(245,32.5)
\psline[linewidth=0.4](255,32.5)(255,0)
\rput(245,80){$\Dott$}
\psline[linewidth=0.4](230,95)(260,65)
\psline[linewidth=0.4](230,95)(230,65)
\psline[linewidth=1.45](255,42.5)(255,65)
\psline[linewidth=0.4](260,65)(230,65)
\psline[linewidth=0.4](235,65)(235,60)
\psline[linewidth=0.4](220,50)(255,15)
\rput(255,15){$\Dott$}
\rput(105,140){\EQLS}
\psline[linewidth=0.4](90,150)(90,130)
\psline[linewidth=0.4](40,150)(90,150)
\psline[linewidth=0.4](80,130)(80,0)
\psline[linewidth=0.4](80,255)(80,150)
\psline[linewidth=0.4](90,130)(40,130)
\rput[l](85,253.75){$\Cee$}
\rput[r](46.25,2.5){$\Aee$}
\rput[r](75,2.5){$\Bee$}
\psline[linewidth=0.4](40,150)(40,130)
\rput[l](43.75,253.75){$\Code$}
\psline[linewidth=0.4](50,130)(50,0)
\newrgbcolor{userLineColour}{1 0 0.2}
\psline[linewidth=0.2,linecolor=userLineColour](235,100)(270,65)
\newrgbcolor{userLineColour}{1 0 0.2}
\psline[linewidth=0.2,linecolor=userLineColour](270,10)(270,65)
\newrgbcolor{userLineColour}{1 0 0.2}
\psline[linewidth=0.2,linecolor=userLineColour](211.25,10)(211.25,100)
\newrgbcolor{userLineColour}{1 0 0.2}
\psline[linewidth=0.2,linecolor=userLineColour](270,10)(211.25,10)
\rput(65,140){$\quu$}
\rput(238.75,72.5){$\prrrr$}
\rput(238.75,176.25){$\prrrr$}
\rput(248.12,125){$\pjjjj$}
\rput(250,121.25){}
\rput[r](232.5,160){$\Aee$}
\rput(273.75,173.75){$\PadUniv$}
\rput(263.75,51.25){$\PadFee$}
\psline[linewidth=0.4](245,52.5)(225,52.5)
\psline[linewidth=0.4](235,60)(220,55)
\psline[linewidth=0.4](220,55)(220,50)
\psline[linewidth=1.45,border=0.65](228.75,33.75)(236.25,41.25)
\psline[linewidth=0.4](237.5,23.75)(217.5,23.75)
\psline[linewidth=0.4](217.5,43.75)(237.5,23.75)
\psline[linewidth=0.4](217.5,43.75)(217.5,23.75)
\newrgbcolor{userLineColour}{1 0 0.2}
\psline[linewidth=0.2,linecolor=userLineColour](211.25,100)(235,100)
\rput(223.75,30){$\programm$}
\rput[r](251.25,2.5){$\Aee$}
\rput(40,192.5){$\Fee$}
\rput[l](53.75,172.5){$\Aee$}
\psline[linewidth=1.45](40,230)(40,255)
\rput(50,192.5){$\Dott$}
\psline[linewidth=0.4](60,182.5)(40,182.5)
\psline[linewidth=0.4](40,202.5)(60,182.5)
\psline[linewidth=0.4](20,202.5)(40,182.5)
\psline[linewidth=0.4](50,182.5)(50,150)
\rput(40,230){$\Dott$}
\psline[linewidth=0.4](25,245)(55,215)
\psline[linewidth=0.4](25,245)(25,215)
\psline[linewidth=1.45](50,192.5)(50,215)
\psline[linewidth=0.4](55,215)(25,215)
\psline[linewidth=0.4](30,215)(30,210)
\psline[linewidth=0.4](15,200)(50,165)
\rput(50,165){$\Dott$}
\newrgbcolor{userLineColour}{1 0 0.2}
\psline[linewidth=0.2,linecolor=userLineColour](30,250)(65,215)
\newrgbcolor{userLineColour}{1 0 0.2}
\psline[linewidth=0.2,linecolor=userLineColour](65,160)(65,215)
\newrgbcolor{userLineColour}{1 0 0.2}
\psline[linewidth=0.2,linecolor=userLineColour](6.25,160)(6.25,250)
\newrgbcolor{userLineColour}{1 0 0.2}
\psline[linewidth=0.2,linecolor=userLineColour](65,160)(6.25,160)
\rput(33.75,222.5){$\prrrr$}
\rput(58.75,201.25){$\PadFee$}
\psline[linewidth=0.4](40,202.5)(20,202.5)
\psline[linewidth=0.4](30,210)(15,205)
\psline[linewidth=0.4](15,205)(15,200)
\psline[linewidth=1.45,border=0.65](23.75,183.75)(31.25,191.25)
\psline[linewidth=0.4](32.5,173.75)(12.5,173.75)
\psline[linewidth=0.4](12.5,193.75)(32.5,173.75)
\psline[linewidth=0.4](12.5,193.75)(12.5,173.75)
\rput(18.75,180){$\programm$}
\newrgbcolor{userLineColour}{1 0 0.2}
\psline[linewidth=0.2,linecolor=userLineColour](6.25,250)(30,250)
\psline[linewidth=0.4](260,230)(230,230)
\psline[linewidth=0.4](260,230)(260,200)
\psline[linewidth=0.4](230,230)(260,200)
\rput(248.12,225){$\pjjjj$}
\psline[linewidth=0.4](235,235)(235,230)
\psline[linewidth=1.45](255,230)(255,255)
\rput(235,235){$\Dott$}
\rput[l](258.75,254.38){$\Code$}
\rput(205,140){\EQLS}
\psline[linewidth=0.4](190,160)(190,140)
\psline[linewidth=0.4](140,160)(190,160)
\psline[linewidth=0.4](180,140)(180,0)
\psline[linewidth=0.4](180,255)(180,160)
\psline[linewidth=0.4](190,140)(160,140)
\rput[l](185,253.75){$\Cee$}
\rput[r](141.25,2.5){$\Aee$}
\rput[r](176.25,2.5){$\Bee$}
\psline[linewidth=0.4](140,160)(160,140)
\rput[l](154.38,254.38){$\Code$}
\rput(140,130){$\Fee$}
\rput(150,130){$\Dott$}
\psline[linewidth=0.4](160,120)(140,120)
\psline[linewidth=0.4](140,140)(160,120)
\psline[linewidth=0.4](120,140)(140,120)
\psline[linewidth=0.4](150,120)(150,0)
\psline[linewidth=1.45](150,130)(150,150)
\psline[linewidth=0.4](140,140)(120,140)
\psline[linewidth=1.45](130,110)(130,130)
\psline[linewidth=0.4](140,100)(120,100)
\psline[linewidth=0.4](120,120)(140,100)
\psline[linewidth=0.4](120,120)(120,100)
\rput(126.25,106.25){$\programm$}
\psline[linewidth=1.45](150,160)(150,255)
\rput(228.12,33.12){$\Dott$}
\rput(130,110){$\Dott$}
\rput(23.12,183.12){$\Dott$}
\rput(170,150){$\Univ$}
\end{pspicture}


==> PIC/losless-q.tex <==
%%Created by jPicEdt 1.4.1_03: mixed JPIC-XML/LaTeX format
%%Mon Jan 09 20:51:42 GMT-10:00 2023
%%Begin JPIC-XML
%<?xml version="1.0" standalone="yes"?>
%<jpic x-min="1.25" x-max="300" y-min="0" y-max="300" auto-bounding="true">
%<multicurve fill-style= "none"
%	 points= "(85,160);(85,160);(85,140);(85,140)"
%	 stroke-width= "0.4"
%	 />
%<multicurve fill-style= "none"
%	 points= "(50,130);(50,130);(20,130);(20,130)"
%	 stroke-width= "0.4"
%	 />
%<multicurve fill-style= "none"
%	 points= "(35,160);(35,160);(85,160);(85,160)"
%	 stroke-width= "0.4"
%	 />
%<multicurve fill-style= "none"
%	 points= "(75,140);(75,140);(75,0);(75,0)"
%	 stroke-width= "0.4"
%	 />
%<multicurve fill-style= "none"
%	 points= "(75,300);(75,300);(75,160);(75,160)"
%	 stroke-width= "0.4"
%	 />
%<multicurve fill-style= "none"
%	 points= "(50,130);(50,130);(50,100);(50,100)"
%	 stroke-width= "0.4"
%	 />
%<multicurve fill-style= "none"
%	 points= "(25,170);(25,170);(25,130);(25,130)"
%	 stroke-width= "0.4"
%	 />
%<multicurve fill-style= "none"
%	 points= "(85,140);(85,140);(55,140);(55,140)"
%	 stroke-width= "0.4"
%	 />
%<multicurve fill-style= "none"
%	 points= "(35,160);(35,160);(55,140);(55,140)"
%	 stroke-width= "0.4"
%	 />
%<multicurve fill-style= "none"
%	 points= "(20,130);(20,130);(50,100);(50,100)"
%	 stroke-width= "0.4"
%	 />
%<multicurve fill-style= "none"
%	 points= "(45,130);(45,130);(45,150);(45,150)"
%	 stroke-width= "1.45"
%	 />
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(65,150)"
%	 stroke-width= "0.4"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\Univ$
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(78.75,298.75)"
%	 stroke-width= "0.4"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\Cee$
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(35,42.5)"
%	 stroke-width= "0.4"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\Fee$
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(70,2.5)"
%	 stroke-width= "0.4"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\Bee$
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(35,185)"
%	 stroke-width= "0.4"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\Dott$
%</text>
%<multicurve fill-style= "none"
%	 points= "(45,160);(45,160);(45,170);(45,170)"
%	 stroke-width= "1.45"
%	 />
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(31.25,212.5)"
%	 stroke-width= "0.4"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\Code$
%</text>
%<multicurve fill-style= "none"
%	 points= "(50,170);(50,170);(20,170);(20,170)"
%	 stroke-width= "0.4"
%	 />
%<multicurve fill-style= "none"
%	 points= "(35,80);(35,80);(35,115);(35,115)"
%	 stroke-width= "1.45"
%	 />
%<multicurve fill-style= "none"
%	 points= "(20,200);(20,200);(50,170);(50,170)"
%	 stroke-width= "0.4"
%	 />
%<multicurve fill-style= "none"
%	 points= "(20,200);(20,200);(20,170);(20,170)"
%	 stroke-width= "0.4"
%	 />
%<multicurve fill-style= "none"
%	 points= "(35,185);(35,185);(35,215);(35,215)"
%	 stroke-width= "1.45"
%	 />
%<multicurve fill-style= "none"
%	 stroke-color= "#ff0000"
%	 points= "(15,125);(15,125);(45,95);(45,95)"
%	 stroke-width= "0.2"
%	 />
%<multicurve fill-style= "none"
%	 stroke-color= "#ff0000"
%	 points= "(45,95);(45,95);(90,95);(90,95)"
%	 stroke-width= "0.2"
%	 />
%<multicurve fill-style= "none"
%	 stroke-color= "#ff0000"
%	 points= "(90,95);(90,95);(90,185);(90,185)"
%	 stroke-width= "0.2"
%	 />
%<multicurve fill-style= "none"
%	 stroke-color= "#ff0000"
%	 points= "(45,185);(45,185);(90,185);(90,185)"
%	 stroke-width= "0.2"
%	 />
%<multicurve fill-style= "none"
%	 stroke-color= "#ff0000"
%	 points= "(15,215);(15,215);(45,185);(45,185)"
%	 stroke-width= "0.2"
%	 />
%<multicurve fill-style= "none"
%	 stroke-color= "#ff0000"
%	 points= "(15,125);(15,125);(15,215);(15,215)"
%	 stroke-width= "0.2"
%	 />
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(45,42.5)"
%	 stroke-width= "0.4"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\Dott$
%</text>
%<multicurve fill-style= "none"
%	 points= "(55,32.5);(55,32.5);(35,32.5);(35,32.5)"
%	 stroke-width= "0.4"
%	 />
%<multicurve fill-style= "none"
%	 points= "(35,52.5);(35,52.5);(55,32.5);(55,32.5)"
%	 stroke-width= "0.4"
%	 />
%<multicurve fill-style= "none"
%	 points= "(15,52.5);(15,52.5);(35,32.5);(35,32.5)"
%	 stroke-width= "0.4"
%	 />
%<multicurve fill-style= "none"
%	 points= "(45,32.5);(45,32.5);(45,0);(45,0)"
%	 stroke-width= "0.4"
%	 />
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(35,80)"
%	 stroke-width= "0.4"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\Dott$
%</text>
%<multicurve fill-style= "none"
%	 points= "(20,95);(20,95);(50,65);(50,65)"
%	 stroke-width= "0.4"
%	 />
%<multicurve fill-style= "none"
%	 points= "(20,95);(20,95);(20,65);(20,65)"
%	 stroke-width= "0.4"
%	 />
%<multicurve fill-style= "none"
%	 points= "(45,42.5);(45,42.5);(45,65);(45,65)"
%	 stroke-width= "1.45"
%	 />
%<multicurve fill-style= "none"
%	 points= "(50,65);(50,65);(20,65);(20,65)"
%	 stroke-width= "0.4"
%	 />
%<multicurve fill-style= "none"
%	 points= "(25,65);(25,65);(25,60);(25,60)"
%	 stroke-width= "0.4"
%	 />
%<multicurve fill-style= "none"
%	 points= "(10,50);(10,50);(45,15);(45,15)"
%	 stroke-width= "0.4"
%	 />
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(45,15)"
%	 stroke-width= "0.4"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\Dott$
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(225,150)"
%	 stroke-width= "0.4"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\EQLS
%</text>
%<multicurve fill-style= "none"
%	 points= "(200,160);(200,160);(200,140);(200,140)"
%	 stroke-width= "0.4"
%	 />
%<multicurve fill-style= "none"
%	 points= "(150,160);(150,160);(200,160);(200,160)"
%	 stroke-width= "0.4"
%	 />
%<multicurve fill-style= "none"
%	 points= "(190,140);(190,140);(190,0);(190,0)"
%	 stroke-width= "0.4"
%	 />
%<multicurve fill-style= "none"
%	 points= "(190,300);(190,300);(190,160);(190,160)"
%	 stroke-width= "0.4"
%	 />
%<multicurve fill-style= "none"
%	 points= "(200,140);(200,140);(150,140);(150,140)"
%	 stroke-width= "0.4"
%	 />
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(193.75,298.75)"
%	 stroke-width= "0.4"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\Cee$
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(156.25,2.5)"
%	 stroke-width= "0.4"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\Aee$
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(185,2.5)"
%	 stroke-width= "0.4"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\Bee$
%</text>
%<multicurve fill-style= "none"
%	 points= "(150,160);(150,160);(150,140);(150,140)"
%	 stroke-width= "0.4"
%	 />
%<multicurve fill-style= "none"
%	 points= "(160,140);(160,140);(160,0);(160,0)"
%	 stroke-width= "0.4"
%	 />
%<multicurve fill-style= "none"
%	 stroke-color= "#ff0033"
%	 points= "(25,100);(25,100);(60,65);(60,65)"
%	 stroke-width= "0.2"
%	 />
%<multicurve fill-style= "none"
%	 stroke-color= "#ff0033"
%	 points= "(60,10);(60,10);(60,65);(60,65)"
%	 stroke-width= "0.2"
%	 />
%<multicurve fill-style= "none"
%	 stroke-color= "#ff0033"
%	 points= "(1.25,10);(1.25,10);(1.25,100);(1.25,100)"
%	 stroke-width= "0.2"
%	 />
%<multicurve fill-style= "none"
%	 stroke-color= "#ff0033"
%	 points= "(60,10);(60,10);(1.25,10);(1.25,10)"
%	 stroke-width= "0.2"
%	 />
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(175,150)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\quu$
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(28.75,72.5)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\prrrr$
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(28.75,176.25)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\prrrr$
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(38.12,125)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\pjjjj$
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(40,121.25)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(22.5,160)"
%	 stroke-width= "0.4"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\Aee$
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(63.75,173.75)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\PadUniv$
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(53.75,51.25)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\PadFee$
%</text>
%<multicurve fill-style= "none"
%	 points= "(35,52.5);(35,52.5);(15,52.5);(15,52.5)"
%	 stroke-width= "0.4"
%	 />
%<multicurve fill-style= "none"
%	 points= "(25,60);(25,60);(10,55);(10,55)"
%	 stroke-width= "0.4"
%	 />
%<multicurve fill-style= "none"
%	 points= "(10,55);(10,55);(10,50);(10,50)"
%	 stroke-width= "0.4"
%	 />
%<multicurve stroke-overstrike= "true"
%	 fill-style= "none"
%	 points= "(18.75,33.75);(18.75,33.75);(26.25,41.25);(26.25,41.25)"
%	 stroke-width= "1.45"
%	 stroke-overstrike-width= "0.65"
%	 />
%<multicurve fill-style= "none"
%	 points= "(27.5,23.75);(27.5,23.75);(7.5,23.75);(7.5,23.75)"
%	 stroke-width= "0.4"
%	 />
%<multicurve fill-style= "none"
%	 points= "(7.5,43.75);(7.5,43.75);(27.5,23.75);(27.5,23.75)"
%	 stroke-width= "0.4"
%	 />
%<multicurve fill-style= "none"
%	 points= "(7.5,43.75);(7.5,43.75);(7.5,23.75);(7.5,23.75)"
%	 stroke-width= "0.4"
%	 />
%<multicurve fill-style= "none"
%	 stroke-color= "#ff0033"
%	 points= "(1.25,100);(1.25,100);(25,100);(25,100)"
%	 stroke-width= "0.2"
%	 />
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(13.75,30)"
%	 stroke-width= "0.35"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\programm$
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(41.25,2.5)"
%	 stroke-width= "0.4"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\Aee$
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(150,202.5)"
%	 stroke-width= "0.4"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\Fee$
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(163.75,182.5)"
%	 stroke-width= "0.4"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\Aee$
%</text>
%<multicurve fill-style= "none"
%	 points= "(150,240);(150,240);(150,260);(150,260)"
%	 stroke-width= "1.45"
%	 />
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(160,202.5)"
%	 stroke-width= "0.4"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\Dott$
%</text>
%<multicurve fill-style= "none"
%	 points= "(170,192.5);(170,192.5);(150,192.5);(150,192.5)"
%	 stroke-width= "0.4"
%	 />
%<multicurve fill-style= "none"
%	 points= "(150,212.5);(150,212.5);(170,192.5);(170,192.5)"
%	 stroke-width= "0.4"
%	 />
%<multicurve fill-style= "none"
%	 points= "(130,212.5);(130,212.5);(150,192.5);(150,192.5)"
%	 stroke-width= "0.4"
%	 />
%<multicurve fill-style= "none"
%	 points= "(160,192.5);(160,192.5);(160,160);(160,160)"
%	 stroke-width= "0.4"
%	 />
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(150,240)"
%	 stroke-width= "0.4"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\Dott$
%</text>
%<multicurve fill-style= "none"
%	 points= "(135,255);(135,255);(165,225);(165,225)"
%	 stroke-width= "0.4"
%	 />
%<multicurve fill-style= "none"
%	 points= "(135,255);(135,255);(135,225);(135,225)"
%	 stroke-width= "0.4"
%	 />
%<multicurve fill-style= "none"
%	 points= "(160,202.5);(160,202.5);(160,225);(160,225)"
%	 stroke-width= "1.45"
%	 />
%<multicurve fill-style= "none"
%	 points= "(165,225);(165,225);(135,225);(135,225)"
%	 stroke-width= "0.4"
%	 />
%<multicurve fill-style= "none"
%	 points= "(140,225);(140,225);(140,220);(140,220)"
%	 stroke-width= "0.4"
%	 />
%<multicurve fill-style= "none"
%	 points= "(125,210);(125,210);(160,175);(160,175)"
%	 stroke-width= "0.4"
%	 />
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(160,175)"
%	 stroke-width= "0.4"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\Dott$
%</text>
%<multicurve fill-style= "none"
%	 stroke-color= "#ff0033"
%	 points= "(140,260);(140,260);(175,225);(175,225)"
%	 stroke-width= "0.2"
%	 />
%<multicurve fill-style= "none"
%	 stroke-color= "#ff0033"
%	 points= "(175,170);(175,170);(175,225);(175,225)"
%	 stroke-width= "0.2"
%	 />
%<multicurve fill-style= "none"
%	 stroke-color= "#ff0033"
%	 points= "(116.25,170);(116.25,170);(116.25,260);(116.25,260)"
%	 stroke-width= "0.2"
%	 />
%<multicurve fill-style= "none"
%	 stroke-color= "#ff0033"
%	 points= "(175,170);(175,170);(116.25,170);(116.25,170)"
%	 stroke-width= "0.2"
%	 />
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(143.75,232.5)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\prrrr$
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(168.75,211.25)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\PadFee$
%</text>
%<multicurve fill-style= "none"
%	 points= "(150,212.5);(150,212.5);(130,212.5);(130,212.5)"
%	 stroke-width= "0.4"
%	 />
%<multicurve fill-style= "none"
%	 points= "(140,220);(140,220);(125,215);(125,215)"
%	 stroke-width= "0.4"
%	 />
%<multicurve fill-style= "none"
%	 points= "(125,215);(125,215);(125,210);(125,210)"
%	 stroke-width= "0.4"
%	 />
%<multicurve stroke-overstrike= "true"
%	 fill-style= "none"
%	 points= "(133.75,193.75);(133.75,193.75);(141.25,201.25);(141.25,201.25)"
%	 stroke-width= "1.45"
%	 stroke-overstrike-width= "0.65"
%	 />
%<multicurve fill-style= "none"
%	 points= "(142.5,183.75);(142.5,183.75);(122.5,183.75);(122.5,183.75)"
%	 stroke-width= "0.4"
%	 />
%<multicurve fill-style= "none"
%	 points= "(122.5,203.75);(122.5,203.75);(142.5,183.75);(142.5,183.75)"
%	 stroke-width= "0.4"
%	 />
%<multicurve fill-style= "none"
%	 points= "(122.5,203.75);(122.5,203.75);(122.5,183.75);(122.5,183.75)"
%	 stroke-width= "0.4"
%	 />
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(128.75,190)"
%	 stroke-width= "0.35"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\programm$
%</text>
%<multicurve fill-style= "none"
%	 stroke-color= "#ff0033"
%	 points= "(116.25,260);(116.25,260);(140,260);(140,260)"
%	 stroke-width= "0.2"
%	 />
%<multicurve fill-style= "none"
%	 points= "(50,230);(50,230);(20,230);(20,230)"
%	 stroke-width= "0.4"
%	 />
%<multicurve fill-style= "none"
%	 points= "(50,230);(50,230);(50,200);(50,200)"
%	 stroke-width= "0.4"
%	 />
%<multicurve fill-style= "none"
%	 points= "(20,230);(20,230);(50,200);(50,200)"
%	 stroke-width= "0.4"
%	 />
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(38.12,225)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\pjjjj$
%</text>
%<multicurve fill-style= "none"
%	 points= "(25,235);(25,235);(25,230);(25,230)"
%	 stroke-width= "0.4"
%	 />
%<multicurve fill-style= "none"
%	 points= "(45,230);(45,230);(45,260);(45,260)"
%	 stroke-width= "1.45"
%	 />
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(25,235)"
%	 stroke-width= "0.4"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\Dott$
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(110,150)"
%	 stroke-width= "0.4"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\EQLS
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(18.12,33.12)"
%	 stroke-width= "0.4"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\Dott$
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(133.12,193.12)"
%	 stroke-width= "0.4"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\Dott$
%</text>
%<multicurve fill-style= "none"
%	 points= "(60,275);(60,275);(30,275);(30,275)"
%	 stroke-width= "0.4"
%	 />
%<multicurve fill-style= "none"
%	 points= "(60,275);(60,275);(60,245);(60,245)"
%	 stroke-width= "0.4"
%	 />
%<multicurve fill-style= "none"
%	 points= "(30,275);(30,275);(60,245);(60,245)"
%	 stroke-width= "0.4"
%	 />
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(48.12,270)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\pjjjj$
%</text>
%<multicurve fill-style= "none"
%	 points= "(35,300);(35,300);(35,275);(35,275)"
%	 stroke-width= "0.4"
%	 />
%<multicurve fill-style= "none"
%	 points= "(55,275);(55,275);(55,280);(55,280)"
%	 stroke-width= "1.45"
%	 />
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(55,280)"
%	 stroke-width= "0.4"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\Dott$
%</text>
%<multicurve fill-style= "none"
%	 points= "(165,275);(165,275);(135,275);(135,275)"
%	 stroke-width= "0.4"
%	 />
%<multicurve fill-style= "none"
%	 points= "(165,275);(165,275);(165,245);(165,245)"
%	 stroke-width= "0.4"
%	 />
%<multicurve fill-style= "none"
%	 points= "(135,275);(135,275);(165,245);(165,245)"
%	 stroke-width= "0.4"
%	 />
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(153.12,270)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\pjjjj$
%</text>
%<multicurve fill-style= "none"
%	 points= "(140,300);(140,300);(140,275);(140,275)"
%	 stroke-width= "0.4"
%	 />
%<multicurve fill-style= "none"
%	 points= "(160,275);(160,275);(160,280);(160,280)"
%	 stroke-width= "1.45"
%	 />
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(160,280)"
%	 stroke-width= "0.4"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\Dott$
%</text>
%<multicurve fill-style= "none"
%	 points= "(300,160);(300,160);(300,140);(300,140)"
%	 stroke-width= "0.4"
%	 />
%<multicurve fill-style= "none"
%	 points= "(250,160);(250,160);(300,160);(300,160)"
%	 stroke-width= "0.4"
%	 />
%<multicurve fill-style= "none"
%	 points= "(290,140);(290,140);(290,0);(290,0)"
%	 stroke-width= "0.4"
%	 />
%<multicurve fill-style= "none"
%	 points= "(290,300);(290,300);(290,160);(290,160)"
%	 stroke-width= "0.4"
%	 />
%<multicurve fill-style= "none"
%	 points= "(300,140);(300,140);(250,140);(250,140)"
%	 stroke-width= "0.4"
%	 />
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(293.75,298.75)"
%	 stroke-width= "0.4"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\Cee$
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(256.25,2.5)"
%	 stroke-width= "0.4"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\Aee$
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(285,2.5)"
%	 stroke-width= "0.4"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\Bee$
%</text>
%<multicurve fill-style= "none"
%	 points= "(250,160);(250,160);(250,140);(250,140)"
%	 stroke-width= "0.4"
%	 />
%<multicurve fill-style= "none"
%	 points= "(260,140);(260,140);(260,0);(260,0)"
%	 stroke-width= "0.4"
%	 />
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(275,150)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\quu$
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(263.75,300)"
%	 stroke-width= "0.4"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\Aee$
%</text>
%<multicurve fill-style= "none"
%	 points= "(260,300);(260,300);(260,160);(260,160)"
%	 stroke-width= "0.4"
%	 />
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(38.75,298.75)"
%	 stroke-width= "0.4"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\Aee$
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(143.75,298.75)"
%	 stroke-width= "0.4"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\Aee$
%</text>
%</jpic>
%%End JPIC-XML
%PSTricks content-type (pstricks.sty package needed)
%Add \usepackage{pstricks} in the preamble of your LaTeX file
%You can rescale the whole picture (to 80% for instance) by using the command \def\JPicScale{0.8}
\ifx\JPicScale\undefined\def\JPicScale{1}\fi
\psset{unit=\JPicScale mm}
\psset{linewidth=0.3,dotsep=1,hatchwidth=0.3,hatchsep=1.5,shadowsize=1,dimen=middle}
\psset{dotsize=0.7 2.5,dotscale=1 1,fillcolor=black}
\psset{arrowsize=1 2,arrowlength=1,arrowinset=0.25,tbarsize=0.7 5,bracketlength=0.15,rbracketlength=0.15}
\begin{pspicture}(0,0)(300,300)
\psline[linewidth=0.4](85,160)(85,140)
\psline[linewidth=0.4](50,130)(20,130)
\psline[linewidth=0.4](35,160)(85,160)
\psline[linewidth=0.4](75,140)(75,0)
\psline[linewidth=0.4](75,300)(75,160)
\psline[linewidth=0.4](50,130)(50,100)
\psline[linewidth=0.4](25,170)(25,130)
\psline[linewidth=0.4](85,140)(55,140)
\psline[linewidth=0.4](35,160)(55,140)
\psline[linewidth=0.4](20,130)(50,100)
\psline[linewidth=1.45](45,130)(45,150)
\rput(65,150){$\Univ$}
\rput[l](78.75,298.75){$\Cee$}
\rput(35,42.5){$\Fee$}
\rput[r](70,2.5){$\Bee$}
\rput(35,185){$\Dott$}
\psline[linewidth=1.45](45,160)(45,170)
\rput[r](31.25,212.5){$\Code$}
\psline[linewidth=0.4](50,170)(20,170)
\psline[linewidth=1.45](35,80)(35,115)
\psline[linewidth=0.4](20,200)(50,170)
\psline[linewidth=0.4](20,200)(20,170)
\psline[linewidth=1.45](35,185)(35,215)
\psline[linewidth=0.2,linecolor=red](15,125)(45,95)
\psline[linewidth=0.2,linecolor=red](45,95)(90,95)
\psline[linewidth=0.2,linecolor=red](90,95)(90,185)
\psline[linewidth=0.2,linecolor=red](45,185)(90,185)
\psline[linewidth=0.2,linecolor=red](15,215)(45,185)
\psline[linewidth=0.2,linecolor=red](15,125)(15,215)
\rput(45,42.5){$\Dott$}
\psline[linewidth=0.4](55,32.5)(35,32.5)
\psline[linewidth=0.4](35,52.5)(55,32.5)
\psline[linewidth=0.4](15,52.5)(35,32.5)
\psline[linewidth=0.4](45,32.5)(45,0)
\rput(35,80){$\Dott$}
\psline[linewidth=0.4](20,95)(50,65)
\psline[linewidth=0.4](20,95)(20,65)
\psline[linewidth=1.45](45,42.5)(45,65)
\psline[linewidth=0.4](50,65)(20,65)
\psline[linewidth=0.4](25,65)(25,60)
\psline[linewidth=0.4](10,50)(45,15)
\rput(45,15){$\Dott$}
\rput(225,150){\EQLS}
\psline[linewidth=0.4](200,160)(200,140)
\psline[linewidth=0.4](150,160)(200,160)
\psline[linewidth=0.4](190,140)(190,0)
\psline[linewidth=0.4](190,300)(190,160)
\psline[linewidth=0.4](200,140)(150,140)
\rput[l](193.75,298.75){$\Cee$}
\rput[r](156.25,2.5){$\Aee$}
\rput[r](185,2.5){$\Bee$}
\psline[linewidth=0.4](150,160)(150,140)
\psline[linewidth=0.4](160,140)(160,0)
\newrgbcolor{userLineColour}{1 0 0.2}
\psline[linewidth=0.2,linecolor=userLineColour](25,100)(60,65)
\newrgbcolor{userLineColour}{1 0 0.2}
\psline[linewidth=0.2,linecolor=userLineColour](60,10)(60,65)
\newrgbcolor{userLineColour}{1 0 0.2}
\psline[linewidth=0.2,linecolor=userLineColour](1.25,10)(1.25,100)
\newrgbcolor{userLineColour}{1 0 0.2}
\psline[linewidth=0.2,linecolor=userLineColour](60,10)(1.25,10)
\rput(175,150){$\quu$}
\rput(28.75,72.5){$\prrrr$}
\rput(28.75,176.25){$\prrrr$}
\rput(38.12,125){$\pjjjj$}
\rput(40,121.25){}
\rput[r](22.5,160){$\Aee$}
\rput(63.75,173.75){$\PadUniv$}
\rput(53.75,51.25){$\PadFee$}
\psline[linewidth=0.4](35,52.5)(15,52.5)
\psline[linewidth=0.4](25,60)(10,55)
\psline[linewidth=0.4](10,55)(10,50)
\psline[linewidth=1.45,border=0.65](18.75,33.75)(26.25,41.25)
\psline[linewidth=0.4](27.5,23.75)(7.5,23.75)
\psline[linewidth=0.4](7.5,43.75)(27.5,23.75)
\psline[linewidth=0.4](7.5,43.75)(7.5,23.75)
\newrgbcolor{userLineColour}{1 0 0.2}
\psline[linewidth=0.2,linecolor=userLineColour](1.25,100)(25,100)
\rput(13.75,30){$\programm$}
\rput[r](41.25,2.5){$\Aee$}
\rput(150,202.5){$\Fee$}
\rput[l](163.75,182.5){$\Aee$}
\psline[linewidth=1.45](150,240)(150,260)
\rput(160,202.5){$\Dott$}
\psline[linewidth=0.4](170,192.5)(150,192.5)
\psline[linewidth=0.4](150,212.5)(170,192.5)
\psline[linewidth=0.4](130,212.5)(150,192.5)
\psline[linewidth=0.4](160,192.5)(160,160)
\rput(150,240){$\Dott$}
\psline[linewidth=0.4](135,255)(165,225)
\psline[linewidth=0.4](135,255)(135,225)
\psline[linewidth=1.45](160,202.5)(160,225)
\psline[linewidth=0.4](165,225)(135,225)
\psline[linewidth=0.4](140,225)(140,220)
\psline[linewidth=0.4](125,210)(160,175)
\rput(160,175){$\Dott$}
\newrgbcolor{userLineColour}{1 0 0.2}
\psline[linewidth=0.2,linecolor=userLineColour](140,260)(175,225)
\newrgbcolor{userLineColour}{1 0 0.2}
\psline[linewidth=0.2,linecolor=userLineColour](175,170)(175,225)
\newrgbcolor{userLineColour}{1 0 0.2}
\psline[linewidth=0.2,linecolor=userLineColour](116.25,170)(116.25,260)
\newrgbcolor{userLineColour}{1 0 0.2}
\psline[linewidth=0.2,linecolor=userLineColour](175,170)(116.25,170)
\rput(143.75,232.5){$\prrrr$}
\rput(168.75,211.25){$\PadFee$}
\psline[linewidth=0.4](150,212.5)(130,212.5)
\psline[linewidth=0.4](140,220)(125,215)
\psline[linewidth=0.4](125,215)(125,210)
\psline[linewidth=1.45,border=0.65](133.75,193.75)(141.25,201.25)
\psline[linewidth=0.4](142.5,183.75)(122.5,183.75)
\psline[linewidth=0.4](122.5,203.75)(142.5,183.75)
\psline[linewidth=0.4](122.5,203.75)(122.5,183.75)
\rput(128.75,190){$\programm$}
\newrgbcolor{userLineColour}{1 0 0.2}
\psline[linewidth=0.2,linecolor=userLineColour](116.25,260)(140,260)
\psline[linewidth=0.4](50,230)(20,230)
\psline[linewidth=0.4](50,230)(50,200)
\psline[linewidth=0.4](20,230)(50,200)
\rput(38.12,225){$\pjjjj$}
\psline[linewidth=0.4](25,235)(25,230)
\psline[linewidth=1.45](45,230)(45,260)
\rput(25,235){$\Dott$}
\rput(110,150){\EQLS}
\rput(18.12,33.12){$\Dott$}
\rput(133.12,193.12){$\Dott$}
\psline[linewidth=0.4](60,275)(30,275)
\psline[linewidth=0.4](60,275)(60,245)
\psline[linewidth=0.4](30,275)(60,245)
\rput(48.12,270){$\pjjjj$}
\psline[linewidth=0.4](35,300)(35,275)
\psline[linewidth=1.45](55,275)(55,280)
\rput(55,280){$\Dott$}
\psline[linewidth=0.4](165,275)(135,275)
\psline[linewidth=0.4](165,275)(165,245)
\psline[linewidth=0.4](135,275)(165,245)
\rput(153.12,270){$\pjjjj$}
\psline[linewidth=0.4](140,300)(140,275)
\psline[linewidth=1.45](160,275)(160,280)
\rput(160,280){$\Dott$}
\psline[linewidth=0.4](300,160)(300,140)
\psline[linewidth=0.4](250,160)(300,160)
\psline[linewidth=0.4](290,140)(290,0)
\psline[linewidth=0.4](290,300)(290,160)
\psline[linewidth=0.4](300,140)(250,140)
\rput[l](293.75,298.75){$\Cee$}
\rput[r](256.25,2.5){$\Aee$}
\rput[r](285,2.5){$\Bee$}
\psline[linewidth=0.4](250,160)(250,140)
\psline[linewidth=0.4](260,140)(260,0)
\rput(275,150){$\quu$}
\rput[l](263.75,300){$\Aee$}
\psline[linewidth=0.4](260,300)(260,160)
\rput[l](38.75,298.75){$\Aee$}
\rput[l](143.75,298.75){$\Aee$}
\end{pspicture}


==> PIC/losless.tex <==
%%Created by jPicEdt 1.4.1_03: mixed JPIC-XML/LaTeX format
%%Mon Jan 09 19:15:05 GMT-10:00 2023
%%Begin JPIC-XML
%<?xml version="1.0" standalone="yes"?>
%<jpic x-min="0" x-max="290" y-min="0" y-max="240" auto-bounding="true">
%<multicurve fill-style= "none"
%	 points= "(70,160);(70,160);(70,140);(70,140)"
%	 stroke-width= "0.4"
%	 />
%<multicurve fill-style= "none"
%	 points= "(35,130);(35,130);(5,130);(5,130)"
%	 stroke-width= "0.4"
%	 />
%<multicurve fill-style= "none"
%	 points= "(40,160);(40,160);(70,160);(70,160)"
%	 stroke-width= "0.4"
%	 />
%<multicurve fill-style= "none"
%	 points= "(60,140);(60,140);(60,0);(60,0)"
%	 stroke-width= "0.4"
%	 />
%<multicurve fill-style= "none"
%	 points= "(60,240);(60,240);(60,160);(60,160)"
%	 stroke-width= "0.4"
%	 />
%<multicurve fill-style= "none"
%	 points= "(35,130);(35,130);(35,100);(35,100)"
%	 stroke-width= "0.4"
%	 />
%<multicurve fill-style= "none"
%	 points= "(10,190);(10,190);(10,130);(10,130)"
%	 stroke-width= "0.4"
%	 />
%<multicurve fill-style= "none"
%	 points= "(70,140);(70,140);(40,140);(40,140)"
%	 stroke-width= "0.4"
%	 />
%<multicurve fill-style= "none"
%	 points= "(20,160);(20,160);(40,140);(40,140)"
%	 stroke-width= "0.4"
%	 />
%<multicurve fill-style= "none"
%	 points= "(5,130);(5,130);(35,100);(35,100)"
%	 stroke-width= "0.4"
%	 />
%<multicurve fill-style= "none"
%	 points= "(30,130);(30,130);(30,150);(30,150)"
%	 stroke-width= "1.45"
%	 />
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(50,150)"
%	 stroke-width= "0.4"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\Univ$
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(97.5,150)"
%	 stroke-width= "0.4"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\EQLS
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(65,238.75)"
%	 stroke-width= "0.4"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\Cee$
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(26.25,45)"
%	 stroke-width= "0.4"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\Fee$
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(26.25,2.5)"
%	 stroke-width= "0.4"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\Aee$
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(55,2.5)"
%	 stroke-width= "0.4"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\Bee$
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(20,205)"
%	 stroke-width= "0.4"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\Dott$
%</text>
%<multicurve fill-style= "none"
%	 points= "(20,180);(20,180);(40,160);(40,160)"
%	 stroke-width= "0.4"
%	 />
%<multicurve fill-style= "none"
%	 points= "(20,180);(20,180);(20,160);(20,160)"
%	 stroke-width= "0.4"
%	 />
%<multicurve fill-style= "none"
%	 points= "(30,170);(30,170);(30,190);(30,190)"
%	 stroke-width= "1.45"
%	 />
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(25,238.75)"
%	 stroke-width= "0.4"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\Code$
%</text>
%<multicurve fill-style= "none"
%	 points= "(35,190);(35,190);(5,190);(5,190)"
%	 stroke-width= "0.4"
%	 />
%<multicurve fill-style= "none"
%	 points= "(20,80);(20,80);(20,115);(20,115)"
%	 stroke-width= "1.45"
%	 />
%<multicurve fill-style= "none"
%	 points= "(5,220);(5,220);(35,190);(35,190)"
%	 stroke-width= "0.4"
%	 />
%<multicurve fill-style= "none"
%	 points= "(5,220);(5,220);(5,190);(5,190)"
%	 stroke-width= "0.4"
%	 />
%<multicurve fill-style= "none"
%	 points= "(20,205);(20,205);(20,240);(20,240)"
%	 stroke-width= "1.45"
%	 />
%<multicurve fill-style= "none"
%	 stroke-color= "#ff0000"
%	 points= "(0,125);(0,125);(30,95);(30,95)"
%	 stroke-width= "0.2"
%	 />
%<multicurve fill-style= "none"
%	 stroke-color= "#ff0000"
%	 points= "(30,95);(30,95);(75,95);(75,95)"
%	 stroke-width= "0.2"
%	 />
%<multicurve fill-style= "none"
%	 stroke-color= "#ff0000"
%	 points= "(75,95);(75,95);(75,205);(75,205)"
%	 stroke-width= "0.2"
%	 />
%<multicurve fill-style= "none"
%	 stroke-color= "#ff0000"
%	 points= "(30,205);(30,205);(75,205);(75,205)"
%	 stroke-width= "0.2"
%	 />
%<multicurve fill-style= "none"
%	 stroke-color= "#ff0000"
%	 points= "(0,235);(0,235);(30,205);(30,205)"
%	 stroke-width= "0.2"
%	 />
%<multicurve fill-style= "none"
%	 stroke-color= "#ff0000"
%	 points= "(0,125);(0,125);(0,235);(0,235)"
%	 stroke-width= "0.2"
%	 />
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(30,50)"
%	 stroke-width= "0.4"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\Dott$
%</text>
%<multicurve fill-style= "none"
%	 points= "(40,40);(40,40);(20,40);(20,40)"
%	 stroke-width= "0.4"
%	 />
%<multicurve fill-style= "none"
%	 points= "(20,60);(20,60);(40,40);(40,40)"
%	 stroke-width= "0.4"
%	 />
%<multicurve fill-style= "none"
%	 points= "(20,60);(20,60);(20,40);(20,40)"
%	 stroke-width= "0.4"
%	 />
%<multicurve fill-style= "none"
%	 points= "(30,40);(30,40);(30,0);(30,0)"
%	 stroke-width= "0.4"
%	 />
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(20,80)"
%	 stroke-width= "0.4"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\Dott$
%</text>
%<multicurve fill-style= "none"
%	 points= "(5,95);(5,95);(35,65);(35,65)"
%	 stroke-width= "0.4"
%	 />
%<multicurve fill-style= "none"
%	 points= "(5,95);(5,95);(5,65);(5,65)"
%	 stroke-width= "0.4"
%	 />
%<multicurve fill-style= "none"
%	 points= "(30,50);(30,50);(30,65);(30,65)"
%	 stroke-width= "1.45"
%	 />
%<multicurve fill-style= "none"
%	 points= "(35,65);(35,65);(5,65);(5,65)"
%	 stroke-width= "0.4"
%	 />
%<multicurve fill-style= "none"
%	 points= "(10,65);(10,65);(10,30);(10,30)"
%	 stroke-width= "0.4"
%	 />
%<multicurve fill-style= "none"
%	 points= "(10,30);(10,30);(30,10);(30,10)"
%	 stroke-width= "0.4"
%	 />
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(30,10)"
%	 stroke-width= "0.4"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\Dott$
%</text>
%<multicurve fill-style= "none"
%	 points= "(180,160);(180,160);(180,140);(180,140)"
%	 stroke-width= "0.4"
%	 />
%<multicurve fill-style= "none"
%	 points= "(150,160);(150,160);(180,160);(180,160)"
%	 stroke-width= "0.4"
%	 />
%<multicurve fill-style= "none"
%	 points= "(170,140);(170,140);(170,0);(170,0)"
%	 stroke-width= "0.4"
%	 />
%<multicurve fill-style= "none"
%	 points= "(170,240);(170,240);(170,160);(170,160)"
%	 stroke-width= "0.4"
%	 />
%<multicurve fill-style= "none"
%	 points= "(120,190);(120,190);(120,120);(120,120)"
%	 stroke-width= "0.4"
%	 />
%<multicurve fill-style= "none"
%	 points= "(180,140);(180,140);(150,140);(150,140)"
%	 stroke-width= "0.4"
%	 />
%<multicurve fill-style= "none"
%	 points= "(130,160);(130,160);(150,140);(150,140)"
%	 stroke-width= "0.4"
%	 />
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(160,150)"
%	 stroke-width= "0.4"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\Univ$
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(202.5,150)"
%	 stroke-width= "0.4"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\EQLS
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(175,238.75)"
%	 stroke-width= "0.4"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\Cee$
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(136.25,135)"
%	 stroke-width= "0.4"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\Fee$
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(136.25,2.5)"
%	 stroke-width= "0.4"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\Aee$
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(165,2.5)"
%	 stroke-width= "0.4"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\Bee$
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(130,205)"
%	 stroke-width= "0.4"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\Dott$
%</text>
%<multicurve fill-style= "none"
%	 points= "(130,180);(130,180);(150,160);(150,160)"
%	 stroke-width= "0.4"
%	 />
%<multicurve fill-style= "none"
%	 points= "(130,180);(130,180);(130,160);(130,160)"
%	 stroke-width= "0.4"
%	 />
%<multicurve fill-style= "none"
%	 points= "(140,170);(140,170);(140,190);(140,190)"
%	 stroke-width= "1.45"
%	 />
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(135,238.75)"
%	 stroke-width= "0.4"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\Code$
%</text>
%<multicurve fill-style= "none"
%	 points= "(145,190);(145,190);(115,190);(115,190)"
%	 stroke-width= "0.4"
%	 />
%<multicurve fill-style= "none"
%	 points= "(115,220);(115,220);(145,190);(145,190)"
%	 stroke-width= "0.4"
%	 />
%<multicurve fill-style= "none"
%	 points= "(115,220);(115,220);(115,190);(115,190)"
%	 stroke-width= "0.4"
%	 />
%<multicurve fill-style= "none"
%	 points= "(130,205);(130,205);(130,240);(130,240)"
%	 stroke-width= "1.45"
%	 />
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(140,140)"
%	 stroke-width= "0.4"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\Dott$
%</text>
%<multicurve fill-style= "none"
%	 points= "(150,130);(150,130);(130,130);(130,130)"
%	 stroke-width= "0.4"
%	 />
%<multicurve fill-style= "none"
%	 points= "(130,150);(130,150);(150,130);(150,130)"
%	 stroke-width= "0.4"
%	 />
%<multicurve fill-style= "none"
%	 points= "(130,150);(130,150);(130,130);(130,130)"
%	 stroke-width= "0.4"
%	 />
%<multicurve fill-style= "none"
%	 points= "(140,130);(140,130);(140,0);(140,0)"
%	 stroke-width= "0.4"
%	 />
%<multicurve fill-style= "none"
%	 points= "(140,140);(140,140);(140,150);(140,150)"
%	 stroke-width= "1.45"
%	 />
%<multicurve fill-style= "none"
%	 points= "(120,120);(120,120);(140,100);(140,100)"
%	 stroke-width= "0.4"
%	 />
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(140,100)"
%	 stroke-width= "0.4"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\Dott$
%</text>
%<multicurve fill-style= "none"
%	 points= "(290,150);(290,150);(290,130);(290,130)"
%	 stroke-width= "0.4"
%	 />
%<multicurve fill-style= "none"
%	 points= "(240,150);(240,150);(290,150);(290,150)"
%	 stroke-width= "0.4"
%	 />
%<multicurve fill-style= "none"
%	 points= "(280,130);(280,130);(280,0);(280,0)"
%	 stroke-width= "0.4"
%	 />
%<multicurve fill-style= "none"
%	 points= "(280,240);(280,240);(280,150);(280,150)"
%	 stroke-width= "0.4"
%	 />
%<multicurve fill-style= "none"
%	 points= "(230,190);(230,190);(230,120);(230,120)"
%	 stroke-width= "0.4"
%	 />
%<multicurve fill-style= "none"
%	 points= "(290,130);(290,130);(240,130);(240,130)"
%	 stroke-width= "0.4"
%	 />
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(285,238.75)"
%	 stroke-width= "0.4"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\Cee$
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(246.25,170)"
%	 stroke-width= "0.4"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\Fee$
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(246.25,2.5)"
%	 stroke-width= "0.4"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\Aee$
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(275,2.5)"
%	 stroke-width= "0.4"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\Bee$
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(240,205)"
%	 stroke-width= "0.4"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\Dott$
%</text>
%<multicurve fill-style= "none"
%	 points= "(240,150);(240,150);(240,130);(240,130)"
%	 stroke-width= "0.4"
%	 />
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(245,238.75)"
%	 stroke-width= "0.4"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\Code$
%</text>
%<multicurve fill-style= "none"
%	 points= "(255,190);(255,190);(225,190);(225,190)"
%	 stroke-width= "0.4"
%	 />
%<multicurve fill-style= "none"
%	 points= "(225,220);(225,220);(255,190);(255,190)"
%	 stroke-width= "0.4"
%	 />
%<multicurve fill-style= "none"
%	 points= "(225,220);(225,220);(225,190);(225,190)"
%	 stroke-width= "0.4"
%	 />
%<multicurve fill-style= "none"
%	 points= "(240,205);(240,205);(240,240);(240,240)"
%	 stroke-width= "1.45"
%	 />
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(250,175)"
%	 stroke-width= "0.4"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\Dott$
%</text>
%<multicurve fill-style= "none"
%	 points= "(260,165);(260,165);(240,165);(240,165)"
%	 stroke-width= "0.4"
%	 />
%<multicurve fill-style= "none"
%	 points= "(240,185);(240,185);(260,165);(260,165)"
%	 stroke-width= "0.4"
%	 />
%<multicurve fill-style= "none"
%	 points= "(240,185);(240,185);(240,165);(240,165)"
%	 stroke-width= "0.4"
%	 />
%<multicurve fill-style= "none"
%	 points= "(250,130);(250,130);(250,0);(250,0)"
%	 stroke-width= "0.4"
%	 />
%<multicurve fill-style= "none"
%	 points= "(250,175);(250,175);(250,190);(250,190)"
%	 stroke-width= "1.45"
%	 />
%<multicurve fill-style= "none"
%	 points= "(230,120);(230,120);(250,100);(250,100)"
%	 stroke-width= "0.4"
%	 />
%<multicurve fill-style= "none"
%	 points= "(250,165);(250,165);(250,150);(250,150)"
%	 stroke-width= "0.4"
%	 />
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(250,100)"
%	 stroke-width= "0.4"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\Dott$
%</text>
%<multicurve fill-style= "none"
%	 stroke-color= "#ff0033"
%	 points= "(0,110);(0,110);(45,65);(45,65)"
%	 stroke-width= "0.2"
%	 />
%<multicurve fill-style= "none"
%	 stroke-color= "#ff0033"
%	 points= "(45,35);(45,35);(45,65);(45,65)"
%	 stroke-width= "0.2"
%	 />
%<multicurve fill-style= "none"
%	 stroke-color= "#ff0033"
%	 points= "(0,35);(0,35);(0,110);(0,110)"
%	 stroke-width= "0.2"
%	 />
%<multicurve fill-style= "none"
%	 stroke-color= "#ff0033"
%	 points= "(45,35);(45,35);(0,35);(0,35)"
%	 stroke-width= "0.2"
%	 />
%<multicurve fill-style= "none"
%	 stroke-color= "#ff0000"
%	 points= "(220,235);(220,235);(265,190);(265,190)"
%	 stroke-width= "0.2"
%	 />
%<multicurve fill-style= "none"
%	 stroke-color= "#ff0000"
%	 points= "(265,160);(265,160);(265,190);(265,190)"
%	 stroke-width= "0.2"
%	 />
%<multicurve fill-style= "none"
%	 stroke-color= "#ff0000"
%	 points= "(220,160);(220,160);(220,235);(220,235)"
%	 stroke-width= "0.2"
%	 />
%<multicurve fill-style= "none"
%	 stroke-color= "#ff0000"
%	 points= "(265,160);(265,160);(220,160);(220,160)"
%	 stroke-width= "0.2"
%	 />
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(265,140)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\quu$
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(233.75,197.5)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\prrrr$
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(123.75,197.5)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\prrrr$
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(13.75,72.5)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\prrrr$
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(13.75,196.25)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\prrrr$
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(23.12,125)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\pjjjj$
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(25,121.25)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(7.5,160)"
%	 stroke-width= "0.4"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\Aee$
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(116.25,160)"
%	 stroke-width= "0.4"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\Aee$
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(227.5,173.75)"
%	 stroke-width= "0.4"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\Aee$
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(247.5,155)"
%	 stroke-width= "0.4"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\Aee$
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(45,175)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\PadUniv$
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(258.75,185)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\PadFee$
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(38.75,58.75)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\PadFee$
%</text>
%</jpic>
%%End JPIC-XML
%PSTricks content-type (pstricks.sty package needed)
%Add \usepackage{pstricks} in the preamble of your LaTeX file
%You can rescale the whole picture (to 80% for instance) by using the command \def\JPicScale{0.8}
\ifx\JPicScale\undefined\def\JPicScale{1}\fi
\psset{unit=\JPicScale mm}
\psset{linewidth=0.3,dotsep=1,hatchwidth=0.3,hatchsep=1.5,shadowsize=1,dimen=middle}
\psset{dotsize=0.7 2.5,dotscale=1 1,fillcolor=black}
\psset{arrowsize=1 2,arrowlength=1,arrowinset=0.25,tbarsize=0.7 5,bracketlength=0.15,rbracketlength=0.15}
\begin{pspicture}(0,0)(290,240)
\psline[linewidth=0.4](70,160)(70,140)
\psline[linewidth=0.4](35,130)(5,130)
\psline[linewidth=0.4](40,160)(70,160)
\psline[linewidth=0.4](60,140)(60,0)
\psline[linewidth=0.4](60,240)(60,160)
\psline[linewidth=0.4](35,130)(35,100)
\psline[linewidth=0.4](10,190)(10,130)
\psline[linewidth=0.4](70,140)(40,140)
\psline[linewidth=0.4](20,160)(40,140)
\psline[linewidth=0.4](5,130)(35,100)
\psline[linewidth=1.45](30,130)(30,150)
\rput(50,150){$\Univ$}
\rput(97.5,150){\EQLS}
\rput[l](65,238.75){$\Cee$}
\rput(26.25,45){$\Fee$}
\rput[r](26.25,2.5){$\Aee$}
\rput[r](55,2.5){$\Bee$}
\rput(20,205){$\Dott$}
\psline[linewidth=0.4](20,180)(40,160)
\psline[linewidth=0.4](20,180)(20,160)
\psline[linewidth=1.45](30,170)(30,190)
\rput[l](25,238.75){$\Code$}
\psline[linewidth=0.4](35,190)(5,190)
\psline[linewidth=1.45](20,80)(20,115)
\psline[linewidth=0.4](5,220)(35,190)
\psline[linewidth=0.4](5,220)(5,190)
\psline[linewidth=1.45](20,205)(20,240)
\psline[linewidth=0.2,linecolor=red](0,125)(30,95)
\psline[linewidth=0.2,linecolor=red](30,95)(75,95)
\psline[linewidth=0.2,linecolor=red](75,95)(75,205)
\psline[linewidth=0.2,linecolor=red](30,205)(75,205)
\psline[linewidth=0.2,linecolor=red](0,235)(30,205)
\psline[linewidth=0.2,linecolor=red](0,125)(0,235)
\rput(30,50){$\Dott$}
\psline[linewidth=0.4](40,40)(20,40)
\psline[linewidth=0.4](20,60)(40,40)
\psline[linewidth=0.4](20,60)(20,40)
\psline[linewidth=0.4](30,40)(30,0)
\rput(20,80){$\Dott$}
\psline[linewidth=0.4](5,95)(35,65)
\psline[linewidth=0.4](5,95)(5,65)
\psline[linewidth=1.45](30,50)(30,65)
\psline[linewidth=0.4](35,65)(5,65)
\psline[linewidth=0.4](10,65)(10,30)
\psline[linewidth=0.4](10,30)(30,10)
\rput(30,10){$\Dott$}
\psline[linewidth=0.4](180,160)(180,140)
\psline[linewidth=0.4](150,160)(180,160)
\psline[linewidth=0.4](170,140)(170,0)
\psline[linewidth=0.4](170,240)(170,160)
\psline[linewidth=0.4](120,190)(120,120)
\psline[linewidth=0.4](180,140)(150,140)
\psline[linewidth=0.4](130,160)(150,140)
\rput(160,150){$\Univ$}
\rput(202.5,150){\EQLS}
\rput[l](175,238.75){$\Cee$}
\rput(136.25,135){$\Fee$}
\rput[r](136.25,2.5){$\Aee$}
\rput[r](165,2.5){$\Bee$}
\rput(130,205){$\Dott$}
\psline[linewidth=0.4](130,180)(150,160)
\psline[linewidth=0.4](130,180)(130,160)
\psline[linewidth=1.45](140,170)(140,190)
\rput[l](135,238.75){$\Code$}
\psline[linewidth=0.4](145,190)(115,190)
\psline[linewidth=0.4](115,220)(145,190)
\psline[linewidth=0.4](115,220)(115,190)
\psline[linewidth=1.45](130,205)(130,240)
\rput(140,140){$\Dott$}
\psline[linewidth=0.4](150,130)(130,130)
\psline[linewidth=0.4](130,150)(150,130)
\psline[linewidth=0.4](130,150)(130,130)
\psline[linewidth=0.4](140,130)(140,0)
\psline[linewidth=1.45](140,140)(140,150)
\psline[linewidth=0.4](120,120)(140,100)
\rput(140,100){$\Dott$}
\psline[linewidth=0.4](290,150)(290,130)
\psline[linewidth=0.4](240,150)(290,150)
\psline[linewidth=0.4](280,130)(280,0)
\psline[linewidth=0.4](280,240)(280,150)
\psline[linewidth=0.4](230,190)(230,120)
\psline[linewidth=0.4](290,130)(240,130)
\rput[l](285,238.75){$\Cee$}
\rput(246.25,170){$\Fee$}
\rput[r](246.25,2.5){$\Aee$}
\rput[r](275,2.5){$\Bee$}
\rput(240,205){$\Dott$}
\psline[linewidth=0.4](240,150)(240,130)
\rput[l](245,238.75){$\Code$}
\psline[linewidth=0.4](255,190)(225,190)
\psline[linewidth=0.4](225,220)(255,190)
\psline[linewidth=0.4](225,220)(225,190)
\psline[linewidth=1.45](240,205)(240,240)
\rput(250,175){$\Dott$}
\psline[linewidth=0.4](260,165)(240,165)
\psline[linewidth=0.4](240,185)(260,165)
\psline[linewidth=0.4](240,185)(240,165)
\psline[linewidth=0.4](250,130)(250,0)
\psline[linewidth=1.45](250,175)(250,190)
\psline[linewidth=0.4](230,120)(250,100)
\psline[linewidth=0.4](250,165)(250,150)
\rput(250,100){$\Dott$}
\newrgbcolor{userLineColour}{1 0 0.2}
\psline[linewidth=0.2,linecolor=userLineColour](0,110)(45,65)
\newrgbcolor{userLineColour}{1 0 0.2}
\psline[linewidth=0.2,linecolor=userLineColour](45,35)(45,65)
\newrgbcolor{userLineColour}{1 0 0.2}
\psline[linewidth=0.2,linecolor=userLineColour](0,35)(0,110)
\newrgbcolor{userLineColour}{1 0 0.2}
\psline[linewidth=0.2,linecolor=userLineColour](45,35)(0,35)
\psline[linewidth=0.2,linecolor=red](220,235)(265,190)
\psline[linewidth=0.2,linecolor=red](265,160)(265,190)
\psline[linewidth=0.2,linecolor=red](220,160)(220,235)
\psline[linewidth=0.2,linecolor=red](265,160)(220,160)
\rput(265,140){$\quu$}
\rput(233.75,197.5){$\prrrr$}
\rput(123.75,197.5){$\prrrr$}
\rput(13.75,72.5){$\prrrr$}
\rput(13.75,196.25){$\prrrr$}
\rput(23.12,125){$\pjjjj$}
\rput(25,121.25){}
\rput[r](7.5,160){$\Aee$}
\rput[r](116.25,160){$\Aee$}
\rput[r](227.5,173.75){$\Aee$}
\rput[r](247.5,155){$\Aee$}
\rput(45,175){$\PadUniv$}
\rput(258.75,185){$\PadFee$}
\rput(38.75,58.75){$\PadFee$}
\end{pspicture}


==> PIC/mach-1.tex <==
%%Created by jPicEdt 1.4.1_03: mixed JPIC-XML/LaTeX format
%%Tue Nov 07 13:07:34 HST 2017
%%Begin JPIC-XML
%<?xml version="1.0" standalone="yes"?>
%<jpic x-min="0" x-max="80" y-min="1.25" y-max="71.25" auto-bounding="true">
%<multicurve points= "(0,47.5);(0,47.5);(80,47.5);(80,47.5)"
%	 fill-style= "none"
%	 />
%<multicurve points= "(0,47.5);(0,47.5);(0,22.5);(0,22.5)"
%	 fill-style= "none"
%	 />
%<multicurve points= "(80,22.5);(80,22.5);(80,47.5);(80,47.5)"
%	 fill-style= "none"
%	 />
%<multicurve points= "(40,67.5);(40,67.5);(40,47.5);(40,47.5)"
%	 fill-style= "none"
%	 />
%<text text-vert-align= "center-v"
%	 anchor-point= "(40,71.25)"
%	 text-frame= "noframe"
%	 fill-style= "none"
%	 text-hor-align= "center-h"
%	 >
%$\nameslang$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(40,1.25)"
%	 text-frame= "noframe"
%	 fill-style= "none"
%	 text-hor-align= "center-h"
%	 >
%$\inputt$
%</text>
%<multicurve points= "(0,22.5);(0,22.5);(80,22.5);(80,22.5)"
%	 fill-style= "none"
%	 />
%<multicurve points= "(40,22.5);(40,22.5);(40,3.75);(40,3.75)"
%	 fill-style= "none"
%	 />
%<text text-vert-align= "center-v"
%	 anchor-point= "(40,35)"
%	 text-frame= "noframe"
%	 fill-style= "none"
%	 text-hor-align= "center-h"
%	 >
%\machine
%</text>
%</jpic>
%%End JPIC-XML
%PSTricks content-type (pstricks.sty package needed)
%Add \usepackage{pstricks} in the preamble of your LaTeX file
%You can rescale the whole picture (to 80% for instance) by using the command \def\JPicScale{0.8}
\ifx\JPicScale\undefined\def\JPicScale{1}\fi
\psset{unit=\JPicScale mm}
\psset{linewidth=0.3,dotsep=1,hatchwidth=0.3,hatchsep=1.5,shadowsize=1,dimen=middle}
\psset{dotsize=0.7 2.5,dotscale=1 1,fillcolor=black}
\psset{arrowsize=1 2,arrowlength=1,arrowinset=0.25,tbarsize=0.7 5,bracketlength=0.15,rbracketlength=0.15}
\begin{pspicture}(0,0)(80,71.25)
\psline(0,47.5)(80,47.5)
\psline(0,47.5)(0,22.5)
\psline(80,22.5)(80,47.5)
\psline(40,67.5)(40,47.5)
\rput(40,71.25){$\nameslang$}
\rput(40,1.25){$\inputt$}
\psline(0,22.5)(80,22.5)
\psline(40,22.5)(40,3.75)
\rput(40,35){\machine}
\end{pspicture}


==> PIC/mach-2.tex <==
%%Created by jPicEdt 1.4.1_03: mixed JPIC-XML/LaTeX format
%%Sun Nov 15 19:32:38 GMT-10:00 2020
%%Begin JPIC-XML
%<?xml version="1.0" standalone="yes"?>
%<jpic x-min="0" x-max="40" y-min="1.25" y-max="71.25" auto-bounding="true">
%<multicurve fill-style= "none"
%	 points= "(0,47.5);(0,47.5);(40,47.5);(40,47.5)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(0,47.5);(0,47.5);(0,22.5);(0,22.5)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(40,22.5);(40,22.5);(40,47.5);(40,47.5)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(20,67.5);(20,67.5);(20,47.5);(20,47.5)"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(20,71.25)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\nameslang$
%</text>
%<multicurve fill-style= "none"
%	 points= "(0,22.5);(0,22.5);(40,22.5);(40,22.5)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(10,22.5);(10,22.5);(10,3.75);(10,3.75)"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(20,35)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\machine
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(30,1.25)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\inputt$
%</text>
%<multicurve fill-style= "none"
%	 points= "(30,22.5);(30,22.5);(30,3.75);(30,3.75)"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(10,1.25)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\inputtt$
%</text>
%</jpic>
%%End JPIC-XML
%LaTeX-picture environment using emulated lines and arcs
%You can rescale the whole picture (to 80% for instance) by using the command \def\JPicScale{0.8}
\ifx\JPicScale\undefined\def\JPicScale{1}\fi
\unitlength \JPicScale mm
\begin{picture}(40,71.25)(0,0)
\linethickness{0.3mm}
\put(0,47.5){\line(1,0){40}}
\linethickness{0.3mm}
\put(0,22.5){\line(0,1){25}}
\linethickness{0.3mm}
\put(40,22.5){\line(0,1){25}}
\linethickness{0.3mm}
\put(20,47.5){\line(0,1){20}}
\put(20,71.25){\makebox(0,0)[cc]{$\nameslang$}}

\linethickness{0.3mm}
\put(0,22.5){\line(1,0){40}}
\linethickness{0.3mm}
\put(10,3.75){\line(0,1){18.75}}
\put(20,35){\makebox(0,0)[cc]{\machine}}

\put(30,1.25){\makebox(0,0)[cc]{$\inputt$}}

\linethickness{0.3mm}
\put(30,3.75){\line(0,1){18.75}}
\put(10,1.25){\makebox(0,0)[cc]{$\inputtt$}}

\end{picture}


==> PIC/mach-M.tex <==
%%Created by jPicEdt 1.4.1_03: mixed JPIC-XML/LaTeX format
%%Tue Nov 05 13:44:42 GMT-10:00 2019
%%Begin JPIC-XML
%<?xml version="1.0" standalone="yes"?>
%<jpic x-min="0" x-max="40" y-min="1.25" y-max="71.25" auto-bounding="true">
%<multicurve fill-style= "none"
%	 points= "(0,47.5);(0,47.5);(0,22.5);(0,22.5)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(40,22.5);(40,22.5);(40,47.5);(40,47.5)"
%	 />
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(20,71.25)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\nameslang$
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(20,1.25)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\inputt$
%</text>
%<multicurve fill-style= "none"
%	 points= "(0,22.5);(0,22.5);(40,22.5);(40,22.5)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(20,22.5);(20,22.5);(20,3.75);(20,3.75)"
%	 />
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(20,35)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\machine
%</text>
%<parallelogram fill-style= "solid"
%	 p3= "(17.5,47.5)"
%	 fill-color= "#999999"
%	 p2= "(17.5,67.5)"
%	 p1= "(22.5,67.5)"
%	 stroke-color= "#999999"
%	 stroke-width= "0.1"
%	 />
%<multicurve fill-style= "none"
%	 points= "(0,47.5);(0,47.5);(40,47.5);(40,47.5)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(20,67.5);(20,67.5);(20,47.5);(20,47.5)"
%	 />
%</jpic>
%%End JPIC-XML
%PSTricks content-type (pstricks.sty package needed)
%Add \usepackage{pstricks} in the preamble of your LaTeX file
%You can rescale the whole picture (to 80% for instance) by using the command \def\JPicScale{0.8}
\ifx\JPicScale\undefined\def\JPicScale{1}\fi
\psset{unit=\JPicScale mm}
\psset{linewidth=0.3,dotsep=1,hatchwidth=0.3,hatchsep=1.5,shadowsize=1,dimen=middle}
\psset{dotsize=0.7 2.5,dotscale=1 1,fillcolor=black}
\psset{arrowsize=1 2,arrowlength=1,arrowinset=0.25,tbarsize=0.7 5,bracketlength=0.15,rbracketlength=0.15}
\begin{pspicture}(0,0)(40,71.25)
\psline(0,47.5)(0,22.5)
\psline(40,22.5)(40,47.5)
\rput(20,71.25){$\nameslang$}
\rput(20,1.25){$\inputt$}
\psline(0,22.5)(40,22.5)
\psline(20,22.5)(20,3.75)
\rput(20,35){\machine}
\newrgbcolor{userLineColour}{0.6 0.6 0.6}
\newrgbcolor{userFillColour}{0.6 0.6 0.6}
\pspolygon[linewidth=0.1,linecolor=userLineColour,fillcolor=userFillColour,fillstyle=solid](22.5,67.5)(17.5,67.5)(17.5,47.5)(22.5,47.5)
\psline(0,47.5)(40,47.5)
\psline(20,67.5)(20,47.5)
\end{pspicture}


==> PIC/mach-beh.tex <==
%%Created by jPicEdt 1.4.1_03: mixed JPIC-XML/LaTeX format
%%Sat Jan 14 18:22:03 GMT 2012
%%Begin JPIC-XML
%<?xml version="1.0" standalone="yes"?>
%<jpic x-min="-1" x-max="70" y-min="0" y-max="40" auto-bounding="true">
%<text text-vert-align= "center-v"
%	 anchor-point= "(-1,40)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%\Machines
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(2,0)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%\Languages
%</text>
%<multicurve stroke-width= "0.4"
%	 fill-style= "none"
%	 arrow-head-width-minimum= "1.05"
%	 right-arrow= "head"
%	 points= "(20,35);(20,35);(20,5);(20,5)"
%	 arrow-head-length-scale= "2"
%	 />
%<text text-vert-align= "center-v"
%	 anchor-point= "(22,20)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\accept$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(70,25)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\nothing
%</text>
%</jpic>
%%End JPIC-XML
%PSTricks content-type (pstricks.sty package needed)
%Add \usepackage{pstricks} in the preamble of your LaTeX file
%You can rescale the whole picture (to 80% for instance) by using the command \def\JPicScale{0.8}
\ifx\JPicScale\undefined\def\JPicScale{1}\fi
\psset{unit=\JPicScale mm}
\psset{linewidth=0.3,dotsep=1,hatchwidth=0.3,hatchsep=1.5,shadowsize=1,dimen=middle}
\psset{dotsize=0.7 2.5,dotscale=1 1,fillcolor=black}
\psset{arrowsize=1 2,arrowlength=1,arrowinset=0.25,tbarsize=0.7 5,bracketlength=0.15,rbracketlength=0.15}
\begin{pspicture}(0,0)(70,40)
\rput[l](-1,40){\Machines}
\rput[l](2,0){\Languages}
\psline[linewidth=0.4,arrowsize=1.05 2,arrowlength=2]{->}(20,35)(20,5)
\rput[l](22,20){$\accept$}
\rput(70,25){\nothing}
\end{pspicture}


==> PIC/mach-lang-epi.tex <==
%%Created by jPicEdt 1.4.1_03: mixed JPIC-XML/LaTeX format
%%Wed Jan 11 10:54:35 GMT 2012
%%Begin JPIC-XML
%<?xml version="1.0" standalone="yes"?>
%<jpic x-min="20" x-max="22" y-min="0" y-max="40" auto-bounding="true">
%<text text-vert-align= "center-v"
%	 anchor-point= "(20,40)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\Machines
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(20,0)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\Languages
%</text>
%<multicurve stroke-width= "0.4"
%	 fill-style= "none"
%	 arrow-head-width-minimum= "1.05"
%	 right-arrow= "double-head"
%	 points= "(20,35);(20,35);(20,5);(20,5)"
%	 arrow-head-length-scale= "2"
%	 />
%<text text-vert-align= "center-v"
%	 anchor-point= "(22,21)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\accept$
%</text>
%</jpic>
%%End JPIC-XML
%PSTricks content-type (pstricks.sty package needed)
%Add \usepackage{pstricks} in the preamble of your LaTeX file
%You can rescale the whole picture (to 80% for instance) by using the command \def\JPicScale{0.8}
\ifx\JPicScale\undefined\def\JPicScale{1}\fi
\psset{unit=\JPicScale mm}
\psset{linewidth=0.3,dotsep=1,hatchwidth=0.3,hatchsep=1.5,shadowsize=1,dimen=middle}
\psset{dotsize=0.7 2.5,dotscale=1 1,fillcolor=black}
\psset{arrowsize=1 2,arrowlength=1,arrowinset=0.25,tbarsize=0.7 5,bracketlength=0.15,rbracketlength=0.15}
\begin{pspicture}(0,0)(22,40)
\rput(20,40){\Machines}
\rput(20,0){\Languages}
\psline[linewidth=0.4,arrowsize=1.05 2,arrowlength=2]{->>}(20,35)(20,5)
\rput[l](22,21){$\accept$}
\end{pspicture}


==> PIC/mach-lang.tex <==
%%Created by jPicEdt 1.4.1_03: mixed JPIC-XML/LaTeX format
%%Tue Jan 10 19:23:24 GMT 2012
%%Begin JPIC-XML
%<?xml version="1.0" standalone="yes"?>
%<jpic x-min="20" x-max="22" y-min="0" y-max="40" auto-bounding="true">
%<text text-vert-align= "center-v"
%	 anchor-point= "(20,40)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\Machines
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(20,0)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\Languages
%</text>
%<multicurve stroke-width= "0.4"
%	 fill-style= "none"
%	 arrow-head-width-minimum= "1.05"
%	 right-arrow= "head"
%	 points= "(20,35);(20,35);(20,5);(20,5)"
%	 arrow-head-length-scale= "2"
%	 />
%<text text-vert-align= "center-v"
%	 anchor-point= "(22,21)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\accept$
%</text>
%</jpic>
%%End JPIC-XML
%PSTricks content-type (pstricks.sty package needed)
%Add \usepackage{pstricks} in the preamble of your LaTeX file
%You can rescale the whole picture (to 80% for instance) by using the command \def\JPicScale{0.8}
\ifx\JPicScale\undefined\def\JPicScale{1}\fi
\psset{unit=\JPicScale mm}
\psset{linewidth=0.3,dotsep=1,hatchwidth=0.3,hatchsep=1.5,shadowsize=1,dimen=middle}
\psset{dotsize=0.7 2.5,dotscale=1 1,fillcolor=black}
\psset{arrowsize=1 2,arrowlength=1,arrowinset=0.25,tbarsize=0.7 5,bracketlength=0.15,rbracketlength=0.15}
\begin{pspicture}(0,0)(22,40)
\rput(20,40){\Machines}
\rput(20,0){\Languages}
\psline[linewidth=0.4,arrowsize=1.05 2,arrowlength=2]{->}(20,35)(20,5)
\rput[l](22,21){$\accept$}
\end{pspicture}


==> PIC/mach.tex <==
%%Created by jPicEdt 1.4.1_03: mixed JPIC-XML/LaTeX format
%%Tue Nov 07 13:08:38 HST 2017
%%Begin JPIC-XML
%<?xml version="1.0" standalone="yes"?>
%<jpic x-min="0" x-max="40" y-min="1.25" y-max="71.25" auto-bounding="true">
%<multicurve points= "(0,47.5);(0,47.5);(40,47.5);(40,47.5)"
%	 fill-style= "none"
%	 />
%<multicurve points= "(0,47.5);(0,47.5);(0,22.5);(0,22.5)"
%	 fill-style= "none"
%	 />
%<multicurve points= "(40,22.5);(40,22.5);(40,47.5);(40,47.5)"
%	 fill-style= "none"
%	 />
%<multicurve points= "(20,67.5);(20,67.5);(20,47.5);(20,47.5)"
%	 fill-style= "none"
%	 />
%<text text-vert-align= "center-v"
%	 anchor-point= "(20,71.25)"
%	 text-frame= "noframe"
%	 fill-style= "none"
%	 text-hor-align= "center-h"
%	 >
%$\nameslang$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(20,1.25)"
%	 text-frame= "noframe"
%	 fill-style= "none"
%	 text-hor-align= "center-h"
%	 >
%$\inputt$
%</text>
%<multicurve points= "(0,22.5);(0,22.5);(40,22.5);(40,22.5)"
%	 fill-style= "none"
%	 />
%<multicurve points= "(20,22.5);(20,22.5);(20,3.75);(20,3.75)"
%	 fill-style= "none"
%	 />
%<text text-vert-align= "center-v"
%	 anchor-point= "(20,35)"
%	 text-frame= "noframe"
%	 fill-style= "none"
%	 text-hor-align= "center-h"
%	 >
%\machine
%</text>
%</jpic>
%%End JPIC-XML
%PSTricks content-type (pstricks.sty package needed)
%Add \usepackage{pstricks} in the preamble of your LaTeX file
%You can rescale the whole picture (to 80% for instance) by using the command \def\JPicScale{0.8}
\ifx\JPicScale\undefined\def\JPicScale{1}\fi
\psset{unit=\JPicScale mm}
\psset{linewidth=0.3,dotsep=1,hatchwidth=0.3,hatchsep=1.5,shadowsize=1,dimen=middle}
\psset{dotsize=0.7 2.5,dotscale=1 1,fillcolor=black}
\psset{arrowsize=1 2,arrowlength=1,arrowinset=0.25,tbarsize=0.7 5,bracketlength=0.15,rbracketlength=0.15}
\begin{pspicture}(0,0)(40,71.25)
\psline(0,47.5)(40,47.5)
\psline(0,47.5)(0,22.5)
\psline(40,22.5)(40,47.5)
\psline(20,67.5)(20,47.5)
\rput(20,71.25){$\nameslang$}
\rput(20,1.25){$\inputt$}
\psline(0,22.5)(40,22.5)
\psline(20,22.5)(20,3.75)
\rput(20,35){\machine}
\end{pspicture}


==> PIC/numberb-1.tex <==
%%Created by jPicEdt 1.4.1_03: mixed JPIC-XML/LaTeX format
%%Sun Oct 09 12:08:29 HST 2016
%%Begin JPIC-XML
%<?xml version="1.0" standalone="yes"?>
%<jpic x-min="0" x-max="60" y-min="0" y-max="70" auto-bounding="true">
%<multicurve stroke-width= "0.6"
%	 fill-style= "none"
%	 points= "(0,60);(0,60);(60,60);(60,60)"
%	 />
%<multicurve stroke-width= "0.6"
%	 fill-style= "none"
%	 points= "(60,40);(60,40);(60,60);(60,60)"
%	 />
%<multicurve stroke-width= "0.6"
%	 fill-style= "none"
%	 points= "(0,40);(0,40);(60,40);(60,40)"
%	 />
%<multicurve stroke-width= "0.6"
%	 fill-style= "none"
%	 points= "(0,60);(0,60);(0,40);(0,40)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(30,70);(30,70);(30,60);(30,60)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(12.5,39.38);(12.5,39.38);(12.5,17.5);(12.5,17.5)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(0,5);(0,5);(25,5);(25,5)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(0,5);(0,5);(0,30);(0,30)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(0,30);(0,30);(25,5);(25,5)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(47.5,39.38);(47.5,39.38);(47.5,0);(47.5,0)"
%	 />
%<text text-vert-align= "center-v"
%	 anchor-point= "(30,50)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\pairtag$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(7.5,12.5)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\toptag$
%</text>
%</jpic>
%%End JPIC-XML
%PSTricks content-type (pstricks.sty package needed)
%Add \usepackage{pstricks} in the preamble of your LaTeX file
%You can rescale the whole picture (to 80% for instance) by using the command \def\JPicScale{0.8}
\ifx\JPicScale\undefined\def\JPicScale{1}\fi
\psset{unit=\JPicScale mm}
\psset{linewidth=0.3,dotsep=1,hatchwidth=0.3,hatchsep=1.5,shadowsize=1,dimen=middle}
\psset{dotsize=0.7 2.5,dotscale=1 1,fillcolor=black}
\psset{arrowsize=1 2,arrowlength=1,arrowinset=0.25,tbarsize=0.7 5,bracketlength=0.15,rbracketlength=0.15}
\begin{pspicture}(0,0)(60,70)
\psline[linewidth=0.6](0,60)(60,60)
\psline[linewidth=0.6](60,40)(60,60)
\psline[linewidth=0.6](0,40)(60,40)
\psline[linewidth=0.6](0,60)(0,40)
\psline[linewidth=0.75](30,70)(30,60)
\psline[linewidth=0.75](12.5,39.38)(12.5,17.5)
\psline[linewidth=0.75](0,5)(25,5)
\psline[linewidth=0.75](0,5)(0,30)
\psline[linewidth=0.75](0,30)(25,5)
\psline[linewidth=0.75](47.5,39.38)(47.5,0)
\rput(30,50){$\pairtag$}
\rput(7.5,12.5){$\toptag$}
\end{pspicture}


==> PIC/numberb-2.tex <==
%%Created by jPicEdt 1.4.1_03: mixed JPIC-XML/LaTeX format
%%Sun Dec 23 08:42:40 GMT-10:00 2018
%%Begin JPIC-XML
%<?xml version="1.0" standalone="yes"?>
%<jpic x-min="7.5" x-max="352.5" y-min="-10" y-max="112.5" auto-bounding="true">
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(270,60)"
%	 stroke-width= "0.75"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\EQLS
%</text>
%<multicurve fill-style= "none"
%	 points= "(10,85);(10,85);(50,85);(50,85)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(50,65);(50,65);(50,85);(50,85)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(40,95);(40,95);(40,85);(40,85)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(30,65);(30,65);(50,65);(50,65)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(20,75);(20,75);(20,7.5);(20,7.5)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(10,85);(10,85);(30,65);(30,65)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(7.5,-5);(7.5,-5);(32.5,-5);(32.5,-5)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(7.5,-5);(7.5,-5);(7.5,20);(7.5,20)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(7.5,20);(7.5,20);(32.5,-5);(32.5,-5)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(40,65);(40,65);(40,-10);(40,-10)"
%	 stroke-width= "0.75"
%	 />
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(65,60)"
%	 stroke-width= "0.75"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\EQLS
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(16.25,2.5)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\oone$
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(35,75)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\ueval$
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(235,1.88)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\nextt$
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(335,2.5)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\enn$
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(320,30)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\bottag$
%</text>
%<multicurve fill-style= "none"
%	 points= "(95,25);(95,25);(115,25);(115,25)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(95,25);(95,25);(95,45);(95,45)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(95,45);(95,45);(115,25);(115,25)"
%	 stroke-width= "0.75"
%	 />
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(100,30)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\toptag$
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(65,112.5)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\leqn$
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(270,112.5)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\reqn$
%</text>
%<multicurve fill-style= "none"
%	 points= "(80,70);(80,70);(110,70);(110,70)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(130,50);(130,50);(110,70);(110,70)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(120,75);(120,75);(120,60);(120,60)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(100,50);(100,50);(130,50);(130,50)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(105,50);(105,50);(105,35);(105,35)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(90,60);(90,60);(80,50);(80,50)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(80,70);(80,70);(100,50);(100,50)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(70,45);(70,45);(90,25);(90,25)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(70,25);(70,25);(89.38,25);(89.38,25)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(70,25);(70,25);(70,44.99);(70,44.99)"
%	 stroke-width= "0.75"
%	 />
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(75,30)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\iiftag$
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(105,60)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\stag$
%</text>
%<multicurve fill-style= "none"
%	 points= "(110,85);(110,85);(150,85);(150,85)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(150,65);(150,65);(150,85);(150,85)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(140,95);(140,95);(140,85);(140,85)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(130,65);(130,65);(150,65);(150,65)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(110,85);(110,85);(130,65);(130,65)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(140,65);(140,65);(140,-10);(140,-10)"
%	 stroke-width= "0.75"
%	 />
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(135,75)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\ueval$
%</text>
%<multicurve fill-style= "none"
%	 points= "(80,50);(80,50);(80,35);(80,35)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(122.5,50);(122.5,50);(122.5,7.5);(122.5,7.5)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(110,-5);(110,-5);(135,-5);(135,-5)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(110,-5);(110,-5);(110,20);(110,20)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(110,20);(110,20);(135,-5);(135,-5)"
%	 stroke-width= "0.75"
%	 />
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(118.75,2.5)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\oone$
%</text>
%<multicurve fill-style= "none"
%	 points= "(240,95);(240,95);(240,7.5);(240,7.5)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(227.5,-5);(227.5,-5);(252.5,-5);(252.5,-5)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(227.5,-5);(227.5,-5);(227.5,20);(227.5,20)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(227.5,20);(227.5,20);(252.5,-5);(252.5,-5)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(312.5,25);(312.5,25);(332.5,25);(332.5,25)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(312.5,25);(312.5,25);(312.5,45);(312.5,45)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(312.5,45);(312.5,45);(332.5,25);(332.5,25)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(297.5,70);(297.5,70);(327.5,70);(327.5,70)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(347.5,50);(347.5,50);(327.5,70);(327.5,70)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(337.5,95);(337.5,95);(337.5,60);(337.5,60)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(318.12,50);(318.12,50);(347.5,50);(347.5,50)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(322.5,50);(322.5,50);(322.5,35);(322.5,35)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(307.5,60);(307.5,60);(297.5,50);(297.5,50)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(297.5,70);(297.5,70);(317.5,50);(317.5,50)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(287.5,45);(287.5,45);(307.5,25);(307.5,25)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(287.5,25);(287.5,25);(306.88,25);(306.88,25)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(287.5,25);(287.5,25);(287.5,44.99);(287.5,44.99)"
%	 stroke-width= "0.75"
%	 />
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(292.5,30)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\iiftag$
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(322.5,60)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\stag$
%</text>
%<multicurve fill-style= "none"
%	 points= "(297.5,50);(297.5,50);(297.5,35);(297.5,35)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(340,50);(340,50);(340,7.5);(340,7.5)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(327.5,-5);(327.5,-5);(352.5,-5);(352.5,-5)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(327.5,-5);(327.5,-5);(327.5,20);(327.5,20)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(327.5,20);(327.5,20);(352.5,-5);(352.5,-5)"
%	 stroke-width= "0.75"
%	 />
%</jpic>
%%End JPIC-XML
%PSTricks content-type (pstricks.sty package needed)
%Add \usepackage{pstricks} in the preamble of your LaTeX file
%You can rescale the whole picture (to 80% for instance) by using the command \def\JPicScale{0.8}
\ifx\JPicScale\undefined\def\JPicScale{1}\fi
\psset{unit=\JPicScale mm}
\psset{linewidth=0.3,dotsep=1,hatchwidth=0.3,hatchsep=1.5,shadowsize=1,dimen=middle}
\psset{dotsize=0.7 2.5,dotscale=1 1,fillcolor=black}
\psset{arrowsize=1 2,arrowlength=1,arrowinset=0.25,tbarsize=0.7 5,bracketlength=0.15,rbracketlength=0.15}
\begin{pspicture}(0,0)(352.5,112.5)
\rput(270,60){\EQLS}
\psline[linewidth=0.75](10,85)(50,85)
\psline[linewidth=0.75](50,65)(50,85)
\psline[linewidth=0.75](40,95)(40,85)
\psline[linewidth=0.75](30,65)(50,65)
\psline[linewidth=0.75](20,75)(20,7.5)
\psline[linewidth=0.75](10,85)(30,65)
\psline[linewidth=0.75](7.5,-5)(32.5,-5)
\psline[linewidth=0.75](7.5,-5)(7.5,20)
\psline[linewidth=0.75](7.5,20)(32.5,-5)
\psline[linewidth=0.75](40,65)(40,-10)
\rput(65,60){\EQLS}
\rput(16.25,2.5){$\oone$}
\rput(35,75){$\ueval$}
\rput(235,1.88){$\nextt$}
\rput(335,2.5){$\enn$}
\rput(320,30){$\bottag$}
\psline[linewidth=0.75](95,25)(115,25)
\psline[linewidth=0.75](95,25)(95,45)
\psline[linewidth=0.75](95,45)(115,25)
\rput(100,30){$\toptag$}
\rput(65,112.5){$\leqn$}
\rput(270,112.5){$\reqn$}
\psline[linewidth=0.75](80,70)(110,70)
\psline[linewidth=0.75](130,50)(110,70)
\psline[linewidth=0.75](120,75)(120,60)
\psline[linewidth=0.75](100,50)(130,50)
\psline[linewidth=0.75](105,50)(105,35)
\psline[linewidth=0.75](90,60)(80,50)
\psline[linewidth=0.75](80,70)(100,50)
\psline[linewidth=0.75](70,45)(90,25)
\psline[linewidth=0.75](70,25)(89.38,25)
\psline[linewidth=0.75](70,25)(70,44.99)
\rput(75,30){$\iiftag$}
\rput(105,60){$\stag$}
\psline[linewidth=0.75](110,85)(150,85)
\psline[linewidth=0.75](150,65)(150,85)
\psline[linewidth=0.75](140,95)(140,85)
\psline[linewidth=0.75](130,65)(150,65)
\psline[linewidth=0.75](110,85)(130,65)
\psline[linewidth=0.75](140,65)(140,-10)
\rput(135,75){$\ueval$}
\psline[linewidth=0.75](80,50)(80,35)
\psline[linewidth=0.75](122.5,50)(122.5,7.5)
\psline[linewidth=0.75](110,-5)(135,-5)
\psline[linewidth=0.75](110,-5)(110,20)
\psline[linewidth=0.75](110,20)(135,-5)
\rput(118.75,2.5){$\oone$}
\psline[linewidth=0.75](240,95)(240,7.5)
\psline[linewidth=0.75](227.5,-5)(252.5,-5)
\psline[linewidth=0.75](227.5,-5)(227.5,20)
\psline[linewidth=0.75](227.5,20)(252.5,-5)
\psline[linewidth=0.75](312.5,25)(332.5,25)
\psline[linewidth=0.75](312.5,25)(312.5,45)
\psline[linewidth=0.75](312.5,45)(332.5,25)
\psline[linewidth=0.75](297.5,70)(327.5,70)
\psline[linewidth=0.75](347.5,50)(327.5,70)
\psline[linewidth=0.75](337.5,95)(337.5,60)
\psline[linewidth=0.75](318.12,50)(347.5,50)
\psline[linewidth=0.75](322.5,50)(322.5,35)
\psline[linewidth=0.75](307.5,60)(297.5,50)
\psline[linewidth=0.75](297.5,70)(317.5,50)
\psline[linewidth=0.75](287.5,45)(307.5,25)
\psline[linewidth=0.75](287.5,25)(306.88,25)
\psline[linewidth=0.75](287.5,25)(287.5,44.99)
\rput(292.5,30){$\iiftag$}
\rput(322.5,60){$\stag$}
\psline[linewidth=0.75](297.5,50)(297.5,35)
\psline[linewidth=0.75](340,50)(340,7.5)
\psline[linewidth=0.75](327.5,-5)(352.5,-5)
\psline[linewidth=0.75](327.5,-5)(327.5,20)
\psline[linewidth=0.75](327.5,20)(352.5,-5)
\end{pspicture}


==> PIC/numberb.tex <==
%%Created by jPicEdt 1.4.1_03: mixed JPIC-XML/LaTeX format
%%Sat Dec 22 17:25:00 GMT-10:00 2018
%%Begin JPIC-XML
%<?xml version="1.0" standalone="yes"?>
%<jpic x-min="7.5" x-max="370" y-min="0" y-max="130" auto-bounding="true">
%<multicurve fill-style= "none"
%	 points= "(310,55);(310,55);(370,55);(370,55)"
%	 stroke-width= "0.6"
%	 />
%<multicurve fill-style= "none"
%	 points= "(370,35);(370,35);(370,55);(370,55)"
%	 stroke-width= "0.6"
%	 />
%<multicurve fill-style= "none"
%	 points= "(310,35);(310,35);(370,35);(370,35)"
%	 stroke-width= "0.6"
%	 />
%<multicurve fill-style= "none"
%	 points= "(310,55);(310,55);(310,35);(310,35)"
%	 stroke-width= "0.6"
%	 />
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(275,35)"
%	 stroke-width= "0.75"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\EQLS
%</text>
%<multicurve fill-style= "none"
%	 points= "(10,50);(10,50);(50,50);(50,50)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(50,30);(50,30);(50,50);(50,50)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(40,65);(40,65);(40,50);(40,50)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(30,30);(30,30);(50,30);(50,30)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(20,40);(20,40);(20,12.5);(20,12.5)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(10,50);(10,50);(30,30);(30,30)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(7.5,0);(7.5,0);(32.5,0);(32.5,0)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(7.5,0);(7.5,0);(7.5,25);(7.5,25)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(7.5,25);(7.5,25);(32.5,0);(32.5,0)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(40,30);(40,30);(40,0);(40,0)"
%	 stroke-width= "0.75"
%	 />
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(65,35)"
%	 stroke-width= "0.75"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\EQLS
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(16.25,7.5)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\oone$
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(35,40)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\ueval$
%</text>
%<multicurve fill-style= "none"
%	 points= "(340,65);(340,65);(340,55);(340,55)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(322.5,33.75);(322.5,33.75);(322.5,12.5);(322.5,12.5)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(310,0);(310,0);(335,0);(335,0)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(310,0);(310,0);(310,25);(310,25)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(310,25);(310,25);(335,0);(335,0)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(357.5,33.75);(357.5,33.75);(357.5,12.5);(357.5,12.5)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(345,0);(345,0);(370,0);(370,0)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(345,0);(345,0);(345,25);(345,25)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(345,25);(345,25);(370,0);(370,0)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(250,65);(250,65);(250,15);(250,15)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(235,0);(235,0);(265,0);(265,0)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(235,30);(235,30);(265,0);(265,0)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(235,30);(235,30);(235,0);(235,0)"
%	 stroke-width= "0.75"
%	 />
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(340,45)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\pairtag$
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(245,7.5)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\nextt$
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(353.12,6.88)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\enn$
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(317.5,6.25)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\bottag$
%</text>
%<multicurve fill-style= "none"
%	 points= "(95,55);(95,55);(155,55);(155,55)"
%	 stroke-width= "0.6"
%	 />
%<multicurve fill-style= "none"
%	 points= "(155,35);(155,35);(155,55);(155,55)"
%	 stroke-width= "0.6"
%	 />
%<multicurve fill-style= "none"
%	 points= "(95,35);(95,35);(155,35);(155,35)"
%	 stroke-width= "0.6"
%	 />
%<multicurve fill-style= "none"
%	 points= "(95,55);(95,55);(95,35);(95,35)"
%	 stroke-width= "0.6"
%	 />
%<multicurve fill-style= "none"
%	 points= "(125,65);(125,65);(125,55);(125,55)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(107.5,33.75);(107.5,33.75);(107.5,12.5);(107.5,12.5)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(95,0);(95,0);(120,0);(120,0)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(95,0);(95,0);(95,25);(95,25)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(95,25);(95,25);(120,0);(120,0)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(142.5,33.75);(142.5,33.75);(142.5,12.5);(142.5,12.5)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(130,0);(130,0);(155,0);(155,0)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(130,0);(130,0);(130,25);(130,25)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(130,25);(130,25);(155,0);(155,0)"
%	 stroke-width= "0.75"
%	 />
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(125,45)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\pairtag$
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(138.12,7.5)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\oone$
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(102.5,7.5)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\toptag$
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(65,90)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\leqn$
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(275,90)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\reqn$
%</text>
%<multicurve fill-style= "none"
%	 points= "(165,120);(165,120);(195,120);(195,120)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(215,100);(215,100);(195,120);(195,120)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(205,130);(205,130);(205,110);(205,110)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(185.62,100);(185.62,100);(215,100);(215,100)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(190,100);(190,100);(190,75);(190,75)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(175,110);(175,110);(175,100);(175,100)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(165,120);(165,120);(185,100);(185,100)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(165,110);(165,110);(185,90);(185,90)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(165,90);(165,90);(184.38,90);(184.38,90)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(165,90);(165,90);(165,109.99);(165,109.99)"
%	 stroke-width= "0.75"
%	 />
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(170,95)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\iiftag$
%</text>
%<multicurve fill-style= "none"
%	 points= "(208.75,100);(208.75,100);(208.75,75);(208.75,75)"
%	 stroke-width= "0.75"
%	 />
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(190,110)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\stag$
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(189.38,80.62)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\eex$
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(207.5,80.62)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\why$
%</text>
%</jpic>
%%End JPIC-XML
%PSTricks content-type (pstricks.sty package needed)
%Add \usepackage{pstricks} in the preamble of your LaTeX file
%You can rescale the whole picture (to 80% for instance) by using the command \def\JPicScale{0.8}
\ifx\JPicScale\undefined\def\JPicScale{1}\fi
\psset{unit=\JPicScale mm}
\psset{linewidth=0.3,dotsep=1,hatchwidth=0.3,hatchsep=1.5,shadowsize=1,dimen=middle}
\psset{dotsize=0.7 2.5,dotscale=1 1,fillcolor=black}
\psset{arrowsize=1 2,arrowlength=1,arrowinset=0.25,tbarsize=0.7 5,bracketlength=0.15,rbracketlength=0.15}
\begin{pspicture}(0,0)(370,130)
\psline[linewidth=0.6](310,55)(370,55)
\psline[linewidth=0.6](370,35)(370,55)
\psline[linewidth=0.6](310,35)(370,35)
\psline[linewidth=0.6](310,55)(310,35)
\rput(275,35){\EQLS}
\psline[linewidth=0.75](10,50)(50,50)
\psline[linewidth=0.75](50,30)(50,50)
\psline[linewidth=0.75](40,65)(40,50)
\psline[linewidth=0.75](30,30)(50,30)
\psline[linewidth=0.75](20,40)(20,12.5)
\psline[linewidth=0.75](10,50)(30,30)
\psline[linewidth=0.75](7.5,0)(32.5,0)
\psline[linewidth=0.75](7.5,0)(7.5,25)
\psline[linewidth=0.75](7.5,25)(32.5,0)
\psline[linewidth=0.75](40,30)(40,0)
\rput(65,35){\EQLS}
\rput(16.25,7.5){$\oone$}
\rput(35,40){$\ueval$}
\psline[linewidth=0.75](340,65)(340,55)
\psline[linewidth=0.75](322.5,33.75)(322.5,12.5)
\psline[linewidth=0.75](310,0)(335,0)
\psline[linewidth=0.75](310,0)(310,25)
\psline[linewidth=0.75](310,25)(335,0)
\psline[linewidth=0.75](357.5,33.75)(357.5,12.5)
\psline[linewidth=0.75](345,0)(370,0)
\psline[linewidth=0.75](345,0)(345,25)
\psline[linewidth=0.75](345,25)(370,0)
\psline[linewidth=0.75](250,65)(250,15)
\psline[linewidth=0.75](235,0)(265,0)
\psline[linewidth=0.75](235,30)(265,0)
\psline[linewidth=0.75](235,30)(235,0)
\rput(340,45){$\pairtag$}
\rput(245,7.5){$\nextt$}
\rput(353.12,6.88){$\enn$}
\rput(317.5,6.25){$\bottag$}
\psline[linewidth=0.6](95,55)(155,55)
\psline[linewidth=0.6](155,35)(155,55)
\psline[linewidth=0.6](95,35)(155,35)
\psline[linewidth=0.6](95,55)(95,35)
\psline[linewidth=0.75](125,65)(125,55)
\psline[linewidth=0.75](107.5,33.75)(107.5,12.5)
\psline[linewidth=0.75](95,0)(120,0)
\psline[linewidth=0.75](95,0)(95,25)
\psline[linewidth=0.75](95,25)(120,0)
\psline[linewidth=0.75](142.5,33.75)(142.5,12.5)
\psline[linewidth=0.75](130,0)(155,0)
\psline[linewidth=0.75](130,0)(130,25)
\psline[linewidth=0.75](130,25)(155,0)
\rput(125,45){$\pairtag$}
\rput(138.12,7.5){$\oone$}
\rput(102.5,7.5){$\toptag$}
\rput(65,90){$\leqn$}
\rput(275,90){$\reqn$}
\psline[linewidth=0.75](165,120)(195,120)
\psline[linewidth=0.75](215,100)(195,120)
\psline[linewidth=0.75](205,130)(205,110)
\psline[linewidth=0.75](185.62,100)(215,100)
\psline[linewidth=0.75](190,100)(190,75)
\psline[linewidth=0.75](175,110)(175,100)
\psline[linewidth=0.75](165,120)(185,100)
\psline[linewidth=0.75](165,110)(185,90)
\psline[linewidth=0.75](165,90)(184.38,90)
\psline[linewidth=0.75](165,90)(165,109.99)
\rput(170,95){$\iiftag$}
\psline[linewidth=0.75](208.75,100)(208.75,75)
\rput(190,110){$\stag$}
\rput[r](189.38,80.62){$\eex$}
\rput[r](207.5,80.62){$\why$}
\end{pspicture}


==> PIC/numberc-2.tex <==
%%Created by jPicEdt 1.4.1_03: mixed JPIC-XML/LaTeX format
%%Sat Dec 22 23:29:42 GMT-10:00 2018
%%Begin JPIC-XML
%<?xml version="1.0" standalone="yes"?>
%<jpic x-min="0" x-max="490" y-min="0" y-max="75" auto-bounding="true">
%<multicurve fill-style= "none"
%	 points= "(450,50);(450,50);(490,50);(490,50)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(490,30);(490,30);(490,50);(490,50)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(480,60);(480,60);(480,50);(480,50)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(470,30);(470,30);(490,30);(490,30)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(480,30);(480,30);(480,15);(480,15)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(460,40);(460,40);(460,0);(460,0)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(450,50);(450,50);(470,30);(470,30)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(470,25);(470,25);(490,5);(490,5)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(470,5);(470,5);(489.38,5);(489.38,5)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(470,5);(470,5);(470,24.99);(470,24.99)"
%	 stroke-width= "0.75"
%	 />
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(435,40)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\EQLS$
%</text>
%<multicurve fill-style= "none"
%	 points= "(260,50);(260,50);(300,50);(300,50)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(300,30);(300,30);(300,50);(300,50)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(290,60);(290,60);(290,50);(290,50)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(280,30);(280,30);(300,30);(300,30)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(290,30);(290,30);(290,15);(290,15)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(270,40);(270,40);(270,0);(270,0)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(260,50);(260,50);(280,30);(280,30)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(280,25);(280,25);(300,5);(300,5)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(280,5);(280,5);(299.38,5);(299.38,5)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(280,5);(280,5);(280,24.99);(280,24.99)"
%	 stroke-width= "0.75"
%	 />
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(245,40)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\EQLS$
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(285,10)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\toptag$
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(475,10)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\bottag$
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(475,40)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\utag$
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(285,40)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\utag$
%</text>
%<multicurve fill-style= "none"
%	 points= "(400,30);(400,30);(400,0);(400,0)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(380,50);(380,50);(420,50);(420,50)"
%	 stroke-width= "0.6"
%	 />
%<multicurve fill-style= "none"
%	 points= "(420,30);(420,30);(420,50);(420,50)"
%	 stroke-width= "0.6"
%	 />
%<multicurve fill-style= "none"
%	 points= "(380,30);(380,30);(420,30);(420,30)"
%	 stroke-width= "0.6"
%	 />
%<multicurve fill-style= "none"
%	 points= "(380,50);(380,50);(380,30);(380,30)"
%	 stroke-width= "0.6"
%	 />
%<multicurve fill-style= "none"
%	 points= "(400,60);(400,60);(400,50);(400,50)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(210,30);(210,30);(210,0);(210,0)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(190,50);(190,50);(230,50);(230,50)"
%	 stroke-width= "0.6"
%	 />
%<multicurve fill-style= "none"
%	 points= "(230,30);(230,30);(230,50);(230,50)"
%	 stroke-width= "0.6"
%	 />
%<multicurve fill-style= "none"
%	 points= "(190,30);(190,30);(230,30);(230,30)"
%	 stroke-width= "0.6"
%	 />
%<multicurve fill-style= "none"
%	 points= "(190,50);(190,50);(190,30);(190,30)"
%	 stroke-width= "0.6"
%	 />
%<multicurve fill-style= "none"
%	 points= "(210,60);(210,60);(210,50);(210,50)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(20,30);(20,30);(20,0);(20,0)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(0,50);(0,50);(40,50);(40,50)"
%	 stroke-width= "0.6"
%	 />
%<multicurve fill-style= "none"
%	 points= "(40,30);(40,30);(40,50);(40,50)"
%	 stroke-width= "0.6"
%	 />
%<multicurve fill-style= "none"
%	 points= "(0,30);(0,30);(40,30);(40,30)"
%	 stroke-width= "0.6"
%	 />
%<multicurve fill-style= "none"
%	 points= "(0,50);(0,50);(0,30);(0,30)"
%	 stroke-width= "0.6"
%	 />
%<multicurve fill-style= "none"
%	 points= "(20,60);(20,60);(20,50);(20,50)"
%	 stroke-width= "0.75"
%	 />
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(20,40)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\sucetag$
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(400,40)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\predtag$
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(210,40)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\zerotag$
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(92.5,10)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\bottag$
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(55,40)"
%	 stroke-width= "0.75"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\EQLS
%</text>
%<multicurve fill-style= "none"
%	 points= "(85,5);(85,5);(105,5);(105,5)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(85,5);(85,5);(85,25);(85,25)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(85,25);(85,25);(105,5);(105,5)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(70,50);(70,50);(97.5,50);(97.5,50)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(117.5,30);(117.5,30);(97.5,50);(97.5,50)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(107.5,60);(107.5,60);(107.5,40);(107.5,40)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(90,30);(90,30);(117.5,30);(117.5,30)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(95,30);(95,30);(95,15);(95,15)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(80,40);(80,40);(70,30);(70,30)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(70,50);(70,50);(90,30);(90,30)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(60,25);(60,25);(80,5);(80,5)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(60,5);(60,5);(79.38,5);(79.38,5)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(60,5);(60,5);(60,24.99);(60,24.99)"
%	 stroke-width= "0.75"
%	 />
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(65,10)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\iiftag$
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(95,40)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\stag$
%</text>
%<multicurve fill-style= "none"
%	 points= "(70,30);(70,30);(70,15);(70,15)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(112.5,30);(112.5,30);(112.5,0);(112.5,0)"
%	 stroke-width= "0.75"
%	 />
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(435,75)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\predeq$
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(245,75)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\zeroeq$
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(55,75)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\suceq$
%</text>
%</jpic>
%%End JPIC-XML
%PSTricks content-type (pstricks.sty package needed)
%Add \usepackage{pstricks} in the preamble of your LaTeX file
%You can rescale the whole picture (to 80% for instance) by using the command \def\JPicScale{0.8}
\ifx\JPicScale\undefined\def\JPicScale{1}\fi
\psset{unit=\JPicScale mm}
\psset{linewidth=0.3,dotsep=1,hatchwidth=0.3,hatchsep=1.5,shadowsize=1,dimen=middle}
\psset{dotsize=0.7 2.5,dotscale=1 1,fillcolor=black}
\psset{arrowsize=1 2,arrowlength=1,arrowinset=0.25,tbarsize=0.7 5,bracketlength=0.15,rbracketlength=0.15}
\begin{pspicture}(0,0)(490,75)
\psline[linewidth=0.75](450,50)(490,50)
\psline[linewidth=0.75](490,30)(490,50)
\psline[linewidth=0.75](480,60)(480,50)
\psline[linewidth=0.75](470,30)(490,30)
\psline[linewidth=0.75](480,30)(480,15)
\psline[linewidth=0.75](460,40)(460,0)
\psline[linewidth=0.75](450,50)(470,30)
\psline[linewidth=0.75](470,25)(490,5)
\psline[linewidth=0.75](470,5)(489.38,5)
\psline[linewidth=0.75](470,5)(470,24.99)
\rput(435,40){$\EQLS$}
\psline[linewidth=0.75](260,50)(300,50)
\psline[linewidth=0.75](300,30)(300,50)
\psline[linewidth=0.75](290,60)(290,50)
\psline[linewidth=0.75](280,30)(300,30)
\psline[linewidth=0.75](290,30)(290,15)
\psline[linewidth=0.75](270,40)(270,0)
\psline[linewidth=0.75](260,50)(280,30)
\psline[linewidth=0.75](280,25)(300,5)
\psline[linewidth=0.75](280,5)(299.38,5)
\psline[linewidth=0.75](280,5)(280,24.99)
\rput(245,40){$\EQLS$}
\rput(285,10){$\toptag$}
\rput(475,10){$\bottag$}
\rput(475,40){$\utag$}
\rput(285,40){$\utag$}
\psline[linewidth=0.75](400,30)(400,0)
\psline[linewidth=0.6](380,50)(420,50)
\psline[linewidth=0.6](420,30)(420,50)
\psline[linewidth=0.6](380,30)(420,30)
\psline[linewidth=0.6](380,50)(380,30)
\psline[linewidth=0.75](400,60)(400,50)
\psline[linewidth=0.75](210,30)(210,0)
\psline[linewidth=0.6](190,50)(230,50)
\psline[linewidth=0.6](230,30)(230,50)
\psline[linewidth=0.6](190,30)(230,30)
\psline[linewidth=0.6](190,50)(190,30)
\psline[linewidth=0.75](210,60)(210,50)
\psline[linewidth=0.75](20,30)(20,0)
\psline[linewidth=0.6](0,50)(40,50)
\psline[linewidth=0.6](40,30)(40,50)
\psline[linewidth=0.6](0,30)(40,30)
\psline[linewidth=0.6](0,50)(0,30)
\psline[linewidth=0.75](20,60)(20,50)
\rput(20,40){$\sucetag$}
\rput(400,40){$\predtag$}
\rput(210,40){$\zerotag$}
\rput(92.5,10){$\bottag$}
\rput(55,40){\EQLS}
\psline[linewidth=0.75](85,5)(105,5)
\psline[linewidth=0.75](85,5)(85,25)
\psline[linewidth=0.75](85,25)(105,5)
\psline[linewidth=0.75](70,50)(97.5,50)
\psline[linewidth=0.75](117.5,30)(97.5,50)
\psline[linewidth=0.75](107.5,60)(107.5,40)
\psline[linewidth=0.75](90,30)(117.5,30)
\psline[linewidth=0.75](95,30)(95,15)
\psline[linewidth=0.75](80,40)(70,30)
\psline[linewidth=0.75](70,50)(90,30)
\psline[linewidth=0.75](60,25)(80,5)
\psline[linewidth=0.75](60,5)(79.38,5)
\psline[linewidth=0.75](60,5)(60,24.99)
\rput(65,10){$\iiftag$}
\rput(95,40){$\stag$}
\psline[linewidth=0.75](70,30)(70,15)
\psline[linewidth=0.75](112.5,30)(112.5,0)
\rput(435,75){$\predeq$}
\rput(245,75){$\zeroeq$}
\rput(55,75){$\suceq$}
\end{pspicture}


==> PIC/numberc.tex <==
%%Created by jPicEdt 1.4.1_03: mixed JPIC-XML/LaTeX format
%%Tue Oct 04 17:59:32 HST 2016
%%Begin JPIC-XML
%<?xml version="1.0" standalone="yes"?>
%<jpic x-min="0" x-max="220" y-min="0" y-max="205" auto-bounding="true">
%<multicurve stroke-width= "0.75"
%	 points= "(180,120);(180,120);(220,120);(220,120)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.75"
%	 points= "(220,100);(220,100);(220,120);(220,120)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.75"
%	 points= "(210,130);(210,130);(210,120);(210,120)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.75"
%	 points= "(200.62,100);(200.62,100);(220,100);(220,100)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.75"
%	 points= "(210,100);(210,100);(210,85);(210,85)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.75"
%	 points= "(190,110);(190,110);(190,75);(190,75)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.75"
%	 points= "(180,120);(180,120);(200,100);(200,100)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.75"
%	 points= "(110,100);(110,100);(110,75);(110,75)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.6"
%	 points= "(90,120);(90,120);(130,120);(130,120)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.6"
%	 points= "(130,100);(130,100);(130,120);(130,120)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.6"
%	 points= "(90,100);(90,100);(130,100);(130,100)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.6"
%	 points= "(90,120);(90,120);(90,100);(90,100)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.75"
%	 points= "(110,130);(110,130);(110,120);(110,120)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.75"
%	 points= "(200,95);(200,95);(220,75);(220,75)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.75"
%	 points= "(200,75);(200,75);(219.38,75);(219.38,75)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.75"
%	 points= "(200,75);(200,75);(200,94.99);(200,94.99)"
%	 fill-style= "none"
%	 />
%<text text-vert-align= "center-v"
%	 anchor-point= "(155,95)"
%	 text-frame= "noframe"
%	 fill-style= "none"
%	 text-hor-align= "center-h"
%	 >
%$\EQLS$
%</text>
%<multicurve stroke-width= "0.75"
%	 points= "(180,45);(180,45);(220,45);(220,45)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.75"
%	 points= "(220,25);(220,25);(220,45);(220,45)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.75"
%	 points= "(210,55);(210,55);(210,45);(210,45)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.75"
%	 points= "(200.62,25);(200.62,25);(220,25);(220,25)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.75"
%	 points= "(210,25);(210,25);(210,10);(210,10)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.75"
%	 points= "(190,35);(190,35);(190,0);(190,0)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.75"
%	 points= "(180,45);(180,45);(200,25);(200,25)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.75"
%	 points= "(110,25);(110,25);(110,0);(110,0)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.6"
%	 points= "(90,45);(90,45);(130,45);(130,45)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.6"
%	 points= "(130,25);(130,25);(130,45);(130,45)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.6"
%	 points= "(90,25);(90,25);(130,25);(130,25)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.6"
%	 points= "(90,45);(90,45);(90,25);(90,25)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.75"
%	 points= "(110,55);(110,55);(110,45);(110,45)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.75"
%	 points= "(200,20);(200,20);(220,0);(220,0)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.75"
%	 points= "(200,0);(200,0);(219.38,0);(219.38,0)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.75"
%	 points= "(200,0);(200,0);(200,19.99);(200,19.99)"
%	 fill-style= "none"
%	 />
%<text text-vert-align= "center-v"
%	 anchor-point= "(155,20)"
%	 text-frame= "noframe"
%	 fill-style= "none"
%	 text-hor-align= "center-h"
%	 >
%$\EQLS$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(110,35)"
%	 text-frame= "noframe"
%	 fill-style= "none"
%	 text-hor-align= "center-h"
%	 >
%$\fsttag$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(110,110)"
%	 text-frame= "noframe"
%	 fill-style= "none"
%	 text-hor-align= "center-h"
%	 >
%$\sndtag$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(205,5)"
%	 text-frame= "noframe"
%	 fill-style= "none"
%	 text-hor-align= "center-h"
%	 >
%$\toptag$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(205,80)"
%	 text-frame= "noframe"
%	 fill-style= "none"
%	 text-hor-align= "center-h"
%	 >
%$\bottag$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(205,110)"
%	 text-frame= "noframe"
%	 fill-style= "none"
%	 text-hor-align= "center-h"
%	 >
%$\utag$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(205,35)"
%	 text-frame= "noframe"
%	 fill-style= "none"
%	 text-hor-align= "center-h"
%	 >
%$\utag$
%</text>
%<multicurve stroke-width= "0.75"
%	 points= "(20,100);(20,100);(20,75);(20,75)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.6"
%	 points= "(0,120);(0,120);(40,120);(40,120)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.6"
%	 points= "(40,100);(40,100);(40,120);(40,120)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.6"
%	 points= "(0,100);(0,100);(40,100);(40,100)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.6"
%	 points= "(0,120);(0,120);(0,100);(0,100)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.75"
%	 points= "(20,130);(20,130);(20,120);(20,120)"
%	 fill-style= "none"
%	 />
%<text text-vert-align= "center-v"
%	 anchor-point= "(65,95)"
%	 text-frame= "noframe"
%	 fill-style= "none"
%	 text-hor-align= "center-h"
%	 >
%$\EQLS$
%</text>
%<multicurve stroke-width= "0.75"
%	 points= "(20,25);(20,25);(20,0);(20,0)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.6"
%	 points= "(0,45);(0,45);(40,45);(40,45)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.6"
%	 points= "(40,25);(40,25);(40,45);(40,45)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.6"
%	 points= "(0,25);(0,25);(40,25);(40,25)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.6"
%	 points= "(0,45);(0,45);(0,25);(0,25)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.75"
%	 points= "(20,55);(20,55);(20,45);(20,45)"
%	 fill-style= "none"
%	 />
%<text text-vert-align= "center-v"
%	 anchor-point= "(65,20)"
%	 text-frame= "noframe"
%	 fill-style= "none"
%	 text-hor-align= "center-h"
%	 >
%$\EQLS$
%</text>
%<multicurve stroke-width= "0.75"
%	 points= "(120,175);(120,175);(120,150);(120,150)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.6"
%	 points= "(90,195);(90,195);(130,195);(130,195)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.6"
%	 points= "(130,175);(130,175);(130,195);(130,195)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.6"
%	 points= "(90,175);(90,175);(130,175);(130,175)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.6"
%	 points= "(90,195);(90,195);(90,175);(90,175)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.75"
%	 points= "(110,205);(110,205);(110,195);(110,195)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.75"
%	 points= "(20,175);(20,175);(20,150);(20,150)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.6"
%	 points= "(0,195);(0,195);(40,195);(40,195)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.6"
%	 points= "(40,175);(40,175);(40,195);(40,195)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.6"
%	 points= "(0,175);(0,175);(40,175);(40,175)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.6"
%	 points= "(0,195);(0,195);(0,175);(0,175)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.75"
%	 points= "(20,205);(20,205);(20,195);(20,195)"
%	 fill-style= "none"
%	 />
%<text text-vert-align= "center-v"
%	 anchor-point= "(65,170)"
%	 text-frame= "noframe"
%	 fill-style= "none"
%	 text-hor-align= "center-h"
%	 >
%$\EQLS$
%</text>
%<multicurve stroke-width= "0.75"
%	 points= "(100,175);(100,175);(100,160);(100,160)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.75"
%	 points= "(90,170);(90,170);(110,150);(110,150)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.75"
%	 points= "(90,150);(90,150);(109.38,150);(109.38,150)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.75"
%	 points= "(90,150);(90,150);(90,169.99);(90,169.99)"
%	 fill-style= "none"
%	 />
%<text text-vert-align= "center-v"
%	 anchor-point= "(110,185)"
%	 text-frame= "noframe"
%	 fill-style= "none"
%	 text-hor-align= "center-h"
%	 >
%$\pairtag$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(20,185)"
%	 text-frame= "noframe"
%	 fill-style= "none"
%	 text-hor-align= "center-h"
%	 >
%$\sucetag$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(20,110)"
%	 text-frame= "noframe"
%	 fill-style= "none"
%	 text-hor-align= "center-h"
%	 >
%$\predtag$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(20,35)"
%	 text-frame= "noframe"
%	 fill-style= "none"
%	 text-hor-align= "center-h"
%	 >
%$\zerotag$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(95,155)"
%	 text-frame= "noframe"
%	 fill-style= "none"
%	 text-hor-align= "center-h"
%	 >
%$\bottag$
%</text>
%</jpic>
%%End JPIC-XML
%PSTricks content-type (pstricks.sty package needed)
%Add \usepackage{pstricks} in the preamble of your LaTeX file
%You can rescale the whole picture (to 80% for instance) by using the command \def\JPicScale{0.8}
\ifx\JPicScale\undefined\def\JPicScale{1}\fi
\psset{unit=\JPicScale mm}
\psset{linewidth=0.3,dotsep=1,hatchwidth=0.3,hatchsep=1.5,shadowsize=1,dimen=middle}
\psset{dotsize=0.7 2.5,dotscale=1 1,fillcolor=black}
\psset{arrowsize=1 2,arrowlength=1,arrowinset=0.25,tbarsize=0.7 5,bracketlength=0.15,rbracketlength=0.15}
\begin{pspicture}(0,0)(220,205)
\psline[linewidth=0.75](180,120)(220,120)
\psline[linewidth=0.75](220,100)(220,120)
\psline[linewidth=0.75](210,130)(210,120)
\psline[linewidth=0.75](200.62,100)(220,100)
\psline[linewidth=0.75](210,100)(210,85)
\psline[linewidth=0.75](190,110)(190,75)
\psline[linewidth=0.75](180,120)(200,100)
\psline[linewidth=0.75](110,100)(110,75)
\psline[linewidth=0.6](90,120)(130,120)
\psline[linewidth=0.6](130,100)(130,120)
\psline[linewidth=0.6](90,100)(130,100)
\psline[linewidth=0.6](90,120)(90,100)
\psline[linewidth=0.75](110,130)(110,120)
\psline[linewidth=0.75](200,95)(220,75)
\psline[linewidth=0.75](200,75)(219.38,75)
\psline[linewidth=0.75](200,75)(200,94.99)
\rput(155,95){$\EQLS$}
\psline[linewidth=0.75](180,45)(220,45)
\psline[linewidth=0.75](220,25)(220,45)
\psline[linewidth=0.75](210,55)(210,45)
\psline[linewidth=0.75](200.62,25)(220,25)
\psline[linewidth=0.75](210,25)(210,10)
\psline[linewidth=0.75](190,35)(190,0)
\psline[linewidth=0.75](180,45)(200,25)
\psline[linewidth=0.75](110,25)(110,0)
\psline[linewidth=0.6](90,45)(130,45)
\psline[linewidth=0.6](130,25)(130,45)
\psline[linewidth=0.6](90,25)(130,25)
\psline[linewidth=0.6](90,45)(90,25)
\psline[linewidth=0.75](110,55)(110,45)
\psline[linewidth=0.75](200,20)(220,0)
\psline[linewidth=0.75](200,0)(219.38,0)
\psline[linewidth=0.75](200,0)(200,19.99)
\rput(155,20){$\EQLS$}
\rput(110,35){$\fsttag$}
\rput(110,110){$\sndtag$}
\rput(205,5){$\toptag$}
\rput(205,80){$\bottag$}
\rput(205,110){$\utag$}
\rput(205,35){$\utag$}
\psline[linewidth=0.75](20,100)(20,75)
\psline[linewidth=0.6](0,120)(40,120)
\psline[linewidth=0.6](40,100)(40,120)
\psline[linewidth=0.6](0,100)(40,100)
\psline[linewidth=0.6](0,120)(0,100)
\psline[linewidth=0.75](20,130)(20,120)
\rput(65,95){$\EQLS$}
\psline[linewidth=0.75](20,25)(20,0)
\psline[linewidth=0.6](0,45)(40,45)
\psline[linewidth=0.6](40,25)(40,45)
\psline[linewidth=0.6](0,25)(40,25)
\psline[linewidth=0.6](0,45)(0,25)
\psline[linewidth=0.75](20,55)(20,45)
\rput(65,20){$\EQLS$}
\psline[linewidth=0.75](120,175)(120,150)
\psline[linewidth=0.6](90,195)(130,195)
\psline[linewidth=0.6](130,175)(130,195)
\psline[linewidth=0.6](90,175)(130,175)
\psline[linewidth=0.6](90,195)(90,175)
\psline[linewidth=0.75](110,205)(110,195)
\psline[linewidth=0.75](20,175)(20,150)
\psline[linewidth=0.6](0,195)(40,195)
\psline[linewidth=0.6](40,175)(40,195)
\psline[linewidth=0.6](0,175)(40,175)
\psline[linewidth=0.6](0,195)(0,175)
\psline[linewidth=0.75](20,205)(20,195)
\rput(65,170){$\EQLS$}
\psline[linewidth=0.75](100,175)(100,160)
\psline[linewidth=0.75](90,170)(110,150)
\psline[linewidth=0.75](90,150)(109.38,150)
\psline[linewidth=0.75](90,150)(90,169.99)
\rput(110,185){$\pairtag$}
\rput(20,185){$\sucetag$}
\rput(20,110){$\predtag$}
\rput(20,35){$\zerotag$}
\rput(95,155){$\bottag$}
\end{pspicture}


==> PIC/numbers-0.tex <==
%%Created by jPicEdt 1.4.1_03: mixed JPIC-XML/LaTeX format
%%Thu Oct 20 14:47:27 HST 2016
%%Begin JPIC-XML
%<?xml version="1.0" standalone="yes"?>
%<jpic x-min="-10" x-max="280.62" y-min="0" y-max="180" auto-bounding="true">
%<multicurve stroke-width= "0.75"
%	 points= "(160,90);(160,90);(200,90);(200,90)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.75"
%	 points= "(200,70);(200,70);(200,90);(200,90)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.75"
%	 points= "(190,110);(190,110);(190,90);(190,90)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.75"
%	 points= "(180.62,70);(180.62,70);(200,70);(200,70)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.75"
%	 points= "(190,70);(190,70);(190,60);(190,60)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.75"
%	 points= "(170,80.01);(170,80.01);(170,60);(170,60)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.75"
%	 points= "(160,90);(160,90);(180,70);(180,70)"
%	 fill-style= "none"
%	 />
%<ellipse p3= "(172.58,67.42)"
%	 p2= "(172.58,72.58)"
%	 p1= "(167.42,72.58)"
%	 closure= "open"
%	 fill-color= "#330033"
%	 angle-end= "0"
%	 fill-style= "solid"
%	 angle-start= "0"
%	 />
%<multicurve stroke-width= "0.75"
%	 points= "(169.38,109.38);(169.38,109.38);(150,90);(150,90)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.75"
%	 points= "(150,90);(150,90);(170,70);(170,70)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.75"
%	 points= "(80,90);(80,90);(120,90);(120,90)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.75"
%	 points= "(120,70);(120,70);(120,90);(120,90)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.75"
%	 points= "(110,100);(110,100);(110,90);(110,90)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.75"
%	 points= "(100.62,70);(100.62,70);(120,70);(120,70)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.75"
%	 points= "(110,70);(110,70);(110,60);(110,60)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.75"
%	 points= "(90,80.01);(90,80.01);(90,60);(90,60)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.75"
%	 points= "(80,90);(80,90);(100,70);(100,70)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.75"
%	 points= "(160,130);(160,130);(200,130);(200,130)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.75"
%	 points= "(200,110);(200,110);(200,130);(200,130)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.75"
%	 points= "(190,140);(190,140);(190,130);(190,130)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.75"
%	 points= "(180.62,110);(180.62,110);(200,110);(200,110)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.75"
%	 points= "(170,120.01);(170,120.01);(170,109.38);(170,109.38)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.75"
%	 points= "(160,130);(160,130);(180,110);(180,110)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.75"
%	 points= "(240,90);(240,90);(280,90);(280,90)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.75"
%	 points= "(280,70);(280,70);(280,90);(280,90)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.75"
%	 points= "(270,110);(270,110);(270,90);(270,90)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.75"
%	 points= "(260.62,70);(260.62,70);(280,70);(280,70)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.75"
%	 points= "(270,70);(270,70);(270,60);(270,60)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.75"
%	 points= "(250,80.01);(250,80.01);(250,60);(250,60)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.75"
%	 points= "(240,90);(240,90);(260,70);(260,70)"
%	 fill-style= "none"
%	 />
%<ellipse p3= "(252.58,67.42)"
%	 p2= "(252.58,72.58)"
%	 p1= "(247.42,72.58)"
%	 closure= "open"
%	 fill-color= "#330033"
%	 angle-end= "0"
%	 fill-style= "solid"
%	 angle-start= "0"
%	 />
%<multicurve stroke-width= "0.75"
%	 points= "(249.38,109.38);(249.38,109.38);(230,90);(230,90)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.75"
%	 points= "(230,90);(230,90);(250,70);(250,70)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.75"
%	 points= "(240,130);(240,130);(280,130);(280,130)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.75"
%	 points= "(280,110);(280,110);(280,130);(280,130)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.75"
%	 points= "(270,150);(270,150);(270,130);(270,130)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.75"
%	 points= "(260.62,110);(260.62,110);(280,110);(280,110)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.75"
%	 points= "(250,120.01);(250,120.01);(250,109.38);(250,109.38)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.75"
%	 points= "(240,130);(240,130);(260,110);(260,110)"
%	 fill-style= "none"
%	 />
%<ellipse p3= "(252.58,107.42)"
%	 p2= "(252.58,112.58)"
%	 p1= "(247.42,112.58)"
%	 closure= "open"
%	 fill-color= "#330033"
%	 angle-end= "0"
%	 fill-style= "solid"
%	 angle-start= "0"
%	 />
%<multicurve stroke-width= "0.75"
%	 points= "(230,130);(230,130);(250,110);(250,110)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.75"
%	 points= "(240.62,170);(240.62,170);(280.62,170);(280.62,170)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.75"
%	 points= "(280.62,150);(280.62,150);(280.62,170);(280.62,170)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.75"
%	 points= "(270.62,180);(270.62,180);(270.62,170);(270.62,170)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.75"
%	 points= "(261.25,150);(261.25,150);(280.62,150);(280.62,150)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.75"
%	 points= "(250.62,160.01);(250.62,160.01);(250.62,150);(250.62,150)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.75"
%	 points= "(240.62,170);(240.62,170);(260.62,150);(260.62,150)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.75"
%	 points= "(250.62,150);(250.62,150);(230,130);(230,130)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.75"
%	 points= "(30,100);(30,100);(30,60);(30,60)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.75"
%	 points= "(10.62,80.01);(10.62,80.01);(10.62,60);(10.62,60)"
%	 fill-style= "none"
%	 />
%<ellipse p3= "(13.2,77.42)"
%	 p2= "(13.2,82.58)"
%	 p1= "(8.05,82.58)"
%	 closure= "open"
%	 fill-color= "#330033"
%	 angle-end= "0"
%	 fill-style= "solid"
%	 angle-start= "0"
%	 />
%<multicurve stroke-width= "0.6"
%	 points= "(0,90);(0,90);(40,90);(40,90)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.6"
%	 points= "(40,70);(40,70);(40,90);(40,90)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.6"
%	 points= "(0,70);(0,70);(40,70);(40,70)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.6"
%	 points= "(0,90);(0,90);(0,70);(0,70)"
%	 fill-style= "none"
%	 />
%<text text-vert-align= "center-v"
%	 stroke-width= "0.75"
%	 anchor-point= "(20,50)"
%	 text-frame= "noframe"
%	 fill-style= "none"
%	 text-hor-align= "center-h"
%	 >
%\EQLS
%</text>
%<multicurve stroke-width= "0.75"
%	 points= "(70,30);(70,30);(120,30);(120,30)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.75"
%	 points= "(120,10);(120,10);(120,30);(120,30)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.75"
%	 points= "(105,40);(105,40);(105,30);(105,30)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.75"
%	 points= "(90,10);(90,10);(120,10);(120,10)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.75"
%	 points= "(115,10);(115,10);(115,0);(115,0)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.75"
%	 points= "(80,20.01);(80,20.01);(80,10);(80,10)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.75"
%	 points= "(70,30);(70,30);(90,10);(90,10)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.75"
%	 points= "(70,0);(70,0);(90,0);(90,0)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.75"
%	 points= "(70,0);(70,0);(70,20);(70,20)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.75"
%	 points= "(70,20);(70,20);(90,0);(90,0)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.75"
%	 points= "(95,10);(95,10);(95,0);(95,0)"
%	 fill-style= "none"
%	 />
%<text text-vert-align= "center-v"
%	 stroke-width= "0.75"
%	 anchor-point= "(100,50)"
%	 text-frame= "noframe"
%	 fill-style= "none"
%	 text-hor-align= "center-h"
%	 >
%\EQLS
%</text>
%<text text-vert-align= "center-v"
%	 stroke-width= "0.75"
%	 anchor-point= "(180,50)"
%	 text-frame= "noframe"
%	 fill-style= "none"
%	 text-hor-align= "center-h"
%	 >
%\EQLS
%</text>
%<text text-vert-align= "center-v"
%	 stroke-width= "0.75"
%	 anchor-point= "(260,50)"
%	 text-frame= "noframe"
%	 fill-style= "none"
%	 text-hor-align= "center-h"
%	 >
%\EQLS
%</text>
%<multicurve stroke-width= "0.75"
%	 points= "(150,30);(150,30);(200,30);(200,30)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.75"
%	 points= "(200,10);(200,10);(200,30);(200,30)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.75"
%	 points= "(185,40);(185,40);(185,30);(185,30)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.75"
%	 points= "(170,10);(170,10);(200,10);(200,10)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.75"
%	 points= "(195,10);(195,10);(195,0);(195,0)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.75"
%	 points= "(160,20.01);(160,20.01);(160,10);(160,10)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.75"
%	 points= "(150,30);(150,30);(170,10);(170,10)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.75"
%	 points= "(150,0);(150,0);(170,0);(170,0)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.75"
%	 points= "(150,0);(150,0);(150,20);(150,20)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.75"
%	 points= "(150,20);(150,20);(170,0);(170,0)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.75"
%	 points= "(175,10);(175,10);(175,0);(175,0)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.75"
%	 points= "(230,30);(230,30);(280,30);(280,30)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.75"
%	 points= "(280,10);(280,10);(280,30);(280,30)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.75"
%	 points= "(265,40);(265,40);(265,30);(265,30)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.75"
%	 points= "(250,10);(250,10);(280,10);(280,10)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.75"
%	 points= "(275,10);(275,10);(275,0);(275,0)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.75"
%	 points= "(240,20.01);(240,20.01);(240,10);(240,10)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.75"
%	 points= "(230,30);(230,30);(250,10);(250,10)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.75"
%	 points= "(230,0);(230,0);(250,0);(250,0)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.75"
%	 points= "(230,0);(230,0);(230,20);(230,20)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.75"
%	 points= "(230,20);(230,20);(250,0);(250,0)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.75"
%	 points= "(255,10);(255,10);(255,0);(255,0)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.75"
%	 points= "(-10,30);(-10,30);(40,30);(40,30)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.75"
%	 points= "(40,10);(40,10);(40,30);(40,30)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.75"
%	 points= "(25,40);(25,40);(25,30);(25,30)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.75"
%	 points= "(10,10);(10,10);(40,10);(40,10)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.75"
%	 points= "(35,10);(35,10);(35,0);(35,0)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.75"
%	 points= "(0,20.01);(0,20.01);(0,10);(0,10)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.75"
%	 points= "(-10,30);(-10,30);(10,10);(10,10)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.75"
%	 points= "(-10,0);(-10,0);(10,0);(10,0)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.75"
%	 points= "(-10,0);(-10,0);(-10,20);(-10,20)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.75"
%	 points= "(-10,20);(-10,20);(10,0);(10,0)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.75"
%	 points= "(15,10);(15,10);(15,0);(15,0)"
%	 fill-style= "none"
%	 />
%<text text-vert-align= "center-v"
%	 anchor-point= "(75,5)"
%	 text-frame= "noframe"
%	 fill-style= "none"
%	 text-hor-align= "center-h"
%	 >
%$\oone$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(155,5)"
%	 text-frame= "noframe"
%	 fill-style= "none"
%	 text-hor-align= "center-h"
%	 >
%$\ttwo$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(-5,5)"
%	 text-frame= "noframe"
%	 fill-style= "none"
%	 text-hor-align= "center-h"
%	 >
%$\zzero$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(235,5)"
%	 text-frame= "noframe"
%	 fill-style= "none"
%	 text-hor-align= "center-h"
%	 >
%$\tthree$
%</text>
%</jpic>
%%End JPIC-XML
%PSTricks content-type (pstricks.sty package needed)
%Add \usepackage{pstricks} in the preamble of your LaTeX file
%You can rescale the whole picture (to 80% for instance) by using the command \def\JPicScale{0.8}
\ifx\JPicScale\undefined\def\JPicScale{1}\fi
\psset{unit=\JPicScale mm}
\psset{linewidth=0.3,dotsep=1,hatchwidth=0.3,hatchsep=1.5,shadowsize=1,dimen=middle}
\psset{dotsize=0.7 2.5,dotscale=1 1,fillcolor=black}
\psset{arrowsize=1 2,arrowlength=1,arrowinset=0.25,tbarsize=0.7 5,bracketlength=0.15,rbracketlength=0.15}
\begin{pspicture}(0,0)(280.62,180)
\psline[linewidth=0.75](160,90)(200,90)
\psline[linewidth=0.75](200,70)(200,90)
\psline[linewidth=0.75](190,110)(190,90)
\psline[linewidth=0.75](180.62,70)(200,70)
\psline[linewidth=0.75](190,70)(190,60)
\psline[linewidth=0.75](170,80.01)(170,60)
\psline[linewidth=0.75](160,90)(180,70)
\newrgbcolor{userFillColour}{0.2 0 0.2}
\rput{0}(170,70){\psellipse[fillcolor=userFillColour,fillstyle=solid](0,0)(2.58,-2.58)}
\psline[linewidth=0.75](169.38,109.38)(150,90)
\psline[linewidth=0.75](150,90)(170,70)
\psline[linewidth=0.75](80,90)(120,90)
\psline[linewidth=0.75](120,70)(120,90)
\psline[linewidth=0.75](110,100)(110,90)
\psline[linewidth=0.75](100.62,70)(120,70)
\psline[linewidth=0.75](110,70)(110,60)
\psline[linewidth=0.75](90,80.01)(90,60)
\psline[linewidth=0.75](80,90)(100,70)
\psline[linewidth=0.75](160,130)(200,130)
\psline[linewidth=0.75](200,110)(200,130)
\psline[linewidth=0.75](190,140)(190,130)
\psline[linewidth=0.75](180.62,110)(200,110)
\psline[linewidth=0.75](170,120.01)(170,109.38)
\psline[linewidth=0.75](160,130)(180,110)
\psline[linewidth=0.75](240,90)(280,90)
\psline[linewidth=0.75](280,70)(280,90)
\psline[linewidth=0.75](270,110)(270,90)
\psline[linewidth=0.75](260.62,70)(280,70)
\psline[linewidth=0.75](270,70)(270,60)
\psline[linewidth=0.75](250,80.01)(250,60)
\psline[linewidth=0.75](240,90)(260,70)
\newrgbcolor{userFillColour}{0.2 0 0.2}
\rput{0}(250,70){\psellipse[fillcolor=userFillColour,fillstyle=solid](0,0)(2.58,-2.58)}
\psline[linewidth=0.75](249.38,109.38)(230,90)
\psline[linewidth=0.75](230,90)(250,70)
\psline[linewidth=0.75](240,130)(280,130)
\psline[linewidth=0.75](280,110)(280,130)
\psline[linewidth=0.75](270,150)(270,130)
\psline[linewidth=0.75](260.62,110)(280,110)
\psline[linewidth=0.75](250,120.01)(250,109.38)
\psline[linewidth=0.75](240,130)(260,110)
\newrgbcolor{userFillColour}{0.2 0 0.2}
\rput{0}(250,110){\psellipse[fillcolor=userFillColour,fillstyle=solid](0,0)(2.58,-2.58)}
\psline[linewidth=0.75](230,130)(250,110)
\psline[linewidth=0.75](240.62,170)(280.62,170)
\psline[linewidth=0.75](280.62,150)(280.62,170)
\psline[linewidth=0.75](270.62,180)(270.62,170)
\psline[linewidth=0.75](261.25,150)(280.62,150)
\psline[linewidth=0.75](250.62,160.01)(250.62,150)
\psline[linewidth=0.75](240.62,170)(260.62,150)
\psline[linewidth=0.75](250.62,150)(230,130)
\psline[linewidth=0.75](30,100)(30,60)
\psline[linewidth=0.75](10.62,80.01)(10.62,60)
\newrgbcolor{userFillColour}{0.2 0 0.2}
\rput{90}(10.62,80){\psellipse[fillcolor=userFillColour,fillstyle=solid](0,0)(2.58,-2.58)}
\psline[linewidth=0.6](0,90)(40,90)
\psline[linewidth=0.6](40,70)(40,90)
\psline[linewidth=0.6](0,70)(40,70)
\psline[linewidth=0.6](0,90)(0,70)
\rput(20,50){\EQLS}
\psline[linewidth=0.75](70,30)(120,30)
\psline[linewidth=0.75](120,10)(120,30)
\psline[linewidth=0.75](105,40)(105,30)
\psline[linewidth=0.75](90,10)(120,10)
\psline[linewidth=0.75](115,10)(115,0)
\psline[linewidth=0.75](80,20.01)(80,10)
\psline[linewidth=0.75](70,30)(90,10)
\psline[linewidth=0.75](70,0)(90,0)
\psline[linewidth=0.75](70,0)(70,20)
\psline[linewidth=0.75](70,20)(90,0)
\psline[linewidth=0.75](95,10)(95,0)
\rput(100,50){\EQLS}
\rput(180,50){\EQLS}
\rput(260,50){\EQLS}
\psline[linewidth=0.75](150,30)(200,30)
\psline[linewidth=0.75](200,10)(200,30)
\psline[linewidth=0.75](185,40)(185,30)
\psline[linewidth=0.75](170,10)(200,10)
\psline[linewidth=0.75](195,10)(195,0)
\psline[linewidth=0.75](160,20.01)(160,10)
\psline[linewidth=0.75](150,30)(170,10)
\psline[linewidth=0.75](150,0)(170,0)
\psline[linewidth=0.75](150,0)(150,20)
\psline[linewidth=0.75](150,20)(170,0)
\psline[linewidth=0.75](175,10)(175,0)
\psline[linewidth=0.75](230,30)(280,30)
\psline[linewidth=0.75](280,10)(280,30)
\psline[linewidth=0.75](265,40)(265,30)
\psline[linewidth=0.75](250,10)(280,10)
\psline[linewidth=0.75](275,10)(275,0)
\psline[linewidth=0.75](240,20.01)(240,10)
\psline[linewidth=0.75](230,30)(250,10)
\psline[linewidth=0.75](230,0)(250,0)
\psline[linewidth=0.75](230,0)(230,20)
\psline[linewidth=0.75](230,20)(250,0)
\psline[linewidth=0.75](255,10)(255,0)
\psline[linewidth=0.75](-10,30)(40,30)
\psline[linewidth=0.75](40,10)(40,30)
\psline[linewidth=0.75](25,40)(25,30)
\psline[linewidth=0.75](10,10)(40,10)
\psline[linewidth=0.75](35,10)(35,0)
\psline[linewidth=0.75](0,20.01)(0,10)
\psline[linewidth=0.75](-10,30)(10,10)
\psline[linewidth=0.75](-10,0)(10,0)
\psline[linewidth=0.75](-10,0)(-10,20)
\psline[linewidth=0.75](-10,20)(10,0)
\psline[linewidth=0.75](15,10)(15,0)
\rput(75,5){$\oone$}
\rput(155,5){$\ttwo$}
\rput(-5,5){$\zzero$}
\rput(235,5){$\tthree$}
\end{pspicture}


==> PIC/numbers-1.tex <==
%%Created by jPicEdt 1.4.1_03: mixed JPIC-XML/LaTeX format
%%Thu Oct 20 14:46:58 HST 2016
%%Begin JPIC-XML
%<?xml version="1.0" standalone="yes"?>
%<jpic x-min="-10" x-max="280.62" y-min="0" y-max="180" auto-bounding="true">
%<multicurve stroke-width= "0.75"
%	 points= "(160,90);(160,90);(200,90);(200,90)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.75"
%	 points= "(200,70);(200,70);(200,90);(200,90)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.75"
%	 points= "(190,110);(190,110);(190,90);(190,90)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.75"
%	 points= "(180.62,70);(180.62,70);(200,70);(200,70)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.75"
%	 points= "(190,70);(190,70);(190,60);(190,60)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.75"
%	 points= "(170,80.01);(170,80.01);(170,60);(170,60)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.75"
%	 points= "(160,90);(160,90);(180,70);(180,70)"
%	 fill-style= "none"
%	 />
%<ellipse p3= "(172.58,67.42)"
%	 p2= "(172.58,72.58)"
%	 p1= "(167.42,72.58)"
%	 closure= "open"
%	 fill-color= "#330033"
%	 angle-end= "0"
%	 fill-style= "solid"
%	 angle-start= "0"
%	 />
%<multicurve stroke-width= "0.75"
%	 points= "(169.38,109.38);(169.38,109.38);(150,90);(150,90)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.75"
%	 points= "(150,90);(150,90);(170,70);(170,70)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.75"
%	 points= "(80,90);(80,90);(120,90);(120,90)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.75"
%	 points= "(120,70);(120,70);(120,90);(120,90)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.75"
%	 points= "(110,100);(110,100);(110,90);(110,90)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.75"
%	 points= "(100.62,70);(100.62,70);(120,70);(120,70)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.75"
%	 points= "(110,70);(110,70);(110,60);(110,60)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.75"
%	 points= "(90,80.01);(90,80.01);(90,60);(90,60)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.75"
%	 points= "(80,90);(80,90);(100,70);(100,70)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.75"
%	 points= "(160,130);(160,130);(200,130);(200,130)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.75"
%	 points= "(200,110);(200,110);(200,130);(200,130)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.75"
%	 points= "(190,140);(190,140);(190,130);(190,130)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.75"
%	 points= "(180.62,110);(180.62,110);(200,110);(200,110)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.75"
%	 points= "(170,120.01);(170,120.01);(170,109.38);(170,109.38)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.75"
%	 points= "(160,130);(160,130);(180,110);(180,110)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.75"
%	 points= "(240,90);(240,90);(280,90);(280,90)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.75"
%	 points= "(280,70);(280,70);(280,90);(280,90)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.75"
%	 points= "(270,110);(270,110);(270,90);(270,90)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.75"
%	 points= "(260.62,70);(260.62,70);(280,70);(280,70)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.75"
%	 points= "(270,70);(270,70);(270,60);(270,60)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.75"
%	 points= "(250,80.01);(250,80.01);(250,60);(250,60)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.75"
%	 points= "(240,90);(240,90);(260,70);(260,70)"
%	 fill-style= "none"
%	 />
%<ellipse p3= "(252.58,67.42)"
%	 p2= "(252.58,72.58)"
%	 p1= "(247.42,72.58)"
%	 closure= "open"
%	 fill-color= "#330033"
%	 angle-end= "0"
%	 fill-style= "solid"
%	 angle-start= "0"
%	 />
%<multicurve stroke-width= "0.75"
%	 points= "(249.38,109.38);(249.38,109.38);(230,90);(230,90)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.75"
%	 points= "(230,90);(230,90);(250,70);(250,70)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.75"
%	 points= "(240,130);(240,130);(280,130);(280,130)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.75"
%	 points= "(280,110);(280,110);(280,130);(280,130)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.75"
%	 points= "(270,150);(270,150);(270,130);(270,130)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.75"
%	 points= "(260.62,110);(260.62,110);(280,110);(280,110)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.75"
%	 points= "(250,120.01);(250,120.01);(250,109.38);(250,109.38)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.75"
%	 points= "(240,130);(240,130);(260,110);(260,110)"
%	 fill-style= "none"
%	 />
%<ellipse p3= "(252.58,107.42)"
%	 p2= "(252.58,112.58)"
%	 p1= "(247.42,112.58)"
%	 closure= "open"
%	 fill-color= "#330033"
%	 angle-end= "0"
%	 fill-style= "solid"
%	 angle-start= "0"
%	 />
%<multicurve stroke-width= "0.75"
%	 points= "(230,130);(230,130);(250,110);(250,110)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.75"
%	 points= "(240.62,170);(240.62,170);(280.62,170);(280.62,170)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.75"
%	 points= "(280.62,150);(280.62,150);(280.62,170);(280.62,170)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.75"
%	 points= "(270.62,180);(270.62,180);(270.62,170);(270.62,170)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.75"
%	 points= "(261.25,150);(261.25,150);(280.62,150);(280.62,150)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.75"
%	 points= "(250.62,160.01);(250.62,160.01);(250.62,150);(250.62,150)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.75"
%	 points= "(240.62,170);(240.62,170);(260.62,150);(260.62,150)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.75"
%	 points= "(250.62,150);(250.62,150);(230,130);(230,130)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.75"
%	 points= "(30,100);(30,100);(30,60);(30,60)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.75"
%	 points= "(10.62,80.01);(10.62,80.01);(10.62,60);(10.62,60)"
%	 fill-style= "none"
%	 />
%<ellipse p3= "(13.2,77.42)"
%	 p2= "(13.2,82.58)"
%	 p1= "(8.05,82.58)"
%	 closure= "open"
%	 fill-color= "#330033"
%	 angle-end= "0"
%	 fill-style= "solid"
%	 angle-start= "0"
%	 />
%<multicurve stroke-width= "0.6"
%	 points= "(0,90);(0,90);(40,90);(40,90)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.6"
%	 points= "(40,70);(40,70);(40,90);(40,90)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.6"
%	 points= "(0,70);(0,70);(40,70);(40,70)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.6"
%	 points= "(0,90);(0,90);(0,70);(0,70)"
%	 fill-style= "none"
%	 />
%<text text-vert-align= "center-v"
%	 anchor-point= "(-10,0)"
%	 text-frame= "noframe"
%	 fill-style= "none"
%	 text-hor-align= "center-h"
%	 >
%$\zzero$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(280,0)"
%	 text-frame= "noframe"
%	 fill-style= "none"
%	 text-hor-align= "center-h"
%	 >
%$\tthree$
%</text>
%</jpic>
%%End JPIC-XML
%PSTricks content-type (pstricks.sty package needed)
%Add \usepackage{pstricks} in the preamble of your LaTeX file
%You can rescale the whole picture (to 80% for instance) by using the command \def\JPicScale{0.8}
\ifx\JPicScale\undefined\def\JPicScale{1}\fi
\psset{unit=\JPicScale mm}
\psset{linewidth=0.3,dotsep=1,hatchwidth=0.3,hatchsep=1.5,shadowsize=1,dimen=middle}
\psset{dotsize=0.7 2.5,dotscale=1 1,fillcolor=black}
\psset{arrowsize=1 2,arrowlength=1,arrowinset=0.25,tbarsize=0.7 5,bracketlength=0.15,rbracketlength=0.15}
\begin{pspicture}(0,0)(280.62,180)
\psline[linewidth=0.75](160,90)(200,90)
\psline[linewidth=0.75](200,70)(200,90)
\psline[linewidth=0.75](190,110)(190,90)
\psline[linewidth=0.75](180.62,70)(200,70)
\psline[linewidth=0.75](190,70)(190,60)
\psline[linewidth=0.75](170,80.01)(170,60)
\psline[linewidth=0.75](160,90)(180,70)
\newrgbcolor{userFillColour}{0.2 0 0.2}
\rput{0}(170,70){\psellipse[fillcolor=userFillColour,fillstyle=solid](0,0)(2.58,-2.58)}
\psline[linewidth=0.75](169.38,109.38)(150,90)
\psline[linewidth=0.75](150,90)(170,70)
\psline[linewidth=0.75](80,90)(120,90)
\psline[linewidth=0.75](120,70)(120,90)
\psline[linewidth=0.75](110,100)(110,90)
\psline[linewidth=0.75](100.62,70)(120,70)
\psline[linewidth=0.75](110,70)(110,60)
\psline[linewidth=0.75](90,80.01)(90,60)
\psline[linewidth=0.75](80,90)(100,70)
\psline[linewidth=0.75](160,130)(200,130)
\psline[linewidth=0.75](200,110)(200,130)
\psline[linewidth=0.75](190,140)(190,130)
\psline[linewidth=0.75](180.62,110)(200,110)
\psline[linewidth=0.75](170,120.01)(170,109.38)
\psline[linewidth=0.75](160,130)(180,110)
\psline[linewidth=0.75](240,90)(280,90)
\psline[linewidth=0.75](280,70)(280,90)
\psline[linewidth=0.75](270,110)(270,90)
\psline[linewidth=0.75](260.62,70)(280,70)
\psline[linewidth=0.75](270,70)(270,60)
\psline[linewidth=0.75](250,80.01)(250,60)
\psline[linewidth=0.75](240,90)(260,70)
\newrgbcolor{userFillColour}{0.2 0 0.2}
\rput{0}(250,70){\psellipse[fillcolor=userFillColour,fillstyle=solid](0,0)(2.58,-2.58)}
\psline[linewidth=0.75](249.38,109.38)(230,90)
\psline[linewidth=0.75](230,90)(250,70)
\psline[linewidth=0.75](240,130)(280,130)
\psline[linewidth=0.75](280,110)(280,130)
\psline[linewidth=0.75](270,150)(270,130)
\psline[linewidth=0.75](260.62,110)(280,110)
\psline[linewidth=0.75](250,120.01)(250,109.38)
\psline[linewidth=0.75](240,130)(260,110)
\newrgbcolor{userFillColour}{0.2 0 0.2}
\rput{0}(250,110){\psellipse[fillcolor=userFillColour,fillstyle=solid](0,0)(2.58,-2.58)}
\psline[linewidth=0.75](230,130)(250,110)
\psline[linewidth=0.75](240.62,170)(280.62,170)
\psline[linewidth=0.75](280.62,150)(280.62,170)
\psline[linewidth=0.75](270.62,180)(270.62,170)
\psline[linewidth=0.75](261.25,150)(280.62,150)
\psline[linewidth=0.75](250.62,160.01)(250.62,150)
\psline[linewidth=0.75](240.62,170)(260.62,150)
\psline[linewidth=0.75](250.62,150)(230,130)
\psline[linewidth=0.75](30,100)(30,60)
\psline[linewidth=0.75](10.62,80.01)(10.62,60)
\newrgbcolor{userFillColour}{0.2 0 0.2}
\rput{90}(10.62,80){\psellipse[fillcolor=userFillColour,fillstyle=solid](0,0)(2.58,-2.58)}
\psline[linewidth=0.6](0,90)(40,90)
\psline[linewidth=0.6](40,70)(40,90)
\psline[linewidth=0.6](0,70)(40,70)
\psline[linewidth=0.6](0,90)(0,70)
\rput(-10,0){$\zzero$}
\rput(280,0){$\tthree$}
\end{pspicture}


==> PIC/numbers.tex <==
%%Created by jPicEdt 1.4.1_03: mixed JPIC-XML/LaTeX format
%%Sun Oct 02 16:02:42 HST 2016
%%Begin JPIC-XML
%<?xml version="1.0" standalone="yes"?>
%<jpic x-min="0" x-max="270.62" y-min="59.38" y-max="179.38" auto-bounding="true">
%<multicurve stroke-width= "0.75"
%	 points= "(150,89.38);(150,89.38);(190,89.37);(190,89.37)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.75"
%	 points= "(190,69.38);(190,69.38);(190,89.37);(190,89.37)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.75"
%	 points= "(180,109.38);(180,109.38);(180,89.38);(180,89.38)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.75"
%	 points= "(170.62,69.38);(170.62,69.38);(190,69.38);(190,69.38)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.75"
%	 points= "(180,69.38);(180,69.38);(180,59.38);(180,59.38)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.75"
%	 points= "(160,79.38);(160,79.38);(160,59.38);(160,59.38)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.75"
%	 points= "(150,89.38);(150,89.38);(170,69.38);(170,69.38)"
%	 fill-style= "none"
%	 />
%<ellipse p3= "(162.58,66.8)"
%	 p2= "(162.58,71.96)"
%	 p1= "(157.42,71.96)"
%	 closure= "open"
%	 fill-color= "#330033"
%	 angle-end= "0"
%	 fill-style= "solid"
%	 angle-start= "0"
%	 />
%<multicurve stroke-width= "0.75"
%	 points= "(159.38,108.76);(159.38,108.76);(140,89.38);(140,89.38)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.75"
%	 points= "(140,89.38);(140,89.38);(160,69.38);(160,69.38)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.75"
%	 points= "(70,89.38);(70,89.38);(110,89.37);(110,89.37)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.75"
%	 points= "(110,69.38);(110,69.38);(110,89.37);(110,89.37)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.75"
%	 points= "(100,99.38);(100,99.38);(100,89.37);(100,89.37)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.75"
%	 points= "(90.62,69.38);(90.62,69.38);(110,69.38);(110,69.38)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.75"
%	 points= "(100,69.38);(100,69.38);(100,59.38);(100,59.38)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.75"
%	 points= "(80,79.38);(80,79.38);(80,59.38);(80,59.38)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.75"
%	 points= "(70,89.38);(70,89.38);(90,69.38);(90,69.38)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.75"
%	 points= "(150,129.38);(150,129.38);(190,129.37);(190,129.37)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.75"
%	 points= "(190,109.38);(190,109.38);(190,129.37);(190,129.37)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.75"
%	 points= "(180,139.38);(180,139.38);(180,129.37);(180,129.37)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.75"
%	 points= "(170.62,109.38);(170.62,109.38);(190,109.38);(190,109.38)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.75"
%	 points= "(160,119.38);(160,119.38);(160,108.75);(160,108.75)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.75"
%	 points= "(150,129.38);(150,129.38);(170,109.38);(170,109.38)"
%	 fill-style= "none"
%	 />
%<ellipse p3= "(162.58,106.8)"
%	 p2= "(162.58,111.96)"
%	 p1= "(157.42,111.96)"
%	 closure= "open"
%	 fill-color= "#330033"
%	 angle-end= "0"
%	 fill-style= "solid"
%	 angle-start= "0"
%	 />
%<multicurve stroke-width= "0.75"
%	 points= "(140,129.38);(140,129.38);(160,109.38);(160,109.38)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.75"
%	 points= "(230,89.38);(230,89.38);(270,89.37);(270,89.37)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.75"
%	 points= "(270,69.38);(270,69.38);(270,89.37);(270,89.37)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.75"
%	 points= "(260,109.38);(260,109.38);(260,89.38);(260,89.38)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.75"
%	 points= "(250.62,69.38);(250.62,69.38);(270,69.38);(270,69.38)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.75"
%	 points= "(260,69.38);(260,69.38);(260,59.38);(260,59.38)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.75"
%	 points= "(240,79.38);(240,79.38);(240,59.38);(240,59.38)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.75"
%	 points= "(230,89.38);(230,89.38);(250,69.38);(250,69.38)"
%	 fill-style= "none"
%	 />
%<ellipse p3= "(242.58,66.8)"
%	 p2= "(242.58,71.96)"
%	 p1= "(237.42,71.96)"
%	 closure= "open"
%	 fill-color= "#330033"
%	 angle-end= "0"
%	 fill-style= "solid"
%	 angle-start= "0"
%	 />
%<multicurve stroke-width= "0.75"
%	 points= "(239.38,108.76);(239.38,108.76);(220,89.38);(220,89.38)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.75"
%	 points= "(220,89.38);(220,89.38);(240,69.38);(240,69.38)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.75"
%	 points= "(230,129.38);(230,129.38);(270,129.37);(270,129.37)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.75"
%	 points= "(270,109.38);(270,109.38);(270,129.37);(270,129.37)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.75"
%	 points= "(260,149.38);(260,149.38);(260,129.37);(260,129.37)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.75"
%	 points= "(250.62,109.38);(250.62,109.38);(270,109.38);(270,109.38)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.75"
%	 points= "(240,119.38);(240,119.38);(240,108.75);(240,108.75)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.75"
%	 points= "(230,129.38);(230,129.38);(250,109.38);(250,109.38)"
%	 fill-style= "none"
%	 />
%<ellipse p3= "(242.58,106.8)"
%	 p2= "(242.58,111.96)"
%	 p1= "(237.42,111.96)"
%	 closure= "open"
%	 fill-color= "#330033"
%	 angle-end= "0"
%	 fill-style= "solid"
%	 angle-start= "0"
%	 />
%<multicurve stroke-width= "0.75"
%	 points= "(220,129.38);(220,129.38);(240,109.38);(240,109.38)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.75"
%	 points= "(230.62,169.38);(230.62,169.38);(270.62,169.37);(270.62,169.37)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.75"
%	 points= "(270.62,149.38);(270.62,149.38);(270.62,169.37);(270.62,169.37)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.75"
%	 points= "(260.62,179.38);(260.62,179.38);(260.62,169.37);(260.62,169.37)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.75"
%	 points= "(251.25,149.38);(251.25,149.38);(270.62,149.38);(270.62,149.38)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.75"
%	 points= "(240.62,159.38);(240.62,159.38);(240.62,149.38);(240.62,149.38)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.75"
%	 points= "(230.62,169.38);(230.62,169.38);(250.62,149.38);(250.62,149.38)"
%	 fill-style= "none"
%	 />
%<ellipse p3= "(243.2,146.8)"
%	 p2= "(243.2,151.95)"
%	 p1= "(238.05,151.95)"
%	 closure= "open"
%	 fill-color= "#330033"
%	 angle-end= "0"
%	 fill-style= "solid"
%	 angle-start= "0"
%	 />
%<multicurve stroke-width= "0.75"
%	 points= "(220.62,169.38);(220.62,169.38);(240.62,149.38);(240.62,149.38)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.75"
%	 points= "(240.62,149.38);(240.62,149.38);(220,129.38);(220,129.38)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.75"
%	 points= "(30,99.38);(30,99.38);(30,59.38);(30,59.38)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.75"
%	 points= "(10.62,79.38);(10.62,79.38);(10.62,59.38);(10.62,59.38)"
%	 fill-style= "none"
%	 />
%<ellipse p3= "(13.2,76.8)"
%	 p2= "(13.2,81.96)"
%	 p1= "(8.05,81.96)"
%	 closure= "open"
%	 fill-color= "#330033"
%	 angle-end= "0"
%	 fill-style= "solid"
%	 angle-start= "0"
%	 />
%<multicurve stroke-width= "0.6"
%	 points= "(0,89.38);(0,89.38);(40,89.37);(40,89.37)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.6"
%	 points= "(40,69.38);(40,69.38);(40,89.37);(40,89.37)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.6"
%	 points= "(0,69.38);(0,69.38);(40,69.38);(40,69.38)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.6"
%	 points= "(0,89.38);(0,89.38);(0,69.38);(0,69.38)"
%	 fill-style= "none"
%	 />
%</jpic>
%%End JPIC-XML
%PSTricks content-type (pstricks.sty package needed)
%Add \usepackage{pstricks} in the preamble of your LaTeX file
%You can rescale the whole picture (to 80% for instance) by using the command \def\JPicScale{0.8}
\ifx\JPicScale\undefined\def\JPicScale{1}\fi
\psset{unit=\JPicScale mm}
\psset{linewidth=0.3,dotsep=1,hatchwidth=0.3,hatchsep=1.5,shadowsize=1,dimen=middle}
\psset{dotsize=0.7 2.5,dotscale=1 1,fillcolor=black}
\psset{arrowsize=1 2,arrowlength=1,arrowinset=0.25,tbarsize=0.7 5,bracketlength=0.15,rbracketlength=0.15}
\begin{pspicture}(0,0)(270.62,179.38)
\psline[linewidth=0.75](150,89.38)(190,89.37)
\psline[linewidth=0.75](190,69.38)(190,89.37)
\psline[linewidth=0.75](180,109.38)(180,89.38)
\psline[linewidth=0.75](170.62,69.38)(190,69.38)
\psline[linewidth=0.75](180,69.38)(180,59.38)
\psline[linewidth=0.75](160,79.38)(160,59.38)
\psline[linewidth=0.75](150,89.38)(170,69.38)
\newrgbcolor{userFillColour}{0.2 0 0.2}
\rput{0}(160,69.38){\psellipse[fillcolor=userFillColour,fillstyle=solid](0,0)(2.58,-2.58)}
\psline[linewidth=0.75](159.38,108.76)(140,89.38)
\psline[linewidth=0.75](140,89.38)(160,69.38)
\psline[linewidth=0.75](70,89.38)(110,89.37)
\psline[linewidth=0.75](110,69.38)(110,89.37)
\psline[linewidth=0.75](100,99.38)(100,89.37)
\psline[linewidth=0.75](90.62,69.38)(110,69.38)
\psline[linewidth=0.75](100,69.38)(100,59.38)
\psline[linewidth=0.75](80,79.38)(80,59.38)
\psline[linewidth=0.75](70,89.38)(90,69.38)
\psline[linewidth=0.75](150,129.38)(190,129.37)
\psline[linewidth=0.75](190,109.38)(190,129.37)
\psline[linewidth=0.75](180,139.38)(180,129.37)
\psline[linewidth=0.75](170.62,109.38)(190,109.38)
\psline[linewidth=0.75](160,119.38)(160,108.75)
\psline[linewidth=0.75](150,129.38)(170,109.38)
\newrgbcolor{userFillColour}{0.2 0 0.2}
\rput{0}(160,109.38){\psellipse[fillcolor=userFillColour,fillstyle=solid](0,0)(2.58,-2.58)}
\psline[linewidth=0.75](140,129.38)(160,109.38)
\psline[linewidth=0.75](230,89.38)(270,89.37)
\psline[linewidth=0.75](270,69.38)(270,89.37)
\psline[linewidth=0.75](260,109.38)(260,89.38)
\psline[linewidth=0.75](250.62,69.38)(270,69.38)
\psline[linewidth=0.75](260,69.38)(260,59.38)
\psline[linewidth=0.75](240,79.38)(240,59.38)
\psline[linewidth=0.75](230,89.38)(250,69.38)
\newrgbcolor{userFillColour}{0.2 0 0.2}
\rput{0}(240,69.38){\psellipse[fillcolor=userFillColour,fillstyle=solid](0,0)(2.58,-2.58)}
\psline[linewidth=0.75](239.38,108.76)(220,89.38)
\psline[linewidth=0.75](220,89.38)(240,69.38)
\psline[linewidth=0.75](230,129.38)(270,129.37)
\psline[linewidth=0.75](270,109.38)(270,129.37)
\psline[linewidth=0.75](260,149.38)(260,129.37)
\psline[linewidth=0.75](250.62,109.38)(270,109.38)
\psline[linewidth=0.75](240,119.38)(240,108.75)
\psline[linewidth=0.75](230,129.38)(250,109.38)
\newrgbcolor{userFillColour}{0.2 0 0.2}
\rput{0}(240,109.38){\psellipse[fillcolor=userFillColour,fillstyle=solid](0,0)(2.58,-2.58)}
\psline[linewidth=0.75](220,129.38)(240,109.38)
\psline[linewidth=0.75](230.62,169.38)(270.62,169.37)
\psline[linewidth=0.75](270.62,149.38)(270.62,169.37)
\psline[linewidth=0.75](260.62,179.38)(260.62,169.37)
\psline[linewidth=0.75](251.25,149.38)(270.62,149.38)
\psline[linewidth=0.75](240.62,159.38)(240.62,149.38)
\psline[linewidth=0.75](230.62,169.38)(250.62,149.38)
\newrgbcolor{userFillColour}{0.2 0 0.2}
\rput{0}(240.62,149.38){\psellipse[fillcolor=userFillColour,fillstyle=solid](0,0)(2.58,-2.58)}
\psline[linewidth=0.75](220.62,169.38)(240.62,149.38)
\psline[linewidth=0.75](240.62,149.38)(220,129.38)
\psline[linewidth=0.75](30,99.38)(30,59.38)
\psline[linewidth=0.75](10.62,79.38)(10.62,59.38)
\newrgbcolor{userFillColour}{0.2 0 0.2}
\rput{0}(10.62,79.38){\psellipse[fillcolor=userFillColour,fillstyle=solid](0,0)(2.58,-2.58)}
\psline[linewidth=0.6](0,89.38)(40,89.37)
\psline[linewidth=0.6](40,69.38)(40,89.37)
\psline[linewidth=0.6](0,69.38)(40,69.38)
\psline[linewidth=0.6](0,89.38)(0,69.38)
\end{pspicture}


==> PIC/omega-3.tex <==
%%Created by jPicEdt 1.4.1_03: mixed JPIC-XML/LaTeX format
%%Mon Feb 22 17:07:47 GMT-10:00 2021
%%Begin JPIC-XML
%<?xml version="1.0" standalone="yes"?>
%<jpic x-min="2.5" x-max="197.5" y-min="0" y-max="100" auto-bounding="true">
%<multicurve fill-style= "none"
%	 points= "(75,10);(75,10);(75,0);(75,0)"
%	 stroke-width= "0.5"
%	 />
%<ellipse p3= "(76.25,8.75)"
%	 fill-style= "solid"
%	 p2= "(76.25,11.25)"
%	 p1= "(73.75,11.25)"
%	 closure= "open"
%	 angle-end= "0"
%	 stroke-width= "0.5"
%	 angle-start= "0"
%	 />
%<multicurve fill-style= "none"
%	 points= "(80,15);(80,15);(75,10);(75,10)"
%	 stroke-width= "0.5"
%	 />
%<multicurve fill-style= "none"
%	 points= "(75,10);(75,10);(70,15);(70,15)"
%	 stroke-width= "0.5"
%	 />
%<multicurve fill-style= "none"
%	 points= "(70,15);(70,15);(70,18.75);(70,18.75)"
%	 stroke-width= "0.5"
%	 />
%<multicurve fill-style= "none"
%	 points= "(80,15);(80,15);(80,55);(80,55)"
%	 stroke-width= "0.5"
%	 />
%<multicurve fill-style= "none"
%	 points= "(65,40);(65,40);(75,40);(75,40)"
%	 stroke-width= "0.5"
%	 />
%<multicurve fill-style= "none"
%	 points= "(55,50);(55,50);(65,50);(65,50)"
%	 stroke-width= "0.5"
%	 />
%<ellipse p3= "(73.52,18.98)"
%	 fill-style= "none"
%	 p2= "(73.52,26.02)"
%	 p1= "(66.48,26.02)"
%	 closure= "open"
%	 angle-end= "0"
%	 stroke-width= "0.5"
%	 angle-start= "0"
%	 />
%<multicurve fill-style= "none"
%	 points= "(70,26.25);(70,26.25);(70,40);(70,40)"
%	 stroke-width= "0.5"
%	 />
%<multicurve fill-style= "none"
%	 points= "(65,50);(65,50);(75,40);(75,40)"
%	 stroke-width= "0.5"
%	 />
%<multicurve fill-style= "none"
%	 points= "(55,50);(55,50);(65,40);(65,40)"
%	 stroke-width= "0.5"
%	 />
%<multicurve fill-style= "none"
%	 points= "(55,42.5);(55,42.5);(65,32.5);(65,32.5)"
%	 stroke-width= "0.5"
%	 />
%<multicurve fill-style= "none"
%	 points= "(70,45);(70,45);(70,55);(70,55)"
%	 stroke-width= "0.5"
%	 />
%<multicurve fill-style= "none"
%	 points= "(60,37.5);(60,37.5);(60,45);(60,45)"
%	 stroke-width= "0.5"
%	 />
%<multicurve fill-style= "none"
%	 points= "(55,32.5);(55,32.5);(65,32.5);(65,32.5)"
%	 stroke-width= "0.5"
%	 />
%<multicurve fill-style= "none"
%	 points= "(55,42.5);(55,42.5);(55,32.5);(55,32.5)"
%	 stroke-width= "0.5"
%	 />
%<multicurve fill-style= "none"
%	 points= "(67.5,55);(67.5,55);(82.5,55);(82.5,55)"
%	 stroke-width= "0.5"
%	 />
%<multicurve fill-style= "none"
%	 points= "(67.5,70);(67.5,70);(67.5,55);(67.5,55)"
%	 stroke-width= "0.5"
%	 />
%<multicurve fill-style= "none"
%	 points= "(67.5,70);(67.5,70);(82.5,55);(82.5,55)"
%	 stroke-width= "0.5"
%	 />
%<multicurve fill-style= "none"
%	 points= "(75,72.5);(75,72.5);(75,62.5);(75,62.5)"
%	 stroke-width= "0.5"
%	 />
%<multicurve fill-style= "none"
%	 points= "(15,40);(15,40);(27.5,40);(27.5,40)"
%	 stroke-width= "0.5"
%	 />
%<multicurve fill-style= "none"
%	 points= "(5,50);(5,50);(27.5,50);(27.5,50)"
%	 stroke-width= "0.5"
%	 />
%<multicurve fill-style= "none"
%	 points= "(20,0);(20,0);(20,40);(20,40)"
%	 stroke-width= "0.5"
%	 />
%<multicurve fill-style= "none"
%	 points= "(5,50);(5,50);(15,40);(15,40)"
%	 stroke-width= "0.5"
%	 />
%<multicurve fill-style= "none"
%	 points= "(5,42.5);(5,42.5);(15,32.5);(15,32.5)"
%	 stroke-width= "0.5"
%	 />
%<multicurve fill-style= "none"
%	 points= "(10,37.5);(10,37.5);(10,45);(10,45)"
%	 stroke-width= "0.5"
%	 />
%<multicurve fill-style= "none"
%	 points= "(5,32.5);(5,32.5);(15,32.5);(15,32.5)"
%	 stroke-width= "0.5"
%	 />
%<multicurve fill-style= "none"
%	 points= "(5,42.5);(5,42.5);(5,32.5);(5,32.5)"
%	 stroke-width= "0.5"
%	 />
%<multicurve fill-style= "none"
%	 points= "(27.5,50);(27.5,50);(27.5,40);(27.5,40)"
%	 stroke-width= "0.5"
%	 />
%<multicurve fill-style= "none"
%	 points= "(20,72.5);(20,72.5);(20,50);(20,50)"
%	 stroke-width= "0.5"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "solid"
%	 anchor-point= "(40,45)"
%	 text-frame= "noframe"
%	 stroke-width= "0.5"
%	 text-hor-align= "center-h"
%	 >
%\EQLS
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "solid"
%	 anchor-point= "(57.5,35)"
%	 text-frame= "noframe"
%	 stroke-width= "0.5"
%	 text-hor-align= "center-h"
%	 >
%$\Nee$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "solid"
%	 anchor-point= "(7.5,35)"
%	 text-frame= "noframe"
%	 stroke-width= "0.5"
%	 text-hor-align= "center-h"
%	 >
%$\Nee$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "solid"
%	 anchor-point= "(70,22.5)"
%	 text-frame= "noframe"
%	 stroke-width= "0.5"
%	 text-hor-align= "center-h"
%	 >
%$\addd$
%</text>
%<multicurve fill-style= "solid"
%	 points= "(2.5,52.5);(2.5,52.5);(30,52.5);(30,52.5)"
%	 stroke-width= "0.15"
%	 />
%<multicurve fill-style= "solid"
%	 points= "(2.5,30);(2.5,30);(2.5,52.5);(2.5,52.5)"
%	 stroke-width= "0.15"
%	 />
%<multicurve fill-style= "solid"
%	 points= "(30,30);(30,30);(2.5,30);(2.5,30)"
%	 stroke-width= "0.15"
%	 />
%<multicurve fill-style= "solid"
%	 points= "(30,52.5);(30,52.5);(30,30);(30,30)"
%	 stroke-width= "0.15"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "solid"
%	 anchor-point= "(27.5,32.5)"
%	 text-frame= "noframe"
%	 stroke-width= "0.5"
%	 text-hor-align= "center-h"
%	 >
%$\Homega$
%</text>
%<multicurve fill-style= "none"
%	 points= "(67.5,80);(67.5,80);(82.5,80);(82.5,80)"
%	 stroke-width= "0.5"
%	 />
%<multicurve fill-style= "none"
%	 points= "(82.5,80);(82.5,80);(82.5,65);(82.5,65)"
%	 stroke-width= "0.5"
%	 />
%<multicurve fill-style= "none"
%	 points= "(67.5,80);(67.5,80);(82.5,65);(82.5,65)"
%	 stroke-width= "0.5"
%	 />
%<multicurve fill-style= "none"
%	 points= "(70,90);(70,90);(70,80);(70,80)"
%	 stroke-width= "0.5"
%	 />
%<multicurve fill-style= "none"
%	 points= "(80,85);(80,85);(80,80);(80,80)"
%	 stroke-width= "0.5"
%	 />
%<ellipse p3= "(81.25,83.75)"
%	 fill-style= "solid"
%	 p2= "(81.25,86.25)"
%	 p1= "(78.75,86.25)"
%	 closure= "open"
%	 angle-end= "0"
%	 stroke-width= "0.5"
%	 angle-start= "0"
%	 />
%<multicurve fill-style= "none"
%	 points= "(75,95);(75,95);(75,85);(75,85)"
%	 stroke-width= "0.5"
%	 />
%<multicurve fill-style= "none"
%	 points= "(70,100);(70,100);(70,95);(70,95)"
%	 stroke-width= "0.5"
%	 />
%<multicurve fill-style= "none"
%	 points= "(65,95);(65,95);(75,85);(75,85)"
%	 stroke-width= "0.5"
%	 />
%<multicurve fill-style= "none"
%	 points= "(75,95);(75,95);(65,95);(65,95)"
%	 stroke-width= "0.5"
%	 />
%<multicurve fill-style= "none"
%	 points= "(12.5,80);(12.5,80);(27.5,80);(27.5,80)"
%	 stroke-width= "0.5"
%	 />
%<multicurve fill-style= "none"
%	 points= "(27.5,80);(27.5,80);(27.5,65);(27.5,65)"
%	 stroke-width= "0.5"
%	 />
%<multicurve fill-style= "none"
%	 points= "(12.5,80);(12.5,80);(27.5,65);(27.5,65)"
%	 stroke-width= "0.5"
%	 />
%<multicurve fill-style= "none"
%	 points= "(15,90);(15,90);(15,80);(15,80)"
%	 stroke-width= "0.5"
%	 />
%<multicurve fill-style= "none"
%	 points= "(25,85);(25,85);(25,80);(25,80)"
%	 stroke-width= "0.5"
%	 />
%<ellipse p3= "(26.25,83.75)"
%	 fill-style= "solid"
%	 p2= "(26.25,86.25)"
%	 p1= "(23.75,86.25)"
%	 closure= "open"
%	 angle-end= "0"
%	 stroke-width= "0.5"
%	 angle-start= "0"
%	 />
%<multicurve fill-style= "none"
%	 points= "(20,95);(20,95);(20,85);(20,85)"
%	 stroke-width= "0.5"
%	 />
%<multicurve fill-style= "none"
%	 points= "(15,97.5);(15,97.5);(15,95);(15,95)"
%	 stroke-width= "0.5"
%	 />
%<multicurve fill-style= "none"
%	 points= "(10,95);(10,95);(20,85);(20,85)"
%	 stroke-width= "0.5"
%	 />
%<multicurve fill-style= "none"
%	 points= "(20,95);(20,95);(10,95);(10,95)"
%	 stroke-width= "0.5"
%	 />
%<multicurve fill-style= "none"
%	 points= "(135,10);(135,10);(135,0);(135,0)"
%	 stroke-width= "0.5"
%	 />
%<ellipse p3= "(136.25,8.75)"
%	 fill-style= "solid"
%	 p2= "(136.25,11.25)"
%	 p1= "(133.75,11.25)"
%	 closure= "open"
%	 angle-end= "0"
%	 stroke-width= "0.5"
%	 angle-start= "0"
%	 />
%<multicurve fill-style= "none"
%	 points= "(140,15);(140,15);(135,10);(135,10)"
%	 stroke-width= "0.5"
%	 />
%<multicurve fill-style= "none"
%	 points= "(135,10);(135,10);(130,15);(130,15)"
%	 stroke-width= "0.5"
%	 />
%<multicurve fill-style= "none"
%	 points= "(130,15);(130,15);(130,18.75);(130,18.75)"
%	 stroke-width= "0.5"
%	 />
%<multicurve fill-style= "none"
%	 points= "(140,15);(140,15);(140,55);(140,55)"
%	 stroke-width= "0.5"
%	 />
%<multicurve fill-style= "none"
%	 points= "(125,40);(125,40);(135,40);(135,40)"
%	 stroke-width= "0.5"
%	 />
%<multicurve fill-style= "none"
%	 points= "(115,50);(115,50);(125,50);(125,50)"
%	 stroke-width= "0.5"
%	 />
%<ellipse p3= "(133.52,18.98)"
%	 fill-style= "none"
%	 p2= "(133.52,26.02)"
%	 p1= "(126.48,26.02)"
%	 closure= "open"
%	 angle-end= "0"
%	 stroke-width= "0.5"
%	 angle-start= "0"
%	 />
%<multicurve fill-style= "none"
%	 points= "(130,26.25);(130,26.25);(130,40);(130,40)"
%	 stroke-width= "0.5"
%	 />
%<multicurve fill-style= "none"
%	 points= "(125,50);(125,50);(135,40);(135,40)"
%	 stroke-width= "0.5"
%	 />
%<multicurve fill-style= "none"
%	 points= "(115,50);(115,50);(125,40);(125,40)"
%	 stroke-width= "0.5"
%	 />
%<multicurve fill-style= "none"
%	 points= "(115,42.5);(115,42.5);(125,32.5);(125,32.5)"
%	 stroke-width= "0.5"
%	 />
%<multicurve fill-style= "none"
%	 points= "(130,45);(130,45);(130,55);(130,55)"
%	 stroke-width= "0.5"
%	 />
%<multicurve fill-style= "none"
%	 points= "(120,37.5);(120,37.5);(120,45);(120,45)"
%	 stroke-width= "0.5"
%	 />
%<multicurve fill-style= "none"
%	 points= "(115,32.5);(115,32.5);(125,32.5);(125,32.5)"
%	 stroke-width= "0.5"
%	 />
%<multicurve fill-style= "none"
%	 points= "(115,42.5);(115,42.5);(115,32.5);(115,32.5)"
%	 stroke-width= "0.5"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "solid"
%	 anchor-point= "(100,45)"
%	 text-frame= "noframe"
%	 stroke-width= "0.5"
%	 text-hor-align= "center-h"
%	 >
%\EQLS
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "solid"
%	 anchor-point= "(117.5,35)"
%	 text-frame= "noframe"
%	 stroke-width= "0.5"
%	 text-hor-align= "center-h"
%	 >
%$\Nee$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "solid"
%	 anchor-point= "(130,22.5)"
%	 text-frame= "noframe"
%	 stroke-width= "0.5"
%	 text-hor-align= "center-h"
%	 >
%$\addd$
%</text>
%<ellipse p3= "(141.25,53.75)"
%	 fill-style= "solid"
%	 p2= "(141.25,56.25)"
%	 p1= "(138.75,56.25)"
%	 closure= "open"
%	 angle-end= "0"
%	 stroke-width= "0.5"
%	 angle-start= "0"
%	 />
%<multicurve fill-style= "none"
%	 points= "(135,60);(135,60);(135,50);(135,50)"
%	 stroke-width= "0.5"
%	 />
%<multicurve fill-style= "none"
%	 points= "(130,100);(130,100);(130,60);(130,60)"
%	 stroke-width= "0.5"
%	 />
%<multicurve fill-style= "none"
%	 points= "(125,60);(125,60);(135,50);(135,50)"
%	 stroke-width= "0.5"
%	 />
%<multicurve fill-style= "none"
%	 points= "(135,60);(135,60);(125,60);(125,60)"
%	 stroke-width= "0.5"
%	 />
%<multicurve fill-style= "none"
%	 points= "(190,0);(190,0);(190,18.75);(190,18.75)"
%	 stroke-width= "0.5"
%	 />
%<multicurve fill-style= "none"
%	 points= "(185,40);(185,40);(195,40);(195,40)"
%	 stroke-width= "0.5"
%	 />
%<multicurve fill-style= "none"
%	 points= "(175,50);(175,50);(195,50);(195,50)"
%	 stroke-width= "0.5"
%	 />
%<ellipse p3= "(193.52,18.98)"
%	 fill-style= "none"
%	 p2= "(193.52,26.02)"
%	 p1= "(186.48,26.02)"
%	 closure= "open"
%	 angle-end= "0"
%	 stroke-width= "0.5"
%	 angle-start= "0"
%	 />
%<multicurve fill-style= "none"
%	 points= "(190,26.25);(190,26.25);(190,40);(190,40)"
%	 stroke-width= "0.5"
%	 />
%<multicurve fill-style= "none"
%	 points= "(175,50);(175,50);(185,40);(185,40)"
%	 stroke-width= "0.5"
%	 />
%<multicurve fill-style= "none"
%	 points= "(175,42.5);(175,42.5);(185,32.5);(185,32.5)"
%	 stroke-width= "0.5"
%	 />
%<multicurve fill-style= "none"
%	 points= "(180,37.5);(180,37.5);(180,45);(180,45)"
%	 stroke-width= "0.5"
%	 />
%<multicurve fill-style= "none"
%	 points= "(175,32.5);(175,32.5);(185,32.5);(185,32.5)"
%	 stroke-width= "0.5"
%	 />
%<multicurve fill-style= "none"
%	 points= "(175,42.5);(175,42.5);(175,32.5);(175,32.5)"
%	 stroke-width= "0.5"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "solid"
%	 anchor-point= "(160,45)"
%	 text-frame= "noframe"
%	 stroke-width= "0.5"
%	 text-hor-align= "center-h"
%	 >
%\EQLS
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "solid"
%	 anchor-point= "(177.5,35)"
%	 text-frame= "noframe"
%	 stroke-width= "0.5"
%	 text-hor-align= "center-h"
%	 >
%$\Nee$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "solid"
%	 anchor-point= "(190,22.5)"
%	 text-frame= "noframe"
%	 stroke-width= "0.5"
%	 text-hor-align= "center-h"
%	 >
%$\addd$
%</text>
%<multicurve fill-style= "none"
%	 points= "(195,50);(195,50);(195,40);(195,40)"
%	 stroke-width= "0.5"
%	 />
%<multicurve fill-style= "none"
%	 points= "(190,100);(190,100);(190,50);(190,50)"
%	 stroke-width= "0.5"
%	 />
%<multicurve fill-style= "solid"
%	 points= "(172.5,52.5);(172.5,52.5);(197.5,52.5);(197.5,52.5)"
%	 stroke-width= "0.15"
%	 />
%<multicurve fill-style= "solid"
%	 points= "(172.5,30);(172.5,30);(172.5,52.5);(172.5,52.5)"
%	 stroke-width= "0.15"
%	 />
%<multicurve fill-style= "solid"
%	 points= "(197.5,30);(197.5,30);(172.5,30);(172.5,30)"
%	 stroke-width= "0.15"
%	 />
%<multicurve fill-style= "solid"
%	 points= "(197.5,52.5);(197.5,52.5);(197.5,30);(197.5,30)"
%	 stroke-width= "0.15"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "solid"
%	 anchor-point= "(195,32.5)"
%	 text-frame= "noframe"
%	 stroke-width= "0.5"
%	 text-hor-align= "center-h"
%	 >
%$\Homega$
%</text>
%<multicurve fill-style= "solid"
%	 points= "(7.5,97.5);(7.5,97.5);(30,97.5);(30,97.5)"
%	 stroke-width= "0.15"
%	 />
%<multicurve fill-style= "solid"
%	 points= "(7.5,62.5);(7.5,62.5);(7.5,97.5);(7.5,97.5)"
%	 stroke-width= "0.15"
%	 />
%<multicurve fill-style= "solid"
%	 points= "(30,62.5);(30,62.5);(7.5,62.5);(7.5,62.5)"
%	 stroke-width= "0.15"
%	 />
%<multicurve fill-style= "solid"
%	 points= "(30,97.5);(30,97.5);(30,62.5);(30,62.5)"
%	 stroke-width= "0.15"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "solid"
%	 anchor-point= "(12.5,65)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\pseey$
%</text>
%<multicurve fill-style= "none"
%	 points= "(15,100);(15,100);(15,97.5);(15,97.5)"
%	 stroke-width= "0.5"
%	 />
%</jpic>
%%End JPIC-XML
%PSTricks content-type (pstricks.sty package needed)
%Add \usepackage{pstricks} in the preamble of your LaTeX file
%You can rescale the whole picture (to 80% for instance) by using the command \def\JPicScale{0.8}
\ifx\JPicScale\undefined\def\JPicScale{1}\fi
\psset{unit=\JPicScale mm}
\psset{linewidth=0.3,dotsep=1,hatchwidth=0.3,hatchsep=1.5,shadowsize=1,dimen=middle}
\psset{dotsize=0.7 2.5,dotscale=1 1,fillcolor=black}
\psset{arrowsize=1 2,arrowlength=1,arrowinset=0.25,tbarsize=0.7 5,bracketlength=0.15,rbracketlength=0.15}
\begin{pspicture}(0,0)(197.5,100)
\psline[linewidth=0.5](75,10)(75,0)
\rput{0}(75,10){\psellipse[linewidth=0.5,fillstyle=solid](0,0)(1.25,-1.25)}
\psline[linewidth=0.5](80,15)(75,10)
\psline[linewidth=0.5](75,10)(70,15)
\psline[linewidth=0.5](70,15)(70,18.75)
\psline[linewidth=0.5](80,15)(80,55)
\psline[linewidth=0.5](65,40)(75,40)
\psline[linewidth=0.5](55,50)(65,50)
\rput{90}(70,22.5){\psellipse[linewidth=0.5](0,0)(3.52,-3.52)}
\psline[linewidth=0.5](70,26.25)(70,40)
\psline[linewidth=0.5](65,50)(75,40)
\psline[linewidth=0.5](55,50)(65,40)
\psline[linewidth=0.5](55,42.5)(65,32.5)
\psline[linewidth=0.5](70,45)(70,55)
\psline[linewidth=0.5](60,37.5)(60,45)
\psline[linewidth=0.5](55,32.5)(65,32.5)
\psline[linewidth=0.5](55,42.5)(55,32.5)
\psline[linewidth=0.5](67.5,55)(82.5,55)
\psline[linewidth=0.5](67.5,70)(67.5,55)
\psline[linewidth=0.5](67.5,70)(82.5,55)
\psline[linewidth=0.5](75,72.5)(75,62.5)
\psline[linewidth=0.5](15,40)(27.5,40)
\psline[linewidth=0.5](5,50)(27.5,50)
\psline[linewidth=0.5](20,0)(20,40)
\psline[linewidth=0.5](5,50)(15,40)
\psline[linewidth=0.5](5,42.5)(15,32.5)
\psline[linewidth=0.5](10,37.5)(10,45)
\psline[linewidth=0.5](5,32.5)(15,32.5)
\psline[linewidth=0.5](5,42.5)(5,32.5)
\psline[linewidth=0.5](27.5,50)(27.5,40)
\psline[linewidth=0.5](20,72.5)(20,50)
\rput(40,45){\EQLS}
\rput(57.5,35){$\Nee$}
\rput(7.5,35){$\Nee$}
\rput(70,22.5){$\addd$}
\psline[linewidth=0.15,fillstyle=solid](2.5,52.5)(30,52.5)
\psline[linewidth=0.15,fillstyle=solid](2.5,30)(2.5,52.5)
\psline[linewidth=0.15,fillstyle=solid](30,30)(2.5,30)
\psline[linewidth=0.15,fillstyle=solid](30,52.5)(30,30)
\rput(27.5,32.5){$\Homega$}
\psline[linewidth=0.5](67.5,80)(82.5,80)
\psline[linewidth=0.5](82.5,80)(82.5,65)
\psline[linewidth=0.5](67.5,80)(82.5,65)
\psline[linewidth=0.5](70,90)(70,80)
\psline[linewidth=0.5](80,85)(80,80)
\rput{0}(80,85){\psellipse[linewidth=0.5,fillstyle=solid](0,0)(1.25,-1.25)}
\psline[linewidth=0.5](75,95)(75,85)
\psline[linewidth=0.5](70,100)(70,95)
\psline[linewidth=0.5](65,95)(75,85)
\psline[linewidth=0.5](75,95)(65,95)
\psline[linewidth=0.5](12.5,80)(27.5,80)
\psline[linewidth=0.5](27.5,80)(27.5,65)
\psline[linewidth=0.5](12.5,80)(27.5,65)
\psline[linewidth=0.5](15,90)(15,80)
\psline[linewidth=0.5](25,85)(25,80)
\rput{0}(25,85){\psellipse[linewidth=0.5,fillstyle=solid](0,0)(1.25,-1.25)}
\psline[linewidth=0.5](20,95)(20,85)
\psline[linewidth=0.5](15,97.5)(15,95)
\psline[linewidth=0.5](10,95)(20,85)
\psline[linewidth=0.5](20,95)(10,95)
\psline[linewidth=0.5](135,10)(135,0)
\rput{0}(135,10){\psellipse[linewidth=0.5,fillstyle=solid](0,0)(1.25,-1.25)}
\psline[linewidth=0.5](140,15)(135,10)
\psline[linewidth=0.5](135,10)(130,15)
\psline[linewidth=0.5](130,15)(130,18.75)
\psline[linewidth=0.5](140,15)(140,55)
\psline[linewidth=0.5](125,40)(135,40)
\psline[linewidth=0.5](115,50)(125,50)
\rput{0}(130,22.5){\psellipse[linewidth=0.5](0,0)(3.52,-3.52)}
\psline[linewidth=0.5](130,26.25)(130,40)
\psline[linewidth=0.5](125,50)(135,40)
\psline[linewidth=0.5](115,50)(125,40)
\psline[linewidth=0.5](115,42.5)(125,32.5)
\psline[linewidth=0.5](130,45)(130,55)
\psline[linewidth=0.5](120,37.5)(120,45)
\psline[linewidth=0.5](115,32.5)(125,32.5)
\psline[linewidth=0.5](115,42.5)(115,32.5)
\rput(100,45){\EQLS}
\rput(117.5,35){$\Nee$}
\rput(130,22.5){$\addd$}
\rput{0}(140,55){\psellipse[linewidth=0.5,fillstyle=solid](0,0)(1.25,-1.25)}
\psline[linewidth=0.5](135,60)(135,50)
\psline[linewidth=0.5](130,100)(130,60)
\psline[linewidth=0.5](125,60)(135,50)
\psline[linewidth=0.5](135,60)(125,60)
\psline[linewidth=0.5](190,0)(190,18.75)
\psline[linewidth=0.5](185,40)(195,40)
\psline[linewidth=0.5](175,50)(195,50)
\rput{0}(190,22.5){\psellipse[linewidth=0.5](0,0)(3.52,-3.52)}
\psline[linewidth=0.5](190,26.25)(190,40)
\psline[linewidth=0.5](175,50)(185,40)
\psline[linewidth=0.5](175,42.5)(185,32.5)
\psline[linewidth=0.5](180,37.5)(180,45)
\psline[linewidth=0.5](175,32.5)(185,32.5)
\psline[linewidth=0.5](175,42.5)(175,32.5)
\rput(160,45){\EQLS}
\rput(177.5,35){$\Nee$}
\rput(190,22.5){$\addd$}
\psline[linewidth=0.5](195,50)(195,40)
\psline[linewidth=0.5](190,100)(190,50)
\psline[linewidth=0.15,fillstyle=solid](172.5,52.5)(197.5,52.5)
\psline[linewidth=0.15,fillstyle=solid](172.5,30)(172.5,52.5)
\psline[linewidth=0.15,fillstyle=solid](197.5,30)(172.5,30)
\psline[linewidth=0.15,fillstyle=solid](197.5,52.5)(197.5,30)
\rput(195,32.5){$\Homega$}
\psline[linewidth=0.15,fillstyle=solid](7.5,97.5)(30,97.5)
\psline[linewidth=0.15,fillstyle=solid](7.5,62.5)(7.5,97.5)
\psline[linewidth=0.15,fillstyle=solid](30,62.5)(7.5,62.5)
\psline[linewidth=0.15,fillstyle=solid](30,97.5)(30,62.5)
\rput(12.5,65){$\pseey$}
\psline[linewidth=0.5](15,100)(15,97.5)
\end{pspicture}


==> PIC/otimes.tex <==
%%Created by jPicEdt 1.4.1_03: mixed JPIC-XML/LaTeX format
%%Wed Sep 28 22:27:05 HST 2016
%%Begin JPIC-XML
%<?xml version="1.0" standalone="yes"?>
%<jpic x-min="0" x-max="110" y-min="-33.75" y-max="36.25" auto-bounding="true">
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(0,12.5);(0,12.5);(40,12.5);(40,12.5)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(0,12.5);(0,12.5);(0,-12.5);(0,-12.5)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(40,-12.5);(40,-12.5);(40,12.5);(40,12.5)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(20,30);(20,30);(20,12.5);(20,12.5)"
%	 />
%<text stroke-width= "0.75"
%	 text-vert-align= "center-v"
%	 anchor-point= "(20,36.25)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\nameslang$
%</text>
%<text stroke-width= "0.75"
%	 text-vert-align= "center-v"
%	 anchor-point= "(20,-33.75)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\inputt$
%</text>
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(0,-12.5);(0,-12.5);(40,-12.5);(40,-12.5)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(20,-12.5);(20,-12.5);(20,-27.5);(20,-27.5)"
%	 />
%<text stroke-width= "0.75"
%	 text-vert-align= "center-v"
%	 anchor-point= "(20,0)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\machine
%</text>
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(70,12.5);(70,12.5);(110,12.5);(110,12.5)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(70,12.5);(70,12.5);(70,-12.5);(70,-12.5)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(110,-12.5);(110,-12.5);(110,12.5);(110,12.5)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(90,30);(90,30);(90,12.5);(90,12.5)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(70,-12.5);(70,-12.5);(110,-12.5);(110,-12.5)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(90,-12.5);(90,-12.5);(90,-27.5);(90,-27.5)"
%	 />
%<text text-vert-align= "center-v"
%	 anchor-point= "(90,-33.12)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\inputg$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(90,0)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\otherfun
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(90,36.25)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\outputg$
%</text>
%</jpic>
%%End JPIC-XML
%PSTricks content-type (pstricks.sty package needed)
%Add \usepackage{pstricks} in the preamble of your LaTeX file
%You can rescale the whole picture (to 80% for instance) by using the command \def\JPicScale{0.8}
\ifx\JPicScale\undefined\def\JPicScale{1}\fi
\psset{unit=\JPicScale mm}
\psset{linewidth=0.3,dotsep=1,hatchwidth=0.3,hatchsep=1.5,shadowsize=1,dimen=middle}
\psset{dotsize=0.7 2.5,dotscale=1 1,fillcolor=black}
\psset{arrowsize=1 2,arrowlength=1,arrowinset=0.25,tbarsize=0.7 5,bracketlength=0.15,rbracketlength=0.15}
\begin{pspicture}(0,0)(110,36.25)
\psline[linewidth=0.75](0,12.5)(40,12.5)
\psline[linewidth=0.75](0,12.5)(0,-12.5)
\psline[linewidth=0.75](40,-12.5)(40,12.5)
\psline[linewidth=0.75](20,30)(20,12.5)
\rput(20,36.25){$\nameslang$}
\rput(20,-33.75){$\inputt$}
\psline[linewidth=0.75](0,-12.5)(40,-12.5)
\psline[linewidth=0.75](20,-12.5)(20,-27.5)
\rput(20,0){\machine}
\psline[linewidth=0.75](70,12.5)(110,12.5)
\psline[linewidth=0.75](70,12.5)(70,-12.5)
\psline[linewidth=0.75](110,-12.5)(110,12.5)
\psline[linewidth=0.75](90,30)(90,12.5)
\psline[linewidth=0.75](70,-12.5)(110,-12.5)
\psline[linewidth=0.75](90,-12.5)(90,-27.5)
\rput(90,-33.12){$\inputg$}
\rput(90,0){\otherfun}
\rput(90,36.25){$\outputg$}
\end{pspicture}


==> PIC/pair-0.tex <==
%%Created by jPicEdt 1.4.1_03: mixed JPIC-XML/LaTeX format
%%Fri Dec 21 12:47:56 GMT-08:00 2018
%%Begin JPIC-XML
%<?xml version="1.0" standalone="yes"?>
%<jpic x-min="0" x-max="385" y-min="0" y-max="75" auto-bounding="true">
%<multicurve fill-style= "none"
%	 points= "(70,45);(70,45);(100,45);(100,45)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(120,25);(120,25);(100,45);(100,45)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(110,55);(110,55);(110,35);(110,35)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(90.62,25);(90.62,25);(120,25);(120,25)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(95,25);(95,25);(95,0);(95,0)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(80,35);(80,35);(80,25);(80,25)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(70,45);(70,45);(90,25);(90,25)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(30,25);(30,25);(30,0);(30,0)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(10,25);(10,25);(10,0);(10,0)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(0,45);(0,45);(40,45);(40,45)"
%	 stroke-width= "0.6"
%	 />
%<multicurve fill-style= "none"
%	 points= "(40,25);(40,25);(40,45);(40,45)"
%	 stroke-width= "0.6"
%	 />
%<multicurve fill-style= "none"
%	 points= "(0,25);(0,25);(40,25);(40,25)"
%	 stroke-width= "0.6"
%	 />
%<multicurve fill-style= "none"
%	 points= "(0,45);(0,45);(0,25);(0,25)"
%	 stroke-width= "0.6"
%	 />
%<multicurve fill-style= "none"
%	 points= "(20,55);(20,55);(20,45);(20,45)"
%	 stroke-width= "0.75"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(20,35)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\pairtag$
%</text>
%<multicurve fill-style= "none"
%	 points= "(70,35);(70,35);(90,15);(90,15)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(70,15);(70,15);(89.38,15);(89.38,15)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(70,15);(70,15);(70,34.99);(70,34.99)"
%	 stroke-width= "0.75"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(75,20)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\iiftag$
%</text>
%<multicurve fill-style= "none"
%	 points= "(113.75,25);(113.75,25);(113.75,0);(113.75,0)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(240,45);(240,45);(300,45);(300,45)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(300,25.01);(300,25.01);(300,45);(300,45)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(280,55);(280,55);(280,44.99);(280,44.99)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(260.62,25);(260.62,25);(300,25);(300,25)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(265,25);(265,25);(265,0);(265,0)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(250,35);(250,35);(250,25);(250,25)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(240,45);(240,45);(260,25);(260,25)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(240,35);(240,35);(260,15);(260,15)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(240,15);(240,15);(259.38,15);(259.38,15)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(240,15);(240,15);(240,34.99);(240,34.99)"
%	 stroke-width= "0.75"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(245,20)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\iiftag$
%</text>
%<multicurve fill-style= "none"
%	 points= "(295,25);(295,25);(295,0);(295,0)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(280,25);(280,25);(280,0);(280,0)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(330,45);(330,45);(375,45);(375,45)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(375,25);(375,25);(375,44.99);(375,44.99)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(365,55);(365,55);(365,44.99);(365,44.99)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(340,35);(340,35);(340,25);(340,25)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(330,45);(330,45);(350,25);(350,25)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(340,25);(340,25);(350,15);(350,15)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(350,15);(350,15);(380,15);(380,15)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(385,0);(385,0);(385,10);(385,10)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 stroke-overstrike-width= "2"
%	 points= "(355,25);(355,25);(355,0);(355,0)"
%	 stroke-overstrike= "true"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 stroke-overstrike-width= "2"
%	 points= "(370,25);(370,25);(370,0);(370,0)"
%	 stroke-overstrike= "true"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(350.62,25);(350.62,25);(375,25);(375,25)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(380,15);(380,15);(385,10);(385,10)"
%	 stroke-width= "0.75"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(360,35)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\iiftagg$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(315,35)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\EQLS$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(55,35)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\EQLS$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(185,35)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\where
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(95,35)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\stag$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(275,35)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\uevaltag$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(385,5)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\bee$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(355,5)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\eex$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(370,5)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\why$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(295,5)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\bee$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(265,5)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\eex$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(280,5)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\why$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(10,5)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\eex$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(30,5)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\why$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(94.38,5.62)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\eex$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(112.5,5.62)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\why$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(55,75)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\ceqn$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(315,75)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\deqn$
%</text>
%</jpic>
%%End JPIC-XML
%PSTricks content-type (pstricks.sty package needed)
%Add \usepackage{pstricks} in the preamble of your LaTeX file
%You can rescale the whole picture (to 80% for instance) by using the command \def\JPicScale{0.8}
\ifx\JPicScale\undefined\def\JPicScale{1}\fi
\psset{unit=\JPicScale mm}
\psset{linewidth=0.3,dotsep=1,hatchwidth=0.3,hatchsep=1.5,shadowsize=1,dimen=middle}
\psset{dotsize=0.7 2.5,dotscale=1 1,fillcolor=black}
\psset{arrowsize=1 2,arrowlength=1,arrowinset=0.25,tbarsize=0.7 5,bracketlength=0.15,rbracketlength=0.15}
\begin{pspicture}(0,0)(385,75)
\psline[linewidth=0.75](70,45)(100,45)
\psline[linewidth=0.75](120,25)(100,45)
\psline[linewidth=0.75](110,55)(110,35)
\psline[linewidth=0.75](90.62,25)(120,25)
\psline[linewidth=0.75](95,25)(95,0)
\psline[linewidth=0.75](80,35)(80,25)
\psline[linewidth=0.75](70,45)(90,25)
\psline[linewidth=0.75](30,25)(30,0)
\psline[linewidth=0.75](10,25)(10,0)
\psline[linewidth=0.6](0,45)(40,45)
\psline[linewidth=0.6](40,25)(40,45)
\psline[linewidth=0.6](0,25)(40,25)
\psline[linewidth=0.6](0,45)(0,25)
\psline[linewidth=0.75](20,55)(20,45)
\rput(20,35){$\pairtag$}
\psline[linewidth=0.75](70,35)(90,15)
\psline[linewidth=0.75](70,15)(89.38,15)
\psline[linewidth=0.75](70,15)(70,34.99)
\rput(75,20){$\iiftag$}
\psline[linewidth=0.75](113.75,25)(113.75,0)
\psline[linewidth=0.75](240,45)(300,45)
\psline[linewidth=0.75](300,25.01)(300,45)
\psline[linewidth=0.75](280,55)(280,44.99)
\psline[linewidth=0.75](260.62,25)(300,25)
\psline[linewidth=0.75](265,25)(265,0)
\psline[linewidth=0.75](250,35)(250,25)
\psline[linewidth=0.75](240,45)(260,25)
\psline[linewidth=0.75](240,35)(260,15)
\psline[linewidth=0.75](240,15)(259.38,15)
\psline[linewidth=0.75](240,15)(240,34.99)
\rput(245,20){$\iiftag$}
\psline[linewidth=0.75](295,25)(295,0)
\psline[linewidth=0.75](280,25)(280,0)
\psline[linewidth=0.75](330,45)(375,45)
\psline[linewidth=0.75](375,25)(375,44.99)
\psline[linewidth=0.75](365,55)(365,44.99)
\psline[linewidth=0.75](340,35)(340,25)
\psline[linewidth=0.75](330,45)(350,25)
\psline[linewidth=0.75](340,25)(350,15)
\psline[linewidth=0.75](350,15)(380,15)
\psline[linewidth=0.75](385,0)(385,10)
\psline[linewidth=0.75,border=2](355,25)(355,0)
\psline[linewidth=0.75,border=2](370,25)(370,0)
\psline[linewidth=0.75](350.62,25)(375,25)
\psline[linewidth=0.75](380,15)(385,10)
\rput(360,35){$\iiftagg$}
\rput(315,35){$\EQLS$}
\rput(55,35){$\EQLS$}
\rput(185,35){\where}
\rput(95,35){$\stag$}
\rput(275,35){$\uevaltag$}
\rput[r](385,5){$\bee$}
\rput[r](355,5){$\eex$}
\rput[r](370,5){$\why$}
\rput[r](295,5){$\bee$}
\rput[r](265,5){$\eex$}
\rput[r](280,5){$\why$}
\rput[r](10,5){$\eex$}
\rput[r](30,5){$\why$}
\rput[r](94.38,5.62){$\eex$}
\rput[r](112.5,5.62){$\why$}
\rput(55,75){$\ceqn$}
\rput(315,75){$\deqn$}
\end{pspicture}


==> PIC/pair-proj-1.tex <==
%%Created by jPicEdt 1.4.1_03: mixed JPIC-XML/LaTeX format
%%Sat Dec 22 17:20:59 GMT-10:00 2018
%%Begin JPIC-XML
%<?xml version="1.0" standalone="yes"?>
%<jpic x-min="20" x-max="380" y-min="0" y-max="275" auto-bounding="true">
%<multicurve fill-style= "none"
%	 points= "(330,255);(330,255);(360,255);(360,255)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(380,235);(380,235);(360,255);(360,255)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(370,265);(370,265);(370,245);(370,245)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(350.62,235);(350.62,235);(380,235);(380,235)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(355,235);(355,235);(355,210);(355,210)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(340,245);(340,245);(340,235);(340,235)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(330,255);(330,255);(350,235);(350,235)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(290,235);(290,235);(290,210);(290,210)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(270,235);(270,235);(270,210);(270,210)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(260,255);(260,255);(300,255);(300,255)"
%	 stroke-width= "0.6"
%	 />
%<multicurve fill-style= "none"
%	 points= "(300,235);(300,235);(300,255);(300,255)"
%	 stroke-width= "0.6"
%	 />
%<multicurve fill-style= "none"
%	 points= "(260,235);(260,235);(300,235);(300,235)"
%	 stroke-width= "0.6"
%	 />
%<multicurve fill-style= "none"
%	 points= "(260,255);(260,255);(260,235);(260,235)"
%	 stroke-width= "0.6"
%	 />
%<multicurve fill-style= "none"
%	 points= "(280,265);(280,265);(280,255);(280,255)"
%	 stroke-width= "0.75"
%	 />
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(280,245)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\pairtag$
%</text>
%<multicurve fill-style= "none"
%	 points= "(330,245);(330,245);(350,225);(350,225)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(330,225);(330,225);(349.38,225);(349.38,225)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(330,225);(330,225);(330,244.99);(330,244.99)"
%	 stroke-width= "0.75"
%	 />
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(335,230)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\iiftag$
%</text>
%<multicurve fill-style= "none"
%	 points= "(373.75,235);(373.75,235);(373.75,210);(373.75,210)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(20,255);(20,255);(80,255);(80,255)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(80,235.01);(80,235.01);(80,255);(80,255)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(60,265);(60,265);(60,254.99);(60,254.99)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(40.62,235);(40.62,235);(80,235);(80,235)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(45,235);(45,235);(45,210);(45,210)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(30,245);(30,245);(30,235);(30,235)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(20,255);(20,255);(40,235);(40,235)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(20,245);(20,245);(40,225);(40,225)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(20,225);(20,225);(39.38,225);(39.38,225)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(20,225);(20,225);(20,244.99);(20,244.99)"
%	 stroke-width= "0.75"
%	 />
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(25,230)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\iiftag$
%</text>
%<multicurve fill-style= "none"
%	 points= "(75,235);(75,235);(75,210);(75,210)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(60,235);(60,235);(60,210);(60,210)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(105,255);(105,255);(150,255);(150,255)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(150,235);(150,235);(150,254.99);(150,254.99)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(140,265);(140,265);(140,254.99);(140,254.99)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(115,245);(115,245);(115,235);(115,235)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(105,255);(105,255);(125,235);(125,235)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(115,235);(115,235);(125,225);(125,225)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(125,225);(125,225);(155,225);(155,225)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(160,210);(160,210);(160,220);(160,220)"
%	 stroke-width= "0.75"
%	 />
%<multicurve stroke-overstrike= "true"
%	 fill-style= "none"
%	 points= "(130,235);(130,235);(130,210);(130,210)"
%	 stroke-width= "0.75"
%	 stroke-overstrike-width= "2"
%	 />
%<multicurve stroke-overstrike= "true"
%	 fill-style= "none"
%	 points= "(145,235);(145,235);(145,210);(145,210)"
%	 stroke-width= "0.75"
%	 stroke-overstrike-width= "2"
%	 />
%<multicurve fill-style= "none"
%	 points= "(125.62,235);(125.62,235);(150,235);(150,235)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(155,225);(155,225);(160,220);(160,220)"
%	 stroke-width= "0.75"
%	 />
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(135,245)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\iiftagg$
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(95,245)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\EQLS$
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(315,245)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\EQLS$
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(245,275)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\where
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(355,245)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\stag$
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(55,245)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\uevaltag$
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(160,215)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\bee$
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(130,215)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\eex$
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(145,215)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\why$
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(75,215)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\bee$
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(45,215)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\eex$
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(60,215)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\why$
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(270,215)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\eex$
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(290,215)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\why$
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(354.38,215.62)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\eex$
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(372.5,215.62)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\why$
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(315,275)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\ceqn$
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(95,275)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\deqn$
%</text>
%<multicurve fill-style= "none"
%	 points= "(325,155);(325,155);(365,155);(365,155)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(365,135);(365,135);(365,155);(365,155)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(355,165);(355,165);(355,155);(355,155)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(345.62,135);(345.62,135);(365,135);(365,135)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(355,135);(355,135);(355,120);(355,120)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(335,145);(335,145);(335,105);(335,105)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(325,155);(325,155);(345,135);(345,135)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(285,135);(285,135);(285,105);(285,105)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(265,155);(265,155);(305,155);(305,155)"
%	 stroke-width= "0.6"
%	 />
%<multicurve fill-style= "none"
%	 points= "(305,135);(305,135);(305,155);(305,155)"
%	 stroke-width= "0.6"
%	 />
%<multicurve fill-style= "none"
%	 points= "(265,135);(265,135);(305,135);(305,135)"
%	 stroke-width= "0.6"
%	 />
%<multicurve fill-style= "none"
%	 points= "(265,155);(265,155);(265,135);(265,135)"
%	 stroke-width= "0.6"
%	 />
%<multicurve fill-style= "none"
%	 points= "(285,165);(285,165);(285,155);(285,155)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(345,130);(345,130);(365,110);(365,110)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(345,110);(345,110);(364.38,110);(364.38,110)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(345,110);(345,110);(345,129.99);(345,129.99)"
%	 stroke-width= "0.75"
%	 />
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(315,145)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\EQLS$
%</text>
%<multicurve fill-style= "none"
%	 points= "(325,50);(325,50);(365,50);(365,50)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(365,30);(365,30);(365,50);(365,50)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(355,60);(355,60);(355,50);(355,50)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(345.62,30);(345.62,30);(365,30);(365,30)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(355,30);(355,30);(355,15);(355,15)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(335,40);(335,40);(335,0);(335,0)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(325,50);(325,50);(345,30);(345,30)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(285,30);(285,30);(285,0);(285,0)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(265,50);(265,50);(305,50);(305,50)"
%	 stroke-width= "0.6"
%	 />
%<multicurve fill-style= "none"
%	 points= "(305,30);(305,30);(305,50);(305,50)"
%	 stroke-width= "0.6"
%	 />
%<multicurve fill-style= "none"
%	 points= "(265,30);(265,30);(305,30);(305,30)"
%	 stroke-width= "0.6"
%	 />
%<multicurve fill-style= "none"
%	 points= "(265,50);(265,50);(265,30);(265,30)"
%	 stroke-width= "0.6"
%	 />
%<multicurve fill-style= "none"
%	 points= "(285,60);(285,60);(285,50);(285,50)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(345,25);(345,25);(365,5);(365,5)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(345,5);(345,5);(364.38,5);(364.38,5)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(345,5);(345,5);(345,24.99);(345,24.99)"
%	 stroke-width= "0.75"
%	 />
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(315,40)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\EQLS$
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(285,145)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\fsttag$
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(285,40)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\sndtag$
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(350,115)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\toptag$
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(350,10)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\bottag$
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(350,145)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\utag$
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(350,40)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\utag$
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(315,175)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\oneqn$
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(315,70)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\twoeqn$
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(225,70)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\andalso
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(225,175)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\moreover
%</text>
%</jpic>
%%End JPIC-XML
%PSTricks content-type (pstricks.sty package needed)
%Add \usepackage{pstricks} in the preamble of your LaTeX file
%You can rescale the whole picture (to 80% for instance) by using the command \def\JPicScale{0.8}
\ifx\JPicScale\undefined\def\JPicScale{1}\fi
\psset{unit=\JPicScale mm}
\psset{linewidth=0.3,dotsep=1,hatchwidth=0.3,hatchsep=1.5,shadowsize=1,dimen=middle}
\psset{dotsize=0.7 2.5,dotscale=1 1,fillcolor=black}
\psset{arrowsize=1 2,arrowlength=1,arrowinset=0.25,tbarsize=0.7 5,bracketlength=0.15,rbracketlength=0.15}
\begin{pspicture}(0,0)(380,275)
\psline[linewidth=0.75](330,255)(360,255)
\psline[linewidth=0.75](380,235)(360,255)
\psline[linewidth=0.75](370,265)(370,245)
\psline[linewidth=0.75](350.62,235)(380,235)
\psline[linewidth=0.75](355,235)(355,210)
\psline[linewidth=0.75](340,245)(340,235)
\psline[linewidth=0.75](330,255)(350,235)
\psline[linewidth=0.75](290,235)(290,210)
\psline[linewidth=0.75](270,235)(270,210)
\psline[linewidth=0.6](260,255)(300,255)
\psline[linewidth=0.6](300,235)(300,255)
\psline[linewidth=0.6](260,235)(300,235)
\psline[linewidth=0.6](260,255)(260,235)
\psline[linewidth=0.75](280,265)(280,255)
\rput(280,245){$\pairtag$}
\psline[linewidth=0.75](330,245)(350,225)
\psline[linewidth=0.75](330,225)(349.38,225)
\psline[linewidth=0.75](330,225)(330,244.99)
\rput(335,230){$\iiftag$}
\psline[linewidth=0.75](373.75,235)(373.75,210)
\psline[linewidth=0.75](20,255)(80,255)
\psline[linewidth=0.75](80,235.01)(80,255)
\psline[linewidth=0.75](60,265)(60,254.99)
\psline[linewidth=0.75](40.62,235)(80,235)
\psline[linewidth=0.75](45,235)(45,210)
\psline[linewidth=0.75](30,245)(30,235)
\psline[linewidth=0.75](20,255)(40,235)
\psline[linewidth=0.75](20,245)(40,225)
\psline[linewidth=0.75](20,225)(39.38,225)
\psline[linewidth=0.75](20,225)(20,244.99)
\rput(25,230){$\iiftag$}
\psline[linewidth=0.75](75,235)(75,210)
\psline[linewidth=0.75](60,235)(60,210)
\psline[linewidth=0.75](105,255)(150,255)
\psline[linewidth=0.75](150,235)(150,254.99)
\psline[linewidth=0.75](140,265)(140,254.99)
\psline[linewidth=0.75](115,245)(115,235)
\psline[linewidth=0.75](105,255)(125,235)
\psline[linewidth=0.75](115,235)(125,225)
\psline[linewidth=0.75](125,225)(155,225)
\psline[linewidth=0.75](160,210)(160,220)
\psline[linewidth=0.75,border=2](130,235)(130,210)
\psline[linewidth=0.75,border=2](145,235)(145,210)
\psline[linewidth=0.75](125.62,235)(150,235)
\psline[linewidth=0.75](155,225)(160,220)
\rput(135,245){$\iiftagg$}
\rput(95,245){$\EQLS$}
\rput(315,245){$\EQLS$}
\rput(245,275){\where}
\rput(355,245){$\stag$}
\rput(55,245){$\uevaltag$}
\rput[r](160,215){$\bee$}
\rput[r](130,215){$\eex$}
\rput[r](145,215){$\why$}
\rput[r](75,215){$\bee$}
\rput[r](45,215){$\eex$}
\rput[r](60,215){$\why$}
\rput[r](270,215){$\eex$}
\rput[r](290,215){$\why$}
\rput[r](354.38,215.62){$\eex$}
\rput[r](372.5,215.62){$\why$}
\rput(315,275){$\ceqn$}
\rput(95,275){$\deqn$}
\psline[linewidth=0.75](325,155)(365,155)
\psline[linewidth=0.75](365,135)(365,155)
\psline[linewidth=0.75](355,165)(355,155)
\psline[linewidth=0.75](345.62,135)(365,135)
\psline[linewidth=0.75](355,135)(355,120)
\psline[linewidth=0.75](335,145)(335,105)
\psline[linewidth=0.75](325,155)(345,135)
\psline[linewidth=0.75](285,135)(285,105)
\psline[linewidth=0.6](265,155)(305,155)
\psline[linewidth=0.6](305,135)(305,155)
\psline[linewidth=0.6](265,135)(305,135)
\psline[linewidth=0.6](265,155)(265,135)
\psline[linewidth=0.75](285,165)(285,155)
\psline[linewidth=0.75](345,130)(365,110)
\psline[linewidth=0.75](345,110)(364.38,110)
\psline[linewidth=0.75](345,110)(345,129.99)
\rput(315,145){$\EQLS$}
\psline[linewidth=0.75](325,50)(365,50)
\psline[linewidth=0.75](365,30)(365,50)
\psline[linewidth=0.75](355,60)(355,50)
\psline[linewidth=0.75](345.62,30)(365,30)
\psline[linewidth=0.75](355,30)(355,15)
\psline[linewidth=0.75](335,40)(335,0)
\psline[linewidth=0.75](325,50)(345,30)
\psline[linewidth=0.75](285,30)(285,0)
\psline[linewidth=0.6](265,50)(305,50)
\psline[linewidth=0.6](305,30)(305,50)
\psline[linewidth=0.6](265,30)(305,30)
\psline[linewidth=0.6](265,50)(265,30)
\psline[linewidth=0.75](285,60)(285,50)
\psline[linewidth=0.75](345,25)(365,5)
\psline[linewidth=0.75](345,5)(364.38,5)
\psline[linewidth=0.75](345,5)(345,24.99)
\rput(315,40){$\EQLS$}
\rput(285,145){$\fsttag$}
\rput(285,40){$\sndtag$}
\rput(350,115){$\toptag$}
\rput(350,10){$\bottag$}
\rput(350,145){$\utag$}
\rput(350,40){$\utag$}
\rput(315,175){$\oneqn$}
\rput(315,70){$\twoeqn$}
\rput(225,70){\andalso}
\rput(225,175){\moreover}
\end{pspicture}


==> PIC/pair-proj.tex <==
%%Created by jPicEdt 1.4.1_03: mixed JPIC-XML/LaTeX format
%%Sat Dec 22 17:07:55 GMT-10:00 2018
%%Begin JPIC-XML
%<?xml version="1.0" standalone="yes"?>
%<jpic x-min="0" x-max="415" y-min="0" y-max="160" auto-bounding="true">
%<multicurve fill-style= "none"
%	 points= "(310,140);(310,140);(340,140);(340,140)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(360,120);(360,120);(340,140);(340,140)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(350,150);(350,150);(350,130);(350,130)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(330.62,120);(330.62,120);(360,120);(360,120)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(335,120);(335,120);(335,95);(335,95)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(320,130);(320,130);(320,120);(320,120)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(310,140);(310,140);(330,120);(330,120)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(270,120);(270,120);(270,95);(270,95)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(250,120);(250,120);(250,95);(250,95)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(240,140);(240,140);(280,140);(280,140)"
%	 stroke-width= "0.6"
%	 />
%<multicurve fill-style= "none"
%	 points= "(280,120);(280,120);(280,140);(280,140)"
%	 stroke-width= "0.6"
%	 />
%<multicurve fill-style= "none"
%	 points= "(240,120);(240,120);(280,120);(280,120)"
%	 stroke-width= "0.6"
%	 />
%<multicurve fill-style= "none"
%	 points= "(240,140);(240,140);(240,120);(240,120)"
%	 stroke-width= "0.6"
%	 />
%<multicurve fill-style= "none"
%	 points= "(260,150);(260,150);(260,140);(260,140)"
%	 stroke-width= "0.75"
%	 />
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(260,130)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\pairtag$
%</text>
%<multicurve fill-style= "none"
%	 points= "(310,130);(310,130);(330,110);(330,110)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(310,110);(310,110);(329.38,110);(329.38,110)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(310,110);(310,110);(310,129.99);(310,129.99)"
%	 stroke-width= "0.75"
%	 />
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(315,115)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\iiftag$
%</text>
%<multicurve fill-style= "none"
%	 points= "(353.75,120);(353.75,120);(353.75,95);(353.75,95)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(0,140);(0,140);(60,140);(60,140)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(60,120.01);(60,120.01);(60,140);(60,140)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(40,150);(40,150);(40,139.99);(40,139.99)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(20.62,120);(20.62,120);(60,120);(60,120)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(25,120);(25,120);(25,95);(25,95)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(10,130);(10,130);(10,120);(10,120)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(0,140);(0,140);(20,120);(20,120)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(0,130);(0,130);(20,110);(20,110)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(0,110);(0,110);(19.38,110);(19.38,110)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(0,110);(0,110);(0,129.99);(0,129.99)"
%	 stroke-width= "0.75"
%	 />
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(5,115)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\iiftag$
%</text>
%<multicurve fill-style= "none"
%	 points= "(55,120);(55,120);(55,95);(55,95)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(40,120);(40,120);(40,95);(40,95)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(85,140);(85,140);(130,140);(130,140)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(130,120);(130,120);(130,139.99);(130,139.99)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(120,150);(120,150);(120,139.99);(120,139.99)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(95,130);(95,130);(95,120);(95,120)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(85,140);(85,140);(105,120);(105,120)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(95,120);(95,120);(105,110);(105,110)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(105,110);(105,110);(135,110);(135,110)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(140,95);(140,95);(140,105);(140,105)"
%	 stroke-width= "0.75"
%	 />
%<multicurve stroke-overstrike= "true"
%	 fill-style= "none"
%	 points= "(110,120);(110,120);(110,95);(110,95)"
%	 stroke-width= "0.75"
%	 stroke-overstrike-width= "2"
%	 />
%<multicurve stroke-overstrike= "true"
%	 fill-style= "none"
%	 points= "(125,120);(125,120);(125,95);(125,95)"
%	 stroke-width= "0.75"
%	 stroke-overstrike-width= "2"
%	 />
%<multicurve fill-style= "none"
%	 points= "(105.62,120);(105.62,120);(130,120);(130,120)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(135,110);(135,110);(140,105);(140,105)"
%	 stroke-width= "0.75"
%	 />
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(115,130)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\iiftagg$
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(75,130)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\EQLS$
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(295,130)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\EQLS$
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(225,160)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\where
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(335,130)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\stag$
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(35,130)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\uevaltag$
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(140,100)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\bee$
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(110,100)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\eex$
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(125,100)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\why$
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(55,100)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\bee$
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(25,100)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\eex$
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(40,100)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\why$
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(250,100)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\eex$
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(270,100)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\why$
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(334.38,100.62)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\eex$
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(352.5,100.62)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\why$
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(295,160)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\ceqn$
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(75,160)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\deqn$
%</text>
%<multicurve fill-style= "none"
%	 points= "(235,50);(235,50);(275,50);(275,50)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(275,30);(275,30);(275,50);(275,50)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(265,60);(265,60);(265,50);(265,50)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(255.62,30);(255.62,30);(275,30);(275,30)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(265,30);(265,30);(265,15);(265,15)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(245,40);(245,40);(245,0);(245,0)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(235,50);(235,50);(255,30);(255,30)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(195,30);(195,30);(195,0);(195,0)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(175,50);(175,50);(215,50);(215,50)"
%	 stroke-width= "0.6"
%	 />
%<multicurve fill-style= "none"
%	 points= "(215,30);(215,30);(215,50);(215,50)"
%	 stroke-width= "0.6"
%	 />
%<multicurve fill-style= "none"
%	 points= "(175,30);(175,30);(215,30);(215,30)"
%	 stroke-width= "0.6"
%	 />
%<multicurve fill-style= "none"
%	 points= "(175,50);(175,50);(175,30);(175,30)"
%	 stroke-width= "0.6"
%	 />
%<multicurve fill-style= "none"
%	 points= "(195,60);(195,60);(195,50);(195,50)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(255,25);(255,25);(275,5);(275,5)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(255,5);(255,5);(274.38,5);(274.38,5)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(255,5);(255,5);(255,24.99);(255,24.99)"
%	 stroke-width= "0.75"
%	 />
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(225,40)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\EQLS$
%</text>
%<multicurve fill-style= "none"
%	 points= "(375,50);(375,50);(415,50);(415,50)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(415,30);(415,30);(415,50);(415,50)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(405,60);(405,60);(405,50);(405,50)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(395.62,30);(395.62,30);(415,30);(415,30)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(405,30);(405,30);(405,15);(405,15)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(385,40);(385,40);(385,0);(385,0)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(375,50);(375,50);(395,30);(395,30)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(335,30);(335,30);(335,0);(335,0)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(315,50);(315,50);(355,50);(355,50)"
%	 stroke-width= "0.6"
%	 />
%<multicurve fill-style= "none"
%	 points= "(355,30);(355,30);(355,50);(355,50)"
%	 stroke-width= "0.6"
%	 />
%<multicurve fill-style= "none"
%	 points= "(315,30);(315,30);(355,30);(355,30)"
%	 stroke-width= "0.6"
%	 />
%<multicurve fill-style= "none"
%	 points= "(315,50);(315,50);(315,30);(315,30)"
%	 stroke-width= "0.6"
%	 />
%<multicurve fill-style= "none"
%	 points= "(335,60);(335,60);(335,50);(335,50)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(395,25);(395,25);(415,5);(415,5)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(395,5);(395,5);(414.38,5);(414.38,5)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(395,5);(395,5);(395,24.99);(395,24.99)"
%	 stroke-width= "0.75"
%	 />
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(365,40)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\EQLS$
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(195,40)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\fsttag$
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(335,40)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\sndtag$
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(260,10)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\toptag$
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(400,10)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\bottag$
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(260,40)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\utag$
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(400,40)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\utag$
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(225,70)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\oneqn$
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(365,70)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\twoeqn$
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(295,70)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\andalso
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(135,70)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\moreover
%</text>
%</jpic>
%%End JPIC-XML
%PSTricks content-type (pstricks.sty package needed)
%Add \usepackage{pstricks} in the preamble of your LaTeX file
%You can rescale the whole picture (to 80% for instance) by using the command \def\JPicScale{0.8}
\ifx\JPicScale\undefined\def\JPicScale{1}\fi
\psset{unit=\JPicScale mm}
\psset{linewidth=0.3,dotsep=1,hatchwidth=0.3,hatchsep=1.5,shadowsize=1,dimen=middle}
\psset{dotsize=0.7 2.5,dotscale=1 1,fillcolor=black}
\psset{arrowsize=1 2,arrowlength=1,arrowinset=0.25,tbarsize=0.7 5,bracketlength=0.15,rbracketlength=0.15}
\begin{pspicture}(0,0)(415,160)
\psline[linewidth=0.75](310,140)(340,140)
\psline[linewidth=0.75](360,120)(340,140)
\psline[linewidth=0.75](350,150)(350,130)
\psline[linewidth=0.75](330.62,120)(360,120)
\psline[linewidth=0.75](335,120)(335,95)
\psline[linewidth=0.75](320,130)(320,120)
\psline[linewidth=0.75](310,140)(330,120)
\psline[linewidth=0.75](270,120)(270,95)
\psline[linewidth=0.75](250,120)(250,95)
\psline[linewidth=0.6](240,140)(280,140)
\psline[linewidth=0.6](280,120)(280,140)
\psline[linewidth=0.6](240,120)(280,120)
\psline[linewidth=0.6](240,140)(240,120)
\psline[linewidth=0.75](260,150)(260,140)
\rput(260,130){$\pairtag$}
\psline[linewidth=0.75](310,130)(330,110)
\psline[linewidth=0.75](310,110)(329.38,110)
\psline[linewidth=0.75](310,110)(310,129.99)
\rput(315,115){$\iiftag$}
\psline[linewidth=0.75](353.75,120)(353.75,95)
\psline[linewidth=0.75](0,140)(60,140)
\psline[linewidth=0.75](60,120.01)(60,140)
\psline[linewidth=0.75](40,150)(40,139.99)
\psline[linewidth=0.75](20.62,120)(60,120)
\psline[linewidth=0.75](25,120)(25,95)
\psline[linewidth=0.75](10,130)(10,120)
\psline[linewidth=0.75](0,140)(20,120)
\psline[linewidth=0.75](0,130)(20,110)
\psline[linewidth=0.75](0,110)(19.38,110)
\psline[linewidth=0.75](0,110)(0,129.99)
\rput(5,115){$\iiftag$}
\psline[linewidth=0.75](55,120)(55,95)
\psline[linewidth=0.75](40,120)(40,95)
\psline[linewidth=0.75](85,140)(130,140)
\psline[linewidth=0.75](130,120)(130,139.99)
\psline[linewidth=0.75](120,150)(120,139.99)
\psline[linewidth=0.75](95,130)(95,120)
\psline[linewidth=0.75](85,140)(105,120)
\psline[linewidth=0.75](95,120)(105,110)
\psline[linewidth=0.75](105,110)(135,110)
\psline[linewidth=0.75](140,95)(140,105)
\psline[linewidth=0.75,border=2](110,120)(110,95)
\psline[linewidth=0.75,border=2](125,120)(125,95)
\psline[linewidth=0.75](105.62,120)(130,120)
\psline[linewidth=0.75](135,110)(140,105)
\rput(115,130){$\iiftagg$}
\rput(75,130){$\EQLS$}
\rput(295,130){$\EQLS$}
\rput(225,160){\where}
\rput(335,130){$\stag$}
\rput(35,130){$\uevaltag$}
\rput[r](140,100){$\bee$}
\rput[r](110,100){$\eex$}
\rput[r](125,100){$\why$}
\rput[r](55,100){$\bee$}
\rput[r](25,100){$\eex$}
\rput[r](40,100){$\why$}
\rput[r](250,100){$\eex$}
\rput[r](270,100){$\why$}
\rput[r](334.38,100.62){$\eex$}
\rput[r](352.5,100.62){$\why$}
\rput(295,160){$\ceqn$}
\rput(75,160){$\deqn$}
\psline[linewidth=0.75](235,50)(275,50)
\psline[linewidth=0.75](275,30)(275,50)
\psline[linewidth=0.75](265,60)(265,50)
\psline[linewidth=0.75](255.62,30)(275,30)
\psline[linewidth=0.75](265,30)(265,15)
\psline[linewidth=0.75](245,40)(245,0)
\psline[linewidth=0.75](235,50)(255,30)
\psline[linewidth=0.75](195,30)(195,0)
\psline[linewidth=0.6](175,50)(215,50)
\psline[linewidth=0.6](215,30)(215,50)
\psline[linewidth=0.6](175,30)(215,30)
\psline[linewidth=0.6](175,50)(175,30)
\psline[linewidth=0.75](195,60)(195,50)
\psline[linewidth=0.75](255,25)(275,5)
\psline[linewidth=0.75](255,5)(274.38,5)
\psline[linewidth=0.75](255,5)(255,24.99)
\rput(225,40){$\EQLS$}
\psline[linewidth=0.75](375,50)(415,50)
\psline[linewidth=0.75](415,30)(415,50)
\psline[linewidth=0.75](405,60)(405,50)
\psline[linewidth=0.75](395.62,30)(415,30)
\psline[linewidth=0.75](405,30)(405,15)
\psline[linewidth=0.75](385,40)(385,0)
\psline[linewidth=0.75](375,50)(395,30)
\psline[linewidth=0.75](335,30)(335,0)
\psline[linewidth=0.6](315,50)(355,50)
\psline[linewidth=0.6](355,30)(355,50)
\psline[linewidth=0.6](315,30)(355,30)
\psline[linewidth=0.6](315,50)(315,30)
\psline[linewidth=0.75](335,60)(335,50)
\psline[linewidth=0.75](395,25)(415,5)
\psline[linewidth=0.75](395,5)(414.38,5)
\psline[linewidth=0.75](395,5)(395,24.99)
\rput(365,40){$\EQLS$}
\rput(195,40){$\fsttag$}
\rput(335,40){$\sndtag$}
\rput(260,10){$\toptag$}
\rput(400,10){$\bottag$}
\rput(260,40){$\utag$}
\rput(400,40){$\utag$}
\rput(225,70){$\oneqn$}
\rput(365,70){$\twoeqn$}
\rput(295,70){\andalso}
\rput(135,70){\moreover}
\end{pspicture}


==> PIC/pairing.tex <==
%%Created by jPicEdt 1.4.1_03: mixed JPIC-XML/LaTeX format
%%Sat Sep 24 20:35:12 CDT 2016
%%Begin JPIC-XML
%<?xml version="1.0" standalone="yes"?>
%<jpic x-min="0" x-max="155" y-min="0.62" y-max="110.62" auto-bounding="true">
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(10,25);(10,25);(10,9.38);(10,9.38)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(50,25);(50,25);(50,9.38);(50,9.38)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(20,45);(20,45);(40,45);(40,45)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(60,25);(60,25);(0,25);(0,25)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(20,65);(20,65);(0,85);(0,85)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(40,45);(40,45);(60,25);(60,25)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(0,85);(0,85);(60,85);(60,85)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(30,65);(30,65);(30,45);(30,45)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(20,65);(20,65);(40,65);(40,65)"
%	 />
%<text stroke-width= "0.75"
%	 text-vert-align= "center-v"
%	 anchor-point= "(85.62,54.38)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\EQLS
%</text>
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(60,85);(60,85);(40,65);(40,65)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(20,45);(20,45);(0,25);(0,25)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(10,103.75);(10,103.75);(10,85);(10,85)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(50,103.75);(50,103.75);(50,85);(50,85)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(115,106.25);(115,106.25);(115,9.38);(115,9.38)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(155,106.25);(155,106.25);(155,9.38);(155,9.38)"
%	 />
%<text stroke-width= "0.75"
%	 text-vert-align= "center-v"
%	 anchor-point= "(10.62,110.62)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\Progtype$
%</text>
%<text stroke-width= "0.75"
%	 text-vert-align= "center-v"
%	 anchor-point= "(50,110)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\Progtype$
%</text>
%<text stroke-width= "0.75"
%	 text-vert-align= "center-v"
%	 anchor-point= "(115,0.62)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\Progtype$
%</text>
%<text stroke-width= "0.75"
%	 text-vert-align= "center-v"
%	 anchor-point= "(10,0.62)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\Progtype$
%</text>
%<text stroke-width= "0.75"
%	 text-vert-align= "center-v"
%	 anchor-point= "(155,1.25)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\Progtype$
%</text>
%<text stroke-width= "0.75"
%	 text-vert-align= "center-v"
%	 anchor-point= "(26.25,54.38)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\Progtype$
%</text>
%<text stroke-width= "0.75"
%	 text-vert-align= "center-v"
%	 anchor-point= "(50.62,0.62)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\Progtype$
%</text>
%<text stroke-width= "0.75"
%	 text-vert-align= "center-v"
%	 anchor-point= "(30,35)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\pairing$
%</text>
%<text stroke-width= "0.75"
%	 text-vert-align= "center-v"
%	 anchor-point= "(30,75)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\projections$
%</text>
%</jpic>
%%End JPIC-XML
%PSTricks content-type (pstricks.sty package needed)
%Add \usepackage{pstricks} in the preamble of your LaTeX file
%You can rescale the whole picture (to 80% for instance) by using the command \def\JPicScale{0.8}
\ifx\JPicScale\undefined\def\JPicScale{1}\fi
\psset{unit=\JPicScale mm}
\psset{linewidth=0.3,dotsep=1,hatchwidth=0.3,hatchsep=1.5,shadowsize=1,dimen=middle}
\psset{dotsize=0.7 2.5,dotscale=1 1,fillcolor=black}
\psset{arrowsize=1 2,arrowlength=1,arrowinset=0.25,tbarsize=0.7 5,bracketlength=0.15,rbracketlength=0.15}
\begin{pspicture}(0,0)(155,110.62)
\psline[linewidth=0.75](10,25)(10,9.38)
\psline[linewidth=0.75](50,25)(50,9.38)
\psline[linewidth=0.75](20,45)(40,45)
\psline[linewidth=0.75](60,25)(0,25)
\psline[linewidth=0.75](20,65)(0,85)
\psline[linewidth=0.75](40,45)(60,25)
\psline[linewidth=0.75](0,85)(60,85)
\psline[linewidth=0.75](30,65)(30,45)
\psline[linewidth=0.75](20,65)(40,65)
\rput(85.62,54.38){\EQLS}
\psline[linewidth=0.75](60,85)(40,65)
\psline[linewidth=0.75](20,45)(0,25)
\psline[linewidth=0.75](10,103.75)(10,85)
\psline[linewidth=0.75](50,103.75)(50,85)
\psline[linewidth=0.75](115,106.25)(115,9.38)
\psline[linewidth=0.75](155,106.25)(155,9.38)
\rput(10.62,110.62){$\Progtype$}
\rput(50,110){$\Progtype$}
\rput(115,0.62){$\Progtype$}
\rput(10,0.62){$\Progtype$}
\rput(155,1.25){$\Progtype$}
\rput[r](26.25,54.38){$\Progtype$}
\rput(50.62,0.62){$\Progtype$}
\rput(30,35){$\pairing$}
\rput(30,75){$\projections$}
\end{pspicture}


==> PIC/part.tex <==
%%Created by jPicEdt 1.4.1_03: mixed JPIC-XML/LaTeX format
%%Wed Sep 28 19:30:03 HST 2016
%%Begin JPIC-XML
%<?xml version="1.0" standalone="yes"?>
%<jpic x-min="-9.38" x-max="159.38" y-min="2.5" y-max="118.12" auto-bounding="true">
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(20.62,43.12);(20.62,43.12);(20.62,10);(20.62,10)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(42.5,43.12);(42.5,43.12);(42.5,10);(42.5,10)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(10.62,43.12);(10.62,43.12);(-9.38,63.12);(-9.38,63.12)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(-9.38,63.12);(-9.38,63.12);(50,63.12);(50,63.12)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(10.62,43.12);(10.62,43.12);(50,43.12);(50,43.12)"
%	 />
%<text stroke-width= "0.75"
%	 text-vert-align= "center-v"
%	 anchor-point= "(75,32.5)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\EQLS
%</text>
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(50,63.12);(50,63.12);(50,43.12);(50,43.12)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(31.88,81.88);(31.88,81.88);(31.88,63.12);(31.88,63.12)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(0,53.12);(0,53.12);(0,10);(0,10)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(107.5,35.62);(107.5,35.62);(107.5,10.01);(107.5,10.01)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(128.12,25.62);(128.12,25.62);(128.12,10.01);(128.12,10.01)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(97.5,45.62);(97.5,45.62);(118.75,45.62);(118.75,45.62)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(138.75,25.62);(138.75,25.62);(117.5,25.62);(117.5,25.62)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(139.38,42.5);(139.38,42.5);(119.38,62.5);(119.38,62.5)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(118.75,45.62);(118.75,45.62);(138.75,25.62);(138.75,25.62)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(119.38,62.5);(119.38,62.5);(159.38,62.5);(159.38,62.5)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(127.5,54.38);(127.5,54.38);(127.5,37.5);(127.5,37.5)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(139.38,42.5);(139.38,42.5);(159.38,42.5);(159.38,42.5)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(159.38,62.5);(159.38,62.5);(159.38,42.5);(159.38,42.5)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(97.5,45.62);(97.5,45.62);(117.5,25.62);(117.5,25.62)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(149.38,81.24);(149.38,81.24);(149.38,62.5);(149.38,62.5)"
%	 />
%<text stroke-width= "0.75"
%	 text-vert-align= "center-v"
%	 anchor-point= "(125.62,50)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\Progtype$
%</text>
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(150,42.5);(150,42.5);(150,10);(150,10)"
%	 />
%<text text-vert-align= "center-v"
%	 anchor-point= "(118.12,35.62)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\partial$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(146.88,52.5)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\universal$
%</text>
%<multicurve arrow-head-width-minimum= "1.5"
%	 stroke-width= "1.2"
%	 left-arrow= "head"
%	 right-arrow= "head"
%	 arrow-head-length-scale= "1.6"
%	 fill-style= "none"
%	 points= "(85,118.12);(85,118.12);(58.75,118.12);(58.75,118.12)"
%	 />
%<text stroke-width= "0.8"
%	 left-arrow= "head"
%	 text-vert-align= "center-v"
%	 right-arrow= "head"
%	 anchor-point= "(23.12,118.12)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\computations
%</text>
%<text stroke-width= "0.8"
%	 left-arrow= "head"
%	 text-vert-align= "center-v"
%	 right-arrow= "head"
%	 anchor-point= "(130.62,118.12)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\data
%</text>
%<text stroke-width= "0.8"
%	 text-vert-align= "center-v"
%	 anchor-point= "(20.62,2.5)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\Progk$
%</text>
%<text stroke-width= "0.8"
%	 text-vert-align= "center-v"
%	 anchor-point= "(41.88,2.5)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\Progm$
%</text>
%<text stroke-width= "0.8"
%	 text-vert-align= "center-v"
%	 anchor-point= "(31.88,88.12)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\Progn$
%</text>
%<text stroke-width= "0.8"
%	 text-vert-align= "center-v"
%	 anchor-point= "(149.38,87.5)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\Progn$
%</text>
%<text stroke-width= "0.8"
%	 text-vert-align= "center-v"
%	 anchor-point= "(149.38,2.5)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\Progm$
%</text>
%<text stroke-width= "0.8"
%	 text-vert-align= "center-v"
%	 anchor-point= "(128.12,2.5)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\Progk$
%</text>
%<text stroke-width= "0.8"
%	 text-vert-align= "center-v"
%	 anchor-point= "(25.62,53.12)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\universalmkn$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(0,2.5)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\Progg$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(107.5,2.5)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\Progg$
%</text>
%</jpic>
%%End JPIC-XML
%PSTricks content-type (pstricks.sty package needed)
%Add \usepackage{pstricks} in the preamble of your LaTeX file
%You can rescale the whole picture (to 80% for instance) by using the command \def\JPicScale{0.8}
\ifx\JPicScale\undefined\def\JPicScale{1}\fi
\psset{unit=\JPicScale mm}
\psset{linewidth=0.3,dotsep=1,hatchwidth=0.3,hatchsep=1.5,shadowsize=1,dimen=middle}
\psset{dotsize=0.7 2.5,dotscale=1 1,fillcolor=black}
\psset{arrowsize=1 2,arrowlength=1,arrowinset=0.25,tbarsize=0.7 5,bracketlength=0.15,rbracketlength=0.15}
\begin{pspicture}(0,0)(159.38,118.12)
\psline[linewidth=0.75](20.62,43.12)(20.62,10)
\psline[linewidth=0.75](42.5,43.12)(42.5,10)
\psline[linewidth=0.75](10.62,43.12)(-9.38,63.12)
\psline[linewidth=0.75](-9.38,63.12)(50,63.12)
\psline[linewidth=0.75](10.62,43.12)(50,43.12)
\rput(75,32.5){\EQLS}
\psline[linewidth=0.75](50,63.12)(50,43.12)
\psline[linewidth=0.75](31.88,81.88)(31.88,63.12)
\psline[linewidth=0.75](0,53.12)(0,10)
\psline[linewidth=0.75](107.5,35.62)(107.5,10.01)
\psline[linewidth=0.75](128.12,25.62)(128.12,10.01)
\psline[linewidth=0.75](97.5,45.62)(118.75,45.62)
\psline[linewidth=0.75](138.75,25.62)(117.5,25.62)
\psline[linewidth=0.75](139.38,42.5)(119.38,62.5)
\psline[linewidth=0.75](118.75,45.62)(138.75,25.62)
\psline[linewidth=0.75](119.38,62.5)(159.38,62.5)
\psline[linewidth=0.75](127.5,54.38)(127.5,37.5)
\psline[linewidth=0.75](139.38,42.5)(159.38,42.5)
\psline[linewidth=0.75](159.38,62.5)(159.38,42.5)
\psline[linewidth=0.75](97.5,45.62)(117.5,25.62)
\psline[linewidth=0.75](149.38,81.24)(149.38,62.5)
\rput[r](125.62,50){$\Progtype$}
\psline[linewidth=0.75](150,42.5)(150,10)
\rput(118.12,35.62){$\partial$}
\rput(146.88,52.5){$\universal$}
\psline[linewidth=1.2,arrowsize=1.5 2,arrowlength=1.6]{<->}(85,118.12)(58.75,118.12)
\rput(23.12,118.12){\computations}
\rput(130.62,118.12){\data}
\rput(20.62,2.5){$\Progk$}
\rput(41.88,2.5){$\Progm$}
\rput(31.88,88.12){$\Progn$}
\rput(149.38,87.5){$\Progn$}
\rput(149.38,2.5){$\Progm$}
\rput(128.12,2.5){$\Progk$}
\rput(25.62,53.12){$\universalmkn$}
\rput(0,2.5){$\Progg$}
\rput(107.5,2.5){$\Progg$}
\end{pspicture}


==> PIC/parteval.tex <==
%%Created by jPicEdt 1.4.1_03: mixed JPIC-XML/LaTeX format
%%Sun Sep 25 17:46:11 CDT 2016
%%Begin JPIC-XML
%<?xml version="1.0" standalone="yes"?>
%<jpic x-min="-14.38" x-max="154.38" y-min="0.62" y-max="110" auto-bounding="true">
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(16.88,25);(16.88,25);(16.88,9.38);(16.88,9.38)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(43.75,25);(43.75,25);(43.75,9.38);(43.75,9.38)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(20,45);(20,45);(40,45);(40,45)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(60,25);(60,25);(0,25);(0,25)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(5.62,65);(5.62,65);(-14.38,85);(-14.38,85)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(40,45);(40,45);(60,25);(60,25)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(-14.38,85);(-14.38,85);(40,85);(40,85)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(30,65);(30,65);(30,45);(30,45)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(5.62,65);(5.62,65);(40,65);(40,65)"
%	 />
%<text stroke-width= "0.75"
%	 text-vert-align= "center-v"
%	 anchor-point= "(75.62,54.38)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\EQLS
%</text>
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(40,85);(40,85);(40,65);(40,65)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(20,45);(20,45);(0,25);(0,25)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(30,103.75);(30,103.75);(30,85);(30,85)"
%	 />
%<text stroke-width= "0.75"
%	 text-vert-align= "center-v"
%	 anchor-point= "(30,110)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\Progtype$
%</text>
%<text stroke-width= "0.75"
%	 text-vert-align= "center-v"
%	 anchor-point= "(-5.62,0.62)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\Progtype$
%</text>
%<text stroke-width= "0.75"
%	 text-vert-align= "center-v"
%	 anchor-point= "(17.5,0.62)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\Progtype$
%</text>
%<text stroke-width= "0.75"
%	 text-vert-align= "center-v"
%	 anchor-point= "(26.25,54.38)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\Progtype$
%</text>
%<text stroke-width= "0.75"
%	 text-vert-align= "center-v"
%	 anchor-point= "(50.62,0.62)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\Progtype$
%</text>
%<text stroke-width= "0.75"
%	 text-vert-align= "center-v"
%	 anchor-point= "(30,35)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\pairing$
%</text>
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(-5,75);(-5,75);(-5,9.38);(-5,9.38)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(102.5,35);(102.5,35);(102.5,9.38);(102.5,9.38)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(123.12,25);(123.12,25);(123.12,9.38);(123.12,9.38)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(92.5,45);(92.5,45);(113.75,45);(113.75,45)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(133.75,25);(133.75,25);(112.5,25);(112.5,25)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(134.38,64.38);(134.38,64.38);(114.38,84.38);(114.38,84.38)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(113.75,45);(113.75,45);(133.75,25);(133.75,25)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(114.38,84.38);(114.38,84.38);(154.38,84.38);(154.38,84.38)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(122.5,76.25);(122.5,76.25);(122.5,36.25);(122.5,36.25)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(134.38,64.38);(134.38,64.38);(154.38,64.38);(154.38,64.38)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(154.38,84.38);(154.38,84.38);(154.38,64.38);(154.38,64.38)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(92.5,45);(92.5,45);(112.5,25);(112.5,25)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(144.38,103.12);(144.38,103.12);(144.38,84.38);(144.38,84.38)"
%	 />
%<text stroke-width= "0.75"
%	 text-vert-align= "center-v"
%	 anchor-point= "(144.38,1.25)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\Progtype$
%</text>
%<text stroke-width= "0.75"
%	 text-vert-align= "center-v"
%	 anchor-point= "(143.75,109.38)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\Progtype$
%</text>
%<text stroke-width= "0.75"
%	 text-vert-align= "center-v"
%	 anchor-point= "(103.75,1.25)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\Progtype$
%</text>
%<text stroke-width= "0.75"
%	 text-vert-align= "center-v"
%	 anchor-point= "(120,54.38)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\Progtype$
%</text>
%<text stroke-width= "0.75"
%	 text-vert-align= "center-v"
%	 anchor-point= "(123.75,1.25)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\Progtype$
%</text>
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(145,64.38);(145,64.38);(145,8.75);(145,8.75)"
%	 />
%<text text-vert-align= "center-v"
%	 anchor-point= "(113.12,35)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\partial$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(16.88,75)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\universal$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(141.88,74.38)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\universal$
%</text>
%</jpic>
%%End JPIC-XML
%PSTricks content-type (pstricks.sty package needed)
%Add \usepackage{pstricks} in the preamble of your LaTeX file
%You can rescale the whole picture (to 80% for instance) by using the command \def\JPicScale{0.8}
\ifx\JPicScale\undefined\def\JPicScale{1}\fi
\psset{unit=\JPicScale mm}
\psset{linewidth=0.3,dotsep=1,hatchwidth=0.3,hatchsep=1.5,shadowsize=1,dimen=middle}
\psset{dotsize=0.7 2.5,dotscale=1 1,fillcolor=black}
\psset{arrowsize=1 2,arrowlength=1,arrowinset=0.25,tbarsize=0.7 5,bracketlength=0.15,rbracketlength=0.15}
\begin{pspicture}(0,0)(154.38,110)
\psline[linewidth=0.75](16.88,25)(16.88,9.38)
\psline[linewidth=0.75](43.75,25)(43.75,9.38)
\psline[linewidth=0.75](20,45)(40,45)
\psline[linewidth=0.75](60,25)(0,25)
\psline[linewidth=0.75](5.62,65)(-14.38,85)
\psline[linewidth=0.75](40,45)(60,25)
\psline[linewidth=0.75](-14.38,85)(40,85)
\psline[linewidth=0.75](30,65)(30,45)
\psline[linewidth=0.75](5.62,65)(40,65)
\rput(75.62,54.38){\EQLS}
\psline[linewidth=0.75](40,85)(40,65)
\psline[linewidth=0.75](20,45)(0,25)
\psline[linewidth=0.75](30,103.75)(30,85)
\rput(30,110){$\Progtype$}
\rput(-5.62,0.62){$\Progtype$}
\rput(17.5,0.62){$\Progtype$}
\rput[r](26.25,54.38){$\Progtype$}
\rput(50.62,0.62){$\Progtype$}
\rput(30,35){$\pairing$}
\psline[linewidth=0.75](-5,75)(-5,9.38)
\psline[linewidth=0.75](102.5,35)(102.5,9.38)
\psline[linewidth=0.75](123.12,25)(123.12,9.38)
\psline[linewidth=0.75](92.5,45)(113.75,45)
\psline[linewidth=0.75](133.75,25)(112.5,25)
\psline[linewidth=0.75](134.38,64.38)(114.38,84.38)
\psline[linewidth=0.75](113.75,45)(133.75,25)
\psline[linewidth=0.75](114.38,84.38)(154.38,84.38)
\psline[linewidth=0.75](122.5,76.25)(122.5,36.25)
\psline[linewidth=0.75](134.38,64.38)(154.38,64.38)
\psline[linewidth=0.75](154.38,84.38)(154.38,64.38)
\psline[linewidth=0.75](92.5,45)(112.5,25)
\psline[linewidth=0.75](144.38,103.12)(144.38,84.38)
\rput(144.38,1.25){$\Progtype$}
\rput(143.75,109.38){$\Progtype$}
\rput(103.75,1.25){$\Progtype$}
\rput[r](120,54.38){$\Progtype$}
\rput(123.75,1.25){$\Progtype$}
\psline[linewidth=0.75](145,64.38)(145,8.75)
\rput(113.12,35){$\partial$}
\rput(16.88,75){$\universal$}
\rput(141.88,74.38){$\universal$}
\end{pspicture}


==> PIC/plus-times.tex <==
%%Created by jPicEdt 1.4.1_03: mixed JPIC-XML/LaTeX format
%%Fri Aug 26 00:25:05 GMT-10:00 2022
%%Begin JPIC-XML
%<?xml version="1.0" standalone="yes"?>
%<jpic x-min="0" x-max="105" y-min="-2.5" y-max="42.5" auto-bounding="true">
%<multicurve fill-style= "none"
%	 points= "(5,10);(5,10);(5,-2.5);(5,-2.5)"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(0,30);(0,30);(30,30);(30,30)"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(0,30);(0,30);(0,10);(0,10)"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(30,10);(30,10);(30,30);(30,30)"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(15,42.5);(15,42.5);(15,30);(15,30)"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(0,10);(0,10);(30,10);(30,10)"
%	 stroke-width= "0.35"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(15,20)"
%	 text-frame= "noframe"
%	 stroke-width= "0.35"
%	 text-hor-align= "center-h"
%	 >
%\gee
%</text>
%<multicurve fill-style= "none"
%	 points= "(80,10);(80,10);(80,-2.5);(80,-2.5)"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(75,30);(75,30);(75,10);(75,10)"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(105,10);(105,10);(105,30);(105,30)"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(90,42.5);(90,42.5);(90,30);(90,30)"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(75,10);(75,10);(105,10);(105,10)"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(75,30);(75,30);(105,30);(105,30)"
%	 stroke-width= "0.35"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(90,20)"
%	 text-frame= "noframe"
%	 stroke-width= "0.35"
%	 text-hor-align= "center-h"
%	 >
%\kee
%</text>
%<multicurve fill-style= "none"
%	 points= "(25,10);(25,10);(25,-2.5);(25,-2.5)"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(100,10);(100,10);(100,-2.5);(100,-2.5)"
%	 stroke-width= "0.35"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(3.75,0)"
%	 text-frame= "noframe"
%	 stroke-width= "0.35"
%	 text-hor-align= "right"
%	 >
%$\mee$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(23.75,0)"
%	 text-frame= "noframe"
%	 stroke-width= "0.35"
%	 text-hor-align= "right"
%	 >
%$\nee$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(78.75,0)"
%	 text-frame= "noframe"
%	 stroke-width= "0.35"
%	 text-hor-align= "right"
%	 >
%$\mee$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(98.75,0)"
%	 text-frame= "noframe"
%	 stroke-width= "0.35"
%	 text-hor-align= "right"
%	 >
%$\nee$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(17.5,40)"
%	 text-frame= "noframe"
%	 stroke-width= "0.35"
%	 text-hor-align= "left"
%	 >
%$\outplus$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(92.5,40)"
%	 text-frame= "noframe"
%	 stroke-width= "0.35"
%	 text-hor-align= "left"
%	 >
%$\outtimes$
%</text>
%</jpic>
%%End JPIC-XML
%LaTeX-picture environment using emulated lines and arcs
%You can rescale the whole picture (to 80% for instance) by using the command \def\JPicScale{0.8}
\ifx\JPicScale\undefined\def\JPicScale{1}\fi
\unitlength \JPicScale mm
\begin{picture}(105,42.5)(0,0)
\linethickness{0.35mm}
\put(5,-2.5){\line(0,1){12.5}}
\linethickness{0.35mm}
\put(0,30){\line(1,0){30}}
\linethickness{0.35mm}
\put(0,10){\line(0,1){20}}
\linethickness{0.35mm}
\put(30,10){\line(0,1){20}}
\linethickness{0.35mm}
\put(15,30){\line(0,1){12.5}}
\linethickness{0.35mm}
\put(0,10){\line(1,0){30}}
\put(15,20){\makebox(0,0)[cc]{\gee}}

\linethickness{0.35mm}
\put(80,-2.5){\line(0,1){12.5}}
\linethickness{0.35mm}
\put(75,10){\line(0,1){20}}
\linethickness{0.35mm}
\put(105,10){\line(0,1){20}}
\linethickness{0.35mm}
\put(90,30){\line(0,1){12.5}}
\linethickness{0.35mm}
\put(75,10){\line(1,0){30}}
\linethickness{0.35mm}
\put(75,30){\line(1,0){30}}
\put(90,20){\makebox(0,0)[cc]{\kee}}

\linethickness{0.35mm}
\put(25,-2.5){\line(0,1){12.5}}
\linethickness{0.35mm}
\put(100,-2.5){\line(0,1){12.5}}
\put(3.75,0){\makebox(0,0)[cr]{$\mee$}}

\put(23.75,0){\makebox(0,0)[cr]{$\nee$}}

\put(78.75,0){\makebox(0,0)[cr]{$\mee$}}

\put(98.75,0){\makebox(0,0)[cr]{$\nee$}}

\put(17.5,40){\makebox(0,0)[cl]{$\outplus$}}

\put(92.5,40){\makebox(0,0)[cl]{$\outtimes$}}

\end{picture}


==> PIC/plustimes-1.tex <==
%%Created by jPicEdt 1.4.1_03: mixed JPIC-XML/LaTeX format
%%Fri Aug 26 09:04:11 GMT-10:00 2022
%%Begin JPIC-XML
%<?xml version="1.0" standalone="yes"?>
%<jpic x-min="0" x-max="80" y-min="1.25" y-max="68.75" auto-bounding="true">
%<multicurve fill-style= "none"
%	 points= "(5,45);(5,45);(5,35);(5,35)"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(0,55);(0,55);(30,55);(30,55)"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(0,55);(0,55);(0,45);(0,45)"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(30,45);(30,45);(30,55);(30,55)"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(15,65);(15,65);(15,55);(15,55)"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(0,45);(0,45);(30,45);(30,45)"
%	 stroke-width= "0.35"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(15,50)"
%	 text-frame= "noframe"
%	 stroke-width= "0.35"
%	 text-hor-align= "center-h"
%	 >
%\gee
%</text>
%<multicurve fill-style= "none"
%	 points= "(55,45);(55,45);(55,35);(55,35)"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(50,55);(50,55);(50,45);(50,45)"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(80,45);(80,45);(80,55);(80,55)"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(65,65);(65,65);(65,55);(65,55)"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(50,45);(50,45);(80,45);(80,45)"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(50,55);(50,55);(80,55);(80,55)"
%	 stroke-width= "0.35"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(65,50)"
%	 text-frame= "noframe"
%	 stroke-width= "0.35"
%	 text-hor-align= "center-h"
%	 >
%\kee
%</text>
%<multicurve fill-style= "none"
%	 points= "(25,45);(25,45);(25,35);(25,35)"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(75,45);(75,45);(75,35);(75,35)"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(50,15);(50,15);(50,5);(50,5)"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(75,40);(75,40);(50,15);(50,15)"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(55,40);(55,40);(30,15);(30,15)"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(25,40);(25,40);(50,15);(50,15)"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(5,40);(5,40);(30,15);(30,15)"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(30,15);(30,15);(30,5);(30,5)"
%	 stroke-width= "0.35"
%	 />
%<text text-vert-align= "bottom"
%	 fill-style= "none"
%	 anchor-point= "(50,20)"
%	 text-frame= "noframe"
%	 stroke-width= "0.35"
%	 text-hor-align= "center-h"
%	 >
%\hee
%</text>
%<text text-vert-align= "bottom"
%	 fill-style= "none"
%	 anchor-point= "(30,20)"
%	 text-frame= "noframe"
%	 stroke-width= "0.35"
%	 text-hor-align= "center-h"
%	 >
%\hee
%</text>
%<text text-vert-align= "bottom"
%	 fill-style= "none"
%	 anchor-point= "(40,28.75)"
%	 text-frame= "noframe"
%	 stroke-width= "0.35"
%	 text-hor-align= "center-h"
%	 >
%\see
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(30,1.25)"
%	 text-frame= "noframe"
%	 stroke-width= "0.35"
%	 text-hor-align= "center-h"
%	 >
%$\mee$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(50,1.25)"
%	 text-frame= "noframe"
%	 stroke-width= "0.35"
%	 text-hor-align= "center-h"
%	 >
%$\nee$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(3.75,42.5)"
%	 text-frame= "noframe"
%	 stroke-width= "0.35"
%	 text-hor-align= "right"
%	 >
%$\mee$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(23.75,42.5)"
%	 text-frame= "noframe"
%	 stroke-width= "0.35"
%	 text-hor-align= "right"
%	 >
%$\nee$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(53.75,42.5)"
%	 text-frame= "noframe"
%	 stroke-width= "0.35"
%	 text-hor-align= "right"
%	 >
%$\mee$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(73.75,42.5)"
%	 text-frame= "noframe"
%	 stroke-width= "0.35"
%	 text-hor-align= "right"
%	 >
%$\nee$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(15,68.75)"
%	 text-frame= "noframe"
%	 stroke-width= "0.35"
%	 text-hor-align= "center-h"
%	 >
%$\outplus$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(65,68.75)"
%	 text-frame= "noframe"
%	 stroke-width= "0.35"
%	 text-hor-align= "center-h"
%	 >
%$\outtimes$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(30,15)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\Dottt
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(50,15)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\Dottt
%</text>
%</jpic>
%%End JPIC-XML
%LaTeX-picture environment using emulated lines and arcs
%You can rescale the whole picture (to 80% for instance) by using the command \def\JPicScale{0.8}
\ifx\JPicScale\undefined\def\JPicScale{1}\fi
\unitlength \JPicScale mm
\begin{picture}(80,68.75)(0,0)
\linethickness{0.35mm}
\put(5,35){\line(0,1){10}}
\linethickness{0.35mm}
\put(0,55){\line(1,0){30}}
\linethickness{0.35mm}
\put(0,45){\line(0,1){10}}
\linethickness{0.35mm}
\put(30,45){\line(0,1){10}}
\linethickness{0.35mm}
\put(15,55){\line(0,1){10}}
\linethickness{0.35mm}
\put(0,45){\line(1,0){30}}
\put(15,50){\makebox(0,0)[cc]{\gee}}

\linethickness{0.35mm}
\put(55,35){\line(0,1){10}}
\linethickness{0.35mm}
\put(50,45){\line(0,1){10}}
\linethickness{0.35mm}
\put(80,45){\line(0,1){10}}
\linethickness{0.35mm}
\put(65,55){\line(0,1){10}}
\linethickness{0.35mm}
\put(50,45){\line(1,0){30}}
\linethickness{0.35mm}
\put(50,55){\line(1,0){30}}
\put(65,50){\makebox(0,0)[cc]{\kee}}

\linethickness{0.35mm}
\put(25,35){\line(0,1){10}}
\linethickness{0.35mm}
\put(75,35){\line(0,1){10}}
\linethickness{0.35mm}
\put(50,5){\line(0,1){10}}
\linethickness{0.35mm}
\multiput(50,15)(0.12,0.12){208}{\line(1,0){0.12}}
\linethickness{0.35mm}
\multiput(30,15)(0.12,0.12){208}{\line(1,0){0.12}}
\linethickness{0.35mm}
\multiput(25,40)(0.12,-0.12){208}{\line(1,0){0.12}}
\linethickness{0.35mm}
\multiput(5,40)(0.12,-0.12){208}{\line(1,0){0.12}}
\linethickness{0.35mm}
\put(30,5){\line(0,1){10}}
\put(50,20){\makebox(0,0)[bc]{\hee}}

\put(30,20){\makebox(0,0)[bc]{\hee}}

\put(40,28.75){\makebox(0,0)[bc]{\see}}

\put(30,1.25){\makebox(0,0)[cc]{$\mee$}}

\put(50,1.25){\makebox(0,0)[cc]{$\nee$}}

\put(3.75,42.5){\makebox(0,0)[cr]{$\mee$}}

\put(23.75,42.5){\makebox(0,0)[cr]{$\nee$}}

\put(53.75,42.5){\makebox(0,0)[cr]{$\mee$}}

\put(73.75,42.5){\makebox(0,0)[cr]{$\nee$}}

\put(15,68.75){\makebox(0,0)[cc]{$\outplus$}}

\put(65,68.75){\makebox(0,0)[cc]{$\outtimes$}}

\put(30,15){\makebox(0,0)[cc]{\Dottt}}

\put(50,15){\makebox(0,0)[cc]{\Dottt}}

\end{picture}


==> PIC/plustimes-2.tex <==
%%Created by jPicEdt 1.4.1_03: mixed JPIC-XML/LaTeX format
%%Fri Aug 26 08:23:26 GMT-10:00 2022
%%Begin JPIC-XML
%<?xml version="1.0" standalone="yes"?>
%<jpic x-min="0" x-max="80" y-min="1.25" y-max="73.75" auto-bounding="true">
%<multicurve fill-style= "none"
%	 points= "(5,50);(5,50);(5,40);(5,40)"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(0,60);(0,60);(30,60);(30,60)"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(0,60);(0,60);(0,50);(0,50)"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(30,50);(30,50);(30,60);(30,60)"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(15,70);(15,70);(15,60);(15,60)"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(0,50);(0,50);(30,50);(30,50)"
%	 stroke-width= "0.35"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(15,55)"
%	 text-frame= "noframe"
%	 stroke-width= "0.35"
%	 text-hor-align= "center-h"
%	 >
%\gee
%</text>
%<multicurve fill-style= "none"
%	 points= "(55,50);(55,50);(55,40);(55,40)"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(50,60);(50,60);(50,50);(50,50)"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(80,50);(80,50);(80,60);(80,60)"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(65,70);(65,70);(65,60);(65,60)"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(50,50);(50,50);(80,50);(80,50)"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(50,60);(50,60);(80,60);(80,60)"
%	 stroke-width= "0.35"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(65,55)"
%	 text-frame= "noframe"
%	 stroke-width= "0.35"
%	 text-hor-align= "center-h"
%	 >
%\kee
%</text>
%<multicurve fill-style= "none"
%	 points= "(25,50);(25,50);(25,40);(25,40)"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(75,50);(75,50);(75,40);(75,40)"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(50,15);(50,15);(50,5);(50,5)"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(75,40);(75,40);(50,15);(50,15)"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(55,40);(55,40);(30,15);(30,15)"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(25,40);(25,40);(50,15);(50,15)"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(5,40);(5,40);(30,15);(30,15)"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(30,15);(30,15);(30,5);(30,5)"
%	 stroke-width= "0.35"
%	 />
%<text text-vert-align= "bottom"
%	 fill-style= "none"
%	 anchor-point= "(50,20)"
%	 text-frame= "noframe"
%	 stroke-width= "0.35"
%	 text-hor-align= "center-h"
%	 >
%\hee
%</text>
%<text text-vert-align= "bottom"
%	 fill-style= "none"
%	 anchor-point= "(30,20)"
%	 text-frame= "noframe"
%	 stroke-width= "0.35"
%	 text-hor-align= "center-h"
%	 >
%\hee
%</text>
%<text text-vert-align= "bottom"
%	 fill-style= "none"
%	 anchor-point= "(40,28.75)"
%	 text-frame= "noframe"
%	 stroke-width= "0.35"
%	 text-hor-align= "center-h"
%	 >
%\see
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(30,1.25)"
%	 text-frame= "noframe"
%	 stroke-width= "0.35"
%	 text-hor-align= "center-h"
%	 >
%$\mee$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(50,1.25)"
%	 text-frame= "noframe"
%	 stroke-width= "0.35"
%	 text-hor-align= "center-h"
%	 >
%$\nee$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(3.75,42.5)"
%	 text-frame= "noframe"
%	 stroke-width= "0.35"
%	 text-hor-align= "right"
%	 >
%$\mee$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(23.75,42.5)"
%	 text-frame= "noframe"
%	 stroke-width= "0.35"
%	 text-hor-align= "right"
%	 >
%$\nee$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(53.75,42.5)"
%	 text-frame= "noframe"
%	 stroke-width= "0.35"
%	 text-hor-align= "right"
%	 >
%$\mee$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(73.75,42.5)"
%	 text-frame= "noframe"
%	 stroke-width= "0.35"
%	 text-hor-align= "right"
%	 >
%$\nee$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(15,73.75)"
%	 text-frame= "noframe"
%	 stroke-width= "0.35"
%	 text-hor-align= "center-h"
%	 >
%$\outplus$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(65,73.75)"
%	 text-frame= "noframe"
%	 stroke-width= "0.35"
%	 text-hor-align= "center-h"
%	 >
%$\outtimes$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(30,15)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\Dottt
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(50,15)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\Dottt
%</text>
%</jpic>
%%End JPIC-XML
%LaTeX-picture environment using emulated lines and arcs
%You can rescale the whole picture (to 80% for instance) by using the command \def\JPicScale{0.8}
\ifx\JPicScale\undefined\def\JPicScale{1}\fi
\unitlength \JPicScale mm
\begin{picture}(80,73.75)(0,0)
\linethickness{0.35mm}
\put(5,40){\line(0,1){10}}
\linethickness{0.35mm}
\put(0,60){\line(1,0){30}}
\linethickness{0.35mm}
\put(0,50){\line(0,1){10}}
\linethickness{0.35mm}
\put(30,50){\line(0,1){10}}
\linethickness{0.35mm}
\put(15,60){\line(0,1){10}}
\linethickness{0.35mm}
\put(0,50){\line(1,0){30}}
\put(15,55){\makebox(0,0)[cc]{\gee}}

\linethickness{0.35mm}
\put(55,40){\line(0,1){10}}
\linethickness{0.35mm}
\put(50,50){\line(0,1){10}}
\linethickness{0.35mm}
\put(80,50){\line(0,1){10}}
\linethickness{0.35mm}
\put(65,60){\line(0,1){10}}
\linethickness{0.35mm}
\put(50,50){\line(1,0){30}}
\linethickness{0.35mm}
\put(50,60){\line(1,0){30}}
\put(65,55){\makebox(0,0)[cc]{\kee}}

\linethickness{0.35mm}
\put(25,40){\line(0,1){10}}
\linethickness{0.35mm}
\put(75,40){\line(0,1){10}}
\linethickness{0.35mm}
\put(50,5){\line(0,1){10}}
\linethickness{0.35mm}
\multiput(50,15)(0.12,0.12){208}{\line(1,0){0.12}}
\linethickness{0.35mm}
\multiput(30,15)(0.12,0.12){208}{\line(1,0){0.12}}
\linethickness{0.35mm}
\multiput(25,40)(0.12,-0.12){208}{\line(1,0){0.12}}
\linethickness{0.35mm}
\multiput(5,40)(0.12,-0.12){208}{\line(1,0){0.12}}
\linethickness{0.35mm}
\put(30,5){\line(0,1){10}}
\put(50,20){\makebox(0,0)[bc]{\hee}}

\put(30,20){\makebox(0,0)[bc]{\hee}}

\put(40,28.75){\makebox(0,0)[bc]{\see}}

\put(30,1.25){\makebox(0,0)[cc]{$\mee$}}

\put(50,1.25){\makebox(0,0)[cc]{$\nee$}}

\put(3.75,42.5){\makebox(0,0)[cr]{$\mee$}}

\put(23.75,42.5){\makebox(0,0)[cr]{$\nee$}}

\put(53.75,42.5){\makebox(0,0)[cr]{$\mee$}}

\put(73.75,42.5){\makebox(0,0)[cr]{$\nee$}}

\put(15,73.75){\makebox(0,0)[cc]{$\outplus$}}

\put(65,73.75){\makebox(0,0)[cc]{$\outtimes$}}

\put(30,15){\makebox(0,0)[cc]{\Dottt}}

\put(50,15){\makebox(0,0)[cc]{\Dottt}}

\end{picture}


==> PIC/plustimes-3.tex <==
%%Created by jPicEdt 1.4.1_03: mixed JPIC-XML/LaTeX format
%%Fri Aug 26 08:41:26 GMT-10:00 2022
%%Begin JPIC-XML
%<?xml version="1.0" standalone="yes"?>
%<jpic x-min="0" x-max="40" y-min="1.25" y-max="73.75" auto-bounding="true">
%<multicurve fill-style= "none"
%	 points= "(5,50);(5,50);(5,20);(5,20)"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(0,60);(0,60);(30,60);(30,60)"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(0,60);(0,60);(0,50);(0,50)"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(30,50);(30,50);(30,60);(30,60)"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(15,70);(15,70);(15,60);(15,60)"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(0,50);(0,50);(30,50);(30,50)"
%	 stroke-width= "0.35"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(25,35)"
%	 text-frame= "noframe"
%	 stroke-width= "0.35"
%	 text-hor-align= "center-h"
%	 >
%\gee
%</text>
%<multicurve fill-style= "none"
%	 points= "(15,30);(15,30);(15,20);(15,20)"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(10,40);(10,40);(10,30);(10,30)"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(40,30);(40,30);(40,40);(40,40)"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(25,50);(25,50);(25,40);(25,40)"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(10,30);(10,30);(40,30);(40,30)"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(10,40);(10,40);(40,40);(40,40)"
%	 stroke-width= "0.35"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(15,55)"
%	 text-frame= "noframe"
%	 stroke-width= "0.35"
%	 text-hor-align= "center-h"
%	 >
%\kee
%</text>
%<multicurve fill-style= "none"
%	 points= "(35,30);(35,30);(35,5);(35,5)"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(15,20);(15,20);(10,15);(10,15)"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(5,20);(5,20);(10,15);(10,15)"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(10,15);(10,15);(10,5);(10,5)"
%	 stroke-width= "0.35"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(10,1.25)"
%	 text-frame= "noframe"
%	 stroke-width= "0.35"
%	 text-hor-align= "center-h"
%	 >
%$\mee$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(35,1.25)"
%	 text-frame= "noframe"
%	 stroke-width= "0.35"
%	 text-hor-align= "center-h"
%	 >
%$\nee$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(15,73.75)"
%	 text-frame= "noframe"
%	 stroke-width= "0.35"
%	 text-hor-align= "center-h"
%	 >
%$\outplus$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(10,15)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\Dottt
%</text>
%</jpic>
%%End JPIC-XML
%LaTeX-picture environment using emulated lines and arcs
%You can rescale the whole picture (to 80% for instance) by using the command \def\JPicScale{0.8}
\ifx\JPicScale\undefined\def\JPicScale{1}\fi
\unitlength \JPicScale mm
\begin{picture}(40,73.75)(0,0)
\linethickness{0.35mm}
\put(5,20){\line(0,1){30}}
\linethickness{0.35mm}
\put(0,60){\line(1,0){30}}
\linethickness{0.35mm}
\put(0,50){\line(0,1){10}}
\linethickness{0.35mm}
\put(30,50){\line(0,1){10}}
\linethickness{0.35mm}
\put(15,60){\line(0,1){10}}
\linethickness{0.35mm}
\put(0,50){\line(1,0){30}}
\put(25,35){\makebox(0,0)[cc]{\gee}}

\linethickness{0.35mm}
\put(15,20){\line(0,1){10}}
\linethickness{0.35mm}
\put(10,30){\line(0,1){10}}
\linethickness{0.35mm}
\put(40,30){\line(0,1){10}}
\linethickness{0.35mm}
\put(25,40){\line(0,1){10}}
\linethickness{0.35mm}
\put(10,30){\line(1,0){30}}
\linethickness{0.35mm}
\put(10,40){\line(1,0){30}}
\put(15,55){\makebox(0,0)[cc]{\kee}}

\linethickness{0.35mm}
\put(35,5){\line(0,1){25}}
\linethickness{0.35mm}
\multiput(10,15)(0.12,0.12){42}{\line(1,0){0.12}}
\linethickness{0.35mm}
\multiput(5,20)(0.12,-0.12){42}{\line(1,0){0.12}}
\linethickness{0.35mm}
\put(10,5){\line(0,1){10}}
\put(10,1.25){\makebox(0,0)[cc]{$\mee$}}

\put(35,1.25){\makebox(0,0)[cc]{$\nee$}}

\put(15,73.75){\makebox(0,0)[cc]{$\outplus$}}

\put(10,15){\makebox(0,0)[cc]{\Dottt}}

\end{picture}


==> PIC/plustimes-4.tex <==
%%Created by jPicEdt 1.4.1_03: mixed JPIC-XML/LaTeX format
%%Fri Aug 26 09:06:08 GMT-10:00 2022
%%Begin JPIC-XML
%<?xml version="1.0" standalone="yes"?>
%<jpic x-min="0" x-max="40" y-min="1.25" y-max="78.75" auto-bounding="true">
%<multicurve fill-style= "none"
%	 points= "(15,55);(15,55);(15,45);(15,45)"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(10,65);(10,65);(40,65);(40,65)"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(10,65);(10,65);(10,55);(10,55)"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(40,55);(40,55);(40,65);(40,65)"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(25,75);(25,75);(25,65);(25,65)"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(10,55);(10,55);(40,55);(40,55)"
%	 stroke-width= "0.35"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(15,40)"
%	 text-frame= "noframe"
%	 stroke-width= "0.35"
%	 text-hor-align= "center-h"
%	 >
%\gee
%</text>
%<multicurve fill-style= "none"
%	 points= "(5,35);(5,35);(5,25);(5,25)"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(0,45);(0,45);(0,35);(0,35)"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(30,35);(30,35);(30,45);(30,45)"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(35,55);(35,55);(35,5);(35,5)"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(0,35);(0,35);(30,35);(30,35)"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(0,45);(0,45);(30,45);(30,45)"
%	 stroke-width= "0.35"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(25,60)"
%	 text-frame= "noframe"
%	 stroke-width= "0.35"
%	 text-hor-align= "center-h"
%	 >
%\kee
%</text>
%<multicurve fill-style= "none"
%	 points= "(25,35);(25,35);(25,25);(25,25)"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(25,25);(25,25);(15,15);(15,15)"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(5,25);(5,25);(15,15);(15,15)"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(15,15);(15,15);(15,5);(15,5)"
%	 stroke-width= "0.35"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(15,1.25)"
%	 text-frame= "noframe"
%	 stroke-width= "0.35"
%	 text-hor-align= "center-h"
%	 >
%$\mee$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(35,1.25)"
%	 text-frame= "noframe"
%	 stroke-width= "0.35"
%	 text-hor-align= "center-h"
%	 >
%$\nee$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(25,78.75)"
%	 text-frame= "noframe"
%	 stroke-width= "0.35"
%	 text-hor-align= "center-h"
%	 >
%$\outplus$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(15,15)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\Dottt
%</text>
%</jpic>
%%End JPIC-XML
%LaTeX-picture environment using emulated lines and arcs
%You can rescale the whole picture (to 80% for instance) by using the command \def\JPicScale{0.8}
\ifx\JPicScale\undefined\def\JPicScale{1}\fi
\unitlength \JPicScale mm
\begin{picture}(40,78.75)(0,0)
\linethickness{0.35mm}
\put(15,45){\line(0,1){10}}
\linethickness{0.35mm}
\put(10,65){\line(1,0){30}}
\linethickness{0.35mm}
\put(10,55){\line(0,1){10}}
\linethickness{0.35mm}
\put(40,55){\line(0,1){10}}
\linethickness{0.35mm}
\put(25,65){\line(0,1){10}}
\linethickness{0.35mm}
\put(10,55){\line(1,0){30}}
\put(15,40){\makebox(0,0)[cc]{\gee}}

\linethickness{0.35mm}
\put(5,25){\line(0,1){10}}
\linethickness{0.35mm}
\put(0,35){\line(0,1){10}}
\linethickness{0.35mm}
\put(30,35){\line(0,1){10}}
\linethickness{0.35mm}
\put(35,5){\line(0,1){50}}
\linethickness{0.35mm}
\put(0,35){\line(1,0){30}}
\linethickness{0.35mm}
\put(0,45){\line(1,0){30}}
\put(25,60){\makebox(0,0)[cc]{\kee}}

\linethickness{0.35mm}
\put(25,25){\line(0,1){10}}
\linethickness{0.35mm}
\multiput(15,15)(0.12,0.12){83}{\line(1,0){0.12}}
\linethickness{0.35mm}
\multiput(5,25)(0.12,-0.12){83}{\line(1,0){0.12}}
\linethickness{0.35mm}
\put(15,5){\line(0,1){10}}
\put(15,1.25){\makebox(0,0)[cc]{$\mee$}}

\put(35,1.25){\makebox(0,0)[cc]{$\nee$}}

\put(25,78.75){\makebox(0,0)[cc]{$\outplus$}}

\put(15,15){\makebox(0,0)[cc]{\Dottt}}

\end{picture}


==> PIC/plustimes-5.tex <==
%%Created by jPicEdt 1.4.1_03: mixed JPIC-XML/LaTeX format
%%Fri Aug 26 09:13:37 GMT-10:00 2022
%%Begin JPIC-XML
%<?xml version="1.0" standalone="yes"?>
%<jpic x-min="-5" x-max="40" y-min="1.25" y-max="78.75" auto-bounding="true">
%<multicurve fill-style= "none"
%	 points= "(15,55);(15,55);(15,45);(15,45)"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(10,65);(10,65);(40,65);(40,65)"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(10,65);(10,65);(10,55);(10,55)"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(40,55);(40,55);(40,65);(40,65)"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(25,75);(25,75);(25,65);(25,65)"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(10,55);(10,55);(40,55);(40,55)"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(5,35);(5,35);(5,30);(5,30)"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(0,45);(0,45);(0,35);(0,35)"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(30,35);(30,35);(30,45);(30,45)"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(35,55);(35,55);(35,20);(35,20)"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(0,35);(0,35);(30,35);(30,35)"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(0,45);(0,45);(30,45);(30,45)"
%	 stroke-width= "0.35"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(25,60)"
%	 text-frame= "noframe"
%	 stroke-width= "0.35"
%	 text-hor-align= "center-h"
%	 >
%\kee
%</text>
%<multicurve fill-style= "none"
%	 points= "(25,35);(25,35);(25,30);(25,30)"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(25,30);(25,30);(15,20);(15,20)"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(5,30);(5,30);(15,20);(15,20)"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(25,10);(25,10);(25,5);(25,5)"
%	 stroke-width= "0.35"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(-5,1.25)"
%	 text-frame= "noframe"
%	 stroke-width= "0.35"
%	 text-hor-align= "center-h"
%	 >
%$\mee$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(25,1.25)"
%	 text-frame= "noframe"
%	 stroke-width= "0.35"
%	 text-hor-align= "center-h"
%	 >
%$\nee$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(25,78.75)"
%	 text-frame= "noframe"
%	 stroke-width= "0.35"
%	 text-hor-align= "center-h"
%	 >
%$\outplus$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(15,20)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\Dottt
%</text>
%<multicurve fill-style= "none"
%	 points= "(15,20);(15,20);(25,10);(25,10)"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(35,20);(35,20);(25,10);(25,10)"
%	 stroke-width= "0.35"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(25,10)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\Dottt
%</text>
%<multicurve fill-style= "none"
%	 points= "(-5,20);(-5,20);(-5,5);(-5,5)"
%	 stroke-width= "0.35"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(-5,20)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\Dottt
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(15,40)"
%	 text-frame= "noframe"
%	 stroke-width= "0.35"
%	 text-hor-align= "center-h"
%	 >
%\kee
%</text>
%</jpic>
%%End JPIC-XML
%LaTeX-picture environment using emulated lines and arcs
%You can rescale the whole picture (to 80% for instance) by using the command \def\JPicScale{0.8}
\ifx\JPicScale\undefined\def\JPicScale{1}\fi
\unitlength \JPicScale mm
\begin{picture}(40,78.75)(0,0)
\linethickness{0.35mm}
\put(15,45){\line(0,1){10}}
\linethickness{0.35mm}
\put(10,65){\line(1,0){30}}
\linethickness{0.35mm}
\put(10,55){\line(0,1){10}}
\linethickness{0.35mm}
\put(40,55){\line(0,1){10}}
\linethickness{0.35mm}
\put(25,65){\line(0,1){10}}
\linethickness{0.35mm}
\put(10,55){\line(1,0){30}}
\linethickness{0.35mm}
\put(5,30){\line(0,1){5}}
\linethickness{0.35mm}
\put(0,35){\line(0,1){10}}
\linethickness{0.35mm}
\put(30,35){\line(0,1){10}}
\linethickness{0.35mm}
\put(35,20){\line(0,1){35}}
\linethickness{0.35mm}
\put(0,35){\line(1,0){30}}
\linethickness{0.35mm}
\put(0,45){\line(1,0){30}}
\put(25,60){\makebox(0,0)[cc]{\kee}}

\linethickness{0.35mm}
\put(25,30){\line(0,1){5}}
\linethickness{0.35mm}
\multiput(15,20)(0.12,0.12){83}{\line(1,0){0.12}}
\linethickness{0.35mm}
\multiput(5,30)(0.12,-0.12){83}{\line(1,0){0.12}}
\linethickness{0.35mm}
\put(25,5){\line(0,1){5}}
\put(-5,1.25){\makebox(0,0)[cc]{$\mee$}}

\put(25,1.25){\makebox(0,0)[cc]{$\nee$}}

\put(25,78.75){\makebox(0,0)[cc]{$\outplus$}}

\put(15,20){\makebox(0,0)[cc]{\Dottt}}

\linethickness{0.35mm}
\multiput(15,20)(0.12,-0.12){83}{\line(1,0){0.12}}
\linethickness{0.35mm}
\multiput(25,10)(0.12,0.12){83}{\line(1,0){0.12}}
\put(25,10){\makebox(0,0)[cc]{\Dottt}}

\linethickness{0.35mm}
\put(-5,5){\line(0,1){15}}
\put(-5,20){\makebox(0,0)[cc]{\Dottt}}

\put(15,40){\makebox(0,0)[cc]{\kee}}

\end{picture}


==> PIC/plustimes.tex <==
%%Created by jPicEdt 1.4.1_03: mixed JPIC-XML/LaTeX format
%%Fri Aug 26 00:46:44 GMT-10:00 2022
%%Begin JPIC-XML
%<?xml version="1.0" standalone="yes"?>
%<jpic x-min="0" x-max="80" y-min="1.25" y-max="83.75" auto-bounding="true">
%<multicurve fill-style= "none"
%	 points= "(5,50);(5,50);(5,40);(5,40)"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(0,70);(0,70);(30,70);(30,70)"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(0,70);(0,70);(0,50);(0,50)"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(30,50);(30,50);(30,70);(30,70)"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(15,80);(15,80);(15,70);(15,70)"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(0,50);(0,50);(30,50);(30,50)"
%	 stroke-width= "0.35"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(15,60)"
%	 text-frame= "noframe"
%	 stroke-width= "0.35"
%	 text-hor-align= "center-h"
%	 >
%\gee
%</text>
%<multicurve fill-style= "none"
%	 points= "(55,50);(55,50);(55,40);(55,40)"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(50,70);(50,70);(50,50);(50,50)"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(80,50);(80,50);(80,70);(80,70)"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(65,80);(65,80);(65,70);(65,70)"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(50,50);(50,50);(80,50);(80,50)"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(50,70);(50,70);(80,70);(80,70)"
%	 stroke-width= "0.35"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(65,60)"
%	 text-frame= "noframe"
%	 stroke-width= "0.35"
%	 text-hor-align= "center-h"
%	 >
%\kee
%</text>
%<multicurve fill-style= "none"
%	 points= "(25,50);(25,50);(25,40);(25,40)"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(75,50);(75,50);(75,40);(75,40)"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(50,15);(50,15);(50,5);(50,5)"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(75,40);(75,40);(50,15);(50,15)"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(55,40);(55,40);(30,15);(30,15)"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(25,40);(25,40);(50,15);(50,15)"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(5,40);(5,40);(30,15);(30,15)"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(30,15);(30,15);(30,5);(30,5)"
%	 stroke-width= "0.35"
%	 />
%<text text-vert-align= "bottom"
%	 fill-style= "none"
%	 anchor-point= "(50,20)"
%	 text-frame= "noframe"
%	 stroke-width= "0.35"
%	 text-hor-align= "center-h"
%	 >
%\hee
%</text>
%<text text-vert-align= "bottom"
%	 fill-style= "none"
%	 anchor-point= "(30,20)"
%	 text-frame= "noframe"
%	 stroke-width= "0.35"
%	 text-hor-align= "center-h"
%	 >
%\hee
%</text>
%<text text-vert-align= "bottom"
%	 fill-style= "none"
%	 anchor-point= "(40,28.75)"
%	 text-frame= "noframe"
%	 stroke-width= "0.35"
%	 text-hor-align= "center-h"
%	 >
%\see
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(30,1.25)"
%	 text-frame= "noframe"
%	 stroke-width= "0.35"
%	 text-hor-align= "center-h"
%	 >
%$\mee$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(50,1.25)"
%	 text-frame= "noframe"
%	 stroke-width= "0.35"
%	 text-hor-align= "center-h"
%	 >
%$\nee$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(3.75,42.5)"
%	 text-frame= "noframe"
%	 stroke-width= "0.35"
%	 text-hor-align= "right"
%	 >
%$\mee$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(23.75,42.5)"
%	 text-frame= "noframe"
%	 stroke-width= "0.35"
%	 text-hor-align= "right"
%	 >
%$\nee$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(53.75,42.5)"
%	 text-frame= "noframe"
%	 stroke-width= "0.35"
%	 text-hor-align= "right"
%	 >
%$\mee$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(73.75,42.5)"
%	 text-frame= "noframe"
%	 stroke-width= "0.35"
%	 text-hor-align= "right"
%	 >
%$\nee$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(15,83.75)"
%	 text-frame= "noframe"
%	 stroke-width= "0.35"
%	 text-hor-align= "center-h"
%	 >
%$\outplus$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(65,83.75)"
%	 text-frame= "noframe"
%	 stroke-width= "0.35"
%	 text-hor-align= "center-h"
%	 >
%$\outtimes$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(30,15)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\Dottt
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(50,15)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\Dottt
%</text>
%</jpic>
%%End JPIC-XML
%LaTeX-picture environment using emulated lines and arcs
%You can rescale the whole picture (to 80% for instance) by using the command \def\JPicScale{0.8}
\ifx\JPicScale\undefined\def\JPicScale{1}\fi
\unitlength \JPicScale mm
\begin{picture}(80,83.75)(0,0)
\linethickness{0.35mm}
\put(5,40){\line(0,1){10}}
\linethickness{0.35mm}
\put(0,70){\line(1,0){30}}
\linethickness{0.35mm}
\put(0,50){\line(0,1){20}}
\linethickness{0.35mm}
\put(30,50){\line(0,1){20}}
\linethickness{0.35mm}
\put(15,70){\line(0,1){10}}
\linethickness{0.35mm}
\put(0,50){\line(1,0){30}}
\put(15,60){\makebox(0,0)[cc]{\gee}}

\linethickness{0.35mm}
\put(55,40){\line(0,1){10}}
\linethickness{0.35mm}
\put(50,50){\line(0,1){20}}
\linethickness{0.35mm}
\put(80,50){\line(0,1){20}}
\linethickness{0.35mm}
\put(65,70){\line(0,1){10}}
\linethickness{0.35mm}
\put(50,50){\line(1,0){30}}
\linethickness{0.35mm}
\put(50,70){\line(1,0){30}}
\put(65,60){\makebox(0,0)[cc]{\kee}}

\linethickness{0.35mm}
\put(25,40){\line(0,1){10}}
\linethickness{0.35mm}
\put(75,40){\line(0,1){10}}
\linethickness{0.35mm}
\put(50,5){\line(0,1){10}}
\linethickness{0.35mm}
\multiput(50,15)(0.12,0.12){208}{\line(1,0){0.12}}
\linethickness{0.35mm}
\multiput(30,15)(0.12,0.12){208}{\line(1,0){0.12}}
\linethickness{0.35mm}
\multiput(25,40)(0.12,-0.12){208}{\line(1,0){0.12}}
\linethickness{0.35mm}
\multiput(5,40)(0.12,-0.12){208}{\line(1,0){0.12}}
\linethickness{0.35mm}
\put(30,5){\line(0,1){10}}
\put(50,20){\makebox(0,0)[bc]{\hee}}

\put(30,20){\makebox(0,0)[bc]{\hee}}

\put(40,28.75){\makebox(0,0)[bc]{\see}}

\put(30,1.25){\makebox(0,0)[cc]{$\mee$}}

\put(50,1.25){\makebox(0,0)[cc]{$\nee$}}

\put(3.75,42.5){\makebox(0,0)[cr]{$\mee$}}

\put(23.75,42.5){\makebox(0,0)[cr]{$\nee$}}

\put(53.75,42.5){\makebox(0,0)[cr]{$\mee$}}

\put(73.75,42.5){\makebox(0,0)[cr]{$\nee$}}

\put(15,83.75){\makebox(0,0)[cc]{$\outplus$}}

\put(65,83.75){\makebox(0,0)[cc]{$\outtimes$}}

\put(30,15){\makebox(0,0)[cc]{\Dottt}}

\put(50,15){\makebox(0,0)[cc]{\Dottt}}

\end{picture}


==> PIC/prog-compilation-2.tex <==
%%Created by jPicEdt 1.4.1_03: mixed JPIC-XML/LaTeX format
%%Tue Nov 22 12:16:54 GMT-10:00 2022
%%Begin JPIC-XML
%<?xml version="1.0" standalone="yes"?>
%<jpic x-min="25" x-max="340" y-min="30" y-max="195" auto-bounding="true">
%<multicurve fill-style= "none"
%	 stroke-width= "0.95"
%	 points= "(30,180);(30,180);(80,180);(80,180)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.95"
%	 points= "(30,160);(30,160);(30,140);(30,140)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.95"
%	 points= "(80,160);(80,160);(80,180);(80,180)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.95"
%	 points= "(65,195);(65,195);(65,180);(65,180)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.95"
%	 points= "(50,160);(50,160);(80,160);(80,160)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.95"
%	 points= "(65,160);(65,160);(65,135);(65,135)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.95"
%	 points= "(30,140);(30,140);(50,140);(50,140)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.95"
%	 points= "(30,160);(30,160);(50,140);(50,140)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.95"
%	 points= "(40,170);(40,170);(40,150);(40,150)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.95"
%	 points= "(30,180);(30,180);(50,160);(50,160)"
%	 />
%<text fill-style= "none"
%	 stroke-width= "0.95"
%	 text-vert-align= "center-v"
%	 anchor-point= "(25,135)"
%	 text-rotation= "45"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%\programnote
%</text>
%<multicurve fill-style= "none"
%	 stroke-width= "0.95"
%	 points= "(155,180);(155,180);(205,180);(205,180)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.95"
%	 points= "(205,160);(205,160);(205,180);(205,180)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.95"
%	 points= "(190,195);(190,195);(190,180);(190,180)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.95"
%	 points= "(175,160);(175,160);(205,160);(205,160)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.95"
%	 points= "(190,160);(190,160);(190,80);(190,80)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.95"
%	 points= "(155,180);(155,180);(175,160);(175,160)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.95"
%	 points= "(130,150);(130,150);(180,150);(180,150)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.95"
%	 points= "(130,130);(130,130);(130,110);(130,110)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.95"
%	 points= "(180,130);(180,130);(180,150);(180,150)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.95"
%	 points= "(165,170);(165,170);(165,150);(165,150)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.95"
%	 points= "(150,130);(150,130);(180,130);(180,130)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.95"
%	 points= "(165,130);(165,130);(165,95);(165,95)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.95"
%	 points= "(130,110);(130,110);(150,110);(150,110)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.95"
%	 points= "(130,130);(130,130);(150,110);(150,110)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.95"
%	 points= "(140,140);(140,140);(140,120);(140,120)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.95"
%	 points= "(130,150);(130,150);(150,130);(150,130)"
%	 />
%<text fill-style= "none"
%	 stroke-width= "0.95"
%	 text-vert-align= "center-v"
%	 anchor-point= "(125,105)"
%	 text-rotation= "45"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%\metaprogramnote
%</text>
%<multicurve fill-style= "none"
%	 stroke-width= "0.95"
%	 points= "(290,180);(290,180);(340,180);(340,180)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.95"
%	 points= "(340,160);(340,160);(340,180);(340,180)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.95"
%	 points= "(325,195);(325,195);(325,180);(325,180)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.95"
%	 points= "(310,160);(310,160);(340,160);(340,160)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.95"
%	 points= "(325,160);(325,160);(325,30);(325,30)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.95"
%	 points= "(290,180);(290,180);(310,160);(310,160)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.95"
%	 points= "(265,150);(265,150);(315,150);(315,150)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.95"
%	 points= "(265,130);(265,130);(265,110);(265,110)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.95"
%	 points= "(315,130);(315,130);(315,150);(315,150)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.95"
%	 points= "(300,170);(300,170);(300,150);(300,150)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.95"
%	 points= "(285,130);(285,130);(315,130);(315,130)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.95"
%	 points= "(300,130);(300,130);(300,100);(300,100)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.95"
%	 points= "(265,110);(265,110);(285,110);(285,110)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.95"
%	 points= "(265,130);(265,130);(285,110);(285,110)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.95"
%	 points= "(275,140);(275,140);(275,120);(275,120)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.95"
%	 points= "(265,150);(265,150);(285,130);(285,130)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.95"
%	 points= "(155,105);(155,105);(155,85);(155,85)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.95"
%	 points= "(155,85);(155,85);(175,85);(175,85)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.95"
%	 points= "(155,105);(155,105);(175,85);(175,85)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.95"
%	 points= "(265,100);(265,100);(315,100);(315,100)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.95"
%	 points= "(265,80);(265,80);(265,60);(265,60)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.95"
%	 points= "(315,80);(315,80);(315,100);(315,100)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.95"
%	 points= "(285,80);(285,80);(315,80);(315,80)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.95"
%	 points= "(300,80);(300,80);(300,45);(300,45)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.95"
%	 points= "(265,60);(265,60);(285,60);(285,60)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.95"
%	 points= "(265,80);(265,80);(285,60);(285,60)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.95"
%	 points= "(275,90);(275,90);(275,70);(275,70)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.95"
%	 points= "(265,100);(265,100);(285,80);(285,80)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.95"
%	 points= "(290,55);(290,55);(290,35);(290,35)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.95"
%	 points= "(290,35);(290,35);(310,35);(310,35)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.95"
%	 points= "(290,55);(290,55);(310,35);(310,35)"
%	 />
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(38.75,163.75)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\Progtype$
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(162.5,161.25)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\Progtype$
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(297.5,161.25)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\Progtype$
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(162.5,117.5)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\Lprogtype$
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(297.5,117.5)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\Lprogtype$
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(297.5,68.75)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\Hprogtype$
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(150,80)"
%	 text-rotation= "45"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%\lprogramnote
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(285,30)"
%	 text-rotation= "45"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%\hprogramnote
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(260,55)"
%	 text-rotation= "45"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%\compilernote
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(160,90)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\ltag$
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(295,40)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\htag$
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(270,65)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\ctag$
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(135,115)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\itag$
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(35,145)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\mtag$
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(110,170)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\EQLS
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(245,170)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\EQLS
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(270,115)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\itag$
%</text>
%<ellipse fill-color= "#330033"
%	 fill-style= "solid"
%	 p3= "(167.57,92.42)"
%	 p2= "(167.57,97.58)"
%	 p1= "(162.43,97.58)"
%	 closure= "open"
%	 angle-end= "0"
%	 angle-start= "0"
%	 />
%<ellipse fill-color= "#330033"
%	 fill-style= "solid"
%	 p3= "(142.57,117.42)"
%	 p2= "(142.57,122.58)"
%	 p1= "(137.43,122.58)"
%	 closure= "open"
%	 angle-end= "0"
%	 angle-start= "0"
%	 />
%<ellipse fill-color= "#330033"
%	 fill-style= "solid"
%	 p3= "(277.57,67.42)"
%	 p2= "(277.57,72.58)"
%	 p1= "(272.43,72.58)"
%	 closure= "open"
%	 angle-end= "0"
%	 angle-start= "0"
%	 />
%<ellipse fill-color= "#330033"
%	 fill-style= "solid"
%	 p3= "(277.57,117.42)"
%	 p2= "(277.57,122.58)"
%	 p1= "(272.43,122.58)"
%	 closure= "open"
%	 angle-end= "0"
%	 angle-start= "0"
%	 />
%<ellipse fill-color= "#330033"
%	 fill-style= "solid"
%	 p3= "(302.57,42.42)"
%	 p2= "(302.57,47.58)"
%	 p1= "(297.43,47.58)"
%	 closure= "open"
%	 angle-end= "0"
%	 angle-start= "0"
%	 />
%<ellipse fill-color= "#330033"
%	 fill-style= "solid"
%	 p3= "(42.57,147.42)"
%	 p2= "(42.57,152.58)"
%	 p1= "(37.43,152.58)"
%	 closure= "open"
%	 angle-end= "0"
%	 angle-start= "0"
%	 />
%</jpic>
%%End JPIC-XML
%PSTricks content-type (pstricks.sty package needed)
%Add \usepackage{pstricks} in the preamble of your LaTeX file
%You can rescale the whole picture (to 80% for instance) by using the command \def\JPicScale{0.8}
\ifx\JPicScale\undefined\def\JPicScale{1}\fi
\psset{unit=\JPicScale mm}
\psset{linewidth=0.3,dotsep=1,hatchwidth=0.3,hatchsep=1.5,shadowsize=1,dimen=middle}
\psset{dotsize=0.7 2.5,dotscale=1 1,fillcolor=black}
\psset{arrowsize=1 2,arrowlength=1,arrowinset=0.25,tbarsize=0.7 5,bracketlength=0.15,rbracketlength=0.15}
\begin{pspicture}(0,0)(340,195)
\psline[linewidth=0.95](30,180)(80,180)
\psline[linewidth=0.95](30,160)(30,140)
\psline[linewidth=0.95](80,160)(80,180)
\psline[linewidth=0.95](65,195)(65,180)
\psline[linewidth=0.95](50,160)(80,160)
\psline[linewidth=0.95](65,160)(65,135)
\psline[linewidth=0.95](30,140)(50,140)
\psline[linewidth=0.95](30,160)(50,140)
\psline[linewidth=0.95](40,170)(40,150)
\psline[linewidth=0.95](30,180)(50,160)
\rput[r]{45}(25,135){\programnote}
\psline[linewidth=0.95](155,180)(205,180)
\psline[linewidth=0.95](205,160)(205,180)
\psline[linewidth=0.95](190,195)(190,180)
\psline[linewidth=0.95](175,160)(205,160)
\psline[linewidth=0.95](190,160)(190,80)
\psline[linewidth=0.95](155,180)(175,160)
\psline[linewidth=0.95](130,150)(180,150)
\psline[linewidth=0.95](130,130)(130,110)
\psline[linewidth=0.95](180,130)(180,150)
\psline[linewidth=0.95](165,170)(165,150)
\psline[linewidth=0.95](150,130)(180,130)
\psline[linewidth=0.95](165,130)(165,95)
\psline[linewidth=0.95](130,110)(150,110)
\psline[linewidth=0.95](130,130)(150,110)
\psline[linewidth=0.95](140,140)(140,120)
\psline[linewidth=0.95](130,150)(150,130)
\rput[r]{45}(125,105){\metaprogramnote}
\psline[linewidth=0.95](290,180)(340,180)
\psline[linewidth=0.95](340,160)(340,180)
\psline[linewidth=0.95](325,195)(325,180)
\psline[linewidth=0.95](310,160)(340,160)
\psline[linewidth=0.95](325,160)(325,30)
\psline[linewidth=0.95](290,180)(310,160)
\psline[linewidth=0.95](265,150)(315,150)
\psline[linewidth=0.95](265,130)(265,110)
\psline[linewidth=0.95](315,130)(315,150)
\psline[linewidth=0.95](300,170)(300,150)
\psline[linewidth=0.95](285,130)(315,130)
\psline[linewidth=0.95](300,130)(300,100)
\psline[linewidth=0.95](265,110)(285,110)
\psline[linewidth=0.95](265,130)(285,110)
\psline[linewidth=0.95](275,140)(275,120)
\psline[linewidth=0.95](265,150)(285,130)
\psline[linewidth=0.95](155,105)(155,85)
\psline[linewidth=0.95](155,85)(175,85)
\psline[linewidth=0.95](155,105)(175,85)
\psline[linewidth=0.95](265,100)(315,100)
\psline[linewidth=0.95](265,80)(265,60)
\psline[linewidth=0.95](315,80)(315,100)
\psline[linewidth=0.95](285,80)(315,80)
\psline[linewidth=0.95](300,80)(300,45)
\psline[linewidth=0.95](265,60)(285,60)
\psline[linewidth=0.95](265,80)(285,60)
\psline[linewidth=0.95](275,90)(275,70)
\psline[linewidth=0.95](265,100)(285,80)
\psline[linewidth=0.95](290,55)(290,35)
\psline[linewidth=0.95](290,35)(310,35)
\psline[linewidth=0.95](290,55)(310,35)
\rput[r](38.75,163.75){$\Progtype$}
\rput[r](162.5,161.25){$\Progtype$}
\rput[r](297.5,161.25){$\Progtype$}
\rput[r](162.5,117.5){$\Lprogtype$}
\rput[r](297.5,117.5){$\Lprogtype$}
\rput[r](297.5,68.75){$\Hprogtype$}
\rput[r]{45}(150,80){\lprogramnote}
\rput[r]{45}(285,30){\hprogramnote}
\rput[r]{45}(260,55){\compilernote}
\rput(160,90){$\ltag$}
\rput(295,40){$\htag$}
\rput(270,65){$\ctag$}
\rput(135,115){$\itag$}
\rput(35,145){$\mtag$}
\rput(110,170){\EQLS}
\rput(245,170){\EQLS}
\rput(270,115){$\itag$}
\newrgbcolor{userFillColour}{0.2 0 0.2}
\rput{90}(165,95){\psellipse[fillcolor=userFillColour,fillstyle=solid](0,0)(2.58,-2.57)}
\newrgbcolor{userFillColour}{0.2 0 0.2}
\rput{90}(140,120){\psellipse[fillcolor=userFillColour,fillstyle=solid](0,0)(2.58,-2.57)}
\newrgbcolor{userFillColour}{0.2 0 0.2}
\rput{90}(275,70){\psellipse[fillcolor=userFillColour,fillstyle=solid](0,0)(2.58,-2.57)}
\newrgbcolor{userFillColour}{0.2 0 0.2}
\rput{90}(275,120){\psellipse[fillcolor=userFillColour,fillstyle=solid](0,0)(2.58,-2.57)}
\newrgbcolor{userFillColour}{0.2 0 0.2}
\rput{90}(300,45){\psellipse[fillcolor=userFillColour,fillstyle=solid](0,0)(2.58,-2.57)}
\newrgbcolor{userFillColour}{0.2 0 0.2}
\rput{90}(40,150){\psellipse[fillcolor=userFillColour,fillstyle=solid](0,0)(2.58,-2.57)}
\end{pspicture}


==> PIC/prog-compilation.tex <==
%%Created by jPicEdt 1.4.1_03: mixed JPIC-XML/LaTeX format
%%Thu Nov 22 12:40:42 GMT-10:00 2018
%%Begin JPIC-XML
%<?xml version="1.0" standalone="yes"?>
%<jpic x-min="25" x-max="340" y-min="30" y-max="195" auto-bounding="true">
%<multicurve fill-style= "none"
%	 points= "(30,180);(30,180);(80,180);(80,180)"
%	 stroke-width= "0.95"
%	 />
%<multicurve fill-style= "none"
%	 points= "(30,160);(30,160);(30,140);(30,140)"
%	 stroke-width= "0.95"
%	 />
%<multicurve fill-style= "none"
%	 points= "(80,160);(80,160);(80,180);(80,180)"
%	 stroke-width= "0.95"
%	 />
%<multicurve fill-style= "none"
%	 points= "(65,195);(65,195);(65,180);(65,180)"
%	 stroke-width= "0.95"
%	 />
%<multicurve fill-style= "none"
%	 points= "(50,160);(50,160);(80,160);(80,160)"
%	 stroke-width= "0.95"
%	 />
%<multicurve fill-style= "none"
%	 points= "(65,160);(65,160);(65,135);(65,135)"
%	 stroke-width= "0.95"
%	 />
%<multicurve fill-style= "none"
%	 points= "(30,140);(30,140);(50,140);(50,140)"
%	 stroke-width= "0.95"
%	 />
%<multicurve fill-style= "none"
%	 points= "(30,160);(30,160);(50,140);(50,140)"
%	 stroke-width= "0.95"
%	 />
%<multicurve fill-style= "none"
%	 points= "(40,170);(40,170);(40,150);(40,150)"
%	 stroke-width= "0.95"
%	 />
%<multicurve fill-style= "none"
%	 points= "(30,180);(30,180);(50,160);(50,160)"
%	 stroke-width= "0.95"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(25,135)"
%	 text-rotation= "45"
%	 text-frame= "noframe"
%	 stroke-width= "0.95"
%	 text-hor-align= "right"
%	 >
%\programnote
%</text>
%<multicurve fill-style= "none"
%	 points= "(155,180);(155,180);(205,180);(205,180)"
%	 stroke-width= "0.95"
%	 />
%<multicurve fill-style= "none"
%	 points= "(205,160);(205,160);(205,180);(205,180)"
%	 stroke-width= "0.95"
%	 />
%<multicurve fill-style= "none"
%	 points= "(190,195);(190,195);(190,180);(190,180)"
%	 stroke-width= "0.95"
%	 />
%<multicurve fill-style= "none"
%	 points= "(175,160);(175,160);(205,160);(205,160)"
%	 stroke-width= "0.95"
%	 />
%<multicurve fill-style= "none"
%	 points= "(190,160);(190,160);(190,80);(190,80)"
%	 stroke-width= "0.95"
%	 />
%<multicurve fill-style= "none"
%	 points= "(155,180);(155,180);(175,160);(175,160)"
%	 stroke-width= "0.95"
%	 />
%<multicurve fill-style= "none"
%	 points= "(130,150);(130,150);(180,150);(180,150)"
%	 stroke-width= "0.95"
%	 />
%<multicurve fill-style= "none"
%	 points= "(130,130);(130,130);(130,110);(130,110)"
%	 stroke-width= "0.95"
%	 />
%<multicurve fill-style= "none"
%	 points= "(180,130);(180,130);(180,150);(180,150)"
%	 stroke-width= "0.95"
%	 />
%<multicurve fill-style= "none"
%	 points= "(165,170);(165,170);(165,150);(165,150)"
%	 stroke-width= "0.95"
%	 />
%<multicurve fill-style= "none"
%	 points= "(150,130);(150,130);(180,130);(180,130)"
%	 stroke-width= "0.95"
%	 />
%<multicurve fill-style= "none"
%	 points= "(165,130);(165,130);(165,95);(165,95)"
%	 stroke-width= "0.95"
%	 />
%<multicurve fill-style= "none"
%	 points= "(130,110);(130,110);(150,110);(150,110)"
%	 stroke-width= "0.95"
%	 />
%<multicurve fill-style= "none"
%	 points= "(130,130);(130,130);(150,110);(150,110)"
%	 stroke-width= "0.95"
%	 />
%<multicurve fill-style= "none"
%	 points= "(140,140);(140,140);(140,120);(140,120)"
%	 stroke-width= "0.95"
%	 />
%<multicurve fill-style= "none"
%	 points= "(130,150);(130,150);(150,130);(150,130)"
%	 stroke-width= "0.95"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(125,105)"
%	 text-rotation= "45"
%	 text-frame= "noframe"
%	 stroke-width= "0.95"
%	 text-hor-align= "right"
%	 >
%\metaprogramnote
%</text>
%<multicurve fill-style= "none"
%	 points= "(290,180);(290,180);(340,180);(340,180)"
%	 stroke-width= "0.95"
%	 />
%<multicurve fill-style= "none"
%	 points= "(340,160);(340,160);(340,180);(340,180)"
%	 stroke-width= "0.95"
%	 />
%<multicurve fill-style= "none"
%	 points= "(325,195);(325,195);(325,180);(325,180)"
%	 stroke-width= "0.95"
%	 />
%<multicurve fill-style= "none"
%	 points= "(310,160);(310,160);(340,160);(340,160)"
%	 stroke-width= "0.95"
%	 />
%<multicurve fill-style= "none"
%	 points= "(325,160);(325,160);(325,30);(325,30)"
%	 stroke-width= "0.95"
%	 />
%<multicurve fill-style= "none"
%	 points= "(290,180);(290,180);(310,160);(310,160)"
%	 stroke-width= "0.95"
%	 />
%<multicurve fill-style= "none"
%	 points= "(265,150);(265,150);(315,150);(315,150)"
%	 stroke-width= "0.95"
%	 />
%<multicurve fill-style= "none"
%	 points= "(265,130);(265,130);(265,110);(265,110)"
%	 stroke-width= "0.95"
%	 />
%<multicurve fill-style= "none"
%	 points= "(315,130);(315,130);(315,150);(315,150)"
%	 stroke-width= "0.95"
%	 />
%<multicurve fill-style= "none"
%	 points= "(300,170);(300,170);(300,150);(300,150)"
%	 stroke-width= "0.95"
%	 />
%<multicurve fill-style= "none"
%	 points= "(285,130);(285,130);(315,130);(315,130)"
%	 stroke-width= "0.95"
%	 />
%<multicurve fill-style= "none"
%	 points= "(300,130);(300,130);(300,100);(300,100)"
%	 stroke-width= "0.95"
%	 />
%<multicurve fill-style= "none"
%	 points= "(265,110);(265,110);(285,110);(285,110)"
%	 stroke-width= "0.95"
%	 />
%<multicurve fill-style= "none"
%	 points= "(265,130);(265,130);(285,110);(285,110)"
%	 stroke-width= "0.95"
%	 />
%<multicurve fill-style= "none"
%	 points= "(275,140);(275,140);(275,120);(275,120)"
%	 stroke-width= "0.95"
%	 />
%<multicurve fill-style= "none"
%	 points= "(265,150);(265,150);(285,130);(285,130)"
%	 stroke-width= "0.95"
%	 />
%<multicurve fill-style= "none"
%	 points= "(155,105);(155,105);(155,85);(155,85)"
%	 stroke-width= "0.95"
%	 />
%<multicurve fill-style= "none"
%	 points= "(155,85);(155,85);(175,85);(175,85)"
%	 stroke-width= "0.95"
%	 />
%<multicurve fill-style= "none"
%	 points= "(155,105);(155,105);(175,85);(175,85)"
%	 stroke-width= "0.95"
%	 />
%<multicurve fill-style= "none"
%	 points= "(265,100);(265,100);(315,100);(315,100)"
%	 stroke-width= "0.95"
%	 />
%<multicurve fill-style= "none"
%	 points= "(265,80);(265,80);(265,60);(265,60)"
%	 stroke-width= "0.95"
%	 />
%<multicurve fill-style= "none"
%	 points= "(315,80);(315,80);(315,100);(315,100)"
%	 stroke-width= "0.95"
%	 />
%<multicurve fill-style= "none"
%	 points= "(285,80);(285,80);(315,80);(315,80)"
%	 stroke-width= "0.95"
%	 />
%<multicurve fill-style= "none"
%	 points= "(300,80);(300,80);(300,45);(300,45)"
%	 stroke-width= "0.95"
%	 />
%<multicurve fill-style= "none"
%	 points= "(265,60);(265,60);(285,60);(285,60)"
%	 stroke-width= "0.95"
%	 />
%<multicurve fill-style= "none"
%	 points= "(265,80);(265,80);(285,60);(285,60)"
%	 stroke-width= "0.95"
%	 />
%<multicurve fill-style= "none"
%	 points= "(275,90);(275,90);(275,70);(275,70)"
%	 stroke-width= "0.95"
%	 />
%<multicurve fill-style= "none"
%	 points= "(265,100);(265,100);(285,80);(285,80)"
%	 stroke-width= "0.95"
%	 />
%<multicurve fill-style= "none"
%	 points= "(290,55);(290,55);(290,35);(290,35)"
%	 stroke-width= "0.95"
%	 />
%<multicurve fill-style= "none"
%	 points= "(290,35);(290,35);(310,35);(310,35)"
%	 stroke-width= "0.95"
%	 />
%<multicurve fill-style= "none"
%	 points= "(290,55);(290,55);(310,35);(310,35)"
%	 stroke-width= "0.95"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(38.75,163.75)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\Progtype$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(162.5,161.25)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\Progtype$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(297.5,161.25)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\Progtype$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(162.5,117.5)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\Lprogtype$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(297.5,117.5)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\Lprogtype$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(297.5,68.75)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\Hprogtype$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(150,80)"
%	 text-rotation= "45"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%\lprogramnote
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(285,30)"
%	 text-rotation= "45"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%\hprogramnote
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(260,55)"
%	 text-rotation= "45"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%\compilernote
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(160,90)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\ltag$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(295,40)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\htag$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(270,65)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\ctag$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(135,115)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\itag$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(35,145)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\mtag$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(110,170)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\EQLS
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(245,170)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\EQLS
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(270,115)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\itag$
%</text>
%</jpic>
%%End JPIC-XML
%PSTricks content-type (pstricks.sty package needed)
%Add \usepackage{pstricks} in the preamble of your LaTeX file
%You can rescale the whole picture (to 80% for instance) by using the command \def\JPicScale{0.8}
\ifx\JPicScale\undefined\def\JPicScale{1}\fi
\psset{unit=\JPicScale mm}
\psset{linewidth=0.3,dotsep=1,hatchwidth=0.3,hatchsep=1.5,shadowsize=1,dimen=middle}
\psset{dotsize=0.7 2.5,dotscale=1 1,fillcolor=black}
\psset{arrowsize=1 2,arrowlength=1,arrowinset=0.25,tbarsize=0.7 5,bracketlength=0.15,rbracketlength=0.15}
\begin{pspicture}(0,0)(340,195)
\psline[linewidth=0.95](30,180)(80,180)
\psline[linewidth=0.95](30,160)(30,140)
\psline[linewidth=0.95](80,160)(80,180)
\psline[linewidth=0.95](65,195)(65,180)
\psline[linewidth=0.95](50,160)(80,160)
\psline[linewidth=0.95](65,160)(65,135)
\psline[linewidth=0.95](30,140)(50,140)
\psline[linewidth=0.95](30,160)(50,140)
\psline[linewidth=0.95](40,170)(40,150)
\psline[linewidth=0.95](30,180)(50,160)
\rput[r]{45}(25,135){\programnote}
\psline[linewidth=0.95](155,180)(205,180)
\psline[linewidth=0.95](205,160)(205,180)
\psline[linewidth=0.95](190,195)(190,180)
\psline[linewidth=0.95](175,160)(205,160)
\psline[linewidth=0.95](190,160)(190,80)
\psline[linewidth=0.95](155,180)(175,160)
\psline[linewidth=0.95](130,150)(180,150)
\psline[linewidth=0.95](130,130)(130,110)
\psline[linewidth=0.95](180,130)(180,150)
\psline[linewidth=0.95](165,170)(165,150)
\psline[linewidth=0.95](150,130)(180,130)
\psline[linewidth=0.95](165,130)(165,95)
\psline[linewidth=0.95](130,110)(150,110)
\psline[linewidth=0.95](130,130)(150,110)
\psline[linewidth=0.95](140,140)(140,120)
\psline[linewidth=0.95](130,150)(150,130)
\rput[r]{45}(125,105){\metaprogramnote}
\psline[linewidth=0.95](290,180)(340,180)
\psline[linewidth=0.95](340,160)(340,180)
\psline[linewidth=0.95](325,195)(325,180)
\psline[linewidth=0.95](310,160)(340,160)
\psline[linewidth=0.95](325,160)(325,30)
\psline[linewidth=0.95](290,180)(310,160)
\psline[linewidth=0.95](265,150)(315,150)
\psline[linewidth=0.95](265,130)(265,110)
\psline[linewidth=0.95](315,130)(315,150)
\psline[linewidth=0.95](300,170)(300,150)
\psline[linewidth=0.95](285,130)(315,130)
\psline[linewidth=0.95](300,130)(300,100)
\psline[linewidth=0.95](265,110)(285,110)
\psline[linewidth=0.95](265,130)(285,110)
\psline[linewidth=0.95](275,140)(275,120)
\psline[linewidth=0.95](265,150)(285,130)
\psline[linewidth=0.95](155,105)(155,85)
\psline[linewidth=0.95](155,85)(175,85)
\psline[linewidth=0.95](155,105)(175,85)
\psline[linewidth=0.95](265,100)(315,100)
\psline[linewidth=0.95](265,80)(265,60)
\psline[linewidth=0.95](315,80)(315,100)
\psline[linewidth=0.95](285,80)(315,80)
\psline[linewidth=0.95](300,80)(300,45)
\psline[linewidth=0.95](265,60)(285,60)
\psline[linewidth=0.95](265,80)(285,60)
\psline[linewidth=0.95](275,90)(275,70)
\psline[linewidth=0.95](265,100)(285,80)
\psline[linewidth=0.95](290,55)(290,35)
\psline[linewidth=0.95](290,35)(310,35)
\psline[linewidth=0.95](290,55)(310,35)
\rput[r](38.75,163.75){$\Progtype$}
\rput[r](162.5,161.25){$\Progtype$}
\rput[r](297.5,161.25){$\Progtype$}
\rput[r](162.5,117.5){$\Lprogtype$}
\rput[r](297.5,117.5){$\Lprogtype$}
\rput[r](297.5,68.75){$\Hprogtype$}
\rput[r]{45}(150,80){\lprogramnote}
\rput[r]{45}(285,30){\hprogramnote}
\rput[r]{45}(260,55){\compilernote}
\rput(160,90){$\ltag$}
\rput(295,40){$\htag$}
\rput(270,65){$\ctag$}
\rput(135,115){$\itag$}
\rput(35,145){$\mtag$}
\rput(110,170){\EQLS}
\rput(245,170){\EQLS}
\rput(270,115){$\itag$}
\end{pspicture}


==> PIC/prog-compiler.tex <==
%%Created by jPicEdt 1.4.1_03: mixed JPIC-XML/LaTeX format
%%Mon Nov 21 15:26:21 HST 2016
%%Begin JPIC-XML
%<?xml version="1.0" standalone="yes"?>
%<jpic x-min="55" x-max="130" y-min="15" y-max="75" auto-bounding="true">
%<multicurve stroke-width= "0.75"
%	 points= "(80,60);(80,60);(130,60);(130,60)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.75"
%	 points= "(80,40);(80,40);(80,20);(80,20)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.75"
%	 points= "(130,40);(130,40);(130,60);(130,60)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.75"
%	 points= "(115,75);(115,75);(115,60);(115,60)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.75"
%	 points= "(100,40);(100,40);(130,40);(130,40)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.75"
%	 points= "(115,40);(115,40);(115,15);(115,15)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.75"
%	 points= "(80,20);(80,20);(100,20);(100,20)"
%	 fill-style= "none"
%	 />
%<text text-vert-align= "center-v"
%	 stroke-width= "0.75"
%	 anchor-point= "(108.12,45)"
%	 text-frame= "noframe"
%	 fill-style= "none"
%	 text-hor-align= "center-h"
%	 >
%\universal
%</text>
%<text text-vert-align= "center-v"
%	 stroke-width= "0.75"
%	 anchor-point= "(85,25)"
%	 text-frame= "noframe"
%	 fill-style= "none"
%	 text-hor-align= "center-h"
%	 >
%\program
%</text>
%<text text-vert-align= "center-v"
%	 stroke-width= "0.75"
%	 anchor-point= "(55,35)"
%	 text-frame= "noframe"
%	 fill-style= "none"
%	 text-hor-align= "center-h"
%	 >
%\EQLS
%</text>
%<multicurve stroke-width= "0.75"
%	 points= "(80,40);(80,40);(100,20);(100,20)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.75"
%	 points= "(90,50);(90,50);(90,30);(90,30)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.75"
%	 points= "(80,60);(80,60);(100,40);(100,40)"
%	 fill-style= "none"
%	 />
%<text text-vert-align= "center-v"
%	 stroke-width= "0.8"
%	 anchor-point= "(88.12,44.38)"
%	 text-frame= "noframe"
%	 fill-style= "none"
%	 text-hor-align= "right"
%	 >
%\progtype
%</text>
%</jpic>
%%End JPIC-XML
%PSTricks content-type (pstricks.sty package needed)
%Add \usepackage{pstricks} in the preamble of your LaTeX file
%You can rescale the whole picture (to 80% for instance) by using the command \def\JPicScale{0.8}
\ifx\JPicScale\undefined\def\JPicScale{1}\fi
\psset{unit=\JPicScale mm}
\psset{linewidth=0.3,dotsep=1,hatchwidth=0.3,hatchsep=1.5,shadowsize=1,dimen=middle}
\psset{dotsize=0.7 2.5,dotscale=1 1,fillcolor=black}
\psset{arrowsize=1 2,arrowlength=1,arrowinset=0.25,tbarsize=0.7 5,bracketlength=0.15,rbracketlength=0.15}
\begin{pspicture}(0,0)(130,75)
\psline[linewidth=0.75](80,60)(130,60)
\psline[linewidth=0.75](80,40)(80,20)
\psline[linewidth=0.75](130,40)(130,60)
\psline[linewidth=0.75](115,75)(115,60)
\psline[linewidth=0.75](100,40)(130,40)
\psline[linewidth=0.75](115,40)(115,15)
\psline[linewidth=0.75](80,20)(100,20)
\rput(108.12,45){\universal}
\rput(85,25){\program}
\rput(55,35){\EQLS}
\psline[linewidth=0.75](80,40)(100,20)
\psline[linewidth=0.75](90,50)(90,30)
\psline[linewidth=0.75](80,60)(100,40)
\rput[r](88.12,44.38){\progtype}
\end{pspicture}


==> PIC/prog-hi-lo-compile.tex <==
%%Created by jPicEdt 1.4.1_03: mixed JPIC-XML/LaTeX format
%%Wed Nov 21 23:29:22 GMT-10:00 2018
%%Begin JPIC-XML
%<?xml version="1.0" standalone="yes"?>
%<jpic x-min="40" x-max="330" y-min="10" y-max="95" auto-bounding="true">
%<multicurve fill-style= "none"
%	 points= "(40,80);(40,80);(90,80);(90,80)"
%	 stroke-width= "0.95"
%	 />
%<multicurve fill-style= "none"
%	 points= "(90,60);(90,60);(90,80);(90,80)"
%	 stroke-width= "0.95"
%	 />
%<multicurve fill-style= "none"
%	 points= "(75,95);(75,95);(75,80);(75,80)"
%	 stroke-width= "0.95"
%	 />
%<multicurve fill-style= "none"
%	 points= "(60,60);(60,60);(90,60);(90,60)"
%	 stroke-width= "0.95"
%	 />
%<multicurve fill-style= "none"
%	 points= "(75,60);(75,60);(75,25);(75,25)"
%	 stroke-width= "0.95"
%	 />
%<multicurve fill-style= "none"
%	 points= "(50,70);(50,70);(50,25);(50,25)"
%	 stroke-width= "0.95"
%	 />
%<multicurve fill-style= "none"
%	 points= "(40,80);(40,80);(60,60);(60,60)"
%	 stroke-width= "0.95"
%	 />
%<multicurve fill-style= "none"
%	 points= "(155,80);(155,80);(205,80);(205,80)"
%	 stroke-width= "0.95"
%	 />
%<multicurve fill-style= "none"
%	 points= "(205,60);(205,60);(205,80);(205,80)"
%	 stroke-width= "0.95"
%	 />
%<multicurve fill-style= "none"
%	 points= "(190,95);(190,95);(190,80);(190,80)"
%	 stroke-width= "0.95"
%	 />
%<multicurve fill-style= "none"
%	 points= "(175,60);(175,60);(205,60);(205,60)"
%	 stroke-width= "0.95"
%	 />
%<multicurve fill-style= "none"
%	 points= "(190,60);(190,60);(190,15);(190,15)"
%	 stroke-width= "0.95"
%	 />
%<multicurve fill-style= "none"
%	 points= "(155,80);(155,80);(175,60);(175,60)"
%	 stroke-width= "0.95"
%	 />
%<multicurve fill-style= "none"
%	 points= "(155,60);(155,60);(175,40);(175,40)"
%	 stroke-width= "0.95"
%	 />
%<multicurve fill-style= "none"
%	 points= "(175,20);(175,20);(175,40);(175,40)"
%	 stroke-width= "0.95"
%	 />
%<multicurve fill-style= "none"
%	 points= "(165,70);(165,70);(165,50);(165,50)"
%	 stroke-width= "0.95"
%	 />
%<multicurve fill-style= "none"
%	 points= "(155,40);(155,40);(175,20);(175,20)"
%	 stroke-width= "0.95"
%	 />
%<multicurve fill-style= "none"
%	 points= "(165,30);(165,30);(165,15);(165,15)"
%	 stroke-width= "0.95"
%	 />
%<multicurve fill-style= "none"
%	 points= "(155,60);(155,60);(155,40);(155,40)"
%	 stroke-width= "0.95"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(120,70)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\EQLS$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(75,70)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\highunitag$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(48.12,26.88)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\Highprogtype$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(163.12,63.12)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\Lowprogtype$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(190,70)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\lowunitag$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(163.12,21.88)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\Highprogtype$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(150,40.62)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%\compilernote
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(165,40)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\copilertag$
%</text>
%<multicurve fill-style= "none"
%	 points= "(280,80);(280,80);(330,80);(330,80)"
%	 stroke-width= "0.95"
%	 />
%<multicurve fill-style= "none"
%	 points= "(330,60);(330,60);(330,80);(330,80)"
%	 stroke-width= "0.95"
%	 />
%<multicurve fill-style= "none"
%	 points= "(315,95);(315,95);(315,80);(315,80)"
%	 stroke-width= "0.95"
%	 />
%<multicurve fill-style= "none"
%	 points= "(300,60);(300,60);(330,60);(330,60)"
%	 stroke-width= "0.95"
%	 />
%<multicurve fill-style= "none"
%	 points= "(315,60);(315,60);(315,15);(315,15)"
%	 stroke-width= "0.95"
%	 />
%<multicurve fill-style= "none"
%	 points= "(280,80);(280,80);(300,60);(300,60)"
%	 stroke-width= "0.95"
%	 />
%<multicurve fill-style= "none"
%	 points= "(290,70);(290,70);(290,50);(290,50)"
%	 stroke-width= "0.95"
%	 />
%<multicurve fill-style= "none"
%	 points= "(290,30);(290,30);(290,15);(290,15)"
%	 stroke-width= "0.95"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(235,70)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\EQLS$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(288.12,63.12)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\Lowprogtype$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(315,70)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\lowunitag$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(288.12,21.88)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\Highprogtype$
%</text>
%<multicurve fill-style= "none"
%	 points= "(255,50);(255,50);(305,50);(305,50)"
%	 stroke-width= "0.95"
%	 />
%<multicurve fill-style= "none"
%	 points= "(255,30);(255,30);(255,10);(255,10)"
%	 stroke-width= "0.95"
%	 />
%<multicurve fill-style= "none"
%	 points= "(305,30);(305,30);(305,50);(305,50)"
%	 stroke-width= "0.95"
%	 />
%<multicurve fill-style= "none"
%	 points= "(275,30);(275,30);(305,30);(305,30)"
%	 stroke-width= "0.95"
%	 />
%<multicurve fill-style= "none"
%	 points= "(255,10);(255,10);(275,10);(275,10)"
%	 stroke-width= "0.95"
%	 />
%<multicurve fill-style= "none"
%	 points= "(255,30);(255,30);(275,10);(275,10)"
%	 stroke-width= "0.95"
%	 />
%<multicurve fill-style= "none"
%	 points= "(265,40);(265,40);(265,20);(265,20)"
%	 stroke-width= "0.95"
%	 />
%<multicurve fill-style= "none"
%	 points= "(255,50);(255,50);(275,30);(275,30)"
%	 stroke-width= "0.95"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(290,40)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\lowunitag$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(247.5,15)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%\compilerote
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(260,15)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\Compiler$
%</text>
%</jpic>
%%End JPIC-XML
%PSTricks content-type (pstricks.sty package needed)
%Add \usepackage{pstricks} in the preamble of your LaTeX file
%You can rescale the whole picture (to 80% for instance) by using the command \def\JPicScale{0.8}
\ifx\JPicScale\undefined\def\JPicScale{1}\fi
\psset{unit=\JPicScale mm}
\psset{linewidth=0.3,dotsep=1,hatchwidth=0.3,hatchsep=1.5,shadowsize=1,dimen=middle}
\psset{dotsize=0.7 2.5,dotscale=1 1,fillcolor=black}
\psset{arrowsize=1 2,arrowlength=1,arrowinset=0.25,tbarsize=0.7 5,bracketlength=0.15,rbracketlength=0.15}
\begin{pspicture}(0,0)(330,95)
\psline[linewidth=0.95](40,80)(90,80)
\psline[linewidth=0.95](90,60)(90,80)
\psline[linewidth=0.95](75,95)(75,80)
\psline[linewidth=0.95](60,60)(90,60)
\psline[linewidth=0.95](75,60)(75,25)
\psline[linewidth=0.95](50,70)(50,25)
\psline[linewidth=0.95](40,80)(60,60)
\psline[linewidth=0.95](155,80)(205,80)
\psline[linewidth=0.95](205,60)(205,80)
\psline[linewidth=0.95](190,95)(190,80)
\psline[linewidth=0.95](175,60)(205,60)
\psline[linewidth=0.95](190,60)(190,15)
\psline[linewidth=0.95](155,80)(175,60)
\psline[linewidth=0.95](155,60)(175,40)
\psline[linewidth=0.95](175,20)(175,40)
\psline[linewidth=0.95](165,70)(165,50)
\psline[linewidth=0.95](155,40)(175,20)
\psline[linewidth=0.95](165,30)(165,15)
\psline[linewidth=0.95](155,60)(155,40)
\rput(120,70){$\EQLS$}
\rput(75,70){$\highunitag$}
\rput[r](48.12,26.88){$\Highprogtype$}
\rput[r](163.12,63.12){$\Lowprogtype$}
\rput(190,70){$\lowunitag$}
\rput[r](163.12,21.88){$\Highprogtype$}
\rput[r](150,40.62){\compilernote}
\rput(165,40){$\copilertag$}
\psline[linewidth=0.95](280,80)(330,80)
\psline[linewidth=0.95](330,60)(330,80)
\psline[linewidth=0.95](315,95)(315,80)
\psline[linewidth=0.95](300,60)(330,60)
\psline[linewidth=0.95](315,60)(315,15)
\psline[linewidth=0.95](280,80)(300,60)
\psline[linewidth=0.95](290,70)(290,50)
\psline[linewidth=0.95](290,30)(290,15)
\rput(235,70){$\EQLS$}
\rput[r](288.12,63.12){$\Lowprogtype$}
\rput(315,70){$\lowunitag$}
\rput[r](288.12,21.88){$\Highprogtype$}
\psline[linewidth=0.95](255,50)(305,50)
\psline[linewidth=0.95](255,30)(255,10)
\psline[linewidth=0.95](305,30)(305,50)
\psline[linewidth=0.95](275,30)(305,30)
\psline[linewidth=0.95](255,10)(275,10)
\psline[linewidth=0.95](255,30)(275,10)
\psline[linewidth=0.95](265,40)(265,20)
\psline[linewidth=0.95](255,50)(275,30)
\rput(290,40){$\lowunitag$}
\rput[r](247.5,15){\compilerote}
\rput(260,15){$\Compiler$}
\end{pspicture}


==> PIC/prog-hi-lo-compiler.tex <==
%%Created by jPicEdt 1.4.1_03: mixed JPIC-XML/LaTeX format
%%Mon Nov 21 23:20:01 HST 2016
%%Begin JPIC-XML
%<?xml version="1.0" standalone="yes"?>
%<jpic x-min="40" x-max="240" y-min="10" y-max="95" auto-bounding="true">
%<multicurve stroke-width= "0.95"
%	 points= "(40,80);(40,80);(90,80);(90,80)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.95"
%	 points= "(90,60);(90,60);(90,80);(90,80)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.95"
%	 points= "(75,95);(75,95);(75,80);(75,80)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.95"
%	 points= "(60,60);(60,60);(90,60);(90,60)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.95"
%	 points= "(75,60);(75,60);(75,25);(75,25)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.95"
%	 points= "(50,70);(50,70);(50,25);(50,25)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.95"
%	 points= "(40,80);(40,80);(60,60);(60,60)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.95"
%	 points= "(190,80);(190,80);(240,80);(240,80)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.95"
%	 points= "(240,60);(240,60);(240,80);(240,80)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.95"
%	 points= "(225,95);(225,95);(225,80);(225,80)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.95"
%	 points= "(210,60);(210,60);(240,60);(240,60)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.95"
%	 points= "(225,60);(225,60);(225,15);(225,15)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.95"
%	 points= "(190,80);(190,80);(210,60);(210,60)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.95"
%	 points= "(200,70);(200,70);(200,50);(200,50)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.95"
%	 points= "(200,30);(200,30);(200,15);(200,15)"
%	 fill-style= "none"
%	 />
%<text text-vert-align= "center-v"
%	 anchor-point= "(130,70)"
%	 text-frame= "noframe"
%	 fill-style= "none"
%	 text-hor-align= "center-h"
%	 >
%$\EQLS$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(75,70)"
%	 text-frame= "noframe"
%	 fill-style= "none"
%	 text-hor-align= "center-h"
%	 >
%$\highunitag$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(48.12,26.88)"
%	 text-frame= "noframe"
%	 fill-style= "none"
%	 text-hor-align= "right"
%	 >
%$\Highprogtype$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(198.12,63.12)"
%	 text-frame= "noframe"
%	 fill-style= "none"
%	 text-hor-align= "right"
%	 >
%$\Lowprogtype$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(225,70)"
%	 text-frame= "noframe"
%	 fill-style= "none"
%	 text-hor-align= "center-h"
%	 >
%$\lowunitag$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(198.12,21.88)"
%	 text-frame= "noframe"
%	 fill-style= "none"
%	 text-hor-align= "right"
%	 >
%$\Highprogtype$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(171.25,15)"
%	 text-frame= "noframe"
%	 fill-style= "none"
%	 text-hor-align= "center-h"
%	 >
%$\copilertag$
%</text>
%<multicurve stroke-width= "0.95"
%	 points= "(165,50);(165,50);(215,50);(215,50)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.95"
%	 points= "(165,30);(165,30);(165,10);(165,10)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.95"
%	 points= "(215,30);(215,30);(215,50);(215,50)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.95"
%	 points= "(185,30);(185,30);(215,30);(215,30)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.95"
%	 points= "(165,10);(165,10);(185,10);(185,10)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.95"
%	 points= "(165,30);(165,30);(185,10);(185,10)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.95"
%	 points= "(175,40);(175,40);(175,20);(175,20)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.95"
%	 points= "(165,50);(165,50);(185,30);(185,30)"
%	 fill-style= "none"
%	 />
%<text text-vert-align= "center-v"
%	 anchor-point= "(200,40)"
%	 text-frame= "noframe"
%	 fill-style= "none"
%	 text-hor-align= "center-h"
%	 >
%$\lowunitag$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(157.5,15)"
%	 text-frame= "noframe"
%	 fill-style= "none"
%	 text-hor-align= "right"
%	 >
%\compilernote
%</text>
%</jpic>
%%End JPIC-XML
%PSTricks content-type (pstricks.sty package needed)
%Add \usepackage{pstricks} in the preamble of your LaTeX file
%You can rescale the whole picture (to 80% for instance) by using the command \def\JPicScale{0.8}
\ifx\JPicScale\undefined\def\JPicScale{1}\fi
\psset{unit=\JPicScale mm}
\psset{linewidth=0.3,dotsep=1,hatchwidth=0.3,hatchsep=1.5,shadowsize=1,dimen=middle}
\psset{dotsize=0.7 2.5,dotscale=1 1,fillcolor=black}
\psset{arrowsize=1 2,arrowlength=1,arrowinset=0.25,tbarsize=0.7 5,bracketlength=0.15,rbracketlength=0.15}
\begin{pspicture}(0,0)(240,95)
\psline[linewidth=0.95](40,80)(90,80)
\psline[linewidth=0.95](90,60)(90,80)
\psline[linewidth=0.95](75,95)(75,80)
\psline[linewidth=0.95](60,60)(90,60)
\psline[linewidth=0.95](75,60)(75,25)
\psline[linewidth=0.95](50,70)(50,25)
\psline[linewidth=0.95](40,80)(60,60)
\psline[linewidth=0.95](190,80)(240,80)
\psline[linewidth=0.95](240,60)(240,80)
\psline[linewidth=0.95](225,95)(225,80)
\psline[linewidth=0.95](210,60)(240,60)
\psline[linewidth=0.95](225,60)(225,15)
\psline[linewidth=0.95](190,80)(210,60)
\psline[linewidth=0.95](200,70)(200,50)
\psline[linewidth=0.95](200,30)(200,15)
\rput(130,70){$\EQLS$}
\rput(75,70){$\highunitag$}
\rput[r](48.12,26.88){$\Highprogtype$}
\rput[r](198.12,63.12){$\Lowprogtype$}
\rput(225,70){$\lowunitag$}
\rput[r](198.12,21.88){$\Highprogtype$}
\rput(171.25,15){$\copilertag$}
\psline[linewidth=0.95](165,50)(215,50)
\psline[linewidth=0.95](165,30)(165,10)
\psline[linewidth=0.95](215,30)(215,50)
\psline[linewidth=0.95](185,30)(215,30)
\psline[linewidth=0.95](165,10)(185,10)
\psline[linewidth=0.95](165,30)(185,10)
\psline[linewidth=0.95](175,40)(175,20)
\psline[linewidth=0.95](165,50)(185,30)
\rput(200,40){$\lowunitag$}
\rput[r](157.5,15){\compilernote}
\end{pspicture}


==> PIC/prog-hi-lo.tex <==
%%Created by jPicEdt 1.4.1_03: mixed JPIC-XML/LaTeX format
%%Mon Nov 21 18:17:14 HST 2016
%%Begin JPIC-XML
%<?xml version="1.0" standalone="yes"?>
%<jpic x-min="40" x-max="240" y-min="25" y-max="95" auto-bounding="true">
%<multicurve stroke-width= "0.95"
%	 points= "(40,80);(40,80);(90,80);(90,80)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.95"
%	 points= "(90,60);(90,60);(90,80);(90,80)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.95"
%	 points= "(75,95);(75,95);(75,80);(75,80)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.95"
%	 points= "(60,60);(60,60);(90,60);(90,60)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.95"
%	 points= "(75,60);(75,60);(75,25);(75,25)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.95"
%	 points= "(50,70);(50,70);(50,25);(50,25)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.95"
%	 points= "(40,80);(40,80);(60,60);(60,60)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.95"
%	 points= "(190,80);(190,80);(240,80);(240,80)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.95"
%	 points= "(240,60);(240,60);(240,80);(240,80)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.95"
%	 points= "(225,95);(225,95);(225,80);(225,80)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.95"
%	 points= "(210,60);(210,60);(240,60);(240,60)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.95"
%	 points= "(225,60);(225,60);(225,25);(225,25)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.95"
%	 points= "(190,80);(190,80);(210,60);(210,60)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.95"
%	 points= "(200,70);(200,70);(200,25);(200,25)"
%	 fill-style= "none"
%	 />
%<text text-vert-align= "center-v"
%	 anchor-point= "(75,70)"
%	 text-frame= "noframe"
%	 fill-style= "none"
%	 text-hor-align= "center-h"
%	 >
%$\highunitag$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(48.12,26.88)"
%	 text-frame= "noframe"
%	 fill-style= "none"
%	 text-hor-align= "right"
%	 >
%$\Highprogtype$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(198.12,27.5)"
%	 text-frame= "noframe"
%	 fill-style= "none"
%	 text-hor-align= "right"
%	 >
%$\Lowprogtype$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(225,70)"
%	 text-frame= "noframe"
%	 fill-style= "none"
%	 text-hor-align= "center-h"
%	 >
%$\lowunitag$
%</text>
%</jpic>
%%End JPIC-XML
%PSTricks content-type (pstricks.sty package needed)
%Add \usepackage{pstricks} in the preamble of your LaTeX file
%You can rescale the whole picture (to 80% for instance) by using the command \def\JPicScale{0.8}
\ifx\JPicScale\undefined\def\JPicScale{1}\fi
\psset{unit=\JPicScale mm}
\psset{linewidth=0.3,dotsep=1,hatchwidth=0.3,hatchsep=1.5,shadowsize=1,dimen=middle}
\psset{dotsize=0.7 2.5,dotscale=1 1,fillcolor=black}
\psset{arrowsize=1 2,arrowlength=1,arrowinset=0.25,tbarsize=0.7 5,bracketlength=0.15,rbracketlength=0.15}
\begin{pspicture}(0,0)(240,95)
\psline[linewidth=0.95](40,80)(90,80)
\psline[linewidth=0.95](90,60)(90,80)
\psline[linewidth=0.95](75,95)(75,80)
\psline[linewidth=0.95](60,60)(90,60)
\psline[linewidth=0.95](75,60)(75,25)
\psline[linewidth=0.95](50,70)(50,25)
\psline[linewidth=0.95](40,80)(60,60)
\psline[linewidth=0.95](190,80)(240,80)
\psline[linewidth=0.95](240,60)(240,80)
\psline[linewidth=0.95](225,95)(225,80)
\psline[linewidth=0.95](210,60)(240,60)
\psline[linewidth=0.95](225,60)(225,25)
\psline[linewidth=0.95](190,80)(210,60)
\psline[linewidth=0.95](200,70)(200,25)
\rput(75,70){$\highunitag$}
\rput[r](48.12,26.88){$\Highprogtype$}
\rput[r](198.12,27.5){$\Lowprogtype$}
\rput(225,70){$\lowunitag$}
\end{pspicture}


==> PIC/prog-interpretation.tex <==
%%Created by jPicEdt 1.4.1_03: mixed JPIC-XML/LaTeX format
%%Tue Nov 22 10:56:24 HST 2016
%%Begin JPIC-XML
%<?xml version="1.0" standalone="yes"?>
%<jpic x-min="25" x-max="340" y-min="0" y-max="165" auto-bounding="true">
%<multicurve stroke-width= "0.95"
%	 points= "(30,150);(30,150);(80,150);(80,150)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.95"
%	 points= "(30,130);(30,130);(30,110);(30,110)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.95"
%	 points= "(80,130);(80,130);(80,150);(80,150)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.95"
%	 points= "(65,165);(65,165);(65,150);(65,150)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.95"
%	 points= "(50,130);(50,130);(80,130);(80,130)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.95"
%	 points= "(65,130);(65,130);(65,105);(65,105)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.95"
%	 points= "(30,110);(30,110);(50,110);(50,110)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.95"
%	 points= "(30,130);(30,130);(50,110);(50,110)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.95"
%	 points= "(40,140);(40,140);(40,120);(40,120)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.95"
%	 points= "(30,150);(30,150);(50,130);(50,130)"
%	 fill-style= "none"
%	 />
%<text text-vert-align= "center-v"
%	 stroke-width= "0.95"
%	 anchor-point= "(25,105)"
%	 text-rotation= "45"
%	 text-frame= "noframe"
%	 fill-style= "none"
%	 text-hor-align= "right"
%	 >
%\programnote
%</text>
%<multicurve stroke-width= "0.95"
%	 points= "(155,150);(155,150);(205,150);(205,150)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.95"
%	 points= "(205,130);(205,130);(205,150);(205,150)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.95"
%	 points= "(190,165);(190,165);(190,150);(190,150)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.95"
%	 points= "(175,130);(175,130);(205,130);(205,130)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.95"
%	 points= "(190,130);(190,130);(190,50);(190,50)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.95"
%	 points= "(155,150);(155,150);(175,130);(175,130)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.95"
%	 points= "(130,120);(130,120);(180,120);(180,120)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.95"
%	 points= "(130,100);(130,100);(130,80);(130,80)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.95"
%	 points= "(180,100);(180,100);(180,120);(180,120)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.95"
%	 points= "(165,140);(165,140);(165,120);(165,120)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.95"
%	 points= "(150,100);(150,100);(180,100);(180,100)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.95"
%	 points= "(165,100);(165,100);(165,65);(165,65)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.95"
%	 points= "(130,80);(130,80);(150,80);(150,80)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.95"
%	 points= "(130,100);(130,100);(150,80);(150,80)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.95"
%	 points= "(140,110);(140,110);(140,90);(140,90)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.95"
%	 points= "(130,120);(130,120);(150,100);(150,100)"
%	 fill-style= "none"
%	 />
%<text text-vert-align= "center-v"
%	 stroke-width= "0.95"
%	 anchor-point= "(125,75)"
%	 text-rotation= "45"
%	 text-frame= "noframe"
%	 fill-style= "none"
%	 text-hor-align= "right"
%	 >
%\metaprogramnote
%</text>
%<multicurve stroke-width= "0.95"
%	 points= "(155,75);(155,75);(155,55);(155,55)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.95"
%	 points= "(155,55);(155,55);(175,55);(175,55)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.95"
%	 points= "(155,75);(155,75);(175,55);(175,55)"
%	 fill-style= "none"
%	 />
%<text text-vert-align= "center-v"
%	 anchor-point= "(38.75,133.75)"
%	 text-frame= "noframe"
%	 fill-style= "none"
%	 text-hor-align= "right"
%	 >
%$\Progtype$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(162.5,131.25)"
%	 text-frame= "noframe"
%	 fill-style= "none"
%	 text-hor-align= "right"
%	 >
%$\Progtype$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(162.5,87.5)"
%	 text-frame= "noframe"
%	 fill-style= "none"
%	 text-hor-align= "right"
%	 >
%$\Lprogtype$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(340,150)"
%	 text-frame= "noframe"
%	 fill-style= "none"
%	 text-hor-align= "right"
%	 >
%$\Hprogtype$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(150,50)"
%	 text-rotation= "45"
%	 text-frame= "noframe"
%	 fill-style= "none"
%	 text-hor-align= "right"
%	 >
%\lprogramnote
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(285,0)"
%	 text-rotation= "45"
%	 text-frame= "noframe"
%	 fill-style= "none"
%	 text-hor-align= "right"
%	 >
%\hprogramnote
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(160,60)"
%	 text-frame= "noframe"
%	 fill-style= "none"
%	 text-hor-align= "center-h"
%	 >
%$\ltag$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(135,85)"
%	 text-frame= "noframe"
%	 fill-style= "none"
%	 text-hor-align= "center-h"
%	 >
%$\itag$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(35,115)"
%	 text-frame= "noframe"
%	 fill-style= "none"
%	 text-hor-align= "center-h"
%	 >
%$\mtag$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(110,140)"
%	 text-frame= "noframe"
%	 fill-style= "none"
%	 text-hor-align= "center-h"
%	 >
%\EQLS
%</text>
%</jpic>
%%End JPIC-XML
%PSTricks content-type (pstricks.sty package needed)
%Add \usepackage{pstricks} in the preamble of your LaTeX file
%You can rescale the whole picture (to 80% for instance) by using the command \def\JPicScale{0.8}
\ifx\JPicScale\undefined\def\JPicScale{1}\fi
\psset{unit=\JPicScale mm}
\psset{linewidth=0.3,dotsep=1,hatchwidth=0.3,hatchsep=1.5,shadowsize=1,dimen=middle}
\psset{dotsize=0.7 2.5,dotscale=1 1,fillcolor=black}
\psset{arrowsize=1 2,arrowlength=1,arrowinset=0.25,tbarsize=0.7 5,bracketlength=0.15,rbracketlength=0.15}
\begin{pspicture}(0,0)(340,165)
\psline[linewidth=0.95](30,150)(80,150)
\psline[linewidth=0.95](30,130)(30,110)
\psline[linewidth=0.95](80,130)(80,150)
\psline[linewidth=0.95](65,165)(65,150)
\psline[linewidth=0.95](50,130)(80,130)
\psline[linewidth=0.95](65,130)(65,105)
\psline[linewidth=0.95](30,110)(50,110)
\psline[linewidth=0.95](30,130)(50,110)
\psline[linewidth=0.95](40,140)(40,120)
\psline[linewidth=0.95](30,150)(50,130)
\rput[r]{45}(25,105){\programnote}
\psline[linewidth=0.95](155,150)(205,150)
\psline[linewidth=0.95](205,130)(205,150)
\psline[linewidth=0.95](190,165)(190,150)
\psline[linewidth=0.95](175,130)(205,130)
\psline[linewidth=0.95](190,130)(190,50)
\psline[linewidth=0.95](155,150)(175,130)
\psline[linewidth=0.95](130,120)(180,120)
\psline[linewidth=0.95](130,100)(130,80)
\psline[linewidth=0.95](180,100)(180,120)
\psline[linewidth=0.95](165,140)(165,120)
\psline[linewidth=0.95](150,100)(180,100)
\psline[linewidth=0.95](165,100)(165,65)
\psline[linewidth=0.95](130,80)(150,80)
\psline[linewidth=0.95](130,100)(150,80)
\psline[linewidth=0.95](140,110)(140,90)
\psline[linewidth=0.95](130,120)(150,100)
\rput[r]{45}(125,75){\metaprogramnote}
\psline[linewidth=0.95](155,75)(155,55)
\psline[linewidth=0.95](155,55)(175,55)
\psline[linewidth=0.95](155,75)(175,55)
\rput[r](38.75,133.75){$\Progtype$}
\rput[r](162.5,131.25){$\Progtype$}
\rput[r](162.5,87.5){$\Lprogtype$}
\rput[r](340,150){$\Hprogtype$}
\rput[r]{45}(150,50){\lprogramnote}
\rput[r]{45}(285,0){\hprogramnote}
\rput(160,60){$\ltag$}
\rput(135,85){$\itag$}
\rput(35,115){$\mtag$}
\rput(110,140){\EQLS}
\end{pspicture}


==> PIC/prog-interpreter-compiler-slant.tex <==
%%Created by jPicEdt 1.4.1_03: mixed JPIC-XML/LaTeX format
%%Tue Nov 22 10:42:10 HST 2016
%%Begin JPIC-XML
%<?xml version="1.0" standalone="yes"?>
%<jpic x-min="25" x-max="340" y-min="0" y-max="165" auto-bounding="true">
%<multicurve stroke-width= "0.95"
%	 points= "(30,150);(30,150);(80,150);(80,150)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.95"
%	 points= "(30,130);(30,130);(30,110);(30,110)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.95"
%	 points= "(80,130);(80,130);(80,150);(80,150)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.95"
%	 points= "(65,165);(65,165);(65,150);(65,150)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.95"
%	 points= "(50,130);(50,130);(80,130);(80,130)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.95"
%	 points= "(65,130);(65,130);(65,105);(65,105)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.95"
%	 points= "(30,110);(30,110);(50,110);(50,110)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.95"
%	 points= "(30,130);(30,130);(50,110);(50,110)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.95"
%	 points= "(40,140);(40,140);(40,120);(40,120)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.95"
%	 points= "(30,150);(30,150);(50,130);(50,130)"
%	 fill-style= "none"
%	 />
%<text text-vert-align= "center-v"
%	 stroke-width= "0.95"
%	 anchor-point= "(25,105)"
%	 text-rotation= "45"
%	 text-frame= "noframe"
%	 fill-style= "none"
%	 text-hor-align= "right"
%	 >
%\programnote
%</text>
%<multicurve stroke-width= "0.95"
%	 points= "(155,150);(155,150);(205,150);(205,150)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.95"
%	 points= "(205,130);(205,130);(205,150);(205,150)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.95"
%	 points= "(190,165);(190,165);(190,150);(190,150)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.95"
%	 points= "(175,130);(175,130);(205,130);(205,130)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.95"
%	 points= "(190,130);(190,130);(190,50);(190,50)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.95"
%	 points= "(155,150);(155,150);(175,130);(175,130)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.95"
%	 points= "(130,120);(130,120);(180,120);(180,120)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.95"
%	 points= "(130,100);(130,100);(130,80);(130,80)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.95"
%	 points= "(180,100);(180,100);(180,120);(180,120)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.95"
%	 points= "(165,140);(165,140);(165,120);(165,120)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.95"
%	 points= "(150,100);(150,100);(180,100);(180,100)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.95"
%	 points= "(165,100);(165,100);(165,65);(165,65)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.95"
%	 points= "(130,80);(130,80);(150,80);(150,80)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.95"
%	 points= "(130,100);(130,100);(150,80);(150,80)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.95"
%	 points= "(140,110);(140,110);(140,90);(140,90)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.95"
%	 points= "(130,120);(130,120);(150,100);(150,100)"
%	 fill-style= "none"
%	 />
%<text text-vert-align= "center-v"
%	 stroke-width= "0.95"
%	 anchor-point= "(125,75)"
%	 text-rotation= "45"
%	 text-frame= "noframe"
%	 fill-style= "none"
%	 text-hor-align= "right"
%	 >
%\metaprogramnote
%</text>
%<multicurve stroke-width= "0.95"
%	 points= "(290,150);(290,150);(340,150);(340,150)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.95"
%	 points= "(340,130);(340,130);(340,150);(340,150)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.95"
%	 points= "(325,165);(325,165);(325,150);(325,150)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.95"
%	 points= "(310,130);(310,130);(340,130);(340,130)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.95"
%	 points= "(325,130);(325,130);(325,0);(325,0)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.95"
%	 points= "(290,150);(290,150);(310,130);(310,130)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.95"
%	 points= "(265,120);(265,120);(315,120);(315,120)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.95"
%	 points= "(265,100);(265,100);(265,80);(265,80)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.95"
%	 points= "(315,100);(315,100);(315,120);(315,120)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.95"
%	 points= "(300,140);(300,140);(300,120);(300,120)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.95"
%	 points= "(285,100);(285,100);(315,100);(315,100)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.95"
%	 points= "(300,100);(300,100);(300,70);(300,70)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.95"
%	 points= "(265,80);(265,80);(285,80);(285,80)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.95"
%	 points= "(265,100);(265,100);(285,80);(285,80)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.95"
%	 points= "(275,110);(275,110);(275,90);(275,90)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.95"
%	 points= "(265,120);(265,120);(285,100);(285,100)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.95"
%	 points= "(155,75);(155,75);(155,55);(155,55)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.95"
%	 points= "(155,55);(155,55);(175,55);(175,55)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.95"
%	 points= "(155,75);(155,75);(175,55);(175,55)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.95"
%	 points= "(265,70);(265,70);(315,70);(315,70)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.95"
%	 points= "(265,50);(265,50);(265,30);(265,30)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.95"
%	 points= "(315,50);(315,50);(315,70);(315,70)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.95"
%	 points= "(285,50);(285,50);(315,50);(315,50)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.95"
%	 points= "(300,50);(300,50);(300,15);(300,15)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.95"
%	 points= "(265,30);(265,30);(285,30);(285,30)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.95"
%	 points= "(265,50);(265,50);(285,30);(285,30)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.95"
%	 points= "(275,60);(275,60);(275,40);(275,40)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.95"
%	 points= "(265,70);(265,70);(285,50);(285,50)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.95"
%	 points= "(290,25);(290,25);(290,5);(290,5)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.95"
%	 points= "(290,5);(290,5);(310,5);(310,5)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.95"
%	 points= "(290,25);(290,25);(310,5);(310,5)"
%	 fill-style= "none"
%	 />
%<text text-vert-align= "center-v"
%	 anchor-point= "(38.75,133.75)"
%	 text-frame= "noframe"
%	 fill-style= "none"
%	 text-hor-align= "right"
%	 >
%$\Progtype$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(162.5,131.25)"
%	 text-frame= "noframe"
%	 fill-style= "none"
%	 text-hor-align= "right"
%	 >
%$\Progtype$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(297.5,131.25)"
%	 text-frame= "noframe"
%	 fill-style= "none"
%	 text-hor-align= "right"
%	 >
%$\Progtype$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(162.5,87.5)"
%	 text-frame= "noframe"
%	 fill-style= "none"
%	 text-hor-align= "right"
%	 >
%$\Lprogtype$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(297.5,87.5)"
%	 text-frame= "noframe"
%	 fill-style= "none"
%	 text-hor-align= "right"
%	 >
%$\Lprogtype$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(297.5,38.75)"
%	 text-frame= "noframe"
%	 fill-style= "none"
%	 text-hor-align= "right"
%	 >
%$\Hprogtype$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(150,50)"
%	 text-rotation= "45"
%	 text-frame= "noframe"
%	 fill-style= "none"
%	 text-hor-align= "right"
%	 >
%\lprogramnote
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(285,0)"
%	 text-rotation= "45"
%	 text-frame= "noframe"
%	 fill-style= "none"
%	 text-hor-align= "right"
%	 >
%\hprogramnote
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(260,25)"
%	 text-rotation= "45"
%	 text-frame= "noframe"
%	 fill-style= "none"
%	 text-hor-align= "right"
%	 >
%\compilernote
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(160,60)"
%	 text-frame= "noframe"
%	 fill-style= "none"
%	 text-hor-align= "center-h"
%	 >
%$\ltag$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(295,10)"
%	 text-frame= "noframe"
%	 fill-style= "none"
%	 text-hor-align= "center-h"
%	 >
%$\htag$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(270,35)"
%	 text-frame= "noframe"
%	 fill-style= "none"
%	 text-hor-align= "center-h"
%	 >
%$\ctag$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(135,85)"
%	 text-frame= "noframe"
%	 fill-style= "none"
%	 text-hor-align= "center-h"
%	 >
%$\itag$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(35,115)"
%	 text-frame= "noframe"
%	 fill-style= "none"
%	 text-hor-align= "center-h"
%	 >
%$\mtag$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(110,140)"
%	 text-frame= "noframe"
%	 fill-style= "none"
%	 text-hor-align= "center-h"
%	 >
%\EQLS
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(245,140)"
%	 text-frame= "noframe"
%	 fill-style= "none"
%	 text-hor-align= "center-h"
%	 >
%\EQLS
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(270,85)"
%	 text-frame= "noframe"
%	 fill-style= "none"
%	 text-hor-align= "center-h"
%	 >
%$\itag$
%</text>
%</jpic>
%%End JPIC-XML
%PSTricks content-type (pstricks.sty package needed)
%Add \usepackage{pstricks} in the preamble of your LaTeX file
%You can rescale the whole picture (to 80% for instance) by using the command \def\JPicScale{0.8}
\ifx\JPicScale\undefined\def\JPicScale{1}\fi
\psset{unit=\JPicScale mm}
\psset{linewidth=0.3,dotsep=1,hatchwidth=0.3,hatchsep=1.5,shadowsize=1,dimen=middle}
\psset{dotsize=0.7 2.5,dotscale=1 1,fillcolor=black}
\psset{arrowsize=1 2,arrowlength=1,arrowinset=0.25,tbarsize=0.7 5,bracketlength=0.15,rbracketlength=0.15}
\begin{pspicture}(0,0)(340,165)
\psline[linewidth=0.95](30,150)(80,150)
\psline[linewidth=0.95](30,130)(30,110)
\psline[linewidth=0.95](80,130)(80,150)
\psline[linewidth=0.95](65,165)(65,150)
\psline[linewidth=0.95](50,130)(80,130)
\psline[linewidth=0.95](65,130)(65,105)
\psline[linewidth=0.95](30,110)(50,110)
\psline[linewidth=0.95](30,130)(50,110)
\psline[linewidth=0.95](40,140)(40,120)
\psline[linewidth=0.95](30,150)(50,130)
\rput[r]{45}(25,105){\programnote}
\psline[linewidth=0.95](155,150)(205,150)
\psline[linewidth=0.95](205,130)(205,150)
\psline[linewidth=0.95](190,165)(190,150)
\psline[linewidth=0.95](175,130)(205,130)
\psline[linewidth=0.95](190,130)(190,50)
\psline[linewidth=0.95](155,150)(175,130)
\psline[linewidth=0.95](130,120)(180,120)
\psline[linewidth=0.95](130,100)(130,80)
\psline[linewidth=0.95](180,100)(180,120)
\psline[linewidth=0.95](165,140)(165,120)
\psline[linewidth=0.95](150,100)(180,100)
\psline[linewidth=0.95](165,100)(165,65)
\psline[linewidth=0.95](130,80)(150,80)
\psline[linewidth=0.95](130,100)(150,80)
\psline[linewidth=0.95](140,110)(140,90)
\psline[linewidth=0.95](130,120)(150,100)
\rput[r]{45}(125,75){\metaprogramnote}
\psline[linewidth=0.95](290,150)(340,150)
\psline[linewidth=0.95](340,130)(340,150)
\psline[linewidth=0.95](325,165)(325,150)
\psline[linewidth=0.95](310,130)(340,130)
\psline[linewidth=0.95](325,130)(325,0)
\psline[linewidth=0.95](290,150)(310,130)
\psline[linewidth=0.95](265,120)(315,120)
\psline[linewidth=0.95](265,100)(265,80)
\psline[linewidth=0.95](315,100)(315,120)
\psline[linewidth=0.95](300,140)(300,120)
\psline[linewidth=0.95](285,100)(315,100)
\psline[linewidth=0.95](300,100)(300,70)
\psline[linewidth=0.95](265,80)(285,80)
\psline[linewidth=0.95](265,100)(285,80)
\psline[linewidth=0.95](275,110)(275,90)
\psline[linewidth=0.95](265,120)(285,100)
\psline[linewidth=0.95](155,75)(155,55)
\psline[linewidth=0.95](155,55)(175,55)
\psline[linewidth=0.95](155,75)(175,55)
\psline[linewidth=0.95](265,70)(315,70)
\psline[linewidth=0.95](265,50)(265,30)
\psline[linewidth=0.95](315,50)(315,70)
\psline[linewidth=0.95](285,50)(315,50)
\psline[linewidth=0.95](300,50)(300,15)
\psline[linewidth=0.95](265,30)(285,30)
\psline[linewidth=0.95](265,50)(285,30)
\psline[linewidth=0.95](275,60)(275,40)
\psline[linewidth=0.95](265,70)(285,50)
\psline[linewidth=0.95](290,25)(290,5)
\psline[linewidth=0.95](290,5)(310,5)
\psline[linewidth=0.95](290,25)(310,5)
\rput[r](38.75,133.75){$\Progtype$}
\rput[r](162.5,131.25){$\Progtype$}
\rput[r](297.5,131.25){$\Progtype$}
\rput[r](162.5,87.5){$\Lprogtype$}
\rput[r](297.5,87.5){$\Lprogtype$}
\rput[r](297.5,38.75){$\Hprogtype$}
\rput[r]{45}(150,50){\lprogramnote}
\rput[r]{45}(285,0){\hprogramnote}
\rput[r]{45}(260,25){\compilernote}
\rput(160,60){$\ltag$}
\rput(295,10){$\htag$}
\rput(270,35){$\ctag$}
\rput(135,85){$\itag$}
\rput(35,115){$\mtag$}
\rput(110,140){\EQLS}
\rput(245,140){\EQLS}
\rput(270,85){$\itag$}
\end{pspicture}


==> PIC/prog-interpreter-compiler.tex <==
%%Created by jPicEdt 1.4.1_03: mixed JPIC-XML/LaTeX format
%%Tue Nov 22 10:40:49 HST 2016
%%Begin JPIC-XML
%<?xml version="1.0" standalone="yes"?>
%<jpic x-min="25" x-max="340" y-min="0" y-max="165" auto-bounding="true">
%<multicurve stroke-width= "0.95"
%	 points= "(30,150);(30,150);(80,150);(80,150)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.95"
%	 points= "(30,130);(30,130);(30,110);(30,110)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.95"
%	 points= "(80,130);(80,130);(80,150);(80,150)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.95"
%	 points= "(65,165);(65,165);(65,150);(65,150)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.95"
%	 points= "(50,130);(50,130);(80,130);(80,130)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.95"
%	 points= "(65,130);(65,130);(65,105);(65,105)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.95"
%	 points= "(30,110);(30,110);(50,110);(50,110)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.95"
%	 points= "(30,130);(30,130);(50,110);(50,110)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.95"
%	 points= "(40,140);(40,140);(40,120);(40,120)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.95"
%	 points= "(30,150);(30,150);(50,130);(50,130)"
%	 fill-style= "none"
%	 />
%<text text-vert-align= "center-v"
%	 stroke-width= "0.95"
%	 anchor-point= "(25,115)"
%	 text-frame= "noframe"
%	 fill-style= "none"
%	 text-hor-align= "right"
%	 >
%\programnote
%</text>
%<multicurve stroke-width= "0.95"
%	 points= "(155,150);(155,150);(205,150);(205,150)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.95"
%	 points= "(205,130);(205,130);(205,150);(205,150)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.95"
%	 points= "(190,165);(190,165);(190,150);(190,150)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.95"
%	 points= "(175,130);(175,130);(205,130);(205,130)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.95"
%	 points= "(190,130);(190,130);(190,50);(190,50)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.95"
%	 points= "(155,150);(155,150);(175,130);(175,130)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.95"
%	 points= "(130,120);(130,120);(180,120);(180,120)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.95"
%	 points= "(130,100);(130,100);(130,80);(130,80)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.95"
%	 points= "(180,100);(180,100);(180,120);(180,120)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.95"
%	 points= "(165,140);(165,140);(165,120);(165,120)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.95"
%	 points= "(150,100);(150,100);(180,100);(180,100)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.95"
%	 points= "(165,100);(165,100);(165,65);(165,65)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.95"
%	 points= "(130,80);(130,80);(150,80);(150,80)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.95"
%	 points= "(130,100);(130,100);(150,80);(150,80)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.95"
%	 points= "(140,110);(140,110);(140,90);(140,90)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.95"
%	 points= "(130,120);(130,120);(150,100);(150,100)"
%	 fill-style= "none"
%	 />
%<text text-vert-align= "center-v"
%	 stroke-width= "0.95"
%	 anchor-point= "(125,85)"
%	 text-frame= "noframe"
%	 fill-style= "none"
%	 text-hor-align= "right"
%	 >
%\metaprogramnote
%</text>
%<multicurve stroke-width= "0.95"
%	 points= "(290,150);(290,150);(340,150);(340,150)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.95"
%	 points= "(340,130);(340,130);(340,150);(340,150)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.95"
%	 points= "(325,165);(325,165);(325,150);(325,150)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.95"
%	 points= "(310,130);(310,130);(340,130);(340,130)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.95"
%	 points= "(325,130);(325,130);(325,0);(325,0)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.95"
%	 points= "(290,150);(290,150);(310,130);(310,130)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.95"
%	 points= "(265,120);(265,120);(315,120);(315,120)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.95"
%	 points= "(265,100);(265,100);(265,80);(265,80)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.95"
%	 points= "(315,100);(315,100);(315,120);(315,120)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.95"
%	 points= "(300,140);(300,140);(300,120);(300,120)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.95"
%	 points= "(285,100);(285,100);(315,100);(315,100)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.95"
%	 points= "(300,100);(300,100);(300,70);(300,70)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.95"
%	 points= "(265,80);(265,80);(285,80);(285,80)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.95"
%	 points= "(265,100);(265,100);(285,80);(285,80)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.95"
%	 points= "(275,110);(275,110);(275,90);(275,90)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.95"
%	 points= "(265,120);(265,120);(285,100);(285,100)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.95"
%	 points= "(155,75);(155,75);(155,55);(155,55)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.95"
%	 points= "(155,55);(155,55);(175,55);(175,55)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.95"
%	 points= "(155,75);(155,75);(175,55);(175,55)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.95"
%	 points= "(265,70);(265,70);(315,70);(315,70)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.95"
%	 points= "(265,50);(265,50);(265,30);(265,30)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.95"
%	 points= "(315,50);(315,50);(315,70);(315,70)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.95"
%	 points= "(285,50);(285,50);(315,50);(315,50)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.95"
%	 points= "(300,50);(300,50);(300,15);(300,15)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.95"
%	 points= "(265,30);(265,30);(285,30);(285,30)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.95"
%	 points= "(265,50);(265,50);(285,30);(285,30)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.95"
%	 points= "(275,60);(275,60);(275,40);(275,40)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.95"
%	 points= "(265,70);(265,70);(285,50);(285,50)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.95"
%	 points= "(290,25);(290,25);(290,5);(290,5)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.95"
%	 points= "(290,5);(290,5);(310,5);(310,5)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.95"
%	 points= "(290,25);(290,25);(310,5);(310,5)"
%	 fill-style= "none"
%	 />
%<text text-vert-align= "center-v"
%	 anchor-point= "(38.75,133.75)"
%	 text-frame= "noframe"
%	 fill-style= "none"
%	 text-hor-align= "right"
%	 >
%$\Progtype$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(162.5,131.25)"
%	 text-frame= "noframe"
%	 fill-style= "none"
%	 text-hor-align= "right"
%	 >
%$\Progtype$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(297.5,131.25)"
%	 text-frame= "noframe"
%	 fill-style= "none"
%	 text-hor-align= "right"
%	 >
%$\Progtype$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(162.5,87.5)"
%	 text-frame= "noframe"
%	 fill-style= "none"
%	 text-hor-align= "right"
%	 >
%$\Lprogtype$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(297.5,87.5)"
%	 text-frame= "noframe"
%	 fill-style= "none"
%	 text-hor-align= "right"
%	 >
%$\Lprogtype$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(297.5,38.75)"
%	 text-frame= "noframe"
%	 fill-style= "none"
%	 text-hor-align= "right"
%	 >
%$\Hprogtype$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(150,65)"
%	 text-frame= "noframe"
%	 fill-style= "none"
%	 text-hor-align= "right"
%	 >
%\lprogramnote
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(285,10)"
%	 text-frame= "noframe"
%	 fill-style= "none"
%	 text-hor-align= "right"
%	 >
%\hprogramnote
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(260,40)"
%	 text-frame= "noframe"
%	 fill-style= "none"
%	 text-hor-align= "right"
%	 >
%\compilernote
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(160,60)"
%	 text-frame= "noframe"
%	 fill-style= "none"
%	 text-hor-align= "center-h"
%	 >
%$\ltag$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(295,10)"
%	 text-frame= "noframe"
%	 fill-style= "none"
%	 text-hor-align= "center-h"
%	 >
%$\htag$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(270,35)"
%	 text-frame= "noframe"
%	 fill-style= "none"
%	 text-hor-align= "center-h"
%	 >
%$\ctag$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(135,85)"
%	 text-frame= "noframe"
%	 fill-style= "none"
%	 text-hor-align= "center-h"
%	 >
%$\itag$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(35,115)"
%	 text-frame= "noframe"
%	 fill-style= "none"
%	 text-hor-align= "center-h"
%	 >
%$\mtag$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(110,140)"
%	 text-frame= "noframe"
%	 fill-style= "none"
%	 text-hor-align= "center-h"
%	 >
%\EQLS
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(245,140)"
%	 text-frame= "noframe"
%	 fill-style= "none"
%	 text-hor-align= "center-h"
%	 >
%\EQLS
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(270,85)"
%	 text-frame= "noframe"
%	 fill-style= "none"
%	 text-hor-align= "center-h"
%	 >
%$\itag$
%</text>
%</jpic>
%%End JPIC-XML
%PSTricks content-type (pstricks.sty package needed)
%Add \usepackage{pstricks} in the preamble of your LaTeX file
%You can rescale the whole picture (to 80% for instance) by using the command \def\JPicScale{0.8}
\ifx\JPicScale\undefined\def\JPicScale{1}\fi
\psset{unit=\JPicScale mm}
\psset{linewidth=0.3,dotsep=1,hatchwidth=0.3,hatchsep=1.5,shadowsize=1,dimen=middle}
\psset{dotsize=0.7 2.5,dotscale=1 1,fillcolor=black}
\psset{arrowsize=1 2,arrowlength=1,arrowinset=0.25,tbarsize=0.7 5,bracketlength=0.15,rbracketlength=0.15}
\begin{pspicture}(0,0)(340,165)
\psline[linewidth=0.95](30,150)(80,150)
\psline[linewidth=0.95](30,130)(30,110)
\psline[linewidth=0.95](80,130)(80,150)
\psline[linewidth=0.95](65,165)(65,150)
\psline[linewidth=0.95](50,130)(80,130)
\psline[linewidth=0.95](65,130)(65,105)
\psline[linewidth=0.95](30,110)(50,110)
\psline[linewidth=0.95](30,130)(50,110)
\psline[linewidth=0.95](40,140)(40,120)
\psline[linewidth=0.95](30,150)(50,130)
\rput[r](25,115){\programnote}
\psline[linewidth=0.95](155,150)(205,150)
\psline[linewidth=0.95](205,130)(205,150)
\psline[linewidth=0.95](190,165)(190,150)
\psline[linewidth=0.95](175,130)(205,130)
\psline[linewidth=0.95](190,130)(190,50)
\psline[linewidth=0.95](155,150)(175,130)
\psline[linewidth=0.95](130,120)(180,120)
\psline[linewidth=0.95](130,100)(130,80)
\psline[linewidth=0.95](180,100)(180,120)
\psline[linewidth=0.95](165,140)(165,120)
\psline[linewidth=0.95](150,100)(180,100)
\psline[linewidth=0.95](165,100)(165,65)
\psline[linewidth=0.95](130,80)(150,80)
\psline[linewidth=0.95](130,100)(150,80)
\psline[linewidth=0.95](140,110)(140,90)
\psline[linewidth=0.95](130,120)(150,100)
\rput[r](125,85){\metaprogramnote}
\psline[linewidth=0.95](290,150)(340,150)
\psline[linewidth=0.95](340,130)(340,150)
\psline[linewidth=0.95](325,165)(325,150)
\psline[linewidth=0.95](310,130)(340,130)
\psline[linewidth=0.95](325,130)(325,0)
\psline[linewidth=0.95](290,150)(310,130)
\psline[linewidth=0.95](265,120)(315,120)
\psline[linewidth=0.95](265,100)(265,80)
\psline[linewidth=0.95](315,100)(315,120)
\psline[linewidth=0.95](300,140)(300,120)
\psline[linewidth=0.95](285,100)(315,100)
\psline[linewidth=0.95](300,100)(300,70)
\psline[linewidth=0.95](265,80)(285,80)
\psline[linewidth=0.95](265,100)(285,80)
\psline[linewidth=0.95](275,110)(275,90)
\psline[linewidth=0.95](265,120)(285,100)
\psline[linewidth=0.95](155,75)(155,55)
\psline[linewidth=0.95](155,55)(175,55)
\psline[linewidth=0.95](155,75)(175,55)
\psline[linewidth=0.95](265,70)(315,70)
\psline[linewidth=0.95](265,50)(265,30)
\psline[linewidth=0.95](315,50)(315,70)
\psline[linewidth=0.95](285,50)(315,50)
\psline[linewidth=0.95](300,50)(300,15)
\psline[linewidth=0.95](265,30)(285,30)
\psline[linewidth=0.95](265,50)(285,30)
\psline[linewidth=0.95](275,60)(275,40)
\psline[linewidth=0.95](265,70)(285,50)
\psline[linewidth=0.95](290,25)(290,5)
\psline[linewidth=0.95](290,5)(310,5)
\psline[linewidth=0.95](290,25)(310,5)
\rput[r](38.75,133.75){$\Progtype$}
\rput[r](162.5,131.25){$\Progtype$}
\rput[r](297.5,131.25){$\Progtype$}
\rput[r](162.5,87.5){$\Lprogtype$}
\rput[r](297.5,87.5){$\Lprogtype$}
\rput[r](297.5,38.75){$\Hprogtype$}
\rput[r](150,65){\lprogramnote}
\rput[r](285,10){\hprogramnote}
\rput[r](260,40){\compilernote}
\rput(160,60){$\ltag$}
\rput(295,10){$\htag$}
\rput(270,35){$\ctag$}
\rput(135,85){$\itag$}
\rput(35,115){$\mtag$}
\rput(110,140){\EQLS}
\rput(245,140){\EQLS}
\rput(270,85){$\itag$}
\end{pspicture}


==> PIC/prog-mach-beh-lang.tex <==
%%Created by jPicEdt 1.4.1_03: mixed JPIC-XML/LaTeX format
%%Tue Jan 10 19:17:56 GMT 2012
%%Begin JPIC-XML
%<?xml version="1.0" standalone="yes"?>
%<jpic x-min="20" x-max="50" y-min="0" y-max="60" auto-bounding="true">
%<text text-vert-align= "center-v"
%	 anchor-point= "(20,40)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\Machines
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(20,20)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\Behaviors
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(20,0)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\Languages
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(50,40)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\Measures
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(20,60)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\Programs
%</text>
%</jpic>
%%End JPIC-XML
%PSTricks content-type (pstricks.sty package needed)
%Add \usepackage{pstricks} in the preamble of your LaTeX file
%You can rescale the whole picture (to 80% for instance) by using the command \def\JPicScale{0.8}
\ifx\JPicScale\undefined\def\JPicScale{1}\fi
\psset{unit=\JPicScale mm}
\psset{linewidth=0.3,dotsep=1,hatchwidth=0.3,hatchsep=1.5,shadowsize=1,dimen=middle}
\psset{dotsize=0.7 2.5,dotscale=1 1,fillcolor=black}
\psset{arrowsize=1 2,arrowlength=1,arrowinset=0.25,tbarsize=0.7 5,bracketlength=0.15,rbracketlength=0.15}
\begin{pspicture}(0,0)(50,60)
\rput(20,40){\Machines}
\rput(20,20){\Behaviors}
\rput(20,0){\Languages}
\rput(50,40){\Measures}
\rput(20,60){\Programs}
\end{pspicture}


==> PIC/prog-mach-lang-down.tex <==
%%Created by jPicEdt 1.4.1_03: mixed JPIC-XML/LaTeX format
%%Wed Jan 25 11:00:47 GMT 2012
%%Begin JPIC-XML
%<?xml version="1.0" standalone="yes"?>
%<jpic x-min="5" x-max="23" y-min="0" y-max="70" auto-bounding="true">
%<text text-vert-align= "center-v"
%	 anchor-point= "(5,35)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%\Machines
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(8,0)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%\Behaviors
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(5,70)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%\Programs
%</text>
%<multicurve arrow-head-length-scale= "2"
%	 right-arrow= "head"
%	 fill-style= "none"
%	 points= "(20,32);(20,32);(20,2.5);(20,2.5)"
%	 stroke-width= "0.4"
%	 arrow-head-width-minimum= "1.05"
%	 />
%<text text-vert-align= "center-v"
%	 anchor-point= "(21,17)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\accept$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(23,52)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\enc$
%</text>
%<multicurve arrow-head-length-scale= "2"
%	 right-arrow= "head"
%	 fill-style= "none"
%	 points= "(22,39.5);(22,39.5);(22,66);(22,66)"
%	 stroke-width= "0.4"
%	 arrow-head-width-minimum= "1.05"
%	 />
%<multicurve arrow-head-length-scale= "2"
%	 right-arrow= "head"
%	 fill-style= "none"
%	 points= "(18,66);(18,66);(18,39);(18,39)"
%	 stroke-width= "0.4"
%	 arrow-head-width-minimum= "1.05"
%	 />
%<text text-vert-align= "center-v"
%	 anchor-point= "(17,53)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\dec$
%</text>
%</jpic>
%%End JPIC-XML
%PSTricks content-type (pstricks.sty package needed)
%Add \usepackage{pstricks} in the preamble of your LaTeX file
%You can rescale the whole picture (to 80% for instance) by using the command \def\JPicScale{0.8}
\ifx\JPicScale\undefined\def\JPicScale{1}\fi
\psset{unit=\JPicScale mm}
\psset{linewidth=0.3,dotsep=1,hatchwidth=0.3,hatchsep=1.5,shadowsize=1,dimen=middle}
\psset{dotsize=0.7 2.5,dotscale=1 1,fillcolor=black}
\psset{arrowsize=1 2,arrowlength=1,arrowinset=0.25,tbarsize=0.7 5,bracketlength=0.15,rbracketlength=0.15}
\begin{pspicture}(0,0)(23,70)
\rput[l](5,35){\Machines}
\rput[l](8,0){\Behaviors}
\rput[l](5,70){\Programs}
\psline[linewidth=0.4,arrowsize=1.05 2,arrowlength=2]{->}(20,32)(20,2.5)
\rput[l](21,17){$\accept$}
\rput[l](23,52){$\enc$}
\psline[linewidth=0.4,arrowsize=1.05 2,arrowlength=2]{->}(22,39.5)(22,66)
\psline[linewidth=0.4,arrowsize=1.05 2,arrowlength=2]{->}(18,66)(18,39)
\rput[r](17,53){$\dec$}
\end{pspicture}


==> PIC/prog-mach-lang-noline.tex <==
%%Created by jPicEdt 1.4.1_03: mixed JPIC-XML/LaTeX format
%%Sat Jan 14 18:16:38 GMT 2012
%%Begin JPIC-XML
%<?xml version="1.0" standalone="yes"?>
%<jpic x-min="5" x-max="22" y-min="0" y-max="70" auto-bounding="true">
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(5,35)"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%\Machines
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(7,0)"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%\Behaviors
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(5,70)"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%\Programs
%</text>
%<multicurve stroke-width= "0.4"
%	 arrow-head-width-minimum= "1.05"
%	 fill-style= "none"
%	 arrow-head-length-scale= "2"
%	 points= "(20,32);(20,32);(20,2.5);(20,2.5)"
%	 right-arrow= "head"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(21,13)"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\accept$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(22,52)"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\enc$
%</text>
%</jpic>
%%End JPIC-XML
%PSTricks content-type (pstricks.sty package needed)
%Add \usepackage{pstricks} in the preamble of your LaTeX file
%You can rescale the whole picture (to 80% for instance) by using the command \def\JPicScale{0.8}
\ifx\JPicScale\undefined\def\JPicScale{1}\fi
\psset{unit=\JPicScale mm}
\psset{linewidth=0.3,dotsep=1,hatchwidth=0.3,hatchsep=1.5,shadowsize=1,dimen=middle}
\psset{dotsize=0.7 2.5,dotscale=1 1,fillcolor=black}
\psset{arrowsize=1 2,arrowlength=1,arrowinset=0.25,tbarsize=0.7 5,bracketlength=0.15,rbracketlength=0.15}
\begin{pspicture}(0,0)(22,70)
\rput[l](5,35){\Machines}
\rput[l](7,0){\Behaviors}
\rput[l](5,70){\Programs}
\psline[linewidth=0.4,arrowsize=1.05 2,arrowlength=2]{->}(20,32)(20,2.5)
\rput[l](21,13){$\accept$}
\rput[l](22,52){$\enc$}
\end{pspicture}


==> PIC/prog-mach-lang.tex <==
%%Created by jPicEdt 1.4.1_03: mixed JPIC-XML/LaTeX format
%%Sat Jan 14 18:16:38 GMT 2012
%%Begin JPIC-XML
%<?xml version="1.0" standalone="yes"?>
%<jpic x-min="5" x-max="22" y-min="0" y-max="70" auto-bounding="true">
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(5,35)"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%\Machines
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(8,0)"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%\Behaviors
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(5,70)"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%\Programs
%</text>
%<multicurve stroke-width= "0.4"
%	 arrow-head-width-minimum= "1.05"
%	 fill-style= "none"
%	 arrow-head-length-scale= "2"
%	 points= "(20,32);(20,32);(20,2.5);(20,2.5)"
%	 right-arrow= "head"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(21,17)"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\accept$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(22,52)"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\enc$
%</text>
%<multicurve stroke-width= "0.4"
%	 arrow-head-width-minimum= "1.05"
%	 fill-style= "none"
%	 arrow-head-length-scale= "2"
%	 points= "(20,39.5);(20,39.5);(20,66);(20,66)"
%	 right-arrow= "head"
%	 />
%</jpic>
%%End JPIC-XML
%PSTricks content-type (pstricks.sty package needed)
%Add \usepackage{pstricks} in the preamble of your LaTeX file
%You can rescale the whole picture (to 80% for instance) by using the command \def\JPicScale{0.8}
\ifx\JPicScale\undefined\def\JPicScale{1}\fi
\psset{unit=\JPicScale mm}
\psset{linewidth=0.3,dotsep=1,hatchwidth=0.3,hatchsep=1.5,shadowsize=1,dimen=middle}
\psset{dotsize=0.7 2.5,dotscale=1 1,fillcolor=black}
\psset{arrowsize=1 2,arrowlength=1,arrowinset=0.25,tbarsize=0.7 5,bracketlength=0.15,rbracketlength=0.15}
\begin{pspicture}(0,0)(22,70)
\rput[l](5,35){\Machines}
\rput[l](8,0){\Behaviors}
\rput[l](5,70){\Programs}
\psline[linewidth=0.4,arrowsize=1.05 2,arrowlength=2]{->}(20,32)(20,2.5)
\rput[l](21,17){$\accept$}
\rput[l](22,52){$\enc$}
\psline[linewidth=0.4,arrowsize=1.05 2,arrowlength=2]{->}(20,39.5)(20,66)
\end{pspicture}


==> PIC/prog-metaprog-1.tex <==
%%Created by jPicEdt 1.4.1_03: mixed JPIC-XML/LaTeX format
%%Wed Nov 21 16:58:08 GMT-10:00 2018
%%Begin JPIC-XML
%<?xml version="1.0" standalone="yes"?>
%<jpic x-min="40" x-max="240" y-min="15" y-max="105" auto-bounding="true">
%<multicurve stroke-width= "0.95"
%	 points= "(40,90);(40,90);(90,90);(90,90)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.95"
%	 points= "(40,70);(40,70);(40,50);(40,50)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.95"
%	 points= "(90,70);(90,70);(90,90);(90,90)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.95"
%	 points= "(75,105);(75,105);(75,90);(75,90)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.95"
%	 points= "(60,70);(60,70);(90,70);(90,70)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.95"
%	 points= "(75,70);(75,70);(75,45);(75,45)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.95"
%	 points= "(40,50);(40,50);(60,50);(60,50)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.95"
%	 points= "(40,70);(40,70);(60,50);(60,50)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.95"
%	 points= "(50,80);(50,80);(50,60);(50,60)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.95"
%	 points= "(40,90);(40,90);(60,70);(60,70)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.95"
%	 points= "(190,90);(190,90);(240,90);(240,90)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.95"
%	 points= "(240,70);(240,70);(240,90);(240,90)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.95"
%	 points= "(225,105);(225,105);(225,90);(225,90)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.95"
%	 points= "(210,70);(210,70);(240,70);(240,70)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.95"
%	 points= "(225,70);(225,70);(225,15);(225,15)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.95"
%	 points= "(190,90);(190,90);(210,70);(210,70)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.95"
%	 points= "(165,60);(165,60);(215,60);(215,60)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.95"
%	 points= "(165,40);(165,40);(165,20);(165,20)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.95"
%	 points= "(215,40);(215,40);(215,60);(215,60)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.95"
%	 points= "(200,80);(200,80);(200,60);(200,60)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.95"
%	 points= "(185,40);(185,40);(215,40);(215,40)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.95"
%	 points= "(200,40);(200,40);(200,15);(200,15)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.95"
%	 points= "(165,20);(165,20);(185,20);(185,20)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.95"
%	 points= "(165,40);(165,40);(185,20);(185,20)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.95"
%	 points= "(175,50);(175,50);(175,30);(175,30)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.95"
%	 points= "(165,60);(165,60);(185,40);(185,40)"
%	 fill-style= "none"
%	 />
%<text text-vert-align= "center-v"
%	 anchor-point= "(135,80)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 fill-style= "none"
%	 >
%\EQLS
%</text>
%</jpic>
%%End JPIC-XML
%PSTricks content-type (pstricks.sty package needed)
%Add \usepackage{pstricks} in the preamble of your LaTeX file
%You can rescale the whole picture (to 80% for instance) by using the command \def\JPicScale{0.8}
\ifx\JPicScale\undefined\def\JPicScale{1}\fi
\psset{unit=\JPicScale mm}
\psset{linewidth=0.3,dotsep=1,hatchwidth=0.3,hatchsep=1.5,shadowsize=1,dimen=middle}
\psset{dotsize=0.7 2.5,dotscale=1 1,fillcolor=black}
\psset{arrowsize=1 2,arrowlength=1,arrowinset=0.25,tbarsize=0.7 5,bracketlength=0.15,rbracketlength=0.15}
\begin{pspicture}(0,0)(240,105)
\psline[linewidth=0.95](40,90)(90,90)
\psline[linewidth=0.95](40,70)(40,50)
\psline[linewidth=0.95](90,70)(90,90)
\psline[linewidth=0.95](75,105)(75,90)
\psline[linewidth=0.95](60,70)(90,70)
\psline[linewidth=0.95](75,70)(75,45)
\psline[linewidth=0.95](40,50)(60,50)
\psline[linewidth=0.95](40,70)(60,50)
\psline[linewidth=0.95](50,80)(50,60)
\psline[linewidth=0.95](40,90)(60,70)
\psline[linewidth=0.95](190,90)(240,90)
\psline[linewidth=0.95](240,70)(240,90)
\psline[linewidth=0.95](225,105)(225,90)
\psline[linewidth=0.95](210,70)(240,70)
\psline[linewidth=0.95](225,70)(225,15)
\psline[linewidth=0.95](190,90)(210,70)
\psline[linewidth=0.95](165,60)(215,60)
\psline[linewidth=0.95](165,40)(165,20)
\psline[linewidth=0.95](215,40)(215,60)
\psline[linewidth=0.95](200,80)(200,60)
\psline[linewidth=0.95](185,40)(215,40)
\psline[linewidth=0.95](200,40)(200,15)
\psline[linewidth=0.95](165,20)(185,20)
\psline[linewidth=0.95](165,40)(185,20)
\psline[linewidth=0.95](175,50)(175,30)
\psline[linewidth=0.95](165,60)(185,40)
\rput(135,80){\EQLS}
\end{pspicture}


==> PIC/prog-metaprog.tex <==
%%Created by jPicEdt 1.4.1_03: mixed JPIC-XML/LaTeX format
%%Wed Nov 21 17:24:35 GMT-10:00 2018
%%Begin JPIC-XML
%<?xml version="1.0" standalone="yes"?>
%<jpic x-min="-5" x-max="280" y-min="-5" y-max="85" auto-bounding="true">
%<multicurve stroke-width= "0.95"
%	 points= "(100,70);(100,70);(150,70);(150,70)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.95"
%	 points= "(100,50);(100,50);(100,30);(100,30)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.95"
%	 points= "(150,50);(150,50);(150,70);(150,70)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.95"
%	 points= "(135,85);(135,85);(135,70);(135,70)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.95"
%	 points= "(120,50);(120,50);(150,50);(150,50)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.95"
%	 points= "(135,50);(135,50);(135,-5);(135,-5)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.95"
%	 points= "(100,30);(100,30);(120,30);(120,30)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.95"
%	 points= "(100,50);(100,50);(120,30);(120,30)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.95"
%	 points= "(110,60);(110,60);(110,40);(110,40)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.95"
%	 points= "(100,70);(100,70);(120,50);(120,50)"
%	 fill-style= "none"
%	 />
%<text text-vert-align= "center-v"
%	 anchor-point= "(95,37.5)"
%	 stroke-width= "0.95"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 fill-style= "none"
%	 >
%\programnote
%</text>
%<multicurve stroke-width= "0.95"
%	 points= "(230,70);(230,70);(280,70);(280,70)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.95"
%	 points= "(280,50);(280,50);(280,70);(280,70)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.95"
%	 points= "(265,85);(265,85);(265,70);(265,70)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.95"
%	 points= "(250,50);(250,50);(280,50);(280,50)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.95"
%	 points= "(265,50);(265,50);(265,-5);(265,-5)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.95"
%	 points= "(230,70);(230,70);(250,50);(250,50)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.95"
%	 points= "(205,40);(205,40);(255,40);(255,40)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.95"
%	 points= "(205,20);(205,20);(205,0);(205,0)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.95"
%	 points= "(255,20);(255,20);(255,40);(255,40)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.95"
%	 points= "(240,60);(240,60);(240,40);(240,40)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.95"
%	 points= "(225,20);(225,20);(255,20);(255,20)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.95"
%	 points= "(240,20);(240,20);(240,-5);(240,-5)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.95"
%	 points= "(205,0);(205,0);(225,0);(225,0)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.95"
%	 points= "(205,20);(205,20);(225,0);(225,0)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.95"
%	 points= "(215,30);(215,30);(215,10);(215,10)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.95"
%	 points= "(205,40);(205,40);(225,20);(225,20)"
%	 fill-style= "none"
%	 />
%<text text-vert-align= "center-v"
%	 anchor-point= "(200,10)"
%	 stroke-width= "0.95"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 fill-style= "none"
%	 >
%\metaprogramnote
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(180,60)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 fill-style= "none"
%	 >
%\EQLS
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(265,60)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 fill-style= "none"
%	 >
%$\runone$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(240,30)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 fill-style= "none"
%	 >
%$\runone$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(135,60)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 fill-style= "none"
%	 >
%$\runone$
%</text>
%<multicurve stroke-width= "0.95"
%	 points= "(110,30);(110,30);(110,-5);(110,-5)"
%	 fill-style= "none"
%	 />
%<text text-vert-align= "center-v"
%	 anchor-point= "(211.25,5)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 fill-style= "none"
%	 >
%$\Progtwo$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(106.25,35)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 fill-style= "none"
%	 >
%$\Progone$
%</text>
%<multicurve stroke-width= "0.95"
%	 points= "(0,70);(0,70);(40,70);(40,70)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.95"
%	 points= "(40,50);(40,50);(40,70);(40,70)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.95"
%	 points= "(20,85);(20,85);(20,70);(20,70)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.95"
%	 points= "(0,50);(0,50);(40,50);(40,50)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.95"
%	 points= "(30,50);(30,50);(30,-5);(30,-5)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.95"
%	 points= "(10,50);(10,50);(10,-5);(10,-5)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.95"
%	 points= "(0,70);(0,70);(0,50);(0,50)"
%	 fill-style= "none"
%	 />
%<text text-vert-align= "center-v"
%	 anchor-point= "(70,60)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 fill-style= "none"
%	 >
%\EQLS
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(20,60)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 fill-style= "none"
%	 >
%$\computation$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(-5,60)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 fill-style= "none"
%	 >
%\comnote
%</text>
%</jpic>
%%End JPIC-XML
%PSTricks content-type (pstricks.sty package needed)
%Add \usepackage{pstricks} in the preamble of your LaTeX file
%You can rescale the whole picture (to 80% for instance) by using the command \def\JPicScale{0.8}
\ifx\JPicScale\undefined\def\JPicScale{1}\fi
\psset{unit=\JPicScale mm}
\psset{linewidth=0.3,dotsep=1,hatchwidth=0.3,hatchsep=1.5,shadowsize=1,dimen=middle}
\psset{dotsize=0.7 2.5,dotscale=1 1,fillcolor=black}
\psset{arrowsize=1 2,arrowlength=1,arrowinset=0.25,tbarsize=0.7 5,bracketlength=0.15,rbracketlength=0.15}
\begin{pspicture}(0,0)(280,85)
\psline[linewidth=0.95](100,70)(150,70)
\psline[linewidth=0.95](100,50)(100,30)
\psline[linewidth=0.95](150,50)(150,70)
\psline[linewidth=0.95](135,85)(135,70)
\psline[linewidth=0.95](120,50)(150,50)
\psline[linewidth=0.95](135,50)(135,-5)
\psline[linewidth=0.95](100,30)(120,30)
\psline[linewidth=0.95](100,50)(120,30)
\psline[linewidth=0.95](110,60)(110,40)
\psline[linewidth=0.95](100,70)(120,50)
\rput[r](95,37.5){\programnote}
\psline[linewidth=0.95](230,70)(280,70)
\psline[linewidth=0.95](280,50)(280,70)
\psline[linewidth=0.95](265,85)(265,70)
\psline[linewidth=0.95](250,50)(280,50)
\psline[linewidth=0.95](265,50)(265,-5)
\psline[linewidth=0.95](230,70)(250,50)
\psline[linewidth=0.95](205,40)(255,40)
\psline[linewidth=0.95](205,20)(205,0)
\psline[linewidth=0.95](255,20)(255,40)
\psline[linewidth=0.95](240,60)(240,40)
\psline[linewidth=0.95](225,20)(255,20)
\psline[linewidth=0.95](240,20)(240,-5)
\psline[linewidth=0.95](205,0)(225,0)
\psline[linewidth=0.95](205,20)(225,0)
\psline[linewidth=0.95](215,30)(215,10)
\psline[linewidth=0.95](205,40)(225,20)
\rput[r](200,10){\metaprogramnote}
\rput(180,60){\EQLS}
\rput(265,60){$\runone$}
\rput(240,30){$\runone$}
\rput(135,60){$\runone$}
\psline[linewidth=0.95](110,30)(110,-5)
\rput(211.25,5){$\Progtwo$}
\rput(106.25,35){$\Progone$}
\psline[linewidth=0.95](0,70)(40,70)
\psline[linewidth=0.95](40,50)(40,70)
\psline[linewidth=0.95](20,85)(20,70)
\psline[linewidth=0.95](0,50)(40,50)
\psline[linewidth=0.95](30,50)(30,-5)
\psline[linewidth=0.95](10,50)(10,-5)
\psline[linewidth=0.95](0,70)(0,50)
\rput(70,60){\EQLS}
\rput(20,60){$\computation$}
\rput[r](-5,60){\comnote}
\end{pspicture}


==> PIC/progenc.tex <==
%%Created by jPicEdt 1.4.1_03: mixed JPIC-XML/LaTeX format
%%Thu Dec 19 20:45:25 GMT-10:00 2019
%%Begin JPIC-XML
%<?xml version="1.0" standalone="yes"?>
%<jpic x-min="2.5" x-max="227.5" y-min="0" y-max="90" auto-bounding="true">
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(35,70);(35,70);(85,70);(85,70)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(85,45);(85,45);(85,70);(85,70)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(70,90);(70,90);(70,70);(70,70)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(60,45);(60,45);(85,45);(85,45)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(70,45);(70,45);(70,0);(70,0)"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 stroke-width= "0.75"
%	 anchor-point= "(68.12,56.88)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\universal
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 stroke-width= "0.75"
%	 anchor-point= "(20,45)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\EQLS
%</text>
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(47.5,57.5);(47.5,57.5);(47.5,22.5);(47.5,22.5)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(35,70);(35,70);(60,45);(60,45)"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 stroke-width= "0.75"
%	 anchor-point= "(2.5,1.25)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\inputt$
%</text>
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(5,90);(5,90);(5,0);(5,0)"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(45,45)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\progtype$
%</text>
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(35,35);(35,35);(60,10);(60,10)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(35,10);(35,10);(35,35);(35,35)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(35,10);(35,10);(60,10);(60,10)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(140,70);(140,70);(165,70);(165,70)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(165,45);(165,45);(165,70);(165,70)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(152.5,90);(152.5,90);(152.5,70);(152.5,70)"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 stroke-width= "0.75"
%	 anchor-point= "(150,1.25)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\inputt$
%</text>
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(140,22.5);(140,22.5);(165,22.5);(165,22.5)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(152.5,22.5);(152.5,22.5);(152.5,0);(152.5,0)"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 stroke-width= "0.75"
%	 anchor-point= "(157.5,62.5)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\universal
%</text>
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(127.5,35);(127.5,35);(127.5,22.5);(127.5,22.5)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(115,47.5);(115,47.5);(140,22.5);(140,22.5)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(115,35);(115,35);(140,10);(140,10)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(115,10);(115,10);(115,35);(115,35)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(115,10);(115,10);(140,10);(140,10)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(140,47.5);(140,47.5);(165,22.5);(165,22.5)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(115,47.5);(115,47.5);(140,47.5);(140,47.5)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(152.5,57.5);(152.5,57.5);(152.5,35);(152.5,35)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(140,70);(140,70);(165,45);(165,45)"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 stroke-width= "0.75"
%	 anchor-point= "(67.5,1.25)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\inputt$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 stroke-width= "0.75"
%	 anchor-point= "(156.25,88.75)"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\inputt$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 stroke-width= "0.75"
%	 anchor-point= "(73.75,88.75)"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\inputt$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(150,50)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\progtype$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 stroke-width= "0.75"
%	 anchor-point= "(100,45)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\EQLS
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 stroke-width= "0.75"
%	 anchor-point= "(185,45)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\EQLS
%</text>
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(202.5,70);(202.5,70);(227.5,70);(227.5,70)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(227.5,45);(227.5,45);(227.5,70);(227.5,70)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(215,90);(215,90);(215,70);(215,70)"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 stroke-width= "0.75"
%	 anchor-point= "(212.5,1.25)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\inputt$
%</text>
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(202.5,20);(202.5,20);(227.5,20);(227.5,20)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(215,20);(215,20);(215,0);(215,0)"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 stroke-width= "0.75"
%	 anchor-point= "(220,62.5)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\universal
%</text>
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(202.5,20);(202.5,20);(202.5,45);(202.5,45)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(202.5,45);(202.5,45);(227.5,20);(227.5,20)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(215,57.5);(215,57.5);(215,32.5);(215,32.5)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(202.5,70);(202.5,70);(227.5,45);(227.5,45)"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 stroke-width= "0.75"
%	 anchor-point= "(218.75,88.75)"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\inputt$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(212.5,50)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\progtype$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(210,26.25)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\encoding$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(138.75,36.25)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\partl$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(121.25,16.25)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\idcode$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(43.75,16.25)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\idcode$
%</text>
%</jpic>
%%End JPIC-XML
%PSTricks content-type (pstricks.sty package needed)
%Add \usepackage{pstricks} in the preamble of your LaTeX file
%You can rescale the whole picture (to 80% for instance) by using the command \def\JPicScale{0.8}
\ifx\JPicScale\undefined\def\JPicScale{1}\fi
\psset{unit=\JPicScale mm}
\psset{linewidth=0.3,dotsep=1,hatchwidth=0.3,hatchsep=1.5,shadowsize=1,dimen=middle}
\psset{dotsize=0.7 2.5,dotscale=1 1,fillcolor=black}
\psset{arrowsize=1 2,arrowlength=1,arrowinset=0.25,tbarsize=0.7 5,bracketlength=0.15,rbracketlength=0.15}
\begin{pspicture}(0,0)(227.5,90)
\psline[linewidth=0.75](35,70)(85,70)
\psline[linewidth=0.75](85,45)(85,70)
\psline[linewidth=0.75](70,90)(70,70)
\psline[linewidth=0.75](60,45)(85,45)
\psline[linewidth=0.75](70,45)(70,0)
\rput(68.12,56.88){\universal}
\rput(20,45){\EQLS}
\psline[linewidth=0.75](47.5,57.5)(47.5,22.5)
\psline[linewidth=0.75](35,70)(60,45)
\rput[r](2.5,1.25){$\inputt$}
\psline[linewidth=0.75](5,90)(5,0)
\rput[r](45,45){$\progtype$}
\psline[linewidth=0.75](35,35)(60,10)
\psline[linewidth=0.75](35,10)(35,35)
\psline[linewidth=0.75](35,10)(60,10)
\psline[linewidth=0.75](140,70)(165,70)
\psline[linewidth=0.75](165,45)(165,70)
\psline[linewidth=0.75](152.5,90)(152.5,70)
\rput[r](150,1.25){$\inputt$}
\psline[linewidth=0.75](140,22.5)(165,22.5)
\psline[linewidth=0.75](152.5,22.5)(152.5,0)
\rput(157.5,62.5){\universal}
\psline[linewidth=0.75](127.5,35)(127.5,22.5)
\psline[linewidth=0.75](115,47.5)(140,22.5)
\psline[linewidth=0.75](115,35)(140,10)
\psline[linewidth=0.75](115,10)(115,35)
\psline[linewidth=0.75](115,10)(140,10)
\psline[linewidth=0.75](140,47.5)(165,22.5)
\psline[linewidth=0.75](115,47.5)(140,47.5)
\psline[linewidth=0.75](152.5,57.5)(152.5,35)
\psline[linewidth=0.75](140,70)(165,45)
\rput[r](67.5,1.25){$\inputt$}
\rput[l](156.25,88.75){$\inputt$}
\rput[l](73.75,88.75){$\inputt$}
\rput[r](150,50){$\progtype$}
\rput(100,45){\EQLS}
\rput(185,45){\EQLS}
\psline[linewidth=0.75](202.5,70)(227.5,70)
\psline[linewidth=0.75](227.5,45)(227.5,70)
\psline[linewidth=0.75](215,90)(215,70)
\rput[r](212.5,1.25){$\inputt$}
\psline[linewidth=0.75](202.5,20)(227.5,20)
\psline[linewidth=0.75](215,20)(215,0)
\rput(220,62.5){\universal}
\psline[linewidth=0.75](202.5,20)(202.5,45)
\psline[linewidth=0.75](202.5,45)(227.5,20)
\psline[linewidth=0.75](215,57.5)(215,32.5)
\psline[linewidth=0.75](202.5,70)(227.5,45)
\rput[l](218.75,88.75){$\inputt$}
\rput[r](212.5,50){$\progtype$}
\rput(210,26.25){$\encoding$}
\rput(138.75,36.25){$\partl$}
\rput(121.25,16.25){$\idcode$}
\rput(43.75,16.25){$\idcode$}
\end{pspicture}


==> PIC/projections-1.tex <==
%%Created by jPicEdt 1.4.1_03: mixed JPIC-XML/LaTeX format
%%Sat Dec 22 17:29:27 GMT-10:00 2018
%%Begin JPIC-XML
%<?xml version="1.0" standalone="yes"?>
%<jpic x-min="0" x-max="280" y-min="0" y-max="85" auto-bounding="true">
%<multicurve fill-style= "none"
%	 points= "(280,70);(280,70);(280,0);(280,0)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(260,35);(260,35);(260,0);(260,0)"
%	 stroke-width= "0.75"
%	 />
%<ellipse fill-style= "solid"
%	 p3= "(262.58,32.42)"
%	 fill-color= "#330033"
%	 p2= "(262.58,37.58)"
%	 p1= "(257.42,37.58)"
%	 closure= "open"
%	 angle-end= "0"
%	 angle-start= "0"
%	 />
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(235,35)"
%	 stroke-width= "0.75"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\EQLS
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(65,35)"
%	 stroke-width= "0.75"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\EQLS
%</text>
%<multicurve fill-style= "none"
%	 points= "(90,70);(90,70);(90,0);(90,0)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(110,35.01);(110,35.01);(110,0);(110,0)"
%	 stroke-width= "0.75"
%	 />
%<ellipse fill-style= "solid"
%	 p3= "(112.57,32.42)"
%	 fill-color= "#330033"
%	 p2= "(112.57,37.58)"
%	 p1= "(107.43,37.58)"
%	 closure= "open"
%	 angle-end= "0"
%	 angle-start= "0"
%	 />
%<multicurve fill-style= "none"
%	 points= "(20,40);(20,40);(20,30);(20,30)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(0,60);(0,60);(40,60);(40,60)"
%	 stroke-width= "0.6"
%	 />
%<multicurve fill-style= "none"
%	 points= "(40,40);(40,40);(40,60);(40,60)"
%	 stroke-width= "0.6"
%	 />
%<multicurve fill-style= "none"
%	 points= "(0,40);(0,40);(40,40);(40,40)"
%	 stroke-width= "0.6"
%	 />
%<multicurve fill-style= "none"
%	 points= "(0,60);(0,60);(0,40);(0,40)"
%	 stroke-width= "0.6"
%	 />
%<multicurve fill-style= "none"
%	 points= "(20,70);(20,70);(20,60);(20,60)"
%	 stroke-width= "0.75"
%	 />
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(20,50)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\fsttag$
%</text>
%<multicurve fill-style= "none"
%	 points= "(190,40);(190,40);(190,30);(190,30)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(170,60);(170,60);(210,60);(210,60)"
%	 stroke-width= "0.6"
%	 />
%<multicurve fill-style= "none"
%	 points= "(210,40);(210,40);(210,60);(210,60)"
%	 stroke-width= "0.6"
%	 />
%<multicurve fill-style= "none"
%	 points= "(170,40);(170,40);(210,40);(210,40)"
%	 stroke-width= "0.6"
%	 />
%<multicurve fill-style= "none"
%	 points= "(170,60);(170,60);(170,40);(170,40)"
%	 stroke-width= "0.6"
%	 />
%<multicurve fill-style= "none"
%	 points= "(190,70);(190,70);(190,60);(190,60)"
%	 stroke-width= "0.75"
%	 />
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(190,50)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\sndtag$
%</text>
%<multicurve fill-style= "none"
%	 points= "(180,10);(180,10);(180,0);(180,0)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(170,30);(170,30);(210,30);(210,30)"
%	 stroke-width= "0.6"
%	 />
%<multicurve fill-style= "none"
%	 points= "(210,10);(210,10);(210,30);(210,30)"
%	 stroke-width= "0.6"
%	 />
%<multicurve fill-style= "none"
%	 points= "(170,10);(170,10);(210,10);(210,10)"
%	 stroke-width= "0.6"
%	 />
%<multicurve fill-style= "none"
%	 points= "(170,30);(170,30);(170,10);(170,10)"
%	 stroke-width= "0.6"
%	 />
%<multicurve fill-style= "none"
%	 points= "(0,30);(0,30);(40,30);(40,30)"
%	 stroke-width= "0.6"
%	 />
%<multicurve fill-style= "none"
%	 points= "(40,10);(40,10);(40,30);(40,30)"
%	 stroke-width= "0.6"
%	 />
%<multicurve fill-style= "none"
%	 points= "(0,10);(0,10);(40,10);(40,10)"
%	 stroke-width= "0.6"
%	 />
%<multicurve fill-style= "none"
%	 points= "(0,30);(0,30);(0,10);(0,10)"
%	 stroke-width= "0.6"
%	 />
%<multicurve fill-style= "none"
%	 points= "(200,10);(200,10);(200,0);(200,0)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(10,10);(10,10);(10,0);(10,0)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(30,10);(30,10);(30,0);(30,0)"
%	 stroke-width= "0.75"
%	 />
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(190,20)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\pairtag$
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(20,20)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\pairtag$
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(65,85)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\leqn$
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(235,85)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\reqn$
%</text>
%</jpic>
%%End JPIC-XML
%PSTricks content-type (pstricks.sty package needed)
%Add \usepackage{pstricks} in the preamble of your LaTeX file
%You can rescale the whole picture (to 80% for instance) by using the command \def\JPicScale{0.8}
\ifx\JPicScale\undefined\def\JPicScale{1}\fi
\psset{unit=\JPicScale mm}
\psset{linewidth=0.3,dotsep=1,hatchwidth=0.3,hatchsep=1.5,shadowsize=1,dimen=middle}
\psset{dotsize=0.7 2.5,dotscale=1 1,fillcolor=black}
\psset{arrowsize=1 2,arrowlength=1,arrowinset=0.25,tbarsize=0.7 5,bracketlength=0.15,rbracketlength=0.15}
\begin{pspicture}(0,0)(280,85)
\psline[linewidth=0.75](280,70)(280,0)
\psline[linewidth=0.75](260,35)(260,0)
\newrgbcolor{userFillColour}{0.2 0 0.2}
\rput{0}(260,35){\psellipse[fillcolor=userFillColour,fillstyle=solid](0,0)(2.58,-2.58)}
\rput(235,35){\EQLS}
\rput(65,35){\EQLS}
\psline[linewidth=0.75](90,70)(90,0)
\psline[linewidth=0.75](110,35.01)(110,0)
\newrgbcolor{userFillColour}{0.2 0 0.2}
\rput{90}(110,35){\psellipse[fillcolor=userFillColour,fillstyle=solid](0,0)(2.58,-2.57)}
\psline[linewidth=0.75](20,40)(20,30)
\psline[linewidth=0.6](0,60)(40,60)
\psline[linewidth=0.6](40,40)(40,60)
\psline[linewidth=0.6](0,40)(40,40)
\psline[linewidth=0.6](0,60)(0,40)
\psline[linewidth=0.75](20,70)(20,60)
\rput(20,50){$\fsttag$}
\psline[linewidth=0.75](190,40)(190,30)
\psline[linewidth=0.6](170,60)(210,60)
\psline[linewidth=0.6](210,40)(210,60)
\psline[linewidth=0.6](170,40)(210,40)
\psline[linewidth=0.6](170,60)(170,40)
\psline[linewidth=0.75](190,70)(190,60)
\rput(190,50){$\sndtag$}
\psline[linewidth=0.75](180,10)(180,0)
\psline[linewidth=0.6](170,30)(210,30)
\psline[linewidth=0.6](210,10)(210,30)
\psline[linewidth=0.6](170,10)(210,10)
\psline[linewidth=0.6](170,30)(170,10)
\psline[linewidth=0.6](0,30)(40,30)
\psline[linewidth=0.6](40,10)(40,30)
\psline[linewidth=0.6](0,10)(40,10)
\psline[linewidth=0.6](0,30)(0,10)
\psline[linewidth=0.75](200,10)(200,0)
\psline[linewidth=0.75](10,10)(10,0)
\psline[linewidth=0.75](30,10)(30,0)
\rput(190,20){$\pairtag$}
\rput(20,20){$\pairtag$}
\rput(65,85){$\leqn$}
\rput(235,85){$\reqn$}
\end{pspicture}


==> PIC/projections.tex <==
%%Created by jPicEdt 1.4.1_03: mixed JPIC-XML/LaTeX format
%%Sat Dec 22 17:25:00 GMT-10:00 2018
%%Begin JPIC-XML
%<?xml version="1.0" standalone="yes"?>
%<jpic x-min="0" x-max="340" y-min="0" y-max="75" auto-bounding="true">
%<multicurve fill-style= "none"
%	 points= "(80,50);(80,50);(120,50);(120,50)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(120,30);(120,30);(120,50);(120,50)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(110,60);(110,60);(110,50);(110,50)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(100.62,30);(100.62,30);(120,30);(120,30)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(110,30);(110,30);(110,15);(110,15)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(90,40);(90,40);(90,0);(90,0)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(80,50);(80,50);(100,30);(100,30)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(20,30);(20,30);(20,0);(20,0)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(0,50);(0,50);(40,50);(40,50)"
%	 stroke-width= "0.6"
%	 />
%<multicurve fill-style= "none"
%	 points= "(40,30);(40,30);(40,50);(40,50)"
%	 stroke-width= "0.6"
%	 />
%<multicurve fill-style= "none"
%	 points= "(0,30);(0,30);(40,30);(40,30)"
%	 stroke-width= "0.6"
%	 />
%<multicurve fill-style= "none"
%	 points= "(0,50);(0,50);(0,30);(0,30)"
%	 stroke-width= "0.6"
%	 />
%<multicurve fill-style= "none"
%	 points= "(20,60);(20,60);(20,50);(20,50)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(100,25);(100,25);(120,5);(120,5)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(100,5);(100,5);(119.38,5);(119.38,5)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(100,5);(100,5);(100,24.99);(100,24.99)"
%	 stroke-width= "0.75"
%	 />
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(60,25)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\EQLS$
%</text>
%<multicurve fill-style= "none"
%	 points= "(300,50);(300,50);(340,50);(340,50)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(340,30);(340,30);(340,50);(340,50)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(330,60);(330,60);(330,50);(330,50)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(320.62,30);(320.62,30);(340,30);(340,30)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(330,30);(330,30);(330,15);(330,15)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(310,40);(310,40);(310,0);(310,0)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(300,50);(300,50);(320,30);(320,30)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(240,30);(240,30);(240,0);(240,0)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(220,50);(220,50);(260,50);(260,50)"
%	 stroke-width= "0.6"
%	 />
%<multicurve fill-style= "none"
%	 points= "(260,30);(260,30);(260,50);(260,50)"
%	 stroke-width= "0.6"
%	 />
%<multicurve fill-style= "none"
%	 points= "(220,30);(220,30);(260,30);(260,30)"
%	 stroke-width= "0.6"
%	 />
%<multicurve fill-style= "none"
%	 points= "(220,50);(220,50);(220,30);(220,30)"
%	 stroke-width= "0.6"
%	 />
%<multicurve fill-style= "none"
%	 points= "(240,60);(240,60);(240,50);(240,50)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(320,25);(320,25);(340,5);(340,5)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(320,5);(320,5);(339.38,5);(339.38,5)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(320,5);(320,5);(320,24.99);(320,24.99)"
%	 stroke-width= "0.75"
%	 />
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(280,25)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\EQLS$
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(20,40)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\fsttag$
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(240,40)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\sndtag$
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(105,10)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\toptag$
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(325,10)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\bottag$
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(105,40)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\utag$
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(325,40)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\utag$
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(60,75)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\oneqn$
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(280,75)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\twoeqn$
%</text>
%</jpic>
%%End JPIC-XML
%PSTricks content-type (pstricks.sty package needed)
%Add \usepackage{pstricks} in the preamble of your LaTeX file
%You can rescale the whole picture (to 80% for instance) by using the command \def\JPicScale{0.8}
\ifx\JPicScale\undefined\def\JPicScale{1}\fi
\psset{unit=\JPicScale mm}
\psset{linewidth=0.3,dotsep=1,hatchwidth=0.3,hatchsep=1.5,shadowsize=1,dimen=middle}
\psset{dotsize=0.7 2.5,dotscale=1 1,fillcolor=black}
\psset{arrowsize=1 2,arrowlength=1,arrowinset=0.25,tbarsize=0.7 5,bracketlength=0.15,rbracketlength=0.15}
\begin{pspicture}(0,0)(340,75)
\psline[linewidth=0.75](80,50)(120,50)
\psline[linewidth=0.75](120,30)(120,50)
\psline[linewidth=0.75](110,60)(110,50)
\psline[linewidth=0.75](100.62,30)(120,30)
\psline[linewidth=0.75](110,30)(110,15)
\psline[linewidth=0.75](90,40)(90,0)
\psline[linewidth=0.75](80,50)(100,30)
\psline[linewidth=0.75](20,30)(20,0)
\psline[linewidth=0.6](0,50)(40,50)
\psline[linewidth=0.6](40,30)(40,50)
\psline[linewidth=0.6](0,30)(40,30)
\psline[linewidth=0.6](0,50)(0,30)
\psline[linewidth=0.75](20,60)(20,50)
\psline[linewidth=0.75](100,25)(120,5)
\psline[linewidth=0.75](100,5)(119.38,5)
\psline[linewidth=0.75](100,5)(100,24.99)
\rput(60,25){$\EQLS$}
\psline[linewidth=0.75](300,50)(340,50)
\psline[linewidth=0.75](340,30)(340,50)
\psline[linewidth=0.75](330,60)(330,50)
\psline[linewidth=0.75](320.62,30)(340,30)
\psline[linewidth=0.75](330,30)(330,15)
\psline[linewidth=0.75](310,40)(310,0)
\psline[linewidth=0.75](300,50)(320,30)
\psline[linewidth=0.75](240,30)(240,0)
\psline[linewidth=0.6](220,50)(260,50)
\psline[linewidth=0.6](260,30)(260,50)
\psline[linewidth=0.6](220,30)(260,30)
\psline[linewidth=0.6](220,50)(220,30)
\psline[linewidth=0.75](240,60)(240,50)
\psline[linewidth=0.75](320,25)(340,5)
\psline[linewidth=0.75](320,5)(339.38,5)
\psline[linewidth=0.75](320,5)(320,24.99)
\rput(280,25){$\EQLS$}
\rput(20,40){$\fsttag$}
\rput(240,40){$\sndtag$}
\rput(105,10){$\toptag$}
\rput(325,10){$\bottag$}
\rput(105,40){$\utag$}
\rput(325,40){$\utag$}
\rput(60,75){$\oneqn$}
\rput(280,75){$\twoeqn$}
\end{pspicture}


==> PIC/projs-1.tex <==
%%Created by jPicEdt 1.4.1_03: mixed JPIC-XML/LaTeX format
%%Tue Dec 26 22:15:41 PST 2017
%%Begin JPIC-XML
%<?xml version="1.0" standalone="yes"?>
%<jpic x-min="0" x-max="230" y-min="0" y-max="60" auto-bounding="true">
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(220,60);(220,60);(220,0);(220,0)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(200,30);(200,30);(200,0);(200,0)"
%	 />
%<ellipse p3= "(202.58,27.42)"
%	 p2= "(202.58,32.58)"
%	 p1= "(197.42,32.58)"
%	 closure= "open"
%	 fill-style= "solid"
%	 angle-end= "0"
%	 fill-color= "#330033"
%	 angle-start= "0"
%	 />
%<multicurve stroke-width= "0.45"
%	 fill-style= "none"
%	 points= "(190,40);(190,40);(230,40);(230,40)"
%	 />
%<multicurve stroke-width= "0.45"
%	 fill-style= "none"
%	 points= "(230,20);(230,20);(230,40);(230,40)"
%	 />
%<multicurve stroke-width= "0.45"
%	 fill-style= "none"
%	 points= "(190,20);(190,20);(230,20);(230,20)"
%	 />
%<multicurve stroke-width= "0.45"
%	 fill-style= "none"
%	 points= "(190,40);(190,40);(190,20);(190,20)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(10,60);(10,60);(10,0);(10,0)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(30,30.01);(30,30.01);(30,0);(30,0)"
%	 />
%<ellipse p3= "(32.58,27.42)"
%	 p2= "(32.58,32.58)"
%	 p1= "(27.42,32.58)"
%	 closure= "open"
%	 fill-style= "solid"
%	 angle-end= "0"
%	 fill-color= "#330033"
%	 angle-start= "0"
%	 />
%<multicurve stroke-width= "0.45"
%	 fill-style= "none"
%	 points= "(0,40);(0,40);(40,40);(40,40)"
%	 />
%<multicurve stroke-width= "0.45"
%	 fill-style= "none"
%	 points= "(40,20);(40,20);(40,40);(40,40)"
%	 />
%<multicurve stroke-width= "0.45"
%	 fill-style= "none"
%	 points= "(0,20);(0,20);(40,20);(40,20)"
%	 />
%<multicurve stroke-width= "0.45"
%	 fill-style= "none"
%	 points= "(0,40);(0,40);(0,20);(0,20)"
%	 />
%<text text-vert-align= "center-v"
%	 anchor-point= "(20,30)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\pizero$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(210,30)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\pione$
%</text>
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(120,25);(120,25);(110,15);(110,15)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(110,15);(110,15);(110,0);(110,0)"
%	 />
%<ellipse p3= "(112.58,12.42)"
%	 p2= "(112.58,17.58)"
%	 p1= "(107.42,17.58)"
%	 closure= "open"
%	 fill-style= "solid"
%	 angle-end= "0"
%	 fill-color= "#330033"
%	 angle-start= "0"
%	 />
%<multicurve stroke-width= "0.6"
%	 fill-style= "none"
%	 points= "(95,35);(95,35);(105,35);(105,35)"
%	 />
%<multicurve stroke-width= "0.45"
%	 fill-style= "none"
%	 points= "(135,10);(135,10);(135,50);(135,50)"
%	 />
%<multicurve stroke-width= "0.45"
%	 fill-style= "none"
%	 points= "(85,50);(85,50);(135,50);(135,50)"
%	 />
%<multicurve stroke-width= "0.6"
%	 fill-style= "none"
%	 points= "(100,35);(100,35);(100,25);(100,25)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(100,25);(100,25);(110,15);(110,15)"
%	 />
%<multicurve stroke-width= "0.6"
%	 fill-style= "none"
%	 points= "(120,35);(120,35);(120,25);(120,25)"
%	 />
%<multicurve stroke-width= "0.6"
%	 fill-style= "none"
%	 points= "(115,35);(115,35);(125,35);(125,35)"
%	 />
%<multicurve stroke-width= "0.6"
%	 fill-style= "none"
%	 points= "(115,45);(115,45);(125,45);(125,45)"
%	 />
%<multicurve stroke-width= "0.6"
%	 fill-style= "none"
%	 points= "(95,45);(95,45);(105,45);(105,45)"
%	 />
%<multicurve stroke-width= "0.6"
%	 fill-style= "none"
%	 points= "(105,45);(105,45);(105,35);(105,35)"
%	 />
%<multicurve stroke-width= "0.6"
%	 fill-style= "none"
%	 points= "(115,45);(115,45);(115,35);(115,35)"
%	 />
%<multicurve stroke-width= "0.6"
%	 fill-style= "none"
%	 points= "(125,45);(125,45);(125,35);(125,35)"
%	 />
%<multicurve stroke-width= "0.6"
%	 fill-style= "none"
%	 points= "(95,45);(95,45);(95,35);(95,35)"
%	 />
%<multicurve stroke-width= "0.6"
%	 fill-style= "none"
%	 points= "(100,60);(100,60);(100,45);(100,45)"
%	 />
%<multicurve stroke-width= "0.6"
%	 fill-style= "none"
%	 points= "(120,60);(120,60);(120,45);(120,45)"
%	 />
%<multicurve stroke-width= "0.45"
%	 fill-style= "none"
%	 points= "(85,10);(85,10);(85,50);(85,50)"
%	 />
%<multicurve stroke-width= "0.45"
%	 fill-style= "none"
%	 points= "(85,10);(85,10);(135,10);(135,10)"
%	 />
%<text text-vert-align= "center-v"
%	 anchor-point= "(100,40)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\aah$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(120,40)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\bbh$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(7.5,2.5)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\AAh$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(32.5,2.5)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\BBh$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(97.5,57.5)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\AAh$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(122.5,57.5)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\BBh$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(197.5,2.5)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\AAh$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(222.5,2.5)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\BBh$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(107.5,2.5)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\XXh$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(131.25,13.75)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\paire$
%</text>
%</jpic>
%%End JPIC-XML
%PSTricks content-type (pstricks.sty package needed)
%Add \usepackage{pstricks} in the preamble of your LaTeX file
%You can rescale the whole picture (to 80% for instance) by using the command \def\JPicScale{0.8}
\ifx\JPicScale\undefined\def\JPicScale{1}\fi
\psset{unit=\JPicScale mm}
\psset{linewidth=0.3,dotsep=1,hatchwidth=0.3,hatchsep=1.5,shadowsize=1,dimen=middle}
\psset{dotsize=0.7 2.5,dotscale=1 1,fillcolor=black}
\psset{arrowsize=1 2,arrowlength=1,arrowinset=0.25,tbarsize=0.7 5,bracketlength=0.15,rbracketlength=0.15}
\begin{pspicture}(0,0)(230,60)
\psline[linewidth=0.75](220,60)(220,0)
\psline[linewidth=0.75](200,30)(200,0)
\newrgbcolor{userFillColour}{0.2 0 0.2}
\rput{0}(200,30){\psellipse[fillcolor=userFillColour,fillstyle=solid](0,0)(2.58,-2.58)}
\psline[linewidth=0.45](190,40)(230,40)
\psline[linewidth=0.45](230,20)(230,40)
\psline[linewidth=0.45](190,20)(230,20)
\psline[linewidth=0.45](190,40)(190,20)
\psline[linewidth=0.75](10,60)(10,0)
\psline[linewidth=0.75](30,30.01)(30,0)
\newrgbcolor{userFillColour}{0.2 0 0.2}
\rput{0}(30,30){\psellipse[fillcolor=userFillColour,fillstyle=solid](0,0)(2.58,-2.58)}
\psline[linewidth=0.45](0,40)(40,40)
\psline[linewidth=0.45](40,20)(40,40)
\psline[linewidth=0.45](0,20)(40,20)
\psline[linewidth=0.45](0,40)(0,20)
\rput(20,30){$\pizero$}
\rput(210,30){$\pione$}
\psline[linewidth=0.75](120,25)(110,15)
\psline[linewidth=0.75](110,15)(110,0)
\newrgbcolor{userFillColour}{0.2 0 0.2}
\rput{0}(110,15){\psellipse[fillcolor=userFillColour,fillstyle=solid](0,0)(2.58,-2.58)}
\psline[linewidth=0.6](95,35)(105,35)
\psline[linewidth=0.45](135,10)(135,50)
\psline[linewidth=0.45](85,50)(135,50)
\psline[linewidth=0.6](100,35)(100,25)
\psline[linewidth=0.75](100,25)(110,15)
\psline[linewidth=0.6](120,35)(120,25)
\psline[linewidth=0.6](115,35)(125,35)
\psline[linewidth=0.6](115,45)(125,45)
\psline[linewidth=0.6](95,45)(105,45)
\psline[linewidth=0.6](105,45)(105,35)
\psline[linewidth=0.6](115,45)(115,35)
\psline[linewidth=0.6](125,45)(125,35)
\psline[linewidth=0.6](95,45)(95,35)
\psline[linewidth=0.6](100,60)(100,45)
\psline[linewidth=0.6](120,60)(120,45)
\psline[linewidth=0.45](85,10)(85,50)
\psline[linewidth=0.45](85,10)(135,10)
\rput(100,40){$\aah$}
\rput(120,40){$\bbh$}
\rput[r](7.5,2.5){$\AAh$}
\rput[l](32.5,2.5){$\BBh$}
\rput[r](97.5,57.5){$\AAh$}
\rput[l](122.5,57.5){$\BBh$}
\rput[r](197.5,2.5){$\AAh$}
\rput[l](222.5,2.5){$\BBh$}
\rput[r](107.5,2.5){$\XXh$}
\rput[r](131.25,13.75){$\paire$}
\end{pspicture}


==> PIC/projs-6.tex <==
%%Created by jPicEdt 1.4.1_03: mixed JPIC-XML/LaTeX format
%%Thu May 20 15:27:04 GMT-10:00 2021
%%Begin JPIC-XML
%<?xml version="1.0" standalone="yes"?>
%<jpic x-min="0" x-max="230" y-min="0" y-max="60" auto-bounding="true">
%<multicurve fill-style= "none"
%	 points= "(220,60);(220,60);(220,0);(220,0)"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(200,30);(200,30);(200,0);(200,0)"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(190,40);(190,40);(230,40);(230,40)"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(230,20);(230,20);(230,40);(230,40)"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(190,20);(190,20);(230,20);(230,20)"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(190,40);(190,40);(190,20);(190,20)"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(10,60);(10,60);(10,0);(10,0)"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(30,30.01);(30,30.01);(30,0);(30,0)"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(0,40);(0,40);(40,40);(40,40)"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(40,20);(40,20);(40,40);(40,40)"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(0,20);(0,20);(40,20);(40,20)"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(0,40);(0,40);(0,20);(0,20)"
%	 stroke-width= "0.35"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(20,30)"
%	 text-frame= "noframe"
%	 stroke-width= "0.35"
%	 text-hor-align= "center-h"
%	 >
%$\pizero$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(210,30)"
%	 text-frame= "noframe"
%	 stroke-width= "0.35"
%	 text-hor-align= "center-h"
%	 >
%$\pione$
%</text>
%<multicurve fill-style= "none"
%	 points= "(120,25);(120,25);(110,15);(110,15)"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(110,15);(110,15);(110,0);(110,0)"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(95,35);(95,35);(105,35);(105,35)"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(135,7.5);(135,7.5);(135,52.5);(135,52.5)"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(85,52.5);(85,52.5);(135,52.5);(135,52.5)"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(100,35);(100,35);(100,25);(100,25)"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(100,25);(100,25);(110,15);(110,15)"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(120,35);(120,35);(120,25);(120,25)"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(115,35);(115,35);(125,35);(125,35)"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(115,45);(115,45);(125,45);(125,45)"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(95,45);(95,45);(105,45);(105,45)"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(105,45);(105,45);(105,35);(105,35)"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(115,45);(115,45);(115,35);(115,35)"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(125,45);(125,45);(125,35);(125,35)"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(95,45);(95,45);(95,35);(95,35)"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(100,60);(100,60);(100,45);(100,45)"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(120,60);(120,60);(120,45);(120,45)"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(85,7.5);(85,7.5);(85,52.5);(85,52.5)"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(85,7.5);(85,7.5);(135,7.5);(135,7.5)"
%	 stroke-width= "0.35"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(100,40)"
%	 text-frame= "noframe"
%	 stroke-width= "0.35"
%	 text-hor-align= "center-h"
%	 >
%$\aah$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(120,40)"
%	 text-frame= "noframe"
%	 stroke-width= "0.35"
%	 text-hor-align= "center-h"
%	 >
%$\bbh$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(132.5,15)"
%	 text-frame= "noframe"
%	 stroke-width= "0.35"
%	 text-hor-align= "right"
%	 >
%$\pairr$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(7.5,2.5)"
%	 text-frame= "noframe"
%	 stroke-width= "0.35"
%	 text-hor-align= "right"
%	 >
%$\AAh$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(32.5,2.5)"
%	 text-frame= "noframe"
%	 stroke-width= "0.35"
%	 text-hor-align= "left"
%	 >
%$\BBh$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(97.5,57.5)"
%	 text-frame= "noframe"
%	 stroke-width= "0.35"
%	 text-hor-align= "right"
%	 >
%$\AAh$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(122.5,57.5)"
%	 text-frame= "noframe"
%	 stroke-width= "0.35"
%	 text-hor-align= "left"
%	 >
%$\BBh$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(197.5,2.5)"
%	 text-frame= "noframe"
%	 stroke-width= "0.35"
%	 text-hor-align= "right"
%	 >
%$\AAh$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(222.5,2.5)"
%	 text-frame= "noframe"
%	 stroke-width= "0.35"
%	 text-hor-align= "left"
%	 >
%$\BBh$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(107.5,2.5)"
%	 text-frame= "noframe"
%	 stroke-width= "0.35"
%	 text-hor-align= "right"
%	 >
%$\XXh$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(110,15)"
%	 text-frame= "noframe"
%	 stroke-width= "0.35"
%	 text-hor-align= "center-h"
%	 >
%\DOTT
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(100,45)"
%	 text-frame= "noframe"
%	 stroke-width= "0.35"
%	 text-hor-align= "center-h"
%	 >
%\DOTT
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(120,45)"
%	 text-frame= "noframe"
%	 stroke-width= "0.35"
%	 text-hor-align= "center-h"
%	 >
%\DOTT
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(30,30)"
%	 text-frame= "noframe"
%	 stroke-width= "0.35"
%	 text-hor-align= "center-h"
%	 >
%\DOTT
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(200,30)"
%	 text-frame= "noframe"
%	 stroke-width= "0.35"
%	 text-hor-align= "center-h"
%	 >
%\DOTT
%</text>
%</jpic>
%%End JPIC-XML
%LaTeX-picture environment using emulated lines and arcs
%You can rescale the whole picture (to 80% for instance) by using the command \def\JPicScale{0.8}
\ifx\JPicScale\undefined\def\JPicScale{1}\fi
\unitlength \JPicScale mm
\begin{picture}(230,60)(0,0)
\linethickness{0.35mm}
\put(220,0){\line(0,1){60}}
\linethickness{0.35mm}
\put(200,0){\line(0,1){30}}
\linethickness{0.35mm}
\put(190,40){\line(1,0){40}}
\linethickness{0.35mm}
\put(230,20){\line(0,1){20}}
\linethickness{0.35mm}
\put(190,20){\line(1,0){40}}
\linethickness{0.35mm}
\put(190,20){\line(0,1){20}}
\linethickness{0.35mm}
\put(10,0){\line(0,1){60}}
\linethickness{0.35mm}
\put(30,0){\line(0,1){30.01}}
\linethickness{0.35mm}
\put(0,40){\line(1,0){40}}
\linethickness{0.35mm}
\put(40,20){\line(0,1){20}}
\linethickness{0.35mm}
\put(0,20){\line(1,0){40}}
\linethickness{0.35mm}
\put(0,20){\line(0,1){20}}
\put(20,30){\makebox(0,0)[cc]{$\pizero$}}

\put(210,30){\makebox(0,0)[cc]{$\pione$}}

\linethickness{0.35mm}
\multiput(110,15)(0.12,0.12){83}{\line(1,0){0.12}}
\linethickness{0.35mm}
\put(110,0){\line(0,1){15}}
\linethickness{0.35mm}
\put(95,35){\line(1,0){10}}
\linethickness{0.35mm}
\put(135,7.5){\line(0,1){45}}
\linethickness{0.35mm}
\put(85,52.5){\line(1,0){50}}
\linethickness{0.35mm}
\put(100,25){\line(0,1){10}}
\linethickness{0.35mm}
\multiput(100,25)(0.12,-0.12){83}{\line(1,0){0.12}}
\linethickness{0.35mm}
\put(120,25){\line(0,1){10}}
\linethickness{0.35mm}
\put(115,35){\line(1,0){10}}
\linethickness{0.35mm}
\put(115,45){\line(1,0){10}}
\linethickness{0.35mm}
\put(95,45){\line(1,0){10}}
\linethickness{0.35mm}
\put(105,35){\line(0,1){10}}
\linethickness{0.35mm}
\put(115,35){\line(0,1){10}}
\linethickness{0.35mm}
\put(125,35){\line(0,1){10}}
\linethickness{0.35mm}
\put(95,35){\line(0,1){10}}
\linethickness{0.35mm}
\put(100,45){\line(0,1){15}}
\linethickness{0.35mm}
\put(120,45){\line(0,1){15}}
\linethickness{0.35mm}
\put(85,7.5){\line(0,1){45}}
\linethickness{0.35mm}
\put(85,7.5){\line(1,0){50}}
\put(100,40){\makebox(0,0)[cc]{$\aah$}}

\put(120,40){\makebox(0,0)[cc]{$\bbh$}}

\put(132.5,15){\makebox(0,0)[cr]{$\pairr$}}

\put(7.5,2.5){\makebox(0,0)[cr]{$\AAh$}}

\put(32.5,2.5){\makebox(0,0)[cl]{$\BBh$}}

\put(97.5,57.5){\makebox(0,0)[cr]{$\AAh$}}

\put(122.5,57.5){\makebox(0,0)[cl]{$\BBh$}}

\put(197.5,2.5){\makebox(0,0)[cr]{$\AAh$}}

\put(222.5,2.5){\makebox(0,0)[cl]{$\BBh$}}

\put(107.5,2.5){\makebox(0,0)[cr]{$\XXh$}}

\put(110,15){\makebox(0,0)[cc]{\DOTT}}

\put(100,45){\makebox(0,0)[cc]{\DOTT}}

\put(120,45){\makebox(0,0)[cc]{\DOTT}}

\put(30,30){\makebox(0,0)[cc]{\DOTT}}

\put(200,30){\makebox(0,0)[cc]{\DOTT}}

\end{picture}


==> PIC/projs-surj-1.tex <==
%%Created by jPicEdt 1.4.1_03: mixed JPIC-XML/LaTeX format
%%Fri Sep 11 09:53:47 GMT-10:00 2020
%%Begin JPIC-XML
%<?xml version="1.0" standalone="yes"?>
%<jpic x-min="-10" x-max="322.5" y-min="-10" y-max="100" auto-bounding="true">
%<multicurve fill-style= "none"
%	 points= "(90,100);(90,100);(90,40);(90,40)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(70,70);(70,70);(70,40);(70,40)"
%	 stroke-width= "0.75"
%	 />
%<ellipse p3= "(72.58,67.42)"
%	 fill-style= "solid"
%	 p2= "(72.58,72.58)"
%	 fill-color= "#330033"
%	 p1= "(67.42,72.58)"
%	 closure= "open"
%	 angle-end= "0"
%	 angle-start= "0"
%	 />
%<multicurve fill-style= "none"
%	 points= "(60,80);(60,80);(100,80);(100,80)"
%	 stroke-width= "0.45"
%	 />
%<multicurve fill-style= "none"
%	 points= "(100,60);(100,60);(100,80);(100,80)"
%	 stroke-width= "0.45"
%	 />
%<multicurve fill-style= "none"
%	 points= "(60,60);(60,60);(100,60);(100,60)"
%	 stroke-width= "0.45"
%	 />
%<multicurve fill-style= "none"
%	 points= "(60,80);(60,80);(60,60);(60,60)"
%	 stroke-width= "0.45"
%	 />
%<multicurve fill-style= "none"
%	 points= "(10,100);(10,100);(10,40);(10,40)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(30,70.01);(30,70.01);(30,40);(30,40)"
%	 stroke-width= "0.75"
%	 />
%<ellipse p3= "(32.58,67.42)"
%	 fill-style= "solid"
%	 p2= "(32.58,72.58)"
%	 fill-color= "#330033"
%	 p1= "(27.42,72.58)"
%	 closure= "open"
%	 angle-end= "0"
%	 angle-start= "0"
%	 />
%<multicurve fill-style= "none"
%	 points= "(0,80);(0,80);(40,80);(40,80)"
%	 stroke-width= "0.45"
%	 />
%<multicurve fill-style= "none"
%	 points= "(40,60);(40,60);(40,80);(40,80)"
%	 stroke-width= "0.45"
%	 />
%<multicurve fill-style= "none"
%	 points= "(0,60);(0,60);(40,60);(40,60)"
%	 stroke-width= "0.45"
%	 />
%<multicurve fill-style= "none"
%	 points= "(0,80);(0,80);(0,60);(0,60)"
%	 stroke-width= "0.45"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(20,70)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\pizero$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(80,70)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\pione$
%</text>
%<multicurve fill-style= "none"
%	 points= "(-10,0);(-10,0);(-10,90);(-10,90)"
%	 stroke-width= "1"
%	 />
%<multicurve fill-style= "none"
%	 points= "(-10,90);(-10,90);(110,90);(110,90)"
%	 stroke-width= "1"
%	 />
%<multicurve fill-style= "none"
%	 points= "(110,0);(110,0);(110,90);(110,90)"
%	 stroke-width= "1"
%	 />
%<multicurve fill-style= "none"
%	 points= "(-10,0);(-10,0);(110,0);(110,0)"
%	 stroke-width= "1"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(7.5,42.5)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\AAh$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(32.5,42.5)"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\BBh$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(7.5,97.5)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\AAh$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(92.5,97.5)"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\BBh$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(67.5,42.5)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\AAh$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(92.5,42.5)"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\BBh$
%</text>
%<multicurve fill-style= "none"
%	 points= "(90,40);(90,40);(60,10);(60,10)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(70,40);(70,40);(40,10);(40,10)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 stroke-overstrike-width= "1.55"
%	 points= "(60,10);(60,10);(30,40);(30,40)"
%	 stroke-overstrike= "true"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 stroke-overstrike-width= "1.55"
%	 points= "(40,10);(40,10);(10,40);(10,40)"
%	 stroke-overstrike= "true"
%	 stroke-width= "0.75"
%	 />
%<ellipse p3= "(62.58,7.42)"
%	 fill-style= "solid"
%	 p2= "(62.58,12.58)"
%	 fill-color= "#330033"
%	 p1= "(57.42,12.58)"
%	 closure= "open"
%	 angle-end= "0"
%	 angle-start= "0"
%	 />
%<ellipse p3= "(42.58,7.42)"
%	 fill-style= "solid"
%	 p2= "(42.58,12.58)"
%	 fill-color= "#330033"
%	 p1= "(37.42,12.58)"
%	 closure= "open"
%	 angle-end= "0"
%	 angle-start= "0"
%	 />
%<multicurve fill-style= "none"
%	 points= "(60,10);(60,10);(60,-10);(60,-10)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(40,10);(40,10);(40,-10);(40,-10)"
%	 stroke-width= "0.75"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(62.5,-7.5)"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\BBh$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(37.5,-7.5)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\AAh$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(135,45)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\EQLS
%</text>
%<multicurve fill-style= "none"
%	 points= "(240,100);(240,100);(240,40);(240,40)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(210,70);(210,70);(210,40);(210,40)"
%	 stroke-width= "0.75"
%	 />
%<ellipse p3= "(212.58,67.42)"
%	 fill-style= "solid"
%	 p2= "(212.58,72.58)"
%	 fill-color= "#330033"
%	 p1= "(207.42,72.58)"
%	 closure= "open"
%	 angle-end= "0"
%	 angle-start= "0"
%	 />
%<multicurve fill-style= "none"
%	 points= "(160,100);(160,100);(160,40);(160,40)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(190,70);(190,70);(190,39.99);(190,39.99)"
%	 stroke-width= "0.75"
%	 />
%<ellipse p3= "(192.58,67.42)"
%	 fill-style= "solid"
%	 p2= "(192.58,72.58)"
%	 fill-color= "#330033"
%	 p1= "(187.42,72.58)"
%	 closure= "open"
%	 angle-end= "0"
%	 angle-start= "0"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(157.5,97.5)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\AAh$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(242.5,97.5)"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\BBh$
%</text>
%<multicurve fill-style= "none"
%	 points= "(240,40);(240,40);(225,25);(225,25)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(190,40);(190,40);(175,25);(175,25)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 stroke-overstrike-width= "1.55"
%	 points= "(225,25);(225,25);(210,40);(210,40)"
%	 stroke-overstrike= "true"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 stroke-overstrike-width= "1.55"
%	 points= "(175,25);(175,25);(160,40);(160,40)"
%	 stroke-overstrike= "true"
%	 stroke-width= "0.75"
%	 />
%<ellipse p3= "(227.58,22.42)"
%	 fill-style= "solid"
%	 p2= "(227.58,27.58)"
%	 fill-color= "#330033"
%	 p1= "(222.42,27.58)"
%	 closure= "open"
%	 angle-end= "0"
%	 angle-start= "0"
%	 />
%<ellipse p3= "(177.58,22.42)"
%	 fill-style= "solid"
%	 p2= "(177.58,27.58)"
%	 fill-color= "#330033"
%	 p1= "(172.42,27.58)"
%	 closure= "open"
%	 angle-end= "0"
%	 angle-start= "0"
%	 />
%<multicurve fill-style= "none"
%	 points= "(225,25);(225,25);(225,-10);(225,-10)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(175,25);(175,25);(175,-10);(175,-10)"
%	 stroke-width= "0.75"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(227.5,-7.5)"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\BBh$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(172.5,-7.5)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\AAh$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(322.5,53.75)"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%\eempty
%</text>
%</jpic>
%%End JPIC-XML
%PSTricks content-type (pstricks.sty package needed)
%Add \usepackage{pstricks} in the preamble of your LaTeX file
%You can rescale the whole picture (to 80% for instance) by using the command \def\JPicScale{0.8}
\ifx\JPicScale\undefined\def\JPicScale{1}\fi
\psset{unit=\JPicScale mm}
\psset{linewidth=0.3,dotsep=1,hatchwidth=0.3,hatchsep=1.5,shadowsize=1,dimen=middle}
\psset{dotsize=0.7 2.5,dotscale=1 1,fillcolor=black}
\psset{arrowsize=1 2,arrowlength=1,arrowinset=0.25,tbarsize=0.7 5,bracketlength=0.15,rbracketlength=0.15}
\begin{pspicture}(0,0)(322.5,100)
\psline[linewidth=0.75](90,100)(90,40)
\psline[linewidth=0.75](70,70)(70,40)
\newrgbcolor{userFillColour}{0.2 0 0.2}
\rput{0}(70,70){\psellipse[fillcolor=userFillColour,fillstyle=solid](0,0)(2.58,-2.58)}
\psline[linewidth=0.45](60,80)(100,80)
\psline[linewidth=0.45](100,60)(100,80)
\psline[linewidth=0.45](60,60)(100,60)
\psline[linewidth=0.45](60,80)(60,60)
\psline[linewidth=0.75](10,100)(10,40)
\psline[linewidth=0.75](30,70.01)(30,40)
\newrgbcolor{userFillColour}{0.2 0 0.2}
\rput{0}(30,70){\psellipse[fillcolor=userFillColour,fillstyle=solid](0,0)(2.58,-2.58)}
\psline[linewidth=0.45](0,80)(40,80)
\psline[linewidth=0.45](40,60)(40,80)
\psline[linewidth=0.45](0,60)(40,60)
\psline[linewidth=0.45](0,80)(0,60)
\rput(20,70){$\pizero$}
\rput(80,70){$\pione$}
\psline[linewidth=1](-10,0)(-10,90)
\psline[linewidth=1](-10,90)(110,90)
\psline[linewidth=1](110,0)(110,90)
\psline[linewidth=1](-10,0)(110,0)
\rput[r](7.5,42.5){$\AAh$}
\rput[l](32.5,42.5){$\BBh$}
\rput[r](7.5,97.5){$\AAh$}
\rput[l](92.5,97.5){$\BBh$}
\rput[r](67.5,42.5){$\AAh$}
\rput[l](92.5,42.5){$\BBh$}
\psline[linewidth=0.75](90,40)(60,10)
\psline[linewidth=0.75](70,40)(40,10)
\psline[linewidth=0.75,border=1.55](60,10)(30,40)
\psline[linewidth=0.75,border=1.55](40,10)(10,40)
\newrgbcolor{userFillColour}{0.2 0 0.2}
\rput{0}(60,10){\psellipse[fillcolor=userFillColour,fillstyle=solid](0,0)(2.58,-2.58)}
\newrgbcolor{userFillColour}{0.2 0 0.2}
\rput{0}(40,10){\psellipse[fillcolor=userFillColour,fillstyle=solid](0,0)(2.58,-2.58)}
\psline[linewidth=0.75](60,10)(60,-10)
\psline[linewidth=0.75](40,10)(40,-10)
\rput[l](62.5,-7.5){$\BBh$}
\rput[r](37.5,-7.5){$\AAh$}
\rput(135,45){\EQLS}
\psline[linewidth=0.75](240,100)(240,40)
\psline[linewidth=0.75](210,70)(210,40)
\newrgbcolor{userFillColour}{0.2 0 0.2}
\rput{0}(210,70){\psellipse[fillcolor=userFillColour,fillstyle=solid](0,0)(2.58,-2.58)}
\psline[linewidth=0.75](160,100)(160,40)
\psline[linewidth=0.75](190,70)(190,39.99)
\newrgbcolor{userFillColour}{0.2 0 0.2}
\rput{0}(190,70){\psellipse[fillcolor=userFillColour,fillstyle=solid](0,0)(2.58,-2.58)}
\rput[r](157.5,97.5){$\AAh$}
\rput[l](242.5,97.5){$\BBh$}
\psline[linewidth=0.75](240,40)(225,25)
\psline[linewidth=0.75](190,40)(175,25)
\psline[linewidth=0.75,border=1.55](225,25)(210,40)
\psline[linewidth=0.75,border=1.55](175,25)(160,40)
\newrgbcolor{userFillColour}{0.2 0 0.2}
\rput{0}(225,25){\psellipse[fillcolor=userFillColour,fillstyle=solid](0,0)(2.58,-2.58)}
\newrgbcolor{userFillColour}{0.2 0 0.2}
\rput{0}(175,25){\psellipse[fillcolor=userFillColour,fillstyle=solid](0,0)(2.58,-2.58)}
\psline[linewidth=0.75](225,25)(225,-10)
\psline[linewidth=0.75](175,25)(175,-10)
\rput[l](227.5,-7.5){$\BBh$}
\rput[r](172.5,-7.5){$\AAh$}
\rput[l](322.5,53.75){\eempty}
\end{pspicture}


==> PIC/projs-surj-2.tex <==
%%Created by jPicEdt 1.4.1_03: mixed JPIC-XML/LaTeX format
%%Fri Sep 11 09:54:14 GMT-10:00 2020
%%Begin JPIC-XML
%<?xml version="1.0" standalone="yes"?>
%<jpic x-min="-10" x-max="322.5" y-min="-10" y-max="100" auto-bounding="true">
%<multicurve fill-style= "none"
%	 points= "(90,100);(90,100);(90,40);(90,40)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(70,70);(70,70);(70,40);(70,40)"
%	 stroke-width= "0.75"
%	 />
%<ellipse p3= "(72.58,67.42)"
%	 fill-style= "solid"
%	 p2= "(72.58,72.58)"
%	 fill-color= "#330033"
%	 p1= "(67.42,72.58)"
%	 closure= "open"
%	 angle-end= "0"
%	 angle-start= "0"
%	 />
%<multicurve fill-style= "none"
%	 points= "(60,80);(60,80);(100,80);(100,80)"
%	 stroke-width= "0.45"
%	 />
%<multicurve fill-style= "none"
%	 points= "(100,60);(100,60);(100,80);(100,80)"
%	 stroke-width= "0.45"
%	 />
%<multicurve fill-style= "none"
%	 points= "(60,60);(60,60);(100,60);(100,60)"
%	 stroke-width= "0.45"
%	 />
%<multicurve fill-style= "none"
%	 points= "(60,80);(60,80);(60,60);(60,60)"
%	 stroke-width= "0.45"
%	 />
%<multicurve fill-style= "none"
%	 points= "(10,100);(10,100);(10,40);(10,40)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(30,70.01);(30,70.01);(30,40);(30,40)"
%	 stroke-width= "0.75"
%	 />
%<ellipse p3= "(32.58,67.42)"
%	 fill-style= "solid"
%	 p2= "(32.58,72.58)"
%	 fill-color= "#330033"
%	 p1= "(27.42,72.58)"
%	 closure= "open"
%	 angle-end= "0"
%	 angle-start= "0"
%	 />
%<multicurve fill-style= "none"
%	 points= "(0,80);(0,80);(40,80);(40,80)"
%	 stroke-width= "0.45"
%	 />
%<multicurve fill-style= "none"
%	 points= "(40,60);(40,60);(40,80);(40,80)"
%	 stroke-width= "0.45"
%	 />
%<multicurve fill-style= "none"
%	 points= "(0,60);(0,60);(40,60);(40,60)"
%	 stroke-width= "0.45"
%	 />
%<multicurve fill-style= "none"
%	 points= "(0,80);(0,80);(0,60);(0,60)"
%	 stroke-width= "0.45"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(20,70)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\pizero$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(80,70)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\pione$
%</text>
%<multicurve fill-style= "none"
%	 points= "(-10,0);(-10,0);(-10,90);(-10,90)"
%	 stroke-width= "1"
%	 />
%<multicurve fill-style= "none"
%	 points= "(-10,90);(-10,90);(110,90);(110,90)"
%	 stroke-width= "1"
%	 />
%<multicurve fill-style= "none"
%	 points= "(110,0);(110,0);(110,90);(110,90)"
%	 stroke-width= "1"
%	 />
%<multicurve fill-style= "none"
%	 points= "(-10,0);(-10,0);(110,0);(110,0)"
%	 stroke-width= "1"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(7.5,42.5)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\AAh$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(32.5,42.5)"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\BBh$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(7.5,97.5)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\AAh$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(92.5,97.5)"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\BBh$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(67.5,42.5)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\AAh$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(92.5,42.5)"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\BBh$
%</text>
%<multicurve fill-style= "none"
%	 points= "(90,40);(90,40);(60,10);(60,10)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(70,40);(70,40);(40,10);(40,10)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 stroke-overstrike-width= "1.55"
%	 points= "(60,10);(60,10);(30,40);(30,40)"
%	 stroke-overstrike= "true"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 stroke-overstrike-width= "1.55"
%	 points= "(40,10);(40,10);(10,40);(10,40)"
%	 stroke-overstrike= "true"
%	 stroke-width= "0.75"
%	 />
%<ellipse p3= "(62.58,7.42)"
%	 fill-style= "solid"
%	 p2= "(62.58,12.58)"
%	 fill-color= "#330033"
%	 p1= "(57.42,12.58)"
%	 closure= "open"
%	 angle-end= "0"
%	 angle-start= "0"
%	 />
%<ellipse p3= "(42.58,7.42)"
%	 fill-style= "solid"
%	 p2= "(42.58,12.58)"
%	 fill-color= "#330033"
%	 p1= "(37.42,12.58)"
%	 closure= "open"
%	 angle-end= "0"
%	 angle-start= "0"
%	 />
%<multicurve fill-style= "none"
%	 points= "(60,10);(60,10);(60,-10);(60,-10)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(40,10);(40,10);(40,-10);(40,-10)"
%	 stroke-width= "0.75"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(62.5,-7.5)"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\BBh$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(37.5,-7.5)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\AAh$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(322.5,53.75)"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%\eempty
%</text>
%</jpic>
%%End JPIC-XML
%PSTricks content-type (pstricks.sty package needed)
%Add \usepackage{pstricks} in the preamble of your LaTeX file
%You can rescale the whole picture (to 80% for instance) by using the command \def\JPicScale{0.8}
\ifx\JPicScale\undefined\def\JPicScale{1}\fi
\psset{unit=\JPicScale mm}
\psset{linewidth=0.3,dotsep=1,hatchwidth=0.3,hatchsep=1.5,shadowsize=1,dimen=middle}
\psset{dotsize=0.7 2.5,dotscale=1 1,fillcolor=black}
\psset{arrowsize=1 2,arrowlength=1,arrowinset=0.25,tbarsize=0.7 5,bracketlength=0.15,rbracketlength=0.15}
\begin{pspicture}(0,0)(322.5,100)
\psline[linewidth=0.75](90,100)(90,40)
\psline[linewidth=0.75](70,70)(70,40)
\newrgbcolor{userFillColour}{0.2 0 0.2}
\rput{0}(70,70){\psellipse[fillcolor=userFillColour,fillstyle=solid](0,0)(2.58,-2.58)}
\psline[linewidth=0.45](60,80)(100,80)
\psline[linewidth=0.45](100,60)(100,80)
\psline[linewidth=0.45](60,60)(100,60)
\psline[linewidth=0.45](60,80)(60,60)
\psline[linewidth=0.75](10,100)(10,40)
\psline[linewidth=0.75](30,70.01)(30,40)
\newrgbcolor{userFillColour}{0.2 0 0.2}
\rput{0}(30,70){\psellipse[fillcolor=userFillColour,fillstyle=solid](0,0)(2.58,-2.58)}
\psline[linewidth=0.45](0,80)(40,80)
\psline[linewidth=0.45](40,60)(40,80)
\psline[linewidth=0.45](0,60)(40,60)
\psline[linewidth=0.45](0,80)(0,60)
\rput(20,70){$\pizero$}
\rput(80,70){$\pione$}
\psline[linewidth=1](-10,0)(-10,90)
\psline[linewidth=1](-10,90)(110,90)
\psline[linewidth=1](110,0)(110,90)
\psline[linewidth=1](-10,0)(110,0)
\rput[r](7.5,42.5){$\AAh$}
\rput[l](32.5,42.5){$\BBh$}
\rput[r](7.5,97.5){$\AAh$}
\rput[l](92.5,97.5){$\BBh$}
\rput[r](67.5,42.5){$\AAh$}
\rput[l](92.5,42.5){$\BBh$}
\psline[linewidth=0.75](90,40)(60,10)
\psline[linewidth=0.75](70,40)(40,10)
\psline[linewidth=0.75,border=1.55](60,10)(30,40)
\psline[linewidth=0.75,border=1.55](40,10)(10,40)
\newrgbcolor{userFillColour}{0.2 0 0.2}
\rput{0}(60,10){\psellipse[fillcolor=userFillColour,fillstyle=solid](0,0)(2.58,-2.58)}
\newrgbcolor{userFillColour}{0.2 0 0.2}
\rput{0}(40,10){\psellipse[fillcolor=userFillColour,fillstyle=solid](0,0)(2.58,-2.58)}
\psline[linewidth=0.75](60,10)(60,-10)
\psline[linewidth=0.75](40,10)(40,-10)
\rput[l](62.5,-7.5){$\BBh$}
\rput[r](37.5,-7.5){$\AAh$}
\rput[l](322.5,53.75){\eempty}
\end{pspicture}


==> PIC/projs-surj-3.tex <==
%%Created by jPicEdt 1.4.1_03: mixed JPIC-XML/LaTeX format
%%Fri Sep 11 09:56:19 GMT-10:00 2020
%%Begin JPIC-XML
%<?xml version="1.0" standalone="yes"?>
%<jpic x-min="-10" x-max="322.5" y-min="0" y-max="100" auto-bounding="true">
%<multicurve fill-style= "none"
%	 points= "(90,100);(90,100);(90,40);(90,40)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(70,70);(70,70);(70,40);(70,40)"
%	 stroke-width= "0.75"
%	 />
%<ellipse p3= "(72.58,67.42)"
%	 fill-style= "solid"
%	 p2= "(72.58,72.58)"
%	 fill-color= "#330033"
%	 p1= "(67.42,72.58)"
%	 closure= "open"
%	 angle-end= "0"
%	 angle-start= "0"
%	 />
%<multicurve fill-style= "none"
%	 points= "(60,80);(60,80);(100,80);(100,80)"
%	 stroke-width= "0.45"
%	 />
%<multicurve fill-style= "none"
%	 points= "(100,60);(100,60);(100,80);(100,80)"
%	 stroke-width= "0.45"
%	 />
%<multicurve fill-style= "none"
%	 points= "(60,60);(60,60);(100,60);(100,60)"
%	 stroke-width= "0.45"
%	 />
%<multicurve fill-style= "none"
%	 points= "(60,80);(60,80);(60,60);(60,60)"
%	 stroke-width= "0.45"
%	 />
%<multicurve fill-style= "none"
%	 points= "(10,100);(10,100);(10,40);(10,40)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(30,70.01);(30,70.01);(30,40);(30,40)"
%	 stroke-width= "0.75"
%	 />
%<ellipse p3= "(32.58,67.42)"
%	 fill-style= "solid"
%	 p2= "(32.58,72.58)"
%	 fill-color= "#330033"
%	 p1= "(27.42,72.58)"
%	 closure= "open"
%	 angle-end= "0"
%	 angle-start= "0"
%	 />
%<multicurve fill-style= "none"
%	 points= "(0,80);(0,80);(40,80);(40,80)"
%	 stroke-width= "0.45"
%	 />
%<multicurve fill-style= "none"
%	 points= "(40,60);(40,60);(40,80);(40,80)"
%	 stroke-width= "0.45"
%	 />
%<multicurve fill-style= "none"
%	 points= "(0,60);(0,60);(40,60);(40,60)"
%	 stroke-width= "0.45"
%	 />
%<multicurve fill-style= "none"
%	 points= "(0,80);(0,80);(0,60);(0,60)"
%	 stroke-width= "0.45"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(20,70)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\pizero$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(80,70)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\pione$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(7.5,42.5)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\AAh$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(32.5,42.5)"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\BBh$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(7.5,97.5)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\AAh$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(92.5,97.5)"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\BBh$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(67.5,42.5)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\AAh$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(92.5,42.5)"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\BBh$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(322.5,53.75)"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%\eempty
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(50,0)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\eempty
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(-10,90)"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%\eempty
%</text>
%</jpic>
%%End JPIC-XML
%PSTricks content-type (pstricks.sty package needed)
%Add \usepackage{pstricks} in the preamble of your LaTeX file
%You can rescale the whole picture (to 80% for instance) by using the command \def\JPicScale{0.8}
\ifx\JPicScale\undefined\def\JPicScale{1}\fi
\psset{unit=\JPicScale mm}
\psset{linewidth=0.3,dotsep=1,hatchwidth=0.3,hatchsep=1.5,shadowsize=1,dimen=middle}
\psset{dotsize=0.7 2.5,dotscale=1 1,fillcolor=black}
\psset{arrowsize=1 2,arrowlength=1,arrowinset=0.25,tbarsize=0.7 5,bracketlength=0.15,rbracketlength=0.15}
\begin{pspicture}(0,0)(322.5,100)
\psline[linewidth=0.75](90,100)(90,40)
\psline[linewidth=0.75](70,70)(70,40)
\newrgbcolor{userFillColour}{0.2 0 0.2}
\rput{0}(70,70){\psellipse[fillcolor=userFillColour,fillstyle=solid](0,0)(2.58,-2.58)}
\psline[linewidth=0.45](60,80)(100,80)
\psline[linewidth=0.45](100,60)(100,80)
\psline[linewidth=0.45](60,60)(100,60)
\psline[linewidth=0.45](60,80)(60,60)
\psline[linewidth=0.75](10,100)(10,40)
\psline[linewidth=0.75](30,70.01)(30,40)
\newrgbcolor{userFillColour}{0.2 0 0.2}
\rput{0}(30,70){\psellipse[fillcolor=userFillColour,fillstyle=solid](0,0)(2.58,-2.58)}
\psline[linewidth=0.45](0,80)(40,80)
\psline[linewidth=0.45](40,60)(40,80)
\psline[linewidth=0.45](0,60)(40,60)
\psline[linewidth=0.45](0,80)(0,60)
\rput(20,70){$\pizero$}
\rput(80,70){$\pione$}
\rput[r](7.5,42.5){$\AAh$}
\rput[l](32.5,42.5){$\BBh$}
\rput[r](7.5,97.5){$\AAh$}
\rput[l](92.5,97.5){$\BBh$}
\rput[r](67.5,42.5){$\AAh$}
\rput[l](92.5,42.5){$\BBh$}
\rput[l](322.5,53.75){\eempty}
\rput(50,0){\eempty}
\rput[l](-10,90){\eempty}
\end{pspicture}


==> PIC/projs-surj-h.tex <==
%%Created by jPicEdt 1.4.1_03: mixed JPIC-XML/LaTeX format
%%Fri Aug 26 13:36:55 GMT-10:00 2022
%%Begin JPIC-XML
%<?xml version="1.0" standalone="yes"?>
%<jpic x-min="0" x-max="230" y-min="0" y-max="110" auto-bounding="true">
%<multicurve fill-style= "none"
%	 points= "(220,110);(220,110);(220,90);(220,90)"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(210,70);(210,70);(210,50);(210,50)"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(190,90);(190,90);(230,90);(230,90)"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(230,70);(230,70);(230,90);(230,90)"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(190,70);(190,70);(230,70);(230,70)"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(190,90);(190,90);(190,70);(190,70)"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(150,70);(150,70);(150,50);(150,50)"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(160,110);(160,110);(160,90);(160,90)"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(130,90);(130,90);(170,90);(170,90)"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(170,70);(170,70);(170,90);(170,90)"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(130,70);(130,70);(170,70);(170,70)"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(130,90);(130,90);(130,70);(130,70)"
%	 stroke-width= "0.35"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(150,80)"
%	 text-frame= "noframe"
%	 stroke-width= "0.35"
%	 text-hor-align= "center-h"
%	 >
%$\pizero$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(210,80)"
%	 text-frame= "noframe"
%	 stroke-width= "0.35"
%	 text-hor-align= "center-h"
%	 >
%$\pione$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(162.5,108.75)"
%	 text-frame= "noframe"
%	 stroke-width= "0.35"
%	 text-hor-align= "left"
%	 >
%$\BBh$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(142.5,108.75)"
%	 text-frame= "noframe"
%	 stroke-width= "0.35"
%	 text-hor-align= "left"
%	 >
%$\AAh$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(222.5,108.75)"
%	 text-frame= "noframe"
%	 stroke-width= "0.35"
%	 text-hor-align= "left"
%	 >
%$\BBh$
%</text>
%<multicurve fill-style= "none"
%	 points= "(140,110);(140,110);(140,90);(140,90)"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(210,50);(210,50);(180,20);(180,20)"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(180,20);(180,20);(150,50);(150,50)"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(200,110);(200,110);(200,90);(200,90)"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(180,20);(180,20);(180,0);(180,0)"
%	 stroke-width= "0.35"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(203.75,108.75)"
%	 text-frame= "noframe"
%	 stroke-width= "0.35"
%	 text-hor-align= "left"
%	 >
%$\AAh$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(100,60)"
%	 text-frame= "noframe"
%	 stroke-width= "0.35"
%	 text-hor-align= "center-h"
%	 >
%\EQLS
%</text>
%<multicurve fill-style= "none"
%	 points= "(80,110);(80,110);(80,90);(80,90)"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(60,110);(60,110);(60,90);(60,90)"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(0,110);(0,110);(0,90);(0,90)"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(20,110);(20,110);(20,90);(20,90)"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(20,40);(20,40);(60,40);(60,40)"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(60,20);(60,20);(60,40);(60,40)"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(20,20);(20,20);(60,20);(60,20)"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(20,40);(20,40);(20,20);(20,20)"
%	 stroke-width= "0.35"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(40,30)"
%	 text-frame= "noframe"
%	 stroke-width= "0.35"
%	 text-hor-align= "center-h"
%	 >
%$\pizero$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(3.75,108.75)"
%	 text-frame= "noframe"
%	 stroke-width= "0.35"
%	 text-hor-align= "left"
%	 >
%$\AAh$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(22.5,108.75)"
%	 text-frame= "noframe"
%	 stroke-width= "0.35"
%	 text-hor-align= "left"
%	 >
%$\BBh$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(62.5,108.75)"
%	 text-frame= "noframe"
%	 stroke-width= "0.35"
%	 text-hor-align= "left"
%	 >
%$\AAh$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(82.5,108.75)"
%	 text-frame= "noframe"
%	 stroke-width= "0.35"
%	 text-hor-align= "left"
%	 >
%$\BBh$
%</text>
%<multicurve fill-style= "none"
%	 points= "(80,90);(80,90);(50,60);(50,60)"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(60,90);(60,90);(30,60);(30,60)"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(50,60);(50,60);(20,90);(20,90)"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(30,60);(30,60);(0,90);(0,90)"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(50,60);(50,60);(50,40);(50,40)"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(30,60);(30,60);(30,40);(30,40)"
%	 stroke-width= "0.35"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(52.5,50)"
%	 text-frame= "noframe"
%	 stroke-width= "0.35"
%	 text-hor-align= "left"
%	 >
%$\BBh$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(27.5,50)"
%	 text-frame= "noframe"
%	 stroke-width= "0.35"
%	 text-hor-align= "right"
%	 >
%$\AAh$
%</text>
%<multicurve fill-style= "none"
%	 points= "(40,20);(40,20);(40,0);(40,0)"
%	 stroke-width= "0.35"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(177.5,2.5)"
%	 text-frame= "noframe"
%	 stroke-width= "0.35"
%	 text-hor-align= "right"
%	 >
%$\XXh$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(37.5,2.5)"
%	 text-frame= "noframe"
%	 stroke-width= "0.35"
%	 text-hor-align= "right"
%	 >
%$\XXh$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(180,20)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\Dottt
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(30,60)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\Dottt
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(50,60)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\Dottt
%</text>
%</jpic>
%%End JPIC-XML
%LaTeX-picture environment using emulated lines and arcs
%You can rescale the whole picture (to 80% for instance) by using the command \def\JPicScale{0.8}
\ifx\JPicScale\undefined\def\JPicScale{1}\fi
\unitlength \JPicScale mm
\begin{picture}(230,110)(0,0)
\linethickness{0.35mm}
\put(220,90){\line(0,1){20}}
\linethickness{0.35mm}
\put(210,50){\line(0,1){20}}
\linethickness{0.35mm}
\put(190,90){\line(1,0){40}}
\linethickness{0.35mm}
\put(230,70){\line(0,1){20}}
\linethickness{0.35mm}
\put(190,70){\line(1,0){40}}
\linethickness{0.35mm}
\put(190,70){\line(0,1){20}}
\linethickness{0.35mm}
\put(150,50){\line(0,1){20}}
\linethickness{0.35mm}
\put(160,90){\line(0,1){20}}
\linethickness{0.35mm}
\put(130,90){\line(1,0){40}}
\linethickness{0.35mm}
\put(170,70){\line(0,1){20}}
\linethickness{0.35mm}
\put(130,70){\line(1,0){40}}
\linethickness{0.35mm}
\put(130,70){\line(0,1){20}}
\put(150,80){\makebox(0,0)[cc]{$\pizero$}}

\put(210,80){\makebox(0,0)[cc]{$\pione$}}

\put(162.5,108.75){\makebox(0,0)[cl]{$\BBh$}}

\put(142.5,108.75){\makebox(0,0)[cl]{$\AAh$}}

\put(222.5,108.75){\makebox(0,0)[cl]{$\BBh$}}

\linethickness{0.35mm}
\put(140,90){\line(0,1){20}}
\linethickness{0.35mm}
\multiput(180,20)(0.12,0.12){250}{\line(1,0){0.12}}
\linethickness{0.35mm}
\multiput(150,50)(0.12,-0.12){250}{\line(1,0){0.12}}
\linethickness{0.35mm}
\put(200,90){\line(0,1){20}}
\linethickness{0.35mm}
\put(180,0){\line(0,1){20}}
\put(203.75,108.75){\makebox(0,0)[cl]{$\AAh$}}

\put(100,60){\makebox(0,0)[cc]{\EQLS}}

\linethickness{0.35mm}
\put(80,90){\line(0,1){20}}
\linethickness{0.35mm}
\put(60,90){\line(0,1){20}}
\linethickness{0.35mm}
\put(0,90){\line(0,1){20}}
\linethickness{0.35mm}
\put(20,90){\line(0,1){20}}
\linethickness{0.35mm}
\put(20,40){\line(1,0){40}}
\linethickness{0.35mm}
\put(60,20){\line(0,1){20}}
\linethickness{0.35mm}
\put(20,20){\line(1,0){40}}
\linethickness{0.35mm}
\put(20,20){\line(0,1){20}}
\put(40,30){\makebox(0,0)[cc]{$\pizero$}}

\put(3.75,108.75){\makebox(0,0)[cl]{$\AAh$}}

\put(22.5,108.75){\makebox(0,0)[cl]{$\BBh$}}

\put(62.5,108.75){\makebox(0,0)[cl]{$\AAh$}}

\put(82.5,108.75){\makebox(0,0)[cl]{$\BBh$}}

\linethickness{0.35mm}
\multiput(50,60)(0.12,0.12){250}{\line(1,0){0.12}}
\linethickness{0.35mm}
\multiput(30,60)(0.12,0.12){250}{\line(1,0){0.12}}
\linethickness{0.35mm}
\multiput(20,90)(0.12,-0.12){250}{\line(1,0){0.12}}
\linethickness{0.35mm}
\multiput(0,90)(0.12,-0.12){250}{\line(1,0){0.12}}
\linethickness{0.35mm}
\put(50,40){\line(0,1){20}}
\linethickness{0.35mm}
\put(30,40){\line(0,1){20}}
\put(52.5,50){\makebox(0,0)[cl]{$\BBh$}}

\put(27.5,50){\makebox(0,0)[cr]{$\AAh$}}

\linethickness{0.35mm}
\put(40,0){\line(0,1){20}}
\put(177.5,2.5){\makebox(0,0)[cr]{$\XXh$}}

\put(37.5,2.5){\makebox(0,0)[cr]{$\XXh$}}

\put(180,20){\makebox(0,0)[cc]{\Dottt}}

\put(30,60){\makebox(0,0)[cc]{\Dottt}}

\put(50,60){\makebox(0,0)[cc]{\Dottt}}

\end{picture}


==> PIC/projs-surj.tex <==
%%Created by jPicEdt 1.4.1_03: mixed JPIC-XML/LaTeX format
%%Fri Sep 11 09:53:04 GMT-10:00 2020
%%Begin JPIC-XML
%<?xml version="1.0" standalone="yes"?>
%<jpic x-min="-10" x-max="322.5" y-min="-10" y-max="100" auto-bounding="true">
%<multicurve fill-style= "none"
%	 points= "(90,100);(90,100);(90,40);(90,40)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(70,70);(70,70);(70,40);(70,40)"
%	 stroke-width= "0.75"
%	 />
%<ellipse p3= "(72.58,67.42)"
%	 fill-style= "solid"
%	 p2= "(72.58,72.58)"
%	 fill-color= "#330033"
%	 p1= "(67.42,72.58)"
%	 closure= "open"
%	 angle-end= "0"
%	 angle-start= "0"
%	 />
%<multicurve fill-style= "none"
%	 points= "(60,80);(60,80);(100,80);(100,80)"
%	 stroke-width= "0.45"
%	 />
%<multicurve fill-style= "none"
%	 points= "(100,60);(100,60);(100,80);(100,80)"
%	 stroke-width= "0.45"
%	 />
%<multicurve fill-style= "none"
%	 points= "(60,60);(60,60);(100,60);(100,60)"
%	 stroke-width= "0.45"
%	 />
%<multicurve fill-style= "none"
%	 points= "(60,80);(60,80);(60,60);(60,60)"
%	 stroke-width= "0.45"
%	 />
%<multicurve fill-style= "none"
%	 points= "(10,100);(10,100);(10,40);(10,40)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(30,70.01);(30,70.01);(30,40);(30,40)"
%	 stroke-width= "0.75"
%	 />
%<ellipse p3= "(32.58,67.42)"
%	 fill-style= "solid"
%	 p2= "(32.58,72.58)"
%	 fill-color= "#330033"
%	 p1= "(27.42,72.58)"
%	 closure= "open"
%	 angle-end= "0"
%	 angle-start= "0"
%	 />
%<multicurve fill-style= "none"
%	 points= "(0,80);(0,80);(40,80);(40,80)"
%	 stroke-width= "0.45"
%	 />
%<multicurve fill-style= "none"
%	 points= "(40,60);(40,60);(40,80);(40,80)"
%	 stroke-width= "0.45"
%	 />
%<multicurve fill-style= "none"
%	 points= "(0,60);(0,60);(40,60);(40,60)"
%	 stroke-width= "0.45"
%	 />
%<multicurve fill-style= "none"
%	 points= "(0,80);(0,80);(0,60);(0,60)"
%	 stroke-width= "0.45"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(20,70)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\pizero$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(80,70)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\pione$
%</text>
%<multicurve fill-style= "none"
%	 points= "(-10,0);(-10,0);(-10,90);(-10,90)"
%	 stroke-width= "1"
%	 />
%<multicurve fill-style= "none"
%	 points= "(-10,90);(-10,90);(110,90);(110,90)"
%	 stroke-width= "1"
%	 />
%<multicurve fill-style= "none"
%	 points= "(110,0);(110,0);(110,90);(110,90)"
%	 stroke-width= "1"
%	 />
%<multicurve fill-style= "none"
%	 points= "(-10,0);(-10,0);(110,0);(110,0)"
%	 stroke-width= "1"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(7.5,42.5)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\AAh$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(32.5,42.5)"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\BBh$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(7.5,97.5)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\AAh$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(92.5,97.5)"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\BBh$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(67.5,42.5)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\AAh$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(92.5,42.5)"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\BBh$
%</text>
%<multicurve fill-style= "none"
%	 points= "(90,40);(90,40);(60,10);(60,10)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(70,40);(70,40);(40,10);(40,10)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 stroke-overstrike-width= "1.55"
%	 points= "(60,10);(60,10);(30,40);(30,40)"
%	 stroke-overstrike= "true"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 stroke-overstrike-width= "1.55"
%	 points= "(40,10);(40,10);(10,40);(10,40)"
%	 stroke-overstrike= "true"
%	 stroke-width= "0.75"
%	 />
%<ellipse p3= "(62.58,7.42)"
%	 fill-style= "solid"
%	 p2= "(62.58,12.58)"
%	 fill-color= "#330033"
%	 p1= "(57.42,12.58)"
%	 closure= "open"
%	 angle-end= "0"
%	 angle-start= "0"
%	 />
%<ellipse p3= "(42.58,7.42)"
%	 fill-style= "solid"
%	 p2= "(42.58,12.58)"
%	 fill-color= "#330033"
%	 p1= "(37.42,12.58)"
%	 closure= "open"
%	 angle-end= "0"
%	 angle-start= "0"
%	 />
%<multicurve fill-style= "none"
%	 points= "(60,10);(60,10);(60,-10);(60,-10)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(40,10);(40,10);(40,-10);(40,-10)"
%	 stroke-width= "0.75"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(62.5,-7.5)"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\BBh$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(37.5,-7.5)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\AAh$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(135,45)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\EQLS
%</text>
%<multicurve fill-style= "none"
%	 points= "(240,100);(240,100);(240,40);(240,40)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(210,70);(210,70);(210,40);(210,40)"
%	 stroke-width= "0.75"
%	 />
%<ellipse p3= "(212.58,67.42)"
%	 fill-style= "solid"
%	 p2= "(212.58,72.58)"
%	 fill-color= "#330033"
%	 p1= "(207.42,72.58)"
%	 closure= "open"
%	 angle-end= "0"
%	 angle-start= "0"
%	 />
%<multicurve fill-style= "none"
%	 points= "(160,100);(160,100);(160,40);(160,40)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(190,70);(190,70);(190,39.99);(190,39.99)"
%	 stroke-width= "0.75"
%	 />
%<ellipse p3= "(192.58,67.42)"
%	 fill-style= "solid"
%	 p2= "(192.58,72.58)"
%	 fill-color= "#330033"
%	 p1= "(187.42,72.58)"
%	 closure= "open"
%	 angle-end= "0"
%	 angle-start= "0"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(157.5,97.5)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\AAh$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(242.5,97.5)"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\BBh$
%</text>
%<multicurve fill-style= "none"
%	 points= "(240,40);(240,40);(225,25);(225,25)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(190,40);(190,40);(175,25);(175,25)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 stroke-overstrike-width= "1.55"
%	 points= "(225,25);(225,25);(210,40);(210,40)"
%	 stroke-overstrike= "true"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 stroke-overstrike-width= "1.55"
%	 points= "(175,25);(175,25);(160,40);(160,40)"
%	 stroke-overstrike= "true"
%	 stroke-width= "0.75"
%	 />
%<ellipse p3= "(227.58,22.42)"
%	 fill-style= "solid"
%	 p2= "(227.58,27.58)"
%	 fill-color= "#330033"
%	 p1= "(222.42,27.58)"
%	 closure= "open"
%	 angle-end= "0"
%	 angle-start= "0"
%	 />
%<ellipse p3= "(177.58,22.42)"
%	 fill-style= "solid"
%	 p2= "(177.58,27.58)"
%	 fill-color= "#330033"
%	 p1= "(172.42,27.58)"
%	 closure= "open"
%	 angle-end= "0"
%	 angle-start= "0"
%	 />
%<multicurve fill-style= "none"
%	 points= "(225,25);(225,25);(225,-10);(225,-10)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(175,25);(175,25);(175,-10);(175,-10)"
%	 stroke-width= "0.75"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(227.5,-7.5)"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\BBh$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(172.5,-7.5)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\AAh$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(265,45)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\EQLS
%</text>
%<multicurve fill-style= "none"
%	 points= "(320,100);(320,100);(320,-10);(320,-10)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(290,100);(290,100);(290,-10);(290,-10)"
%	 stroke-width= "0.75"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(322.5,-7.5)"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\BBh$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(287.5,-7.5)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\AAh$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(322.5,53.75)"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%\eempty
%</text>
%</jpic>
%%End JPIC-XML
%PSTricks content-type (pstricks.sty package needed)
%Add \usepackage{pstricks} in the preamble of your LaTeX file
%You can rescale the whole picture (to 80% for instance) by using the command \def\JPicScale{0.8}
\ifx\JPicScale\undefined\def\JPicScale{1}\fi
\psset{unit=\JPicScale mm}
\psset{linewidth=0.3,dotsep=1,hatchwidth=0.3,hatchsep=1.5,shadowsize=1,dimen=middle}
\psset{dotsize=0.7 2.5,dotscale=1 1,fillcolor=black}
\psset{arrowsize=1 2,arrowlength=1,arrowinset=0.25,tbarsize=0.7 5,bracketlength=0.15,rbracketlength=0.15}
\begin{pspicture}(0,0)(322.5,100)
\psline[linewidth=0.75](90,100)(90,40)
\psline[linewidth=0.75](70,70)(70,40)
\newrgbcolor{userFillColour}{0.2 0 0.2}
\rput{0}(70,70){\psellipse[fillcolor=userFillColour,fillstyle=solid](0,0)(2.58,-2.58)}
\psline[linewidth=0.45](60,80)(100,80)
\psline[linewidth=0.45](100,60)(100,80)
\psline[linewidth=0.45](60,60)(100,60)
\psline[linewidth=0.45](60,80)(60,60)
\psline[linewidth=0.75](10,100)(10,40)
\psline[linewidth=0.75](30,70.01)(30,40)
\newrgbcolor{userFillColour}{0.2 0 0.2}
\rput{0}(30,70){\psellipse[fillcolor=userFillColour,fillstyle=solid](0,0)(2.58,-2.58)}
\psline[linewidth=0.45](0,80)(40,80)
\psline[linewidth=0.45](40,60)(40,80)
\psline[linewidth=0.45](0,60)(40,60)
\psline[linewidth=0.45](0,80)(0,60)
\rput(20,70){$\pizero$}
\rput(80,70){$\pione$}
\psline[linewidth=1](-10,0)(-10,90)
\psline[linewidth=1](-10,90)(110,90)
\psline[linewidth=1](110,0)(110,90)
\psline[linewidth=1](-10,0)(110,0)
\rput[r](7.5,42.5){$\AAh$}
\rput[l](32.5,42.5){$\BBh$}
\rput[r](7.5,97.5){$\AAh$}
\rput[l](92.5,97.5){$\BBh$}
\rput[r](67.5,42.5){$\AAh$}
\rput[l](92.5,42.5){$\BBh$}
\psline[linewidth=0.75](90,40)(60,10)
\psline[linewidth=0.75](70,40)(40,10)
\psline[linewidth=0.75,border=1.55](60,10)(30,40)
\psline[linewidth=0.75,border=1.55](40,10)(10,40)
\newrgbcolor{userFillColour}{0.2 0 0.2}
\rput{0}(60,10){\psellipse[fillcolor=userFillColour,fillstyle=solid](0,0)(2.58,-2.58)}
\newrgbcolor{userFillColour}{0.2 0 0.2}
\rput{0}(40,10){\psellipse[fillcolor=userFillColour,fillstyle=solid](0,0)(2.58,-2.58)}
\psline[linewidth=0.75](60,10)(60,-10)
\psline[linewidth=0.75](40,10)(40,-10)
\rput[l](62.5,-7.5){$\BBh$}
\rput[r](37.5,-7.5){$\AAh$}
\rput(135,45){\EQLS}
\psline[linewidth=0.75](240,100)(240,40)
\psline[linewidth=0.75](210,70)(210,40)
\newrgbcolor{userFillColour}{0.2 0 0.2}
\rput{0}(210,70){\psellipse[fillcolor=userFillColour,fillstyle=solid](0,0)(2.58,-2.58)}
\psline[linewidth=0.75](160,100)(160,40)
\psline[linewidth=0.75](190,70)(190,39.99)
\newrgbcolor{userFillColour}{0.2 0 0.2}
\rput{0}(190,70){\psellipse[fillcolor=userFillColour,fillstyle=solid](0,0)(2.58,-2.58)}
\rput[r](157.5,97.5){$\AAh$}
\rput[l](242.5,97.5){$\BBh$}
\psline[linewidth=0.75](240,40)(225,25)
\psline[linewidth=0.75](190,40)(175,25)
\psline[linewidth=0.75,border=1.55](225,25)(210,40)
\psline[linewidth=0.75,border=1.55](175,25)(160,40)
\newrgbcolor{userFillColour}{0.2 0 0.2}
\rput{0}(225,25){\psellipse[fillcolor=userFillColour,fillstyle=solid](0,0)(2.58,-2.58)}
\newrgbcolor{userFillColour}{0.2 0 0.2}
\rput{0}(175,25){\psellipse[fillcolor=userFillColour,fillstyle=solid](0,0)(2.58,-2.58)}
\psline[linewidth=0.75](225,25)(225,-10)
\psline[linewidth=0.75](175,25)(175,-10)
\rput[l](227.5,-7.5){$\BBh$}
\rput[r](172.5,-7.5){$\AAh$}
\rput(265,45){\EQLS}
\psline[linewidth=0.75](320,100)(320,-10)
\psline[linewidth=0.75](290,100)(290,-10)
\rput[l](322.5,-7.5){$\BBh$}
\rput[r](287.5,-7.5){$\AAh$}
\rput[l](322.5,53.75){\eempty}
\end{pspicture}


==> PIC/projs-work-1.tex <==
%%Created by jPicEdt 1.4.1_03: mixed JPIC-XML/LaTeX format
%%Fri Sep 11 09:21:20 GMT-10:00 2020
%%Begin JPIC-XML
%<?xml version="1.0" standalone="yes"?>
%<jpic x-min="0" x-max="235" y-min="0" y-max="110" auto-bounding="true">
%<multicurve fill-style= "none"
%	 points= "(15,110);(15,110);(15,45);(15,45)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(35,80.01);(35,80.01);(35,45);(35,45)"
%	 stroke-width= "0.75"
%	 />
%<ellipse p3= "(37.58,77.42)"
%	 fill-style= "solid"
%	 p2= "(37.58,82.58)"
%	 fill-color= "#330033"
%	 p1= "(32.42,82.58)"
%	 closure= "open"
%	 angle-end= "0"
%	 angle-start= "0"
%	 />
%<multicurve fill-style= "none"
%	 points= "(5,90);(5,90);(45,90);(45,90)"
%	 stroke-width= "0.45"
%	 />
%<multicurve fill-style= "none"
%	 points= "(45,70);(45,70);(45,90);(45,90)"
%	 stroke-width= "0.45"
%	 />
%<multicurve fill-style= "none"
%	 points= "(5,70);(5,70);(45,70);(45,70)"
%	 stroke-width= "0.45"
%	 />
%<multicurve fill-style= "none"
%	 points= "(5,90);(5,90);(5,70);(5,70)"
%	 stroke-width= "0.45"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(25,80)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\pizero$
%</text>
%<multicurve fill-style= "none"
%	 points= "(35,25);(35,25);(25,15);(25,15)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(25,15);(25,15);(25,0);(25,0)"
%	 stroke-width= "0.75"
%	 />
%<ellipse p3= "(27.58,12.42)"
%	 fill-style= "solid"
%	 p2= "(27.58,17.58)"
%	 fill-color= "#330033"
%	 p1= "(22.42,17.58)"
%	 closure= "open"
%	 angle-end= "0"
%	 angle-start= "0"
%	 />
%<multicurve fill-style= "none"
%	 points= "(10,35);(10,35);(20,35);(20,35)"
%	 stroke-width= "0.6"
%	 />
%<multicurve fill-style= "none"
%	 points= "(50,10);(50,10);(50,50);(50,50)"
%	 stroke-width= "0.45"
%	 />
%<multicurve fill-style= "none"
%	 points= "(0,50);(0,50);(50,50);(50,50)"
%	 stroke-width= "0.45"
%	 />
%<multicurve fill-style= "none"
%	 points= "(15,35);(15,35);(15,25);(15,25)"
%	 stroke-width= "0.6"
%	 />
%<multicurve fill-style= "none"
%	 points= "(15,25);(15,25);(25,15);(25,15)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(35,35);(35,35);(35,25);(35,25)"
%	 stroke-width= "0.6"
%	 />
%<multicurve fill-style= "none"
%	 points= "(30,35);(30,35);(40,35);(40,35)"
%	 stroke-width= "0.6"
%	 />
%<multicurve fill-style= "none"
%	 points= "(30,45);(30,45);(40,45);(40,45)"
%	 stroke-width= "0.6"
%	 />
%<multicurve fill-style= "none"
%	 points= "(10,45);(10,45);(20,45);(20,45)"
%	 stroke-width= "0.6"
%	 />
%<multicurve fill-style= "none"
%	 points= "(20,45);(20,45);(20,35);(20,35)"
%	 stroke-width= "0.6"
%	 />
%<multicurve fill-style= "none"
%	 points= "(30,45);(30,45);(30,35);(30,35)"
%	 stroke-width= "0.6"
%	 />
%<multicurve fill-style= "none"
%	 points= "(40,45);(40,45);(40,35);(40,35)"
%	 stroke-width= "0.6"
%	 />
%<multicurve fill-style= "none"
%	 points= "(10,45);(10,45);(10,35);(10,35)"
%	 stroke-width= "0.6"
%	 />
%<multicurve fill-style= "none"
%	 points= "(0,10);(0,10);(0,50);(0,50)"
%	 stroke-width= "0.45"
%	 />
%<multicurve fill-style= "none"
%	 points= "(0,10);(0,10);(50,10);(50,10)"
%	 stroke-width= "0.45"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(15,40)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\aah$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(35,40)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\bbh$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(47.5,15)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\pairr$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(12.5,57.5)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\AAh$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(37.5,57.5)"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\BBh$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(22.5,2.5)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\XXh$
%</text>
%<multicurve fill-style= "none"
%	 points= "(95,110);(95,110);(95,45);(95,45)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(115,80.01);(115,80.01);(115,25);(115,25)"
%	 stroke-width= "0.75"
%	 />
%<ellipse p3= "(117.58,77.42)"
%	 fill-style= "solid"
%	 p2= "(117.58,82.58)"
%	 fill-color= "#330033"
%	 p1= "(112.42,82.58)"
%	 closure= "open"
%	 angle-end= "0"
%	 angle-start= "0"
%	 />
%<multicurve fill-style= "none"
%	 points= "(115,25);(115,25);(105,15);(105,15)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(105,15);(105,15);(105,0);(105,0)"
%	 stroke-width= "0.75"
%	 />
%<ellipse p3= "(107.58,12.42)"
%	 fill-style= "solid"
%	 p2= "(107.58,17.58)"
%	 fill-color= "#330033"
%	 p1= "(102.42,17.58)"
%	 closure= "open"
%	 angle-end= "0"
%	 angle-start= "0"
%	 />
%<multicurve fill-style= "none"
%	 points= "(90,35);(90,35);(100,35);(100,35)"
%	 stroke-width= "0.6"
%	 />
%<multicurve fill-style= "none"
%	 points= "(95,35);(95,35);(95,25);(95,25)"
%	 stroke-width= "0.6"
%	 />
%<multicurve fill-style= "none"
%	 points= "(95,25);(95,25);(105,15);(105,15)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(90,45);(90,45);(100,45);(100,45)"
%	 stroke-width= "0.6"
%	 />
%<multicurve fill-style= "none"
%	 points= "(100,45);(100,45);(100,35);(100,35)"
%	 stroke-width= "0.6"
%	 />
%<multicurve fill-style= "none"
%	 points= "(90,45);(90,45);(90,35);(90,35)"
%	 stroke-width= "0.6"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(95,40)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\aah$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(92.5,57.5)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\AAh$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(102.5,2.5)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\XXh$
%</text>
%<multicurve fill-style= "none"
%	 points= "(165,110);(165,110);(165,45);(165,45)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(185,40);(185,40);(185,25);(185,25)"
%	 stroke-width= "0.75"
%	 />
%<ellipse p3= "(187.58,37.42)"
%	 fill-style= "solid"
%	 p2= "(187.58,42.58)"
%	 fill-color= "#330033"
%	 p1= "(182.42,42.58)"
%	 closure= "open"
%	 angle-end= "0"
%	 angle-start= "0"
%	 />
%<multicurve fill-style= "none"
%	 points= "(185,25);(185,25);(175,15);(175,15)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(175,15);(175,15);(175,0);(175,0)"
%	 stroke-width= "0.75"
%	 />
%<ellipse p3= "(177.58,12.42)"
%	 fill-style= "solid"
%	 p2= "(177.58,17.58)"
%	 fill-color= "#330033"
%	 p1= "(172.42,17.58)"
%	 closure= "open"
%	 angle-end= "0"
%	 angle-start= "0"
%	 />
%<multicurve fill-style= "none"
%	 points= "(160,35);(160,35);(170,35);(170,35)"
%	 stroke-width= "0.6"
%	 />
%<multicurve fill-style= "none"
%	 points= "(165,35);(165,35);(165,25);(165,25)"
%	 stroke-width= "0.6"
%	 />
%<multicurve fill-style= "none"
%	 points= "(165,25);(165,25);(175,15);(175,15)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(160,45);(160,45);(170,45);(170,45)"
%	 stroke-width= "0.6"
%	 />
%<multicurve fill-style= "none"
%	 points= "(170,45);(170,45);(170,35);(170,35)"
%	 stroke-width= "0.6"
%	 />
%<multicurve fill-style= "none"
%	 points= "(160,45);(160,45);(160,35);(160,35)"
%	 stroke-width= "0.6"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(165,40)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\aah$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(162.5,57.5)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\AAh$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(172.5,2.5)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\XXh$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(70,40)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\EQLS
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(140,40)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\EQLS
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(235,60)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\eempty
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(117.5,57.5)"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\XXh$
%</text>
%</jpic>
%%End JPIC-XML
%PSTricks content-type (pstricks.sty package needed)
%Add \usepackage{pstricks} in the preamble of your LaTeX file
%You can rescale the whole picture (to 80% for instance) by using the command \def\JPicScale{0.8}
\ifx\JPicScale\undefined\def\JPicScale{1}\fi
\psset{unit=\JPicScale mm}
\psset{linewidth=0.3,dotsep=1,hatchwidth=0.3,hatchsep=1.5,shadowsize=1,dimen=middle}
\psset{dotsize=0.7 2.5,dotscale=1 1,fillcolor=black}
\psset{arrowsize=1 2,arrowlength=1,arrowinset=0.25,tbarsize=0.7 5,bracketlength=0.15,rbracketlength=0.15}
\begin{pspicture}(0,0)(235,110)
\psline[linewidth=0.75](15,110)(15,45)
\psline[linewidth=0.75](35,80.01)(35,45)
\newrgbcolor{userFillColour}{0.2 0 0.2}
\rput{0}(35,80){\psellipse[fillcolor=userFillColour,fillstyle=solid](0,0)(2.58,-2.58)}
\psline[linewidth=0.45](5,90)(45,90)
\psline[linewidth=0.45](45,70)(45,90)
\psline[linewidth=0.45](5,70)(45,70)
\psline[linewidth=0.45](5,90)(5,70)
\rput(25,80){$\pizero$}
\psline[linewidth=0.75](35,25)(25,15)
\psline[linewidth=0.75](25,15)(25,0)
\newrgbcolor{userFillColour}{0.2 0 0.2}
\rput{0}(25,15){\psellipse[fillcolor=userFillColour,fillstyle=solid](0,0)(2.58,-2.58)}
\psline[linewidth=0.6](10,35)(20,35)
\psline[linewidth=0.45](50,10)(50,50)
\psline[linewidth=0.45](0,50)(50,50)
\psline[linewidth=0.6](15,35)(15,25)
\psline[linewidth=0.75](15,25)(25,15)
\psline[linewidth=0.6](35,35)(35,25)
\psline[linewidth=0.6](30,35)(40,35)
\psline[linewidth=0.6](30,45)(40,45)
\psline[linewidth=0.6](10,45)(20,45)
\psline[linewidth=0.6](20,45)(20,35)
\psline[linewidth=0.6](30,45)(30,35)
\psline[linewidth=0.6](40,45)(40,35)
\psline[linewidth=0.6](10,45)(10,35)
\psline[linewidth=0.45](0,10)(0,50)
\psline[linewidth=0.45](0,10)(50,10)
\rput(15,40){$\aah$}
\rput(35,40){$\bbh$}
\rput[r](47.5,15){$\pairr$}
\rput[r](12.5,57.5){$\AAh$}
\rput[l](37.5,57.5){$\BBh$}
\rput[r](22.5,2.5){$\XXh$}
\psline[linewidth=0.75](95,110)(95,45)
\psline[linewidth=0.75](115,80.01)(115,25)
\newrgbcolor{userFillColour}{0.2 0 0.2}
\rput{0}(115,80){\psellipse[fillcolor=userFillColour,fillstyle=solid](0,0)(2.58,-2.58)}
\psline[linewidth=0.75](115,25)(105,15)
\psline[linewidth=0.75](105,15)(105,0)
\newrgbcolor{userFillColour}{0.2 0 0.2}
\rput{0}(105,15){\psellipse[fillcolor=userFillColour,fillstyle=solid](0,0)(2.58,-2.58)}
\psline[linewidth=0.6](90,35)(100,35)
\psline[linewidth=0.6](95,35)(95,25)
\psline[linewidth=0.75](95,25)(105,15)
\psline[linewidth=0.6](90,45)(100,45)
\psline[linewidth=0.6](100,45)(100,35)
\psline[linewidth=0.6](90,45)(90,35)
\rput(95,40){$\aah$}
\rput[r](92.5,57.5){$\AAh$}
\rput[r](102.5,2.5){$\XXh$}
\psline[linewidth=0.75](165,110)(165,45)
\psline[linewidth=0.75](185,40)(185,25)
\newrgbcolor{userFillColour}{0.2 0 0.2}
\rput{0}(185,40){\psellipse[fillcolor=userFillColour,fillstyle=solid](0,0)(2.58,-2.58)}
\psline[linewidth=0.75](185,25)(175,15)
\psline[linewidth=0.75](175,15)(175,0)
\newrgbcolor{userFillColour}{0.2 0 0.2}
\rput{0}(175,15){\psellipse[fillcolor=userFillColour,fillstyle=solid](0,0)(2.58,-2.58)}
\psline[linewidth=0.6](160,35)(170,35)
\psline[linewidth=0.6](165,35)(165,25)
\psline[linewidth=0.75](165,25)(175,15)
\psline[linewidth=0.6](160,45)(170,45)
\psline[linewidth=0.6](170,45)(170,35)
\psline[linewidth=0.6](160,45)(160,35)
\rput(165,40){$\aah$}
\rput[r](162.5,57.5){$\AAh$}
\rput[r](172.5,2.5){$\XXh$}
\rput(70,40){\EQLS}
\rput(140,40){\EQLS}
\rput(235,60){\eempty}
\rput[l](117.5,57.5){$\XXh$}
\end{pspicture}


==> PIC/projs-work-2.tex <==
%%Created by jPicEdt 1.4.1_03: mixed JPIC-XML/LaTeX format
%%Fri Sep 11 09:22:33 GMT-10:00 2020
%%Begin JPIC-XML
%<?xml version="1.0" standalone="yes"?>
%<jpic x-min="0" x-max="235" y-min="0" y-max="110" auto-bounding="true">
%<multicurve fill-style= "none"
%	 points= "(15,110);(15,110);(15,45);(15,45)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(35,80.01);(35,80.01);(35,45);(35,45)"
%	 stroke-width= "0.75"
%	 />
%<ellipse p3= "(37.58,77.42)"
%	 fill-style= "solid"
%	 p2= "(37.58,82.58)"
%	 fill-color= "#330033"
%	 p1= "(32.42,82.58)"
%	 closure= "open"
%	 angle-end= "0"
%	 angle-start= "0"
%	 />
%<multicurve fill-style= "none"
%	 points= "(5,90);(5,90);(45,90);(45,90)"
%	 stroke-width= "0.45"
%	 />
%<multicurve fill-style= "none"
%	 points= "(45,70);(45,70);(45,90);(45,90)"
%	 stroke-width= "0.45"
%	 />
%<multicurve fill-style= "none"
%	 points= "(5,70);(5,70);(45,70);(45,70)"
%	 stroke-width= "0.45"
%	 />
%<multicurve fill-style= "none"
%	 points= "(5,90);(5,90);(5,70);(5,70)"
%	 stroke-width= "0.45"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(25,80)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\pizero$
%</text>
%<multicurve fill-style= "none"
%	 points= "(35,25);(35,25);(25,15);(25,15)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(25,15);(25,15);(25,0);(25,0)"
%	 stroke-width= "0.75"
%	 />
%<ellipse p3= "(27.58,12.42)"
%	 fill-style= "solid"
%	 p2= "(27.58,17.58)"
%	 fill-color= "#330033"
%	 p1= "(22.42,17.58)"
%	 closure= "open"
%	 angle-end= "0"
%	 angle-start= "0"
%	 />
%<multicurve fill-style= "none"
%	 points= "(10,35);(10,35);(20,35);(20,35)"
%	 stroke-width= "0.6"
%	 />
%<multicurve fill-style= "none"
%	 points= "(50,10);(50,10);(50,50);(50,50)"
%	 stroke-width= "0.45"
%	 />
%<multicurve fill-style= "none"
%	 points= "(0,50);(0,50);(50,50);(50,50)"
%	 stroke-width= "0.45"
%	 />
%<multicurve fill-style= "none"
%	 points= "(15,35);(15,35);(15,25);(15,25)"
%	 stroke-width= "0.6"
%	 />
%<multicurve fill-style= "none"
%	 points= "(15,25);(15,25);(25,15);(25,15)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(35,35);(35,35);(35,25);(35,25)"
%	 stroke-width= "0.6"
%	 />
%<multicurve fill-style= "none"
%	 points= "(30,35);(30,35);(40,35);(40,35)"
%	 stroke-width= "0.6"
%	 />
%<multicurve fill-style= "none"
%	 points= "(30,45);(30,45);(40,45);(40,45)"
%	 stroke-width= "0.6"
%	 />
%<multicurve fill-style= "none"
%	 points= "(10,45);(10,45);(20,45);(20,45)"
%	 stroke-width= "0.6"
%	 />
%<multicurve fill-style= "none"
%	 points= "(20,45);(20,45);(20,35);(20,35)"
%	 stroke-width= "0.6"
%	 />
%<multicurve fill-style= "none"
%	 points= "(30,45);(30,45);(30,35);(30,35)"
%	 stroke-width= "0.6"
%	 />
%<multicurve fill-style= "none"
%	 points= "(40,45);(40,45);(40,35);(40,35)"
%	 stroke-width= "0.6"
%	 />
%<multicurve fill-style= "none"
%	 points= "(10,45);(10,45);(10,35);(10,35)"
%	 stroke-width= "0.6"
%	 />
%<multicurve fill-style= "none"
%	 points= "(0,10);(0,10);(0,50);(0,50)"
%	 stroke-width= "0.45"
%	 />
%<multicurve fill-style= "none"
%	 points= "(0,10);(0,10);(50,10);(50,10)"
%	 stroke-width= "0.45"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(15,40)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\aah$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(35,40)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\bbh$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(47.5,15)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\pairr$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(12.5,57.5)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\AAh$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(37.5,57.5)"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\BBh$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(22.5,2.5)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\XXh$
%</text>
%<multicurve fill-style= "none"
%	 points= "(95,110);(95,110);(95,45);(95,45)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(115,80.01);(115,80.01);(115,25);(115,25)"
%	 stroke-width= "0.75"
%	 />
%<ellipse p3= "(117.58,77.42)"
%	 fill-style= "solid"
%	 p2= "(117.58,82.58)"
%	 fill-color= "#330033"
%	 p1= "(112.42,82.58)"
%	 closure= "open"
%	 angle-end= "0"
%	 angle-start= "0"
%	 />
%<multicurve fill-style= "none"
%	 points= "(115,25);(115,25);(105,15);(105,15)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(105,15);(105,15);(105,0);(105,0)"
%	 stroke-width= "0.75"
%	 />
%<ellipse p3= "(107.58,12.42)"
%	 fill-style= "solid"
%	 p2= "(107.58,17.58)"
%	 fill-color= "#330033"
%	 p1= "(102.42,17.58)"
%	 closure= "open"
%	 angle-end= "0"
%	 angle-start= "0"
%	 />
%<multicurve fill-style= "none"
%	 points= "(90,35);(90,35);(100,35);(100,35)"
%	 stroke-width= "0.6"
%	 />
%<multicurve fill-style= "none"
%	 points= "(95,35);(95,35);(95,25);(95,25)"
%	 stroke-width= "0.6"
%	 />
%<multicurve fill-style= "none"
%	 points= "(95,25);(95,25);(105,15);(105,15)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(90,45);(90,45);(100,45);(100,45)"
%	 stroke-width= "0.6"
%	 />
%<multicurve fill-style= "none"
%	 points= "(100,45);(100,45);(100,35);(100,35)"
%	 stroke-width= "0.6"
%	 />
%<multicurve fill-style= "none"
%	 points= "(90,45);(90,45);(90,35);(90,35)"
%	 stroke-width= "0.6"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(95,40)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\aah$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(92.5,57.5)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\AAh$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(102.5,2.5)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\XXh$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(70,40)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\EQLS
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(235,60)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\eempty
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(117.5,57.5)"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\XXh$
%</text>
%</jpic>
%%End JPIC-XML
%PSTricks content-type (pstricks.sty package needed)
%Add \usepackage{pstricks} in the preamble of your LaTeX file
%You can rescale the whole picture (to 80% for instance) by using the command \def\JPicScale{0.8}
\ifx\JPicScale\undefined\def\JPicScale{1}\fi
\psset{unit=\JPicScale mm}
\psset{linewidth=0.3,dotsep=1,hatchwidth=0.3,hatchsep=1.5,shadowsize=1,dimen=middle}
\psset{dotsize=0.7 2.5,dotscale=1 1,fillcolor=black}
\psset{arrowsize=1 2,arrowlength=1,arrowinset=0.25,tbarsize=0.7 5,bracketlength=0.15,rbracketlength=0.15}
\begin{pspicture}(0,0)(235,110)
\psline[linewidth=0.75](15,110)(15,45)
\psline[linewidth=0.75](35,80.01)(35,45)
\newrgbcolor{userFillColour}{0.2 0 0.2}
\rput{0}(35,80){\psellipse[fillcolor=userFillColour,fillstyle=solid](0,0)(2.58,-2.58)}
\psline[linewidth=0.45](5,90)(45,90)
\psline[linewidth=0.45](45,70)(45,90)
\psline[linewidth=0.45](5,70)(45,70)
\psline[linewidth=0.45](5,90)(5,70)
\rput(25,80){$\pizero$}
\psline[linewidth=0.75](35,25)(25,15)
\psline[linewidth=0.75](25,15)(25,0)
\newrgbcolor{userFillColour}{0.2 0 0.2}
\rput{0}(25,15){\psellipse[fillcolor=userFillColour,fillstyle=solid](0,0)(2.58,-2.58)}
\psline[linewidth=0.6](10,35)(20,35)
\psline[linewidth=0.45](50,10)(50,50)
\psline[linewidth=0.45](0,50)(50,50)
\psline[linewidth=0.6](15,35)(15,25)
\psline[linewidth=0.75](15,25)(25,15)
\psline[linewidth=0.6](35,35)(35,25)
\psline[linewidth=0.6](30,35)(40,35)
\psline[linewidth=0.6](30,45)(40,45)
\psline[linewidth=0.6](10,45)(20,45)
\psline[linewidth=0.6](20,45)(20,35)
\psline[linewidth=0.6](30,45)(30,35)
\psline[linewidth=0.6](40,45)(40,35)
\psline[linewidth=0.6](10,45)(10,35)
\psline[linewidth=0.45](0,10)(0,50)
\psline[linewidth=0.45](0,10)(50,10)
\rput(15,40){$\aah$}
\rput(35,40){$\bbh$}
\rput[r](47.5,15){$\pairr$}
\rput[r](12.5,57.5){$\AAh$}
\rput[l](37.5,57.5){$\BBh$}
\rput[r](22.5,2.5){$\XXh$}
\psline[linewidth=0.75](95,110)(95,45)
\psline[linewidth=0.75](115,80.01)(115,25)
\newrgbcolor{userFillColour}{0.2 0 0.2}
\rput{0}(115,80){\psellipse[fillcolor=userFillColour,fillstyle=solid](0,0)(2.58,-2.58)}
\psline[linewidth=0.75](115,25)(105,15)
\psline[linewidth=0.75](105,15)(105,0)
\newrgbcolor{userFillColour}{0.2 0 0.2}
\rput{0}(105,15){\psellipse[fillcolor=userFillColour,fillstyle=solid](0,0)(2.58,-2.58)}
\psline[linewidth=0.6](90,35)(100,35)
\psline[linewidth=0.6](95,35)(95,25)
\psline[linewidth=0.75](95,25)(105,15)
\psline[linewidth=0.6](90,45)(100,45)
\psline[linewidth=0.6](100,45)(100,35)
\psline[linewidth=0.6](90,45)(90,35)
\rput(95,40){$\aah$}
\rput[r](92.5,57.5){$\AAh$}
\rput[r](102.5,2.5){$\XXh$}
\rput(70,40){\EQLS}
\rput(235,60){\eempty}
\rput[l](117.5,57.5){$\XXh$}
\end{pspicture}


==> PIC/projs-work-3.tex <==
%%Created by jPicEdt 1.4.1_03: mixed JPIC-XML/LaTeX format
%%Fri Sep 11 08:59:06 GMT-10:00 2020
%%Begin JPIC-XML
%<?xml version="1.0" standalone="yes"?>
%<jpic x-min="0" x-max="235" y-min="0" y-max="110" auto-bounding="true">
%<multicurve fill-style= "none"
%	 points= "(15,110);(15,110);(15,45);(15,45)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(35,80.01);(35,80.01);(35,45);(35,45)"
%	 stroke-width= "0.75"
%	 />
%<ellipse p3= "(37.58,77.42)"
%	 fill-style= "solid"
%	 p2= "(37.58,82.58)"
%	 fill-color= "#330033"
%	 p1= "(32.42,82.58)"
%	 closure= "open"
%	 angle-end= "0"
%	 angle-start= "0"
%	 />
%<multicurve fill-style= "none"
%	 points= "(5,90);(5,90);(45,90);(45,90)"
%	 stroke-width= "0.45"
%	 />
%<multicurve fill-style= "none"
%	 points= "(45,70);(45,70);(45,90);(45,90)"
%	 stroke-width= "0.45"
%	 />
%<multicurve fill-style= "none"
%	 points= "(5,70);(5,70);(45,70);(45,70)"
%	 stroke-width= "0.45"
%	 />
%<multicurve fill-style= "none"
%	 points= "(5,90);(5,90);(5,70);(5,70)"
%	 stroke-width= "0.45"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(25,80)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\pizero$
%</text>
%<multicurve fill-style= "none"
%	 points= "(35,25);(35,25);(25,15);(25,15)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(25,15);(25,15);(25,0);(25,0)"
%	 stroke-width= "0.75"
%	 />
%<ellipse p3= "(27.58,12.42)"
%	 fill-style= "solid"
%	 p2= "(27.58,17.58)"
%	 fill-color= "#330033"
%	 p1= "(22.42,17.58)"
%	 closure= "open"
%	 angle-end= "0"
%	 angle-start= "0"
%	 />
%<multicurve fill-style= "none"
%	 points= "(10,35);(10,35);(20,35);(20,35)"
%	 stroke-width= "0.6"
%	 />
%<multicurve fill-style= "none"
%	 points= "(50,10);(50,10);(50,50);(50,50)"
%	 stroke-width= "0.45"
%	 />
%<multicurve fill-style= "none"
%	 points= "(0,50);(0,50);(50,50);(50,50)"
%	 stroke-width= "0.45"
%	 />
%<multicurve fill-style= "none"
%	 points= "(15,35);(15,35);(15,25);(15,25)"
%	 stroke-width= "0.6"
%	 />
%<multicurve fill-style= "none"
%	 points= "(15,25);(15,25);(25,15);(25,15)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(35,35);(35,35);(35,25);(35,25)"
%	 stroke-width= "0.6"
%	 />
%<multicurve fill-style= "none"
%	 points= "(30,35);(30,35);(40,35);(40,35)"
%	 stroke-width= "0.6"
%	 />
%<multicurve fill-style= "none"
%	 points= "(30,45);(30,45);(40,45);(40,45)"
%	 stroke-width= "0.6"
%	 />
%<multicurve fill-style= "none"
%	 points= "(10,45);(10,45);(20,45);(20,45)"
%	 stroke-width= "0.6"
%	 />
%<multicurve fill-style= "none"
%	 points= "(20,45);(20,45);(20,35);(20,35)"
%	 stroke-width= "0.6"
%	 />
%<multicurve fill-style= "none"
%	 points= "(30,45);(30,45);(30,35);(30,35)"
%	 stroke-width= "0.6"
%	 />
%<multicurve fill-style= "none"
%	 points= "(40,45);(40,45);(40,35);(40,35)"
%	 stroke-width= "0.6"
%	 />
%<multicurve fill-style= "none"
%	 points= "(10,45);(10,45);(10,35);(10,35)"
%	 stroke-width= "0.6"
%	 />
%<multicurve fill-style= "none"
%	 points= "(0,10);(0,10);(0,50);(0,50)"
%	 stroke-width= "0.45"
%	 />
%<multicurve fill-style= "none"
%	 points= "(0,10);(0,10);(50,10);(50,10)"
%	 stroke-width= "0.45"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(15,40)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\aah$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(35,40)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\bbh$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(47.5,15)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\pairr$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(12.5,57.5)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\AAh$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(37.5,57.5)"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\BBh$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(22.5,2.5)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\XXh$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(235,60)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\eempty
%</text>
%</jpic>
%%End JPIC-XML
%PSTricks content-type (pstricks.sty package needed)
%Add \usepackage{pstricks} in the preamble of your LaTeX file
%You can rescale the whole picture (to 80% for instance) by using the command \def\JPicScale{0.8}
\ifx\JPicScale\undefined\def\JPicScale{1}\fi
\psset{unit=\JPicScale mm}
\psset{linewidth=0.3,dotsep=1,hatchwidth=0.3,hatchsep=1.5,shadowsize=1,dimen=middle}
\psset{dotsize=0.7 2.5,dotscale=1 1,fillcolor=black}
\psset{arrowsize=1 2,arrowlength=1,arrowinset=0.25,tbarsize=0.7 5,bracketlength=0.15,rbracketlength=0.15}
\begin{pspicture}(0,0)(235,110)
\psline[linewidth=0.75](15,110)(15,45)
\psline[linewidth=0.75](35,80.01)(35,45)
\newrgbcolor{userFillColour}{0.2 0 0.2}
\rput{0}(35,80){\psellipse[fillcolor=userFillColour,fillstyle=solid](0,0)(2.58,-2.58)}
\psline[linewidth=0.45](5,90)(45,90)
\psline[linewidth=0.45](45,70)(45,90)
\psline[linewidth=0.45](5,70)(45,70)
\psline[linewidth=0.45](5,90)(5,70)
\rput(25,80){$\pizero$}
\psline[linewidth=0.75](35,25)(25,15)
\psline[linewidth=0.75](25,15)(25,0)
\newrgbcolor{userFillColour}{0.2 0 0.2}
\rput{0}(25,15){\psellipse[fillcolor=userFillColour,fillstyle=solid](0,0)(2.58,-2.58)}
\psline[linewidth=0.6](10,35)(20,35)
\psline[linewidth=0.45](50,10)(50,50)
\psline[linewidth=0.45](0,50)(50,50)
\psline[linewidth=0.6](15,35)(15,25)
\psline[linewidth=0.75](15,25)(25,15)
\psline[linewidth=0.6](35,35)(35,25)
\psline[linewidth=0.6](30,35)(40,35)
\psline[linewidth=0.6](30,45)(40,45)
\psline[linewidth=0.6](10,45)(20,45)
\psline[linewidth=0.6](20,45)(20,35)
\psline[linewidth=0.6](30,45)(30,35)
\psline[linewidth=0.6](40,45)(40,35)
\psline[linewidth=0.6](10,45)(10,35)
\psline[linewidth=0.45](0,10)(0,50)
\psline[linewidth=0.45](0,10)(50,10)
\rput(15,40){$\aah$}
\rput(35,40){$\bbh$}
\rput[r](47.5,15){$\pairr$}
\rput[r](12.5,57.5){$\AAh$}
\rput[l](37.5,57.5){$\BBh$}
\rput[r](22.5,2.5){$\XXh$}
\rput(235,60){\eempty}
\end{pspicture}


==> PIC/projs-work-red.tex <==
%%Created by jPicEdt 1.4.1_03: mixed JPIC-XML/LaTeX format
%%Fri Sep 11 09:17:30 GMT-10:00 2020
%%Begin JPIC-XML
%<?xml version="1.0" standalone="yes"?>
%<jpic x-min="0" x-max="235" y-min="0" y-max="110" auto-bounding="true">
%<multicurve fill-style= "none"
%	 points= "(15,110);(15,110);(15,45);(15,45)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(35,80.01);(35,80.01);(35,45);(35,45)"
%	 stroke-color= "#ff0033"
%	 stroke-width= "0.75"
%	 />
%<ellipse p3= "(37.58,77.42)"
%	 fill-style= "solid"
%	 p2= "(37.58,82.58)"
%	 fill-color= "#ff0066"
%	 p1= "(32.42,82.58)"
%	 closure= "open"
%	 angle-end= "0"
%	 stroke-color= "#ff0033"
%	 angle-start= "0"
%	 />
%<multicurve fill-style= "none"
%	 points= "(5,90);(5,90);(45,90);(45,90)"
%	 stroke-width= "0.45"
%	 />
%<multicurve fill-style= "none"
%	 points= "(45,70);(45,70);(45,90);(45,90)"
%	 stroke-width= "0.45"
%	 />
%<multicurve fill-style= "none"
%	 points= "(5,70);(5,70);(45,70);(45,70)"
%	 stroke-width= "0.45"
%	 />
%<multicurve fill-style= "none"
%	 points= "(5,90);(5,90);(5,70);(5,70)"
%	 stroke-width= "0.45"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(25,80)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\pizero$
%</text>
%<multicurve fill-style= "none"
%	 points= "(35,25);(35,25);(25,15);(25,15)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(25,15);(25,15);(25,0);(25,0)"
%	 stroke-width= "0.75"
%	 />
%<ellipse p3= "(27.58,12.42)"
%	 fill-style= "solid"
%	 p2= "(27.58,17.58)"
%	 fill-color= "#330033"
%	 p1= "(22.42,17.58)"
%	 closure= "open"
%	 angle-end= "0"
%	 angle-start= "0"
%	 />
%<multicurve fill-style= "none"
%	 points= "(10,35);(10,35);(20,35);(20,35)"
%	 stroke-width= "0.6"
%	 />
%<multicurve fill-style= "none"
%	 points= "(50,10);(50,10);(50,50);(50,50)"
%	 stroke-width= "0.45"
%	 />
%<multicurve fill-style= "none"
%	 points= "(0,50);(0,50);(50,50);(50,50)"
%	 stroke-width= "0.45"
%	 />
%<multicurve fill-style= "none"
%	 points= "(15,35);(15,35);(15,25);(15,25)"
%	 stroke-width= "0.6"
%	 />
%<multicurve fill-style= "none"
%	 points= "(15,25);(15,25);(25,15);(25,15)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(35,35);(35,35);(35,25);(35,25)"
%	 stroke-color= "#ff0033"
%	 stroke-width= "0.6"
%	 />
%<multicurve fill-style= "none"
%	 points= "(30,35);(30,35);(40,35);(40,35)"
%	 stroke-color= "#ff0033"
%	 stroke-width= "0.6"
%	 />
%<multicurve fill-style= "none"
%	 points= "(30,45);(30,45);(40,45);(40,45)"
%	 stroke-color= "#ff0033"
%	 stroke-width= "0.6"
%	 />
%<multicurve fill-style= "none"
%	 points= "(10,45);(10,45);(20,45);(20,45)"
%	 stroke-width= "0.6"
%	 />
%<multicurve fill-style= "none"
%	 points= "(20,45);(20,45);(20,35);(20,35)"
%	 stroke-width= "0.6"
%	 />
%<multicurve fill-style= "none"
%	 points= "(30,45);(30,45);(30,35);(30,35)"
%	 stroke-color= "#ff0033"
%	 stroke-width= "0.6"
%	 />
%<multicurve fill-style= "none"
%	 points= "(40,45);(40,45);(40,35);(40,35)"
%	 stroke-color= "#ff0033"
%	 stroke-width= "0.6"
%	 />
%<multicurve fill-style= "none"
%	 points= "(10,45);(10,45);(10,35);(10,35)"
%	 stroke-width= "0.6"
%	 />
%<multicurve fill-style= "none"
%	 points= "(0,10);(0,10);(0,50);(0,50)"
%	 stroke-width= "0.45"
%	 />
%<multicurve fill-style= "none"
%	 points= "(0,10);(0,10);(50,10);(50,10)"
%	 stroke-width= "0.45"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(15,40)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\aah$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(35,40)"
%	 stroke-color= "#ff0033"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\bbh$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(47.5,15)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\pairr$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(12.5,57.5)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\AAh$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(37.5,57.5)"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\BBh$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(22.5,2.5)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\XXh$
%</text>
%<multicurve fill-style= "none"
%	 points= "(95,110);(95,110);(95,45);(95,45)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(115,80.01);(115,80.01);(115,25);(115,25)"
%	 stroke-color= "#ff0033"
%	 stroke-width= "0.75"
%	 />
%<ellipse p3= "(117.58,77.42)"
%	 fill-style= "solid"
%	 p2= "(117.58,82.58)"
%	 fill-color= "#ff0066"
%	 p1= "(112.42,82.58)"
%	 closure= "open"
%	 angle-end= "0"
%	 stroke-color= "#ff0033"
%	 angle-start= "0"
%	 />
%<multicurve fill-style= "none"
%	 points= "(115,25);(115,25);(105,15);(105,15)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(105,15);(105,15);(105,0);(105,0)"
%	 stroke-width= "0.75"
%	 />
%<ellipse p3= "(107.58,12.42)"
%	 fill-style= "solid"
%	 p2= "(107.58,17.58)"
%	 fill-color= "#330033"
%	 p1= "(102.42,17.58)"
%	 closure= "open"
%	 angle-end= "0"
%	 angle-start= "0"
%	 />
%<multicurve fill-style= "none"
%	 points= "(90,35);(90,35);(100,35);(100,35)"
%	 stroke-width= "0.6"
%	 />
%<multicurve fill-style= "none"
%	 points= "(95,35);(95,35);(95,25);(95,25)"
%	 stroke-width= "0.6"
%	 />
%<multicurve fill-style= "none"
%	 points= "(95,25);(95,25);(105,15);(105,15)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(90,45);(90,45);(100,45);(100,45)"
%	 stroke-width= "0.6"
%	 />
%<multicurve fill-style= "none"
%	 points= "(100,45);(100,45);(100,35);(100,35)"
%	 stroke-width= "0.6"
%	 />
%<multicurve fill-style= "none"
%	 points= "(90,45);(90,45);(90,35);(90,35)"
%	 stroke-width= "0.6"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(95,40)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\aah$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(92.5,57.5)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\AAh$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(102.5,2.5)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\XXh$
%</text>
%<multicurve fill-style= "none"
%	 points= "(165,110);(165,110);(165,45);(165,45)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(185,40);(185,40);(185,25);(185,25)"
%	 stroke-width= "0.75"
%	 />
%<ellipse p3= "(187.58,37.42)"
%	 fill-style= "solid"
%	 p2= "(187.58,42.58)"
%	 fill-color= "#330033"
%	 p1= "(182.42,42.58)"
%	 closure= "open"
%	 angle-end= "0"
%	 angle-start= "0"
%	 />
%<multicurve fill-style= "none"
%	 points= "(185,25);(185,25);(175,15);(175,15)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(175,15);(175,15);(175,0);(175,0)"
%	 stroke-width= "0.75"
%	 />
%<ellipse p3= "(177.58,12.42)"
%	 fill-style= "solid"
%	 p2= "(177.58,17.58)"
%	 fill-color= "#330033"
%	 p1= "(172.42,17.58)"
%	 closure= "open"
%	 angle-end= "0"
%	 angle-start= "0"
%	 />
%<multicurve fill-style= "none"
%	 points= "(160,35);(160,35);(170,35);(170,35)"
%	 stroke-width= "0.6"
%	 />
%<multicurve fill-style= "none"
%	 points= "(165,35);(165,35);(165,25);(165,25)"
%	 stroke-width= "0.6"
%	 />
%<multicurve fill-style= "none"
%	 points= "(165,25);(165,25);(175,15);(175,15)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(160,45);(160,45);(170,45);(170,45)"
%	 stroke-width= "0.6"
%	 />
%<multicurve fill-style= "none"
%	 points= "(170,45);(170,45);(170,35);(170,35)"
%	 stroke-width= "0.6"
%	 />
%<multicurve fill-style= "none"
%	 points= "(160,45);(160,45);(160,35);(160,35)"
%	 stroke-width= "0.6"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(165,40)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\aah$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(162.5,57.5)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\AAh$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(172.5,2.5)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\XXh$
%</text>
%<multicurve fill-style= "none"
%	 points= "(230,110);(230,110);(230,45);(230,45)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(225,35);(225,35);(235,35);(235,35)"
%	 stroke-width= "0.6"
%	 />
%<multicurve fill-style= "none"
%	 points= "(230,35);(230,35);(230,0);(230,0)"
%	 stroke-width= "0.6"
%	 />
%<multicurve fill-style= "none"
%	 points= "(225,45);(225,45);(235,45);(235,45)"
%	 stroke-width= "0.6"
%	 />
%<multicurve fill-style= "none"
%	 points= "(235,45);(235,45);(235,35);(235,35)"
%	 stroke-width= "0.6"
%	 />
%<multicurve fill-style= "none"
%	 points= "(225,45);(225,45);(225,35);(225,35)"
%	 stroke-width= "0.6"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(230,40)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\aah$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(227.5,57.5)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\AAh$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(227.5,2.5)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\XXh$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(70,40)"
%	 stroke-color= "#ff0033"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\EQLS
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(140,40)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\EQLS
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(207.5,40)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\EQLS
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(117.5,57.5)"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\XXred$
%</text>
%</jpic>
%%End JPIC-XML
%PSTricks content-type (pstricks.sty package needed)
%Add \usepackage{pstricks} in the preamble of your LaTeX file
%You can rescale the whole picture (to 80% for instance) by using the command \def\JPicScale{0.8}
\ifx\JPicScale\undefined\def\JPicScale{1}\fi
\psset{unit=\JPicScale mm}
\psset{linewidth=0.3,dotsep=1,hatchwidth=0.3,hatchsep=1.5,shadowsize=1,dimen=middle}
\psset{dotsize=0.7 2.5,dotscale=1 1,fillcolor=black}
\psset{arrowsize=1 2,arrowlength=1,arrowinset=0.25,tbarsize=0.7 5,bracketlength=0.15,rbracketlength=0.15}
\begin{pspicture}(0,0)(235,110)
\psline[linewidth=0.75](15,110)(15,45)
\newrgbcolor{userLineColour}{1 0 0.2}
\psline[linewidth=0.75,linecolor=userLineColour](35,80.01)(35,45)
\newrgbcolor{userLineColour}{1 0 0.2}
\newrgbcolor{userFillColour}{1 0 0.4}
\rput{0}(35,80){\psellipse[linecolor=userLineColour,fillcolor=userFillColour,fillstyle=solid](0,0)(2.58,-2.58)}
\psline[linewidth=0.45](5,90)(45,90)
\psline[linewidth=0.45](45,70)(45,90)
\psline[linewidth=0.45](5,70)(45,70)
\psline[linewidth=0.45](5,90)(5,70)
\rput(25,80){$\pizero$}
\psline[linewidth=0.75](35,25)(25,15)
\psline[linewidth=0.75](25,15)(25,0)
\newrgbcolor{userFillColour}{0.2 0 0.2}
\rput{0}(25,15){\psellipse[fillcolor=userFillColour,fillstyle=solid](0,0)(2.58,-2.58)}
\psline[linewidth=0.6](10,35)(20,35)
\psline[linewidth=0.45](50,10)(50,50)
\psline[linewidth=0.45](0,50)(50,50)
\psline[linewidth=0.6](15,35)(15,25)
\psline[linewidth=0.75](15,25)(25,15)
\newrgbcolor{userLineColour}{1 0 0.2}
\psline[linewidth=0.6,linecolor=userLineColour](35,35)(35,25)
\newrgbcolor{userLineColour}{1 0 0.2}
\psline[linewidth=0.6,linecolor=userLineColour](30,35)(40,35)
\newrgbcolor{userLineColour}{1 0 0.2}
\psline[linewidth=0.6,linecolor=userLineColour](30,45)(40,45)
\psline[linewidth=0.6](10,45)(20,45)
\psline[linewidth=0.6](20,45)(20,35)
\newrgbcolor{userLineColour}{1 0 0.2}
\psline[linewidth=0.6,linecolor=userLineColour](30,45)(30,35)
\newrgbcolor{userLineColour}{1 0 0.2}
\psline[linewidth=0.6,linecolor=userLineColour](40,45)(40,35)
\psline[linewidth=0.6](10,45)(10,35)
\psline[linewidth=0.45](0,10)(0,50)
\psline[linewidth=0.45](0,10)(50,10)
\rput(15,40){$\aah$}
\newrgbcolor{userLineColour}{1 0 0.2}
\rput(35,40){$\bbh$}
\rput[r](47.5,15){$\pairr$}
\rput[r](12.5,57.5){$\AAh$}
\rput[l](37.5,57.5){$\BBh$}
\rput[r](22.5,2.5){$\XXh$}
\psline[linewidth=0.75](95,110)(95,45)
\newrgbcolor{userLineColour}{1 0 0.2}
\psline[linewidth=0.75,linecolor=userLineColour](115,80.01)(115,25)
\newrgbcolor{userLineColour}{1 0 0.2}
\newrgbcolor{userFillColour}{1 0 0.4}
\rput{0}(115,80){\psellipse[linecolor=userLineColour,fillcolor=userFillColour,fillstyle=solid](0,0)(2.58,-2.58)}
\psline[linewidth=0.75](115,25)(105,15)
\psline[linewidth=0.75](105,15)(105,0)
\newrgbcolor{userFillColour}{0.2 0 0.2}
\rput{0}(105,15){\psellipse[fillcolor=userFillColour,fillstyle=solid](0,0)(2.58,-2.58)}
\psline[linewidth=0.6](90,35)(100,35)
\psline[linewidth=0.6](95,35)(95,25)
\psline[linewidth=0.75](95,25)(105,15)
\psline[linewidth=0.6](90,45)(100,45)
\psline[linewidth=0.6](100,45)(100,35)
\psline[linewidth=0.6](90,45)(90,35)
\rput(95,40){$\aah$}
\rput[r](92.5,57.5){$\AAh$}
\rput[r](102.5,2.5){$\XXh$}
\psline[linewidth=0.75](165,110)(165,45)
\psline[linewidth=0.75](185,40)(185,25)
\newrgbcolor{userFillColour}{0.2 0 0.2}
\rput{0}(185,40){\psellipse[fillcolor=userFillColour,fillstyle=solid](0,0)(2.58,-2.58)}
\psline[linewidth=0.75](185,25)(175,15)
\psline[linewidth=0.75](175,15)(175,0)
\newrgbcolor{userFillColour}{0.2 0 0.2}
\rput{0}(175,15){\psellipse[fillcolor=userFillColour,fillstyle=solid](0,0)(2.58,-2.58)}
\psline[linewidth=0.6](160,35)(170,35)
\psline[linewidth=0.6](165,35)(165,25)
\psline[linewidth=0.75](165,25)(175,15)
\psline[linewidth=0.6](160,45)(170,45)
\psline[linewidth=0.6](170,45)(170,35)
\psline[linewidth=0.6](160,45)(160,35)
\rput(165,40){$\aah$}
\rput[r](162.5,57.5){$\AAh$}
\rput[r](172.5,2.5){$\XXh$}
\psline[linewidth=0.75](230,110)(230,45)
\psline[linewidth=0.6](225,35)(235,35)
\psline[linewidth=0.6](230,35)(230,0)
\psline[linewidth=0.6](225,45)(235,45)
\psline[linewidth=0.6](235,45)(235,35)
\psline[linewidth=0.6](225,45)(225,35)
\rput(230,40){$\aah$}
\rput[r](227.5,57.5){$\AAh$}
\rput[r](227.5,2.5){$\XXh$}
\newrgbcolor{userLineColour}{1 0 0.2}
\rput(70,40){\EQLS}
\rput(140,40){\EQLS}
\rput(207.5,40){\EQLS}
\rput[l](117.5,57.5){$\XXred$}
\end{pspicture}


==> PIC/projs-work.tex <==
%%Created by jPicEdt 1.4.1_03: mixed JPIC-XML/LaTeX format
%%Fri Sep 11 09:20:47 GMT-10:00 2020
%%Begin JPIC-XML
%<?xml version="1.0" standalone="yes"?>
%<jpic x-min="0" x-max="235" y-min="0" y-max="110" auto-bounding="true">
%<multicurve fill-style= "none"
%	 points= "(15,110);(15,110);(15,45);(15,45)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(35,80.01);(35,80.01);(35,45);(35,45)"
%	 stroke-width= "0.75"
%	 />
%<ellipse p3= "(37.58,77.42)"
%	 fill-style= "solid"
%	 p2= "(37.58,82.58)"
%	 fill-color= "#330033"
%	 p1= "(32.42,82.58)"
%	 closure= "open"
%	 angle-end= "0"
%	 angle-start= "0"
%	 />
%<multicurve fill-style= "none"
%	 points= "(5,90);(5,90);(45,90);(45,90)"
%	 stroke-width= "0.45"
%	 />
%<multicurve fill-style= "none"
%	 points= "(45,70);(45,70);(45,90);(45,90)"
%	 stroke-width= "0.45"
%	 />
%<multicurve fill-style= "none"
%	 points= "(5,70);(5,70);(45,70);(45,70)"
%	 stroke-width= "0.45"
%	 />
%<multicurve fill-style= "none"
%	 points= "(5,90);(5,90);(5,70);(5,70)"
%	 stroke-width= "0.45"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(25,80)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\pizero$
%</text>
%<multicurve fill-style= "none"
%	 points= "(35,25);(35,25);(25,15);(25,15)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(25,15);(25,15);(25,0);(25,0)"
%	 stroke-width= "0.75"
%	 />
%<ellipse p3= "(27.58,12.42)"
%	 fill-style= "solid"
%	 p2= "(27.58,17.58)"
%	 fill-color= "#330033"
%	 p1= "(22.42,17.58)"
%	 closure= "open"
%	 angle-end= "0"
%	 angle-start= "0"
%	 />
%<multicurve fill-style= "none"
%	 points= "(10,35);(10,35);(20,35);(20,35)"
%	 stroke-width= "0.6"
%	 />
%<multicurve fill-style= "none"
%	 points= "(50,10);(50,10);(50,50);(50,50)"
%	 stroke-width= "0.45"
%	 />
%<multicurve fill-style= "none"
%	 points= "(0,50);(0,50);(50,50);(50,50)"
%	 stroke-width= "0.45"
%	 />
%<multicurve fill-style= "none"
%	 points= "(15,35);(15,35);(15,25);(15,25)"
%	 stroke-width= "0.6"
%	 />
%<multicurve fill-style= "none"
%	 points= "(15,25);(15,25);(25,15);(25,15)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(35,35);(35,35);(35,25);(35,25)"
%	 stroke-width= "0.6"
%	 />
%<multicurve fill-style= "none"
%	 points= "(30,35);(30,35);(40,35);(40,35)"
%	 stroke-width= "0.6"
%	 />
%<multicurve fill-style= "none"
%	 points= "(30,45);(30,45);(40,45);(40,45)"
%	 stroke-width= "0.6"
%	 />
%<multicurve fill-style= "none"
%	 points= "(10,45);(10,45);(20,45);(20,45)"
%	 stroke-width= "0.6"
%	 />
%<multicurve fill-style= "none"
%	 points= "(20,45);(20,45);(20,35);(20,35)"
%	 stroke-width= "0.6"
%	 />
%<multicurve fill-style= "none"
%	 points= "(30,45);(30,45);(30,35);(30,35)"
%	 stroke-width= "0.6"
%	 />
%<multicurve fill-style= "none"
%	 points= "(40,45);(40,45);(40,35);(40,35)"
%	 stroke-width= "0.6"
%	 />
%<multicurve fill-style= "none"
%	 points= "(10,45);(10,45);(10,35);(10,35)"
%	 stroke-width= "0.6"
%	 />
%<multicurve fill-style= "none"
%	 points= "(0,10);(0,10);(0,50);(0,50)"
%	 stroke-width= "0.45"
%	 />
%<multicurve fill-style= "none"
%	 points= "(0,10);(0,10);(50,10);(50,10)"
%	 stroke-width= "0.45"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(15,40)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\aah$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(35,40)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\bbh$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(47.5,15)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\pairr$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(12.5,57.5)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\AAh$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(37.5,57.5)"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\BBh$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(22.5,2.5)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\XXh$
%</text>
%<multicurve fill-style= "none"
%	 points= "(95,110);(95,110);(95,45);(95,45)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(115,80.01);(115,80.01);(115,25);(115,25)"
%	 stroke-width= "0.75"
%	 />
%<ellipse p3= "(117.58,77.42)"
%	 fill-style= "solid"
%	 p2= "(117.58,82.58)"
%	 fill-color= "#330033"
%	 p1= "(112.42,82.58)"
%	 closure= "open"
%	 angle-end= "0"
%	 angle-start= "0"
%	 />
%<multicurve fill-style= "none"
%	 points= "(115,25);(115,25);(105,15);(105,15)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(105,15);(105,15);(105,0);(105,0)"
%	 stroke-width= "0.75"
%	 />
%<ellipse p3= "(107.58,12.42)"
%	 fill-style= "solid"
%	 p2= "(107.58,17.58)"
%	 fill-color= "#330033"
%	 p1= "(102.42,17.58)"
%	 closure= "open"
%	 angle-end= "0"
%	 angle-start= "0"
%	 />
%<multicurve fill-style= "none"
%	 points= "(90,35);(90,35);(100,35);(100,35)"
%	 stroke-width= "0.6"
%	 />
%<multicurve fill-style= "none"
%	 points= "(95,35);(95,35);(95,25);(95,25)"
%	 stroke-width= "0.6"
%	 />
%<multicurve fill-style= "none"
%	 points= "(95,25);(95,25);(105,15);(105,15)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(90,45);(90,45);(100,45);(100,45)"
%	 stroke-width= "0.6"
%	 />
%<multicurve fill-style= "none"
%	 points= "(100,45);(100,45);(100,35);(100,35)"
%	 stroke-width= "0.6"
%	 />
%<multicurve fill-style= "none"
%	 points= "(90,45);(90,45);(90,35);(90,35)"
%	 stroke-width= "0.6"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(95,40)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\aah$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(92.5,57.5)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\AAh$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(102.5,2.5)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\XXh$
%</text>
%<multicurve fill-style= "none"
%	 points= "(165,110);(165,110);(165,45);(165,45)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(185,40);(185,40);(185,25);(185,25)"
%	 stroke-width= "0.75"
%	 />
%<ellipse p3= "(187.58,37.42)"
%	 fill-style= "solid"
%	 p2= "(187.58,42.58)"
%	 fill-color= "#330033"
%	 p1= "(182.42,42.58)"
%	 closure= "open"
%	 angle-end= "0"
%	 angle-start= "0"
%	 />
%<multicurve fill-style= "none"
%	 points= "(185,25);(185,25);(175,15);(175,15)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(175,15);(175,15);(175,0);(175,0)"
%	 stroke-width= "0.75"
%	 />
%<ellipse p3= "(177.58,12.42)"
%	 fill-style= "solid"
%	 p2= "(177.58,17.58)"
%	 fill-color= "#330033"
%	 p1= "(172.42,17.58)"
%	 closure= "open"
%	 angle-end= "0"
%	 angle-start= "0"
%	 />
%<multicurve fill-style= "none"
%	 points= "(160,35);(160,35);(170,35);(170,35)"
%	 stroke-width= "0.6"
%	 />
%<multicurve fill-style= "none"
%	 points= "(165,35);(165,35);(165,25);(165,25)"
%	 stroke-width= "0.6"
%	 />
%<multicurve fill-style= "none"
%	 points= "(165,25);(165,25);(175,15);(175,15)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(160,45);(160,45);(170,45);(170,45)"
%	 stroke-width= "0.6"
%	 />
%<multicurve fill-style= "none"
%	 points= "(170,45);(170,45);(170,35);(170,35)"
%	 stroke-width= "0.6"
%	 />
%<multicurve fill-style= "none"
%	 points= "(160,45);(160,45);(160,35);(160,35)"
%	 stroke-width= "0.6"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(165,40)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\aah$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(162.5,57.5)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\AAh$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(172.5,2.5)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\XXh$
%</text>
%<multicurve fill-style= "none"
%	 points= "(230,110);(230,110);(230,45);(230,45)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(225,35);(225,35);(235,35);(235,35)"
%	 stroke-width= "0.6"
%	 />
%<multicurve fill-style= "none"
%	 points= "(230,35);(230,35);(230,0);(230,0)"
%	 stroke-width= "0.6"
%	 />
%<multicurve fill-style= "none"
%	 points= "(225,45);(225,45);(235,45);(235,45)"
%	 stroke-width= "0.6"
%	 />
%<multicurve fill-style= "none"
%	 points= "(235,45);(235,45);(235,35);(235,35)"
%	 stroke-width= "0.6"
%	 />
%<multicurve fill-style= "none"
%	 points= "(225,45);(225,45);(225,35);(225,35)"
%	 stroke-width= "0.6"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(230,40)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\aah$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(227.5,57.5)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\AAh$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(227.5,2.5)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\XXh$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(70,40)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\EQLS
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(140,40)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\EQLS
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(207.5,40)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\EQLS
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(117.5,57.5)"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\XXh$
%</text>
%</jpic>
%%End JPIC-XML
%PSTricks content-type (pstricks.sty package needed)
%Add \usepackage{pstricks} in the preamble of your LaTeX file
%You can rescale the whole picture (to 80% for instance) by using the command \def\JPicScale{0.8}
\ifx\JPicScale\undefined\def\JPicScale{1}\fi
\psset{unit=\JPicScale mm}
\psset{linewidth=0.3,dotsep=1,hatchwidth=0.3,hatchsep=1.5,shadowsize=1,dimen=middle}
\psset{dotsize=0.7 2.5,dotscale=1 1,fillcolor=black}
\psset{arrowsize=1 2,arrowlength=1,arrowinset=0.25,tbarsize=0.7 5,bracketlength=0.15,rbracketlength=0.15}
\begin{pspicture}(0,0)(235,110)
\psline[linewidth=0.75](15,110)(15,45)
\psline[linewidth=0.75](35,80.01)(35,45)
\newrgbcolor{userFillColour}{0.2 0 0.2}
\rput{0}(35,80){\psellipse[fillcolor=userFillColour,fillstyle=solid](0,0)(2.58,-2.58)}
\psline[linewidth=0.45](5,90)(45,90)
\psline[linewidth=0.45](45,70)(45,90)
\psline[linewidth=0.45](5,70)(45,70)
\psline[linewidth=0.45](5,90)(5,70)
\rput(25,80){$\pizero$}
\psline[linewidth=0.75](35,25)(25,15)
\psline[linewidth=0.75](25,15)(25,0)
\newrgbcolor{userFillColour}{0.2 0 0.2}
\rput{0}(25,15){\psellipse[fillcolor=userFillColour,fillstyle=solid](0,0)(2.58,-2.58)}
\psline[linewidth=0.6](10,35)(20,35)
\psline[linewidth=0.45](50,10)(50,50)
\psline[linewidth=0.45](0,50)(50,50)
\psline[linewidth=0.6](15,35)(15,25)
\psline[linewidth=0.75](15,25)(25,15)
\psline[linewidth=0.6](35,35)(35,25)
\psline[linewidth=0.6](30,35)(40,35)
\psline[linewidth=0.6](30,45)(40,45)
\psline[linewidth=0.6](10,45)(20,45)
\psline[linewidth=0.6](20,45)(20,35)
\psline[linewidth=0.6](30,45)(30,35)
\psline[linewidth=0.6](40,45)(40,35)
\psline[linewidth=0.6](10,45)(10,35)
\psline[linewidth=0.45](0,10)(0,50)
\psline[linewidth=0.45](0,10)(50,10)
\rput(15,40){$\aah$}
\rput(35,40){$\bbh$}
\rput[r](47.5,15){$\pairr$}
\rput[r](12.5,57.5){$\AAh$}
\rput[l](37.5,57.5){$\BBh$}
\rput[r](22.5,2.5){$\XXh$}
\psline[linewidth=0.75](95,110)(95,45)
\psline[linewidth=0.75](115,80.01)(115,25)
\newrgbcolor{userFillColour}{0.2 0 0.2}
\rput{0}(115,80){\psellipse[fillcolor=userFillColour,fillstyle=solid](0,0)(2.58,-2.58)}
\psline[linewidth=0.75](115,25)(105,15)
\psline[linewidth=0.75](105,15)(105,0)
\newrgbcolor{userFillColour}{0.2 0 0.2}
\rput{0}(105,15){\psellipse[fillcolor=userFillColour,fillstyle=solid](0,0)(2.58,-2.58)}
\psline[linewidth=0.6](90,35)(100,35)
\psline[linewidth=0.6](95,35)(95,25)
\psline[linewidth=0.75](95,25)(105,15)
\psline[linewidth=0.6](90,45)(100,45)
\psline[linewidth=0.6](100,45)(100,35)
\psline[linewidth=0.6](90,45)(90,35)
\rput(95,40){$\aah$}
\rput[r](92.5,57.5){$\AAh$}
\rput[r](102.5,2.5){$\XXh$}
\psline[linewidth=0.75](165,110)(165,45)
\psline[linewidth=0.75](185,40)(185,25)
\newrgbcolor{userFillColour}{0.2 0 0.2}
\rput{0}(185,40){\psellipse[fillcolor=userFillColour,fillstyle=solid](0,0)(2.58,-2.58)}
\psline[linewidth=0.75](185,25)(175,15)
\psline[linewidth=0.75](175,15)(175,0)
\newrgbcolor{userFillColour}{0.2 0 0.2}
\rput{0}(175,15){\psellipse[fillcolor=userFillColour,fillstyle=solid](0,0)(2.58,-2.58)}
\psline[linewidth=0.6](160,35)(170,35)
\psline[linewidth=0.6](165,35)(165,25)
\psline[linewidth=0.75](165,25)(175,15)
\psline[linewidth=0.6](160,45)(170,45)
\psline[linewidth=0.6](170,45)(170,35)
\psline[linewidth=0.6](160,45)(160,35)
\rput(165,40){$\aah$}
\rput[r](162.5,57.5){$\AAh$}
\rput[r](172.5,2.5){$\XXh$}
\psline[linewidth=0.75](230,110)(230,45)
\psline[linewidth=0.6](225,35)(235,35)
\psline[linewidth=0.6](230,35)(230,0)
\psline[linewidth=0.6](225,45)(235,45)
\psline[linewidth=0.6](235,45)(235,35)
\psline[linewidth=0.6](225,45)(225,35)
\rput(230,40){$\aah$}
\rput[r](227.5,57.5){$\AAh$}
\rput[r](227.5,2.5){$\XXh$}
\rput(70,40){\EQLS}
\rput(140,40){\EQLS}
\rput(207.5,40){\EQLS}
\rput[l](117.5,57.5){$\XXh$}
\end{pspicture}


==> PIC/projs.tex <==
%%Created by jPicEdt 1.4.1_03: mixed JPIC-XML/LaTeX format
%%Thu May 20 15:20:16 GMT-10:00 2021
%%Begin JPIC-XML
%<?xml version="1.0" standalone="yes"?>
%<jpic x-min="0" x-max="230" y-min="0" y-max="60" auto-bounding="true">
%<multicurve fill-style= "none"
%	 points= "(220,60);(220,60);(220,0);(220,0)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(200,30);(200,30);(200,0);(200,0)"
%	 stroke-width= "0.75"
%	 />
%<ellipse p3= "(202.58,27.42)"
%	 fill-style= "solid"
%	 p2= "(202.58,32.58)"
%	 fill-color= "#330033"
%	 p1= "(197.42,32.58)"
%	 closure= "open"
%	 angle-end= "0"
%	 angle-start= "0"
%	 />
%<multicurve fill-style= "none"
%	 points= "(190,40);(190,40);(230,40);(230,40)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(230,20);(230,20);(230,40);(230,40)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(190,20);(190,20);(230,20);(230,20)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(190,40);(190,40);(190,20);(190,20)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(10,60);(10,60);(10,0);(10,0)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(30,30.01);(30,30.01);(30,0);(30,0)"
%	 stroke-width= "0.75"
%	 />
%<ellipse p3= "(32.58,27.42)"
%	 fill-style= "solid"
%	 p2= "(32.58,32.58)"
%	 fill-color= "#330033"
%	 p1= "(27.42,32.58)"
%	 closure= "open"
%	 angle-end= "0"
%	 angle-start= "0"
%	 />
%<multicurve fill-style= "none"
%	 points= "(0,40);(0,40);(40,40);(40,40)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(40,20);(40,20);(40,40);(40,40)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(0,20);(0,20);(40,20);(40,20)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(0,40);(0,40);(0,20);(0,20)"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(20,30)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\pizero$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(210,30)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\pione$
%</text>
%<multicurve fill-style= "none"
%	 points= "(120,25);(120,25);(110,15);(110,15)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(110,15);(110,15);(110,0);(110,0)"
%	 stroke-width= "0.75"
%	 />
%<ellipse p3= "(112.58,12.42)"
%	 fill-style= "solid"
%	 p2= "(112.58,17.58)"
%	 fill-color= "#330033"
%	 p1= "(107.42,17.58)"
%	 closure= "open"
%	 angle-end= "0"
%	 angle-start= "0"
%	 />
%<multicurve fill-style= "none"
%	 points= "(95,35);(95,35);(105,35);(105,35)"
%	 stroke-width= "0.6"
%	 />
%<multicurve fill-style= "none"
%	 points= "(135,7.5);(135,7.5);(135,52.5);(135,52.5)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(85,52.5);(85,52.5);(135,52.5);(135,52.5)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(100,35);(100,35);(100,25);(100,25)"
%	 stroke-width= "0.6"
%	 />
%<multicurve fill-style= "none"
%	 points= "(100,25);(100,25);(110,15);(110,15)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(120,35);(120,35);(120,25);(120,25)"
%	 stroke-width= "0.6"
%	 />
%<multicurve fill-style= "none"
%	 points= "(115,35);(115,35);(125,35);(125,35)"
%	 stroke-width= "0.6"
%	 />
%<multicurve fill-style= "none"
%	 points= "(115,45);(115,45);(125,45);(125,45)"
%	 stroke-width= "0.6"
%	 />
%<multicurve fill-style= "none"
%	 points= "(95,45);(95,45);(105,45);(105,45)"
%	 stroke-width= "0.6"
%	 />
%<multicurve fill-style= "none"
%	 points= "(105,45);(105,45);(105,35);(105,35)"
%	 stroke-width= "0.6"
%	 />
%<multicurve fill-style= "none"
%	 points= "(115,45);(115,45);(115,35);(115,35)"
%	 stroke-width= "0.6"
%	 />
%<multicurve fill-style= "none"
%	 points= "(125,45);(125,45);(125,35);(125,35)"
%	 stroke-width= "0.6"
%	 />
%<multicurve fill-style= "none"
%	 points= "(95,45);(95,45);(95,35);(95,35)"
%	 stroke-width= "0.6"
%	 />
%<multicurve fill-style= "none"
%	 points= "(100,60);(100,60);(100,45);(100,45)"
%	 stroke-width= "0.6"
%	 />
%<multicurve fill-style= "none"
%	 points= "(120,60);(120,60);(120,45);(120,45)"
%	 stroke-width= "0.6"
%	 />
%<multicurve fill-style= "none"
%	 points= "(85,7.5);(85,7.5);(85,52.5);(85,52.5)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(85,7.5);(85,7.5);(135,7.5);(135,7.5)"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(100,40)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\aah$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(120,40)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\bbh$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(132.5,15)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\pairr$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(7.5,2.5)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\AAh$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(32.5,2.5)"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\BBh$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(97.5,57.5)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\AAh$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(122.5,57.5)"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\BBh$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(197.5,2.5)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\AAh$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(222.5,2.5)"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\BBh$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(107.5,2.5)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\XXh$
%</text>
%<ellipse p3= "(122.58,42.42)"
%	 fill-style= "solid"
%	 p2= "(122.58,47.58)"
%	 fill-color= "#330033"
%	 p1= "(117.42,47.58)"
%	 closure= "open"
%	 angle-end= "0"
%	 angle-start= "0"
%	 />
%<ellipse p3= "(102.58,42.42)"
%	 fill-style= "solid"
%	 p2= "(102.58,47.58)"
%	 fill-color= "#330033"
%	 p1= "(97.42,47.58)"
%	 closure= "open"
%	 angle-end= "0"
%	 angle-start= "0"
%	 />
%</jpic>
%%End JPIC-XML
%PSTricks content-type (pstricks.sty package needed)
%Add \usepackage{pstricks} in the preamble of your LaTeX file
%You can rescale the whole picture (to 80% for instance) by using the command \def\JPicScale{0.8}
\ifx\JPicScale\undefined\def\JPicScale{1}\fi
\psset{unit=\JPicScale mm}
\psset{linewidth=0.3,dotsep=1,hatchwidth=0.3,hatchsep=1.5,shadowsize=1,dimen=middle}
\psset{dotsize=0.7 2.5,dotscale=1 1,fillcolor=black}
\psset{arrowsize=1 2,arrowlength=1,arrowinset=0.25,tbarsize=0.7 5,bracketlength=0.15,rbracketlength=0.15}
\begin{pspicture}(0,0)(230,60)
\psline[linewidth=0.75](220,60)(220,0)
\psline[linewidth=0.75](200,30)(200,0)
\newrgbcolor{userFillColour}{0.2 0 0.2}
\rput{0}(200,30){\psellipse[fillcolor=userFillColour,fillstyle=solid](0,0)(2.58,-2.58)}
\psline(190,40)(230,40)
\psline(230,20)(230,40)
\psline(190,20)(230,20)
\psline(190,40)(190,20)
\psline[linewidth=0.75](10,60)(10,0)
\psline[linewidth=0.75](30,30.01)(30,0)
\newrgbcolor{userFillColour}{0.2 0 0.2}
\rput{0}(30,30){\psellipse[fillcolor=userFillColour,fillstyle=solid](0,0)(2.58,-2.58)}
\psline(0,40)(40,40)
\psline(40,20)(40,40)
\psline(0,20)(40,20)
\psline(0,40)(0,20)
\rput(20,30){$\pizero$}
\rput(210,30){$\pione$}
\psline[linewidth=0.75](120,25)(110,15)
\psline[linewidth=0.75](110,15)(110,0)
\newrgbcolor{userFillColour}{0.2 0 0.2}
\rput{0}(110,15){\psellipse[fillcolor=userFillColour,fillstyle=solid](0,0)(2.58,-2.58)}
\psline[linewidth=0.6](95,35)(105,35)
\psline(135,7.5)(135,52.5)
\psline(85,52.5)(135,52.5)
\psline[linewidth=0.6](100,35)(100,25)
\psline[linewidth=0.75](100,25)(110,15)
\psline[linewidth=0.6](120,35)(120,25)
\psline[linewidth=0.6](115,35)(125,35)
\psline[linewidth=0.6](115,45)(125,45)
\psline[linewidth=0.6](95,45)(105,45)
\psline[linewidth=0.6](105,45)(105,35)
\psline[linewidth=0.6](115,45)(115,35)
\psline[linewidth=0.6](125,45)(125,35)
\psline[linewidth=0.6](95,45)(95,35)
\psline[linewidth=0.6](100,60)(100,45)
\psline[linewidth=0.6](120,60)(120,45)
\psline(85,7.5)(85,52.5)
\psline(85,7.5)(135,7.5)
\rput(100,40){$\aah$}
\rput(120,40){$\bbh$}
\rput[r](132.5,15){$\pairr$}
\rput[r](7.5,2.5){$\AAh$}
\rput[l](32.5,2.5){$\BBh$}
\rput[r](97.5,57.5){$\AAh$}
\rput[l](122.5,57.5){$\BBh$}
\rput[r](197.5,2.5){$\AAh$}
\rput[l](222.5,2.5){$\BBh$}
\rput[r](107.5,2.5){$\XXh$}
\newrgbcolor{userFillColour}{0.2 0 0.2}
\rput{0}(120,45){\psellipse[fillcolor=userFillColour,fillstyle=solid](0,0)(2.58,-2.58)}
\newrgbcolor{userFillColour}{0.2 0 0.2}
\rput{0}(100,45){\psellipse[fillcolor=userFillColour,fillstyle=solid](0,0)(2.58,-2.58)}
\end{pspicture}


==> PIC/remainder-moore.tex <==
%%Created by jPicEdt 1.4.1_03: mixed JPIC-XML/LaTeX format
%%Sun Aug 31 14:18:08 HST 2014
%%Begin JPIC-XML
%<?xml version="1.0" standalone="yes"?>
%<jpic x-min="0" x-max="311.88" y-min="5.62" y-max="138.12" auto-bounding="true">
%<text stroke-width= "1"
%	 text-vert-align= "center-v"
%	 anchor-point= "(32.5,40)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\oneleft
%</text>
%<text stroke-width= "1"
%	 text-vert-align= "center-v"
%	 anchor-point= "(122.5,40)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\oneright
%</text>
%<ellipse stroke-width= "1.05"
%	 p3= "(137.5,25)"
%	 p2= "(137.5,55)"
%	 p1= "(107.5,55)"
%	 closure= "open"
%	 fill-style= "none"
%	 angle-end= "0"
%	 angle-start= "0"
%	 />
%<ellipse stroke-width= "1.05"
%	 p3= "(47.5,25)"
%	 p2= "(47.5,55)"
%	 p1= "(17.5,55)"
%	 closure= "open"
%	 fill-style= "none"
%	 angle-end= "0"
%	 angle-start= "0"
%	 />
%<multicurve arrow-head-width-minimum= "2"
%	 stroke-width= "0.8"
%	 right-arrow= "head"
%	 arrow-bracket-length-scale= "0.65"
%	 arrow-head-length-scale= "1.5"
%	 arrow-head-inset-scale= "0"
%	 fill-style= "none"
%	 points= "(50,46.25);(50,46.25);(105,46.25);(105,46.25)"
%	 />
%<multicurve arrow-head-width-minimum= "2"
%	 stroke-width= "0.8"
%	 right-arrow= "head"
%	 arrow-bracket-length-scale= "0.65"
%	 arrow-head-length-scale= "1.5"
%	 arrow-head-inset-scale= "0"
%	 fill-style= "none"
%	 points= "(0,40);(0,40);(17.5,40);(17.5,40)"
%	 />
%<ellipse arrow-head-width-minimum= "2"
%	 stroke-width= "0.8"
%	 p3= "(50,8.12)"
%	 p2= "(15,8.12)"
%	 right-arrow= "head"
%	 p1= "(15,26.88)"
%	 arrow-head-length-scale= "2"
%	 closure= "open"
%	 fill-style= "none"
%	 angle-end= "144.46"
%	 angle-start= "-147.99"
%	 />
%<text text-vert-align= "bottom"
%	 anchor-point= "(75,48.12)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\transtwo
%</text>
%<text text-vert-align= "top"
%	 anchor-point= "(31.88,5.62)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\transone
%</text>
%<multicurve polydots-superimpose= "false"
%	 polydots-angle= "0"
%	 polydots-scale-v= "1"
%	 polydots-scale-h= "1"
%	 fill-style= "none"
%	 polydots-size-minimum= "0.7"
%	 polydots-size-linewidth-scale= "2.5"
%	 points= "(93.12,60.62);(93.12,60.62);(221.88,138.12);(221.88,138.12)"
%	 polydots-style= "polydots-circle"
%	 />
%<multicurve arrow-head-width-minimum= "2"
%	 stroke-width= "0.8"
%	 right-arrow= "head"
%	 arrow-bracket-length-scale= "0.65"
%	 arrow-head-length-scale= "1.5"
%	 arrow-head-inset-scale= "0"
%	 fill-style= "none"
%	 points= "(105,32.5);(105,32.5);(48.75,32.5);(48.75,32.5)"
%	 />
%<text text-vert-align= "top"
%	 anchor-point= "(75,31.25)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\transfour
%</text>
%<ellipse stroke-width= "1.05"
%	 p3= "(227.5,25)"
%	 p2= "(227.5,55)"
%	 p1= "(197.5,55)"
%	 closure= "open"
%	 fill-style= "none"
%	 angle-end= "0"
%	 angle-start= "0"
%	 />
%<multicurve arrow-head-width-minimum= "2"
%	 stroke-width= "0.8"
%	 right-arrow= "head"
%	 arrow-bracket-length-scale= "0.65"
%	 arrow-head-length-scale= "1.5"
%	 arrow-head-inset-scale= "0"
%	 fill-style= "none"
%	 points= "(140,46.25);(140,46.25);(195,46.25);(195,46.25)"
%	 />
%<ellipse arrow-head-width-minimum= "2"
%	 stroke-width= "0.8"
%	 p3= "(230,8.12)"
%	 p2= "(195,8.12)"
%	 right-arrow= "head"
%	 p1= "(195,26.88)"
%	 arrow-head-length-scale= "2"
%	 closure= "open"
%	 fill-style= "none"
%	 angle-end= "144.46"
%	 angle-start= "-147.99"
%	 />
%<multicurve polydots-superimpose= "false"
%	 polydots-angle= "0"
%	 polydots-scale-v= "1"
%	 polydots-scale-h= "1"
%	 fill-style= "none"
%	 polydots-size-minimum= "0.7"
%	 polydots-size-linewidth-scale= "2.5"
%	 points= "(183.12,60.62);(183.12,60.62);(311.88,138.12);(311.88,138.12)"
%	 polydots-style= "polydots-circle"
%	 />
%<multicurve arrow-head-width-minimum= "2"
%	 stroke-width= "0.8"
%	 right-arrow= "head"
%	 arrow-bracket-length-scale= "0.65"
%	 arrow-head-length-scale= "1.5"
%	 arrow-head-inset-scale= "0"
%	 fill-style= "none"
%	 points= "(195,32.5);(195,32.5);(138.75,32.5);(138.75,32.5)"
%	 />
%<text text-vert-align= "top"
%	 anchor-point= "(211.25,6.88)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\transfive
%</text>
%<text text-vert-align= "bottom"
%	 anchor-point= "(165.62,49.38)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\transsix
%</text>
%<text text-vert-align= "top"
%	 anchor-point= "(165,31.25)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\transeight
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(213.12,39.38)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\onerightright
%</text>
%</jpic>
%%End JPIC-XML
%PSTricks content-type (pstricks.sty package needed)
%Add \usepackage{pstricks} in the preamble of your LaTeX file
%You can rescale the whole picture (to 80% for instance) by using the command \def\JPicScale{0.8}
\ifx\JPicScale\undefined\def\JPicScale{1}\fi
\psset{unit=\JPicScale mm}
\psset{linewidth=0.3,dotsep=1,hatchwidth=0.3,hatchsep=1.5,shadowsize=1,dimen=middle}
\psset{dotsize=0.7 2.5,dotscale=1 1,fillcolor=black}
\psset{arrowsize=1 2,arrowlength=1,arrowinset=0.25,tbarsize=0.7 5,bracketlength=0.15,rbracketlength=0.15}
\begin{pspicture}(0,0)(311.88,138.12)
\rput(32.5,40){\oneleft}
\rput(122.5,40){\oneright}
\rput{0}(122.5,40){\psellipse[linewidth=1.05](0,0)(15,-15)}
\rput{0}(32.5,40){\psellipse[linewidth=1.05](0,0)(15,-15)}
\psline[linewidth=0.8,arrowsize=2 2,arrowlength=1.5,arrowinset=0,bracketlength=0.65]{->}(50,46.25)(105,46.25)
\psline[linewidth=0.8,arrowsize=2 2,arrowlength=1.5,arrowinset=0,bracketlength=0.65]{->}(0,40)(17.5,40)
\rput{0}(32.5,17.5){\psellipticarc[linewidth=0.8,arrowsize=2 2,arrowlength=2]{->}(0,0)(17.5,9.38){122.01}{414.46}}
\rput[b](75,48.12){\transtwo}
\rput[t](31.88,5.62){\transone}
\psdots[dotstyle=o](93.12,60.62)
(221.88,138.12)
\psline[linewidth=0.8,arrowsize=2 2,arrowlength=1.5,arrowinset=0,bracketlength=0.65]{->}(105,32.5)(48.75,32.5)
\rput[t](75,31.25){\transfour}
\rput{0}(212.5,40){\psellipse[linewidth=1.05](0,0)(15,-15)}
\psline[linewidth=0.8,arrowsize=2 2,arrowlength=1.5,arrowinset=0,bracketlength=0.65]{->}(140,46.25)(195,46.25)
\rput{0}(212.5,17.5){\psellipticarc[linewidth=0.8,arrowsize=2 2,arrowlength=2]{->}(0,0)(17.5,9.38){122.01}{414.46}}
\psdots[dotstyle=o](183.12,60.62)
(311.88,138.12)
\psline[linewidth=0.8,arrowsize=2 2,arrowlength=1.5,arrowinset=0,bracketlength=0.65]{->}(195,32.5)(138.75,32.5)
\rput[t](211.25,6.88){\transfive}
\rput[b](165.62,49.38){\transsix}
\rput[t](165,31.25){\transeight}
\rput(213.12,39.38){\onerightright}
\end{pspicture}


==> PIC/retraction.tex <==
%%Created by jPicEdt 1.4.1_03: mixed JPIC-XML/LaTeX format
%%Sun Nov 22 18:21:19 GMT-10:00 2020
%%Begin JPIC-XML
%<?xml version="1.0" standalone="yes"?>
%<jpic x-min="-2.5" x-max="155" y-min="0" y-max="90" auto-bounding="true">
%<multicurve stroke-width= "0.2"
%	 fill-style= "none"
%	 points= "(0,0);(0,0);(0,90);(0,90)"
%	 />
%<text stroke-width= "0.35"
%	 fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(120,45)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\EQLS
%</text>
%<multicurve stroke-width= "0.2"
%	 fill-style= "none"
%	 points= "(145,70);(145,70);(145,90);(145,90)"
%	 />
%<multicurve stroke-width= "1"
%	 fill-style= "none"
%	 points= "(145,60);(145,60);(145,30);(145,30)"
%	 />
%<multicurve stroke-width= "0.2"
%	 fill-style= "none"
%	 points= "(145,0);(145,0);(145,20);(145,20)"
%	 />
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(147.5,65)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\qee$
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(142.5,25)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\iee$
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(-2.5,0)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\Ree$
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(142.5,0)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\Ree$
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(146.25,90)"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\Ree$
%</text>
%<multicurve stroke-width= "0.35"
%	 fill-style= "none"
%	 points= "(135,40);(135,40);(155,20);(155,20)"
%	 />
%<multicurve stroke-width= "0.35"
%	 fill-style= "none"
%	 points= "(135,20);(135,20);(155,20);(155,20)"
%	 />
%<multicurve stroke-width= "0.35"
%	 fill-style= "none"
%	 points= "(135,40);(135,40);(135,20);(135,20)"
%	 />
%<multicurve stroke-width= "0.35"
%	 fill-style= "none"
%	 points= "(135,70);(135,70);(155,70);(155,70)"
%	 />
%<multicurve stroke-width= "0.35"
%	 fill-style= "none"
%	 points= "(135,70);(135,70);(155,50);(155,50)"
%	 />
%<multicurve stroke-width= "0.35"
%	 fill-style= "none"
%	 points= "(155,70);(155,70);(155,50);(155,50)"
%	 />
%<multicurve stroke-width= "0.2"
%	 fill-style= "none"
%	 points= "(95,70);(95,70);(95,90);(95,90)"
%	 />
%<multicurve stroke-width= "1"
%	 fill-style= "none"
%	 points= "(95,60);(95,60);(95,45);(95,45)"
%	 />
%<multicurve stroke-width= "0.2"
%	 fill-style= "none"
%	 points= "(100,0);(100,0);(100,35);(100,35)"
%	 />
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(97.5,65)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\qee$
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(98.75,47.5)"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\Aee$
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(97.5,0)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\Ree$
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(96.25,90)"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\Ree$
%</text>
%<multicurve stroke-width= "0.35"
%	 fill-style= "none"
%	 points= "(85,55);(85,55);(105,35);(105,35)"
%	 />
%<multicurve stroke-width= "0.35"
%	 fill-style= "none"
%	 points= "(85,20);(85,20);(95,20);(95,20)"
%	 />
%<multicurve stroke-width= "0.35"
%	 fill-style= "none"
%	 points= "(85,30);(85,30);(85,20);(85,20)"
%	 />
%<multicurve stroke-width= "0.35"
%	 fill-style= "none"
%	 points= "(85,70);(85,70);(105,70);(105,70)"
%	 />
%<multicurve stroke-width= "0.35"
%	 fill-style= "none"
%	 points= "(85,70);(85,70);(105,50);(105,50)"
%	 />
%<multicurve stroke-width= "0.35"
%	 fill-style= "none"
%	 points= "(105,70);(105,70);(105,50);(105,50)"
%	 />
%<multicurve stroke-width= "0.35"
%	 fill-style= "none"
%	 points= "(95,35);(95,35);(105,35);(105,35)"
%	 />
%<multicurve stroke-width= "0.35"
%	 fill-style= "none"
%	 points= "(85,45);(85,45);(85,55);(85,55)"
%	 />
%<multicurve stroke-width= "0.35"
%	 fill-style= "none"
%	 points= "(85,45);(85,45);(95,35);(95,35)"
%	 />
%<multicurve stroke-width= "1"
%	 fill-style= "none"
%	 points= "(90,40);(90,40);(90,25);(90,25)"
%	 />
%<multicurve stroke-width= "0.35"
%	 fill-style= "none"
%	 points= "(85,30);(85,30);(95,20);(95,20)"
%	 />
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(147.5,45)"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\Aee$
%</text>
%<text stroke-width= "0.35"
%	 fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(70,45)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\EQLS
%</text>
%<multicurve stroke-width= "0.2"
%	 fill-style= "none"
%	 points= "(45,70);(45,70);(45,90);(45,90)"
%	 />
%<multicurve stroke-width= "0.2"
%	 fill-style= "none"
%	 points= "(50,0);(50,0);(50,50);(50,50)"
%	 />
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(47.5,0)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\Ree$
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(46.25,90)"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\Ree$
%</text>
%<multicurve stroke-width= "0.35"
%	 fill-style= "none"
%	 points= "(35,35);(35,35);(45,35);(45,35)"
%	 />
%<multicurve stroke-width= "0.35"
%	 fill-style= "none"
%	 points= "(35,45);(35,45);(35,35);(35,35)"
%	 />
%<multicurve stroke-width= "0.35"
%	 fill-style= "none"
%	 points= "(35,70);(35,70);(55,70);(55,70)"
%	 />
%<multicurve stroke-width= "0.35"
%	 fill-style= "none"
%	 points= "(55,70);(55,70);(55,50);(55,50)"
%	 />
%<multicurve stroke-width= "0.35"
%	 fill-style= "none"
%	 points= "(45,50);(45,50);(55,50);(55,50)"
%	 />
%<multicurve stroke-width= "0.35"
%	 fill-style= "none"
%	 points= "(35,60);(35,60);(35,70);(35,70)"
%	 />
%<multicurve stroke-width= "0.35"
%	 fill-style= "none"
%	 points= "(35,60);(35,60);(45,50);(45,50)"
%	 />
%<multicurve stroke-width= "1"
%	 fill-style= "none"
%	 points= "(40,55);(40,55);(40,40);(40,40)"
%	 />
%<multicurve stroke-width= "0.35"
%	 fill-style= "none"
%	 points= "(35,45);(35,45);(45,35);(45,35)"
%	 />
%<text stroke-width= "0.35"
%	 fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(20,45)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\EQLS
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(37.5,48.75)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\Aee$
%</text>
%<text stroke-width= "0.35"
%	 fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(92.5,42.5)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\prtll$
%</text>
%<text stroke-width= "0.35"
%	 fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(88.75,22.5)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\Jee$
%</text>
%<text stroke-width= "0.35"
%	 fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(37.5,37.5)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\Jee$
%</text>
%<text stroke-width= "0.35"
%	 fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(45,61.25)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\univrsl$
%</text>
%</jpic>
%%End JPIC-XML
%LaTeX-picture environment using emulated lines and arcs
%You can rescale the whole picture (to 80% for instance) by using the command \def\JPicScale{0.8}
\ifx\JPicScale\undefined\def\JPicScale{1}\fi
\unitlength \JPicScale mm
\begin{picture}(155,90)(0,0)
\linethickness{0.2mm}
\put(0,0){\line(0,1){90}}
\put(120,45){\makebox(0,0)[cc]{\EQLS}}

\linethickness{0.2mm}
\put(145,70){\line(0,1){20}}
\linethickness{1mm}
\put(145,30){\line(0,1){30}}
\linethickness{0.2mm}
\put(145,0){\line(0,1){20}}
\put(147.5,65){\makebox(0,0)[cc]{$\qee$}}

\put(142.5,25){\makebox(0,0)[cc]{$\iee$}}

\put(-2.5,0){\makebox(0,0)[cr]{$\Ree$}}

\put(142.5,0){\makebox(0,0)[cr]{$\Ree$}}

\put(146.25,90){\makebox(0,0)[cl]{$\Ree$}}

\linethickness{0.35mm}
\multiput(135,40)(0.12,-0.12){167}{\line(1,0){0.12}}
\linethickness{0.35mm}
\put(135,20){\line(1,0){20}}
\linethickness{0.35mm}
\put(135,20){\line(0,1){20}}
\linethickness{0.35mm}
\put(135,70){\line(1,0){20}}
\linethickness{0.35mm}
\multiput(135,70)(0.12,-0.12){167}{\line(1,0){0.12}}
\linethickness{0.35mm}
\put(155,50){\line(0,1){20}}
\linethickness{0.2mm}
\put(95,70){\line(0,1){20}}
\linethickness{1mm}
\put(95,45){\line(0,1){15}}
\linethickness{0.2mm}
\put(100,0){\line(0,1){35}}
\put(97.5,65){\makebox(0,0)[cc]{$\qee$}}

\put(98.75,47.5){\makebox(0,0)[cl]{$\Aee$}}

\put(97.5,0){\makebox(0,0)[cr]{$\Ree$}}

\put(96.25,90){\makebox(0,0)[cl]{$\Ree$}}

\linethickness{0.35mm}
\multiput(85,55)(0.12,-0.12){167}{\line(1,0){0.12}}
\linethickness{0.35mm}
\put(85,20){\line(1,0){10}}
\linethickness{0.35mm}
\put(85,20){\line(0,1){10}}
\linethickness{0.35mm}
\put(85,70){\line(1,0){20}}
\linethickness{0.35mm}
\multiput(85,70)(0.12,-0.12){167}{\line(1,0){0.12}}
\linethickness{0.35mm}
\put(105,50){\line(0,1){20}}
\linethickness{0.35mm}
\put(95,35){\line(1,0){10}}
\linethickness{0.35mm}
\put(85,45){\line(0,1){10}}
\linethickness{0.35mm}
\multiput(85,45)(0.12,-0.12){83}{\line(1,0){0.12}}
\linethickness{1mm}
\put(90,25){\line(0,1){15}}
\linethickness{0.35mm}
\multiput(85,30)(0.12,-0.12){83}{\line(1,0){0.12}}
\put(147.5,45){\makebox(0,0)[cl]{$\Aee$}}

\put(70,45){\makebox(0,0)[cc]{\EQLS}}

\linethickness{0.2mm}
\put(45,70){\line(0,1){20}}
\linethickness{0.2mm}
\put(50,0){\line(0,1){50}}
\put(47.5,0){\makebox(0,0)[cr]{$\Ree$}}

\put(46.25,90){\makebox(0,0)[cl]{$\Ree$}}

\linethickness{0.35mm}
\put(35,35){\line(1,0){10}}
\linethickness{0.35mm}
\put(35,35){\line(0,1){10}}
\linethickness{0.35mm}
\put(35,70){\line(1,0){20}}
\linethickness{0.35mm}
\put(55,50){\line(0,1){20}}
\linethickness{0.35mm}
\put(45,50){\line(1,0){10}}
\linethickness{0.35mm}
\put(35,60){\line(0,1){10}}
\linethickness{0.35mm}
\multiput(35,60)(0.12,-0.12){83}{\line(1,0){0.12}}
\linethickness{1mm}
\put(40,40){\line(0,1){15}}
\linethickness{0.35mm}
\multiput(35,45)(0.12,-0.12){83}{\line(1,0){0.12}}
\put(20,45){\makebox(0,0)[cc]{\EQLS}}

\put(37.5,48.75){\makebox(0,0)[cr]{$\Aee$}}

\put(92.5,42.5){\makebox(0,0)[cc]{$\prtll$}}

\put(88.75,22.5){\makebox(0,0)[cc]{$\Jee$}}

\put(37.5,37.5){\makebox(0,0)[cc]{$\Jee$}}

\put(45,61.25){\makebox(0,0)[cc]{$\univrsl$}}

\end{picture}


==> PIC/sciences.tex <==
%%Created by jPicEdt 1.4.1_03: mixed JPIC-XML/LaTeX format
%%Tue Aug 09 15:27:37 HST 2016
%%Begin JPIC-XML
%<?xml version="1.0" standalone="yes"?>
%<jpic x-min="0" x-max="150" y-min="-1.25" y-max="150" auto-bounding="true">
%<ellipse p3= "(150,0)"
%	 p2= "(150,150)"
%	 p1= "(0,150)"
%	 closure= "open"
%	 fill-style= "none"
%	 angle-end= "0"
%	 angle-start= "0"
%	 />
%<ellipse p3= "(140,-1.25)"
%	 p2= "(140,128.75)"
%	 p1= "(10,131.25)"
%	 closure= "open"
%	 fill-style= "none"
%	 angle-end= "0"
%	 angle-start= "0"
%	 />
%<ellipse p3= "(130,-1.25)"
%	 p2= "(130,108.75)"
%	 p1= "(20,111.25)"
%	 closure= "open"
%	 fill-style= "none"
%	 angle-end= "0"
%	 angle-start= "0"
%	 />
%<ellipse p3= "(120,0)"
%	 p2= "(120,90)"
%	 p1= "(30,90)"
%	 closure= "open"
%	 fill-style= "none"
%	 angle-end= "0"
%	 angle-start= "0"
%	 />
%<ellipse stroke-width= "1"
%	 p3= "(110,0)"
%	 p2= "(110,70)"
%	 p1= "(40,70)"
%	 closure= "open"
%	 fill-style= "none"
%	 angle-end= "0"
%	 angle-start= "0"
%	 />
%<ellipse p3= "(100,0)"
%	 p2= "(100,50)"
%	 stroke-style= "dashed"
%	 p1= "(50,50)"
%	 stroke-dasharray= "1;1"
%	 closure= "open"
%	 fill-style= "none"
%	 angle-end= "0"
%	 angle-start= "0"
%	 />
%<text text-vert-align= "center-v"
%	 anchor-point= "(75,140)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\physics
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(75,120)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\chemistry
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(75,100)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\biology
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(75,80)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\linguistics
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(75,58.12)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\compSci
%</text>
%<ellipse p3= "(92.5,0)"
%	 p2= "(92.5,35)"
%	 stroke-style= "dashed"
%	 p1= "(57.5,35)"
%	 stroke-dasharray= "1;1"
%	 closure= "open"
%	 fill-style= "none"
%	 angle-end= "0"
%	 angle-start= "0"
%	 />
%<text text-vert-align= "center-v"
%	 anchor-point= "(75,41.25)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\computer
%</text>
%<ellipse p3= "(85.94,0.16)"
%	 p2= "(84.69,20.78)"
%	 stroke-style= "dashed"
%	 p1= "(64.06,19.84)"
%	 stroke-dasharray= "1;1"
%	 closure= "open"
%	 fill-style= "none"
%	 angle-end= "0"
%	 angle-start= "0"
%	 />
%<text text-vert-align= "center-v"
%	 anchor-point= "(75,25.62)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\resource
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(75,10)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\network
%</text>
%</jpic>
%%End JPIC-XML
%PSTricks content-type (pstricks.sty package needed)
%Add \usepackage{pstricks} in the preamble of your LaTeX file
%You can rescale the whole picture (to 80% for instance) by using the command \def\JPicScale{0.8}
\ifx\JPicScale\undefined\def\JPicScale{1}\fi
\psset{unit=\JPicScale mm}
\psset{linewidth=0.3,dotsep=1,hatchwidth=0.3,hatchsep=1.5,shadowsize=1,dimen=middle}
\psset{dotsize=0.7 2.5,dotscale=1 1,fillcolor=black}
\psset{arrowsize=1 2,arrowlength=1,arrowinset=0.25,tbarsize=0.7 5,bracketlength=0.15,rbracketlength=0.15}
\begin{pspicture}(0,0)(150,150)
\rput{0}(75,75){\psellipse[](0,0)(75,-75)}
\rput{134.72}(75,65){\psellipse[](0,0)(65.63,-64.38)}
\rput{134.67}(75,55){\psellipse[](0,0)(55.63,-54.38)}
\rput{0}(75,45){\psellipse[](0,0)(45,-45)}
\rput{0}(75,35){\psellipse[linewidth=1](0,0)(35,-35)}
\rput{0}(75,25){\psellipse[linestyle=dashed,dash=1 1](0,0)(25,-25)}
\rput(75,140){\physics}
\rput(75,120){\chemistry}
\rput(75,100){\biology}
\rput(75,80){\linguistics}
\rput(75,58.12){\compSci}
\rput{0}(75,17.5){\psellipse[linestyle=dashed,dash=1 1](0,0)(17.5,-17.5)}
\rput(75,41.25){\computer}
\rput{-42.56}(75,10){\psellipse[linestyle=dashed,dash=1 1](0,0)(10.4,-10.25)}
\rput(75,25.62){\resource}
\rput(75,10){\network}
\end{pspicture}


==> PIC/seq-1.tex <==
%%Created by jPicEdt 1.4.1_03: mixed JPIC-XML/LaTeX format
%%Wed Jul 24 17:31:57 GMT-10:00 2019
%%Begin JPIC-XML
%<?xml version="1.0" standalone="yes"?>
%<jpic x-min="0" x-max="80" y-min="-55" y-max="55" auto-bounding="true">
%<multicurve fill-style= "none"
%	 points= "(0,-15);(0,-15);(30,-15);(30,-15)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(0,-15);(0,-15);(0,-35);(0,-35)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(30,-35);(30,-35);(30,-15);(30,-15)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(15,15);(15,15);(15,-15);(15,-15)"
%	 stroke-width= "0.75"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(12.5,0)"
%	 text-frame= "noframe"
%	 stroke-width= "0.75"
%	 text-hor-align= "right"
%	 >
%$\nameslang$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(12.5,-52.5)"
%	 text-frame= "noframe"
%	 stroke-width= "0.75"
%	 text-hor-align= "right"
%	 >
%$\inputt$
%</text>
%<multicurve fill-style= "none"
%	 points= "(0,-35);(0,-35);(30,-35);(30,-35)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(15,-35);(15,-35);(15,-55);(15,-55)"
%	 stroke-width= "0.75"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(15,-25)"
%	 text-frame= "noframe"
%	 stroke-width= "0.75"
%	 text-hor-align= "center-h"
%	 >
%\machine
%</text>
%<multicurve fill-style= "none"
%	 points= "(0,35);(0,35);(30,35);(30,35)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(0,35);(0,35);(0,15);(0,15)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(30,15);(30,15);(30,35);(30,35)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(15,55);(15,55);(15,35);(15,35)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(0,15);(0,15);(30,15);(30,15)"
%	 stroke-width= "0.75"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(15,25)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\gee
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(17.5,52.5)"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%\outpt
%</text>
%<multicurve fill-style= "none"
%	 points= "(50,10);(50,10);(80,10);(80,10)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(50,10);(50,10);(50,-10);(50,-10)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(80,-10);(80,-10);(80,10);(80,10)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(65,55);(65,55);(65,10);(65,10)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(50,-10);(50,-10);(80,-10);(80,-10)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(65,-10);(65,-10);(65,-55);(65,-55)"
%	 stroke-width= "0.75"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(62.5,-52.5)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\otherinputt$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(67.5,52.5)"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\otheroutpt$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(65,0)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\hee$
%</text>
%</jpic>
%%End JPIC-XML
%PSTricks content-type (pstricks.sty package needed)
%Add \usepackage{pstricks} in the preamble of your LaTeX file
%You can rescale the whole picture (to 80% for instance) by using the command \def\JPicScale{0.8}
\ifx\JPicScale\undefined\def\JPicScale{1}\fi
\psset{unit=\JPicScale mm}
\psset{linewidth=0.3,dotsep=1,hatchwidth=0.3,hatchsep=1.5,shadowsize=1,dimen=middle}
\psset{dotsize=0.7 2.5,dotscale=1 1,fillcolor=black}
\psset{arrowsize=1 2,arrowlength=1,arrowinset=0.25,tbarsize=0.7 5,bracketlength=0.15,rbracketlength=0.15}
\begin{pspicture}(0,0)(80,55)
\psline[linewidth=0.75](0,-15)(30,-15)
\psline[linewidth=0.75](0,-15)(0,-35)
\psline[linewidth=0.75](30,-35)(30,-15)
\psline[linewidth=0.75](15,15)(15,-15)
\rput[r](12.5,0){$\nameslang$}
\rput[r](12.5,-52.5){$\inputt$}
\psline[linewidth=0.75](0,-35)(30,-35)
\psline[linewidth=0.75](15,-35)(15,-55)
\rput(15,-25){\machine}
\psline[linewidth=0.75](0,35)(30,35)
\psline[linewidth=0.75](0,35)(0,15)
\psline[linewidth=0.75](30,15)(30,35)
\psline[linewidth=0.75](15,55)(15,35)
\psline[linewidth=0.75](0,15)(30,15)
\rput(15,25){\gee}
\rput[l](17.5,52.5){\outpt}
\psline[linewidth=0.75](50,10)(80,10)
\psline[linewidth=0.75](50,10)(50,-10)
\psline[linewidth=0.75](80,-10)(80,10)
\psline[linewidth=0.75](65,55)(65,10)
\psline[linewidth=0.75](50,-10)(80,-10)
\psline[linewidth=0.75](65,-10)(65,-55)
\rput[r](62.5,-52.5){$\otherinputt$}
\rput[l](67.5,52.5){$\otheroutpt$}
\rput(65,0){$\hee$}
\end{pspicture}


==> PIC/seq-2.tex <==
%%Created by jPicEdt 1.4.1_03: mixed JPIC-XML/LaTeX format
%%Wed Jul 24 17:31:07 GMT-10:00 2019
%%Begin JPIC-XML
%<?xml version="1.0" standalone="yes"?>
%<jpic x-min="0" x-max="80" y-min="-55" y-max="55" auto-bounding="true">
%<multicurve fill-style= "none"
%	 points= "(0,-15);(0,-15);(30,-15);(30,-15)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(0,-15);(0,-15);(0,-35);(0,-35)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(30,-35);(30,-35);(30,-15);(30,-15)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(15,15);(15,15);(15,-15);(15,-15)"
%	 stroke-width= "0.75"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(12.5,0)"
%	 text-frame= "noframe"
%	 stroke-width= "0.75"
%	 text-hor-align= "right"
%	 >
%$\nameslang$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(12.5,-52.5)"
%	 text-frame= "noframe"
%	 stroke-width= "0.75"
%	 text-hor-align= "right"
%	 >
%$\inputt$
%</text>
%<multicurve fill-style= "none"
%	 points= "(0,-35);(0,-35);(30,-35);(30,-35)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(15,-35);(15,-35);(15,-55);(15,-55)"
%	 stroke-width= "0.75"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(15,-25)"
%	 text-frame= "noframe"
%	 stroke-width= "0.75"
%	 text-hor-align= "center-h"
%	 >
%\machine
%</text>
%<multicurve fill-style= "none"
%	 points= "(0,35);(0,35);(30,35);(30,35)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(0,35);(0,35);(0,15);(0,15)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(30,15);(30,15);(30,35);(30,35)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(15,55);(15,55);(15,35);(15,35)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(0,15);(0,15);(30,15);(30,15)"
%	 stroke-width= "0.75"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(15,25)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\gee
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(17.5,52.5)"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%\outpt
%</text>
%<multicurve fill-style= "none"
%	 points= "(50,35);(50,35);(80,35);(80,35)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(50,35);(50,35);(50,15);(50,15)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(80,15);(80,15);(80,35);(80,35)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(65,55);(65,55);(65,35);(65,35)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(50,15);(50,15);(80,15);(80,15)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(65,15);(65,15);(65,-55);(65,-55)"
%	 stroke-width= "0.75"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(62.5,-52.5)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\otherinputt$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(67.5,52.5)"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\otheroutpt$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(65,25)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\hee$
%</text>
%</jpic>
%%End JPIC-XML
%PSTricks content-type (pstricks.sty package needed)
%Add \usepackage{pstricks} in the preamble of your LaTeX file
%You can rescale the whole picture (to 80% for instance) by using the command \def\JPicScale{0.8}
\ifx\JPicScale\undefined\def\JPicScale{1}\fi
\psset{unit=\JPicScale mm}
\psset{linewidth=0.3,dotsep=1,hatchwidth=0.3,hatchsep=1.5,shadowsize=1,dimen=middle}
\psset{dotsize=0.7 2.5,dotscale=1 1,fillcolor=black}
\psset{arrowsize=1 2,arrowlength=1,arrowinset=0.25,tbarsize=0.7 5,bracketlength=0.15,rbracketlength=0.15}
\begin{pspicture}(0,0)(80,55)
\psline[linewidth=0.75](0,-15)(30,-15)
\psline[linewidth=0.75](0,-15)(0,-35)
\psline[linewidth=0.75](30,-35)(30,-15)
\psline[linewidth=0.75](15,15)(15,-15)
\rput[r](12.5,0){$\nameslang$}
\rput[r](12.5,-52.5){$\inputt$}
\psline[linewidth=0.75](0,-35)(30,-35)
\psline[linewidth=0.75](15,-35)(15,-55)
\rput(15,-25){\machine}
\psline[linewidth=0.75](0,35)(30,35)
\psline[linewidth=0.75](0,35)(0,15)
\psline[linewidth=0.75](30,15)(30,35)
\psline[linewidth=0.75](15,55)(15,35)
\psline[linewidth=0.75](0,15)(30,15)
\rput(15,25){\gee}
\rput[l](17.5,52.5){\outpt}
\psline[linewidth=0.75](50,35)(80,35)
\psline[linewidth=0.75](50,35)(50,15)
\psline[linewidth=0.75](80,15)(80,35)
\psline[linewidth=0.75](65,55)(65,35)
\psline[linewidth=0.75](50,15)(80,15)
\psline[linewidth=0.75](65,15)(65,-55)
\rput[r](62.5,-52.5){$\otherinputt$}
\rput[l](67.5,52.5){$\otheroutpt$}
\rput(65,25){$\hee$}
\end{pspicture}


==> PIC/seq-3.tex <==
%%Created by jPicEdt 1.4.1_03: mixed JPIC-XML/LaTeX format
%%Wed Oct 25 15:30:40 EDT 2017
%%Begin JPIC-XML
%<?xml version="1.0" standalone="yes"?>
%<jpic x-min="25" x-max="265" y-min="25" y-max="135" auto-bounding="true">
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(125,80);(125,80);(125,30);(125,30)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(140,80);(140,80);(140,30);(140,30)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(119.99,80);(119.99,80);(99.99,100);(99.99,100)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(99.99,100);(99.99,100);(160,100);(160,100)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(119.99,80);(119.99,80);(160,80);(160,80)"
%	 />
%<text stroke-width= "0.75"
%	 text-vert-align= "center-v"
%	 anchor-point= "(175,80)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\EQLS
%</text>
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(160,100);(160,100);(160,80);(160,80)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(155,130);(155,130);(155,100);(155,100)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(110,90);(110,90);(100,80);(100,80)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(50,90);(50,90);(30,110);(30,110)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(30,110);(30,110);(60,110);(60,110)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(40,100);(40,100);(25,85);(25,85)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(50,90);(50,90);(60,90);(60,90)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(60,110);(60,110);(60,90);(60,90)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(55,130);(55,130);(55,110);(55,110)"
%	 />
%<text stroke-width= "0.75"
%	 text-vert-align= "center-v"
%	 anchor-point= "(25,25)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\Progtype$
%</text>
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(55,90);(55,90);(55,70);(55,70)"
%	 />
%<text text-vert-align= "center-v"
%	 anchor-point= "(52.5,100)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\universal$
%</text>
%<text stroke-width= "0.8"
%	 text-vert-align= "center-v"
%	 anchor-point= "(155,135)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\Progn$
%</text>
%<text stroke-width= "0.8"
%	 text-vert-align= "center-v"
%	 anchor-point= "(55,135)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\Progn$
%</text>
%<text stroke-width= "0.8"
%	 text-vert-align= "center-v"
%	 anchor-point= "(52.5,80)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\Progm$
%</text>
%<text stroke-width= "0.8"
%	 text-vert-align= "center-v"
%	 anchor-point= "(140,90)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\universalmkn$
%</text>
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(90,90);(90,90);(90,70);(90,70)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(90,70);(90,70);(110,70);(110,70)"
%	 />
%<text stroke-width= "0.75"
%	 text-vert-align= "center-v"
%	 anchor-point= "(96.25,76.25)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\program
%</text>
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(90,90);(90,90);(110,70);(110,70)"
%	 />
%<text stroke-width= "0.75"
%	 text-vert-align= "center-v"
%	 anchor-point= "(75,80)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\EQLS
%</text>
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(50,50);(50,50);(30,70);(30,70)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(30,70);(30,70);(60,70);(60,70)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(40,60);(40,60);(40,30);(40,30)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(50,50);(50,50);(60,50);(60,50)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(60,70);(60,70);(60,50);(60,50)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(55,50);(55,50);(55,30);(55,30)"
%	 />
%<text text-vert-align= "center-v"
%	 anchor-point= "(52.5,60)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\universal$
%</text>
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(25,85);(25,85);(25,30);(25,30)"
%	 />
%<text stroke-width= "0.75"
%	 text-vert-align= "center-v"
%	 anchor-point= "(40,25)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\Progtype$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(55,25)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\Progell$
%</text>
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(155,80);(155,80);(155,30);(155,30)"
%	 />
%<text text-vert-align= "center-v"
%	 anchor-point= "(155,25)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\Progell$
%</text>
%<text stroke-width= "0.75"
%	 text-vert-align= "center-v"
%	 anchor-point= "(140,25)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\Progtype$
%</text>
%<text stroke-width= "0.75"
%	 text-vert-align= "center-v"
%	 anchor-point= "(125,25)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\Progtype$
%</text>
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(225,70);(225,70);(225,30);(225,30)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(237.5,70);(237.5,70);(237.5,30);(237.5,30)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(219.99,70);(219.99,70);(199.99,90);(199.99,90)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(235,100);(235,100);(265,100);(265,100)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(255,80);(255,80);(265,80);(265,80)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(265,100);(265,100);(265,80);(265,80)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(260,130);(260,130);(260,100);(260,100)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(210,80);(210,80);(200,70);(200,70)"
%	 />
%<text stroke-width= "0.8"
%	 text-vert-align= "center-v"
%	 anchor-point= "(260,135)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\Progn$
%</text>
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(190,80);(190,80);(190,60);(190,60)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(190,60);(190,60);(210,60);(210,60)"
%	 />
%<text stroke-width= "0.75"
%	 text-vert-align= "center-v"
%	 anchor-point= "(196.25,66.25)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\program
%</text>
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(190,80);(190,80);(210,60);(210,60)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(260,80);(260,80);(260,30);(260,30)"
%	 />
%<text text-vert-align= "center-v"
%	 anchor-point= "(260,25)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\Progell$
%</text>
%<text stroke-width= "0.75"
%	 text-vert-align= "center-v"
%	 anchor-point= "(237.5,25)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\Progtype$
%</text>
%<text stroke-width= "0.75"
%	 text-vert-align= "center-v"
%	 anchor-point= "(225,25)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\Progtype$
%</text>
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(255,80);(255,80);(235,100);(235,100)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(220,70);(220,70);(245,70);(245,70)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(245,70);(245,70);(225,90);(225,90)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(200,90);(200,90);(225,90);(225,90)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(245,90);(245,90);(235,80);(235,80)"
%	 />
%<text text-vert-align= "center-v"
%	 anchor-point= "(257.5,90)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\universal$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(222.5,80)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\partial$
%</text>
%<multicurve stroke-width= "0.75"
%	 stroke-color= "#ff6666"
%	 fill-style= "none"
%	 points= "(185,95);(185,95);(185,55);(185,55)"
%	 />
%<multicurve stroke-width= "0.75"
%	 stroke-color= "#ff6666"
%	 fill-style= "none"
%	 points= "(185,55);(185,55);(255,55);(255,55)"
%	 />
%<multicurve stroke-width= "0.75"
%	 stroke-color= "#ff6666"
%	 fill-style= "none"
%	 points= "(185,95);(185,95);(230,95);(230,95)"
%	 />
%<multicurve stroke-width= "0.75"
%	 stroke-color= "#ff6666"
%	 fill-style= "none"
%	 points= "(230,95);(230,95);(255,70);(255,70)"
%	 />
%<multicurve stroke-width= "0.75"
%	 stroke-color= "#ff6666"
%	 fill-style= "none"
%	 points= "(255,55);(255,55);(255,70);(255,70)"
%	 />
%<text text-vert-align= "bottom"
%	 anchor-point= "(252.5,58.75)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\seqq$
%</text>
%</jpic>
%%End JPIC-XML
%PSTricks content-type (pstricks.sty package needed)
%Add \usepackage{pstricks} in the preamble of your LaTeX file
%You can rescale the whole picture (to 80% for instance) by using the command \def\JPicScale{0.8}
\ifx\JPicScale\undefined\def\JPicScale{1}\fi
\psset{unit=\JPicScale mm}
\psset{linewidth=0.3,dotsep=1,hatchwidth=0.3,hatchsep=1.5,shadowsize=1,dimen=middle}
\psset{dotsize=0.7 2.5,dotscale=1 1,fillcolor=black}
\psset{arrowsize=1 2,arrowlength=1,arrowinset=0.25,tbarsize=0.7 5,bracketlength=0.15,rbracketlength=0.15}
\begin{pspicture}(0,0)(265,135)
\psline[linewidth=0.75](125,80)(125,30)
\psline[linewidth=0.75](140,80)(140,30)
\psline[linewidth=0.75](119.99,80)(99.99,100)
\psline[linewidth=0.75](99.99,100)(160,100)
\psline[linewidth=0.75](119.99,80)(160,80)
\rput(175,80){\EQLS}
\psline[linewidth=0.75](160,100)(160,80)
\psline[linewidth=0.75](155,130)(155,100)
\psline[linewidth=0.75](110,90)(100,80)
\psline[linewidth=0.75](50,90)(30,110)
\psline[linewidth=0.75](30,110)(60,110)
\psline[linewidth=0.75](40,100)(25,85)
\psline[linewidth=0.75](50,90)(60,90)
\psline[linewidth=0.75](60,110)(60,90)
\psline[linewidth=0.75](55,130)(55,110)
\rput(25,25){$\Progtype$}
\psline[linewidth=0.75](55,90)(55,70)
\rput(52.5,100){$\universal$}
\rput(155,135){$\Progn$}
\rput(55,135){$\Progn$}
\rput[r](52.5,80){$\Progm$}
\rput(140,90){$\universalmkn$}
\psline[linewidth=0.75](90,90)(90,70)
\psline[linewidth=0.75](90,70)(110,70)
\rput(96.25,76.25){\program}
\psline[linewidth=0.75](90,90)(110,70)
\rput(75,80){\EQLS}
\psline[linewidth=0.75](50,50)(30,70)
\psline[linewidth=0.75](30,70)(60,70)
\psline[linewidth=0.75](40,60)(40,30)
\psline[linewidth=0.75](50,50)(60,50)
\psline[linewidth=0.75](60,70)(60,50)
\psline[linewidth=0.75](55,50)(55,30)
\rput(52.5,60){$\universal$}
\psline[linewidth=0.75](25,85)(25,30)
\rput(40,25){$\Progtype$}
\rput(55,25){$\Progell$}
\psline[linewidth=0.75](155,80)(155,30)
\rput(155,25){$\Progell$}
\rput(140,25){$\Progtype$}
\rput(125,25){$\Progtype$}
\psline[linewidth=0.75](225,70)(225,30)
\psline[linewidth=0.75](237.5,70)(237.5,30)
\psline[linewidth=0.75](219.99,70)(199.99,90)
\psline[linewidth=0.75](235,100)(265,100)
\psline[linewidth=0.75](255,80)(265,80)
\psline[linewidth=0.75](265,100)(265,80)
\psline[linewidth=0.75](260,130)(260,100)
\psline[linewidth=0.75](210,80)(200,70)
\rput(260,135){$\Progn$}
\psline[linewidth=0.75](190,80)(190,60)
\psline[linewidth=0.75](190,60)(210,60)
\rput(196.25,66.25){\program}
\psline[linewidth=0.75](190,80)(210,60)
\psline[linewidth=0.75](260,80)(260,30)
\rput(260,25){$\Progell$}
\rput(237.5,25){$\Progtype$}
\rput(225,25){$\Progtype$}
\psline[linewidth=0.75](255,80)(235,100)
\psline[linewidth=0.75](220,70)(245,70)
\psline[linewidth=0.75](245,70)(225,90)
\psline[linewidth=0.75](200,90)(225,90)
\psline[linewidth=0.75](245,90)(235,80)
\rput(257.5,90){$\universal$}
\rput(222.5,80){$\partial$}
\newrgbcolor{userLineColour}{1 0.4 0.4}
\psline[linewidth=0.75,linecolor=userLineColour](185,95)(185,55)
\newrgbcolor{userLineColour}{1 0.4 0.4}
\psline[linewidth=0.75,linecolor=userLineColour](185,55)(255,55)
\newrgbcolor{userLineColour}{1 0.4 0.4}
\psline[linewidth=0.75,linecolor=userLineColour](185,95)(230,95)
\newrgbcolor{userLineColour}{1 0.4 0.4}
\psline[linewidth=0.75,linecolor=userLineColour](230,95)(255,70)
\newrgbcolor{userLineColour}{1 0.4 0.4}
\psline[linewidth=0.75,linecolor=userLineColour](255,55)(255,70)
\rput[br](252.5,58.75){$\seqq$}
\end{pspicture}


==> PIC/seq-33.tex <==
%%Created by jPicEdt 1.4.1_03: mixed JPIC-XML/LaTeX format
%%Sun Jul 24 16:40:04 GMT+01:00 2022
%%Begin JPIC-XML
%<?xml version="1.0" standalone="yes"?>
%<jpic x-min="16.25" x-max="246.25" y-min="0" y-max="100" auto-bounding="true">
%<multicurve fill-style= "none"
%	 points= "(110,50);(110,50);(110,0);(110,0)"
%	 stroke-width= "0.7"
%	 />
%<multicurve fill-style= "none"
%	 points= "(125,50);(125,50);(125,0);(125,0)"
%	 stroke-width= "0.7"
%	 />
%<multicurve fill-style= "none"
%	 points= "(104.99,50);(104.99,50);(84.99,70);(84.99,70)"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(84.99,70);(84.99,70);(145,70);(145,70)"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(104.99,50);(104.99,50);(145,50);(145,50)"
%	 stroke-width= "0.35"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(160,50)"
%	 text-frame= "noframe"
%	 stroke-width= "0.35"
%	 text-hor-align= "center-h"
%	 >
%\EQLS
%</text>
%<multicurve fill-style= "none"
%	 points= "(145,70);(145,70);(145,50);(145,50)"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(140,100);(140,100);(140,70);(140,70)"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(45,60);(45,60);(25,80);(25,80)"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(25,80);(25,80);(55,80);(55,80)"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(35,70);(35,70);(20,55);(20,55)"
%	 stroke-width= "0.7"
%	 />
%<multicurve fill-style= "none"
%	 points= "(45,60);(45,60);(55,60);(55,60)"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(55,80);(55,80);(55,60);(55,60)"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(50,100);(50,100);(50,80);(50,80)"
%	 stroke-width= "0.35"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(16.25,1.25)"
%	 text-frame= "noframe"
%	 stroke-width= "0.35"
%	 text-hor-align= "center-h"
%	 >
%$\Progtype$
%</text>
%<multicurve fill-style= "none"
%	 points= "(50,60);(50,60);(50,40);(50,40)"
%	 stroke-width= "0.35"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(47.5,70)"
%	 text-frame= "noframe"
%	 stroke-width= "0.35"
%	 text-hor-align= "center-h"
%	 >
%$\universal$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(146.25,98.75)"
%	 text-frame= "noframe"
%	 stroke-width= "0.35"
%	 text-hor-align= "center-h"
%	 >
%$\Progn$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(56.25,98.75)"
%	 text-frame= "noframe"
%	 stroke-width= "0.35"
%	 text-hor-align= "center-h"
%	 >
%$\Progn$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(47.5,50)"
%	 text-frame= "noframe"
%	 stroke-width= "0.35"
%	 text-hor-align= "right"
%	 >
%$\Progm$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(125,60)"
%	 text-frame= "noframe"
%	 stroke-width= "0.35"
%	 text-hor-align= "center-h"
%	 >
%$\universalmkn$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(70,50)"
%	 text-frame= "noframe"
%	 stroke-width= "0.35"
%	 text-hor-align= "center-h"
%	 >
%\EQLS
%</text>
%<multicurve fill-style= "none"
%	 points= "(45,20);(45,20);(25,40);(25,40)"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(25,40);(25,40);(55,40);(55,40)"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(35,30);(35,30);(35,0);(35,0)"
%	 stroke-width= "0.7"
%	 />
%<multicurve fill-style= "none"
%	 points= "(45,20);(45,20);(55,20);(55,20)"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(55,40);(55,40);(55,20);(55,20)"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(50,20);(50,20);(50,0);(50,0)"
%	 stroke-width= "0.35"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(47.5,30)"
%	 text-frame= "noframe"
%	 stroke-width= "0.35"
%	 text-hor-align= "center-h"
%	 >
%$\universal$
%</text>
%<multicurve fill-style= "none"
%	 points= "(20,55);(20,55);(20,0);(20,0)"
%	 stroke-width= "0.7"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(31.25,1.25)"
%	 text-frame= "noframe"
%	 stroke-width= "0.35"
%	 text-hor-align= "center-h"
%	 >
%$\Progtype$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(46.25,1.25)"
%	 text-frame= "noframe"
%	 stroke-width= "0.35"
%	 text-hor-align= "center-h"
%	 >
%$\Progell$
%</text>
%<multicurve fill-style= "none"
%	 points= "(140,50);(140,50);(140,0);(140,0)"
%	 stroke-width= "0.35"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(136.25,1.25)"
%	 text-frame= "noframe"
%	 stroke-width= "0.35"
%	 text-hor-align= "center-h"
%	 >
%$\Progell$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(121.25,1.25)"
%	 text-frame= "noframe"
%	 stroke-width= "0.35"
%	 text-hor-align= "center-h"
%	 >
%$\Progtype$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(106.25,1.25)"
%	 text-frame= "noframe"
%	 stroke-width= "0.35"
%	 text-hor-align= "center-h"
%	 >
%$\Progtype$
%</text>
%<multicurve fill-style= "none"
%	 points= "(205,40);(205,40);(205,0);(205,0)"
%	 stroke-width= "0.7"
%	 />
%<multicurve fill-style= "none"
%	 points= "(217.5,40);(217.5,40);(217.5,0);(217.5,0)"
%	 stroke-width= "0.7"
%	 />
%<multicurve fill-style= "none"
%	 points= "(199.99,40);(199.99,40);(179.99,60);(179.99,60)"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(215,70);(215,70);(245,70);(245,70)"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(235,50);(235,50);(245,50);(245,50)"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(245,70);(245,70);(245,50);(245,50)"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(240,100);(240,100);(240,70);(240,70)"
%	 stroke-width= "0.35"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(246.25,98.75)"
%	 text-frame= "noframe"
%	 stroke-width= "0.35"
%	 text-hor-align= "center-h"
%	 >
%$\Progn$
%</text>
%<multicurve fill-style= "none"
%	 points= "(240,50);(240,50);(240,0);(240,0)"
%	 stroke-width= "0.35"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(236.25,1.25)"
%	 text-frame= "noframe"
%	 stroke-width= "0.35"
%	 text-hor-align= "center-h"
%	 >
%$\Progell$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(213.75,1.25)"
%	 text-frame= "noframe"
%	 stroke-width= "0.35"
%	 text-hor-align= "center-h"
%	 >
%$\Progtype$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(201.25,1.25)"
%	 text-frame= "noframe"
%	 stroke-width= "0.35"
%	 text-hor-align= "center-h"
%	 >
%$\Progtype$
%</text>
%<multicurve fill-style= "none"
%	 points= "(235,50);(235,50);(215,70);(215,70)"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(200,40);(200,40);(225,40);(225,40)"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(225,40);(225,40);(205,60);(205,60)"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(180,60);(180,60);(205,60);(205,60)"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(225,60);(225,60);(215,50);(215,50)"
%	 stroke-width= "0.7"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(237.5,60)"
%	 text-frame= "noframe"
%	 stroke-width= "0.35"
%	 text-hor-align= "center-h"
%	 >
%$\universal$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(202.5,50)"
%	 text-frame= "noframe"
%	 stroke-width= "0.35"
%	 text-hor-align= "center-h"
%	 >
%$\partial$
%</text>
%<multicurve fill-style= "none"
%	 points= "(175,65);(175,65);(175,25);(175,25)"
%	 stroke-color= "#ff0033"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(175,25);(175,25);(235,25);(235,25)"
%	 stroke-color= "#ff0033"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(175,65);(175,65);(210,65);(210,65)"
%	 stroke-color= "#ff0033"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(210,65);(210,65);(235,40);(235,40)"
%	 stroke-color= "#ff0033"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(235,25);(235,25);(235,40);(235,40)"
%	 stroke-color= "#ff0033"
%	 stroke-width= "0.35"
%	 />
%<text text-vert-align= "bottom"
%	 fill-style= "none"
%	 anchor-point= "(232.5,28.75)"
%	 text-frame= "noframe"
%	 stroke-width= "0.35"
%	 text-hor-align= "right"
%	 >
%$\seqq$
%</text>
%<multicurve fill-style= "none"
%	 points= "(95,60);(95,60);(95,50);(95,50)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(85,60);(85,60);(85,40);(85,40)"
%	 stroke-width= "0.4"
%	 />
%<multicurve fill-style= "none"
%	 points= "(85,40);(85,40);(105,40);(105,40)"
%	 stroke-width= "0.4"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(91.25,46.25)"
%	 text-frame= "noframe"
%	 stroke-width= "0.4"
%	 text-hor-align= "center-h"
%	 >
%\program
%</text>
%<multicurve fill-style= "none"
%	 points= "(85,60);(85,60);(105,40);(105,40)"
%	 stroke-width= "0.4"
%	 />
%<multicurve fill-style= "none"
%	 points= "(190,50);(190,50);(190,40);(190,40)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(180,50);(180,50);(180,30);(180,30)"
%	 stroke-width= "0.4"
%	 />
%<multicurve fill-style= "none"
%	 points= "(180,30);(180,30);(200,30);(200,30)"
%	 stroke-width= "0.4"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(186.25,36.25)"
%	 text-frame= "noframe"
%	 stroke-width= "0.4"
%	 text-hor-align= "center-h"
%	 >
%\program
%</text>
%<multicurve fill-style= "none"
%	 points= "(180,50);(180,50);(200,30);(200,30)"
%	 stroke-width= "0.4"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(215,50)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\Dottt
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(190,40)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\Dottt
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(95,50)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\Dottt
%</text>
%</jpic>
%%End JPIC-XML
%LaTeX-picture environment using emulated lines and arcs
%You can rescale the whole picture (to 80% for instance) by using the command \def\JPicScale{0.8}
\ifx\JPicScale\undefined\def\JPicScale{1}\fi
\unitlength \JPicScale mm
\begin{picture}(246.25,100)(0,0)
\linethickness{0.7mm}
\put(110,0){\line(0,1){50}}
\linethickness{0.7mm}
\put(125,0){\line(0,1){50}}
\linethickness{0.35mm}
\multiput(84.99,70)(0.12,-0.12){167}{\line(1,0){0.12}}
\linethickness{0.35mm}
\put(84.99,70){\line(1,0){60.01}}
\linethickness{0.35mm}
\put(104.99,50){\line(1,0){40.01}}
\put(160,50){\makebox(0,0)[cc]{\EQLS}}

\linethickness{0.35mm}
\put(145,50){\line(0,1){20}}
\linethickness{0.35mm}
\put(140,70){\line(0,1){30}}
\linethickness{0.35mm}
\multiput(25,80)(0.12,-0.12){167}{\line(1,0){0.12}}
\linethickness{0.35mm}
\put(25,80){\line(1,0){30}}
\linethickness{0.7mm}
\multiput(20,55)(0.12,0.12){125}{\line(1,0){0.12}}
\linethickness{0.35mm}
\put(45,60){\line(1,0){10}}
\linethickness{0.35mm}
\put(55,60){\line(0,1){20}}
\linethickness{0.35mm}
\put(50,80){\line(0,1){20}}
\put(16.25,1.25){\makebox(0,0)[cc]{$\Progtype$}}

\linethickness{0.35mm}
\put(50,40){\line(0,1){20}}
\put(47.5,70){\makebox(0,0)[cc]{$\universal$}}

\put(146.25,98.75){\makebox(0,0)[cc]{$\Progn$}}

\put(56.25,98.75){\makebox(0,0)[cc]{$\Progn$}}

\put(47.5,50){\makebox(0,0)[cr]{$\Progm$}}

\put(125,60){\makebox(0,0)[cc]{$\universalmkn$}}

\put(70,50){\makebox(0,0)[cc]{\EQLS}}

\linethickness{0.35mm}
\multiput(25,40)(0.12,-0.12){167}{\line(1,0){0.12}}
\linethickness{0.35mm}
\put(25,40){\line(1,0){30}}
\linethickness{0.7mm}
\put(35,0){\line(0,1){30}}
\linethickness{0.35mm}
\put(45,20){\line(1,0){10}}
\linethickness{0.35mm}
\put(55,20){\line(0,1){20}}
\linethickness{0.35mm}
\put(50,0){\line(0,1){20}}
\put(47.5,30){\makebox(0,0)[cc]{$\universal$}}

\linethickness{0.7mm}
\put(20,0){\line(0,1){55}}
\put(31.25,1.25){\makebox(0,0)[cc]{$\Progtype$}}

\put(46.25,1.25){\makebox(0,0)[cc]{$\Progell$}}

\linethickness{0.35mm}
\put(140,0){\line(0,1){50}}
\put(136.25,1.25){\makebox(0,0)[cc]{$\Progell$}}

\put(121.25,1.25){\makebox(0,0)[cc]{$\Progtype$}}

\put(106.25,1.25){\makebox(0,0)[cc]{$\Progtype$}}

\linethickness{0.7mm}
\put(205,0){\line(0,1){40}}
\linethickness{0.7mm}
\put(217.5,0){\line(0,1){40}}
\linethickness{0.35mm}
\multiput(179.99,60)(0.12,-0.12){167}{\line(1,0){0.12}}
\linethickness{0.35mm}
\put(215,70){\line(1,0){30}}
\linethickness{0.35mm}
\put(235,50){\line(1,0){10}}
\linethickness{0.35mm}
\put(245,50){\line(0,1){20}}
\linethickness{0.35mm}
\put(240,70){\line(0,1){30}}
\put(246.25,98.75){\makebox(0,0)[cc]{$\Progn$}}

\linethickness{0.35mm}
\put(240,0){\line(0,1){50}}
\put(236.25,1.25){\makebox(0,0)[cc]{$\Progell$}}

\put(213.75,1.25){\makebox(0,0)[cc]{$\Progtype$}}

\put(201.25,1.25){\makebox(0,0)[cc]{$\Progtype$}}

\linethickness{0.35mm}
\multiput(215,70)(0.12,-0.12){167}{\line(1,0){0.12}}
\linethickness{0.35mm}
\put(200,40){\line(1,0){25}}
\linethickness{0.35mm}
\multiput(205,60)(0.12,-0.12){167}{\line(1,0){0.12}}
\linethickness{0.35mm}
\put(180,60){\line(1,0){25}}
\linethickness{0.7mm}
\multiput(215,50)(0.12,0.12){83}{\line(1,0){0.12}}
\put(237.5,60){\makebox(0,0)[cc]{$\universal$}}

\put(202.5,50){\makebox(0,0)[cc]{$\partial$}}

\linethickness{0.35mm}
\put(175,25){\line(0,1){40}}
\linethickness{0.35mm}
\put(175,25){\line(1,0){60}}
\linethickness{0.35mm}
\put(175,65){\line(1,0){35}}
\linethickness{0.35mm}
\multiput(210,65)(0.12,-0.12){208}{\line(1,0){0.12}}
\linethickness{0.35mm}
\put(235,25){\line(0,1){15}}
\put(232.5,28.75){\makebox(0,0)[br]{$\seqq$}}

\linethickness{0.75mm}
\put(95,50){\line(0,1){10}}
\linethickness{0.4mm}
\put(85,40){\line(0,1){20}}
\linethickness{0.4mm}
\put(85,40){\line(1,0){20}}
\put(91.25,46.25){\makebox(0,0)[cc]{\program}}

\linethickness{0.4mm}
\multiput(85,60)(0.12,-0.12){167}{\line(1,0){0.12}}
\linethickness{0.75mm}
\put(190,40){\line(0,1){10}}
\linethickness{0.4mm}
\put(180,30){\line(0,1){20}}
\linethickness{0.4mm}
\put(180,30){\line(1,0){20}}
\put(186.25,36.25){\makebox(0,0)[cc]{\program}}

\linethickness{0.4mm}
\multiput(180,50)(0.12,-0.12){167}{\line(1,0){0.12}}
\put(215,50){\makebox(0,0)[cc]{\Dottt}}

\put(190,40){\makebox(0,0)[cc]{\Dottt}}

\put(95,50){\makebox(0,0)[cc]{\Dottt}}

\end{picture}


==> PIC/seq-34.tex <==
%%Created by jPicEdt 1.4.1_03: mixed JPIC-XML/LaTeX format
%%Wed May 18 19:12:35 GMT+01:00 2022
%%Begin JPIC-XML
%<?xml version="1.0" standalone="yes"?>
%<jpic x-min="-2.5" x-max="240" y-min="0" y-max="100" auto-bounding="true">
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(100,50);(100,50);(100,0);(100,0)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(115,50);(115,50);(115,0);(115,0)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.4"
%	 points= "(94.99,50);(94.99,50);(74.99,70);(74.99,70)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.4"
%	 points= "(74.99,70);(74.99,70);(135,70);(135,70)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.4"
%	 points= "(94.99,50);(94.99,50);(135,50);(135,50)"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 stroke-width= "0.4"
%	 anchor-point= "(150,50)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\EQLS
%</text>
%<multicurve fill-style= "none"
%	 stroke-width= "0.4"
%	 points= "(135,70);(135,70);(135,50);(135,50)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.4"
%	 points= "(130,100);(130,100);(130,70);(130,70)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(85,60);(85,60);(75,50);(75,50)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.4"
%	 points= "(25,60);(25,60);(5,80);(5,80)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.4"
%	 points= "(5,80);(5,80);(35,80);(35,80)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(15,70);(15,70);(0,55);(0,55)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.4"
%	 points= "(25,60);(25,60);(35,60);(35,60)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.4"
%	 points= "(35,80);(35,80);(35,60);(35,60)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.4"
%	 points= "(30,100);(30,100);(30,80);(30,80)"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 stroke-width= "0.4"
%	 anchor-point= "(-2.5,0)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\Progtype$
%</text>
%<multicurve fill-style= "none"
%	 stroke-width= "0.4"
%	 points= "(30,60);(30,60);(30,40);(30,40)"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 stroke-width= "0.4"
%	 anchor-point= "(27.5,70)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\universal$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 stroke-width= "0.4"
%	 anchor-point= "(132.5,100)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\Progn$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 stroke-width= "0.4"
%	 anchor-point= "(32.5,100)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\Progn$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 stroke-width= "0.4"
%	 anchor-point= "(27.5,50)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\Progm$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 stroke-width= "0.4"
%	 anchor-point= "(115,60)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\universalmkn$
%</text>
%<multicurve fill-style= "none"
%	 stroke-width= "0.4"
%	 points= "(65,60);(65,60);(65,40);(65,40)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.4"
%	 points= "(65,40);(65,40);(85,40);(85,40)"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 stroke-width= "0.4"
%	 anchor-point= "(71.25,46.25)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\program
%</text>
%<multicurve fill-style= "none"
%	 stroke-width= "0.4"
%	 points= "(65,60);(65,60);(85,40);(85,40)"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 stroke-width= "0.4"
%	 anchor-point= "(50,50)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\EQLS
%</text>
%<multicurve fill-style= "none"
%	 stroke-width= "0.4"
%	 points= "(25,20);(25,20);(5,40);(5,40)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.4"
%	 points= "(5,40);(5,40);(35,40);(35,40)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(15,30);(15,30);(15,0);(15,0)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.4"
%	 points= "(25,20);(25,20);(35,20);(35,20)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.4"
%	 points= "(35,40);(35,40);(35,20);(35,20)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.4"
%	 points= "(30,20);(30,20);(30,0);(30,0)"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 stroke-width= "0.4"
%	 anchor-point= "(27.5,30)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\universal$
%</text>
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(0,55);(0,55);(0,0);(0,0)"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 stroke-width= "0.4"
%	 anchor-point= "(12.5,0)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\Progtype$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 stroke-width= "0.4"
%	 anchor-point= "(27.5,0)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\Progell$
%</text>
%<multicurve fill-style= "none"
%	 stroke-width= "0.4"
%	 points= "(130,50);(130,50);(130,0);(130,0)"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 stroke-width= "0.4"
%	 anchor-point= "(127.5,0)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\Progell$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 stroke-width= "0.4"
%	 anchor-point= "(112.5,0)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\Progtype$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 stroke-width= "0.4"
%	 anchor-point= "(97.5,0)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\Progtype$
%</text>
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(200,40);(200,40);(200,0);(200,0)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(212.5,40);(212.5,40);(212.5,0);(212.5,0)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.4"
%	 points= "(194.99,40);(194.99,40);(174.99,60);(174.99,60)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.4"
%	 points= "(210,70);(210,70);(240,70);(240,70)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.4"
%	 points= "(230,50);(230,50);(240,50);(240,50)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.4"
%	 points= "(240,70);(240,70);(240,50);(240,50)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.4"
%	 points= "(235,100);(235,100);(235,70);(235,70)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(185,50);(185,50);(175,40);(175,40)"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 stroke-width= "0.4"
%	 anchor-point= "(237.5,100)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\Progn$
%</text>
%<multicurve fill-style= "none"
%	 stroke-width= "0.4"
%	 points= "(165,50);(165,50);(165,30);(165,30)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.4"
%	 points= "(165,30);(165,30);(185,30);(185,30)"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 stroke-width= "0.4"
%	 anchor-point= "(171.25,36.25)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\program
%</text>
%<multicurve fill-style= "none"
%	 stroke-width= "0.4"
%	 points= "(165,50);(165,50);(185,30);(185,30)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.4"
%	 points= "(235,50);(235,50);(235,0);(235,0)"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 stroke-width= "0.4"
%	 anchor-point= "(232.5,0)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\Progell$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 stroke-width= "0.4"
%	 anchor-point= "(210,0)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\Progtype$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 stroke-width= "0.4"
%	 anchor-point= "(197.5,0)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\Progtype$
%</text>
%<multicurve fill-style= "none"
%	 stroke-width= "0.4"
%	 points= "(230,50);(230,50);(210,70);(210,70)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.4"
%	 points= "(195,40);(195,40);(220,40);(220,40)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.4"
%	 points= "(220,40);(220,40);(200,60);(200,60)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.4"
%	 points= "(175,60);(175,60);(200,60);(200,60)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(220,60);(220,60);(210,50);(210,50)"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 stroke-width= "0.4"
%	 anchor-point= "(232.5,60)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\universal$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 stroke-width= "0.4"
%	 anchor-point= "(197.5,50)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\partial$
%</text>
%<multicurve fill-style= "none"
%	 stroke-width= "0.4"
%	 points= "(160,65);(160,65);(160,25);(160,25)"
%	 stroke-color= "#ff0033"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.4"
%	 points= "(160,25);(160,25);(230,25);(230,25)"
%	 stroke-color= "#ff0033"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.4"
%	 points= "(160,65);(160,65);(205,65);(205,65)"
%	 stroke-color= "#ff0033"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.4"
%	 points= "(205,65);(205,65);(230,40);(230,40)"
%	 stroke-color= "#ff0033"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.4"
%	 points= "(230,25);(230,25);(230,40);(230,40)"
%	 stroke-color= "#ff0033"
%	 />
%<text text-vert-align= "bottom"
%	 fill-style= "none"
%	 stroke-width= "0.4"
%	 anchor-point= "(227.5,28.75)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\seqq$
%</text>
%<ellipse p3= "(73.12,48.12)"
%	 p2= "(73.12,51.88)"
%	 fill-style= "solid"
%	 p1= "(76.88,51.88)"
%	 stroke-width= "0.4"
%	 closure= "open"
%	 angle-end= "360"
%	 angle-start= "0"
%	 />
%<ellipse p3= "(173.12,38.12)"
%	 p2= "(173.12,41.88)"
%	 fill-style= "solid"
%	 p1= "(176.88,41.88)"
%	 stroke-width= "0.4"
%	 closure= "open"
%	 angle-end= "360"
%	 angle-start= "0"
%	 />
%<ellipse p3= "(208.12,48.12)"
%	 p2= "(208.12,51.88)"
%	 fill-style= "solid"
%	 p1= "(211.88,51.88)"
%	 stroke-width= "0.4"
%	 closure= "open"
%	 angle-end= "360"
%	 angle-start= "0"
%	 />
%</jpic>
%%End JPIC-XML
%PSTricks content-type (pstricks.sty package needed)
%Add \usepackage{pstricks} in the preamble of your LaTeX file
%You can rescale the whole picture (to 80% for instance) by using the command \def\JPicScale{0.8}
\ifx\JPicScale\undefined\def\JPicScale{1}\fi
\psset{unit=\JPicScale mm}
\psset{linewidth=0.3,dotsep=1,hatchwidth=0.3,hatchsep=1.5,shadowsize=1,dimen=middle}
\psset{dotsize=0.7 2.5,dotscale=1 1,fillcolor=black}
\psset{arrowsize=1 2,arrowlength=1,arrowinset=0.25,tbarsize=0.7 5,bracketlength=0.15,rbracketlength=0.15}
\begin{pspicture}(0,0)(240,100)
\psline[linewidth=0.75](100,50)(100,0)
\psline[linewidth=0.75](115,50)(115,0)
\psline[linewidth=0.4](94.99,50)(74.99,70)
\psline[linewidth=0.4](74.99,70)(135,70)
\psline[linewidth=0.4](94.99,50)(135,50)
\rput(150,50){\EQLS}
\psline[linewidth=0.4](135,70)(135,50)
\psline[linewidth=0.4](130,100)(130,70)
\psline[linewidth=0.75](85,60)(75,50)
\psline[linewidth=0.4](25,60)(5,80)
\psline[linewidth=0.4](5,80)(35,80)
\psline[linewidth=0.75](15,70)(0,55)
\psline[linewidth=0.4](25,60)(35,60)
\psline[linewidth=0.4](35,80)(35,60)
\psline[linewidth=0.4](30,100)(30,80)
\rput(-2.5,0){$\Progtype$}
\psline[linewidth=0.4](30,60)(30,40)
\rput(27.5,70){$\universal$}
\rput(132.5,100){$\Progn$}
\rput(32.5,100){$\Progn$}
\rput[r](27.5,50){$\Progm$}
\rput(115,60){$\universalmkn$}
\psline[linewidth=0.4](65,60)(65,40)
\psline[linewidth=0.4](65,40)(85,40)
\rput(71.25,46.25){\program}
\psline[linewidth=0.4](65,60)(85,40)
\rput(50,50){\EQLS}
\psline[linewidth=0.4](25,20)(5,40)
\psline[linewidth=0.4](5,40)(35,40)
\psline[linewidth=0.75](15,30)(15,0)
\psline[linewidth=0.4](25,20)(35,20)
\psline[linewidth=0.4](35,40)(35,20)
\psline[linewidth=0.4](30,20)(30,0)
\rput(27.5,30){$\universal$}
\psline[linewidth=0.75](0,55)(0,0)
\rput(12.5,0){$\Progtype$}
\rput(27.5,0){$\Progell$}
\psline[linewidth=0.4](130,50)(130,0)
\rput(127.5,0){$\Progell$}
\rput(112.5,0){$\Progtype$}
\rput(97.5,0){$\Progtype$}
\psline[linewidth=0.75](200,40)(200,0)
\psline[linewidth=0.75](212.5,40)(212.5,0)
\psline[linewidth=0.4](194.99,40)(174.99,60)
\psline[linewidth=0.4](210,70)(240,70)
\psline[linewidth=0.4](230,50)(240,50)
\psline[linewidth=0.4](240,70)(240,50)
\psline[linewidth=0.4](235,100)(235,70)
\psline[linewidth=0.75](185,50)(175,40)
\rput(237.5,100){$\Progn$}
\psline[linewidth=0.4](165,50)(165,30)
\psline[linewidth=0.4](165,30)(185,30)
\rput(171.25,36.25){\program}
\psline[linewidth=0.4](165,50)(185,30)
\psline[linewidth=0.4](235,50)(235,0)
\rput(232.5,0){$\Progell$}
\rput(210,0){$\Progtype$}
\rput(197.5,0){$\Progtype$}
\psline[linewidth=0.4](230,50)(210,70)
\psline[linewidth=0.4](195,40)(220,40)
\psline[linewidth=0.4](220,40)(200,60)
\psline[linewidth=0.4](175,60)(200,60)
\psline[linewidth=0.75](220,60)(210,50)
\rput(232.5,60){$\universal$}
\rput(197.5,50){$\partial$}
\newrgbcolor{userLineColour}{1 0 0.2}
\psline[linewidth=0.4,linecolor=userLineColour](160,65)(160,25)
\newrgbcolor{userLineColour}{1 0 0.2}
\psline[linewidth=0.4,linecolor=userLineColour](160,25)(230,25)
\newrgbcolor{userLineColour}{1 0 0.2}
\psline[linewidth=0.4,linecolor=userLineColour](160,65)(205,65)
\newrgbcolor{userLineColour}{1 0 0.2}
\psline[linewidth=0.4,linecolor=userLineColour](205,65)(230,40)
\newrgbcolor{userLineColour}{1 0 0.2}
\psline[linewidth=0.4,linecolor=userLineColour](230,25)(230,40)
\rput[br](227.5,28.75){$\seqq$}
\rput{0}(75,50){\psellipse[linewidth=0.4,fillstyle=solid](0,0)(1.88,1.88)}
\rput{0}(175,40){\psellipse[linewidth=0.4,fillstyle=solid](0,0)(1.88,1.88)}
\rput{0}(210,50){\psellipse[linewidth=0.4,fillstyle=solid](0,0)(1.88,1.88)}
\end{pspicture}


==> PIC/seq-par-33.tex <==
%%Created by jPicEdt 1.4.1_03: mixed JPIC-XML/LaTeX format
%%Mon Dec 05 22:13:40 GMT-10:00 2022
%%Begin JPIC-XML
%<?xml version="1.0" standalone="yes"?>
%<jpic x-min="15" x-max="305" y-min="0" y-max="70" auto-bounding="true">
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(145,40);(145,40);(145,0);(145,0)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(160,40);(160,40);(160,0);(160,0)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.4"
%	 points= "(139.99,40);(139.99,40);(119.99,60);(119.99,60)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.4"
%	 points= "(119.99,60);(119.99,60);(195,60);(195,60)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.4"
%	 points= "(139.99,40);(139.99,40);(195,40);(195,40)"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 stroke-width= "0.4"
%	 anchor-point= "(210,45)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\EQLS
%</text>
%<multicurve fill-style= "none"
%	 stroke-width= "0.4"
%	 points= "(195,60);(195,60);(195,40);(195,40)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.4"
%	 points= "(175,70);(175,70);(175,60);(175,60)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(130,50);(130,50);(130,40);(130,40)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.4"
%	 points= "(75,40);(75,40);(55,60);(55,60)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.4"
%	 points= "(55,60);(55,60);(90,60);(90,60)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(65,50);(65,50);(65,30);(65,30)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.4"
%	 points= "(75,40);(75,40);(90,40);(90,40)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.4"
%	 points= "(90,60);(90,60);(90,40);(90,40)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.4"
%	 points= "(85,70);(85,70);(85,60);(85,60)"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 stroke-width= "0.4"
%	 anchor-point= "(42.5,0)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\Progtype$
%</text>
%<multicurve fill-style= "none"
%	 stroke-width= "0.4"
%	 points= "(85,40);(85,40);(85,0);(85,0)"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 stroke-width= "0.4"
%	 anchor-point= "(77.5,50)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\universal$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 stroke-width= "0.4"
%	 anchor-point= "(177.5,70)"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\Progn$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 stroke-width= "0.4"
%	 anchor-point= "(47.5,70)"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\Progn$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 stroke-width= "0.4"
%	 anchor-point= "(82.5,0)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\Progm$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 stroke-width= "0.4"
%	 anchor-point= "(165,50)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\universalmkn$
%</text>
%<multicurve fill-style= "none"
%	 stroke-width= "0.4"
%	 points= "(120,50);(120,50);(120,30);(120,30)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.4"
%	 points= "(120,30);(120,30);(140,30);(140,30)"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 stroke-width= "0.4"
%	 anchor-point= "(126.25,36.25)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\program
%</text>
%<multicurve fill-style= "none"
%	 stroke-width= "0.4"
%	 points= "(120,50);(120,50);(140,30);(140,30)"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 stroke-width= "0.4"
%	 anchor-point= "(105,45)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\EQLS
%</text>
%<multicurve fill-style= "none"
%	 stroke-width= "0.4"
%	 points= "(35,40);(35,40);(15,60);(15,60)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.4"
%	 points= "(15,60);(15,60);(50,60);(50,60)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(25,50);(25,50);(25,0);(25,0)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.4"
%	 points= "(35,40);(35,40);(50,40);(50,40)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.4"
%	 points= "(50,60);(50,60);(50,40);(50,40)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.4"
%	 points= "(45,40);(45,40);(45,30);(45,30)"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 stroke-width= "0.4"
%	 anchor-point= "(37.5,50)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\universal$
%</text>
%<multicurve fill-style= "none"
%	 stroke-width= "0.4"
%	 points= "(65,10);(65,10);(45,30);(45,30)"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 stroke-width= "0.4"
%	 anchor-point= "(22.5,0)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\Progtype$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 stroke-width= "0.4"
%	 anchor-point= "(62.5,0)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\Progell$
%</text>
%<multicurve fill-style= "none"
%	 stroke-width= "0.4"
%	 points= "(175,40);(175,40);(175,0);(175,0)"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 stroke-width= "0.4"
%	 anchor-point= "(175,0)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\Progell$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 stroke-width= "0.4"
%	 anchor-point= "(157.5,0)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\Progtype$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 stroke-width= "0.4"
%	 anchor-point= "(142.5,0)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\Progtype$
%</text>
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(250,30);(250,30);(250,0);(250,0)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(265,30);(265,30);(265,0);(265,0)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.4"
%	 points= "(244.99,30);(244.99,30);(224.99,50);(224.99,50)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.4"
%	 points= "(260,60);(260,60);(305,60);(305,60)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.4"
%	 points= "(280,40);(280,40);(305,40);(305,40)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.4"
%	 points= "(305,60);(305,60);(305,40);(305,40)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.4"
%	 points= "(285,70);(285,70);(285,60);(285,60)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(235,40);(235,40);(235,30);(235,30)"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 stroke-width= "0.4"
%	 anchor-point= "(287.5,70)"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\Progn$
%</text>
%<multicurve fill-style= "none"
%	 stroke-width= "0.4"
%	 points= "(225,40);(225,40);(225,20);(225,20)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.4"
%	 points= "(225,20);(225,20);(245,20);(245,20)"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 stroke-width= "0.4"
%	 anchor-point= "(231.25,26.25)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\program
%</text>
%<multicurve fill-style= "none"
%	 stroke-width= "0.4"
%	 points= "(225,40);(225,40);(245,20);(245,20)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.4"
%	 points= "(285,40);(285,40);(285,0);(285,0)"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 stroke-width= "0.4"
%	 anchor-point= "(282.5,0)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\Progell$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 stroke-width= "0.4"
%	 anchor-point= "(262.5,0)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\Progtype$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 stroke-width= "0.4"
%	 anchor-point= "(247.5,0)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\Progtype$
%</text>
%<multicurve fill-style= "none"
%	 stroke-width= "0.4"
%	 points= "(280,40);(280,40);(260,60);(260,60)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.4"
%	 points= "(245,30);(245,30);(270,30);(270,30)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.4"
%	 points= "(270,30);(270,30);(250,50);(250,50)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.4"
%	 points= "(225,50);(225,50);(250,50);(250,50)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(270,50);(270,50);(260,40);(260,40)"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 stroke-width= "0.4"
%	 anchor-point= "(292.5,50)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\universal$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 stroke-width= "0.4"
%	 anchor-point= "(247.5,40)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\partial$
%</text>
%<multicurve fill-style= "none"
%	 stroke-width= "0.4"
%	 points= "(220,55);(220,55);(220,15);(220,15)"
%	 stroke-color= "#ff6666"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.4"
%	 points= "(220,15);(220,15);(280,15);(280,15)"
%	 stroke-color= "#ff6666"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.4"
%	 points= "(220,55);(220,55);(255,55);(255,55)"
%	 stroke-color= "#ff6666"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.4"
%	 points= "(255,55);(255,55);(280,30);(280,30)"
%	 stroke-color= "#ff6666"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.4"
%	 points= "(280,15);(280,15);(280,30);(280,30)"
%	 stroke-color= "#ff6666"
%	 />
%<text text-vert-align= "bottom"
%	 fill-style= "none"
%	 stroke-width= "0.4"
%	 anchor-point= "(278.75,16.25)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\seqq$
%</text>
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(45,10);(45,10);(65,30);(65,30)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(45,10);(45,10);(45,0);(45,0)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.4"
%	 points= "(65,10);(65,10);(65,0);(65,0)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.4"
%	 points= "(45,70);(45,70);(45,60);(45,60)"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 stroke-width= "0.4"
%	 anchor-point= "(87.5,70)"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\Progp$
%</text>
%<multicurve fill-style= "none"
%	 stroke-width= "0.4"
%	 points= "(190,40);(190,40);(190,0);(190,0)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.4"
%	 points= "(190,70);(190,70);(190,60);(190,60)"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 stroke-width= "0.4"
%	 anchor-point= "(192.5,70)"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\Progp$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 stroke-width= "0.4"
%	 anchor-point= "(190,0)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\Progm$
%</text>
%<multicurve fill-style= "none"
%	 stroke-width= "0.4"
%	 points= "(300,40);(300,40);(300,0);(300,0)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.4"
%	 points= "(300,70);(300,70);(300,60);(300,60)"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 stroke-width= "0.4"
%	 anchor-point= "(297.5,0)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\Progm$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 stroke-width= "0.4"
%	 anchor-point= "(302.5,70)"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\Progp$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(130,40)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\Dottt
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(235,30)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\Dottt
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(260,40)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\Dottt
%</text>
%</jpic>
%%End JPIC-XML
%LaTeX-picture environment using emulated lines and arcs
%You can rescale the whole picture (to 80% for instance) by using the command \def\JPicScale{0.8}
\ifx\JPicScale\undefined\def\JPicScale{1}\fi
\unitlength \JPicScale mm
\begin{picture}(305,70)(0,0)
\linethickness{0.75mm}
\put(145,0){\line(0,1){40}}
\linethickness{0.75mm}
\put(160,0){\line(0,1){40}}
\linethickness{0.4mm}
\multiput(119.99,60)(0.12,-0.12){167}{\line(1,0){0.12}}
\linethickness{0.4mm}
\put(119.99,60){\line(1,0){75.01}}
\linethickness{0.4mm}
\put(139.99,40){\line(1,0){55.01}}
\put(210,45){\makebox(0,0)[cc]{\EQLS}}

\linethickness{0.4mm}
\put(195,40){\line(0,1){20}}
\linethickness{0.4mm}
\put(175,60){\line(0,1){10}}
\linethickness{0.75mm}
\put(130,40){\line(0,1){10}}
\linethickness{0.4mm}
\multiput(55,60)(0.12,-0.12){167}{\line(1,0){0.12}}
\linethickness{0.4mm}
\put(55,60){\line(1,0){35}}
\linethickness{0.75mm}
\put(65,30){\line(0,1){20}}
\linethickness{0.4mm}
\put(75,40){\line(1,0){15}}
\linethickness{0.4mm}
\put(90,40){\line(0,1){20}}
\linethickness{0.4mm}
\put(85,60){\line(0,1){10}}
\put(42.5,0){\makebox(0,0)[cr]{$\Progtype$}}

\linethickness{0.4mm}
\put(85,0){\line(0,1){40}}
\put(77.5,50){\makebox(0,0)[cc]{$\universal$}}

\put(177.5,70){\makebox(0,0)[cl]{$\Progn$}}

\put(47.5,70){\makebox(0,0)[cl]{$\Progn$}}

\put(82.5,0){\makebox(0,0)[cr]{$\Progm$}}

\put(165,50){\makebox(0,0)[cc]{$\universalmkn$}}

\linethickness{0.4mm}
\put(120,30){\line(0,1){20}}
\linethickness{0.4mm}
\put(120,30){\line(1,0){20}}
\put(126.25,36.25){\makebox(0,0)[cc]{\program}}

\linethickness{0.4mm}
\multiput(120,50)(0.12,-0.12){167}{\line(1,0){0.12}}
\put(105,45){\makebox(0,0)[cc]{\EQLS}}

\linethickness{0.4mm}
\multiput(15,60)(0.12,-0.12){167}{\line(1,0){0.12}}
\linethickness{0.4mm}
\put(15,60){\line(1,0){35}}
\linethickness{0.75mm}
\put(25,0){\line(0,1){50}}
\linethickness{0.4mm}
\put(35,40){\line(1,0){15}}
\linethickness{0.4mm}
\put(50,40){\line(0,1){20}}
\linethickness{0.4mm}
\put(45,30){\line(0,1){10}}
\put(37.5,50){\makebox(0,0)[cc]{$\universal$}}

\linethickness{0.4mm}
\multiput(45,30)(0.12,-0.12){167}{\line(1,0){0.12}}
\put(22.5,0){\makebox(0,0)[cr]{$\Progtype$}}

\put(62.5,0){\makebox(0,0)[cr]{$\Progell$}}

\linethickness{0.4mm}
\put(175,0){\line(0,1){40}}
\put(175,0){\makebox(0,0)[cr]{$\Progell$}}

\put(157.5,0){\makebox(0,0)[cr]{$\Progtype$}}

\put(142.5,0){\makebox(0,0)[cr]{$\Progtype$}}

\linethickness{0.75mm}
\put(250,0){\line(0,1){30}}
\linethickness{0.75mm}
\put(265,0){\line(0,1){30}}
\linethickness{0.4mm}
\multiput(224.99,50)(0.12,-0.12){167}{\line(1,0){0.12}}
\linethickness{0.4mm}
\put(260,60){\line(1,0){45}}
\linethickness{0.4mm}
\put(280,40){\line(1,0){25}}
\linethickness{0.4mm}
\put(305,40){\line(0,1){20}}
\linethickness{0.4mm}
\put(285,60){\line(0,1){10}}
\linethickness{0.75mm}
\put(235,30){\line(0,1){10}}
\put(287.5,70){\makebox(0,0)[cl]{$\Progn$}}

\linethickness{0.4mm}
\put(225,20){\line(0,1){20}}
\linethickness{0.4mm}
\put(225,20){\line(1,0){20}}
\put(231.25,26.25){\makebox(0,0)[cc]{\program}}

\linethickness{0.4mm}
\multiput(225,40)(0.12,-0.12){167}{\line(1,0){0.12}}
\linethickness{0.4mm}
\put(285,0){\line(0,1){40}}
\put(282.5,0){\makebox(0,0)[cr]{$\Progell$}}

\put(262.5,0){\makebox(0,0)[cr]{$\Progtype$}}

\put(247.5,0){\makebox(0,0)[cr]{$\Progtype$}}

\linethickness{0.4mm}
\multiput(260,60)(0.12,-0.12){167}{\line(1,0){0.12}}
\linethickness{0.4mm}
\put(245,30){\line(1,0){25}}
\linethickness{0.4mm}
\multiput(250,50)(0.12,-0.12){167}{\line(1,0){0.12}}
\linethickness{0.4mm}
\put(225,50){\line(1,0){25}}
\linethickness{0.75mm}
\multiput(260,40)(0.12,0.12){83}{\line(1,0){0.12}}
\put(292.5,50){\makebox(0,0)[cc]{$\universal$}}

\put(247.5,40){\makebox(0,0)[cc]{$\partial$}}

\linethickness{0.4mm}
\put(220,15){\line(0,1){40}}
\linethickness{0.4mm}
\put(220,15){\line(1,0){60}}
\linethickness{0.4mm}
\put(220,55){\line(1,0){35}}
\linethickness{0.4mm}
\multiput(255,55)(0.12,-0.12){208}{\line(1,0){0.12}}
\linethickness{0.4mm}
\put(280,15){\line(0,1){15}}
\put(278.75,16.25){\makebox(0,0)[br]{$\seqq$}}

\linethickness{0.75mm}
\multiput(45,10)(0.12,0.12){167}{\line(1,0){0.12}}
\linethickness{0.75mm}
\put(45,0){\line(0,1){10}}
\linethickness{0.4mm}
\put(65,0){\line(0,1){10}}
\linethickness{0.4mm}
\put(45,60){\line(0,1){10}}
\put(87.5,70){\makebox(0,0)[cl]{$\Progp$}}

\linethickness{0.4mm}
\put(190,0){\line(0,1){40}}
\linethickness{0.4mm}
\put(190,60){\line(0,1){10}}
\put(192.5,70){\makebox(0,0)[cl]{$\Progp$}}

\put(190,0){\makebox(0,0)[cr]{$\Progm$}}

\linethickness{0.4mm}
\put(300,0){\line(0,1){40}}
\linethickness{0.4mm}
\put(300,60){\line(0,1){10}}
\put(297.5,0){\makebox(0,0)[cr]{$\Progm$}}

\put(302.5,70){\makebox(0,0)[cl]{$\Progp$}}

\put(130,40){\makebox(0,0)[cc]{\Dottt}}

\put(235,30){\makebox(0,0)[cc]{\Dottt}}

\put(260,40){\makebox(0,0)[cc]{\Dottt}}

\end{picture}


==> PIC/seq-par.tex <==
%%Created by jPicEdt 1.4.1_03: mixed JPIC-XML/LaTeX format
%%Mon Dec 16 23:08:36 GMT-10:00 2019
%%Begin JPIC-XML
%<?xml version="1.0" standalone="yes"?>
%<jpic x-min="15" x-max="305" y-min="0" y-max="70" auto-bounding="true">
%<multicurve fill-style= "none"
%	 points= "(145,40);(145,40);(145,0);(145,0)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(160,40);(160,40);(160,0);(160,0)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(139.99,40);(139.99,40);(119.99,60);(119.99,60)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(119.99,60);(119.99,60);(195,60);(195,60)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(139.99,40);(139.99,40);(195,40);(195,40)"
%	 stroke-width= "0.75"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(210,45)"
%	 text-frame= "noframe"
%	 stroke-width= "0.75"
%	 text-hor-align= "center-h"
%	 >
%\EQLS
%</text>
%<multicurve fill-style= "none"
%	 points= "(195,60);(195,60);(195,40);(195,40)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(175,70);(175,70);(175,60);(175,60)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(130,50);(130,50);(130,40);(130,40)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(75,40);(75,40);(55,60);(55,60)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(55,60);(55,60);(90,60);(90,60)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(65,50);(65,50);(65,30);(65,30)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(75,40);(75,40);(90,40);(90,40)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(90,60);(90,60);(90,40);(90,40)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(85,70);(85,70);(85,60);(85,60)"
%	 stroke-width= "0.75"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(42.5,0)"
%	 text-frame= "noframe"
%	 stroke-width= "0.75"
%	 text-hor-align= "right"
%	 >
%$\Progtype$
%</text>
%<multicurve fill-style= "none"
%	 points= "(85,40);(85,40);(85,0);(85,0)"
%	 stroke-width= "0.75"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(77.5,50)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\universal$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(177.5,70)"
%	 text-frame= "noframe"
%	 stroke-width= "0.8"
%	 text-hor-align= "left"
%	 >
%$\Progn$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(47.5,70)"
%	 text-frame= "noframe"
%	 stroke-width= "0.8"
%	 text-hor-align= "left"
%	 >
%$\Progn$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(82.5,0)"
%	 text-frame= "noframe"
%	 stroke-width= "0.8"
%	 text-hor-align= "right"
%	 >
%$\Progm$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(165,50)"
%	 text-frame= "noframe"
%	 stroke-width= "0.8"
%	 text-hor-align= "center-h"
%	 >
%$\universalmkn$
%</text>
%<multicurve fill-style= "none"
%	 points= "(120,50);(120,50);(120,30);(120,30)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(120,30);(120,30);(140,30);(140,30)"
%	 stroke-width= "0.75"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(126.25,36.25)"
%	 text-frame= "noframe"
%	 stroke-width= "0.75"
%	 text-hor-align= "center-h"
%	 >
%\program
%</text>
%<multicurve fill-style= "none"
%	 points= "(120,50);(120,50);(140,30);(140,30)"
%	 stroke-width= "0.75"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(105,45)"
%	 text-frame= "noframe"
%	 stroke-width= "0.75"
%	 text-hor-align= "center-h"
%	 >
%\EQLS
%</text>
%<multicurve fill-style= "none"
%	 points= "(35,40);(35,40);(15,60);(15,60)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(15,60);(15,60);(50,60);(50,60)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(25,50);(25,50);(25,0);(25,0)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(35,40);(35,40);(50,40);(50,40)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(50,60);(50,60);(50,40);(50,40)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(45,40);(45,40);(45,30);(45,30)"
%	 stroke-width= "0.75"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(37.5,50)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\universal$
%</text>
%<multicurve fill-style= "none"
%	 points= "(65,10);(65,10);(45,30);(45,30)"
%	 stroke-width= "0.75"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(22.5,0)"
%	 text-frame= "noframe"
%	 stroke-width= "0.75"
%	 text-hor-align= "right"
%	 >
%$\Progtype$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(62.5,0)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\Progell$
%</text>
%<multicurve fill-style= "none"
%	 points= "(175,40);(175,40);(175,0);(175,0)"
%	 stroke-width= "0.75"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(175,0)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\Progell$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(157.5,0)"
%	 text-frame= "noframe"
%	 stroke-width= "0.75"
%	 text-hor-align= "right"
%	 >
%$\Progtype$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(142.5,0)"
%	 text-frame= "noframe"
%	 stroke-width= "0.75"
%	 text-hor-align= "right"
%	 >
%$\Progtype$
%</text>
%<multicurve fill-style= "none"
%	 points= "(250,30);(250,30);(250,0);(250,0)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(265,30);(265,30);(265,0);(265,0)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(244.99,30);(244.99,30);(224.99,50);(224.99,50)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(260,60);(260,60);(305,60);(305,60)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(280,40);(280,40);(305,40);(305,40)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(305,60);(305,60);(305,40);(305,40)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(285,70);(285,70);(285,60);(285,60)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(235,40);(235,40);(235,30);(235,30)"
%	 stroke-width= "0.75"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(287.5,70)"
%	 text-frame= "noframe"
%	 stroke-width= "0.8"
%	 text-hor-align= "left"
%	 >
%$\Progn$
%</text>
%<multicurve fill-style= "none"
%	 points= "(225,40);(225,40);(225,20);(225,20)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(225,20);(225,20);(245,20);(245,20)"
%	 stroke-width= "0.75"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(231.25,26.25)"
%	 text-frame= "noframe"
%	 stroke-width= "0.75"
%	 text-hor-align= "center-h"
%	 >
%\program
%</text>
%<multicurve fill-style= "none"
%	 points= "(225,40);(225,40);(245,20);(245,20)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(285,40);(285,40);(285,0);(285,0)"
%	 stroke-width= "0.75"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(282.5,0)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\Progell$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(262.5,0)"
%	 text-frame= "noframe"
%	 stroke-width= "0.75"
%	 text-hor-align= "right"
%	 >
%$\Progtype$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(247.5,0)"
%	 text-frame= "noframe"
%	 stroke-width= "0.75"
%	 text-hor-align= "right"
%	 >
%$\Progtype$
%</text>
%<multicurve fill-style= "none"
%	 points= "(280,40);(280,40);(260,60);(260,60)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(245,30);(245,30);(270,30);(270,30)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(270,30);(270,30);(250,50);(250,50)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(225,50);(225,50);(250,50);(250,50)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(270,50);(270,50);(260,40);(260,40)"
%	 stroke-width= "0.75"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(292.5,50)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\universal$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(247.5,40)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\partial$
%</text>
%<multicurve fill-style= "none"
%	 points= "(220,55);(220,55);(220,15);(220,15)"
%	 stroke-color= "#ff6666"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(220,15);(220,15);(280,15);(280,15)"
%	 stroke-color= "#ff6666"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(220,55);(220,55);(255,55);(255,55)"
%	 stroke-color= "#ff6666"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(255,55);(255,55);(280,30);(280,30)"
%	 stroke-color= "#ff6666"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(280,15);(280,15);(280,30);(280,30)"
%	 stroke-color= "#ff6666"
%	 stroke-width= "0.75"
%	 />
%<text text-vert-align= "bottom"
%	 fill-style= "none"
%	 anchor-point= "(278.75,16.25)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\seqq$
%</text>
%<multicurve fill-style= "none"
%	 stroke-overstrike-width= "1.05"
%	 points= "(45,10);(45,10);(65,30);(65,30)"
%	 stroke-overstrike= "true"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(45,10);(45,10);(45,0);(45,0)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(65,10);(65,10);(65,0);(65,0)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(45,70);(45,70);(45,60);(45,60)"
%	 stroke-width= "0.75"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(87.5,70)"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\Progp$
%</text>
%<multicurve fill-style= "none"
%	 points= "(190,40);(190,40);(190,0);(190,0)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(190,70);(190,70);(190,60);(190,60)"
%	 stroke-width= "0.75"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(192.5,70)"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\Progp$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(190,0)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\Progm$
%</text>
%<multicurve fill-style= "none"
%	 points= "(300,40);(300,40);(300,0);(300,0)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(300,70);(300,70);(300,60);(300,60)"
%	 stroke-width= "0.75"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(297.5,0)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\Progm$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(302.5,70)"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\Progp$
%</text>
%</jpic>
%%End JPIC-XML
%PSTricks content-type (pstricks.sty package needed)
%Add \usepackage{pstricks} in the preamble of your LaTeX file
%You can rescale the whole picture (to 80% for instance) by using the command \def\JPicScale{0.8}
\ifx\JPicScale\undefined\def\JPicScale{1}\fi
\psset{unit=\JPicScale mm}
\psset{linewidth=0.3,dotsep=1,hatchwidth=0.3,hatchsep=1.5,shadowsize=1,dimen=middle}
\psset{dotsize=0.7 2.5,dotscale=1 1,fillcolor=black}
\psset{arrowsize=1 2,arrowlength=1,arrowinset=0.25,tbarsize=0.7 5,bracketlength=0.15,rbracketlength=0.15}
\begin{pspicture}(0,0)(305,70)
\psline[linewidth=0.75](145,40)(145,0)
\psline[linewidth=0.75](160,40)(160,0)
\psline[linewidth=0.75](139.99,40)(119.99,60)
\psline[linewidth=0.75](119.99,60)(195,60)
\psline[linewidth=0.75](139.99,40)(195,40)
\rput(210,45){\EQLS}
\psline[linewidth=0.75](195,60)(195,40)
\psline[linewidth=0.75](175,70)(175,60)
\psline[linewidth=0.75](130,50)(130,40)
\psline[linewidth=0.75](75,40)(55,60)
\psline[linewidth=0.75](55,60)(90,60)
\psline[linewidth=0.75](65,50)(65,30)
\psline[linewidth=0.75](75,40)(90,40)
\psline[linewidth=0.75](90,60)(90,40)
\psline[linewidth=0.75](85,70)(85,60)
\rput[r](42.5,0){$\Progtype$}
\psline[linewidth=0.75](85,40)(85,0)
\rput(77.5,50){$\universal$}
\rput[l](177.5,70){$\Progn$}
\rput[l](47.5,70){$\Progn$}
\rput[r](82.5,0){$\Progm$}
\rput(165,50){$\universalmkn$}
\psline[linewidth=0.75](120,50)(120,30)
\psline[linewidth=0.75](120,30)(140,30)
\rput(126.25,36.25){\program}
\psline[linewidth=0.75](120,50)(140,30)
\rput(105,45){\EQLS}
\psline[linewidth=0.75](35,40)(15,60)
\psline[linewidth=0.75](15,60)(50,60)
\psline[linewidth=0.75](25,50)(25,0)
\psline[linewidth=0.75](35,40)(50,40)
\psline[linewidth=0.75](50,60)(50,40)
\psline[linewidth=0.75](45,40)(45,30)
\rput(37.5,50){$\universal$}
\psline[linewidth=0.75](65,10)(45,30)
\rput[r](22.5,0){$\Progtype$}
\rput[r](62.5,0){$\Progell$}
\psline[linewidth=0.75](175,40)(175,0)
\rput[r](175,0){$\Progell$}
\rput[r](157.5,0){$\Progtype$}
\rput[r](142.5,0){$\Progtype$}
\psline[linewidth=0.75](250,30)(250,0)
\psline[linewidth=0.75](265,30)(265,0)
\psline[linewidth=0.75](244.99,30)(224.99,50)
\psline[linewidth=0.75](260,60)(305,60)
\psline[linewidth=0.75](280,40)(305,40)
\psline[linewidth=0.75](305,60)(305,40)
\psline[linewidth=0.75](285,70)(285,60)
\psline[linewidth=0.75](235,40)(235,30)
\rput[l](287.5,70){$\Progn$}
\psline[linewidth=0.75](225,40)(225,20)
\psline[linewidth=0.75](225,20)(245,20)
\rput(231.25,26.25){\program}
\psline[linewidth=0.75](225,40)(245,20)
\psline[linewidth=0.75](285,40)(285,0)
\rput[r](282.5,0){$\Progell$}
\rput[r](262.5,0){$\Progtype$}
\rput[r](247.5,0){$\Progtype$}
\psline[linewidth=0.75](280,40)(260,60)
\psline[linewidth=0.75](245,30)(270,30)
\psline[linewidth=0.75](270,30)(250,50)
\psline[linewidth=0.75](225,50)(250,50)
\psline[linewidth=0.75](270,50)(260,40)
\rput(292.5,50){$\universal$}
\rput(247.5,40){$\partial$}
\newrgbcolor{userLineColour}{1 0.4 0.4}
\psline[linewidth=0.75,linecolor=userLineColour](220,55)(220,15)
\newrgbcolor{userLineColour}{1 0.4 0.4}
\psline[linewidth=0.75,linecolor=userLineColour](220,15)(280,15)
\newrgbcolor{userLineColour}{1 0.4 0.4}
\psline[linewidth=0.75,linecolor=userLineColour](220,55)(255,55)
\newrgbcolor{userLineColour}{1 0.4 0.4}
\psline[linewidth=0.75,linecolor=userLineColour](255,55)(280,30)
\newrgbcolor{userLineColour}{1 0.4 0.4}
\psline[linewidth=0.75,linecolor=userLineColour](280,15)(280,30)
\rput[br](278.75,16.25){$\seqq$}
\psline[linewidth=0.75,border=1.05](45,10)(65,30)
\psline[linewidth=0.75](45,10)(45,0)
\psline[linewidth=0.75](65,10)(65,0)
\psline[linewidth=0.75](45,70)(45,60)
\rput[l](87.5,70){$\Progp$}
\psline[linewidth=0.75](190,40)(190,0)
\psline[linewidth=0.75](190,70)(190,60)
\rput[l](192.5,70){$\Progp$}
\rput[r](190,0){$\Progm$}
\psline[linewidth=0.75](300,40)(300,0)
\psline[linewidth=0.75](300,70)(300,60)
\rput[r](297.5,0){$\Progm$}
\rput[l](302.5,70){$\Progp$}
\end{pspicture}


==> PIC/seq.tex <==
%%Created by jPicEdt 1.4.1_03: mixed JPIC-XML/LaTeX format
%%Wed Jul 24 18:28:01 GMT-10:00 2019
%%Begin JPIC-XML
%<?xml version="1.0" standalone="yes"?>
%<jpic x-min="0" x-max="80" y-min="-55" y-max="55" auto-bounding="true">
%<multicurve fill-style= "none"
%	 points= "(0,-15);(0,-15);(30,-15);(30,-15)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(0,-15);(0,-15);(0,-35);(0,-35)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(30,-35);(30,-35);(30,-15);(30,-15)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(15,15);(15,15);(15,-15);(15,-15)"
%	 stroke-width= "0.75"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(12.5,0)"
%	 text-frame= "noframe"
%	 stroke-width= "0.75"
%	 text-hor-align= "right"
%	 >
%$\nameslang$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(12.5,-52.5)"
%	 text-frame= "noframe"
%	 stroke-width= "0.75"
%	 text-hor-align= "right"
%	 >
%$\inputt$
%</text>
%<multicurve fill-style= "none"
%	 points= "(0,-35);(0,-35);(30,-35);(30,-35)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(15,-35);(15,-35);(15,-55);(15,-55)"
%	 stroke-width= "0.75"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(15,-25)"
%	 text-frame= "noframe"
%	 stroke-width= "0.75"
%	 text-hor-align= "center-h"
%	 >
%\machine
%</text>
%<multicurve fill-style= "none"
%	 points= "(0,35);(0,35);(30,35);(30,35)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(0,35);(0,35);(0,15);(0,15)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(30,15);(30,15);(30,35);(30,35)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(15,55);(15,55);(15,35);(15,35)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(0,15);(0,15);(30,15);(30,15)"
%	 stroke-width= "0.75"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(15,25)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\gee
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(17.5,52.5)"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%\outpt
%</text>
%<multicurve fill-style= "none"
%	 points= "(50,-15);(50,-15);(80,-15);(80,-15)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(50,-15);(50,-15);(50,-35);(50,-35)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(80,-35);(80,-35);(80,-15);(80,-15)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(65,55);(65,55);(65,-15);(65,-15)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(50,-35);(50,-35);(80,-35);(80,-35)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(65,-35);(65,-35);(65,-55);(65,-55)"
%	 stroke-width= "0.75"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(62.5,-52.5)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\otherinputt$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(67.5,52.5)"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\otheroutpt$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(65,-25)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\hee$
%</text>
%</jpic>
%%End JPIC-XML
%PSTricks content-type (pstricks.sty package needed)
%Add \usepackage{pstricks} in the preamble of your LaTeX file
%You can rescale the whole picture (to 80% for instance) by using the command \def\JPicScale{0.8}
\ifx\JPicScale\undefined\def\JPicScale{1}\fi
\psset{unit=\JPicScale mm}
\psset{linewidth=0.3,dotsep=1,hatchwidth=0.3,hatchsep=1.5,shadowsize=1,dimen=middle}
\psset{dotsize=0.7 2.5,dotscale=1 1,fillcolor=black}
\psset{arrowsize=1 2,arrowlength=1,arrowinset=0.25,tbarsize=0.7 5,bracketlength=0.15,rbracketlength=0.15}
\begin{pspicture}(0,0)(80,55)
\psline[linewidth=0.75](0,-15)(30,-15)
\psline[linewidth=0.75](0,-15)(0,-35)
\psline[linewidth=0.75](30,-35)(30,-15)
\psline[linewidth=0.75](15,15)(15,-15)
\rput[r](12.5,0){$\nameslang$}
\rput[r](12.5,-52.5){$\inputt$}
\psline[linewidth=0.75](0,-35)(30,-35)
\psline[linewidth=0.75](15,-35)(15,-55)
\rput(15,-25){\machine}
\psline[linewidth=0.75](0,35)(30,35)
\psline[linewidth=0.75](0,35)(0,15)
\psline[linewidth=0.75](30,15)(30,35)
\psline[linewidth=0.75](15,55)(15,35)
\psline[linewidth=0.75](0,15)(30,15)
\rput(15,25){\gee}
\rput[l](17.5,52.5){\outpt}
\psline[linewidth=0.75](50,-15)(80,-15)
\psline[linewidth=0.75](50,-15)(50,-35)
\psline[linewidth=0.75](80,-35)(80,-15)
\psline[linewidth=0.75](65,55)(65,-15)
\psline[linewidth=0.75](50,-35)(80,-35)
\psline[linewidth=0.75](65,-35)(65,-55)
\rput[r](62.5,-52.5){$\otherinputt$}
\rput[l](67.5,52.5){$\otheroutpt$}
\rput(65,-25){$\hee$}
\end{pspicture}


==> PIC/seqcomp.tex <==
%%Created by jPicEdt 1.4.1_03: mixed JPIC-XML/LaTeX format
%%Wed Sep 28 22:42:11 HST 2016
%%Begin JPIC-XML
%<?xml version="1.0" standalone="yes"?>
%<jpic x-min="0" x-max="40" y-min="-49.38" y-max="51.25" auto-bounding="true">
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(0,35);(0,35);(40,35);(40,35)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(0,35);(0,35);(0,10);(0,10)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(40,10);(40,10);(40,35);(40,35)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(20,45);(20,45);(20,35);(20,35)"
%	 />
%<text stroke-width= "0.75"
%	 text-vert-align= "center-v"
%	 anchor-point= "(20,51.25)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\nameslang$
%</text>
%<text stroke-width= "0.75"
%	 text-vert-align= "center-v"
%	 anchor-point= "(21.88,0.62)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\inputt$
%</text>
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(0,10);(0,10);(40,10);(40,10)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(20,10);(20,10);(20,-10);(20,-10)"
%	 />
%<text stroke-width= "0.75"
%	 text-vert-align= "center-v"
%	 anchor-point= "(20,22.5)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\machine
%</text>
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(0,-10);(0,-10);(40,-10);(40,-10)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(0,-10);(0,-10);(0,-35);(0,-35)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(40,-35);(40,-35);(40,-10);(40,-10)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(0,-35);(0,-35);(40,-35);(40,-35)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(20,-35);(20,-35);(20,-44.38);(20,-44.38)"
%	 />
%<text text-vert-align= "center-v"
%	 anchor-point= "(20,-49.38)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\inputg$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(20,-22.5)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\otherfun
%</text>
%</jpic>
%%End JPIC-XML
%PSTricks content-type (pstricks.sty package needed)
%Add \usepackage{pstricks} in the preamble of your LaTeX file
%You can rescale the whole picture (to 80% for instance) by using the command \def\JPicScale{0.8}
\ifx\JPicScale\undefined\def\JPicScale{1}\fi
\psset{unit=\JPicScale mm}
\psset{linewidth=0.3,dotsep=1,hatchwidth=0.3,hatchsep=1.5,shadowsize=1,dimen=middle}
\psset{dotsize=0.7 2.5,dotscale=1 1,fillcolor=black}
\psset{arrowsize=1 2,arrowlength=1,arrowinset=0.25,tbarsize=0.7 5,bracketlength=0.15,rbracketlength=0.15}
\begin{pspicture}(0,0)(40,51.25)
\psline[linewidth=0.75](0,35)(40,35)
\psline[linewidth=0.75](0,35)(0,10)
\psline[linewidth=0.75](40,10)(40,35)
\psline[linewidth=0.75](20,45)(20,35)
\rput(20,51.25){$\nameslang$}
\rput[l](21.88,0.62){$\inputt$}
\psline[linewidth=0.75](0,10)(40,10)
\psline[linewidth=0.75](20,10)(20,-10)
\rput(20,22.5){\machine}
\psline[linewidth=0.75](0,-10)(40,-10)
\psline[linewidth=0.75](0,-10)(0,-35)
\psline[linewidth=0.75](40,-35)(40,-10)
\psline[linewidth=0.75](0,-35)(40,-35)
\psline[linewidth=0.75](20,-35)(20,-44.38)
\rput(20,-49.38){$\inputg$}
\rput(20,-22.5){\otherfun}
\end{pspicture}


==> PIC/simulation.tex <==
%%Created by jPicEdt 1.4.1_03: mixed JPIC-XML/LaTeX format
%%Mon May 23 11:51:46 GMT+01:00 2022
%%Begin JPIC-XML
%<?xml version="1.0" standalone="yes"?>
%<jpic x-min="1.88" x-max="66.25" y-min="-1.25" y-max="45.62" auto-bounding="true">
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 stroke-width= "0.15"
%	 anchor-point= "(54.38,21.88)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\ahh$
%</text>
%<multicurve fill-style= "none"
%	 stroke-width= "0.15"
%	 points= "(20.62,-1.25);(20.62,-1.25);(20.62,16.88);(20.62,16.88)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.15"
%	 points= "(8.12,-1.25);(8.12,-1.25);(8.12,16.88);(8.12,16.88)"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 stroke-width= "0.15"
%	 anchor-point= "(6.88,-0.62)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\xxh$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 stroke-width= "0.15"
%	 anchor-point= "(33.75,22.5)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\EQLS
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 stroke-width= "0.15"
%	 anchor-point= "(14.38,21.88)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\bhh$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 stroke-width= "0.15"
%	 anchor-point= "(19.38,-0.62)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\ah$
%</text>
%<multicurve fill-style= "none"
%	 stroke-width= "0.15"
%	 points= "(20,26.88);(20,26.88);(20,45.62);(20,45.62)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.15"
%	 points= "(8.12,26.88);(8.12,26.88);(8.12,33.75);(8.12,33.75)"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 stroke-width= "0.15"
%	 anchor-point= "(8.12,36.25)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\aah$
%</text>
%<multicurve fill-style= "none"
%	 stroke-width= "0.15"
%	 points= "(1.88,26.88);(1.88,26.88);(1.88,16.88);(1.88,16.88);(1.88,16.88);(26.25,16.88);
%	(26.25,16.88);(26.25,16.88);(26.25,26.88);(26.25,26.88);(26.25,26.88);(1.88,26.88);
%	(1.88,26.88);(1.88,26.88);(21.25,26.86);(21.25,26.86);(21.25,26.86);(1.88,26.88);
%	(1.88,26.88);(1.88,26.88);(1.88,26.88);(1.88,26.88)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.15"
%	 points= "(8.12,38.75);(8.12,38.75);(8.12,45.62);(8.12,45.62)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.15"
%	 points= "(60.62,-1.25);(60.62,-1.25);(60.62,16.88);(60.62,16.88)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.15"
%	 points= "(48.12,10);(48.12,10);(48.12,16.88);(48.12,16.88)"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 stroke-width= "0.15"
%	 anchor-point= "(46.88,-0.62)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\xxh$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 stroke-width= "0.15"
%	 anchor-point= "(59.38,-0.62)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\ah$
%</text>
%<multicurve fill-style= "none"
%	 stroke-width= "0.15"
%	 points= "(60,26.88);(60,26.88);(60,45.62);(60,45.62)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.15"
%	 points= "(41.88,26.88);(41.88,26.88);(41.88,16.88);(41.88,16.88);(41.88,16.88);(66.25,16.88);
%	(66.25,16.88);(66.25,16.88);(66.25,26.88);(66.25,26.88);(66.25,26.88);(41.88,26.88);
%	(41.88,26.88);(41.88,26.88);(61.25,26.86);(61.25,26.86);(61.25,26.86);(41.88,26.88);
%	(41.88,26.88);(41.88,26.88);(41.88,26.88);(41.88,26.88)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.15"
%	 points= "(48.12,26.88);(48.12,26.88);(48.12,45.62);(48.12,45.62)"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 stroke-width= "0.15"
%	 anchor-point= "(49.38,44.38)"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\ssbbh$
%</text>
%<parallelogram p3= "(13.12,33.75)"
%	 p2= "(13.12,38.75)"
%	 fill-style= "none"
%	 p1= "(3.12,38.75)"
%	 stroke-width= "0.15"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 stroke-width= "0.15"
%	 anchor-point= "(48.12,7.5)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\aah$
%</text>
%<parallelogram p3= "(53.12,5)"
%	 p2= "(53.12,10)"
%	 fill-style= "none"
%	 p1= "(43.12,10)"
%	 stroke-width= "0.15"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.15"
%	 points= "(48.12,-1.25);(48.12,-1.25);(48.12,5);(48.12,5)"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 stroke-width= "0.15"
%	 anchor-point= "(58.75,44.38)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\xxbbh$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 stroke-width= "0.15"
%	 anchor-point= "(10,44.38)"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\ssbbh$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 stroke-width= "0.15"
%	 anchor-point= "(19.38,44.38)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\xxbbh$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 stroke-width= "0.15"
%	 anchor-point= "(9.38,30)"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\xxh$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 stroke-width= "0.15"
%	 anchor-point= "(46.88,13.12)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\ssbbh$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 stroke-width= "0.15"
%	 anchor-point= "(48.12,10)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\Dott$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 stroke-width= "0.15"
%	 anchor-point= "(8.12,38.75)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\Dott$
%</text>
%</jpic>
%%End JPIC-XML
%PSTricks content-type (pstricks.sty package needed)
%Add \usepackage{pstricks} in the preamble of your LaTeX file
%You can rescale the whole picture (to 80% for instance) by using the command \def\JPicScale{0.8}
\ifx\JPicScale\undefined\def\JPicScale{1}\fi
\psset{unit=\JPicScale mm}
\psset{linewidth=0.3,dotsep=1,hatchwidth=0.3,hatchsep=1.5,shadowsize=1,dimen=middle}
\psset{dotsize=0.7 2.5,dotscale=1 1,fillcolor=black}
\psset{arrowsize=1 2,arrowlength=1,arrowinset=0.25,tbarsize=0.7 5,bracketlength=0.15,rbracketlength=0.15}
\begin{pspicture}(0,0)(66.25,45.62)
\rput(54.38,21.88){$\ahh$}
\psline[linewidth=0.15](20.62,-1.25)(20.62,16.88)
\psline[linewidth=0.15](8.12,-1.25)(8.12,16.88)
\rput[r](6.88,-0.62){$\xxh$}
\rput(33.75,22.5){\EQLS}
\rput(14.38,21.88){$\bhh$}
\rput[r](19.38,-0.62){$\ah$}
\psline[linewidth=0.15](20,26.88)(20,45.62)
\psline[linewidth=0.15](8.12,26.88)(8.12,33.75)
\rput(8.12,36.25){$\aah$}
\pscustom[linewidth=0.15]{\psline(1.88,26.88)(1.88,16.88)
\psline(1.88,16.88)(26.25,16.88)
\psline(26.25,16.88)(26.25,26.88)
\psline(26.25,26.88)(1.88,26.88)
\psline(1.88,26.88)(21.25,26.86)
\psline(21.25,26.86)(1.88,26.88)
\psbezier(1.88,26.88)(1.88,26.88)(1.88,26.88)
}
\psline[linewidth=0.15](8.12,38.75)(8.12,45.62)
\psline[linewidth=0.15](60.62,-1.25)(60.62,16.88)
\psline[linewidth=0.15](48.12,10)(48.12,16.88)
\rput[r](46.88,-0.62){$\xxh$}
\rput[r](59.38,-0.62){$\ah$}
\psline[linewidth=0.15](60,26.88)(60,45.62)
\pscustom[linewidth=0.15]{\psline(41.88,26.88)(41.88,16.88)
\psline(41.88,16.88)(66.25,16.88)
\psline(66.25,16.88)(66.25,26.88)
\psline(66.25,26.88)(41.88,26.88)
\psline(41.88,26.88)(61.25,26.86)
\psline(61.25,26.86)(41.88,26.88)
\psbezier(41.88,26.88)(41.88,26.88)(41.88,26.88)
}
\psline[linewidth=0.15](48.12,26.88)(48.12,45.62)
\rput[l](49.38,44.38){$\ssbbh$}
\pspolygon[linewidth=0.15](3.12,38.75)(13.12,38.75)(13.12,33.75)(3.12,33.75)
\rput(48.12,7.5){$\aah$}
\pspolygon[linewidth=0.15](43.12,10)(53.12,10)(53.12,5)(43.12,5)
\psline[linewidth=0.15](48.12,-1.25)(48.12,5)
\rput[r](58.75,44.38){$\xxbbh$}
\rput[l](10,44.38){$\ssbbh$}
\rput[r](19.38,44.38){$\xxbbh$}
\rput[l](9.38,30){$\xxh$}
\rput[r](46.88,13.12){$\ssbbh$}
\rput(48.12,10){$\Dott$}
\rput(8.12,38.75){$\Dott$}
\end{pspicture}


==> PIC/slicing-1.tex <==
%%Created by jPicEdt 1.4.1_03: mixed JPIC-XML/LaTeX format
%%Sun Nov 29 15:30:26 GMT-10:00 2020
%%Begin JPIC-XML
%<?xml version="1.0" standalone="yes"?>
%<jpic x-min="0" x-max="425" y-min="5" y-max="130" auto-bounding="true">
%<text fill-style= "none"
%	 stroke-width= "0.35"
%	 text-vert-align= "center-v"
%	 anchor-point= "(262.5,87.5)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\Progtype$
%</text>
%<text fill-style= "none"
%	 stroke-width= "0.35"
%	 text-vert-align= "center-v"
%	 anchor-point= "(247.5,77.5)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\partial$
%</text>
%<text fill-style= "none"
%	 stroke-width= "0.35"
%	 text-vert-align= "center-v"
%	 anchor-point= "(282.5,97.5)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\universal$
%</text>
%<text fill-style= "none"
%	 stroke-width= "0.35"
%	 text-vert-align= "center-v"
%	 anchor-point= "(280,130)"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\Progn$
%</text>
%<text fill-style= "none"
%	 stroke-width= "0.35"
%	 text-vert-align= "center-v"
%	 anchor-point= "(287.5,30)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\Progm$
%</text>
%<text fill-style= "none"
%	 stroke-width= "0.35"
%	 text-vert-align= "center-v"
%	 anchor-point= "(262.5,30)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\Progk$
%</text>
%<text fill-style= "none"
%	 stroke-width= "0.35"
%	 text-vert-align= "center-v"
%	 anchor-point= "(235,45)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\program
%</text>
%<text fill-style= "none"
%	 stroke-width= "0.35"
%	 text-vert-align= "center-v"
%	 anchor-point= "(237.5,62.5)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\Progtype$
%</text>
%<text fill-style= "none"
%	 stroke-width= "0.35"
%	 text-vert-align= "center-v"
%	 anchor-point= "(22.5,97.5)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\gee
%</text>
%<text fill-style= "none"
%	 stroke-width= "0.35"
%	 text-vert-align= "center-v"
%	 anchor-point= "(200,97.5)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\eqlsb$
%</text>
%<text fill-style= "none"
%	 stroke-width= "0.35"
%	 text-vert-align= "center-v"
%	 anchor-point= "(330,97.5)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\eqlsc$
%</text>
%<text fill-style= "none"
%	 stroke-width= "0.35"
%	 text-vert-align= "center-v"
%	 anchor-point= "(75,97.5)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\eqlsa$
%</text>
%<text fill-style= "none"
%	 stroke-width= "0.35"
%	 text-vert-align= "center-v"
%	 anchor-point= "(135,5)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\ux$
%</text>
%<text fill-style= "none"
%	 stroke-width= "0.35"
%	 text-vert-align= "center-v"
%	 anchor-point= "(265,5)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\sx$
%</text>
%<text fill-style= "none"
%	 stroke-width= "0.35"
%	 text-vert-align= "center-v"
%	 anchor-point= "(200,5)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\eqlsb$
%</text>
%<text fill-style= "none"
%	 stroke-width= "0.35"
%	 text-vert-align= "center-v"
%	 anchor-point= "(75,5)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\eqlsa$
%</text>
%<text fill-style= "none"
%	 stroke-width= "0.35"
%	 text-vert-align= "center-v"
%	 anchor-point= "(370,75)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\Gx$
%</text>
%<text fill-style= "none"
%	 stroke-width= "0.35"
%	 text-vert-align= "center-v"
%	 anchor-point= "(25,5)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\gx$
%</text>
%<text fill-style= "none"
%	 stroke-width= "0.35"
%	 text-vert-align= "center-v"
%	 anchor-point= "(330,5)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\eqlsc$
%</text>
%<text fill-style= "none"
%	 stroke-width= "0.35"
%	 text-vert-align= "center-v"
%	 anchor-point= "(390,5)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\tx$
%</text>
%<multicurve fill-style= "none"
%	 points= "(300,115);(300,115);(300,80);(300,80)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(300,80);(300,80);(280,80);(280,80)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(280,60);(280,60);(250,60);(250,60)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(250,40);(250,40);(230,40);(230,40)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(230,60);(230,60);(230,40);(230,40)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(230,60);(230,60);(250,40);(250,40)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(250,60);(250,60);(230,80);(230,80)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(230,80);(230,80);(230,95);(230,95)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(245,95);(245,95);(280,60);(280,60)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(280,80);(280,80);(245,115);(245,115)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(245,115);(245,115);(300,115);(300,115)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(240,70);(240,70);(240,50);(240,50)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(265,95);(265,95);(265,75);(265,75)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(265,60);(265,60);(265,30);(265,30)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(290,80);(290,80);(290,30);(290,30)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(277.5,130);(277.5,130);(277.5,115);(277.5,115)"
%	 />
%<text fill-style= "none"
%	 stroke-width= "0.35"
%	 text-vert-align= "center-v"
%	 anchor-point= "(387.5,87.5)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\Progtype$
%</text>
%<text fill-style= "none"
%	 stroke-width= "0.35"
%	 text-vert-align= "center-v"
%	 anchor-point= "(407.5,97.5)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\universal$
%</text>
%<text fill-style= "none"
%	 stroke-width= "0.35"
%	 text-vert-align= "center-v"
%	 anchor-point= "(405,130)"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\Progn$
%</text>
%<text fill-style= "none"
%	 stroke-width= "0.35"
%	 text-vert-align= "center-v"
%	 anchor-point= "(412.5,30)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\Progm$
%</text>
%<text fill-style= "none"
%	 stroke-width= "0.35"
%	 text-vert-align= "center-v"
%	 anchor-point= "(377.5,30)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\Progk$
%</text>
%<multicurve fill-style= "none"
%	 points= "(425,115);(425,115);(425,80);(425,80)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(425,80);(425,80);(405,80);(405,80)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(405,60);(405,60);(355,60);(355,60)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(355,60);(355,60);(355,95);(355,95)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(370,95);(370,95);(405,60);(405,60)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(405,80);(405,80);(370,115);(370,115)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(370,115);(370,115);(425,115);(425,115)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(390,95);(390,95);(390,75);(390,75)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(380,60);(380,60);(380,30);(380,30)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(415,80);(415,80);(415,30);(415,30)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(402.5,130);(402.5,130);(402.5,115);(402.5,115)"
%	 />
%<text fill-style= "none"
%	 stroke-width= "0.35"
%	 text-vert-align= "center-v"
%	 anchor-point= "(147.5,97.5)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\universal$
%</text>
%<text fill-style= "none"
%	 stroke-width= "0.35"
%	 text-vert-align= "center-v"
%	 anchor-point= "(150,130)"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\Progn$
%</text>
%<text fill-style= "none"
%	 stroke-width= "0.35"
%	 text-vert-align= "center-v"
%	 anchor-point= "(157.5,30)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\Progm$
%</text>
%<text fill-style= "none"
%	 stroke-width= "0.35"
%	 text-vert-align= "center-v"
%	 anchor-point= "(132.5,30)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\Progk$
%</text>
%<text fill-style= "none"
%	 stroke-width= "0.35"
%	 text-vert-align= "center-v"
%	 anchor-point= "(110,65)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\program
%</text>
%<text fill-style= "none"
%	 stroke-width= "0.35"
%	 text-vert-align= "center-v"
%	 anchor-point= "(112.5,82.5)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\Progtype$
%</text>
%<multicurve fill-style= "none"
%	 points= "(170,115);(170,115);(170,80);(170,80)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(170,80);(170,80);(125,80);(125,80)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(125,60);(125,60);(105,60);(105,60)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(105,80);(105,80);(105,60);(105,60)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(105,80);(105,80);(125,60);(125,60)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(125,80);(125,80);(105,100);(105,100)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(105,100);(105,100);(105,115);(105,115)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(105,115);(105,115);(170,115);(170,115)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(115,90);(115,90);(115,70);(115,70)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(135,80);(135,80);(135,30);(135,30)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(160,80);(160,80);(160,30);(160,30)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(147.5,130);(147.5,130);(147.5,115);(147.5,115)"
%	 />
%<text fill-style= "none"
%	 stroke-width= "0.35"
%	 text-vert-align= "center-v"
%	 anchor-point= "(25,130)"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\Progn$
%</text>
%<text fill-style= "none"
%	 stroke-width= "0.35"
%	 text-vert-align= "center-v"
%	 anchor-point= "(32.5,30)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\Progm$
%</text>
%<text fill-style= "none"
%	 stroke-width= "0.35"
%	 text-vert-align= "center-v"
%	 anchor-point= "(7.5,30)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\Progk$
%</text>
%<multicurve fill-style= "none"
%	 points= "(45,115);(45,115);(45,80);(45,80)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(45,80);(45,80);(0,80);(0,80)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(0,115);(0,115);(45,115);(45,115)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(10,80);(10,80);(10,30);(10,30)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(35,80);(35,80);(35,30);(35,30)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(22.5,130);(22.5,130);(22.5,115);(22.5,115)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(0,115);(0,115);(0,80);(0,80)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(245,95);(245,95);(230,95);(230,95)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(370,95);(370,95);(355,95);(355,95)"
%	 />
%</jpic>
%%End JPIC-XML
%LaTeX-picture environment using emulated lines and arcs
%You can rescale the whole picture (to 80% for instance) by using the command \def\JPicScale{0.8}
\ifx\JPicScale\undefined\def\JPicScale{1}\fi
\unitlength \JPicScale mm
\begin{picture}(425,130)(0,0)
\put(262.5,87.5){\makebox(0,0)[cr]{$\Progtype$}}

\put(247.5,77.5){\makebox(0,0)[cc]{$\partial$}}

\put(282.5,97.5){\makebox(0,0)[cc]{$\universal$}}

\put(280,130){\makebox(0,0)[cl]{$\Progn$}}

\put(287.5,30){\makebox(0,0)[cr]{$\Progm$}}

\put(262.5,30){\makebox(0,0)[cr]{$\Progk$}}

\put(235,45){\makebox(0,0)[cc]{\program}}

\put(237.5,62.5){\makebox(0,0)[cr]{$\Progtype$}}

\put(22.5,97.5){\makebox(0,0)[cc]{\gee}}

\put(200,97.5){\makebox(0,0)[cc]{$\eqlsb$}}

\put(330,97.5){\makebox(0,0)[cc]{$\eqlsc$}}

\put(75,97.5){\makebox(0,0)[cc]{$\eqlsa$}}

\put(135,5){\makebox(0,0)[cc]{$\ux$}}

\put(265,5){\makebox(0,0)[cc]{$\sx$}}

\put(200,5){\makebox(0,0)[cc]{$\eqlsb$}}

\put(75,5){\makebox(0,0)[cc]{$\eqlsa$}}

\put(370,75){\makebox(0,0)[cc]{$\Gx$}}

\put(25,5){\makebox(0,0)[cc]{$\gx$}}

\put(330,5){\makebox(0,0)[cc]{$\eqlsc$}}

\put(390,5){\makebox(0,0)[cc]{$\tx$}}

\linethickness{0.3mm}
\put(300,80){\line(0,1){35}}
\linethickness{0.3mm}
\put(280,80){\line(1,0){20}}
\linethickness{0.3mm}
\put(250,60){\line(1,0){30}}
\linethickness{0.3mm}
\put(230,40){\line(1,0){20}}
\linethickness{0.3mm}
\put(230,40){\line(0,1){20}}
\linethickness{0.3mm}
\multiput(230,60)(0.12,-0.12){167}{\line(1,0){0.12}}
\linethickness{0.3mm}
\multiput(230,80)(0.12,-0.12){167}{\line(1,0){0.12}}
\linethickness{0.3mm}
\put(230,80){\line(0,1){15}}
\linethickness{0.3mm}
\multiput(245,95)(0.12,-0.12){292}{\line(1,0){0.12}}
\linethickness{0.3mm}
\multiput(245,115)(0.12,-0.12){292}{\line(1,0){0.12}}
\linethickness{0.3mm}
\put(245,115){\line(1,0){55}}
\linethickness{0.3mm}
\put(240,50){\line(0,1){20}}
\linethickness{0.3mm}
\put(265,75){\line(0,1){20}}
\linethickness{0.3mm}
\put(265,30){\line(0,1){30}}
\linethickness{0.3mm}
\put(290,30){\line(0,1){50}}
\linethickness{0.3mm}
\put(277.5,115){\line(0,1){15}}
\put(387.5,87.5){\makebox(0,0)[cr]{$\Progtype$}}

\put(407.5,97.5){\makebox(0,0)[cc]{$\universal$}}

\put(405,130){\makebox(0,0)[cl]{$\Progn$}}

\put(412.5,30){\makebox(0,0)[cr]{$\Progm$}}

\put(377.5,30){\makebox(0,0)[cr]{$\Progk$}}

\linethickness{0.3mm}
\put(425,80){\line(0,1){35}}
\linethickness{0.3mm}
\put(405,80){\line(1,0){20}}
\linethickness{0.3mm}
\put(355,60){\line(1,0){50}}
\linethickness{0.3mm}
\put(355,60){\line(0,1){35}}
\linethickness{0.3mm}
\multiput(370,95)(0.12,-0.12){292}{\line(1,0){0.12}}
\linethickness{0.3mm}
\multiput(370,115)(0.12,-0.12){292}{\line(1,0){0.12}}
\linethickness{0.3mm}
\put(370,115){\line(1,0){55}}
\linethickness{0.3mm}
\put(390,75){\line(0,1){20}}
\linethickness{0.3mm}
\put(380,30){\line(0,1){30}}
\linethickness{0.3mm}
\put(415,30){\line(0,1){50}}
\linethickness{0.3mm}
\put(402.5,115){\line(0,1){15}}
\put(147.5,97.5){\makebox(0,0)[cc]{$\universal$}}

\put(150,130){\makebox(0,0)[cl]{$\Progn$}}

\put(157.5,30){\makebox(0,0)[cr]{$\Progm$}}

\put(132.5,30){\makebox(0,0)[cr]{$\Progk$}}

\put(110,65){\makebox(0,0)[cc]{\program}}

\put(112.5,82.5){\makebox(0,0)[cr]{$\Progtype$}}

\linethickness{0.3mm}
\put(170,80){\line(0,1){35}}
\linethickness{0.3mm}
\put(125,80){\line(1,0){45}}
\linethickness{0.3mm}
\put(105,60){\line(1,0){20}}
\linethickness{0.3mm}
\put(105,60){\line(0,1){20}}
\linethickness{0.3mm}
\multiput(105,80)(0.12,-0.12){167}{\line(1,0){0.12}}
\linethickness{0.3mm}
\multiput(105,100)(0.12,-0.12){167}{\line(1,0){0.12}}
\linethickness{0.3mm}
\put(105,100){\line(0,1){15}}
\linethickness{0.3mm}
\put(105,115){\line(1,0){65}}
\linethickness{0.3mm}
\put(115,70){\line(0,1){20}}
\linethickness{0.3mm}
\put(135,30){\line(0,1){50}}
\linethickness{0.3mm}
\put(160,30){\line(0,1){50}}
\linethickness{0.3mm}
\put(147.5,115){\line(0,1){15}}
\put(25,130){\makebox(0,0)[cl]{$\Progn$}}

\put(32.5,30){\makebox(0,0)[cr]{$\Progm$}}

\put(7.5,30){\makebox(0,0)[cr]{$\Progk$}}

\linethickness{0.3mm}
\put(45,80){\line(0,1){35}}
\linethickness{0.3mm}
\put(0,80){\line(1,0){45}}
\linethickness{0.3mm}
\put(0,115){\line(1,0){45}}
\linethickness{0.3mm}
\put(10,30){\line(0,1){50}}
\linethickness{0.3mm}
\put(35,30){\line(0,1){50}}
\linethickness{0.3mm}
\put(22.5,115){\line(0,1){15}}
\linethickness{0.3mm}
\put(0,80){\line(0,1){35}}
\linethickness{0.3mm}
\put(230,95){\line(1,0){15}}
\linethickness{0.3mm}
\put(355,95){\line(1,0){15}}
\end{picture}


==> PIC/slicing-computation.tex <==
%%Created by jPicEdt 1.4.1_03: mixed JPIC-XML/LaTeX format
%%Sun Nov 22 10:04:33 GMT-10:00 2020
%%Begin JPIC-XML
%<?xml version="1.0" standalone="yes"?>
%<jpic x-min="0" x-max="340" y-min="5" y-max="155" auto-bounding="true">
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(282.5,72.5)"
%	 stroke-width= "0.35"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\Progtype$
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(277.5,52.5)"
%	 stroke-width= "0.35"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\partial$
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(310,85)"
%	 stroke-width= "0.35"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\universal$
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(312.5,130)"
%	 stroke-width= "0.35"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\Progn$
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(322.5,5)"
%	 stroke-width= "0.35"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\Progm$
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(290,5)"
%	 stroke-width= "0.35"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\Progk$
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(265,20)"
%	 stroke-width= "0.35"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\program
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(267.5,37.5)"
%	 stroke-width= "0.35"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\Progtype$
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(30,85)"
%	 stroke-width= "0.35"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\gee
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(230,85)"
%	 stroke-width= "0.35"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\eqlsb$
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(90,85)"
%	 stroke-width= "0.35"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\eqlsa$
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(150,155)"
%	 stroke-width= "0.35"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\ux$
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(295,155)"
%	 stroke-width= "0.35"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\sx$
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(30,155)"
%	 stroke-width= "0.35"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\gx$
%</text>
%<multicurve fill-style= "none"
%	 points= "(340,115);(340,115);(340,55);(340,55)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(340,55);(340,55);(310,55);(310,55)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(310,35);(310,35);(280,35);(280,35)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(280,15);(280,15);(260,15);(260,15)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(260,35);(260,35);(260,15);(260,15)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(260,35);(260,35);(280,15);(280,15)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(280,35);(280,35);(260,55);(260,55)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(260,55);(260,55);(260,85);(260,85)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(260,85);(260,85);(310,35);(310,35)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(310,55);(310,55);(260,105);(260,105)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(260,105);(260,105);(260,115);(260,115)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(260,115);(260,115);(340,115);(340,115)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(270,45);(270,45);(270,25);(270,25)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(285,80);(285,80);(285,60);(285,60)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(292.5,35);(292.5,35);(292.5,5);(292.5,5)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(325,55);(325,55);(325,5);(325,5)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(310,130);(310,130);(310,115);(310,115)"
%	 />
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(170,85)"
%	 stroke-width= "0.35"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\universal$
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(172.5,130)"
%	 stroke-width= "0.35"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\Progn$
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(182.5,5)"
%	 stroke-width= "0.35"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\Progm$
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(152.5,5)"
%	 stroke-width= "0.35"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\Progk$
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(125,40)"
%	 stroke-width= "0.35"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\program
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(127.5,57.5)"
%	 stroke-width= "0.35"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\Progtype$
%</text>
%<multicurve fill-style= "none"
%	 points= "(200,115);(200,115);(200,55);(200,55)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(200,55);(200,55);(140,55);(140,55)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(140,35);(140,35);(120,35);(120,35)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(120,55);(120,55);(120,35);(120,35)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(120,55);(120,55);(140,35);(140,35)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(140,55);(140,55);(120,75);(120,75)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(120,75);(120,75);(120,115);(120,115)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(120,115);(120,115);(200,115);(200,115)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(130,65);(130,65);(130,45);(130,45)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(155,55);(155,55);(155,5);(155,5)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(185,55);(185,55);(185,5);(185,5)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(170,130);(170,130);(170,115);(170,115)"
%	 />
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(32.5,130)"
%	 stroke-width= "0.35"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\Progn$
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(42.5,5)"
%	 stroke-width= "0.35"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\Progm$
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(12.5,5)"
%	 stroke-width= "0.35"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\Progk$
%</text>
%<multicurve fill-style= "none"
%	 points= "(60,115);(60,115);(60,55);(60,55)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(60,55);(60,55);(0,55);(0,55)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(0,115);(0,115);(60,115);(60,115)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(15,55);(15,55);(15,5);(15,5)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(45,55);(45,55);(45,5);(45,5)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(30,130);(30,130);(30,115);(30,115)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(0,115);(0,115);(0,55);(0,55)"
%	 />
%</jpic>
%%End JPIC-XML
%LaTeX-picture environment using emulated lines and arcs
%You can rescale the whole picture (to 80% for instance) by using the command \def\JPicScale{0.8}
\ifx\JPicScale\undefined\def\JPicScale{1}\fi
\unitlength \JPicScale mm
\begin{picture}(340,155)(0,0)
\put(282.5,72.5){\makebox(0,0)[cr]{$\Progtype$}}

\put(277.5,52.5){\makebox(0,0)[cc]{$\partial$}}

\put(310,85){\makebox(0,0)[cc]{$\universal$}}

\put(312.5,130){\makebox(0,0)[cl]{$\Progn$}}

\put(322.5,5){\makebox(0,0)[cr]{$\Progm$}}

\put(290,5){\makebox(0,0)[cr]{$\Progk$}}

\put(265,20){\makebox(0,0)[cc]{\program}}

\put(267.5,37.5){\makebox(0,0)[cr]{$\Progtype$}}

\put(30,85){\makebox(0,0)[cc]{\gee}}

\put(230,85){\makebox(0,0)[cc]{$\eqlsb$}}

\put(90,85){\makebox(0,0)[cc]{$\eqlsa$}}

\put(150,155){\makebox(0,0)[cc]{$\ux$}}

\put(295,155){\makebox(0,0)[cc]{$\sx$}}

\put(30,155){\makebox(0,0)[cc]{$\gx$}}

\linethickness{0.3mm}
\put(340,55){\line(0,1){60}}
\linethickness{0.3mm}
\put(310,55){\line(1,0){30}}
\linethickness{0.3mm}
\put(280,35){\line(1,0){30}}
\linethickness{0.3mm}
\put(260,15){\line(1,0){20}}
\linethickness{0.3mm}
\put(260,15){\line(0,1){20}}
\linethickness{0.3mm}
\multiput(260,35)(0.12,-0.12){167}{\line(1,0){0.12}}
\linethickness{0.3mm}
\multiput(260,55)(0.12,-0.12){167}{\line(1,0){0.12}}
\linethickness{0.3mm}
\put(260,55){\line(0,1){30}}
\linethickness{0.3mm}
\multiput(260,85)(0.12,-0.12){417}{\line(1,0){0.12}}
\linethickness{0.3mm}
\multiput(260,105)(0.12,-0.12){417}{\line(1,0){0.12}}
\linethickness{0.3mm}
\put(260,105){\line(0,1){10}}
\linethickness{0.3mm}
\put(260,115){\line(1,0){80}}
\linethickness{0.3mm}
\put(270,25){\line(0,1){20}}
\linethickness{0.3mm}
\put(285,60){\line(0,1){20}}
\linethickness{0.3mm}
\put(292.5,5){\line(0,1){30}}
\linethickness{0.3mm}
\put(325,5){\line(0,1){50}}
\linethickness{0.3mm}
\put(310,115){\line(0,1){15}}
\put(170,85){\makebox(0,0)[cc]{$\universal$}}

\put(172.5,130){\makebox(0,0)[cl]{$\Progn$}}

\put(182.5,5){\makebox(0,0)[cr]{$\Progm$}}

\put(152.5,5){\makebox(0,0)[cr]{$\Progk$}}

\put(125,40){\makebox(0,0)[cc]{\program}}

\put(127.5,57.5){\makebox(0,0)[cr]{$\Progtype$}}

\linethickness{0.3mm}
\put(200,55){\line(0,1){60}}
\linethickness{0.3mm}
\put(140,55){\line(1,0){60}}
\linethickness{0.3mm}
\put(120,35){\line(1,0){20}}
\linethickness{0.3mm}
\put(120,35){\line(0,1){20}}
\linethickness{0.3mm}
\multiput(120,55)(0.12,-0.12){167}{\line(1,0){0.12}}
\linethickness{0.3mm}
\multiput(120,75)(0.12,-0.12){167}{\line(1,0){0.12}}
\linethickness{0.3mm}
\put(120,75){\line(0,1){40}}
\linethickness{0.3mm}
\put(120,115){\line(1,0){80}}
\linethickness{0.3mm}
\put(130,45){\line(0,1){20}}
\linethickness{0.3mm}
\put(155,5){\line(0,1){50}}
\linethickness{0.3mm}
\put(185,5){\line(0,1){50}}
\linethickness{0.3mm}
\put(170,115){\line(0,1){15}}
\put(32.5,130){\makebox(0,0)[cl]{$\Progn$}}

\put(42.5,5){\makebox(0,0)[cr]{$\Progm$}}

\put(12.5,5){\makebox(0,0)[cr]{$\Progk$}}

\linethickness{0.3mm}
\put(60,55){\line(0,1){60}}
\linethickness{0.3mm}
\put(0,55){\line(1,0){60}}
\linethickness{0.3mm}
\put(0,115){\line(1,0){60}}
\linethickness{0.3mm}
\put(15,5){\line(0,1){50}}
\linethickness{0.3mm}
\put(45,5){\line(0,1){50}}
\linethickness{0.3mm}
\put(30,115){\line(0,1){15}}
\linethickness{0.3mm}
\put(0,55){\line(0,1){60}}
\end{picture}


==> PIC/slicing.tex <==
%%Created by jPicEdt 1.4.1_03: mixed JPIC-XML/LaTeX format
%%Sun Nov 22 09:51:09 GMT-10:00 2020
%%Begin JPIC-XML
%<?xml version="1.0" standalone="yes"?>
%<jpic x-min="0" x-max="480" y-min="5" y-max="155" auto-bounding="true">
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(282.5,97.5)"
%	 stroke-width= "0.35"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\Progtype$
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(277.5,77.5)"
%	 stroke-width= "0.35"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\partial$
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(310,110)"
%	 stroke-width= "0.35"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\universal$
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(312.5,155)"
%	 stroke-width= "0.35"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\Progn$
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(322.5,30)"
%	 stroke-width= "0.35"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\Progm$
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(290,30)"
%	 stroke-width= "0.35"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\Progk$
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(265,45)"
%	 stroke-width= "0.35"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\program
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(267.5,62.5)"
%	 stroke-width= "0.35"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\Progtype$
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(30,110)"
%	 stroke-width= "0.35"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\gee
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(230,110)"
%	 stroke-width= "0.35"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\eqlsb$
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(370,110)"
%	 stroke-width= "0.35"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\eqlsc$
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(90,110)"
%	 stroke-width= "0.35"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\eqlsa$
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(155,5)"
%	 stroke-width= "0.35"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\ux$
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(295,5)"
%	 stroke-width= "0.35"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\sx$
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(230,5)"
%	 stroke-width= "0.35"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\eqlsb$
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(90,5)"
%	 stroke-width= "0.35"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\eqlsa$
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(415,75)"
%	 stroke-width= "0.35"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\Gx$
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(30,5)"
%	 stroke-width= "0.35"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\gx$
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(370,5)"
%	 stroke-width= "0.35"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\eqlsc$
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(435,5)"
%	 stroke-width= "0.35"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\tx$
%</text>
%<multicurve fill-style= "none"
%	 points= "(340,140);(340,140);(340,80);(340,80)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(340,80);(340,80);(310,80);(310,80)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(310,60);(310,60);(280,60);(280,60)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(280,40);(280,40);(260,40);(260,40)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(260,60);(260,60);(260,40);(260,40)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(260,60);(260,60);(280,40);(280,40)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(280,60);(280,60);(260,80);(260,80)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(260,80);(260,80);(260,110);(260,110)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(260,110);(260,110);(310,60);(310,60)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(310,80);(310,80);(260,130);(260,130)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(260,130);(260,130);(260,140);(260,140)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(260,140);(260,140);(340,140);(340,140)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(270,70);(270,70);(270,50);(270,50)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(285,105);(285,105);(285,85);(285,85)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(292.5,60);(292.5,60);(292.5,30);(292.5,30)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(325,80);(325,80);(325,30);(325,30)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(310,155);(310,155);(310,140);(310,140)"
%	 />
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(422.5,97.5)"
%	 stroke-width= "0.35"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\Progtype$
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(450,110)"
%	 stroke-width= "0.35"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\universal$
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(452.5,155)"
%	 stroke-width= "0.35"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\Progn$
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(462.5,30)"
%	 stroke-width= "0.35"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\Progm$
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(422.5,30)"
%	 stroke-width= "0.35"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\Progk$
%</text>
%<multicurve fill-style= "none"
%	 points= "(480,140);(480,140);(480,80);(480,80)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(480,80);(480,80);(450,80);(450,80)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(450,60);(450,60);(400,60);(400,60)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(400,60);(400,60);(400,110);(400,110)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(400,110);(400,110);(450,60);(450,60)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(450,80);(450,80);(400,130);(400,130)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(400,130);(400,130);(400,140);(400,140)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(400,140);(400,140);(480,140);(480,140)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(425,105);(425,105);(425,85);(425,85)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(425,60);(425,60);(425,30);(425,30)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(465,80);(465,80);(465,30);(465,30)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(450,155);(450,155);(450,140);(450,140)"
%	 />
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(170,110)"
%	 stroke-width= "0.35"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\universal$
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(172.5,155)"
%	 stroke-width= "0.35"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\Progn$
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(182.5,30)"
%	 stroke-width= "0.35"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\Progm$
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(152.5,30)"
%	 stroke-width= "0.35"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\Progk$
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(125,65)"
%	 stroke-width= "0.35"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\program
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(127.5,82.5)"
%	 stroke-width= "0.35"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\Progtype$
%</text>
%<multicurve fill-style= "none"
%	 points= "(200,140);(200,140);(200,80);(200,80)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(200,80);(200,80);(140,80);(140,80)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(140,60);(140,60);(120,60);(120,60)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(120,80);(120,80);(120,60);(120,60)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(120,80);(120,80);(140,60);(140,60)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(140,80);(140,80);(120,100);(120,100)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(120,100);(120,100);(120,140);(120,140)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(120,140);(120,140);(200,140);(200,140)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(130,90);(130,90);(130,70);(130,70)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(155,80);(155,80);(155,30);(155,30)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(185,80);(185,80);(185,30);(185,30)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(170,155);(170,155);(170,140);(170,140)"
%	 />
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(32.5,155)"
%	 stroke-width= "0.35"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\Progn$
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(42.5,30)"
%	 stroke-width= "0.35"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\Progm$
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(12.5,30)"
%	 stroke-width= "0.35"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\Progk$
%</text>
%<multicurve fill-style= "none"
%	 points= "(60,140);(60,140);(60,80);(60,80)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(60,80);(60,80);(0,80);(0,80)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(0,140);(0,140);(60,140);(60,140)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(15,80);(15,80);(15,30);(15,30)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(45,80);(45,80);(45,30);(45,30)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(30,155);(30,155);(30,140);(30,140)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(0,140);(0,140);(0,80);(0,80)"
%	 />
%</jpic>
%%End JPIC-XML
%LaTeX-picture environment using emulated lines and arcs
%You can rescale the whole picture (to 80% for instance) by using the command \def\JPicScale{0.8}
\ifx\JPicScale\undefined\def\JPicScale{1}\fi
\unitlength \JPicScale mm
\begin{picture}(480,155)(0,0)
\put(282.5,97.5){\makebox(0,0)[cr]{$\Progtype$}}

\put(277.5,77.5){\makebox(0,0)[cc]{$\partial$}}

\put(310,110){\makebox(0,0)[cc]{$\universal$}}

\put(312.5,155){\makebox(0,0)[cl]{$\Progn$}}

\put(322.5,30){\makebox(0,0)[cr]{$\Progm$}}

\put(290,30){\makebox(0,0)[cr]{$\Progk$}}

\put(265,45){\makebox(0,0)[cc]{\program}}

\put(267.5,62.5){\makebox(0,0)[cr]{$\Progtype$}}

\put(30,110){\makebox(0,0)[cc]{\gee}}

\put(230,110){\makebox(0,0)[cc]{$\eqlsb$}}

\put(370,110){\makebox(0,0)[cc]{$\eqlsc$}}

\put(90,110){\makebox(0,0)[cc]{$\eqlsa$}}

\put(155,5){\makebox(0,0)[cc]{$\ux$}}

\put(295,5){\makebox(0,0)[cc]{$\sx$}}

\put(230,5){\makebox(0,0)[cc]{$\eqlsb$}}

\put(90,5){\makebox(0,0)[cc]{$\eqlsa$}}

\put(415,75){\makebox(0,0)[cc]{$\Gx$}}

\put(30,5){\makebox(0,0)[cc]{$\gx$}}

\put(370,5){\makebox(0,0)[cc]{$\eqlsc$}}

\put(435,5){\makebox(0,0)[cc]{$\tx$}}

\linethickness{0.3mm}
\put(340,80){\line(0,1){60}}
\linethickness{0.3mm}
\put(310,80){\line(1,0){30}}
\linethickness{0.3mm}
\put(280,60){\line(1,0){30}}
\linethickness{0.3mm}
\put(260,40){\line(1,0){20}}
\linethickness{0.3mm}
\put(260,40){\line(0,1){20}}
\linethickness{0.3mm}
\multiput(260,60)(0.12,-0.12){167}{\line(1,0){0.12}}
\linethickness{0.3mm}
\multiput(260,80)(0.12,-0.12){167}{\line(1,0){0.12}}
\linethickness{0.3mm}
\put(260,80){\line(0,1){30}}
\linethickness{0.3mm}
\multiput(260,110)(0.12,-0.12){417}{\line(1,0){0.12}}
\linethickness{0.3mm}
\multiput(260,130)(0.12,-0.12){417}{\line(1,0){0.12}}
\linethickness{0.3mm}
\put(260,130){\line(0,1){10}}
\linethickness{0.3mm}
\put(260,140){\line(1,0){80}}
\linethickness{0.3mm}
\put(270,50){\line(0,1){20}}
\linethickness{0.3mm}
\put(285,85){\line(0,1){20}}
\linethickness{0.3mm}
\put(292.5,30){\line(0,1){30}}
\linethickness{0.3mm}
\put(325,30){\line(0,1){50}}
\linethickness{0.3mm}
\put(310,140){\line(0,1){15}}
\put(422.5,97.5){\makebox(0,0)[cr]{$\Progtype$}}

\put(450,110){\makebox(0,0)[cc]{$\universal$}}

\put(452.5,155){\makebox(0,0)[cl]{$\Progn$}}

\put(462.5,30){\makebox(0,0)[cr]{$\Progm$}}

\put(422.5,30){\makebox(0,0)[cr]{$\Progk$}}

\linethickness{0.3mm}
\put(480,80){\line(0,1){60}}
\linethickness{0.3mm}
\put(450,80){\line(1,0){30}}
\linethickness{0.3mm}
\put(400,60){\line(1,0){50}}
\linethickness{0.3mm}
\put(400,60){\line(0,1){50}}
\linethickness{0.3mm}
\multiput(400,110)(0.12,-0.12){417}{\line(1,0){0.12}}
\linethickness{0.3mm}
\multiput(400,130)(0.12,-0.12){417}{\line(1,0){0.12}}
\linethickness{0.3mm}
\put(400,130){\line(0,1){10}}
\linethickness{0.3mm}
\put(400,140){\line(1,0){80}}
\linethickness{0.3mm}
\put(425,85){\line(0,1){20}}
\linethickness{0.3mm}
\put(425,30){\line(0,1){30}}
\linethickness{0.3mm}
\put(465,30){\line(0,1){50}}
\linethickness{0.3mm}
\put(450,140){\line(0,1){15}}
\put(170,110){\makebox(0,0)[cc]{$\universal$}}

\put(172.5,155){\makebox(0,0)[cl]{$\Progn$}}

\put(182.5,30){\makebox(0,0)[cr]{$\Progm$}}

\put(152.5,30){\makebox(0,0)[cr]{$\Progk$}}

\put(125,65){\makebox(0,0)[cc]{\program}}

\put(127.5,82.5){\makebox(0,0)[cr]{$\Progtype$}}

\linethickness{0.3mm}
\put(200,80){\line(0,1){60}}
\linethickness{0.3mm}
\put(140,80){\line(1,0){60}}
\linethickness{0.3mm}
\put(120,60){\line(1,0){20}}
\linethickness{0.3mm}
\put(120,60){\line(0,1){20}}
\linethickness{0.3mm}
\multiput(120,80)(0.12,-0.12){167}{\line(1,0){0.12}}
\linethickness{0.3mm}
\multiput(120,100)(0.12,-0.12){167}{\line(1,0){0.12}}
\linethickness{0.3mm}
\put(120,100){\line(0,1){40}}
\linethickness{0.3mm}
\put(120,140){\line(1,0){80}}
\linethickness{0.3mm}
\put(130,70){\line(0,1){20}}
\linethickness{0.3mm}
\put(155,30){\line(0,1){50}}
\linethickness{0.3mm}
\put(185,30){\line(0,1){50}}
\linethickness{0.3mm}
\put(170,140){\line(0,1){15}}
\put(32.5,155){\makebox(0,0)[cl]{$\Progn$}}

\put(42.5,30){\makebox(0,0)[cr]{$\Progm$}}

\put(12.5,30){\makebox(0,0)[cr]{$\Progk$}}

\linethickness{0.3mm}
\put(60,80){\line(0,1){60}}
\linethickness{0.3mm}
\put(0,80){\line(1,0){60}}
\linethickness{0.3mm}
\put(0,140){\line(1,0){60}}
\linethickness{0.3mm}
\put(15,30){\line(0,1){50}}
\linethickness{0.3mm}
\put(45,30){\line(0,1){50}}
\linethickness{0.3mm}
\put(30,140){\line(0,1){15}}
\linethickness{0.3mm}
\put(0,80){\line(0,1){60}}
\end{picture}


==> PIC/smullyan-1.tex <==
%%Created by jPicEdt 1.4.1_03: mixed JPIC-XML/LaTeX format
%%Tue Nov 05 18:49:02 GMT-10:00 2019
%%Begin JPIC-XML
%<?xml version="1.0" standalone="yes"?>
%<jpic x-min="-7.5" x-max="417.5" y-min="0" y-max="118.12" auto-bounding="true">
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(110,59.38);(110,59.38);(110,34.38);(110,34.38)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(165,80);(165,80);(165,105);(165,105)"
%	 />
%<text text-vert-align= "center-v"
%	 anchor-point= "(156.88,25)"
%	 stroke-width= "0.75"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\inputt$
%</text>
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(135,80);(135,80);(165,80);(165,80)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(160,80);(160,80);(160,25);(160,25)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(110,34.38);(110,34.38);(135,34.38);(135,34.38)"
%	 />
%<text text-vert-align= "center-v"
%	 anchor-point= "(145,92.5)"
%	 stroke-width= "0.75"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\universal
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(117.5,41.24)"
%	 stroke-width= "0.75"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\program
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(95,93.75)"
%	 stroke-width= "0.75"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\EQLS
%</text>
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(110,59.38);(110,59.38);(135,34.38);(135,34.38)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(122.5,92.5);(122.5,92.5);(122.5,47.5);(122.5,47.5)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(110,105);(110,105);(135,80);(135,80)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(70,80);(70,80);(70,105);(70,105)"
%	 />
%<text text-vert-align= "center-v"
%	 anchor-point= "(61.88,25)"
%	 stroke-width= "0.75"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\inputt$
%</text>
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(20,80);(20,80);(70,79.99);(70,79.99)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(65,80);(65,80);(65,25);(65,25)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(25,80);(25,80);(25,62.5);(25,62.5)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(20,105);(20,105);(20,80);(20,80)"
%	 />
%<text text-vert-align= "center-v"
%	 anchor-point= "(45,91.88)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\gee$
%</text>
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(-2.5,70);(-2.5,70);(17.5,70);(17.5,70)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(35,52.5);(35,52.5);(15,52.5);(15,52.5)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(17.5,70);(17.5,70);(35,52.51);(35,52.51)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(-2.5,70);(-2.5,70);(15,52.5);(15,52.5)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(35,37.5);(35,37.5);(35,25);(35,25)"
%	 />
%<ellipse p3= "(36.41,36.09)"
%	 p2= "(36.41,38.91)"
%	 fill-color= "#330033"
%	 p1= "(33.59,38.91)"
%	 closure= "open"
%	 fill-style= "solid"
%	 angle-end= "0"
%	 angle-start= "0"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(45,80);(45,80);(45,47.5);(45,47.5)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(5,62.5);(5,62.5);(5,47.5);(5,47.5)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(45,47.5);(45,47.5);(35,37.5);(35,37.5)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(25,47.5);(25,47.5);(35,37.49);(35,37.49)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(140,80);(140,80);(140,25);(140,25)"
%	 />
%<text text-vert-align= "center-v"
%	 anchor-point= "(136.88,25)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\progtype$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(16.25,61.25)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\parteval$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(28.13,70.62)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\progtype$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(125,60)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\progtype$
%</text>
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(25,52.5);(25,52.5);(25,47.5);(25,47.5)"
%	 />
%<text text-vert-align= "center-v"
%	 anchor-point= "(31.88,25)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\progtype$
%</text>
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(-7.5,60);(-7.5,60);(-7.5,35);(-7.5,35)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(-7.5,35);(-7.5,35);(17.5,35);(17.5,35)"
%	 />
%<text text-vert-align= "center-v"
%	 anchor-point= "(0,42.5)"
%	 stroke-width= "0.75"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\program
%</text>
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(-7.5,60);(-7.5,60);(17.5,35);(17.5,35)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(380,31.88);(380,31.88);(380,6.88);(380,6.88)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(417.5,80);(417.5,80);(417.5,105);(417.5,105)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(405,80);(405,80);(417.5,80);(417.5,80)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(380,6.88);(380,6.88);(405,6.88);(405,6.88)"
%	 />
%<text text-vert-align= "center-v"
%	 anchor-point= "(407.5,92.5)"
%	 stroke-width= "0.75"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\universal
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(365,93.75)"
%	 stroke-width= "0.75"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\EQLS
%</text>
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(380,31.88);(380,31.88);(405,6.88);(405,6.88)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(392.5,92.5);(392.5,92.5);(392.5,19.99);(392.5,19.99)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(380,105);(380,105);(405,80);(405,80)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(340,80);(340,80);(340,105);(340,105)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(290,80);(290,80);(340,79.99);(340,79.99)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(335,80);(335,80);(335,0);(335,0)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(295,80);(295,80);(295,62.5);(295,62.5)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(290,105);(290,105);(290,80);(290,80)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(267.5,70);(267.5,70);(287.5,70);(287.5,70)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(305,52.5);(305,52.5);(285,52.5);(285,52.5)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(287.5,70);(287.5,70);(305,52.51);(305,52.51)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(267.5,70);(267.5,70);(285,52.5);(285,52.5)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(305,37.5);(305,37.5);(305,20);(305,20)"
%	 />
%<ellipse p3= "(306.41,36.09)"
%	 p2= "(306.41,38.91)"
%	 fill-color= "#330033"
%	 p1= "(303.59,38.91)"
%	 closure= "open"
%	 fill-style= "solid"
%	 angle-end= "0"
%	 angle-start= "0"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(315,80);(315,80);(315,47.5);(315,47.5)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(275,62.5);(275,62.5);(275,47.5);(275,47.5)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(315,47.5);(315,47.5);(305,37.5);(305,37.5)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(295,47.5);(295,47.5);(305,37.49);(305,37.49)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(412.5,80);(412.5,80);(412.5,0);(412.5,0)"
%	 />
%<text text-vert-align= "center-v"
%	 anchor-point= "(317.5,71.25)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\progtype$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(286.25,61.25)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\parteval$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(297.5,71.25)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\progtype$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(395,32.5)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\progtype$
%</text>
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(295,52.5);(295,52.5);(295,47.5);(295,47.5)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(262.5,60);(262.5,60);(262.5,35);(262.5,35)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(262.5,35);(262.5,35);(287.5,35);(287.5,35)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(262.5,60);(262.5,60);(287.5,35);(287.5,35)"
%	 />
%<text text-vert-align= "center-v"
%	 anchor-point= "(315,91.25)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\hee$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(388.75,15)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\prohram$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(332.5,0)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\inputtt$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(410,0)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\inputtt$
%</text>
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(292.5,31.88);(292.5,31.88);(292.5,6.88);(292.5,6.88)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(292.5,6.88);(292.5,6.88);(317.5,6.88);(317.5,6.88)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(292.5,31.88);(292.5,31.88);(317.5,6.88);(317.5,6.88)"
%	 />
%<text text-vert-align= "center-v"
%	 anchor-point= "(301.25,15)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\prohram$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(271.25,41.25)"
%	 stroke-width= "0.75"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\program
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(47.5,70)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\progtype$
%</text>
%<parallelogram p3= "(147.5,117.5)"
%	 p2= "(147.5,105)"
%	 fill-color= "#999999"
%	 p1= "(152.5,105)"
%	 stroke-color= "#999999"
%	 fill-style= "solid"
%	 />
%<parallelogram p3= "(42.5,117.5)"
%	 p2= "(42.5,105)"
%	 fill-color= "#999999"
%	 p1= "(47.5,105)"
%	 stroke-color= "#999999"
%	 fill-style= "solid"
%	 />
%<parallelogram p3= "(408.75,117.5)"
%	 p2= "(408.75,105)"
%	 fill-color= "#999999"
%	 p1= "(413.75,105)"
%	 stroke-color= "#999999"
%	 fill-style= "solid"
%	 />
%<parallelogram p3= "(312.5,117.5)"
%	 p2= "(312.5,105)"
%	 fill-color= "#999999"
%	 p1= "(317.5,105)"
%	 stroke-color= "#999999"
%	 fill-style= "solid"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(110,105);(110,105);(165,105);(165,105)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(150,116.88);(150,116.88);(150,105);(150,105)"
%	 />
%<text text-vert-align= "center-v"
%	 anchor-point= "(155,118.12)"
%	 stroke-width= "0.75"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\nameslang$
%</text>
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(20,105);(20,105);(70,105);(70,105)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(45,116.88);(45,116.88);(45,105);(45,105)"
%	 />
%<text text-vert-align= "center-v"
%	 anchor-point= "(50,118.12)"
%	 stroke-width= "0.75"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\nameslang$
%</text>
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(380,105);(380,105);(417.5,105);(417.5,105)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(411.25,117.5);(411.25,117.5);(411.25,105.62);(411.25,105.62)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(290,105);(290,105);(340,105);(340,105)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(315,116.88);(315,116.88);(315,105);(315,105)"
%	 />
%<text text-vert-align= "center-v"
%	 anchor-point= "(416.25,117.5)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\nameslangg$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(320,117.5)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\nameslangg$
%</text>
%</jpic>
%%End JPIC-XML
%PSTricks content-type (pstricks.sty package needed)
%Add \usepackage{pstricks} in the preamble of your LaTeX file
%You can rescale the whole picture (to 80% for instance) by using the command \def\JPicScale{0.8}
\ifx\JPicScale\undefined\def\JPicScale{1}\fi
\psset{unit=\JPicScale mm}
\psset{linewidth=0.3,dotsep=1,hatchwidth=0.3,hatchsep=1.5,shadowsize=1,dimen=middle}
\psset{dotsize=0.7 2.5,dotscale=1 1,fillcolor=black}
\psset{arrowsize=1 2,arrowlength=1,arrowinset=0.25,tbarsize=0.7 5,bracketlength=0.15,rbracketlength=0.15}
\begin{pspicture}(0,0)(417.5,118.12)
\psline[linewidth=0.75](110,59.38)(110,34.38)
\psline[linewidth=0.75](165,80)(165,105)
\rput[r](156.88,25){$\inputt$}
\psline[linewidth=0.75](135,80)(165,80)
\psline[linewidth=0.75](160,80)(160,25)
\psline[linewidth=0.75](110,34.38)(135,34.38)
\rput(145,92.5){\universal}
\rput(117.5,41.24){\program}
\rput(95,93.75){\EQLS}
\psline[linewidth=0.75](110,59.38)(135,34.38)
\psline[linewidth=0.75](122.5,92.5)(122.5,47.5)
\psline[linewidth=0.75](110,105)(135,80)
\psline[linewidth=0.75](70,80)(70,105)
\rput[r](61.88,25){$\inputt$}
\psline[linewidth=0.75](20,80)(70,79.99)
\psline[linewidth=0.75](65,80)(65,25)
\psline[linewidth=0.75](25,80)(25,62.5)
\psline[linewidth=0.75](20,105)(20,80)
\rput(45,91.88){$\gee$}
\psline[linewidth=0.75](-2.5,70)(17.5,70)
\psline[linewidth=0.75](35,52.5)(15,52.5)
\psline[linewidth=0.75](17.5,70)(35,52.51)
\psline[linewidth=0.75](-2.5,70)(15,52.5)
\psline[linewidth=0.75](35,37.5)(35,25)
\newrgbcolor{userFillColour}{0.2 0 0.2}
\rput{0}(35,37.5){\psellipse[fillcolor=userFillColour,fillstyle=solid](0,0)(1.41,-1.41)}
\psline[linewidth=0.75](45,80)(45,47.5)
\psline[linewidth=0.75](5,62.5)(5,47.5)
\psline[linewidth=0.75](45,47.5)(35,37.5)
\psline[linewidth=0.75](25,47.5)(35,37.49)
\psline[linewidth=0.75](140,80)(140,25)
\rput[r](136.88,25){$\progtype$}
\rput(16.25,61.25){$\parteval$}
\rput[l](28.13,70.62){$\progtype$}
\rput[l](125,60){$\progtype$}
\psline[linewidth=0.75](25,52.5)(25,47.5)
\rput[r](31.88,25){$\progtype$}
\psline[linewidth=0.75](-7.5,60)(-7.5,35)
\psline[linewidth=0.75](-7.5,35)(17.5,35)
\rput(0,42.5){\program}
\psline[linewidth=0.75](-7.5,60)(17.5,35)
\psline[linewidth=0.75](380,31.88)(380,6.88)
\psline[linewidth=0.75](417.5,80)(417.5,105)
\psline[linewidth=0.75](405,80)(417.5,80)
\psline[linewidth=0.75](380,6.88)(405,6.88)
\rput(407.5,92.5){\universal}
\rput(365,93.75){\EQLS}
\psline[linewidth=0.75](380,31.88)(405,6.88)
\psline[linewidth=0.75](392.5,92.5)(392.5,19.99)
\psline[linewidth=0.75](380,105)(405,80)
\psline[linewidth=0.75](340,80)(340,105)
\psline[linewidth=0.75](290,80)(340,79.99)
\psline[linewidth=0.75](335,80)(335,0)
\psline[linewidth=0.75](295,80)(295,62.5)
\psline[linewidth=0.75](290,105)(290,80)
\psline[linewidth=0.75](267.5,70)(287.5,70)
\psline[linewidth=0.75](305,52.5)(285,52.5)
\psline[linewidth=0.75](287.5,70)(305,52.51)
\psline[linewidth=0.75](267.5,70)(285,52.5)
\psline[linewidth=0.75](305,37.5)(305,20)
\newrgbcolor{userFillColour}{0.2 0 0.2}
\rput{0}(305,37.5){\psellipse[fillcolor=userFillColour,fillstyle=solid](0,0)(1.41,-1.41)}
\psline[linewidth=0.75](315,80)(315,47.5)
\psline[linewidth=0.75](275,62.5)(275,47.5)
\psline[linewidth=0.75](315,47.5)(305,37.5)
\psline[linewidth=0.75](295,47.5)(305,37.49)
\psline[linewidth=0.75](412.5,80)(412.5,0)
\rput[l](317.5,71.25){$\progtype$}
\rput(286.25,61.25){$\parteval$}
\rput[l](297.5,71.25){$\progtype$}
\rput[l](395,32.5){$\progtype$}
\psline[linewidth=0.75](295,52.5)(295,47.5)
\psline[linewidth=0.75](262.5,60)(262.5,35)
\psline[linewidth=0.75](262.5,35)(287.5,35)
\psline[linewidth=0.75](262.5,60)(287.5,35)
\rput(315,91.25){$\hee$}
\rput(388.75,15){$\prohram$}
\rput[r](332.5,0){$\inputtt$}
\rput[r](410,0){$\inputtt$}
\psline[linewidth=0.75](292.5,31.88)(292.5,6.88)
\psline[linewidth=0.75](292.5,6.88)(317.5,6.88)
\psline[linewidth=0.75](292.5,31.88)(317.5,6.88)
\rput(301.25,15){$\prohram$}
\rput(271.25,41.25){\program}
\rput[l](47.5,70){$\progtype$}
\newrgbcolor{userLineColour}{0.6 0.6 0.6}
\newrgbcolor{userFillColour}{0.6 0.6 0.6}
\pspolygon[linecolor=userLineColour,fillcolor=userFillColour,fillstyle=solid](152.5,105)(147.5,105)(147.5,117.5)(152.5,117.5)
\newrgbcolor{userLineColour}{0.6 0.6 0.6}
\newrgbcolor{userFillColour}{0.6 0.6 0.6}
\pspolygon[linecolor=userLineColour,fillcolor=userFillColour,fillstyle=solid](47.5,105)(42.5,105)(42.5,117.5)(47.5,117.5)
\newrgbcolor{userLineColour}{0.6 0.6 0.6}
\newrgbcolor{userFillColour}{0.6 0.6 0.6}
\pspolygon[linecolor=userLineColour,fillcolor=userFillColour,fillstyle=solid](413.75,105)(408.75,105)(408.75,117.5)(413.75,117.5)
\newrgbcolor{userLineColour}{0.6 0.6 0.6}
\newrgbcolor{userFillColour}{0.6 0.6 0.6}
\pspolygon[linecolor=userLineColour,fillcolor=userFillColour,fillstyle=solid](317.5,105)(312.5,105)(312.5,117.5)(317.5,117.5)
\psline[linewidth=0.75](110,105)(165,105)
\psline[linewidth=0.75](150,116.88)(150,105)
\rput[l](155,118.12){$\nameslang$}
\psline[linewidth=0.75](20,105)(70,105)
\psline[linewidth=0.75](45,116.88)(45,105)
\rput[l](50,118.12){$\nameslang$}
\psline[linewidth=0.75](380,105)(417.5,105)
\psline[linewidth=0.75](411.25,117.5)(411.25,105.62)
\psline[linewidth=0.75](290,105)(340,105)
\psline[linewidth=0.75](315,116.88)(315,105)
\rput[l](416.25,117.5){$\nameslangg$}
\rput[l](320,117.5){$\nameslangg$}
\end{pspicture}


==> PIC/smullyan-2.tex <==
%%Created by jPicEdt 1.4.1_03: mixed JPIC-XML/LaTeX format
%%Wed Dec 11 21:14:06 GMT-10:00 2019
%%Begin JPIC-XML
%<?xml version="1.0" standalone="yes"?>
%<jpic x-min="2.5" x-max="320" y-min="0" y-max="127.5" auto-bounding="true">
%<multicurve fill-style= "none"
%	 points= "(60,55);(60,55);(60,70);(60,70)"
%	 stroke-width= "0.75"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(117.5,2.5)"
%	 text-frame= "noframe"
%	 stroke-width= "0.75"
%	 text-hor-align= "right"
%	 >
%$\inputt$
%</text>
%<multicurve fill-style= "none"
%	 points= "(30,90);(30,90);(125,90);(125,90)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(120,90);(120,90);(120,0);(120,0)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(35,90);(35,90);(35,72.5);(35,72.5)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(30,115);(30,115);(30,90);(30,90)"
%	 stroke-width= "0.75"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(77.5,102.5)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\gee$
%</text>
%<multicurve fill-style= "none"
%	 points= "(7.5,80);(7.5,80);(27.5,80);(27.5,80)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(45,62.5);(45,62.5);(25,62.5);(25,62.5)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(27.5,80);(27.5,80);(45,62.51);(45,62.51)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(7.5,80);(7.5,80);(25,62.5);(25,62.5)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(57.5,52.5);(57.5,52.5);(37.5,52.5);(37.5,52.5)"
%	 stroke-width= "0.75"
%	 />
%<ellipse p3= "(60.18,50)"
%	 fill-style= "solid"
%	 p2= "(60.18,55)"
%	 fill-color= "#330033"
%	 p1= "(54.82,55)"
%	 closure= "open"
%	 angle-end= "0"
%	 angle-start= "0"
%	 />
%<multicurve fill-style= "none"
%	 points= "(15,55);(15,55);(30,40);(30,40)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(15,72.5);(15,72.5);(15,55);(15,55)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(60,55);(60,55);(57.5,52.5);(57.5,52.5)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(35,55.01);(35,55.01);(37.5,52.5);(37.5,52.5)"
%	 stroke-width= "0.75"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(26.25,71.25)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\parteval$
%</text>
%<multicurve fill-style= "none"
%	 points= "(35,62.5);(35,62.5);(35,55);(35,55)"
%	 stroke-width= "0.75"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(267.5,102.5)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\hee$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(307.5,2.5)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\inputtt$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(225,5)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\prohram$
%</text>
%<parallelogram p3= "(75,127.5)"
%	 fill-style= "solid"
%	 p2= "(75,115)"
%	 fill-color= "#999999"
%	 p1= "(80,115)"
%	 stroke-color= "#999999"
%	 />
%<multicurve fill-style= "none"
%	 points= "(30,115);(30,115);(125,115);(125,115)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(77.5,126.88);(77.5,126.88);(77.5,115);(77.5,115)"
%	 stroke-width= "0.75"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(82.5,125)"
%	 text-frame= "noframe"
%	 stroke-width= "0.75"
%	 text-hor-align= "left"
%	 >
%$\nameslang$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(272.5,125)"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\nameslangg$
%</text>
%<multicurve fill-style= "none"
%	 points= "(77.5,90);(77.5,90);(77.5,72.5);(77.5,72.5)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(50,80);(50,80);(70,80);(70,80)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(87.5,62.5);(87.5,62.5);(67.5,62.5);(67.5,62.5)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(70,79.99);(70,79.99);(87.5,62.5);(87.5,62.5)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(50,80);(50,80);(67.5,62.5);(67.5,62.5)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(30,40);(30,40);(30,10);(30,10)"
%	 stroke-width= "0.75"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(68.75,71.25)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\parteval$
%</text>
%<multicurve fill-style= "none"
%	 points= "(77.5,62.5);(77.5,62.5);(77.5,55);(77.5,55)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(20,20);(20,20);(20,0);(20,0)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(20,0);(20,0);(40,0);(40,0)"
%	 stroke-width= "0.75"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(27.5,5)"
%	 text-frame= "noframe"
%	 stroke-width= "0.75"
%	 text-hor-align= "center-h"
%	 >
%\program
%</text>
%<multicurve fill-style= "none"
%	 points= "(20,20);(20,20);(40,0);(40,0)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(125,115);(125,115);(125,90);(125,90)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(57.5,52.5);(57.5,52.5);(57.5,0);(57.5,0)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 stroke-overstrike-width= "1.35"
%	 points= "(62.5,40);(62.5,40);(30,40);(30,40)"
%	 stroke-overstrike= "true"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(77.5,55);(77.5,55);(62.5,40);(62.5,40)"
%	 stroke-width= "0.75"
%	 />
%<ellipse p3= "(32.68,37.5)"
%	 fill-style= "solid"
%	 p2= "(32.68,42.5)"
%	 fill-color= "#330033"
%	 p1= "(27.32,42.5)"
%	 closure= "open"
%	 angle-end= "0"
%	 angle-start= "0"
%	 />
%<multicurve fill-style= "none"
%	 points= "(250,55);(250,55);(250,70);(250,70)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(220,90);(220,90);(315,90);(315,90)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(310,90);(310,90);(310,0);(310,0)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(225,90);(225,90);(225,72.5);(225,72.5)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(220,115);(220,115);(220,90);(220,90)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(197.5,80);(197.5,80);(217.5,80);(217.5,80)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(235,62.5);(235,62.5);(215,62.5);(215,62.5)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(217.5,80);(217.5,80);(235,62.51);(235,62.51)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(197.5,80);(197.5,80);(215,62.5);(215,62.5)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(247.5,52.5);(247.5,52.5);(227.5,52.5);(227.5,52.5)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(205,55);(205,55);(220,40);(220,40)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(205,72.5);(205,72.5);(205,55);(205,55)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(250,55);(250,55);(247.5,52.5);(247.5,52.5)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(225,55.01);(225,55.01);(227.5,52.5);(227.5,52.5)"
%	 stroke-width= "0.75"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(216.25,71.25)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\parteval$
%</text>
%<multicurve fill-style= "none"
%	 points= "(225,62.5);(225,62.5);(225,55);(225,55)"
%	 stroke-width= "0.75"
%	 />
%<parallelogram p3= "(265,127.5)"
%	 fill-style= "solid"
%	 p2= "(265,115)"
%	 fill-color= "#999999"
%	 p1= "(270,115)"
%	 stroke-color= "#999999"
%	 />
%<multicurve fill-style= "none"
%	 points= "(220,115);(220,115);(315,115);(315,115)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(267.5,126.88);(267.5,126.88);(267.5,115);(267.5,115)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(267.5,90);(267.5,90);(267.5,72.5);(267.5,72.5)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(240,80);(240,80);(260,80);(260,80)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(277.5,62.5);(277.5,62.5);(257.5,62.5);(257.5,62.5)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(260,79.99);(260,79.99);(277.5,62.5);(277.5,62.5)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(240,80);(240,80);(257.5,62.5);(257.5,62.5)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(252.5,40);(252.5,40);(252.5,0);(252.5,0)"
%	 stroke-width= "0.75"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(258.75,71.25)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\parteval$
%</text>
%<multicurve fill-style= "none"
%	 points= "(267.5,62.5);(267.5,62.5);(267.5,55);(267.5,55)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(217.5,20);(217.5,20);(217.5,0);(217.5,0)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(217.5,0);(217.5,0);(237.5,0);(237.5,0)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(315,115);(315,115);(315,90);(315,90)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(252.5,40);(252.5,40);(220,40);(220,40)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 stroke-overstrike-width= "1.35"
%	 points= "(227.5,52.5);(227.5,52.5);(227.5,10);(227.5,10)"
%	 stroke-overstrike= "true"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(267.5,55);(267.5,55);(252.5,40);(252.5,40)"
%	 stroke-width= "0.75"
%	 />
%<ellipse p3= "(255.18,37.5)"
%	 fill-style= "solid"
%	 p2= "(255.18,42.5)"
%	 fill-color= "#330033"
%	 p1= "(249.82,42.5)"
%	 closure= "open"
%	 angle-end= "0"
%	 angle-start= "0"
%	 />
%<parallelogram p3= "(320,30)"
%	 fill-style= "none"
%	 p2= "(320,120)"
%	 p1= "(192.5,120)"
%	 />
%<parallelogram p3= "(130,30)"
%	 fill-style= "none"
%	 p2= "(130,120)"
%	 p1= "(2.5,120)"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(290,50)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\heehat$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(100,50)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\geehat$
%</text>
%<multicurve fill-style= "none"
%	 points= "(217.5,20);(217.5,20);(237.5,0);(237.5,0)"
%	 stroke-width= "0.75"
%	 />
%<ellipse p3= "(230.18,50)"
%	 fill-style= "solid"
%	 p2= "(230.18,55)"
%	 fill-color= "#330033"
%	 p1= "(224.82,55)"
%	 closure= "open"
%	 angle-end= "0"
%	 angle-start= "0"
%	 />
%</jpic>
%%End JPIC-XML
%PSTricks content-type (pstricks.sty package needed)
%Add \usepackage{pstricks} in the preamble of your LaTeX file
%You can rescale the whole picture (to 80% for instance) by using the command \def\JPicScale{0.8}
\ifx\JPicScale\undefined\def\JPicScale{1}\fi
\psset{unit=\JPicScale mm}
\psset{linewidth=0.3,dotsep=1,hatchwidth=0.3,hatchsep=1.5,shadowsize=1,dimen=middle}
\psset{dotsize=0.7 2.5,dotscale=1 1,fillcolor=black}
\psset{arrowsize=1 2,arrowlength=1,arrowinset=0.25,tbarsize=0.7 5,bracketlength=0.15,rbracketlength=0.15}
\begin{pspicture}(0,0)(320,127.5)
\psline[linewidth=0.75](60,55)(60,70)
\rput[r](117.5,2.5){$\inputt$}
\psline[linewidth=0.75](30,90)(125,90)
\psline[linewidth=0.75](120,90)(120,0)
\psline[linewidth=0.75](35,90)(35,72.5)
\psline[linewidth=0.75](30,115)(30,90)
\rput(77.5,102.5){$\gee$}
\psline[linewidth=0.75](7.5,80)(27.5,80)
\psline[linewidth=0.75](45,62.5)(25,62.5)
\psline[linewidth=0.75](27.5,80)(45,62.51)
\psline[linewidth=0.75](7.5,80)(25,62.5)
\psline[linewidth=0.75](57.5,52.5)(37.5,52.5)
\newrgbcolor{userFillColour}{0.2 0 0.2}
\rput{0}(57.5,52.5){\psellipse[fillcolor=userFillColour,fillstyle=solid](0,0)(2.68,-2.5)}
\psline[linewidth=0.75](15,55)(30,40)
\psline[linewidth=0.75](15,72.5)(15,55)
\psline[linewidth=0.75](60,55)(57.5,52.5)
\psline[linewidth=0.75](35,55.01)(37.5,52.5)
\rput(26.25,71.25){$\parteval$}
\psline[linewidth=0.75](35,62.5)(35,55)
\rput(267.5,102.5){$\hee$}
\rput[r](307.5,2.5){$\inputtt$}
\rput(225,5){$\prohram$}
\newrgbcolor{userLineColour}{0.6 0.6 0.6}
\newrgbcolor{userFillColour}{0.6 0.6 0.6}
\psline[linewidth=0.75](30,115)(125,115)
\psline[linewidth=0.75](77.5,126.88)(77.5,115)
\rput[l](82.5,125){$\nameslang$}
\rput[l](272.5,125){$\nameslangg$}
\psline[linewidth=0.75](77.5,90)(77.5,72.5)
\psline[linewidth=0.75](50,80)(70,80)
\psline[linewidth=0.75](87.5,62.5)(67.5,62.5)
\psline[linewidth=0.75](70,79.99)(87.5,62.5)
\psline[linewidth=0.75](50,80)(67.5,62.5)
\psline[linewidth=0.75](30,40)(30,10)
\rput(68.75,71.25){$\parteval$}
\psline[linewidth=0.75](77.5,62.5)(77.5,55)
\psline[linewidth=0.75](20,20)(20,0)
\psline[linewidth=0.75](20,0)(40,0)
\rput(27.5,5){\program}
\psline[linewidth=0.75](20,20)(40,0)
\psline[linewidth=0.75](125,115)(125,90)
\psline[linewidth=0.75](57.5,52.5)(57.5,0)
\psline[linewidth=0.75,border=1.35](62.5,40)(30,40)
\psline[linewidth=0.75](77.5,55)(62.5,40)
\newrgbcolor{userFillColour}{0.2 0 0.2}
\rput{0}(30,40){\psellipse[fillcolor=userFillColour,fillstyle=solid](0,0)(2.68,-2.5)}
\psline[linewidth=0.75](250,55)(250,70)
\psline[linewidth=0.75](220,90)(315,90)
\psline[linewidth=0.75](310,90)(310,0)
\psline[linewidth=0.75](225,90)(225,72.5)
\psline[linewidth=0.75](220,115)(220,90)
\psline[linewidth=0.75](197.5,80)(217.5,80)
\psline[linewidth=0.75](235,62.5)(215,62.5)
\psline[linewidth=0.75](217.5,80)(235,62.51)
\psline[linewidth=0.75](197.5,80)(215,62.5)
\psline[linewidth=0.75](247.5,52.5)(227.5,52.5)
\psline[linewidth=0.75](205,55)(220,40)
\psline[linewidth=0.75](205,72.5)(205,55)
\psline[linewidth=0.75](250,55)(247.5,52.5)
\psline[linewidth=0.75](225,55.01)(227.5,52.5)
\rput(216.25,71.25){$\parteval$}
\psline[linewidth=0.75](225,62.5)(225,55)
\newrgbcolor{userLineColour}{0.6 0.6 0.6}
\newrgbcolor{userFillColour}{0.6 0.6 0.6}
\psline[linewidth=0.75](220,115)(315,115)
\psline[linewidth=0.75](267.5,126.88)(267.5,115)
\psline[linewidth=0.75](267.5,90)(267.5,72.5)
\psline[linewidth=0.75](240,80)(260,80)
\psline[linewidth=0.75](277.5,62.5)(257.5,62.5)
\psline[linewidth=0.75](260,79.99)(277.5,62.5)
\psline[linewidth=0.75](240,80)(257.5,62.5)
\psline[linewidth=0.75](252.5,40)(252.5,0)
\rput(258.75,71.25){$\parteval$}
\psline[linewidth=0.75](267.5,62.5)(267.5,55)
\psline[linewidth=0.75](217.5,20)(217.5,0)
\psline[linewidth=0.75](217.5,0)(237.5,0)
\psline[linewidth=0.75](315,115)(315,90)
\psline[linewidth=0.75](252.5,40)(220,40)
\psline[linewidth=0.75,border=1.35](227.5,52.5)(227.5,10)
\psline[linewidth=0.75](267.5,55)(252.5,40)
\newrgbcolor{userFillColour}{0.2 0 0.2}
\rput{0}(252.5,40){\psellipse[fillcolor=userFillColour,fillstyle=solid](0,0)(2.68,-2.5)}
\pspolygon[](192.5,120)(320,120)(320,30)(192.5,30)
\pspolygon[](2.5,120)(130,120)(130,30)(2.5,30)
\rput(290,50){$\heehat$}
\rput(100,50){$\geehat$}
\psline[linewidth=0.75](217.5,20)(237.5,0)
\newrgbcolor{userFillColour}{0.2 0 0.2}
\rput{0}(227.5,52.5){\psellipse[fillcolor=userFillColour,fillstyle=solid](0,0)(2.68,-2.5)}
\end{pspicture}


==> PIC/smullyan-3.tex <==
%%Created by jPicEdt 1.4.1_03: mixed JPIC-XML/LaTeX format
%%Wed Dec 11 22:09:32 GMT-10:00 2019
%%Begin JPIC-XML
%<?xml version="1.0" standalone="yes"?>
%<jpic x-min="3.75" x-max="470" y-min="0" y-max="127.5" auto-bounding="true">
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(117.5,2.5)"
%	 text-frame= "noframe"
%	 stroke-width= "0.75"
%	 text-hor-align= "right"
%	 >
%$\inputt$
%</text>
%<multicurve fill-style= "none"
%	 points= "(30,90);(30,90);(125,90);(125,90)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(120,90);(120,90);(120,0);(120,0)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(35,90);(35,90);(35,72.5);(35,72.5)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(30,115);(30,115);(30,90);(30,90)"
%	 stroke-width= "0.75"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(77.5,102.5)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\gee$
%</text>
%<multicurve fill-style= "none"
%	 points= "(7.5,80);(7.5,80);(27.5,80);(27.5,80)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(45,62.5);(45,62.5);(25,62.5);(25,62.5)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(27.5,80);(27.5,80);(45,62.51);(45,62.51)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(7.5,80);(7.5,80);(25,62.5);(25,62.5)"
%	 stroke-width= "0.75"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(26.25,71.25)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\parteval$
%</text>
%<multicurve fill-style= "none"
%	 points= "(35,62.5);(35,62.5);(35,40);(35,40)"
%	 stroke-width= "0.75"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(210,10)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\prohram$
%</text>
%<parallelogram p3= "(75,127.5)"
%	 fill-style= "solid"
%	 p2= "(75,115)"
%	 fill-color= "#999999"
%	 p1= "(80,115)"
%	 stroke-color= "#999999"
%	 />
%<multicurve fill-style= "none"
%	 points= "(30,115);(30,115);(125,115);(125,115)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(77.5,126.88);(77.5,126.88);(77.5,115);(77.5,115)"
%	 stroke-width= "0.75"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(82.5,125)"
%	 text-frame= "noframe"
%	 stroke-width= "0.75"
%	 text-hor-align= "left"
%	 >
%$\nameslang$
%</text>
%<multicurve fill-style= "none"
%	 points= "(82.5,90);(82.5,90);(82.5,72.5);(82.5,72.5)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(55,80);(55,80);(75,80);(75,80)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(92.5,62.5);(92.5,62.5);(72.5,62.5);(72.5,62.5)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(75,79.99);(75,79.99);(92.5,62.5);(92.5,62.5)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(55,80);(55,80);(72.5,62.5);(72.5,62.5)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(17.5,70);(17.5,70);(17.5,15);(17.5,15)"
%	 stroke-width= "0.75"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(73.75,71.25)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\parteval$
%</text>
%<multicurve fill-style= "none"
%	 points= "(7.5,25);(7.5,25);(7.5,5);(7.5,5)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(7.5,5);(7.5,5);(27.5,5);(27.5,5)"
%	 stroke-width= "0.75"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(15,10)"
%	 text-frame= "noframe"
%	 stroke-width= "0.75"
%	 text-hor-align= "center-h"
%	 >
%\program
%</text>
%<multicurve fill-style= "none"
%	 points= "(7.5,25);(7.5,25);(27.5,5);(27.5,5)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(125,115);(125,115);(125,90);(125,90)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(202.5,25);(202.5,25);(202.5,5);(202.5,5)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(202.5,5);(202.5,5);(222.5,5);(222.5,5)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(202.5,25);(202.5,25);(222.5,5);(222.5,5)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(215,55);(215,55);(215,70);(215,70)"
%	 stroke-width= "0.75"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(272.5,2.5)"
%	 text-frame= "noframe"
%	 stroke-width= "0.75"
%	 text-hor-align= "right"
%	 >
%$\inputt$
%</text>
%<multicurve fill-style= "none"
%	 points= "(185,90);(185,90);(280,90);(280,90)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(275,90);(275,90);(275,0);(275,0)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(190,90);(190,90);(190,72.5);(190,72.5)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(185,115);(185,115);(185,90);(185,90)"
%	 stroke-width= "0.75"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(232.5,102.5)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\gee$
%</text>
%<multicurve fill-style= "none"
%	 points= "(162.5,80);(162.5,80);(182.5,80);(182.5,80)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(200,62.5);(200,62.5);(180,62.5);(180,62.5)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(182.5,80);(182.5,80);(200,62.51);(200,62.51)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(162.5,80);(162.5,80);(180,62.5);(180,62.5)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(212.5,52.5);(212.5,52.5);(192.5,52.5);(192.5,52.5)"
%	 stroke-width= "0.75"
%	 />
%<ellipse p3= "(215.18,50)"
%	 fill-style= "solid"
%	 p2= "(215.18,55)"
%	 fill-color= "#330033"
%	 p1= "(209.82,55)"
%	 closure= "open"
%	 angle-end= "0"
%	 angle-start= "0"
%	 />
%<multicurve fill-style= "none"
%	 points= "(170,55);(170,55);(185,40);(185,40)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(170,72.5);(170,72.5);(170,55);(170,55)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(215,55);(215,55);(212.5,52.5);(212.5,52.5)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(190,55.01);(190,55.01);(192.5,52.5);(192.5,52.5)"
%	 stroke-width= "0.75"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(181.25,71.25)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\parteval$
%</text>
%<multicurve fill-style= "none"
%	 points= "(190,62.5);(190,62.5);(190,55);(190,55)"
%	 stroke-width= "0.75"
%	 />
%<parallelogram p3= "(230,127.5)"
%	 fill-style= "solid"
%	 p2= "(230,115)"
%	 fill-color= "#999999"
%	 p1= "(235,115)"
%	 stroke-color= "#999999"
%	 />
%<multicurve fill-style= "none"
%	 points= "(185,115);(185,115);(280,115);(280,115)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(232.5,126.88);(232.5,126.88);(232.5,115);(232.5,115)"
%	 stroke-width= "0.75"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(237.5,125)"
%	 text-frame= "noframe"
%	 stroke-width= "0.75"
%	 text-hor-align= "left"
%	 >
%$\nameslang$
%</text>
%<multicurve fill-style= "none"
%	 points= "(232.5,90);(232.5,90);(232.5,72.5);(232.5,72.5)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(205,80);(205,80);(225,80);(225,80)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(242.5,62.5);(242.5,62.5);(222.5,62.5);(222.5,62.5)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(225,79.99);(225,79.99);(242.5,62.5);(242.5,62.5)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(205,80);(205,80);(222.5,62.5);(222.5,62.5)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(185,40);(185,40);(185,15);(185,15)"
%	 stroke-width= "0.75"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(223.75,71.25)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\parteval$
%</text>
%<multicurve fill-style= "none"
%	 points= "(232.5,62.5);(232.5,62.5);(232.5,55);(232.5,55)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(175,25);(175,25);(175,5);(175,5)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(175,5);(175,5);(195,5);(195,5)"
%	 stroke-width= "0.75"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(182.5,10)"
%	 text-frame= "noframe"
%	 stroke-width= "0.75"
%	 text-hor-align= "center-h"
%	 >
%\program
%</text>
%<multicurve fill-style= "none"
%	 points= "(175,25);(175,25);(195,5);(195,5)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(280,115);(280,115);(280,90);(280,90)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(212.5,52.5);(212.5,52.5);(212.5,15);(212.5,15)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 stroke-overstrike-width= "1.35"
%	 points= "(217.5,40);(217.5,40);(185,40);(185,40)"
%	 stroke-overstrike= "true"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(232.5,55);(232.5,55);(217.5,40);(217.5,40)"
%	 stroke-width= "0.75"
%	 />
%<ellipse p3= "(187.68,37.5)"
%	 fill-style= "solid"
%	 p2= "(187.68,42.5)"
%	 fill-color= "#330033"
%	 p1= "(182.32,42.5)"
%	 closure= "open"
%	 angle-end= "0"
%	 angle-start= "0"
%	 />
%<parallelogram p3= "(285,30)"
%	 fill-style= "none"
%	 p2= "(285,120)"
%	 p1= "(157.5,120)"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(255,50)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\geehat$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(32.5,35)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\prohram$
%</text>
%<multicurve fill-style= "none"
%	 points= "(25,50);(25,50);(25,30);(25,30)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(25,30);(25,30);(45,30);(45,30)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(25,50);(25,50);(45,30);(45,30)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(65,70);(65,70);(65,40);(65,40)"
%	 stroke-width= "0.75"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(62.5,35)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\prohram$
%</text>
%<multicurve fill-style= "none"
%	 points= "(55,50);(55,50);(55,30);(55,30)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(55,30);(55,30);(75,30);(75,30)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(55,50);(55,50);(75,30);(75,30)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(80,62.5);(80,62.5);(80,15);(80,15)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(70,25);(70,25);(70,5);(70,5)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(70,5);(70,5);(90,5);(90,5)"
%	 stroke-width= "0.75"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(77.5,10)"
%	 text-frame= "noframe"
%	 stroke-width= "0.75"
%	 text-hor-align= "center-h"
%	 >
%\program
%</text>
%<multicurve fill-style= "none"
%	 points= "(70,25);(70,25);(90,5);(90,5)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(30,85);(30,85);(47.5,67.51);(47.5,67.51)"
%	 stroke-color= "#ff0000"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(47.5,67.49);(47.5,67.49);(47.5,0);(47.5,0)"
%	 stroke-color= "#ff0000"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(3.75,85);(3.75,85);(30,85);(30,85)"
%	 stroke-color= "#ff0000"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(3.75,85);(3.75,85);(3.75,0);(3.75,0)"
%	 stroke-color= "#ff0000"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(47.5,0);(47.5,0);(5,0);(5,0)"
%	 stroke-color= "#ff0000"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(78.75,85);(78.75,85);(96.25,67.51);(96.25,67.51)"
%	 stroke-color= "#ff0000"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(96.25,67.49);(96.25,67.49);(96.25,0);(96.25,0)"
%	 stroke-color= "#ff0000"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(52.5,85);(52.5,85);(78.75,85);(78.75,85)"
%	 stroke-color= "#ff0000"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(52.5,85);(52.5,85);(52.5,0);(52.5,0)"
%	 stroke-color= "#ff0000"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(96.25,0);(96.25,0);(53.75,0);(53.75,0)"
%	 stroke-color= "#ff0000"
%	 stroke-width= "0.35"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(140,60)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\EQLS
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(60,10)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\Peeh$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(40,10)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\Peeg$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(382.5,60)"
%	 text-frame= "noframe"
%	 stroke-width= "0.75"
%	 text-hor-align= "center-h"
%	 >
%\EQLS
%</text>
%<multicurve fill-style= "none"
%	 points= "(430,102.5);(430,102.5);(430,72.5);(430,72.5)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(402.5,80);(402.5,80);(422.5,80);(422.5,80)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(440,62.5);(440,62.5);(420,62.5);(420,62.5)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(422.5,80);(422.5,80);(440,62.51);(440,62.51)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(402.5,80);(402.5,80);(420,62.5);(420,62.5)"
%	 stroke-width= "0.75"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(421.25,71.25)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\parteval$
%</text>
%<multicurve fill-style= "none"
%	 points= "(430,62.5);(430,62.5);(430,40);(430,40)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(412.5,70);(412.5,70);(412.5,15);(412.5,15)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(402.5,25);(402.5,25);(402.5,5);(402.5,5)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(402.5,5);(402.5,5);(422.5,5);(422.5,5)"
%	 stroke-width= "0.75"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(410,10)"
%	 text-frame= "noframe"
%	 stroke-width= "0.75"
%	 text-hor-align= "center-h"
%	 >
%\program
%</text>
%<multicurve fill-style= "none"
%	 points= "(402.5,25);(402.5,25);(422.5,5);(422.5,5)"
%	 stroke-width= "0.75"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(427.5,35)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\prohram$
%</text>
%<multicurve fill-style= "none"
%	 points= "(420,50);(420,50);(420,30);(420,30)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(420,30);(420,30);(440,30);(440,30)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(420,50);(420,50);(440,30);(440,30)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(425,85);(425,85);(442.5,67.51);(442.5,67.51)"
%	 stroke-color= "#ff0000"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(442.5,67.49);(442.5,67.49);(442.5,0);(442.5,0)"
%	 stroke-color= "#ff0000"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(398.75,85);(398.75,85);(425,85);(425,85)"
%	 stroke-color= "#ff0000"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(398.75,85);(398.75,85);(398.75,0);(398.75,0)"
%	 stroke-color= "#ff0000"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(442.5,0);(442.5,0);(400,0);(400,0)"
%	 stroke-color= "#ff0000"
%	 stroke-width= "0.35"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(435,10)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\Peeg$
%</text>
%<multicurve fill-style= "none"
%	 points= "(470,92.5);(470,92.5);(470,110);(470,110)"
%	 stroke-width= "0.75"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(455,125.62)"
%	 text-frame= "noframe"
%	 stroke-width= "0.75"
%	 text-hor-align= "left"
%	 >
%$\nameslang$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(458.12,2.5)"
%	 text-frame= "noframe"
%	 stroke-width= "0.75"
%	 text-hor-align= "right"
%	 >
%$\inputt$
%</text>
%<multicurve fill-style= "none"
%	 points= "(440,92.5);(440,92.5);(470,92.5);(470,92.5)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(460,90);(460,90);(460,0.63);(460,0.63)"
%	 stroke-width= "0.75"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(448.12,101.88)"
%	 text-frame= "noframe"
%	 stroke-width= "0.75"
%	 text-hor-align= "center-h"
%	 >
%\universal
%</text>
%<multicurve fill-style= "none"
%	 points= "(422.5,110);(422.5,110);(440,92.5);(440,92.5)"
%	 stroke-width= "0.75"
%	 />
%<parallelogram p3= "(447.5,127.5)"
%	 fill-style= "solid"
%	 p2= "(447.5,110)"
%	 fill-color= "#999999"
%	 p1= "(452.5,110)"
%	 stroke-color= "#999999"
%	 />
%<multicurve fill-style= "none"
%	 points= "(422.5,110);(422.5,110);(470,110);(470,110)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(450,126.88);(450,126.88);(450,110);(450,110)"
%	 stroke-width= "0.75"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(300,60)"
%	 text-frame= "noframe"
%	 stroke-width= "0.75"
%	 text-hor-align= "center-h"
%	 >
%\EQLS
%</text>
%<multicurve fill-style= "none"
%	 points= "(337.5,92.5);(337.5,92.5);(337.5,40);(337.5,40)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(310,110);(310,110);(327.5,92.5);(327.5,92.5)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(320,100);(320,100);(320,15);(320,15)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(310,25);(310,25);(310,5);(310,5)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(310,5);(310,5);(330,5);(330,5)"
%	 stroke-width= "0.75"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(317.5,10)"
%	 text-frame= "noframe"
%	 stroke-width= "0.75"
%	 text-hor-align= "center-h"
%	 >
%\program
%</text>
%<multicurve fill-style= "none"
%	 points= "(310,25);(310,25);(330,5);(330,5)"
%	 stroke-width= "0.75"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(335,35)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\prohram$
%</text>
%<multicurve fill-style= "none"
%	 points= "(327.5,50);(327.5,50);(327.5,30);(327.5,30)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(327.5,30);(327.5,30);(347.5,30);(347.5,30)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(327.5,50);(327.5,50);(347.5,30);(347.5,30)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(377.5,92.5);(377.5,92.5);(377.5,110);(377.5,110)"
%	 stroke-width= "0.75"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(360,125.62)"
%	 text-frame= "noframe"
%	 stroke-width= "0.75"
%	 text-hor-align= "left"
%	 >
%$\nameslang$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(365.62,2.5)"
%	 text-frame= "noframe"
%	 stroke-width= "0.75"
%	 text-hor-align= "right"
%	 >
%$\inputt$
%</text>
%<multicurve fill-style= "none"
%	 points= "(327.5,92.5);(327.5,92.5);(377.5,92.5);(377.5,92.5)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(367.5,92.5);(367.5,92.5);(367.5,0.63);(367.5,0.63)"
%	 stroke-width= "0.75"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(350,101.25)"
%	 text-frame= "noframe"
%	 stroke-width= "0.75"
%	 text-hor-align= "center-h"
%	 >
%\universal
%</text>
%<parallelogram p3= "(352.5,127.5)"
%	 fill-style= "solid"
%	 p2= "(352.5,110)"
%	 fill-color= "#999999"
%	 p1= "(357.5,110)"
%	 stroke-color= "#999999"
%	 />
%<multicurve fill-style= "none"
%	 points= "(310,110);(310,110);(377.5,110);(377.5,110)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(355,126.88);(355,126.88);(355,110);(355,110)"
%	 stroke-width= "0.75"
%	 />
%</jpic>
%%End JPIC-XML
%PSTricks content-type (pstricks.sty package needed)
%Add \usepackage{pstricks} in the preamble of your LaTeX file
%You can rescale the whole picture (to 80% for instance) by using the command \def\JPicScale{0.8}
\ifx\JPicScale\undefined\def\JPicScale{1}\fi
\psset{unit=\JPicScale mm}
\psset{linewidth=0.3,dotsep=1,hatchwidth=0.3,hatchsep=1.5,shadowsize=1,dimen=middle}
\psset{dotsize=0.7 2.5,dotscale=1 1,fillcolor=black}
\psset{arrowsize=1 2,arrowlength=1,arrowinset=0.25,tbarsize=0.7 5,bracketlength=0.15,rbracketlength=0.15}
\begin{pspicture}(0,0)(470,127.5)
\rput[r](117.5,2.5){$\inputt$}
\psline[linewidth=0.75](30,90)(125,90)
\psline[linewidth=0.75](120,90)(120,0)
\psline[linewidth=0.75](35,90)(35,72.5)
\psline[linewidth=0.75](30,115)(30,90)
\rput(77.5,102.5){$\gee$}
\psline[linewidth=0.75](7.5,80)(27.5,80)
\psline[linewidth=0.75](45,62.5)(25,62.5)
\psline[linewidth=0.75](27.5,80)(45,62.51)
\psline[linewidth=0.75](7.5,80)(25,62.5)
\rput(26.25,71.25){$\parteval$}
\psline[linewidth=0.75](35,62.5)(35,40)
\rput(210,10){$\prohram$}
\newrgbcolor{userLineColour}{0.6 0.6 0.6}
\newrgbcolor{userFillColour}{0.6 0.6 0.6}
\psline[linewidth=0.75](30,115)(125,115)
\psline[linewidth=0.75](77.5,126.88)(77.5,115)
\rput[l](82.5,125){$\nameslang$}
\psline[linewidth=0.75](82.5,90)(82.5,72.5)
\psline[linewidth=0.75](55,80)(75,80)
\psline[linewidth=0.75](92.5,62.5)(72.5,62.5)
\psline[linewidth=0.75](75,79.99)(92.5,62.5)
\psline[linewidth=0.75](55,80)(72.5,62.5)
\psline[linewidth=0.75](17.5,70)(17.5,15)
\rput(73.75,71.25){$\parteval$}
\psline[linewidth=0.75](7.5,25)(7.5,5)
\psline[linewidth=0.75](7.5,5)(27.5,5)
\rput(15,10){\program}
\psline[linewidth=0.75](7.5,25)(27.5,5)
\psline[linewidth=0.75](125,115)(125,90)
\psline[linewidth=0.75](202.5,25)(202.5,5)
\psline[linewidth=0.75](202.5,5)(222.5,5)
\psline[linewidth=0.75](202.5,25)(222.5,5)
\psline[linewidth=0.75](215,55)(215,70)
\rput[r](272.5,2.5){$\inputt$}
\psline[linewidth=0.75](185,90)(280,90)
\psline[linewidth=0.75](275,90)(275,0)
\psline[linewidth=0.75](190,90)(190,72.5)
\psline[linewidth=0.75](185,115)(185,90)
\rput(232.5,102.5){$\gee$}
\psline[linewidth=0.75](162.5,80)(182.5,80)
\psline[linewidth=0.75](200,62.5)(180,62.5)
\psline[linewidth=0.75](182.5,80)(200,62.51)
\psline[linewidth=0.75](162.5,80)(180,62.5)
\psline[linewidth=0.75](212.5,52.5)(192.5,52.5)
\newrgbcolor{userFillColour}{0.2 0 0.2}
\rput{0}(212.5,52.5){\psellipse[fillcolor=userFillColour,fillstyle=solid](0,0)(2.68,-2.5)}
\psline[linewidth=0.75](170,55)(185,40)
\psline[linewidth=0.75](170,72.5)(170,55)
\psline[linewidth=0.75](215,55)(212.5,52.5)
\psline[linewidth=0.75](190,55.01)(192.5,52.5)
\rput(181.25,71.25){$\parteval$}
\psline[linewidth=0.75](190,62.5)(190,55)
\newrgbcolor{userLineColour}{0.6 0.6 0.6}
\newrgbcolor{userFillColour}{0.6 0.6 0.6}
\psline[linewidth=0.75](185,115)(280,115)
\psline[linewidth=0.75](232.5,126.88)(232.5,115)
\rput[l](237.5,125){$\nameslang$}
\psline[linewidth=0.75](232.5,90)(232.5,72.5)
\psline[linewidth=0.75](205,80)(225,80)
\psline[linewidth=0.75](242.5,62.5)(222.5,62.5)
\psline[linewidth=0.75](225,79.99)(242.5,62.5)
\psline[linewidth=0.75](205,80)(222.5,62.5)
\psline[linewidth=0.75](185,40)(185,15)
\rput(223.75,71.25){$\parteval$}
\psline[linewidth=0.75](232.5,62.5)(232.5,55)
\psline[linewidth=0.75](175,25)(175,5)
\psline[linewidth=0.75](175,5)(195,5)
\rput(182.5,10){\program}
\psline[linewidth=0.75](175,25)(195,5)
\psline[linewidth=0.75](280,115)(280,90)
\psline[linewidth=0.75](212.5,52.5)(212.5,15)
\psline[linewidth=0.75,border=1.35](217.5,40)(185,40)
\psline[linewidth=0.75](232.5,55)(217.5,40)
\newrgbcolor{userFillColour}{0.2 0 0.2}
\rput{0}(185,40){\psellipse[fillcolor=userFillColour,fillstyle=solid](0,0)(2.68,-2.5)}
\pspolygon[](157.5,120)(285,120)(285,30)(157.5,30)
\rput(255,50){$\geehat$}
\rput(32.5,35){$\prohram$}
\psline[linewidth=0.75](25,50)(25,30)
\psline[linewidth=0.75](25,30)(45,30)
\psline[linewidth=0.75](25,50)(45,30)
\psline[linewidth=0.75](65,70)(65,40)
\rput(62.5,35){$\prohram$}
\psline[linewidth=0.75](55,50)(55,30)
\psline[linewidth=0.75](55,30)(75,30)
\psline[linewidth=0.75](55,50)(75,30)
\psline[linewidth=0.75](80,62.5)(80,15)
\psline[linewidth=0.75](70,25)(70,5)
\psline[linewidth=0.75](70,5)(90,5)
\rput(77.5,10){\program}
\psline[linewidth=0.75](70,25)(90,5)
\psline[linewidth=0.35,linecolor=red](30,85)(47.5,67.51)
\psline[linewidth=0.35,linecolor=red](47.5,67.49)(47.5,0)
\psline[linewidth=0.35,linecolor=red](3.75,85)(30,85)
\psline[linewidth=0.35,linecolor=red](3.75,85)(3.75,0)
\psline[linewidth=0.35,linecolor=red](47.5,0)(5,0)
\psline[linewidth=0.35,linecolor=red](78.75,85)(96.25,67.51)
\psline[linewidth=0.35,linecolor=red](96.25,67.49)(96.25,0)
\psline[linewidth=0.35,linecolor=red](52.5,85)(78.75,85)
\psline[linewidth=0.35,linecolor=red](52.5,85)(52.5,0)
\psline[linewidth=0.35,linecolor=red](96.25,0)(53.75,0)
\rput(140,60){\EQLS}
\rput(60,10){$\Peeh$}
\rput(40,10){$\Peeg$}
\rput(382.5,60){\EQLS}
\psline[linewidth=0.75](430,102.5)(430,72.5)
\psline[linewidth=0.75](402.5,80)(422.5,80)
\psline[linewidth=0.75](440,62.5)(420,62.5)
\psline[linewidth=0.75](422.5,80)(440,62.51)
\psline[linewidth=0.75](402.5,80)(420,62.5)
\rput(421.25,71.25){$\parteval$}
\psline[linewidth=0.75](430,62.5)(430,40)
\psline[linewidth=0.75](412.5,70)(412.5,15)
\psline[linewidth=0.75](402.5,25)(402.5,5)
\psline[linewidth=0.75](402.5,5)(422.5,5)
\rput(410,10){\program}
\psline[linewidth=0.75](402.5,25)(422.5,5)
\rput(427.5,35){$\prohram$}
\psline[linewidth=0.75](420,50)(420,30)
\psline[linewidth=0.75](420,30)(440,30)
\psline[linewidth=0.75](420,50)(440,30)
\psline[linewidth=0.35,linecolor=red](425,85)(442.5,67.51)
\psline[linewidth=0.35,linecolor=red](442.5,67.49)(442.5,0)
\psline[linewidth=0.35,linecolor=red](398.75,85)(425,85)
\psline[linewidth=0.35,linecolor=red](398.75,85)(398.75,0)
\psline[linewidth=0.35,linecolor=red](442.5,0)(400,0)
\rput(435,10){$\Peeg$}
\psline[linewidth=0.75](470,92.5)(470,110)
\rput[l](455,125.62){$\nameslang$}
\rput[r](458.12,2.5){$\inputt$}
\psline[linewidth=0.75](440,92.5)(470,92.5)
\psline[linewidth=0.75](460,90)(460,0.63)
\rput(448.12,101.88){\universal}
\psline[linewidth=0.75](422.5,110)(440,92.5)
\newrgbcolor{userLineColour}{0.6 0.6 0.6}
\newrgbcolor{userFillColour}{0.6 0.6 0.6}
\psline[linewidth=0.75](422.5,110)(470,110)
\psline[linewidth=0.75](450,126.88)(450,110)
\rput(300,60){\EQLS}
\psline[linewidth=0.75](337.5,92.5)(337.5,40)
\psline[linewidth=0.75](310,110)(327.5,92.5)
\psline[linewidth=0.75](320,100)(320,15)
\psline[linewidth=0.75](310,25)(310,5)
\psline[linewidth=0.75](310,5)(330,5)
\rput(317.5,10){\program}
\psline[linewidth=0.75](310,25)(330,5)
\rput(335,35){$\prohram$}
\psline[linewidth=0.75](327.5,50)(327.5,30)
\psline[linewidth=0.75](327.5,30)(347.5,30)
\psline[linewidth=0.75](327.5,50)(347.5,30)
\psline[linewidth=0.75](377.5,92.5)(377.5,110)
\rput[l](360,125.62){$\nameslang$}
\rput[r](365.62,2.5){$\inputt$}
\psline[linewidth=0.75](327.5,92.5)(377.5,92.5)
\psline[linewidth=0.75](367.5,92.5)(367.5,0.63)
\rput(350,101.25){\universal}
\newrgbcolor{userLineColour}{0.6 0.6 0.6}
\newrgbcolor{userFillColour}{0.6 0.6 0.6}
\pspolygon[linecolor=userLineColour,fillcolor=userFillColour,fillstyle=solid](357.5,110)(352.5,110)(352.5,127.5)(357.5,127.5)
\psline[linewidth=0.75](310,110)(377.5,110)
\psline[linewidth=0.75](355,126.88)(355,110)
\end{pspicture}


==> PIC/smullyan-4.tex <==
%%Created by jPicEdt 1.4.1_03: mixed JPIC-XML/LaTeX format
%%Tue Nov 24 19:39:59 GMT-10:00 2020
%%Begin JPIC-XML
%<?xml version="1.0" standalone="yes"?>
%<jpic x-min="3.75" x-max="470" y-min="0" y-max="151.88" auto-bounding="true">
%<text stroke-width= "0.35"
%	 fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(117.5,2.5)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\inputt$
%</text>
%<multicurve stroke-width= "0.35"
%	 fill-style= "none"
%	 points= "(30,90);(30,90);(125,90);(125,90)"
%	 />
%<multicurve stroke-width= "0.35"
%	 fill-style= "none"
%	 points= "(120,90);(120,90);(120,0);(120,0)"
%	 />
%<multicurve stroke-width= "0.35"
%	 fill-style= "none"
%	 points= "(35,90);(35,90);(35,72.5);(35,72.5)"
%	 />
%<multicurve stroke-width= "0.35"
%	 fill-style= "none"
%	 points= "(30,115);(30,115);(30,90);(30,90)"
%	 />
%<text stroke-width= "0.35"
%	 fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(77.5,102.5)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\gee$
%</text>
%<multicurve stroke-width= "0.35"
%	 fill-style= "none"
%	 points= "(7.5,80);(7.5,80);(27.5,80);(27.5,80)"
%	 />
%<multicurve stroke-width= "0.35"
%	 fill-style= "none"
%	 points= "(45,62.5);(45,62.5);(25,62.5);(25,62.5)"
%	 />
%<multicurve stroke-width= "0.35"
%	 fill-style= "none"
%	 points= "(27.5,80);(27.5,80);(45,62.51);(45,62.51)"
%	 />
%<multicurve stroke-width= "0.35"
%	 fill-style= "none"
%	 points= "(7.5,80);(7.5,80);(25,62.5);(25,62.5)"
%	 />
%<text stroke-width= "0.35"
%	 fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(26.25,71.25)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\parteval$
%</text>
%<multicurve stroke-width= "0.35"
%	 fill-style= "none"
%	 points= "(35,62.5);(35,62.5);(35,40);(35,40)"
%	 />
%<text stroke-width= "0.35"
%	 fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(210,10)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\prohram$
%</text>
%<multicurve stroke-width= "0.35"
%	 fill-style= "none"
%	 points= "(30,115);(30,115);(125,115);(125,115)"
%	 />
%<multicurve stroke-width= "0.35"
%	 fill-style= "none"
%	 points= "(77.5,126.88);(77.5,126.88);(77.5,115);(77.5,115)"
%	 />
%<text stroke-width= "0.35"
%	 fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(82.5,125)"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\nameslang$
%</text>
%<multicurve stroke-width= "0.35"
%	 fill-style= "none"
%	 points= "(82.5,90);(82.5,90);(82.5,72.5);(82.5,72.5)"
%	 />
%<multicurve stroke-width= "0.35"
%	 fill-style= "none"
%	 points= "(55,80);(55,80);(75,80);(75,80)"
%	 />
%<multicurve stroke-width= "0.35"
%	 fill-style= "none"
%	 points= "(92.5,62.5);(92.5,62.5);(72.5,62.5);(72.5,62.5)"
%	 />
%<multicurve stroke-width= "0.35"
%	 fill-style= "none"
%	 points= "(75,79.99);(75,79.99);(92.5,62.5);(92.5,62.5)"
%	 />
%<multicurve stroke-width= "0.35"
%	 fill-style= "none"
%	 points= "(55,80);(55,80);(72.5,62.5);(72.5,62.5)"
%	 />
%<multicurve stroke-width= "0.35"
%	 fill-style= "none"
%	 points= "(17.5,70);(17.5,70);(17.5,15);(17.5,15)"
%	 />
%<text stroke-width= "0.35"
%	 fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(73.75,71.25)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\parteval$
%</text>
%<multicurve stroke-width= "0.35"
%	 fill-style= "none"
%	 points= "(7.5,25);(7.5,25);(7.5,5);(7.5,5)"
%	 />
%<multicurve stroke-width= "0.35"
%	 fill-style= "none"
%	 points= "(7.5,5);(7.5,5);(27.5,5);(27.5,5)"
%	 />
%<text stroke-width= "0.35"
%	 fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(15,10)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\program
%</text>
%<multicurve stroke-width= "0.35"
%	 fill-style= "none"
%	 points= "(7.5,25);(7.5,25);(27.5,5);(27.5,5)"
%	 />
%<multicurve stroke-width= "0.35"
%	 fill-style= "none"
%	 points= "(125,115);(125,115);(125,90);(125,90)"
%	 />
%<multicurve stroke-width= "0.35"
%	 fill-style= "none"
%	 points= "(202.5,25);(202.5,25);(202.5,5);(202.5,5)"
%	 />
%<multicurve stroke-width= "0.35"
%	 fill-style= "none"
%	 points= "(202.5,5);(202.5,5);(222.5,5);(222.5,5)"
%	 />
%<multicurve stroke-width= "0.35"
%	 fill-style= "none"
%	 points= "(202.5,25);(202.5,25);(222.5,5);(222.5,5)"
%	 />
%<multicurve stroke-width= "0.35"
%	 fill-style= "none"
%	 points= "(215,55);(215,55);(215,70);(215,70)"
%	 />
%<text stroke-width= "0.35"
%	 fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(272.5,2.5)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\inputt$
%</text>
%<multicurve stroke-width= "0.35"
%	 fill-style= "none"
%	 points= "(185,90);(185,90);(280,90);(280,90)"
%	 />
%<multicurve stroke-width= "0.35"
%	 fill-style= "none"
%	 points= "(275,90);(275,90);(275,0);(275,0)"
%	 />
%<multicurve stroke-width= "0.35"
%	 fill-style= "none"
%	 points= "(190,90);(190,90);(190,72.5);(190,72.5)"
%	 />
%<multicurve stroke-width= "0.35"
%	 fill-style= "none"
%	 points= "(185,115);(185,115);(185,90);(185,90)"
%	 />
%<text stroke-width= "0.35"
%	 fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(232.5,102.5)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\gee$
%</text>
%<multicurve stroke-width= "0.35"
%	 fill-style= "none"
%	 points= "(162.5,80);(162.5,80);(182.5,80);(182.5,80)"
%	 />
%<multicurve stroke-width= "0.35"
%	 fill-style= "none"
%	 points= "(200,62.5);(200,62.5);(180,62.5);(180,62.5)"
%	 />
%<multicurve stroke-width= "0.35"
%	 fill-style= "none"
%	 points= "(182.5,80);(182.5,80);(200,62.51);(200,62.51)"
%	 />
%<multicurve stroke-width= "0.35"
%	 fill-style= "none"
%	 points= "(162.5,80);(162.5,80);(180,62.5);(180,62.5)"
%	 />
%<multicurve stroke-width= "0.35"
%	 fill-style= "none"
%	 points= "(212.5,52.5);(212.5,52.5);(192.5,52.5);(192.5,52.5)"
%	 />
%<multicurve stroke-width= "0.35"
%	 fill-style= "none"
%	 points= "(170,55);(170,55);(185,40);(185,40)"
%	 />
%<multicurve stroke-width= "0.35"
%	 fill-style= "none"
%	 points= "(170,72.5);(170,72.5);(170,55);(170,55)"
%	 />
%<multicurve stroke-width= "0.35"
%	 fill-style= "none"
%	 points= "(215,55);(215,55);(212.5,52.5);(212.5,52.5)"
%	 />
%<multicurve stroke-width= "0.35"
%	 fill-style= "none"
%	 points= "(190,55.01);(190,55.01);(192.5,52.5);(192.5,52.5)"
%	 />
%<text stroke-width= "0.35"
%	 fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(181.25,71.25)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\parteval$
%</text>
%<multicurve stroke-width= "0.35"
%	 fill-style= "none"
%	 points= "(190,62.5);(190,62.5);(190,55);(190,55)"
%	 />
%<multicurve stroke-width= "0.35"
%	 fill-style= "none"
%	 points= "(185,115);(185,115);(280,115);(280,115)"
%	 />
%<multicurve stroke-width= "0.35"
%	 fill-style= "none"
%	 points= "(232.5,126.88);(232.5,126.88);(232.5,115);(232.5,115)"
%	 />
%<text stroke-width= "0.35"
%	 fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(237.5,125)"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\nameslang$
%</text>
%<multicurve stroke-width= "0.35"
%	 fill-style= "none"
%	 points= "(232.5,90);(232.5,90);(232.5,72.5);(232.5,72.5)"
%	 />
%<multicurve stroke-width= "0.35"
%	 fill-style= "none"
%	 points= "(205,80);(205,80);(225,80);(225,80)"
%	 />
%<multicurve stroke-width= "0.35"
%	 fill-style= "none"
%	 points= "(242.5,62.5);(242.5,62.5);(222.5,62.5);(222.5,62.5)"
%	 />
%<multicurve stroke-width= "0.35"
%	 fill-style= "none"
%	 points= "(225,79.99);(225,79.99);(242.5,62.5);(242.5,62.5)"
%	 />
%<multicurve stroke-width= "0.35"
%	 fill-style= "none"
%	 points= "(205,80);(205,80);(222.5,62.5);(222.5,62.5)"
%	 />
%<multicurve stroke-width= "0.35"
%	 fill-style= "none"
%	 points= "(185,40);(185,40);(185,15);(185,15)"
%	 />
%<text stroke-width= "0.35"
%	 fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(223.75,71.25)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\parteval$
%</text>
%<multicurve stroke-width= "0.35"
%	 fill-style= "none"
%	 points= "(232.5,62.5);(232.5,62.5);(232.5,55);(232.5,55)"
%	 />
%<multicurve stroke-width= "0.35"
%	 fill-style= "none"
%	 points= "(175,25);(175,25);(175,5);(175,5)"
%	 />
%<multicurve stroke-width= "0.35"
%	 fill-style= "none"
%	 points= "(175,5);(175,5);(195,5);(195,5)"
%	 />
%<text stroke-width= "0.35"
%	 fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(182.5,10)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\program
%</text>
%<multicurve stroke-width= "0.35"
%	 fill-style= "none"
%	 points= "(175,25);(175,25);(195,5);(195,5)"
%	 />
%<multicurve stroke-width= "0.35"
%	 fill-style= "none"
%	 points= "(280,115);(280,115);(280,90);(280,90)"
%	 />
%<multicurve stroke-width= "0.35"
%	 fill-style= "none"
%	 points= "(212.5,52.5);(212.5,52.5);(212.5,15);(212.5,15)"
%	 />
%<multicurve stroke-width= "0.35"
%	 fill-style= "none"
%	 points= "(217.5,40);(217.5,40);(185,40);(185,40)"
%	 />
%<multicurve stroke-width= "0.35"
%	 fill-style= "none"
%	 points= "(232.5,55);(232.5,55);(217.5,40);(217.5,40)"
%	 />
%<parallelogram stroke-width= "0.35"
%	 fill-style= "none"
%	 p3= "(285,30)"
%	 p2= "(285,120)"
%	 p1= "(157.5,120)"
%	 />
%<text stroke-width= "0.35"
%	 fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(255,50)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\geehat$
%</text>
%<text stroke-width= "0.35"
%	 fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(32.5,35)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\prohram$
%</text>
%<multicurve stroke-width= "0.35"
%	 fill-style= "none"
%	 points= "(25,50);(25,50);(25,30);(25,30)"
%	 />
%<multicurve stroke-width= "0.35"
%	 fill-style= "none"
%	 points= "(25,30);(25,30);(45,30);(45,30)"
%	 />
%<multicurve stroke-width= "0.35"
%	 fill-style= "none"
%	 points= "(25,50);(25,50);(45,30);(45,30)"
%	 />
%<multicurve stroke-width= "0.35"
%	 fill-style= "none"
%	 points= "(65,70);(65,70);(65,40);(65,40)"
%	 />
%<text stroke-width= "0.35"
%	 fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(62.5,35)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\prohram$
%</text>
%<multicurve stroke-width= "0.35"
%	 fill-style= "none"
%	 points= "(55,50);(55,50);(55,30);(55,30)"
%	 />
%<multicurve stroke-width= "0.35"
%	 fill-style= "none"
%	 points= "(55,30);(55,30);(75,30);(75,30)"
%	 />
%<multicurve stroke-width= "0.35"
%	 fill-style= "none"
%	 points= "(55,50);(55,50);(75,30);(75,30)"
%	 />
%<multicurve stroke-width= "0.35"
%	 fill-style= "none"
%	 points= "(80,62.5);(80,62.5);(80,15);(80,15)"
%	 />
%<multicurve stroke-width= "0.35"
%	 fill-style= "none"
%	 points= "(70,25);(70,25);(70,5);(70,5)"
%	 />
%<multicurve stroke-width= "0.35"
%	 fill-style= "none"
%	 points= "(70,5);(70,5);(90,5);(90,5)"
%	 />
%<text stroke-width= "0.35"
%	 fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(77.5,10)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\program
%</text>
%<multicurve stroke-width= "0.35"
%	 fill-style= "none"
%	 points= "(70,25);(70,25);(90,5);(90,5)"
%	 />
%<multicurve stroke-width= "0.35"
%	 fill-style= "none"
%	 stroke-color= "#ff0000"
%	 points= "(30,85);(30,85);(47.5,67.51);(47.5,67.51)"
%	 />
%<multicurve stroke-width= "0.35"
%	 fill-style= "none"
%	 stroke-color= "#ff0000"
%	 points= "(47.5,67.49);(47.5,67.49);(47.5,0);(47.5,0)"
%	 />
%<multicurve stroke-width= "0.35"
%	 fill-style= "none"
%	 stroke-color= "#ff0000"
%	 points= "(3.75,85);(3.75,85);(30,85);(30,85)"
%	 />
%<multicurve stroke-width= "0.35"
%	 fill-style= "none"
%	 stroke-color= "#ff0000"
%	 points= "(3.75,85);(3.75,85);(3.75,0);(3.75,0)"
%	 />
%<multicurve stroke-width= "0.35"
%	 fill-style= "none"
%	 stroke-color= "#ff0000"
%	 points= "(47.5,0);(47.5,0);(5,0);(5,0)"
%	 />
%<multicurve stroke-width= "0.35"
%	 fill-style= "none"
%	 stroke-color= "#ff0000"
%	 points= "(78.75,85);(78.75,85);(96.25,67.51);(96.25,67.51)"
%	 />
%<multicurve stroke-width= "0.35"
%	 fill-style= "none"
%	 stroke-color= "#ff0000"
%	 points= "(96.25,67.49);(96.25,67.49);(96.25,0);(96.25,0)"
%	 />
%<multicurve stroke-width= "0.35"
%	 fill-style= "none"
%	 stroke-color= "#ff0000"
%	 points= "(52.5,85);(52.5,85);(78.75,85);(78.75,85)"
%	 />
%<multicurve stroke-width= "0.35"
%	 fill-style= "none"
%	 stroke-color= "#ff0000"
%	 points= "(52.5,85);(52.5,85);(52.5,0);(52.5,0)"
%	 />
%<multicurve stroke-width= "0.35"
%	 fill-style= "none"
%	 stroke-color= "#ff0000"
%	 points= "(96.25,0);(96.25,0);(53.75,0);(53.75,0)"
%	 />
%<text stroke-width= "0.35"
%	 fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(140,60)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\EQLS
%</text>
%<text stroke-width= "0.35"
%	 fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(60,10)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\Peeh$
%</text>
%<text stroke-width= "0.35"
%	 fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(40,10)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\Peeg$
%</text>
%<text stroke-width= "0.35"
%	 fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(382.5,60)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\EQLS
%</text>
%<multicurve stroke-width= "0.35"
%	 fill-style= "none"
%	 points= "(430,102.5);(430,102.5);(430,72.5);(430,72.5)"
%	 />
%<multicurve stroke-width= "0.35"
%	 fill-style= "none"
%	 points= "(402.5,80);(402.5,80);(402.5,100);(402.5,100)"
%	 />
%<multicurve stroke-width= "0.35"
%	 fill-style= "none"
%	 points= "(440,62.5);(440,62.5);(420,62.5);(420,62.5)"
%	 />
%<multicurve stroke-width= "0.35"
%	 fill-style= "none"
%	 points= "(402.5,100);(402.5,100);(440,62.51);(440,62.51)"
%	 />
%<multicurve stroke-width= "0.35"
%	 fill-style= "none"
%	 points= "(402.5,80);(402.5,80);(420,62.5);(420,62.5)"
%	 />
%<text stroke-width= "0.35"
%	 fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(416.25,76.25)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\parteval$
%</text>
%<multicurve stroke-width= "0.35"
%	 fill-style= "none"
%	 points= "(430,62.5);(430,62.5);(430,40);(430,40)"
%	 />
%<multicurve stroke-width= "0.35"
%	 fill-style= "none"
%	 points= "(412.5,70);(412.5,70);(412.5,15);(412.5,15)"
%	 />
%<multicurve stroke-width= "0.35"
%	 fill-style= "none"
%	 points= "(402.5,25);(402.5,25);(402.5,5);(402.5,5)"
%	 />
%<multicurve stroke-width= "0.35"
%	 fill-style= "none"
%	 points= "(402.5,5);(402.5,5);(422.5,5);(422.5,5)"
%	 />
%<text stroke-width= "0.35"
%	 fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(410,10)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\program
%</text>
%<multicurve stroke-width= "0.35"
%	 fill-style= "none"
%	 points= "(402.5,25);(402.5,25);(422.5,5);(422.5,5)"
%	 />
%<text stroke-width= "0.35"
%	 fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(427.5,35)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\prohram$
%</text>
%<multicurve stroke-width= "0.35"
%	 fill-style= "none"
%	 points= "(420,50);(420,50);(420,30);(420,30)"
%	 />
%<multicurve stroke-width= "0.35"
%	 fill-style= "none"
%	 points= "(420,30);(420,30);(440,30);(440,30)"
%	 />
%<multicurve stroke-width= "0.35"
%	 fill-style= "none"
%	 points= "(420,50);(420,50);(440,30);(440,30)"
%	 />
%<multicurve stroke-width= "0.35"
%	 fill-style= "none"
%	 stroke-color= "#ff0000"
%	 points= "(405,105);(405,105);(442.5,67.51);(442.5,67.51)"
%	 />
%<multicurve stroke-width= "0.35"
%	 fill-style= "none"
%	 stroke-color= "#ff0000"
%	 points= "(442.5,67.49);(442.5,67.49);(442.5,0);(442.5,0)"
%	 />
%<multicurve stroke-width= "0.35"
%	 fill-style= "none"
%	 stroke-color= "#ff0000"
%	 points= "(398.75,105);(398.75,105);(398.75,0);(398.75,0)"
%	 />
%<multicurve stroke-width= "0.35"
%	 fill-style= "none"
%	 stroke-color= "#ff0000"
%	 points= "(442.5,0);(442.5,0);(400,0);(400,0)"
%	 />
%<text stroke-width= "0.35"
%	 fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(435,10)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\Peeg$
%</text>
%<multicurve stroke-width= "0.35"
%	 fill-style= "none"
%	 points= "(470,92.5);(470,92.5);(470,135);(470,135)"
%	 />
%<text stroke-width= "0.35"
%	 fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(455,150.62)"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\nameslang$
%</text>
%<text stroke-width= "0.35"
%	 fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(458.12,2.5)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\inputt$
%</text>
%<multicurve stroke-width= "0.35"
%	 fill-style= "none"
%	 points= "(440,92.5);(440,92.5);(470,92.5);(470,92.5)"
%	 />
%<multicurve stroke-width= "0.35"
%	 fill-style= "none"
%	 points= "(460,92.5);(460,92.5);(460,0.63);(460,0.63)"
%	 />
%<text stroke-width= "0.35"
%	 fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(445,115)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\universal
%</text>
%<multicurve stroke-width= "0.35"
%	 fill-style= "none"
%	 points= "(402.5,130);(402.5,130);(440,92.5);(440,92.5)"
%	 />
%<multicurve stroke-width= "0.35"
%	 fill-style= "none"
%	 points= "(402.5,135);(402.5,135);(470,135);(470,135)"
%	 />
%<multicurve stroke-width= "0.35"
%	 fill-style= "none"
%	 points= "(450,151.88);(450,151.88);(450,135);(450,135)"
%	 />
%<text stroke-width= "0.35"
%	 fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(300,60)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\EQLS
%</text>
%<multicurve stroke-width= "0.35"
%	 fill-style= "none"
%	 points= "(337.5,92.5);(337.5,92.5);(337.5,40);(337.5,40)"
%	 />
%<multicurve stroke-width= "0.35"
%	 fill-style= "none"
%	 points= "(310,110);(310,110);(327.5,92.5);(327.5,92.5)"
%	 />
%<multicurve stroke-width= "0.35"
%	 fill-style= "none"
%	 points= "(320,100);(320,100);(320,15);(320,15)"
%	 />
%<multicurve stroke-width= "0.35"
%	 fill-style= "none"
%	 points= "(310,25);(310,25);(310,5);(310,5)"
%	 />
%<multicurve stroke-width= "0.35"
%	 fill-style= "none"
%	 points= "(310,5);(310,5);(330,5);(330,5)"
%	 />
%<text stroke-width= "0.35"
%	 fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(317.5,10)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\program
%</text>
%<multicurve stroke-width= "0.35"
%	 fill-style= "none"
%	 points= "(310,25);(310,25);(330,5);(330,5)"
%	 />
%<text stroke-width= "0.35"
%	 fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(335,35)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\prohram$
%</text>
%<multicurve stroke-width= "0.35"
%	 fill-style= "none"
%	 points= "(327.5,50);(327.5,50);(327.5,30);(327.5,30)"
%	 />
%<multicurve stroke-width= "0.35"
%	 fill-style= "none"
%	 points= "(327.5,30);(327.5,30);(347.5,30);(347.5,30)"
%	 />
%<multicurve stroke-width= "0.35"
%	 fill-style= "none"
%	 points= "(327.5,50);(327.5,50);(347.5,30);(347.5,30)"
%	 />
%<multicurve stroke-width= "0.35"
%	 fill-style= "none"
%	 points= "(377.5,92.5);(377.5,92.5);(377.5,110);(377.5,110)"
%	 />
%<text stroke-width= "0.35"
%	 fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(360,125.62)"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\nameslang$
%</text>
%<text stroke-width= "0.35"
%	 fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(365.62,2.5)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\inputt$
%</text>
%<multicurve stroke-width= "0.35"
%	 fill-style= "none"
%	 points= "(327.5,92.5);(327.5,92.5);(377.5,92.5);(377.5,92.5)"
%	 />
%<multicurve stroke-width= "0.35"
%	 fill-style= "none"
%	 points= "(367.5,92.5);(367.5,92.5);(367.5,0.63);(367.5,0.63)"
%	 />
%<text stroke-width= "0.35"
%	 fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(350,101.25)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\universal
%</text>
%<multicurve stroke-width= "0.35"
%	 fill-style= "none"
%	 points= "(310,110);(310,110);(377.5,110);(377.5,110)"
%	 />
%<multicurve stroke-width= "0.35"
%	 fill-style= "none"
%	 points= "(355,126.88);(355,126.88);(355,110);(355,110)"
%	 />
%<multicurve stroke-width= "0.35"
%	 fill-style= "none"
%	 points= "(402.5,130);(402.5,130);(402.5,135);(402.5,135)"
%	 />
%<multicurve stroke-width= "0.35"
%	 fill-style= "none"
%	 stroke-color= "#ff0000"
%	 points= "(405,105);(405,105);(398.75,105);(398.75,105)"
%	 />
%<ellipse stroke-width= "3.85"
%	 fill-style= "solid"
%	 p3= "(188.75,36.25)"
%	 p2= "(188.75,43.75)"
%	 p1= "(181.25,43.75)"
%	 closure= "open"
%	 angle-end= "0"
%	 fill-color= "#333333"
%	 angle-start= "0"
%	 />
%</jpic>
%%End JPIC-XML
%LaTeX-picture environment using emulated lines and arcs
%You can rescale the whole picture (to 80% for instance) by using the command \def\JPicScale{0.8}
\ifx\JPicScale\undefined\def\JPicScale{1}\fi
\unitlength \JPicScale mm
\begin{picture}(470,151.88)(0,0)
\put(117.5,2.5){\makebox(0,0)[cr]{$\inputt$}}

\linethickness{0.35mm}
\put(30,90){\line(1,0){95}}
\linethickness{0.35mm}
\put(120,0){\line(0,1){90}}
\linethickness{0.35mm}
\put(35,72.5){\line(0,1){17.5}}
\linethickness{0.35mm}
\put(30,90){\line(0,1){25}}
\put(77.5,102.5){\makebox(0,0)[cc]{$\gee$}}

\linethickness{0.35mm}
\put(7.5,80){\line(1,0){20}}
\linethickness{0.35mm}
\put(25,62.5){\line(1,0){20}}
\linethickness{0.35mm}
\multiput(27.5,80)(0.12,-0.12){146}{\line(1,0){0.12}}
\linethickness{0.35mm}
\multiput(7.5,80)(0.12,-0.12){146}{\line(1,0){0.12}}
\put(26.25,71.25){\makebox(0,0)[cc]{$\parteval$}}

\linethickness{0.35mm}
\put(35,40){\line(0,1){22.5}}
\put(210,10){\makebox(0,0)[cc]{$\prohram$}}

\linethickness{0.35mm}
\put(30,115){\line(1,0){95}}
\linethickness{0.35mm}
\put(77.5,115){\line(0,1){11.88}}
\put(82.5,125){\makebox(0,0)[cl]{$\nameslang$}}

\linethickness{0.35mm}
\put(82.5,72.5){\line(0,1){17.5}}
\linethickness{0.35mm}
\put(55,80){\line(1,0){20}}
\linethickness{0.35mm}
\put(72.5,62.5){\line(1,0){20}}
\linethickness{0.35mm}
\multiput(75,79.99)(0.12,-0.12){146}{\line(1,0){0.12}}
\linethickness{0.35mm}
\multiput(55,80)(0.12,-0.12){146}{\line(1,0){0.12}}
\linethickness{0.35mm}
\put(17.5,15){\line(0,1){55}}
\put(73.75,71.25){\makebox(0,0)[cc]{$\parteval$}}

\linethickness{0.35mm}
\put(7.5,5){\line(0,1){20}}
\linethickness{0.35mm}
\put(7.5,5){\line(1,0){20}}
\put(15,10){\makebox(0,0)[cc]{\program}}

\linethickness{0.35mm}
\multiput(7.5,25)(0.12,-0.12){167}{\line(1,0){0.12}}
\linethickness{0.35mm}
\put(125,90){\line(0,1){25}}
\linethickness{0.35mm}
\put(202.5,5){\line(0,1){20}}
\linethickness{0.35mm}
\put(202.5,5){\line(1,0){20}}
\linethickness{0.35mm}
\multiput(202.5,25)(0.12,-0.12){167}{\line(1,0){0.12}}
\linethickness{0.35mm}
\put(215,55){\line(0,1){15}}
\put(272.5,2.5){\makebox(0,0)[cr]{$\inputt$}}

\linethickness{0.35mm}
\put(185,90){\line(1,0){95}}
\linethickness{0.35mm}
\put(275,0){\line(0,1){90}}
\linethickness{0.35mm}
\put(190,72.5){\line(0,1){17.5}}
\linethickness{0.35mm}
\put(185,90){\line(0,1){25}}
\put(232.5,102.5){\makebox(0,0)[cc]{$\gee$}}

\linethickness{0.35mm}
\put(162.5,80){\line(1,0){20}}
\linethickness{0.35mm}
\put(180,62.5){\line(1,0){20}}
\linethickness{0.35mm}
\multiput(182.5,80)(0.12,-0.12){146}{\line(1,0){0.12}}
\linethickness{0.35mm}
\multiput(162.5,80)(0.12,-0.12){146}{\line(1,0){0.12}}
\linethickness{0.35mm}
\put(192.5,52.5){\line(1,0){20}}
\linethickness{0.35mm}
\multiput(170,55)(0.12,-0.12){125}{\line(1,0){0.12}}
\linethickness{0.35mm}
\put(170,55){\line(0,1){17.5}}
\linethickness{0.35mm}
\multiput(212.5,52.5)(0.12,0.12){21}{\line(1,0){0.12}}
\linethickness{0.35mm}
\multiput(190,55.01)(0.12,-0.12){21}{\line(0,-1){0.12}}
\put(181.25,71.25){\makebox(0,0)[cc]{$\parteval$}}

\linethickness{0.35mm}
\put(190,55){\line(0,1){7.5}}
\linethickness{0.35mm}
\put(185,115){\line(1,0){95}}
\linethickness{0.35mm}
\put(232.5,115){\line(0,1){11.88}}
\put(237.5,125){\makebox(0,0)[cl]{$\nameslang$}}

\linethickness{0.35mm}
\put(232.5,72.5){\line(0,1){17.5}}
\linethickness{0.35mm}
\put(205,80){\line(1,0){20}}
\linethickness{0.35mm}
\put(222.5,62.5){\line(1,0){20}}
\linethickness{0.35mm}
\multiput(225,79.99)(0.12,-0.12){146}{\line(1,0){0.12}}
\linethickness{0.35mm}
\multiput(205,80)(0.12,-0.12){146}{\line(1,0){0.12}}
\linethickness{0.35mm}
\put(185,15){\line(0,1){25}}
\put(223.75,71.25){\makebox(0,0)[cc]{$\parteval$}}

\linethickness{0.35mm}
\put(232.5,55){\line(0,1){7.5}}
\linethickness{0.35mm}
\put(175,5){\line(0,1){20}}
\linethickness{0.35mm}
\put(175,5){\line(1,0){20}}
\put(182.5,10){\makebox(0,0)[cc]{\program}}

\linethickness{0.35mm}
\multiput(175,25)(0.12,-0.12){167}{\line(1,0){0.12}}
\linethickness{0.35mm}
\put(280,90){\line(0,1){25}}
\linethickness{0.35mm}
\put(212.5,15){\line(0,1){37.5}}
\linethickness{0.35mm}
\put(185,40){\line(1,0){32.5}}
\linethickness{0.35mm}
\multiput(217.5,40)(0.12,0.12){125}{\line(1,0){0.12}}
\linethickness{0.35mm}
\put(157.5,120){\line(1,0){127.5}}
\put(157.5,30){\line(0,1){90}}
\put(285,30){\line(0,1){90}}
\put(157.5,30){\line(1,0){127.5}}
\put(255,50){\makebox(0,0)[cc]{$\geehat$}}

\put(32.5,35){\makebox(0,0)[cc]{$\prohram$}}

\linethickness{0.35mm}
\put(25,30){\line(0,1){20}}
\linethickness{0.35mm}
\put(25,30){\line(1,0){20}}
\linethickness{0.35mm}
\multiput(25,50)(0.12,-0.12){167}{\line(1,0){0.12}}
\linethickness{0.35mm}
\put(65,40){\line(0,1){30}}
\put(62.5,35){\makebox(0,0)[cc]{$\prohram$}}

\linethickness{0.35mm}
\put(55,30){\line(0,1){20}}
\linethickness{0.35mm}
\put(55,30){\line(1,0){20}}
\linethickness{0.35mm}
\multiput(55,50)(0.12,-0.12){167}{\line(1,0){0.12}}
\linethickness{0.35mm}
\put(80,15){\line(0,1){47.5}}
\linethickness{0.35mm}
\put(70,5){\line(0,1){20}}
\linethickness{0.35mm}
\put(70,5){\line(1,0){20}}
\put(77.5,10){\makebox(0,0)[cc]{\program}}

\linethickness{0.35mm}
\multiput(70,25)(0.12,-0.12){167}{\line(1,0){0.12}}
\linethickness{0.35mm}
\multiput(30,85)(0.12,-0.12){146}{\line(1,0){0.12}}
\linethickness{0.35mm}
\put(47.5,0){\line(0,1){67.49}}
\linethickness{0.35mm}
\put(3.75,85){\line(1,0){26.25}}
\linethickness{0.35mm}
\put(3.75,0){\line(0,1){85}}
\linethickness{0.35mm}
\put(5,0){\line(1,0){42.5}}
\linethickness{0.35mm}
\multiput(78.75,85)(0.12,-0.12){146}{\line(1,0){0.12}}
\linethickness{0.35mm}
\put(96.25,0){\line(0,1){67.49}}
\linethickness{0.35mm}
\put(52.5,85){\line(1,0){26.25}}
\linethickness{0.35mm}
\put(52.5,0){\line(0,1){85}}
\linethickness{0.35mm}
\put(53.75,0){\line(1,0){42.5}}
\put(140,60){\makebox(0,0)[cc]{\EQLS}}

\put(60,10){\makebox(0,0)[cc]{$\Peeh$}}

\put(40,10){\makebox(0,0)[cc]{$\Peeg$}}

\put(382.5,60){\makebox(0,0)[cc]{\EQLS}}

\linethickness{0.35mm}
\put(430,72.5){\line(0,1){30}}
\linethickness{0.35mm}
\put(402.5,80){\line(0,1){20}}
\linethickness{0.35mm}
\put(420,62.5){\line(1,0){20}}
\linethickness{0.35mm}
\multiput(402.5,100)(0.12,-0.12){312}{\line(1,0){0.12}}
\linethickness{0.35mm}
\multiput(402.5,80)(0.12,-0.12){146}{\line(1,0){0.12}}
\put(416.25,76.25){\makebox(0,0)[cc]{$\parteval$}}

\linethickness{0.35mm}
\put(430,40){\line(0,1){22.5}}
\linethickness{0.35mm}
\put(412.5,15){\line(0,1){55}}
\linethickness{0.35mm}
\put(402.5,5){\line(0,1){20}}
\linethickness{0.35mm}
\put(402.5,5){\line(1,0){20}}
\put(410,10){\makebox(0,0)[cc]{\program}}

\linethickness{0.35mm}
\multiput(402.5,25)(0.12,-0.12){167}{\line(1,0){0.12}}
\put(427.5,35){\makebox(0,0)[cc]{$\prohram$}}

\linethickness{0.35mm}
\put(420,30){\line(0,1){20}}
\linethickness{0.35mm}
\put(420,30){\line(1,0){20}}
\linethickness{0.35mm}
\multiput(420,50)(0.12,-0.12){167}{\line(1,0){0.12}}
\linethickness{0.35mm}
\multiput(405,105)(0.12,-0.12){312}{\line(1,0){0.12}}
\linethickness{0.35mm}
\put(442.5,0){\line(0,1){67.49}}
\linethickness{0.35mm}
\put(398.75,0){\line(0,1){105}}
\linethickness{0.35mm}
\put(400,0){\line(1,0){42.5}}
\put(435,10){\makebox(0,0)[cc]{$\Peeg$}}

\linethickness{0.35mm}
\put(470,92.5){\line(0,1){42.5}}
\put(455,150.62){\makebox(0,0)[cl]{$\nameslang$}}

\put(458.12,2.5){\makebox(0,0)[cr]{$\inputt$}}

\linethickness{0.35mm}
\put(440,92.5){\line(1,0){30}}
\linethickness{0.35mm}
\put(460,0.63){\line(0,1){91.87}}
\put(445,115){\makebox(0,0)[cc]{\universal}}

\linethickness{0.35mm}
\multiput(402.5,130)(0.12,-0.12){313}{\line(1,0){0.12}}
\linethickness{0.35mm}
\put(402.5,135){\line(1,0){67.5}}
\linethickness{0.35mm}
\put(450,135){\line(0,1){16.88}}
\put(300,60){\makebox(0,0)[cc]{\EQLS}}

\linethickness{0.35mm}
\put(337.5,40){\line(0,1){52.5}}
\linethickness{0.35mm}
\multiput(310,110)(0.12,-0.12){146}{\line(1,0){0.12}}
\linethickness{0.35mm}
\put(320,15){\line(0,1){85}}
\linethickness{0.35mm}
\put(310,5){\line(0,1){20}}
\linethickness{0.35mm}
\put(310,5){\line(1,0){20}}
\put(317.5,10){\makebox(0,0)[cc]{\program}}

\linethickness{0.35mm}
\multiput(310,25)(0.12,-0.12){167}{\line(1,0){0.12}}
\put(335,35){\makebox(0,0)[cc]{$\prohram$}}

\linethickness{0.35mm}
\put(327.5,30){\line(0,1){20}}
\linethickness{0.35mm}
\put(327.5,30){\line(1,0){20}}
\linethickness{0.35mm}
\multiput(327.5,50)(0.12,-0.12){167}{\line(1,0){0.12}}
\linethickness{0.35mm}
\put(377.5,92.5){\line(0,1){17.5}}
\put(360,125.62){\makebox(0,0)[cl]{$\nameslang$}}

\put(365.62,2.5){\makebox(0,0)[cr]{$\inputt$}}

\linethickness{0.35mm}
\put(327.5,92.5){\line(1,0){50}}
\linethickness{0.35mm}
\put(367.5,0.63){\line(0,1){91.87}}
\put(350,101.25){\makebox(0,0)[cc]{\universal}}

\linethickness{0.35mm}
\put(310,110){\line(1,0){67.5}}
\linethickness{0.35mm}
\put(355,110){\line(0,1){16.88}}
\linethickness{0.35mm}
\put(402.5,130){\line(0,1){5}}
\linethickness{0.35mm}
\put(398.75,105){\line(1,0){6.25}}
\linethickness{3.85mm}
\put(185,40){\circle{7.5}}

\end{picture}


==> PIC/smullyan-5.tex <==
%%Created by jPicEdt 1.4.1_03: mixed JPIC-XML/LaTeX format
%%Tue Nov 24 21:38:59 GMT-10:00 2020
%%Begin JPIC-XML
%<?xml version="1.0" standalone="yes"?>
%<jpic x-min="3.75" x-max="470" y-min="0" y-max="126.88" auto-bounding="true">
%<text stroke-width= "0.35"
%	 fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(117.5,2.5)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 stroke-overstrike= "true"
%	 >
%$\inputt$
%</text>
%<multicurve stroke-width= "0.35"
%	 fill-style= "none"
%	 points= "(30,90);(30,90);(125,90);(125,90)"
%	 stroke-overstrike= "true"
%	 />
%<multicurve stroke-width= "0.35"
%	 fill-style= "none"
%	 points= "(120,90);(120,90);(120,0);(120,0)"
%	 stroke-overstrike= "true"
%	 />
%<multicurve stroke-width= "0.35"
%	 fill-style= "none"
%	 points= "(35,90);(35,90);(35,72.5);(35,72.5)"
%	 stroke-overstrike= "true"
%	 />
%<multicurve stroke-width= "0.35"
%	 fill-style= "none"
%	 points= "(30,115);(30,115);(30,90);(30,90)"
%	 stroke-overstrike= "true"
%	 />
%<text stroke-width= "0.35"
%	 fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(77.5,102.5)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 stroke-overstrike= "true"
%	 >
%$\gee$
%</text>
%<multicurve stroke-width= "0.35"
%	 fill-style= "none"
%	 points= "(7.5,80);(7.5,80);(27.5,80);(27.5,80)"
%	 stroke-overstrike= "true"
%	 />
%<multicurve stroke-width= "0.35"
%	 fill-style= "none"
%	 points= "(45,62.5);(45,62.5);(25,62.5);(25,62.5)"
%	 stroke-overstrike= "true"
%	 />
%<multicurve stroke-width= "0.35"
%	 fill-style= "none"
%	 points= "(27.5,80);(27.5,80);(45,62.51);(45,62.51)"
%	 stroke-overstrike= "true"
%	 />
%<multicurve stroke-width= "0.35"
%	 fill-style= "none"
%	 points= "(7.5,80);(7.5,80);(25,62.5);(25,62.5)"
%	 stroke-overstrike= "true"
%	 />
%<text stroke-width= "0.35"
%	 fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(26.25,71.25)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 stroke-overstrike= "true"
%	 >
%$\parteval$
%</text>
%<multicurve stroke-width= "0.35"
%	 fill-style= "none"
%	 points= "(35,62.5);(35,62.5);(35,40);(35,40)"
%	 stroke-overstrike= "true"
%	 />
%<text stroke-width= "0.35"
%	 fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(210,10)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 stroke-overstrike= "true"
%	 >
%$\prohram$
%</text>
%<multicurve stroke-width= "0.35"
%	 fill-style= "none"
%	 points= "(30,115);(30,115);(125,115);(125,115)"
%	 stroke-overstrike= "true"
%	 />
%<multicurve stroke-width= "0.35"
%	 fill-style= "none"
%	 points= "(77.5,126.88);(77.5,126.88);(77.5,115);(77.5,115)"
%	 stroke-overstrike= "true"
%	 />
%<text stroke-width= "0.35"
%	 fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(82.5,125)"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 stroke-overstrike= "true"
%	 >
%$\nameslang$
%</text>
%<multicurve stroke-width= "0.35"
%	 fill-style= "none"
%	 points= "(82.5,90);(82.5,90);(82.5,72.5);(82.5,72.5)"
%	 stroke-overstrike= "true"
%	 />
%<multicurve stroke-width= "0.35"
%	 fill-style= "none"
%	 points= "(55,80);(55,80);(75,80);(75,80)"
%	 stroke-overstrike= "true"
%	 />
%<multicurve stroke-width= "0.35"
%	 fill-style= "none"
%	 points= "(92.5,62.5);(92.5,62.5);(72.5,62.5);(72.5,62.5)"
%	 stroke-overstrike= "true"
%	 />
%<multicurve stroke-width= "0.35"
%	 fill-style= "none"
%	 points= "(75,79.99);(75,79.99);(92.5,62.5);(92.5,62.5)"
%	 stroke-overstrike= "true"
%	 />
%<multicurve stroke-width= "0.35"
%	 fill-style= "none"
%	 points= "(55,80);(55,80);(72.5,62.5);(72.5,62.5)"
%	 stroke-overstrike= "true"
%	 />
%<multicurve stroke-width= "0.35"
%	 fill-style= "none"
%	 points= "(17.5,70);(17.5,70);(17.5,15);(17.5,15)"
%	 stroke-overstrike= "true"
%	 />
%<text stroke-width= "0.35"
%	 fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(73.75,71.25)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 stroke-overstrike= "true"
%	 >
%$\parteval$
%</text>
%<multicurve stroke-width= "0.35"
%	 fill-style= "none"
%	 points= "(7.5,25);(7.5,25);(7.5,5);(7.5,5)"
%	 stroke-overstrike= "true"
%	 />
%<multicurve stroke-width= "0.35"
%	 fill-style= "none"
%	 points= "(7.5,5);(7.5,5);(27.5,5);(27.5,5)"
%	 stroke-overstrike= "true"
%	 />
%<text stroke-width= "0.35"
%	 fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(15,10)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 stroke-overstrike= "true"
%	 >
%\program
%</text>
%<multicurve stroke-width= "0.35"
%	 fill-style= "none"
%	 points= "(7.5,25);(7.5,25);(27.5,5);(27.5,5)"
%	 stroke-overstrike= "true"
%	 />
%<multicurve stroke-width= "0.35"
%	 fill-style= "none"
%	 points= "(125,115);(125,115);(125,90);(125,90)"
%	 stroke-overstrike= "true"
%	 />
%<multicurve stroke-width= "0.35"
%	 fill-style= "none"
%	 points= "(202.5,25);(202.5,25);(202.5,5);(202.5,5)"
%	 stroke-overstrike= "true"
%	 />
%<multicurve stroke-width= "0.35"
%	 fill-style= "none"
%	 points= "(202.5,5);(202.5,5);(222.5,5);(222.5,5)"
%	 stroke-overstrike= "true"
%	 />
%<multicurve stroke-width= "0.35"
%	 fill-style= "none"
%	 points= "(202.5,25);(202.5,25);(222.5,5);(222.5,5)"
%	 stroke-overstrike= "true"
%	 />
%<multicurve stroke-width= "0.35"
%	 fill-style= "none"
%	 points= "(215,55);(215,55);(215,70);(215,70)"
%	 stroke-overstrike= "true"
%	 />
%<text stroke-width= "0.35"
%	 fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(272.5,2.5)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 stroke-overstrike= "true"
%	 >
%$\inputt$
%</text>
%<multicurve stroke-width= "0.35"
%	 fill-style= "none"
%	 points= "(185,90);(185,90);(280,90);(280,90)"
%	 stroke-overstrike= "true"
%	 />
%<multicurve stroke-width= "0.35"
%	 fill-style= "none"
%	 points= "(275,90);(275,90);(275,0);(275,0)"
%	 stroke-overstrike= "true"
%	 />
%<multicurve stroke-width= "0.35"
%	 fill-style= "none"
%	 points= "(190,90);(190,90);(190,72.5);(190,72.5)"
%	 stroke-overstrike= "true"
%	 />
%<multicurve stroke-width= "0.35"
%	 fill-style= "none"
%	 points= "(185,115);(185,115);(185,90);(185,90)"
%	 stroke-overstrike= "true"
%	 />
%<text stroke-width= "0.35"
%	 fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(232.5,102.5)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 stroke-overstrike= "true"
%	 >
%$\gee$
%</text>
%<multicurve stroke-width= "0.35"
%	 fill-style= "none"
%	 points= "(162.5,80);(162.5,80);(182.5,80);(182.5,80)"
%	 stroke-overstrike= "true"
%	 />
%<multicurve stroke-width= "0.35"
%	 fill-style= "none"
%	 points= "(200,62.5);(200,62.5);(180,62.5);(180,62.5)"
%	 stroke-overstrike= "true"
%	 />
%<multicurve stroke-width= "0.35"
%	 fill-style= "none"
%	 points= "(182.5,80);(182.5,80);(200,62.51);(200,62.51)"
%	 stroke-overstrike= "true"
%	 />
%<multicurve stroke-width= "0.35"
%	 fill-style= "none"
%	 points= "(162.5,80);(162.5,80);(180,62.5);(180,62.5)"
%	 stroke-overstrike= "true"
%	 />
%<multicurve stroke-width= "0.35"
%	 fill-style= "none"
%	 points= "(212.5,52.5);(212.5,52.5);(192.5,52.5);(192.5,52.5)"
%	 stroke-overstrike= "true"
%	 />
%<multicurve stroke-width= "0.35"
%	 fill-style= "none"
%	 points= "(170,55);(170,55);(185,40);(185,40)"
%	 stroke-overstrike= "true"
%	 />
%<multicurve stroke-width= "0.35"
%	 fill-style= "none"
%	 points= "(170,72.5);(170,72.5);(170,55);(170,55)"
%	 stroke-overstrike= "true"
%	 />
%<multicurve stroke-width= "0.35"
%	 fill-style= "none"
%	 points= "(215,55);(215,55);(212.5,52.5);(212.5,52.5)"
%	 stroke-overstrike= "true"
%	 />
%<multicurve stroke-width= "0.35"
%	 fill-style= "none"
%	 points= "(190,55.01);(190,55.01);(192.5,52.5);(192.5,52.5)"
%	 stroke-overstrike= "true"
%	 />
%<text stroke-width= "0.35"
%	 fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(181.25,71.25)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 stroke-overstrike= "true"
%	 >
%$\parteval$
%</text>
%<multicurve stroke-width= "0.35"
%	 fill-style= "none"
%	 points= "(190,62.5);(190,62.5);(190,55);(190,55)"
%	 stroke-overstrike= "true"
%	 />
%<multicurve stroke-width= "0.35"
%	 fill-style= "none"
%	 points= "(185,115);(185,115);(280,115);(280,115)"
%	 stroke-overstrike= "true"
%	 />
%<multicurve stroke-width= "0.35"
%	 fill-style= "none"
%	 points= "(232.5,126.88);(232.5,126.88);(232.5,115);(232.5,115)"
%	 stroke-overstrike= "true"
%	 />
%<text stroke-width= "0.35"
%	 fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(237.5,125)"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 stroke-overstrike= "true"
%	 >
%$\nameslang$
%</text>
%<multicurve stroke-width= "0.35"
%	 fill-style= "none"
%	 points= "(232.5,90);(232.5,90);(232.5,72.5);(232.5,72.5)"
%	 stroke-overstrike= "true"
%	 />
%<multicurve stroke-width= "0.35"
%	 fill-style= "none"
%	 points= "(205,80);(205,80);(225,80);(225,80)"
%	 stroke-overstrike= "true"
%	 />
%<multicurve stroke-width= "0.35"
%	 fill-style= "none"
%	 points= "(242.5,62.5);(242.5,62.5);(222.5,62.5);(222.5,62.5)"
%	 stroke-overstrike= "true"
%	 />
%<multicurve stroke-width= "0.35"
%	 fill-style= "none"
%	 points= "(225,79.99);(225,79.99);(242.5,62.5);(242.5,62.5)"
%	 stroke-overstrike= "true"
%	 />
%<multicurve stroke-width= "0.35"
%	 fill-style= "none"
%	 points= "(205,80);(205,80);(222.5,62.5);(222.5,62.5)"
%	 stroke-overstrike= "true"
%	 />
%<multicurve stroke-width= "0.35"
%	 fill-style= "none"
%	 points= "(185,40);(185,40);(185,15);(185,15)"
%	 stroke-overstrike= "true"
%	 />
%<text stroke-width= "0.35"
%	 fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(223.75,71.25)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 stroke-overstrike= "true"
%	 >
%$\parteval$
%</text>
%<multicurve stroke-width= "0.35"
%	 fill-style= "none"
%	 points= "(232.5,62.5);(232.5,62.5);(232.5,55);(232.5,55)"
%	 stroke-overstrike= "true"
%	 />
%<multicurve stroke-width= "0.35"
%	 fill-style= "none"
%	 points= "(175,25);(175,25);(175,5);(175,5)"
%	 stroke-overstrike= "true"
%	 />
%<multicurve stroke-width= "0.35"
%	 fill-style= "none"
%	 points= "(175,5);(175,5);(195,5);(195,5)"
%	 stroke-overstrike= "true"
%	 />
%<text stroke-width= "0.35"
%	 fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(182.5,10)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 stroke-overstrike= "true"
%	 >
%\program
%</text>
%<multicurve stroke-width= "0.35"
%	 fill-style= "none"
%	 points= "(175,25);(175,25);(195,5);(195,5)"
%	 stroke-overstrike= "true"
%	 />
%<multicurve stroke-width= "0.35"
%	 fill-style= "none"
%	 points= "(280,115);(280,115);(280,90);(280,90)"
%	 stroke-overstrike= "true"
%	 />
%<multicurve stroke-width= "0.35"
%	 fill-style= "none"
%	 points= "(212.5,52.5);(212.5,52.5);(212.5,15);(212.5,15)"
%	 stroke-overstrike= "true"
%	 />
%<multicurve stroke-width= "0.35"
%	 fill-style= "none"
%	 stroke-overstrike-width= "1.35"
%	 points= "(217.5,40);(217.5,40);(185,40);(185,40)"
%	 stroke-overstrike= "true"
%	 />
%<multicurve stroke-width= "0.35"
%	 fill-style= "none"
%	 points= "(232.5,55);(232.5,55);(217.5,40);(217.5,40)"
%	 stroke-overstrike= "true"
%	 />
%<ellipse stroke-width= "2"
%	 fill-style= "solid"
%	 p3= "(186.61,38.44)"
%	 p2= "(186.61,41.56)"
%	 p1= "(183.39,41.56)"
%	 closure= "open"
%	 angle-end= "0"
%	 fill-color= "#330033"
%	 angle-start= "0"
%	 stroke-overstrike= "true"
%	 />
%<parallelogram stroke-width= "0.2"
%	 fill-style= "none"
%	 p3= "(285,30)"
%	 p2= "(285,120)"
%	 p1= "(157.5,120)"
%	 />
%<text stroke-width= "0.35"
%	 fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(255,50)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 stroke-overstrike= "true"
%	 >
%$\geehat$
%</text>
%<text stroke-width= "0.35"
%	 fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(32.5,35)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 stroke-overstrike= "true"
%	 >
%$\prohram$
%</text>
%<multicurve stroke-width= "0.35"
%	 fill-style= "none"
%	 points= "(25,50);(25,50);(25,30);(25,30)"
%	 stroke-overstrike= "true"
%	 />
%<multicurve stroke-width= "0.35"
%	 fill-style= "none"
%	 points= "(25,30);(25,30);(45,30);(45,30)"
%	 stroke-overstrike= "true"
%	 />
%<multicurve stroke-width= "0.35"
%	 fill-style= "none"
%	 points= "(25,50);(25,50);(45,30);(45,30)"
%	 stroke-overstrike= "true"
%	 />
%<multicurve stroke-width= "0.35"
%	 fill-style= "none"
%	 points= "(65,70);(65,70);(65,40);(65,40)"
%	 stroke-overstrike= "true"
%	 />
%<text stroke-width= "0.35"
%	 fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(62.5,35)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 stroke-overstrike= "true"
%	 >
%$\prohram$
%</text>
%<multicurve stroke-width= "0.35"
%	 fill-style= "none"
%	 points= "(55,50);(55,50);(55,30);(55,30)"
%	 stroke-overstrike= "true"
%	 />
%<multicurve stroke-width= "0.35"
%	 fill-style= "none"
%	 points= "(55,30);(55,30);(75,30);(75,30)"
%	 stroke-overstrike= "true"
%	 />
%<multicurve stroke-width= "0.35"
%	 fill-style= "none"
%	 points= "(55,50);(55,50);(75,30);(75,30)"
%	 stroke-overstrike= "true"
%	 />
%<multicurve stroke-width= "0.35"
%	 fill-style= "none"
%	 points= "(80,62.5);(80,62.5);(80,15);(80,15)"
%	 stroke-overstrike= "true"
%	 />
%<multicurve stroke-width= "0.35"
%	 fill-style= "none"
%	 points= "(70,25);(70,25);(70,5);(70,5)"
%	 stroke-overstrike= "true"
%	 />
%<multicurve stroke-width= "0.35"
%	 fill-style= "none"
%	 points= "(70,5);(70,5);(90,5);(90,5)"
%	 stroke-overstrike= "true"
%	 />
%<text stroke-width= "0.35"
%	 fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(77.5,10)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 stroke-overstrike= "true"
%	 >
%\program
%</text>
%<multicurve stroke-width= "0.35"
%	 fill-style= "none"
%	 points= "(70,25);(70,25);(90,5);(90,5)"
%	 stroke-overstrike= "true"
%	 />
%<multicurve stroke-width= "0.2"
%	 fill-style= "none"
%	 stroke-color= "#ff0000"
%	 points= "(30,85);(30,85);(47.5,67.51);(47.5,67.51)"
%	 stroke-overstrike= "true"
%	 />
%<multicurve stroke-width= "0.2"
%	 fill-style= "none"
%	 stroke-color= "#ff0000"
%	 points= "(47.5,67.49);(47.5,67.49);(47.5,0);(47.5,0)"
%	 stroke-overstrike= "true"
%	 />
%<multicurve stroke-width= "0.2"
%	 fill-style= "none"
%	 stroke-color= "#ff0000"
%	 points= "(3.75,85);(3.75,85);(30,85);(30,85)"
%	 stroke-overstrike= "true"
%	 />
%<multicurve stroke-width= "0.2"
%	 fill-style= "none"
%	 stroke-color= "#ff0000"
%	 points= "(3.75,85);(3.75,85);(3.75,0);(3.75,0)"
%	 stroke-overstrike= "true"
%	 />
%<multicurve stroke-width= "0.2"
%	 fill-style= "none"
%	 stroke-color= "#ff0000"
%	 points= "(47.5,0);(47.5,0);(5,0);(5,0)"
%	 stroke-overstrike= "true"
%	 />
%<multicurve stroke-width= "0.2"
%	 fill-style= "none"
%	 stroke-color= "#ff0000"
%	 points= "(78.75,85);(78.75,85);(96.25,67.51);(96.25,67.51)"
%	 stroke-overstrike= "true"
%	 />
%<multicurve stroke-width= "0.2"
%	 fill-style= "none"
%	 stroke-color= "#ff0000"
%	 points= "(96.25,67.49);(96.25,67.49);(96.25,0);(96.25,0)"
%	 stroke-overstrike= "true"
%	 />
%<multicurve stroke-width= "0.2"
%	 fill-style= "none"
%	 stroke-color= "#ff0000"
%	 points= "(52.5,85);(52.5,85);(78.75,85);(78.75,85)"
%	 stroke-overstrike= "true"
%	 />
%<multicurve stroke-width= "0.2"
%	 fill-style= "none"
%	 stroke-color= "#ff0000"
%	 points= "(52.5,85);(52.5,85);(52.5,0);(52.5,0)"
%	 stroke-overstrike= "true"
%	 />
%<multicurve stroke-width= "0.2"
%	 fill-style= "none"
%	 stroke-color= "#ff0000"
%	 points= "(96.25,0);(96.25,0);(53.75,0);(53.75,0)"
%	 stroke-overstrike= "true"
%	 />
%<text stroke-width= "0.35"
%	 fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(140,60)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 stroke-overstrike= "true"
%	 >
%\EQLS
%</text>
%<text stroke-width= "0.35"
%	 fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(60,10)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 stroke-overstrike= "true"
%	 >
%$\Peeh$
%</text>
%<text stroke-width= "0.35"
%	 fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(40,10)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 stroke-overstrike= "true"
%	 >
%$\Peeg$
%</text>
%<text stroke-width= "0.35"
%	 fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(382.5,60)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 stroke-overstrike= "true"
%	 >
%\EQLS
%</text>
%<multicurve stroke-width= "0.35"
%	 fill-style= "none"
%	 points= "(430,102.5);(430,102.5);(430,72.5);(430,72.5)"
%	 stroke-overstrike= "true"
%	 />
%<multicurve stroke-width= "0.35"
%	 fill-style= "none"
%	 points= "(402.5,80);(402.5,80);(422.5,80);(422.5,80)"
%	 stroke-overstrike= "true"
%	 />
%<multicurve stroke-width= "0.35"
%	 fill-style= "none"
%	 points= "(440,62.5);(440,62.5);(420,62.5);(420,62.5)"
%	 stroke-overstrike= "true"
%	 />
%<multicurve stroke-width= "0.35"
%	 fill-style= "none"
%	 points= "(422.5,80);(422.5,80);(440,62.51);(440,62.51)"
%	 stroke-overstrike= "true"
%	 />
%<multicurve stroke-width= "0.35"
%	 fill-style= "none"
%	 points= "(402.5,80);(402.5,80);(420,62.5);(420,62.5)"
%	 stroke-overstrike= "true"
%	 />
%<text stroke-width= "0.35"
%	 fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(421.25,71.25)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 stroke-overstrike= "true"
%	 >
%$\parteval$
%</text>
%<multicurve stroke-width= "0.35"
%	 fill-style= "none"
%	 points= "(430,62.5);(430,62.5);(430,40);(430,40)"
%	 stroke-overstrike= "true"
%	 />
%<multicurve stroke-width= "0.35"
%	 fill-style= "none"
%	 points= "(412.5,70);(412.5,70);(412.5,15);(412.5,15)"
%	 stroke-overstrike= "true"
%	 />
%<multicurve stroke-width= "0.35"
%	 fill-style= "none"
%	 points= "(402.5,25);(402.5,25);(402.5,5);(402.5,5)"
%	 stroke-overstrike= "true"
%	 />
%<multicurve stroke-width= "0.35"
%	 fill-style= "none"
%	 points= "(402.5,5);(402.5,5);(422.5,5);(422.5,5)"
%	 stroke-overstrike= "true"
%	 />
%<text stroke-width= "0.35"
%	 fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(410,10)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 stroke-overstrike= "true"
%	 >
%\program
%</text>
%<multicurve stroke-width= "0.35"
%	 fill-style= "none"
%	 points= "(402.5,25);(402.5,25);(422.5,5);(422.5,5)"
%	 stroke-overstrike= "true"
%	 />
%<text stroke-width= "0.35"
%	 fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(427.5,35)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 stroke-overstrike= "true"
%	 >
%$\prohram$
%</text>
%<multicurve stroke-width= "0.35"
%	 fill-style= "none"
%	 points= "(420,50);(420,50);(420,30);(420,30)"
%	 stroke-overstrike= "true"
%	 />
%<multicurve stroke-width= "0.35"
%	 fill-style= "none"
%	 points= "(420,30);(420,30);(440,30);(440,30)"
%	 stroke-overstrike= "true"
%	 />
%<multicurve stroke-width= "0.35"
%	 fill-style= "none"
%	 points= "(420,50);(420,50);(440,30);(440,30)"
%	 stroke-overstrike= "true"
%	 />
%<multicurve stroke-width= "0.2"
%	 fill-style= "none"
%	 stroke-color= "#ff0000"
%	 points= "(425,85);(425,85);(442.5,67.51);(442.5,67.51)"
%	 />
%<multicurve stroke-width= "0.35"
%	 fill-style= "none"
%	 stroke-color= "#ff0000"
%	 points= "(442.5,67.49);(442.5,67.49);(442.5,0);(442.5,0)"
%	 stroke-overstrike= "true"
%	 />
%<multicurve stroke-width= "0.2"
%	 fill-style= "none"
%	 stroke-color= "#ff0000"
%	 points= "(398.75,85);(398.75,85);(425,85);(425,85)"
%	 />
%<multicurve stroke-width= "0.2"
%	 fill-style= "none"
%	 stroke-color= "#ff0000"
%	 points= "(398.75,85);(398.75,85);(398.75,0);(398.75,0)"
%	 />
%<multicurve stroke-width= "0.2"
%	 fill-style= "none"
%	 stroke-color= "#ff0000"
%	 points= "(442.5,0);(442.5,0);(400,0);(400,0)"
%	 />
%<text stroke-width= "0.35"
%	 fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(435,10)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 stroke-overstrike= "true"
%	 >
%$\Peeg$
%</text>
%<multicurve stroke-width= "0.35"
%	 fill-style= "none"
%	 points= "(470,92.5);(470,92.5);(470,110);(470,110)"
%	 stroke-overstrike= "true"
%	 />
%<text stroke-width= "0.35"
%	 fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(455,125.62)"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 stroke-overstrike= "true"
%	 >
%$\nameslang$
%</text>
%<text stroke-width= "0.35"
%	 fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(458.12,2.5)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 stroke-overstrike= "true"
%	 >
%$\inputt$
%</text>
%<multicurve stroke-width= "0.35"
%	 fill-style= "none"
%	 points= "(440,92.5);(440,92.5);(470,92.5);(470,92.5)"
%	 stroke-overstrike= "true"
%	 />
%<multicurve stroke-width= "0.35"
%	 fill-style= "none"
%	 points= "(460,92.5);(460,92.5);(460,0.63);(460,0.63)"
%	 stroke-overstrike= "true"
%	 />
%<text stroke-width= "0.35"
%	 fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(448.12,101.88)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 stroke-overstrike= "true"
%	 >
%\universal
%</text>
%<multicurve stroke-width= "0.35"
%	 fill-style= "none"
%	 points= "(422.5,110);(422.5,110);(440,92.5);(440,92.5)"
%	 stroke-overstrike= "true"
%	 />
%<multicurve stroke-width= "0.35"
%	 fill-style= "none"
%	 points= "(422.5,110);(422.5,110);(470,110);(470,110)"
%	 stroke-overstrike= "true"
%	 />
%<multicurve stroke-width= "0.35"
%	 fill-style= "none"
%	 points= "(450,126.88);(450,126.88);(450,110);(450,110)"
%	 stroke-overstrike= "true"
%	 />
%<text stroke-width= "0.35"
%	 fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(300,60)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 stroke-overstrike= "true"
%	 >
%\EQLS
%</text>
%<multicurve stroke-width= "0.35"
%	 fill-style= "none"
%	 points= "(337.5,92.5);(337.5,92.5);(337.5,40);(337.5,40)"
%	 stroke-overstrike= "true"
%	 />
%<multicurve stroke-width= "0.35"
%	 fill-style= "none"
%	 points= "(310,110);(310,110);(327.5,92.5);(327.5,92.5)"
%	 stroke-overstrike= "true"
%	 />
%<multicurve stroke-width= "0.35"
%	 fill-style= "none"
%	 points= "(320,100);(320,100);(320,15);(320,15)"
%	 stroke-overstrike= "true"
%	 />
%<multicurve stroke-width= "0.35"
%	 fill-style= "none"
%	 points= "(310,25);(310,25);(310,5);(310,5)"
%	 stroke-overstrike= "true"
%	 />
%<multicurve stroke-width= "0.35"
%	 fill-style= "none"
%	 points= "(310,5);(310,5);(330,5);(330,5)"
%	 stroke-overstrike= "true"
%	 />
%<text stroke-width= "0.35"
%	 fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(317.5,10)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 stroke-overstrike= "true"
%	 >
%\program
%</text>
%<multicurve stroke-width= "0.35"
%	 fill-style= "none"
%	 points= "(310,25);(310,25);(330,5);(330,5)"
%	 stroke-overstrike= "true"
%	 />
%<text stroke-width= "0.35"
%	 fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(335,35)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 stroke-overstrike= "true"
%	 >
%$\prohram$
%</text>
%<multicurve stroke-width= "0.35"
%	 fill-style= "none"
%	 points= "(327.5,50);(327.5,50);(327.5,30);(327.5,30)"
%	 stroke-overstrike= "true"
%	 />
%<multicurve stroke-width= "0.35"
%	 fill-style= "none"
%	 points= "(327.5,30);(327.5,30);(347.5,30);(347.5,30)"
%	 stroke-overstrike= "true"
%	 />
%<multicurve stroke-width= "0.35"
%	 fill-style= "none"
%	 points= "(327.5,50);(327.5,50);(347.5,30);(347.5,30)"
%	 stroke-overstrike= "true"
%	 />
%<multicurve stroke-width= "0.35"
%	 fill-style= "none"
%	 points= "(377.5,92.5);(377.5,92.5);(377.5,110);(377.5,110)"
%	 stroke-overstrike= "true"
%	 />
%<text stroke-width= "0.35"
%	 fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(360,125.62)"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 stroke-overstrike= "true"
%	 >
%$\nameslang$
%</text>
%<text stroke-width= "0.35"
%	 fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(365.62,2.5)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 stroke-overstrike= "true"
%	 >
%$\inputt$
%</text>
%<multicurve stroke-width= "0.35"
%	 fill-style= "none"
%	 points= "(327.5,92.5);(327.5,92.5);(377.5,92.5);(377.5,92.5)"
%	 stroke-overstrike= "true"
%	 />
%<multicurve stroke-width= "0.35"
%	 fill-style= "none"
%	 points= "(367.5,92.5);(367.5,92.5);(367.5,0.63);(367.5,0.63)"
%	 stroke-overstrike= "true"
%	 />
%<text stroke-width= "0.35"
%	 fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(350,101.25)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 stroke-overstrike= "true"
%	 >
%\universal
%</text>
%<multicurve stroke-width= "0.35"
%	 fill-style= "none"
%	 points= "(310,110);(310,110);(377.5,110);(377.5,110)"
%	 stroke-overstrike= "true"
%	 />
%<multicurve stroke-width= "0.35"
%	 fill-style= "none"
%	 points= "(355,126.88);(355,126.88);(355,110);(355,110)"
%	 stroke-overstrike= "true"
%	 />
%<ellipse stroke-width= "2"
%	 fill-style= "solid"
%	 p3= "(214.11,50.94)"
%	 p2= "(214.11,54.06)"
%	 p1= "(210.89,54.06)"
%	 closure= "open"
%	 angle-end= "0"
%	 fill-color= "#330033"
%	 angle-start= "0"
%	 stroke-overstrike= "true"
%	 />
%<ellipse stroke-width= "2"
%	 fill-style= "solid"
%	 p3= "(213.3,51.72)"
%	 p2= "(213.3,53.28)"
%	 p1= "(211.7,53.28)"
%	 closure= "open"
%	 angle-end= "0"
%	 fill-color= "#330033"
%	 angle-start= "0"
%	 stroke-overstrike= "true"
%	 />
%</jpic>
%%End JPIC-XML
%LaTeX-picture environment using emulated lines and arcs
%You can rescale the whole picture (to 80% for instance) by using the command \def\JPicScale{0.8}
\ifx\JPicScale\undefined\def\JPicScale{1}\fi
\unitlength \JPicScale mm
\begin{picture}(470,126.88)(0,0)
\put(117.5,2.5){\makebox(0,0)[cr]{$\inputt$}}

\linethickness{0.35mm}
\put(30,90){\line(1,0){95}}
\linethickness{0.35mm}
\put(120,0){\line(0,1){90}}
\linethickness{0.35mm}
\put(35,72.5){\line(0,1){17.5}}
\linethickness{0.35mm}
\put(30,90){\line(0,1){25}}
\put(77.5,102.5){\makebox(0,0)[cc]{$\gee$}}

\linethickness{0.35mm}
\put(7.5,80){\line(1,0){20}}
\linethickness{0.35mm}
\put(25,62.5){\line(1,0){20}}
\linethickness{0.35mm}
\multiput(27.5,80)(0.12,-0.12){146}{\line(1,0){0.12}}
\linethickness{0.35mm}
\multiput(7.5,80)(0.12,-0.12){146}{\line(1,0){0.12}}
\put(26.25,71.25){\makebox(0,0)[cc]{$\parteval$}}

\linethickness{0.35mm}
\put(35,40){\line(0,1){22.5}}
\put(210,10){\makebox(0,0)[cc]{$\prohram$}}

\linethickness{0.35mm}
\put(30,115){\line(1,0){95}}
\linethickness{0.35mm}
\put(77.5,115){\line(0,1){11.88}}
\put(82.5,125){\makebox(0,0)[cl]{$\nameslang$}}

\linethickness{0.35mm}
\put(82.5,72.5){\line(0,1){17.5}}
\linethickness{0.35mm}
\put(55,80){\line(1,0){20}}
\linethickness{0.35mm}
\put(72.5,62.5){\line(1,0){20}}
\linethickness{0.35mm}
\multiput(75,79.99)(0.12,-0.12){146}{\line(1,0){0.12}}
\linethickness{0.35mm}
\multiput(55,80)(0.12,-0.12){146}{\line(1,0){0.12}}
\linethickness{0.35mm}
\put(17.5,15){\line(0,1){55}}
\put(73.75,71.25){\makebox(0,0)[cc]{$\parteval$}}

\linethickness{0.35mm}
\put(7.5,5){\line(0,1){20}}
\linethickness{0.35mm}
\put(7.5,5){\line(1,0){20}}
\put(15,10){\makebox(0,0)[cc]{\program}}

\linethickness{0.35mm}
\multiput(7.5,25)(0.12,-0.12){167}{\line(1,0){0.12}}
\linethickness{0.35mm}
\put(125,90){\line(0,1){25}}
\linethickness{0.35mm}
\put(202.5,5){\line(0,1){20}}
\linethickness{0.35mm}
\put(202.5,5){\line(1,0){20}}
\linethickness{0.35mm}
\multiput(202.5,25)(0.12,-0.12){167}{\line(1,0){0.12}}
\linethickness{0.35mm}
\put(215,55){\line(0,1){15}}
\put(272.5,2.5){\makebox(0,0)[cr]{$\inputt$}}

\linethickness{0.35mm}
\put(185,90){\line(1,0){95}}
\linethickness{0.35mm}
\put(275,0){\line(0,1){90}}
\linethickness{0.35mm}
\put(190,72.5){\line(0,1){17.5}}
\linethickness{0.35mm}
\put(185,90){\line(0,1){25}}
\put(232.5,102.5){\makebox(0,0)[cc]{$\gee$}}

\linethickness{0.35mm}
\put(162.5,80){\line(1,0){20}}
\linethickness{0.35mm}
\put(180,62.5){\line(1,0){20}}
\linethickness{0.35mm}
\multiput(182.5,80)(0.12,-0.12){146}{\line(1,0){0.12}}
\linethickness{0.35mm}
\multiput(162.5,80)(0.12,-0.12){146}{\line(1,0){0.12}}
\linethickness{0.35mm}
\put(192.5,52.5){\line(1,0){20}}
\linethickness{0.35mm}
\multiput(170,55)(0.12,-0.12){125}{\line(1,0){0.12}}
\linethickness{0.35mm}
\put(170,55){\line(0,1){17.5}}
\linethickness{0.35mm}
\multiput(212.5,52.5)(0.12,0.12){21}{\line(1,0){0.12}}
\linethickness{0.35mm}
\multiput(190,55.01)(0.12,-0.12){21}{\line(0,-1){0.12}}
\put(181.25,71.25){\makebox(0,0)[cc]{$\parteval$}}

\linethickness{0.35mm}
\put(190,55){\line(0,1){7.5}}
\linethickness{0.35mm}
\put(185,115){\line(1,0){95}}
\linethickness{0.35mm}
\put(232.5,115){\line(0,1){11.88}}
\put(237.5,125){\makebox(0,0)[cl]{$\nameslang$}}

\linethickness{0.35mm}
\put(232.5,72.5){\line(0,1){17.5}}
\linethickness{0.35mm}
\put(205,80){\line(1,0){20}}
\linethickness{0.35mm}
\put(222.5,62.5){\line(1,0){20}}
\linethickness{0.35mm}
\multiput(225,79.99)(0.12,-0.12){146}{\line(1,0){0.12}}
\linethickness{0.35mm}
\multiput(205,80)(0.12,-0.12){146}{\line(1,0){0.12}}
\linethickness{0.35mm}
\put(185,15){\line(0,1){25}}
\put(223.75,71.25){\makebox(0,0)[cc]{$\parteval$}}

\linethickness{0.35mm}
\put(232.5,55){\line(0,1){7.5}}
\linethickness{0.35mm}
\put(175,5){\line(0,1){20}}
\linethickness{0.35mm}
\put(175,5){\line(1,0){20}}
\put(182.5,10){\makebox(0,0)[cc]{\program}}

\linethickness{0.35mm}
\multiput(175,25)(0.12,-0.12){167}{\line(1,0){0.12}}
\linethickness{0.35mm}
\put(280,90){\line(0,1){25}}
\linethickness{0.35mm}
\put(212.5,15){\line(0,1){37.5}}
\linethickness{0.35mm}
\put(185,40){\line(1,0){32.5}}
\linethickness{0.35mm}
\multiput(217.5,40)(0.12,0.12){125}{\line(1,0){0.12}}
\linethickness{2mm}
\put(186.59,39.76){\line(0,1){0.49}}
\multiput(186.43,39.29)(0.16,0.46){1}{\line(0,1){0.46}}
\multiput(186.14,38.9)(0.15,0.2){2}{\line(0,1){0.2}}
\multiput(185.73,38.61)(0.2,0.14){2}{\line(1,0){0.2}}
\multiput(185.25,38.46)(0.48,0.15){1}{\line(1,0){0.48}}
\put(184.75,38.46){\line(1,0){0.5}}
\multiput(184.27,38.61)(0.48,-0.15){1}{\line(1,0){0.48}}
\multiput(183.86,38.9)(0.2,-0.14){2}{\line(1,0){0.2}}
\multiput(183.57,39.29)(0.15,-0.2){2}{\line(0,-1){0.2}}
\multiput(183.41,39.76)(0.16,-0.46){1}{\line(0,-1){0.46}}
\put(183.41,39.76){\line(0,1){0.49}}
\multiput(183.41,40.24)(0.16,0.46){1}{\line(0,1){0.46}}
\multiput(183.57,40.71)(0.15,0.2){2}{\line(0,1){0.2}}
\multiput(183.86,41.1)(0.2,0.14){2}{\line(1,0){0.2}}
\multiput(184.27,41.39)(0.48,0.15){1}{\line(1,0){0.48}}
\put(184.75,41.54){\line(1,0){0.5}}
\multiput(185.25,41.54)(0.48,-0.15){1}{\line(1,0){0.48}}
\multiput(185.73,41.39)(0.2,-0.14){2}{\line(1,0){0.2}}
\multiput(186.14,41.1)(0.15,-0.2){2}{\line(0,-1){0.2}}
\multiput(186.43,40.71)(0.16,-0.46){1}{\line(0,-1){0.46}}

\linethickness{0.2mm}
\put(157.5,120){\line(1,0){127.5}}
\put(157.5,30){\line(0,1){90}}
\put(285,30){\line(0,1){90}}
\put(157.5,30){\line(1,0){127.5}}
\put(255,50){\makebox(0,0)[cc]{$\geehat$}}

\put(32.5,35){\makebox(0,0)[cc]{$\prohram$}}

\linethickness{0.35mm}
\put(25,30){\line(0,1){20}}
\linethickness{0.35mm}
\put(25,30){\line(1,0){20}}
\linethickness{0.35mm}
\multiput(25,50)(0.12,-0.12){167}{\line(1,0){0.12}}
\linethickness{0.35mm}
\put(65,40){\line(0,1){30}}
\put(62.5,35){\makebox(0,0)[cc]{$\prohram$}}

\linethickness{0.35mm}
\put(55,30){\line(0,1){20}}
\linethickness{0.35mm}
\put(55,30){\line(1,0){20}}
\linethickness{0.35mm}
\multiput(55,50)(0.12,-0.12){167}{\line(1,0){0.12}}
\linethickness{0.35mm}
\put(80,15){\line(0,1){47.5}}
\linethickness{0.35mm}
\put(70,5){\line(0,1){20}}
\linethickness{0.35mm}
\put(70,5){\line(1,0){20}}
\put(77.5,10){\makebox(0,0)[cc]{\program}}

\linethickness{0.35mm}
\multiput(70,25)(0.12,-0.12){167}{\line(1,0){0.12}}
\linethickness{0.2mm}
\multiput(30,85)(0.12,-0.12){146}{\line(1,0){0.12}}
\linethickness{0.2mm}
\put(47.5,0){\line(0,1){67.49}}
\linethickness{0.2mm}
\put(3.75,85){\line(1,0){26.25}}
\linethickness{0.2mm}
\put(3.75,0){\line(0,1){85}}
\linethickness{0.2mm}
\put(5,0){\line(1,0){42.5}}
\linethickness{0.2mm}
\multiput(78.75,85)(0.12,-0.12){146}{\line(1,0){0.12}}
\linethickness{0.2mm}
\put(96.25,0){\line(0,1){67.49}}
\linethickness{0.2mm}
\put(52.5,85){\line(1,0){26.25}}
\linethickness{0.2mm}
\put(52.5,0){\line(0,1){85}}
\linethickness{0.2mm}
\put(53.75,0){\line(1,0){42.5}}
\put(140,60){\makebox(0,0)[cc]{\EQLS}}

\put(60,10){\makebox(0,0)[cc]{$\Peeh$}}

\put(40,10){\makebox(0,0)[cc]{$\Peeg$}}

\put(382.5,60){\makebox(0,0)[cc]{\EQLS}}

\linethickness{0.35mm}
\put(430,72.5){\line(0,1){30}}
\linethickness{0.35mm}
\put(402.5,80){\line(1,0){20}}
\linethickness{0.35mm}
\put(420,62.5){\line(1,0){20}}
\linethickness{0.35mm}
\multiput(422.5,80)(0.12,-0.12){146}{\line(1,0){0.12}}
\linethickness{0.35mm}
\multiput(402.5,80)(0.12,-0.12){146}{\line(1,0){0.12}}
\put(421.25,71.25){\makebox(0,0)[cc]{$\parteval$}}

\linethickness{0.35mm}
\put(430,40){\line(0,1){22.5}}
\linethickness{0.35mm}
\put(412.5,15){\line(0,1){55}}
\linethickness{0.35mm}
\put(402.5,5){\line(0,1){20}}
\linethickness{0.35mm}
\put(402.5,5){\line(1,0){20}}
\put(410,10){\makebox(0,0)[cc]{\program}}

\linethickness{0.35mm}
\multiput(402.5,25)(0.12,-0.12){167}{\line(1,0){0.12}}
\put(427.5,35){\makebox(0,0)[cc]{$\prohram$}}

\linethickness{0.35mm}
\put(420,30){\line(0,1){20}}
\linethickness{0.35mm}
\put(420,30){\line(1,0){20}}
\linethickness{0.35mm}
\multiput(420,50)(0.12,-0.12){167}{\line(1,0){0.12}}
\linethickness{0.2mm}
\multiput(425,85)(0.12,-0.12){146}{\line(1,0){0.12}}
\linethickness{0.35mm}
\put(442.5,0){\line(0,1){67.49}}
\linethickness{0.2mm}
\put(398.75,85){\line(1,0){26.25}}
\linethickness{0.2mm}
\put(398.75,0){\line(0,1){85}}
\linethickness{0.2mm}
\put(400,0){\line(1,0){42.5}}
\put(435,10){\makebox(0,0)[cc]{$\Peeg$}}

\linethickness{0.35mm}
\put(470,92.5){\line(0,1){17.5}}
\put(455,125.62){\makebox(0,0)[cl]{$\nameslang$}}

\put(458.12,2.5){\makebox(0,0)[cr]{$\inputt$}}

\linethickness{0.35mm}
\put(440,92.5){\line(1,0){30}}
\linethickness{0.35mm}
\put(460,0.63){\line(0,1){91.87}}
\put(448.12,101.88){\makebox(0,0)[cc]{\universal}}

\linethickness{0.35mm}
\multiput(422.5,110)(0.12,-0.12){146}{\line(1,0){0.12}}
\linethickness{0.35mm}
\put(422.5,110){\line(1,0){47.5}}
\linethickness{0.35mm}
\put(450,110){\line(0,1){16.88}}
\put(300,60){\makebox(0,0)[cc]{\EQLS}}

\linethickness{0.35mm}
\put(337.5,40){\line(0,1){52.5}}
\linethickness{0.35mm}
\multiput(310,110)(0.12,-0.12){146}{\line(1,0){0.12}}
\linethickness{0.35mm}
\put(320,15){\line(0,1){85}}
\linethickness{0.35mm}
\put(310,5){\line(0,1){20}}
\linethickness{0.35mm}
\put(310,5){\line(1,0){20}}
\put(317.5,10){\makebox(0,0)[cc]{\program}}

\linethickness{0.35mm}
\multiput(310,25)(0.12,-0.12){167}{\line(1,0){0.12}}
\put(335,35){\makebox(0,0)[cc]{$\prohram$}}

\linethickness{0.35mm}
\put(327.5,30){\line(0,1){20}}
\linethickness{0.35mm}
\put(327.5,30){\line(1,0){20}}
\linethickness{0.35mm}
\multiput(327.5,50)(0.12,-0.12){167}{\line(1,0){0.12}}
\linethickness{0.35mm}
\put(377.5,92.5){\line(0,1){17.5}}
\put(360,125.62){\makebox(0,0)[cl]{$\nameslang$}}

\put(365.62,2.5){\makebox(0,0)[cr]{$\inputt$}}

\linethickness{0.35mm}
\put(327.5,92.5){\line(1,0){50}}
\linethickness{0.35mm}
\put(367.5,0.63){\line(0,1){91.87}}
\put(350,101.25){\makebox(0,0)[cc]{\universal}}

\linethickness{0.35mm}
\put(310,110){\line(1,0){67.5}}
\linethickness{0.35mm}
\put(355,110){\line(0,1){16.88}}
\linethickness{2mm}
\put(214.09,52.26){\line(0,1){0.49}}
\multiput(213.93,51.79)(0.16,0.46){1}{\line(0,1){0.46}}
\multiput(213.64,51.4)(0.15,0.2){2}{\line(0,1){0.2}}
\multiput(213.23,51.11)(0.2,0.14){2}{\line(1,0){0.2}}
\multiput(212.75,50.96)(0.48,0.15){1}{\line(1,0){0.48}}
\put(212.25,50.96){\line(1,0){0.5}}
\multiput(211.77,51.11)(0.48,-0.15){1}{\line(1,0){0.48}}
\multiput(211.36,51.4)(0.2,-0.14){2}{\line(1,0){0.2}}
\multiput(211.07,51.79)(0.15,-0.2){2}{\line(0,-1){0.2}}
\multiput(210.91,52.26)(0.16,-0.46){1}{\line(0,-1){0.46}}
\put(210.91,52.26){\line(0,1){0.49}}
\multiput(210.91,52.74)(0.16,0.46){1}{\line(0,1){0.46}}
\multiput(211.07,53.21)(0.15,0.2){2}{\line(0,1){0.2}}
\multiput(211.36,53.6)(0.2,0.14){2}{\line(1,0){0.2}}
\multiput(211.77,53.89)(0.48,0.15){1}{\line(1,0){0.48}}
\put(212.25,54.04){\line(1,0){0.5}}
\multiput(212.75,54.04)(0.48,-0.15){1}{\line(1,0){0.48}}
\multiput(213.23,53.89)(0.2,-0.14){2}{\line(1,0){0.2}}
\multiput(213.64,53.6)(0.15,-0.2){2}{\line(0,-1){0.2}}
\multiput(213.93,53.21)(0.16,-0.46){1}{\line(0,-1){0.46}}

\linethickness{2mm}
\put(213.28,52.3){\line(0,1){0.4}}
\multiput(213.07,51.95)(0.1,0.18){2}{\line(0,1){0.18}}
\multiput(212.71,51.75)(0.18,0.1){2}{\line(1,0){0.18}}
\put(212.29,51.75){\line(1,0){0.42}}
\multiput(211.93,51.95)(0.18,-0.1){2}{\line(1,0){0.18}}
\multiput(211.72,52.3)(0.1,-0.18){2}{\line(0,-1){0.18}}
\put(211.72,52.3){\line(0,1){0.4}}
\multiput(211.72,52.7)(0.1,0.18){2}{\line(0,1){0.18}}
\multiput(211.93,53.05)(0.18,0.1){2}{\line(1,0){0.18}}
\put(212.29,53.25){\line(1,0){0.42}}
\multiput(212.71,53.25)(0.18,-0.1){2}{\line(1,0){0.18}}
\multiput(213.07,53.05)(0.1,-0.18){2}{\line(0,-1){0.18}}

\end{picture}


==> PIC/smullyan.tex <==
%%Created by jPicEdt 1.4.1_03: mixed JPIC-XML/LaTeX format
%%Mon Dec 11 21:08:17 HST 2017
%%Begin JPIC-XML
%<?xml version="1.0" standalone="yes"?>
%<jpic x-min="-6.25" x-max="268.75" y-min="0.62" y-max="128.75" auto-bounding="true">
%<multicurve fill-style= "none"
%	 points= "(111.25,91.24);(111.25,91.24);(166.25,91.25);(166.25,91.25)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(111.25,45.62);(111.25,45.62);(111.25,20.62);(111.25,20.62)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(166.25,66.25);(166.25,66.25);(166.25,91.25);(166.25,91.25)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(151.25,103.12);(151.25,103.12);(151.25,91.24);(151.25,91.24)"
%	 stroke-width= "0.75"
%	 />
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(153.75,101.88)"
%	 text-frame= "noframe"
%	 stroke-width= "0.75"
%	 text-hor-align= "left"
%	 >
%$\nameslang$
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(158.12,2.5)"
%	 text-frame= "noframe"
%	 stroke-width= "0.75"
%	 text-hor-align= "right"
%	 >
%$\inputt$
%</text>
%<multicurve fill-style= "none"
%	 points= "(136.25,66.24);(136.25,66.24);(166.25,66.25);(166.25,66.25)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(161.25,66.25);(161.25,66.25);(161.25,1.25);(161.25,1.25)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(111.25,20.62);(111.25,20.62);(136.25,20.62);(136.25,20.62)"
%	 stroke-width= "0.75"
%	 />
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(146.25,78.75)"
%	 text-frame= "noframe"
%	 stroke-width= "0.75"
%	 text-hor-align= "center-h"
%	 >
%\universal
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(118.75,27.49)"
%	 text-frame= "noframe"
%	 stroke-width= "0.75"
%	 text-hor-align= "center-h"
%	 >
%\program
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(96.25,80)"
%	 text-frame= "noframe"
%	 stroke-width= "0.75"
%	 text-hor-align= "center-h"
%	 >
%\EQLS
%</text>
%<multicurve fill-style= "none"
%	 points= "(111.25,45.62);(111.25,45.62);(136.25,20.62);(136.25,20.62)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(123.75,78.75);(123.75,78.75);(123.75,33.74);(123.75,33.74)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(111.25,91.24);(111.25,91.24);(136.25,66.24);(136.25,66.24)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(21.25,91.26);(21.25,91.26);(71.25,91.24);(71.25,91.24)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(71.25,66.24);(71.25,66.24);(71.25,91.24);(71.25,91.24)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(46.25,103.12);(46.25,103.12);(46.25,91.24);(46.25,91.24)"
%	 stroke-width= "0.75"
%	 />
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(48.75,101.88)"
%	 text-frame= "noframe"
%	 stroke-width= "0.75"
%	 text-hor-align= "left"
%	 >
%$\nameslang$
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(63.12,2.5)"
%	 text-frame= "noframe"
%	 stroke-width= "0.75"
%	 text-hor-align= "right"
%	 >
%$\inputt$
%</text>
%<multicurve fill-style= "none"
%	 points= "(21.25,66.25);(21.25,66.25);(71.25,66.24);(71.25,66.24)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(66.25,66.25);(66.25,66.25);(66.25,1.25);(66.25,1.25)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(26.25,66.26);(26.25,66.26);(26.25,48.75);(26.25,48.75)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(21.25,91.26);(21.25,91.26);(21.25,66.26);(21.25,66.26)"
%	 stroke-width= "0.75"
%	 />
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(46.25,78.12)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\gee$
%</text>
%<multicurve fill-style= "none"
%	 points= "(-1.25,56.25);(-1.25,56.25);(18.75,56.25);(18.75,56.25)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(36.25,38.75);(36.25,38.75);(16.25,38.75);(16.25,38.75)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(18.75,56.25);(18.75,56.25);(36.25,38.76);(36.25,38.76)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(-1.25,56.25);(-1.25,56.25);(16.25,38.75);(16.25,38.75)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(36.25,23.75);(36.25,23.75);(36.25,1.25);(36.25,1.25)"
%	 stroke-width= "0.75"
%	 />
%<ellipse fill-style= "solid"
%	 p3= "(37.66,22.34)"
%	 p2= "(37.66,25.16)"
%	 p1= "(34.84,25.16)"
%	 closure= "open"
%	 angle-end= "0"
%	 fill-color= "#330033"
%	 angle-start= "0"
%	 />
%<multicurve fill-style= "none"
%	 points= "(46.25,66.25);(46.25,66.25);(46.25,33.75);(46.25,33.75)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(6.25,48.75);(6.25,48.75);(6.25,33.75);(6.25,33.75)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(46.25,33.75);(46.25,33.75);(36.25,23.75);(36.25,23.75)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(26.25,33.75);(26.25,33.75);(36.25,23.74);(36.25,23.74)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(141.25,66.25);(141.25,66.25);(141.25,1.25);(141.25,1.25)"
%	 stroke-width= "0.75"
%	 />
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(138.12,2.5)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\progtype$
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(17.5,47.5)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\parteval$
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(29.38,56.88)"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\progtype$
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(126.25,46.24)"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\progtype$
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(101.25,128.75)"
%	 text-frame= "noframe"
%	 stroke-width= "0.75"
%	 text-hor-align= "center-h"
%	 >
%\EQLS
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(61.25,128.75)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\lhs$
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(151.25,128.75)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\rhs$
%</text>
%<multicurve fill-style= "none"
%	 points= "(26.25,38.75);(26.25,38.75);(26.25,33.75);(26.25,33.75)"
%	 stroke-width= "0.75"
%	 />
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(33.12,2.5)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\progtype$
%</text>
%<multicurve fill-style= "none"
%	 points= "(-6.25,46.25);(-6.25,46.25);(-6.25,21.25);(-6.25,21.25)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(-6.25,21.25);(-6.25,21.25);(18.75,21.25);(18.75,21.25)"
%	 stroke-width= "0.75"
%	 />
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(1.25,28.75)"
%	 text-frame= "noframe"
%	 stroke-width= "0.75"
%	 text-hor-align= "center-h"
%	 >
%\program
%</text>
%<multicurve fill-style= "none"
%	 points= "(-6.25,46.25);(-6.25,46.25);(18.75,21.25);(18.75,21.25)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(230,91.25);(230,91.25);(268.75,91.25);(268.75,91.25)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(210,45);(210,45);(210,20);(210,20)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(268.75,66.25);(268.75,66.25);(268.75,91.25);(268.75,91.25)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(253.75,103.12);(253.75,103.12);(253.75,91.24);(253.75,91.24)"
%	 stroke-width= "0.75"
%	 />
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(256.25,101.88)"
%	 text-frame= "noframe"
%	 stroke-width= "0.75"
%	 text-hor-align= "left"
%	 >
%$\nameslang$
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(260.62,2.5)"
%	 text-frame= "noframe"
%	 stroke-width= "0.75"
%	 text-hor-align= "right"
%	 >
%$\inputt$
%</text>
%<multicurve fill-style= "none"
%	 points= "(255,66.25);(255,66.25);(268.75,66.25);(268.75,66.25)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(263.75,66.25);(263.75,66.25);(263.75,0.62);(263.75,0.62)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(210,20);(210,20);(235,20);(235,20)"
%	 stroke-width= "0.75"
%	 />
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(257.5,78.75)"
%	 text-frame= "noframe"
%	 stroke-width= "0.75"
%	 text-hor-align= "center-h"
%	 >
%\universal
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(218.75,27.49)"
%	 text-frame= "noframe"
%	 stroke-width= "0.75"
%	 text-hor-align= "center-h"
%	 >
%\program
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(191.25,80.62)"
%	 text-frame= "noframe"
%	 stroke-width= "0.75"
%	 text-hor-align= "center-h"
%	 >
%\EQLS
%</text>
%<multicurve fill-style= "none"
%	 points= "(210,45);(210,45);(235,20);(235,20)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(221.25,48.75);(221.25,48.75);(221.25,33.74);(221.25,33.74)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(230,91.25);(230,91.25);(255,66.25);(255,66.25)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(241.25,38.75);(241.25,38.75);(241.25,0.62);(241.25,0.62)"
%	 stroke-width= "0.75"
%	 />
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(238.12,2.5)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\progtype$
%</text>
%<multicurve fill-style= "none"
%	 points= "(213.75,56.25);(213.75,56.25);(231.25,38.75);(231.25,38.75)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(233.75,56.25);(233.75,56.25);(251.25,38.75);(251.25,38.75)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(213.75,56.25);(213.75,56.25);(233.75,56.25);(233.75,56.25)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(231.25,38.75);(231.25,38.75);(251.25,38.75);(251.25,38.75)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(241.25,80);(241.25,80);(241.25,48.75);(241.25,48.75)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(235.62,66.25);(235.62,66.25);(255.62,46.25);(255.62,46.25)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(201.25,66.25);(201.25,66.25);(235.62,66.25);(235.62,66.25)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(201.25,11.25);(201.25,11.25);(255.62,11.25);(255.62,11.25)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(201.25,11.25);(201.25,11.25);(201.25,66.25);(201.25,66.25)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(255.62,11.25);(255.62,11.25);(255.62,46.25);(255.62,46.25)"
%	 />
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(231.88,47.5)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\parteval$
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(206.25,61.25)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\geefix$
%</text>
%</jpic>
%%End JPIC-XML
%PSTricks content-type (pstricks.sty package needed)
%Add \usepackage{pstricks} in the preamble of your LaTeX file
%You can rescale the whole picture (to 80% for instance) by using the command \def\JPicScale{0.8}
\ifx\JPicScale\undefined\def\JPicScale{1}\fi
\psset{unit=\JPicScale mm}
\psset{linewidth=0.3,dotsep=1,hatchwidth=0.3,hatchsep=1.5,shadowsize=1,dimen=middle}
\psset{dotsize=0.7 2.5,dotscale=1 1,fillcolor=black}
\psset{arrowsize=1 2,arrowlength=1,arrowinset=0.25,tbarsize=0.7 5,bracketlength=0.15,rbracketlength=0.15}
\begin{pspicture}(0,0)(268.75,128.75)
\psline[linewidth=0.75](111.25,91.24)(166.25,91.25)
\psline[linewidth=0.75](111.25,45.62)(111.25,20.62)
\psline[linewidth=0.75](166.25,66.25)(166.25,91.25)
\psline[linewidth=0.75](151.25,103.12)(151.25,91.24)
\rput[l](153.75,101.88){$\nameslang$}
\rput[r](158.12,2.5){$\inputt$}
\psline[linewidth=0.75](136.25,66.24)(166.25,66.25)
\psline[linewidth=0.75](161.25,66.25)(161.25,1.25)
\psline[linewidth=0.75](111.25,20.62)(136.25,20.62)
\rput(146.25,78.75){\universal}
\rput(118.75,27.49){\program}
\rput(96.25,80){\EQLS}
\psline[linewidth=0.75](111.25,45.62)(136.25,20.62)
\psline[linewidth=0.75](123.75,78.75)(123.75,33.74)
\psline[linewidth=0.75](111.25,91.24)(136.25,66.24)
\psline[linewidth=0.75](21.25,91.26)(71.25,91.24)
\psline[linewidth=0.75](71.25,66.24)(71.25,91.24)
\psline[linewidth=0.75](46.25,103.12)(46.25,91.24)
\rput[l](48.75,101.88){$\nameslang$}
\rput[r](63.12,2.5){$\inputt$}
\psline[linewidth=0.75](21.25,66.25)(71.25,66.24)
\psline[linewidth=0.75](66.25,66.25)(66.25,1.25)
\psline[linewidth=0.75](26.25,66.26)(26.25,48.75)
\psline[linewidth=0.75](21.25,91.26)(21.25,66.26)
\rput(46.25,78.12){$\gee$}
\psline[linewidth=0.75](-1.25,56.25)(18.75,56.25)
\psline[linewidth=0.75](36.25,38.75)(16.25,38.75)
\psline[linewidth=0.75](18.75,56.25)(36.25,38.76)
\psline[linewidth=0.75](-1.25,56.25)(16.25,38.75)
\psline[linewidth=0.75](36.25,23.75)(36.25,1.25)
\newrgbcolor{userFillColour}{0.2 0 0.2}
\rput{0}(36.25,23.75){\psellipse[fillcolor=userFillColour,fillstyle=solid](0,0)(1.41,-1.41)}
\psline[linewidth=0.75](46.25,66.25)(46.25,33.75)
\psline[linewidth=0.75](6.25,48.75)(6.25,33.75)
\psline[linewidth=0.75](46.25,33.75)(36.25,23.75)
\psline[linewidth=0.75](26.25,33.75)(36.25,23.74)
\psline[linewidth=0.75](141.25,66.25)(141.25,1.25)
\rput[r](138.12,2.5){$\progtype$}
\rput(17.5,47.5){$\parteval$}
\rput[l](29.38,56.88){$\progtype$}
\rput[l](126.25,46.24){$\progtype$}
\rput(101.25,128.75){\EQLS}
\rput(61.25,128.75){$\lhs$}
\rput(151.25,128.75){$\rhs$}
\psline[linewidth=0.75](26.25,38.75)(26.25,33.75)
\rput[r](33.12,2.5){$\progtype$}
\psline[linewidth=0.75](-6.25,46.25)(-6.25,21.25)
\psline[linewidth=0.75](-6.25,21.25)(18.75,21.25)
\rput(1.25,28.75){\program}
\psline[linewidth=0.75](-6.25,46.25)(18.75,21.25)
\psline[linewidth=0.75](230,91.25)(268.75,91.25)
\psline[linewidth=0.75](210,45)(210,20)
\psline[linewidth=0.75](268.75,66.25)(268.75,91.25)
\psline[linewidth=0.75](253.75,103.12)(253.75,91.24)
\rput[l](256.25,101.88){$\nameslang$}
\rput[r](260.62,2.5){$\inputt$}
\psline[linewidth=0.75](255,66.25)(268.75,66.25)
\psline[linewidth=0.75](263.75,66.25)(263.75,0.62)
\psline[linewidth=0.75](210,20)(235,20)
\rput(257.5,78.75){\universal}
\rput(218.75,27.49){\program}
\rput(191.25,80.62){\EQLS}
\psline[linewidth=0.75](210,45)(235,20)
\psline[linewidth=0.75](221.25,48.75)(221.25,33.74)
\psline[linewidth=0.75](230,91.25)(255,66.25)
\psline[linewidth=0.75](241.25,38.75)(241.25,0.62)
\rput[r](238.12,2.5){$\progtype$}
\psline[linewidth=0.75](213.75,56.25)(231.25,38.75)
\psline[linewidth=0.75](233.75,56.25)(251.25,38.75)
\psline[linewidth=0.75](213.75,56.25)(233.75,56.25)
\psline[linewidth=0.75](231.25,38.75)(251.25,38.75)
\psline[linewidth=0.75](241.25,80)(241.25,48.75)
\psline(235.62,66.25)(255.62,46.25)
\psline(201.25,66.25)(235.62,66.25)
\psline(201.25,11.25)(255.62,11.25)
\psline(201.25,11.25)(201.25,66.25)
\psline(255.62,11.25)(255.62,46.25)
\rput(231.88,47.5){$\parteval$}
\rput(206.25,61.25){$\geefix$}
\end{pspicture}


==> PIC/spider.tex <==
%%Created by jPicEdt 1.4.1_03: mixed JPIC-XML/LaTeX format
%%Mon Jun 07 14:14:27 GMT-10:00 2021
%%Begin JPIC-XML
%<?xml version="1.0" standalone="yes"?>
%<jpic x-min="0" x-max="180" y-min="0" y-max="85" auto-bounding="true">
%<multicurve fill-style= "none"
%	 points= "(20,0);(20,0);(20,40);(20,40)"
%	 stroke-color= "#ff0033"
%	 />
%<multicurve fill-style= "none"
%	 points= "(40,0);(40,0);(40,30);(40,30)"
%	 stroke-color= "#ff0033"
%	 />
%<multicurve fill-style= "none"
%	 points= "(60,0);(60,0);(60,30);(60,30)"
%	 stroke-color= "#ff0033"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(20,10)"
%	 stroke-color= "#ff0033"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\DOTT
%</text>
%<multicurve fill-style= "none"
%	 points= "(20,10);(20,10);(30,20);(30,20)"
%	 stroke-color= "#ff0033"
%	 />
%<multicurve fill-style= "none"
%	 points= "(40,10);(40,10);(60,30);(60,30)"
%	 stroke-color= "#ff0033"
%	 />
%<multicurve fill-style= "none"
%	 points= "(30,20);(30,20);(40,10);(40,10)"
%	 stroke-color= "#ff0033"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(40,10)"
%	 stroke-color= "#ff0033"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\DOTT
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(60,30)"
%	 stroke-color= "#ff0033"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\DOTT
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(40,30)"
%	 stroke-color= "#ff0033"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\DOTT
%</text>
%<multicurve fill-style= "none"
%	 points= "(30,20);(30,20);(30,40);(30,40)"
%	 stroke-color= "#ff0033"
%	 />
%<multicurve fill-style= "none"
%	 points= "(30,40);(30,40);(40,50);(40,50)"
%	 stroke-color= "#ff0033"
%	 />
%<multicurve fill-style= "none"
%	 points= "(20,50);(20,50);(30,40);(30,40)"
%	 stroke-color= "#ff0033"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(30,20)"
%	 stroke-color= "#ff0033"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\DOTT
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(30,40)"
%	 stroke-color= "#ff0033"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\DOTT
%</text>
%<multicurve fill-style= "none"
%	 points= "(40,50);(40,50);(60,30);(60,30)"
%	 stroke-color= "#ff0033"
%	 />
%<multicurve fill-style= "none"
%	 points= "(10,20);(10,20);(20,10);(20,10)"
%	 stroke-color= "#ff0033"
%	 />
%<multicurve fill-style= "none"
%	 points= "(10,20);(10,20);(10,40);(10,40)"
%	 stroke-color= "#ff0033"
%	 />
%<multicurve fill-style= "none"
%	 points= "(10,40);(10,40);(20,50);(20,50)"
%	 stroke-color= "#ff0033"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(20,50)"
%	 stroke-color= "#ff0033"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\DOTT
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(40,50)"
%	 stroke-color= "#ff0033"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\DOTT
%</text>
%<multicurve fill-style= "none"
%	 points= "(20,40);(20,40);(60,80);(60,80)"
%	 stroke-color= "#ff0033"
%	 />
%<multicurve fill-style= "none"
%	 points= "(40,50);(40,50);(40,60);(40,60)"
%	 stroke-color= "#ff0033"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(40,60)"
%	 stroke-color= "#ff0033"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\DOTT
%</text>
%<multicurve fill-style= "none"
%	 points= "(20,50);(20,50);(20,60);(20,60)"
%	 stroke-color= "#ff0033"
%	 />
%<multicurve fill-style= "none"
%	 points= "(20,60);(20,60);(40,80);(40,80)"
%	 stroke-color= "#ff0033"
%	 />
%<multicurve fill-style= "none"
%	 points= "(0,80);(0,80);(20,60);(20,60)"
%	 stroke-color= "#ff0033"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(20,60)"
%	 stroke-color= "#ff0033"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\DOTT
%</text>
%<multicurve fill-style= "none"
%	 points= "(20,80);(20,80);(10,70);(10,70)"
%	 stroke-color= "#ff0033"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(10,70)"
%	 stroke-color= "#ff0033"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\DOTT
%</text>
%<multicurve fill-style= "none"
%	 points= "(130,0);(130,0);(130,10);(130,10)"
%	 stroke-color= "#ff0033"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(150,30)"
%	 stroke-color= "#ff0033"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\DOTT
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(150,50)"
%	 stroke-color= "#ff0033"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\DOTT
%</text>
%<multicurve fill-style= "none"
%	 points= "(150,0);(150,0);(150,50);(150,50)"
%	 stroke-color= "#ff0033"
%	 />
%<multicurve fill-style= "none"
%	 points= "(170,0);(170,0);(170,10);(170,10)"
%	 stroke-color= "#ff0033"
%	 />
%<multicurve fill-style= "none"
%	 points= "(170,10);(170,10);(150,30);(150,30)"
%	 stroke-color= "#ff0033"
%	 />
%<multicurve fill-style= "none"
%	 points= "(130,10);(130,10);(150,30);(150,30)"
%	 stroke-color= "#ff0033"
%	 />
%<multicurve fill-style= "none"
%	 points= "(150,50);(150,50);(180,80);(180,80)"
%	 stroke-color= "#ff0033"
%	 />
%<multicurve fill-style= "none"
%	 points= "(120,80);(120,80);(150,50);(150,50)"
%	 stroke-color= "#ff0033"
%	 />
%<multicurve fill-style= "none"
%	 points= "(140,80);(140,80);(150,50);(150,50)"
%	 stroke-color= "#ff0033"
%	 />
%<multicurve fill-style= "none"
%	 points= "(160,80);(160,80);(150,50);(150,50)"
%	 stroke-color= "#ff0033"
%	 />
%<multicurve fill-style= "none"
%	 points= "(0,80);(0,80);(0,85);(0,85)"
%	 stroke-color= "#ff0033"
%	 />
%<multicurve fill-style= "none"
%	 points= "(20,80);(20,80);(20,85);(20,85)"
%	 stroke-color= "#ff0033"
%	 />
%<multicurve fill-style= "none"
%	 points= "(40,80);(40,80);(40,85);(40,85)"
%	 stroke-color= "#ff0033"
%	 />
%<multicurve fill-style= "none"
%	 points= "(60,80);(60,80);(60,85);(60,85)"
%	 stroke-color= "#ff0033"
%	 />
%<multicurve fill-style= "none"
%	 points= "(120,80);(120,80);(120,85);(120,85)"
%	 stroke-color= "#ff0033"
%	 />
%<multicurve fill-style= "none"
%	 points= "(140,80);(140,80);(140,85);(140,85)"
%	 stroke-color= "#ff0033"
%	 />
%<multicurve fill-style= "none"
%	 points= "(160,80);(160,80);(160,85);(160,85)"
%	 stroke-color= "#ff0033"
%	 />
%<multicurve fill-style= "none"
%	 points= "(180,80);(180,80);(180,85);(180,85)"
%	 stroke-color= "#ff0033"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(100,43.75)"
%	 stroke-color= "#ff0033"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\EQLS
%</text>
%</jpic>
%%End JPIC-XML
%LaTeX-picture environment using emulated lines and arcs
%You can rescale the whole picture (to 80% for instance) by using the command \def\JPicScale{0.8}
\ifx\JPicScale\undefined\def\JPicScale{1}\fi
\unitlength \JPicScale mm
\begin{picture}(180,85)(0,0)
\linethickness{0.3mm}
\put(20,0){\line(0,1){40}}
\linethickness{0.3mm}
\put(40,0){\line(0,1){30}}
\linethickness{0.3mm}
\put(60,0){\line(0,1){30}}
\put(20,10){\makebox(0,0)[cc]{\DOTT}}

\linethickness{0.3mm}
\multiput(20,10)(0.12,0.12){83}{\line(1,0){0.12}}
\linethickness{0.3mm}
\multiput(40,10)(0.12,0.12){167}{\line(1,0){0.12}}
\linethickness{0.3mm}
\multiput(30,20)(0.12,-0.12){83}{\line(1,0){0.12}}
\put(40,10){\makebox(0,0)[cc]{\DOTT}}

\put(60,30){\makebox(0,0)[cc]{\DOTT}}

\put(40,30){\makebox(0,0)[cc]{\DOTT}}

\linethickness{0.3mm}
\put(30,20){\line(0,1){20}}
\linethickness{0.3mm}
\multiput(30,40)(0.12,0.12){83}{\line(1,0){0.12}}
\linethickness{0.3mm}
\multiput(20,50)(0.12,-0.12){83}{\line(1,0){0.12}}
\put(30,20){\makebox(0,0)[cc]{\DOTT}}

\put(30,40){\makebox(0,0)[cc]{\DOTT}}

\linethickness{0.3mm}
\multiput(40,50)(0.12,-0.12){167}{\line(1,0){0.12}}
\linethickness{0.3mm}
\multiput(10,20)(0.12,-0.12){83}{\line(1,0){0.12}}
\linethickness{0.3mm}
\put(10,20){\line(0,1){20}}
\linethickness{0.3mm}
\multiput(10,40)(0.12,0.12){83}{\line(1,0){0.12}}
\put(20,50){\makebox(0,0)[cc]{\DOTT}}

\put(40,50){\makebox(0,0)[cc]{\DOTT}}

\linethickness{0.3mm}
\multiput(20,40)(0.12,0.12){333}{\line(1,0){0.12}}
\linethickness{0.3mm}
\put(40,50){\line(0,1){10}}
\put(40,60){\makebox(0,0)[cc]{\DOTT}}

\linethickness{0.3mm}
\put(20,50){\line(0,1){10}}
\linethickness{0.3mm}
\multiput(20,60)(0.12,0.12){167}{\line(1,0){0.12}}
\linethickness{0.3mm}
\multiput(0,80)(0.12,-0.12){167}{\line(1,0){0.12}}
\put(20,60){\makebox(0,0)[cc]{\DOTT}}

\linethickness{0.3mm}
\multiput(10,70)(0.12,0.12){83}{\line(1,0){0.12}}
\put(10,70){\makebox(0,0)[cc]{\DOTT}}

\linethickness{0.3mm}
\put(130,0){\line(0,1){10}}
\put(150,30){\makebox(0,0)[cc]{\DOTT}}

\put(150,50){\makebox(0,0)[cc]{\DOTT}}

\linethickness{0.3mm}
\put(150,0){\line(0,1){50}}
\linethickness{0.3mm}
\put(170,0){\line(0,1){10}}
\linethickness{0.3mm}
\multiput(150,30)(0.12,-0.12){167}{\line(1,0){0.12}}
\linethickness{0.3mm}
\multiput(130,10)(0.12,0.12){167}{\line(1,0){0.12}}
\linethickness{0.3mm}
\multiput(150,50)(0.12,0.12){250}{\line(1,0){0.12}}
\linethickness{0.3mm}
\multiput(120,80)(0.12,-0.12){250}{\line(1,0){0.12}}
\linethickness{0.3mm}
\multiput(140,80)(0.12,-0.36){83}{\line(0,-1){0.36}}
\linethickness{0.3mm}
\multiput(150,50)(0.12,0.36){83}{\line(0,1){0.36}}
\linethickness{0.3mm}
\put(0,80){\line(0,1){5}}
\linethickness{0.3mm}
\put(20,80){\line(0,1){5}}
\linethickness{0.3mm}
\put(40,80){\line(0,1){5}}
\linethickness{0.3mm}
\put(60,80){\line(0,1){5}}
\linethickness{0.3mm}
\put(120,80){\line(0,1){5}}
\linethickness{0.3mm}
\put(140,80){\line(0,1){5}}
\linethickness{0.3mm}
\put(160,80){\line(0,1){5}}
\linethickness{0.3mm}
\put(180,80){\line(0,1){5}}
\put(100,43.75){\makebox(0,0)[cc]{\EQLS}}

\end{picture}


==> PIC/straight.tex <==
%%Created by jPicEdt 1.4.1_03: mixed JPIC-XML/LaTeX format
%%Tue Dec 31 13:24:54 GMT-10:00 2019
%%Begin JPIC-XML
%<?xml version="1.0" standalone="yes"?>
%<jpic x-min="0" x-max="140" y-min="8" y-max="45" auto-bounding="true">
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(30,8)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\bottom
%</text>
%<multicurve fill-style= "none"
%	 stroke-width= "0.45"
%	 points= "(0,20);(0,20);(140,20);(140,20)"
%	 />
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(110,45)"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%\Topp
%</text>
%</jpic>
%%End JPIC-XML
%PSTricks content-type (pstricks.sty package needed)
%Add \usepackage{pstricks} in the preamble of your LaTeX file
%You can rescale the whole picture (to 80% for instance) by using the command \def\JPicScale{0.8}
\ifx\JPicScale\undefined\def\JPicScale{1}\fi
\psset{unit=\JPicScale mm}
\psset{linewidth=0.3,dotsep=1,hatchwidth=0.3,hatchsep=1.5,shadowsize=1,dimen=middle}
\psset{dotsize=0.7 2.5,dotscale=1 1,fillcolor=black}
\psset{arrowsize=1 2,arrowlength=1,arrowinset=0.25,tbarsize=0.7 5,bracketlength=0.15,rbracketlength=0.15}
\begin{pspicture}(0,0)(140,45)
\rput(30,8){\bottom}
\psline[linewidth=0.45](0,20)(140,20)
\rput[l](110,45){\Topp}
\end{pspicture}


==> PIC/strict-eqns.tex <==
%%Created by jPicEdt 1.4.1_03: mixed JPIC-XML/LaTeX format
%%Sun Nov 03 14:12:54 GMT-10:00 2019
%%Begin JPIC-XML
%<?xml version="1.0" standalone="yes"?>
%<jpic x-min="0" x-max="237.5" y-min="0" y-max="105" auto-bounding="true">
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(50,75);(50,75);(50,0);(50,0)"
%	 />
%<ellipse fill-style= "solid"
%	 p3= "(54.07,70.93)"
%	 p2= "(54.07,79.07)"
%	 p1= "(45.93,79.07)"
%	 fill-color= "#330033"
%	 closure= "open"
%	 angle-end= "0"
%	 angle-start= "0"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(165,35);(165,35);(150,20);(150,20)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(150,20);(150,20);(150,0);(150,0)"
%	 />
%<ellipse fill-style= "solid"
%	 p3= "(153.79,16.21)"
%	 p2= "(153.79,23.79)"
%	 p1= "(146.21,23.79)"
%	 fill-color= "#330033"
%	 closure= "open"
%	 angle-end= "0"
%	 angle-start= "0"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.6"
%	 points= "(135,45);(135,45);(135,35);(135,35)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(135,35);(135,35);(150,20);(150,20)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.6"
%	 points= "(165,45);(165,45);(165,35);(165,35)"
%	 />
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(217.5,0)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\AAh$
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(12.5,60)"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\BBh$
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(147.5,0)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\AAh$
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(167.5,73.75)"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\BBh$
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(137.5,73.75)"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\BBh$
%</text>
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(10,30);(10,30);(10,0);(10,0)"
%	 />
%<ellipse fill-style= "solid"
%	 p3= "(13.79,71.21)"
%	 p2= "(13.79,78.79)"
%	 p1= "(6.21,78.79)"
%	 fill-color= "#330033"
%	 closure= "open"
%	 angle-end= "0"
%	 angle-start= "0"
%	 />
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(7.5,0)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\AAh$
%</text>
%<parallelogram fill-style= "solid"
%	 p3= "(20,30)"
%	 p2= "(20,50)"
%	 stroke-width= "0.7"
%	 p1= "(0,50)"
%	 fill-color= "#ffffff"
%	 />
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(10,40)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\aah$
%</text>
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(135,75);(135,75);(135,65);(135,65)"
%	 />
%<parallelogram fill-style= "solid"
%	 p3= "(145,45)"
%	 p2= "(145,65)"
%	 stroke-width= "0.7"
%	 p1= "(125,65)"
%	 fill-color= "#ffffff"
%	 />
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(135,55)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\aah$
%</text>
%<parallelogram fill-style= "solid"
%	 p3= "(175,45)"
%	 p2= "(175,65)"
%	 stroke-width= "0.7"
%	 p1= "(155,65)"
%	 fill-color= "#ffffff"
%	 />
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(165,55)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\aah$
%</text>
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(165,75);(165,75);(165,65);(165,65)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(10,73.75);(10,73.75);(10,50);(10,50)"
%	 />
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(47.5,0)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\AAh$
%</text>
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(220,10);(220,10);(220,0);(220,0)"
%	 />
%<parallelogram fill-style= "solid"
%	 p3= "(230,10)"
%	 p2= "(230,30)"
%	 stroke-width= "0.7"
%	 p1= "(210,30)"
%	 fill-color= "#ffffff"
%	 />
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(220,20)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\aah$
%</text>
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(235,55);(235,55);(220,40);(220,40)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(220,40);(220,40);(220,30);(220,30)"
%	 />
%<ellipse fill-style= "solid"
%	 p3= "(223.79,36.21)"
%	 p2= "(223.79,43.79)"
%	 p1= "(216.21,43.79)"
%	 fill-color= "#330033"
%	 closure= "open"
%	 angle-end= "0"
%	 angle-start= "0"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.6"
%	 points= "(205,73.75);(205,73.75);(205,55);(205,55)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(205,55);(205,55);(220,40);(220,40)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.6"
%	 points= "(235,73.75);(235,73.75);(235,55);(235,55)"
%	 />
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(237.5,72.5)"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\BBh$
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(207.5,72.5)"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\BBh$
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(35,40)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\EQLS
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(190,40)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\EQLS
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 stroke-width= "0.7"
%	 anchor-point= "(35,105)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\totall
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 stroke-width= "0.7"
%	 anchor-point= "(190,105)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\singlevalued
%</text>
%</jpic>
%%End JPIC-XML
%PSTricks content-type (pstricks.sty package needed)
%Add \usepackage{pstricks} in the preamble of your LaTeX file
%You can rescale the whole picture (to 80% for instance) by using the command \def\JPicScale{0.8}
\ifx\JPicScale\undefined\def\JPicScale{1}\fi
\psset{unit=\JPicScale mm}
\psset{linewidth=0.3,dotsep=1,hatchwidth=0.3,hatchsep=1.5,shadowsize=1,dimen=middle}
\psset{dotsize=0.7 2.5,dotscale=1 1,fillcolor=black}
\psset{arrowsize=1 2,arrowlength=1,arrowinset=0.25,tbarsize=0.7 5,bracketlength=0.15,rbracketlength=0.15}
\begin{pspicture}(0,0)(237.5,105)
\psline[linewidth=0.75](50,75)(50,0)
\newrgbcolor{userFillColour}{0.2 0 0.2}
\rput{0}(50,75){\psellipse[fillcolor=userFillColour,fillstyle=solid](0,0)(4.07,-4.07)}
\psline[linewidth=0.75](165,35)(150,20)
\psline[linewidth=0.75](150,20)(150,0)
\newrgbcolor{userFillColour}{0.2 0 0.2}
\rput{0}(150,20){\psellipse[fillcolor=userFillColour,fillstyle=solid](0,0)(3.79,-3.79)}
\psline[linewidth=0.6](135,45)(135,35)
\psline[linewidth=0.75](135,35)(150,20)
\psline[linewidth=0.6](165,45)(165,35)
\rput[r](217.5,0){$\AAh$}
\rput[l](12.5,60){$\BBh$}
\rput[r](147.5,0){$\AAh$}
\rput[l](167.5,73.75){$\BBh$}
\rput[l](137.5,73.75){$\BBh$}
\psline[linewidth=0.75](10,30)(10,0)
\newrgbcolor{userFillColour}{0.2 0 0.2}
\rput{0}(10,75){\psellipse[fillcolor=userFillColour,fillstyle=solid](0,0)(3.79,-3.79)}
\rput[r](7.5,0){$\AAh$}
\pspolygon[linewidth=0.7,fillcolor=white,fillstyle=solid](0,50)(20,50)(20,30)(0,30)
\rput(10,40){$\aah$}
\psline[linewidth=0.75](135,75)(135,65)
\pspolygon[linewidth=0.7,fillcolor=white,fillstyle=solid](125,65)(145,65)(145,45)(125,45)
\rput(135,55){$\aah$}
\pspolygon[linewidth=0.7,fillcolor=white,fillstyle=solid](155,65)(175,65)(175,45)(155,45)
\rput(165,55){$\aah$}
\psline[linewidth=0.75](165,75)(165,65)
\psline[linewidth=0.75](10,73.75)(10,50)
\rput[r](47.5,0){$\AAh$}
\psline[linewidth=0.75](220,10)(220,0)
\pspolygon[linewidth=0.7,fillcolor=white,fillstyle=solid](210,30)(230,30)(230,10)(210,10)
\rput(220,20){$\aah$}
\psline[linewidth=0.75](235,55)(220,40)
\psline[linewidth=0.75](220,40)(220,30)
\newrgbcolor{userFillColour}{0.2 0 0.2}
\rput{0}(220,40){\psellipse[fillcolor=userFillColour,fillstyle=solid](0,0)(3.79,-3.79)}
\psline[linewidth=0.6](205,73.75)(205,55)
\psline[linewidth=0.75](205,55)(220,40)
\psline[linewidth=0.6](235,73.75)(235,55)
\rput[l](237.5,72.5){$\BBh$}
\rput[l](207.5,72.5){$\BBh$}
\rput(35,40){\EQLS}
\rput(190,40){\EQLS}
\rput(35,105){\totall}
\rput(190,105){\singlevalued}
\end{pspicture}


==> PIC/strict-sv-4.tex <==
%%Created by jPicEdt 1.4.1_03: mixed JPIC-XML/LaTeX format
%%Sun Nov 03 14:47:08 GMT-10:00 2019
%%Begin JPIC-XML
%<?xml version="1.0" standalone="yes"?>
%<jpic x-min="-15" x-max="17.5" y-min="-35" y-max="38.75" auto-bounding="true">
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(-2.5,-35)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\AAh$
%</text>
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(0,-25);(0,-25);(0,-35);(0,-35)"
%	 />
%<parallelogram fill-style= "solid"
%	 p3= "(10,-25)"
%	 p2= "(10,-5)"
%	 stroke-width= "0.7"
%	 p1= "(-10,-5)"
%	 fill-color= "#ffffff"
%	 />
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(0,-15)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\aah$
%</text>
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(15,20);(15,20);(0,5);(0,5)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(0,5);(0,5);(0,-5);(0,-5)"
%	 />
%<ellipse fill-style= "solid"
%	 p3= "(3.79,1.21)"
%	 p2= "(3.79,8.79)"
%	 p1= "(-3.79,8.79)"
%	 fill-color= "#330033"
%	 closure= "open"
%	 angle-end= "0"
%	 angle-start= "0"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.6"
%	 points= "(-15,38.75);(-15,38.75);(-15,20);(-15,20)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(-15,20);(-15,20);(0,5);(0,5)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.6"
%	 points= "(15,38.75);(15,38.75);(15,20);(15,20)"
%	 />
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(17.5,37.5)"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\BBh$
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(-12.5,37.5)"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\BBh$
%</text>
%</jpic>
%%End JPIC-XML
%PSTricks content-type (pstricks.sty package needed)
%Add \usepackage{pstricks} in the preamble of your LaTeX file
%You can rescale the whole picture (to 80% for instance) by using the command \def\JPicScale{0.8}
\ifx\JPicScale\undefined\def\JPicScale{1}\fi
\psset{unit=\JPicScale mm}
\psset{linewidth=0.3,dotsep=1,hatchwidth=0.3,hatchsep=1.5,shadowsize=1,dimen=middle}
\psset{dotsize=0.7 2.5,dotscale=1 1,fillcolor=black}
\psset{arrowsize=1 2,arrowlength=1,arrowinset=0.25,tbarsize=0.7 5,bracketlength=0.15,rbracketlength=0.15}
\begin{pspicture}(0,0)(17.5,38.75)
\rput[r](-2.5,-35){$\AAh$}
\psline[linewidth=0.75](0,-25)(0,-35)
\pspolygon[linewidth=0.7,fillcolor=white,fillstyle=solid](-10,-5)(10,-5)(10,-25)(-10,-25)
\rput(0,-15){$\aah$}
\psline[linewidth=0.75](15,20)(0,5)
\psline[linewidth=0.75](0,5)(0,-5)
\newrgbcolor{userFillColour}{0.2 0 0.2}
\rput{0}(0,5){\psellipse[fillcolor=userFillColour,fillstyle=solid](0,0)(3.79,-3.79)}
\psline[linewidth=0.6](-15,38.75)(-15,20)
\psline[linewidth=0.75](-15,20)(0,5)
\psline[linewidth=0.6](15,38.75)(15,20)
\rput[l](17.5,37.5){$\BBh$}
\rput[l](-12.5,37.5){$\BBh$}
\end{pspicture}


==> PIC/strict.tex <==
%%Created by jPicEdt 1.4.1_03: mixed JPIC-XML/LaTeX format
%%Sat Nov 02 18:55:56 GMT-10:00 2019
%%Begin JPIC-XML
%<?xml version="1.0" standalone="yes"?>
%<jpic x-min="0" x-max="237.5" y-min="0" y-max="79.07" auto-bounding="true">
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(50,75);(50,75);(50,0);(50,0)"
%	 />
%<ellipse fill-style= "solid"
%	 p3= "(54.07,70.93)"
%	 p2= "(54.07,79.07)"
%	 p1= "(45.93,79.07)"
%	 fill-color= "#330033"
%	 closure= "open"
%	 angle-end= "0"
%	 angle-start= "0"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(165,35);(165,35);(150,20);(150,20)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(150,20);(150,20);(150,0);(150,0)"
%	 />
%<ellipse fill-style= "solid"
%	 p3= "(153.79,16.21)"
%	 p2= "(153.79,23.79)"
%	 p1= "(146.21,23.79)"
%	 fill-color= "#330033"
%	 closure= "open"
%	 angle-end= "0"
%	 angle-start= "0"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.6"
%	 points= "(135,45);(135,45);(135,35);(135,35)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(135,35);(135,35);(150,20);(150,20)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.6"
%	 points= "(165,45);(165,45);(165,35);(165,35)"
%	 />
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(217.5,0)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\AAh$
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(12.5,60)"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\BBh$
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(147.5,0)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\AAh$
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(167.5,73.75)"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\BBh$
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(137.5,73.75)"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\BBh$
%</text>
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(10,30);(10,30);(10,0);(10,0)"
%	 />
%<ellipse fill-style= "solid"
%	 p3= "(13.79,71.21)"
%	 p2= "(13.79,78.79)"
%	 p1= "(6.21,78.79)"
%	 fill-color= "#330033"
%	 closure= "open"
%	 angle-end= "0"
%	 angle-start= "0"
%	 />
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(7.5,0)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\AAh$
%</text>
%<parallelogram fill-style= "solid"
%	 p3= "(20,30)"
%	 p2= "(20,50)"
%	 stroke-width= "0.7"
%	 p1= "(0,50)"
%	 fill-color= "#ffffff"
%	 />
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(10,40)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\aah$
%</text>
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(135,75);(135,75);(135,65);(135,65)"
%	 />
%<parallelogram fill-style= "solid"
%	 p3= "(145,45)"
%	 p2= "(145,65)"
%	 stroke-width= "0.7"
%	 p1= "(125,65)"
%	 fill-color= "#ffffff"
%	 />
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(135,55)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\aah$
%</text>
%<parallelogram fill-style= "solid"
%	 p3= "(175,45)"
%	 p2= "(175,65)"
%	 stroke-width= "0.7"
%	 p1= "(155,65)"
%	 fill-color= "#ffffff"
%	 />
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(165,55)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\aah$
%</text>
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(165,75);(165,75);(165,65);(165,65)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(10,73.75);(10,73.75);(10,50);(10,50)"
%	 />
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(47.5,0)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\AAh$
%</text>
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(220,10);(220,10);(220,0);(220,0)"
%	 />
%<parallelogram fill-style= "solid"
%	 p3= "(230,10)"
%	 p2= "(230,30)"
%	 stroke-width= "0.7"
%	 p1= "(210,30)"
%	 fill-color= "#ffffff"
%	 />
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(220,20)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\aah$
%</text>
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(235,55);(235,55);(220,40);(220,40)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(220,40);(220,40);(220,30);(220,30)"
%	 />
%<ellipse fill-style= "solid"
%	 p3= "(223.79,36.21)"
%	 p2= "(223.79,43.79)"
%	 p1= "(216.21,43.79)"
%	 fill-color= "#330033"
%	 closure= "open"
%	 angle-end= "0"
%	 angle-start= "0"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.6"
%	 points= "(205,73.75);(205,73.75);(205,55);(205,55)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(205,55);(205,55);(220,40);(220,40)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.6"
%	 points= "(235,73.75);(235,73.75);(235,55);(235,55)"
%	 />
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(237.5,72.5)"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\BBh$
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(207.5,72.5)"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\BBh$
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(35,40)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\EQLS
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(190,40)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\EQLS
%</text>
%</jpic>
%%End JPIC-XML
%PSTricks content-type (pstricks.sty package needed)
%Add \usepackage{pstricks} in the preamble of your LaTeX file
%You can rescale the whole picture (to 80% for instance) by using the command \def\JPicScale{0.8}
\ifx\JPicScale\undefined\def\JPicScale{1}\fi
\psset{unit=\JPicScale mm}
\psset{linewidth=0.3,dotsep=1,hatchwidth=0.3,hatchsep=1.5,shadowsize=1,dimen=middle}
\psset{dotsize=0.7 2.5,dotscale=1 1,fillcolor=black}
\psset{arrowsize=1 2,arrowlength=1,arrowinset=0.25,tbarsize=0.7 5,bracketlength=0.15,rbracketlength=0.15}
\begin{pspicture}(0,0)(237.5,79.07)
\psline[linewidth=0.75](50,75)(50,0)
\newrgbcolor{userFillColour}{0.2 0 0.2}
\rput{0}(50,75){\psellipse[fillcolor=userFillColour,fillstyle=solid](0,0)(4.07,-4.07)}
\psline[linewidth=0.75](165,35)(150,20)
\psline[linewidth=0.75](150,20)(150,0)
\newrgbcolor{userFillColour}{0.2 0 0.2}
\rput{0}(150,20){\psellipse[fillcolor=userFillColour,fillstyle=solid](0,0)(3.79,-3.79)}
\psline[linewidth=0.6](135,45)(135,35)
\psline[linewidth=0.75](135,35)(150,20)
\psline[linewidth=0.6](165,45)(165,35)
\rput[r](217.5,0){$\AAh$}
\rput[l](12.5,60){$\BBh$}
\rput[r](147.5,0){$\AAh$}
\rput[l](167.5,73.75){$\BBh$}
\rput[l](137.5,73.75){$\BBh$}
\psline[linewidth=0.75](10,30)(10,0)
\newrgbcolor{userFillColour}{0.2 0 0.2}
\rput{0}(10,75){\psellipse[fillcolor=userFillColour,fillstyle=solid](0,0)(3.79,-3.79)}
\rput[r](7.5,0){$\AAh$}
\pspolygon[linewidth=0.7,fillcolor=white,fillstyle=solid](0,50)(20,50)(20,30)(0,30)
\rput(10,40){$\aah$}
\psline[linewidth=0.75](135,75)(135,65)
\pspolygon[linewidth=0.7,fillcolor=white,fillstyle=solid](125,65)(145,65)(145,45)(125,45)
\rput(135,55){$\aah$}
\pspolygon[linewidth=0.7,fillcolor=white,fillstyle=solid](155,65)(175,65)(175,45)(155,45)
\rput(165,55){$\aah$}
\psline[linewidth=0.75](165,75)(165,65)
\psline[linewidth=0.75](10,73.75)(10,50)
\rput[r](47.5,0){$\AAh$}
\psline[linewidth=0.75](220,10)(220,0)
\pspolygon[linewidth=0.7,fillcolor=white,fillstyle=solid](210,30)(230,30)(230,10)(210,10)
\rput(220,20){$\aah$}
\psline[linewidth=0.75](235,55)(220,40)
\psline[linewidth=0.75](220,40)(220,30)
\newrgbcolor{userFillColour}{0.2 0 0.2}
\rput{0}(220,40){\psellipse[fillcolor=userFillColour,fillstyle=solid](0,0)(3.79,-3.79)}
\psline[linewidth=0.6](205,73.75)(205,55)
\psline[linewidth=0.75](205,55)(220,40)
\psline[linewidth=0.6](235,73.75)(235,55)
\rput[l](237.5,72.5){$\BBh$}
\rput[l](207.5,72.5){$\BBh$}
\rput(35,40){\EQLS}
\rput(190,40){\EQLS}
\end{pspicture}


==> PIC/strings-0.tex <==
%%Created by jPicEdt 1.4.1_03: mixed JPIC-XML/LaTeX format
%%Tue Oct 23 15:34:50 GMT-05:00 2018
%%Begin JPIC-XML
%<?xml version="1.0" standalone="yes"?>
%<jpic x-min="0" x-max="52.5" y-min="-1.88" y-max="85" auto-bounding="true">
%<ellipse p3= "(24.06,78.44)"
%	 fill-style= "solid"
%	 p2= "(24.06,81.56)"
%	 p1= "(20.94,81.56)"
%	 closure= "open"
%	 angle-end= "0"
%	 angle-start= "0"
%	 />
%<multicurve fill-style= "none"
%	 points= "(7.5,55);(7.5,55);(17.5,55);(17.5,55);(17.5,55);(12.5,50);
%	(12.5,50);(12.5,50);(7.5,55);(7.5,55)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(22.5,75);(22.5,75);(22.5,81.25);(22.5,81.25)"
%	 />
%<parallelogram p3= "(52.5,70)"
%	 fill-style= "none"
%	 p2= "(52.5,75)"
%	 p1= "(7.5,75)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(12.5,65);(12.5,65);(12.5,70);(12.5,70)"
%	 />
%<parallelogram p3= "(51.25,60)"
%	 fill-style= "none"
%	 p2= "(51.25,65)"
%	 p1= "(43.75,65)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(32.5,50);(32.5,50);(32.5,70);(32.5,70)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(37.5,35);(37.5,35);(37.5,70);(37.5,70)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(47.5,65);(47.5,65);(47.5,70);(47.5,70)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(47.5,45);(47.5,45);(47.5,60);(47.5,60)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(37.5,35);(37.5,35);(47.5,45);(47.5,45)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(17.5,35);(17.5,35);(32.5,50);(32.5,50)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-overstrike-width= "1"
%	 points= "(22.5,50);(22.5,50);(37.5,35);(37.5,35)"
%	 stroke-overstrike= "true"
%	 />
%<ellipse p3= "(39.06,33.44)"
%	 fill-style= "solid"
%	 p2= "(39.06,36.56)"
%	 p1= "(35.94,36.56)"
%	 closure= "open"
%	 angle-end= "0"
%	 angle-start= "0"
%	 />
%<parallelogram p3= "(25,60)"
%	 fill-style= "none"
%	 p2= "(25,65)"
%	 p1= "(0,65)"
%	 />
%<ellipse p3= "(19.06,33.44)"
%	 fill-style= "solid"
%	 p2= "(19.06,36.56)"
%	 p1= "(15.94,36.56)"
%	 closure= "open"
%	 angle-end= "0"
%	 angle-start= "0"
%	 />
%<multicurve fill-style= "none"
%	 points= "(2.5,50);(2.5,50);(17.5,35);(17.5,35)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(2.5,50);(2.5,50);(2.5,60);(2.5,60)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(22.5,50);(22.5,50);(22.5,60);(22.5,60)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(37.5,75);(37.5,75);(37.5,83.75);(37.5,83.75)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(17.5,25);(17.5,25);(17.5,35);(17.5,35)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(17.5,5);(17.5,5);(37.5,25);(37.5,25)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(37.5,25);(37.5,25);(37.5,35);(37.5,35)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-overstrike-width= "1"
%	 points= "(17.5,25);(17.5,25);(37.5,5);(37.5,5)"
%	 stroke-overstrike= "true"
%	 />
%<multicurve fill-style= "none"
%	 points= "(37.5,0);(37.5,0);(37.5,5);(37.5,5)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(17.5,0);(17.5,0);(17.5,5);(17.5,5)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(12.5,55);(12.5,55);(12.5,60);(12.5,60)"
%	 />
%<text text-vert-align= "top"
%	 fill-style= "none"
%	 anchor-point= "(52.5,85)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%\northeast
%</text>
%<text text-vert-align= "top"
%	 fill-style= "none"
%	 anchor-point= "(0,85)"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%\northwest
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(47.5,62.5)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\gee$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(12.5,62.5)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\fun$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(30,72.5)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\eich$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(12.5,53.12)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\zero$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(16.88,3.12)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\Ah$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(36.88,3.12)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\Bee$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(16.88,30)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\Bee$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(36.88,30)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\Ah$
%</text>
%<text text-vert-align= "top"
%	 fill-style= "none"
%	 anchor-point= "(17.5,-1.88)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\eex$
%</text>
%<text text-vert-align= "top"
%	 fill-style= "none"
%	 anchor-point= "(37.5,-1.25)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\why$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(36.88,78.75)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\Eee$
%</text>
%</jpic>
%%End JPIC-XML
%PSTricks content-type (pstricks.sty package needed)
%Add \usepackage{pstricks} in the preamble of your LaTeX file
%You can rescale the whole picture (to 80% for instance) by using the command \def\JPicScale{0.8}
\ifx\JPicScale\undefined\def\JPicScale{1}\fi
\psset{unit=\JPicScale mm}
\psset{linewidth=0.3,dotsep=1,hatchwidth=0.3,hatchsep=1.5,shadowsize=1,dimen=middle}
\psset{dotsize=0.7 2.5,dotscale=1 1,fillcolor=black}
\psset{arrowsize=1 2,arrowlength=1,arrowinset=0.25,tbarsize=0.7 5,bracketlength=0.15,rbracketlength=0.15}
\begin{pspicture}(0,0)(52.5,85)
\rput{90}(22.5,80){\psellipse[fillstyle=solid](0,0)(1.56,-1.56)}
\psline(7.5,55)
(17.5,55)
(12.5,50)(7.5,55)
\psline(22.5,75)(22.5,81.25)
\pspolygon[](7.5,75)(52.5,75)(52.5,70)(7.5,70)
\psline(12.5,65)(12.5,70)
\pspolygon[](43.75,65)(51.25,65)(51.25,60)(43.75,60)
\psline(32.5,50)(32.5,70)
\psline(37.5,35)(37.5,70)
\psline(47.5,65)(47.5,70)
\psline(47.5,45)(47.5,60)
\psline(37.5,35)(47.5,45)
\psline(17.5,35)(32.5,50)
\psline[border=1](22.5,50)(37.5,35)
\rput{0}(37.5,35){\psellipse[fillstyle=solid](0,0)(1.56,-1.56)}
\pspolygon[](0,65)(25,65)(25,60)(0,60)
\rput{0}(17.5,35){\psellipse[fillstyle=solid](0,0)(1.56,-1.56)}
\psline(2.5,50)(17.5,35)
\psline(2.5,50)(2.5,60)
\psline(22.5,50)(22.5,60)
\psline(37.5,75)(37.5,83.75)
\psline(17.5,25)(17.5,35)
\psline(17.5,5)(37.5,25)
\psline(37.5,25)(37.5,35)
\psline[border=1](17.5,25)(37.5,5)
\psline(37.5,0)(37.5,5)
\psline(17.5,0)(17.5,5)
\psline(12.5,55)(12.5,60)
\rput[tr](52.5,85){\northeast}
\rput[tl](0,85){\northwest}
\rput(47.5,62.5){$\gee$}
\rput(12.5,62.5){$\fun$}
\rput(30,72.5){$\eich$}
\rput(12.5,53.12){$\zero$}
\rput[r](16.88,3.12){$\Ah$}
\rput[r](36.88,3.12){$\Bee$}
\rput[r](16.88,30){$\Bee$}
\rput[r](36.88,30){$\Ah$}
\rput[t](17.5,-1.88){$\eex$}
\rput[t](37.5,-1.25){$\why$}
\rput[r](36.88,78.75){$\Eee$}
\end{pspicture}


==> PIC/successor.tex <==
%%Created by jPicEdt 1.4.1_03: mixed JPIC-XML/LaTeX format
%%Fri Sep 05 14:02:52 HST 2014
%%Begin JPIC-XML
%<?xml version="1.0" standalone="yes"?>
%<jpic x-min="0" x-max="140" y-min="5.62" y-max="55" auto-bounding="true">
%<text stroke-width= "1"
%	 text-vert-align= "center-v"
%	 anchor-point= "(32.5,40)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\oneleft
%</text>
%<text stroke-width= "1"
%	 text-vert-align= "center-v"
%	 anchor-point= "(122.5,40)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\oneright
%</text>
%<ellipse stroke-width= "1.05"
%	 p3= "(137.5,25)"
%	 p2= "(137.5,55)"
%	 p1= "(107.5,55)"
%	 closure= "open"
%	 fill-style= "none"
%	 angle-end= "0"
%	 angle-start= "0"
%	 />
%<ellipse stroke-width= "1.05"
%	 p3= "(47.5,25)"
%	 p2= "(47.5,55)"
%	 p1= "(17.5,55)"
%	 closure= "open"
%	 fill-style= "none"
%	 angle-end= "0"
%	 angle-start= "0"
%	 />
%<multicurve arrow-head-width-minimum= "2"
%	 stroke-width= "0.8"
%	 right-arrow= "head"
%	 arrow-bracket-length-scale= "0.65"
%	 arrow-head-length-scale= "1.5"
%	 arrow-head-inset-scale= "0"
%	 fill-style= "none"
%	 points= "(50,40);(50,40);(105,40);(105,40)"
%	 />
%<ellipse arrow-head-width-minimum= "2"
%	 stroke-width= "0.8"
%	 p3= "(140,8.12)"
%	 p2= "(105,8.12)"
%	 right-arrow= "head"
%	 p1= "(105,26.88)"
%	 arrow-head-length-scale= "2"
%	 closure= "open"
%	 fill-style= "none"
%	 angle-end= "144.46"
%	 angle-start= "-147.99"
%	 />
%<multicurve arrow-head-width-minimum= "2"
%	 stroke-width= "0.8"
%	 right-arrow= "head"
%	 arrow-bracket-length-scale= "0.65"
%	 arrow-head-length-scale= "1.5"
%	 arrow-head-inset-scale= "0"
%	 fill-style= "none"
%	 points= "(0,40);(0,40);(17.5,40);(17.5,40)"
%	 />
%<ellipse arrow-head-width-minimum= "2"
%	 stroke-width= "0.8"
%	 p3= "(50,8.12)"
%	 p2= "(15,8.12)"
%	 right-arrow= "head"
%	 p1= "(15,26.88)"
%	 arrow-head-length-scale= "2"
%	 closure= "open"
%	 fill-style= "none"
%	 angle-end= "144.46"
%	 angle-start= "-147.99"
%	 />
%<text text-vert-align= "bottom"
%	 anchor-point= "(72.5,41.88)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\transtwo
%</text>
%<text text-vert-align= "top"
%	 anchor-point= "(31.88,5.62)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\transone
%</text>
%<text text-vert-align= "top"
%	 anchor-point= "(122.5,5.62)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\transthree
%</text>
%</jpic>
%%End JPIC-XML
%PSTricks content-type (pstricks.sty package needed)
%Add \usepackage{pstricks} in the preamble of your LaTeX file
%You can rescale the whole picture (to 80% for instance) by using the command \def\JPicScale{0.8}
\ifx\JPicScale\undefined\def\JPicScale{1}\fi
\psset{unit=\JPicScale mm}
\psset{linewidth=0.3,dotsep=1,hatchwidth=0.3,hatchsep=1.5,shadowsize=1,dimen=middle}
\psset{dotsize=0.7 2.5,dotscale=1 1,fillcolor=black}
\psset{arrowsize=1 2,arrowlength=1,arrowinset=0.25,tbarsize=0.7 5,bracketlength=0.15,rbracketlength=0.15}
\begin{pspicture}(0,0)(140,55)
\rput(32.5,40){\oneleft}
\rput(122.5,40){\oneright}
\rput{0}(122.5,40){\psellipse[linewidth=1.05](0,0)(15,-15)}
\rput{0}(32.5,40){\psellipse[linewidth=1.05](0,0)(15,-15)}
\psline[linewidth=0.8,arrowsize=2 2,arrowlength=1.5,arrowinset=0,bracketlength=0.65]{->}(50,40)(105,40)
\rput{0}(122.5,17.5){\psellipticarc[linewidth=0.8,arrowsize=2 2,arrowlength=2]{->}(0,0)(17.5,9.38){122.01}{414.46}}
\psline[linewidth=0.8,arrowsize=2 2,arrowlength=1.5,arrowinset=0,bracketlength=0.65]{->}(0,40)(17.5,40)
\rput{0}(32.5,17.5){\psellipticarc[linewidth=0.8,arrowsize=2 2,arrowlength=2]{->}(0,0)(17.5,9.38){122.01}{414.46}}
\rput[b](72.5,41.88){\transtwo}
\rput[t](31.88,5.62){\transone}
\rput[t](122.5,5.62){\transthree}
\end{pspicture}


==> PIC/summary-TM.tex <==
%%Created by jPicEdt 1.4.1_03: mixed JPIC-XML/LaTeX format
%%Tue Jan 31 22:41:59 GMT 2012
%%Begin JPIC-XML
%<?xml version="1.0" standalone="yes"?>
%<jpic x-min="5" x-max="68" y-min="0" y-max="60" auto-bounding="true">
%<text text-vert-align= "center-v"
%	 anchor-point= "(7,10)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%\one
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(20,43)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\two
%</text>
%<multicurve stroke-width= "0.4"
%	 fill-style= "none"
%	 arrow-head-width-minimum= "1.25"
%	 right-arrow= "head"
%	 points= "(53.75,40);(53.75,40);(61.25,40);(61.25,40)"
%	 arrow-head-length-scale= "1.6"
%	 />
%<text text-vert-align= "center-v"
%	 anchor-point= "(50,39.75)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\iso$
%</text>
%<multicurve stroke-width= "0.4"
%	 fill-style= "none"
%	 arrow-head-width-minimum= "1.25"
%	 right-arrow= "head"
%	 points= "(46.88,40);(46.88,40);(40,40);(40,40)"
%	 arrow-head-length-scale= "1.6"
%	 />
%<multicurve stroke-width= "0.4"
%	 fill-style= "none"
%	 arrow-head-width-minimum= "1.25"
%	 right-arrow= "head"
%	 points= "(53.75,20);(53.75,20);(60.62,20);(60.62,20)"
%	 arrow-head-length-scale= "1.6"
%	 />
%<text text-vert-align= "center-v"
%	 anchor-point= "(50,19.75)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\iso$
%</text>
%<multicurve stroke-width= "0.4"
%	 fill-style= "none"
%	 arrow-head-width-minimum= "1.25"
%	 right-arrow= "head"
%	 points= "(46.88,20);(46.88,20);(40,20);(40,20)"
%	 arrow-head-length-scale= "1.6"
%	 />
%<multicurve stroke-width= "0.4"
%	 fill-style= "none"
%	 arrow-head-width-minimum= "1.25"
%	 right-arrow= "head"
%	 points= "(23.75,40);(23.75,40);(31.25,40);(31.25,40)"
%	 arrow-head-length-scale= "1.6"
%	 />
%<text text-vert-align= "center-v"
%	 anchor-point= "(20,39.75)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\iso$
%</text>
%<multicurve stroke-width= "0.4"
%	 fill-style= "none"
%	 arrow-head-width-minimum= "1.25"
%	 right-arrow= "head"
%	 points= "(16.88,40);(16.88,40);(10.62,40);(10.62,40)"
%	 arrow-head-length-scale= "1.6"
%	 />
%<multicurve stroke-width= "0.4"
%	 fill-style= "none"
%	 arrow-head-width-minimum= "1.25"
%	 right-arrow= "head"
%	 points= "(23.75,20);(23.75,20);(31.25,20);(31.25,20)"
%	 arrow-head-length-scale= "1.6"
%	 />
%<text text-vert-align= "center-v"
%	 anchor-point= "(20,19.75)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\iso$
%</text>
%<multicurve stroke-width= "0.4"
%	 fill-style= "none"
%	 arrow-head-width-minimum= "1.25"
%	 right-arrow= "head"
%	 points= "(16.88,20);(16.88,20);(10.62,20);(10.62,20)"
%	 arrow-head-length-scale= "1.6"
%	 />
%<text text-vert-align= "center-v"
%	 anchor-point= "(20,23)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\two
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(7,50)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%\one
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(50,43)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\three
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(50,23)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\four
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(63,30)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%\five
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(68,30)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%\six
%</text>
%<multicurve stroke-width= "0.4"
%	 fill-style= "none"
%	 arrow-head-width-minimum= "1.25"
%	 right-arrow= "head"
%	 points= "(65,47);(65,47);(65,42);(65,42)"
%	 arrow-head-length-scale= "1.6"
%	 />
%<text text-vert-align= "center-v"
%	 anchor-point= "(65,49.38)"
%	 fill-style= "none"
%	 text-rotation= "90"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\iso$
%</text>
%<multicurve stroke-width= "0.4"
%	 fill-style= "none"
%	 arrow-head-width-minimum= "1.25"
%	 right-arrow= "head"
%	 points= "(65,52);(65,52);(65,58);(65,58)"
%	 arrow-head-length-scale= "1.6"
%	 />
%<text text-vert-align= "center-v"
%	 anchor-point= "(5,40)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\CTF$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(35,20)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\RPF$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(65,20)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\RE$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(5,20)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\CPF$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(35,40)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\RTF$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(65,40)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\REC$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(65,60)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\NREC$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(5,60)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\NCTF$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(5,0)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\NCPF$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(65,0)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\NRE$
%</text>
%<multicurve stroke-width= "0.4"
%	 fill-style= "none"
%	 arrow-head-width-minimum= "1.35"
%	 right-arrow= "double-head"
%	 points= "(67,24);(67,24);(67,37);(67,37)"
%	 arrow-head-length-scale= "1.75"
%	 />
%<multicurve stroke-width= "0.4"
%	 fill-style= "none"
%	 arrow-head-width-minimum= "1.35"
%	 right-arrow= "head"
%	 left-arrow= "reverse-head"
%	 points= "(64,37);(64,37);(64,23);(64,23)"
%	 arrow-head-length-scale= "1.75"
%	 />
%<multicurve stroke-width= "0.4"
%	 fill-style= "none"
%	 arrow-head-width-minimum= "1.25"
%	 right-arrow= "head"
%	 points= "(5,47);(5,47);(5,42);(5,42)"
%	 arrow-head-length-scale= "1.6"
%	 />
%<text text-vert-align= "center-v"
%	 anchor-point= "(5,49.38)"
%	 fill-style= "none"
%	 text-rotation= "90"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\iso$
%</text>
%<multicurve stroke-width= "0.4"
%	 fill-style= "none"
%	 arrow-head-width-minimum= "1.25"
%	 right-arrow= "head"
%	 points= "(5,52);(5,52);(5,58);(5,58)"
%	 arrow-head-length-scale= "1.6"
%	 />
%<multicurve stroke-width= "0.4"
%	 fill-style= "none"
%	 arrow-head-width-minimum= "1.25"
%	 right-arrow= "head"
%	 points= "(5,7);(5,7);(5,2);(5,2)"
%	 arrow-head-length-scale= "1.6"
%	 />
%<text text-vert-align= "center-v"
%	 anchor-point= "(5,9.38)"
%	 fill-style= "none"
%	 text-rotation= "90"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\iso$
%</text>
%<multicurve stroke-width= "0.4"
%	 fill-style= "none"
%	 arrow-head-width-minimum= "1.25"
%	 right-arrow= "head"
%	 points= "(5,12);(5,12);(5,18);(5,18)"
%	 arrow-head-length-scale= "1.6"
%	 />
%<multicurve stroke-width= "0.4"
%	 fill-style= "none"
%	 arrow-head-width-minimum= "1.25"
%	 right-arrow= "head"
%	 points= "(65,7);(65,7);(65,2);(65,2)"
%	 arrow-head-length-scale= "1.6"
%	 />
%<text text-vert-align= "center-v"
%	 anchor-point= "(65,9.38)"
%	 fill-style= "none"
%	 text-rotation= "90"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\iso$
%</text>
%<multicurve stroke-width= "0.4"
%	 fill-style= "none"
%	 arrow-head-width-minimum= "1.25"
%	 right-arrow= "head"
%	 points= "(65,12);(65,12);(65,18);(65,18)"
%	 arrow-head-length-scale= "1.6"
%	 />
%</jpic>
%%End JPIC-XML
%PSTricks content-type (pstricks.sty package needed)
%Add \usepackage{pstricks} in the preamble of your LaTeX file
%You can rescale the whole picture (to 80% for instance) by using the command \def\JPicScale{0.8}
\ifx\JPicScale\undefined\def\JPicScale{1}\fi
\psset{unit=\JPicScale mm}
\psset{linewidth=0.3,dotsep=1,hatchwidth=0.3,hatchsep=1.5,shadowsize=1,dimen=middle}
\psset{dotsize=0.7 2.5,dotscale=1 1,fillcolor=black}
\psset{arrowsize=1 2,arrowlength=1,arrowinset=0.25,tbarsize=0.7 5,bracketlength=0.15,rbracketlength=0.15}
\begin{pspicture}(0,0)(68,60)
\rput[l](7,10){\one}
\rput(20,43){\two}
\psline[linewidth=0.4,arrowsize=1.25 2,arrowlength=1.6]{->}(53.75,40)(61.25,40)
\rput(50,39.75){$\iso$}
\psline[linewidth=0.4,arrowsize=1.25 2,arrowlength=1.6]{->}(46.88,40)(40,40)
\psline[linewidth=0.4,arrowsize=1.25 2,arrowlength=1.6]{->}(53.75,20)(60.62,20)
\rput(50,19.75){$\iso$}
\psline[linewidth=0.4,arrowsize=1.25 2,arrowlength=1.6]{->}(46.88,20)(40,20)
\psline[linewidth=0.4,arrowsize=1.25 2,arrowlength=1.6]{->}(23.75,40)(31.25,40)
\rput(20,39.75){$\iso$}
\psline[linewidth=0.4,arrowsize=1.25 2,arrowlength=1.6]{->}(16.88,40)(10.62,40)
\psline[linewidth=0.4,arrowsize=1.25 2,arrowlength=1.6]{->}(23.75,20)(31.25,20)
\rput(20,19.75){$\iso$}
\psline[linewidth=0.4,arrowsize=1.25 2,arrowlength=1.6]{->}(16.88,20)(10.62,20)
\rput(20,23){\two}
\rput[l](7,50){\one}
\rput(50,43){\three}
\rput(50,23){\four}
\rput[r](63,30){\five}
\rput[l](68,30){\six}
\psline[linewidth=0.4,arrowsize=1.25 2,arrowlength=1.6]{->}(65,47)(65,42)
\rput{90}(65,49.38){$\iso$}
\psline[linewidth=0.4,arrowsize=1.25 2,arrowlength=1.6]{->}(65,52)(65,58)
\rput(5,40){$\CTF$}
\rput(35,20){$\RPF$}
\rput(65,20){$\RE$}
\rput(5,20){$\CPF$}
\rput(35,40){$\RTF$}
\rput(65,40){$\REC$}
\rput(65,60){$\NREC$}
\rput(5,60){$\NCTF$}
\rput(5,0){$\NCPF$}
\rput(65,0){$\NRE$}
\psline[linewidth=0.4,arrowsize=1.35 2,arrowlength=1.75]{->>}(67,24)(67,37)
\psline[linewidth=0.4,arrowsize=1.35 2,arrowlength=1.75]{>->}(64,37)(64,23)
\psline[linewidth=0.4,arrowsize=1.25 2,arrowlength=1.6]{->}(5,47)(5,42)
\rput{90}(5,49.38){$\iso$}
\psline[linewidth=0.4,arrowsize=1.25 2,arrowlength=1.6]{->}(5,52)(5,58)
\psline[linewidth=0.4,arrowsize=1.25 2,arrowlength=1.6]{->}(5,7)(5,2)
\rput{90}(5,9.38){$\iso$}
\psline[linewidth=0.4,arrowsize=1.25 2,arrowlength=1.6]{->}(5,12)(5,18)
\psline[linewidth=0.4,arrowsize=1.25 2,arrowlength=1.6]{->}(65,7)(65,2)
\rput{90}(65,9.38){$\iso$}
\psline[linewidth=0.4,arrowsize=1.25 2,arrowlength=1.6]{->}(65,12)(65,18)
\end{pspicture}


==> PIC/summary.tex <==
%%Created by jPicEdt 1.4.1_03: mixed JPIC-XML/LaTeX format
%%Fri Jan 20 11:51:11 GMT 2012
%%Begin JPIC-XML
%<?xml version="1.0" standalone="yes"?>
%<jpic x-min="5" x-max="75" y-min="-0.25" y-max="43" auto-bounding="true">
%<text text-vert-align= "center-v"
%	 anchor-point= "(5,40)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\REG
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(5,20)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\REGF
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(5,0)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\REGR
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(35,0)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\MoR
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(65,0)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\MeR
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(35,20)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\MoF
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(65,20)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\MeF
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(35,40)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\DL
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(65,40)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\NL
%</text>
%<multicurve stroke-width= "0.4"
%	 fill-style= "none"
%	 arrow-head-width-minimum= "1.25"
%	 right-arrow= "head"
%	 points= "(23.75,40);(23.75,40);(31.25,40);(31.25,40)"
%	 arrow-head-length-scale= "1.6"
%	 />
%<text text-vert-align= "center-v"
%	 anchor-point= "(20,39.75)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\iso$
%</text>
%<multicurve stroke-width= "0.4"
%	 fill-style= "none"
%	 arrow-head-width-minimum= "1.25"
%	 right-arrow= "head"
%	 points= "(16.88,40);(16.88,40);(10,40);(10,40)"
%	 arrow-head-length-scale= "1.6"
%	 />
%<text text-vert-align= "center-v"
%	 anchor-point= "(20,43)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\one
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(20,23)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\two
%</text>
%<multicurve stroke-width= "0.4"
%	 fill-style= "none"
%	 arrow-head-width-minimum= "1.25"
%	 right-arrow= "head"
%	 points= "(53.75,40);(53.75,40);(61.25,40);(61.25,40)"
%	 arrow-head-length-scale= "1.6"
%	 />
%<text text-vert-align= "center-v"
%	 anchor-point= "(50,39.75)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\iso$
%</text>
%<multicurve stroke-width= "0.4"
%	 fill-style= "none"
%	 arrow-head-width-minimum= "1.25"
%	 right-arrow= "head"
%	 points= "(46.88,40);(46.88,40);(40,40);(40,40)"
%	 arrow-head-length-scale= "1.6"
%	 />
%<multicurve stroke-width= "0.4"
%	 fill-style= "none"
%	 arrow-head-width-minimum= "1.25"
%	 right-arrow= "head"
%	 points= "(53.75,20);(53.75,20);(61.25,20);(61.25,20)"
%	 arrow-head-length-scale= "1.6"
%	 />
%<text text-vert-align= "center-v"
%	 anchor-point= "(50,19.75)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\iso$
%</text>
%<multicurve stroke-width= "0.4"
%	 fill-style= "none"
%	 arrow-head-width-minimum= "1.25"
%	 right-arrow= "head"
%	 points= "(46.88,20);(46.88,20);(40,20);(40,20)"
%	 arrow-head-length-scale= "1.6"
%	 />
%<multicurve stroke-width= "0.4"
%	 fill-style= "none"
%	 arrow-head-width-minimum= "1.25"
%	 right-arrow= "head"
%	 points= "(53.75,0);(53.75,0);(60.62,0);(60.62,0)"
%	 arrow-head-length-scale= "1.6"
%	 />
%<text text-vert-align= "center-v"
%	 anchor-point= "(50,-0.25)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\iso$
%</text>
%<multicurve stroke-width= "0.4"
%	 fill-style= "none"
%	 arrow-head-width-minimum= "1.25"
%	 right-arrow= "head"
%	 points= "(46.88,0);(46.88,0);(40,0);(40,0)"
%	 arrow-head-length-scale= "1.6"
%	 />
%<multicurve stroke-width= "0.4"
%	 fill-style= "none"
%	 arrow-head-width-minimum= "1.25"
%	 right-arrow= "head"
%	 points= "(23.75,20);(23.75,20);(31.25,20);(31.25,20)"
%	 arrow-head-length-scale= "1.6"
%	 />
%<text text-vert-align= "center-v"
%	 anchor-point= "(20,19.75)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\iso$
%</text>
%<multicurve stroke-width= "0.4"
%	 fill-style= "none"
%	 arrow-head-width-minimum= "1.25"
%	 right-arrow= "head"
%	 points= "(16.88,20);(16.88,20);(10.62,20);(10.62,20)"
%	 arrow-head-length-scale= "1.6"
%	 />
%<multicurve stroke-width= "0.4"
%	 fill-style= "none"
%	 arrow-head-width-minimum= "1.25"
%	 right-arrow= "head"
%	 points= "(23.75,0);(23.75,0);(31.25,0);(31.25,0)"
%	 arrow-head-length-scale= "1.6"
%	 />
%<text text-vert-align= "center-v"
%	 anchor-point= "(20,-0.25)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\iso$
%</text>
%<multicurve stroke-width= "0.4"
%	 fill-style= "none"
%	 arrow-head-width-minimum= "1.25"
%	 right-arrow= "head"
%	 points= "(16.88,0);(16.88,0);(10.62,0);(10.62,0)"
%	 arrow-head-length-scale= "1.6"
%	 />
%<text text-vert-align= "center-v"
%	 anchor-point= "(50,23)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\two
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(50,43)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\one
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(20,3)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\three
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(50,3)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\three
%</text>
%<multicurve stroke-width= "0.4"
%	 fill-style= "none"
%	 arrow-head-width-minimum= "1.35"
%	 right-arrow= "head"
%	 left-arrow= "reverse-head"
%	 points= "(35,36.25);(35,36.25);(35,22.5);(35,22.5)"
%	 arrow-head-length-scale= "1.75"
%	 />
%<multicurve stroke-width= "0.4"
%	 fill-style= "none"
%	 arrow-head-width-minimum= "1.35"
%	 right-arrow= "head"
%	 left-arrow= "reverse-head"
%	 points= "(35,17.5);(35,17.5);(35,3.75);(35,3.75)"
%	 arrow-head-length-scale= "1.75"
%	 />
%<multicurve stroke-width= "0.4"
%	 fill-style= "none"
%	 arrow-head-width-minimum= "1.35"
%	 right-arrow= "head"
%	 left-arrow= "reverse-head"
%	 points= "(65,23.75);(65,23.75);(65,36.25);(65,36.25)"
%	 arrow-head-length-scale= "1.75"
%	 />
%<multicurve stroke-width= "0.4"
%	 fill-style= "none"
%	 points= "(65,2.5);(65,2.5);(68.75,7.5);(70.62,10.62);(72.5,13.75);(73.75,18.12);
%	(73.75,21.88);(73.75,25.62);(73.12,28.75);(71.25,31.88);(69.38,35);(66.88,36.88);
%	(66.88,36.88)"
%	 />
%<multicurve stroke-width= "0.25"
%	 fill-style= "none"
%	 arrow-head-width-minimum= "1.35"
%	 right-arrow= "head"
%	 points= "(68.75,35);(68.75,35);(66.88,36.88);(66.88,36.88)"
%	 arrow-head-length-scale= "1.75"
%	 />
%<multicurve stroke-width= "0.25"
%	 fill-style= "none"
%	 arrow-head-width-minimum= "1.35"
%	 right-arrow= "head"
%	 points= "(65,2.5);(65,2.5);(66.88,5);(66.88,5)"
%	 arrow-head-length-scale= "1.75"
%	 />
%<text text-vert-align= "center-v"
%	 anchor-point= "(32.5,30)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%\four
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(63.12,30)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%\five
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(75,22.5)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%\six
%</text>
%</jpic>
%%End JPIC-XML
%PSTricks content-type (pstricks.sty package needed)
%Add \usepackage{pstricks} in the preamble of your LaTeX file
%You can rescale the whole picture (to 80% for instance) by using the command \def\JPicScale{0.8}
\ifx\JPicScale\undefined\def\JPicScale{1}\fi
\psset{unit=\JPicScale mm}
\psset{linewidth=0.3,dotsep=1,hatchwidth=0.3,hatchsep=1.5,shadowsize=1,dimen=middle}
\psset{dotsize=0.7 2.5,dotscale=1 1,fillcolor=black}
\psset{arrowsize=1 2,arrowlength=1,arrowinset=0.25,tbarsize=0.7 5,bracketlength=0.15,rbracketlength=0.15}
\begin{pspicture}(0,0)(75,43)
\rput(5,40){\REG}
\rput(5,20){\REGF}
\rput(5,0){\REGR}
\rput(35,0){\MoR}
\rput(65,0){\MeR}
\rput(35,20){\MoF}
\rput(65,20){\MeF}
\rput(35,40){\DL}
\rput(65,40){\NL}
\psline[linewidth=0.4,arrowsize=1.25 2,arrowlength=1.6]{->}(23.75,40)(31.25,40)
\rput(20,39.75){$\iso$}
\psline[linewidth=0.4,arrowsize=1.25 2,arrowlength=1.6]{->}(16.88,40)(10,40)
\rput(20,43){\one}
\rput(20,23){\two}
\psline[linewidth=0.4,arrowsize=1.25 2,arrowlength=1.6]{->}(53.75,40)(61.25,40)
\rput(50,39.75){$\iso$}
\psline[linewidth=0.4,arrowsize=1.25 2,arrowlength=1.6]{->}(46.88,40)(40,40)
\psline[linewidth=0.4,arrowsize=1.25 2,arrowlength=1.6]{->}(53.75,20)(61.25,20)
\rput(50,19.75){$\iso$}
\psline[linewidth=0.4,arrowsize=1.25 2,arrowlength=1.6]{->}(46.88,20)(40,20)
\psline[linewidth=0.4,arrowsize=1.25 2,arrowlength=1.6]{->}(53.75,0)(60.62,0)
\rput(50,-0.25){$\iso$}
\psline[linewidth=0.4,arrowsize=1.25 2,arrowlength=1.6]{->}(46.88,0)(40,0)
\psline[linewidth=0.4,arrowsize=1.25 2,arrowlength=1.6]{->}(23.75,20)(31.25,20)
\rput(20,19.75){$\iso$}
\psline[linewidth=0.4,arrowsize=1.25 2,arrowlength=1.6]{->}(16.88,20)(10.62,20)
\psline[linewidth=0.4,arrowsize=1.25 2,arrowlength=1.6]{->}(23.75,0)(31.25,0)
\rput(20,-0.25){$\iso$}
\psline[linewidth=0.4,arrowsize=1.25 2,arrowlength=1.6]{->}(16.88,0)(10.62,0)
\rput(50,23){\two}
\rput(50,43){\one}
\rput(20,3){\three}
\rput(50,3){\three}
\psline[linewidth=0.4,arrowsize=1.35 2,arrowlength=1.75]{>->}(35,36.25)(35,22.5)
\psline[linewidth=0.4,arrowsize=1.35 2,arrowlength=1.75]{>->}(35,17.5)(35,3.75)
\psline[linewidth=0.4,arrowsize=1.35 2,arrowlength=1.75]{>->}(65,23.75)(65,36.25)
\pscustom[linewidth=0.4]{\psbezier(65,2.5)(65,2.5)(68.75,7.5)(70.62,10.62)
\psbezier(72.5,13.75)(73.75,18.12)(73.75,21.88)
\psbezier(73.75,25.62)(73.12,28.75)(71.25,31.88)
\psbezier(69.38,35)(66.88,36.88)(66.88,36.88)
}
\psline[linewidth=0.25,arrowsize=1.35 2,arrowlength=1.75]{->}(68.75,35)(66.88,36.88)
\psline[linewidth=0.25,arrowsize=1.35 2,arrowlength=1.75]{->}(65,2.5)(66.88,5)
\rput[r](32.5,30){\four}
\rput[r](63.12,30){\five}
\rput[l](75,22.5){\six}
\end{pspicture}


==> PIC/switch.tex <==
%%Created by jPicEdt 1.4.1_03: mixed JPIC-XML/LaTeX format
%%Sun Oct 09 11:30:08 HST 2016
%%Begin JPIC-XML
%<?xml version="1.0" standalone="yes"?>
%<jpic x-min="8.75" x-max="31.88" y-min="0" y-max="40" auto-bounding="true">
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(30,10);(30,10);(30,0);(30,0)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(30,40);(30,40);(30,30);(30,30)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(10,40);(10,40);(10,30);(10,30)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(30,30);(30,30);(10,10);(10,10)"
%	 />
%<multicurve stroke-overstrike= "true"
%	 stroke-width= "0.75"
%	 stroke-overstrike-width= "1.1"
%	 fill-style= "none"
%	 points= "(10,30);(10,30);(30,10);(30,10)"
%	 />
%<text stroke-width= "0.75"
%	 text-vert-align= "center-v"
%	 anchor-point= "(8.75,37.5)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\inputt$
%</text>
%<text stroke-width= "0.75"
%	 text-vert-align= "center-v"
%	 anchor-point= "(31.88,1.88)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\inputt$
%</text>
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(10,10);(10,10);(10,0);(10,0)"
%	 />
%<text text-vert-align= "center-v"
%	 anchor-point= "(8.75,1.88)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\eem$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(31.88,37.5)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\eem$
%</text>
%</jpic>
%%End JPIC-XML
%PSTricks content-type (pstricks.sty package needed)
%Add \usepackage{pstricks} in the preamble of your LaTeX file
%You can rescale the whole picture (to 80% for instance) by using the command \def\JPicScale{0.8}
\ifx\JPicScale\undefined\def\JPicScale{1}\fi
\psset{unit=\JPicScale mm}
\psset{linewidth=0.3,dotsep=1,hatchwidth=0.3,hatchsep=1.5,shadowsize=1,dimen=middle}
\psset{dotsize=0.7 2.5,dotscale=1 1,fillcolor=black}
\psset{arrowsize=1 2,arrowlength=1,arrowinset=0.25,tbarsize=0.7 5,bracketlength=0.15,rbracketlength=0.15}
\begin{pspicture}(0,0)(31.88,40)
\psline[linewidth=0.75](30,10)(30,0)
\psline[linewidth=0.75](30,40)(30,30)
\psline[linewidth=0.75](10,40)(10,30)
\psline[linewidth=0.75](30,30)(10,10)
\psline[linewidth=0.75,border=1.1](10,30)(30,10)
\rput[r](8.75,37.5){$\inputt$}
\rput[l](31.88,1.88){$\inputt$}
\psline[linewidth=0.75](10,10)(10,0)
\rput[r](8.75,1.88){$\eem$}
\rput[l](31.88,37.5){$\eem$}
\end{pspicture}


==> PIC/sym.tex <==
%%Created by jPicEdt 1.4.1_03: mixed JPIC-XML/LaTeX format
%%Wed Sep 16 18:25:31 GMT-10:00 2020
%%Begin JPIC-XML
%<?xml version="1.0" standalone="yes"?>
%<jpic x-min="3.75" x-max="16.25" y-min="-1.88" y-max="31.25" auto-bounding="true">
%<multicurve fill-style= "none"
%	 points= "(15,30);(15,30);(15,20);(15,20)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(5,30);(5,30);(5,20);(5,20)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(15,20);(15,20);(5,10);(5,10)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(15,10);(15,10);(5,20);(5,20)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(5,10);(5,10);(5,0);(5,0)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(15,10);(15,10);(15,0);(15,0)"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(3.75,5)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\Ah$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(16.25,5)"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\Uh$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(16.25,25)"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\Ah$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(3.75,25)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\Uh$
%</text>
%<text text-vert-align= "top"
%	 fill-style= "none"
%	 anchor-point= "(5,-1.88)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\eex$
%</text>
%<text text-vert-align= "top"
%	 fill-style= "none"
%	 anchor-point= "(15,-1.25)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\why$
%</text>
%<text text-vert-align= "bottom"
%	 fill-style= "none"
%	 anchor-point= "(15,31.25)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\eex$
%</text>
%<text text-vert-align= "bottom"
%	 fill-style= "none"
%	 anchor-point= "(5,31.25)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\why$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(12.5,15)"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\swap$
%</text>
%</jpic>
%%End JPIC-XML
%PSTricks content-type (pstricks.sty package needed)
%Add \usepackage{pstricks} in the preamble of your LaTeX file
%You can rescale the whole picture (to 80% for instance) by using the command \def\JPicScale{0.8}
\ifx\JPicScale\undefined\def\JPicScale{1}\fi
\psset{unit=\JPicScale mm}
\psset{linewidth=0.3,dotsep=1,hatchwidth=0.3,hatchsep=1.5,shadowsize=1,dimen=middle}
\psset{dotsize=0.7 2.5,dotscale=1 1,fillcolor=black}
\psset{arrowsize=1 2,arrowlength=1,arrowinset=0.25,tbarsize=0.7 5,bracketlength=0.15,rbracketlength=0.15}
\begin{pspicture}(0,0)(16.25,31.25)
\psline(15,30)(15,20)
\psline(5,30)(5,20)
\psline(15,20)(5,10)
\psline(15,10)(5,20)
\psline(5,10)(5,0)
\psline(15,10)(15,0)
\rput[r](3.75,5){$\Ah$}
\rput[l](16.25,5){$\Uh$}
\rput[l](16.25,25){$\Ah$}
\rput[r](3.75,25){$\Uh$}
\rput[t](5,-1.88){$\eex$}
\rput[t](15,-1.25){$\why$}
\rput[b](15,31.25){$\eex$}
\rput[b](5,31.25){$\why$}
\rput[l](12.5,15){$\swap$}
\end{pspicture}


==> PIC/tfalse-0.tex <==
%%Created by jPicEdt 1.4.1_03: mixed JPIC-XML/LaTeX format
%%Sun Oct 02 16:48:13 HST 2016
%%Begin JPIC-XML
%<?xml version="1.0" standalone="yes"?>
%<jpic x-min="-10" x-max="130" y-min="0" y-max="100" auto-bounding="true">
%<multicurve stroke-width= "0.75"
%	 points= "(30,100);(30,100);(30,60);(30,60)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.75"
%	 points= "(10.62,80.01);(10.62,80.01);(10.62,60);(10.62,60)"
%	 fill-style= "none"
%	 />
%<ellipse p3= "(13.2,77.42)"
%	 p2= "(13.2,82.58)"
%	 p1= "(8.05,82.58)"
%	 closure= "open"
%	 fill-color= "#330033"
%	 angle-end= "0"
%	 fill-style= "solid"
%	 angle-start= "0"
%	 />
%<multicurve stroke-width= "0.6"
%	 points= "(0,90);(0,90);(40,90);(40,90)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.6"
%	 points= "(40,70);(40,70);(40,90);(40,90)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.6"
%	 points= "(0,70);(0,70);(40,70);(40,70)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.6"
%	 points= "(0,90);(0,90);(0,70);(0,70)"
%	 fill-style= "none"
%	 />
%<text text-vert-align= "center-v"
%	 stroke-width= "0.75"
%	 anchor-point= "(20,50)"
%	 text-frame= "noframe"
%	 fill-style= "none"
%	 text-hor-align= "center-h"
%	 >
%\EQLS
%</text>
%<multicurve stroke-width= "0.75"
%	 points= "(80,30);(80,30);(130,30);(130,30)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.75"
%	 points= "(130,10);(130,10);(130,30);(130,30)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.75"
%	 points= "(115,40);(115,40);(115,30);(115,30)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.75"
%	 points= "(100,10);(100,10);(130,10);(130,10)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.75"
%	 points= "(125,10);(125,10);(125,0);(125,0)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.75"
%	 points= "(90,20.01);(90,20.01);(90,10);(90,10)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.75"
%	 points= "(80,30);(80,30);(100,10);(100,10)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.75"
%	 points= "(80,0);(80,0);(100,0);(100,0)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.75"
%	 points= "(80,0);(80,0);(80,20);(80,20)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.75"
%	 points= "(80,20);(80,20);(100,0);(100,0)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.75"
%	 points= "(105,10);(105,10);(105,0);(105,0)"
%	 fill-style= "none"
%	 />
%<text text-vert-align= "center-v"
%	 stroke-width= "0.75"
%	 anchor-point= "(110,50)"
%	 text-frame= "noframe"
%	 fill-style= "none"
%	 text-hor-align= "center-h"
%	 >
%\EQLS
%</text>
%<multicurve stroke-width= "0.75"
%	 points= "(-10,30);(-10,30);(40,30);(40,30)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.75"
%	 points= "(40,10);(40,10);(40,30);(40,30)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.75"
%	 points= "(25,40);(25,40);(25,30);(25,30)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.75"
%	 points= "(10,10);(10,10);(40,10);(40,10)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.75"
%	 points= "(35,10);(35,10);(35,0);(35,0)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.75"
%	 points= "(0,20.01);(0,20.01);(0,10);(0,10)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.75"
%	 points= "(-10,30);(-10,30);(10,10);(10,10)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.75"
%	 points= "(-10,0);(-10,0);(10,0);(10,0)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.75"
%	 points= "(-10,0);(-10,0);(-10,20);(-10,20)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.75"
%	 points= "(-10,20);(-10,20);(10,0);(10,0)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.75"
%	 points= "(15,10);(15,10);(15,0);(15,0)"
%	 fill-style= "none"
%	 />
%<text text-vert-align= "center-v"
%	 anchor-point= "(85,5)"
%	 text-frame= "noframe"
%	 fill-style= "none"
%	 text-hor-align= "center-h"
%	 >
%$\oone$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(-5,5)"
%	 text-frame= "noframe"
%	 fill-style= "none"
%	 text-hor-align= "center-h"
%	 >
%$\zzero$
%</text>
%<multicurve stroke-width= "0.75"
%	 points= "(100,100);(100,100);(100,60);(100,60)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.75"
%	 points= "(120.62,80.01);(120.62,80.01);(120.62,60);(120.62,60)"
%	 fill-style= "none"
%	 />
%<ellipse p3= "(123.2,77.42)"
%	 p2= "(123.2,82.58)"
%	 p1= "(118.05,82.58)"
%	 closure= "open"
%	 fill-color= "#330033"
%	 angle-end= "0"
%	 fill-style= "solid"
%	 angle-start= "0"
%	 />
%<multicurve stroke-width= "0.6"
%	 points= "(90,90);(90,90);(130,90);(130,90)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.6"
%	 points= "(130,70);(130,70);(130,90);(130,90)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.6"
%	 points= "(90,70);(90,70);(130,70);(130,70)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.6"
%	 points= "(90,90);(90,90);(90,70);(90,70)"
%	 fill-style= "none"
%	 />
%</jpic>
%%End JPIC-XML
%PSTricks content-type (pstricks.sty package needed)
%Add \usepackage{pstricks} in the preamble of your LaTeX file
%You can rescale the whole picture (to 80% for instance) by using the command \def\JPicScale{0.8}
\ifx\JPicScale\undefined\def\JPicScale{1}\fi
\psset{unit=\JPicScale mm}
\psset{linewidth=0.3,dotsep=1,hatchwidth=0.3,hatchsep=1.5,shadowsize=1,dimen=middle}
\psset{dotsize=0.7 2.5,dotscale=1 1,fillcolor=black}
\psset{arrowsize=1 2,arrowlength=1,arrowinset=0.25,tbarsize=0.7 5,bracketlength=0.15,rbracketlength=0.15}
\begin{pspicture}(0,0)(130,100)
\psline[linewidth=0.75](30,100)(30,60)
\psline[linewidth=0.75](10.62,80.01)(10.62,60)
\newrgbcolor{userFillColour}{0.2 0 0.2}
\rput{90}(10.62,80){\psellipse[fillcolor=userFillColour,fillstyle=solid](0,0)(2.58,-2.58)}
\psline[linewidth=0.6](0,90)(40,90)
\psline[linewidth=0.6](40,70)(40,90)
\psline[linewidth=0.6](0,70)(40,70)
\psline[linewidth=0.6](0,90)(0,70)
\rput(20,50){\EQLS}
\psline[linewidth=0.75](80,30)(130,30)
\psline[linewidth=0.75](130,10)(130,30)
\psline[linewidth=0.75](115,40)(115,30)
\psline[linewidth=0.75](100,10)(130,10)
\psline[linewidth=0.75](125,10)(125,0)
\psline[linewidth=0.75](90,20.01)(90,10)
\psline[linewidth=0.75](80,30)(100,10)
\psline[linewidth=0.75](80,0)(100,0)
\psline[linewidth=0.75](80,0)(80,20)
\psline[linewidth=0.75](80,20)(100,0)
\psline[linewidth=0.75](105,10)(105,0)
\rput(110,50){\EQLS}
\psline[linewidth=0.75](-10,30)(40,30)
\psline[linewidth=0.75](40,10)(40,30)
\psline[linewidth=0.75](25,40)(25,30)
\psline[linewidth=0.75](10,10)(40,10)
\psline[linewidth=0.75](35,10)(35,0)
\psline[linewidth=0.75](0,20.01)(0,10)
\psline[linewidth=0.75](-10,30)(10,10)
\psline[linewidth=0.75](-10,0)(10,0)
\psline[linewidth=0.75](-10,0)(-10,20)
\psline[linewidth=0.75](-10,20)(10,0)
\psline[linewidth=0.75](15,10)(15,0)
\rput(85,5){$\oone$}
\rput(-5,5){$\zzero$}
\psline[linewidth=0.75](100,100)(100,60)
\psline[linewidth=0.75](120.62,80.01)(120.62,60)
\newrgbcolor{userFillColour}{0.2 0 0.2}
\rput{90}(120.62,80){\psellipse[fillcolor=userFillColour,fillstyle=solid](0,0)(2.58,-2.58)}
\psline[linewidth=0.6](90,90)(130,90)
\psline[linewidth=0.6](130,70)(130,90)
\psline[linewidth=0.6](90,70)(130,70)
\psline[linewidth=0.6](90,90)(90,70)
\end{pspicture}


==> PIC/tfalse-1.tex <==
%%Created by jPicEdt 1.4.1_03: mixed JPIC-XML/LaTeX format
%%Sun Oct 02 16:49:42 HST 2016
%%Begin JPIC-XML
%<?xml version="1.0" standalone="yes"?>
%<jpic x-min="-10" x-max="130" y-min="0" y-max="100" auto-bounding="true">
%<multicurve stroke-width= "0.75"
%	 points= "(30,100);(30,100);(30,60);(30,60)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.75"
%	 points= "(10.62,80.01);(10.62,80.01);(10.62,60);(10.62,60)"
%	 fill-style= "none"
%	 />
%<ellipse p3= "(13.2,77.42)"
%	 p2= "(13.2,82.58)"
%	 p1= "(8.05,82.58)"
%	 closure= "open"
%	 fill-color= "#330033"
%	 angle-end= "0"
%	 fill-style= "solid"
%	 angle-start= "0"
%	 />
%<multicurve stroke-width= "0.6"
%	 points= "(0,90);(0,90);(40,90);(40,90)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.6"
%	 points= "(40,70);(40,70);(40,90);(40,90)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.6"
%	 points= "(0,70);(0,70);(40,70);(40,70)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.6"
%	 points= "(0,90);(0,90);(0,70);(0,70)"
%	 fill-style= "none"
%	 />
%<text text-vert-align= "center-v"
%	 anchor-point= "(130,0)"
%	 text-frame= "noframe"
%	 fill-style= "none"
%	 text-hor-align= "center-h"
%	 >
%$\oone$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(-10,0)"
%	 text-frame= "noframe"
%	 fill-style= "none"
%	 text-hor-align= "center-h"
%	 >
%$\zzero$
%</text>
%<multicurve stroke-width= "0.75"
%	 points= "(100,100);(100,100);(100,60);(100,60)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.75"
%	 points= "(120.62,80.01);(120.62,80.01);(120.62,60);(120.62,60)"
%	 fill-style= "none"
%	 />
%<ellipse p3= "(123.2,77.42)"
%	 p2= "(123.2,82.58)"
%	 p1= "(118.05,82.58)"
%	 closure= "open"
%	 fill-color= "#330033"
%	 angle-end= "0"
%	 fill-style= "solid"
%	 angle-start= "0"
%	 />
%<multicurve stroke-width= "0.6"
%	 points= "(90,90);(90,90);(130,90);(130,90)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.6"
%	 points= "(130,70);(130,70);(130,90);(130,90)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.6"
%	 points= "(90,70);(90,70);(130,70);(130,70)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.6"
%	 points= "(90,90);(90,90);(90,70);(90,70)"
%	 fill-style= "none"
%	 />
%</jpic>
%%End JPIC-XML
%PSTricks content-type (pstricks.sty package needed)
%Add \usepackage{pstricks} in the preamble of your LaTeX file
%You can rescale the whole picture (to 80% for instance) by using the command \def\JPicScale{0.8}
\ifx\JPicScale\undefined\def\JPicScale{1}\fi
\psset{unit=\JPicScale mm}
\psset{linewidth=0.3,dotsep=1,hatchwidth=0.3,hatchsep=1.5,shadowsize=1,dimen=middle}
\psset{dotsize=0.7 2.5,dotscale=1 1,fillcolor=black}
\psset{arrowsize=1 2,arrowlength=1,arrowinset=0.25,tbarsize=0.7 5,bracketlength=0.15,rbracketlength=0.15}
\begin{pspicture}(0,0)(130,100)
\psline[linewidth=0.75](30,100)(30,60)
\psline[linewidth=0.75](10.62,80.01)(10.62,60)
\newrgbcolor{userFillColour}{0.2 0 0.2}
\rput{90}(10.62,80){\psellipse[fillcolor=userFillColour,fillstyle=solid](0,0)(2.58,-2.58)}
\psline[linewidth=0.6](0,90)(40,90)
\psline[linewidth=0.6](40,70)(40,90)
\psline[linewidth=0.6](0,70)(40,70)
\psline[linewidth=0.6](0,90)(0,70)
\rput(130,0){$\oone$}
\rput(-10,0){$\zzero$}
\psline[linewidth=0.75](100,100)(100,60)
\psline[linewidth=0.75](120.62,80.01)(120.62,60)
\newrgbcolor{userFillColour}{0.2 0 0.2}
\rput{90}(120.62,80){\psellipse[fillcolor=userFillColour,fillstyle=solid](0,0)(2.58,-2.58)}
\psline[linewidth=0.6](90,90)(130,90)
\psline[linewidth=0.6](130,70)(130,90)
\psline[linewidth=0.6](90,70)(130,70)
\psline[linewidth=0.6](90,90)(90,70)
\end{pspicture}


==> PIC/tfalse-2.tex <==
%%Created by jPicEdt 1.4.1_03: mixed JPIC-XML/LaTeX format
%%Mon Oct 03 10:25:17 HST 2016
%%Begin JPIC-XML
%<?xml version="1.0" standalone="yes"?>
%<jpic x-min="0" x-max="130" y-min="0" y-max="120" auto-bounding="true">
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(120,50);(120,50);(120,0);(120,0)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(100,30);(100,30);(100,0);(100,0)"
%	 />
%<ellipse fill-style= "solid"
%	 p3= "(102.58,27.42)"
%	 p2= "(102.58,32.58)"
%	 p1= "(97.42,32.58)"
%	 closure= "open"
%	 fill-color= "#330033"
%	 angle-end= "0"
%	 angle-start= "0"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.6"
%	 points= "(90,40);(90,40);(130,40);(130,40)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.6"
%	 points= "(130,20);(130,20);(130,40);(130,40)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.6"
%	 points= "(90,20);(90,20);(130,20);(130,20)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.6"
%	 points= "(90,40);(90,40);(90,20);(90,20)"
%	 />
%<text fill-style= "none"
%	 stroke-width= "0.75"
%	 text-vert-align= "center-v"
%	 anchor-point= "(70,30)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\EQLS
%</text>
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(0,110);(0,110);(50,110);(50,110)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(50,90);(50,90);(50,110);(50,110)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(35,120);(35,120);(35,110);(35,110)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(20,90);(20,90);(50,90);(50,90)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(45,90);(45,90);(45,70);(45,70)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(10,100.01);(10,100.01);(10,90);(10,90)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(0,110);(0,110);(20,90);(20,90)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(0,80);(0,80);(20,80);(20,80)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(0,80);(0,80);(0,100);(0,100)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(0,100);(0,100);(20,80);(20,80)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(25,90);(25,90);(25,70);(25,70)"
%	 />
%<text fill-style= "none"
%	 stroke-width= "0.75"
%	 text-vert-align= "center-v"
%	 anchor-point= "(70,100)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\EQLS
%</text>
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(0,40);(0,40);(50,40);(50,40)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(50,20);(50,20);(50,40);(50,40)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(35,50);(35,50);(35,40);(35,40)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(20,20);(20,20);(50,20);(50,20)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(45,20);(45,20);(45,0);(45,0)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(10,30.01);(10,30.01);(10,20);(10,20)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(0,40);(0,40);(20,20);(20,20)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(0,10);(0,10);(20,10);(20,10)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(0,10);(0,10);(0,30);(0,30)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(0,30);(0,30);(20,10);(20,10)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(25,20);(25,20);(25,0);(25,0)"
%	 />
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(5,85)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\oone$
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(5,15)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\zzero$
%</text>
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(100,120);(100,120);(100,70);(100,70)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(120,100.01);(120,100.01);(120,70);(120,70)"
%	 />
%<ellipse fill-style= "solid"
%	 p3= "(122.58,97.42)"
%	 p2= "(122.58,102.58)"
%	 p1= "(117.42,102.58)"
%	 closure= "open"
%	 fill-color= "#330033"
%	 angle-end= "0"
%	 angle-start= "0"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.6"
%	 points= "(90,110);(90,110);(130,110);(130,110)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.6"
%	 points= "(130,90);(130,90);(130,110);(130,110)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.6"
%	 points= "(90,90);(90,90);(130,90);(130,90)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.6"
%	 points= "(90,110);(90,110);(90,90);(90,90)"
%	 />
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(30,100)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\ueval$
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(30,30)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\ueval$
%</text>
%</jpic>
%%End JPIC-XML
%PSTricks content-type (pstricks.sty package needed)
%Add \usepackage{pstricks} in the preamble of your LaTeX file
%You can rescale the whole picture (to 80% for instance) by using the command \def\JPicScale{0.8}
\ifx\JPicScale\undefined\def\JPicScale{1}\fi
\psset{unit=\JPicScale mm}
\psset{linewidth=0.3,dotsep=1,hatchwidth=0.3,hatchsep=1.5,shadowsize=1,dimen=middle}
\psset{dotsize=0.7 2.5,dotscale=1 1,fillcolor=black}
\psset{arrowsize=1 2,arrowlength=1,arrowinset=0.25,tbarsize=0.7 5,bracketlength=0.15,rbracketlength=0.15}
\begin{pspicture}(0,0)(130,120)
\psline[linewidth=0.75](120,50)(120,0)
\psline[linewidth=0.75](100,30)(100,0)
\newrgbcolor{userFillColour}{0.2 0 0.2}
\rput{90}(100,30){\psellipse[fillcolor=userFillColour,fillstyle=solid](0,0)(2.58,-2.58)}
\psline[linewidth=0.6](90,40)(130,40)
\psline[linewidth=0.6](130,20)(130,40)
\psline[linewidth=0.6](90,20)(130,20)
\psline[linewidth=0.6](90,40)(90,20)
\rput(70,30){\EQLS}
\psline[linewidth=0.75](0,110)(50,110)
\psline[linewidth=0.75](50,90)(50,110)
\psline[linewidth=0.75](35,120)(35,110)
\psline[linewidth=0.75](20,90)(50,90)
\psline[linewidth=0.75](45,90)(45,70)
\psline[linewidth=0.75](10,100.01)(10,90)
\psline[linewidth=0.75](0,110)(20,90)
\psline[linewidth=0.75](0,80)(20,80)
\psline[linewidth=0.75](0,80)(0,100)
\psline[linewidth=0.75](0,100)(20,80)
\psline[linewidth=0.75](25,90)(25,70)
\rput(70,100){\EQLS}
\psline[linewidth=0.75](0,40)(50,40)
\psline[linewidth=0.75](50,20)(50,40)
\psline[linewidth=0.75](35,50)(35,40)
\psline[linewidth=0.75](20,20)(50,20)
\psline[linewidth=0.75](45,20)(45,0)
\psline[linewidth=0.75](10,30.01)(10,20)
\psline[linewidth=0.75](0,40)(20,20)
\psline[linewidth=0.75](0,10)(20,10)
\psline[linewidth=0.75](0,10)(0,30)
\psline[linewidth=0.75](0,30)(20,10)
\psline[linewidth=0.75](25,20)(25,0)
\rput(5,85){$\oone$}
\rput(5,15){$\zzero$}
\psline[linewidth=0.75](100,120)(100,70)
\psline[linewidth=0.75](120,100.01)(120,70)
\newrgbcolor{userFillColour}{0.2 0 0.2}
\rput{90}(120,100){\psellipse[fillcolor=userFillColour,fillstyle=solid](0,0)(2.58,-2.58)}
\psline[linewidth=0.6](90,110)(130,110)
\psline[linewidth=0.6](130,90)(130,110)
\psline[linewidth=0.6](90,90)(130,90)
\psline[linewidth=0.6](90,110)(90,90)
\rput(30,100){$\ueval$}
\rput(30,30){$\ueval$}
\end{pspicture}


==> PIC/tfalse-3.tex <==
%%Created by jPicEdt 1.4.1_03: mixed JPIC-XML/LaTeX format
%%Mon Oct 03 10:27:37 HST 2016
%%Begin JPIC-XML
%<?xml version="1.0" standalone="yes"?>
%<jpic x-min="0" x-max="130" y-min="0" y-max="120" auto-bounding="true">
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(120,50);(120,50);(120,0);(120,0)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(100,30);(100,30);(100,0);(100,0)"
%	 />
%<ellipse fill-style= "solid"
%	 p3= "(102.58,27.42)"
%	 p2= "(102.58,32.58)"
%	 p1= "(97.42,32.58)"
%	 closure= "open"
%	 fill-color= "#330033"
%	 angle-end= "0"
%	 angle-start= "0"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.6"
%	 points= "(90,40);(90,40);(130,40);(130,40)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.6"
%	 points= "(130,20);(130,20);(130,40);(130,40)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.6"
%	 points= "(90,20);(90,20);(130,20);(130,20)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.6"
%	 points= "(90,40);(90,40);(90,20);(90,20)"
%	 />
%<text fill-style= "none"
%	 stroke-width= "0.75"
%	 text-vert-align= "center-v"
%	 anchor-point= "(0,0)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\EQLS
%</text>
%<text fill-style= "none"
%	 stroke-width= "0.75"
%	 text-vert-align= "center-v"
%	 anchor-point= "(0,120)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\EQLS
%</text>
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(100,120);(100,120);(100,70);(100,70)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(120,100.01);(120,100.01);(120,70);(120,70)"
%	 />
%<ellipse fill-style= "solid"
%	 p3= "(122.58,97.42)"
%	 p2= "(122.58,102.58)"
%	 p1= "(117.42,102.58)"
%	 closure= "open"
%	 fill-color= "#330033"
%	 angle-end= "0"
%	 angle-start= "0"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.6"
%	 points= "(90,110);(90,110);(130,110);(130,110)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.6"
%	 points= "(130,90);(130,90);(130,110);(130,110)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.6"
%	 points= "(90,90);(90,90);(130,90);(130,90)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.6"
%	 points= "(90,110);(90,110);(90,90);(90,90)"
%	 />
%</jpic>
%%End JPIC-XML
%PSTricks content-type (pstricks.sty package needed)
%Add \usepackage{pstricks} in the preamble of your LaTeX file
%You can rescale the whole picture (to 80% for instance) by using the command \def\JPicScale{0.8}
\ifx\JPicScale\undefined\def\JPicScale{1}\fi
\psset{unit=\JPicScale mm}
\psset{linewidth=0.3,dotsep=1,hatchwidth=0.3,hatchsep=1.5,shadowsize=1,dimen=middle}
\psset{dotsize=0.7 2.5,dotscale=1 1,fillcolor=black}
\psset{arrowsize=1 2,arrowlength=1,arrowinset=0.25,tbarsize=0.7 5,bracketlength=0.15,rbracketlength=0.15}
\begin{pspicture}(0,0)(130,120)
\psline[linewidth=0.75](120,50)(120,0)
\psline[linewidth=0.75](100,30)(100,0)
\newrgbcolor{userFillColour}{0.2 0 0.2}
\rput{90}(100,30){\psellipse[fillcolor=userFillColour,fillstyle=solid](0,0)(2.58,-2.58)}
\psline[linewidth=0.6](90,40)(130,40)
\psline[linewidth=0.6](130,20)(130,40)
\psline[linewidth=0.6](90,20)(130,20)
\psline[linewidth=0.6](90,40)(90,20)
\rput(0,0){\EQLS}
\rput(0,120){\EQLS}
\psline[linewidth=0.75](100,120)(100,70)
\psline[linewidth=0.75](120,100.01)(120,70)
\newrgbcolor{userFillColour}{0.2 0 0.2}
\rput{90}(120,100){\psellipse[fillcolor=userFillColour,fillstyle=solid](0,0)(2.58,-2.58)}
\psline[linewidth=0.6](90,110)(130,110)
\psline[linewidth=0.6](130,90)(130,110)
\psline[linewidth=0.6](90,90)(130,90)
\psline[linewidth=0.6](90,110)(90,90)
\end{pspicture}


==> PIC/tfalse-4.tex <==
%%Created by jPicEdt 1.4.1_03: mixed JPIC-XML/LaTeX format
%%Wed May 19 19:41:20 GMT-10:00 2021
%%Begin JPIC-XML
%<?xml version="1.0" standalone="yes"?>
%<jpic x-min="0" x-max="280" y-min="-5" y-max="50" auto-bounding="true">
%<multicurve fill-style= "none"
%	 points= "(270,50);(270,50);(270,0);(270,0)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(250,30);(250,30);(250,0);(250,0)"
%	 stroke-width= "0.75"
%	 />
%<ellipse p3= "(252.58,27.42)"
%	 fill-style= "solid"
%	 p2= "(252.58,32.58)"
%	 fill-color= "#330033"
%	 p1= "(247.42,32.58)"
%	 closure= "open"
%	 angle-end= "0"
%	 angle-start= "0"
%	 />
%<multicurve fill-style= "none"
%	 points= "(240,40);(240,40);(280,40);(280,40)"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(280,20);(280,20);(280,40);(280,40)"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(240,20);(240,20);(280,20);(280,20)"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(240,40);(240,40);(240,20);(240,20)"
%	 stroke-width= "0.35"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(230,30)"
%	 text-frame= "noframe"
%	 stroke-width= "0.75"
%	 text-hor-align= "center-h"
%	 >
%\EQLS
%</text>
%<multicurve fill-style= "none"
%	 points= "(0,40);(0,40);(50,40);(50,40)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(50,20);(50,20);(50,40);(50,40)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(35,50);(35,50);(35,40);(35,40)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(20,20);(20,20);(50,20);(50,20)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(45,20);(45,20);(45,0);(45,0)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(10,30.01);(10,30.01);(10,20);(10,20)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(0,40);(0,40);(20,20);(20,20)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(0,10);(0,10);(20,10);(20,10)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(0,10);(0,10);(0,30);(0,30)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(0,30);(0,30);(20,10);(20,10)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(25,20);(25,20);(25,0);(25,0)"
%	 stroke-width= "0.75"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(60,30)"
%	 text-frame= "noframe"
%	 stroke-width= "0.75"
%	 text-hor-align= "center-h"
%	 >
%\EQLS
%</text>
%<multicurve fill-style= "none"
%	 points= "(170,40);(170,40);(220,40);(220,40)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(220,20);(220,20);(220,40);(220,40)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(205,50);(205,50);(205,40);(205,40)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(190,20);(190,20);(220,20);(220,20)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(215,20);(215,20);(215,0);(215,0)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(180,30.01);(180,30.01);(180,20);(180,20)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(170,40);(170,40);(190,20);(190,20)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(170,10);(170,10);(190,10);(190,10)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(170,10);(170,10);(170,30);(170,30)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(170,30);(170,30);(190,10);(190,10)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(195,20);(195,20);(195,0);(195,0)"
%	 stroke-width= "0.75"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(5,15)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\oone$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(175,15)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\zzero$
%</text>
%<multicurve fill-style= "none"
%	 points= "(80,50);(80,50);(80,0);(80,0)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(100,30.01);(100,30.01);(100,0);(100,0)"
%	 stroke-width= "0.75"
%	 />
%<ellipse p3= "(102.58,27.42)"
%	 fill-style= "solid"
%	 p2= "(102.58,32.58)"
%	 fill-color= "#330033"
%	 p1= "(97.42,32.58)"
%	 closure= "open"
%	 angle-end= "0"
%	 angle-start= "0"
%	 />
%<multicurve fill-style= "none"
%	 points= "(70,40);(70,40);(110,40);(110,40)"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(110,20);(110,20);(110,40);(110,40)"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(70,20);(70,20);(110,20);(110,20)"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(70,40);(70,40);(70,20);(70,20)"
%	 stroke-width= "0.35"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(30,30)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\ueval$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(200,30)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\ueval$
%</text>
%<multicurve fill-style= "none"
%	 points= "(5,35);(5,35);(55,35);(55,35)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(55,15);(55,15);(55,35);(55,35)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(40,45);(40,45);(40,35);(40,35)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(25,15);(25,15);(55,15);(55,15)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(50,15);(50,15);(50,-5);(50,-5)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(15,25.01);(15,25.01);(15,15);(15,15)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(5,35);(5,35);(25,15);(25,15)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(5,5);(5,5);(25,5);(25,5)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(5,5);(5,5);(5,25);(5,25)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(5,25);(5,25);(25,5);(25,5)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(30,15);(30,15);(30,-5);(30,-5)"
%	 stroke-width= "0.75"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(65,25)"
%	 text-frame= "noframe"
%	 stroke-width= "0.75"
%	 text-hor-align= "center-h"
%	 >
%\EQLS
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(10,10)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\oone$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(35,25)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\ueval$
%</text>
%</jpic>
%%End JPIC-XML
%PSTricks content-type (pstricks.sty package needed)
%Add \usepackage{pstricks} in the preamble of your LaTeX file
%You can rescale the whole picture (to 80% for instance) by using the command \def\JPicScale{0.8}
\ifx\JPicScale\undefined\def\JPicScale{1}\fi
\psset{unit=\JPicScale mm}
\psset{linewidth=0.3,dotsep=1,hatchwidth=0.3,hatchsep=1.5,shadowsize=1,dimen=middle}
\psset{dotsize=0.7 2.5,dotscale=1 1,fillcolor=black}
\psset{arrowsize=1 2,arrowlength=1,arrowinset=0.25,tbarsize=0.7 5,bracketlength=0.15,rbracketlength=0.15}
\begin{pspicture}(0,0)(280,50)
\psline[linewidth=0.75](270,50)(270,0)
\psline[linewidth=0.75](250,30)(250,0)
\newrgbcolor{userFillColour}{0.2 0 0.2}
\rput{0}(250,30){\psellipse[fillcolor=userFillColour,fillstyle=solid](0,0)(2.58,-2.58)}
\psline[linewidth=0.35](240,40)(280,40)
\psline[linewidth=0.35](280,20)(280,40)
\psline[linewidth=0.35](240,20)(280,20)
\psline[linewidth=0.35](240,40)(240,20)
\rput(230,30){\EQLS}
\psline[linewidth=0.75](0,40)(50,40)
\psline[linewidth=0.75](50,20)(50,40)
\psline[linewidth=0.75](35,50)(35,40)
\psline[linewidth=0.75](20,20)(50,20)
\psline[linewidth=0.75](45,20)(45,0)
\psline[linewidth=0.75](10,30.01)(10,20)
\psline[linewidth=0.75](0,40)(20,20)
\psline[linewidth=0.75](0,10)(20,10)
\psline[linewidth=0.75](0,10)(0,30)
\psline[linewidth=0.75](0,30)(20,10)
\psline[linewidth=0.75](25,20)(25,0)
\rput(60,30){\EQLS}
\psline[linewidth=0.75](170,40)(220,40)
\psline[linewidth=0.75](220,20)(220,40)
\psline[linewidth=0.75](205,50)(205,40)
\psline[linewidth=0.75](190,20)(220,20)
\psline[linewidth=0.75](215,20)(215,0)
\psline[linewidth=0.75](180,30.01)(180,20)
\psline[linewidth=0.75](170,40)(190,20)
\psline[linewidth=0.75](170,10)(190,10)
\psline[linewidth=0.75](170,10)(170,30)
\psline[linewidth=0.75](170,30)(190,10)
\psline[linewidth=0.75](195,20)(195,0)
\rput(5,15){$\oone$}
\rput(175,15){$\zzero$}
\psline[linewidth=0.75](80,50)(80,0)
\psline[linewidth=0.75](100,30.01)(100,0)
\newrgbcolor{userFillColour}{0.2 0 0.2}
\rput{0}(100,30){\psellipse[fillcolor=userFillColour,fillstyle=solid](0,0)(2.58,-2.58)}
\psline[linewidth=0.35](70,40)(110,40)
\psline[linewidth=0.35](110,20)(110,40)
\psline[linewidth=0.35](70,20)(110,20)
\psline[linewidth=0.35](70,40)(70,20)
\rput(30,30){$\ueval$}
\rput(200,30){$\ueval$}
\psline[linewidth=0.75](5,35)(55,35)
\psline[linewidth=0.75](55,15)(55,35)
\psline[linewidth=0.75](40,45)(40,35)
\psline[linewidth=0.75](25,15)(55,15)
\psline[linewidth=0.75](50,15)(50,-5)
\psline[linewidth=0.75](15,25.01)(15,15)
\psline[linewidth=0.75](5,35)(25,15)
\psline[linewidth=0.75](5,5)(25,5)
\psline[linewidth=0.75](5,5)(5,25)
\psline[linewidth=0.75](5,25)(25,5)
\psline[linewidth=0.75](30,15)(30,-5)
\rput(65,25){\EQLS}
\rput(10,10){$\oone$}
\rput(35,25){$\ueval$}
\end{pspicture}


==> PIC/tfalse-5.tex <==
%%Created by jPicEdt 1.4.1_03: mixed JPIC-XML/LaTeX format
%%Sun Jul 24 16:08:23 GMT+01:00 2022
%%Begin JPIC-XML
%<?xml version="1.0" standalone="yes"?>
%<jpic x-min="0" x-max="200" y-min="0" y-max="50" auto-bounding="true">
%<multicurve fill-style= "none"
%	 points= "(0,35);(0,35);(20,35);(20,35)"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(20,15);(20,15);(20,35);(20,35)"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(10,50);(10,50);(10,35);(10,35)"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(0,15);(0,15);(20,15);(20,15)"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(10,15);(10,15);(10,0);(10,0)"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(0,35);(0,35);(0,15);(0,15)"
%	 stroke-width= "0.35"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(70,30)"
%	 text-frame= "noframe"
%	 stroke-width= "0.35"
%	 text-hor-align= "center-h"
%	 >
%\EQLS
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(185,5)"
%	 text-frame= "noframe"
%	 stroke-width= "0.35"
%	 text-hor-align= "center-h"
%	 >
%$\zzero$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(10,25)"
%	 text-frame= "noframe"
%	 stroke-width= "0.35"
%	 text-hor-align= "center-h"
%	 >
%$\ueval$
%</text>
%<multicurve fill-style= "none"
%	 points= "(40,50);(40,50);(40,10);(40,10)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(30,0);(30,0);(50,0);(50,0)"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(30,0);(30,0);(30,20);(30,20)"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(30,20);(30,20);(50,0);(50,0)"
%	 stroke-width= "0.35"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(35,5)"
%	 text-frame= "noframe"
%	 stroke-width= "0.35"
%	 text-hor-align= "center-h"
%	 >
%$\oone$
%</text>
%<multicurve fill-style= "none"
%	 points= "(90,35);(90,35);(110,35);(110,35)"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(110,15);(110,15);(110,35);(110,35)"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(100,50);(100,50);(100,35);(100,35)"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(90,15);(90,15);(110,15);(110,15)"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(100,15);(100,15);(100,0);(100,0)"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(90,35);(90,35);(90,15);(90,15)"
%	 stroke-width= "0.35"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(100,25)"
%	 text-frame= "noframe"
%	 stroke-width= "0.35"
%	 text-hor-align= "center-h"
%	 >
%$\ueval$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(130,30)"
%	 text-frame= "noframe"
%	 stroke-width= "0.35"
%	 text-hor-align= "center-h"
%	 >
%\EQLS
%</text>
%<multicurve fill-style= "none"
%	 points= "(150,35);(150,35);(170,35);(170,35)"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(170,15);(170,15);(170,35);(170,35)"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(160,50);(160,50);(160,35);(160,35)"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(150,15);(150,15);(170,15);(170,15)"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(160,15);(160,15);(160,0);(160,0)"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(150,35);(150,35);(150,15);(150,15)"
%	 stroke-width= "0.35"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(160,25)"
%	 text-frame= "noframe"
%	 stroke-width= "0.35"
%	 text-hor-align= "center-h"
%	 >
%$\ueval$
%</text>
%<multicurve fill-style= "none"
%	 points= "(190,50);(190,50);(190,10);(190,10)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(180,0);(180,0);(200,0);(200,0)"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(180,0);(180,0);(180,20);(180,20)"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(180,20);(180,20);(200,0);(200,0)"
%	 stroke-width= "0.35"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(40,50)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\DOTT
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(40,10)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\DOTT
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(190,50)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\DOTT
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(190,10)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\DOTT
%</text>
%</jpic>
%%End JPIC-XML
%LaTeX-picture environment using emulated lines and arcs
%You can rescale the whole picture (to 80% for instance) by using the command \def\JPicScale{0.8}
\ifx\JPicScale\undefined\def\JPicScale{1}\fi
\unitlength \JPicScale mm
\begin{picture}(200,50)(0,0)
\linethickness{0.35mm}
\put(0,35){\line(1,0){20}}
\linethickness{0.35mm}
\put(20,15){\line(0,1){20}}
\linethickness{0.35mm}
\put(10,35){\line(0,1){15}}
\linethickness{0.35mm}
\put(0,15){\line(1,0){20}}
\linethickness{0.35mm}
\put(10,0){\line(0,1){15}}
\linethickness{0.35mm}
\put(0,15){\line(0,1){20}}
\put(70,30){\makebox(0,0)[cc]{\EQLS}}

\put(185,5){\makebox(0,0)[cc]{$\zzero$}}

\put(10,25){\makebox(0,0)[cc]{$\ueval$}}

\linethickness{0.75mm}
\put(40,10){\line(0,1){40}}
\linethickness{0.35mm}
\put(30,0){\line(1,0){20}}
\linethickness{0.35mm}
\put(30,0){\line(0,1){20}}
\linethickness{0.35mm}
\multiput(30,20)(0.12,-0.12){167}{\line(1,0){0.12}}
\put(35,5){\makebox(0,0)[cc]{$\oone$}}

\linethickness{0.35mm}
\put(90,35){\line(1,0){20}}
\linethickness{0.35mm}
\put(110,15){\line(0,1){20}}
\linethickness{0.35mm}
\put(100,35){\line(0,1){15}}
\linethickness{0.35mm}
\put(90,15){\line(1,0){20}}
\linethickness{0.35mm}
\put(100,0){\line(0,1){15}}
\linethickness{0.35mm}
\put(90,15){\line(0,1){20}}
\put(100,25){\makebox(0,0)[cc]{$\ueval$}}

\put(130,30){\makebox(0,0)[cc]{\EQLS}}

\linethickness{0.35mm}
\put(150,35){\line(1,0){20}}
\linethickness{0.35mm}
\put(170,15){\line(0,1){20}}
\linethickness{0.35mm}
\put(160,35){\line(0,1){15}}
\linethickness{0.35mm}
\put(150,15){\line(1,0){20}}
\linethickness{0.35mm}
\put(160,0){\line(0,1){15}}
\linethickness{0.35mm}
\put(150,15){\line(0,1){20}}
\put(160,25){\makebox(0,0)[cc]{$\ueval$}}

\linethickness{0.75mm}
\put(190,10){\line(0,1){40}}
\linethickness{0.35mm}
\put(180,0){\line(1,0){20}}
\linethickness{0.35mm}
\put(180,0){\line(0,1){20}}
\linethickness{0.35mm}
\multiput(180,20)(0.12,-0.12){167}{\line(1,0){0.12}}
\put(40,50){\makebox(0,0)[cc]{\DOTT}}

\put(40,10){\makebox(0,0)[cc]{\DOTT}}

\put(190,50){\makebox(0,0)[cc]{\DOTT}}

\put(190,10){\makebox(0,0)[cc]{\DOTT}}

\end{picture}


==> PIC/tfalse-6.tex <==
%%Created by jPicEdt 1.4.1_03: mixed JPIC-XML/LaTeX format
%%Sun Jul 24 16:25:37 GMT+01:00 2022
%%Begin JPIC-XML
%<?xml version="1.0" standalone="yes"?>
%<jpic x-min="0" x-max="200" y-min="0" y-max="50" auto-bounding="true">
%<multicurve fill-style= "none"
%	 points= "(0,35);(0,35);(20,35);(20,35)"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(20,15);(20,15);(20,35);(20,35)"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(10,50);(10,50);(10,35);(10,35)"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(0,15);(0,15);(20,15);(20,15)"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(10,15);(10,15);(10,0);(10,0)"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(0,35);(0,35);(0,15);(0,15)"
%	 stroke-width= "0.35"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(70,30)"
%	 text-frame= "noframe"
%	 stroke-width= "0.35"
%	 text-hor-align= "center-h"
%	 >
%\EQLS
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(185,5)"
%	 text-frame= "noframe"
%	 stroke-width= "0.35"
%	 text-hor-align= "center-h"
%	 >
%$\zzero$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(10,25)"
%	 text-frame= "noframe"
%	 stroke-width= "0.35"
%	 text-hor-align= "center-h"
%	 >
%$\ueval$
%</text>
%<multicurve fill-style= "none"
%	 points= "(40,50);(40,50);(40,10);(40,10)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(30,0);(30,0);(50,0);(50,0)"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(30,0);(30,0);(30,20);(30,20)"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(30,20);(30,20);(50,0);(50,0)"
%	 stroke-width= "0.35"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(35,5)"
%	 text-frame= "noframe"
%	 stroke-width= "0.35"
%	 text-hor-align= "center-h"
%	 >
%$\oone$
%</text>
%<multicurve fill-style= "none"
%	 points= "(90,35);(90,35);(110,35);(110,35)"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(110,15);(110,15);(110,35);(110,35)"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(100,50);(100,50);(100,35);(100,35)"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(90,15);(90,15);(110,15);(110,15)"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(100,15);(100,15);(100,0);(100,0)"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(90,35);(90,35);(90,15);(90,15)"
%	 stroke-width= "0.35"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(100,25)"
%	 text-frame= "noframe"
%	 stroke-width= "0.35"
%	 text-hor-align= "center-h"
%	 >
%$\ueval$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(130,30)"
%	 text-frame= "noframe"
%	 stroke-width= "0.35"
%	 text-hor-align= "center-h"
%	 >
%\EQLS
%</text>
%<multicurve fill-style= "none"
%	 points= "(150,35);(150,35);(170,35);(170,35)"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(170,15);(170,15);(170,35);(170,35)"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(160,50);(160,50);(160,35);(160,35)"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(150,15);(150,15);(170,15);(170,15)"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(160,15);(160,15);(160,0);(160,0)"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(150,35);(150,35);(150,15);(150,15)"
%	 stroke-width= "0.35"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(160,25)"
%	 text-frame= "noframe"
%	 stroke-width= "0.35"
%	 text-hor-align= "center-h"
%	 >
%$\ueval$
%</text>
%<multicurve fill-style= "none"
%	 points= "(190,50);(190,50);(190,10);(190,10)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(180,0);(180,0);(200,0);(200,0)"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(180,0);(180,0);(180,20);(180,20)"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(180,20);(180,20);(200,0);(200,0)"
%	 stroke-width= "0.35"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(40,50)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\Dottt
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(40,10)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\Dottt
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(190,50)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\Dottt
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(190,10)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\Dottt
%</text>
%</jpic>
%%End JPIC-XML
%LaTeX-picture environment using emulated lines and arcs
%You can rescale the whole picture (to 80% for instance) by using the command \def\JPicScale{0.8}
\ifx\JPicScale\undefined\def\JPicScale{1}\fi
\unitlength \JPicScale mm
\begin{picture}(200,50)(0,0)
\linethickness{0.35mm}
\put(0,35){\line(1,0){20}}
\linethickness{0.35mm}
\put(20,15){\line(0,1){20}}
\linethickness{0.35mm}
\put(10,35){\line(0,1){15}}
\linethickness{0.35mm}
\put(0,15){\line(1,0){20}}
\linethickness{0.35mm}
\put(10,0){\line(0,1){15}}
\linethickness{0.35mm}
\put(0,15){\line(0,1){20}}
\put(70,30){\makebox(0,0)[cc]{\EQLS}}

\put(185,5){\makebox(0,0)[cc]{$\zzero$}}

\put(10,25){\makebox(0,0)[cc]{$\ueval$}}

\linethickness{0.75mm}
\put(40,10){\line(0,1){40}}
\linethickness{0.35mm}
\put(30,0){\line(1,0){20}}
\linethickness{0.35mm}
\put(30,0){\line(0,1){20}}
\linethickness{0.35mm}
\multiput(30,20)(0.12,-0.12){167}{\line(1,0){0.12}}
\put(35,5){\makebox(0,0)[cc]{$\oone$}}

\linethickness{0.35mm}
\put(90,35){\line(1,0){20}}
\linethickness{0.35mm}
\put(110,15){\line(0,1){20}}
\linethickness{0.35mm}
\put(100,35){\line(0,1){15}}
\linethickness{0.35mm}
\put(90,15){\line(1,0){20}}
\linethickness{0.35mm}
\put(100,0){\line(0,1){15}}
\linethickness{0.35mm}
\put(90,15){\line(0,1){20}}
\put(100,25){\makebox(0,0)[cc]{$\ueval$}}

\put(130,30){\makebox(0,0)[cc]{\EQLS}}

\linethickness{0.35mm}
\put(150,35){\line(1,0){20}}
\linethickness{0.35mm}
\put(170,15){\line(0,1){20}}
\linethickness{0.35mm}
\put(160,35){\line(0,1){15}}
\linethickness{0.35mm}
\put(150,15){\line(1,0){20}}
\linethickness{0.35mm}
\put(160,0){\line(0,1){15}}
\linethickness{0.35mm}
\put(150,15){\line(0,1){20}}
\put(160,25){\makebox(0,0)[cc]{$\ueval$}}

\linethickness{0.75mm}
\put(190,10){\line(0,1){40}}
\linethickness{0.35mm}
\put(180,0){\line(1,0){20}}
\linethickness{0.35mm}
\put(180,0){\line(0,1){20}}
\linethickness{0.35mm}
\multiput(180,20)(0.12,-0.12){167}{\line(1,0){0.12}}
\put(40,50){\makebox(0,0)[cc]{\Dottt}}

\put(40,10){\makebox(0,0)[cc]{\Dottt}}

\put(190,50){\makebox(0,0)[cc]{\Dottt}}

\put(190,10){\makebox(0,0)[cc]{\Dottt}}

\end{picture}


==> PIC/tracing-accu.tex <==
%%Created by jPicEdt 1.4.1_03: mixed JPIC-XML/LaTeX format
%%Sun Jan 12 12:16:41 GMT-10:00 2020
%%Begin JPIC-XML
%<?xml version="1.0" standalone="yes"?>
%<jpic x-min="-2.5" x-max="375" y-min="0" y-max="150" auto-bounding="true">
%<multicurve fill-style= "none"
%	 points= "(0,70);(0,70);(45,70);(45,70)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(45,50);(45,50);(45,70);(45,70)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(20,50);(20,50);(45,50);(45,50)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(40,50);(40,50);(40,0);(40,0)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(10,35);(10,35);(10,25);(10,25)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(10,60);(10,60);(10,50);(10,50)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(0,70);(0,70);(20,50);(20,50)"
%	 stroke-width= "0.75"
%	 />
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(30,60)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\universal$
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(37.5,0)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\Atype$
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(12.5,150)"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\Progtype$
%</text>
%<multicurve fill-style= "none"
%	 points= "(40,150);(40,150);(40,70);(40,70)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(10,150);(10,150);(10,70);(10,70)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(20,35);(20,35);(0,35);(0,35)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(0,55);(0,55);(0,35);(0,35)"
%	 stroke-width= "0.75"
%	 />
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(42.5,150)"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\Btype$
%</text>
%<multicurve fill-style= "none"
%	 points= "(20,40);(20,40);(20,35);(20,35)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(5,55);(5,55);(0,55);(0,55)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(20,40);(20,40);(5,55);(5,55)"
%	 stroke-width= "0.75"
%	 />
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(7.5,42.5)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\trtr$
%</text>
%<multicurve fill-style= "none"
%	 points= "(10,10);(10,10);(10,0);(10,0)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(20,10);(20,10);(0,10);(0,10)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(0,30);(0,30);(0,10);(0,10)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(20,15);(20,15);(20,10);(20,10)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(5,30);(5,30);(0,30);(0,30)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(20,15);(20,15);(5,30);(5,30)"
%	 stroke-width= "0.75"
%	 />
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(65,60)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\EQLS
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(7.5,0)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\Xtype$
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(12.5,30)"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\Progtype$
%</text>
%<multicurve fill-style= "none"
%	 points= "(215,70);(215,70);(260,70);(260,70)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(260,50);(260,50);(260,70);(260,70)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(235,50);(235,50);(260,50);(260,50)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(255,50);(255,50);(255,0);(255,0)"
%	 stroke-width= "0.75"
%	 />
%<ellipse fill-style= "solid"
%	 p3= "(227.58,12.42)"
%	 fill-color= "#330033"
%	 p2= "(227.58,17.58)"
%	 p1= "(222.42,17.58)"
%	 closure= "open"
%	 angle-end= "0"
%	 angle-start= "0"
%	 />
%<multicurve fill-style= "none"
%	 points= "(195,30);(195,30);(210,15);(210,15)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(225,60);(225,60);(225,52.5);(225,52.5)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(215,70);(215,70);(235,50);(235,50)"
%	 stroke-width= "0.75"
%	 />
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(245,60)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\universal$
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(252.5,0)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\Atype$
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(227.5,120)"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\Progtype$
%</text>
%<multicurve fill-style= "none"
%	 points= "(255,150);(255,150);(255,70);(255,70)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(195,125);(195,125);(195,52.5);(195,52.5)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(190,135);(190,135);(230,135);(230,135)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(230,125);(230,125);(230,135);(230,135)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(210,150);(210,150);(210,135);(210,135)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(190,125);(190,125);(230,125);(230,125)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(190,135);(190,135);(190,125);(190,125)"
%	 stroke-width= "0.75"
%	 />
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(210,130)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\universallift$
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(212.5,148.75)"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\Progtype$
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(257.5,150)"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\Btype$
%</text>
%<multicurve fill-style= "none"
%	 points= "(225,125);(225,125);(225,115);(225,115)"
%	 stroke-width= "0.75"
%	 />
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(227.5,85)"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\Progtype$
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(165,60)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\EQLS
%</text>
%<multicurve fill-style= "none"
%	 points= "(215,120);(215,120);(215,100);(215,100)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(235,105);(235,105);(235,100);(235,100)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(220,120);(220,120);(215,120);(215,120)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(235,105);(235,105);(220,120);(220,120)"
%	 stroke-width= "0.75"
%	 />
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(222.5,107.5)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\trtr$
%</text>
%<multicurve fill-style= "none"
%	 points= "(225,100);(225,100);(225,70);(225,70)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(235,100);(235,100);(215,100);(215,100)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(225,37.5);(225,37.5);(225,0);(225,0)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(235,37.5);(235,37.5);(215,37.5);(215,37.5)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(215,57.5);(215,57.5);(215,37.5);(215,37.5)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(235,42.5);(235,42.5);(235,37.5);(235,37.5)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(220,57.5);(220,57.5);(215,57.5);(215,57.5)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(235,42.5);(235,42.5);(220,57.5);(220,57.5)"
%	 stroke-width= "0.75"
%	 />
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(222.5,0)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\Xtype$
%</text>
%<multicurve fill-style= "none"
%	 points= "(100,70);(100,70);(145,70);(145,70)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(145,50);(145,50);(145,70);(145,70)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(120,50);(120,50);(145,50);(145,50)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(140,50);(140,50);(140,0);(140,0)"
%	 stroke-width= "0.75"
%	 />
%<ellipse fill-style= "solid"
%	 p3= "(112.58,42.42)"
%	 fill-color= "#330033"
%	 p2= "(112.58,47.5)"
%	 p1= "(107.42,47.5)"
%	 closure= "open"
%	 angle-end= "0"
%	 angle-start= "0"
%	 />
%<multicurve fill-style= "none"
%	 points= "(80,60);(80,60);(95,45);(95,45)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(110,60);(110,60);(110,25);(110,25)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(100,70);(100,70);(120,50);(120,50)"
%	 stroke-width= "0.75"
%	 />
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(130,60)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\universal$
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(137.5,0)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\Atype$
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(112.5,120)"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\Progtype$
%</text>
%<multicurve fill-style= "none"
%	 points= "(140,150);(140,150);(140,70);(140,70)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(80,125);(80,125);(80,60);(80,60)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(75,135);(75,135);(115,135);(115,135)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(115,125);(115,125);(115,135);(115,135)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(95,150);(95,150);(95,135);(95,135)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(75,125);(75,125);(115,125);(115,125)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(75,135);(75,135);(75,125);(75,125)"
%	 stroke-width= "0.75"
%	 />
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(95,130)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\universallift$
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(77.5,120)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\Progtype$
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(97.5,148.75)"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\Progtype$
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(142.5,150)"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\Btype$
%</text>
%<multicurve fill-style= "none"
%	 points= "(110,125);(110,125);(110,115);(110,115)"
%	 stroke-width= "0.75"
%	 />
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(112.5,85)"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\Progtype$
%</text>
%<multicurve fill-style= "none"
%	 points= "(100,120);(100,120);(100,100);(100,100)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(120,105);(120,105);(120,100);(120,100)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(105,120);(105,120);(100,120);(100,120)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(120,105);(120,105);(105,120);(105,120)"
%	 stroke-width= "0.75"
%	 />
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(107.5,107.5)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\trtr$
%</text>
%<multicurve fill-style= "none"
%	 points= "(110,100);(110,100);(110,70);(110,70)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(120,100);(120,100);(100,100);(100,100)"
%	 stroke-width= "0.75"
%	 />
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(112.5,30)"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\Progtype$
%</text>
%<multicurve fill-style= "none"
%	 points= "(110,10);(110,10);(110,0);(110,0)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(120,10);(120,10);(100,10);(100,10)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(100,30);(100,30);(100,10);(100,10)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(120,15);(120,15);(120,10);(120,10)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(105,30);(105,30);(100,30);(100,30)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(120,15);(120,15);(105,30);(105,30)"
%	 stroke-width= "0.75"
%	 />
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(107.5,0)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\Xtype$
%</text>
%<multicurve fill-style= "none"
%	 points= "(185,57.5);(185,57.5);(185,37.5);(185,37.5)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(205,42.5);(205,42.5);(205,37.5);(205,37.5)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(190,57.5);(190,57.5);(185,57.5);(185,57.5)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(205,42.5);(205,42.5);(190,57.5);(190,57.5)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(330,70);(330,70);(375,70);(375,70)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(375,50);(375,50);(375,70);(375,70)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(330,50);(330,50);(375,50);(375,50)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(370,50);(370,50);(370,0);(370,0)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(330,70);(330,70);(330,50);(330,50)"
%	 stroke-width= "0.75"
%	 />
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(367.5,0)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\Atype$
%</text>
%<multicurve fill-style= "none"
%	 points= "(370,150);(370,150);(370,70);(370,70)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(310,125);(310,125);(310,90);(310,90)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(305,135);(305,135);(345,135);(345,135)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(345,125);(345,125);(345,135);(345,135)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(325,150);(325,150);(325,135);(325,135)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(305,125);(305,125);(345,125);(345,125)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(340,75);(340,75);(340,70);(340,70)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(305,135);(305,135);(305,125);(305,125)"
%	 stroke-width= "0.75"
%	 />
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(325,130)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\universallift$
%</text>
%<multicurve fill-style= "none"
%	 points= "(350,75);(350,75);(330,75);(330,75)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(330,95);(330,95);(330,75);(330,75)"
%	 stroke-width= "0.75"
%	 />
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(307.5,120)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\Progtype$
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(327.5,150)"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\Progtype$
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(372.5,150)"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\Btype$
%</text>
%<multicurve fill-style= "none"
%	 points= "(350,80);(350,80);(350,75);(350,75)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(335,95);(335,95);(330,95);(330,95)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(340,125);(340,125);(340,115);(340,115)"
%	 stroke-width= "0.75"
%	 />
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(342.5,95)"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\Progtype$
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(280,60)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\EQLS
%</text>
%<multicurve fill-style= "none"
%	 points= "(330,120);(330,120);(330,100);(330,100)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(350,105);(350,105);(350,100);(350,100)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(335,120);(335,120);(330,120);(330,120)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(350,105);(350,105);(335,120);(335,120)"
%	 stroke-width= "0.75"
%	 />
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(337.5,107.5)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\trtr$
%</text>
%<multicurve fill-style= "none"
%	 points= "(340,100);(340,100);(340,90);(340,90)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(350,80);(350,80);(335,95);(335,95)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(350,100);(350,100);(330,100);(330,100)"
%	 stroke-width= "0.75"
%	 />
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(337.5,0)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\Xtype$
%</text>
%<multicurve fill-style= "none"
%	 points= "(320,75);(320,75);(300,75);(300,75)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(300,95);(300,95);(300,75);(300,75)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(320,80);(320,80);(320,75);(320,75)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(305,95);(305,95);(300,95);(300,95)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(320,80);(320,80);(305,95);(305,95)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(195,37.5);(195,37.5);(195,30);(195,30)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(205,37.5);(205,37.5);(185,37.5);(185,37.5)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(210,15);(210,15);(225,15);(225,15)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(95,45);(95,45);(110,45);(110,45)"
%	 stroke-width= "0.75"
%	 />
%<ellipse fill-style= "solid"
%	 p3= "(340.08,12.42)"
%	 fill-color= "#330033"
%	 p2= "(340.08,17.58)"
%	 p1= "(334.92,17.58)"
%	 closure= "open"
%	 angle-end= "0"
%	 angle-start= "0"
%	 />
%<multicurve fill-style= "none"
%	 points= "(307.5,30);(307.5,30);(322.5,15);(322.5,15)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(337.5,50);(337.5,50);(337.5,0);(337.5,0)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(307.5,75);(307.5,75);(307.5,30);(307.5,30)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(322.5,15);(322.5,15);(337.5,15);(337.5,15)"
%	 stroke-width= "0.75"
%	 />
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(7.5,16.25)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\gsim$
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(107.5,16.25)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\gsim$
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(192.5,43.75)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\gsim$
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(222.5,43.75)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\gsim$
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(307.5,81.25)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\gsim$
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(337.5,81.25)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\gsim$
%</text>
%<multicurve fill-style= "none"
%	 stroke-color= "#ff0033"
%	 points= "(352.5,72.5);(352.5,72.5);(327.5,72.5);(327.5,72.5)"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 stroke-color= "#ff0033"
%	 points= "(335,122.5);(335,122.5);(327.5,122.5);(327.5,122.5)"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 stroke-color= "#ff0033"
%	 points= "(352.5,105);(352.5,105);(335,122.5);(335,122.5)"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 stroke-color= "#ff0033"
%	 points= "(352.5,72.5);(352.5,72.5);(352.5,105);(352.5,105)"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 stroke-color= "#ff0033"
%	 points= "(327.5,72.5);(327.5,72.5);(327.5,122.5);(327.5,122.5)"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 stroke-color= "#ff0033"
%	 points= "(22.5,7.5);(22.5,7.5);(-2.5,7.5);(-2.5,7.5)"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 stroke-color= "#ff0033"
%	 points= "(5,57.5);(5,57.5);(-2.5,57.5);(-2.5,57.5)"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 stroke-color= "#ff0033"
%	 points= "(22.5,40);(22.5,40);(5,57.5);(5,57.5)"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 stroke-color= "#ff0033"
%	 points= "(22.5,7.5);(22.5,7.5);(22.5,40);(22.5,40)"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 stroke-color= "#ff0033"
%	 points= "(-2.5,7.5);(-2.5,7.5);(-2.5,57.5);(-2.5,57.5)"
%	 stroke-width= "0.35"
%	 />
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(355,60)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\geee$
%</text>
%</jpic>
%%End JPIC-XML
%PSTricks content-type (pstricks.sty package needed)
%Add \usepackage{pstricks} in the preamble of your LaTeX file
%You can rescale the whole picture (to 80% for instance) by using the command \def\JPicScale{0.8}
\ifx\JPicScale\undefined\def\JPicScale{1}\fi
\psset{unit=\JPicScale mm}
\psset{linewidth=0.3,dotsep=1,hatchwidth=0.3,hatchsep=1.5,shadowsize=1,dimen=middle}
\psset{dotsize=0.7 2.5,dotscale=1 1,fillcolor=black}
\psset{arrowsize=1 2,arrowlength=1,arrowinset=0.25,tbarsize=0.7 5,bracketlength=0.15,rbracketlength=0.15}
\begin{pspicture}(0,0)(375,150)
\psline[linewidth=0.75](0,70)(45,70)
\psline[linewidth=0.75](45,50)(45,70)
\psline[linewidth=0.75](20,50)(45,50)
\psline[linewidth=0.75](40,50)(40,0)
\psline[linewidth=0.75](10,35)(10,25)
\psline[linewidth=0.75](10,60)(10,50)
\psline[linewidth=0.75](0,70)(20,50)
\rput(30,60){$\universal$}
\rput[r](37.5,0){$\Atype$}
\rput[l](12.5,150){$\Progtype$}
\psline[linewidth=0.75](40,150)(40,70)
\psline[linewidth=0.75](10,150)(10,70)
\psline[linewidth=0.75](20,35)(0,35)
\psline[linewidth=0.75](0,55)(0,35)
\rput[l](42.5,150){$\Btype$}
\psline[linewidth=0.75](20,40)(20,35)
\psline[linewidth=0.75](5,55)(0,55)
\psline[linewidth=0.75](20,40)(5,55)
\rput(7.5,42.5){$\trtr$}
\psline[linewidth=0.75](10,10)(10,0)
\psline[linewidth=0.75](20,10)(0,10)
\psline[linewidth=0.75](0,30)(0,10)
\psline[linewidth=0.75](20,15)(20,10)
\psline[linewidth=0.75](5,30)(0,30)
\psline[linewidth=0.75](20,15)(5,30)
\rput(65,60){\EQLS}
\rput[r](7.5,0){$\Xtype$}
\rput[l](12.5,30){$\Progtype$}
\psline[linewidth=0.75](215,70)(260,70)
\psline[linewidth=0.75](260,50)(260,70)
\psline[linewidth=0.75](235,50)(260,50)
\psline[linewidth=0.75](255,50)(255,0)
\newrgbcolor{userFillColour}{0.2 0 0.2}
\rput{0}(225,15){\psellipse[fillcolor=userFillColour,fillstyle=solid](0,0)(2.58,-2.58)}
\psline[linewidth=0.75](195,30)(210,15)
\psline[linewidth=0.75](225,60)(225,52.5)
\psline[linewidth=0.75](215,70)(235,50)
\rput(245,60){$\universal$}
\rput[r](252.5,0){$\Atype$}
\rput[l](227.5,120){$\Progtype$}
\psline[linewidth=0.75](255,150)(255,70)
\psline[linewidth=0.75](195,125)(195,52.5)
\psline[linewidth=0.75](190,135)(230,135)
\psline[linewidth=0.75](230,125)(230,135)
\psline[linewidth=0.75](210,150)(210,135)
\psline[linewidth=0.75](190,125)(230,125)
\psline[linewidth=0.75](190,135)(190,125)
\rput(210,130){$\universallift$}
\rput[l](212.5,148.75){$\Progtype$}
\rput[l](257.5,150){$\Btype$}
\psline[linewidth=0.75](225,125)(225,115)
\rput[l](227.5,85){$\Progtype$}
\rput(165,60){\EQLS}
\psline[linewidth=0.75](215,120)(215,100)
\psline[linewidth=0.75](235,105)(235,100)
\psline[linewidth=0.75](220,120)(215,120)
\psline[linewidth=0.75](235,105)(220,120)
\rput(222.5,107.5){$\trtr$}
\psline[linewidth=0.75](225,100)(225,70)
\psline[linewidth=0.75](235,100)(215,100)
\psline[linewidth=0.75](225,37.5)(225,0)
\psline[linewidth=0.75](235,37.5)(215,37.5)
\psline[linewidth=0.75](215,57.5)(215,37.5)
\psline[linewidth=0.75](235,42.5)(235,37.5)
\psline[linewidth=0.75](220,57.5)(215,57.5)
\psline[linewidth=0.75](235,42.5)(220,57.5)
\rput[r](222.5,0){$\Xtype$}
\psline[linewidth=0.75](100,70)(145,70)
\psline[linewidth=0.75](145,50)(145,70)
\psline[linewidth=0.75](120,50)(145,50)
\psline[linewidth=0.75](140,50)(140,0)
\newrgbcolor{userFillColour}{0.2 0 0.2}
\rput{0}(110,44.96){\psellipse[fillcolor=userFillColour,fillstyle=solid](0,0)(2.58,-2.54)}
\psline[linewidth=0.75](80,60)(95,45)
\psline[linewidth=0.75](110,60)(110,25)
\psline[linewidth=0.75](100,70)(120,50)
\rput(130,60){$\universal$}
\rput[r](137.5,0){$\Atype$}
\rput[l](112.5,120){$\Progtype$}
\psline[linewidth=0.75](140,150)(140,70)
\psline[linewidth=0.75](80,125)(80,60)
\psline[linewidth=0.75](75,135)(115,135)
\psline[linewidth=0.75](115,125)(115,135)
\psline[linewidth=0.75](95,150)(95,135)
\psline[linewidth=0.75](75,125)(115,125)
\psline[linewidth=0.75](75,135)(75,125)
\rput(95,130){$\universallift$}
\rput[r](77.5,120){$\Progtype$}
\rput[l](97.5,148.75){$\Progtype$}
\rput[l](142.5,150){$\Btype$}
\psline[linewidth=0.75](110,125)(110,115)
\rput[l](112.5,85){$\Progtype$}
\psline[linewidth=0.75](100,120)(100,100)
\psline[linewidth=0.75](120,105)(120,100)
\psline[linewidth=0.75](105,120)(100,120)
\psline[linewidth=0.75](120,105)(105,120)
\rput(107.5,107.5){$\trtr$}
\psline[linewidth=0.75](110,100)(110,70)
\psline[linewidth=0.75](120,100)(100,100)
\rput[l](112.5,30){$\Progtype$}
\psline[linewidth=0.75](110,10)(110,0)
\psline[linewidth=0.75](120,10)(100,10)
\psline[linewidth=0.75](100,30)(100,10)
\psline[linewidth=0.75](120,15)(120,10)
\psline[linewidth=0.75](105,30)(100,30)
\psline[linewidth=0.75](120,15)(105,30)
\rput[r](107.5,0){$\Xtype$}
\psline[linewidth=0.75](185,57.5)(185,37.5)
\psline[linewidth=0.75](205,42.5)(205,37.5)
\psline[linewidth=0.75](190,57.5)(185,57.5)
\psline[linewidth=0.75](205,42.5)(190,57.5)
\psline[linewidth=0.75](330,70)(375,70)
\psline[linewidth=0.75](375,50)(375,70)
\psline[linewidth=0.75](330,50)(375,50)
\psline[linewidth=0.75](370,50)(370,0)
\psline[linewidth=0.75](330,70)(330,50)
\rput[r](367.5,0){$\Atype$}
\psline[linewidth=0.75](370,150)(370,70)
\psline[linewidth=0.75](310,125)(310,90)
\psline[linewidth=0.75](305,135)(345,135)
\psline[linewidth=0.75](345,125)(345,135)
\psline[linewidth=0.75](325,150)(325,135)
\psline[linewidth=0.75](305,125)(345,125)
\psline[linewidth=0.75](340,75)(340,70)
\psline[linewidth=0.75](305,135)(305,125)
\rput(325,130){$\universallift$}
\psline[linewidth=0.75](350,75)(330,75)
\psline[linewidth=0.75](330,95)(330,75)
\rput[r](307.5,120){$\Progtype$}
\rput[l](327.5,150){$\Progtype$}
\rput[l](372.5,150){$\Btype$}
\psline[linewidth=0.75](350,80)(350,75)
\psline[linewidth=0.75](335,95)(330,95)
\psline[linewidth=0.75](340,125)(340,115)
\rput[l](342.5,95){$\Progtype$}
\rput(280,60){\EQLS}
\psline[linewidth=0.75](330,120)(330,100)
\psline[linewidth=0.75](350,105)(350,100)
\psline[linewidth=0.75](335,120)(330,120)
\psline[linewidth=0.75](350,105)(335,120)
\rput(337.5,107.5){$\trtr$}
\psline[linewidth=0.75](340,100)(340,90)
\psline[linewidth=0.75](350,80)(335,95)
\psline[linewidth=0.75](350,100)(330,100)
\rput[r](337.5,0){$\Xtype$}
\psline[linewidth=0.75](320,75)(300,75)
\psline[linewidth=0.75](300,95)(300,75)
\psline[linewidth=0.75](320,80)(320,75)
\psline[linewidth=0.75](305,95)(300,95)
\psline[linewidth=0.75](320,80)(305,95)
\psline[linewidth=0.75](195,37.5)(195,30)
\psline[linewidth=0.75](205,37.5)(185,37.5)
\psline[linewidth=0.75](210,15)(225,15)
\psline[linewidth=0.75](95,45)(110,45)
\newrgbcolor{userFillColour}{0.2 0 0.2}
\rput{0}(337.5,15){\psellipse[fillcolor=userFillColour,fillstyle=solid](0,0)(2.58,-2.58)}
\psline[linewidth=0.75](307.5,30)(322.5,15)
\psline[linewidth=0.75](337.5,50)(337.5,0)
\psline[linewidth=0.75](307.5,75)(307.5,30)
\psline[linewidth=0.75](322.5,15)(337.5,15)
\rput(7.5,16.25){$\gsim$}
\rput(107.5,16.25){$\gsim$}
\rput(192.5,43.75){$\gsim$}
\rput(222.5,43.75){$\gsim$}
\rput(307.5,81.25){$\gsim$}
\rput(337.5,81.25){$\gsim$}
\newrgbcolor{userLineColour}{1 0 0.2}
\psline[linewidth=0.35,linecolor=userLineColour](352.5,72.5)(327.5,72.5)
\newrgbcolor{userLineColour}{1 0 0.2}
\psline[linewidth=0.35,linecolor=userLineColour](335,122.5)(327.5,122.5)
\newrgbcolor{userLineColour}{1 0 0.2}
\psline[linewidth=0.35,linecolor=userLineColour](352.5,105)(335,122.5)
\newrgbcolor{userLineColour}{1 0 0.2}
\psline[linewidth=0.35,linecolor=userLineColour](352.5,72.5)(352.5,105)
\newrgbcolor{userLineColour}{1 0 0.2}
\psline[linewidth=0.35,linecolor=userLineColour](327.5,72.5)(327.5,122.5)
\newrgbcolor{userLineColour}{1 0 0.2}
\psline[linewidth=0.35,linecolor=userLineColour](22.5,7.5)(-2.5,7.5)
\newrgbcolor{userLineColour}{1 0 0.2}
\psline[linewidth=0.35,linecolor=userLineColour](5,57.5)(-2.5,57.5)
\newrgbcolor{userLineColour}{1 0 0.2}
\psline[linewidth=0.35,linecolor=userLineColour](22.5,40)(5,57.5)
\newrgbcolor{userLineColour}{1 0 0.2}
\psline[linewidth=0.35,linecolor=userLineColour](22.5,7.5)(22.5,40)
\newrgbcolor{userLineColour}{1 0 0.2}
\psline[linewidth=0.35,linecolor=userLineColour](-2.5,7.5)(-2.5,57.5)
\rput(355,60){$\geee$}
\end{pspicture}


==> PIC/tracingev.tex <==
%%Created by jPicEdt 1.4.1_03: mixed JPIC-XML/LaTeX format
%%Tue Jan 07 17:24:16 GMT-10:00 2020
%%Begin JPIC-XML
%<?xml version="1.0" standalone="yes"?>
%<jpic x-min="-0" x-max="90" y-min="0" y-max="100" auto-bounding="true">
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(20,50);(20,50);(85,50);(85,50)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(85,30);(85,30);(85,50);(85,50)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(40,30);(40,30);(85,30);(85,30)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(80,30);(80,30);(80,0);(80,0)"
%	 />
%<ellipse fill-style= "solid"
%	 p3= "(32.58,27.42)"
%	 p2= "(32.58,32.58)"
%	 p1= "(27.42,32.58)"
%	 fill-color= "#330033"
%	 closure= "open"
%	 angle-end= "0"
%	 angle-start= "0"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(10,50);(10,50);(30,30);(30,30)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(30,40);(30,40);(30,0);(30,0)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(20,50);(20,50);(40,30);(40,30)"
%	 />
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(52.5,40)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\universal$
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(77.5,1.25)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\Atype$
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(27.5,1.25)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\Progtype$
%</text>
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(80,100);(80,100);(80,50);(80,50)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(10,70);(10,70);(10,50);(10,50)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(5,80);(5,80);(35,80);(35,80)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(35,70);(35,70);(35,80);(35,80)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(20,100);(20,100);(20,80);(20,80)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(5,70);(5,70);(35,70);(35,70)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(30,55);(30,55);(30,50);(30,50)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(5,80);(5,80);(5,70);(5,70)"
%	 />
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(20,75)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\universallift$
%</text>
%<multicurve fill-style= "none"
%	 stroke-color= "#ff0033"
%	 points= "(25,25);(25,25);(90,25);(90,25)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-color= "#ff0033"
%	 points= "(90,25);(90,25);(90,55);(90,55)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-color= "#ff0033"
%	 points= "(90,55);(90,55);(65,55);(65,55)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-color= "#ff0033"
%	 points= "(65,55);(65,55);(35,85);(35,85)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-color= "#ff0033"
%	 points= "(25,25);(25,25);(-0,50);(-0,50)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-color= "#ff0033"
%	 points= "(0,85);(0,85);(0,50);(0,50)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-color= "#ff0033"
%	 points= "(35,85);(35,85);(0,85);(0,85)"
%	 />
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(7.5,55)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\Progtype$
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(22.5,98.75)"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\Progtype$
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(82.5,100)"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\Btype$
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(45,60)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\tracing$
%</text>
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(35,55);(35,55);(25,55);(25,55)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(25,65);(25,65);(25,55);(25,55)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(35,57.5);(35,57.5);(35,55);(35,55)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(35,57.5);(35,57.5);(27.5,65);(27.5,65)"
%	 />
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(28.75,58.75)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\trtr$
%</text>
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(27.5,65);(27.5,65);(25,65);(25,65)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(30,70);(30,70);(30,62.5);(30,62.5)"
%	 />
%</jpic>
%%End JPIC-XML
%PSTricks content-type (pstricks.sty package needed)
%Add \usepackage{pstricks} in the preamble of your LaTeX file
%You can rescale the whole picture (to 80% for instance) by using the command \def\JPicScale{0.8}
\ifx\JPicScale\undefined\def\JPicScale{1}\fi
\psset{unit=\JPicScale mm}
\psset{linewidth=0.3,dotsep=1,hatchwidth=0.3,hatchsep=1.5,shadowsize=1,dimen=middle}
\psset{dotsize=0.7 2.5,dotscale=1 1,fillcolor=black}
\psset{arrowsize=1 2,arrowlength=1,arrowinset=0.25,tbarsize=0.7 5,bracketlength=0.15,rbracketlength=0.15}
\begin{pspicture}(0,0)(90,100)
\psline[linewidth=0.75](20,50)(85,50)
\psline[linewidth=0.75](85,30)(85,50)
\psline[linewidth=0.75](40,30)(85,30)
\psline[linewidth=0.75](80,30)(80,0)
\newrgbcolor{userFillColour}{0.2 0 0.2}
\rput{0}(30,30){\psellipse[fillcolor=userFillColour,fillstyle=solid](0,0)(2.58,-2.58)}
\psline[linewidth=0.75](10,50)(30,30)
\psline[linewidth=0.75](30,40)(30,0)
\psline[linewidth=0.75](20,50)(40,30)
\rput(52.5,40){$\universal$}
\rput[r](77.5,1.25){$\Atype$}
\rput[r](27.5,1.25){$\Progtype$}
\psline[linewidth=0.75](80,100)(80,50)
\psline[linewidth=0.75](10,70)(10,50)
\psline[linewidth=0.75](5,80)(35,80)
\psline[linewidth=0.75](35,70)(35,80)
\psline[linewidth=0.75](20,100)(20,80)
\psline[linewidth=0.75](5,70)(35,70)
\psline[linewidth=0.75](30,55)(30,50)
\psline[linewidth=0.75](5,80)(5,70)
\rput(20,75){$\universallift$}
\newrgbcolor{userLineColour}{1 0 0.2}
\psline[linecolor=userLineColour](25,25)(90,25)
\newrgbcolor{userLineColour}{1 0 0.2}
\psline[linecolor=userLineColour](90,25)(90,55)
\newrgbcolor{userLineColour}{1 0 0.2}
\psline[linecolor=userLineColour](90,55)(65,55)
\newrgbcolor{userLineColour}{1 0 0.2}
\psline[linecolor=userLineColour](65,55)(35,85)
\newrgbcolor{userLineColour}{1 0 0.2}
\psline[linecolor=userLineColour](25,25)(-0,50)
\newrgbcolor{userLineColour}{1 0 0.2}
\psline[linecolor=userLineColour](0,85)(0,50)
\newrgbcolor{userLineColour}{1 0 0.2}
\psline[linecolor=userLineColour](35,85)(0,85)
\rput[r](7.5,55){$\Progtype$}
\rput[l](22.5,98.75){$\Progtype$}
\rput[l](82.5,100){$\Btype$}
\rput(45,60){$\tracing$}
\psline[linewidth=0.75](35,55)(25,55)
\psline[linewidth=0.75](25,65)(25,55)
\psline[linewidth=0.75](35,57.5)(35,55)
\psline[linewidth=0.75](35,57.5)(27.5,65)
\rput(28.75,58.75){$\trtr$}
\psline[linewidth=0.75](27.5,65)(25,65)
\psline[linewidth=0.75](30,70)(30,62.5)
\end{pspicture}


==> PIC/tracingproof.tex <==
%%Created by jPicEdt 1.4.1_03: mixed JPIC-XML/LaTeX format
%%Tue Jan 07 22:33:34 GMT-10:00 2020
%%Begin JPIC-XML
%<?xml version="1.0" standalone="yes"?>
%<jpic x-min="0" x-max="257.5" y-min="0" y-max="110" auto-bounding="true">
%<multicurve fill-style= "none"
%	 points= "(27.5,50);(27.5,50);(72.5,50);(72.5,50)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(72.5,30);(72.5,30);(72.5,50);(72.5,50)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(47.5,30);(47.5,30);(72.5,30);(72.5,30)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(67.5,30);(67.5,30);(67.5,0);(67.5,0)"
%	 stroke-width= "0.75"
%	 />
%<ellipse fill-style= "solid"
%	 p3= "(40.08,27.42)"
%	 fill-color= "#330033"
%	 p2= "(40.08,32.58)"
%	 p1= "(34.92,32.58)"
%	 closure= "open"
%	 angle-end= "0"
%	 angle-start= "0"
%	 />
%<multicurve fill-style= "none"
%	 points= "(17.5,50);(17.5,50);(37.5,30);(37.5,30)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(37.5,40);(37.5,40);(37.5,0);(37.5,0)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(27.5,50);(27.5,50);(47.5,30);(47.5,30)"
%	 stroke-width= "0.75"
%	 />
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(57.5,40)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\universal$
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(65,1.25)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\Atype$
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(35,1.25)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\Progtype$
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(35,55)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\Progtype$
%</text>
%<multicurve fill-style= "none"
%	 points= "(67.5,110);(67.5,110);(67.5,50);(67.5,50)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(27.5,70);(27.5,70);(7.5,50);(7.5,50)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(12.5,97.5);(12.5,97.5);(42.5,97.5);(42.5,97.5)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(42.5,87.5);(42.5,87.5);(42.5,97.5);(42.5,97.5)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(27.5,110);(27.5,110);(27.5,97.5);(27.5,97.5)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(37.5,62.5);(37.5,62.5);(37.5,50);(37.5,50)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(12.5,97.5);(12.5,97.5);(12.5,87.5);(12.5,87.5)"
%	 stroke-width= "0.75"
%	 />
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(27.5,92.5)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\universallift$
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(15,80)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\Progtype$
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(30,108.75)"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\Progtype$
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(70,108.75)"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\Btype$
%</text>
%<multicurve fill-style= "none"
%	 points= "(37.5,87.5);(37.5,87.5);(37.5,72.5);(37.5,72.5)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(107.5,80);(107.5,80);(167.5,80);(167.5,80)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(167.5,60);(167.5,60);(167.5,80);(167.5,80)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(127.5,60);(127.5,60);(167.5,60);(167.5,60)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(162.5,60);(162.5,60);(162.5,0);(162.5,0)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(135,60);(135,60);(135,0);(135,0)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(107.5,80);(107.5,80);(127.5,60);(127.5,60)"
%	 stroke-width= "0.75"
%	 />
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(148.75,70)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\universal$
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(160,1.25)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\Atype$
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(132.5,1.25)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\Progtype$
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(137.5,108.75)"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\Progtype$
%</text>
%<multicurve fill-style= "none"
%	 points= "(162.5,110);(162.5,110);(162.5,80);(162.5,80)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(135,110);(135,110);(135,80);(135,80)"
%	 stroke-width= "0.75"
%	 />
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(165,108.75)"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\Btype$
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(40,81.25)"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\Progtype$
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(95,60)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\EQLS
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(5,5)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\trtr$
%</text>
%<multicurve fill-style= "none"
%	 points= "(20,77.5);(20,77.5);(35,62.5);(35,62.5)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(35,62.5);(35,62.5);(47.5,62.5);(47.5,62.5)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(20,77.5);(20,77.5);(32.5,77.5);(32.5,77.5)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(32.5,77.5);(32.5,77.5);(47.5,62.5);(47.5,62.5)"
%	 stroke-width= "0.75"
%	 />
%<multicurve stroke-overstrike= "true"
%	 fill-style= "none"
%	 points= "(17.5,87.5);(17.5,87.5);(17.5,50);(17.5,50)"
%	 stroke-width= "0.75"
%	 stroke-overstrike-width= "1"
%	 />
%<multicurve fill-style= "none"
%	 points= "(7.5,50);(7.5,50);(7.5,10);(7.5,10)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(0,17.5);(0,17.5);(17.5,0);(17.5,0)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(0,0);(0,0);(17.5,0);(17.5,0)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(0,17.5);(0,17.5);(0,0);(0,0)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(12.5,87.5);(12.5,87.5);(42.5,87.5);(42.5,87.5)"
%	 stroke-width= "0.75"
%	 />
%<parallelogram fill-style= "none"
%	 p3= "(77.5,25)"
%	 p2= "(77.5,102.5)"
%	 p1= "(2.5,102.5)"
%	 />
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(115,5)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\trtr$
%</text>
%<multicurve fill-style= "none"
%	 points= "(117.5,70);(117.5,70);(117.5,10);(117.5,10)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(110,17.5);(110,17.5);(127.5,0);(127.5,0)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(110,0);(110,0);(127.5,0);(127.5,0)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(110,17.5);(110,17.5);(110,0);(110,0)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(212.5,80);(212.5,80);(257.5,80);(257.5,80)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(257.5,60);(257.5,60);(257.5,80);(257.5,80)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(232.5,60);(232.5,60);(257.5,60);(257.5,60)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(252.5,60);(252.5,60);(252.5,0);(252.5,0)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(222.5,31.25);(222.5,31.25);(222.5,0);(222.5,0)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(200,47.5);(200,47.5);(216.25,31.25);(216.25,31.25)"
%	 stroke-width= "0.75"
%	 />
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(242.5,70)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\universal$
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(250,1.25)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\Atype$
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(220,1.25)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\Progtype$
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(225,108.75)"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\Progtype$
%</text>
%<multicurve fill-style= "none"
%	 points= "(252.5,110);(252.5,110);(252.5,80);(252.5,80)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(222.5,110);(222.5,110);(222.5,80);(222.5,80)"
%	 stroke-width= "0.75"
%	 />
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(255,108.75)"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\Btype$
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(185,60)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\EQLS
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(205,20)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\trtr$
%</text>
%<multicurve fill-style= "none"
%	 points= "(207.5,40);(207.5,40);(207.5,25);(207.5,25)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(200,32.5);(200,32.5);(217.5,15);(217.5,15)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(200,15);(200,15);(217.5,15);(217.5,15)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(200,32.5);(200,32.5);(200,15);(200,15)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(216.25,31.25);(216.25,31.25);(231.25,31.25);(231.25,31.25)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(215,47.5);(215,47.5);(231.25,31.25);(231.25,31.25)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(200,47.5);(200,47.5);(215,47.5);(215,47.5)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(212.5,80);(212.5,80);(232.5,60);(232.5,60)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(222.5,40);(222.5,40);(222.5,70);(222.5,70)"
%	 stroke-width= "0.75"
%	 />
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(33.75,70)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\partl$
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(215,40)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\partl$
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(17.5,33.75)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\teee$
%</text>
%<multicurve fill-style= "none"
%	 stroke-color= "#ff0033"
%	 points= "(197.5,50);(197.5,50);(217.5,50);(217.5,50)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-color= "#ff0033"
%	 points= "(197.5,12.5);(197.5,12.5);(235,12.5);(235,12.5)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-color= "#ff0033"
%	 points= "(197.5,12.5);(197.5,12.5);(197.5,50);(197.5,50)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-color= "#ff0033"
%	 points= "(235,12.5);(235,12.5);(235,32.5);(235,32.5)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-color= "#ff0033"
%	 points= "(235,32.5);(235,32.5);(217.5,50);(217.5,50)"
%	 />
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(230,17.5)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\tauu$
%</text>
%</jpic>
%%End JPIC-XML
%PSTricks content-type (pstricks.sty package needed)
%Add \usepackage{pstricks} in the preamble of your LaTeX file
%You can rescale the whole picture (to 80% for instance) by using the command \def\JPicScale{0.8}
\ifx\JPicScale\undefined\def\JPicScale{1}\fi
\psset{unit=\JPicScale mm}
\psset{linewidth=0.3,dotsep=1,hatchwidth=0.3,hatchsep=1.5,shadowsize=1,dimen=middle}
\psset{dotsize=0.7 2.5,dotscale=1 1,fillcolor=black}
\psset{arrowsize=1 2,arrowlength=1,arrowinset=0.25,tbarsize=0.7 5,bracketlength=0.15,rbracketlength=0.15}
\begin{pspicture}(0,0)(257.5,110)
\psline[linewidth=0.75](27.5,50)(72.5,50)
\psline[linewidth=0.75](72.5,30)(72.5,50)
\psline[linewidth=0.75](47.5,30)(72.5,30)
\psline[linewidth=0.75](67.5,30)(67.5,0)
\newrgbcolor{userFillColour}{0.2 0 0.2}
\rput{0}(37.5,30){\psellipse[fillcolor=userFillColour,fillstyle=solid](0,0)(2.58,-2.58)}
\psline[linewidth=0.75](17.5,50)(37.5,30)
\psline[linewidth=0.75](37.5,40)(37.5,0)
\psline[linewidth=0.75](27.5,50)(47.5,30)
\rput(57.5,40){$\universal$}
\rput[r](65,1.25){$\Atype$}
\rput[r](35,1.25){$\Progtype$}
\rput[r](35,55){$\Progtype$}
\psline[linewidth=0.75](67.5,110)(67.5,50)
\psline[linewidth=0.75](27.5,70)(7.5,50)
\psline[linewidth=0.75](12.5,97.5)(42.5,97.5)
\psline[linewidth=0.75](42.5,87.5)(42.5,97.5)
\psline[linewidth=0.75](27.5,110)(27.5,97.5)
\psline[linewidth=0.75](37.5,62.5)(37.5,50)
\psline[linewidth=0.75](12.5,97.5)(12.5,87.5)
\rput(27.5,92.5){$\universallift$}
\rput[r](15,80){$\Progtype$}
\rput[l](30,108.75){$\Progtype$}
\rput[l](70,108.75){$\Btype$}
\psline[linewidth=0.75](37.5,87.5)(37.5,72.5)
\psline[linewidth=0.75](107.5,80)(167.5,80)
\psline[linewidth=0.75](167.5,60)(167.5,80)
\psline[linewidth=0.75](127.5,60)(167.5,60)
\psline[linewidth=0.75](162.5,60)(162.5,0)
\psline[linewidth=0.75](135,60)(135,0)
\psline[linewidth=0.75](107.5,80)(127.5,60)
\rput(148.75,70){$\universal$}
\rput[r](160,1.25){$\Atype$}
\rput[r](132.5,1.25){$\Progtype$}
\rput[l](137.5,108.75){$\Progtype$}
\psline[linewidth=0.75](162.5,110)(162.5,80)
\psline[linewidth=0.75](135,110)(135,80)
\rput[l](165,108.75){$\Btype$}
\rput[l](40,81.25){$\Progtype$}
\rput(95,60){\EQLS}
\rput(5,5){$\trtr$}
\psline[linewidth=0.75](20,77.5)(35,62.5)
\psline[linewidth=0.75](35,62.5)(47.5,62.5)
\psline[linewidth=0.75](20,77.5)(32.5,77.5)
\psline[linewidth=0.75](32.5,77.5)(47.5,62.5)
\psline[linewidth=0.75,border=1](17.5,87.5)(17.5,50)
\psline[linewidth=0.75](7.5,50)(7.5,10)
\psline[linewidth=0.75](0,17.5)(17.5,0)
\psline[linewidth=0.75](0,0)(17.5,0)
\psline[linewidth=0.75](0,17.5)(0,0)
\psline[linewidth=0.75](12.5,87.5)(42.5,87.5)
\pspolygon[](2.5,102.5)(77.5,102.5)(77.5,25)(2.5,25)
\rput(115,5){$\trtr$}
\psline[linewidth=0.75](117.5,70)(117.5,10)
\psline[linewidth=0.75](110,17.5)(127.5,0)
\psline[linewidth=0.75](110,0)(127.5,0)
\psline[linewidth=0.75](110,17.5)(110,0)
\psline[linewidth=0.75](212.5,80)(257.5,80)
\psline[linewidth=0.75](257.5,60)(257.5,80)
\psline[linewidth=0.75](232.5,60)(257.5,60)
\psline[linewidth=0.75](252.5,60)(252.5,0)
\psline[linewidth=0.75](222.5,31.25)(222.5,0)
\psline[linewidth=0.75](200,47.5)(216.25,31.25)
\rput(242.5,70){$\universal$}
\rput[r](250,1.25){$\Atype$}
\rput[r](220,1.25){$\Progtype$}
\rput[l](225,108.75){$\Progtype$}
\psline[linewidth=0.75](252.5,110)(252.5,80)
\psline[linewidth=0.75](222.5,110)(222.5,80)
\rput[l](255,108.75){$\Btype$}
\rput(185,60){\EQLS}
\rput(205,20){$\trtr$}
\psline[linewidth=0.75](207.5,40)(207.5,25)
\psline[linewidth=0.75](200,32.5)(217.5,15)
\psline[linewidth=0.75](200,15)(217.5,15)
\psline[linewidth=0.75](200,32.5)(200,15)
\psline[linewidth=0.75](216.25,31.25)(231.25,31.25)
\psline[linewidth=0.75](215,47.5)(231.25,31.25)
\psline[linewidth=0.75](200,47.5)(215,47.5)
\psline[linewidth=0.75](212.5,80)(232.5,60)
\psline[linewidth=0.75](222.5,40)(222.5,70)
\rput(33.75,70){$\partl$}
\rput(215,40){$\partl$}
\rput(17.5,33.75){$\teee$}
\newrgbcolor{userLineColour}{1 0 0.2}
\psline[linecolor=userLineColour](197.5,50)(217.5,50)
\newrgbcolor{userLineColour}{1 0 0.2}
\psline[linecolor=userLineColour](197.5,12.5)(235,12.5)
\newrgbcolor{userLineColour}{1 0 0.2}
\psline[linecolor=userLineColour](197.5,12.5)(197.5,50)
\newrgbcolor{userLineColour}{1 0 0.2}
\psline[linecolor=userLineColour](235,12.5)(235,32.5)
\newrgbcolor{userLineColour}{1 0 0.2}
\psline[linecolor=userLineColour](235,32.5)(217.5,50)
\rput(230,17.5){$\tauu$}
\end{pspicture}


==> PIC/tracingtr.tex <==
%%Created by jPicEdt 1.4.1_03: mixed JPIC-XML/LaTeX format
%%Tue Jan 07 17:10:15 GMT-10:00 2020
%%Begin JPIC-XML
%<?xml version="1.0" standalone="yes"?>
%<jpic x-min="0" x-max="150" y-min="0" y-max="110" auto-bounding="true">
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(105,50);(105,50);(150,50);(150,50)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(150,30);(150,30);(150,50);(150,50)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(125,30);(125,30);(150,30);(150,30)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(145,30);(145,30);(145,0);(145,0)"
%	 />
%<ellipse fill-style= "solid"
%	 p3= "(117.58,27.42)"
%	 p2= "(117.58,32.58)"
%	 p1= "(112.42,32.58)"
%	 fill-color= "#330033"
%	 closure= "open"
%	 angle-end= "0"
%	 angle-start= "0"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(95,50);(95,50);(115,30);(115,30)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(115,40);(115,40);(115,0);(115,0)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(105,50);(105,50);(125,30);(125,30)"
%	 />
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(135,40)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\universal$
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(142.5,1.25)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\Atype$
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(112.5,1.25)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\Progtype$
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(112.5,55)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\Progtype$
%</text>
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(145,110);(145,110);(145,50);(145,50)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(95,87.5);(95,87.5);(95,50);(95,50)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(90,97.5);(90,97.5);(120,97.5);(120,97.5)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(120,87.5);(120,87.5);(120,97.5);(120,97.5)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(105,110);(105,110);(105,97.5);(105,97.5)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(90,87.5);(90,87.5);(120,87.5);(120,87.5)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(115,60);(115,60);(115,50);(115,50)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(90,97.5);(90,97.5);(90,87.5);(90,87.5)"
%	 />
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(105,92.5)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\universallift$
%</text>
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 stroke-color= "#ff0033"
%	 points= "(125,60);(125,60);(105,60);(105,60)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 stroke-color= "#ff0033"
%	 points= "(105,80);(105,80);(105,60);(105,60)"
%	 />
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(92.5,55)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\Progtype$
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(107.5,108.75)"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\Progtype$
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(147.5,108.75)"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\Btype$
%</text>
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 stroke-color= "#ff0033"
%	 points= "(125,65);(125,65);(125,60);(125,60)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 stroke-color= "#ff0033"
%	 points= "(110,80);(110,80);(105,80);(105,80)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(115,87.5);(115,87.5);(115,75);(115,75)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 stroke-color= "#ff0033"
%	 points= "(125,65);(125,65);(110,80);(110,80)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(0,50);(0,50);(45,50);(45,50)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(45,30);(45,30);(45,50);(45,50)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(20,30);(20,30);(45,30);(45,30)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(40,30);(40,30);(40,0);(40,0)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(10,15);(10,15);(10,0);(10,0)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(10,40);(10,40);(10,30);(10,30)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(0,50);(0,50);(20,30);(20,30)"
%	 />
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(30,40)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\universal$
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(37.5,1.25)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\Atype$
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(7.5,1.25)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\Progtype$
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(12.5,108.75)"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\Progtype$
%</text>
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(40,110);(40,110);(40,50);(40,50)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(10,110);(10,110);(10,50);(10,50)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 stroke-color= "#ff0033"
%	 points= "(20,15);(20,15);(0,15);(0,15)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 stroke-color= "#ff0033"
%	 points= "(0,35);(0,35);(0,15);(0,15)"
%	 />
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(42.5,108.75)"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\Btype$
%</text>
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 stroke-color= "#ff0033"
%	 points= "(20,20);(20,20);(20,15);(20,15)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 stroke-color= "#ff0033"
%	 points= "(5,35);(5,35);(0,35);(0,35)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 stroke-color= "#ff0033"
%	 points= "(20,20);(20,20);(5,35);(5,35)"
%	 />
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(117.5,81.25)"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\Progtype$
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(70,40)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\EQLS
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(112.5,67.5)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\trtr$
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(7.5,22.5)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\trtr$
%</text>
%</jpic>
%%End JPIC-XML
%PSTricks content-type (pstricks.sty package needed)
%Add \usepackage{pstricks} in the preamble of your LaTeX file
%You can rescale the whole picture (to 80% for instance) by using the command \def\JPicScale{0.8}
\ifx\JPicScale\undefined\def\JPicScale{1}\fi
\psset{unit=\JPicScale mm}
\psset{linewidth=0.3,dotsep=1,hatchwidth=0.3,hatchsep=1.5,shadowsize=1,dimen=middle}
\psset{dotsize=0.7 2.5,dotscale=1 1,fillcolor=black}
\psset{arrowsize=1 2,arrowlength=1,arrowinset=0.25,tbarsize=0.7 5,bracketlength=0.15,rbracketlength=0.15}
\begin{pspicture}(0,0)(150,110)
\psline[linewidth=0.75](105,50)(150,50)
\psline[linewidth=0.75](150,30)(150,50)
\psline[linewidth=0.75](125,30)(150,30)
\psline[linewidth=0.75](145,30)(145,0)
\newrgbcolor{userFillColour}{0.2 0 0.2}
\rput{0}(115,30){\psellipse[fillcolor=userFillColour,fillstyle=solid](0,0)(2.58,-2.58)}
\psline[linewidth=0.75](95,50)(115,30)
\psline[linewidth=0.75](115,40)(115,0)
\psline[linewidth=0.75](105,50)(125,30)
\rput(135,40){$\universal$}
\rput[r](142.5,1.25){$\Atype$}
\rput[r](112.5,1.25){$\Progtype$}
\rput[r](112.5,55){$\Progtype$}
\psline[linewidth=0.75](145,110)(145,50)
\psline[linewidth=0.75](95,87.5)(95,50)
\psline[linewidth=0.75](90,97.5)(120,97.5)
\psline[linewidth=0.75](120,87.5)(120,97.5)
\psline[linewidth=0.75](105,110)(105,97.5)
\psline[linewidth=0.75](90,87.5)(120,87.5)
\psline[linewidth=0.75](115,60)(115,50)
\psline[linewidth=0.75](90,97.5)(90,87.5)
\rput(105,92.5){$\universallift$}
\newrgbcolor{userLineColour}{1 0 0.2}
\psline[linewidth=0.75,linecolor=userLineColour](125,60)(105,60)
\newrgbcolor{userLineColour}{1 0 0.2}
\psline[linewidth=0.75,linecolor=userLineColour](105,80)(105,60)
\rput[r](92.5,55){$\Progtype$}
\rput[l](107.5,108.75){$\Progtype$}
\rput[l](147.5,108.75){$\Btype$}
\newrgbcolor{userLineColour}{1 0 0.2}
\psline[linewidth=0.75,linecolor=userLineColour](125,65)(125,60)
\newrgbcolor{userLineColour}{1 0 0.2}
\psline[linewidth=0.75,linecolor=userLineColour](110,80)(105,80)
\psline[linewidth=0.75](115,87.5)(115,75)
\newrgbcolor{userLineColour}{1 0 0.2}
\psline[linewidth=0.75,linecolor=userLineColour](125,65)(110,80)
\psline[linewidth=0.75](0,50)(45,50)
\psline[linewidth=0.75](45,30)(45,50)
\psline[linewidth=0.75](20,30)(45,30)
\psline[linewidth=0.75](40,30)(40,0)
\psline[linewidth=0.75](10,15)(10,0)
\psline[linewidth=0.75](10,40)(10,30)
\psline[linewidth=0.75](0,50)(20,30)
\rput(30,40){$\universal$}
\rput[r](37.5,1.25){$\Atype$}
\rput[r](7.5,1.25){$\Progtype$}
\rput[l](12.5,108.75){$\Progtype$}
\psline[linewidth=0.75](40,110)(40,50)
\psline[linewidth=0.75](10,110)(10,50)
\newrgbcolor{userLineColour}{1 0 0.2}
\psline[linewidth=0.75,linecolor=userLineColour](20,15)(0,15)
\newrgbcolor{userLineColour}{1 0 0.2}
\psline[linewidth=0.75,linecolor=userLineColour](0,35)(0,15)
\rput[l](42.5,108.75){$\Btype$}
\newrgbcolor{userLineColour}{1 0 0.2}
\psline[linewidth=0.75,linecolor=userLineColour](20,20)(20,15)
\newrgbcolor{userLineColour}{1 0 0.2}
\psline[linewidth=0.75,linecolor=userLineColour](5,35)(0,35)
\newrgbcolor{userLineColour}{1 0 0.2}
\psline[linewidth=0.75,linecolor=userLineColour](20,20)(5,35)
\rput[l](117.5,81.25){$\Progtype$}
\rput(70,40){\EQLS}
\rput(112.5,67.5){$\trtr$}
\rput(7.5,22.5){$\trtr$}
\end{pspicture}


==> PIC/triple-1.tex <==
%%Created by jPicEdt 1.4.1_03: mixed JPIC-XML/LaTeX format
%%Wed Jul 31 21:53:14 GMT-10:00 2019
%%Begin JPIC-XML
%<?xml version="1.0" standalone="yes"?>
%<jpic x-min="5" x-max="186.25" y-min="0" y-max="60" auto-bounding="true">
%<multicurve fill-style= "none"
%	 points= "(75,40);(75,40);(75,20);(75,20)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(105,20);(105,20);(105,40);(105,40)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(90,60);(90,60);(90,40);(90,40)"
%	 stroke-color= "#999999"
%	 stroke-width= "3"
%	 />
%<multicurve fill-style= "none"
%	 points= "(75,20);(75,20);(105,20);(105,20)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(90,20);(90,20);(90,0);(90,0)"
%	 stroke-width= "0.75"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(87.5,0)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\otherinputt$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(93.75,60)"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\otheroutpt$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(90,30)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\hee$
%</text>
%<multicurve fill-style= "none"
%	 points= "(10,60);(10,60);(10,35);(10,35)"
%	 stroke-color= "#999999"
%	 stroke-width= "3"
%	 />
%<multicurve fill-style= "none"
%	 points= "(10,25);(10,25);(10,0);(10,0)"
%	 stroke-width= "0.75"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(7.5,0)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\otherinputt$
%</text>
%<multicurve fill-style= "none"
%	 points= "(5,35);(5,35);(15,35);(15,35)"
%	 stroke-width= "0.75"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 stroke-dasharray= "8;8"
%	 anchor-point= "(10,30)"
%	 stroke-style= "dashed"
%	 text-frame= "noframe"
%	 stroke-width= "0.75"
%	 text-hor-align= "center-h"
%	 >
%$\unit$
%</text>
%<multicurve fill-style= "none"
%	 points= "(5,25);(5,25);(15,25);(15,25)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(15,35);(15,35);(15,25);(15,25)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(5,35);(5,35);(5,25);(5,25)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(75,40);(75,40);(105,40);(105,40)"
%	 stroke-width= "0.75"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 stroke-dasharray= "8;8"
%	 anchor-point= "(165,30)"
%	 stroke-style= "dashed"
%	 text-frame= "noframe"
%	 stroke-width= "0.75"
%	 text-hor-align= "center-h"
%	 >
%$\eehee$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 stroke-dasharray= "8;8"
%	 anchor-point= "(161.25,0)"
%	 stroke-style= "dashed"
%	 text-frame= "noframe"
%	 stroke-width= "0.75"
%	 text-hor-align= "right"
%	 >
%$\eeinptt$
%</text>
%<multicurve fill-style= "none"
%	 points= "(150,40);(150,40);(150,20);(150,20)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(180,20);(180,20);(180,40);(180,40)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(165,60);(165,60);(165,40);(165,40)"
%	 stroke-color= "#999999"
%	 stroke-width= "3"
%	 />
%<multicurve fill-style= "none"
%	 points= "(150,20);(150,20);(180,20);(180,20)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(165,20);(165,20);(165,0);(165,0)"
%	 stroke-width= "0.75"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(168.75,60)"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\otheroutpt$
%</text>
%<multicurve fill-style= "none"
%	 points= "(150,40);(150,40);(180,40);(180,40)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(145,46.25);(145,46.25);(145,13.75);(145,13.75)"
%	 stroke-color= "#999999"
%	 stroke-width= "3"
%	 />
%<multicurve fill-style= "none"
%	 points= "(185,46.25);(185,46.25);(185,13.75);(185,13.75)"
%	 stroke-color= "#999999"
%	 stroke-width= "3"
%	 />
%<multicurve fill-style= "none"
%	 points= "(186.25,45);(186.25,45);(143.75,45);(143.75,45)"
%	 stroke-color= "#999999"
%	 stroke-width= "3"
%	 />
%<multicurve fill-style= "none"
%	 points= "(186.25,15);(186.25,15);(143.75,15);(143.75,15)"
%	 stroke-color= "#999999"
%	 stroke-width= "3"
%	 />
%<multicurve fill-style= "none"
%	 points= "(165,0);(165,0);(165,15);(165,15)"
%	 stroke-color= "#999999"
%	 stroke-width= "3"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 stroke-dasharray= "8;8"
%	 anchor-point= "(125,30)"
%	 stroke-style= "dashed"
%	 text-frame= "noframe"
%	 stroke-width= "0.75"
%	 text-hor-align= "center-h"
%	 >
%\goesto
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 stroke-dasharray= "8;8"
%	 anchor-point= "(13.75,60)"
%	 stroke-style= "dashed"
%	 text-frame= "noframe"
%	 stroke-width= "0.75"
%	 text-hor-align= "left"
%	 >
%$\eeinptt$
%</text>
%</jpic>
%%End JPIC-XML
%PSTricks content-type (pstricks.sty package needed)
%Add \usepackage{pstricks} in the preamble of your LaTeX file
%You can rescale the whole picture (to 80% for instance) by using the command \def\JPicScale{0.8}
\ifx\JPicScale\undefined\def\JPicScale{1}\fi
\psset{unit=\JPicScale mm}
\psset{linewidth=0.3,dotsep=1,hatchwidth=0.3,hatchsep=1.5,shadowsize=1,dimen=middle}
\psset{dotsize=0.7 2.5,dotscale=1 1,fillcolor=black}
\psset{arrowsize=1 2,arrowlength=1,arrowinset=0.25,tbarsize=0.7 5,bracketlength=0.15,rbracketlength=0.15}
\begin{pspicture}(0,0)(186.25,60)
\psline[linewidth=0.75](75,40)(75,20)
\psline[linewidth=0.75](105,20)(105,40)
\newrgbcolor{userLineColour}{0.6 0.6 0.6}
\psline[linewidth=3,linecolor=userLineColour](90,60)(90,40)
\psline[linewidth=0.75](75,20)(105,20)
\psline[linewidth=0.75](90,20)(90,0)
\rput[r](87.5,0){$\otherinputt$}
\rput[l](93.75,60){$\otheroutpt$}
\rput(90,30){$\hee$}
\newrgbcolor{userLineColour}{0.6 0.6 0.6}
\psline[linewidth=3,linecolor=userLineColour](10,60)(10,35)
\psline[linewidth=0.75](10,25)(10,0)
\rput[r](7.5,0){$\otherinputt$}
\psline[linewidth=0.75](5,35)(15,35)
\rput(10,30){$\unit$}
\psline[linewidth=0.75](5,25)(15,25)
\psline[linewidth=0.75](15,35)(15,25)
\psline[linewidth=0.75](5,35)(5,25)
\psline[linewidth=0.75](75,40)(105,40)
\rput(165,30){$\eehee$}
\rput[r](161.25,0){$\eeinptt$}
\psline[linewidth=0.75](150,40)(150,20)
\psline[linewidth=0.75](180,20)(180,40)
\newrgbcolor{userLineColour}{0.6 0.6 0.6}
\psline[linewidth=3,linecolor=userLineColour](165,60)(165,40)
\psline[linewidth=0.75](150,20)(180,20)
\psline[linewidth=0.75](165,20)(165,0)
\rput[l](168.75,60){$\otheroutpt$}
\psline[linewidth=0.75](150,40)(180,40)
\newrgbcolor{userLineColour}{0.6 0.6 0.6}
\psline[linewidth=3,linecolor=userLineColour](145,46.25)(145,13.75)
\newrgbcolor{userLineColour}{0.6 0.6 0.6}
\psline[linewidth=3,linecolor=userLineColour](185,46.25)(185,13.75)
\newrgbcolor{userLineColour}{0.6 0.6 0.6}
\psline[linewidth=3,linecolor=userLineColour](186.25,45)(143.75,45)
\newrgbcolor{userLineColour}{0.6 0.6 0.6}
\psline[linewidth=3,linecolor=userLineColour](186.25,15)(143.75,15)
\newrgbcolor{userLineColour}{0.6 0.6 0.6}
\psline[linewidth=3,linecolor=userLineColour](165,0)(165,15)
\rput(125,30){\goesto}
\rput[l](13.75,60){$\eeinptt$}
\end{pspicture}


==> PIC/triple-2.tex <==
%%Created by jPicEdt 1.4.1_03: mixed JPIC-XML/LaTeX format
%%Sun Nov 03 11:26:33 GMT-10:00 2019
%%Begin JPIC-XML
%<?xml version="1.0" standalone="yes"?>
%<jpic x-min="5" x-max="222.5" y-min="0" y-max="60" auto-bounding="true">
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(115,40);(115,40);(115,20);(115,20)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(135,20);(135,20);(135,40);(135,40)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(115,20);(115,20);(135,20);(135,20)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(125,20);(125,20);(125,0);(125,0)"
%	 />
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(122.5,0)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\otherinputt$
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(128.75,60)"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\otheroutpt$
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(125,30)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\hee$
%</text>
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(10,25);(10,25);(10,0);(10,0)"
%	 />
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(7.5,0)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\otherinputt$
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 stroke-width= "0.75"
%	 stroke-dasharray= "8;8"
%	 stroke-style= "dashed"
%	 anchor-point= "(10,30)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\unit$
%</text>
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(5,25);(5,25);(15,25);(15,25)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(15,35);(15,35);(15,25);(15,25)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(5,35);(5,35);(5,25);(5,25)"
%	 />
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 stroke-width= "0.75"
%	 stroke-dasharray= "8;8"
%	 stroke-style= "dashed"
%	 anchor-point= "(171.25,0)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\eeinptt$
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(178.75,60)"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\otheroutpt$
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 stroke-width= "0.75"
%	 stroke-dasharray= "8;8"
%	 stroke-style= "dashed"
%	 anchor-point= "(150,33.75)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\goesto
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 stroke-width= "0.75"
%	 stroke-dasharray= "8;8"
%	 stroke-style= "dashed"
%	 anchor-point= "(13.75,60)"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\eeinptt$
%</text>
%<parallelogram fill-style= "solid"
%	 p3= "(172.5,60)"
%	 p2= "(172.5,40)"
%	 p1= "(177.5,40)"
%	 fill-color= "#999999"
%	 stroke-color= "#999999"
%	 />
%<parallelogram fill-style= "solid"
%	 p3= "(172.5,20)"
%	 p2= "(172.5,0)"
%	 p1= "(177.5,0)"
%	 fill-color= "#999999"
%	 stroke-color= "#999999"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(175,60);(175,60);(175,40);(175,40)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(175,20);(175,20);(175,0);(175,0)"
%	 />
%<parallelogram fill-style= "solid"
%	 p3= "(185,20)"
%	 p2= "(185,40)"
%	 stroke-width= "0.75"
%	 p1= "(165,40)"
%	 fill-color= "#ffffff"
%	 />
%<text fill-style= "solid"
%	 text-vert-align= "center-v"
%	 stroke-width= "0.75"
%	 fill-color= "#ffffff"
%	 stroke-dasharray= "8;8"
%	 stroke-style= "dashed"
%	 anchor-point= "(175,30)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\eehee$
%</text>
%<parallelogram fill-style= "solid"
%	 p3= "(122.5,60)"
%	 p2= "(122.5,40)"
%	 p1= "(127.5,40)"
%	 fill-color= "#999999"
%	 stroke-color= "#999999"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(125,60);(125,60);(125,40);(125,40)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(115,40);(115,40);(135,40);(135,40)"
%	 />
%<parallelogram fill-style= "solid"
%	 p3= "(7.5,60)"
%	 p2= "(7.5,35)"
%	 p1= "(12.5,35)"
%	 fill-color= "#999999"
%	 stroke-color= "#999999"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(10,60);(10,60);(10,35);(10,35)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(5,35);(5,35);(15,35);(15,35)"
%	 />
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 stroke-width= "0.75"
%	 stroke-dasharray= "8;8"
%	 stroke-style= "dashed"
%	 anchor-point= "(211.25,0)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\eeinptt$
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(213.75,60)"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\otheroutpt$
%</text>
%<parallelogram fill-style= "solid"
%	 p3= "(197.5,42.5)"
%	 p2= "(197.5,17.5)"
%	 p1= "(222.5,17.5)"
%	 fill-color= "#999999"
%	 stroke-color= "#999999"
%	 />
%<parallelogram fill-style= "solid"
%	 p3= "(207.5,60)"
%	 p2= "(207.5,40)"
%	 p1= "(212.5,40)"
%	 fill-color= "#999999"
%	 stroke-color= "#999999"
%	 />
%<parallelogram fill-style= "solid"
%	 p3= "(207.5,20)"
%	 p2= "(207.5,0)"
%	 p1= "(212.5,0)"
%	 fill-color= "#999999"
%	 stroke-color= "#999999"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(210,60);(210,60);(210,40);(210,40)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(210,20);(210,20);(210,0);(210,0)"
%	 />
%<parallelogram fill-style= "solid"
%	 p3= "(220,20)"
%	 p2= "(220,40)"
%	 stroke-width= "0.75"
%	 p1= "(200,40)"
%	 fill-color= "#ffffff"
%	 />
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(192.5,30)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\EQLS
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(210,30)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\hee$
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 stroke-width= "0.7"
%	 anchor-point= "(25,30)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\ORR
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 stroke-width= "0.75"
%	 stroke-dasharray= "8;8"
%	 stroke-style= "dashed"
%	 anchor-point= "(40,30)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\unit$
%</text>
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(35,25);(35,25);(45,25);(45,25)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(45,35);(45,35);(45,25);(45,25)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(35,35);(35,35);(35,25);(35,25)"
%	 />
%<parallelogram fill-style= "solid"
%	 p3= "(37.5,60)"
%	 p2= "(37.5,35)"
%	 p1= "(42.5,35)"
%	 fill-color= "#999999"
%	 stroke-color= "#999999"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(35,35);(35,35);(45,35);(45,35)"
%	 />
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 stroke-width= "0.7"
%	 anchor-point= "(45,60)"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\Mii$
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 stroke-width= "0.7"
%	 anchor-point= "(37.5,17.5)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\Jii$
%</text>
%</jpic>
%%End JPIC-XML
%PSTricks content-type (pstricks.sty package needed)
%Add \usepackage{pstricks} in the preamble of your LaTeX file
%You can rescale the whole picture (to 80% for instance) by using the command \def\JPicScale{0.8}
\ifx\JPicScale\undefined\def\JPicScale{1}\fi
\psset{unit=\JPicScale mm}
\psset{linewidth=0.3,dotsep=1,hatchwidth=0.3,hatchsep=1.5,shadowsize=1,dimen=middle}
\psset{dotsize=0.7 2.5,dotscale=1 1,fillcolor=black}
\psset{arrowsize=1 2,arrowlength=1,arrowinset=0.25,tbarsize=0.7 5,bracketlength=0.15,rbracketlength=0.15}
\begin{pspicture}(0,0)(222.5,60)
\psline[linewidth=0.75](115,40)(115,20)
\psline[linewidth=0.75](135,20)(135,40)
\psline[linewidth=0.75](115,20)(135,20)
\psline[linewidth=0.75](125,20)(125,0)
\rput[r](122.5,0){$\otherinputt$}
\rput[l](128.75,60){$\otheroutpt$}
\rput(125,30){$\hee$}
\psline[linewidth=0.75](10,25)(10,0)
\rput[r](7.5,0){$\otherinputt$}
\rput(10,30){$\unit$}
\psline[linewidth=0.75](5,25)(15,25)
\psline[linewidth=0.75](15,35)(15,25)
\psline[linewidth=0.75](5,35)(5,25)
\rput[r](171.25,0){$\eeinptt$}
\rput[l](178.75,60){$\otheroutpt$}
\rput(150,33.75){\goesto}
\rput[l](13.75,60){$\eeinptt$}
\newrgbcolor{userLineColour}{0.6 0.6 0.6}
\newrgbcolor{userFillColour}{0.6 0.6 0.6}
\pspolygon[linecolor=userLineColour,fillcolor=userFillColour,fillstyle=solid](177.5,40)(172.5,40)(172.5,60)(177.5,60)
\newrgbcolor{userLineColour}{0.6 0.6 0.6}
\newrgbcolor{userFillColour}{0.6 0.6 0.6}
\pspolygon[linecolor=userLineColour,fillcolor=userFillColour,fillstyle=solid](177.5,0)(172.5,0)(172.5,20)(177.5,20)
\psline[linewidth=0.75](175,60)(175,40)
\psline[linewidth=0.75](175,20)(175,0)
\pspolygon[linewidth=0.75,fillcolor=white,fillstyle=solid](165,40)(185,40)(185,20)(165,20)
\rput(175,30){$\eehee$}
\newrgbcolor{userLineColour}{0.6 0.6 0.6}
\newrgbcolor{userFillColour}{0.6 0.6 0.6}
\pspolygon[linecolor=userLineColour,fillcolor=userFillColour,fillstyle=solid](127.5,40)(122.5,40)(122.5,60)(127.5,60)
\psline[linewidth=0.75](125,60)(125,40)
\psline[linewidth=0.75](115,40)(135,40)
\newrgbcolor{userLineColour}{0.6 0.6 0.6}
\newrgbcolor{userFillColour}{0.6 0.6 0.6}
\pspolygon[linecolor=userLineColour,fillcolor=userFillColour,fillstyle=solid](12.5,35)(7.5,35)(7.5,60)(12.5,60)
\psline[linewidth=0.75](10,60)(10,35)
\psline[linewidth=0.75](5,35)(15,35)
\rput[r](211.25,0){$\eeinptt$}
\rput[l](213.75,60){$\otheroutpt$}
\newrgbcolor{userLineColour}{0.6 0.6 0.6}
\newrgbcolor{userFillColour}{0.6 0.6 0.6}
\pspolygon[linecolor=userLineColour,fillcolor=userFillColour,fillstyle=solid](222.5,17.5)(197.5,17.5)(197.5,42.5)(222.5,42.5)
\newrgbcolor{userLineColour}{0.6 0.6 0.6}
\newrgbcolor{userFillColour}{0.6 0.6 0.6}
\pspolygon[linecolor=userLineColour,fillcolor=userFillColour,fillstyle=solid](212.5,40)(207.5,40)(207.5,60)(212.5,60)
\newrgbcolor{userLineColour}{0.6 0.6 0.6}
\newrgbcolor{userFillColour}{0.6 0.6 0.6}
\pspolygon[linecolor=userLineColour,fillcolor=userFillColour,fillstyle=solid](212.5,0)(207.5,0)(207.5,20)(212.5,20)
\psline[linewidth=0.75](210,60)(210,40)
\psline[linewidth=0.75](210,20)(210,0)
\pspolygon[linewidth=0.75,fillcolor=white,fillstyle=solid](200,40)(220,40)(220,20)(200,20)
\rput(192.5,30){\EQLS}
\rput(210,30){$\hee$}
\rput(25,30){\ORR}
\rput(40,30){$\unit$}
\psline[linewidth=0.75](35,25)(45,25)
\psline[linewidth=0.75](45,35)(45,25)
\psline[linewidth=0.75](35,35)(35,25)
\newrgbcolor{userLineColour}{0.6 0.6 0.6}
\newrgbcolor{userFillColour}{0.6 0.6 0.6}
\pspolygon[linecolor=userLineColour,fillcolor=userFillColour,fillstyle=solid](42.5,35)(37.5,35)(37.5,60)(42.5,60)
\psline[linewidth=0.75](35,35)(45,35)
\rput[l](45,60){$\Mii$}
\rput[r](37.5,17.5){$\Jii$}
\end{pspicture}


==> PIC/triple-3.tex <==
%%Created by jPicEdt 1.4.1_03: mixed JPIC-XML/LaTeX format
%%Mon Dec 30 00:16:27 GMT-10:00 2019
%%Begin JPIC-XML
%<?xml version="1.0" standalone="yes"?>
%<jpic x-min="0" x-max="265" y-min="0" y-max="60" auto-bounding="true">
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(65,20);(65,20);(65,0);(65,0)"
%	 />
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(62.5,0)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\otherinputt$
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(78.75,60)"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\otheroutpt$
%</text>
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(5,25);(5,25);(5,0);(5,0)"
%	 />
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(2.5,0)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\otherinputt$
%</text>
%<text fill-style= "none"
%	 stroke-width= "0.75"
%	 text-vert-align= "center-v"
%	 stroke-dasharray= "8;8"
%	 anchor-point= "(5,30)"
%	 text-frame= "noframe"
%	 stroke-style= "dashed"
%	 text-hor-align= "center-h"
%	 >
%$\unit$
%</text>
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(0,25);(0,25);(10,25);(10,25)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(10,35);(10,35);(10,25);(10,25)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(0,35);(0,35);(0,25);(0,25)"
%	 />
%<text fill-style= "none"
%	 stroke-width= "0.75"
%	 text-vert-align= "center-v"
%	 stroke-dasharray= "8;8"
%	 anchor-point= "(91.25,33.75)"
%	 text-frame= "noframe"
%	 stroke-style= "dashed"
%	 text-hor-align= "center-h"
%	 >
%\goesto
%</text>
%<text fill-style= "none"
%	 stroke-width= "0.75"
%	 text-vert-align= "center-v"
%	 stroke-dasharray= "8;8"
%	 anchor-point= "(8.75,60)"
%	 text-frame= "noframe"
%	 stroke-style= "dashed"
%	 text-hor-align= "left"
%	 >
%$\eeinptt$
%</text>
%<text fill-style= "none"
%	 stroke-width= "0.75"
%	 text-vert-align= "center-v"
%	 stroke-dasharray= "8;8"
%	 anchor-point= "(236.25,0)"
%	 text-frame= "noframe"
%	 stroke-style= "dashed"
%	 text-hor-align= "right"
%	 >
%$\eeinptt$
%</text>
%<parallelogram fill-color= "#999999"
%	 fill-style= "solid"
%	 p3= "(237.5,30)"
%	 p2= "(237.5,0)"
%	 p1= "(242.5,0)"
%	 stroke-color= "#999999"
%	 />
%<parallelogram fill-color= "#999999"
%	 fill-style= "solid"
%	 p3= "(257.5,30)"
%	 p2= "(257.5,0)"
%	 p1= "(262.5,0)"
%	 stroke-color= "#999999"
%	 />
%<parallelogram fill-color= "#999999"
%	 fill-style= "solid"
%	 p3= "(237.5,60)"
%	 p2= "(237.5,35)"
%	 p1= "(262.5,35)"
%	 stroke-color= "#999999"
%	 />
%<parallelogram fill-color= "#999999"
%	 fill-style= "solid"
%	 p3= "(152.5,42.5)"
%	 p2= "(152.5,17.5)"
%	 p1= "(187.5,17.5)"
%	 stroke-color= "#999999"
%	 />
%<parallelogram fill-color= "#999999"
%	 fill-style= "solid"
%	 p3= "(167.5,20)"
%	 p2= "(167.5,0)"
%	 p1= "(172.5,0)"
%	 stroke-color= "#999999"
%	 />
%<parallelogram fill-color= "#999999"
%	 fill-style= "solid"
%	 p3= "(72.5,60)"
%	 p2= "(72.5,40)"
%	 p1= "(77.5,40)"
%	 stroke-color= "#999999"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(75,60);(75,60);(75,40);(75,40)"
%	 />
%<parallelogram fill-color= "#999999"
%	 fill-style= "solid"
%	 p3= "(2.5,60)"
%	 p2= "(2.5,35)"
%	 p1= "(7.5,35)"
%	 stroke-color= "#999999"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(5,60);(5,60);(5,35);(5,35)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(0,35);(0,35);(10,35);(10,35)"
%	 />
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 stroke-color= "#999999"
%	 anchor-point= "(256.25,0)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\beeinptt$
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 stroke-color= "#999999"
%	 anchor-point= "(263.75,60)"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\ceeoutpt$
%</text>
%<parallelogram fill-color= "#ffffff"
%	 fill-style= "solid"
%	 stroke-width= "0.75"
%	 p3= "(265,25)"
%	 p2= "(265,35)"
%	 p1= "(235,35)"
%	 />
%<text fill-color= "#ffffff"
%	 fill-style= "solid"
%	 text-vert-align= "center-v"
%	 stroke-color= "#999999"
%	 anchor-point= "(250,30)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\ffubini$
%</text>
%<parallelogram fill-color= "#999999"
%	 fill-style= "solid"
%	 p3= "(52.5,60)"
%	 p2= "(52.5,40)"
%	 p1= "(57.5,40)"
%	 stroke-color= "#999999"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(55,60);(55,60);(55,40);(55,40)"
%	 />
%<parallelogram fill-color= "#ffffff"
%	 fill-style= "solid"
%	 stroke-width= "0.75"
%	 p3= "(80,20)"
%	 p2= "(80,40)"
%	 p1= "(50,40)"
%	 />
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(65,30)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\hee$
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 stroke-color= "#999999"
%	 anchor-point= "(66.25,46.88)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\inbit
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 stroke-color= "#999999"
%	 anchor-point= "(251.25,46.25)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\inbit
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 stroke-color= "#999999"
%	 anchor-point= "(250.62,17.5)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\inbit
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(58.12,60)"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\firstoutpt$
%</text>
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(170,20);(170,20);(170,0);(170,0)"
%	 />
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(167.5,0)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\otherinputt$
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(183.75,60)"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\otheroutpt$
%</text>
%<parallelogram fill-color= "#999999"
%	 fill-style= "solid"
%	 p3= "(177.5,60)"
%	 p2= "(177.5,40)"
%	 p1= "(182.5,40)"
%	 stroke-color= "#999999"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(180,60);(180,60);(180,40);(180,40)"
%	 />
%<parallelogram fill-color= "#999999"
%	 fill-style= "solid"
%	 p3= "(157.5,60)"
%	 p2= "(157.5,40)"
%	 p1= "(162.5,40)"
%	 stroke-color= "#999999"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(160,60);(160,60);(160,40);(160,40)"
%	 />
%<parallelogram fill-color= "#ffffff"
%	 fill-style= "solid"
%	 stroke-width= "0.75"
%	 p3= "(185,20)"
%	 p2= "(185,40)"
%	 p1= "(155,40)"
%	 />
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(170,30)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\hee$
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 stroke-color= "#999999"
%	 anchor-point= "(171.25,46.88)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\inbit
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(163.75,60)"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\firstoutpt$
%</text>
%<parallelogram fill-color= "#999999"
%	 fill-style= "solid"
%	 p3= "(117.5,20)"
%	 p2= "(117.5,0)"
%	 p1= "(122.5,0)"
%	 stroke-color= "#999999"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(120,20);(120,20);(120,0);(120,0)"
%	 />
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(117.5,0)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\otherinputt$
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(133.75,60)"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\otheroutpt$
%</text>
%<parallelogram fill-color= "#999999"
%	 fill-style= "solid"
%	 p3= "(127.5,60)"
%	 p2= "(127.5,40)"
%	 p1= "(132.5,40)"
%	 stroke-color= "#999999"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(130,60);(130,60);(130,40);(130,40)"
%	 />
%<parallelogram fill-color= "#999999"
%	 fill-style= "solid"
%	 p3= "(107.5,60)"
%	 p2= "(107.5,40)"
%	 p1= "(112.5,40)"
%	 stroke-color= "#999999"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(110,60);(110,60);(110,40);(110,40)"
%	 />
%<parallelogram fill-color= "#ffffff"
%	 fill-style= "solid"
%	 stroke-width= "0.75"
%	 p3= "(135,20)"
%	 p2= "(135,40)"
%	 p1= "(105,40)"
%	 />
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 stroke-color= "#999999"
%	 anchor-point= "(121.25,46.88)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\inbit
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(113.75,60)"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\firstoutpt$
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(143.75,30)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\EQLS
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(120,30)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\ehee$
%</text>
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(260,60);(260,60);(260,0);(260,0)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(240,60);(240,60);(240,0);(240,0)"
%	 />
%</jpic>
%%End JPIC-XML
%PSTricks content-type (pstricks.sty package needed)
%Add \usepackage{pstricks} in the preamble of your LaTeX file
%You can rescale the whole picture (to 80% for instance) by using the command \def\JPicScale{0.8}
\ifx\JPicScale\undefined\def\JPicScale{1}\fi
\psset{unit=\JPicScale mm}
\psset{linewidth=0.3,dotsep=1,hatchwidth=0.3,hatchsep=1.5,shadowsize=1,dimen=middle}
\psset{dotsize=0.7 2.5,dotscale=1 1,fillcolor=black}
\psset{arrowsize=1 2,arrowlength=1,arrowinset=0.25,tbarsize=0.7 5,bracketlength=0.15,rbracketlength=0.15}
\begin{pspicture}(0,0)(265,60)
\psline[linewidth=0.75](65,20)(65,0)
\rput[r](62.5,0){$\otherinputt$}
\rput[l](78.75,60){$\otheroutpt$}
\psline[linewidth=0.75](5,25)(5,0)
\rput[r](2.5,0){$\otherinputt$}
\rput(5,30){$\unit$}
\psline[linewidth=0.75](0,25)(10,25)
\psline[linewidth=0.75](10,35)(10,25)
\psline[linewidth=0.75](0,35)(0,25)
\rput(91.25,33.75){\goesto}
\rput[l](8.75,60){$\eeinptt$}
\rput[r](236.25,0){$\eeinptt$}
\newrgbcolor{userLineColour}{0.6 0.6 0.6}
\newrgbcolor{userFillColour}{0.6 0.6 0.6}
\pspolygon[linecolor=userLineColour,fillcolor=userFillColour,fillstyle=solid](242.5,0)(237.5,0)(237.5,30)(242.5,30)
\newrgbcolor{userLineColour}{0.6 0.6 0.6}
\newrgbcolor{userFillColour}{0.6 0.6 0.6}
\pspolygon[linecolor=userLineColour,fillcolor=userFillColour,fillstyle=solid](262.5,0)(257.5,0)(257.5,30)(262.5,30)
\newrgbcolor{userLineColour}{0.6 0.6 0.6}
\newrgbcolor{userFillColour}{0.6 0.6 0.6}
\pspolygon[linecolor=userLineColour,fillcolor=userFillColour,fillstyle=solid](262.5,35)(237.5,35)(237.5,60)(262.5,60)
\newrgbcolor{userLineColour}{0.6 0.6 0.6}
\newrgbcolor{userFillColour}{0.6 0.6 0.6}
\pspolygon[linecolor=userLineColour,fillcolor=userFillColour,fillstyle=solid](187.5,17.5)(152.5,17.5)(152.5,42.5)(187.5,42.5)
\newrgbcolor{userLineColour}{0.6 0.6 0.6}
\newrgbcolor{userFillColour}{0.6 0.6 0.6}
\pspolygon[linecolor=userLineColour,fillcolor=userFillColour,fillstyle=solid](172.5,0)(167.5,0)(167.5,20)(172.5,20)
\newrgbcolor{userLineColour}{0.6 0.6 0.6}
\newrgbcolor{userFillColour}{0.6 0.6 0.6}
\pspolygon[linecolor=userLineColour,fillcolor=userFillColour,fillstyle=solid](77.5,40)(72.5,40)(72.5,60)(77.5,60)
\psline[linewidth=0.75](75,60)(75,40)
\newrgbcolor{userLineColour}{0.6 0.6 0.6}
\newrgbcolor{userFillColour}{0.6 0.6 0.6}
\pspolygon[linecolor=userLineColour,fillcolor=userFillColour,fillstyle=solid](7.5,35)(2.5,35)(2.5,60)(7.5,60)
\psline[linewidth=0.75](5,60)(5,35)
\psline[linewidth=0.75](0,35)(10,35)
\newrgbcolor{userLineColour}{0.6 0.6 0.6}
\rput[r](256.25,0){$\beeinptt$}
\newrgbcolor{userLineColour}{0.6 0.6 0.6}
\rput[l](263.75,60){$\ceeoutpt$}
\pspolygon[linewidth=0.75,fillcolor=white,fillstyle=solid](235,35)(265,35)(265,25)(235,25)
\newrgbcolor{userLineColour}{0.6 0.6 0.6}
\rput(250,30){$\ffubini$}
\newrgbcolor{userLineColour}{0.6 0.6 0.6}
\newrgbcolor{userFillColour}{0.6 0.6 0.6}
\pspolygon[linecolor=userLineColour,fillcolor=userFillColour,fillstyle=solid](57.5,40)(52.5,40)(52.5,60)(57.5,60)
\psline[linewidth=0.75](55,60)(55,40)
\pspolygon[linewidth=0.75,fillcolor=white,fillstyle=solid](50,40)(80,40)(80,20)(50,20)
\rput(65,30){$\hee$}
\newrgbcolor{userLineColour}{0.6 0.6 0.6}
\rput(66.25,46.88){\inbit}
\newrgbcolor{userLineColour}{0.6 0.6 0.6}
\rput(251.25,46.25){\inbit}
\newrgbcolor{userLineColour}{0.6 0.6 0.6}
\rput(250.62,17.5){\inbit}
\rput[l](58.12,60){$\firstoutpt$}
\psline[linewidth=0.75](170,20)(170,0)
\rput[r](167.5,0){$\otherinputt$}
\rput[l](183.75,60){$\otheroutpt$}
\newrgbcolor{userLineColour}{0.6 0.6 0.6}
\newrgbcolor{userFillColour}{0.6 0.6 0.6}
\pspolygon[linecolor=userLineColour,fillcolor=userFillColour,fillstyle=solid](182.5,40)(177.5,40)(177.5,60)(182.5,60)
\psline[linewidth=0.75](180,60)(180,40)
\newrgbcolor{userLineColour}{0.6 0.6 0.6}
\newrgbcolor{userFillColour}{0.6 0.6 0.6}
\pspolygon[linecolor=userLineColour,fillcolor=userFillColour,fillstyle=solid](162.5,40)(157.5,40)(157.5,60)(162.5,60)
\psline[linewidth=0.75](160,60)(160,40)
\pspolygon[linewidth=0.75,fillcolor=white,fillstyle=solid](155,40)(185,40)(185,20)(155,20)
\rput(170,30){$\hee$}
\newrgbcolor{userLineColour}{0.6 0.6 0.6}
\rput(171.25,46.88){\inbit}
\rput[l](163.75,60){$\firstoutpt$}
\newrgbcolor{userLineColour}{0.6 0.6 0.6}
\newrgbcolor{userFillColour}{0.6 0.6 0.6}
\pspolygon[linecolor=userLineColour,fillcolor=userFillColour,fillstyle=solid](122.5,0)(117.5,0)(117.5,20)(122.5,20)
\psline[linewidth=0.75](120,20)(120,0)
\rput[r](117.5,0){$\otherinputt$}
\rput[l](133.75,60){$\otheroutpt$}
\newrgbcolor{userLineColour}{0.6 0.6 0.6}
\newrgbcolor{userFillColour}{0.6 0.6 0.6}
\pspolygon[linecolor=userLineColour,fillcolor=userFillColour,fillstyle=solid](132.5,40)(127.5,40)(127.5,60)(132.5,60)
\psline[linewidth=0.75](130,60)(130,40)
\newrgbcolor{userLineColour}{0.6 0.6 0.6}
\newrgbcolor{userFillColour}{0.6 0.6 0.6}
\pspolygon[linecolor=userLineColour,fillcolor=userFillColour,fillstyle=solid](112.5,40)(107.5,40)(107.5,60)(112.5,60)
\psline[linewidth=0.75](110,60)(110,40)
\pspolygon[linewidth=0.75,fillcolor=white,fillstyle=solid](105,40)(135,40)(135,20)(105,20)
\newrgbcolor{userLineColour}{0.6 0.6 0.6}
\rput(121.25,46.88){\inbit}
\rput[l](113.75,60){$\firstoutpt$}
\rput(143.75,30){\EQLS}
\rput(120,30){$\ehee$}
\psline[linewidth=0.75](260,60)(260,0)
\psline[linewidth=0.75](240,60)(240,0)
\end{pspicture}


==> PIC/triple-commutative.tex <==
%%Created by jPicEdt 1.4.1_03: mixed JPIC-XML/LaTeX format
%%Mon Dec 30 00:20:44 GMT-10:00 2019
%%Begin JPIC-XML
%<?xml version="1.0" standalone="yes"?>
%<jpic x-min="0" x-max="327.5" y-min="0" y-max="120" auto-bounding="true">
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(5,55);(5,55);(5,0);(5,0)"
%	 />
%<text fill-style= "none"
%	 stroke-width= "0.75"
%	 text-vert-align= "center-v"
%	 stroke-dasharray= "8;8"
%	 anchor-point= "(5,60)"
%	 text-frame= "noframe"
%	 stroke-style= "dashed"
%	 text-hor-align= "center-h"
%	 >
%$\unit$
%</text>
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(0,55);(0,55);(10,55);(10,55)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(10,65);(10,65);(10,55);(10,55)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(0,65);(0,65);(0,55);(0,55)"
%	 />
%<parallelogram fill-color= "#999999"
%	 fill-style= "solid"
%	 p3= "(2.5,120)"
%	 p2= "(2.5,100)"
%	 p1= "(32.5,100)"
%	 stroke-color= "#999999"
%	 />
%<parallelogram fill-color= "#999999"
%	 fill-style= "solid"
%	 p3= "(142.5,72.5)"
%	 p2= "(142.5,47.5)"
%	 p1= "(177.5,47.5)"
%	 stroke-color= "#999999"
%	 />
%<parallelogram fill-color= "#999999"
%	 fill-style= "solid"
%	 p3= "(157.5,50)"
%	 p2= "(157.5,0)"
%	 p1= "(162.5,0)"
%	 stroke-color= "#999999"
%	 />
%<parallelogram fill-color= "#999999"
%	 fill-style= "solid"
%	 p3= "(2.5,90)"
%	 p2= "(2.5,65)"
%	 p1= "(7.5,65)"
%	 stroke-color= "#999999"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(5,90);(5,90);(5,65);(5,65)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(0,65);(0,65);(10,65);(10,65)"
%	 />
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 stroke-color= "#999999"
%	 anchor-point= "(18.75,110.62)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\inbit
%</text>
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(160,50);(160,50);(160,0);(160,0)"
%	 />
%<parallelogram fill-color= "#999999"
%	 fill-style= "solid"
%	 p3= "(167.5,90)"
%	 p2= "(167.5,70)"
%	 p1= "(172.5,70)"
%	 stroke-color= "#999999"
%	 />
%<parallelogram fill-color= "#999999"
%	 fill-style= "solid"
%	 p3= "(147.5,90)"
%	 p2= "(147.5,70)"
%	 p1= "(152.5,70)"
%	 stroke-color= "#999999"
%	 />
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 stroke-color= "#999999"
%	 anchor-point= "(161.25,80)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\inbit
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(45,60)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\EQLS
%</text>
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(30,55);(30,55);(30,0);(30,0)"
%	 />
%<text fill-style= "none"
%	 stroke-width= "0.75"
%	 text-vert-align= "center-v"
%	 stroke-dasharray= "8;8"
%	 anchor-point= "(30,60)"
%	 text-frame= "noframe"
%	 stroke-style= "dashed"
%	 text-hor-align= "center-h"
%	 >
%$\unit$
%</text>
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(25,55);(25,55);(35,55);(35,55)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(35,65);(35,65);(35,55);(35,55)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(25,65);(25,65);(25,55);(25,55)"
%	 />
%<parallelogram fill-color= "#999999"
%	 fill-style= "solid"
%	 p3= "(27.5,90)"
%	 p2= "(27.5,65)"
%	 p1= "(32.5,65)"
%	 stroke-color= "#999999"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(30,90);(30,90);(30,65);(30,65)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(25,65);(25,65);(35,65);(35,65)"
%	 />
%<parallelogram fill-color= "#ffffff"
%	 fill-style= "solid"
%	 stroke-width= "0.75"
%	 p3= "(35,90)"
%	 p2= "(35,100)"
%	 p1= "(0,100)"
%	 />
%<text fill-color= "#ffffff"
%	 fill-style= "solid"
%	 text-vert-align= "center-v"
%	 stroke-color= "#999999"
%	 anchor-point= "(17.5,95)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\ffubini$
%</text>
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(5,120);(5,120);(5,90);(5,90)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(30,120);(30,120);(30,90);(30,90)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(60,55);(60,55);(60,0);(60,0)"
%	 />
%<parallelogram fill-color= "#999999"
%	 fill-style= "solid"
%	 p3= "(57.5,120)"
%	 p2= "(57.5,65)"
%	 p1= "(87.5,65)"
%	 stroke-color= "#999999"
%	 />
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 stroke-color= "#999999"
%	 anchor-point= "(73.12,110)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\inbit
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 stroke-color= "#999999"
%	 anchor-point= "(73.75,10)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\inbit
%</text>
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(85,55);(85,55);(85,0);(85,0)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(60,120);(60,120);(60,65);(60,65)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(85,120);(85,120);(85,65);(85,65)"
%	 />
%<parallelogram fill-color= "#ffffff"
%	 fill-style= "solid"
%	 stroke-width= "0.75"
%	 p3= "(90,55)"
%	 p2= "(90,65)"
%	 p1= "(55,65)"
%	 />
%<text fill-style= "none"
%	 stroke-width= "0.75"
%	 text-vert-align= "center-v"
%	 stroke-dasharray= "8;8"
%	 anchor-point= "(72.5,60)"
%	 text-frame= "noframe"
%	 stroke-style= "dashed"
%	 text-hor-align= "center-h"
%	 >
%$\unit$
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 stroke-color= "#999999"
%	 anchor-point= "(18.75,10)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\inbit
%</text>
%<parallelogram fill-color= "#999999"
%	 fill-style= "solid"
%	 p3= "(192.5,72.5)"
%	 p2= "(192.5,47.5)"
%	 p1= "(227.5,47.5)"
%	 stroke-color= "#999999"
%	 />
%<parallelogram fill-color= "#999999"
%	 fill-style= "solid"
%	 p3= "(207.5,50)"
%	 p2= "(207.5,0)"
%	 p1= "(212.5,0)"
%	 stroke-color= "#999999"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(210,50);(210,50);(210,0);(210,0)"
%	 />
%<parallelogram fill-color= "#999999"
%	 fill-style= "solid"
%	 p3= "(217.5,90)"
%	 p2= "(217.5,70)"
%	 p1= "(222.5,70)"
%	 stroke-color= "#999999"
%	 />
%<parallelogram fill-color= "#999999"
%	 fill-style= "solid"
%	 p3= "(197.5,90)"
%	 p2= "(197.5,70)"
%	 p1= "(202.5,70)"
%	 stroke-color= "#999999"
%	 />
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 stroke-color= "#999999"
%	 anchor-point= "(211.25,80)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\inbit
%</text>
%<parallelogram fill-color= "#ffffff"
%	 fill-style= "solid"
%	 stroke-width= "0.75"
%	 p3= "(225,50)"
%	 p2= "(225,70)"
%	 p1= "(195,70)"
%	 />
%<parallelogram fill-color= "#ffffff"
%	 fill-style= "solid"
%	 stroke-width= "0.75"
%	 p3= "(175,50)"
%	 p2= "(175,70)"
%	 p1= "(145,70)"
%	 />
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(160,60)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\hee$
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(210,60)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\fee$
%</text>
%<parallelogram fill-color= "#999999"
%	 fill-style= "solid"
%	 p3= "(147.5,120)"
%	 p2= "(147.5,100)"
%	 p1= "(222.5,100)"
%	 stroke-color= "#999999"
%	 />
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 stroke-color= "#999999"
%	 anchor-point= "(185,110)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\inbit
%</text>
%<parallelogram fill-color= "#ffffff"
%	 fill-style= "solid"
%	 stroke-width= "0.75"
%	 p3= "(225,90)"
%	 p2= "(225,100)"
%	 p1= "(145,100)"
%	 />
%<text fill-color= "#ffffff"
%	 fill-style= "solid"
%	 text-vert-align= "center-v"
%	 stroke-color= "#999999"
%	 anchor-point= "(185,95)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\ffubini$
%</text>
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(150,120);(150,120);(150,70);(150,70)"
%	 />
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 stroke-color= "#999999"
%	 anchor-point= "(186.25,10)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\inbit
%</text>
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(170,120);(170,120);(170,70);(170,70)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(220,120);(220,120);(220,70);(220,70)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(200,120);(200,120);(200,70);(200,70)"
%	 />
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 stroke-color= "#999999"
%	 anchor-point= "(160,110)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\inbit
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 stroke-color= "#999999"
%	 anchor-point= "(211.25,110)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\inbit
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(235,60)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\EQLS
%</text>
%<parallelogram fill-color= "#999999"
%	 fill-style= "solid"
%	 p3= "(257.5,47.5)"
%	 p2= "(257.5,30)"
%	 p1= "(312.5,30)"
%	 stroke-color= "#999999"
%	 />
%<parallelogram fill-color= "#999999"
%	 fill-style= "solid"
%	 p3= "(242.5,102.5)"
%	 p2= "(242.5,47.5)"
%	 p1= "(327.5,47.5)"
%	 stroke-color= "#999999"
%	 />
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 stroke-color= "#999999"
%	 anchor-point= "(261.25,80)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\inbit
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 stroke-color= "#999999"
%	 anchor-point= "(311.25,80)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\inbit
%</text>
%<parallelogram fill-color= "#ffffff"
%	 fill-style= "solid"
%	 stroke-width= "0.75"
%	 p3= "(325,50)"
%	 p2= "(325,70)"
%	 p1= "(295,70)"
%	 />
%<parallelogram fill-color= "#ffffff"
%	 fill-style= "solid"
%	 stroke-width= "0.75"
%	 p3= "(275,50)"
%	 p2= "(275,70)"
%	 p1= "(245,70)"
%	 />
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(260,60)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\hee$
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(310,60)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\fee$
%</text>
%<parallelogram fill-color= "#999999"
%	 fill-style= "solid"
%	 p3= "(247.5,120)"
%	 p2= "(247.5,100)"
%	 p1= "(322.5,100)"
%	 stroke-color= "#999999"
%	 />
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 stroke-color= "#999999"
%	 anchor-point= "(285,110)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\inbit
%</text>
%<parallelogram fill-color= "#ffffff"
%	 fill-style= "solid"
%	 stroke-width= "0.75"
%	 p3= "(325,90)"
%	 p2= "(325,100)"
%	 p1= "(245,100)"
%	 />
%<text fill-color= "#ffffff"
%	 fill-style= "solid"
%	 text-vert-align= "center-v"
%	 stroke-color= "#999999"
%	 anchor-point= "(285,95)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\ffubini$
%</text>
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(250,120);(250,120);(250,70);(250,70)"
%	 />
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 stroke-color= "#999999"
%	 anchor-point= "(285,80)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\inbit
%</text>
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(270,120);(270,120);(270,70);(270,70)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(320,120);(320,120);(320,70);(320,70)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(300,120);(300,120);(300,70);(300,70)"
%	 />
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 stroke-color= "#999999"
%	 anchor-point= "(260,110)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\inbit
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 stroke-color= "#999999"
%	 anchor-point= "(311.25,110)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\inbit
%</text>
%<parallelogram fill-color= "#999999"
%	 fill-style= "solid"
%	 p3= "(257.5,20)"
%	 p2= "(257.5,0)"
%	 p1= "(262.5,0)"
%	 stroke-color= "#999999"
%	 />
%<parallelogram fill-color= "#999999"
%	 fill-style= "solid"
%	 p3= "(307.5,20)"
%	 p2= "(307.5,0)"
%	 p1= "(312.5,0)"
%	 stroke-color= "#999999"
%	 />
%<parallelogram fill-color= "#ffffff"
%	 fill-style= "solid"
%	 stroke-width= "0.75"
%	 p3= "(315,20)"
%	 p2= "(315,30)"
%	 p1= "(255,30)"
%	 />
%<text fill-color= "#ffffff"
%	 fill-style= "solid"
%	 text-vert-align= "center-v"
%	 stroke-color= "#999999"
%	 anchor-point= "(285,25)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\ffubini$
%</text>
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(260,50);(260,50);(260,0);(260,0)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(310,50);(310,50);(310,0);(310,0)"
%	 />
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 stroke-color= "#999999"
%	 anchor-point= "(286.25,10)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\inbit
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 stroke-color= "#999999"
%	 anchor-point= "(287.5,40)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\inbit
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(45,10)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\ffour
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(235,10)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\ffive
%</text>
%</jpic>
%%End JPIC-XML
%PSTricks content-type (pstricks.sty package needed)
%Add \usepackage{pstricks} in the preamble of your LaTeX file
%You can rescale the whole picture (to 80% for instance) by using the command \def\JPicScale{0.8}
\ifx\JPicScale\undefined\def\JPicScale{1}\fi
\psset{unit=\JPicScale mm}
\psset{linewidth=0.3,dotsep=1,hatchwidth=0.3,hatchsep=1.5,shadowsize=1,dimen=middle}
\psset{dotsize=0.7 2.5,dotscale=1 1,fillcolor=black}
\psset{arrowsize=1 2,arrowlength=1,arrowinset=0.25,tbarsize=0.7 5,bracketlength=0.15,rbracketlength=0.15}
\begin{pspicture}(0,0)(327.5,120)
\psline[linewidth=0.75](5,55)(5,0)
\rput(5,60){$\unit$}
\psline[linewidth=0.75](0,55)(10,55)
\psline[linewidth=0.75](10,65)(10,55)
\psline[linewidth=0.75](0,65)(0,55)
\newrgbcolor{userLineColour}{0.6 0.6 0.6}
\newrgbcolor{userFillColour}{0.6 0.6 0.6}
\pspolygon[linecolor=userLineColour,fillcolor=userFillColour,fillstyle=solid](32.5,100)(2.5,100)(2.5,120)(32.5,120)
\newrgbcolor{userLineColour}{0.6 0.6 0.6}
\newrgbcolor{userFillColour}{0.6 0.6 0.6}
\pspolygon[linecolor=userLineColour,fillcolor=userFillColour,fillstyle=solid](177.5,47.5)(142.5,47.5)(142.5,72.5)(177.5,72.5)
\newrgbcolor{userLineColour}{0.6 0.6 0.6}
\newrgbcolor{userFillColour}{0.6 0.6 0.6}
\pspolygon[linecolor=userLineColour,fillcolor=userFillColour,fillstyle=solid](162.5,0)(157.5,0)(157.5,50)(162.5,50)
\newrgbcolor{userLineColour}{0.6 0.6 0.6}
\newrgbcolor{userFillColour}{0.6 0.6 0.6}
\pspolygon[linecolor=userLineColour,fillcolor=userFillColour,fillstyle=solid](7.5,65)(2.5,65)(2.5,90)(7.5,90)
\psline[linewidth=0.75](5,90)(5,65)
\psline[linewidth=0.75](0,65)(10,65)
\newrgbcolor{userLineColour}{0.6 0.6 0.6}
\rput(18.75,110.62){\inbit}
\psline[linewidth=0.75](160,50)(160,0)
\newrgbcolor{userLineColour}{0.6 0.6 0.6}
\newrgbcolor{userFillColour}{0.6 0.6 0.6}
\pspolygon[linecolor=userLineColour,fillcolor=userFillColour,fillstyle=solid](172.5,70)(167.5,70)(167.5,90)(172.5,90)
\newrgbcolor{userLineColour}{0.6 0.6 0.6}
\newrgbcolor{userFillColour}{0.6 0.6 0.6}
\pspolygon[linecolor=userLineColour,fillcolor=userFillColour,fillstyle=solid](152.5,70)(147.5,70)(147.5,90)(152.5,90)
\newrgbcolor{userLineColour}{0.6 0.6 0.6}
\rput(161.25,80){\inbit}
\rput(45,60){\EQLS}
\psline[linewidth=0.75](30,55)(30,0)
\rput(30,60){$\unit$}
\psline[linewidth=0.75](25,55)(35,55)
\psline[linewidth=0.75](35,65)(35,55)
\psline[linewidth=0.75](25,65)(25,55)
\newrgbcolor{userLineColour}{0.6 0.6 0.6}
\newrgbcolor{userFillColour}{0.6 0.6 0.6}
\pspolygon[linecolor=userLineColour,fillcolor=userFillColour,fillstyle=solid](32.5,65)(27.5,65)(27.5,90)(32.5,90)
\psline[linewidth=0.75](30,90)(30,65)
\psline[linewidth=0.75](25,65)(35,65)
\pspolygon[linewidth=0.75,fillcolor=white,fillstyle=solid](0,100)(35,100)(35,90)(0,90)
\newrgbcolor{userLineColour}{0.6 0.6 0.6}
\rput(17.5,95){$\ffubini$}
\psline[linewidth=0.75](5,120)(5,90)
\psline[linewidth=0.75](30,120)(30,90)
\psline[linewidth=0.75](60,55)(60,0)
\newrgbcolor{userLineColour}{0.6 0.6 0.6}
\newrgbcolor{userFillColour}{0.6 0.6 0.6}
\pspolygon[linecolor=userLineColour,fillcolor=userFillColour,fillstyle=solid](87.5,65)(57.5,65)(57.5,120)(87.5,120)
\newrgbcolor{userLineColour}{0.6 0.6 0.6}
\rput(73.12,110){\inbit}
\newrgbcolor{userLineColour}{0.6 0.6 0.6}
\rput(73.75,10){\inbit}
\psline[linewidth=0.75](85,55)(85,0)
\psline[linewidth=0.75](60,120)(60,65)
\psline[linewidth=0.75](85,120)(85,65)
\pspolygon[linewidth=0.75,fillcolor=white,fillstyle=solid](55,65)(90,65)(90,55)(55,55)
\rput(72.5,60){$\unit$}
\newrgbcolor{userLineColour}{0.6 0.6 0.6}
\rput(18.75,10){\inbit}
\newrgbcolor{userLineColour}{0.6 0.6 0.6}
\newrgbcolor{userFillColour}{0.6 0.6 0.6}
\pspolygon[linecolor=userLineColour,fillcolor=userFillColour,fillstyle=solid](227.5,47.5)(192.5,47.5)(192.5,72.5)(227.5,72.5)
\newrgbcolor{userLineColour}{0.6 0.6 0.6}
\newrgbcolor{userFillColour}{0.6 0.6 0.6}
\pspolygon[linecolor=userLineColour,fillcolor=userFillColour,fillstyle=solid](212.5,0)(207.5,0)(207.5,50)(212.5,50)
\psline[linewidth=0.75](210,50)(210,0)
\newrgbcolor{userLineColour}{0.6 0.6 0.6}
\newrgbcolor{userFillColour}{0.6 0.6 0.6}
\pspolygon[linecolor=userLineColour,fillcolor=userFillColour,fillstyle=solid](222.5,70)(217.5,70)(217.5,90)(222.5,90)
\newrgbcolor{userLineColour}{0.6 0.6 0.6}
\newrgbcolor{userFillColour}{0.6 0.6 0.6}
\pspolygon[linecolor=userLineColour,fillcolor=userFillColour,fillstyle=solid](202.5,70)(197.5,70)(197.5,90)(202.5,90)
\newrgbcolor{userLineColour}{0.6 0.6 0.6}
\rput(211.25,80){\inbit}
\pspolygon[linewidth=0.75,fillcolor=white,fillstyle=solid](195,70)(225,70)(225,50)(195,50)
\pspolygon[linewidth=0.75,fillcolor=white,fillstyle=solid](145,70)(175,70)(175,50)(145,50)
\rput(160,60){$\hee$}
\rput(210,60){$\fee$}
\newrgbcolor{userLineColour}{0.6 0.6 0.6}
\newrgbcolor{userFillColour}{0.6 0.6 0.6}
\pspolygon[linecolor=userLineColour,fillcolor=userFillColour,fillstyle=solid](222.5,100)(147.5,100)(147.5,120)(222.5,120)
\newrgbcolor{userLineColour}{0.6 0.6 0.6}
\rput(185,110){\inbit}
\pspolygon[linewidth=0.75,fillcolor=white,fillstyle=solid](145,100)(225,100)(225,90)(145,90)
\newrgbcolor{userLineColour}{0.6 0.6 0.6}
\rput(185,95){$\ffubini$}
\psline[linewidth=0.75](150,120)(150,70)
\newrgbcolor{userLineColour}{0.6 0.6 0.6}
\rput(186.25,10){\inbit}
\psline[linewidth=0.75](170,120)(170,70)
\psline[linewidth=0.75](220,120)(220,70)
\psline[linewidth=0.75](200,120)(200,70)
\newrgbcolor{userLineColour}{0.6 0.6 0.6}
\rput(160,110){\inbit}
\newrgbcolor{userLineColour}{0.6 0.6 0.6}
\rput(211.25,110){\inbit}
\rput(235,60){\EQLS}
\newrgbcolor{userLineColour}{0.6 0.6 0.6}
\newrgbcolor{userFillColour}{0.6 0.6 0.6}
\pspolygon[linecolor=userLineColour,fillcolor=userFillColour,fillstyle=solid](312.5,30)(257.5,30)(257.5,47.5)(312.5,47.5)
\newrgbcolor{userLineColour}{0.6 0.6 0.6}
\newrgbcolor{userFillColour}{0.6 0.6 0.6}
\pspolygon[linecolor=userLineColour,fillcolor=userFillColour,fillstyle=solid](327.5,47.5)(242.5,47.5)(242.5,102.5)(327.5,102.5)
\newrgbcolor{userLineColour}{0.6 0.6 0.6}
\rput(261.25,80){\inbit}
\newrgbcolor{userLineColour}{0.6 0.6 0.6}
\rput(311.25,80){\inbit}
\pspolygon[linewidth=0.75,fillcolor=white,fillstyle=solid](295,70)(325,70)(325,50)(295,50)
\pspolygon[linewidth=0.75,fillcolor=white,fillstyle=solid](245,70)(275,70)(275,50)(245,50)
\rput(260,60){$\hee$}
\rput(310,60){$\fee$}
\newrgbcolor{userLineColour}{0.6 0.6 0.6}
\newrgbcolor{userFillColour}{0.6 0.6 0.6}
\pspolygon[linecolor=userLineColour,fillcolor=userFillColour,fillstyle=solid](322.5,100)(247.5,100)(247.5,120)(322.5,120)
\newrgbcolor{userLineColour}{0.6 0.6 0.6}
\rput(285,110){\inbit}
\pspolygon[linewidth=0.75,fillcolor=white,fillstyle=solid](245,100)(325,100)(325,90)(245,90)
\newrgbcolor{userLineColour}{0.6 0.6 0.6}
\rput(285,95){$\ffubini$}
\psline[linewidth=0.75](250,120)(250,70)
\newrgbcolor{userLineColour}{0.6 0.6 0.6}
\rput(285,80){\inbit}
\psline[linewidth=0.75](270,120)(270,70)
\psline[linewidth=0.75](320,120)(320,70)
\psline[linewidth=0.75](300,120)(300,70)
\newrgbcolor{userLineColour}{0.6 0.6 0.6}
\rput(260,110){\inbit}
\newrgbcolor{userLineColour}{0.6 0.6 0.6}
\rput(311.25,110){\inbit}
\newrgbcolor{userLineColour}{0.6 0.6 0.6}
\newrgbcolor{userFillColour}{0.6 0.6 0.6}
\pspolygon[linecolor=userLineColour,fillcolor=userFillColour,fillstyle=solid](262.5,0)(257.5,0)(257.5,20)(262.5,20)
\newrgbcolor{userLineColour}{0.6 0.6 0.6}
\newrgbcolor{userFillColour}{0.6 0.6 0.6}
\pspolygon[linecolor=userLineColour,fillcolor=userFillColour,fillstyle=solid](312.5,0)(307.5,0)(307.5,20)(312.5,20)
\pspolygon[linewidth=0.75,fillcolor=white,fillstyle=solid](255,30)(315,30)(315,20)(255,20)
\newrgbcolor{userLineColour}{0.6 0.6 0.6}
\rput(285,25){$\ffubini$}
\psline[linewidth=0.75](260,50)(260,0)
\psline[linewidth=0.75](310,50)(310,0)
\newrgbcolor{userLineColour}{0.6 0.6 0.6}
\rput(286.25,10){\inbit}
\newrgbcolor{userLineColour}{0.6 0.6 0.6}
\rput(287.5,40){\inbit}
\rput(45,10){\ffour}
\rput(235,10){\ffive}
\end{pspicture}


==> PIC/triple-eqns-2.tex <==
%%Created by jPicEdt 1.4.1_03: mixed JPIC-XML/LaTeX format
%%Sun Nov 03 12:11:37 GMT-10:00 2019
%%Begin JPIC-XML
%<?xml version="1.0" standalone="yes"?>
%<jpic x-min="0" x-max="277.5" y-min="0" y-max="90" auto-bounding="true">
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(140,60);(140,60);(140,40);(140,40)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(160,40);(160,40);(160,60);(160,60)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(140,40);(140,40);(160,40);(160,40)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(150,40);(150,40);(150,0);(150,0)"
%	 />
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(150,50)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\hee$
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 stroke-width= "0.75"
%	 stroke-dasharray= "8;8"
%	 stroke-style= "dashed"
%	 anchor-point= "(22.5,50)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\EQLS
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 stroke-width= "0.75"
%	 stroke-dasharray= "8;8"
%	 stroke-style= "dashed"
%	 anchor-point= "(245,50)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\EQLS
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 stroke-width= "0.75"
%	 stroke-dasharray= "8;8"
%	 stroke-style= "dashed"
%	 anchor-point= "(130,50)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\EQLS
%</text>
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(107.5,12.5);(107.5,12.5);(107.5,0);(107.5,0)"
%	 />
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 stroke-width= "0.75"
%	 stroke-dasharray= "8;8"
%	 stroke-style= "dashed"
%	 anchor-point= "(22.5,5)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\oone
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 stroke-width= "0.75"
%	 stroke-dasharray= "8;8"
%	 stroke-style= "dashed"
%	 anchor-point= "(130,5)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\ttwo
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 stroke-width= "0.75"
%	 stroke-dasharray= "8;8"
%	 stroke-style= "dashed"
%	 anchor-point= "(245,5)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\tthree
%</text>
%<parallelogram fill-style= "solid"
%	 p3= "(5,90)"
%	 p2= "(5,55)"
%	 p1= "(10,55)"
%	 fill-color= "#999999"
%	 stroke-color= "#999999"
%	 />
%<parallelogram fill-style= "solid"
%	 p3= "(0,57.5)"
%	 p2= "(0,42.5)"
%	 p1= "(15,42.5)"
%	 fill-color= "#999999"
%	 stroke-color= "#999999"
%	 />
%<parallelogram fill-style= "solid"
%	 p3= "(12.5,45)"
%	 p2= "(12.5,55)"
%	 stroke-width= "0.75"
%	 p1= "(2.5,55)"
%	 fill-color= "#ffffff"
%	 />
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 stroke-width= "0.75"
%	 stroke-dasharray= "8;8"
%	 stroke-style= "dashed"
%	 anchor-point= "(7.5,50)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\unit$
%</text>
%<parallelogram fill-style= "solid"
%	 p3= "(5,42.5)"
%	 p2= "(5,0)"
%	 p1= "(10,0)"
%	 fill-color= "#999999"
%	 stroke-color= "#999999"
%	 />
%<parallelogram fill-style= "solid"
%	 p3= "(30,90)"
%	 p2= "(30,0)"
%	 p1= "(35,0)"
%	 fill-color= "#999999"
%	 stroke-color= "#999999"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(7.5,45);(7.5,45);(7.5,0);(7.5,0)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(7.5,90);(7.5,90);(7.5,55);(7.5,55)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(32.5,90);(32.5,90);(32.5,0);(32.5,0)"
%	 />
%<parallelogram fill-style= "solid"
%	 p3= "(95,62.5)"
%	 p2= "(95,37.5)"
%	 p1= "(120,37.5)"
%	 fill-color= "#999999"
%	 stroke-color= "#999999"
%	 />
%<parallelogram fill-style= "solid"
%	 p3= "(105,90)"
%	 p2= "(105,60)"
%	 p1= "(110,60)"
%	 fill-color= "#999999"
%	 stroke-color= "#999999"
%	 />
%<parallelogram fill-style= "solid"
%	 p3= "(105,40)"
%	 p2= "(105,22.5)"
%	 p1= "(110,22.5)"
%	 fill-color= "#999999"
%	 stroke-color= "#999999"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(107.5,90);(107.5,90);(107.5,60);(107.5,60)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(107.5,40);(107.5,40);(107.5,22.5);(107.5,22.5)"
%	 />
%<parallelogram fill-style= "solid"
%	 p3= "(117.5,40)"
%	 p2= "(117.5,60)"
%	 stroke-width= "0.75"
%	 p1= "(97.5,60)"
%	 fill-color= "#ffffff"
%	 />
%<text fill-style= "solid"
%	 text-vert-align= "center-v"
%	 stroke-width= "0.75"
%	 fill-color= "#ffffff"
%	 stroke-dasharray= "8;8"
%	 stroke-style= "dashed"
%	 anchor-point= "(107.5,50)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\eehee$
%</text>
%<parallelogram fill-style= "solid"
%	 p3= "(112.5,12.5)"
%	 p2= "(112.5,22.5)"
%	 stroke-width= "0.75"
%	 p1= "(102.5,22.5)"
%	 fill-color= "#ffffff"
%	 />
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 stroke-width= "0.75"
%	 stroke-dasharray= "8;8"
%	 stroke-style= "dashed"
%	 anchor-point= "(107.5,17.5)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\unit$
%</text>
%<parallelogram fill-style= "solid"
%	 p3= "(147.5,90)"
%	 p2= "(147.5,60)"
%	 p1= "(152.5,60)"
%	 fill-color= "#999999"
%	 stroke-color= "#999999"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(150,90);(150,90);(150,60);(150,60)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(140,60);(140,60);(160,60);(160,60)"
%	 />
%<parallelogram fill-style= "solid"
%	 p3= "(212.5,77.5)"
%	 p2= "(212.5,17.5)"
%	 p1= "(237.5,17.5)"
%	 fill-color= "#999999"
%	 stroke-color= "#999999"
%	 />
%<parallelogram fill-style= "solid"
%	 p3= "(235,20)"
%	 p2= "(235,40)"
%	 stroke-width= "0.75"
%	 p1= "(215,40)"
%	 fill-color= "#ffffff"
%	 />
%<parallelogram fill-style= "solid"
%	 p3= "(222.5,90)"
%	 p2= "(222.5,75)"
%	 p1= "(227.5,75)"
%	 fill-color= "#999999"
%	 stroke-color= "#999999"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(225,90);(225,90);(225,75);(225,75)"
%	 />
%<parallelogram fill-style= "solid"
%	 p3= "(222.5,55)"
%	 p2= "(222.5,42.5)"
%	 p1= "(227.5,42.5)"
%	 fill-color= "#999999"
%	 stroke-color= "#999999"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(225,55);(225,55);(225,40);(225,40)"
%	 />
%<parallelogram fill-style= "solid"
%	 p3= "(222.5,17.5)"
%	 p2= "(222.5,0)"
%	 p1= "(227.5,0)"
%	 fill-color= "#999999"
%	 stroke-color= "#999999"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(225,20);(225,20);(225,0);(225,0)"
%	 />
%<parallelogram fill-style= "solid"
%	 p3= "(235,55)"
%	 p2= "(235,75)"
%	 stroke-width= "0.75"
%	 p1= "(215,75)"
%	 fill-color= "#ffffff"
%	 />
%<parallelogram fill-style= "solid"
%	 p3= "(252.5,77.5)"
%	 p2= "(252.5,52.5)"
%	 p1= "(277.5,52.5)"
%	 fill-color= "#999999"
%	 stroke-color= "#999999"
%	 />
%<parallelogram fill-style= "solid"
%	 p3= "(252.5,42.5)"
%	 p2= "(252.5,17.5)"
%	 p1= "(277.5,17.5)"
%	 fill-color= "#999999"
%	 stroke-color= "#999999"
%	 />
%<parallelogram fill-style= "solid"
%	 p3= "(275,20)"
%	 p2= "(275,40)"
%	 stroke-width= "0.75"
%	 p1= "(255,40)"
%	 fill-color= "#ffffff"
%	 />
%<parallelogram fill-style= "solid"
%	 p3= "(262.5,90)"
%	 p2= "(262.5,75)"
%	 p1= "(267.5,75)"
%	 fill-color= "#999999"
%	 stroke-color= "#999999"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(265,90);(265,90);(265,75);(265,75)"
%	 />
%<parallelogram fill-style= "solid"
%	 p3= "(262.5,55)"
%	 p2= "(262.5,42.5)"
%	 p1= "(267.5,42.5)"
%	 fill-color= "#999999"
%	 stroke-color= "#999999"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(265,55);(265,55);(265,40);(265,40)"
%	 />
%<parallelogram fill-style= "solid"
%	 p3= "(262.5,17.5)"
%	 p2= "(262.5,0)"
%	 p1= "(267.5,0)"
%	 fill-color= "#999999"
%	 stroke-color= "#999999"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(265,20);(265,20);(265,0);(265,0)"
%	 />
%<parallelogram fill-style= "solid"
%	 p3= "(275,55)"
%	 p2= "(275,75)"
%	 stroke-width= "0.75"
%	 p1= "(255,75)"
%	 fill-color= "#ffffff"
%	 />
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 stroke-width= "0.75"
%	 stroke-dasharray= "8;8"
%	 stroke-style= "dashed"
%	 anchor-point= "(225,30)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\gee$
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 stroke-width= "0.7"
%	 anchor-point= "(265,30)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\eegee$
%</text>
%<text fill-style= "solid"
%	 text-vert-align= "center-v"
%	 stroke-width= "0.75"
%	 fill-color= "#ffffff"
%	 stroke-dasharray= "8;8"
%	 stroke-style= "dashed"
%	 anchor-point= "(225,65)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\eehee$
%</text>
%<text fill-style= "solid"
%	 text-vert-align= "center-v"
%	 stroke-width= "0.75"
%	 fill-color= "#ffffff"
%	 stroke-dasharray= "8;8"
%	 stroke-style= "dashed"
%	 anchor-point= "(265,65)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\eehee$
%</text>
%</jpic>
%%End JPIC-XML
%PSTricks content-type (pstricks.sty package needed)
%Add \usepackage{pstricks} in the preamble of your LaTeX file
%You can rescale the whole picture (to 80% for instance) by using the command \def\JPicScale{0.8}
\ifx\JPicScale\undefined\def\JPicScale{1}\fi
\psset{unit=\JPicScale mm}
\psset{linewidth=0.3,dotsep=1,hatchwidth=0.3,hatchsep=1.5,shadowsize=1,dimen=middle}
\psset{dotsize=0.7 2.5,dotscale=1 1,fillcolor=black}
\psset{arrowsize=1 2,arrowlength=1,arrowinset=0.25,tbarsize=0.7 5,bracketlength=0.15,rbracketlength=0.15}
\begin{pspicture}(0,0)(277.5,90)
\psline[linewidth=0.75](140,60)(140,40)
\psline[linewidth=0.75](160,40)(160,60)
\psline[linewidth=0.75](140,40)(160,40)
\psline[linewidth=0.75](150,40)(150,0)
\rput(150,50){$\hee$}
\rput(22.5,50){\EQLS}
\rput(245,50){\EQLS}
\rput(130,50){\EQLS}
\psline[linewidth=0.75](107.5,12.5)(107.5,0)
\rput(22.5,5){\oone}
\rput(130,5){\ttwo}
\rput(245,5){\tthree}
\newrgbcolor{userLineColour}{0.6 0.6 0.6}
\newrgbcolor{userFillColour}{0.6 0.6 0.6}
\pspolygon[linecolor=userLineColour,fillcolor=userFillColour,fillstyle=solid](10,55)(5,55)(5,90)(10,90)
\newrgbcolor{userLineColour}{0.6 0.6 0.6}
\newrgbcolor{userFillColour}{0.6 0.6 0.6}
\pspolygon[linecolor=userLineColour,fillcolor=userFillColour,fillstyle=solid](15,42.5)(0,42.5)(0,57.5)(15,57.5)
\pspolygon[linewidth=0.75,fillcolor=white,fillstyle=solid](2.5,55)(12.5,55)(12.5,45)(2.5,45)
\rput(7.5,50){$\unit$}
\newrgbcolor{userLineColour}{0.6 0.6 0.6}
\newrgbcolor{userFillColour}{0.6 0.6 0.6}
\pspolygon[linecolor=userLineColour,fillcolor=userFillColour,fillstyle=solid](10,0)(5,0)(5,42.5)(10,42.5)
\newrgbcolor{userLineColour}{0.6 0.6 0.6}
\newrgbcolor{userFillColour}{0.6 0.6 0.6}
\pspolygon[linecolor=userLineColour,fillcolor=userFillColour,fillstyle=solid](35,0)(30,0)(30,90)(35,90)
\psline[linewidth=0.75](7.5,45)(7.5,0)
\psline[linewidth=0.75](7.5,90)(7.5,55)
\psline[linewidth=0.75](32.5,90)(32.5,0)
\newrgbcolor{userLineColour}{0.6 0.6 0.6}
\newrgbcolor{userFillColour}{0.6 0.6 0.6}
\pspolygon[linecolor=userLineColour,fillcolor=userFillColour,fillstyle=solid](120,37.5)(95,37.5)(95,62.5)(120,62.5)
\newrgbcolor{userLineColour}{0.6 0.6 0.6}
\newrgbcolor{userFillColour}{0.6 0.6 0.6}
\pspolygon[linecolor=userLineColour,fillcolor=userFillColour,fillstyle=solid](110,60)(105,60)(105,90)(110,90)
\newrgbcolor{userLineColour}{0.6 0.6 0.6}
\newrgbcolor{userFillColour}{0.6 0.6 0.6}
\pspolygon[linecolor=userLineColour,fillcolor=userFillColour,fillstyle=solid](110,22.5)(105,22.5)(105,40)(110,40)
\psline[linewidth=0.75](107.5,90)(107.5,60)
\psline[linewidth=0.75](107.5,40)(107.5,22.5)
\pspolygon[linewidth=0.75,fillcolor=white,fillstyle=solid](97.5,60)(117.5,60)(117.5,40)(97.5,40)
\rput(107.5,50){$\eehee$}
\pspolygon[linewidth=0.75,fillcolor=white,fillstyle=solid](102.5,22.5)(112.5,22.5)(112.5,12.5)(102.5,12.5)
\rput(107.5,17.5){$\unit$}
\newrgbcolor{userLineColour}{0.6 0.6 0.6}
\newrgbcolor{userFillColour}{0.6 0.6 0.6}
\pspolygon[linecolor=userLineColour,fillcolor=userFillColour,fillstyle=solid](152.5,60)(147.5,60)(147.5,90)(152.5,90)
\psline[linewidth=0.75](150,90)(150,60)
\psline[linewidth=0.75](140,60)(160,60)
\newrgbcolor{userLineColour}{0.6 0.6 0.6}
\newrgbcolor{userFillColour}{0.6 0.6 0.6}
\pspolygon[linecolor=userLineColour,fillcolor=userFillColour,fillstyle=solid](237.5,17.5)(212.5,17.5)(212.5,77.5)(237.5,77.5)
\pspolygon[linewidth=0.75,fillcolor=white,fillstyle=solid](215,40)(235,40)(235,20)(215,20)
\newrgbcolor{userLineColour}{0.6 0.6 0.6}
\newrgbcolor{userFillColour}{0.6 0.6 0.6}
\pspolygon[linecolor=userLineColour,fillcolor=userFillColour,fillstyle=solid](227.5,75)(222.5,75)(222.5,90)(227.5,90)
\psline[linewidth=0.75](225,90)(225,75)
\newrgbcolor{userLineColour}{0.6 0.6 0.6}
\newrgbcolor{userFillColour}{0.6 0.6 0.6}
\pspolygon[linecolor=userLineColour,fillcolor=userFillColour,fillstyle=solid](227.5,42.5)(222.5,42.5)(222.5,55)(227.5,55)
\psline[linewidth=0.75](225,55)(225,40)
\newrgbcolor{userLineColour}{0.6 0.6 0.6}
\newrgbcolor{userFillColour}{0.6 0.6 0.6}
\pspolygon[linecolor=userLineColour,fillcolor=userFillColour,fillstyle=solid](227.5,0)(222.5,0)(222.5,17.5)(227.5,17.5)
\psline[linewidth=0.75](225,20)(225,0)
\pspolygon[linewidth=0.75,fillcolor=white,fillstyle=solid](215,75)(235,75)(235,55)(215,55)
\newrgbcolor{userLineColour}{0.6 0.6 0.6}
\newrgbcolor{userFillColour}{0.6 0.6 0.6}
\pspolygon[linecolor=userLineColour,fillcolor=userFillColour,fillstyle=solid](277.5,52.5)(252.5,52.5)(252.5,77.5)(277.5,77.5)
\newrgbcolor{userLineColour}{0.6 0.6 0.6}
\newrgbcolor{userFillColour}{0.6 0.6 0.6}
\pspolygon[linecolor=userLineColour,fillcolor=userFillColour,fillstyle=solid](277.5,17.5)(252.5,17.5)(252.5,42.5)(277.5,42.5)
\pspolygon[linewidth=0.75,fillcolor=white,fillstyle=solid](255,40)(275,40)(275,20)(255,20)
\newrgbcolor{userLineColour}{0.6 0.6 0.6}
\newrgbcolor{userFillColour}{0.6 0.6 0.6}
\pspolygon[linecolor=userLineColour,fillcolor=userFillColour,fillstyle=solid](267.5,75)(262.5,75)(262.5,90)(267.5,90)
\psline[linewidth=0.75](265,90)(265,75)
\newrgbcolor{userLineColour}{0.6 0.6 0.6}
\newrgbcolor{userFillColour}{0.6 0.6 0.6}
\pspolygon[linecolor=userLineColour,fillcolor=userFillColour,fillstyle=solid](267.5,42.5)(262.5,42.5)(262.5,55)(267.5,55)
\psline[linewidth=0.75](265,55)(265,40)
\newrgbcolor{userLineColour}{0.6 0.6 0.6}
\newrgbcolor{userFillColour}{0.6 0.6 0.6}
\pspolygon[linecolor=userLineColour,fillcolor=userFillColour,fillstyle=solid](267.5,0)(262.5,0)(262.5,17.5)(267.5,17.5)
\psline[linewidth=0.75](265,20)(265,0)
\pspolygon[linewidth=0.75,fillcolor=white,fillstyle=solid](255,75)(275,75)(275,55)(255,55)
\rput(225,30){$\gee$}
\rput(265,30){$\eegee$}
\rput(225,65){$\eehee$}
\rput(265,65){$\eehee$}
\end{pspicture}


==> PIC/triple-eqns-3.tex <==
%%Created by jPicEdt 1.4.1_03: mixed JPIC-XML/LaTeX format
%%Fri Nov 01 12:35:51 GMT-10:00 2019
%%Begin JPIC-XML
%<?xml version="1.0" standalone="yes"?>
%<jpic x-min="0" x-max="312.5" y-min="0" y-max="90" auto-bounding="true">
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 stroke-dasharray= "8;8"
%	 anchor-point= "(22.5,50)"
%	 stroke-style= "dashed"
%	 text-frame= "noframe"
%	 stroke-width= "0.75"
%	 text-hor-align= "center-h"
%	 >
%\EQLS
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 stroke-dasharray= "8;8"
%	 anchor-point= "(130,50)"
%	 stroke-style= "dashed"
%	 text-frame= "noframe"
%	 stroke-width= "0.75"
%	 text-hor-align= "center-h"
%	 >
%\EQLS
%</text>
%<multicurve fill-style= "none"
%	 points= "(105,15);(105,15);(105,0);(105,0)"
%	 stroke-width= "0.75"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 stroke-dasharray= "8;8"
%	 anchor-point= "(22.5,5)"
%	 stroke-style= "dashed"
%	 text-frame= "noframe"
%	 stroke-width= "0.75"
%	 text-hor-align= "center-h"
%	 >
%\oone
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 stroke-dasharray= "8;8"
%	 anchor-point= "(130,5)"
%	 stroke-style= "dashed"
%	 text-frame= "noframe"
%	 stroke-width= "0.75"
%	 text-hor-align= "center-h"
%	 >
%\ttwo
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 stroke-dasharray= "8;8"
%	 anchor-point= "(270,5)"
%	 stroke-style= "dashed"
%	 text-frame= "noframe"
%	 stroke-width= "0.75"
%	 text-hor-align= "center-h"
%	 >
%\tthree
%</text>
%<parallelogram p3= "(5,90)"
%	 fill-style= "solid"
%	 p2= "(5,55)"
%	 fill-color= "#999999"
%	 p1= "(10,55)"
%	 stroke-color= "#999999"
%	 />
%<parallelogram p3= "(0,57.5)"
%	 fill-style= "solid"
%	 p2= "(0,42.5)"
%	 fill-color= "#999999"
%	 p1= "(15,42.5)"
%	 stroke-color= "#999999"
%	 />
%<parallelogram p3= "(12.5,45)"
%	 fill-style= "solid"
%	 p2= "(12.5,55)"
%	 fill-color= "#ffffff"
%	 p1= "(2.5,55)"
%	 stroke-width= "0.75"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 stroke-dasharray= "8;8"
%	 anchor-point= "(7.5,50)"
%	 stroke-style= "dashed"
%	 text-frame= "noframe"
%	 stroke-width= "0.75"
%	 text-hor-align= "center-h"
%	 >
%$\unit$
%</text>
%<parallelogram p3= "(5,42.5)"
%	 fill-style= "solid"
%	 p2= "(5,0)"
%	 fill-color= "#999999"
%	 p1= "(10,0)"
%	 stroke-color= "#999999"
%	 />
%<parallelogram p3= "(30,90)"
%	 fill-style= "solid"
%	 p2= "(30,0)"
%	 fill-color= "#999999"
%	 p1= "(35,0)"
%	 stroke-color= "#999999"
%	 />
%<multicurve fill-style= "none"
%	 points= "(7.5,45);(7.5,45);(7.5,0);(7.5,0)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(7.5,90);(7.5,90);(7.5,55);(7.5,55)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(32.5,90);(32.5,90);(32.5,0);(32.5,0)"
%	 stroke-width= "0.75"
%	 />
%<parallelogram p3= "(110,15)"
%	 fill-style= "solid"
%	 p2= "(110,25)"
%	 fill-color= "#ffffff"
%	 p1= "(100,25)"
%	 stroke-width= "0.75"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 stroke-dasharray= "8;8"
%	 anchor-point= "(105,20)"
%	 stroke-style= "dashed"
%	 text-frame= "noframe"
%	 stroke-width= "0.75"
%	 text-hor-align= "center-h"
%	 >
%$\unit$
%</text>
%<parallelogram p3= "(87.5,62.5)"
%	 fill-style= "solid"
%	 p2= "(87.5,37.5)"
%	 fill-color= "#999999"
%	 p1= "(122.5,37.5)"
%	 stroke-color= "#999999"
%	 />
%<parallelogram p3= "(102.5,40)"
%	 fill-style= "solid"
%	 p2= "(102.5,25)"
%	 fill-color= "#999999"
%	 p1= "(107.5,25)"
%	 stroke-color= "#999999"
%	 />
%<multicurve fill-style= "none"
%	 points= "(105,40);(105,40);(105,25);(105,25)"
%	 stroke-width= "0.75"
%	 />
%<parallelogram p3= "(112.5,90)"
%	 fill-style= "solid"
%	 p2= "(112.5,60)"
%	 fill-color= "#999999"
%	 p1= "(117.5,60)"
%	 stroke-color= "#999999"
%	 />
%<multicurve fill-style= "none"
%	 points= "(115,90);(115,90);(115,60);(115,60)"
%	 stroke-width= "0.75"
%	 />
%<parallelogram p3= "(92.5,90)"
%	 fill-style= "solid"
%	 p2= "(92.5,60)"
%	 fill-color= "#999999"
%	 p1= "(97.5,60)"
%	 stroke-color= "#999999"
%	 />
%<multicurve fill-style= "none"
%	 points= "(95,90);(95,90);(95,60);(95,60)"
%	 stroke-width= "0.75"
%	 />
%<parallelogram p3= "(120,40)"
%	 fill-style= "solid"
%	 p2= "(120,60)"
%	 fill-color= "#ffffff"
%	 p1= "(90,60)"
%	 stroke-width= "0.75"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(106.25,66.88)"
%	 stroke-color= "#999999"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\inbit
%</text>
%<multicurve fill-style= "none"
%	 points= "(155,40);(155,40);(155,0);(155,0)"
%	 stroke-width= "0.75"
%	 />
%<parallelogram p3= "(162.5,90)"
%	 fill-style= "solid"
%	 p2= "(162.5,60)"
%	 fill-color= "#999999"
%	 p1= "(167.5,60)"
%	 stroke-color= "#999999"
%	 />
%<multicurve fill-style= "none"
%	 points= "(165,90);(165,90);(165,60);(165,60)"
%	 stroke-width= "0.75"
%	 />
%<parallelogram p3= "(142.5,90)"
%	 fill-style= "solid"
%	 p2= "(142.5,60)"
%	 fill-color= "#999999"
%	 p1= "(147.5,60)"
%	 stroke-color= "#999999"
%	 />
%<multicurve fill-style= "none"
%	 points= "(145,90);(145,90);(145,60);(145,60)"
%	 stroke-width= "0.75"
%	 />
%<parallelogram p3= "(170,40)"
%	 fill-style= "solid"
%	 p2= "(170,60)"
%	 fill-color= "#ffffff"
%	 p1= "(140,60)"
%	 stroke-width= "0.75"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(156.25,66.88)"
%	 stroke-color= "#999999"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\inbit
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 stroke-dasharray= "8;8"
%	 anchor-point= "(270,50)"
%	 stroke-style= "dashed"
%	 text-frame= "noframe"
%	 stroke-width= "0.75"
%	 text-hor-align= "center-h"
%	 >
%\EQLS
%</text>
%<parallelogram p3= "(227.5,77.5)"
%	 fill-style= "solid"
%	 p2= "(227.5,17.5)"
%	 fill-color= "#999999"
%	 p1= "(262.5,17.5)"
%	 stroke-color= "#999999"
%	 />
%<parallelogram p3= "(242.5,20)"
%	 fill-style= "solid"
%	 p2= "(242.5,0)"
%	 fill-color= "#999999"
%	 p1= "(247.5,0)"
%	 stroke-color= "#999999"
%	 />
%<multicurve fill-style= "none"
%	 points= "(245,20);(245,20);(245,0);(245,0)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(245,55);(245,55);(245,40);(245,40)"
%	 stroke-width= "0.75"
%	 />
%<parallelogram p3= "(260,20)"
%	 fill-style= "solid"
%	 p2= "(260,40)"
%	 fill-color= "#ffffff"
%	 p1= "(230,40)"
%	 stroke-width= "0.75"
%	 />
%<parallelogram p3= "(252.5,90)"
%	 fill-style= "solid"
%	 p2= "(252.5,75)"
%	 fill-color= "#999999"
%	 p1= "(257.5,75)"
%	 stroke-color= "#999999"
%	 />
%<multicurve fill-style= "none"
%	 points= "(255,90);(255,90);(255,75);(255,75)"
%	 stroke-width= "0.75"
%	 />
%<parallelogram p3= "(232.5,90)"
%	 fill-style= "solid"
%	 p2= "(232.5,75)"
%	 fill-color= "#999999"
%	 p1= "(237.5,75)"
%	 stroke-color= "#999999"
%	 />
%<multicurve fill-style= "none"
%	 points= "(235,90);(235,90);(235,75);(235,75)"
%	 stroke-width= "0.75"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(246.25,81.88)"
%	 stroke-color= "#999999"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\inbit
%</text>
%<parallelogram p3= "(260,55)"
%	 fill-style= "solid"
%	 p2= "(260,75)"
%	 fill-color= "#ffffff"
%	 p1= "(230,75)"
%	 stroke-width= "0.75"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 stroke-dasharray= "8;8"
%	 anchor-point= "(245,65)"
%	 stroke-style= "dashed"
%	 text-frame= "noframe"
%	 stroke-width= "0.75"
%	 text-hor-align= "center-h"
%	 >
%$\gee$
%</text>
%<parallelogram p3= "(277.5,77.5)"
%	 fill-style= "solid"
%	 p2= "(277.5,52.5)"
%	 fill-color= "#999999"
%	 p1= "(312.5,52.5)"
%	 stroke-color= "#999999"
%	 />
%<parallelogram p3= "(292.5,55)"
%	 fill-style= "solid"
%	 p2= "(292.5,42.5)"
%	 fill-color= "#999999"
%	 p1= "(297.5,42.5)"
%	 stroke-color= "#999999"
%	 />
%<parallelogram p3= "(277.5,42.5)"
%	 fill-style= "solid"
%	 p2= "(277.5,17.5)"
%	 fill-color= "#999999"
%	 p1= "(312.5,17.5)"
%	 stroke-color= "#999999"
%	 />
%<parallelogram p3= "(292.5,20)"
%	 fill-style= "solid"
%	 p2= "(292.5,0)"
%	 fill-color= "#999999"
%	 p1= "(297.5,0)"
%	 stroke-color= "#999999"
%	 />
%<multicurve fill-style= "none"
%	 points= "(295,20);(295,20);(295,0);(295,0)"
%	 stroke-width= "0.75"
%	 />
%<parallelogram p3= "(310,20)"
%	 fill-style= "solid"
%	 p2= "(310,40)"
%	 fill-color= "#ffffff"
%	 p1= "(280,40)"
%	 stroke-width= "0.75"
%	 />
%<parallelogram p3= "(302.5,90)"
%	 fill-style= "solid"
%	 p2= "(302.5,75)"
%	 fill-color= "#999999"
%	 p1= "(307.5,75)"
%	 stroke-color= "#999999"
%	 />
%<multicurve fill-style= "none"
%	 points= "(305,90);(305,90);(305,75);(305,75)"
%	 stroke-width= "0.75"
%	 />
%<parallelogram p3= "(282.5,90)"
%	 fill-style= "solid"
%	 p2= "(282.5,75)"
%	 fill-color= "#999999"
%	 p1= "(287.5,75)"
%	 stroke-color= "#999999"
%	 />
%<multicurve fill-style= "none"
%	 points= "(285,90);(285,90);(285,75);(285,75)"
%	 stroke-width= "0.75"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(296.25,81.88)"
%	 stroke-color= "#999999"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\inbit
%</text>
%<multicurve fill-style= "none"
%	 points= "(295,55);(295,55);(295,40);(295,40)"
%	 stroke-width= "0.75"
%	 />
%<parallelogram p3= "(310,55)"
%	 fill-style= "solid"
%	 p2= "(310,75)"
%	 fill-color= "#ffffff"
%	 p1= "(280,75)"
%	 stroke-width= "0.75"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 stroke-dasharray= "8;8"
%	 anchor-point= "(295,65)"
%	 stroke-style= "dashed"
%	 text-frame= "noframe"
%	 stroke-width= "0.75"
%	 text-hor-align= "center-h"
%	 >
%$\gee$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(245,30)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\hee$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(295,30)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\hee$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 stroke-dasharray= "8;8"
%	 anchor-point= "(105,50)"
%	 stroke-style= "dashed"
%	 text-frame= "noframe"
%	 stroke-width= "0.75"
%	 text-hor-align= "center-h"
%	 >
%$\gee$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 stroke-dasharray= "8;8"
%	 anchor-point= "(155,50)"
%	 stroke-style= "dashed"
%	 text-frame= "noframe"
%	 stroke-width= "0.75"
%	 text-hor-align= "center-h"
%	 >
%$\gee$
%</text>
%</jpic>
%%End JPIC-XML
%PSTricks content-type (pstricks.sty package needed)
%Add \usepackage{pstricks} in the preamble of your LaTeX file
%You can rescale the whole picture (to 80% for instance) by using the command \def\JPicScale{0.8}
\ifx\JPicScale\undefined\def\JPicScale{1}\fi
\psset{unit=\JPicScale mm}
\psset{linewidth=0.3,dotsep=1,hatchwidth=0.3,hatchsep=1.5,shadowsize=1,dimen=middle}
\psset{dotsize=0.7 2.5,dotscale=1 1,fillcolor=black}
\psset{arrowsize=1 2,arrowlength=1,arrowinset=0.25,tbarsize=0.7 5,bracketlength=0.15,rbracketlength=0.15}
\begin{pspicture}(0,0)(312.5,90)
\rput(22.5,50){\EQLS}
\rput(130,50){\EQLS}
\psline[linewidth=0.75](105,15)(105,0)
\rput(22.5,5){\oone}
\rput(130,5){\ttwo}
\rput(270,5){\tthree}
\newrgbcolor{userLineColour}{0.6 0.6 0.6}
\newrgbcolor{userFillColour}{0.6 0.6 0.6}
\pspolygon[linecolor=userLineColour,fillcolor=userFillColour,fillstyle=solid](10,55)(5,55)(5,90)(10,90)
\newrgbcolor{userLineColour}{0.6 0.6 0.6}
\newrgbcolor{userFillColour}{0.6 0.6 0.6}
\pspolygon[linecolor=userLineColour,fillcolor=userFillColour,fillstyle=solid](15,42.5)(0,42.5)(0,57.5)(15,57.5)
\pspolygon[linewidth=0.75,fillcolor=white,fillstyle=solid](2.5,55)(12.5,55)(12.5,45)(2.5,45)
\rput(7.5,50){$\unit$}
\newrgbcolor{userLineColour}{0.6 0.6 0.6}
\newrgbcolor{userFillColour}{0.6 0.6 0.6}
\pspolygon[linecolor=userLineColour,fillcolor=userFillColour,fillstyle=solid](10,0)(5,0)(5,42.5)(10,42.5)
\newrgbcolor{userLineColour}{0.6 0.6 0.6}
\newrgbcolor{userFillColour}{0.6 0.6 0.6}
\pspolygon[linecolor=userLineColour,fillcolor=userFillColour,fillstyle=solid](35,0)(30,0)(30,90)(35,90)
\psline[linewidth=0.75](7.5,45)(7.5,0)
\psline[linewidth=0.75](7.5,90)(7.5,55)
\psline[linewidth=0.75](32.5,90)(32.5,0)
\pspolygon[linewidth=0.75,fillcolor=white,fillstyle=solid](100,25)(110,25)(110,15)(100,15)
\rput(105,20){$\unit$}
\newrgbcolor{userLineColour}{0.6 0.6 0.6}
\newrgbcolor{userFillColour}{0.6 0.6 0.6}
\pspolygon[linecolor=userLineColour,fillcolor=userFillColour,fillstyle=solid](122.5,37.5)(87.5,37.5)(87.5,62.5)(122.5,62.5)
\newrgbcolor{userLineColour}{0.6 0.6 0.6}
\newrgbcolor{userFillColour}{0.6 0.6 0.6}
\pspolygon[linecolor=userLineColour,fillcolor=userFillColour,fillstyle=solid](107.5,25)(102.5,25)(102.5,40)(107.5,40)
\psline[linewidth=0.75](105,40)(105,25)
\newrgbcolor{userLineColour}{0.6 0.6 0.6}
\newrgbcolor{userFillColour}{0.6 0.6 0.6}
\pspolygon[linecolor=userLineColour,fillcolor=userFillColour,fillstyle=solid](117.5,60)(112.5,60)(112.5,90)(117.5,90)
\psline[linewidth=0.75](115,90)(115,60)
\newrgbcolor{userLineColour}{0.6 0.6 0.6}
\newrgbcolor{userFillColour}{0.6 0.6 0.6}
\pspolygon[linecolor=userLineColour,fillcolor=userFillColour,fillstyle=solid](97.5,60)(92.5,60)(92.5,90)(97.5,90)
\psline[linewidth=0.75](95,90)(95,60)
\pspolygon[linewidth=0.75,fillcolor=white,fillstyle=solid](90,60)(120,60)(120,40)(90,40)
\newrgbcolor{userLineColour}{0.6 0.6 0.6}
\rput(106.25,66.88){\inbit}
\psline[linewidth=0.75](155,40)(155,0)
\newrgbcolor{userLineColour}{0.6 0.6 0.6}
\newrgbcolor{userFillColour}{0.6 0.6 0.6}
\pspolygon[linecolor=userLineColour,fillcolor=userFillColour,fillstyle=solid](167.5,60)(162.5,60)(162.5,90)(167.5,90)
\psline[linewidth=0.75](165,90)(165,60)
\newrgbcolor{userLineColour}{0.6 0.6 0.6}
\newrgbcolor{userFillColour}{0.6 0.6 0.6}
\pspolygon[linecolor=userLineColour,fillcolor=userFillColour,fillstyle=solid](147.5,60)(142.5,60)(142.5,90)(147.5,90)
\psline[linewidth=0.75](145,90)(145,60)
\pspolygon[linewidth=0.75,fillcolor=white,fillstyle=solid](140,60)(170,60)(170,40)(140,40)
\newrgbcolor{userLineColour}{0.6 0.6 0.6}
\rput(156.25,66.88){\inbit}
\rput(270,50){\EQLS}
\newrgbcolor{userLineColour}{0.6 0.6 0.6}
\newrgbcolor{userFillColour}{0.6 0.6 0.6}
\pspolygon[linecolor=userLineColour,fillcolor=userFillColour,fillstyle=solid](262.5,17.5)(227.5,17.5)(227.5,77.5)(262.5,77.5)
\newrgbcolor{userLineColour}{0.6 0.6 0.6}
\newrgbcolor{userFillColour}{0.6 0.6 0.6}
\pspolygon[linecolor=userLineColour,fillcolor=userFillColour,fillstyle=solid](247.5,0)(242.5,0)(242.5,20)(247.5,20)
\psline[linewidth=0.75](245,20)(245,0)
\psline[linewidth=0.75](245,55)(245,40)
\pspolygon[linewidth=0.75,fillcolor=white,fillstyle=solid](230,40)(260,40)(260,20)(230,20)
\newrgbcolor{userLineColour}{0.6 0.6 0.6}
\newrgbcolor{userFillColour}{0.6 0.6 0.6}
\pspolygon[linecolor=userLineColour,fillcolor=userFillColour,fillstyle=solid](257.5,75)(252.5,75)(252.5,90)(257.5,90)
\psline[linewidth=0.75](255,90)(255,75)
\newrgbcolor{userLineColour}{0.6 0.6 0.6}
\newrgbcolor{userFillColour}{0.6 0.6 0.6}
\pspolygon[linecolor=userLineColour,fillcolor=userFillColour,fillstyle=solid](237.5,75)(232.5,75)(232.5,90)(237.5,90)
\psline[linewidth=0.75](235,90)(235,75)
\newrgbcolor{userLineColour}{0.6 0.6 0.6}
\rput(246.25,81.88){\inbit}
\pspolygon[linewidth=0.75,fillcolor=white,fillstyle=solid](230,75)(260,75)(260,55)(230,55)
\rput(245,65){$\gee$}
\newrgbcolor{userLineColour}{0.6 0.6 0.6}
\newrgbcolor{userFillColour}{0.6 0.6 0.6}
\pspolygon[linecolor=userLineColour,fillcolor=userFillColour,fillstyle=solid](312.5,52.5)(277.5,52.5)(277.5,77.5)(312.5,77.5)
\newrgbcolor{userLineColour}{0.6 0.6 0.6}
\newrgbcolor{userFillColour}{0.6 0.6 0.6}
\pspolygon[linecolor=userLineColour,fillcolor=userFillColour,fillstyle=solid](297.5,42.5)(292.5,42.5)(292.5,55)(297.5,55)
\newrgbcolor{userLineColour}{0.6 0.6 0.6}
\newrgbcolor{userFillColour}{0.6 0.6 0.6}
\pspolygon[linecolor=userLineColour,fillcolor=userFillColour,fillstyle=solid](312.5,17.5)(277.5,17.5)(277.5,42.5)(312.5,42.5)
\newrgbcolor{userLineColour}{0.6 0.6 0.6}
\newrgbcolor{userFillColour}{0.6 0.6 0.6}
\pspolygon[linecolor=userLineColour,fillcolor=userFillColour,fillstyle=solid](297.5,0)(292.5,0)(292.5,20)(297.5,20)
\psline[linewidth=0.75](295,20)(295,0)
\pspolygon[linewidth=0.75,fillcolor=white,fillstyle=solid](280,40)(310,40)(310,20)(280,20)
\newrgbcolor{userLineColour}{0.6 0.6 0.6}
\newrgbcolor{userFillColour}{0.6 0.6 0.6}
\pspolygon[linecolor=userLineColour,fillcolor=userFillColour,fillstyle=solid](307.5,75)(302.5,75)(302.5,90)(307.5,90)
\psline[linewidth=0.75](305,90)(305,75)
\newrgbcolor{userLineColour}{0.6 0.6 0.6}
\newrgbcolor{userFillColour}{0.6 0.6 0.6}
\pspolygon[linecolor=userLineColour,fillcolor=userFillColour,fillstyle=solid](287.5,75)(282.5,75)(282.5,90)(287.5,90)
\psline[linewidth=0.75](285,90)(285,75)
\newrgbcolor{userLineColour}{0.6 0.6 0.6}
\rput(296.25,81.88){\inbit}
\psline[linewidth=0.75](295,55)(295,40)
\pspolygon[linewidth=0.75,fillcolor=white,fillstyle=solid](280,75)(310,75)(310,55)(280,55)
\rput(295,65){$\gee$}
\rput(245,30){$\hee$}
\rput(295,30){$\hee$}
\rput(105,50){$\gee$}
\rput(155,50){$\gee$}
\end{pspicture}


==> PIC/triple-eqns.tex <==
%%Created by jPicEdt 1.4.1_03: mixed JPIC-XML/LaTeX format
%%Thu Aug 01 12:23:16 GMT-10:00 2019
%%Begin JPIC-XML
%<?xml version="1.0" standalone="yes"?>
%<jpic x-min="-1.25" x-max="298.75" y-min="0" y-max="90" auto-bounding="true">
%<multicurve fill-style= "none"
%	 points= "(147.5,60);(147.5,60);(147.5,40);(147.5,40)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(167.5,40);(167.5,40);(167.5,60);(167.5,60)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(157.5,90);(157.5,90);(157.5,60);(157.5,60)"
%	 stroke-color= "#999999"
%	 stroke-width= "3"
%	 />
%<multicurve fill-style= "none"
%	 points= "(147.5,40);(147.5,40);(167.5,40);(167.5,40)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(157.5,40);(157.5,40);(157.5,0);(157.5,0)"
%	 stroke-width= "0.75"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(157.5,50)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\hee$
%</text>
%<multicurve fill-style= "none"
%	 points= "(10,90);(10,90);(10,55);(10,55)"
%	 stroke-color= "#999999"
%	 stroke-width= "3"
%	 />
%<multicurve fill-style= "none"
%	 points= "(10,45);(10,45);(10,20);(10,20)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(5,55);(5,55);(15,55);(15,55)"
%	 stroke-width= "0.75"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 stroke-dasharray= "8;8"
%	 anchor-point= "(10,50)"
%	 stroke-style= "dashed"
%	 text-frame= "noframe"
%	 stroke-width= "0.75"
%	 text-hor-align= "center-h"
%	 >
%$\unit$
%</text>
%<multicurve fill-style= "none"
%	 points= "(5,45);(5,45);(15,45);(15,45)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(15,55);(15,55);(15,45);(15,45)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(5,55);(5,55);(5,45);(5,45)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(147.5,60);(147.5,60);(167.5,60);(167.5,60)"
%	 stroke-width= "0.75"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 stroke-dasharray= "8;8"
%	 anchor-point= "(235,30)"
%	 stroke-style= "dashed"
%	 text-frame= "noframe"
%	 stroke-width= "0.75"
%	 text-hor-align= "center-h"
%	 >
%$\eehee$
%</text>
%<multicurve fill-style= "none"
%	 points= "(225,40);(225,40);(225,20);(225,20)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(245,20);(245,20);(245,40);(245,40)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(235,55);(235,55);(235,40);(235,40)"
%	 stroke-color= "#999999"
%	 stroke-width= "3"
%	 />
%<multicurve fill-style= "none"
%	 points= "(225,20);(225,20);(245,20);(245,20)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(235,20);(235,20);(235,0);(235,0)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(225,40);(225,40);(245,40);(245,40)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(220,81.25);(220,81.25);(220,13.75);(220,13.75)"
%	 stroke-color= "#999999"
%	 stroke-width= "3"
%	 />
%<multicurve fill-style= "none"
%	 points= "(250,81.25);(250,81.25);(250,13.75);(250,13.75)"
%	 stroke-color= "#999999"
%	 stroke-width= "3"
%	 />
%<multicurve fill-style= "none"
%	 points= "(251.25,80);(251.25,80);(218.75,80);(218.75,80)"
%	 stroke-color= "#999999"
%	 stroke-width= "3"
%	 />
%<multicurve fill-style= "none"
%	 points= "(251.25,15);(251.25,15);(218.75,15);(218.75,15)"
%	 stroke-color= "#999999"
%	 stroke-width= "3"
%	 />
%<multicurve fill-style= "none"
%	 points= "(235,0);(235,0);(235,15);(235,15)"
%	 stroke-color= "#999999"
%	 stroke-width= "3"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 stroke-dasharray= "8;8"
%	 anchor-point= "(30,50)"
%	 stroke-style= "dashed"
%	 text-frame= "noframe"
%	 stroke-width= "0.75"
%	 text-hor-align= "center-h"
%	 >
%\EQLS
%</text>
%<multicurve fill-style= "none"
%	 points= "(40,90);(40,90);(40,0);(40,0)"
%	 stroke-color= "#999999"
%	 stroke-width= "3"
%	 />
%<multicurve fill-style= "none"
%	 points= "(0,61.25);(0,61.25);(0,38.75);(0,38.75)"
%	 stroke-color= "#999999"
%	 stroke-width= "3"
%	 />
%<multicurve fill-style= "none"
%	 points= "(20,61.25);(20,61.25);(20,38.75);(20,38.75)"
%	 stroke-color= "#999999"
%	 stroke-width= "3"
%	 />
%<multicurve fill-style= "none"
%	 points= "(21.25,60);(21.25,60);(-1.25,60);(-1.25,60)"
%	 stroke-color= "#999999"
%	 stroke-width= "3"
%	 />
%<multicurve fill-style= "none"
%	 points= "(21.25,40);(21.25,40);(-1.25,40);(-1.25,40)"
%	 stroke-color= "#999999"
%	 stroke-width= "3"
%	 />
%<multicurve fill-style= "none"
%	 points= "(10,0);(10,0);(10,40);(10,40)"
%	 stroke-color= "#999999"
%	 stroke-width= "3"
%	 />
%<multicurve fill-style= "none"
%	 points= "(225,75);(225,75);(225,55);(225,55)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(245,55);(245,55);(245,75);(245,75)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(225,55);(225,55);(245,55);(245,55)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(225,75);(225,75);(245,75);(245,75)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(235,90);(235,90);(235,75);(235,75)"
%	 stroke-color= "#999999"
%	 stroke-width= "3"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 stroke-dasharray= "8;8"
%	 anchor-point= "(235,65)"
%	 stroke-style= "dashed"
%	 text-frame= "noframe"
%	 stroke-width= "0.75"
%	 text-hor-align= "center-h"
%	 >
%$\gee$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 stroke-dasharray= "8;8"
%	 anchor-point= "(260,50)"
%	 stroke-style= "dashed"
%	 text-frame= "noframe"
%	 stroke-width= "0.75"
%	 text-hor-align= "center-h"
%	 >
%\EQLS
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 stroke-dasharray= "8;8"
%	 anchor-point= "(282.5,30)"
%	 stroke-style= "dashed"
%	 text-frame= "noframe"
%	 stroke-width= "0.75"
%	 text-hor-align= "center-h"
%	 >
%$\eehee$
%</text>
%<multicurve fill-style= "none"
%	 points= "(272.5,40);(272.5,40);(272.5,20);(272.5,20)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(292.5,20);(292.5,20);(292.5,40);(292.5,40)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(282.5,55);(282.5,55);(282.5,40);(282.5,40)"
%	 stroke-color= "#999999"
%	 stroke-width= "3"
%	 />
%<multicurve fill-style= "none"
%	 points= "(272.5,20);(272.5,20);(292.5,20);(292.5,20)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(282.5,20);(282.5,20);(282.5,0);(282.5,0)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(272.5,40);(272.5,40);(292.5,40);(292.5,40)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(267.5,46.25);(267.5,46.25);(267.5,13.75);(267.5,13.75)"
%	 stroke-color= "#999999"
%	 stroke-width= "3"
%	 />
%<multicurve fill-style= "none"
%	 points= "(297.5,46.25);(297.5,46.25);(297.5,13.75);(297.5,13.75)"
%	 stroke-color= "#999999"
%	 stroke-width= "3"
%	 />
%<multicurve fill-style= "none"
%	 points= "(298.75,45);(298.75,45);(266.25,45);(266.25,45)"
%	 stroke-color= "#999999"
%	 stroke-width= "3"
%	 />
%<multicurve fill-style= "none"
%	 points= "(298.75,15);(298.75,15);(266.25,15);(266.25,15)"
%	 stroke-color= "#999999"
%	 stroke-width= "3"
%	 />
%<multicurve fill-style= "none"
%	 points= "(282.5,0);(282.5,0);(282.5,15);(282.5,15)"
%	 stroke-color= "#999999"
%	 stroke-width= "3"
%	 />
%<multicurve fill-style= "none"
%	 points= "(272.5,75);(272.5,75);(272.5,55);(272.5,55)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(292.5,55);(292.5,55);(292.5,75);(292.5,75)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(272.5,55);(272.5,55);(292.5,55);(292.5,55)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(272.5,75);(272.5,75);(292.5,75);(292.5,75)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(282.5,90);(282.5,90);(282.5,75);(282.5,75)"
%	 stroke-color= "#999999"
%	 stroke-width= "3"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 stroke-dasharray= "8;8"
%	 anchor-point= "(282.5,65)"
%	 stroke-style= "dashed"
%	 text-frame= "noframe"
%	 stroke-width= "0.75"
%	 text-hor-align= "center-h"
%	 >
%$\gee$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 stroke-dasharray= "8;8"
%	 anchor-point= "(140,50)"
%	 stroke-style= "dashed"
%	 text-frame= "noframe"
%	 stroke-width= "0.75"
%	 text-hor-align= "center-h"
%	 >
%\EQLS
%</text>
%<multicurve fill-style= "none"
%	 points= "(105,60);(105,60);(105,40);(105,40)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(125,40);(125,40);(125,60);(125,60)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(115,90);(115,90);(115,60);(115,60)"
%	 stroke-color= "#999999"
%	 stroke-width= "3"
%	 />
%<multicurve fill-style= "none"
%	 points= "(105,40);(105,40);(125,40);(125,40)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(115,40);(115,40);(115,30);(115,30)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(105,60);(105,60);(125,60);(125,60)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(100,66.25);(100,66.25);(100,33.75);(100,33.75)"
%	 stroke-color= "#999999"
%	 stroke-width= "3"
%	 />
%<multicurve fill-style= "none"
%	 points= "(130,66.25);(130,66.25);(130,33.75);(130,33.75)"
%	 stroke-color= "#999999"
%	 stroke-width= "3"
%	 />
%<multicurve fill-style= "none"
%	 points= "(131.25,65);(131.25,65);(98.75,65);(98.75,65)"
%	 stroke-color= "#999999"
%	 stroke-width= "3"
%	 />
%<multicurve fill-style= "none"
%	 points= "(131.25,35);(131.25,35);(98.75,35);(98.75,35)"
%	 stroke-color= "#999999"
%	 stroke-width= "3"
%	 />
%<multicurve fill-style= "none"
%	 points= "(115,22.5);(115,22.5);(115,35);(115,35)"
%	 stroke-color= "#999999"
%	 stroke-width= "3"
%	 />
%<multicurve fill-style= "none"
%	 points= "(115,12.5);(115,12.5);(115,0);(115,0)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(110,22.5);(110,22.5);(120,22.5);(120,22.5)"
%	 stroke-width= "0.75"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 stroke-dasharray= "8;8"
%	 anchor-point= "(115,17.5)"
%	 stroke-style= "dashed"
%	 text-frame= "noframe"
%	 stroke-width= "0.75"
%	 text-hor-align= "center-h"
%	 >
%$\unit$
%</text>
%<multicurve fill-style= "none"
%	 points= "(110,12.5);(110,12.5);(120,12.5);(120,12.5)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(120,22.5);(120,22.5);(120,12.5);(120,12.5)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(110,22.5);(110,22.5);(110,12.5);(110,12.5)"
%	 stroke-width= "0.75"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 stroke-dasharray= "8;8"
%	 anchor-point= "(115,50)"
%	 stroke-style= "dashed"
%	 text-frame= "noframe"
%	 stroke-width= "0.75"
%	 text-hor-align= "center-h"
%	 >
%$\eehee$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 stroke-dasharray= "8;8"
%	 anchor-point= "(30,5)"
%	 stroke-style= "dashed"
%	 text-frame= "noframe"
%	 stroke-width= "0.75"
%	 text-hor-align= "center-h"
%	 >
%\oone
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 stroke-dasharray= "8;8"
%	 anchor-point= "(140,5)"
%	 stroke-style= "dashed"
%	 text-frame= "noframe"
%	 stroke-width= "0.75"
%	 text-hor-align= "center-h"
%	 >
%\ttwo
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 stroke-dasharray= "8;8"
%	 anchor-point= "(260,5)"
%	 stroke-style= "dashed"
%	 text-frame= "noframe"
%	 stroke-width= "0.75"
%	 text-hor-align= "center-h"
%	 >
%\tthree
%</text>
%</jpic>
%%End JPIC-XML
%PSTricks content-type (pstricks.sty package needed)
%Add \usepackage{pstricks} in the preamble of your LaTeX file
%You can rescale the whole picture (to 80% for instance) by using the command \def\JPicScale{0.8}
\ifx\JPicScale\undefined\def\JPicScale{1}\fi
\psset{unit=\JPicScale mm}
\psset{linewidth=0.3,dotsep=1,hatchwidth=0.3,hatchsep=1.5,shadowsize=1,dimen=middle}
\psset{dotsize=0.7 2.5,dotscale=1 1,fillcolor=black}
\psset{arrowsize=1 2,arrowlength=1,arrowinset=0.25,tbarsize=0.7 5,bracketlength=0.15,rbracketlength=0.15}
\begin{pspicture}(0,0)(298.75,90)
\psline[linewidth=0.75](147.5,60)(147.5,40)
\psline[linewidth=0.75](167.5,40)(167.5,60)
\newrgbcolor{userLineColour}{0.6 0.6 0.6}
\psline[linewidth=3,linecolor=userLineColour](157.5,90)(157.5,60)
\psline[linewidth=0.75](147.5,40)(167.5,40)
\psline[linewidth=0.75](157.5,40)(157.5,0)
\rput(157.5,50){$\hee$}
\newrgbcolor{userLineColour}{0.6 0.6 0.6}
\psline[linewidth=3,linecolor=userLineColour](10,90)(10,55)
\psline[linewidth=0.75](10,45)(10,20)
\psline[linewidth=0.75](5,55)(15,55)
\rput(10,50){$\unit$}
\psline[linewidth=0.75](5,45)(15,45)
\psline[linewidth=0.75](15,55)(15,45)
\psline[linewidth=0.75](5,55)(5,45)
\psline[linewidth=0.75](147.5,60)(167.5,60)
\rput(235,30){$\eehee$}
\psline[linewidth=0.75](225,40)(225,20)
\psline[linewidth=0.75](245,20)(245,40)
\newrgbcolor{userLineColour}{0.6 0.6 0.6}
\psline[linewidth=3,linecolor=userLineColour](235,55)(235,40)
\psline[linewidth=0.75](225,20)(245,20)
\psline[linewidth=0.75](235,20)(235,0)
\psline[linewidth=0.75](225,40)(245,40)
\newrgbcolor{userLineColour}{0.6 0.6 0.6}
\psline[linewidth=3,linecolor=userLineColour](220,81.25)(220,13.75)
\newrgbcolor{userLineColour}{0.6 0.6 0.6}
\psline[linewidth=3,linecolor=userLineColour](250,81.25)(250,13.75)
\newrgbcolor{userLineColour}{0.6 0.6 0.6}
\psline[linewidth=3,linecolor=userLineColour](251.25,80)(218.75,80)
\newrgbcolor{userLineColour}{0.6 0.6 0.6}
\psline[linewidth=3,linecolor=userLineColour](251.25,15)(218.75,15)
\newrgbcolor{userLineColour}{0.6 0.6 0.6}
\psline[linewidth=3,linecolor=userLineColour](235,0)(235,15)
\rput(30,50){\EQLS}
\newrgbcolor{userLineColour}{0.6 0.6 0.6}
\psline[linewidth=3,linecolor=userLineColour](40,90)(40,0)
\newrgbcolor{userLineColour}{0.6 0.6 0.6}
\psline[linewidth=3,linecolor=userLineColour](0,61.25)(0,38.75)
\newrgbcolor{userLineColour}{0.6 0.6 0.6}
\psline[linewidth=3,linecolor=userLineColour](20,61.25)(20,38.75)
\newrgbcolor{userLineColour}{0.6 0.6 0.6}
\psline[linewidth=3,linecolor=userLineColour](21.25,60)(-1.25,60)
\newrgbcolor{userLineColour}{0.6 0.6 0.6}
\psline[linewidth=3,linecolor=userLineColour](21.25,40)(-1.25,40)
\newrgbcolor{userLineColour}{0.6 0.6 0.6}
\psline[linewidth=3,linecolor=userLineColour](10,0)(10,40)
\psline[linewidth=0.75](225,75)(225,55)
\psline[linewidth=0.75](245,55)(245,75)
\psline[linewidth=0.75](225,55)(245,55)
\psline[linewidth=0.75](225,75)(245,75)
\newrgbcolor{userLineColour}{0.6 0.6 0.6}
\psline[linewidth=3,linecolor=userLineColour](235,90)(235,75)
\rput(235,65){$\gee$}
\rput(260,50){\EQLS}
\rput(282.5,30){$\eehee$}
\psline[linewidth=0.75](272.5,40)(272.5,20)
\psline[linewidth=0.75](292.5,20)(292.5,40)
\newrgbcolor{userLineColour}{0.6 0.6 0.6}
\psline[linewidth=3,linecolor=userLineColour](282.5,55)(282.5,40)
\psline[linewidth=0.75](272.5,20)(292.5,20)
\psline[linewidth=0.75](282.5,20)(282.5,0)
\psline[linewidth=0.75](272.5,40)(292.5,40)
\newrgbcolor{userLineColour}{0.6 0.6 0.6}
\psline[linewidth=3,linecolor=userLineColour](267.5,46.25)(267.5,13.75)
\newrgbcolor{userLineColour}{0.6 0.6 0.6}
\psline[linewidth=3,linecolor=userLineColour](297.5,46.25)(297.5,13.75)
\newrgbcolor{userLineColour}{0.6 0.6 0.6}
\psline[linewidth=3,linecolor=userLineColour](298.75,45)(266.25,45)
\newrgbcolor{userLineColour}{0.6 0.6 0.6}
\psline[linewidth=3,linecolor=userLineColour](298.75,15)(266.25,15)
\newrgbcolor{userLineColour}{0.6 0.6 0.6}
\psline[linewidth=3,linecolor=userLineColour](282.5,0)(282.5,15)
\psline[linewidth=0.75](272.5,75)(272.5,55)
\psline[linewidth=0.75](292.5,55)(292.5,75)
\psline[linewidth=0.75](272.5,55)(292.5,55)
\psline[linewidth=0.75](272.5,75)(292.5,75)
\newrgbcolor{userLineColour}{0.6 0.6 0.6}
\psline[linewidth=3,linecolor=userLineColour](282.5,90)(282.5,75)
\rput(282.5,65){$\gee$}
\rput(140,50){\EQLS}
\psline[linewidth=0.75](105,60)(105,40)
\psline[linewidth=0.75](125,40)(125,60)
\newrgbcolor{userLineColour}{0.6 0.6 0.6}
\psline[linewidth=3,linecolor=userLineColour](115,90)(115,60)
\psline[linewidth=0.75](105,40)(125,40)
\psline[linewidth=0.75](115,40)(115,30)
\psline[linewidth=0.75](105,60)(125,60)
\newrgbcolor{userLineColour}{0.6 0.6 0.6}
\psline[linewidth=3,linecolor=userLineColour](100,66.25)(100,33.75)
\newrgbcolor{userLineColour}{0.6 0.6 0.6}
\psline[linewidth=3,linecolor=userLineColour](130,66.25)(130,33.75)
\newrgbcolor{userLineColour}{0.6 0.6 0.6}
\psline[linewidth=3,linecolor=userLineColour](131.25,65)(98.75,65)
\newrgbcolor{userLineColour}{0.6 0.6 0.6}
\psline[linewidth=3,linecolor=userLineColour](131.25,35)(98.75,35)
\newrgbcolor{userLineColour}{0.6 0.6 0.6}
\psline[linewidth=3,linecolor=userLineColour](115,22.5)(115,35)
\psline[linewidth=0.75](115,12.5)(115,0)
\psline[linewidth=0.75](110,22.5)(120,22.5)
\rput(115,17.5){$\unit$}
\psline[linewidth=0.75](110,12.5)(120,12.5)
\psline[linewidth=0.75](120,22.5)(120,12.5)
\psline[linewidth=0.75](110,22.5)(110,12.5)
\rput(115,50){$\eehee$}
\rput(30,5){\oone}
\rput(140,5){\ttwo}
\rput(260,5){\tthree}
\end{pspicture}


==> PIC/triple-notations-1.tex <==
%%Created by jPicEdt 1.4.1_03: mixed JPIC-XML/LaTeX format
%%Fri Nov 01 13:40:47 GMT-10:00 2019
%%Begin JPIC-XML
%<?xml version="1.0" standalone="yes"?>
%<jpic x-min="0" x-max="122.5" y-min="5" y-max="80" auto-bounding="true">
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 stroke-dasharray= "8;8"
%	 anchor-point= "(66.25,20)"
%	 stroke-style= "dashed"
%	 text-frame= "noframe"
%	 stroke-width= "0.75"
%	 text-hor-align= "right"
%	 >
%$\eeinptt$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(73.75,80)"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\otheroutpt$
%</text>
%<parallelogram p3= "(67.5,80)"
%	 fill-style= "solid"
%	 p2= "(67.5,60)"
%	 fill-color= "#999999"
%	 p1= "(72.5,60)"
%	 stroke-color= "#999999"
%	 />
%<parallelogram p3= "(67.5,40)"
%	 fill-style= "solid"
%	 p2= "(67.5,20)"
%	 fill-color= "#999999"
%	 p1= "(72.5,20)"
%	 stroke-color= "#999999"
%	 />
%<multicurve fill-style= "none"
%	 points= "(70,80);(70,80);(70,60);(70,60)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(70,40);(70,40);(70,20);(70,20)"
%	 stroke-width= "0.75"
%	 />
%<parallelogram p3= "(80,40)"
%	 fill-style= "solid"
%	 p2= "(80,60)"
%	 fill-color= "#ffffff"
%	 p1= "(60,60)"
%	 stroke-width= "0.75"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "solid"
%	 fill-color= "#ffffff"
%	 stroke-dasharray= "8;8"
%	 anchor-point= "(70,50)"
%	 stroke-style= "dashed"
%	 text-frame= "noframe"
%	 stroke-width= "0.75"
%	 text-hor-align= "center-h"
%	 >
%$\eehee$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 stroke-dasharray= "8;8"
%	 anchor-point= "(106.25,20)"
%	 stroke-style= "dashed"
%	 text-frame= "noframe"
%	 stroke-width= "0.75"
%	 text-hor-align= "right"
%	 >
%$\eeinptt$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(113.75,80)"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\otheroutpt$
%</text>
%<parallelogram p3= "(97.5,70)"
%	 fill-style= "solid"
%	 p2= "(97.5,27.5)"
%	 fill-color= "#999999"
%	 p1= "(122.5,27.5)"
%	 stroke-color= "#999999"
%	 />
%<parallelogram p3= "(107.5,80)"
%	 fill-style= "solid"
%	 p2= "(107.5,60)"
%	 fill-color= "#999999"
%	 p1= "(112.5,60)"
%	 stroke-color= "#999999"
%	 />
%<parallelogram p3= "(107.5,40)"
%	 fill-style= "solid"
%	 p2= "(107.5,20)"
%	 fill-color= "#999999"
%	 p1= "(112.5,20)"
%	 stroke-color= "#999999"
%	 />
%<multicurve fill-style= "none"
%	 points= "(110,80);(110,80);(110,67.5);(110,67.5)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(110,40);(110,40);(110,20);(110,20)"
%	 stroke-width= "0.75"
%	 />
%<parallelogram p3= "(115,57.5)"
%	 fill-style= "solid"
%	 p2= "(115,67.5)"
%	 fill-color= "#ffffff"
%	 p1= "(105,67.5)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(0,60);(0,60);(0,40);(0,40)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(20,40);(20,40);(20,60);(20,60)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(0,40);(0,40);(20,40);(20,40)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(10,40);(10,40);(10,20);(10,20)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(10,80);(10,80);(10,60);(10,60)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(0,60);(0,60);(20,60);(20,60)"
%	 stroke-width= "0.75"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(10,5)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\strict
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(90,5)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\homomorphism
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(10,50)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\see$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(40,52.5)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\goesto
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(90,50)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\EQLS
%</text>
%<parallelogram p3= "(120,30)"
%	 fill-style= "solid"
%	 p2= "(120,50)"
%	 fill-color= "#ffffff"
%	 p1= "(100,50)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(110,57.5);(110,57.5);(110,50);(110,50)"
%	 stroke-width= "0.75"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(110,40)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\see$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(110,62.5)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\hee$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(13.75,80)"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%\outpt
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(7.5,20)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%\inputt
%</text>
%</jpic>
%%End JPIC-XML
%PSTricks content-type (pstricks.sty package needed)
%Add \usepackage{pstricks} in the preamble of your LaTeX file
%You can rescale the whole picture (to 80% for instance) by using the command \def\JPicScale{0.8}
\ifx\JPicScale\undefined\def\JPicScale{1}\fi
\psset{unit=\JPicScale mm}
\psset{linewidth=0.3,dotsep=1,hatchwidth=0.3,hatchsep=1.5,shadowsize=1,dimen=middle}
\psset{dotsize=0.7 2.5,dotscale=1 1,fillcolor=black}
\psset{arrowsize=1 2,arrowlength=1,arrowinset=0.25,tbarsize=0.7 5,bracketlength=0.15,rbracketlength=0.15}
\begin{pspicture}(0,0)(122.5,80)
\rput[r](66.25,20){$\eeinptt$}
\rput[l](73.75,80){$\otheroutpt$}
\newrgbcolor{userLineColour}{0.6 0.6 0.6}
\newrgbcolor{userFillColour}{0.6 0.6 0.6}
\pspolygon[linecolor=userLineColour,fillcolor=userFillColour,fillstyle=solid](72.5,60)(67.5,60)(67.5,80)(72.5,80)
\newrgbcolor{userLineColour}{0.6 0.6 0.6}
\newrgbcolor{userFillColour}{0.6 0.6 0.6}
\pspolygon[linecolor=userLineColour,fillcolor=userFillColour,fillstyle=solid](72.5,20)(67.5,20)(67.5,40)(72.5,40)
\psline[linewidth=0.75](70,80)(70,60)
\psline[linewidth=0.75](70,40)(70,20)
\pspolygon[linewidth=0.75,fillcolor=white,fillstyle=solid](60,60)(80,60)(80,40)(60,40)
\rput(70,50){$\eehee$}
\rput[r](106.25,20){$\eeinptt$}
\rput[l](113.75,80){$\otheroutpt$}
\newrgbcolor{userLineColour}{0.6 0.6 0.6}
\newrgbcolor{userFillColour}{0.6 0.6 0.6}
\pspolygon[linecolor=userLineColour,fillcolor=userFillColour,fillstyle=solid](122.5,27.5)(97.5,27.5)(97.5,70)(122.5,70)
\newrgbcolor{userLineColour}{0.6 0.6 0.6}
\newrgbcolor{userFillColour}{0.6 0.6 0.6}
\pspolygon[linecolor=userLineColour,fillcolor=userFillColour,fillstyle=solid](112.5,60)(107.5,60)(107.5,80)(112.5,80)
\newrgbcolor{userLineColour}{0.6 0.6 0.6}
\newrgbcolor{userFillColour}{0.6 0.6 0.6}
\pspolygon[linecolor=userLineColour,fillcolor=userFillColour,fillstyle=solid](112.5,20)(107.5,20)(107.5,40)(112.5,40)
\psline[linewidth=0.75](110,80)(110,67.5)
\psline[linewidth=0.75](110,40)(110,20)
\pspolygon[linewidth=0.75,fillcolor=white,fillstyle=solid](105,67.5)(115,67.5)(115,57.5)(105,57.5)
\psline[linewidth=0.75](0,60)(0,40)
\psline[linewidth=0.75](20,40)(20,60)
\psline[linewidth=0.75](0,40)(20,40)
\psline[linewidth=0.75](10,40)(10,20)
\psline[linewidth=0.75](10,80)(10,60)
\psline[linewidth=0.75](0,60)(20,60)
\rput(10,5){\strict}
\rput(90,5){\homomorphism}
\rput(10,50){$\see$}
\rput(40,52.5){\goesto}
\rput(90,50){\EQLS}
\pspolygon[linewidth=0.75,fillcolor=white,fillstyle=solid](100,50)(120,50)(120,30)(100,30)
\psline[linewidth=0.75](110,57.5)(110,50)
\rput(110,40){$\see$}
\rput(110,62.5){$\hee$}
\rput[l](13.75,80){\outpt}
\rput[r](7.5,20){\inputt}
\end{pspicture}


==> PIC/triple-notations-2.tex <==
%%Created by jPicEdt 1.4.1_03: mixed JPIC-XML/LaTeX format
%%Fri Nov 01 13:40:26 GMT-10:00 2019
%%Begin JPIC-XML
%<?xml version="1.0" standalone="yes"?>
%<jpic x-min="0" x-max="122.5" y-min="5" y-max="80" auto-bounding="true">
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 stroke-dasharray= "8;8"
%	 anchor-point= "(66.25,20)"
%	 stroke-style= "dashed"
%	 text-frame= "noframe"
%	 stroke-width= "0.75"
%	 text-hor-align= "right"
%	 >
%$\eeinptt$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(73.75,80)"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\otheroutpt$
%</text>
%<parallelogram p3= "(67.5,80)"
%	 fill-style= "solid"
%	 p2= "(67.5,60)"
%	 fill-color= "#999999"
%	 p1= "(72.5,60)"
%	 stroke-color= "#999999"
%	 />
%<parallelogram p3= "(67.5,40)"
%	 fill-style= "solid"
%	 p2= "(67.5,20)"
%	 fill-color= "#999999"
%	 p1= "(72.5,20)"
%	 stroke-color= "#999999"
%	 />
%<multicurve fill-style= "none"
%	 points= "(70,80);(70,80);(70,60);(70,60)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(70,40);(70,40);(70,20);(70,20)"
%	 stroke-width= "0.75"
%	 />
%<parallelogram p3= "(80,40)"
%	 fill-style= "solid"
%	 p2= "(80,60)"
%	 fill-color= "#ffffff"
%	 p1= "(60,60)"
%	 stroke-width= "0.75"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "solid"
%	 fill-color= "#ffffff"
%	 stroke-dasharray= "8;8"
%	 anchor-point= "(70,50)"
%	 stroke-style= "dashed"
%	 text-frame= "noframe"
%	 stroke-width= "0.75"
%	 text-hor-align= "center-h"
%	 >
%$\eehee$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 stroke-dasharray= "8;8"
%	 anchor-point= "(106.25,20)"
%	 stroke-style= "dashed"
%	 text-frame= "noframe"
%	 stroke-width= "0.75"
%	 text-hor-align= "right"
%	 >
%$\eeinptt$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(113.75,80)"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\otheroutpt$
%</text>
%<parallelogram p3= "(97.5,62.5)"
%	 fill-style= "solid"
%	 p2= "(97.5,37.5)"
%	 fill-color= "#999999"
%	 p1= "(122.5,37.5)"
%	 stroke-color= "#999999"
%	 />
%<parallelogram p3= "(107.5,80)"
%	 fill-style= "solid"
%	 p2= "(107.5,60)"
%	 fill-color= "#999999"
%	 p1= "(112.5,60)"
%	 stroke-color= "#999999"
%	 />
%<parallelogram p3= "(107.5,40)"
%	 fill-style= "solid"
%	 p2= "(107.5,20)"
%	 fill-color= "#999999"
%	 p1= "(112.5,20)"
%	 stroke-color= "#999999"
%	 />
%<multicurve fill-style= "none"
%	 points= "(110,40);(110,40);(110,20);(110,20)"
%	 stroke-width= "0.75"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(10,5)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\strict
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(90,5)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\homomorphism
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(40,52.5)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\goesto
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(90,50)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\EQLS
%</text>
%<parallelogram p3= "(120,40)"
%	 fill-style= "solid"
%	 p2= "(120,60)"
%	 fill-color= "#ffffff"
%	 p1= "(100,60)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(110,80);(110,80);(110,60);(110,60)"
%	 stroke-width= "0.75"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(110,50)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\see$
%</text>
%<parallelogram p3= "(7.5,80)"
%	 fill-style= "solid"
%	 p2= "(7.5,60)"
%	 fill-color= "#999999"
%	 p1= "(12.5,60)"
%	 stroke-color= "#999999"
%	 />
%<multicurve fill-style= "none"
%	 points= "(0,60);(0,60);(0,40);(0,40)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(20,40);(20,40);(20,60);(20,60)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(0,40);(0,40);(20,40);(20,40)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(10,40);(10,40);(10,20);(10,20)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(10,80);(10,80);(10,60);(10,60)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(0,60);(0,60);(20,60);(20,60)"
%	 stroke-width= "0.75"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(10,50)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\see$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(13.75,80)"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%\outpt
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(7.5,20)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%\inputt
%</text>
%</jpic>
%%End JPIC-XML
%PSTricks content-type (pstricks.sty package needed)
%Add \usepackage{pstricks} in the preamble of your LaTeX file
%You can rescale the whole picture (to 80% for instance) by using the command \def\JPicScale{0.8}
\ifx\JPicScale\undefined\def\JPicScale{1}\fi
\psset{unit=\JPicScale mm}
\psset{linewidth=0.3,dotsep=1,hatchwidth=0.3,hatchsep=1.5,shadowsize=1,dimen=middle}
\psset{dotsize=0.7 2.5,dotscale=1 1,fillcolor=black}
\psset{arrowsize=1 2,arrowlength=1,arrowinset=0.25,tbarsize=0.7 5,bracketlength=0.15,rbracketlength=0.15}
\begin{pspicture}(0,0)(122.5,80)
\rput[r](66.25,20){$\eeinptt$}
\rput[l](73.75,80){$\otheroutpt$}
\newrgbcolor{userLineColour}{0.6 0.6 0.6}
\newrgbcolor{userFillColour}{0.6 0.6 0.6}
\pspolygon[linecolor=userLineColour,fillcolor=userFillColour,fillstyle=solid](72.5,60)(67.5,60)(67.5,80)(72.5,80)
\newrgbcolor{userLineColour}{0.6 0.6 0.6}
\newrgbcolor{userFillColour}{0.6 0.6 0.6}
\pspolygon[linecolor=userLineColour,fillcolor=userFillColour,fillstyle=solid](72.5,20)(67.5,20)(67.5,40)(72.5,40)
\psline[linewidth=0.75](70,80)(70,60)
\psline[linewidth=0.75](70,40)(70,20)
\pspolygon[linewidth=0.75,fillcolor=white,fillstyle=solid](60,60)(80,60)(80,40)(60,40)
\rput(70,50){$\eehee$}
\rput[r](106.25,20){$\eeinptt$}
\rput[l](113.75,80){$\otheroutpt$}
\newrgbcolor{userLineColour}{0.6 0.6 0.6}
\newrgbcolor{userFillColour}{0.6 0.6 0.6}
\pspolygon[linecolor=userLineColour,fillcolor=userFillColour,fillstyle=solid](122.5,37.5)(97.5,37.5)(97.5,62.5)(122.5,62.5)
\newrgbcolor{userLineColour}{0.6 0.6 0.6}
\newrgbcolor{userFillColour}{0.6 0.6 0.6}
\pspolygon[linecolor=userLineColour,fillcolor=userFillColour,fillstyle=solid](112.5,60)(107.5,60)(107.5,80)(112.5,80)
\newrgbcolor{userLineColour}{0.6 0.6 0.6}
\newrgbcolor{userFillColour}{0.6 0.6 0.6}
\pspolygon[linecolor=userLineColour,fillcolor=userFillColour,fillstyle=solid](112.5,20)(107.5,20)(107.5,40)(112.5,40)
\psline[linewidth=0.75](110,40)(110,20)
\rput(10,5){\strict}
\rput(90,5){\homomorphism}
\rput(40,52.5){\goesto}
\rput(90,50){\EQLS}
\pspolygon[linewidth=0.75,fillcolor=white,fillstyle=solid](100,60)(120,60)(120,40)(100,40)
\psline[linewidth=0.75](110,80)(110,60)
\rput(110,50){$\see$}
\newrgbcolor{userLineColour}{0.6 0.6 0.6}
\newrgbcolor{userFillColour}{0.6 0.6 0.6}
\pspolygon[linecolor=userLineColour,fillcolor=userFillColour,fillstyle=solid](12.5,60)(7.5,60)(7.5,80)(12.5,80)
\psline[linewidth=0.75](0,60)(0,40)
\psline[linewidth=0.75](20,40)(20,60)
\psline[linewidth=0.75](0,40)(20,40)
\psline[linewidth=0.75](10,40)(10,20)
\psline[linewidth=0.75](10,80)(10,60)
\psline[linewidth=0.75](0,60)(20,60)
\rput(10,50){$\see$}
\rput[l](13.75,80){\outpt}
\rput[r](7.5,20){\inputt}
\end{pspicture}


==> PIC/triple-notations-3.tex <==
%%Created by jPicEdt 1.4.1_03: mixed JPIC-XML/LaTeX format
%%Sat Dec 28 15:14:00 GMT-10:00 2019
%%Begin JPIC-XML
%<?xml version="1.0" standalone="yes"?>
%<jpic x-min="0" x-max="122.5" y-min="5" y-max="80" auto-bounding="true">
%<text fill-style= "none"
%	 stroke-width= "0.75"
%	 text-vert-align= "center-v"
%	 stroke-dasharray= "8;8"
%	 anchor-point= "(66.25,20)"
%	 text-frame= "noframe"
%	 stroke-style= "dashed"
%	 text-hor-align= "right"
%	 >
%$\eeinptt$
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(73.75,80)"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\otheroutpt$
%</text>
%<parallelogram fill-color= "#999999"
%	 fill-style= "solid"
%	 p3= "(57.5,62.5)"
%	 p2= "(57.5,37.5)"
%	 p1= "(82.5,37.5)"
%	 stroke-color= "#999999"
%	 />
%<parallelogram fill-color= "#999999"
%	 fill-style= "solid"
%	 p3= "(67.5,80)"
%	 p2= "(67.5,60)"
%	 p1= "(72.5,60)"
%	 stroke-color= "#999999"
%	 />
%<parallelogram fill-color= "#999999"
%	 fill-style= "solid"
%	 p3= "(67.5,40)"
%	 p2= "(67.5,20)"
%	 p1= "(72.5,20)"
%	 stroke-color= "#999999"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(70,40);(70,40);(70,20);(70,20)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(0,60);(0,60);(0,40);(0,40)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(20,40);(20,40);(20,60);(20,60)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(0,40);(0,40);(20,40);(20,40)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(10,40);(10,40);(10,20);(10,20)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(10,80);(10,80);(10,60);(10,60)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(0,60);(0,60);(20,60);(20,60)"
%	 />
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(10,5)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\strict
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(90,5)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\homomorphism
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(10,50)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\see$
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(40,52.5)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\goesto
%</text>
%<parallelogram fill-style= "none"
%	 stroke-width= "0.75"
%	 p3= "(80,40)"
%	 p2= "(80,60)"
%	 p1= "(60,60)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(70,80);(70,80);(70,60);(70,60)"
%	 />
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(13.75,80)"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%\outpt
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(7.5,20)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%\inputt
%</text>
%<text fill-color= "#ffffff"
%	 fill-style= "solid"
%	 stroke-width= "0.75"
%	 text-vert-align= "center-v"
%	 stroke-dasharray= "8;8"
%	 anchor-point= "(70,50)"
%	 text-frame= "noframe"
%	 stroke-style= "dashed"
%	 text-hor-align= "center-h"
%	 >
%$\eehee$
%</text>
%<text fill-style= "none"
%	 stroke-width= "0.75"
%	 text-vert-align= "center-v"
%	 stroke-dasharray= "8;8"
%	 anchor-point= "(106.25,20)"
%	 text-frame= "noframe"
%	 stroke-style= "dashed"
%	 text-hor-align= "right"
%	 >
%$\eeinptt$
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(113.75,80)"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\otheroutpt$
%</text>
%<parallelogram fill-color= "#999999"
%	 fill-style= "solid"
%	 p3= "(97.5,72.5)"
%	 p2= "(97.5,26.25)"
%	 p1= "(122.5,26.25)"
%	 stroke-color= "#999999"
%	 />
%<parallelogram fill-color= "#999999"
%	 fill-style= "solid"
%	 p3= "(107.5,80)"
%	 p2= "(107.5,60)"
%	 p1= "(112.5,60)"
%	 stroke-color= "#999999"
%	 />
%<parallelogram fill-color= "#999999"
%	 fill-style= "solid"
%	 p3= "(107.5,40)"
%	 p2= "(107.5,20)"
%	 p1= "(112.5,20)"
%	 stroke-color= "#999999"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(110,80);(110,80);(110,70);(110,70)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(110,40);(110,40);(110,20);(110,20)"
%	 />
%<parallelogram fill-color= "#ffffff"
%	 fill-style= "solid"
%	 stroke-width= "0.75"
%	 p3= "(115,60)"
%	 p2= "(115,70)"
%	 p1= "(105,70)"
%	 />
%<parallelogram fill-color= "#ffffff"
%	 fill-style= "solid"
%	 stroke-width= "0.75"
%	 p3= "(120,28.75)"
%	 p2= "(120,48.75)"
%	 p1= "(100,48.75)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(110,60);(110,60);(110,48.75);(110,48.75)"
%	 />
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(110,38.75)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\see$
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(110,65)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\hee$
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(90,50)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\EQLS
%</text>
%</jpic>
%%End JPIC-XML
%PSTricks content-type (pstricks.sty package needed)
%Add \usepackage{pstricks} in the preamble of your LaTeX file
%You can rescale the whole picture (to 80% for instance) by using the command \def\JPicScale{0.8}
\ifx\JPicScale\undefined\def\JPicScale{1}\fi
\psset{unit=\JPicScale mm}
\psset{linewidth=0.3,dotsep=1,hatchwidth=0.3,hatchsep=1.5,shadowsize=1,dimen=middle}
\psset{dotsize=0.7 2.5,dotscale=1 1,fillcolor=black}
\psset{arrowsize=1 2,arrowlength=1,arrowinset=0.25,tbarsize=0.7 5,bracketlength=0.15,rbracketlength=0.15}
\begin{pspicture}(0,0)(122.5,80)
\rput[r](66.25,20){$\eeinptt$}
\rput[l](73.75,80){$\otheroutpt$}
\newrgbcolor{userLineColour}{0.6 0.6 0.6}
\newrgbcolor{userFillColour}{0.6 0.6 0.6}
\pspolygon[linecolor=userLineColour,fillcolor=userFillColour,fillstyle=solid](82.5,37.5)(57.5,37.5)(57.5,62.5)(82.5,62.5)
\newrgbcolor{userLineColour}{0.6 0.6 0.6}
\newrgbcolor{userFillColour}{0.6 0.6 0.6}
\pspolygon[linecolor=userLineColour,fillcolor=userFillColour,fillstyle=solid](72.5,60)(67.5,60)(67.5,80)(72.5,80)
\newrgbcolor{userLineColour}{0.6 0.6 0.6}
\newrgbcolor{userFillColour}{0.6 0.6 0.6}
\pspolygon[linecolor=userLineColour,fillcolor=userFillColour,fillstyle=solid](72.5,20)(67.5,20)(67.5,40)(72.5,40)
\psline[linewidth=0.75](70,40)(70,20)
\psline[linewidth=0.75](0,60)(0,40)
\psline[linewidth=0.75](20,40)(20,60)
\psline[linewidth=0.75](0,40)(20,40)
\psline[linewidth=0.75](10,40)(10,20)
\psline[linewidth=0.75](10,80)(10,60)
\psline[linewidth=0.75](0,60)(20,60)
\rput(10,5){\strict}
\rput(90,5){\homomorphism}
\rput(10,50){$\see$}
\rput(40,52.5){\goesto}
\pspolygon[linewidth=0.75](60,60)(80,60)(80,40)(60,40)
\psline[linewidth=0.75](70,80)(70,60)
\rput[l](13.75,80){\outpt}
\rput[r](7.5,20){\inputt}
\rput(70,50){$\eehee$}
\rput[r](106.25,20){$\eeinptt$}
\rput[l](113.75,80){$\otheroutpt$}
\newrgbcolor{userLineColour}{0.6 0.6 0.6}
\newrgbcolor{userFillColour}{0.6 0.6 0.6}
\pspolygon[linecolor=userLineColour,fillcolor=userFillColour,fillstyle=solid](122.5,26.25)(97.5,26.25)(97.5,72.5)(122.5,72.5)
\newrgbcolor{userLineColour}{0.6 0.6 0.6}
\newrgbcolor{userFillColour}{0.6 0.6 0.6}
\pspolygon[linecolor=userLineColour,fillcolor=userFillColour,fillstyle=solid](112.5,60)(107.5,60)(107.5,80)(112.5,80)
\newrgbcolor{userLineColour}{0.6 0.6 0.6}
\newrgbcolor{userFillColour}{0.6 0.6 0.6}
\pspolygon[linecolor=userLineColour,fillcolor=userFillColour,fillstyle=solid](112.5,20)(107.5,20)(107.5,40)(112.5,40)
\psline[linewidth=0.75](110,80)(110,70)
\psline[linewidth=0.75](110,40)(110,20)
\pspolygon[linewidth=0.75,fillcolor=white,fillstyle=solid](105,70)(115,70)(115,60)(105,60)
\pspolygon[linewidth=0.75,fillcolor=white,fillstyle=solid](100,48.75)(120,48.75)(120,28.75)(100,28.75)
\psline[linewidth=0.75](110,60)(110,48.75)
\rput(110,38.75){$\see$}
\rput(110,65){$\hee$}
\rput(90,50){\EQLS}
\end{pspicture}


==> PIC/triple-notations-4.tex <==
%%Created by jPicEdt 1.4.1_03: mixed JPIC-XML/LaTeX format
%%Sun Nov 03 11:52:47 GMT-10:00 2019
%%Begin JPIC-XML
%<?xml version="1.0" standalone="yes"?>
%<jpic x-min="0" x-max="82.5" y-min="5" y-max="80" auto-bounding="true">
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 stroke-width= "0.75"
%	 stroke-dasharray= "8;8"
%	 stroke-style= "dashed"
%	 anchor-point= "(66.25,20)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\eeinptt$
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(73.75,80)"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\otheroutpt$
%</text>
%<parallelogram fill-style= "solid"
%	 p3= "(57.5,62.5)"
%	 p2= "(57.5,37.5)"
%	 p1= "(82.5,37.5)"
%	 fill-color= "#999999"
%	 stroke-color= "#999999"
%	 />
%<parallelogram fill-style= "solid"
%	 p3= "(67.5,80)"
%	 p2= "(67.5,60)"
%	 p1= "(72.5,60)"
%	 fill-color= "#999999"
%	 stroke-color= "#999999"
%	 />
%<parallelogram fill-style= "solid"
%	 p3= "(67.5,40)"
%	 p2= "(67.5,20)"
%	 p1= "(72.5,20)"
%	 fill-color= "#999999"
%	 stroke-color= "#999999"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(70,40);(70,40);(70,20);(70,20)"
%	 />
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(10,5)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\strict
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(70,5)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\homomorphism
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(40,52.5)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\goesto
%</text>
%<parallelogram fill-style= "solid"
%	 p3= "(80,40)"
%	 p2= "(80,60)"
%	 stroke-width= "0.75"
%	 p1= "(60,60)"
%	 fill-color= "#ffffff"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(70,80);(70,80);(70,60);(70,60)"
%	 />
%<parallelogram fill-style= "solid"
%	 p3= "(7.5,80)"
%	 p2= "(7.5,60)"
%	 p1= "(12.5,60)"
%	 fill-color= "#999999"
%	 stroke-color= "#999999"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(0,60);(0,60);(0,40);(0,40)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(20,40);(20,40);(20,60);(20,60)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(0,40);(0,40);(20,40);(20,40)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(10,40);(10,40);(10,20);(10,20)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(10,80);(10,80);(10,60);(10,60)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(0,60);(0,60);(20,60);(20,60)"
%	 />
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(10,50)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\see$
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(13.75,80)"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%\outpt
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(7.5,20)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%\inputt
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 stroke-width= "0.7"
%	 anchor-point= "(70,50)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\seesharp$
%</text>
%</jpic>
%%End JPIC-XML
%PSTricks content-type (pstricks.sty package needed)
%Add \usepackage{pstricks} in the preamble of your LaTeX file
%You can rescale the whole picture (to 80% for instance) by using the command \def\JPicScale{0.8}
\ifx\JPicScale\undefined\def\JPicScale{1}\fi
\psset{unit=\JPicScale mm}
\psset{linewidth=0.3,dotsep=1,hatchwidth=0.3,hatchsep=1.5,shadowsize=1,dimen=middle}
\psset{dotsize=0.7 2.5,dotscale=1 1,fillcolor=black}
\psset{arrowsize=1 2,arrowlength=1,arrowinset=0.25,tbarsize=0.7 5,bracketlength=0.15,rbracketlength=0.15}
\begin{pspicture}(0,0)(82.5,80)
\rput[r](66.25,20){$\eeinptt$}
\rput[l](73.75,80){$\otheroutpt$}
\newrgbcolor{userLineColour}{0.6 0.6 0.6}
\newrgbcolor{userFillColour}{0.6 0.6 0.6}
\pspolygon[linecolor=userLineColour,fillcolor=userFillColour,fillstyle=solid](82.5,37.5)(57.5,37.5)(57.5,62.5)(82.5,62.5)
\newrgbcolor{userLineColour}{0.6 0.6 0.6}
\newrgbcolor{userFillColour}{0.6 0.6 0.6}
\pspolygon[linecolor=userLineColour,fillcolor=userFillColour,fillstyle=solid](72.5,60)(67.5,60)(67.5,80)(72.5,80)
\newrgbcolor{userLineColour}{0.6 0.6 0.6}
\newrgbcolor{userFillColour}{0.6 0.6 0.6}
\pspolygon[linecolor=userLineColour,fillcolor=userFillColour,fillstyle=solid](72.5,20)(67.5,20)(67.5,40)(72.5,40)
\psline[linewidth=0.75](70,40)(70,20)
\rput(10,5){\strict}
\rput(70,5){\homomorphism}
\rput(40,52.5){\goesto}
\pspolygon[linewidth=0.75,fillcolor=white,fillstyle=solid](60,60)(80,60)(80,40)(60,40)
\psline[linewidth=0.75](70,80)(70,60)
\newrgbcolor{userLineColour}{0.6 0.6 0.6}
\newrgbcolor{userFillColour}{0.6 0.6 0.6}
\pspolygon[linecolor=userLineColour,fillcolor=userFillColour,fillstyle=solid](12.5,60)(7.5,60)(7.5,80)(12.5,80)
\psline[linewidth=0.75](0,60)(0,40)
\psline[linewidth=0.75](20,40)(20,60)
\psline[linewidth=0.75](0,40)(20,40)
\psline[linewidth=0.75](10,40)(10,20)
\psline[linewidth=0.75](10,80)(10,60)
\psline[linewidth=0.75](0,60)(20,60)
\rput(10,50){$\see$}
\rput[l](13.75,80){\outpt}
\rput[r](7.5,20){\inputt}
\rput(70,50){$\seesharp$}
\end{pspicture}


==> PIC/triple-notations-5.tex <==
%%Created by jPicEdt 1.4.1_03: mixed JPIC-XML/LaTeX format
%%Mon Nov 04 18:24:47 GMT-10:00 2019
%%Begin JPIC-XML
%<?xml version="1.0" standalone="yes"?>
%<jpic x-min="0" x-max="70" y-min="0" y-max="60" auto-bounding="true">
%<parallelogram p3= "(7.5,60)"
%	 p2= "(7.5,40)"
%	 fill-color= "#999999"
%	 p1= "(12.5,40)"
%	 stroke-color= "#999999"
%	 fill-style= "solid"
%	 />
%<parallelogram p3= "(57.5,60)"
%	 p2= "(57.5,40)"
%	 fill-color= "#999999"
%	 p1= "(62.5,40)"
%	 stroke-color= "#999999"
%	 fill-style= "solid"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(60,60);(60,60);(60,50);(60,50)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(60,20);(60,20);(60,0);(60,0)"
%	 />
%<parallelogram p3= "(65,40)"
%	 p2= "(65,50)"
%	 fill-color= "#ffffff"
%	 p1= "(55,50)"
%	 stroke-width= "0.75"
%	 fill-style= "solid"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(0,40);(0,40);(0,20);(0,20)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(20,20);(20,20);(20,40);(20,40)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(0,20);(0,20);(20,20);(20,20)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(10,20);(10,20);(10,0);(10,0)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(10,60);(10,60);(10,40);(10,40)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(0,40);(0,40);(20,40);(20,40)"
%	 />
%<text text-vert-align= "center-v"
%	 anchor-point= "(35,30)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\goesto
%</text>
%<parallelogram p3= "(70,10)"
%	 p2= "(70,30)"
%	 fill-color= "#ffffff"
%	 p1= "(50,30)"
%	 stroke-width= "0.75"
%	 fill-style= "solid"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(60,40);(60,40);(60,30);(60,30)"
%	 />
%<text text-vert-align= "center-v"
%	 anchor-point= "(60,20)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\see$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(60,45)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\hee$
%</text>
%<text text-vert-align= "center-v"
%	 fill-color= "#ffffff"
%	 stroke-dasharray= "8;8"
%	 anchor-point= "(10,30)"
%	 stroke-width= "0.75"
%	 fill-style= "solid"
%	 stroke-style= "dashed"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\eehee$
%</text>
%</jpic>
%%End JPIC-XML
%PSTricks content-type (pstricks.sty package needed)
%Add \usepackage{pstricks} in the preamble of your LaTeX file
%You can rescale the whole picture (to 80% for instance) by using the command \def\JPicScale{0.8}
\ifx\JPicScale\undefined\def\JPicScale{1}\fi
\psset{unit=\JPicScale mm}
\psset{linewidth=0.3,dotsep=1,hatchwidth=0.3,hatchsep=1.5,shadowsize=1,dimen=middle}
\psset{dotsize=0.7 2.5,dotscale=1 1,fillcolor=black}
\psset{arrowsize=1 2,arrowlength=1,arrowinset=0.25,tbarsize=0.7 5,bracketlength=0.15,rbracketlength=0.15}
\begin{pspicture}(0,0)(70,60)
\newrgbcolor{userLineColour}{0.6 0.6 0.6}
\newrgbcolor{userFillColour}{0.6 0.6 0.6}
\pspolygon[linecolor=userLineColour,fillcolor=userFillColour,fillstyle=solid](12.5,40)(7.5,40)(7.5,60)(12.5,60)
\newrgbcolor{userLineColour}{0.6 0.6 0.6}
\newrgbcolor{userFillColour}{0.6 0.6 0.6}
\pspolygon[linecolor=userLineColour,fillcolor=userFillColour,fillstyle=solid](62.5,40)(57.5,40)(57.5,60)(62.5,60)
\psline[linewidth=0.75](60,60)(60,50)
\psline[linewidth=0.75](60,20)(60,0)
\pspolygon[linewidth=0.75,fillcolor=white,fillstyle=solid](55,50)(65,50)(65,40)(55,40)
\psline[linewidth=0.75](0,40)(0,20)
\psline[linewidth=0.75](20,20)(20,40)
\psline[linewidth=0.75](0,20)(20,20)
\psline[linewidth=0.75](10,20)(10,0)
\psline[linewidth=0.75](10,60)(10,40)
\psline[linewidth=0.75](0,40)(20,40)
\rput(35,30){\goesto}
\pspolygon[linewidth=0.75,fillcolor=white,fillstyle=solid](50,30)(70,30)(70,10)(50,10)
\psline[linewidth=0.75](60,40)(60,30)
\rput(60,20){$\see$}
\rput(60,45){$\hee$}
\rput(10,30){$\eehee$}
\end{pspicture}


==> PIC/triple-notations.tex <==
%%Created by jPicEdt 1.4.1_03: mixed JPIC-XML/LaTeX format
%%Fri Nov 01 12:33:32 GMT-10:00 2019
%%Begin JPIC-XML
%<?xml version="1.0" standalone="yes"?>
%<jpic x-min="20" x-max="242.5" y-min="5" y-max="80" auto-bounding="true">
%<multicurve fill-style= "none"
%	 points= "(95,60);(95,60);(95,40);(95,40)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(115,40);(115,40);(115,60);(115,60)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(95,40);(95,40);(115,40);(115,40)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(105,40);(105,40);(105,20);(105,20)"
%	 stroke-width= "0.75"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(102.5,20)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\otherinputt$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(108.75,80)"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\otheroutpt$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(105,50)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\hee$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 stroke-dasharray= "8;8"
%	 anchor-point= "(186.25,20)"
%	 stroke-style= "dashed"
%	 text-frame= "noframe"
%	 stroke-width= "0.75"
%	 text-hor-align= "right"
%	 >
%$\eeinptt$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(193.75,80)"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\otheroutpt$
%</text>
%<parallelogram p3= "(187.5,80)"
%	 fill-style= "solid"
%	 p2= "(187.5,60)"
%	 fill-color= "#999999"
%	 p1= "(192.5,60)"
%	 stroke-color= "#999999"
%	 />
%<parallelogram p3= "(187.5,40)"
%	 fill-style= "solid"
%	 p2= "(187.5,20)"
%	 fill-color= "#999999"
%	 p1= "(192.5,20)"
%	 stroke-color= "#999999"
%	 />
%<multicurve fill-style= "none"
%	 points= "(190,80);(190,80);(190,60);(190,60)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(190,40);(190,40);(190,20);(190,20)"
%	 stroke-width= "0.75"
%	 />
%<parallelogram p3= "(200,40)"
%	 fill-style= "solid"
%	 p2= "(200,60)"
%	 fill-color= "#ffffff"
%	 p1= "(180,60)"
%	 stroke-width= "0.75"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "solid"
%	 fill-color= "#ffffff"
%	 stroke-dasharray= "8;8"
%	 anchor-point= "(190,50)"
%	 stroke-style= "dashed"
%	 text-frame= "noframe"
%	 stroke-width= "0.75"
%	 text-hor-align= "center-h"
%	 >
%$\eehee$
%</text>
%<parallelogram p3= "(102.5,80)"
%	 fill-style= "solid"
%	 p2= "(102.5,60)"
%	 fill-color= "#999999"
%	 p1= "(107.5,60)"
%	 stroke-color= "#999999"
%	 />
%<multicurve fill-style= "none"
%	 points= "(105,80);(105,80);(105,60);(105,60)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(95,60);(95,60);(115,60);(115,60)"
%	 stroke-width= "0.75"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 stroke-dasharray= "8;8"
%	 anchor-point= "(226.25,20)"
%	 stroke-style= "dashed"
%	 text-frame= "noframe"
%	 stroke-width= "0.75"
%	 text-hor-align= "right"
%	 >
%$\eeinptt$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(233.75,80)"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\otheroutpt$
%</text>
%<parallelogram p3= "(217.5,62.5)"
%	 fill-style= "solid"
%	 p2= "(217.5,37.5)"
%	 fill-color= "#999999"
%	 p1= "(242.5,37.5)"
%	 stroke-color= "#999999"
%	 />
%<parallelogram p3= "(227.5,80)"
%	 fill-style= "solid"
%	 p2= "(227.5,60)"
%	 fill-color= "#999999"
%	 p1= "(232.5,60)"
%	 stroke-color= "#999999"
%	 />
%<parallelogram p3= "(227.5,40)"
%	 fill-style= "solid"
%	 p2= "(227.5,20)"
%	 fill-color= "#999999"
%	 p1= "(232.5,20)"
%	 stroke-color= "#999999"
%	 />
%<multicurve fill-style= "none"
%	 points= "(230,80);(230,80);(230,60);(230,60)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(230,40);(230,40);(230,20);(230,20)"
%	 stroke-width= "0.75"
%	 />
%<parallelogram p3= "(240,40)"
%	 fill-style= "solid"
%	 p2= "(240,60)"
%	 fill-color= "#ffffff"
%	 p1= "(220,60)"
%	 stroke-width= "0.75"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(230,50)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\hee$
%</text>
%<multicurve fill-style= "none"
%	 points= "(20,60);(20,60);(20,40);(20,40)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(40,40);(40,40);(40,60);(40,60)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(20,40);(20,40);(40,40);(40,40)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(30,40);(30,40);(30,20);(30,20)"
%	 stroke-width= "0.75"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(27.5,20)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\otherinputt$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(33.75,80)"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\otheroutpt$
%</text>
%<multicurve fill-style= "none"
%	 points= "(30,80);(30,80);(30,60);(30,60)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(20,60);(20,60);(40,60);(40,60)"
%	 stroke-width= "0.75"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(30,5)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\strict
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(105,5)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\effect
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(210,5)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\homomorphism
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(210,50)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\oor
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(30,50)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\see$
%</text>
%</jpic>
%%End JPIC-XML
%PSTricks content-type (pstricks.sty package needed)
%Add \usepackage{pstricks} in the preamble of your LaTeX file
%You can rescale the whole picture (to 80% for instance) by using the command \def\JPicScale{0.8}
\ifx\JPicScale\undefined\def\JPicScale{1}\fi
\psset{unit=\JPicScale mm}
\psset{linewidth=0.3,dotsep=1,hatchwidth=0.3,hatchsep=1.5,shadowsize=1,dimen=middle}
\psset{dotsize=0.7 2.5,dotscale=1 1,fillcolor=black}
\psset{arrowsize=1 2,arrowlength=1,arrowinset=0.25,tbarsize=0.7 5,bracketlength=0.15,rbracketlength=0.15}
\begin{pspicture}(0,0)(242.5,80)
\psline[linewidth=0.75](95,60)(95,40)
\psline[linewidth=0.75](115,40)(115,60)
\psline[linewidth=0.75](95,40)(115,40)
\psline[linewidth=0.75](105,40)(105,20)
\rput[r](102.5,20){$\otherinputt$}
\rput[l](108.75,80){$\otheroutpt$}
\rput(105,50){$\hee$}
\rput[r](186.25,20){$\eeinptt$}
\rput[l](193.75,80){$\otheroutpt$}
\newrgbcolor{userLineColour}{0.6 0.6 0.6}
\newrgbcolor{userFillColour}{0.6 0.6 0.6}
\pspolygon[linecolor=userLineColour,fillcolor=userFillColour,fillstyle=solid](192.5,60)(187.5,60)(187.5,80)(192.5,80)
\newrgbcolor{userLineColour}{0.6 0.6 0.6}
\newrgbcolor{userFillColour}{0.6 0.6 0.6}
\pspolygon[linecolor=userLineColour,fillcolor=userFillColour,fillstyle=solid](192.5,20)(187.5,20)(187.5,40)(192.5,40)
\psline[linewidth=0.75](190,80)(190,60)
\psline[linewidth=0.75](190,40)(190,20)
\pspolygon[linewidth=0.75,fillcolor=white,fillstyle=solid](180,60)(200,60)(200,40)(180,40)
\rput(190,50){$\eehee$}
\newrgbcolor{userLineColour}{0.6 0.6 0.6}
\newrgbcolor{userFillColour}{0.6 0.6 0.6}
\pspolygon[linecolor=userLineColour,fillcolor=userFillColour,fillstyle=solid](107.5,60)(102.5,60)(102.5,80)(107.5,80)
\psline[linewidth=0.75](105,80)(105,60)
\psline[linewidth=0.75](95,60)(115,60)
\rput[r](226.25,20){$\eeinptt$}
\rput[l](233.75,80){$\otheroutpt$}
\newrgbcolor{userLineColour}{0.6 0.6 0.6}
\newrgbcolor{userFillColour}{0.6 0.6 0.6}
\pspolygon[linecolor=userLineColour,fillcolor=userFillColour,fillstyle=solid](242.5,37.5)(217.5,37.5)(217.5,62.5)(242.5,62.5)
\newrgbcolor{userLineColour}{0.6 0.6 0.6}
\newrgbcolor{userFillColour}{0.6 0.6 0.6}
\pspolygon[linecolor=userLineColour,fillcolor=userFillColour,fillstyle=solid](232.5,60)(227.5,60)(227.5,80)(232.5,80)
\newrgbcolor{userLineColour}{0.6 0.6 0.6}
\newrgbcolor{userFillColour}{0.6 0.6 0.6}
\pspolygon[linecolor=userLineColour,fillcolor=userFillColour,fillstyle=solid](232.5,20)(227.5,20)(227.5,40)(232.5,40)
\psline[linewidth=0.75](230,80)(230,60)
\psline[linewidth=0.75](230,40)(230,20)
\pspolygon[linewidth=0.75,fillcolor=white,fillstyle=solid](220,60)(240,60)(240,40)(220,40)
\rput(230,50){$\hee$}
\psline[linewidth=0.75](20,60)(20,40)
\psline[linewidth=0.75](40,40)(40,60)
\psline[linewidth=0.75](20,40)(40,40)
\psline[linewidth=0.75](30,40)(30,20)
\rput[r](27.5,20){$\otherinputt$}
\rput[l](33.75,80){$\otheroutpt$}
\psline[linewidth=0.75](30,80)(30,60)
\psline[linewidth=0.75](20,60)(40,60)
\rput(30,5){\strict}
\rput(105,5){\effect}
\rput(210,5){\homomorphism}
\rput(210,50){\oor}
\rput(30,50){$\see$}
\end{pspicture}


==> PIC/triple.tex <==
%%Created by jPicEdt 1.4.1_03: mixed JPIC-XML/LaTeX format
%%Sun Nov 03 12:04:40 GMT-10:00 2019
%%Begin JPIC-XML
%<?xml version="1.0" standalone="yes"?>
%<jpic x-min="5" x-max="187.5" y-min="0" y-max="60" auto-bounding="true">
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(115,40);(115,40);(115,20);(115,20)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(135,20);(135,20);(135,40);(135,40)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(115,20);(115,20);(135,20);(135,20)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(125,20);(125,20);(125,0);(125,0)"
%	 />
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(122.5,0)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\otherinputt$
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(128.75,60)"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\otheroutpt$
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(125,30)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\hee$
%</text>
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(10,25);(10,25);(10,0);(10,0)"
%	 />
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(7.5,0)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\otherinputt$
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 stroke-width= "0.75"
%	 stroke-dasharray= "8;8"
%	 stroke-style= "dashed"
%	 anchor-point= "(10,30)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\unit$
%</text>
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(5,25);(5,25);(15,25);(15,25)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(15,35);(15,35);(15,25);(15,25)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(5,35);(5,35);(5,25);(5,25)"
%	 />
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 stroke-width= "0.75"
%	 stroke-dasharray= "8;8"
%	 stroke-style= "dashed"
%	 anchor-point= "(150,33.75)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\goesto
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 stroke-width= "0.75"
%	 stroke-dasharray= "8;8"
%	 stroke-style= "dashed"
%	 anchor-point= "(13.75,60)"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\eeinptt$
%</text>
%<parallelogram fill-style= "solid"
%	 p3= "(122.5,60)"
%	 p2= "(122.5,40)"
%	 p1= "(127.5,40)"
%	 fill-color= "#999999"
%	 stroke-color= "#999999"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(125,60);(125,60);(125,40);(125,40)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(115,40);(115,40);(135,40);(135,40)"
%	 />
%<parallelogram fill-style= "solid"
%	 p3= "(7.5,60)"
%	 p2= "(7.5,35)"
%	 p1= "(12.5,35)"
%	 fill-color= "#999999"
%	 stroke-color= "#999999"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(10,60);(10,60);(10,35);(10,35)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(5,35);(5,35);(15,35);(15,35)"
%	 />
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 stroke-width= "0.75"
%	 stroke-dasharray= "8;8"
%	 stroke-style= "dashed"
%	 anchor-point= "(171.25,0)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\eeinptt$
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(178.75,60)"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\otheroutpt$
%</text>
%<parallelogram fill-style= "solid"
%	 p3= "(162.5,42.5)"
%	 p2= "(162.5,17.5)"
%	 p1= "(187.5,17.5)"
%	 fill-color= "#999999"
%	 stroke-color= "#999999"
%	 />
%<parallelogram fill-style= "solid"
%	 p3= "(172.5,60)"
%	 p2= "(172.5,40)"
%	 p1= "(177.5,40)"
%	 fill-color= "#999999"
%	 stroke-color= "#999999"
%	 />
%<parallelogram fill-style= "solid"
%	 p3= "(172.5,20)"
%	 p2= "(172.5,0)"
%	 p1= "(177.5,0)"
%	 fill-color= "#999999"
%	 stroke-color= "#999999"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(175,60);(175,60);(175,40);(175,40)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(175,20);(175,20);(175,0);(175,0)"
%	 />
%<parallelogram fill-style= "solid"
%	 p3= "(185,20)"
%	 p2= "(185,40)"
%	 stroke-width= "0.75"
%	 p1= "(165,40)"
%	 fill-color= "#ffffff"
%	 />
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 stroke-width= "0.7"
%	 anchor-point= "(25,30)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\ORR
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 stroke-width= "0.75"
%	 stroke-dasharray= "8;8"
%	 stroke-style= "dashed"
%	 anchor-point= "(40,30)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\unit$
%</text>
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(35,25);(35,25);(45,25);(45,25)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(45,35);(45,35);(45,25);(45,25)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(35,35);(35,35);(35,25);(35,25)"
%	 />
%<parallelogram fill-style= "solid"
%	 p3= "(37.5,60)"
%	 p2= "(37.5,35)"
%	 p1= "(42.5,35)"
%	 fill-color= "#999999"
%	 stroke-color= "#999999"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.75"
%	 points= "(35,35);(35,35);(45,35);(45,35)"
%	 />
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 stroke-width= "0.7"
%	 anchor-point= "(45,60)"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\Mii$
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 stroke-width= "0.7"
%	 anchor-point= "(37.5,17.5)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\Jii$
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 stroke-width= "0.7"
%	 anchor-point= "(175,30)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\eehee$
%</text>
%</jpic>
%%End JPIC-XML
%PSTricks content-type (pstricks.sty package needed)
%Add \usepackage{pstricks} in the preamble of your LaTeX file
%You can rescale the whole picture (to 80% for instance) by using the command \def\JPicScale{0.8}
\ifx\JPicScale\undefined\def\JPicScale{1}\fi
\psset{unit=\JPicScale mm}
\psset{linewidth=0.3,dotsep=1,hatchwidth=0.3,hatchsep=1.5,shadowsize=1,dimen=middle}
\psset{dotsize=0.7 2.5,dotscale=1 1,fillcolor=black}
\psset{arrowsize=1 2,arrowlength=1,arrowinset=0.25,tbarsize=0.7 5,bracketlength=0.15,rbracketlength=0.15}
\begin{pspicture}(0,0)(187.5,60)
\psline[linewidth=0.75](115,40)(115,20)
\psline[linewidth=0.75](135,20)(135,40)
\psline[linewidth=0.75](115,20)(135,20)
\psline[linewidth=0.75](125,20)(125,0)
\rput[r](122.5,0){$\otherinputt$}
\rput[l](128.75,60){$\otheroutpt$}
\rput(125,30){$\hee$}
\psline[linewidth=0.75](10,25)(10,0)
\rput[r](7.5,0){$\otherinputt$}
\rput(10,30){$\unit$}
\psline[linewidth=0.75](5,25)(15,25)
\psline[linewidth=0.75](15,35)(15,25)
\psline[linewidth=0.75](5,35)(5,25)
\rput(150,33.75){\goesto}
\rput[l](13.75,60){$\eeinptt$}
\newrgbcolor{userLineColour}{0.6 0.6 0.6}
\newrgbcolor{userFillColour}{0.6 0.6 0.6}
\pspolygon[linecolor=userLineColour,fillcolor=userFillColour,fillstyle=solid](127.5,40)(122.5,40)(122.5,60)(127.5,60)
\psline[linewidth=0.75](125,60)(125,40)
\psline[linewidth=0.75](115,40)(135,40)
\newrgbcolor{userLineColour}{0.6 0.6 0.6}
\newrgbcolor{userFillColour}{0.6 0.6 0.6}
\pspolygon[linecolor=userLineColour,fillcolor=userFillColour,fillstyle=solid](12.5,35)(7.5,35)(7.5,60)(12.5,60)
\psline[linewidth=0.75](10,60)(10,35)
\psline[linewidth=0.75](5,35)(15,35)
\rput[r](171.25,0){$\eeinptt$}
\rput[l](178.75,60){$\otheroutpt$}
\newrgbcolor{userLineColour}{0.6 0.6 0.6}
\newrgbcolor{userFillColour}{0.6 0.6 0.6}
\pspolygon[linecolor=userLineColour,fillcolor=userFillColour,fillstyle=solid](187.5,17.5)(162.5,17.5)(162.5,42.5)(187.5,42.5)
\newrgbcolor{userLineColour}{0.6 0.6 0.6}
\newrgbcolor{userFillColour}{0.6 0.6 0.6}
\pspolygon[linecolor=userLineColour,fillcolor=userFillColour,fillstyle=solid](177.5,40)(172.5,40)(172.5,60)(177.5,60)
\newrgbcolor{userLineColour}{0.6 0.6 0.6}
\newrgbcolor{userFillColour}{0.6 0.6 0.6}
\pspolygon[linecolor=userLineColour,fillcolor=userFillColour,fillstyle=solid](177.5,0)(172.5,0)(172.5,20)(177.5,20)
\psline[linewidth=0.75](175,60)(175,40)
\psline[linewidth=0.75](175,20)(175,0)
\pspolygon[linewidth=0.75,fillcolor=white,fillstyle=solid](165,40)(185,40)(185,20)(165,20)
\rput(25,30){\ORR}
\rput(40,30){$\unit$}
\psline[linewidth=0.75](35,25)(45,25)
\psline[linewidth=0.75](45,35)(45,25)
\psline[linewidth=0.75](35,35)(35,25)
\newrgbcolor{userLineColour}{0.6 0.6 0.6}
\newrgbcolor{userFillColour}{0.6 0.6 0.6}
\pspolygon[linecolor=userLineColour,fillcolor=userFillColour,fillstyle=solid](42.5,35)(37.5,35)(37.5,60)(42.5,60)
\psline[linewidth=0.75](35,35)(45,35)
\rput[l](45,60){$\Mii$}
\rput[r](37.5,17.5){$\Jii$}
\rput(175,30){$\eehee$}
\end{pspicture}


==> PIC/type-prod-3.tex <==
%%Created by jPicEdt 1.4.1_03: mixed JPIC-XML/LaTeX format
%%Mon Aug 31 12:40:36 GMT-10:00 2020
%%Begin JPIC-XML
%<?xml version="1.0" standalone="yes"?>
%<jpic x-min="3.75" x-max="26.25" y-min="-1.88" y-max="30" auto-bounding="true">
%<multicurve fill-style= "none"
%	 points= "(5,30);(5,30);(5,0);(5,0)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(15,30);(15,30);(15,0);(15,0)"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(3.75,5)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\Ah$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(16.25,5)"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\Uh$
%</text>
%<text text-vert-align= "top"
%	 fill-style= "none"
%	 anchor-point= "(5,-1.88)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\eex$
%</text>
%<text text-vert-align= "top"
%	 fill-style= "none"
%	 anchor-point= "(15,-1.25)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\why$
%</text>
%<multicurve fill-style= "none"
%	 points= "(25,30);(25,30);(25,0);(25,0)"
%	 />
%<text text-vert-align= "top"
%	 fill-style= "none"
%	 anchor-point= "(25,-1.25)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\zee$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(26.25,5)"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\Cee$
%</text>
%</jpic>
%%End JPIC-XML
%PSTricks content-type (pstricks.sty package needed)
%Add \usepackage{pstricks} in the preamble of your LaTeX file
%You can rescale the whole picture (to 80% for instance) by using the command \def\JPicScale{0.8}
\ifx\JPicScale\undefined\def\JPicScale{1}\fi
\psset{unit=\JPicScale mm}
\psset{linewidth=0.3,dotsep=1,hatchwidth=0.3,hatchsep=1.5,shadowsize=1,dimen=middle}
\psset{dotsize=0.7 2.5,dotscale=1 1,fillcolor=black}
\psset{arrowsize=1 2,arrowlength=1,arrowinset=0.25,tbarsize=0.7 5,bracketlength=0.15,rbracketlength=0.15}
\begin{pspicture}(0,0)(26.25,30)
\psline(5,30)(5,0)
\psline(15,30)(15,0)
\rput[r](3.75,5){$\Ah$}
\rput[l](16.25,5){$\Uh$}
\rput[t](5,-1.88){$\eex$}
\rput[t](15,-1.25){$\why$}
\psline(25,30)(25,0)
\rput[t](25,-1.25){$\zee$}
\rput[l](26.25,5){$\Cee$}
\end{pspicture}


==> PIC/type-prod.tex <==
%%Created by jPicEdt 1.4.1_03: mixed JPIC-XML/LaTeX format
%%Mon Aug 31 12:24:59 GMT-10:00 2020
%%Begin JPIC-XML
%<?xml version="1.0" standalone="yes"?>
%<jpic x-min="3.75" x-max="26.25" y-min="-1.88" y-max="30" auto-bounding="true">
%<multicurve fill-style= "none"
%	 points= "(5,30);(5,30);(5,0);(5,0)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(15,30);(15,30);(15,0);(15,0)"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(3.75,5)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\Ah$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(16.25,5)"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\Uh$
%</text>
%<text text-vert-align= "top"
%	 fill-style= "none"
%	 anchor-point= "(5,-1.88)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\eex$
%</text>
%<text text-vert-align= "top"
%	 fill-style= "none"
%	 anchor-point= "(15,-1.25)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\why$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(26.25,5)"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\Cee$
%</text>
%</jpic>
%%End JPIC-XML
%PSTricks content-type (pstricks.sty package needed)
%Add \usepackage{pstricks} in the preamble of your LaTeX file
%You can rescale the whole picture (to 80% for instance) by using the command \def\JPicScale{0.8}
\ifx\JPicScale\undefined\def\JPicScale{1}\fi
\psset{unit=\JPicScale mm}
\psset{linewidth=0.3,dotsep=1,hatchwidth=0.3,hatchsep=1.5,shadowsize=1,dimen=middle}
\psset{dotsize=0.7 2.5,dotscale=1 1,fillcolor=black}
\psset{arrowsize=1 2,arrowlength=1,arrowinset=0.25,tbarsize=0.7 5,bracketlength=0.15,rbracketlength=0.15}
\begin{pspicture}(0,0)(26.25,30)
\psline(5,30)(5,0)
\psline(15,30)(15,0)
\rput[r](3.75,5){$\Ah$}
\rput[l](16.25,5){$\Uh$}
\rput[t](5,-1.88){$\eex$}
\rput[t](15,-1.25){$\why$}
\rput[l](26.25,5){$\Cee$}
\end{pspicture}


==> PIC/type-string-1.tex <==
%%Created by jPicEdt 1.4.1_03: mixed JPIC-XML/LaTeX format
%%Sat May 15 09:48:57 GMT-10:00 2021
%%Begin JPIC-XML
%<?xml version="1.0" standalone="yes"?>
%<jpic x-min="0" x-max="60" y-min="-5" y-max="65" auto-bounding="true">
%<multicurve fill-style= "none"
%	 stroke-width= "0.7"
%	 stroke-overstrike= "true"
%	 points= "(0,0);(0,10);(0,-5);(0,5);(0,15);(60,45);
%	(60,55);(60,65);(60,60);(60,60);(60,60);(60,60);
%	(60,60);(60,60);(60,60);(60,60)"
%	 stroke-overstrike-width= "1.05"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.7"
%	 stroke-overstrike= "true"
%	 points= "(20,0);(20,0);(20,60);(20,60)"
%	 stroke-overstrike-width= "0.8"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.7"
%	 stroke-overstrike= "true"
%	 points= "(40,0);(40,5);(40,0);(40,10);(40,20);(0,40);
%	(0,50);(0,50);(0,60);(0,60);(0,60);(0,60);
%	(0,60);(0,60);(0,60);(0,60)"
%	 stroke-overstrike-width= "1.05"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.7"
%	 stroke-overstrike= "true"
%	 points= "(60,0);(60,10);(60,5);(60,15);(60,25);(40,35);
%	(40,45);(40,45);(40,60);(40,60);(40,60);(40,60);
%	(40,60);(40,60);(40,60);(40,60)"
%	 stroke-overstrike-width= "1.05"
%	 />
%<text text-vert-align= "top"
%	 fill-style= "none"
%	 anchor-point= "(0,-2.5)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\eex$
%</text>
%<text text-vert-align= "top"
%	 fill-style= "none"
%	 anchor-point= "(20,-2.5)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\why$
%</text>
%<text text-vert-align= "top"
%	 fill-style= "none"
%	 anchor-point= "(40,-2.5)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\you$
%</text>
%<text text-vert-align= "top"
%	 fill-style= "none"
%	 anchor-point= "(60,-2.5)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\vea$
%</text>
%<text text-vert-align= "bottom"
%	 fill-style= "none"
%	 anchor-point= "(60,62.5)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\eex$
%</text>
%<text text-vert-align= "bottom"
%	 fill-style= "none"
%	 anchor-point= "(20,62.5)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\why$
%</text>
%<text text-vert-align= "bottom"
%	 fill-style= "none"
%	 anchor-point= "(0,62.5)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\you$
%</text>
%<text text-vert-align= "bottom"
%	 fill-style= "none"
%	 anchor-point= "(40,62.5)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\vea$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(1.88,6.25)"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\Ah$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(21.25,15)"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\Bh$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(34.38,21.25)"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\Ce$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(54.38,28.75)"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\De$
%</text>
%</jpic>
%%End JPIC-XML
%PSTricks content-type (pstricks.sty package needed)
%Add \usepackage{pstricks} in the preamble of your LaTeX file
%You can rescale the whole picture (to 80% for instance) by using the command \def\JPicScale{0.8}
\ifx\JPicScale\undefined\def\JPicScale{1}\fi
\psset{unit=\JPicScale mm}
\psset{linewidth=0.3,dotsep=1,hatchwidth=0.3,hatchsep=1.5,shadowsize=1,dimen=middle}
\psset{dotsize=0.7 2.5,dotscale=1 1,fillcolor=black}
\psset{arrowsize=1 2,arrowlength=1,arrowinset=0.25,tbarsize=0.7 5,bracketlength=0.15,rbracketlength=0.15}
\begin{pspicture}(0,0)(60,65)
\pscustom[linewidth=0.7,border=1.05]{\psbezier(0,0)(0,10)(0,-5)(0,5)
\psbezier(0,15)(60,45)(60,55)
\psbezier(60,65)(60,60)(60,60)
\psbezier(60,60)(60,60)(60,60)
\psbezier(60,60)(60,60)(60,60)
\stroke[linewidth=2.8,linecolor=white]}
\psline[linewidth=0.7,border=0.8](20,0)(20,60)
\pscustom[linewidth=0.7,border=1.05]{\psbezier(40,0)(40,5)(40,0)(40,10)
\psbezier(40,20)(0,40)(0,50)
\psline(0,50)(0,60)
\psbezier(0,60)(0,60)(0,60)
\psbezier(0,60)(0,60)(0,60)
\stroke[linewidth=2.8,linecolor=white]}
\pscustom[linewidth=0.7,border=1.05]{\psbezier(60,0)(60,10)(60,5)(60,15)
\psbezier(60,25)(40,35)(40,45)
\psline(40,45)(40,60)
\psbezier(40,60)(40,60)(40,60)
\psbezier(40,60)(40,60)(40,60)
\stroke[linewidth=2.8,linecolor=white]}
\rput[t](0,-2.5){$\eex$}
\rput[t](20,-2.5){$\why$}
\rput[t](40,-2.5){$\you$}
\rput[t](60,-2.5){$\vea$}
\rput[b](60,62.5){$\eex$}
\rput[b](20,62.5){$\why$}
\rput[b](0,62.5){$\you$}
\rput[b](40,62.5){$\vea$}
\rput[l](1.88,6.25){$\Ah$}
\rput[l](21.25,15){$\Bh$}
\rput[l](34.38,21.25){$\Ce$}
\rput[l](54.38,28.75){$\De$}
\end{pspicture}


==> PIC/type-string-2.tex <==
%%Created by jPicEdt 1.4.1_03: mixed JPIC-XML/LaTeX format
%%Sat May 15 10:17:09 GMT-10:00 2021
%%Begin JPIC-XML
%<?xml version="1.0" standalone="yes"?>
%<jpic x-min="0" x-max="60" y-min="-5" y-max="65" auto-bounding="true">
%<multicurve fill-style= "none"
%	 stroke-width= "0.7"
%	 stroke-overstrike= "true"
%	 points= "(0,0);(0,10);(0,-5);(0,5);(0,15);(60,45);
%	(60,55);(60,65);(60,60);(60,60);(60,60);(60,60);
%	(60,60);(60,60);(60,60);(60,60)"
%	 stroke-overstrike-width= "1.05"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.7"
%	 stroke-overstrike= "true"
%	 points= "(20,0);(20,0);(20,60);(20,60)"
%	 stroke-overstrike-width= "0.8"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.7"
%	 stroke-overstrike= "true"
%	 points= "(40,0);(40,5);(40,0);(40,10);(40,20);(0,40);
%	(0,50);(0,50);(0,60);(0,60);(0,60);(0,60);
%	(0,60);(0,60);(0,60);(0,60)"
%	 stroke-overstrike-width= "1.05"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.7"
%	 stroke-overstrike= "true"
%	 points= "(60,0);(60,10);(60,5);(60,15);(60,25);(40,35);
%	(40,45);(40,45);(40,60);(40,60);(40,60);(40,60);
%	(40,60);(40,60);(40,60);(40,60)"
%	 stroke-overstrike-width= "1.05"
%	 />
%<text text-vert-align= "top"
%	 fill-style= "none"
%	 anchor-point= "(0,-2.5)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\eex$
%</text>
%<text text-vert-align= "top"
%	 fill-style= "none"
%	 anchor-point= "(20,-2.5)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\why$
%</text>
%<text text-vert-align= "top"
%	 fill-style= "none"
%	 anchor-point= "(40,-2.5)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\you$
%</text>
%<text text-vert-align= "top"
%	 fill-style= "none"
%	 anchor-point= "(60,-2.5)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\vea$
%</text>
%<text text-vert-align= "bottom"
%	 fill-style= "none"
%	 anchor-point= "(60,62.5)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\eex$
%</text>
%<text text-vert-align= "bottom"
%	 fill-style= "none"
%	 anchor-point= "(20,62.5)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\why$
%</text>
%<text text-vert-align= "bottom"
%	 fill-style= "none"
%	 anchor-point= "(0,62.5)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\you$
%</text>
%<text text-vert-align= "bottom"
%	 fill-style= "none"
%	 anchor-point= "(40,62.5)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\vea$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(1.88,6.25)"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\Ah$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(21.25,15)"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\Bh$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(34.38,21.25)"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\Ce$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(54.38,28.75)"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\De$
%</text>
%</jpic>
%%End JPIC-XML
%LaTeX-picture environment using emulated lines and arcs
%You can rescale the whole picture (to 80% for instance) by using the command \def\JPicScale{0.8}
\ifx\JPicScale\undefined\def\JPicScale{1}\fi
\unitlength \JPicScale mm
\begin{picture}(60,65)(0,0)
\linethickness{0.7mm}
\qbezier(0,0)(0,5.94)(0,2.5)
\qbezier(0,2.5)(0,-0.94)(0,5)
\qbezier(0,5)(3.75,13.75)(30,30)
\qbezier(30,30)(56.25,46.25)(60,55)
\qbezier(60,55)(60,61.88)(60,61.25)
\qbezier(60,61.25)(60,60.62)(60,60)
\qbezier(60,60)(60,60)(60,60)
\qbezier(60,60)(60,60)(60,60)
\qbezier(60,60)(60,60)(60,60)
\qbezier(60,60)(60,60)(60,60)
\linethickness{0.7mm}
\put(20,0){\line(0,1){60}}
\linethickness{0.7mm}
\qbezier(40,0)(40,2.97)(40,3.12)
\qbezier(40,3.12)(40,3.28)(40,10)
\qbezier(40,10)(37.5,18.12)(20,30)
\qbezier(20,30)(2.5,41.88)(0,50)
\put(0,50){\line(0,1){10}}
\qbezier(0,60)(0,60)(0,60)
\qbezier(0,60)(0,60)(0,60)
\qbezier(0,60)(0,60)(0,60)
\qbezier(0,60)(0,60)(0,60)
\linethickness{0.7mm}
\qbezier(60,0)(60,6.56)(60,7.5)
\qbezier(60,7.5)(60,8.44)(60,15)
\qbezier(60,15)(58.75,22.5)(50,30)
\qbezier(50,30)(41.25,37.5)(40,45)
\put(40,45){\line(0,1){15}}
\qbezier(40,60)(40,60)(40,60)
\qbezier(40,60)(40,60)(40,60)
\qbezier(40,60)(40,60)(40,60)
\qbezier(40,60)(40,60)(40,60)
\put(0,-2.5){\makebox(0,0)[tc]{$\eex$}}

\put(20,-2.5){\makebox(0,0)[tc]{$\why$}}

\put(40,-2.5){\makebox(0,0)[tc]{$\you$}}

\put(60,-2.5){\makebox(0,0)[tc]{$\vea$}}

\put(60,62.5){\makebox(0,0)[bc]{$\eex$}}

\put(20,62.5){\makebox(0,0)[bc]{$\why$}}

\put(0,62.5){\makebox(0,0)[bc]{$\you$}}

\put(40,62.5){\makebox(0,0)[bc]{$\vea$}}

\put(1.88,6.25){\makebox(0,0)[cl]{$\Ah$}}

\put(21.25,15){\makebox(0,0)[cl]{$\Bh$}}

\put(34.38,21.25){\makebox(0,0)[cl]{$\Ce$}}

\put(54.38,28.75){\makebox(0,0)[cl]{$\De$}}

\end{picture}


==> PIC/type-string-color.tex <==
%%Created by jPicEdt 1.4.1_03: mixed JPIC-XML/LaTeX format
%%Mon Aug 31 12:06:30 GMT-10:00 2020
%%Begin JPIC-XML
%<?xml version="1.0" standalone="yes"?>
%<jpic x-min="0" x-max="60" y-min="-5" y-max="65" auto-bounding="true">
%<multicurve fill-style= "none"
%	 stroke-overstrike-width= "1.05"
%	 points= "(0,0);(0,10);(0,-5);(0,5);(0,15);(60,45);
%	(60,55);(60,65);(60,60);(60,60);(60,60);(60,60);
%	(60,60);(60,60);(60,60);(60,60)"
%	 stroke-color= "#0066ff"
%	 stroke-overstrike= "true"
%	 stroke-width= "1"
%	 />
%<multicurve fill-style= "none"
%	 stroke-overstrike-width= "0.8"
%	 points= "(20,0);(20,0);(20,60);(20,60)"
%	 stroke-color= "#ff33cc"
%	 stroke-overstrike= "true"
%	 stroke-width= "1"
%	 />
%<multicurve fill-style= "none"
%	 stroke-overstrike-width= "1.05"
%	 points= "(40,0);(40,5);(40,0);(40,10);(40,20);(0,40);
%	(0,50);(0,50);(0,60);(0,60);(0,60);(0,60);
%	(0,60);(0,60);(0,60);(0,60)"
%	 stroke-color= "#ff9933"
%	 stroke-overstrike= "true"
%	 stroke-width= "1"
%	 />
%<multicurve fill-style= "none"
%	 stroke-overstrike-width= "1.05"
%	 points= "(60,0);(60,10);(60,5);(60,15);(60,25);(40,35);
%	(40,45);(40,45);(40,60);(40,60);(40,60);(40,60);
%	(40,60);(40,60);(40,60);(40,60)"
%	 stroke-color= "#66cc00"
%	 stroke-overstrike= "true"
%	 stroke-width= "1"
%	 />
%<text text-vert-align= "top"
%	 fill-style= "none"
%	 anchor-point= "(0,-2.5)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\eex$
%</text>
%<text text-vert-align= "top"
%	 fill-style= "none"
%	 anchor-point= "(20,-2.5)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\why$
%</text>
%<text text-vert-align= "top"
%	 fill-style= "none"
%	 anchor-point= "(40,-2.5)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\you$
%</text>
%<text text-vert-align= "top"
%	 fill-style= "none"
%	 anchor-point= "(60,-2.5)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\vea$
%</text>
%<text text-vert-align= "bottom"
%	 fill-style= "none"
%	 anchor-point= "(60,62.5)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\eex$
%</text>
%<text text-vert-align= "bottom"
%	 fill-style= "none"
%	 anchor-point= "(20,62.5)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\why$
%</text>
%<text text-vert-align= "bottom"
%	 fill-style= "none"
%	 anchor-point= "(0,62.5)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\you$
%</text>
%<text text-vert-align= "bottom"
%	 fill-style= "none"
%	 anchor-point= "(40,62.5)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\vea$
%</text>
%</jpic>
%%End JPIC-XML
%PSTricks content-type (pstricks.sty package needed)
%Add \usepackage{pstricks} in the preamble of your LaTeX file
%You can rescale the whole picture (to 80% for instance) by using the command \def\JPicScale{0.8}
\ifx\JPicScale\undefined\def\JPicScale{1}\fi
\psset{unit=\JPicScale mm}
\psset{linewidth=0.3,dotsep=1,hatchwidth=0.3,hatchsep=1.5,shadowsize=1,dimen=middle}
\psset{dotsize=0.7 2.5,dotscale=1 1,fillcolor=black}
\psset{arrowsize=1 2,arrowlength=1,arrowinset=0.25,tbarsize=0.7 5,bracketlength=0.15,rbracketlength=0.15}
\begin{pspicture}(0,0)(60,65)
\newrgbcolor{userLineColour}{0 0.4 1}
\pscustom[linewidth=1,linecolor=userLineColour,border=1.05]{\psbezier(0,0)(0,10)(0,-5)(0,5)
\psbezier(0,15)(60,45)(60,55)
\psbezier(60,65)(60,60)(60,60)
\psbezier(60,60)(60,60)(60,60)
\psbezier(60,60)(60,60)(60,60)
\stroke[linewidth=3.1,linecolor=white]}
\newrgbcolor{userLineColour}{1 0.2 0.8}
\psline[linewidth=1,linecolor=userLineColour,border=0.8](20,0)(20,60)
\newrgbcolor{userLineColour}{1 0.6 0.2}
\pscustom[linewidth=1,linecolor=userLineColour,border=1.05]{\psbezier(40,0)(40,5)(40,0)(40,10)
\psbezier(40,20)(0,40)(0,50)
\psline(0,50)(0,60)
\psbezier(0,60)(0,60)(0,60)
\psbezier(0,60)(0,60)(0,60)
\stroke[linewidth=3.1,linecolor=white]}
\newrgbcolor{userLineColour}{0.4 0.8 0}
\pscustom[linewidth=1,linecolor=userLineColour,border=1.05]{\psbezier(60,0)(60,10)(60,5)(60,15)
\psbezier(60,25)(40,35)(40,45)
\psline(40,45)(40,60)
\psbezier(40,60)(40,60)(40,60)
\psbezier(40,60)(40,60)(40,60)
\stroke[linewidth=3.1,linecolor=white]}
\rput[t](0,-2.5){$\eex$}
\rput[t](20,-2.5){$\why$}
\rput[t](40,-2.5){$\you$}
\rput[t](60,-2.5){$\vea$}
\rput[b](60,62.5){$\eex$}
\rput[b](20,62.5){$\why$}
\rput[b](0,62.5){$\you$}
\rput[b](40,62.5){$\vea$}
\end{pspicture}


==> PIC/type-string-invis-1.tex <==
%%Created by jPicEdt 1.4.1_03: mixed JPIC-XML/LaTeX format
%%Mon Aug 31 18:59:33 GMT-10:00 2020
%%Begin JPIC-XML
%<?xml version="1.0" standalone="yes"?>
%<jpic x-min="7.5" x-max="33.75" y-min="0" y-max="45" auto-bounding="true">
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(7.5,25)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\AAh$
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(10,0)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\eex$
%</text>
%<multicurve fill-style= "none"
%	 stroke-width= "2"
%	 stroke-color= "#ffffff"
%	 points= "(30,45);(30,45);(30,5);(30,5)"
%	 />
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(30,0)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\none$
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(33.75,11.25)"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\JJh$
%</text>
%</jpic>
%%End JPIC-XML
%PSTricks content-type (pstricks.sty package needed)
%Add \usepackage{pstricks} in the preamble of your LaTeX file
%You can rescale the whole picture (to 80% for instance) by using the command \def\JPicScale{0.8}
\ifx\JPicScale\undefined\def\JPicScale{1}\fi
\psset{unit=\JPicScale mm}
\psset{linewidth=0.3,dotsep=1,hatchwidth=0.3,hatchsep=1.5,shadowsize=1,dimen=middle}
\psset{dotsize=0.7 2.5,dotscale=1 1,fillcolor=black}
\psset{arrowsize=1 2,arrowlength=1,arrowinset=0.25,tbarsize=0.7 5,bracketlength=0.15,rbracketlength=0.15}
\begin{pspicture}(0,0)(33.75,45)
\rput[r](7.5,25){$\AAh$}
\rput(10,0){$\eex$}
\psline[linewidth=2,linecolor=white](30,45)(30,5)
\rput(30,0){$\none$}
\rput[l](33.75,11.25){$\JJh$}
\end{pspicture}


==> PIC/type-string-invis.tex <==
%%Created by jPicEdt 1.4.1_03: mixed JPIC-XML/LaTeX format
%%Mon Aug 31 18:56:16 GMT-10:00 2020
%%Begin JPIC-XML
%<?xml version="1.0" standalone="yes"?>
%<jpic x-min="7.5" x-max="33.75" y-min="0" y-max="45" auto-bounding="true">
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(7.5,25)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\AAh$
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(10,0)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\eex$
%</text>
%<multicurve fill-style= "none"
%	 stroke-width= "2"
%	 stroke-color= "#999999"
%	 points= "(30,45);(30,45);(30,5);(30,5)"
%	 />
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(30,0)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\none$
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(33.75,11.25)"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\JJh$
%</text>
%</jpic>
%%End JPIC-XML
%PSTricks content-type (pstricks.sty package needed)
%Add \usepackage{pstricks} in the preamble of your LaTeX file
%You can rescale the whole picture (to 80% for instance) by using the command \def\JPicScale{0.8}
\ifx\JPicScale\undefined\def\JPicScale{1}\fi
\psset{unit=\JPicScale mm}
\psset{linewidth=0.3,dotsep=1,hatchwidth=0.3,hatchsep=1.5,shadowsize=1,dimen=middle}
\psset{dotsize=0.7 2.5,dotscale=1 1,fillcolor=black}
\psset{arrowsize=1 2,arrowlength=1,arrowinset=0.25,tbarsize=0.7 5,bracketlength=0.15,rbracketlength=0.15}
\begin{pspicture}(0,0)(33.75,45)
\rput[r](7.5,25){$\AAh$}
\rput(10,0){$\eex$}
\newrgbcolor{userLineColour}{0.6 0.6 0.6}
\psline[linewidth=2,linecolor=userLineColour](30,45)(30,5)
\rput(30,0){$\none$}
\rput[l](33.75,11.25){$\JJh$}
\end{pspicture}


==> PIC/type-string-unit-1.tex <==
%%Created by jPicEdt 1.4.1_03: mixed JPIC-XML/LaTeX format
%%Mon Aug 31 19:09:08 GMT-10:00 2020
%%Begin JPIC-XML
%<?xml version="1.0" standalone="yes"?>
%<jpic x-min="7.5" x-max="33.75" y-min="0" y-max="45" auto-bounding="true">
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(7.5,11.25)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\AAh$
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(10,0)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\eex$
%</text>
%<multicurve fill-style= "none"
%	 stroke-width= "2"
%	 stroke-color= "#ffffff"
%	 points= "(30,45);(30,45);(30,5);(30,5)"
%	 />
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(30,0)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\none$
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(33.75,11.25)"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\JJh$
%</text>
%<multicurve fill-style= "none"
%	 stroke-width= "0.7"
%	 points= "(10,45);(10,45);(10,5);(10,5)"
%	 />
%</jpic>
%%End JPIC-XML
%PSTricks content-type (pstricks.sty package needed)
%Add \usepackage{pstricks} in the preamble of your LaTeX file
%You can rescale the whole picture (to 80% for instance) by using the command \def\JPicScale{0.8}
\ifx\JPicScale\undefined\def\JPicScale{1}\fi
\psset{unit=\JPicScale mm}
\psset{linewidth=0.3,dotsep=1,hatchwidth=0.3,hatchsep=1.5,shadowsize=1,dimen=middle}
\psset{dotsize=0.7 2.5,dotscale=1 1,fillcolor=black}
\psset{arrowsize=1 2,arrowlength=1,arrowinset=0.25,tbarsize=0.7 5,bracketlength=0.15,rbracketlength=0.15}
\begin{pspicture}(0,0)(33.75,45)
\rput[r](7.5,11.25){$\AAh$}
\rput(10,0){$\eex$}
\psline[linewidth=2,linecolor=white](30,45)(30,5)
\rput(30,0){$\none$}
\rput[l](33.75,11.25){$\JJh$}
\psline[linewidth=0.7](10,45)(10,5)
\end{pspicture}


==> PIC/type-string-unit.tex <==
%%Created by jPicEdt 1.4.1_03: mixed JPIC-XML/LaTeX format
%%Tue Sep 01 07:47:56 GMT-10:00 2020
%%Begin JPIC-XML
%<?xml version="1.0" standalone="yes"?>
%<jpic x-min="7.5" x-max="33.75" y-min="0" y-max="45" auto-bounding="true">
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(7.5,11.25)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\AAh$
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(10,0)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\eex$
%</text>
%<multicurve fill-style= "none"
%	 stroke-width= "2"
%	 stroke-color= "#999999"
%	 points= "(30,45);(30,45);(30,5);(30,5)"
%	 />
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(30,0)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\none$
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(33.75,11.25)"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\JJh$
%</text>
%<multicurve fill-style= "none"
%	 stroke-width= "0.7"
%	 points= "(10,45);(10,45);(10,5);(10,5)"
%	 />
%</jpic>
%%End JPIC-XML
%PSTricks content-type (pstricks.sty package needed)
%Add \usepackage{pstricks} in the preamble of your LaTeX file
%You can rescale the whole picture (to 80% for instance) by using the command \def\JPicScale{0.8}
\ifx\JPicScale\undefined\def\JPicScale{1}\fi
\psset{unit=\JPicScale mm}
\psset{linewidth=0.3,dotsep=1,hatchwidth=0.3,hatchsep=1.5,shadowsize=1,dimen=middle}
\psset{dotsize=0.7 2.5,dotscale=1 1,fillcolor=black}
\psset{arrowsize=1 2,arrowlength=1,arrowinset=0.25,tbarsize=0.7 5,bracketlength=0.15,rbracketlength=0.15}
\begin{pspicture}(0,0)(33.75,45)
\rput[r](7.5,11.25){$\AAh$}
\rput(10,0){$\eex$}
\newrgbcolor{userLineColour}{0.6 0.6 0.6}
\psline[linewidth=2,linecolor=userLineColour](30,45)(30,5)
\rput(30,0){$\none$}
\rput[l](33.75,11.25){$\JJh$}
\psline[linewidth=0.7](10,45)(10,5)
\end{pspicture}


==> PIC/type-string.tex <==
%%Created by jPicEdt 1.4.1_03: mixed JPIC-XML/LaTeX format
%%Mon Aug 31 08:08:36 GMT-10:00 2020
%%Begin JPIC-XML
%<?xml version="1.0" standalone="yes"?>
%<jpic x-min="0" x-max="60" y-min="-5" y-max="65" auto-bounding="true">
%<multicurve fill-style= "none"
%	 stroke-overstrike-width= "1.05"
%	 points= "(0,0);(0,10);(0,-5);(0,5);(0,15);(60,45);
%	(60,55);(60,65);(60,60);(60,60);(60,60);(60,60);
%	(60,60);(60,60);(60,60);(60,60)"
%	 stroke-overstrike= "true"
%	 stroke-width= "0.7"
%	 />
%<multicurve fill-style= "none"
%	 stroke-overstrike-width= "0.8"
%	 points= "(20,0);(20,0);(20,60);(20,60)"
%	 stroke-overstrike= "true"
%	 stroke-width= "0.7"
%	 />
%<multicurve fill-style= "none"
%	 stroke-overstrike-width= "1.05"
%	 points= "(40,0);(40,5);(40,0);(40,10);(40,20);(0,40);
%	(0,50);(0,50);(0,60);(0,60);(0,60);(0,60);
%	(0,60);(0,60);(0,60);(0,60)"
%	 stroke-overstrike= "true"
%	 stroke-width= "0.7"
%	 />
%<multicurve fill-style= "none"
%	 stroke-overstrike-width= "1.05"
%	 points= "(60,0);(60,10);(60,5);(60,15);(60,25);(40,35);
%	(40,45);(40,45);(40,60);(40,60);(40,60);(40,60);
%	(40,60);(40,60);(40,60);(40,60)"
%	 stroke-overstrike= "true"
%	 stroke-width= "0.7"
%	 />
%<text text-vert-align= "top"
%	 fill-style= "none"
%	 anchor-point= "(0,-2.5)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\eex$
%</text>
%<text text-vert-align= "top"
%	 fill-style= "none"
%	 anchor-point= "(20,-2.5)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\why$
%</text>
%<text text-vert-align= "top"
%	 fill-style= "none"
%	 anchor-point= "(40,-2.5)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\you$
%</text>
%<text text-vert-align= "top"
%	 fill-style= "none"
%	 anchor-point= "(60,-2.5)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\vea$
%</text>
%<text text-vert-align= "bottom"
%	 fill-style= "none"
%	 anchor-point= "(60,62.5)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\eex$
%</text>
%<text text-vert-align= "bottom"
%	 fill-style= "none"
%	 anchor-point= "(20,62.5)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\why$
%</text>
%<text text-vert-align= "bottom"
%	 fill-style= "none"
%	 anchor-point= "(0,62.5)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\you$
%</text>
%<text text-vert-align= "bottom"
%	 fill-style= "none"
%	 anchor-point= "(40,62.5)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\vea$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(1.88,6.25)"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\Ah$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(21.25,15)"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\Bh$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(34.38,21.25)"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\Ce$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(54.38,28.75)"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\De$
%</text>
%</jpic>
%%End JPIC-XML
%PSTricks content-type (pstricks.sty package needed)
%Add \usepackage{pstricks} in the preamble of your LaTeX file
%You can rescale the whole picture (to 80% for instance) by using the command \def\JPicScale{0.8}
\ifx\JPicScale\undefined\def\JPicScale{1}\fi
\psset{unit=\JPicScale mm}
\psset{linewidth=0.3,dotsep=1,hatchwidth=0.3,hatchsep=1.5,shadowsize=1,dimen=middle}
\psset{dotsize=0.7 2.5,dotscale=1 1,fillcolor=black}
\psset{arrowsize=1 2,arrowlength=1,arrowinset=0.25,tbarsize=0.7 5,bracketlength=0.15,rbracketlength=0.15}
\begin{pspicture}(0,0)(60,65)
\pscustom[linewidth=0.7,border=1.05]{\psbezier(0,0)(0,10)(0,-5)(0,5)
\psbezier(0,15)(60,45)(60,55)
\psbezier(60,65)(60,60)(60,60)
\psbezier(60,60)(60,60)(60,60)
\psbezier(60,60)(60,60)(60,60)
\stroke[linewidth=2.8,linecolor=white]}
\psline[linewidth=0.7,border=0.8](20,0)(20,60)
\pscustom[linewidth=0.7,border=1.05]{\psbezier(40,0)(40,5)(40,0)(40,10)
\psbezier(40,20)(0,40)(0,50)
\psline(0,50)(0,60)
\psbezier(0,60)(0,60)(0,60)
\psbezier(0,60)(0,60)(0,60)
\stroke[linewidth=2.8,linecolor=white]}
\pscustom[linewidth=0.7,border=1.05]{\psbezier(60,0)(60,10)(60,5)(60,15)
\psbezier(60,25)(40,35)(40,45)
\psline(40,45)(40,60)
\psbezier(40,60)(40,60)(40,60)
\psbezier(40,60)(40,60)(40,60)
\stroke[linewidth=2.8,linecolor=white]}
\rput[t](0,-2.5){$\eex$}
\rput[t](20,-2.5){$\why$}
\rput[t](40,-2.5){$\you$}
\rput[t](60,-2.5){$\vea$}
\rput[b](60,62.5){$\eex$}
\rput[b](20,62.5){$\why$}
\rput[b](0,62.5){$\you$}
\rput[b](40,62.5){$\vea$}
\rput[l](1.88,6.25){$\Ah$}
\rput[l](21.25,15){$\Bh$}
\rput[l](34.38,21.25){$\Ce$}
\rput[l](54.38,28.75){$\De$}
\end{pspicture}


==> PIC/uni-eval-f-all.tex <==
%%Created by jPicEdt 1.4.1_03: mixed JPIC-XML/LaTeX format
%%Fri Nov 20 13:55:23 GMT-10:00 2020
%%Begin JPIC-XML
%<?xml version="1.0" standalone="yes"?>
%<jpic x-min="0" x-max="50" y-min="0" y-max="30" auto-bounding="true">
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(43.75,20)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\ahh$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(43.75,0)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\chh$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(46.25,30)"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\Lhh$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(20,15)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\EQLS
%</text>
%<multicurve fill-style= "none"
%	 points= "(30,15);(30,15);(30,5);(30,5)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(30,15);(30,15);(40,5);(40,5)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(30,5);(30,5);(40,5);(40,5)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(30,25);(30,25);(40,15);(40,15)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(40,15);(40,15);(50,15);(50,15)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(50,15);(50,15);(50,25);(50,25)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(50,25);(50,25);(30,25);(30,25)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(45,15);(45,15);(45,0);(45,0)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(35,20);(35,20);(35,10);(35,10)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(45,25);(45,25);(45,30);(45,30)"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(33.75,16.25)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\dh$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(3.75,0)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\chh$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(6.25,30)"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\Lhh$
%</text>
%<multicurve fill-style= "none"
%	 points= "(0,20);(0,20);(0,10);(0,10)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(0,10);(0,10);(10,10);(10,10)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(10,10);(10,10);(10,20);(10,20)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(10,20);(10,20);(0,20);(0,20)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(5,10);(5,10);(5,0);(5,0)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(5,20);(5,20);(5,30);(5,30)"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(5,15)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\fee$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(32.5,8.12)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\Fee$
%</text>
%</jpic>
%%End JPIC-XML
%LaTeX-picture environment using emulated lines and arcs
%You can rescale the whole picture (to 80% for instance) by using the command \def\JPicScale{0.8}
\ifx\JPicScale\undefined\def\JPicScale{1}\fi
\unitlength \JPicScale mm
\begin{picture}(50,30)(0,0)
\put(43.75,20){\makebox(0,0)[cc]{$\ahh$}}

\put(43.75,0){\makebox(0,0)[cr]{$\chh$}}

\put(46.25,30){\makebox(0,0)[cl]{$\Lhh$}}

\put(20,15){\makebox(0,0)[cc]{\EQLS}}

\linethickness{0.3mm}
\put(30,5){\line(0,1){10}}
\linethickness{0.3mm}
\multiput(30,15)(0.12,-0.12){83}{\line(1,0){0.12}}
\linethickness{0.3mm}
\put(30,5){\line(1,0){10}}
\linethickness{0.3mm}
\multiput(30,25)(0.12,-0.12){83}{\line(1,0){0.12}}
\linethickness{0.3mm}
\put(40,15){\line(1,0){10}}
\linethickness{0.3mm}
\put(50,15){\line(0,1){10}}
\linethickness{0.3mm}
\put(30,25){\line(1,0){20}}
\linethickness{0.3mm}
\put(45,0){\line(0,1){15}}
\linethickness{0.3mm}
\put(35,10){\line(0,1){10}}
\linethickness{0.3mm}
\put(45,25){\line(0,1){5}}
\put(33.75,16.25){\makebox(0,0)[cr]{$\dh$}}

\put(3.75,0){\makebox(0,0)[cr]{$\chh$}}

\put(6.25,30){\makebox(0,0)[cl]{$\Lhh$}}

\linethickness{0.3mm}
\put(0,10){\line(0,1){10}}
\linethickness{0.3mm}
\put(0,10){\line(1,0){10}}
\linethickness{0.3mm}
\put(10,10){\line(0,1){10}}
\linethickness{0.3mm}
\put(0,20){\line(1,0){10}}
\linethickness{0.3mm}
\put(5,0){\line(0,1){10}}
\linethickness{0.3mm}
\put(5,20){\line(0,1){10}}
\put(5,15){\makebox(0,0)[cc]{$\fee$}}

\put(32.5,8.12){\makebox(0,0)[cc]{$\Fee$}}

\end{picture}


==> PIC/uni-eval-f.tex <==
%%Created by jPicEdt 1.4.1_03: mixed JPIC-XML/LaTeX format
%%Sun Mar 26 11:52:55 HST 2017
%%Begin JPIC-XML
%<?xml version="1.0" standalone="yes"?>
%<jpic x-min="-3.76" x-max="13.75" y-min="-13.12" y-max="20" auto-bounding="true">
%<text text-vert-align= "center-v"
%	 anchor-point= "(5,20)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\dh$
%</text>
%<multicurve points= "(5,-8.25);(5,-8.25);(5,-1.25);(5,-1.25)"
%	 fill-style= "none"
%	 />
%<multicurve points= "(5,8.75);(5,8.75);(5,15.5);(5,15.5)"
%	 fill-style= "none"
%	 />
%<text text-vert-align= "center-v"
%	 anchor-point= "(5,3.75)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\ahh$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(5,-13.12)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\aah$
%</text>
%<multicurve points= "(-3.76,4.99);(-3.76,4.99);(-3.75,-1.25);(-3.75,-1.25);(-3.75,-1.25);(13.75,-1.26);
%	(13.75,-1.26);(13.75,-1.26);(13.75,8.74);(13.75,8.74);(13.75,8.74);(-3.76,8.74);
%	(-3.76,8.74);(-3.76,8.74);(13.75,8.74);(13.75,8.74);(13.75,8.74);(-3.76,8.74);
%	(-3.76,8.74);(-3.76,8.74);(-3.76,4.99);(-3.76,4.99)"
%	 fill-style= "none"
%	 />
%</jpic>
%%End JPIC-XML
%PSTricks content-type (pstricks.sty package needed)
%Add \usepackage{pstricks} in the preamble of your LaTeX file
%You can rescale the whole picture (to 80% for instance) by using the command \def\JPicScale{0.8}
\ifx\JPicScale\undefined\def\JPicScale{1}\fi
\psset{unit=\JPicScale mm}
\psset{linewidth=0.3,dotsep=1,hatchwidth=0.3,hatchsep=1.5,shadowsize=1,dimen=middle}
\psset{dotsize=0.7 2.5,dotscale=1 1,fillcolor=black}
\psset{arrowsize=1 2,arrowlength=1,arrowinset=0.25,tbarsize=0.7 5,bracketlength=0.15,rbracketlength=0.15}
\begin{pspicture}(0,0)(13.75,20)
\rput(5,20){$\dh$}
\psline(5,-8.25)(5,-1.25)
\psline(5,8.75)(5,15.5)
\rput(5,3.75){$\ahh$}
\rput(5,-13.12){$\aah$}
\psline(-3.76,4.99)
(-3.75,-1.25)
(13.75,-1.26)
(13.75,8.74)
(-3.76,8.74)
(13.75,8.74)
(-3.76,8.74)(-3.76,4.99)
\end{pspicture}


==> PIC/uni-eval-p.tex <==
%%Created by jPicEdt 1.4.1_03: mixed JPIC-XML/LaTeX format
%%Wed Mar 29 07:11:06 HST 2017
%%Begin JPIC-XML
%<?xml version="1.0" standalone="yes"?>
%<jpic x-min="1.88" x-max="23.12" y-min="-12.5" y-max="20" auto-bounding="true">
%<text text-vert-align= "center-v"
%	 anchor-point= "(16.88,20)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\dh$
%</text>
%<multicurve fill-style= "none"
%	 points= "(6.88,-0.62);(6.88,-0.62);(6.88,3.12);(6.88,3.12)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(16.88,8.12);(16.88,8.12);(16.88,15.62);(16.88,15.62)"
%	 />
%<text text-vert-align= "center-v"
%	 anchor-point= "(16.88,3.12)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\ahh$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(5,-2.5)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\aah$
%</text>
%<multicurve fill-style= "none"
%	 points= "(17.5,-8.11);(17.5,-8.11);(17.5,-1.88);(17.5,-1.88)"
%	 />
%<text text-vert-align= "center-v"
%	 anchor-point= "(17.5,-12.5)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\bhh$
%</text>
%<multicurve fill-style= "none"
%	 points= "(1.88,4.36);(1.88,4.36);(11.86,-5.62);(11.86,-5.62);(11.86,-5.62);(1.88,-5.62);
%	(1.88,-5.62);(1.88,-5.62);(1.88,4.36)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(1.88,8.12);(1.88,8.12);(11.88,-1.87);(11.88,-1.87);(11.88,-1.87);(23.12,-1.88);
%	(23.12,-1.88);(23.12,-1.88);(23.12,8.12);(23.12,8.12);(23.12,8.12);(5.62,8.12);
%	(5.62,8.12);(5.62,8.12);(23.12,8.12);(23.12,8.12);(23.12,8.12);(5.62,8.12);
%	(5.62,8.12);(5.62,8.12);(1.88,8.12);(1.88,8.12)"
%	 />
%</jpic>
%%End JPIC-XML
%PSTricks content-type (pstricks.sty package needed)
%Add \usepackage{pstricks} in the preamble of your LaTeX file
%You can rescale the whole picture (to 80% for instance) by using the command \def\JPicScale{0.8}
\ifx\JPicScale\undefined\def\JPicScale{1}\fi
\psset{unit=\JPicScale mm}
\psset{linewidth=0.3,dotsep=1,hatchwidth=0.3,hatchsep=1.5,shadowsize=1,dimen=middle}
\psset{dotsize=0.7 2.5,dotscale=1 1,fillcolor=black}
\psset{arrowsize=1 2,arrowlength=1,arrowinset=0.25,tbarsize=0.7 5,bracketlength=0.15,rbracketlength=0.15}
\begin{pspicture}(0,0)(23.12,20)
\rput(16.88,20){$\dh$}
\psline(6.88,-0.62)(6.88,3.12)
\psline(16.88,8.12)(16.88,15.62)
\rput(16.88,3.12){$\ahh$}
\rput(5,-2.5){$\aah$}
\psline(17.5,-8.11)(17.5,-1.88)
\rput(17.5,-12.5){$\bhh$}
\pspolygon(1.88,4.36)
(11.86,-5.62)
(1.88,-5.62)(1.88,4.36)
\psline(1.88,8.12)
(11.88,-1.87)
(23.12,-1.88)
(23.12,8.12)
(5.62,8.12)
(23.12,8.12)
(5.62,8.12)(1.88,8.12)
\end{pspicture}


==> PIC/uni-eval-s-all.tex <==
%%Created by jPicEdt 1.4.1_03: mixed JPIC-XML/LaTeX format
%%Fri Nov 20 13:56:37 GMT-10:00 2020
%%Begin JPIC-XML
%<?xml version="1.0" standalone="yes"?>
%<jpic x-min="0" x-max="80" y-min="0" y-max="30" auto-bounding="true">
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(63.75,0)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\bhh$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(73.75,20)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\ahh$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(60,10)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\shh$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(73.75,0)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\chh$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(53.75,0)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\dh$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(76.25,30)"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\Lhh$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(40,15)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\EQLS
%</text>
%<multicurve fill-style= "none"
%	 points= "(50,15);(50,15);(60,5);(60,5)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(60,15);(60,15);(70,5);(70,5)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(50,15);(50,15);(60,15);(60,15)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(60,5);(60,5);(70,5);(70,5)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(60,25);(60,25);(70,15);(70,15)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(70,15);(70,15);(80,15);(80,15)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(80,15);(80,15);(80,25);(80,25)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(80,25);(80,25);(60,25);(60,25)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(65,5);(65,5);(65,0);(65,0)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(75,15);(75,15);(75,0);(75,0)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(55,10);(55,10);(55,0);(55,0)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(65,20);(65,20);(65,10);(65,10)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(75,25);(75,25);(75,30);(75,30)"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(63.75,16.25)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\dh$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(13.75,0)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\bhh$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(20,15)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\ahh$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(23.75,0)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\chh$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(3.75,0)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\dh$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(21.25,30)"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\Lhh$
%</text>
%<multicurve fill-style= "none"
%	 points= "(0,20);(0,20);(10,10);(10,10)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(10,10);(10,10);(30,10);(30,10)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(30,10);(30,10);(30,20);(30,20)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(30,20);(30,20);(0,20);(0,20)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(15,10);(15,10);(15,0);(15,0)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(25,10);(25,10);(25,0);(25,0)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(5,15);(5,15);(5,0);(5,0)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(20,20);(20,20);(20,30);(20,30)"
%	 />
%</jpic>
%%End JPIC-XML
%LaTeX-picture environment using emulated lines and arcs
%You can rescale the whole picture (to 80% for instance) by using the command \def\JPicScale{0.8}
\ifx\JPicScale\undefined\def\JPicScale{1}\fi
\unitlength \JPicScale mm
\begin{picture}(80,30)(0,0)
\put(63.75,0){\makebox(0,0)[cr]{$\bhh$}}

\put(73.75,20){\makebox(0,0)[cc]{$\ahh$}}

\put(60,10){\makebox(0,0)[cc]{$\shh$}}

\put(73.75,0){\makebox(0,0)[cr]{$\chh$}}

\put(53.75,0){\makebox(0,0)[cr]{$\dh$}}

\put(76.25,30){\makebox(0,0)[cl]{$\Lhh$}}

\put(40,15){\makebox(0,0)[cc]{\EQLS}}

\linethickness{0.3mm}
\multiput(50,15)(0.12,-0.12){83}{\line(1,0){0.12}}
\linethickness{0.3mm}
\multiput(60,15)(0.12,-0.12){83}{\line(1,0){0.12}}
\linethickness{0.3mm}
\put(50,15){\line(1,0){10}}
\linethickness{0.3mm}
\put(60,5){\line(1,0){10}}
\linethickness{0.3mm}
\multiput(60,25)(0.12,-0.12){83}{\line(1,0){0.12}}
\linethickness{0.3mm}
\put(70,15){\line(1,0){10}}
\linethickness{0.3mm}
\put(80,15){\line(0,1){10}}
\linethickness{0.3mm}
\put(60,25){\line(1,0){20}}
\linethickness{0.3mm}
\put(65,0){\line(0,1){5}}
\linethickness{0.3mm}
\put(75,0){\line(0,1){15}}
\linethickness{0.3mm}
\put(55,0){\line(0,1){10}}
\linethickness{0.3mm}
\put(65,10){\line(0,1){10}}
\linethickness{0.3mm}
\put(75,25){\line(0,1){5}}
\put(63.75,16.25){\makebox(0,0)[cr]{$\dh$}}

\put(13.75,0){\makebox(0,0)[cr]{$\bhh$}}

\put(20,15){\makebox(0,0)[cc]{$\ahh$}}

\put(23.75,0){\makebox(0,0)[cr]{$\chh$}}

\put(3.75,0){\makebox(0,0)[cr]{$\dh$}}

\put(21.25,30){\makebox(0,0)[cl]{$\Lhh$}}

\linethickness{0.3mm}
\multiput(0,20)(0.12,-0.12){83}{\line(1,0){0.12}}
\linethickness{0.3mm}
\put(10,10){\line(1,0){20}}
\linethickness{0.3mm}
\put(30,10){\line(0,1){10}}
\linethickness{0.3mm}
\put(0,20){\line(1,0){30}}
\linethickness{0.3mm}
\put(15,0){\line(0,1){10}}
\linethickness{0.3mm}
\put(25,0){\line(0,1){10}}
\linethickness{0.3mm}
\put(5,0){\line(0,1){15}}
\linethickness{0.3mm}
\put(20,20){\line(0,1){10}}
\end{picture}


==> PIC/uni-eval-s.tex <==
%%Created by jPicEdt 1.4.1_03: mixed JPIC-XML/LaTeX format
%%Wed Mar 29 07:12:36 HST 2017
%%Begin JPIC-XML
%<?xml version="1.0" standalone="yes"?>
%<jpic x-min="-2.5" x-max="30.01" y-min="-15.62" y-max="13.12" auto-bounding="true">
%<multicurve fill-style= "none"
%	 points= "(2.5,-11.88);(2.5,-11.88);(2.5,-3.1);(2.5,-3.1)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(18.13,-2.5);(18.13,-2.5);(18.13,1.25);(18.13,1.25)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(15,-11.88);(15,-11.88);(15,-7.5);(15,-7.5)"
%	 />
%<text text-vert-align= "center-v"
%	 anchor-point= "(15,-15.62)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\bhh$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(24.37,1.25)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\ahh$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(11.25,-3.12)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\shh$
%</text>
%<multicurve fill-style= "none"
%	 points= "(26.87,-12.5);(26.87,-12.5);(26.87,-3.75);(26.87,-3.75)"
%	 />
%<text text-vert-align= "center-v"
%	 anchor-point= "(26.87,-15.62)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\chh$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(2.5,-15.62)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\dh$
%</text>
%<multicurve fill-style= "none"
%	 points= "(26.87,5.62);(26.87,5.62);(26.87,10.62);(26.87,10.62)"
%	 />
%<text text-vert-align= "center-v"
%	 anchor-point= "(26.87,13.12)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\Lhh$
%</text>
%<multicurve fill-style= "none"
%	 points= "(13.76,5.62);(13.76,5.62);(23.13,-3.75);(23.13,-3.75);(23.13,-3.75);(30.01,-3.75);
%	(30.01,-3.75);(30.01,-3.75);(30.01,5.62);(30.01,5.62);(30.01,5.62);(26.87,5.62);
%	(26.87,5.62);(26.87,5.62);(16.87,5.62);(16.87,5.62);(16.87,5.62);(15,5.62);
%	(15,5.62);(15,5.62);(13.76,5.62);(13.76,5.62)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(-2.5,1.88);(-2.5,1.88);(6.88,-7.5);(6.88,-7.5);(6.88,-7.5);(23.13,-7.5);
%	(23.13,-7.5);(23.13,-7.5);(16.86,-1.25);(16.86,-1.25);(16.86,-1.25);(13.74,1.88);
%	(13.74,1.88);(13.74,1.88);(-2.5,1.88);(-2.5,1.88);(-2.5,1.88);(-1.25,1.88);
%	(-1.25,1.88);(-1.25,1.88);(-1.25,1.88);(-1.25,1.88)"
%	 />
%</jpic>
%%End JPIC-XML
%PSTricks content-type (pstricks.sty package needed)
%Add \usepackage{pstricks} in the preamble of your LaTeX file
%You can rescale the whole picture (to 80% for instance) by using the command \def\JPicScale{0.8}
\ifx\JPicScale\undefined\def\JPicScale{1}\fi
\psset{unit=\JPicScale mm}
\psset{linewidth=0.3,dotsep=1,hatchwidth=0.3,hatchsep=1.5,shadowsize=1,dimen=middle}
\psset{dotsize=0.7 2.5,dotscale=1 1,fillcolor=black}
\psset{arrowsize=1 2,arrowlength=1,arrowinset=0.25,tbarsize=0.7 5,bracketlength=0.15,rbracketlength=0.15}
\begin{pspicture}(0,0)(30.01,13.12)
\psline(2.5,-11.88)(2.5,-3.1)
\psline(18.13,-2.5)(18.13,1.25)
\psline(15,-11.88)(15,-7.5)
\rput(15,-15.62){$\bhh$}
\rput(24.37,1.25){$\ahh$}
\rput(11.25,-3.12){$\shh$}
\psline(26.87,-12.5)(26.87,-3.75)
\rput(26.87,-15.62){$\chh$}
\rput(2.5,-15.62){$\dh$}
\psline(26.87,5.62)(26.87,10.62)
\rput(26.87,13.12){$\Lhh$}
\psline(13.76,5.62)
(23.13,-3.75)
(30.01,-3.75)
(30.01,5.62)
(26.87,5.62)
(16.87,5.62)
(15,5.62)(13.76,5.62)
\pscustom[]{\psline(-2.5,1.88)(6.88,-7.5)
\psline(6.88,-7.5)(23.13,-7.5)
\psline(23.13,-7.5)(16.86,-1.25)
\psline(16.86,-1.25)(13.74,1.88)
\psline(13.74,1.88)(-2.5,1.88)
\psline(-2.5,1.88)(-1.25,1.88)
\psbezier(-1.25,1.88)(-1.25,1.88)(-1.25,1.88)
}
\end{pspicture}


==> PIC/uni-eval-uMN.tex <==
%%Created by jPicEdt 1.4.1_03: mixed JPIC-XML/LaTeX format
%%Wed Mar 29 07:12:15 HST 2017
%%Begin JPIC-XML
%<?xml version="1.0" standalone="yes"?>
%<jpic x-min="-0.62" x-max="25.62" y-min="-11.25" y-max="14.38" auto-bounding="true">
%<text text-vert-align= "center-v"
%	 anchor-point= "(4.38,-11.25)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\dh$
%</text>
%<multicurve fill-style= "none"
%	 points= "(3.75,-7.5);(3.75,-7.5);(3.75,1.88);(3.75,1.88)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(14.38,-7.5);(14.38,-7.5);(14.38,-3.12);(14.38,-3.12)"
%	 />
%<text text-vert-align= "center-v"
%	 anchor-point= "(14.38,-11.25)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\bhh$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(16.25,1.88)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\ahh$
%</text>
%<multicurve fill-style= "none"
%	 points= "(21.25,-7.5);(21.25,-7.5);(21.25,-3.12);(21.25,-3.12)"
%	 />
%<text text-vert-align= "center-v"
%	 anchor-point= "(21.25,-11.25)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\chh$
%</text>
%<multicurve fill-style= "none"
%	 points= "(15.62,6.24);(15.62,6.24);(15.62,11.25);(15.62,11.25)"
%	 />
%<text text-vert-align= "center-v"
%	 anchor-point= "(15.62,14.38)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\Lhh$
%</text>
%<multicurve fill-style= "none"
%	 points= "(-0.62,6.25);(-0.62,6.25);(8.75,-3.12);(8.75,-3.12);(8.75,-3.12);(25.62,-3.12);
%	(25.62,-3.12);(25.62,-3.12);(25.62,6.25);(25.62,6.25);(25.62,6.25);(5.62,6.26);
%	(5.62,6.26);(5.62,6.26);(3.12,6.26);(3.12,6.26);(3.12,6.26);(1.25,6.25);
%	(1.25,6.25);(1.25,6.25);(-0.62,6.25);(-0.62,6.25)"
%	 />
%</jpic>
%%End JPIC-XML
%PSTricks content-type (pstricks.sty package needed)
%Add \usepackage{pstricks} in the preamble of your LaTeX file
%You can rescale the whole picture (to 80% for instance) by using the command \def\JPicScale{0.8}
\ifx\JPicScale\undefined\def\JPicScale{1}\fi
\psset{unit=\JPicScale mm}
\psset{linewidth=0.3,dotsep=1,hatchwidth=0.3,hatchsep=1.5,shadowsize=1,dimen=middle}
\psset{dotsize=0.7 2.5,dotscale=1 1,fillcolor=black}
\psset{arrowsize=1 2,arrowlength=1,arrowinset=0.25,tbarsize=0.7 5,bracketlength=0.15,rbracketlength=0.15}
\begin{pspicture}(0,0)(25.62,14.38)
\rput(4.38,-11.25){$\dh$}
\psline(3.75,-7.5)(3.75,1.88)
\psline(14.38,-7.5)(14.38,-3.12)
\rput(14.38,-11.25){$\bhh$}
\rput(16.25,1.88){$\ahh$}
\psline(21.25,-7.5)(21.25,-3.12)
\rput(21.25,-11.25){$\chh$}
\psline(15.62,6.24)(15.62,11.25)
\rput(15.62,14.38){$\Lhh$}
\psline(-0.62,6.25)
(8.75,-3.12)
(25.62,-3.12)
(25.62,6.25)
(5.62,6.26)
(3.12,6.26)
(1.25,6.25)(-0.62,6.25)
\end{pspicture}


==> PIC/uni-fun-ft-1.tex <==
%%Created by jPicEdt 1.4.1_03: mixed JPIC-XML/LaTeX format
%%Sat Nov 07 14:30:25 GMT-10:00 2020
%%Begin JPIC-XML
%<?xml version="1.0" standalone="yes"?>
%<jpic x-min="1.88" x-max="60" y-min="1.25" y-max="45.62" auto-bounding="true">
%<multicurve fill-style= "none"
%	 points= "(6.88,10.62);(6.88,10.62);(6.88,21.87);(6.88,21.87)"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(13.12,22.5)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\ahh$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(5,8.75)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\aah$
%</text>
%<multicurve fill-style= "none"
%	 points= "(16.25,1.88);(16.25,1.88);(16.25,16.88);(16.25,16.88)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(1.88,15.61);(1.88,15.61);(11.86,5.63);(11.86,5.63);(11.86,5.63);(1.88,5.63);
%	(1.88,5.63);(1.88,5.63);(1.88,15.61)"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(6.25,18.12)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\RRsmall$
%</text>
%<multicurve fill-style= "none"
%	 points= "(11.88,16.87);(11.88,16.87);(1.88,26.88);(1.88,26.88)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(21.25,16.88);(21.25,16.88);(11.88,16.88);(11.88,16.88)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(45,2.5);(45,2.5);(45,16.88);(45,16.88)"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(31.25,22.5)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\EQLS
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(50.62,21.88)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\bhh$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(15,1.25)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\ah$
%</text>
%<multicurve fill-style= "none"
%	 points= "(21.25,26.88);(21.25,26.88);(21.25,16.88);(21.25,16.88)"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(17.5,45)"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\dh$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(51.26,45)"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\dh$
%</text>
%<multicurve fill-style= "none"
%	 points= "(21.25,26.88);(21.25,26.88);(1.88,26.88);(1.88,26.88)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(40,26.88);(40,26.88);(40,16.88);(40,16.88);(40,16.88);(60,16.9);
%	(60,16.9);(60,16.9);(60,26.9);(60,26.9);(60,26.9);(60,26.9);
%	(60,26.9);(60,26.9);(56.25,26.88);(56.25,26.88);(56.25,26.88);(40,26.88);
%	(40,26.88);(40,26.88);(49.37,26.9);(49.37,26.9)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(55,2.5);(55,2.5);(55,16.88);(55,16.88)"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(53.76,1.25)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\ah$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(43.75,1.25)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\xh$
%</text>
%<multicurve fill-style= "none"
%	 points= "(6.87,2.5);(6.87,2.5);(6.88,5.62);(6.88,5.62)"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(5.62,1.25)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\xh$
%</text>
%<multicurve fill-style= "none"
%	 points= "(16.25,26.88);(16.25,26.88);(16.25,45.62);(16.25,45.62)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(50,26.88);(50,26.88);(50,45.62);(50,45.62)"
%	 />
%</jpic>
%%End JPIC-XML
%LaTeX-picture environment using emulated lines and arcs
%You can rescale the whole picture (to 80% for instance) by using the command \def\JPicScale{0.8}
\ifx\JPicScale\undefined\def\JPicScale{1}\fi
\unitlength \JPicScale mm
\begin{picture}(60,45.62)(0,0)
\linethickness{0.3mm}
\put(6.88,10.62){\line(0,1){11.25}}
\put(13.12,22.5){\makebox(0,0)[cc]{$\ahh$}}

\put(5,8.75){\makebox(0,0)[cc]{$\aah$}}

\linethickness{0.3mm}
\put(16.25,1.88){\line(0,1){15}}
\linethickness{0.3mm}
\multiput(1.88,15.61)(0.12,-0.12){83}{\line(1,0){0.12}}
\put(1.88,5.63){\line(1,0){9.98}}
\put(1.88,5.63){\line(0,1){9.98}}
\put(6.25,18.12){\makebox(0,0)[cr]{$\RRsmall$}}

\linethickness{0.3mm}
\multiput(1.88,26.88)(0.12,-0.12){83}{\line(0,-1){0.12}}
\linethickness{0.3mm}
\put(11.88,16.88){\line(1,0){9.37}}
\linethickness{0.3mm}
\put(45,2.5){\line(0,1){14.38}}
\put(31.25,22.5){\makebox(0,0)[cc]{\EQLS}}

\put(50.62,21.88){\makebox(0,0)[cc]{$\bhh$}}

\put(15,1.25){\makebox(0,0)[cr]{$\ah$}}

\linethickness{0.3mm}
\put(21.25,16.88){\line(0,1){10}}
\put(17.5,45){\makebox(0,0)[cl]{$\dh$}}

\put(51.26,45){\makebox(0,0)[cl]{$\dh$}}

\linethickness{0.3mm}
\put(1.88,26.88){\line(1,0){19.37}}
\linethickness{0.3mm}
\put(40,16.88){\line(0,1){10}}
\put(40,16.88){\line(1,0){20}}
\put(60,16.9){\line(0,1){10}}
\qbezier(60,26.9)(60,26.9)(60,26.9)
\qbezier(60,26.9)(60,26.9)(60,26.9)
\multiput(56.25,26.88)(3.75,0.02){1}{\line(1,0){3.75}}
\put(40,26.88){\line(1,0){16.25}}
\multiput(40,26.88)(9.37,0.02){1}{\line(1,0){9.37}}
\linethickness{0.3mm}
\put(55,2.5){\line(0,1){14.38}}
\put(53.76,1.25){\makebox(0,0)[cr]{$\ah$}}

\put(43.75,1.25){\makebox(0,0)[cr]{$\xh$}}

\linethickness{0.3mm}
\multiput(6.87,2.5)(0.01,3.12){1}{\line(0,1){3.12}}
\put(5.62,1.25){\makebox(0,0)[cr]{$\xh$}}

\linethickness{0.3mm}
\put(16.25,26.88){\line(0,1){18.75}}
\linethickness{0.3mm}
\put(50,26.88){\line(0,1){18.75}}
\end{picture}


==> PIC/uni-fun-ft-2.tex <==
%%Created by jPicEdt 1.4.1_03: mixed JPIC-XML/LaTeX format
%%Sat Nov 07 14:31:59 GMT-10:00 2020
%%Begin JPIC-XML
%<?xml version="1.0" standalone="yes"?>
%<jpic x-min="40" x-max="60" y-min="1.25" y-max="45.62" auto-bounding="true">
%<multicurve fill-style= "none"
%	 points= "(45,2.5);(45,2.5);(45,16.88);(45,16.88)"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(50.62,21.88)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\bhh$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(51.26,45)"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\dh$
%</text>
%<multicurve fill-style= "none"
%	 points= "(40,26.88);(40,26.88);(40,16.88);(40,16.88);(40,16.88);(60,16.9);
%	(60,16.9);(60,16.9);(60,26.9);(60,26.9);(60,26.9);(60,26.9);
%	(60,26.9);(60,26.9);(56.25,26.88);(56.25,26.88);(56.25,26.88);(40,26.88);
%	(40,26.88);(40,26.88);(49.37,26.9);(49.37,26.9)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(55,2.5);(55,2.5);(55,16.88);(55,16.88)"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(53.76,1.25)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\ah$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(43.75,1.25)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\xh$
%</text>
%<multicurve fill-style= "none"
%	 points= "(50,26.88);(50,26.88);(50,45.62);(50,45.62)"
%	 />
%</jpic>
%%End JPIC-XML
%LaTeX-picture environment using emulated lines and arcs
%You can rescale the whole picture (to 80% for instance) by using the command \def\JPicScale{0.8}
\ifx\JPicScale\undefined\def\JPicScale{1}\fi
\unitlength \JPicScale mm
\begin{picture}(60,45.62)(0,0)
\linethickness{0.3mm}
\put(45,2.5){\line(0,1){14.38}}
\put(50.62,21.88){\makebox(0,0)[cc]{$\bhh$}}

\put(51.26,45){\makebox(0,0)[cl]{$\dh$}}

\linethickness{0.3mm}
\put(40,16.88){\line(0,1){10}}
\put(40,16.88){\line(1,0){20}}
\put(60,16.9){\line(0,1){10}}
\qbezier(60,26.9)(60,26.9)(60,26.9)
\qbezier(60,26.9)(60,26.9)(60,26.9)
\multiput(56.25,26.88)(3.75,0.02){1}{\line(1,0){3.75}}
\put(40,26.88){\line(1,0){16.25}}
\multiput(40,26.88)(9.37,0.02){1}{\line(1,0){9.37}}
\linethickness{0.3mm}
\put(55,2.5){\line(0,1){14.38}}
\put(53.76,1.25){\makebox(0,0)[cr]{$\ah$}}

\put(43.75,1.25){\makebox(0,0)[cr]{$\xh$}}

\linethickness{0.3mm}
\put(50,26.88){\line(0,1){18.75}}
\end{picture}


==> PIC/uni-fun-ft-3.tex <==
%%Created by jPicEdt 1.4.1_03: mixed JPIC-XML/LaTeX format
%%Sat Nov 07 14:33:21 GMT-10:00 2020
%%Begin JPIC-XML
%<?xml version="1.0" standalone="yes"?>
%<jpic x-min="1.88" x-max="21.25" y-min="1.25" y-max="45.62" auto-bounding="true">
%<multicurve fill-style= "none"
%	 points= "(6.88,10.62);(6.88,10.62);(6.88,21.87);(6.88,21.87)"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(13.12,22.5)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\ahh$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(5,8.75)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\aah$
%</text>
%<multicurve fill-style= "none"
%	 points= "(16.25,1.88);(16.25,1.88);(16.25,16.88);(16.25,16.88)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(1.88,15.61);(1.88,15.61);(11.86,5.63);(11.86,5.63);(11.86,5.63);(1.88,5.63);
%	(1.88,5.63);(1.88,5.63);(1.88,15.61)"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(6.25,18.12)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\RRsmall$
%</text>
%<multicurve fill-style= "none"
%	 points= "(11.88,16.87);(11.88,16.87);(1.88,26.88);(1.88,26.88)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(21.25,16.88);(21.25,16.88);(11.88,16.88);(11.88,16.88)"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(15,1.25)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\ah$
%</text>
%<multicurve fill-style= "none"
%	 points= "(21.25,26.88);(21.25,26.88);(21.25,16.88);(21.25,16.88)"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(17.5,45)"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\dh$
%</text>
%<multicurve fill-style= "none"
%	 points= "(21.25,26.88);(21.25,26.88);(1.88,26.88);(1.88,26.88)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(6.87,2.5);(6.87,2.5);(6.88,5.62);(6.88,5.62)"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(5.62,1.25)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\xh$
%</text>
%<multicurve fill-style= "none"
%	 points= "(16.25,26.88);(16.25,26.88);(16.25,45.62);(16.25,45.62)"
%	 />
%</jpic>
%%End JPIC-XML
%LaTeX-picture environment using emulated lines and arcs
%You can rescale the whole picture (to 80% for instance) by using the command \def\JPicScale{0.8}
\ifx\JPicScale\undefined\def\JPicScale{1}\fi
\unitlength \JPicScale mm
\begin{picture}(21.25,45.62)(0,0)
\linethickness{0.3mm}
\put(6.88,10.62){\line(0,1){11.25}}
\put(13.12,22.5){\makebox(0,0)[cc]{$\ahh$}}

\put(5,8.75){\makebox(0,0)[cc]{$\aah$}}

\linethickness{0.3mm}
\put(16.25,1.88){\line(0,1){15}}
\linethickness{0.3mm}
\multiput(1.88,15.61)(0.12,-0.12){83}{\line(1,0){0.12}}
\put(1.88,5.63){\line(1,0){9.98}}
\put(1.88,5.63){\line(0,1){9.98}}
\put(6.25,18.12){\makebox(0,0)[cr]{$\RRsmall$}}

\linethickness{0.3mm}
\multiput(1.88,26.88)(0.12,-0.12){83}{\line(0,-1){0.12}}
\linethickness{0.3mm}
\put(11.88,16.88){\line(1,0){9.37}}
\put(15,1.25){\makebox(0,0)[cr]{$\ah$}}

\linethickness{0.3mm}
\put(21.25,16.88){\line(0,1){10}}
\put(17.5,45){\makebox(0,0)[cl]{$\dh$}}

\linethickness{0.3mm}
\put(1.88,26.88){\line(1,0){19.37}}
\linethickness{0.3mm}
\multiput(6.87,2.5)(0.01,3.12){1}{\line(0,1){3.12}}
\put(5.62,1.25){\makebox(0,0)[cr]{$\xh$}}

\linethickness{0.3mm}
\put(16.25,26.88){\line(0,1){18.74}}
\end{picture}


==> PIC/uni-fun-ft.tex <==
%%Created by jPicEdt 1.4.1_03: mixed JPIC-XML/LaTeX format
%%Sat Nov 07 14:50:23 GMT-10:00 2020
%%Begin JPIC-XML
%<?xml version="1.0" standalone="yes"?>
%<jpic x-min="1.88" x-max="60" y-min="1.25" y-max="45" auto-bounding="true">
%<multicurve fill-style= "none"
%	 points= "(6.88,10.62);(6.88,10.62);(6.88,21.87);(6.88,21.87)"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(13.12,22.5)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\ahh$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(5,8.75)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\aah$
%</text>
%<multicurve fill-style= "none"
%	 points= "(16.25,1.88);(16.25,1.88);(16.25,16.88);(16.25,16.88)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(1.88,15.61);(1.88,15.61);(11.86,5.63);(11.86,5.63);(11.86,5.63);(1.88,5.63);
%	(1.88,5.63);(1.88,5.63);(1.88,15.61)"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(6.25,18.12)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\RRsmall$
%</text>
%<multicurve fill-style= "none"
%	 points= "(11.88,16.87);(11.88,16.87);(1.88,26.88);(1.88,26.88)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(21.25,16.88);(21.25,16.88);(11.88,16.88);(11.88,16.88)"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(31.25,22.5)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\EQLS
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(15,1.25)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\ah$
%</text>
%<multicurve fill-style= "none"
%	 points= "(21.25,26.88);(21.25,26.88);(21.25,16.88);(21.25,16.88)"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(17.5,45)"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\dh$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(51.26,45)"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\dh$
%</text>
%<multicurve fill-style= "none"
%	 points= "(21.25,26.88);(21.25,26.88);(1.88,26.88);(1.88,26.88)"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(53.76,1.25)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\ah$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(43.75,1.25)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\xh$
%</text>
%<multicurve fill-style= "none"
%	 points= "(6.87,2.5);(6.87,2.5);(6.88,5.62);(6.88,5.62)"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(5.62,1.25)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\xh$
%</text>
%<multicurve fill-style= "none"
%	 points= "(45,2.5);(45,2.5);(45,16.88);(45,16.88)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(55,1.88);(55,1.88);(55,16.88);(55,16.88)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(40,16.88);(40,16.88);(40,26.88);(40,26.88)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(60,16.88);(60,16.88);(40,16.88);(40,16.88)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(60,26.88);(60,26.88);(60,16.88);(60,16.88)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(60,26.88);(60,26.88);(40,26.88);(40,26.88)"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(50,21.88)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\bhh$
%</text>
%<multicurve fill-style= "none"
%	 points= "(50,26.88);(50,26.88);(50,44.38);(50,44.38)"
%	 stroke-color= "#ff33cc"
%	 />
%<multicurve fill-style= "none"
%	 points= "(16.25,26.88);(16.25,26.88);(16.25,44.38);(16.25,44.38)"
%	 />
%</jpic>
%%End JPIC-XML
%LaTeX-picture environment using emulated lines and arcs
%You can rescale the whole picture (to 80% for instance) by using the command \def\JPicScale{0.8}
\ifx\JPicScale\undefined\def\JPicScale{1}\fi
\unitlength \JPicScale mm
\begin{picture}(60,45)(0,0)
\linethickness{0.3mm}
\put(6.88,10.62){\line(0,1){11.25}}
\put(13.12,22.5){\makebox(0,0)[cc]{$\ahh$}}

\put(5,8.75){\makebox(0,0)[cc]{$\aah$}}

\linethickness{0.3mm}
\put(16.25,1.88){\line(0,1){15}}
\linethickness{0.3mm}
\multiput(1.88,15.61)(0.12,-0.12){83}{\line(1,0){0.12}}
\put(1.88,5.63){\line(1,0){9.98}}
\put(1.88,5.63){\line(0,1){9.98}}
\put(6.25,18.12){\makebox(0,0)[cr]{$\RRsmall$}}

\linethickness{0.3mm}
\multiput(1.88,26.88)(0.12,-0.12){83}{\line(0,-1){0.12}}
\linethickness{0.3mm}
\put(11.88,16.88){\line(1,0){9.37}}
\put(31.25,22.5){\makebox(0,0)[cc]{\EQLS}}

\put(15,1.25){\makebox(0,0)[cr]{$\ah$}}

\linethickness{0.3mm}
\put(21.25,16.88){\line(0,1){10}}
\put(17.5,45){\makebox(0,0)[cl]{$\dh$}}

\put(51.26,45){\makebox(0,0)[cl]{$\dh$}}

\linethickness{0.3mm}
\put(1.88,26.88){\line(1,0){19.37}}
\put(53.76,1.25){\makebox(0,0)[cr]{$\ah$}}

\put(43.75,1.25){\makebox(0,0)[cr]{$\xh$}}

\linethickness{0.3mm}
\multiput(6.87,2.5)(0.01,3.12){1}{\line(0,1){3.12}}
\put(5.62,1.25){\makebox(0,0)[cr]{$\xh$}}

\linethickness{0.3mm}
\put(45,2.5){\line(0,1){14.38}}
\linethickness{0.3mm}
\put(55,1.88){\line(0,1){15}}
\linethickness{0.3mm}
\put(40,16.88){\line(0,1){10}}
\linethickness{0.3mm}
\put(40,16.88){\line(1,0){20}}
\linethickness{0.3mm}
\put(60,16.88){\line(0,1){10}}
\linethickness{0.3mm}
\put(40,26.88){\line(1,0){20}}
\put(50,21.88){\makebox(0,0)[cc]{$\bhh$}}

\linethickness{0.3mm}
\put(50,26.88){\line(0,1){17.5}}
\linethickness{0.3mm}
\put(16.25,26.88){\line(0,1){17.5}}
\end{picture}


==> PIC/uni-idem-cons.tex <==
%%Created by jPicEdt 1.4.1_03: mixed JPIC-XML/LaTeX format
%%Tue Jan 03 19:24:14 GMT-10:00 2023
%%Begin JPIC-XML
%<?xml version="1.0" standalone="yes"?>
%<jpic x-min="-5" x-max="165" y-min="0" y-max="95" auto-bounding="true">
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(5,0)"
%	 text-frame= "noframe"
%	 stroke-width= "0.35"
%	 text-hor-align= "right"
%	 >
%$\Progtype$
%</text>
%<multicurve fill-style= "none"
%	 points= "(60,60);(60,60);(60,35);(60,35)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(60,35);(60,35);(20,35);(20,35)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(20,35);(20,35);(-5,60);(-5,60)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(-5,60);(-5,60);(60,60);(60,60)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(7.5,47.5);(7.5,47.5);(7.5,0);(7.5,0)"
%	 stroke-width= "1"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(110,27.5)"
%	 text-frame= "noframe"
%	 stroke-width= "0.35"
%	 text-hor-align= "center-h"
%	 >
%\program
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(80,47.5)"
%	 text-frame= "noframe"
%	 stroke-width= "0.35"
%	 text-hor-align= "center-h"
%	 >
%$\eqlsb$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(145,47.5)"
%	 text-frame= "noframe"
%	 stroke-width= "0.35"
%	 text-hor-align= "center-h"
%	 >
%$\universal$
%</text>
%<multicurve fill-style= "none"
%	 points= "(165,60);(165,60);(165,35);(165,35)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(165,35);(165,35);(125,35);(125,35)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(100,45);(100,45);(100,20);(100,20)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(100,60);(100,60);(165,60);(165,60)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(111.25,20);(111.25,20);(111.25,0);(111.25,0)"
%	 stroke-width= "1"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(107.5,0)"
%	 text-frame= "noframe"
%	 stroke-width= "0.35"
%	 text-hor-align= "right"
%	 >
%$\Progtype$
%</text>
%<multicurve fill-style= "none"
%	 points= "(125,20);(125,20);(100,20);(100,20)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(125,20);(125,20);(100,45);(100,45)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(125,35);(125,35);(100,60);(100,60)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(111.25,48.75);(111.25,48.75);(111.25,33.75);(111.25,33.75)"
%	 stroke-width= "1"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(111.25,33.75)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\Dottt
%</text>
%<multicurve fill-style= "none"
%	 points= "(145,35);(145,35);(145,0);(145,0)"
%	 stroke-width= "1"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(141.25,0)"
%	 text-frame= "noframe"
%	 stroke-width= "0.35"
%	 text-hor-align= "right"
%	 >
%$\Progtype$
%</text>
%<multicurve fill-style= "none"
%	 points= "(145,95);(145,95);(145,60);(145,60)"
%	 stroke-width= "1"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(147.5,93.75)"
%	 text-frame= "noframe"
%	 stroke-width= "0.35"
%	 text-hor-align= "left"
%	 >
%$\Progtype$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(40,47.5)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\Big\{\Big\}^B_A$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(47.5,65)"
%	 text-frame= "noframe"
%	 stroke-width= "0.35"
%	 text-hor-align= "left"
%	 >
%$\Progk$
%</text>
%<multicurve fill-style= "none"
%	 points= "(45,35);(45,35);(45,25);(45,25)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(55,25);(55,25);(35,25);(35,25)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(55,25);(55,25);(55,5);(55,5)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(35,25);(35,25);(55,5);(55,5)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(45,15);(45,15);(45,0);(45,0)"
%	 stroke-width= "1"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(42.5,0)"
%	 text-frame= "noframe"
%	 stroke-width= "0.35"
%	 text-hor-align= "right"
%	 >
%$\Progtype$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(48.75,18.75)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\decok$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(42.5,30)"
%	 text-frame= "noframe"
%	 stroke-width= "0.35"
%	 text-hor-align= "right"
%	 >
%$\Progn$
%</text>
%<multicurve fill-style= "none"
%	 points= "(45,70);(45,70);(45,60);(45,60)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(55,70);(55,70);(35,70);(35,70)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(35,90);(35,90);(35,70);(35,70)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(35,90);(35,90);(55,70);(55,70)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(45,95);(45,95);(45,80);(45,80)"
%	 stroke-width= "1"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(47.5,93.75)"
%	 text-frame= "noframe"
%	 stroke-width= "0.35"
%	 text-hor-align= "left"
%	 >
%$\Progtype$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(41.25,76.25)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\encon$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(45,80)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\Dottt
%</text>
%</jpic>
%%End JPIC-XML
%LaTeX-picture environment using emulated lines and arcs
%You can rescale the whole picture (to 80% for instance) by using the command \def\JPicScale{0.8}
\ifx\JPicScale\undefined\def\JPicScale{1}\fi
\unitlength \JPicScale mm
\begin{picture}(165,95)(0,0)
\put(5,0){\makebox(0,0)[cr]{$\Progtype$}}

\linethickness{0.3mm}
\put(60,35){\line(0,1){25}}
\linethickness{0.3mm}
\put(20,35){\line(1,0){40}}
\linethickness{0.3mm}
\multiput(-5,60)(0.12,-0.12){208}{\line(1,0){0.12}}
\linethickness{0.3mm}
\put(-5,60){\line(1,0){65}}
\linethickness{1mm}
\put(7.5,0){\line(0,1){47.5}}
\put(110,27.5){\makebox(0,0)[cc]{\program}}

\put(80,47.5){\makebox(0,0)[cc]{$\eqlsb$}}

\put(145,47.5){\makebox(0,0)[cc]{$\universal$}}

\linethickness{0.3mm}
\put(165,35){\line(0,1){25}}
\linethickness{0.3mm}
\put(125,35){\line(1,0){40}}
\linethickness{0.3mm}
\put(100,20){\line(0,1){25}}
\linethickness{0.3mm}
\put(100,60){\line(1,0){65}}
\linethickness{1mm}
\put(111.25,0){\line(0,1){20}}
\put(107.5,0){\makebox(0,0)[cr]{$\Progtype$}}

\linethickness{0.3mm}
\put(100,20){\line(1,0){25}}
\linethickness{0.3mm}
\multiput(100,45)(0.12,-0.12){208}{\line(1,0){0.12}}
\linethickness{0.3mm}
\multiput(100,60)(0.12,-0.12){208}{\line(1,0){0.12}}
\linethickness{1mm}
\put(111.25,33.75){\line(0,1){15}}
\put(111.25,33.75){\makebox(0,0)[cc]{\Dottt}}

\linethickness{1mm}
\put(145,0){\line(0,1){35}}
\put(141.25,0){\makebox(0,0)[cr]{$\Progtype$}}

\linethickness{1mm}
\put(145,60){\line(0,1){35}}
\put(147.5,93.75){\makebox(0,0)[cl]{$\Progtype$}}

\put(40,47.5){\makebox(0,0)[cc]{$\Big\{\Big\}^B_A$}}

\put(47.5,65){\makebox(0,0)[cl]{$\Progk$}}

\linethickness{0.3mm}
\put(45,25){\line(0,1){10}}
\linethickness{0.3mm}
\put(35,25){\line(1,0){20}}
\linethickness{0.3mm}
\put(55,5){\line(0,1){20}}
\linethickness{0.3mm}
\multiput(35,25)(0.12,-0.12){167}{\line(1,0){0.12}}
\linethickness{1mm}
\put(45,0){\line(0,1){15}}
\put(42.5,0){\makebox(0,0)[cr]{$\Progtype$}}

\put(48.75,18.75){\makebox(0,0)[cc]{$\decok$}}

\put(42.5,30){\makebox(0,0)[cr]{$\Progn$}}

\linethickness{0.3mm}
\put(45,60){\line(0,1){10}}
\linethickness{0.3mm}
\put(35,70){\line(1,0){20}}
\linethickness{0.3mm}
\put(35,70){\line(0,1){20}}
\linethickness{0.3mm}
\multiput(35,90)(0.12,-0.12){167}{\line(1,0){0.12}}
\linethickness{1mm}
\put(45,80){\line(0,1){15}}
\put(47.5,93.75){\makebox(0,0)[cl]{$\Progtype$}}

\put(41.25,76.25){\makebox(0,0)[cc]{$\encon$}}

\put(45,80){\makebox(0,0)[cc]{\Dottt}}

\end{picture}


==> PIC/uni-idem.tex <==
%%Created by jPicEdt 1.4.1_03: mixed JPIC-XML/LaTeX format
%%Thu Dec 22 17:30:02 GMT-10:00 2022
%%Begin JPIC-XML
%<?xml version="1.0" standalone="yes"?>
%<jpic x-min="-5" x-max="165" y-min="0" y-max="95" auto-bounding="true">
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(5,0)"
%	 text-frame= "noframe"
%	 stroke-width= "0.35"
%	 text-hor-align= "right"
%	 >
%$\Progtype$
%</text>
%<multicurve fill-style= "none"
%	 points= "(60,60);(60,60);(60,35);(60,35)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(60,35);(60,35);(20,35);(20,35)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(20,35);(20,35);(-5,60);(-5,60)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(-5,60);(-5,60);(60,60);(60,60)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(7.5,47.5);(7.5,47.5);(7.5,0);(7.5,0)"
%	 stroke-width= "1"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(38.75,0)"
%	 text-frame= "noframe"
%	 stroke-width= "0.35"
%	 text-hor-align= "right"
%	 >
%$\Progn$
%</text>
%<multicurve fill-style= "none"
%	 points= "(40,95);(40,95);(40,60);(40,60)"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(42.5,93.75)"
%	 text-frame= "noframe"
%	 stroke-width= "0.35"
%	 text-hor-align= "left"
%	 >
%$\Progk$
%</text>
%<multicurve fill-style= "none"
%	 points= "(40,35);(40,35);(40,0);(40,0)"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(110,27.5)"
%	 text-frame= "noframe"
%	 stroke-width= "0.35"
%	 text-hor-align= "center-h"
%	 >
%\program
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(80,47.5)"
%	 text-frame= "noframe"
%	 stroke-width= "0.35"
%	 text-hor-align= "center-h"
%	 >
%$\eqlsb$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(145,47.5)"
%	 text-frame= "noframe"
%	 stroke-width= "0.35"
%	 text-hor-align= "center-h"
%	 >
%$\universal$
%</text>
%<multicurve fill-style= "none"
%	 points= "(165,60);(165,60);(165,35);(165,35)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(165,35);(165,35);(125,35);(125,35)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(100,45);(100,45);(100,20);(100,20)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(100,60);(100,60);(165,60);(165,60)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(111.25,20);(111.25,20);(111.25,0);(111.25,0)"
%	 stroke-width= "1"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(107.5,0)"
%	 text-frame= "noframe"
%	 stroke-width= "0.35"
%	 text-hor-align= "right"
%	 >
%$\Progtype$
%</text>
%<multicurve fill-style= "none"
%	 points= "(125,20);(125,20);(100,20);(100,20)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(125,20);(125,20);(100,45);(100,45)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(125,35);(125,35);(100,60);(100,60)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(111.25,48.75);(111.25,48.75);(111.25,33.75);(111.25,33.75)"
%	 stroke-width= "1"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(111.25,33.75)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\Dottt
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(142.5,1.25)"
%	 text-frame= "noframe"
%	 stroke-width= "0.35"
%	 text-hor-align= "right"
%	 >
%$\Progn$
%</text>
%<multicurve fill-style= "none"
%	 points= "(145,10);(145,10);(145,0);(145,0)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(155,10);(155,10);(135,10);(135,10)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(135,30);(135,30);(135,10);(135,10)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(135,30);(135,30);(155,10);(155,10)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(145,35);(145,35);(145,20);(145,20)"
%	 stroke-width= "1"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(147.5,26.25)"
%	 text-frame= "noframe"
%	 stroke-width= "0.35"
%	 text-hor-align= "left"
%	 >
%$\Progtype$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(141.25,16.25)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\encon$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(145,20)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\Dottt
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(147.5,93.75)"
%	 text-frame= "noframe"
%	 stroke-width= "0.35"
%	 text-hor-align= "left"
%	 >
%$\Progk$
%</text>
%<multicurve fill-style= "none"
%	 points= "(145,95);(145,95);(145,85);(145,85)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(155,85);(155,85);(135,85);(135,85)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(155,85);(155,85);(155,65);(155,65)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(135,85);(135,85);(155,65);(155,65)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(145,75);(145,75);(145,60);(145,60)"
%	 stroke-width= "1"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(142.5,66.25)"
%	 text-frame= "noframe"
%	 stroke-width= "0.35"
%	 text-hor-align= "right"
%	 >
%$\Progtype$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(148.75,78.75)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\decok$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(40,47.5)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\Big\{\Big\}^B_A$
%</text>
%</jpic>
%%End JPIC-XML
%LaTeX-picture environment using emulated lines and arcs
%You can rescale the whole picture (to 80% for instance) by using the command \def\JPicScale{0.8}
\ifx\JPicScale\undefined\def\JPicScale{1}\fi
\unitlength \JPicScale mm
\begin{picture}(165,95)(0,0)
\put(5,0){\makebox(0,0)[cr]{$\Progtype$}}

\linethickness{0.3mm}
\put(60,35){\line(0,1){25}}
\linethickness{0.3mm}
\put(20,35){\line(1,0){40}}
\linethickness{0.3mm}
\multiput(-5,60)(0.12,-0.12){208}{\line(1,0){0.12}}
\linethickness{0.3mm}
\put(-5,60){\line(1,0){65}}
\linethickness{1mm}
\put(7.5,0){\line(0,1){47.5}}
\put(38.75,0){\makebox(0,0)[cr]{$\Progn$}}

\linethickness{0.3mm}
\put(40,60){\line(0,1){35}}
\put(42.5,93.75){\makebox(0,0)[cl]{$\Progk$}}

\linethickness{0.3mm}
\put(40,0){\line(0,1){35}}
\put(110,27.5){\makebox(0,0)[cc]{\program}}

\put(80,47.5){\makebox(0,0)[cc]{$\eqlsb$}}

\put(145,47.5){\makebox(0,0)[cc]{$\universal$}}

\linethickness{0.3mm}
\put(165,35){\line(0,1){25}}
\linethickness{0.3mm}
\put(125,35){\line(1,0){40}}
\linethickness{0.3mm}
\put(100,20){\line(0,1){25}}
\linethickness{0.3mm}
\put(100,60){\line(1,0){65}}
\linethickness{1mm}
\put(111.25,0){\line(0,1){20}}
\put(107.5,0){\makebox(0,0)[cr]{$\Progtype$}}

\linethickness{0.3mm}
\put(100,20){\line(1,0){25}}
\linethickness{0.3mm}
\multiput(100,45)(0.12,-0.12){208}{\line(1,0){0.12}}
\linethickness{0.3mm}
\multiput(100,60)(0.12,-0.12){208}{\line(1,0){0.12}}
\linethickness{1mm}
\put(111.25,33.75){\line(0,1){15}}
\put(111.25,33.75){\makebox(0,0)[cc]{\Dottt}}

\put(142.5,1.25){\makebox(0,0)[cr]{$\Progn$}}

\linethickness{0.3mm}
\put(145,0){\line(0,1){10}}
\linethickness{0.3mm}
\put(135,10){\line(1,0){20}}
\linethickness{0.3mm}
\put(135,10){\line(0,1){20}}
\linethickness{0.3mm}
\multiput(135,30)(0.12,-0.12){167}{\line(1,0){0.12}}
\linethickness{1mm}
\put(145,20){\line(0,1){15}}
\put(147.5,26.25){\makebox(0,0)[cl]{$\Progtype$}}

\put(141.25,16.25){\makebox(0,0)[cc]{$\encon$}}

\put(145,20){\makebox(0,0)[cc]{\Dottt}}

\put(147.5,93.75){\makebox(0,0)[cl]{$\Progk$}}

\linethickness{0.3mm}
\put(145,85){\line(0,1){10}}
\linethickness{0.3mm}
\put(135,85){\line(1,0){20}}
\linethickness{0.3mm}
\put(155,65){\line(0,1){20}}
\linethickness{0.3mm}
\multiput(135,85)(0.12,-0.12){167}{\line(1,0){0.12}}
\linethickness{1mm}
\put(145,60){\line(0,1){15}}
\put(142.5,66.25){\makebox(0,0)[cr]{$\Progtype$}}

\put(148.75,78.75){\makebox(0,0)[cc]{$\decok$}}

\put(40,47.5){\makebox(0,0)[cc]{$\Big\{\Big\}^B_A$}}

\end{picture}


==> PIC/uni-mach-p-stream.tex <==
%%Created by jPicEdt 1.4.1_03: mixed JPIC-XML/LaTeX format
%%Thu Sep 21 08:05:55 HST 2017
%%Begin JPIC-XML
%<?xml version="1.0" standalone="yes"?>
%<jpic x-min="1.25" x-max="18.75" y-min="-23.75" y-max="28.12" auto-bounding="true">
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(15,28.12)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\dh$
%</text>
%<multicurve fill-style= "none"
%	 points= "(10,-10);(10,-10);(10,0);(10,0)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(15,8.75);(15,8.75);(15,25);(15,25)"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(15,3.75)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\ahh$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(7.5,-12.5)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\aah$
%</text>
%<multicurve fill-style= "none"
%	 points= "(5,13.76);(5,13.76);(5,25);(5,25)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(10,-20.62);(10,-20.62);(10,-15.62);(10,-15.62)"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(10,-23.75)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\xxh$
%</text>
%<text text-vert-align= "top"
%	 fill-style= "none"
%	 anchor-point= "(9.38,-1.25)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\RRsmall$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(5,9.38)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\bhh$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(5,28.12)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\RRsmall$
%</text>
%<multicurve fill-style= "none"
%	 points= "(18.75,-8.75);(18.75,-8.75);(1.25,8.75);(1.25,8.75)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(18.75,8.75);(18.75,8.75);(18.75,-8.75);(18.75,-8.75)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(18.75,8.75);(18.75,8.75);(10,8.75);(10,8.75)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(1.25,17.5);(1.25,17.5);(1.25,8.75);(1.25,8.75)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(10,8.75);(10,8.75);(1.25,17.5);(1.25,17.5)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(2.5,-15.62);(2.5,-15.62);(15.62,-15.62);(15.62,-15.62)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(2.5,-2.5);(2.5,-2.5);(15.62,-15.62);(15.62,-15.62)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(2.5,-2.5);(2.5,-2.5);(2.5,-15.62);(2.5,-15.62)"
%	 />
%</jpic>
%%End JPIC-XML
%PSTricks content-type (pstricks.sty package needed)
%Add \usepackage{pstricks} in the preamble of your LaTeX file
%You can rescale the whole picture (to 80% for instance) by using the command \def\JPicScale{0.8}
\ifx\JPicScale\undefined\def\JPicScale{1}\fi
\psset{unit=\JPicScale mm}
\psset{linewidth=0.3,dotsep=1,hatchwidth=0.3,hatchsep=1.5,shadowsize=1,dimen=middle}
\psset{dotsize=0.7 2.5,dotscale=1 1,fillcolor=black}
\psset{arrowsize=1 2,arrowlength=1,arrowinset=0.25,tbarsize=0.7 5,bracketlength=0.15,rbracketlength=0.15}
\begin{pspicture}(0,0)(18.75,28.12)
\rput(15,28.12){$\dh$}
\psline(10,-10)(10,0)
\psline(15,8.75)(15,25)
\rput(15,3.75){$\ahh$}
\rput(7.5,-12.5){$\aah$}
\psline(5,13.76)(5,25)
\psline(10,-20.62)(10,-15.62)
\rput(10,-23.75){$\xxh$}
\rput[tr](9.38,-1.25){$\RRsmall$}
\rput(5,9.38){$\bhh$}
\rput(5,28.12){$\RRsmall$}
\psline(18.75,-8.75)(1.25,8.75)
\psline(18.75,8.75)(18.75,-8.75)
\psline(18.75,8.75)(10,8.75)
\psline(1.25,17.5)(1.25,8.75)
\psline(10,8.75)(1.25,17.5)
\psline(2.5,-15.62)(15.62,-15.62)
\psline(2.5,-2.5)(15.62,-15.62)
\psline(2.5,-2.5)(2.5,-15.62)
\end{pspicture}


==> PIC/uni-mach-p.tex <==
%%Created by jPicEdt 1.4.1_03: mixed JPIC-XML/LaTeX format
%%Wed Dec 25 19:27:21 GMT-10:00 2019
%%Begin JPIC-XML
%<?xml version="1.0" standalone="yes"?>
%<jpic x-min="1.88" x-max="23.12" y-min="-6.25" y-max="43.75" auto-bounding="true">
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(18.75,43.75)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\dh$
%</text>
%<multicurve fill-style= "none"
%	 points= "(6.88,5.62);(6.88,5.62);(6.88,16.87);(6.88,16.87)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(18.88,21.87);(18.88,21.87);(18.75,40.62);(18.75,40.62)"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(13.12,17.5)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\ahh$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(5,3.75)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\aah$
%</text>
%<multicurve fill-style= "none"
%	 points= "(18.75,-2.5);(18.75,-2.5);(18.88,11.87);(18.88,11.87)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(1.88,10.61);(1.88,10.61);(11.86,0.63);(11.86,0.63);(11.86,0.63);(1.88,0.63);
%	(1.88,0.63);(1.88,0.63);(1.88,10.61)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(6.87,26.88);(6.87,26.88);(6.88,40.62);(6.88,40.62)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(6.88,-3.12);(6.88,-3.12);(6.88,0.62);(6.88,0.62)"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(6.88,-6.25)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\xxh$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(6.25,13.12)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\RRsmall$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(18.75,-6.25)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\bhh$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(6.88,43.75)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\RRsmall$
%</text>
%<multicurve fill-style= "none"
%	 points= "(11.88,11.87);(11.88,11.87);(1.88,21.88);(1.88,21.88)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(23.12,11.88);(23.12,11.88);(11.88,11.88);(11.88,11.88)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(23.12,21.88);(23.12,21.88);(23.12,11.88);(23.12,11.88)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(23.12,21.88);(23.12,21.88);(11.88,21.88);(11.88,21.88)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(1.88,31.88);(1.88,31.88);(1.88,21.88);(1.88,21.88)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(11.88,21.88);(11.88,21.88);(1.88,31.88);(1.88,31.88)"
%	 />
%</jpic>
%%End JPIC-XML
%PSTricks content-type (pstricks.sty package needed)
%Add \usepackage{pstricks} in the preamble of your LaTeX file
%You can rescale the whole picture (to 80% for instance) by using the command \def\JPicScale{0.8}
\ifx\JPicScale\undefined\def\JPicScale{1}\fi
\psset{unit=\JPicScale mm}
\psset{linewidth=0.3,dotsep=1,hatchwidth=0.3,hatchsep=1.5,shadowsize=1,dimen=middle}
\psset{dotsize=0.7 2.5,dotscale=1 1,fillcolor=black}
\psset{arrowsize=1 2,arrowlength=1,arrowinset=0.25,tbarsize=0.7 5,bracketlength=0.15,rbracketlength=0.15}
\begin{pspicture}(0,0)(23.12,43.75)
\rput(18.75,43.75){$\dh$}
\psline(6.88,5.62)(6.88,16.87)
\psline(18.88,21.87)(18.75,40.62)
\rput(13.12,17.5){$\ahh$}
\rput(5,3.75){$\aah$}
\psline(18.75,-2.5)(18.88,11.87)
\pspolygon(1.88,10.61)
(11.86,0.63)
(1.88,0.63)(1.88,10.61)
\psline(6.87,26.88)(6.88,40.62)
\psline(6.88,-3.12)(6.88,0.62)
\rput(6.88,-6.25){$\xxh$}
\rput[r](6.25,13.12){$\RRsmall$}
\rput(18.75,-6.25){$\bhh$}
\rput(6.88,43.75){$\RRsmall$}
\psline(11.88,11.87)(1.88,21.88)
\psline(23.12,11.88)(11.88,11.88)
\psline(23.12,21.88)(23.12,11.88)
\psline(23.12,21.88)(11.88,21.88)
\psline(1.88,31.88)(1.88,21.88)
\psline(11.88,21.88)(1.88,31.88)
\end{pspicture}


==> PIC/uni-mach-pt-sim-withM.tex <==
%%Created by jPicEdt 1.4.1_03: mixed JPIC-XML/LaTeX format
%%Fri Dec 27 19:16:12 GMT-10:00 2019
%%Begin JPIC-XML
%<?xml version="1.0" standalone="yes"?>
%<jpic x-min="1.88" x-max="66.25" y-min="-1.25" y-max="45.62" auto-bounding="true">
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(14.38,21.88)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\ahh$
%</text>
%<multicurve fill-style= "none"
%	 points= "(60.62,-1.25);(60.62,-1.25);(60.62,16.88);(60.62,16.88)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(48.12,-1.25);(48.12,-1.25);(48.12,16.88);(48.12,16.88)"
%	 />
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(46.25,-0.62)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\xxh$
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(33.75,22.5)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\EQLS
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(54.38,21.88)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\bhh$
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(59.38,-0.62)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\ah$
%</text>
%<parallelogram fill-color= "#999999"
%	 fill-style= "solid"
%	 p3= "(46.91,36.88)"
%	 p2= "(56.84,36.88)"
%	 p1= "(56.84,26.88)"
%	 stroke-color= "#999999"
%	 />
%<parallelogram fill-color= "#999999"
%	 fill-style= "solid"
%	 p3= "(41.88,40)"
%	 p2= "(52.79,40)"
%	 p1= "(52.79,32.5)"
%	 stroke-color= "#999999"
%	 />
%<parallelogram fill-color= "#999999"
%	 fill-style= "solid"
%	 p3= "(46.72,45.62)"
%	 p2= "(46.72,26.88)"
%	 p1= "(61.25,26.88)"
%	 stroke-color= "#999999"
%	 />
%<multicurve fill-style= "none"
%	 points= "(60,26.88);(60,26.88);(60,45.62);(60,45.62)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(48.12,26.88);(48.12,26.88);(48.12,33.75);(48.12,33.75)"
%	 />
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(48.12,36.25)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\aah$
%</text>
%<multicurve fill-style= "none"
%	 points= "(41.88,26.88);(41.88,26.88);(41.88,16.88);(41.88,16.88);(41.88,16.88);(66.25,16.88);
%	(66.25,16.88);(66.25,16.88);(66.25,26.88);(66.25,26.88);(66.25,26.88);(41.88,26.88);
%	(41.88,26.88);(41.88,26.88);(61.25,26.86);(61.25,26.86);(61.25,26.86);(41.88,26.88);
%	(41.88,26.88);(41.88,26.88);(41.88,26.88);(41.88,26.88)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(48.12,38.75);(48.12,38.75);(48.12,45.62);(48.12,45.62)"
%	 />
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(54.38,30)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\xxbbh$
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(54.38,42.5)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\ssbbh$
%</text>
%<multicurve fill-style= "none"
%	 points= "(20.62,-1.25);(20.62,-1.25);(20.62,16.88);(20.62,16.88)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(8.12,10);(8.12,10);(8.12,16.88);(8.12,16.88)"
%	 />
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(6.88,-1.25)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\xxh$
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(19.38,-0.62)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\ah$
%</text>
%<parallelogram fill-color= "#999999"
%	 fill-style= "solid"
%	 p3= "(6.91,36.88)"
%	 p2= "(16.84,36.88)"
%	 p1= "(16.84,26.88)"
%	 stroke-color= "#999999"
%	 />
%<parallelogram fill-color= "#999999"
%	 fill-style= "solid"
%	 p3= "(6.72,45.62)"
%	 p2= "(6.72,26.88)"
%	 p1= "(21.25,26.88)"
%	 stroke-color= "#999999"
%	 />
%<multicurve fill-style= "none"
%	 points= "(20,26.88);(20,26.88);(20,45.62);(20,45.62)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(1.88,26.88);(1.88,26.88);(1.88,16.88);(1.88,16.88);(1.88,16.88);(26.25,16.88);
%	(26.25,16.88);(26.25,16.88);(26.25,26.88);(26.25,26.88);(26.25,26.88);(1.88,26.88);
%	(1.88,26.88);(1.88,26.88);(21.25,26.86);(21.25,26.86);(21.25,26.86);(1.88,26.88);
%	(1.88,26.88);(1.88,26.88);(1.88,26.88);(1.88,26.88)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(8.12,26.88);(8.12,26.88);(8.12,45.62);(8.12,45.62)"
%	 />
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(14.38,42.5)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\ssbbh$
%</text>
%<parallelogram fill-style= "none"
%	 p3= "(53.12,33.75)"
%	 p2= "(53.12,38.75)"
%	 p1= "(43.12,38.75)"
%	 />
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(8.12,7.5)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\aah$
%</text>
%<parallelogram fill-style= "none"
%	 p3= "(13.12,5)"
%	 p2= "(13.12,10)"
%	 p1= "(3.12,10)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(8.12,-1.25);(8.12,-1.25);(8.12,5);(8.12,5)"
%	 />
%</jpic>
%%End JPIC-XML
%PSTricks content-type (pstricks.sty package needed)
%Add \usepackage{pstricks} in the preamble of your LaTeX file
%You can rescale the whole picture (to 80% for instance) by using the command \def\JPicScale{0.8}
\ifx\JPicScale\undefined\def\JPicScale{1}\fi
\psset{unit=\JPicScale mm}
\psset{linewidth=0.3,dotsep=1,hatchwidth=0.3,hatchsep=1.5,shadowsize=1,dimen=middle}
\psset{dotsize=0.7 2.5,dotscale=1 1,fillcolor=black}
\psset{arrowsize=1 2,arrowlength=1,arrowinset=0.25,tbarsize=0.7 5,bracketlength=0.15,rbracketlength=0.15}
\begin{pspicture}(0,0)(66.25,45.62)
\rput(14.38,21.88){$\ahh$}
\psline(60.62,-1.25)(60.62,16.88)
\psline(48.12,-1.25)(48.12,16.88)
\rput[r](46.25,-0.62){$\xxh$}
\rput(33.75,22.5){\EQLS}
\rput(54.38,21.88){$\bhh$}
\rput[r](59.38,-0.62){$\ah$}
\newrgbcolor{userLineColour}{0.6 0.6 0.6}
\newrgbcolor{userFillColour}{0.6 0.6 0.6}
\pspolygon[linecolor=userLineColour,fillcolor=userFillColour,fillstyle=solid](56.84,26.88)(56.84,36.88)(46.91,36.88)(46.91,26.88)
\newrgbcolor{userLineColour}{0.6 0.6 0.6}
\newrgbcolor{userFillColour}{0.6 0.6 0.6}
\pspolygon[linecolor=userLineColour,fillcolor=userFillColour,fillstyle=solid](52.79,32.5)(52.79,40)(41.88,40)(41.88,32.5)
\newrgbcolor{userLineColour}{0.6 0.6 0.6}
\newrgbcolor{userFillColour}{0.6 0.6 0.6}
\pspolygon[linecolor=userLineColour,fillcolor=userFillColour,fillstyle=solid](61.25,26.88)(46.72,26.88)(46.72,45.62)(61.25,45.62)
\psline(60,26.88)(60,45.62)
\psline(48.12,26.88)(48.12,33.75)
\rput(48.12,36.25){$\aah$}
\pscustom[]{\psline(41.88,26.88)(41.88,16.88)
\psline(41.88,16.88)(66.25,16.88)
\psline(66.25,16.88)(66.25,26.88)
\psline(66.25,26.88)(41.88,26.88)
\psline(41.88,26.88)(61.25,26.86)
\psline(61.25,26.86)(41.88,26.88)
\psbezier(41.88,26.88)(41.88,26.88)(41.88,26.88)
}
\psline(48.12,38.75)(48.12,45.62)
\rput(54.38,30){$\xxbbh$}
\rput(54.38,42.5){$\ssbbh$}
\psline(20.62,-1.25)(20.62,16.88)
\psline(8.12,10)(8.12,16.88)
\rput[r](6.88,-1.25){$\xxh$}
\rput[r](19.38,-0.62){$\ah$}
\newrgbcolor{userLineColour}{0.6 0.6 0.6}
\newrgbcolor{userFillColour}{0.6 0.6 0.6}
\pspolygon[linecolor=userLineColour,fillcolor=userFillColour,fillstyle=solid](16.84,26.88)(16.84,36.88)(6.91,36.88)(6.91,26.88)
\newrgbcolor{userLineColour}{0.6 0.6 0.6}
\newrgbcolor{userFillColour}{0.6 0.6 0.6}
\pspolygon[linecolor=userLineColour,fillcolor=userFillColour,fillstyle=solid](21.25,26.88)(6.72,26.88)(6.72,45.62)(21.25,45.62)
\psline(20,26.88)(20,45.62)
\pscustom[]{\psline(1.88,26.88)(1.88,16.88)
\psline(1.88,16.88)(26.25,16.88)
\psline(26.25,16.88)(26.25,26.88)
\psline(26.25,26.88)(1.88,26.88)
\psline(1.88,26.88)(21.25,26.86)
\psline(21.25,26.86)(1.88,26.88)
\psbezier(1.88,26.88)(1.88,26.88)(1.88,26.88)
}
\psline(8.12,26.88)(8.12,45.62)
\rput(14.38,42.5){$\ssbbh$}
\pspolygon[](43.12,38.75)(53.12,38.75)(53.12,33.75)(43.12,33.75)
\rput(8.12,7.5){$\aah$}
\pspolygon[](3.12,10)(13.12,10)(13.12,5)(3.12,5)
\psline(8.12,-1.25)(8.12,5)
\end{pspicture}


==> PIC/uni-mach-pt-sim.tex <==
%%Created by jPicEdt 1.4.1_03: mixed JPIC-XML/LaTeX format
%%Mon Dec 05 21:04:44 GMT-10:00 2022
%%Begin JPIC-XML
%<?xml version="1.0" standalone="yes"?>
%<jpic x-min="1.88" x-max="66.25" y-min="-1.25" y-max="45.62" auto-bounding="true">
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 stroke-width= "0.15"
%	 anchor-point= "(14.38,21.88)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\ahh$
%</text>
%<multicurve fill-style= "none"
%	 stroke-width= "0.15"
%	 points= "(60.62,-1.25);(60.62,-1.25);(60.62,16.88);(60.62,16.88)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.15"
%	 points= "(48.12,-1.25);(48.12,-1.25);(48.12,16.88);(48.12,16.88)"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 stroke-width= "0.15"
%	 anchor-point= "(46.88,-0.62)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\xxh$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 stroke-width= "0.15"
%	 anchor-point= "(33.75,22.5)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\EQLS
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 stroke-width= "0.15"
%	 anchor-point= "(54.38,21.88)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\bhh$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 stroke-width= "0.15"
%	 anchor-point= "(59.38,-0.62)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\ah$
%</text>
%<multicurve fill-style= "none"
%	 stroke-width= "0.15"
%	 points= "(60,26.88);(60,26.88);(60,45.62);(60,45.62)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.15"
%	 points= "(48.12,26.88);(48.12,26.88);(48.12,33.75);(48.12,33.75)"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 stroke-width= "0.15"
%	 anchor-point= "(48.12,36.25)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\aah$
%</text>
%<multicurve fill-style= "none"
%	 stroke-width= "0.15"
%	 points= "(48.12,38.75);(48.12,38.75);(48.12,45.62);(48.12,45.62)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.15"
%	 points= "(20.62,-1.25);(20.62,-1.25);(20.62,16.88);(20.62,16.88)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.15"
%	 points= "(8.12,10);(8.12,10);(8.12,16.88);(8.12,16.88)"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 stroke-width= "0.15"
%	 anchor-point= "(6.88,-0.62)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\xxh$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 stroke-width= "0.15"
%	 anchor-point= "(19.38,-0.62)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\ah$
%</text>
%<multicurve fill-style= "none"
%	 stroke-width= "0.15"
%	 points= "(20,26.88);(20,26.88);(20,45.62);(20,45.62)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.15"
%	 points= "(8.12,26.88);(8.12,26.88);(8.12,45.62);(8.12,45.62)"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 stroke-width= "0.15"
%	 anchor-point= "(9.38,44.38)"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\ssbbh$
%</text>
%<parallelogram p3= "(53.12,33.75)"
%	 p2= "(53.12,38.75)"
%	 fill-style= "none"
%	 p1= "(43.12,38.75)"
%	 stroke-width= "0.15"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 stroke-width= "0.15"
%	 anchor-point= "(8.12,7.5)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\aah$
%</text>
%<parallelogram p3= "(13.12,5)"
%	 p2= "(13.12,10)"
%	 fill-style= "none"
%	 p1= "(3.12,10)"
%	 stroke-width= "0.15"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.15"
%	 points= "(8.12,-1.25);(8.12,-1.25);(8.12,5);(8.12,5)"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 stroke-width= "0.15"
%	 anchor-point= "(21.25,44.38)"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\xxbbh$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 stroke-width= "0.15"
%	 anchor-point= "(49.38,44.38)"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\ssbbh$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 stroke-width= "0.15"
%	 anchor-point= "(61.25,44.38)"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\xxbbh$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 stroke-width= "0.15"
%	 anchor-point= "(49.38,30)"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\xxh$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 stroke-width= "0.15"
%	 anchor-point= "(6.88,13.12)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\ssbbh$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 stroke-width= "0.15"
%	 anchor-point= "(8.12,10)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\Dott$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 stroke-width= "0.15"
%	 anchor-point= "(48.12,38.75)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\Dott$
%</text>
%<multicurve fill-style= "none"
%	 stroke-width= "0.15"
%	 points= "(42.5,26.88);(42.5,26.88);(66.25,26.88);(66.25,26.88)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.15"
%	 points= "(42.5,16.88);(42.5,16.88);(66.25,16.88);(66.25,16.88)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.15"
%	 points= "(1.88,26.88);(1.88,26.88);(25.62,26.88);(25.62,26.88)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.15"
%	 points= "(1.88,16.88);(1.88,16.88);(25.62,16.88);(25.62,16.88)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.15"
%	 points= "(25.62,26.88);(25.62,26.88);(25.62,16.88);(25.62,16.88)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.15"
%	 points= "(42.5,26.88);(42.5,26.88);(42.5,16.88);(42.5,16.88)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.15"
%	 points= "(66.25,26.88);(66.25,26.88);(66.25,16.88);(66.25,16.88)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.15"
%	 points= "(1.88,26.88);(1.88,26.88);(1.88,16.88);(1.88,16.88)"
%	 />
%</jpic>
%%End JPIC-XML
%LaTeX-picture environment using emulated lines and arcs
%You can rescale the whole picture (to 80% for instance) by using the command \def\JPicScale{0.8}
\ifx\JPicScale\undefined\def\JPicScale{1}\fi
\unitlength \JPicScale mm
\begin{picture}(66.25,45.62)(0,0)
\put(14.38,21.88){\makebox(0,0)[cc]{$\ahh$}}

\linethickness{0.15mm}
\put(60.62,-1.25){\line(0,1){18.13}}
\linethickness{0.15mm}
\put(48.12,-1.25){\line(0,1){18.13}}
\put(46.88,-0.62){\makebox(0,0)[cr]{$\xxh$}}

\put(33.75,22.5){\makebox(0,0)[cc]{\EQLS}}

\put(54.38,21.88){\makebox(0,0)[cc]{$\bhh$}}

\put(59.38,-0.62){\makebox(0,0)[cr]{$\ah$}}

\linethickness{0.15mm}
\put(60,26.88){\line(0,1){18.74}}
\linethickness{0.15mm}
\put(48.12,26.88){\line(0,1){6.87}}
\put(48.12,36.25){\makebox(0,0)[cc]{$\aah$}}

\linethickness{0.15mm}
\put(48.12,38.75){\line(0,1){6.87}}
\linethickness{0.15mm}
\put(20.62,-1.25){\line(0,1){18.13}}
\linethickness{0.15mm}
\put(8.12,10){\line(0,1){6.88}}
\put(6.88,-0.62){\makebox(0,0)[cr]{$\xxh$}}

\put(19.38,-0.62){\makebox(0,0)[cr]{$\ah$}}

\linethickness{0.15mm}
\put(20,26.88){\line(0,1){18.74}}
\linethickness{0.15mm}
\put(8.12,26.88){\line(0,1){18.74}}
\put(9.38,44.38){\makebox(0,0)[cl]{$\ssbbh$}}

\linethickness{0.15mm}
\put(43.12,38.75){\line(1,0){10}}
\put(43.12,33.75){\line(0,1){5}}
\put(53.12,33.75){\line(0,1){5}}
\put(43.12,33.75){\line(1,0){10}}
\put(8.12,7.5){\makebox(0,0)[cc]{$\aah$}}

\linethickness{0.15mm}
\put(3.12,10){\line(1,0){10}}
\put(3.12,5){\line(0,1){5}}
\put(13.12,5){\line(0,1){5}}
\put(3.12,5){\line(1,0){10}}
\linethickness{0.15mm}
\put(8.12,-1.25){\line(0,1){6.25}}
\put(21.25,44.38){\makebox(0,0)[cl]{$\xxbbh$}}

\put(49.38,44.38){\makebox(0,0)[cl]{$\ssbbh$}}

\put(61.25,44.38){\makebox(0,0)[cl]{$\xxbbh$}}

\put(49.38,30){\makebox(0,0)[cl]{$\xxh$}}

\put(6.88,13.12){\makebox(0,0)[cr]{$\ssbbh$}}

\put(8.12,10){\makebox(0,0)[cc]{$\Dott$}}

\put(48.12,38.75){\makebox(0,0)[cc]{$\Dott$}}

\linethickness{0.15mm}
\put(42.5,26.88){\line(1,0){23.75}}
\linethickness{0.15mm}
\put(42.5,16.88){\line(1,0){23.75}}
\linethickness{0.15mm}
\put(1.88,26.88){\line(1,0){23.75}}
\linethickness{0.15mm}
\put(1.88,16.88){\line(1,0){23.75}}
\linethickness{0.15mm}
\put(25.62,16.88){\line(0,1){10}}
\linethickness{0.15mm}
\put(42.5,16.88){\line(0,1){10}}
\linethickness{0.15mm}
\put(66.25,16.88){\line(0,1){10}}
\linethickness{0.15mm}
\put(1.88,16.88){\line(0,1){10}}
\end{picture}


==> PIC/uni-mach-pt.tex <==
%%Created by jPicEdt 1.4.1_03: mixed JPIC-XML/LaTeX format
%%Thu Dec 26 14:35:48 GMT-10:00 2019
%%Begin JPIC-XML
%<?xml version="1.0" standalone="yes"?>
%<jpic x-min="1.88" x-max="66.25" y-min="1.25" y-max="46.88" auto-bounding="true">
%<multicurve fill-style= "none"
%	 points= "(6.88,10.62);(6.88,10.62);(6.88,21.87);(6.88,21.87)"
%	 />
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(13.12,22.5)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\ahh$
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(5,8.75)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\aah$
%</text>
%<multicurve fill-style= "none"
%	 points= "(18.75,2.5);(18.75,2.5);(18.75,16.88);(18.75,16.88)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(1.88,15.61);(1.88,15.61);(11.86,5.63);(11.86,5.63);(11.86,5.63);(1.88,5.63);
%	(1.88,5.63);(1.88,5.63);(1.88,15.61)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(6.88,1.88);(6.88,1.88);(6.88,5.62);(6.88,5.62)"
%	 />
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(6.25,1.25)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\xxh$
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(6.25,18.12)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\RRsmall$
%</text>
%<multicurve fill-style= "none"
%	 points= "(23.12,16.88);(23.12,16.88);(11.88,16.88);(11.88,16.88)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(60.62,2.5);(60.62,2.5);(60.62,16.88);(60.62,16.88)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(48.12,1.88);(48.12,1.88);(48.12,16.88);(48.12,16.88)"
%	 />
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(46.25,1.25)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\xxh$
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(33.75,22.5)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\EQLS
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(54.38,21.88)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\bhh$
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(17.5,1.25)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\ah$
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(59.38,1.25)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\ah$
%</text>
%<parallelogram fill-color= "#999999"
%	 fill-style= "solid"
%	 p3= "(11.88,40.62)"
%	 p2= "(11.88,26.88)"
%	 p1= "(20,26.88)"
%	 stroke-color= "#999999"
%	 />
%<parallelogram fill-color= "#999999"
%	 fill-style= "solid"
%	 p3= "(5.62,46.88)"
%	 p2= "(11.88,40.62)"
%	 p1= "(11.88,26.88)"
%	 stroke-color= "#999999"
%	 />
%<multicurve fill-style= "none"
%	 points= "(11.88,16.87);(11.88,16.87);(1.88,26.88);(1.88,26.88)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(23.12,26.88);(23.12,26.88);(23.12,16.88);(23.12,16.88)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(1.88,36.88);(1.88,36.88);(1.88,26.88);(1.88,26.88)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(18.75,26.88);(18.75,26.88);(18.75,40.62);(18.75,40.62)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(23.12,26.88);(23.12,26.88);(11.88,26.88);(11.88,26.88)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(6.86,31.89);(6.86,31.89);(6.88,45.62);(6.88,45.62)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(11.88,26.87);(11.88,26.87);(1.88,36.88);(1.88,36.88)"
%	 />
%<parallelogram fill-color= "#999999"
%	 fill-style= "solid"
%	 p3= "(46.91,36.88)"
%	 p2= "(56.84,36.88)"
%	 p1= "(56.84,26.88)"
%	 stroke-color= "#999999"
%	 />
%<parallelogram fill-color= "#999999"
%	 fill-style= "solid"
%	 p3= "(42.54,41.88)"
%	 p2= "(52.46,41.88)"
%	 p1= "(52.46,31.88)"
%	 stroke-color= "#999999"
%	 />
%<parallelogram fill-color= "#999999"
%	 fill-style= "solid"
%	 p3= "(46.72,45.62)"
%	 p2= "(46.72,26.88)"
%	 p1= "(61.25,26.88)"
%	 stroke-color= "#999999"
%	 />
%<parallelogram fill-color= "#999999"
%	 fill-style= "solid"
%	 p3= "(42.5,45.62)"
%	 p2= "(50,38.12)"
%	 p1= "(50,29.38)"
%	 stroke-color= "#999999"
%	 />
%<multicurve fill-style= "none"
%	 points= "(60,26.88);(60,26.88);(60,45.62);(60,45.62)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(48.12,26.88);(48.12,26.88);(48.12,33.12);(48.12,33.12)"
%	 />
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(46.5,36.38)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\aah$
%</text>
%<multicurve fill-style= "none"
%	 points= "(43.38,43.24);(43.38,43.24);(53.36,33.25);(53.36,33.25);(53.36,33.25);(43.38,33.25);
%	(43.38,33.25);(43.38,33.25);(43.38,43.24)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(41.88,26.88);(41.88,26.88);(41.88,16.88);(41.88,16.88);(41.88,16.88);(66.25,16.88);
%	(66.25,16.88);(66.25,16.88);(66.25,26.88);(66.25,26.88);(66.25,26.88);(41.88,26.88);
%	(41.88,26.88);(41.88,26.88);(61.25,26.86);(61.25,26.86);(61.25,26.86);(41.88,26.88);
%	(41.88,26.88);(41.88,26.88);(41.88,26.88);(41.88,26.88)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(48.12,38.75);(48.12,38.75);(48.12,45.62);(48.12,45.62)"
%	 />
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(54.38,30)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\xxbbh$
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(13.12,35.62)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\ssbbh$
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(54.38,42.5)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\ssbbh$
%</text>
%</jpic>
%%End JPIC-XML
%PSTricks content-type (pstricks.sty package needed)
%Add \usepackage{pstricks} in the preamble of your LaTeX file
%You can rescale the whole picture (to 80% for instance) by using the command \def\JPicScale{0.8}
\ifx\JPicScale\undefined\def\JPicScale{1}\fi
\psset{unit=\JPicScale mm}
\psset{linewidth=0.3,dotsep=1,hatchwidth=0.3,hatchsep=1.5,shadowsize=1,dimen=middle}
\psset{dotsize=0.7 2.5,dotscale=1 1,fillcolor=black}
\psset{arrowsize=1 2,arrowlength=1,arrowinset=0.25,tbarsize=0.7 5,bracketlength=0.15,rbracketlength=0.15}
\begin{pspicture}(0,0)(66.25,46.88)
\psline(6.88,10.62)(6.88,21.87)
\rput(13.12,22.5){$\ahh$}
\rput(5,8.75){$\aah$}
\psline(18.75,2.5)(18.75,16.88)
\pspolygon(1.88,15.61)
(11.86,5.63)
(1.88,5.63)(1.88,15.61)
\psline(6.88,1.88)(6.88,5.62)
\rput[r](6.25,1.25){$\xxh$}
\rput[r](6.25,18.12){$\RRsmall$}
\psline(23.12,16.88)(11.88,16.88)
\psline(60.62,2.5)(60.62,16.88)
\psline(48.12,1.88)(48.12,16.88)
\rput[r](46.25,1.25){$\xxh$}
\rput(33.75,22.5){\EQLS}
\rput(54.38,21.88){$\bhh$}
\rput[r](17.5,1.25){$\ah$}
\rput[r](59.38,1.25){$\ah$}
\newrgbcolor{userLineColour}{0.6 0.6 0.6}
\newrgbcolor{userFillColour}{0.6 0.6 0.6}
\pspolygon[linecolor=userLineColour,fillcolor=userFillColour,fillstyle=solid](20,26.88)(11.88,26.88)(11.88,40.62)(20,40.62)
\newrgbcolor{userLineColour}{0.6 0.6 0.6}
\newrgbcolor{userFillColour}{0.6 0.6 0.6}
\pspolygon[linecolor=userLineColour,fillcolor=userFillColour,fillstyle=solid](11.88,26.88)(11.88,40.62)(5.62,46.88)(5.62,33.12)
\psline(11.88,16.87)(1.88,26.88)
\psline(23.12,26.88)(23.12,16.88)
\psline(1.88,36.88)(1.88,26.88)
\psline(18.75,26.88)(18.75,40.62)
\psline(23.12,26.88)(11.88,26.88)
\psline(6.86,31.89)(6.88,45.62)
\psline(11.88,26.87)(1.88,36.88)
\newrgbcolor{userLineColour}{0.6 0.6 0.6}
\newrgbcolor{userFillColour}{0.6 0.6 0.6}
\pspolygon[linecolor=userLineColour,fillcolor=userFillColour,fillstyle=solid](56.84,26.88)(56.84,36.88)(46.91,36.88)(46.91,26.88)
\newrgbcolor{userLineColour}{0.6 0.6 0.6}
\newrgbcolor{userFillColour}{0.6 0.6 0.6}
\pspolygon[linecolor=userLineColour,fillcolor=userFillColour,fillstyle=solid](52.46,31.88)(52.46,41.88)(42.54,41.88)(42.54,31.88)
\newrgbcolor{userLineColour}{0.6 0.6 0.6}
\newrgbcolor{userFillColour}{0.6 0.6 0.6}
\pspolygon[linecolor=userLineColour,fillcolor=userFillColour,fillstyle=solid](61.25,26.88)(46.72,26.88)(46.72,45.62)(61.25,45.62)
\newrgbcolor{userLineColour}{0.6 0.6 0.6}
\newrgbcolor{userFillColour}{0.6 0.6 0.6}
\pspolygon[linecolor=userLineColour,fillcolor=userFillColour,fillstyle=solid](50,29.38)(50,38.12)(42.5,45.62)(42.5,36.88)
\psline(60,26.88)(60,45.62)
\psline(48.12,26.88)(48.12,33.12)
\rput(46.5,36.38){$\aah$}
\pspolygon(43.38,43.24)
(53.36,33.25)
(43.38,33.25)(43.38,43.24)
\pscustom[]{\psline(41.88,26.88)(41.88,16.88)
\psline(41.88,16.88)(66.25,16.88)
\psline(66.25,16.88)(66.25,26.88)
\psline(66.25,26.88)(41.88,26.88)
\psline(41.88,26.88)(61.25,26.86)
\psline(61.25,26.86)(41.88,26.88)
\psbezier(41.88,26.88)(41.88,26.88)(41.88,26.88)
}
\psline(48.12,38.75)(48.12,45.62)
\rput(54.38,30){$\xxbbh$}
\rput(13.12,35.62){$\ssbbh$}
\rput(54.38,42.5){$\ssbbh$}
\end{pspicture}


==> PIC/uni-mach-rl.tex <==
%%Created by jPicEdt 1.4.1_03: mixed JPIC-XML/LaTeX format
%%Thu Apr 05 21:32:35 HST 2018
%%Begin JPIC-XML
%<?xml version="1.0" standalone="yes"?>
%<jpic x-min="1.88" x-max="23.12" y-min="-28.75" y-max="33.12" auto-bounding="true">
%<text text-vert-align= "center-v"
%	 stroke-width= "0.5"
%	 anchor-point= "(18.75,33.12)"
%	 text-frame= "noframe"
%	 fill-style= "none"
%	 text-hor-align= "center-h"
%	 >
%$\dh$
%</text>
%<multicurve stroke-width= "0.5"
%	 points= "(6.88,25);(6.88,25);(6.88,30);(6.88,30)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.5"
%	 points= "(18.88,6.87);(18.88,6.87);(18.75,30);(18.75,30)"
%	 fill-style= "none"
%	 />
%<text text-vert-align= "center-v"
%	 stroke-width= "0.5"
%	 anchor-point= "(12.5,1.88)"
%	 text-frame= "noframe"
%	 fill-style= "none"
%	 text-hor-align= "center-h"
%	 >
%$\ahh$
%</text>
%<text text-vert-align= "center-v"
%	 stroke-width= "0.5"
%	 anchor-point= "(6.88,20)"
%	 text-frame= "noframe"
%	 fill-style= "none"
%	 text-hor-align= "center-h"
%	 >
%$\aah$
%</text>
%<multicurve stroke-width= "0.5"
%	 points= "(18.75,-25);(18.75,-25);(18.75,-3.12);(18.75,-3.12)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.5"
%	 points= "(1.88,6.88);(1.88,6.88);(1.88,-3.12);(1.88,-3.12);(1.88,-3.12);(23.12,-3.13);
%	(23.12,-3.13);(23.12,-3.13);(23.12,6.87);(23.12,6.87);(23.12,6.87);(5.62,6.87);
%	(5.62,6.87);(5.62,6.87);(23.12,6.87);(23.12,6.87);(23.12,6.87);(5.62,6.87);
%	(5.62,6.87);(5.62,6.87);(1.88,6.87);(1.88,6.87)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.5"
%	 points= "(6.88,6.88);(6.88,6.88);(6.88,15);(6.88,15)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.5"
%	 points= "(6.88,-25.62);(6.88,-25.62);(6.88,-3.12);(6.88,-3.12)"
%	 fill-style= "none"
%	 />
%<text text-vert-align= "center-v"
%	 stroke-width= "0.5"
%	 anchor-point= "(6.88,-28.75)"
%	 text-frame= "noframe"
%	 fill-style= "none"
%	 text-hor-align= "center-h"
%	 >
%$\xxh$
%</text>
%<text text-vert-align= "center-v"
%	 stroke-width= "0.5"
%	 anchor-point= "(18.75,-28.75)"
%	 text-frame= "noframe"
%	 fill-style= "none"
%	 text-hor-align= "center-h"
%	 >
%$\bhh$
%</text>
%<text text-vert-align= "center-v"
%	 stroke-width= "0.5"
%	 anchor-point= "(6.25,33.12)"
%	 text-frame= "noframe"
%	 fill-style= "none"
%	 text-hor-align= "center-h"
%	 >
%$\RRsmall$
%</text>
%<multicurve stroke-width= "0.5"
%	 points= "(1.88,25);(1.88,25);(1.88,15);(1.88,15);(1.88,15);(11.87,15);
%	(11.87,15);(11.87,15);(11.87,25);(11.87,25);(11.87,25);(5.62,25);
%	(5.62,25);(5.62,25);(11.87,25);(11.87,25);(11.87,25);(5.62,25);
%	(5.62,25);(5.62,25);(1.88,25);(1.88,25)"
%	 fill-style= "none"
%	 />
%<ellipse p3= "(7.97,23.91)"
%	 p2= "(7.97,26.09)"
%	 stroke-width= "0.5"
%	 p1= "(5.78,26.09)"
%	 closure= "open"
%	 angle-end= "360"
%	 fill-style= "solid"
%	 angle-start= "0"
%	 />
%<text text-vert-align= "center-v"
%	 stroke-width= "0.5"
%	 anchor-point= "(5.62,11.25)"
%	 text-frame= "noframe"
%	 fill-style= "none"
%	 text-hor-align= "right"
%	 >
%$\xxh$
%</text>
%</jpic>
%%End JPIC-XML
%PSTricks content-type (pstricks.sty package needed)
%Add \usepackage{pstricks} in the preamble of your LaTeX file
%You can rescale the whole picture (to 80% for instance) by using the command \def\JPicScale{0.8}
\ifx\JPicScale\undefined\def\JPicScale{1}\fi
\psset{unit=\JPicScale mm}
\psset{linewidth=0.3,dotsep=1,hatchwidth=0.3,hatchsep=1.5,shadowsize=1,dimen=middle}
\psset{dotsize=0.7 2.5,dotscale=1 1,fillcolor=black}
\psset{arrowsize=1 2,arrowlength=1,arrowinset=0.25,tbarsize=0.7 5,bracketlength=0.15,rbracketlength=0.15}
\begin{pspicture}(0,0)(23.12,33.12)
\rput(18.75,33.12){$\dh$}
\psline[linewidth=0.5](6.88,25)(6.88,30)
\psline[linewidth=0.5](18.88,6.87)(18.75,30)
\rput(12.5,1.88){$\ahh$}
\rput(6.88,20){$\aah$}
\psline[linewidth=0.5](18.75,-25)(18.75,-3.12)
\psline[linewidth=0.5](1.88,6.88)
(1.88,-3.12)
(23.12,-3.13)
(23.12,6.87)
(5.62,6.87)
(23.12,6.87)
(5.62,6.87)(1.88,6.87)
\psline[linewidth=0.5](6.88,6.88)(6.88,15)
\psline[linewidth=0.5](6.88,-25.62)(6.88,-3.12)
\rput(6.88,-28.75){$\xxh$}
\rput(18.75,-28.75){$\bhh$}
\rput(6.25,33.12){$\RRsmall$}
\psline[linewidth=0.5](1.88,25)
(1.88,15)
(11.87,15)
(11.87,25)
(5.62,25)
(11.87,25)
(5.62,25)(1.88,25)
\rput{0}(6.88,25){\psellipse[linewidth=0.5,fillstyle=solid](0,0)(1.09,-1.09)}
\rput[r](5.62,11.25){$\xxh$}
\end{pspicture}


==> PIC/uni-mach-rr.tex <==
%%Created by jPicEdt 1.4.1_03: mixed JPIC-XML/LaTeX format
%%Thu Apr 05 21:32:12 HST 2018
%%Begin JPIC-XML
%<?xml version="1.0" standalone="yes"?>
%<jpic x-min="1.88" x-max="23.12" y-min="-28.75" y-max="33.12" auto-bounding="true">
%<text text-vert-align= "center-v"
%	 stroke-width= "0.5"
%	 anchor-point= "(18.75,33.12)"
%	 text-frame= "noframe"
%	 fill-style= "none"
%	 text-hor-align= "center-h"
%	 >
%$\dh$
%</text>
%<multicurve stroke-width= "0.5"
%	 points= "(6.88,-11.88);(6.88,-11.88);(6.88,-3.12);(6.88,-3.12)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.5"
%	 points= "(18.88,6.87);(18.88,6.87);(18.75,30);(18.75,30)"
%	 fill-style= "none"
%	 />
%<text text-vert-align= "center-v"
%	 stroke-width= "0.5"
%	 anchor-point= "(12.5,1.88)"
%	 text-frame= "noframe"
%	 fill-style= "none"
%	 text-hor-align= "center-h"
%	 >
%$\ahh$
%</text>
%<text text-vert-align= "center-v"
%	 stroke-width= "0.5"
%	 anchor-point= "(6.88,-16.88)"
%	 text-frame= "noframe"
%	 fill-style= "none"
%	 text-hor-align= "center-h"
%	 >
%$\aah$
%</text>
%<multicurve stroke-width= "0.5"
%	 points= "(18.75,-25);(18.75,-25);(18.75,-3.12);(18.75,-3.12)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.5"
%	 points= "(1.88,6.88);(1.88,6.88);(1.88,-3.12);(1.88,-3.12);(1.88,-3.12);(23.12,-3.13);
%	(23.12,-3.13);(23.12,-3.13);(23.12,6.87);(23.12,6.87);(23.12,6.87);(5.62,6.87);
%	(5.62,6.87);(5.62,6.87);(23.12,6.87);(23.12,6.87);(23.12,6.87);(5.62,6.87);
%	(5.62,6.87);(5.62,6.87);(1.88,6.87);(1.88,6.87)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.5"
%	 points= "(6.88,6.88);(6.88,6.88);(6.88,30);(6.88,30)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.5"
%	 points= "(6.88,-25.62);(6.88,-25.62);(6.88,-21.88);(6.88,-21.88)"
%	 fill-style= "none"
%	 />
%<text text-vert-align= "center-v"
%	 stroke-width= "0.5"
%	 anchor-point= "(6.88,-28.75)"
%	 text-frame= "noframe"
%	 fill-style= "none"
%	 text-hor-align= "center-h"
%	 >
%$\xxh$
%</text>
%<text text-vert-align= "center-v"
%	 stroke-width= "0.5"
%	 anchor-point= "(5.62,-6.88)"
%	 text-frame= "noframe"
%	 fill-style= "none"
%	 text-hor-align= "right"
%	 >
%$\RRsmall$
%</text>
%<text text-vert-align= "center-v"
%	 stroke-width= "0.5"
%	 anchor-point= "(18.75,-28.75)"
%	 text-frame= "noframe"
%	 fill-style= "none"
%	 text-hor-align= "center-h"
%	 >
%$\bhh$
%</text>
%<text text-vert-align= "center-v"
%	 stroke-width= "0.5"
%	 anchor-point= "(6.88,33.12)"
%	 text-frame= "noframe"
%	 fill-style= "none"
%	 text-hor-align= "center-h"
%	 >
%$\RRsmall$
%</text>
%<multicurve stroke-width= "0.5"
%	 points= "(1.88,-11.88);(1.88,-11.88);(1.88,-21.88);(1.88,-21.88);(1.88,-21.88);(11.86,-21.88);
%	(11.86,-21.88);(11.86,-21.88);(11.86,-11.88);(11.86,-11.88);(11.86,-11.88);(5.62,-11.88);
%	(5.62,-11.88);(5.62,-11.88);(11.86,-11.88);(11.86,-11.88);(11.86,-11.88);(5.62,-11.88);
%	(5.62,-11.88);(5.62,-11.88);(1.88,-11.88);(1.88,-11.88)"
%	 fill-style= "none"
%	 />
%<ellipse p3= "(7.97,-12.97)"
%	 p2= "(7.97,-10.78)"
%	 stroke-width= "0.5"
%	 p1= "(5.78,-10.78)"
%	 closure= "open"
%	 angle-end= "360"
%	 fill-style= "solid"
%	 angle-start= "0"
%	 />
%</jpic>
%%End JPIC-XML
%PSTricks content-type (pstricks.sty package needed)
%Add \usepackage{pstricks} in the preamble of your LaTeX file
%You can rescale the whole picture (to 80% for instance) by using the command \def\JPicScale{0.8}
\ifx\JPicScale\undefined\def\JPicScale{1}\fi
\psset{unit=\JPicScale mm}
\psset{linewidth=0.3,dotsep=1,hatchwidth=0.3,hatchsep=1.5,shadowsize=1,dimen=middle}
\psset{dotsize=0.7 2.5,dotscale=1 1,fillcolor=black}
\psset{arrowsize=1 2,arrowlength=1,arrowinset=0.25,tbarsize=0.7 5,bracketlength=0.15,rbracketlength=0.15}
\begin{pspicture}(0,0)(23.12,33.12)
\rput(18.75,33.12){$\dh$}
\psline[linewidth=0.5](6.88,-11.88)(6.88,-3.12)
\psline[linewidth=0.5](18.88,6.87)(18.75,30)
\rput(12.5,1.88){$\ahh$}
\rput(6.88,-16.88){$\aah$}
\psline[linewidth=0.5](18.75,-25)(18.75,-3.12)
\psline[linewidth=0.5](1.88,6.88)
(1.88,-3.12)
(23.12,-3.13)
(23.12,6.87)
(5.62,6.87)
(23.12,6.87)
(5.62,6.87)(1.88,6.87)
\psline[linewidth=0.5](6.88,6.88)(6.88,30)
\psline[linewidth=0.5](6.88,-25.62)(6.88,-21.88)
\rput(6.88,-28.75){$\xxh$}
\rput[r](5.62,-6.88){$\RRsmall$}
\rput(18.75,-28.75){$\bhh$}
\rput(6.88,33.12){$\RRsmall$}
\psline[linewidth=0.5](1.88,-11.88)
(1.88,-21.88)
(11.86,-21.88)
(11.86,-11.88)
(5.62,-11.88)
(11.86,-11.88)
(5.62,-11.88)(1.88,-11.88)
\rput{0}(6.88,-11.88){\psellipse[linewidth=0.5,fillstyle=solid](0,0)(1.09,-1.09)}
\end{pspicture}


==> PIC/uni-mach-t-stream.tex <==
%%Created by jPicEdt 1.4.1_03: mixed JPIC-XML/LaTeX format
%%Thu Sep 21 08:05:33 HST 2017
%%Begin JPIC-XML
%<?xml version="1.0" standalone="yes"?>
%<jpic x-min="0" x-max="20" y-min="-20" y-max="27.5" auto-bounding="true">
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(15,27.5)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\dh$
%</text>
%<multicurve fill-style= "none"
%	 points= "(15,7.5);(15,7.5);(15,23.75);(15,23.75)"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(10,0)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\ahh$
%</text>
%<multicurve fill-style= "none"
%	 points= "(10,-16.25);(10,-16.25);(10,-7.5);(10,-7.5)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(5,7.5);(5,7.5);(5,12.5);(5,12.5)"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(10,-20)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\xxh$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(4.38,10)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\xxh$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(5,27.5)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\RRsmall$
%</text>
%<multicurve fill-style= "none"
%	 points= "(20,-7.5);(20,-7.5);(0,-7.5);(0,-7.5)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(20,7.5);(20,7.5);(0,7.5);(0,7.5)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(20,7.5);(20,7.5);(20,-7.5);(20,-7.5)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(0,7.5);(0,7.5);(0,-7.5);(0,-7.5)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(5,18.75);(5,18.75);(5,23.75);(5,23.75)"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(3.75,15.62)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\aah$
%</text>
%<multicurve fill-style= "none"
%	 points= "(0,12.5);(0,12.5);(11.25,12.5);(11.25,12.5)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(0,23.75);(0,23.75);(11.25,12.5);(11.25,12.5)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(0,23.75);(0,23.75);(0,12.5);(0,12.5)"
%	 />
%</jpic>
%%End JPIC-XML
%PSTricks content-type (pstricks.sty package needed)
%Add \usepackage{pstricks} in the preamble of your LaTeX file
%You can rescale the whole picture (to 80% for instance) by using the command \def\JPicScale{0.8}
\ifx\JPicScale\undefined\def\JPicScale{1}\fi
\psset{unit=\JPicScale mm}
\psset{linewidth=0.3,dotsep=1,hatchwidth=0.3,hatchsep=1.5,shadowsize=1,dimen=middle}
\psset{dotsize=0.7 2.5,dotscale=1 1,fillcolor=black}
\psset{arrowsize=1 2,arrowlength=1,arrowinset=0.25,tbarsize=0.7 5,bracketlength=0.15,rbracketlength=0.15}
\begin{pspicture}(0,0)(20,27.5)
\rput(15,27.5){$\dh$}
\psline(15,7.5)(15,23.75)
\rput(10,0){$\ahh$}
\psline(10,-16.25)(10,-7.5)
\psline(5,7.5)(5,12.5)
\rput(10,-20){$\xxh$}
\rput[r](4.38,10){$\xxh$}
\rput(5,27.5){$\RRsmall$}
\psline(20,-7.5)(0,-7.5)
\psline(20,7.5)(0,7.5)
\psline(20,7.5)(20,-7.5)
\psline(0,7.5)(0,-7.5)
\psline(5,18.75)(5,23.75)
\rput(3.75,15.62){$\aah$}
\psline(0,12.5)(11.25,12.5)
\psline(0,23.75)(11.25,12.5)
\psline(0,23.75)(0,12.5)
\end{pspicture}


==> PIC/uni-mach-t.tex <==
%%Created by jPicEdt 1.4.1_03: mixed JPIC-XML/LaTeX format
%%Wed Dec 25 19:28:09 GMT-10:00 2019
%%Begin JPIC-XML
%<?xml version="1.0" standalone="yes"?>
%<jpic x-min="-1.88" x-max="20" y-min="-6.25" y-max="44.38" auto-bounding="true">
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(15,44.38)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\dh$
%</text>
%<multicurve fill-style= "none"
%	 points= "(15.62,-2.5);(15.62,-2.5);(15.62,11.88);(15.62,11.88)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(15,21.88);(15,21.88);(15,41.25);(15,41.25)"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(8.75,16.88)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\ahh$
%</text>
%<multicurve fill-style= "none"
%	 points= "(-1.88,18.12);(-1.88,18.12);(-1.88,11.88);(-1.88,11.88);(-1.88,11.88);(20,11.88);
%	(20,11.88);(20,11.88);(20,21.88);(20,21.88);(20,21.88);(-1.88,21.88);
%	(-1.88,21.88);(-1.88,21.88);(16.25,21.86);(16.25,21.86);(16.25,21.86);(-1.88,21.88);
%	(-1.88,21.88);(-1.88,21.88);(-1.88,18.12);(-1.88,18.12)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(3.12,-3.12);(3.12,-3.12);(3.12,11.88);(3.12,11.88)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(3.12,21.88);(3.12,21.88);(3.12,30.62);(3.12,30.62)"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(3.12,-6.25)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\xxh$
%</text>
%<multicurve fill-style= "none"
%	 points= "(3.12,36.25);(3.12,36.25);(3.12,41.25);(3.12,41.25)"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(1.5,33.88)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\aah$
%</text>
%<multicurve fill-style= "none"
%	 points= "(-1.62,40.74);(-1.62,40.74);(8.36,30.75);(8.36,30.75);(8.36,30.75);(-1.62,30.75);
%	(-1.62,30.75);(-1.62,30.75);(-1.62,40.74)"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(1.88,26.25)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\xxh$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(15.62,-6.25)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\bhh$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(3.12,44.38)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\RRsmall$
%</text>
%</jpic>
%%End JPIC-XML
%PSTricks content-type (pstricks.sty package needed)
%Add \usepackage{pstricks} in the preamble of your LaTeX file
%You can rescale the whole picture (to 80% for instance) by using the command \def\JPicScale{0.8}
\ifx\JPicScale\undefined\def\JPicScale{1}\fi
\psset{unit=\JPicScale mm}
\psset{linewidth=0.3,dotsep=1,hatchwidth=0.3,hatchsep=1.5,shadowsize=1,dimen=middle}
\psset{dotsize=0.7 2.5,dotscale=1 1,fillcolor=black}
\psset{arrowsize=1 2,arrowlength=1,arrowinset=0.25,tbarsize=0.7 5,bracketlength=0.15,rbracketlength=0.15}
\begin{pspicture}(0,0)(20,44.38)
\rput(15,44.38){$\dh$}
\psline(15.62,-2.5)(15.62,11.88)
\psline(15,21.88)(15,41.25)
\rput(8.75,16.88){$\ahh$}
\psline(-1.88,18.12)
(-1.88,11.88)
(20,11.88)
(20,21.88)
(-1.88,21.88)
(16.25,21.86)
(-1.88,21.88)(-1.88,18.12)
\psline(3.12,-3.12)(3.12,11.88)
\psline(3.12,21.88)(3.12,30.62)
\rput(3.12,-6.25){$\xxh$}
\psline(3.12,36.25)(3.12,41.25)
\rput(1.5,33.88){$\aah$}
\pspolygon(-1.62,40.74)
(8.36,30.75)
(-1.62,30.75)(-1.62,40.74)
\rput[r](1.88,26.25){$\xxh$}
\rput(15.62,-6.25){$\bhh$}
\rput(3.12,44.38){$\RRsmall$}
\end{pspicture}


==> PIC/uniform-1.tex <==
%%Created by jPicEdt 1.4.1_03: mixed JPIC-XML/LaTeX format
%%Tue Dec 08 16:33:52 GMT-10:00 2020
%%Begin JPIC-XML
%<?xml version="1.0" standalone="yes"?>
%<jpic x-min="0" x-max="490" y-min="0" y-max="75" auto-bounding="true">
%<multicurve fill-style= "none"
%	 points= "(450,50);(450,50);(490,50);(490,50)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(490,30);(490,30);(490,50);(490,50)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(480,60);(480,60);(480,50);(480,50)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(470,30);(470,30);(490,30);(490,30)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(480,30);(480,30);(480,15);(480,15)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(460,40);(460,40);(460,0);(460,0)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(450,50);(450,50);(470,30);(470,30)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(470,25);(470,25);(490,5);(490,5)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(470,5);(470,5);(489.38,5);(489.38,5)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(470,5);(470,5);(470,24.99);(470,24.99)"
%	 stroke-width= "0.75"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(435,40)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\EQLS$
%</text>
%<multicurve fill-style= "none"
%	 points= "(260,50);(260,50);(300,50);(300,50)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(300,30);(300,30);(300,50);(300,50)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(290,60);(290,60);(290,50);(290,50)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(280,30);(280,30);(300,30);(300,30)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(290,30);(290,30);(290,15);(290,15)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(270,40);(270,40);(270,0);(270,0)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(260,50);(260,50);(280,30);(280,30)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(280,25);(280,25);(300,5);(300,5)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(280,5);(280,5);(299.38,5);(299.38,5)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(280,5);(280,5);(280,24.99);(280,24.99)"
%	 stroke-width= "0.75"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(245,40)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\EQLS$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(285,10)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\toptag$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(475,10)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\bottag$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(475,40)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\utag$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(285,40)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\utag$
%</text>
%<multicurve fill-style= "none"
%	 points= "(400,30);(400,30);(400,0);(400,0)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(380,50);(380,50);(420,50);(420,50)"
%	 stroke-width= "0.6"
%	 />
%<multicurve fill-style= "none"
%	 points= "(420,30);(420,30);(420,50);(420,50)"
%	 stroke-width= "0.6"
%	 />
%<multicurve fill-style= "none"
%	 points= "(380,30);(380,30);(420,30);(420,30)"
%	 stroke-width= "0.6"
%	 />
%<multicurve fill-style= "none"
%	 points= "(380,50);(380,50);(380,30);(380,30)"
%	 stroke-width= "0.6"
%	 />
%<multicurve fill-style= "none"
%	 points= "(400,60);(400,60);(400,50);(400,50)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(210,30);(210,30);(210,0);(210,0)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(190,50);(190,50);(230,50);(230,50)"
%	 stroke-width= "0.6"
%	 />
%<multicurve fill-style= "none"
%	 points= "(230,30);(230,30);(230,50);(230,50)"
%	 stroke-width= "0.6"
%	 />
%<multicurve fill-style= "none"
%	 points= "(190,30);(190,30);(230,30);(230,30)"
%	 stroke-width= "0.6"
%	 />
%<multicurve fill-style= "none"
%	 points= "(190,50);(190,50);(190,30);(190,30)"
%	 stroke-width= "0.6"
%	 />
%<multicurve fill-style= "none"
%	 points= "(210,60);(210,60);(210,50);(210,50)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(20,30);(20,30);(20,0);(20,0)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(0,50);(0,50);(40,50);(40,50)"
%	 stroke-width= "0.6"
%	 />
%<multicurve fill-style= "none"
%	 points= "(40,30);(40,30);(40,50);(40,50)"
%	 stroke-width= "0.6"
%	 />
%<multicurve fill-style= "none"
%	 points= "(0,30);(0,30);(40,30);(40,30)"
%	 stroke-width= "0.6"
%	 />
%<multicurve fill-style= "none"
%	 points= "(0,50);(0,50);(0,30);(0,30)"
%	 stroke-width= "0.6"
%	 />
%<multicurve fill-style= "none"
%	 points= "(20,60);(20,60);(20,50);(20,50)"
%	 stroke-width= "0.75"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(20,40)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\sucetag$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(400,40)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\predtag$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(210,40)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\zerotag$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(92.5,10)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\bottag$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(55,40)"
%	 text-frame= "noframe"
%	 stroke-width= "0.75"
%	 text-hor-align= "center-h"
%	 >
%\EQLS
%</text>
%<multicurve fill-style= "none"
%	 points= "(85,5);(85,5);(105,5);(105,5)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(85,5);(85,5);(85,25);(85,25)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(85,25);(85,25);(105,5);(105,5)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(70,50);(70,50);(97.5,50);(97.5,50)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(117.5,30);(117.5,30);(97.5,50);(97.5,50)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(107.5,60);(107.5,60);(107.5,40);(107.5,40)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(90,30);(90,30);(117.5,30);(117.5,30)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(95,30);(95,30);(95,15);(95,15)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(80,40);(80,40);(70,30);(70,30)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(70,50);(70,50);(90,30);(90,30)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(60,25);(60,25);(80,5);(80,5)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(60,5);(60,5);(79.38,5);(79.38,5)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(60,5);(60,5);(60,24.99);(60,24.99)"
%	 stroke-width= "0.75"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(65,10)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\iiftag$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(95,40)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\stag$
%</text>
%<multicurve fill-style= "none"
%	 points= "(70,30);(70,30);(70,15);(70,15)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(112.5,30);(112.5,30);(112.5,0);(112.5,0)"
%	 stroke-width= "0.75"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(435,75)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\predeq$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(245,75)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\zeroeq$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(55,75)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\suceq$
%</text>
%</jpic>
%%End JPIC-XML
%LaTeX-picture environment using emulated lines and arcs
%You can rescale the whole picture (to 80% for instance) by using the command \def\JPicScale{0.8}
\ifx\JPicScale\undefined\def\JPicScale{1}\fi
\unitlength \JPicScale mm
\begin{picture}(490,75)(0,0)
\linethickness{0.75mm}
\put(450,50){\line(1,0){40}}
\linethickness{0.75mm}
\put(490,30){\line(0,1){20}}
\linethickness{0.75mm}
\put(480,50){\line(0,1){10}}
\linethickness{0.75mm}
\put(470,30){\line(1,0){20}}
\linethickness{0.75mm}
\put(480,15){\line(0,1){15}}
\linethickness{0.75mm}
\put(460,0){\line(0,1){40}}
\linethickness{0.75mm}
\multiput(450,50)(0.12,-0.12){167}{\line(1,0){0.12}}
\linethickness{0.75mm}
\multiput(470,25)(0.12,-0.12){167}{\line(1,0){0.12}}
\linethickness{0.75mm}
\put(470,5){\line(1,0){19.38}}
\linethickness{0.75mm}
\put(470,5){\line(0,1){19.99}}
\put(435,40){\makebox(0,0)[cc]{$\EQLS$}}

\linethickness{0.75mm}
\put(260,50){\line(1,0){40}}
\linethickness{0.75mm}
\put(300,30){\line(0,1){20}}
\linethickness{0.75mm}
\put(290,50){\line(0,1){10}}
\linethickness{0.75mm}
\put(280,30){\line(1,0){20}}
\linethickness{0.75mm}
\put(290,15){\line(0,1){15}}
\linethickness{0.75mm}
\put(270,0){\line(0,1){40}}
\linethickness{0.75mm}
\multiput(260,50)(0.12,-0.12){167}{\line(1,0){0.12}}
\linethickness{0.75mm}
\multiput(280,25)(0.12,-0.12){167}{\line(1,0){0.12}}
\linethickness{0.75mm}
\put(280,5){\line(1,0){19.38}}
\linethickness{0.75mm}
\put(280,5){\line(0,1){19.99}}
\put(245,40){\makebox(0,0)[cc]{$\EQLS$}}

\put(285,10){\makebox(0,0)[cc]{$\toptag$}}

\put(475,10){\makebox(0,0)[cc]{$\bottag$}}

\put(475,40){\makebox(0,0)[cc]{$\utag$}}

\put(285,40){\makebox(0,0)[cc]{$\utag$}}

\linethickness{0.75mm}
\put(400,0){\line(0,1){30}}
\linethickness{0.6mm}
\put(380,50){\line(1,0){40}}
\linethickness{0.6mm}
\put(420,30){\line(0,1){20}}
\linethickness{0.6mm}
\put(380,30){\line(1,0){40}}
\linethickness{0.6mm}
\put(380,30){\line(0,1){20}}
\linethickness{0.75mm}
\put(400,50){\line(0,1){10}}
\linethickness{0.75mm}
\put(210,0){\line(0,1){30}}
\linethickness{0.6mm}
\put(190,50){\line(1,0){40}}
\linethickness{0.6mm}
\put(230,30){\line(0,1){20}}
\linethickness{0.6mm}
\put(190,30){\line(1,0){40}}
\linethickness{0.6mm}
\put(190,30){\line(0,1){20}}
\linethickness{0.75mm}
\put(210,50){\line(0,1){10}}
\linethickness{0.75mm}
\put(20,0){\line(0,1){30}}
\linethickness{0.6mm}
\put(0,50){\line(1,0){40}}
\linethickness{0.6mm}
\put(40,30){\line(0,1){20}}
\linethickness{0.6mm}
\put(0,30){\line(1,0){40}}
\linethickness{0.6mm}
\put(0,30){\line(0,1){20}}
\linethickness{0.75mm}
\put(20,50){\line(0,1){10}}
\put(20,40){\makebox(0,0)[cc]{$\sucetag$}}

\put(400,40){\makebox(0,0)[cc]{$\predtag$}}

\put(210,40){\makebox(0,0)[cc]{$\zerotag$}}

\put(92.5,10){\makebox(0,0)[cc]{$\bottag$}}

\put(55,40){\makebox(0,0)[cc]{\EQLS}}

\linethickness{0.75mm}
\put(85,5){\line(1,0){20}}
\linethickness{0.75mm}
\put(85,5){\line(0,1){20}}
\linethickness{0.75mm}
\multiput(85,25)(0.12,-0.12){167}{\line(1,0){0.12}}
\linethickness{0.75mm}
\put(70,50){\line(1,0){27.5}}
\linethickness{0.75mm}
\multiput(97.5,50)(0.12,-0.12){167}{\line(1,0){0.12}}
\linethickness{0.75mm}
\put(107.5,40){\line(0,1){20}}
\linethickness{0.75mm}
\put(90,30){\line(1,0){27.5}}
\linethickness{0.75mm}
\put(95,15){\line(0,1){15}}
\linethickness{0.75mm}
\multiput(70,30)(0.12,0.12){83}{\line(1,0){0.12}}
\linethickness{0.75mm}
\multiput(70,50)(0.12,-0.12){167}{\line(1,0){0.12}}
\linethickness{0.75mm}
\multiput(60,25)(0.12,-0.12){167}{\line(1,0){0.12}}
\linethickness{0.75mm}
\put(60,5){\line(1,0){19.38}}
\linethickness{0.75mm}
\put(60,5){\line(0,1){19.99}}
\put(65,10){\makebox(0,0)[cc]{$\iiftag$}}

\put(95,40){\makebox(0,0)[cc]{$\stag$}}

\linethickness{0.75mm}
\put(70,15){\line(0,1){15}}
\linethickness{0.75mm}
\put(112.5,0){\line(0,1){30}}
\put(435,75){\makebox(0,0)[cc]{$\predeq$}}

\put(245,75){\makebox(0,0)[cc]{$\zeroeq$}}

\put(55,75){\makebox(0,0)[cc]{$\suceq$}}

\end{picture}


==> PIC/uniform-collapse.tex <==
%%Created by jPicEdt 1.4.1_03: mixed JPIC-XML/LaTeX format
%%Sat Oct 08 23:50:16 GMT-10:00 2022
%%Begin JPIC-XML
%<?xml version="1.0" standalone="yes"?>
%<jpic x-min="0" x-max="352.5" y-min="0" y-max="246.25" auto-bounding="true">
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 stroke-width= "0.35"
%	 anchor-point= "(35,216.25)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\universal$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 stroke-width= "0.35"
%	 anchor-point= "(7.5,140)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\Progtype$
%</text>
%<multicurve fill-style= "none"
%	 points= "(50,230);(50,230);(50,205);(50,205)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(50,205);(50,205);(20,205);(20,205)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(20,205);(20,205);(0,225);(0,225)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(0,225);(0,225);(0,230);(0,230)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(0,230);(0,230);(50,230);(50,230)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "1"
%	 points= "(10,215);(10,215);(10,140);(10,140)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(50,170);(50,170);(20,170);(20,170)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(20,200);(20,200);(20,170);(20,170)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(20,200);(20,200);(50,170);(50,170)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "1"
%	 points= "(35,205);(35,205);(35,185);(35,185)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "1"
%	 points= "(35,246.25);(35,246.25);(35,230);(35,230)"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 stroke-width= "0.35"
%	 anchor-point= "(38.75,246.25)"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\Progtype$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 stroke-width= "0.35"
%	 anchor-point= "(37.5,195)"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\Progtype$
%</text>
%<multicurve fill-style= "none"
%	 points= "(42.5,170);(42.5,170);(42.5,140);(42.5,140)"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 stroke-width= "0.35"
%	 anchor-point= "(75,217.5)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\eqlsb$
%</text>
%<multicurve fill-style= "none"
%	 points= "(27.5,170);(27.5,170);(27.5,140);(27.5,140)"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 stroke-width= "0.35"
%	 anchor-point= "(135,216.25)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\universal$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 stroke-width= "0.35"
%	 anchor-point= "(107.5,140)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\Progtype$
%</text>
%<multicurve fill-style= "none"
%	 points= "(150,230);(150,230);(150,205);(150,205)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(150,205);(150,205);(120,205);(120,205)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(120,205);(120,205);(100,225);(100,225)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(100,225);(100,225);(100,230);(100,230)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(100,230);(100,230);(150,230);(150,230)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.8"
%	 points= "(110,215);(110,215);(110,140);(110,140)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(142.5,205);(142.5,205);(142.5,140);(142.5,140)"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 stroke-width= "0.35"
%	 anchor-point= "(175,217.5)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\eqlsb$
%</text>
%<multicurve fill-style= "none"
%	 points= "(127.5,205);(127.5,205);(127.5,140);(127.5,140)"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 stroke-width= "0.35"
%	 anchor-point= "(275,217.5)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\eqlsb$
%</text>
%<multicurve fill-style= "none"
%	 stroke-width= "0.8"
%	 points= "(135,105);(135,105);(135,90);(135,90)"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 stroke-width= "0.35"
%	 anchor-point= "(138.75,103.75)"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\Progtype$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 stroke-width= "0.35"
%	 anchor-point= "(175,77.5)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\eqlsb$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 stroke-width= "0.35"
%	 anchor-point= "(235,76.25)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\universal$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 stroke-width= "0.35"
%	 anchor-point= "(207.5,67.5)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\Progtype$
%</text>
%<multicurve fill-style= "none"
%	 points= "(250,90);(250,90);(250,65);(250,65)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(250,65);(250,65);(220,65);(220,65)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(220,65);(220,65);(200,85);(200,85)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(200,85);(200,85);(200,90);(200,90)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(200,90);(200,90);(250,90);(250,90)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.8"
%	 points= "(210,75);(210,75);(210,0);(210,0)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.8"
%	 points= "(235,105);(235,105);(235,90);(235,90)"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 stroke-width= "0.35"
%	 anchor-point= "(238.75,103.75)"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\Progtype$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 stroke-width= "0.35"
%	 anchor-point= "(275,77.5)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\eqlsb$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 stroke-width= "0.35"
%	 anchor-point= "(335,76.25)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\universal$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 stroke-width= "0.35"
%	 anchor-point= "(307.5,67.5)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\Progtype$
%</text>
%<multicurve fill-style= "none"
%	 points= "(350,90);(350,90);(350,65);(350,65)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(350,65);(350,65);(320,65);(320,65)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(320,65);(320,65);(300,85);(300,85)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(300,85);(300,85);(300,90);(300,90)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(300,90);(300,90);(350,90);(350,90)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.8"
%	 points= "(310,75);(310,75);(310,0);(310,0)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(350,30);(350,30);(320,30);(320,30)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(320,60);(320,60);(320,30);(320,30)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(320,60);(320,60);(350,30);(350,30)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.8"
%	 points= "(335,65);(335,65);(335,45);(335,45)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.8"
%	 points= "(335,105);(335,105);(335,90);(335,90)"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 stroke-width= "0.35"
%	 anchor-point= "(338.75,103.75)"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\Progtype$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 stroke-width= "0.35"
%	 anchor-point= "(337.5,60)"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\Progtype$
%</text>
%<multicurve fill-style= "none"
%	 stroke-width= "0.8"
%	 points= "(345,30);(345,30);(345,15);(345,15)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.8"
%	 points= "(325,30);(325,30);(325,15);(325,15)"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 stroke-width= "0.35"
%	 anchor-point= "(75,77.5)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\eqlsb$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 stroke-width= "0.35"
%	 anchor-point= "(237.5,216.25)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\universal$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 stroke-width= "0.35"
%	 anchor-point= "(207.5,140)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\Progtype$
%</text>
%<multicurve fill-style= "none"
%	 points= "(250,230);(250,230);(250,205);(250,205)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(250,205);(250,205);(235,205);(235,205)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(235,205);(235,205);(210,230);(210,230)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(210,230);(210,230);(250,230);(250,230)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.8"
%	 points= "(210,200);(210,200);(210,140);(210,140)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(242.5,205);(242.5,205);(242.5,140);(242.5,140)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(227.5,190);(227.5,190);(227.5,140);(227.5,140)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(220,190);(220,190);(200,210);(200,210)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(200,210);(200,210);(200,215);(200,215)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(235,190);(235,190);(220,190);(220,190)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(235,190);(235,190);(210,215);(210,215)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(210,215);(210,215);(200,215);(200,215)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.8"
%	 points= "(222.5,217.5);(222.5,217.5);(222.5,202.5);(222.5,202.5)"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 stroke-width= "0.35"
%	 anchor-point= "(137.5,76.25)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\universal$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 stroke-width= "0.35"
%	 anchor-point= "(107.5,0)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\Progtype$
%</text>
%<multicurve fill-style= "none"
%	 points= "(150,90);(150,90);(150,65);(150,65)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(150,65);(150,65);(135,65);(135,65)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(135,65);(135,65);(110,90);(110,90)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(110,90);(110,90);(150,90);(150,90)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.8"
%	 points= "(110,60);(110,60);(110,0);(110,0)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(120,50);(120,50);(100,70);(100,70)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(100,70);(100,70);(100,75);(100,75)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(135,50);(135,50);(120,50);(120,50)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(135,50);(135,50);(110,75);(110,75)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(110,75);(110,75);(100,75);(100,75)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.8"
%	 points= "(122.5,77.5);(122.5,77.5);(122.5,62.5);(122.5,62.5)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(352.5,7.5);(352.5,7.5);(337.5,7.5);(337.5,7.5)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(337.5,22.5);(337.5,22.5);(337.5,7.5);(337.5,7.5)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(337.5,22.5);(337.5,22.5);(352.5,7.5);(352.5,7.5)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(332.5,7.5);(332.5,7.5);(317.5,7.5);(317.5,7.5)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(317.5,22.5);(317.5,22.5);(317.5,7.5);(317.5,7.5)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(317.5,22.5);(317.5,22.5);(332.5,7.5);(332.5,7.5)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(345,7.5);(345,7.5);(345,0);(345,0)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(325,7.5);(325,7.5);(325,0);(325,0)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.8"
%	 points= "(245,65);(245,65);(245,37.5);(245,37.5)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.8"
%	 points= "(225,65);(225,65);(225,37.5);(225,37.5)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(252.5,30);(252.5,30);(237.5,30);(237.5,30)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(237.5,45);(237.5,45);(237.5,30);(237.5,30)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(237.5,45);(237.5,45);(252.5,30);(252.5,30)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(232.5,30);(232.5,30);(217.5,30);(217.5,30)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(217.5,45);(217.5,45);(217.5,30);(217.5,30)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(217.5,45);(217.5,45);(232.5,30);(232.5,30)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(245,30);(245,30);(245,0);(245,0)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(225,30);(225,30);(225,0);(225,0)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.8"
%	 points= "(145,65);(145,65);(145,37.5);(145,37.5)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-width= "0.8"
%	 points= "(127.5,50);(127.5,50);(127.5,22.5);(127.5,22.5)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(152.5,30);(152.5,30);(137.5,30);(137.5,30)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(137.5,45);(137.5,45);(137.5,30);(137.5,30)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(137.5,45);(137.5,45);(152.5,30);(152.5,30)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(135,15);(135,15);(120,15);(120,15)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(120,30);(120,30);(120,15);(120,15)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(120,30);(120,30);(135,15);(135,15)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(145,30);(145,30);(145,0);(145,0)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(127.5,15);(127.5,15);(127.5,0);(127.5,0)"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(322.5,11.25)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\encon$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(343.75,11.25)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\encon$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(222.5,33.75)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\encon$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(242.5,33.75)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\encon$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(125,18.75)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\encon$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(142.5,33.75)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\encon$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 stroke-width= "0.35"
%	 anchor-point= "(207.5,0)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\Progtype$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 stroke-width= "0.35"
%	 anchor-point= "(307.5,0)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\Progtype$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(26.25,140)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\Xee$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(125,140)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\Xee$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(225,140)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\Xee$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(125,0)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\Xee$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(222.5,0)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\Xee$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(322.5,0)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\Xee$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(342.5,0)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\Ahh$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(240,140)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\Ahh$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(140,140)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\Ahh$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(40,140)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\Ahh$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(115,62.5)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\artial$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(242.5,0)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\Ahh$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(142.5,0)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\Ahh$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(225,37.5)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\Dottt
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(245,37.5)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\Dottt
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(335,45)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\Dottt
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(325,17.5)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\Dottt
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(345,15)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\Dottt
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(122.5,62.5)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\Dottt
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(145,37.5)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\Dottt
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(127.5,22.5)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\Dottt
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(35,185)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\Dottt
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(222.5,202.5)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\Dottt
%</text>
%<multicurve fill-style= "none"
%	 stroke-width= "0.8"
%	 points= "(135,246.25);(135,246.25);(135,230);(135,230)"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 stroke-width= "0.35"
%	 anchor-point= "(138.75,246.25)"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\Progtype$
%</text>
%<multicurve fill-style= "none"
%	 stroke-width= "0.8"
%	 points= "(235,246.25);(235,246.25);(235,230);(235,230)"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 stroke-width= "0.35"
%	 anchor-point= "(238.75,246.25)"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\Progtype$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(215,202.5)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\artial$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(31.25,176.25)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\bigencon$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(331.25,36.25)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\bigencon$
%</text>
%</jpic>
%%End JPIC-XML
%LaTeX-picture environment using emulated lines and arcs
%You can rescale the whole picture (to 80% for instance) by using the command \def\JPicScale{0.8}
\ifx\JPicScale\undefined\def\JPicScale{1}\fi
\unitlength \JPicScale mm
\begin{picture}(352.5,246.25)(0,0)
\put(35,216.25){\makebox(0,0)[cc]{$\universal$}}

\put(7.5,140){\makebox(0,0)[cr]{$\Progtype$}}

\linethickness{0.3mm}
\put(50,205){\line(0,1){25}}
\linethickness{0.3mm}
\put(20,205){\line(1,0){30}}
\linethickness{0.3mm}
\multiput(0,225)(0.12,-0.12){167}{\line(1,0){0.12}}
\linethickness{0.3mm}
\put(0,225){\line(0,1){5}}
\linethickness{0.3mm}
\put(0,230){\line(1,0){50}}
\linethickness{1mm}
\put(10,140){\line(0,1){75}}
\linethickness{0.3mm}
\put(20,170){\line(1,0){30}}
\linethickness{0.3mm}
\put(20,170){\line(0,1){30}}
\linethickness{0.3mm}
\multiput(20,200)(0.12,-0.12){250}{\line(1,0){0.12}}
\linethickness{1mm}
\put(35,185){\line(0,1){20}}
\linethickness{1mm}
\put(35,230){\line(0,1){16.25}}
\put(38.75,246.25){\makebox(0,0)[cl]{$\Progtype$}}

\put(37.5,195){\makebox(0,0)[cl]{$\Progtype$}}

\linethickness{0.3mm}
\put(42.5,140){\line(0,1){30}}
\put(75,217.5){\makebox(0,0)[cc]{$\eqlsb$}}

\linethickness{0.3mm}
\put(27.5,140){\line(0,1){30}}
\put(135,216.25){\makebox(0,0)[cc]{$\universal$}}

\put(107.5,140){\makebox(0,0)[cr]{$\Progtype$}}

\linethickness{0.3mm}
\put(150,205){\line(0,1){25}}
\linethickness{0.3mm}
\put(120,205){\line(1,0){30}}
\linethickness{0.3mm}
\multiput(100,225)(0.12,-0.12){167}{\line(1,0){0.12}}
\linethickness{0.3mm}
\put(100,225){\line(0,1){5}}
\linethickness{0.3mm}
\put(100,230){\line(1,0){50}}
\linethickness{0.8mm}
\put(110,140){\line(0,1){75}}
\linethickness{0.3mm}
\put(142.5,140){\line(0,1){65}}
\put(175,217.5){\makebox(0,0)[cc]{$\eqlsb$}}

\linethickness{0.3mm}
\put(127.5,140){\line(0,1){65}}
\put(275,217.5){\makebox(0,0)[cc]{$\eqlsb$}}

\linethickness{0.8mm}
\put(135,90){\line(0,1){15}}
\put(138.75,103.75){\makebox(0,0)[cl]{$\Progtype$}}

\put(175,77.5){\makebox(0,0)[cc]{$\eqlsb$}}

\put(235,76.25){\makebox(0,0)[cc]{$\universal$}}

\put(207.5,67.5){\makebox(0,0)[cr]{$\Progtype$}}

\linethickness{0.3mm}
\put(250,65){\line(0,1){25}}
\linethickness{0.3mm}
\put(220,65){\line(1,0){30}}
\linethickness{0.3mm}
\multiput(200,85)(0.12,-0.12){167}{\line(1,0){0.12}}
\linethickness{0.3mm}
\put(200,85){\line(0,1){5}}
\linethickness{0.3mm}
\put(200,90){\line(1,0){50}}
\linethickness{0.8mm}
\put(210,0){\line(0,1){75}}
\linethickness{0.8mm}
\put(235,90){\line(0,1){15}}
\put(238.75,103.75){\makebox(0,0)[cl]{$\Progtype$}}

\put(275,77.5){\makebox(0,0)[cc]{$\eqlsb$}}

\put(335,76.25){\makebox(0,0)[cc]{$\universal$}}

\put(307.5,67.5){\makebox(0,0)[cr]{$\Progtype$}}

\linethickness{0.3mm}
\put(350,65){\line(0,1){25}}
\linethickness{0.3mm}
\put(320,65){\line(1,0){30}}
\linethickness{0.3mm}
\multiput(300,85)(0.12,-0.12){167}{\line(1,0){0.12}}
\linethickness{0.3mm}
\put(300,85){\line(0,1){5}}
\linethickness{0.3mm}
\put(300,90){\line(1,0){50}}
\linethickness{0.8mm}
\put(310,0){\line(0,1){75}}
\linethickness{0.3mm}
\put(320,30){\line(1,0){30}}
\linethickness{0.3mm}
\put(320,30){\line(0,1){30}}
\linethickness{0.3mm}
\multiput(320,60)(0.12,-0.12){250}{\line(1,0){0.12}}
\linethickness{0.8mm}
\put(335,45){\line(0,1){20}}
\linethickness{0.8mm}
\put(335,90){\line(0,1){15}}
\put(338.75,103.75){\makebox(0,0)[cl]{$\Progtype$}}

\put(337.5,60){\makebox(0,0)[cl]{$\Progtype$}}

\linethickness{0.8mm}
\put(345,15){\line(0,1){15}}
\linethickness{0.8mm}
\put(325,15){\line(0,1){15}}
\put(75,77.5){\makebox(0,0)[cc]{$\eqlsb$}}

\put(237.5,216.25){\makebox(0,0)[cc]{$\universal$}}

\put(207.5,140){\makebox(0,0)[cr]{$\Progtype$}}

\linethickness{0.3mm}
\put(250,205){\line(0,1){25}}
\linethickness{0.3mm}
\put(235,205){\line(1,0){15}}
\linethickness{0.3mm}
\multiput(210,230)(0.12,-0.12){208}{\line(1,0){0.12}}
\linethickness{0.3mm}
\put(210,230){\line(1,0){40}}
\linethickness{0.8mm}
\put(210,140){\line(0,1){60}}
\linethickness{0.3mm}
\put(242.5,140){\line(0,1){65}}
\linethickness{0.3mm}
\put(227.5,140){\line(0,1){50}}
\linethickness{0.3mm}
\multiput(200,210)(0.12,-0.12){167}{\line(1,0){0.12}}
\linethickness{0.3mm}
\put(200,210){\line(0,1){5}}
\linethickness{0.3mm}
\put(220,190){\line(1,0){15}}
\linethickness{0.3mm}
\multiput(210,215)(0.12,-0.12){208}{\line(1,0){0.12}}
\linethickness{0.3mm}
\put(200,215){\line(1,0){10}}
\linethickness{0.8mm}
\put(222.5,202.5){\line(0,1){15}}
\put(137.5,76.25){\makebox(0,0)[cc]{$\universal$}}

\put(107.5,0){\makebox(0,0)[cr]{$\Progtype$}}

\linethickness{0.3mm}
\put(150,65){\line(0,1){25}}
\linethickness{0.3mm}
\put(135,65){\line(1,0){15}}
\linethickness{0.3mm}
\multiput(110,90)(0.12,-0.12){208}{\line(1,0){0.12}}
\linethickness{0.3mm}
\put(110,90){\line(1,0){40}}
\linethickness{0.8mm}
\put(110,0){\line(0,1){60}}
\linethickness{0.3mm}
\multiput(100,70)(0.12,-0.12){167}{\line(1,0){0.12}}
\linethickness{0.3mm}
\put(100,70){\line(0,1){5}}
\linethickness{0.3mm}
\put(120,50){\line(1,0){15}}
\linethickness{0.3mm}
\multiput(110,75)(0.12,-0.12){208}{\line(1,0){0.12}}
\linethickness{0.3mm}
\put(100,75){\line(1,0){10}}
\linethickness{0.8mm}
\put(122.5,62.5){\line(0,1){15}}
\linethickness{0.3mm}
\put(337.5,7.5){\line(1,0){15}}
\linethickness{0.3mm}
\put(337.5,7.5){\line(0,1){15}}
\linethickness{0.3mm}
\multiput(337.5,22.5)(0.12,-0.12){125}{\line(1,0){0.12}}
\linethickness{0.3mm}
\put(317.5,7.5){\line(1,0){15}}
\linethickness{0.3mm}
\put(317.5,7.5){\line(0,1){15}}
\linethickness{0.3mm}
\multiput(317.5,22.5)(0.12,-0.12){125}{\line(1,0){0.12}}
\linethickness{0.3mm}
\put(345,0){\line(0,1){7.5}}
\linethickness{0.3mm}
\put(325,0){\line(0,1){7.5}}
\linethickness{0.8mm}
\put(245,37.5){\line(0,1){27.5}}
\linethickness{0.8mm}
\put(225,37.5){\line(0,1){27.5}}
\linethickness{0.3mm}
\put(237.5,30){\line(1,0){15}}
\linethickness{0.3mm}
\put(237.5,30){\line(0,1){15}}
\linethickness{0.3mm}
\multiput(237.5,45)(0.12,-0.12){125}{\line(1,0){0.12}}
\linethickness{0.3mm}
\put(217.5,30){\line(1,0){15}}
\linethickness{0.3mm}
\put(217.5,30){\line(0,1){15}}
\linethickness{0.3mm}
\multiput(217.5,45)(0.12,-0.12){125}{\line(1,0){0.12}}
\linethickness{0.3mm}
\put(245,0){\line(0,1){30}}
\linethickness{0.3mm}
\put(225,0){\line(0,1){30}}
\linethickness{0.8mm}
\put(145,37.5){\line(0,1){27.5}}
\linethickness{0.8mm}
\put(127.5,22.5){\line(0,1){27.5}}
\linethickness{0.3mm}
\put(137.5,30){\line(1,0){15}}
\linethickness{0.3mm}
\put(137.5,30){\line(0,1){15}}
\linethickness{0.3mm}
\multiput(137.5,45)(0.12,-0.12){125}{\line(1,0){0.12}}
\linethickness{0.3mm}
\put(120,15){\line(1,0){15}}
\linethickness{0.3mm}
\put(120,15){\line(0,1){15}}
\linethickness{0.3mm}
\multiput(120,30)(0.12,-0.12){125}{\line(1,0){0.12}}
\linethickness{0.3mm}
\put(145,0){\line(0,1){30}}
\linethickness{0.3mm}
\put(127.5,0){\line(0,1){15}}
\put(322.5,11.25){\makebox(0,0)[cc]{$\encon$}}

\put(343.75,11.25){\makebox(0,0)[cc]{$\encon$}}

\put(222.5,33.75){\makebox(0,0)[cc]{$\encon$}}

\put(242.5,33.75){\makebox(0,0)[cc]{$\encon$}}

\put(125,18.75){\makebox(0,0)[cc]{$\encon$}}

\put(142.5,33.75){\makebox(0,0)[cc]{$\encon$}}

\put(207.5,0){\makebox(0,0)[cr]{$\Progtype$}}

\put(307.5,0){\makebox(0,0)[cr]{$\Progtype$}}

\put(26.25,140){\makebox(0,0)[cr]{$\Xee$}}

\put(125,140){\makebox(0,0)[cr]{$\Xee$}}

\put(225,140){\makebox(0,0)[cr]{$\Xee$}}

\put(125,0){\makebox(0,0)[cr]{$\Xee$}}

\put(222.5,0){\makebox(0,0)[cr]{$\Xee$}}

\put(322.5,0){\makebox(0,0)[cr]{$\Xee$}}

\put(342.5,0){\makebox(0,0)[cr]{$\Ahh$}}

\put(240,140){\makebox(0,0)[cr]{$\Ahh$}}

\put(140,140){\makebox(0,0)[cr]{$\Ahh$}}

\put(40,140){\makebox(0,0)[cr]{$\Ahh$}}

\put(115,62.5){\makebox(0,0)[cc]{$\artial$}}

\put(242.5,0){\makebox(0,0)[cr]{$\Ahh$}}

\put(142.5,0){\makebox(0,0)[cr]{$\Ahh$}}

\put(225,37.5){\makebox(0,0)[cc]{\Dottt}}

\put(245,37.5){\makebox(0,0)[cc]{\Dottt}}

\put(335,45){\makebox(0,0)[cc]{\Dottt}}

\put(325,17.5){\makebox(0,0)[cc]{\Dottt}}

\put(345,15){\makebox(0,0)[cc]{\Dottt}}

\put(122.5,62.5){\makebox(0,0)[cc]{\Dottt}}

\put(145,37.5){\makebox(0,0)[cc]{\Dottt}}

\put(127.5,22.5){\makebox(0,0)[cc]{\Dottt}}

\put(35,185){\makebox(0,0)[cc]{\Dottt}}

\put(222.5,202.5){\makebox(0,0)[cc]{\Dottt}}

\linethickness{0.8mm}
\put(135,230){\line(0,1){16.25}}
\put(138.75,246.25){\makebox(0,0)[cl]{$\Progtype$}}

\linethickness{0.8mm}
\put(235,230){\line(0,1){16.25}}
\put(238.75,246.25){\makebox(0,0)[cl]{$\Progtype$}}

\put(215,202.5){\makebox(0,0)[cc]{$\artial$}}

\put(31.25,176.25){\makebox(0,0)[cc]{$\bigencon$}}

\put(331.25,36.25){\makebox(0,0)[cc]{$\bigencon$}}

\end{picture}


==> PIC/uniform-eval.tex <==
%%Created by jPicEdt 1.4.1_03: mixed JPIC-XML/LaTeX format
%%Sun Aug 21 00:24:34 GMT-10:00 2022
%%Begin JPIC-XML
%<?xml version="1.0" standalone="yes"?>
%<jpic x-min="0" x-max="140" y-min="0" y-max="130" auto-bounding="true">
%<multicurve fill-style= "none"
%	 points= "(45,75);(45,75);(45,55);(45,55)"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(45,55);(45,55);(5,55);(5,55)"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(5,75);(5,75);(45,75);(45,75)"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(35,55);(35,55);(35,45);(35,45)"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(25,85);(25,85);(25,75);(25,75)"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(5,75);(5,75);(5,55);(5,55)"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(15,55);(15,55);(15,0);(15,0)"
%	 stroke-width= "0.35"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(110,65)"
%	 text-frame= "noframe"
%	 stroke-width= "0.35"
%	 text-hor-align= "center-h"
%	 >
%$\Univ$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(26.25,80)"
%	 text-frame= "noframe"
%	 stroke-width= "0.35"
%	 text-hor-align= "left"
%	 >
%$\Cee$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(13.75,1.25)"
%	 text-frame= "noframe"
%	 stroke-width= "0.35"
%	 text-hor-align= "right"
%	 >
%$\Aee$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(33.75,50)"
%	 text-frame= "noframe"
%	 stroke-width= "0.35"
%	 text-hor-align= "right"
%	 >
%$\Bee$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(25,65)"
%	 text-frame= "noframe"
%	 stroke-width= "0.35"
%	 text-hor-align= "center-h"
%	 >
%$\fee$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(97.5,14.38)"
%	 text-frame= "noframe"
%	 stroke-width= "0.35"
%	 text-hor-align= "center-h"
%	 >
%$\Fee$
%</text>
%<multicurve fill-style= "none"
%	 points= "(30,45);(30,45);(40,35);(40,35)"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(40,45);(40,45);(40,35);(40,35)"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(30,45);(30,45);(40,45);(40,45)"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(20,115);(20,115);(30,105);(30,105)"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(30,115);(30,115);(30,105);(30,105)"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(20,115);(20,115);(30,115);(30,115)"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(35,40);(35,40);(35,20);(35,20)"
%	 stroke-width= "1"
%	 />
%<multicurve fill-style= "none"
%	 points= "(25,110);(25,110);(25,90);(25,90)"
%	 stroke-width= "1"
%	 />
%<multicurve fill-style= "none"
%	 points= "(20,95);(20,95);(30,85);(30,85)"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(20,85);(20,85);(30,85);(30,85)"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(20,95);(20,95);(20,85);(20,85)"
%	 stroke-width= "0.35"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(25,90)"
%	 text-frame= "noframe"
%	 stroke-width= "0.35"
%	 text-hor-align= "center-h"
%	 >
%$\Dott$
%</text>
%<multicurve fill-style= "none"
%	 points= "(35,15);(35,15);(35,0);(35,0)"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(30,25);(30,25);(40,15);(40,15)"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(30,15);(30,15);(40,15);(40,15)"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(30,25);(30,25);(30,15);(30,15)"
%	 stroke-width= "0.35"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(35,20)"
%	 text-frame= "noframe"
%	 stroke-width= "0.35"
%	 text-hor-align= "center-h"
%	 >
%$\Dott$
%</text>
%<multicurve fill-style= "none"
%	 points= "(25,130);(25,130);(25,115);(25,115)"
%	 stroke-width= "0.35"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(26.25,128.75)"
%	 text-frame= "noframe"
%	 stroke-width= "0.35"
%	 text-hor-align= "left"
%	 >
%$\Cee$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(33.75,1.25)"
%	 text-frame= "noframe"
%	 stroke-width= "0.35"
%	 text-hor-align= "right"
%	 >
%$\Bee$
%</text>
%<multicurve fill-style= "none"
%	 points= "(50,100);(50,100);(50,30);(50,30)"
%	 stroke-width= "0.15"
%	 />
%<multicurve fill-style= "none"
%	 points= "(0,100);(0,100);(50,100);(50,100)"
%	 stroke-width= "0.15"
%	 />
%<multicurve fill-style= "none"
%	 points= "(0,100);(0,100);(0,30);(0,30)"
%	 stroke-width= "0.15"
%	 />
%<multicurve fill-style= "none"
%	 points= "(0,30);(0,30);(50,30);(50,30)"
%	 stroke-width= "0.15"
%	 />
%<multicurve fill-style= "none"
%	 points= "(130,100);(130,100);(130,30);(130,30)"
%	 stroke-width= "0.15"
%	 />
%<multicurve fill-style= "none"
%	 points= "(130,30);(130,30);(110,30);(110,30)"
%	 stroke-width= "0.15"
%	 />
%<multicurve fill-style= "none"
%	 points= "(90,100);(90,100);(130,100);(130,100)"
%	 stroke-width= "0.15"
%	 />
%<multicurve fill-style= "none"
%	 points= "(90,50);(90,50);(110,30);(110,30)"
%	 stroke-width= "0.15"
%	 />
%<multicurve fill-style= "none"
%	 points= "(105,115);(105,115);(115,105);(115,105)"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(115,115);(115,115);(115,105);(115,105)"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(105,115);(105,115);(115,115);(115,115)"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(120,30);(120,30);(120,20);(120,20)"
%	 stroke-width= "1"
%	 />
%<multicurve fill-style= "none"
%	 points= "(100,40);(100,40);(100,17.5);(100,17.5)"
%	 stroke-width= "1"
%	 />
%<multicurve fill-style= "none"
%	 points= "(110,110);(110,110);(110,100);(110,100)"
%	 stroke-width= "1"
%	 />
%<multicurve fill-style= "none"
%	 points= "(120,15);(120,15);(120,0);(120,0)"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(115,25);(115,25);(125,15);(125,15)"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(115,15);(115,15);(125,15);(125,15)"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(115,25);(115,25);(115,15);(115,15)"
%	 stroke-width= "0.35"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(120,20)"
%	 text-frame= "noframe"
%	 stroke-width= "0.35"
%	 text-hor-align= "center-h"
%	 >
%$\Dott$
%</text>
%<multicurve fill-style= "none"
%	 points= "(100,10);(100,10);(100,0);(100,0)"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(110,130);(110,130);(110,115);(110,115)"
%	 stroke-width= "0.35"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(111.25,128.75)"
%	 text-frame= "noframe"
%	 stroke-width= "0.35"
%	 text-hor-align= "left"
%	 >
%$\Cee$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(98.75,1.25)"
%	 text-frame= "noframe"
%	 stroke-width= "0.35"
%	 text-hor-align= "right"
%	 >
%$\Aee$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(118.75,1.25)"
%	 text-frame= "noframe"
%	 stroke-width= "0.35"
%	 text-hor-align= "right"
%	 >
%$\Bee$
%</text>
%<multicurve fill-style= "none"
%	 points= "(140,120);(140,120);(140,10);(140,10)"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(80,120);(80,120);(140,120);(140,120)"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(80,120);(80,120);(80,45);(80,45)"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(115,10);(115,10);(140,10);(140,10)"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(90,100);(90,100);(90,50);(90,50)"
%	 stroke-width= "0.15"
%	 />
%<multicurve fill-style= "none"
%	 points= "(80,45);(80,45);(115,10);(115,10)"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(92.5,25);(92.5,25);(107.5,10);(107.5,10)"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(92.5,10);(92.5,10);(107.5,10);(107.5,10)"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(92.5,25);(92.5,25);(92.5,10);(92.5,10)"
%	 stroke-width= "0.35"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(100,17.5)"
%	 text-frame= "noframe"
%	 stroke-width= "0.35"
%	 text-hor-align= "center-h"
%	 >
%$\Dott$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(65,65)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\BIGEQLS
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(112.5,111.88)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\decd$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(33.12,17.5)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\encd$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(23.12,87.5)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\encd$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(118.12,17.5)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\encd$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(26.88,111.88)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\decd$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(36.88,41.88)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\decd$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(45,95)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\geh$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(135,112.5)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\UnivAB$
%</text>
%</jpic>
%%End JPIC-XML
%LaTeX-picture environment using emulated lines and arcs
%You can rescale the whole picture (to 80% for instance) by using the command \def\JPicScale{0.8}
\ifx\JPicScale\undefined\def\JPicScale{1}\fi
\unitlength \JPicScale mm
\begin{picture}(140,130)(0,0)
\linethickness{0.35mm}
\put(45,55){\line(0,1){20}}
\linethickness{0.35mm}
\put(5,55){\line(1,0){40}}
\linethickness{0.35mm}
\put(5,75){\line(1,0){40}}
\linethickness{0.35mm}
\put(35,45){\line(0,1){10}}
\linethickness{0.35mm}
\put(25,75){\line(0,1){10}}
\linethickness{0.35mm}
\put(5,55){\line(0,1){20}}
\linethickness{0.35mm}
\put(15,0){\line(0,1){55}}
\put(110,65){\makebox(0,0)[cc]{$\Univ$}}

\put(26.25,80){\makebox(0,0)[cl]{$\Cee$}}

\put(13.75,1.25){\makebox(0,0)[cr]{$\Aee$}}

\put(33.75,50){\makebox(0,0)[cr]{$\Bee$}}

\put(25,65){\makebox(0,0)[cc]{$\fee$}}

\put(97.5,14.38){\makebox(0,0)[cc]{$\Fee$}}

\linethickness{0.35mm}
\multiput(30,45)(0.12,-0.12){83}{\line(1,0){0.12}}
\linethickness{0.35mm}
\put(40,35){\line(0,1){10}}
\linethickness{0.35mm}
\put(30,45){\line(1,0){10}}
\linethickness{0.35mm}
\multiput(20,115)(0.12,-0.12){83}{\line(1,0){0.12}}
\linethickness{0.35mm}
\put(30,105){\line(0,1){10}}
\linethickness{0.35mm}
\put(20,115){\line(1,0){10}}
\linethickness{1mm}
\put(35,20){\line(0,1){20}}
\linethickness{1mm}
\put(25,90){\line(0,1){20}}
\linethickness{0.35mm}
\multiput(20,95)(0.12,-0.12){83}{\line(1,0){0.12}}
\linethickness{0.35mm}
\put(20,85){\line(1,0){10}}
\linethickness{0.35mm}
\put(20,85){\line(0,1){10}}
\put(25,90){\makebox(0,0)[cc]{$\Dott$}}

\linethickness{0.35mm}
\put(35,0){\line(0,1){15}}
\linethickness{0.35mm}
\multiput(30,25)(0.12,-0.12){83}{\line(1,0){0.12}}
\linethickness{0.35mm}
\put(30,15){\line(1,0){10}}
\linethickness{0.35mm}
\put(30,15){\line(0,1){10}}
\put(35,20){\makebox(0,0)[cc]{$\Dott$}}

\linethickness{0.35mm}
\put(25,115){\line(0,1){15}}
\put(26.25,128.75){\makebox(0,0)[cl]{$\Cee$}}

\put(33.75,1.25){\makebox(0,0)[cr]{$\Bee$}}

\linethickness{0.15mm}
\put(50,30){\line(0,1){70}}
\linethickness{0.15mm}
\put(0,100){\line(1,0){50}}
\linethickness{0.15mm}
\put(0,30){\line(0,1){70}}
\linethickness{0.15mm}
\put(0,30){\line(1,0){50}}
\linethickness{0.15mm}
\put(130,30){\line(0,1){70}}
\linethickness{0.15mm}
\put(110,30){\line(1,0){20}}
\linethickness{0.15mm}
\put(90,100){\line(1,0){40}}
\linethickness{0.15mm}
\multiput(90,50)(0.12,-0.12){167}{\line(1,0){0.12}}
\linethickness{0.35mm}
\multiput(105,115)(0.12,-0.12){83}{\line(1,0){0.12}}
\linethickness{0.35mm}
\put(115,105){\line(0,1){10}}
\linethickness{0.35mm}
\put(105,115){\line(1,0){10}}
\linethickness{1mm}
\put(120,20){\line(0,1){10}}
\linethickness{1mm}
\put(100,17.5){\line(0,1){22.5}}
\linethickness{1mm}
\put(110,100){\line(0,1){10}}
\linethickness{0.35mm}
\put(120,0){\line(0,1){15}}
\linethickness{0.35mm}
\multiput(115,25)(0.12,-0.12){83}{\line(1,0){0.12}}
\linethickness{0.35mm}
\put(115,15){\line(1,0){10}}
\linethickness{0.35mm}
\put(115,15){\line(0,1){10}}
\put(120,20){\makebox(0,0)[cc]{$\Dott$}}

\linethickness{0.35mm}
\put(100,0){\line(0,1){10}}
\linethickness{0.35mm}
\put(110,115){\line(0,1){15}}
\put(111.25,128.75){\makebox(0,0)[cl]{$\Cee$}}

\put(98.75,1.25){\makebox(0,0)[cr]{$\Aee$}}

\put(118.75,1.25){\makebox(0,0)[cr]{$\Bee$}}

\linethickness{0.35mm}
\put(140,10){\line(0,1){110}}
\linethickness{0.35mm}
\put(80,120){\line(1,0){60}}
\linethickness{0.35mm}
\put(80,45){\line(0,1){75}}
\linethickness{0.35mm}
\put(115,10){\line(1,0){25}}
\linethickness{0.15mm}
\put(90,50){\line(0,1){50}}
\linethickness{0.35mm}
\multiput(80,45)(0.12,-0.12){292}{\line(1,0){0.12}}
\linethickness{0.35mm}
\multiput(92.5,25)(0.12,-0.12){125}{\line(1,0){0.12}}
\linethickness{0.35mm}
\put(92.5,10){\line(1,0){15}}
\linethickness{0.35mm}
\put(92.5,10){\line(0,1){15}}
\put(100,17.5){\makebox(0,0)[cc]{$\Dott$}}

\put(65,65){\makebox(0,0)[cc]{\BIGEQLS}}

\put(112.5,111.88){\makebox(0,0)[cc]{$\decd$}}

\put(33.12,17.5){\makebox(0,0)[cc]{$\encd$}}

\put(23.12,87.5){\makebox(0,0)[cc]{$\encd$}}

\put(118.12,17.5){\makebox(0,0)[cc]{$\encd$}}

\put(26.88,111.88){\makebox(0,0)[cc]{$\decd$}}

\put(36.88,41.88){\makebox(0,0)[cc]{$\decd$}}

\put(45,95){\makebox(0,0)[cc]{$\geh$}}

\put(135,112.5){\makebox(0,0)[cc]{$\UnivAB$}}

\end{picture}


==> PIC/uniform-op.tex <==
%%Created by jPicEdt 1.4.1_03: mixed JPIC-XML/LaTeX format
%%Thu Dec 22 17:31:32 GMT-10:00 2022
%%Begin JPIC-XML
%<?xml version="1.0" standalone="yes"?>
%<jpic x-min="0" x-max="65" y-min="0" y-max="95" auto-bounding="true">
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(45,47.5)"
%	 text-frame= "noframe"
%	 stroke-width= "0.35"
%	 text-hor-align= "center-h"
%	 >
%$\universal$
%</text>
%<multicurve fill-style= "none"
%	 points= "(65,60);(65,60);(65,35);(65,35)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(65,35);(65,35);(25,35);(25,35)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(0,60);(0,60);(65,60);(65,60)"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(8.75,0)"
%	 text-frame= "noframe"
%	 stroke-width= "0.35"
%	 text-hor-align= "right"
%	 >
%$\Progtype$
%</text>
%<multicurve fill-style= "none"
%	 points= "(25,35);(25,35);(0,60);(0,60)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(11.25,48.75);(11.25,48.75);(11.25,0);(11.25,0)"
%	 stroke-width= "1"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(42.5,0)"
%	 text-frame= "noframe"
%	 stroke-width= "0.35"
%	 text-hor-align= "right"
%	 >
%$\Progn$
%</text>
%<multicurve fill-style= "none"
%	 points= "(45,10);(45,10);(45,0);(45,0)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(55,10);(55,10);(35,10);(35,10)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(35,30);(35,30);(35,10);(35,10)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(35,30);(35,30);(55,10);(55,10)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(45,35);(45,35);(45,20);(45,20)"
%	 stroke-width= "1"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(47.5,26.25)"
%	 text-frame= "noframe"
%	 stroke-width= "0.35"
%	 text-hor-align= "left"
%	 >
%$\Progtype$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(41.25,16.25)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\encon$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(45,20)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\Dottt
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(47.5,93.75)"
%	 text-frame= "noframe"
%	 stroke-width= "0.35"
%	 text-hor-align= "left"
%	 >
%$\Progk$
%</text>
%<multicurve fill-style= "none"
%	 points= "(45,95);(45,95);(45,85);(45,85)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(55,85);(55,85);(35,85);(35,85)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(55,85);(55,85);(55,65);(55,65)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(35,85);(35,85);(55,65);(55,65)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(45,75);(45,75);(45,60);(45,60)"
%	 stroke-width= "1"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(42.5,66.25)"
%	 text-frame= "noframe"
%	 stroke-width= "0.35"
%	 text-hor-align= "right"
%	 >
%$\Progtype$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(48.75,78.75)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\decok$
%</text>
%</jpic>
%%End JPIC-XML
%LaTeX-picture environment using emulated lines and arcs
%You can rescale the whole picture (to 80% for instance) by using the command \def\JPicScale{0.8}
\ifx\JPicScale\undefined\def\JPicScale{1}\fi
\unitlength \JPicScale mm
\begin{picture}(65,95)(0,0)
\put(45,47.5){\makebox(0,0)[cc]{$\universal$}}

\linethickness{0.3mm}
\put(65,35){\line(0,1){25}}
\linethickness{0.3mm}
\put(25,35){\line(1,0){40}}
\linethickness{0.3mm}
\put(0,60){\line(1,0){65}}
\put(8.75,0){\makebox(0,0)[cr]{$\Progtype$}}

\linethickness{0.3mm}
\multiput(0,60)(0.12,-0.12){208}{\line(1,0){0.12}}
\linethickness{1mm}
\put(11.25,0){\line(0,1){48.75}}
\put(42.5,0){\makebox(0,0)[cr]{$\Progn$}}

\linethickness{0.3mm}
\put(45,0){\line(0,1){10}}
\linethickness{0.3mm}
\put(35,10){\line(1,0){20}}
\linethickness{0.3mm}
\put(35,10){\line(0,1){20}}
\linethickness{0.3mm}
\multiput(35,30)(0.12,-0.12){167}{\line(1,0){0.12}}
\linethickness{1mm}
\put(45,20){\line(0,1){15}}
\put(47.5,26.25){\makebox(0,0)[cl]{$\Progtype$}}

\put(41.25,16.25){\makebox(0,0)[cc]{$\encon$}}

\put(45,20){\makebox(0,0)[cc]{\Dottt}}

\put(47.5,93.75){\makebox(0,0)[cl]{$\Progk$}}

\linethickness{0.3mm}
\put(45,85){\line(0,1){10}}
\linethickness{0.3mm}
\put(35,85){\line(1,0){20}}
\linethickness{0.3mm}
\put(55,65){\line(0,1){20}}
\linethickness{0.3mm}
\multiput(35,85)(0.12,-0.12){167}{\line(1,0){0.12}}
\linethickness{1mm}
\put(45,60){\line(0,1){15}}
\put(42.5,66.25){\makebox(0,0)[cr]{$\Progtype$}}

\put(48.75,78.75){\makebox(0,0)[cc]{$\decok$}}

\end{picture}


==> PIC/uniform-q.tex <==
%%Created by jPicEdt 1.4.1_03: mixed JPIC-XML/LaTeX format
%%Tue Dec 08 16:33:38 GMT-10:00 2020
%%Begin JPIC-XML
%<?xml version="1.0" standalone="yes"?>
%<jpic x-min="0" x-max="150" y-min="0" y-max="125" auto-bounding="true">
%<multicurve fill-style= "none"
%	 points= "(35,125);(35,125);(35,105);(35,105)"
%	 stroke-width= "1"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(35,66.25)"
%	 text-frame= "noframe"
%	 stroke-width= "0.35"
%	 text-hor-align= "center-h"
%	 >
%$\universal$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(3.75,41.25)"
%	 text-frame= "noframe"
%	 stroke-width= "0.35"
%	 text-hor-align= "center-h"
%	 >
%\program
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(7.5,57.5)"
%	 text-frame= "noframe"
%	 stroke-width= "0.35"
%	 text-hor-align= "right"
%	 >
%$\Progtype$
%</text>
%<multicurve fill-style= "none"
%	 points= "(50,80);(50,80);(50,55);(50,55)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(50,55);(50,55);(20,55);(20,55)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(0,55);(0,55);(0,35);(0,35)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(0,55);(0,55);(20,35);(20,35)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(20,55);(20,55);(0,75);(0,75)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(0,75);(0,75);(0,80);(0,80)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(0,80);(0,80);(50,80);(50,80)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(10,65);(10,65);(10,45);(10,45)"
%	 stroke-width= "1"
%	 />
%<multicurve fill-style= "none"
%	 points= "(45,10);(45,10);(25,10);(25,10)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(25,30);(25,30);(25,10);(25,10)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(25,30);(25,30);(45,10);(45,10)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(0,35);(0,35);(20,35);(20,35)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(35,55);(35,55);(35,20);(35,20)"
%	 stroke-width= "1"
%	 />
%<multicurve fill-style= "none"
%	 points= "(45,105);(45,105);(25,105);(25,105)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(45,105);(45,105);(45,85);(45,85)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(25,105);(25,105);(45,85);(45,85)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(35,95);(35,95);(35,80);(35,80)"
%	 stroke-width= "1"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(37.5,125)"
%	 text-frame= "noframe"
%	 stroke-width= "0.35"
%	 text-hor-align= "left"
%	 >
%$\Progtype$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(37.5,40)"
%	 text-frame= "noframe"
%	 stroke-width= "0.35"
%	 text-hor-align= "left"
%	 >
%$\Progtype$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(38.75,98.75)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\decok$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(31.25,16.25)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\encon$
%</text>
%<multicurve fill-style= "none"
%	 points= "(35,10);(35,10);(35,0);(35,0)"
%	 stroke-width= "1"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(75,67.5)"
%	 text-frame= "noframe"
%	 stroke-width= "0.35"
%	 text-hor-align= "center-h"
%	 >
%$\eqlsb$
%</text>
%<multicurve fill-style= "none"
%	 points= "(135,125);(135,125);(135,105);(135,105)"
%	 stroke-width= "1"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(135,66.25)"
%	 text-frame= "noframe"
%	 stroke-width= "0.35"
%	 text-hor-align= "center-h"
%	 >
%$\universal$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(103.75,26.25)"
%	 text-frame= "noframe"
%	 stroke-width= "0.35"
%	 text-hor-align= "center-h"
%	 >
%\program
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(107.5,42.5)"
%	 text-frame= "noframe"
%	 stroke-width= "0.35"
%	 text-hor-align= "right"
%	 >
%$\Progtype$
%</text>
%<multicurve fill-style= "none"
%	 points= "(150,80);(150,80);(150,55);(150,55)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(150,40);(150,40);(120,40);(120,40)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(100,40);(100,40);(100,20);(100,20)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(100,40);(100,40);(120,20);(120,20)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(120,40);(120,40);(100,60);(100,60)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(100,60);(100,60);(100,75);(100,75)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(100,80);(100,80);(150,80);(150,80)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(110,50);(110,50);(110,30);(110,30)"
%	 stroke-width= "1"
%	 />
%<multicurve fill-style= "none"
%	 points= "(145,10);(145,10);(125,10);(125,10)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(125,30);(125,30);(125,10);(125,10)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(125,30);(125,30);(145,10);(145,10)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(100,20);(100,20);(120,20);(120,20)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(135,40);(135,40);(135,20);(135,20)"
%	 stroke-width= "1"
%	 />
%<multicurve fill-style= "none"
%	 points= "(145,105);(145,105);(125,105);(125,105)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(145,105);(145,105);(145,85);(145,85)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(125,105);(125,105);(145,85);(145,85)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(135,95);(135,95);(135,80);(135,80)"
%	 stroke-width= "1"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(137.5,125)"
%	 text-frame= "noframe"
%	 stroke-width= "0.35"
%	 text-hor-align= "left"
%	 >
%$\Progtype$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(138.75,98.75)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\decok$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(131.25,16.25)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\encon$
%</text>
%<multicurve fill-style= "none"
%	 points= "(135,10);(135,10);(135,0);(135,0)"
%	 stroke-width= "1"
%	 />
%<multicurve fill-style= "none"
%	 points= "(150,40);(150,40);(115,75);(115,75)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(100,75);(100,75);(115,75);(115,75)"
%	 />
%</jpic>
%%End JPIC-XML
%LaTeX-picture environment using emulated lines and arcs
%You can rescale the whole picture (to 80% for instance) by using the command \def\JPicScale{0.8}
\ifx\JPicScale\undefined\def\JPicScale{1}\fi
\unitlength \JPicScale mm
\begin{picture}(150,125)(0,0)
\linethickness{1mm}
\put(35,105){\line(0,1){20}}
\put(35,66.25){\makebox(0,0)[cc]{$\universal$}}

\put(3.75,41.25){\makebox(0,0)[cc]{\program}}

\put(7.5,57.5){\makebox(0,0)[cr]{$\Progtype$}}

\linethickness{0.3mm}
\put(50,55){\line(0,1){25}}
\linethickness{0.3mm}
\put(20,55){\line(1,0){30}}
\linethickness{0.3mm}
\put(0,35){\line(0,1){20}}
\linethickness{0.3mm}
\multiput(0,55)(0.12,-0.12){167}{\line(1,0){0.12}}
\linethickness{0.3mm}
\multiput(0,75)(0.12,-0.12){167}{\line(1,0){0.12}}
\linethickness{0.3mm}
\put(0,75){\line(0,1){5}}
\linethickness{0.3mm}
\put(0,80){\line(1,0){50}}
\linethickness{1mm}
\put(10,45){\line(0,1){20}}
\linethickness{0.3mm}
\put(25,10){\line(1,0){20}}
\linethickness{0.3mm}
\put(25,10){\line(0,1){20}}
\linethickness{0.3mm}
\multiput(25,30)(0.12,-0.12){167}{\line(1,0){0.12}}
\linethickness{0.3mm}
\put(0,35){\line(1,0){20}}
\linethickness{1mm}
\put(35,20){\line(0,1){35}}
\linethickness{0.3mm}
\put(25,105){\line(1,0){20}}
\linethickness{0.3mm}
\put(45,85){\line(0,1){20}}
\linethickness{0.3mm}
\multiput(25,105)(0.12,-0.12){167}{\line(1,0){0.12}}
\linethickness{1mm}
\put(35,80){\line(0,1){15}}
\put(37.5,125){\makebox(0,0)[cl]{$\Progtype$}}

\put(37.5,40){\makebox(0,0)[cl]{$\Progtype$}}

\put(38.75,98.75){\makebox(0,0)[cc]{$\decok$}}

\put(31.25,16.25){\makebox(0,0)[cc]{$\encon$}}

\linethickness{1mm}
\put(35,0){\line(0,1){10}}
\put(75,67.5){\makebox(0,0)[cc]{$\eqlsb$}}

\linethickness{1mm}
\put(135,105){\line(0,1){20}}
\put(135,66.25){\makebox(0,0)[cc]{$\universal$}}

\put(103.75,26.25){\makebox(0,0)[cc]{\program}}

\put(107.5,42.5){\makebox(0,0)[cr]{$\Progtype$}}

\linethickness{0.3mm}
\put(150,55){\line(0,1){25}}
\linethickness{0.3mm}
\put(120,40){\line(1,0){30}}
\linethickness{0.3mm}
\put(100,20){\line(0,1){20}}
\linethickness{0.3mm}
\multiput(100,40)(0.12,-0.12){167}{\line(1,0){0.12}}
\linethickness{0.3mm}
\multiput(100,60)(0.12,-0.12){167}{\line(1,0){0.12}}
\linethickness{0.3mm}
\put(100,60){\line(0,1){15}}
\linethickness{0.3mm}
\put(100,80){\line(1,0){50}}
\linethickness{1mm}
\put(110,30){\line(0,1){20}}
\linethickness{0.3mm}
\put(125,10){\line(1,0){20}}
\linethickness{0.3mm}
\put(125,10){\line(0,1){20}}
\linethickness{0.3mm}
\multiput(125,30)(0.12,-0.12){167}{\line(1,0){0.12}}
\linethickness{0.3mm}
\put(100,20){\line(1,0){20}}
\linethickness{1mm}
\put(135,20){\line(0,1){20}}
\linethickness{0.3mm}
\put(125,105){\line(1,0){20}}
\linethickness{0.3mm}
\put(145,85){\line(0,1){20}}
\linethickness{0.3mm}
\multiput(125,105)(0.12,-0.12){167}{\line(1,0){0.12}}
\linethickness{1mm}
\put(135,80){\line(0,1){15}}
\put(137.5,125){\makebox(0,0)[cl]{$\Progtype$}}

\put(138.75,98.75){\makebox(0,0)[cc]{$\decok$}}

\put(131.25,16.25){\makebox(0,0)[cc]{$\encon$}}

\linethickness{1mm}
\put(135,0){\line(0,1){10}}
\linethickness{0.3mm}
\multiput(115,75)(0.12,-0.12){292}{\line(1,0){0.12}}
\linethickness{0.3mm}
\put(100,75){\line(1,0){15}}
\end{picture}


==> PIC/uniform.tex <==
%%Created by jPicEdt 1.4.1_03: mixed JPIC-XML/LaTeX format
%%Thu Sep 29 22:35:03 GMT-10:00 2022
%%Begin JPIC-XML
%<?xml version="1.0" standalone="yes"?>
%<jpic x-min="-5" x-max="165" y-min="0" y-max="115" auto-bounding="true">
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(40,56.25)"
%	 text-frame= "noframe"
%	 stroke-width= "0.35"
%	 text-hor-align= "center-h"
%	 >
%$\universal$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(5,0)"
%	 text-frame= "noframe"
%	 stroke-width= "0.35"
%	 text-hor-align= "right"
%	 >
%$\Progtype$
%</text>
%<multicurve fill-style= "none"
%	 points= "(60,70);(60,70);(60,45);(60,45)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(60,45);(60,45);(20,45);(20,45)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(20,45);(20,45);(-5,70);(-5,70)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(-5,70);(-5,70);(60,70);(60,70)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(7.5,57.5);(7.5,57.5);(7.5,0);(7.5,0)"
%	 stroke-width= "1"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(42.5,80)"
%	 text-frame= "noframe"
%	 stroke-width= "0.35"
%	 text-hor-align= "left"
%	 >
%$\Progn$
%</text>
%<multicurve fill-style= "none"
%	 points= "(40,90);(40,90);(40,70);(40,70)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(50,90);(50,90);(30,90);(30,90)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(30,110);(30,110);(30,90);(30,90)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(30,110);(30,110);(50,90);(50,90)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(40,115);(40,115);(40,100);(40,100)"
%	 stroke-width= "1"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(37.5,35)"
%	 text-frame= "noframe"
%	 stroke-width= "0.35"
%	 text-hor-align= "right"
%	 >
%$\Progk$
%</text>
%<multicurve fill-style= "none"
%	 points= "(40,45);(40,45);(40,25);(40,25)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(50,25);(50,25);(30,25);(30,25)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(50,25);(50,25);(50,5);(50,5)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(30,25);(30,25);(50,5);(50,5)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(40,15);(40,15);(40,0);(40,0)"
%	 stroke-width= "1"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(37.5,0)"
%	 text-frame= "noframe"
%	 stroke-width= "0.35"
%	 text-hor-align= "right"
%	 >
%$\Progtype$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(42.5,115)"
%	 text-frame= "noframe"
%	 stroke-width= "0.35"
%	 text-hor-align= "left"
%	 >
%$\Progtype$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(43.75,18.75)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\decok$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(36.25,96.25)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\encon$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(110,37.5)"
%	 text-frame= "noframe"
%	 stroke-width= "0.35"
%	 text-hor-align= "center-h"
%	 >
%\program
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(80,57.5)"
%	 text-frame= "noframe"
%	 stroke-width= "0.35"
%	 text-hor-align= "center-h"
%	 >
%$\eqlsb$
%</text>
%<multicurve fill-style= "none"
%	 points= "(145,45);(145,45);(145,0);(145,0)"
%	 stroke-width= "1"
%	 />
%<multicurve fill-style= "none"
%	 points= "(145,115);(145,115);(145,70);(145,70)"
%	 stroke-width= "1"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(145,57.5)"
%	 text-frame= "noframe"
%	 stroke-width= "0.35"
%	 text-hor-align= "center-h"
%	 >
%$\universal$
%</text>
%<multicurve fill-style= "none"
%	 points= "(165,70);(165,70);(165,45);(165,45)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(165,45);(165,45);(125,45);(125,45)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(100,55);(100,55);(100,30);(100,30)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(100,70);(100,70);(165,70);(165,70)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(111.25,30);(111.25,30);(111.25,0);(111.25,0)"
%	 stroke-width= "1"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(142.5,0)"
%	 text-frame= "noframe"
%	 stroke-width= "0.35"
%	 text-hor-align= "right"
%	 >
%$\Progtype$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(107.5,0)"
%	 text-frame= "noframe"
%	 stroke-width= "0.35"
%	 text-hor-align= "right"
%	 >
%$\Progtype$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(147.5,115)"
%	 text-frame= "noframe"
%	 stroke-width= "0.35"
%	 text-hor-align= "left"
%	 >
%$\Progtype$
%</text>
%<multicurve fill-style= "none"
%	 points= "(125,30);(125,30);(100,30);(100,30)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(125,30);(125,30);(100,55);(100,55)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(125,45);(125,45);(100,70);(100,70)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(111.25,58.75);(111.25,58.75);(111.25,43.75);(111.25,43.75)"
%	 stroke-width= "1"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(40,100)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\Dottt
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(111.25,43.75)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\Dottt
%</text>
%</jpic>
%%End JPIC-XML
%LaTeX-picture environment using emulated lines and arcs
%You can rescale the whole picture (to 80% for instance) by using the command \def\JPicScale{0.8}
\ifx\JPicScale\undefined\def\JPicScale{1}\fi
\unitlength \JPicScale mm
\begin{picture}(165,115)(0,0)
\put(40,56.25){\makebox(0,0)[cc]{$\universal$}}

\put(5,0){\makebox(0,0)[cr]{$\Progtype$}}

\linethickness{0.3mm}
\put(60,45){\line(0,1){25}}
\linethickness{0.3mm}
\put(20,45){\line(1,0){40}}
\linethickness{0.3mm}
\multiput(-5,70)(0.12,-0.12){208}{\line(1,0){0.12}}
\linethickness{0.3mm}
\put(-5,70){\line(1,0){65}}
\linethickness{1mm}
\put(7.5,0){\line(0,1){57.5}}
\put(42.5,80){\makebox(0,0)[cl]{$\Progn$}}

\linethickness{0.3mm}
\put(40,70){\line(0,1){20}}
\linethickness{0.3mm}
\put(30,90){\line(1,0){20}}
\linethickness{0.3mm}
\put(30,90){\line(0,1){20}}
\linethickness{0.3mm}
\multiput(30,110)(0.12,-0.12){167}{\line(1,0){0.12}}
\linethickness{1mm}
\put(40,100){\line(0,1){15}}
\put(37.5,35){\makebox(0,0)[cr]{$\Progk$}}

\linethickness{0.3mm}
\put(40,25){\line(0,1){20}}
\linethickness{0.3mm}
\put(30,25){\line(1,0){20}}
\linethickness{0.3mm}
\put(50,5){\line(0,1){20}}
\linethickness{0.3mm}
\multiput(30,25)(0.12,-0.12){167}{\line(1,0){0.12}}
\linethickness{1mm}
\put(40,0){\line(0,1){15}}
\put(37.5,0){\makebox(0,0)[cr]{$\Progtype$}}

\put(42.5,115){\makebox(0,0)[cl]{$\Progtype$}}

\put(43.75,18.75){\makebox(0,0)[cc]{$\decok$}}

\put(36.25,96.25){\makebox(0,0)[cc]{$\encon$}}

\put(110,37.5){\makebox(0,0)[cc]{\program}}

\put(80,57.5){\makebox(0,0)[cc]{$\eqlsb$}}

\linethickness{1mm}
\put(145,0){\line(0,1){45}}
\linethickness{1mm}
\put(145,70){\line(0,1){45}}
\put(145,57.5){\makebox(0,0)[cc]{$\universal$}}

\linethickness{0.3mm}
\put(165,45){\line(0,1){25}}
\linethickness{0.3mm}
\put(125,45){\line(1,0){40}}
\linethickness{0.3mm}
\put(100,30){\line(0,1){25}}
\linethickness{0.3mm}
\put(100,70){\line(1,0){65}}
\linethickness{1mm}
\put(111.25,0){\line(0,1){30}}
\put(142.5,0){\makebox(0,0)[cr]{$\Progtype$}}

\put(107.5,0){\makebox(0,0)[cr]{$\Progtype$}}

\put(147.5,115){\makebox(0,0)[cl]{$\Progtype$}}

\linethickness{0.3mm}
\put(100,30){\line(1,0){25}}
\linethickness{0.3mm}
\multiput(100,55)(0.12,-0.12){208}{\line(1,0){0.12}}
\linethickness{0.3mm}
\multiput(100,70)(0.12,-0.12){208}{\line(1,0){0.12}}
\linethickness{1mm}
\put(111.25,43.75){\line(0,1){15}}
\put(40,100){\makebox(0,0)[cc]{\Dottt}}

\put(111.25,43.75){\makebox(0,0)[cc]{\Dottt}}

\end{picture}


==> PIC/univeval.tex <==
%%Created by jPicEdt 1.4.1_03: mixed JPIC-XML/LaTeX format
%%Sat Sep 24 20:37:06 CDT 2016
%%Begin JPIC-XML
%<?xml version="1.0" standalone="yes"?>
%<jpic x-min="0" x-max="155" y-min="0.62" y-max="110.62" auto-bounding="true">
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(10,25);(10,25);(10,9.38);(10,9.38)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(50,25);(50,25);(50,9.38);(50,9.38)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(20,45);(20,45);(40,45);(40,45)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(60,25);(60,25);(0,25);(0,25)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(20,65);(20,65);(0,85);(0,85)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(40,45);(40,45);(60,25);(60,25)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(0,85);(0,85);(60,85);(60,85)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(30,65);(30,65);(30,45);(30,45)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(20,65);(20,65);(40,65);(40,65)"
%	 />
%<text stroke-width= "0.75"
%	 text-vert-align= "center-v"
%	 anchor-point= "(85.62,54.38)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\EQLS
%</text>
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(60,85);(60,85);(40,65);(40,65)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(20,45);(20,45);(0,25);(0,25)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(10,103.75);(10,103.75);(10,85);(10,85)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(50,103.75);(50,103.75);(50,85);(50,85)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(115,106.25);(115,106.25);(115,9.38);(115,9.38)"
%	 />
%<multicurve stroke-width= "0.75"
%	 fill-style= "none"
%	 points= "(155,106.25);(155,106.25);(155,9.38);(155,9.38)"
%	 />
%<text stroke-width= "0.75"
%	 text-vert-align= "center-v"
%	 anchor-point= "(10.62,110.62)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\Progtype$
%</text>
%<text stroke-width= "0.75"
%	 text-vert-align= "center-v"
%	 anchor-point= "(50,110)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\Progtype$
%</text>
%<text stroke-width= "0.75"
%	 text-vert-align= "center-v"
%	 anchor-point= "(115,0.62)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\Progtype$
%</text>
%<text stroke-width= "0.75"
%	 text-vert-align= "center-v"
%	 anchor-point= "(10,0.62)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\Progtype$
%</text>
%<text stroke-width= "0.75"
%	 text-vert-align= "center-v"
%	 anchor-point= "(155,1.25)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\Progtype$
%</text>
%<text stroke-width= "0.75"
%	 text-vert-align= "center-v"
%	 anchor-point= "(26.25,54.38)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\Progtype$
%</text>
%<text stroke-width= "0.75"
%	 text-vert-align= "center-v"
%	 anchor-point= "(50.62,0.62)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\Progtype$
%</text>
%<text stroke-width= "0.75"
%	 text-vert-align= "center-v"
%	 anchor-point= "(30,35)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\pairing$
%</text>
%<text stroke-width= "0.75"
%	 text-vert-align= "center-v"
%	 anchor-point= "(30,75)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\projections$
%</text>
%</jpic>
%%End JPIC-XML
%PSTricks content-type (pstricks.sty package needed)
%Add \usepackage{pstricks} in the preamble of your LaTeX file
%You can rescale the whole picture (to 80% for instance) by using the command \def\JPicScale{0.8}
\ifx\JPicScale\undefined\def\JPicScale{1}\fi
\psset{unit=\JPicScale mm}
\psset{linewidth=0.3,dotsep=1,hatchwidth=0.3,hatchsep=1.5,shadowsize=1,dimen=middle}
\psset{dotsize=0.7 2.5,dotscale=1 1,fillcolor=black}
\psset{arrowsize=1 2,arrowlength=1,arrowinset=0.25,tbarsize=0.7 5,bracketlength=0.15,rbracketlength=0.15}
\begin{pspicture}(0,0)(155,110.62)
\psline[linewidth=0.75](10,25)(10,9.38)
\psline[linewidth=0.75](50,25)(50,9.38)
\psline[linewidth=0.75](20,45)(40,45)
\psline[linewidth=0.75](60,25)(0,25)
\psline[linewidth=0.75](20,65)(0,85)
\psline[linewidth=0.75](40,45)(60,25)
\psline[linewidth=0.75](0,85)(60,85)
\psline[linewidth=0.75](30,65)(30,45)
\psline[linewidth=0.75](20,65)(40,65)
\rput(85.62,54.38){\EQLS}
\psline[linewidth=0.75](60,85)(40,65)
\psline[linewidth=0.75](20,45)(0,25)
\psline[linewidth=0.75](10,103.75)(10,85)
\psline[linewidth=0.75](50,103.75)(50,85)
\psline[linewidth=0.75](115,106.25)(115,9.38)
\psline[linewidth=0.75](155,106.25)(155,9.38)
\rput(10.62,110.62){$\Progtype$}
\rput(50,110){$\Progtype$}
\rput(115,0.62){$\Progtype$}
\rput(10,0.62){$\Progtype$}
\rput(155,1.25){$\Progtype$}
\rput[r](26.25,54.38){$\Progtype$}
\rput(50.62,0.62){$\Progtype$}
\rput(30,35){$\pairing$}
\rput(30,75){$\projections$}
\end{pspicture}


==> PIC/vector-scalar.tex <==
%%Created by jPicEdt 1.4.1_03: mixed JPIC-XML/LaTeX format
%%Tue Jul 30 09:37:13 GMT-10:00 2019
%%Begin JPIC-XML
%<?xml version="1.0" standalone="yes"?>
%<jpic x-min="0" x-max="120" y-min="0" y-max="30" auto-bounding="true">
%<multicurve fill-style= "none"
%	 points= "(110,30);(110,30);(100,20);(100,20)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(120,20);(120,20);(110,30);(110,30)"
%	 stroke-width= "0.75"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(107.5,2.5)"
%	 text-frame= "noframe"
%	 stroke-width= "0.75"
%	 text-hor-align= "right"
%	 >
%$\inputt$
%</text>
%<multicurve fill-style= "none"
%	 points= "(100,20);(100,20);(120,20);(120,20)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(110,20);(110,20);(110,0);(110,0)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(20,10);(20,10);(10,0);(10,0)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(10,0);(10,0);(0,10);(0,10)"
%	 stroke-width= "0.75"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(12.5,27.5)"
%	 text-frame= "noframe"
%	 stroke-width= "0.75"
%	 text-hor-align= "left"
%	 >
%$\inputt$
%</text>
%<multicurve fill-style= "none"
%	 points= "(0,10);(0,10);(20,10);(20,10)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(10,30);(10,30);(10,10);(10,10)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(70,15);(70,15);(60,5);(60,5)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(60,5);(60,5);(50,15);(50,15)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(70,15);(70,15);(60,25);(60,25)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(60,25);(60,25);(50,15);(50,15)"
%	 stroke-width= "0.75"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(60,15)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\eex$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(110,24.38)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\ahh$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(10.62,5.62)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\bee$
%</text>
%</jpic>
%%End JPIC-XML
%PSTricks content-type (pstricks.sty package needed)
%Add \usepackage{pstricks} in the preamble of your LaTeX file
%You can rescale the whole picture (to 80% for instance) by using the command \def\JPicScale{0.8}
\ifx\JPicScale\undefined\def\JPicScale{1}\fi
\psset{unit=\JPicScale mm}
\psset{linewidth=0.3,dotsep=1,hatchwidth=0.3,hatchsep=1.5,shadowsize=1,dimen=middle}
\psset{dotsize=0.7 2.5,dotscale=1 1,fillcolor=black}
\psset{arrowsize=1 2,arrowlength=1,arrowinset=0.25,tbarsize=0.7 5,bracketlength=0.15,rbracketlength=0.15}
\begin{pspicture}(0,0)(120,30)
\psline[linewidth=0.75](110,30)(100,20)
\psline[linewidth=0.75](120,20)(110,30)
\rput[r](107.5,2.5){$\inputt$}
\psline[linewidth=0.75](100,20)(120,20)
\psline[linewidth=0.75](110,20)(110,0)
\psline[linewidth=0.75](20,10)(10,0)
\psline[linewidth=0.75](10,0)(0,10)
\rput[l](12.5,27.5){$\inputt$}
\psline[linewidth=0.75](0,10)(20,10)
\psline[linewidth=0.75](10,30)(10,10)
\psline[linewidth=0.75](70,15)(60,5)
\psline[linewidth=0.75](60,5)(50,15)
\psline[linewidth=0.75](70,15)(60,25)
\psline[linewidth=0.75](60,25)(50,15)
\rput(60,15){$\eex$}
\rput(110,24.38){$\ahh$}
\rput(10.62,5.62){$\bee$}
\end{pspicture}


==> PIC/virus-1.tex <==
%%Created by jPicEdt 1.4.1_03: mixed JPIC-XML/LaTeX format
%%Fri Sep 02 17:02:36 GMT-10:00 2022
%%Begin JPIC-XML
%<?xml version="1.0" standalone="yes"?>
%<jpic x-min="0" x-max="229.38" y-min="0" y-max="78.75" auto-bounding="true">
%<multicurve fill-style= "none"
%	 points= "(0,60);(0,60);(40,60);(40,60)"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(0,30);(0,30);(0,10);(0,10)"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(40,40);(40,40);(40,60);(40,60)"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(30,70);(30,70);(30,60);(30,60)"
%	 stroke-width= "0.35"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(28.75,5)"
%	 text-frame= "noframe"
%	 stroke-width= "0.35"
%	 text-hor-align= "right"
%	 >
%$\inputt$
%</text>
%<multicurve fill-style= "none"
%	 points= "(20,40);(20,40);(40,40);(40,40)"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(30,40);(30,40);(30,5);(30,5)"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(0,10);(0,10);(20,10);(20,10)"
%	 stroke-width= "0.35"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(25,50)"
%	 text-frame= "noframe"
%	 stroke-width= "0.35"
%	 text-hor-align= "center-h"
%	 >
%\universal
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(5,15)"
%	 text-frame= "noframe"
%	 stroke-width= "0.35"
%	 text-hor-align= "center-h"
%	 >
%\program
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(50,56.25)"
%	 text-frame= "noframe"
%	 stroke-width= "0.35"
%	 text-hor-align= "center-h"
%	 >
%\EQLS
%</text>
%<multicurve fill-style= "none"
%	 points= "(10,50);(10,50);(10,20);(10,20)"
%	 stroke-width= "0.7"
%	 />
%<multicurve fill-style= "none"
%	 points= "(0,60);(0,60);(20,40);(20,40)"
%	 stroke-width= "0.35"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(93.75,5)"
%	 text-frame= "noframe"
%	 stroke-width= "0.35"
%	 text-hor-align= "right"
%	 >
%$\inputt$
%</text>
%<multicurve fill-style= "none"
%	 points= "(95,45);(95,45);(95,5);(95,5)"
%	 stroke-width= "0.35"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(55,20)"
%	 text-frame= "noframe"
%	 stroke-width= "0.35"
%	 text-hor-align= "center-h"
%	 >
%\program
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(73.75,43.75)"
%	 text-frame= "noframe"
%	 stroke-width= "0.35"
%	 text-hor-align= "center-h"
%	 >
%$\gee$
%</text>
%<multicurve fill-style= "none"
%	 points= "(145,33.12);(145,33.12);(145,8.12);(145,8.12)"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(145,8.12);(145,8.12);(170,8.12);(170,8.12)"
%	 stroke-width= "0.35"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(152.5,15)"
%	 text-frame= "noframe"
%	 stroke-width= "0.35"
%	 text-hor-align= "center-h"
%	 >
%\program
%</text>
%<multicurve fill-style= "none"
%	 points= "(145,33.12);(145,33.12);(170,8.12);(170,8.12)"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(157.5,78.75);(157.5,78.75);(157.5,20.62);(157.5,20.62)"
%	 stroke-width= "0.35"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(140.62,56.87)"
%	 text-frame= "noframe"
%	 stroke-width= "0.35"
%	 text-hor-align= "center-h"
%	 >
%\EQLS
%</text>
%<ellipse p3= "(82.58,47.42)"
%	 fill-style= "solid"
%	 p2= "(82.58,52.58)"
%	 fill-color= "#330033"
%	 p1= "(77.42,52.58)"
%	 closure= "open"
%	 angle-end= "0"
%	 stroke-width= "0.35"
%	 angle-start= "0"
%	 />
%<multicurve fill-style= "none"
%	 points= "(10,70);(10,70);(10,60);(10,60)"
%	 stroke-width= "0.7"
%	 />
%<multicurve fill-style= "none"
%	 points= "(20,70);(20,70);(20,60);(20,60)"
%	 stroke-width= "0.7"
%	 />
%<multicurve fill-style= "none"
%	 points= "(75,70);(75,70);(75,55);(75,55)"
%	 stroke-width= "0.7"
%	 />
%<multicurve fill-style= "none"
%	 points= "(90,55);(90,55);(100,55);(100,55)"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(90,45);(90,45);(100,45);(100,45)"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(90,55);(90,55);(90,45);(90,45)"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(100,55.01);(100,55.01);(100,45);(100,45)"
%	 stroke-width= "0.35"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(95,50)"
%	 text-frame= "noframe"
%	 stroke-width= "0.35"
%	 text-hor-align= "center-h"
%	 >
%\eff
%</text>
%<multicurve fill-style= "none"
%	 points= "(95,70);(95,70);(95,55);(95,55)"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(75,55);(75,55);(80,50);(80,50)"
%	 stroke-width= "0.7"
%	 />
%<multicurve fill-style= "none"
%	 points= "(85,70);(85,70);(85,55);(85,55)"
%	 stroke-width= "0.7"
%	 />
%<multicurve fill-style= "none"
%	 points= "(85,55);(85,55);(80,50);(80,50)"
%	 stroke-width= "0.7"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(96.25,70)"
%	 text-frame= "noframe"
%	 stroke-width= "0.35"
%	 text-hor-align= "left"
%	 >
%$\outputt$
%</text>
%<multicurve fill-style= "none"
%	 points= "(175,32.5);(175,32.5);(175,7.49);(175,7.49)"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(175,7.49);(175,7.49);(200,7.49);(200,7.49)"
%	 stroke-width= "0.35"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(182.5,14.37)"
%	 text-frame= "noframe"
%	 stroke-width= "0.35"
%	 text-hor-align= "center-h"
%	 >
%\program
%</text>
%<multicurve fill-style= "none"
%	 points= "(175,32.5);(175,32.5);(200,7.49);(200,7.49)"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(187.5,78.13);(187.5,78.13);(187.5,20);(187.5,20)"
%	 stroke-width= "0.35"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(213.75,0)"
%	 text-frame= "noframe"
%	 stroke-width= "0.35"
%	 text-hor-align= "right"
%	 >
%$\inputt$
%</text>
%<multicurve fill-style= "none"
%	 points= "(215.62,48.13);(215.62,48.13);(215.62,0.63);(215.62,0.63)"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(204.38,63.13);(204.38,63.13);(229.38,63.13);(229.38,63.13)"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(204.38,48.13);(204.38,48.13);(229.38,48.13);(229.38,48.13)"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(204.38,63.13);(204.38,63.13);(204.38,48.13);(204.38,48.13)"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(229.38,63.13);(229.38,63.13);(229.38,48.12);(229.38,48.12)"
%	 stroke-width= "0.35"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(216.25,55.63)"
%	 text-frame= "noframe"
%	 stroke-width= "0.35"
%	 text-hor-align= "center-h"
%	 >
%\eff
%</text>
%<multicurve fill-style= "none"
%	 points= "(215.62,78.13);(215.62,78.13);(215.62,63.13);(215.62,63.13)"
%	 stroke-width= "0.35"
%	 />
%<ellipse p3= "(160.08,17.42)"
%	 fill-style= "solid"
%	 p2= "(160.08,22.58)"
%	 fill-color= "#330033"
%	 p1= "(154.92,22.58)"
%	 closure= "open"
%	 angle-end= "0"
%	 stroke-width= "0.35"
%	 angle-start= "0"
%	 />
%<ellipse p3= "(190.08,17.42)"
%	 fill-style= "solid"
%	 p2= "(190.08,22.58)"
%	 fill-color= "#330033"
%	 p1= "(184.92,22.58)"
%	 closure= "open"
%	 angle-end= "0"
%	 stroke-width= "0.35"
%	 angle-start= "0"
%	 />
%<ellipse p3= "(12.58,17.42)"
%	 fill-style= "solid"
%	 p2= "(12.58,22.58)"
%	 fill-color= "#330033"
%	 p1= "(7.42,22.58)"
%	 closure= "open"
%	 angle-end= "0"
%	 stroke-width= "0.35"
%	 angle-start= "0"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(218.75,76.25)"
%	 text-frame= "noframe"
%	 stroke-width= "0.35"
%	 text-hor-align= "left"
%	 >
%$\outputt$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(32.5,77.5)"
%	 text-frame= "noframe"
%	 stroke-width= "0.35"
%	 text-hor-align= "left"
%	 >
%$\outputt$
%</text>
%<multicurve fill-style= "none"
%	 points= "(0,30);(0,30);(20,10);(20,10)"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(70,30);(70,30);(70,10);(70,10)"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(70,10);(70,10);(90,10);(90,10)"
%	 stroke-width= "0.35"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(75,15)"
%	 text-frame= "noframe"
%	 stroke-width= "0.35"
%	 text-hor-align= "center-h"
%	 >
%\program
%</text>
%<multicurve fill-style= "none"
%	 points= "(80,50);(80,50);(80,20);(80,20)"
%	 stroke-width= "0.7"
%	 />
%<ellipse p3= "(82.58,17.42)"
%	 fill-style= "solid"
%	 p2= "(82.58,22.58)"
%	 fill-color= "#330033"
%	 p1= "(77.42,22.58)"
%	 closure= "open"
%	 angle-end= "0"
%	 stroke-width= "0.35"
%	 angle-start= "0"
%	 />
%<multicurve fill-style= "none"
%	 points= "(70,30);(70,30);(90,10);(90,10)"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(70,60);(70,60);(103.75,60);(103.75,60)"
%	 stroke-width= "0.15"
%	 />
%<multicurve fill-style= "none"
%	 points= "(70,40);(70,40);(103.75,40);(103.75,40)"
%	 stroke-width= "0.15"
%	 />
%<multicurve fill-style= "none"
%	 points= "(70,60);(70,60);(70,40);(70,40)"
%	 stroke-width= "0.15"
%	 />
%<multicurve fill-style= "none"
%	 points= "(103.75,60);(103.75,60);(103.75,40);(103.75,40)"
%	 stroke-width= "0.15"
%	 />
%</jpic>
%%End JPIC-XML
%LaTeX-picture environment using emulated lines and arcs
%You can rescale the whole picture (to 80% for instance) by using the command \def\JPicScale{0.8}
\ifx\JPicScale\undefined\def\JPicScale{1}\fi
\unitlength \JPicScale mm
\begin{picture}(229.38,78.75)(0,0)
\linethickness{0.35mm}
\put(0,60){\line(1,0){40}}
\linethickness{0.35mm}
\put(0,10){\line(0,1){20}}
\linethickness{0.35mm}
\put(40,40){\line(0,1){20}}
\linethickness{0.35mm}
\put(30,60){\line(0,1){10}}
\put(28.75,5){\makebox(0,0)[cr]{$\inputt$}}

\linethickness{0.35mm}
\put(20,40){\line(1,0){20}}
\linethickness{0.35mm}
\put(30,5){\line(0,1){35}}
\linethickness{0.35mm}
\put(0,10){\line(1,0){20}}
\put(25,50){\makebox(0,0)[cc]{\universal}}

\put(5,15){\makebox(0,0)[cc]{\program}}

\put(50,56.25){\makebox(0,0)[cc]{\EQLS}}

\linethickness{0.7mm}
\put(10,20){\line(0,1){30}}
\linethickness{0.35mm}
\multiput(0,60)(0.12,-0.12){167}{\line(1,0){0.12}}
\put(93.75,5){\makebox(0,0)[cr]{$\inputt$}}

\linethickness{0.35mm}
\put(95,5){\line(0,1){40}}
\put(55,20){\makebox(0,0)[cc]{\program}}

\put(73.75,43.75){\makebox(0,0)[cc]{$\gee$}}

\linethickness{0.35mm}
\put(145,8.12){\line(0,1){25}}
\linethickness{0.35mm}
\put(145,8.12){\line(1,0){25}}
\put(152.5,15){\makebox(0,0)[cc]{\program}}

\linethickness{0.35mm}
\multiput(145,33.12)(0.12,-0.12){208}{\line(1,0){0.12}}
\linethickness{0.35mm}
\put(157.5,20.62){\line(0,1){58.13}}
\put(140.62,56.87){\makebox(0,0)[cc]{\EQLS}}

\linethickness{0.35mm}
\put(80,50){\circle*{5.16}}

\linethickness{0.7mm}
\put(10,60){\line(0,1){10}}
\linethickness{0.7mm}
\put(20,60){\line(0,1){10}}
\linethickness{0.7mm}
\put(75,55){\line(0,1){15}}
\linethickness{0.35mm}
\put(90,55){\line(1,0){10}}
\linethickness{0.35mm}
\put(90,45){\line(1,0){10}}
\linethickness{0.35mm}
\put(90,45){\line(0,1){10}}
\linethickness{0.35mm}
\put(100,45){\line(0,1){10.01}}
\put(95,50){\makebox(0,0)[cc]{\eff}}

\linethickness{0.35mm}
\put(95,55){\line(0,1){15}}
\linethickness{0.7mm}
\multiput(75,55)(0.12,-0.12){42}{\line(1,0){0.12}}
\linethickness{0.7mm}
\put(85,55){\line(0,1){15}}
\linethickness{0.7mm}
\multiput(80,50)(0.12,0.12){42}{\line(1,0){0.12}}
\put(96.25,70){\makebox(0,0)[cl]{$\outputt$}}

\linethickness{0.35mm}
\put(175,7.49){\line(0,1){25.01}}
\linethickness{0.35mm}
\put(175,7.49){\line(1,0){25}}
\put(182.5,14.37){\makebox(0,0)[cc]{\program}}

\linethickness{0.35mm}
\multiput(175,32.5)(0.12,-0.12){208}{\line(0,-1){0.12}}
\linethickness{0.35mm}
\put(187.5,20){\line(0,1){58.13}}
\put(213.75,0){\makebox(0,0)[cr]{$\inputt$}}

\linethickness{0.35mm}
\put(215.62,0.63){\line(0,1){47.5}}
\linethickness{0.35mm}
\put(204.38,63.13){\line(1,0){25}}
\linethickness{0.35mm}
\put(204.38,48.13){\line(1,0){25}}
\linethickness{0.35mm}
\put(204.38,48.13){\line(0,1){15}}
\linethickness{0.35mm}
\put(229.38,48.12){\line(0,1){15.01}}
\put(216.25,55.63){\makebox(0,0)[cc]{\eff}}

\linethickness{0.35mm}
\put(215.62,63.13){\line(0,1){15}}
\linethickness{0.35mm}
\put(157.5,20){\circle*{5.16}}

\linethickness{0.35mm}
\put(187.5,20){\circle*{5.16}}

\linethickness{0.35mm}
\put(10,20){\circle*{5.16}}

\put(218.75,76.25){\makebox(0,0)[cl]{$\outputt$}}

\put(32.5,77.5){\makebox(0,0)[cl]{$\outputt$}}

\linethickness{0.35mm}
\multiput(0,30)(0.12,-0.12){167}{\line(1,0){0.12}}
\linethickness{0.35mm}
\put(70,10){\line(0,1){20}}
\linethickness{0.35mm}
\put(70,10){\line(1,0){20}}
\put(75,15){\makebox(0,0)[cc]{\program}}

\linethickness{0.7mm}
\put(80,20){\line(0,1){30}}
\linethickness{0.35mm}
\put(80,20){\circle*{5.16}}

\linethickness{0.35mm}
\multiput(70,30)(0.12,-0.12){167}{\line(1,0){0.12}}
\linethickness{0.15mm}
\put(70,60){\line(1,0){33.75}}
\linethickness{0.15mm}
\put(70,40){\line(1,0){33.75}}
\linethickness{0.15mm}
\put(70,40){\line(0,1){20}}
\linethickness{0.15mm}
\put(103.75,40){\line(0,1){20}}
\end{picture}


==> PIC/virus-2.tex <==
%%Created by jPicEdt 1.4.1_03: mixed JPIC-XML/LaTeX format
%%Fri Sep 02 17:20:14 GMT-10:00 2022
%%Begin JPIC-XML
%<?xml version="1.0" standalone="yes"?>
%<jpic x-min="0" x-max="239.38" y-min="0" y-max="140" auto-bounding="true">
%<multicurve fill-style= "none"
%	 points= "(0,68.75);(0,68.75);(50,68.75);(50,68.75)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(0,31.87);(0,31.87);(0,6.87);(0,6.87)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(50,43.75);(50,43.75);(50,68.75);(50,68.75)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(40,78.75);(40,78.75);(40,68.75);(40,68.75)"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(37.5,0)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\inputt$
%</text>
%<multicurve fill-style= "none"
%	 points= "(25,43.75);(25,43.75);(50,43.75);(50,43.75)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(40,43.75);(40,43.75);(40,0.63);(40,0.63)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(0,6.87);(0,6.87);(25,6.87);(25,6.87)"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(31.25,56.25)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\universal
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(7.5,13.75)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\program
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(60,56.25)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\EQLS
%</text>
%<multicurve fill-style= "none"
%	 points= "(0,31.87);(0,31.87);(25,6.87);(25,6.87)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(12.5,56.25);(12.5,56.25);(12.5,20);(12.5,20)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(0,68.75);(0,68.75);(25,43.75);(25,43.75)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(70,71.25);(70,71.25);(140,71.25);(140,71.25)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(77.5,31.87);(77.5,31.87);(77.5,6.87);(77.5,6.87)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(140,41.25);(140,41.25);(140,71.25);(140,71.25)"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(117.5,0)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\inputt$
%</text>
%<multicurve fill-style= "none"
%	 points= "(70,41.25);(70,41.25);(140,41.25);(140,41.25)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(120,48.13);(120,48.13);(120,0.63);(120,0.63)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(77.5,6.87);(77.5,6.87);(102.5,6.87);(102.5,6.87)"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(85,13.75)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\program
%</text>
%<multicurve fill-style= "none"
%	 points= "(77.5,31.87);(77.5,31.87);(102.5,6.87);(102.5,6.87)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(90,52.5);(90,52.5);(90,20);(90,20)"
%	 stroke-width= "0.5"
%	 />
%<multicurve fill-style= "none"
%	 points= "(70,71.25);(70,71.25);(70,41.25);(70,41.25)"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(78.12,48.75)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\gee$
%</text>
%<multicurve fill-style= "none"
%	 points= "(155,33.12);(155,33.12);(155,8.12);(155,8.12)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(155,8.12);(155,8.12);(180,8.12);(180,8.12)"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(162.5,15)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\program
%</text>
%<multicurve fill-style= "none"
%	 points= "(155,33.12);(155,33.12);(180,8.12);(180,8.12)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(167.5,78.75);(167.5,78.75);(167.5,20.62);(167.5,20.62)"
%	 stroke-width= "0.75"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(150.62,56.87)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\EQLS
%</text>
%<multicurve fill-style= "none"
%	 points= "(5,78.75);(5,78.75);(5,68.75);(5,68.75)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(21.25,78.75);(21.25,78.75);(21.25,68.75);(21.25,68.75)"
%	 stroke-width= "0.75"
%	 />
%<multicurve fill-style= "none"
%	 points= "(78.75,77.5);(78.75,77.5);(78.75,63.75);(78.75,63.75)"
%	 stroke-width= "0.5"
%	 />
%<multicurve fill-style= "none"
%	 points= "(108.75,63.13);(108.75,63.13);(133.75,63.13);(133.75,63.13)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(108.75,48.13);(108.75,48.13);(133.75,48.13);(133.75,48.13)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(108.75,63.13);(108.75,63.13);(108.75,48.13);(108.75,48.13)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(133.75,63.13);(133.75,63.13);(133.75,48.12);(133.75,48.12)"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(120.62,55.63)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\eff
%</text>
%<multicurve fill-style= "none"
%	 points= "(120,78.13);(120,78.13);(120,63.13);(120,63.13)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(78.75,63.75);(78.75,63.75);(90,52.5);(90,52.5)"
%	 stroke-width= "0.5"
%	 />
%<multicurve fill-style= "none"
%	 points= "(101.25,78.75);(101.25,78.75);(101.25,63.75);(101.25,63.75)"
%	 stroke-width= "0.5"
%	 />
%<multicurve fill-style= "none"
%	 points= "(101.25,63.75);(101.25,63.75);(90,52.5);(90,52.5)"
%	 stroke-width= "0.5"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(122.5,77.5)"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\outputt$
%</text>
%<multicurve fill-style= "none"
%	 points= "(185,32.5);(185,32.5);(185,7.49);(185,7.49)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(185,7.49);(185,7.49);(210,7.49);(210,7.49)"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(192.5,14.37)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\program
%</text>
%<multicurve fill-style= "none"
%	 points= "(185,32.5);(185,32.5);(210,7.49);(210,7.49)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(197.5,78.13);(197.5,78.13);(197.5,20);(197.5,20)"
%	 stroke-width= "0.75"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(223.75,0)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\inputt$
%</text>
%<multicurve fill-style= "none"
%	 points= "(225.62,48.13);(225.62,48.13);(225.62,0.63);(225.62,0.63)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(214.38,63.13);(214.38,63.13);(239.38,63.13);(239.38,63.13)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(214.38,48.13);(214.38,48.13);(239.38,48.13);(239.38,48.13)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(214.38,63.13);(214.38,63.13);(214.38,48.13);(214.38,48.13)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(239.38,63.13);(239.38,63.13);(239.38,48.12);(239.38,48.12)"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(226.25,55.63)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\eff
%</text>
%<multicurve fill-style= "none"
%	 points= "(225.62,78.13);(225.62,78.13);(225.62,63.13);(225.62,63.13)"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(228.75,76.25)"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\outputt$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(42.5,77.5)"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\outputt$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(90,52.5)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\Dottt
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(90,20)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\Dottt
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(12.5,20)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\Dottt
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(167.5,20)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\Dottt
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(197.5,20)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\Dottt
%</text>
%<multicurve fill-style= "none"
%	 points= "(80,120);(80,120);(100,120);(100,120);(100,120);(120,140);
%	(120,140);(120,140);(120,120);(120,120);(120,120);(120,120);
%	(120,120);(120,120);(140,140);(140,140)"
%	 />
%</jpic>
%%End JPIC-XML
%LaTeX-picture environment using emulated lines and arcs
%You can rescale the whole picture (to 80% for instance) by using the command \def\JPicScale{0.8}
\ifx\JPicScale\undefined\def\JPicScale{1}\fi
\unitlength \JPicScale mm
\begin{picture}(239.38,140)(0,0)
\linethickness{0.3mm}
\put(0,68.75){\line(1,0){50}}
\linethickness{0.3mm}
\put(0,6.87){\line(0,1){25}}
\linethickness{0.3mm}
\put(50,43.75){\line(0,1){25}}
\linethickness{0.3mm}
\put(40,68.75){\line(0,1){10}}
\put(37.5,0){\makebox(0,0)[cr]{$\inputt$}}

\linethickness{0.3mm}
\put(25,43.75){\line(1,0){25}}
\linethickness{0.3mm}
\put(40,0.63){\line(0,1){43.12}}
\linethickness{0.3mm}
\put(0,6.87){\line(1,0){25}}
\put(31.25,56.25){\makebox(0,0)[cc]{\universal}}

\put(7.5,13.75){\makebox(0,0)[cc]{\program}}

\put(60,56.25){\makebox(0,0)[cc]{\EQLS}}

\linethickness{0.3mm}
\multiput(0,31.87)(0.12,-0.12){208}{\line(1,0){0.12}}
\linethickness{0.75mm}
\put(12.5,20){\line(0,1){36.25}}
\linethickness{0.3mm}
\multiput(0,68.75)(0.12,-0.12){208}{\line(1,0){0.12}}
\linethickness{0.3mm}
\put(70,71.25){\line(1,0){70}}
\linethickness{0.3mm}
\put(77.5,6.87){\line(0,1){25}}
\linethickness{0.3mm}
\put(140,41.25){\line(0,1){30}}
\put(117.5,0){\makebox(0,0)[cr]{$\inputt$}}

\linethickness{0.3mm}
\put(70,41.25){\line(1,0){70}}
\linethickness{0.3mm}
\put(120,0.63){\line(0,1){47.5}}
\linethickness{0.3mm}
\put(77.5,6.87){\line(1,0){25}}
\put(85,13.75){\makebox(0,0)[cc]{\program}}

\linethickness{0.3mm}
\multiput(77.5,31.87)(0.12,-0.12){208}{\line(1,0){0.12}}
\linethickness{0.5mm}
\put(90,20){\line(0,1){32.5}}
\linethickness{0.3mm}
\put(70,41.25){\line(0,1){30}}
\put(78.12,48.75){\makebox(0,0)[cc]{$\gee$}}

\linethickness{0.3mm}
\put(155,8.12){\line(0,1){25}}
\linethickness{0.3mm}
\put(155,8.12){\line(1,0){25}}
\put(162.5,15){\makebox(0,0)[cc]{\program}}

\linethickness{0.3mm}
\multiput(155,33.12)(0.12,-0.12){208}{\line(1,0){0.12}}
\linethickness{0.75mm}
\put(167.5,20.62){\line(0,1){58.13}}
\put(150.62,56.87){\makebox(0,0)[cc]{\EQLS}}

\linethickness{0.75mm}
\put(5,68.75){\line(0,1){10}}
\linethickness{0.75mm}
\put(21.25,68.75){\line(0,1){10}}
\linethickness{0.5mm}
\put(78.75,63.75){\line(0,1){13.75}}
\linethickness{0.3mm}
\put(108.75,63.13){\line(1,0){25}}
\linethickness{0.3mm}
\put(108.75,48.13){\line(1,0){25}}
\linethickness{0.3mm}
\put(108.75,48.13){\line(0,1){15}}
\linethickness{0.3mm}
\put(133.75,48.12){\line(0,1){15.01}}
\put(120.62,55.63){\makebox(0,0)[cc]{\eff}}

\linethickness{0.3mm}
\put(120,63.13){\line(0,1){15}}
\linethickness{0.5mm}
\multiput(78.75,63.75)(0.12,-0.12){94}{\line(1,0){0.12}}
\linethickness{0.5mm}
\put(101.25,63.75){\line(0,1){15}}
\linethickness{0.5mm}
\multiput(90,52.5)(0.12,0.12){94}{\line(1,0){0.12}}
\put(122.5,77.5){\makebox(0,0)[cl]{$\outputt$}}

\linethickness{0.3mm}
\put(185,7.49){\line(0,1){25.01}}
\linethickness{0.3mm}
\put(185,7.49){\line(1,0){25}}
\put(192.5,14.37){\makebox(0,0)[cc]{\program}}

\linethickness{0.3mm}
\multiput(185,32.5)(0.12,-0.12){208}{\line(0,-1){0.12}}
\linethickness{0.75mm}
\put(197.5,20){\line(0,1){58.13}}
\put(223.75,0){\makebox(0,0)[cr]{$\inputt$}}

\linethickness{0.3mm}
\put(225.62,0.63){\line(0,1){47.5}}
\linethickness{0.3mm}
\put(214.38,63.13){\line(1,0){25}}
\linethickness{0.3mm}
\put(214.38,48.13){\line(1,0){25}}
\linethickness{0.3mm}
\put(214.38,48.13){\line(0,1){15}}
\linethickness{0.3mm}
\put(239.38,48.12){\line(0,1){15.01}}
\put(226.25,55.63){\makebox(0,0)[cc]{\eff}}

\linethickness{0.3mm}
\put(225.62,63.13){\line(0,1){15}}
\put(228.75,76.25){\makebox(0,0)[cl]{$\outputt$}}

\put(42.5,77.5){\makebox(0,0)[cl]{$\outputt$}}

\put(90,52.5){\makebox(0,0)[cc]{\Dottt}}

\put(90,20){\makebox(0,0)[cc]{\Dottt}}

\put(12.5,20){\makebox(0,0)[cc]{\Dottt}}

\put(167.5,20){\makebox(0,0)[cc]{\Dottt}}

\put(197.5,20){\makebox(0,0)[cc]{\Dottt}}

\linethickness{0.3mm}
\put(80,120){\line(1,0){20}}
\multiput(100,120)(0.12,0.12){167}{\line(1,0){0.12}}
\put(120,120){\line(0,1){20}}
\qbezier(120,120)(120,120)(120,120)
\qbezier(120,120)(120,120)(120,120)
\multiput(120,120)(0.12,0.12){167}{\line(1,0){0.12}}
\end{picture}


==> PIC/zero.tex <==
%%Created by jPicEdt 1.4.1_03: mixed JPIC-XML/LaTeX format
%%Fri Dec 11 16:04:55 GMT-10:00 2020
%%Begin JPIC-XML
%<?xml version="1.0" standalone="yes"?>
%<jpic x-min="0" x-max="90" y-min="0" y-max="100" auto-bounding="true">
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(56.25,60)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\EQLS
%</text>
%<multicurve fill-style= "none"
%	 points= "(20,100);(20,100);(20,75);(20,75)"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(83.75,73.75)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\qee$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(14.38,67.5)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\iee$
%</text>
%<multicurve fill-style= "none"
%	 points= "(5,90);(5,90);(35,60);(35,60)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(5,60);(5,60);(35,60);(35,60)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(5,90);(5,90);(5,60);(5,60)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(70,80);(70,80);(90,80);(90,80)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(70,80);(70,80);(90,60);(90,60)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(90,80);(90,80);(90,60);(90,60)"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(22.5,100)"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\Aee$
%</text>
%<multicurve fill-style= "none"
%	 points= "(80,80);(80,80);(80,100);(80,100)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(10,38.75);(10,38.75);(10,60);(10,60)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(30,10);(30,10);(30,30);(30,30)"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(32.5,16.25)"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\Aee$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(7.5,53.75)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\Aee$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(82.5,100)"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\Aee$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(33.75,33.75)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\qee$
%</text>
%<multicurve fill-style= "none"
%	 points= "(20,40);(20,40);(40,40);(40,40)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(20,40);(20,40);(40,20);(40,20)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(40,40);(40,40);(40,20);(40,20)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(30,40);(30,40);(30,60);(30,60)"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(32.5,53.75)"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\Aee$
%</text>
%<multicurve fill-style= "none"
%	 points= "(0,28.75);(0,28.75);(20,28.75);(20,28.75)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(0,48.75);(0,48.75);(20,28.75);(20,28.75)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(0,48.75);(0,48.75);(0,28.75);(0,28.75)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(80,10);(80,10);(80,70);(80,70)"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(82.5,40)"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\Aee$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(6.25,33.75)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\thhh$
%</text>
%<multicurve fill-style= "none"
%	 points= "(20,0);(20,0);(40,0);(40,0)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(20,20);(20,20);(40,0);(40,0)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(20,20);(20,20);(20,0);(20,0)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(70,0);(70,0);(90,0);(90,0)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(70,20);(70,20);(90,0);(90,0)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(70,20);(70,20);(70,0);(70,0)"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(26.25,5)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\blh$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(76.25,5)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\blh$
%</text>
%</jpic>
%%End JPIC-XML
%LaTeX-picture environment using emulated lines and arcs
%You can rescale the whole picture (to 80% for instance) by using the command \def\JPicScale{0.8}
\ifx\JPicScale\undefined\def\JPicScale{1}\fi
\unitlength \JPicScale mm
\begin{picture}(90,100)(0,0)
\put(56.25,60){\makebox(0,0)[cc]{\EQLS}}

\linethickness{0.3mm}
\put(20,75){\line(0,1){25}}
\put(83.75,73.75){\makebox(0,0)[cc]{$\qee$}}

\put(14.38,67.5){\makebox(0,0)[cc]{$\iee$}}

\linethickness{0.3mm}
\multiput(5,90)(0.12,-0.12){250}{\line(1,0){0.12}}
\linethickness{0.3mm}
\put(5,60){\line(1,0){30}}
\linethickness{0.3mm}
\put(5,60){\line(0,1){30}}
\linethickness{0.3mm}
\put(70,80){\line(1,0){20}}
\linethickness{0.3mm}
\multiput(70,80)(0.12,-0.12){167}{\line(1,0){0.12}}
\linethickness{0.3mm}
\put(90,60){\line(0,1){20}}
\put(22.5,100){\makebox(0,0)[cl]{$\Aee$}}

\linethickness{0.3mm}
\put(80,80){\line(0,1){20}}
\linethickness{0.3mm}
\put(10,38.75){\line(0,1){21.25}}
\linethickness{0.3mm}
\put(30,10){\line(0,1){20}}
\put(32.5,16.25){\makebox(0,0)[cl]{$\Aee$}}

\put(7.5,53.75){\makebox(0,0)[cr]{$\Aee$}}

\put(82.5,100){\makebox(0,0)[cl]{$\Aee$}}

\put(33.75,33.75){\makebox(0,0)[cc]{$\qee$}}

\linethickness{0.3mm}
\put(20,40){\line(1,0){20}}
\linethickness{0.3mm}
\multiput(20,40)(0.12,-0.12){167}{\line(1,0){0.12}}
\linethickness{0.3mm}
\put(40,20){\line(0,1){20}}
\linethickness{0.3mm}
\put(30,40){\line(0,1){20}}
\put(32.5,53.75){\makebox(0,0)[cl]{$\Aee$}}

\linethickness{0.3mm}
\put(0,28.75){\line(1,0){20}}
\linethickness{0.3mm}
\multiput(0,48.75)(0.12,-0.12){167}{\line(1,0){0.12}}
\linethickness{0.3mm}
\put(0,28.75){\line(0,1){20}}
\linethickness{0.3mm}
\put(80,10){\line(0,1){60}}
\put(82.5,40){\makebox(0,0)[cl]{$\Aee$}}

\put(6.25,33.75){\makebox(0,0)[cc]{$\thhh$}}

\linethickness{0.3mm}
\put(20,0){\line(1,0){20}}
\linethickness{0.3mm}
\multiput(20,20)(0.12,-0.12){167}{\line(1,0){0.12}}
\linethickness{0.3mm}
\put(20,0){\line(0,1){20}}
\linethickness{0.3mm}
\put(70,0){\line(1,0){20}}
\linethickness{0.3mm}
\multiput(70,20)(0.12,-0.12){167}{\line(1,0){0.12}}
\linethickness{0.3mm}
\put(70,0){\line(0,1){20}}
\put(26.25,5){\makebox(0,0)[cc]{$\blh$}}

\put(76.25,5){\makebox(0,0)[cc]{$\blh$}}

\end{picture}

